Can AI Design a Better nnU-Net? A Hypothesis-Driven Architecture Discovery Loop from Failures to Design Rules

Neural architecture search and LLM-driven evolution often reduce evaluation to a scalar fitness score, discarding failures that could explain why designs succeed or fail. We present a hypothesis-driven architecture discovery loop in which LLM agents diagnose structured error patterns, formulate falsifiable hypotheses, test counterfactual controls under a frozen nnU-Net pipeline, and distill validated mechanisms into executable trigger-to-action rules. Across eight search waves, the loop identifies two principles for 3D medical image segmentation. First, reallocating computation from high-resolution decoders to the mid-encoder preserves thin-anatomy boundaries while reducing cost. Second, support-confined region contrast addresses errors between nested anatomical compartments, with anatomy-dependent triggers selecting when the rule applies. These principles produce LeanNeXt (0.78 MACs and 0.92 training-step time relative to nnU-Net; +1.63 Dice points on four-fold KiTS23 cross-validation) and trigger-routed LeanNeXt+. The latter improves all 15 evaluated CT/MRI settings over nnU-Net and exceeds the 3.3 larger ResEnc-M on 12 of 15 benchmarks at 0.30 its parameter count. Relative to random sampling, one-shot LLM generation, and score-selected agent search, the loop shows how failure analysis can yield reusable design rules across modalities.

==> an_extra_abcost.tex <==
% AUTO-GENERATED by paper_v1/ab_costs.py -- do not edit by hand
\makeatletter
\expandafter\gdef\csname R@v1.abc.1.gmac\endcsname{0.54}
\expandafter\gdef\csname R@v1.abc.1.params\endcsname{0.66}
\expandafter\gdef\csname R@v1.abc.1.step\endcsname{0.75}
\expandafter\gdef\csname R@v1.abc.10.gmac\endcsname{0.84}
\expandafter\gdef\csname R@v1.abc.10.params\endcsname{1.05}
\expandafter\gdef\csname R@v1.abc.10.step\endcsname{1.10}
\expandafter\gdef\csname R@v1.abc.11.gmac\endcsname{0.64}
\expandafter\gdef\csname R@v1.abc.11.params\endcsname{0.67}
\expandafter\gdef\csname R@v1.abc.11.step\endcsname{1.01}
\expandafter\gdef\csname R@v1.abc.2.gmac\endcsname{0.54}
\expandafter\gdef\csname R@v1.abc.2.params\endcsname{0.68}
\expandafter\gdef\csname R@v1.abc.2.step\endcsname{0.77}
\expandafter\gdef\csname R@v1.abc.3.gmac\endcsname{0.77}
\expandafter\gdef\csname R@v1.abc.3.params\endcsname{0.84}
\expandafter\gdef\csname R@v1.abc.3.step\endcsname{0.86}
\expandafter\gdef\csname R@v1.abc.4.gmac\endcsname{0.77}
\expandafter\gdef\csname R@v1.abc.4.params\endcsname{0.84}
\expandafter\gdef\csname R@v1.abc.4.step\endcsname{0.96}
\expandafter\gdef\csname R@v1.abc.5.gmac\endcsname{0.54}
\expandafter\gdef\csname R@v1.abc.5.params\endcsname{0.63}
\expandafter\gdef\csname R@v1.abc.5.step\endcsname{0.77}
\expandafter\gdef\csname R@v1.abc.6.gmac\endcsname{0.54}
\expandafter\gdef\csname R@v1.abc.6.params\endcsname{0.68}
\expandafter\gdef\csname R@v1.abc.6.step\endcsname{0.79}
\expandafter\gdef\csname R@v1.abc.7.gmac\endcsname{0.54}
\expandafter\gdef\csname R@v1.abc.7.params\endcsname{0.49}
\expandafter\gdef\csname R@v1.abc.7.step\endcsname{0.96}
\expandafter\gdef\csname R@v1.abc.8.gmac\endcsname{0.56}
\expandafter\gdef\csname R@v1.abc.8.params\endcsname{0.54}
\expandafter\gdef\csname R@v1.abc.8.step\endcsname{0.68}
\expandafter\gdef\csname R@v1.abc.9.gmac\endcsname{0.30}
\expandafter\gdef\csname R@v1.abc.9.params\endcsname{0.38}
\expandafter\gdef\csname R@v1.abc.9.step\endcsname{0.73}
\makeatother


==> an_extra_counts.tex <==
% AUTO-GENERATED by paper_v1/dump_module.py from scripts/an_counts.py -- do not edit by hand
\makeatletter
\expandafter\gdef\csname R@an.counts.built\endcsname{51}
\expandafter\gdef\csname R@an.counts.built.def\endcsname{design source files built for waves 1 to 8, one per candidate file}
\expandafter\gdef\csname R@an.counts.built.outside\endcsname{9}
\expandafter\gdef\csname R@an.counts.built.outside.def\endcsname{built designs without a row in the verdict table; built minus registered}
\expandafter\gdef\csname R@an.counts.designs\endcsname{28}
\expandafter\gdef\csname R@an.counts.designs.agent\endcsname{25}
\expandafter\gdef\csname R@an.counts.designs.agent.def\endcsname{designs that are agent-designed arms; a subset of designs}
\expandafter\gdef\csname R@an.counts.designs.def\endcsname{trained arms whose discovery screen ran as a design of the search loop; a subset of trained (the other 10 trained arms are controls, reference designs and attribution arms that judge them)}
\expandafter\gdef\csname R@an.counts.gpudays.alloc\endcsname{140}
\expandafter\gdef\csname R@an.counts.gpudays.alloc.def\endcsname{GPU-days of those runs as allocated (queue duration times the 2 GPUs a run holds)}
\expandafter\gdef\csname R@an.counts.gpudays.eff\endcsname{49}
\expandafter\gdef\csname R@an.counts.gpudays.eff.def\endcsname{GPU-days used as a percentage of those allocated}
\expandafter\gdef\csname R@an.counts.gpudays.used\endcsname{68}
\expandafter\gdef\csname R@an.counts.gpudays.used.def\endcsname{GPU-days of those runs on the one device the network trains on (training seconds); 49 percent of the allocated}
\expandafter\gdef\csname R@an.counts.gpus\endcsname{2}
\expandafter\gdef\csname R@an.counts.gpus.def\endcsname{the GPUs one run of the search holds in the queue}
\expandafter\gdef\csname R@an.counts.hierarchy\endcsname{the loop proposed 111 ideas and built 51 designs; 42 of the built designs are rows of the verdict table (the lineage), 38 of those were trained at full budget, 28 as designs of the search and 10 as controls, reference designs and attribution arms that judge them; 25 of the trained arms were replicated on fresh seeds; the 28 designs took 138 full-budget runs, 140 GPU-days as allocated and 68 on the training device}
\expandafter\gdef\csname R@an.counts.ideas\endcsname{111}
\expandafter\gdef\csname R@an.counts.ideas.def\endcsname{ideas named by an ideator agent or a wave brief (the ledger of waves 1 to 4 and the ideator documents of waves 5 to 8); not a superset of the rows below, since controls are built without an idea (44 ideas were funded as a design)}
\expandafter\gdef\csname R@an.counts.ideas.funded\endcsname{44}
\expandafter\gdef\csname R@an.counts.ideas.funded.def\endcsname{ideas funded as a design of the loop; a subset of ideas}
\expandafter\gdef\csname R@an.counts.judges\endcsname{10}
\expandafter\gdef\csname R@an.counts.judges.def\endcsname{trained arms that are not designs; trained minus designs}
\expandafter\gdef\csname R@an.counts.registered\endcsname{42}
\expandafter\gdef\csname R@an.counts.registered.def\endcsname{built designs with a row in the verdict table, the nodes of the lineage; a subset of built (the 9 built designs outside the table were profiled and never run as arms)}
\expandafter\gdef\csname R@an.counts.replicated\endcsname{25}
\expandafter\gdef\csname R@an.counts.replicated.def\endcsname{trained arms with a finished fresh-seed pair (seeds 1 and 2) on some dataset, controls included; a subset of trained (21 of them are designs)}
\expandafter\gdef\csname R@an.counts.replicated.designs\endcsname{21}
\expandafter\gdef\csname R@an.counts.replicated.designs.def\endcsname{replicated arms that are designs; a subset of replicated and of designs}
\expandafter\gdef\csname R@an.counts.reviewed\endcsname{38}
\expandafter\gdef\csname R@an.counts.reviewed.def\endcsname{ideas of the waves with a per-idea review record that carry a recorded verdict; a subset of ideas}
\expandafter\gdef\csname R@an.counts.runs\endcsname{138}
\expandafter\gdef\csname R@an.counts.runs.def\endcsname{finished full-budget runs of the designs (53 discovery screens, 11 ACDC guard runs, 74 fresh-seed replications); controls, baselines, cross-validation and held-out runs are not counted}
\expandafter\gdef\csname R@an.counts.runs.fresh\endcsname{74}
\expandafter\gdef\csname R@an.counts.runs.fresh.def\endcsname{finished fresh-seed replication runs of the designs; a subset of runs}
\expandafter\gdef\csname R@an.counts.runs.guard\endcsname{11}
\expandafter\gdef\csname R@an.counts.runs.guard.def\endcsname{finished ACDC guard runs of the designs; a subset of runs}
\expandafter\gdef\csname R@an.counts.runs.screen\endcsname{53}
\expandafter\gdef\csname R@an.counts.runs.screen.def\endcsname{finished discovery-screen runs of the designs; a subset of runs}
\expandafter\gdef\csname R@an.counts.sentence.funnel\endcsname{over the feedback waves the agents proposed 111 ideas, built 51 designs, registered 42 of them, trained 38 at full budget and replicated 25 on fresh seeds}
\expandafter\gdef\csname R@an.counts.sentence.search\endcsname{the search trained 28 designs at full budget in 138 runs, about 68 GPU-days on the device the network trains on (140 GPU-days as allocated, each run holding 2 GPUs)}
\expandafter\gdef\csname R@an.counts.trained\endcsname{38}
\expandafter\gdef\csname R@an.counts.trained.def\endcsname{registered arms trained at full budget (1000 epochs) at fold 0 with a Dice on a co-primary; a subset of registered (4 registered arms were not trained)}
\expandafter\gdef\csname R@an.counts.untrained\endcsname{4}
\expandafter\gdef\csname R@an.counts.untrained.def\endcsname{registered arms without a full-budget result; registered minus trained}
\makeatother


==> an_extra_cv.tex <==
% AUTO-GENERATED by paper_v1/dump_module.py from scripts/an_cv.py -- do not edit by hand
\makeatletter
\expandafter\gdef\csname R@an.cv.B\endcsname{2000}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.clause\endcsname{LeanDec minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.05}\,pp, 95\,\% interval \ensuremath{-0.19} to \ensuremath{+0.08}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.est\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.hi\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.lo\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.D2.f1\endcsname{91.51}
\expandafter\gdef\csname R@an.cv.acdc.D2.f2\endcsname{91.71}
\expandafter\gdef\csname R@an.cv.acdc.D2.f3\endcsname{91.66}
\expandafter\gdef\csname R@an.cv.acdc.D2.f4\endcsname{90.41}
\expandafter\gdef\csname R@an.cv.acdc.D2.max14\endcsname{91.71}
\expandafter\gdef\csname R@an.cv.acdc.D2.min14\endcsname{90.41}
\expandafter\gdef\csname R@an.cv.acdc.D2.params\endcsname{25.28}
\expandafter\gdef\csname R@an.cv.acdc.D2.params1\endcsname{25.3}
\expandafter\gdef\csname R@an.cv.acdc.D2.span14\endcsname{1.30}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.clause\endcsname{LeanDec minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.02}\,pp, 95\,\% interval \ensuremath{-0.11} to \ensuremath{+0.18}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.est\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.hi\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.lo\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.ctloffset\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.dcv\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.f1\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.f2\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.f3\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.f4\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.hi\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.lo\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.loo.max\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.loo.min\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.loo.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.loo.word\endcsname{changes sign when a single fold is dropped (three of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.share.word\endcsname{fold 2 alone carries 242\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.share_max\endcsname{242}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.span14\endcsname{0.37}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.split\endcsname{LeanDec minus the default is \ensuremath{-0.05}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.08}\,pp, so the margin over the function-identical control is \ensuremath{+0.02}\,pp}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.vsdefault\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.word\endcsname{improves on it on average (2 of 4 folds)}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.D2base.dcv\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.acdc.D2base.f1\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.acdc.D2base.f2\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.D2base.f3\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.acdc.D2base.f4\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.D2base.hi\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.acdc.D2base.lo\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.acdc.D2base.loo.max\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cv.acdc.D2base.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.D2base.loo.min\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.acdc.D2base.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.D2base.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.D2base.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.D2base.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.D2base.share.word\endcsname{fold 3 alone carries 69\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.D2base.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.D2base.share_max\endcsname{69}
\expandafter\gdef\csname R@an.cv.acdc.D2base.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.D2base.span14\endcsname{0.20}
\expandafter\gdef\csname R@an.cv.acdc.D2base.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.clause\endcsname{ResEnc-M minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.37}\,pp, 95\,\% interval \ensuremath{+0.21} to \ensuremath{+0.55}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.est\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.hi\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.lo\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L1.f0\endcsname{92.25}
\expandafter\gdef\csname R@an.cv.acdc.L1.f1\endcsname{91.87}
\expandafter\gdef\csname R@an.cv.acdc.L1.f2\endcsname{92.03}
\expandafter\gdef\csname R@an.cv.acdc.L1.f3\endcsname{92.21}
\expandafter\gdef\csname R@an.cv.acdc.L1.f4\endcsname{90.90}
\expandafter\gdef\csname R@an.cv.acdc.L1.max14\endcsname{92.21}
\expandafter\gdef\csname R@an.cv.acdc.L1.mean14\endcsname{91.75}
\expandafter\gdef\csname R@an.cv.acdc.L1.mean5\endcsname{91.85}
\expandafter\gdef\csname R@an.cv.acdc.L1.min14\endcsname{90.90}
\expandafter\gdef\csname R@an.cv.acdc.L1.params\endcsname{101.53}
\expandafter\gdef\csname R@an.cv.acdc.L1.params1\endcsname{101.5}
\expandafter\gdef\csname R@an.cv.acdc.L1.span14\endcsname{1.32}
\expandafter\gdef\csname R@an.cv.acdc.L1.src0\endcsname{fresh s1-2}
\expandafter\gdef\csname R@an.cv.acdc.L1.src0long\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.cv.acdc.L1.src0mark\endcsname{b}
\expandafter\gdef\csname R@an.cv.acdc.L1.src0n\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.dcv\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.f1\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.f2\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.f3\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.f4\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.hi\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.lo\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.loo.max\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.loo.min\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.loo.minfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.share.word\endcsname{fold 3 alone carries 40\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.share_max\endcsname{40}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.span14\endcsname{0.20}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.boot.casewidth\endcsname{0.30}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.boot.foldwidth\endcsname{0.55}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.boot.hi\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.boot.lo\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.boot.mean\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.boot.n\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.11} to \ensuremath{+0.19}\,pp over the 160 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.dcv\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.f1\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.f2\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.f3\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.f4\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.hi\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.lo\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.loo.max\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.loo.min\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.loo.minfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.loo.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.loo.word\endcsname{changes sign when a single fold is dropped (three of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.share.word\endcsname{fold 3 alone carries 165\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.share_max\endcsname{165}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.span14\endcsname{0.39}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.word\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.clause\endcsname{ResEnc-M minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.45}\,pp, 95\,\% interval \ensuremath{+0.26} to \ensuremath{+0.66}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.est\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.hi\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.lo\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.ctloffset\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.dcv\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.f1\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.f2\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.f3\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.f4\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.hi\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.lo\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.loo.max\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.loo.min\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.share.word\endcsname{fold 2 alone carries 31\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.share_max\endcsname{31}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.span14\endcsname{0.16}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.split\endcsname{ResEnc-M minus the default is \ensuremath{+0.37}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.08}\,pp, so the margin over the function-identical control is \ensuremath{+0.45}\,pp}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.vsdefault\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.word\endcsname{improves on the control in every fold}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.clause\endcsname{ResEnc-matched minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.19}\,pp, 95\,\% interval \ensuremath{+0.04} to \ensuremath{+0.37}\,pp, which lies inside $\pm$0.50\,pp and above zero}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.est\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.hi\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.lo\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L1b.f1\endcsname{91.76}
\expandafter\gdef\csname R@an.cv.acdc.L1b.f2\endcsname{91.94}
\expandafter\gdef\csname R@an.cv.acdc.L1b.f3\endcsname{91.93}
\expandafter\gdef\csname R@an.cv.acdc.L1b.f4\endcsname{90.67}
\expandafter\gdef\csname R@an.cv.acdc.L1b.mean14\endcsname{91.57}
\expandafter\gdef\csname R@an.cv.acdc.L1b.params\endcsname{101.63}
\expandafter\gdef\csname R@an.cv.acdc.L1b.params1\endcsname{101.6}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.dcv\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.f1\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.f2\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.f3\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.f4\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.hi\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.lo\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.loo.max\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.loo.min\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.loo.minfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.share.word\endcsname{fold 2 alone carries 42\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.share_max\endcsname{42}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.span14\endcsname{0.19}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.L1base.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.acdc.L1base.boot.casewidth\endcsname{0.34}
\expandafter\gdef\csname R@an.cv.acdc.L1base.boot.foldwidth\endcsname{0.21}
\expandafter\gdef\csname R@an.cv.acdc.L1base.boot.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.boot.lo\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.boot.mean\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.boot.n\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L1base.boot.vsfold\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.acdc.L1base.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.20} to \ensuremath{+0.54}\,pp over the 160 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.acdc.L1base.d5\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.d5alt\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.dcv\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f0\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f0alt\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f0band\endcsname{0.16}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f0band.note\endcsname{two null SDs of this fold-0 difference, each the frozen default pool's training-seed SD of 0.099\,pp times $\sqrt{1/2 + 1/6}$ for the mean of two runs against the mean of the six-run pool: a locating band, not a test}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f0bandword\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f0gap\endcsname{0.24}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f0rev\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f0se\endcsname{0.081}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f1\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f2\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f3\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f4\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.hi\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.lo\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.loo.max\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L1base.loo.min\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.L1base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L1base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.L1base.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L1base.share.word\endcsname{fold 4 alone carries 30\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.L1base.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.L1base.share_max\endcsname{30}
\expandafter\gdef\csname R@an.cv.acdc.L1base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.L1base.span14\endcsname{0.16}
\expandafter\gdef\csname R@an.cv.acdc.L1base.src0\endcsname{fresh s1-2 for ResEnc-M and frozen pool for default}
\expandafter\gdef\csname R@an.cv.acdc.L1base.src0mark\endcsname{b/a}
\expandafter\gdef\csname R@an.cv.acdc.L1base.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.clause\endcsname{HyReX minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.33}\,pp, 95\,\% interval \ensuremath{+0.19} to \ensuremath{+0.49}\,pp, which lies inside $\pm$0.50\,pp and above zero}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.est\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.hi\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.lo\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L3.f0\endcsname{92.46}
\expandafter\gdef\csname R@an.cv.acdc.L3.f1\endcsname{91.92}
\expandafter\gdef\csname R@an.cv.acdc.L3.f2\endcsname{92.18}
\expandafter\gdef\csname R@an.cv.acdc.L3.f3\endcsname{91.97}
\expandafter\gdef\csname R@an.cv.acdc.L3.f4\endcsname{90.79}
\expandafter\gdef\csname R@an.cv.acdc.L3.max14\endcsname{92.18}
\expandafter\gdef\csname R@an.cv.acdc.L3.mean14\endcsname{91.71}
\expandafter\gdef\csname R@an.cv.acdc.L3.mean5\endcsname{91.86}
\expandafter\gdef\csname R@an.cv.acdc.L3.min14\endcsname{90.79}
\expandafter\gdef\csname R@an.cv.acdc.L3.params\endcsname{28.85}
\expandafter\gdef\csname R@an.cv.acdc.L3.params1\endcsname{28.8}
\expandafter\gdef\csname R@an.cv.acdc.L3.span14\endcsname{1.39}
\expandafter\gdef\csname R@an.cv.acdc.L3.src0\endcsname{fresh s1-2}
\expandafter\gdef\csname R@an.cv.acdc.L3.src0long\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.cv.acdc.L3.src0mark\endcsname{b}
\expandafter\gdef\csname R@an.cv.acdc.L3.src0n\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.boot.casewidth\endcsname{0.31}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.boot.foldwidth\endcsname{0.55}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.boot.hi\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.boot.lo\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.boot.mean\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.boot.n\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.20} to \ensuremath{+0.11}\,pp over the 160 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.d5\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.dcv\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.f0\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.f0gap\endcsname{0.21}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.f0lead\endcsname{the 0.50 pp registered pair floor does not resolve HyReX against ResEnc-M}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.f0rev\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.f1\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.f2\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.f3\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.f4\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.hi\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.lo\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.loo.max\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.loo.min\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.loo.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.loo.word\endcsname{changes sign when a single fold is dropped (one of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.share.word\endcsname{fold 3 alone carries 165\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.share_max\endcsname{165}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.span14\endcsname{0.39}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.src0\endcsname{fresh s1-2 for HyReX and for ResEnc-M}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.src0mark\endcsname{b/b}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.wordrev\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.clause\endcsname{HyReX minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.41}\,pp, 95\,\% interval \ensuremath{+0.22} to \ensuremath{+0.62}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.est\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.hi\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.lo\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.dcv\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.f1\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.f2\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.f3\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.f4\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.hi\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.lo\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.loo.max\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.loo.min\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.share.word\endcsname{fold 2 alone carries 42\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.share_max\endcsname{42}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.span14\endcsname{0.53}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.acdc.L3base.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.acdc.L3base.boot.casewidth\endcsname{0.30}
\expandafter\gdef\csname R@an.cv.acdc.L3base.boot.foldwidth\endcsname{0.46}
\expandafter\gdef\csname R@an.cv.acdc.L3base.boot.hi\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.boot.lo\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.boot.mean\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.boot.n\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L3base.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.acdc.L3base.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.18} to \ensuremath{+0.48}\,pp over the 160 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.acdc.L3base.d5\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.d5alt\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.dcv\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f0\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f0alt\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f0band\endcsname{0.16}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f0band.note\endcsname{two null SDs of this fold-0 difference, each the frozen default pool's training-seed SD of 0.099\,pp times $\sqrt{1/2 + 1/6}$ for the mean of two runs against the mean of the six-run pool: a locating band, not a test}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f0bandword\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f0gap\endcsname{0.45}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f0rev\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f0se\endcsname{0.081}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f1\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f2\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f3\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f4\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.hi\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.lo\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.loo.max\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.L3base.loo.min\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L3base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L3base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.L3base.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L3base.share.word\endcsname{fold 2 alone carries 38\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.L3base.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L3base.share_max\endcsname{38}
\expandafter\gdef\csname R@an.cv.acdc.L3base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.L3base.span14\endcsname{0.35}
\expandafter\gdef\csname R@an.cv.acdc.L3base.src0\endcsname{fresh s1-2 for HyReX and frozen pool for default}
\expandafter\gdef\csname R@an.cv.acdc.L3base.src0mark\endcsname{b/a}
\expandafter\gdef\csname R@an.cv.acdc.L3base.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.clause\endcsname{the function-identical control minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.08}\,pp, 95\,\% interval \ensuremath{-0.20} to \ensuremath{+0.04}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.est\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.hi\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.lo\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.P3c.f1\endcsname{91.47}
\expandafter\gdef\csname R@an.cv.acdc.P3c.f2\endcsname{91.48}
\expandafter\gdef\csname R@an.cv.acdc.P3c.f3\endcsname{91.80}
\expandafter\gdef\csname R@an.cv.acdc.P3c.f4\endcsname{90.46}
\expandafter\gdef\csname R@an.cv.acdc.P3c.max14\endcsname{91.80}
\expandafter\gdef\csname R@an.cv.acdc.P3c.mean14\endcsname{91.30}
\expandafter\gdef\csname R@an.cv.acdc.P3c.min14\endcsname{90.46}
\expandafter\gdef\csname R@an.cv.acdc.P3c.params\endcsname{30.38}
\expandafter\gdef\csname R@an.cv.acdc.P3c.params1\endcsname{30.4}
\expandafter\gdef\csname R@an.cv.acdc.P3c.span14\endcsname{1.34}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.dcv\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.f1\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.f2\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.f3\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.f4\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.hi\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.lo\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.loo.max\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.loo.min\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.share.word\endcsname{fold 2 alone carries 60\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.share_max\endcsname{60}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.span14\endcsname{0.19}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.clause\endcsname{LeanAdd minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.12}\,pp, 95\,\% interval \ensuremath{-0.25} to \ensuremath{+0.01}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.est\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.hi\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.lo\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.f1\endcsname{91.56}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.f2\endcsname{91.61}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.f3\endcsname{91.51}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.f4\endcsname{90.37}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.mean14\endcsname{91.26}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.params\endcsname{20.18}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.params1\endcsname{20.2}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.dcv\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.f1\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.f2\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.f3\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.f4\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.hi\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.lo\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.loo.max\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.loo.min\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.share.word\endcsname{fold 3 alone carries 60\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.share_max\endcsname{60}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.span14\endcsname{0.20}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.clause\endcsname{LeanAdd minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.04}\,pp, 95\,\% interval \ensuremath{-0.17} to \ensuremath{+0.10}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.est\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.hi\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.lo\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.ctloffset\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.dcv\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.f1\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.f2\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.f3\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.f4\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.hi\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.lo\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.loo.max\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.loo.min\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.loo.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.loo.word\endcsname{changes sign when a single fold is dropped (one of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.share.word\endcsname{fold 3 alone carries 184\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.share_max\endcsname{184}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.span14\endcsname{0.42}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.split\endcsname{LeanAdd minus the default is \ensuremath{-0.12}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.08}\,pp, so the margin over the function-identical control is \ensuremath{-0.04}\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.vsdefault\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.word\endcsname{does not improve on it}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.dcv\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.f1\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.f2\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.f3\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.f4\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.hi\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.lo\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.loo.max\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.loo.min\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.share.word\endcsname{fold 3 alone carries 65\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.share_max\endcsname{65}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.span14\endcsname{0.28}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.clause\endcsname{LeanAdd-NeXt minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.11}\,pp, 95\,\% interval \ensuremath{-0.27} to \ensuremath{+0.04}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.est\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.hi\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.lo\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.f1\endcsname{91.31}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.f2\endcsname{91.65}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.f3\endcsname{91.70}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.f4\endcsname{90.41}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.mean14\endcsname{91.27}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.params\endcsname{20.48}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.params1\endcsname{20.5}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.dcv\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.f1\endcsname{\ensuremath{-0.62}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.f2\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.f3\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.f4\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.hi\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.lo\endcsname{\ensuremath{-0.69}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.loo.max\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.loo.min\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.loo.minfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.share.word\endcsname{fold 1 alone carries 34\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.share_max\endcsname{34}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.span14\endcsname{0.35}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.clause\endcsname{LeanAdd-NeXt minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.04}\,pp, 95\,\% interval \ensuremath{-0.19} to \ensuremath{+0.13}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.est\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.hi\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.lo\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.ctloffset\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.dcv\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.f1\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.f2\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.f3\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.f4\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.hi\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.lo\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.loo.max\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.loo.min\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.loo.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.loo.word\endcsname{changes sign when a single fold is dropped (one of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.share.word\endcsname{fold 1 alone carries 118\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.share_max\endcsname{118}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.span14\endcsname{0.34}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.split\endcsname{LeanAdd-NeXt minus the default is \ensuremath{-0.11}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.08}\,pp, so the margin over the function-identical control is \ensuremath{-0.04}\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.vsdefault\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.word\endcsname{does not improve on it}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.dcv\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.f1\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.f2\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.f3\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.f4\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.hi\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.lo\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.loo.max\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.loo.min\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.loo.minfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.loo.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.loo.word\endcsname{changes sign when a single fold is dropped (one of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.share.word\endcsname{fold 3 alone carries 1368\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.share_max\endcsname{1368}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.span14\endcsname{0.44}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.dcv\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.f1\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.f2\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.f3\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.f4\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.hi\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.lo\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.loo.max\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.loo.min\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.share.word\endcsname{fold 1 alone carries 60\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.share_max\endcsname{60}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.span14\endcsname{0.26}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.clause\endcsname{HyReX-k9 minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.31}\,pp, 95\,\% interval \ensuremath{+0.18} to \ensuremath{+0.44}\,pp, which lies inside $\pm$0.50\,pp and above zero}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.est\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.hi\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.lo\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.f1\endcsname{91.95}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.f2\endcsname{91.92}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.f3\endcsname{91.99}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.f4\endcsname{90.88}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.mean14\endcsname{91.69}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.params\endcsname{29.96}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.params1\endcsname{30.0}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.dcv\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.f1\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.f2\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.f3\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.f4\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.hi\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.lo\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.loo.max\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.loo.min\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.loo.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.loo.word\endcsname{changes sign when a single fold is dropped (one of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.share.word\endcsname{fold 2 alone carries 239\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.share_max\endcsname{239}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.span14\endcsname{0.35}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.clause\endcsname{HyReX-k9 minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.38}\,pp, 95\,\% interval \ensuremath{+0.22} to \ensuremath{+0.56}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.est\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.hi\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.lo\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.ctloffset\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.dcv\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.f1\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.f2\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.f3\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.f4\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.hi\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.lo\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.loo.max\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.loo.min\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.share.word\endcsname{fold 1 alone carries 31\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.share_max\endcsname{31}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.span14\endcsname{0.29}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.split\endcsname{HyReX-k9 minus the default is \ensuremath{+0.31}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.08}\,pp, so the margin over the function-identical control is \ensuremath{+0.38}\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.vsdefault\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.word\endcsname{improves on the control in every fold}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.dcv\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.f1\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.f2\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.f3\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.f4\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.hi\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.lo\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.loo.max\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.loo.min\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.share.word\endcsname{fold 4 alone carries 35\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.share_max\endcsname{35}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.span14\endcsname{0.25}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.clause\endcsname{LeanDeepMid minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.08}\,pp, 95\,\% interval \ensuremath{-0.09} to \ensuremath{+0.24}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.est\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.hi\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.lo\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.f1\endcsname{91.57}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.f2\endcsname{91.72}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.f3\endcsname{91.61}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.f4\endcsname{90.94}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.mean14\endcsname{91.46}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.params\endcsname{30.26}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.params1\endcsname{30.3}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.clause\endcsname{LeanDeepMid minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.16}\,pp, 95\,\% interval \ensuremath{-0.02} to \ensuremath{+0.35}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.est\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.hi\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.lo\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.ctloffset\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.dcv\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.f1\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.f2\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.f3\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.f4\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.hi\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.lo\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.loo.max\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.loo.min\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.share.word\endcsname{fold 4 alone carries 76\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.share_max\endcsname{76}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.span14\endcsname{0.67}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.split\endcsname{LeanDeepMid minus the default is \ensuremath{+0.08}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.08}\,pp, so the margin over the function-identical control is \ensuremath{+0.16}\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.vsdefault\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.word\endcsname{improves on it on average (3 of 4 folds)}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.dcv\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.f1\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.f2\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.f3\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.f4\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.hi\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.lo\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.loo.max\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.loo.min\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.share.word\endcsname{fold 4 alone carries 68\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.share_max\endcsname{68}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.span14\endcsname{0.62}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.dcv\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.f1\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.f2\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.f3\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.f4\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.lo\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.loo.max\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.loo.min\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.loo.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.loo.word\endcsname{changes sign when a single fold is dropped (three of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.share.word\endcsname{fold 4 alone carries 152\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.share_max\endcsname{152}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.span14\endcsname{0.69}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.word\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.cv.acdc.V7A2.cbs.clause\endcsname{LeanDeepMid+FD minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.acdc.V7A2.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7A2.params\endcsname{30.38}
\expandafter\gdef\csname R@an.cv.acdc.V7A2.params1\endcsname{30.4}
\expandafter\gdef\csname R@an.cv.acdc.V7A2P3c.cbs.clause\endcsname{LeanDeepMid+FD minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.acdc.V7A2P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7A2P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7A2P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7A2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7A2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7A2V7A1.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7A2V7A1.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7A2base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7A2base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7B1.cbs.clause\endcsname{LeanSep minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.acdc.V7B1.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B1.params\endcsname{19.65}
\expandafter\gdef\csname R@an.cv.acdc.V7B1.params1\endcsname{19.6}
\expandafter\gdef\csname R@an.cv.acdc.V7B1P3c.cbs.clause\endcsname{LeanSep minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.acdc.V7B1P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B1P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B1P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7B1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7B1V5B2.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B1V5B2.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7B1base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B1base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7B2.cbs.clause\endcsname{LeanDil minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.acdc.V7B2.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B2.params\endcsname{19.67}
\expandafter\gdef\csname R@an.cv.acdc.V7B2.params1\endcsname{19.7}
\expandafter\gdef\csname R@an.cv.acdc.V7B2P3c.cbs.clause\endcsname{LeanDil minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.acdc.V7B2P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B2P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B2P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7B2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7B2V5B2.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B2V5B2.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7B2base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B2base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.clause\endcsname{LeanNeXt-s5 minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.19}\,pp, 95\,\% interval \ensuremath{-0.34} to \ensuremath{-0.04}\,pp, which lies inside $\pm$0.50\,pp and below zero}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.est\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.hi\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.lo\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.f1\endcsname{91.30}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.f2\endcsname{91.56}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.f3\endcsname{91.61}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.f4\endcsname{90.29}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.mean14\endcsname{91.19}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.params\endcsname{20.33}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.params1\endcsname{20.3}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.clause\endcsname{LeanNeXt-s5 minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.11}\,pp, 95\,\% interval \ensuremath{-0.25} to \ensuremath{+0.04}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.est\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.hi\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.lo\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.ctloffset\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.dcv\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.f1\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.f2\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.f3\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.f4\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.hi\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.lo\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.loo.max\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.loo.min\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.share.word\endcsname{fold 3 alone carries 43\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.share_max\endcsname{43}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.span14\endcsname{0.27}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.split\endcsname{LeanNeXt-s5 minus the default is \ensuremath{-0.19}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.08}\,pp, so the margin over the function-identical control is \ensuremath{-0.11}\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.vsdefault\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.word\endcsname{does not improve on it}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.dcv\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.f1\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.f2\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.f3\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.f4\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.hi\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.lo\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.loo.max\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.loo.min\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.share.word\endcsname{fold 4 alone carries 39\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.share_max\endcsname{39}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.span14\endcsname{0.11}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.dcv\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.f1\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.f2\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.f3\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.f4\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.hi\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.lo\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.loo.max\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.loo.min\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.share.word\endcsname{fold 1 alone carries 37\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.share_max\endcsname{37}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.span14\endcsname{0.18}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.V8B2.cbs.clause\endcsname{Stem1 minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.acdc.V8B2.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V8B2.params\endcsname{20.32}
\expandafter\gdef\csname R@an.cv.acdc.V8B2.params1\endcsname{20.3}
\expandafter\gdef\csname R@an.cv.acdc.V8B2P3c.cbs.clause\endcsname{Stem1 minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.acdc.V8B2P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V8B2P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V8B2P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V8B2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V8B2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V8B2base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V8B2base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.base.f0\endcsname{92.01}
\expandafter\gdef\csname R@an.cv.acdc.base.f1\endcsname{91.58}
\expandafter\gdef\csname R@an.cv.acdc.base.f2\endcsname{91.67}
\expandafter\gdef\csname R@an.cv.acdc.base.f3\endcsname{91.82}
\expandafter\gdef\csname R@an.cv.acdc.base.f4\endcsname{90.46}
\expandafter\gdef\csname R@an.cv.acdc.base.max14\endcsname{91.82}
\expandafter\gdef\csname R@an.cv.acdc.base.mean14\endcsname{91.38}
\expandafter\gdef\csname R@an.cv.acdc.base.mean5\endcsname{91.51}
\expandafter\gdef\csname R@an.cv.acdc.base.min14\endcsname{90.46}
\expandafter\gdef\csname R@an.cv.acdc.base.params\endcsname{30.38}
\expandafter\gdef\csname R@an.cv.acdc.base.params1\endcsname{30.4}
\expandafter\gdef\csname R@an.cv.acdc.base.span14\endcsname{1.36}
\expandafter\gdef\csname R@an.cv.acdc.base.src0\endcsname{frozen pool}
\expandafter\gdef\csname R@an.cv.acdc.base.src0long\endcsname{the frozen default pool}
\expandafter\gdef\csname R@an.cv.acdc.base.src0mark\endcsname{a}
\expandafter\gdef\csname R@an.cv.acdc.base.src0n\endcsname{6}
\expandafter\gdef\csname R@an.cv.acdc.recovery.L3\endcsname{0.90}
\expandafter\gdef\csname R@an.cv.acdc.recovery.L3.hi\endcsname{1.63}
\expandafter\gdef\csname R@an.cv.acdc.recovery.L3.lo\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.acdc.recovery.L3.method\endcsname{the delta method applied to the two four-fold mean margins, HyReX minus the default and ResEnc-M minus the default, which are differences from the same default runs, so their covariance over the folds enters the variance of the ratio; the interval takes the t quantile on three degrees of freedom of the registered paired-t intervals of the margins; it is descriptive, a description of four folds of one seed each and not a test, and it is withheld when ResEnc-M's own interval over the folds includes zero}
\expandafter\gdef\csname R@an.cv.acdc.recovery.L3.sentence\endcsname{On ACDC, HyReX's mean margin over the default on the four folds that entered no decision, \ensuremath{+0.33}\,pp, is 0.90 of ResEnc-M's, \ensuremath{+0.37}\,pp; the 95\,\% interval of that ratio, 0.17 to 1.63, comes from the delta method on the two fold-mean margins and describes the four folds without testing anything}
\expandafter\gdef\csname R@an.cv.acdc.recovery.L3.state\endcsname{complete}
\expandafter\gdef\csname R@an.cv.acdc.replication\endcsname{ACDC is a registered guard, not a co-primary; the registered ACDC fresh-seed replication has landed, so its fold-0 cells for HyReX and ResEnc-M are fresh seed-1-2 means, while the four confirmation folds remain one seed per arm}
\expandafter\gdef\csname R@an.cv.amos.D2.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.D2.cbs.clause\endcsname{LeanDec minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.43}\,pp, 95\,\% interval \ensuremath{-0.66} to \ensuremath{-0.22}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.amos.D2.cbs.est\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.cv.amos.D2.cbs.hi\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.cv.amos.D2.cbs.lo\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.cv.amos.D2.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.D2.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.D2.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.D2.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.D2.f0\endcsname{87.34}
\expandafter\gdef\csname R@an.cv.amos.D2.f1\endcsname{88.83}
\expandafter\gdef\csname R@an.cv.amos.D2.f2\endcsname{87.92}
\expandafter\gdef\csname R@an.cv.amos.D2.f3\endcsname{88.14}
\expandafter\gdef\csname R@an.cv.amos.D2.f4\endcsname{86.74}
\expandafter\gdef\csname R@an.cv.amos.D2.max14\endcsname{88.83}
\expandafter\gdef\csname R@an.cv.amos.D2.mean14\endcsname{87.91}
\expandafter\gdef\csname R@an.cv.amos.D2.mean5\endcsname{87.79}
\expandafter\gdef\csname R@an.cv.amos.D2.min14\endcsname{86.74}
\expandafter\gdef\csname R@an.cv.amos.D2.params\endcsname{26.03}
\expandafter\gdef\csname R@an.cv.amos.D2.params1\endcsname{26.0}
\expandafter\gdef\csname R@an.cv.amos.D2.span14\endcsname{2.08}
\expandafter\gdef\csname R@an.cv.amos.D2.src0\endcsname{seed 0}
\expandafter\gdef\csname R@an.cv.amos.D2.src0long\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.cv.amos.D2.src0mark\endcsname{c}
\expandafter\gdef\csname R@an.cv.amos.D2.src0n\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.cbs.clause\endcsname{LeanDec minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.40}\,pp, 95\,\% interval \ensuremath{-0.61} to \ensuremath{-0.18}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.cbs.est\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.cbs.hi\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.cbs.lo\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.ctloffset\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.dcv\endcsname{\ensuremath{-0.41}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.f1\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.f2\endcsname{\ensuremath{-0.72}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.f3\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.f4\endcsname{\ensuremath{-0.60}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.hi\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.lo\endcsname{\ensuremath{-0.95}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.loo.max\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.loo.min\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.share.word\endcsname{fold 2 alone carries 44\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.share_max\endcsname{44}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.span14\endcsname{0.78}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.split\endcsname{LeanDec minus the default is \ensuremath{-0.44}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.03}\,pp, so the margin over the function-identical control is \ensuremath{-0.41}\,pp}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.vsdefault\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.word\endcsname{does not improve on it}
\expandafter\gdef\csname R@an.cv.amos.D2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.D2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.D2base.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.amos.D2base.boot.casewidth\endcsname{0.28}
\expandafter\gdef\csname R@an.cv.amos.D2base.boot.foldwidth\endcsname{0.63}
\expandafter\gdef\csname R@an.cv.amos.D2base.boot.hi\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.cv.amos.D2base.boot.lo\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.cv.amos.D2base.boot.mean\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.cv.amos.D2base.boot.n\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.D2base.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.amos.D2base.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.51} to \ensuremath{-0.23}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.amos.D2base.d5\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.cv.amos.D2base.d5alt\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.cv.amos.D2base.dcv\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.cv.amos.D2base.f0\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.cv.amos.D2base.f0alt\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.cv.amos.D2base.f0band\endcsname{0.26}
\expandafter\gdef\csname R@an.cv.amos.D2base.f0band.note\endcsname{two null SDs of this fold-0 difference, each the frozen default pool's training-seed SD of 0.122\,pp times $\sqrt{1/1 + 1/6}$ for the mean of one run against the mean of the six-run pool: a locating band, not a test}
\expandafter\gdef\csname R@an.cv.amos.D2base.f0bandword\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.amos.D2base.f0gap\endcsname{0.36}
\expandafter\gdef\csname R@an.cv.amos.D2base.f0rev\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.amos.D2base.f0se\endcsname{0.132}
\expandafter\gdef\csname R@an.cv.amos.D2base.f1\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.cv.amos.D2base.f2\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.cv.amos.D2base.f3\endcsname{\ensuremath{-0.65}}
\expandafter\gdef\csname R@an.cv.amos.D2base.f4\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.amos.D2base.hi\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.amos.D2base.lo\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.cv.amos.D2base.loo.max\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.cv.amos.D2base.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.D2base.loo.min\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.cv.amos.D2base.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.D2base.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.D2base.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.D2base.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.D2base.share.word\endcsname{fold 3 alone carries 37\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.D2base.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.D2base.share_max\endcsname{37}
\expandafter\gdef\csname R@an.cv.amos.D2base.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.D2base.span14\endcsname{0.40}
\expandafter\gdef\csname R@an.cv.amos.D2base.src0\endcsname{seed 0 for LeanDec and frozen pool for default}
\expandafter\gdef\csname R@an.cv.amos.D2base.src0mark\endcsname{c/a}
\expandafter\gdef\csname R@an.cv.amos.D2base.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.L1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.L1.cbs.clause\endcsname{ResEnc-M minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.40}\,pp, 95\,\% interval \ensuremath{+0.16} to \ensuremath{+0.65}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.amos.L1.cbs.est\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.cv.amos.L1.cbs.hi\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.cv.amos.L1.cbs.lo\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.cv.amos.L1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.L1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.L1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1.f0\endcsname{88.17}
\expandafter\gdef\csname R@an.cv.amos.L1.f1\endcsname{89.46}
\expandafter\gdef\csname R@an.cv.amos.L1.f2\endcsname{89.25}
\expandafter\gdef\csname R@an.cv.amos.L1.f3\endcsname{88.63}
\expandafter\gdef\csname R@an.cv.amos.L1.f4\endcsname{87.68}
\expandafter\gdef\csname R@an.cv.amos.L1.max14\endcsname{89.46}
\expandafter\gdef\csname R@an.cv.amos.L1.mean14\endcsname{88.75}
\expandafter\gdef\csname R@an.cv.amos.L1.mean5\endcsname{88.64}
\expandafter\gdef\csname R@an.cv.amos.L1.min14\endcsname{87.68}
\expandafter\gdef\csname R@an.cv.amos.L1.params\endcsname{102.28}
\expandafter\gdef\csname R@an.cv.amos.L1.params1\endcsname{102.3}
\expandafter\gdef\csname R@an.cv.amos.L1.span14\endcsname{1.78}
\expandafter\gdef\csname R@an.cv.amos.L1.src0\endcsname{fresh s1-2}
\expandafter\gdef\csname R@an.cv.amos.L1.src0long\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.cv.amos.L1.src0mark\endcsname{b}
\expandafter\gdef\csname R@an.cv.amos.L1.src0n\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.dcv\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.f1\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.f2\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.f3\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.f4\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.hi\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.lo\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.loo.max\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.loo.min\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.loo.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.loo.word\endcsname{changes sign when a single fold is dropped (one of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.share.word\endcsname{fold 1 alone carries 202\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.share_max\endcsname{202}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.span14\endcsname{0.39}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.L1L3.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.amos.L1L3.boot.casewidth\endcsname{0.28}
\expandafter\gdef\csname R@an.cv.amos.L1L3.boot.foldwidth\endcsname{1.16}
\expandafter\gdef\csname R@an.cv.amos.L1L3.boot.hi\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.boot.lo\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.boot.mean\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.boot.n\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.L1L3.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.amos.L1L3.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.08} to \ensuremath{+0.21}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.amos.L1L3.dcv\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.f1\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.f2\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.f3\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.f4\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.hi\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.lo\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.loo.max\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.L1L3.loo.min\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.L1L3.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.L1L3.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.L1L3.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.amos.L1L3.share.word\endcsname{fold 2 alone carries 57\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.L1L3.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.L1L3.share_max\endcsname{57}
\expandafter\gdef\csname R@an.cv.amos.L1L3.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.L1L3.span14\endcsname{0.77}
\expandafter\gdef\csname R@an.cv.amos.L1L3.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.cbs.clause\endcsname{ResEnc-M minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.44}\,pp, 95\,\% interval \ensuremath{+0.19} to \ensuremath{+0.71}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.cbs.est\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.cbs.hi\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.cbs.lo\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.ctloffset\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.dcv\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.f1\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.f2\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.f3\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.f4\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.hi\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.lo\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.loo.max\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.loo.min\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.share.word\endcsname{fold 1 alone carries 40\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.share_max\endcsname{40}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.span14\endcsname{0.59}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.split\endcsname{ResEnc-M minus the default is \ensuremath{+0.41}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.03}\,pp, so the margin over the function-identical control is \ensuremath{+0.44}\,pp}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.vsdefault\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.word\endcsname{improves on the control in every fold}
\expandafter\gdef\csname R@an.cv.amos.L1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.L1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.L1b.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.L1b.cbs.clause\endcsname{ResEnc-matched minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.43}\,pp, 95\,\% interval \ensuremath{+0.19} to \ensuremath{+0.68}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.amos.L1b.cbs.est\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.cv.amos.L1b.cbs.hi\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.cv.amos.L1b.cbs.lo\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.amos.L1b.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.L1b.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.L1b.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1b.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1b.f1\endcsname{89.63}
\expandafter\gdef\csname R@an.cv.amos.L1b.f2\endcsname{89.03}
\expandafter\gdef\csname R@an.cv.amos.L1b.f3\endcsname{88.69}
\expandafter\gdef\csname R@an.cv.amos.L1b.f4\endcsname{87.74}
\expandafter\gdef\csname R@an.cv.amos.L1b.mean14\endcsname{88.78}
\expandafter\gdef\csname R@an.cv.amos.L1b.params\endcsname{102.37}
\expandafter\gdef\csname R@an.cv.amos.L1b.params1\endcsname{102.4}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.dcv\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.f1\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.f2\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.f3\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.f4\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.hi\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.lo\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.loo.max\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.loo.min\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.share.word\endcsname{fold 1 alone carries 69\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.share_max\endcsname{69}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.span14\endcsname{0.85}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.amos.L1base.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.amos.L1base.boot.casewidth\endcsname{0.34}
\expandafter\gdef\csname R@an.cv.amos.L1base.boot.foldwidth\endcsname{1.36}
\expandafter\gdef\csname R@an.cv.amos.L1base.boot.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.cv.amos.L1base.boot.lo\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.amos.L1base.boot.mean\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.amos.L1base.boot.n\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.L1base.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.amos.L1base.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.20} to \ensuremath{+0.54}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.amos.L1base.d5\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.cv.amos.L1base.d5alt\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.cv.amos.L1base.dcv\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv.amos.L1base.f0\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.cv.amos.L1base.f0alt\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.amos.L1base.f0band\endcsname{0.20}
\expandafter\gdef\csname R@an.cv.amos.L1base.f0band.note\endcsname{two null SDs of this fold-0 difference, each the frozen default pool's training-seed SD of 0.122\,pp times $\sqrt{1/2 + 1/6}$ for the mean of two runs against the mean of the six-run pool: a locating band, not a test}
\expandafter\gdef\csname R@an.cv.amos.L1base.f0bandword\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.amos.L1base.f0gap\endcsname{0.46}
\expandafter\gdef\csname R@an.cv.amos.L1base.f0rev\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.cv.amos.L1base.f0se\endcsname{0.100}
\expandafter\gdef\csname R@an.cv.amos.L1base.f1\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.cv.amos.L1base.f2\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.cv.amos.L1base.f3\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.amos.L1base.f4\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.cv.amos.L1base.hi\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.cv.amos.L1base.lo\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.cv.amos.L1base.loo.max\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.cv.amos.L1base.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.L1base.loo.min\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.cv.amos.L1base.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.L1base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.L1base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.L1base.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.amos.L1base.share.word\endcsname{fold 2 alone carries 47\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.L1base.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.L1base.share_max\endcsname{47}
\expandafter\gdef\csname R@an.cv.amos.L1base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.L1base.span14\endcsname{0.94}
\expandafter\gdef\csname R@an.cv.amos.L1base.src0\endcsname{fresh s1-2 for ResEnc-M and frozen pool for default}
\expandafter\gdef\csname R@an.cv.amos.L1base.src0mark\endcsname{b/a}
\expandafter\gdef\csname R@an.cv.amos.L1base.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.amos.L3.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.L3.cbs.clause\endcsname{HyReX minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.24}\,pp, 95\,\% interval \ensuremath{+0.01} to \ensuremath{+0.46}\,pp, which lies inside $\pm$0.50\,pp and above zero}
\expandafter\gdef\csname R@an.cv.amos.L3.cbs.est\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.amos.L3.cbs.hi\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.cv.amos.L3.cbs.lo\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.amos.L3.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.L3.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.L3.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L3.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L3.f0\endcsname{87.83}
\expandafter\gdef\csname R@an.cv.amos.L3.f1\endcsname{89.09}
\expandafter\gdef\csname R@an.cv.amos.L3.f2\endcsname{88.84}
\expandafter\gdef\csname R@an.cv.amos.L3.f3\endcsname{88.99}
\expandafter\gdef\csname R@an.cv.amos.L3.f4\endcsname{87.38}
\expandafter\gdef\csname R@an.cv.amos.L3.max14\endcsname{89.09}
\expandafter\gdef\csname R@an.cv.amos.L3.mean14\endcsname{88.58}
\expandafter\gdef\csname R@an.cv.amos.L3.mean5\endcsname{88.43}
\expandafter\gdef\csname R@an.cv.amos.L3.min14\endcsname{87.38}
\expandafter\gdef\csname R@an.cv.amos.L3.params\endcsname{29.59}
\expandafter\gdef\csname R@an.cv.amos.L3.params1\endcsname{29.6}
\expandafter\gdef\csname R@an.cv.amos.L3.span14\endcsname{1.70}
\expandafter\gdef\csname R@an.cv.amos.L3.src0\endcsname{fresh s1-2}
\expandafter\gdef\csname R@an.cv.amos.L3.src0long\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.cv.amos.L3.src0mark\endcsname{b}
\expandafter\gdef\csname R@an.cv.amos.L3.src0n\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.L3L1.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.amos.L3L1.boot.casewidth\endcsname{0.29}
\expandafter\gdef\csname R@an.cv.amos.L3L1.boot.foldwidth\endcsname{1.16}
\expandafter\gdef\csname R@an.cv.amos.L3L1.boot.hi\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.boot.lo\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.boot.mean\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.boot.n\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.L3L1.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.amos.L3L1.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.21} to \ensuremath{+0.08}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.amos.L3L1.d5\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.dcv\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.f0\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.f0gap\endcsname{0.33}
\expandafter\gdef\csname R@an.cv.amos.L3L1.f0lead\endcsname{the 0.50 pp registered pair floor does not resolve HyReX against ResEnc-M}
\expandafter\gdef\csname R@an.cv.amos.L3L1.f0rev\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.f1\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.f2\endcsname{\ensuremath{-0.41}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.f3\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.f4\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.hi\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.lo\endcsname{\ensuremath{-0.76}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.loo.max\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.L3L1.loo.min\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.loo.minfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.L3L1.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.L3L1.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.L3L1.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.amos.L3L1.share.word\endcsname{fold 2 alone carries 57\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.L3L1.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.L3L1.share_max\endcsname{57}
\expandafter\gdef\csname R@an.cv.amos.L3L1.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.L3L1.span14\endcsname{0.77}
\expandafter\gdef\csname R@an.cv.amos.L3L1.src0\endcsname{fresh s1-2 for HyReX and for ResEnc-M}
\expandafter\gdef\csname R@an.cv.amos.L3L1.src0mark\endcsname{b/b}
\expandafter\gdef\csname R@an.cv.amos.L3L1.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.L3L1.wordrev\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.cbs.clause\endcsname{HyReX minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.27}\,pp, 95\,\% interval \ensuremath{+0.07} to \ensuremath{+0.48}\,pp, which lies inside $\pm$0.50\,pp and above zero}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.cbs.est\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.cbs.hi\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.cbs.lo\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.dcv\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.f1\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.f2\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.f3\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.f4\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.hi\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.lo\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.loo.max\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.loo.min\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.loo.minfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.share.word\endcsname{fold 3 alone carries 45\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.share_max\endcsname{45}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.span14\endcsname{0.43}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.amos.L3base.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.amos.L3base.boot.casewidth\endcsname{0.35}
\expandafter\gdef\csname R@an.cv.amos.L3base.boot.foldwidth\endcsname{0.61}
\expandafter\gdef\csname R@an.cv.amos.L3base.boot.hi\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.cv.amos.L3base.boot.lo\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.amos.L3base.boot.mean\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.amos.L3base.boot.n\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.L3base.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.amos.L3base.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.12} to \ensuremath{+0.47}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.amos.L3base.d5\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.amos.L3base.d5alt\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.amos.L3base.dcv\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.amos.L3base.f0\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.cv.amos.L3base.f0alt\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.amos.L3base.f0band\endcsname{0.20}
\expandafter\gdef\csname R@an.cv.amos.L3base.f0band.note\endcsname{two null SDs of this fold-0 difference, each the frozen default pool's training-seed SD of 0.122\,pp times $\sqrt{1/2 + 1/6}$ for the mean of two runs against the mean of the six-run pool: a locating band, not a test}
\expandafter\gdef\csname R@an.cv.amos.L3base.f0bandword\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.amos.L3base.f0gap\endcsname{0.13}
\expandafter\gdef\csname R@an.cv.amos.L3base.f0rev\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.cv.amos.L3base.f0se\endcsname{0.100}
\expandafter\gdef\csname R@an.cv.amos.L3base.f1\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.L3base.f2\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.amos.L3base.f3\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.amos.L3base.f4\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.cv.amos.L3base.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.cv.amos.L3base.lo\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.amos.L3base.loo.max\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.cv.amos.L3base.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L3base.loo.min\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.amos.L3base.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.L3base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.L3base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.L3base.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.amos.L3base.share.word\endcsname{fold 4 alone carries 42\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.L3base.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.L3base.share_max\endcsname{42}
\expandafter\gdef\csname R@an.cv.amos.L3base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.L3base.span14\endcsname{0.42}
\expandafter\gdef\csname R@an.cv.amos.L3base.src0\endcsname{fresh s1-2 for HyReX and frozen pool for default}
\expandafter\gdef\csname R@an.cv.amos.L3base.src0mark\endcsname{b/a}
\expandafter\gdef\csname R@an.cv.amos.L3base.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.amos.P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.P3c.cbs.clause\endcsname{the function-identical control minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.04}\,pp, 95\,\% interval \ensuremath{-0.25} to \ensuremath{+0.17}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.amos.P3c.cbs.est\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.amos.P3c.cbs.hi\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.cv.amos.P3c.cbs.lo\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.amos.P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.P3c.f1\endcsname{88.77}
\expandafter\gdef\csname R@an.cv.amos.P3c.f2\endcsname{88.64}
\expandafter\gdef\csname R@an.cv.amos.P3c.f3\endcsname{88.52}
\expandafter\gdef\csname R@an.cv.amos.P3c.f4\endcsname{87.34}
\expandafter\gdef\csname R@an.cv.amos.P3c.max14\endcsname{88.77}
\expandafter\gdef\csname R@an.cv.amos.P3c.mean14\endcsname{88.32}
\expandafter\gdef\csname R@an.cv.amos.P3c.min14\endcsname{87.34}
\expandafter\gdef\csname R@an.cv.amos.P3c.params\endcsname{31.12}
\expandafter\gdef\csname R@an.cv.amos.P3c.params1\endcsname{31.1}
\expandafter\gdef\csname R@an.cv.amos.P3c.span14\endcsname{1.42}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.dcv\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.f1\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.f2\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.f3\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.f4\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.hi\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.lo\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.loo.max\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.loo.min\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.loo.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.loo.word\endcsname{changes sign when a single fold is dropped (two of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.share.word\endcsname{fold 1 alone carries 281\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.share_max\endcsname{281}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.span14\endcsname{0.70}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.V5B1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V5B1.cbs.clause\endcsname{LeanAdd minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.46}\,pp, 95\,\% interval \ensuremath{-0.67} to \ensuremath{-0.25}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.amos.V5B1.cbs.est\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.cv.amos.V5B1.cbs.hi\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.amos.V5B1.cbs.lo\endcsname{\ensuremath{-0.67}}
\expandafter\gdef\csname R@an.cv.amos.V5B1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V5B1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B1.f1\endcsname{88.65}
\expandafter\gdef\csname R@an.cv.amos.V5B1.f2\endcsname{88.11}
\expandafter\gdef\csname R@an.cv.amos.V5B1.f3\endcsname{88.03}
\expandafter\gdef\csname R@an.cv.amos.V5B1.f4\endcsname{86.76}
\expandafter\gdef\csname R@an.cv.amos.V5B1.mean14\endcsname{87.89}
\expandafter\gdef\csname R@an.cv.amos.V5B1.params\endcsname{20.93}
\expandafter\gdef\csname R@an.cv.amos.V5B1.params1\endcsname{20.9}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.dcv\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.f1\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.f2\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.f3\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.f4\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.hi\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.lo\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.loo.max\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.loo.min\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.loo.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.loo.word\endcsname{changes sign when a single fold is dropped (two of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.share.word\endcsname{fold 1 alone carries 201\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.share_max\endcsname{201}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.span14\endcsname{0.37}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.cbs.clause\endcsname{LeanAdd minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.42}\,pp, 95\,\% interval \ensuremath{-0.61} to \ensuremath{-0.23}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.cbs.est\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.cbs.hi\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.cbs.lo\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.ctloffset\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.dcv\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.f1\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.f2\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.f3\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.f4\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.hi\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.lo\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.loo.max\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.loo.min\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.share.word\endcsname{fold 4 alone carries 34\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.share_max\endcsname{34}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.span14\endcsname{0.47}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.split\endcsname{LeanAdd minus the default is \ensuremath{-0.46}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.03}\,pp, so the margin over the function-identical control is \ensuremath{-0.43}\,pp}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.vsdefault\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.word\endcsname{does not improve on it}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.dcv\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.f1\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.f2\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.f3\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.f4\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.hi\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.lo\endcsname{\ensuremath{-0.82}}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.loo.max\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.loo.min\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.share.word\endcsname{fold 3 alone carries 42\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.share_max\endcsname{42}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.span14\endcsname{0.52}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.V5B2.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V5B2.cbs.clause\endcsname{LeanAdd-NeXt minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.25}\,pp, 95\,\% interval \ensuremath{-0.47} to \ensuremath{-0.04}\,pp, which lies inside $\pm$0.50\,pp and below zero}
\expandafter\gdef\csname R@an.cv.amos.V5B2.cbs.est\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.amos.V5B2.cbs.hi\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.amos.V5B2.cbs.lo\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.cv.amos.V5B2.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V5B2.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B2.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B2.f1\endcsname{88.56}
\expandafter\gdef\csname R@an.cv.amos.V5B2.f2\endcsname{88.28}
\expandafter\gdef\csname R@an.cv.amos.V5B2.f3\endcsname{88.30}
\expandafter\gdef\csname R@an.cv.amos.V5B2.f4\endcsname{87.23}
\expandafter\gdef\csname R@an.cv.amos.V5B2.mean14\endcsname{88.09}
\expandafter\gdef\csname R@an.cv.amos.V5B2.params\endcsname{21.22}
\expandafter\gdef\csname R@an.cv.amos.V5B2.params1\endcsname{21.2}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.dcv\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.f1\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.f2\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.f3\endcsname{\ensuremath{-0.69}}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.f4\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.hi\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.lo\endcsname{\ensuremath{-0.85}}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.loo.max\endcsname{\ensuremath{-0.41}}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.loo.min\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.share.word\endcsname{fold 3 alone carries 36\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.share_max\endcsname{36}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.span14\endcsname{0.53}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.cbs.clause\endcsname{LeanAdd-NeXt minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.21}\,pp, 95\,\% interval \ensuremath{-0.40} to \ensuremath{-0.03}\,pp, which lies inside $\pm$0.50\,pp and below zero}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.cbs.est\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.cbs.hi\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.cbs.lo\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.ctloffset\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.dcv\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.f1\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.f2\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.f3\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.f4\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.hi\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.lo\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.loo.max\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.loo.min\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.share.word\endcsname{fold 2 alone carries 39\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.share_max\endcsname{39}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.span14\endcsname{0.24}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.split\endcsname{LeanAdd-NeXt minus the default is \ensuremath{-0.25}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.03}\,pp, so the margin over the function-identical control is \ensuremath{-0.22}\,pp}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.vsdefault\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.word\endcsname{does not improve on it}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.dcv\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.f1\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.f2\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.f3\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.f4\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.hi\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.lo\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.loo.max\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.loo.min\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.share.word\endcsname{fold 4 alone carries 57\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.share_max\endcsname{57}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.span14\endcsname{0.57}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.dcv\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.f1\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.f2\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.f3\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.f4\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.hi\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.lo\endcsname{\ensuremath{-0.83}}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.loo.max\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.loo.min\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.share.word\endcsname{fold 1 alone carries 55\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.share_max\endcsname{55}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.span14\endcsname{0.79}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.cbs.clause\endcsname{HyReX-k9 minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.21}\,pp, 95\,\% interval \ensuremath{-0.03} to \ensuremath{+0.45}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.cbs.est\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.cbs.hi\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.cbs.lo\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.f1\endcsname{89.02}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.f2\endcsname{88.68}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.f3\endcsname{88.82}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.f4\endcsname{87.67}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.mean14\endcsname{88.55}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.params\endcsname{30.70}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.params1\endcsname{30.7}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.dcv\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.f1\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.f2\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.f3\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.f4\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.hi\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.lo\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.loo.max\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.loo.min\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.loo.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.loo.word\endcsname{changes sign when a single fold is dropped (two of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.share.word\endcsname{fold 3 alone carries 155\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.share_max\endcsname{155}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.span14\endcsname{0.46}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.cbs.clause\endcsname{HyReX-k9 minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.25}\,pp, 95\,\% interval \ensuremath{-0.01} to \ensuremath{+0.51}\,pp, which reaches just below zero}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.cbs.est\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.cbs.hi\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.cbs.lo\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.ctloffset\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.dcv\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.f1\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.f2\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.f3\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.f4\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.hi\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.lo\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.loo.max\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.loo.min\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.share.word\endcsname{fold 4 alone carries 36\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.share_max\endcsname{36}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.span14\endcsname{0.29}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.split\endcsname{HyReX-k9 minus the default is \ensuremath{+0.20}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.03}\,pp, so the margin over the function-identical control is \ensuremath{+0.23}\,pp}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.vsdefault\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.word\endcsname{improves on the control in every fold}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.dcv\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.f1\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.f2\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.f3\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.f4\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.hi\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.lo\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.loo.max\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.loo.min\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.share.word\endcsname{fold 4 alone carries 84\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.share_max\endcsname{84}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.span14\endcsname{0.78}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.amos.V7A1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V7A1.cbs.clause\endcsname{LeanDeepMid minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.26}\,pp, 95\,\% interval \ensuremath{+0.01} to \ensuremath{+0.52}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.amos.V7A1.cbs.est\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.amos.V7A1.cbs.hi\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.cv.amos.V7A1.cbs.lo\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.amos.V7A1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V7A1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7A1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7A1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7A1.f1\endcsname{88.96}
\expandafter\gdef\csname R@an.cv.amos.V7A1.f2\endcsname{88.99}
\expandafter\gdef\csname R@an.cv.amos.V7A1.f3\endcsname{88.66}
\expandafter\gdef\csname R@an.cv.amos.V7A1.f4\endcsname{87.80}
\expandafter\gdef\csname R@an.cv.amos.V7A1.mean14\endcsname{88.61}
\expandafter\gdef\csname R@an.cv.amos.V7A1.params\endcsname{31.00}
\expandafter\gdef\csname R@an.cv.amos.V7A1.params1\endcsname{31.0}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.cbs.clause\endcsname{LeanDeepMid minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.30}\,pp, 95\,\% interval \ensuremath{+0.07} to \ensuremath{+0.55}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.cbs.est\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.cbs.hi\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.cbs.lo\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.ctloffset\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.dcv\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.f1\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.f2\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.f3\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.f4\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.hi\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.lo\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.loo.max\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.loo.min\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.share.word\endcsname{fold 4 alone carries 40\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.share_max\endcsname{40}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.span14\endcsname{0.32}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.split\endcsname{LeanDeepMid minus the default is \ensuremath{+0.26}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.03}\,pp, so the margin over the function-identical control is \ensuremath{+0.29}\,pp}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.vsdefault\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.word\endcsname{improves on the control in every fold}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.dcv\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.f1\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.f2\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.f3\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.f4\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.hi\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.lo\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.loo.max\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.loo.min\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.share.word\endcsname{fold 2 alone carries 35\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.share_max\endcsname{35}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.span14\endcsname{0.35}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.dcv\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.f1\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.f2\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.f3\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.f4\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.hi\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.lo\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.loo.max\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.loo.min\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.share.word\endcsname{fold 4 alone carries 78\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.share_max\endcsname{78}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.span14\endcsname{0.96}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.word\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.cv.amos.V7A2.cbs.clause\endcsname{LeanDeepMid+FD minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.amos.V7A2.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7A2.params\endcsname{31.12}
\expandafter\gdef\csname R@an.cv.amos.V7A2.params1\endcsname{31.1}
\expandafter\gdef\csname R@an.cv.amos.V7A2P3c.cbs.clause\endcsname{LeanDeepMid+FD minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.amos.V7A2P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7A2P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7A2P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7A2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7A2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7A2V7A1.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7A2V7A1.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7A2base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7A2base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7B1.cbs.clause\endcsname{LeanSep minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.amos.V7B1.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B1.params\endcsname{20.40}
\expandafter\gdef\csname R@an.cv.amos.V7B1.params1\endcsname{20.4}
\expandafter\gdef\csname R@an.cv.amos.V7B1P3c.cbs.clause\endcsname{LeanSep minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.amos.V7B1P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B1P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B1P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7B1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7B1V5B2.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B1V5B2.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7B1base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B1base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7B2.cbs.clause\endcsname{LeanDil minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.amos.V7B2.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B2.params\endcsname{20.42}
\expandafter\gdef\csname R@an.cv.amos.V7B2.params1\endcsname{20.4}
\expandafter\gdef\csname R@an.cv.amos.V7B2P3c.cbs.clause\endcsname{LeanDil minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.amos.V7B2P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B2P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B2P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7B2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7B2V5B2.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B2V5B2.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7B2base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B2base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7C1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V7C1.cbs.clause\endcsname{LeanNeXt-s5 minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.46}\,pp, 95\,\% interval \ensuremath{-0.68} to \ensuremath{-0.25}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.amos.V7C1.cbs.est\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.cv.amos.V7C1.cbs.hi\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.amos.V7C1.cbs.lo\endcsname{\ensuremath{-0.68}}
\expandafter\gdef\csname R@an.cv.amos.V7C1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V7C1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7C1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7C1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7C1.f1\endcsname{88.54}
\expandafter\gdef\csname R@an.cv.amos.V7C1.f2\endcsname{88.20}
\expandafter\gdef\csname R@an.cv.amos.V7C1.f3\endcsname{88.09}
\expandafter\gdef\csname R@an.cv.amos.V7C1.f4\endcsname{86.72}
\expandafter\gdef\csname R@an.cv.amos.V7C1.mean14\endcsname{87.89}
\expandafter\gdef\csname R@an.cv.amos.V7C1.params\endcsname{21.08}
\expandafter\gdef\csname R@an.cv.amos.V7C1.params1\endcsname{21.1}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.cbs.clause\endcsname{LeanNeXt-s5 minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.43}\,pp, 95\,\% interval \ensuremath{-0.63} to \ensuremath{-0.25}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.cbs.est\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.cbs.hi\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.cbs.lo\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.ctloffset\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.dcv\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.f1\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.f2\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.f3\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.f4\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.hi\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.lo\endcsname{\ensuremath{-0.69}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.loo.max\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.loo.min\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.share.word\endcsname{fold 4 alone carries 37\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.share_max\endcsname{37}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.span14\endcsname{0.40}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.split\endcsname{LeanNeXt-s5 minus the default is \ensuremath{-0.46}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.03}\,pp, so the margin over the function-identical control is \ensuremath{-0.43}\,pp}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.vsdefault\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.word\endcsname{does not improve on it}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.dcv\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.f1\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.f2\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.f3\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.f4\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.hi\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.lo\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.loo.max\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.loo.min\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.share.word\endcsname{fold 4 alone carries 62\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.share_max\endcsname{62}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.span14\endcsname{0.50}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.dcv\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.f1\endcsname{\ensuremath{-0.58}}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.f2\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.f3\endcsname{\ensuremath{-0.71}}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.f4\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.hi\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.lo\endcsname{\ensuremath{-0.81}}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.loo.max\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.loo.min\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.share.word\endcsname{fold 3 alone carries 39\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.share_max\endcsname{39}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.span14\endcsname{0.44}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.V8B2.cbs.clause\endcsname{Stem1 minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.amos.V8B2.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V8B2.params\endcsname{21.07}
\expandafter\gdef\csname R@an.cv.amos.V8B2.params1\endcsname{21.1}
\expandafter\gdef\csname R@an.cv.amos.V8B2P3c.cbs.clause\endcsname{Stem1 minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.amos.V8B2P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V8B2P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V8B2P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V8B2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V8B2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V8B2base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V8B2base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.base.f0\endcsname{87.70}
\expandafter\gdef\csname R@an.cv.amos.base.f1\endcsname{89.12}
\expandafter\gdef\csname R@an.cv.amos.base.f2\endcsname{88.48}
\expandafter\gdef\csname R@an.cv.amos.base.f3\endcsname{88.80}
\expandafter\gdef\csname R@an.cv.amos.base.f4\endcsname{87.00}
\expandafter\gdef\csname R@an.cv.amos.base.max14\endcsname{89.12}
\expandafter\gdef\csname R@an.cv.amos.base.mean14\endcsname{88.35}
\expandafter\gdef\csname R@an.cv.amos.base.mean5\endcsname{88.22}
\expandafter\gdef\csname R@an.cv.amos.base.min14\endcsname{87.00}
\expandafter\gdef\csname R@an.cv.amos.base.params\endcsname{31.12}
\expandafter\gdef\csname R@an.cv.amos.base.params1\endcsname{31.1}
\expandafter\gdef\csname R@an.cv.amos.base.span14\endcsname{2.12}
\expandafter\gdef\csname R@an.cv.amos.base.src0\endcsname{frozen pool}
\expandafter\gdef\csname R@an.cv.amos.base.src0long\endcsname{the frozen default pool}
\expandafter\gdef\csname R@an.cv.amos.base.src0mark\endcsname{a}
\expandafter\gdef\csname R@an.cv.amos.base.src0n\endcsname{6}
\expandafter\gdef\csname R@an.cv.amos.recovery.L3\endcsname{0.56}
\expandafter\gdef\csname R@an.cv.amos.recovery.L3.method\endcsname{the delta method applied to the two four-fold mean margins, HyReX minus the default and ResEnc-M minus the default, which are differences from the same default runs, so their covariance over the folds enters the variance of the ratio; the interval takes the t quantile on three degrees of freedom of the registered paired-t intervals of the margins; it is descriptive, a description of four folds of one seed each and not a test, and it is withheld when ResEnc-M's own interval over the folds includes zero}
\expandafter\gdef\csname R@an.cv.amos.recovery.L3.sentence\endcsname{On AMOS22, HyReX's mean margin over the default on the four folds that entered no decision, \ensuremath{+0.23}\,pp, is 0.56 of ResEnc-M's, \ensuremath{+0.41}\,pp; ResEnc-M's own interval over the folds includes zero, so the ratio is given without an interval}
\expandafter\gdef\csname R@an.cv.amos.recovery.L3.state\endcsname{interval withheld}
\expandafter\gdef\csname R@an.cv.band.acdc.D2base.word\endcsname{\leavevmode\pend}
\expandafter\gdef\csname R@an.cv.band.acdc.L1base.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.band.acdc.L3L1.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.band.acdc.L3base.word\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.band.acdc.hw\endcsname{0.28}
\expandafter\gdef\csname R@an.cv.band.amos.D2base.word\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.band.amos.L1base.word\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.band.amos.L3L1.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.band.amos.L3base.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.band.amos.hw\endcsname{0.35}
\expandafter\gdef\csname R@an.cv.band.kits.D2base.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.band.kits.L1base.word\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.band.kits.L3L1.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.band.kits.L3base.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.band.kits.hw\endcsname{2.25}
\expandafter\gdef\csname R@an.cv.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.cbs.arms\endcsname{L3, L1, D2, P3c, L1b, V5B1, V5B2, V6A1r, V7A1, V7C1, V7B1, V7B2, V7A2, V8B2}
\expandafter\gdef\csname R@an.cv.cbs.label\endcsname{case-level paired bootstrap}
\expandafter\gdef\csname R@an.cv.cbs.method\endcsname{the unit is the validation case of folds 1 to 4 (every case once), the difference of an arm and its reference is averaged over the seeds available for the arm and its reference in the fold, and the interval is the percentile 95\,\% interval of the mean difference over 10000 resamples of the cases with replacement, stratified by fold, with random-number seed 20261011}
\expandafter\gdef\csname R@an.cv.cbs.n\endcsname{54}
\expandafter\gdef\csname R@an.cv.cbs.note\endcsname{the case-level interval carries case-sampling variance and the averaging over the seeds available for the arm and its reference, not the training-seed variance of a one-seed fold}
\expandafter\gdef\csname R@an.cv.cbs.reference\endcsname{the reference of a contrast is the nnU-Net default, or the function-identical rebuild, trained on the same fold (its cross-validation runs, seeds as available), not a pooled reference}
\expandafter\gdef\csname R@an.cv.cbs.registration\endcsname{Addendum AZ2}
\expandafter\gdef\csname R@an.cv.cbs.seed\endcsname{20261011}
\expandafter\gdef\csname R@an.cv.cbs.total\endcsname{78}
\expandafter\gdef\csname R@an.cv.ci.df\endcsname{3}
\expandafter\gdef\csname R@an.cv.ci.level\endcsname{95\,\%}
\expandafter\gdef\csname R@an.cv.claim.breadth.acdc\endcsname{On ACDC the HyReX-minus-default contrast is carried by the cohort and not by a handful of cases}
\expandafter\gdef\csname R@an.cv.claim.breadth.amos\endcsname{On AMOS22 the HyReX-minus-default contrast is carried by the cohort and not by a handful of cases}
\expandafter\gdef\csname R@an.cv.claim.breadth.def\endcsname{more than 50\,\% of the held-out cases improve and the 10 largest gains carry at most 25\,\% of all gains}
\expandafter\gdef\csname R@an.cv.claim.breadth.kits\endcsname{On KiTS23 the HyReX-minus-default contrast is carried by the cohort and not by a handful of cases}
\expandafter\gdef\csname R@an.cv.claim.repro.acdc\endcsname{On ACDC our ResEnc-M five-fold margin reproduces the published margin to within 1.00\,pp}
\expandafter\gdef\csname R@an.cv.claim.repro.amos\endcsname{On AMOS22 our ResEnc-M five-fold margin reproduces the published margin to within 1.00\,pp}
\expandafter\gdef\csname R@an.cv.claim.repro.def\endcsname{the five-fold ResEnc-M margin over the default differs from the published ResEnc-M margin by at most 1.00\,pp, a tolerance that is smaller than the published margin itself (a tolerance that is not would also hold for a margin of zero, and a sentence that holds whatever was measured reproduces nothing)}
\expandafter\gdef\csname R@an.cv.claim.repro.kits\endcsname{On KiTS23 our ResEnc-M five-fold margin reproduces the published margin to within 1.00\,pp}
\expandafter\gdef\csname R@an.cv.ctl.acdc.narms\endcsname{11}
\expandafter\gdef\csname R@an.cv.ctl.acdc.nready\endcsname{7}
\expandafter\gdef\csname R@an.cv.ctl.acdc.nready3\endcsname{0}
\expandafter\gdef\csname R@an.cv.ctl.amos.narms\endcsname{11}
\expandafter\gdef\csname R@an.cv.ctl.amos.nready\endcsname{7}
\expandafter\gdef\csname R@an.cv.ctl.amos.nready3\endcsname{0}
\expandafter\gdef\csname R@an.cv.ctl.kits.narms\endcsname{11}
\expandafter\gdef\csname R@an.cv.ctl.kits.nready\endcsname{7}
\expandafter\gdef\csname R@an.cv.ctl.kits.nready3\endcsname{0}
\expandafter\gdef\csname R@an.cv.ctl.label\endcsname{margin over the function-identical control}
\expandafter\gdef\csname R@an.cv.ctl.n\endcsname{11}
\expandafter\gdef\csname R@an.cv.ctl.names\endcsname{ResEnc-M, LeanDec, LeanAdd, LeanAdd-NeXt, HyReX-k9, LeanDeepMid, LeanNeXt-s5, LeanSep, LeanDil, LeanDeepMid+FD and Stem1}
\expandafter\gdef\csname R@an.cv.ctl.registration\endcsname{Addendum AV}
\expandafter\gdef\csname R@an.cv.ctl.seeds.n\endcsname{0}
\expandafter\gdef\csname R@an.cv.ctl.seeds.sentence\endcsname{the control's seed-1 and seed-2 runs of the cross-validation folds: none of the 24 have finished, so the secondary reading is pending}
\expandafter\gdef\csname R@an.cv.ctl.seeds.state\endcsname{pending}
\expandafter\gdef\csname R@an.cv.ctl.seeds.total\endcsname{24}
\expandafter\gdef\csname R@an.cv.ctl.tags\endcsname{L1, D2, V5B1, V5B2, V6A1r, V7A1, V7C1, V7B1, V7B2, V7A2, V8B2}
\expandafter\gdef\csname R@an.cv.cvseeds\endcsname{one}
\expandafter\gdef\csname R@an.cv.cvseeds.phrase\endcsname{one seed per arm}
\expandafter\gdef\csname R@an.cv.d5.src0\endcsname{AMOS22 HyReX fresh s1-2 (b); AMOS22 default frozen pool (a); AMOS22 ResEnc-M fresh s1-2 (b); AMOS22 LeanDec seed 0 (c); KiTS23 HyReX fresh s1-2 (b); KiTS23 default frozen pool (a); KiTS23 ResEnc-M fresh s1-2 (b); KiTS23 LeanDec fresh s1-2 (b); ACDC HyReX fresh s1-2 (b); ACDC default frozen pool (a); ACDC ResEnc-M fresh s1-2 (b)}
\expandafter\gdef\csname R@an.cv.d5.src0note\endcsname{the five-fold means published here do NOT all take their fold-0 fifth from the same estimand: fifth, so their fold-0 LeanDec enters from seed 0 on AMOS22, fresh s1-2 on KiTS23s are not like-for-like across datasets}
\expandafter\gdef\csname R@an.cv.decomp.acdc.clause\endcsname{On ACDC, HyReX minus the default is \ensuremath{+0.33}\,pp (95\,\% over folds \ensuremath{+0.10} to \ensuremath{+0.56}, which lies above zero; improves in every fold), and splits into the control's own offset, the function-identical control minus the default, of \ensuremath{-0.08}\,pp (95\,\% over folds \ensuremath{-0.22} to \ensuremath{+0.06}, which lies inside $\pm$0.50\,pp; does not improve in cross-validation) and a design margin over the control, HyReX minus the function-identical control, of \ensuremath{+0.41}\,pp (95\,\% over folds \ensuremath{+0.06} to \ensuremath{+0.76}, which lies above zero; improves in every fold); the two parts add to the registered contrast in every fold}
\expandafter\gdef\csname R@an.cv.decomp.acdc.done\endcsname{4}
\expandafter\gdef\csname R@an.cv.decomp.acdc.everyfold\endcsname{positive in every fold: HyReX minus the default and the design margin over the control}
\expandafter\gdef\csname R@an.cv.decomp.acdc.short\endcsname{ACDC: HyReX minus the default is \ensuremath{+0.33}\,pp and splits into the control's offset of \ensuremath{-0.08}\,pp and a design margin of \ensuremath{+0.41}\,pp}
\expandafter\gdef\csname R@an.cv.decomp.acdc.state\endcsname{complete}
\expandafter\gdef\csname R@an.cv.decomp.amos.clause\endcsname{On AMOS22, HyReX minus the default is \ensuremath{+0.23}\,pp (95\,\% over folds \ensuremath{-0.08} to \ensuremath{+0.54}, which includes zero; improves on average (3/4 folds)), and splits into the control's own offset, the function-identical control minus the default, of \ensuremath{-0.03}\,pp (95\,\% over folds \ensuremath{-0.57} to \ensuremath{+0.51}, which includes zero; does not improve in cross-validation) and a design margin over the control, HyReX minus the function-identical control, of \ensuremath{+0.26}\,pp (95\,\% over folds \ensuremath{-0.03} to \ensuremath{+0.55}, which reaches just below zero; improves in every fold); the two parts add to the registered contrast in every fold}
\expandafter\gdef\csname R@an.cv.decomp.amos.done\endcsname{4}
\expandafter\gdef\csname R@an.cv.decomp.amos.everyfold\endcsname{positive in every fold: the design margin over the control}
\expandafter\gdef\csname R@an.cv.decomp.amos.short\endcsname{AMOS22: HyReX minus the default is \ensuremath{+0.23}\,pp and splits into the control's offset of \ensuremath{-0.03}\,pp and a design margin of \ensuremath{+0.26}\,pp}
\expandafter\gdef\csname R@an.cv.decomp.amos.state\endcsname{complete}
\expandafter\gdef\csname R@an.cv.decomp.kits.clause\endcsname{On KiTS23, HyReX minus the default is \ensuremath{+0.68}\,pp (95\,\% over folds \ensuremath{-1.08} to \ensuremath{+2.44}, which includes zero; improves on average (3/4 folds)), and splits into the control's own offset, the function-identical control minus the default, of \ensuremath{+0.56}\,pp (95\,\% over folds \ensuremath{-1.71} to \ensuremath{+2.82}, which includes zero; improves on average (3/4 folds)) and a design margin over the control, HyReX minus the function-identical control, of \ensuremath{+0.12}\,pp (95\,\% over folds \ensuremath{-0.73} to \ensuremath{+0.98}, which includes zero; improves on average (2/4 folds)); the two parts add to the registered contrast in every fold}
\expandafter\gdef\csname R@an.cv.decomp.kits.done\endcsname{4}
\expandafter\gdef\csname R@an.cv.decomp.kits.everyfold\endcsname{none of the three differences is positive in every fold}
\expandafter\gdef\csname R@an.cv.decomp.kits.short\endcsname{KiTS23: HyReX minus the default is \ensuremath{+0.68}\,pp and splits into the control's offset of \ensuremath{+0.56}\,pp and a design margin of \ensuremath{+0.12}\,pp}
\expandafter\gdef\csname R@an.cv.decomp.kits.state\endcsname{complete}
\expandafter\gdef\csname R@an.cv.decomp.refnote\endcsname{The registered contrast and both of its parts are differences of two runs trained and scored on the same cases of the same fold, so no frozen default pool and no sensitivity reference enters them}
\expandafter\gdef\csname R@an.cv.decompre.acdc.clause\endcsname{On ACDC, ResEnc-M minus HyReX is \ensuremath{+0.04}\,pp (95\,\% over folds \ensuremath{-0.24} to \ensuremath{+0.31}, which lies inside $\pm$0.50\,pp; improves on average (2/4 folds)), and splits into a re-implementation difference, ResEnc-M minus the ResEnc-matched re-implementation, of \ensuremath{+0.18}\,pp (95\,\% over folds \ensuremath{+0.02} to \ensuremath{+0.33}, which lies inside $\pm$0.50\,pp and above zero; improves in every fold) and a like-for-like part, the ResEnc-matched re-implementation minus HyReX, of \ensuremath{-0.14}\,pp (95\,\% over folds \ensuremath{-0.27} to \ensuremath{-0.01}, which lies inside $\pm$0.50\,pp and below zero; does not improve in cross-validation); the two parts add to the registered contrast in every fold}
\expandafter\gdef\csname R@an.cv.decompre.acdc.done\endcsname{4}
\expandafter\gdef\csname R@an.cv.decompre.acdc.short\endcsname{ACDC: ResEnc-M minus HyReX is \ensuremath{+0.04}\,pp and splits into a re-implementation difference of \ensuremath{+0.18}\,pp and a like-for-like part of \ensuremath{-0.14}\,pp}
\expandafter\gdef\csname R@an.cv.decompre.acdc.state\endcsname{complete}
\expandafter\gdef\csname R@an.cv.decompre.amos.clause\endcsname{On AMOS22, ResEnc-M minus HyReX is \ensuremath{+0.18}\,pp (95\,\% over folds \ensuremath{-0.40} to \ensuremath{+0.76}, which includes zero; improves on average (3/4 folds)), and splits into a re-implementation difference, ResEnc-M minus the ResEnc-matched re-implementation, of \ensuremath{-0.02}\,pp (95\,\% over folds \ensuremath{-0.28} to \ensuremath{+0.24}, which lies inside $\pm$0.50\,pp; does not improve in cross-validation) and a like-for-like part, the ResEnc-matched re-implementation minus HyReX, of \ensuremath{+0.20}\,pp (95\,\% over folds \ensuremath{-0.38} to \ensuremath{+0.78}, which includes zero; improves on average (3/4 folds)); the two parts add to the registered contrast in every fold}
\expandafter\gdef\csname R@an.cv.decompre.amos.done\endcsname{4}
\expandafter\gdef\csname R@an.cv.decompre.amos.short\endcsname{AMOS22: ResEnc-M minus HyReX is \ensuremath{+0.18}\,pp and splits into a re-implementation difference of \ensuremath{-0.02}\,pp and a like-for-like part of \ensuremath{+0.20}\,pp}
\expandafter\gdef\csname R@an.cv.decompre.amos.state\endcsname{complete}
\expandafter\gdef\csname R@an.cv.decompre.kits.clause\endcsname{On KiTS23, ResEnc-M minus HyReX is \ensuremath{+1.47}\,pp (95\,\% over folds \ensuremath{-0.24} to \ensuremath{+3.17}, which includes zero; improves in every fold), and splits into a re-implementation difference, ResEnc-M minus the ResEnc-matched re-implementation, of \ensuremath{+0.60}\,pp (95\,\% over folds \ensuremath{-0.45} to \ensuremath{+1.66}, which includes zero; improves on average (3/4 folds)) and a like-for-like part, the ResEnc-matched re-implementation minus HyReX, of \ensuremath{+0.86}\,pp (95\,\% over folds \ensuremath{-0.10} to \ensuremath{+1.82}, which includes zero; improves in every fold); the two parts add to the registered contrast in every fold}
\expandafter\gdef\csname R@an.cv.decompre.kits.done\endcsname{4}
\expandafter\gdef\csname R@an.cv.decompre.kits.short\endcsname{KiTS23: ResEnc-M minus HyReX is \ensuremath{+1.47}\,pp and splits into a re-implementation difference of \ensuremath{+0.60}\,pp and a like-for-like part of \ensuremath{+0.86}\,pp}
\expandafter\gdef\csname R@an.cv.decompre.kits.state\endcsname{complete}
\expandafter\gdef\csname R@an.cv.decompre.refnote\endcsname{The registered contrast and both of its parts are differences of two runs trained and scored on the same cases of the same fold, so no frozen default pool and no sensitivity reference enters them}
\expandafter\gdef\csname R@an.cv.decompre.why\endcsname{ResEnc-M is the stock library network and HyReX is a plan-aware build, and the ResEnc-matched re-implementation (built through the plan-aware path; it differs from the library preset in the default stem, the shortcut form and the zero-initialisation) splits their registered contrast into a re-implementation difference, ResEnc-M minus the re-implementation, and a like-for-like part, the re-implementation minus HyReX}
\expandafter\gdef\csname R@an.cv.fold.fifth\endcsname{fifth}
\expandafter\gdef\csname R@an.cv.fold0.share\endcsname{one fifth}
\expandafter\gdef\csname R@an.cv.gate.sent1\endcsname{writable today: all 14 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent10\endcsname{writable today: all 7 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent11\endcsname{writable today: all 8 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent12\endcsname{writable today: all 5 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent13\endcsname{writable today: all 3 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent14\endcsname{writable today: all 1 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent2\endcsname{writable today: all 5 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent3\endcsname{writable today: all 6 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent4\endcsname{writable today: all 6 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent5\endcsname{writable today: all 16 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent6\endcsname{writable today: all 4 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent6c\endcsname{writable today: all 1 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent7\endcsname{writable today: all 6 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent8\endcsname{writable today: all 8 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent9\endcsname{writable today: all 8 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sentTfolds\endcsname{writable today: all 4 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sentToof\endcsname{writable today: all 1 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sentTp3c\endcsname{writable today: all 4 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sentTpositioning\endcsname{writable today: all 6 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sentTrobust\endcsname{writable today: all 6 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.summary\endcsname{20 of the 20 proposed sentences of the cv note are writable today (sentence 1, sentence 2, sentence 3, sentence 4, sentence 5, sentence 6, sentence 6c, sentence 7, sentence 8, sentence 9, sentence 10, sentence 11, sentence 12, sentence 13, sentence 14, takeaway folds, takeaway oof, takeaway p3c, takeaway positioning, takeaway robust)}
\expandafter\gdef\csname R@an.cv.hetero.acdc.D2base.casese\endcsname{0.13}
\expandafter\gdef\csname R@an.cv.hetero.acdc.D2base.ratio\endcsname{0.18}
\expandafter\gdef\csname R@an.cv.hetero.acdc.D2base.sdfold\endcsname{0.08}
\expandafter\gdef\csname R@an.cv.hetero.acdc.D2base.seedexp\endcsname{0.14}
\expandafter\gdef\csname R@an.cv.hetero.acdc.D2base.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L1base.casese\endcsname{0.18}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L1base.ratio\endcsname{0.09}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L1base.sdfold\endcsname{0.07}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L1base.seedexp\endcsname{0.14}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L1base.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3L1.casese\endcsname{0.15}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3L1.ratio\endcsname{0.72}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3L1.sdfold\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3L1.seedexp\endcsname{0.14}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3L1.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3base.casese\endcsname{0.15}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3base.ratio\endcsname{0.50}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3base.sdfold\endcsname{0.14}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3base.seedexp\endcsname{0.14}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3base.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.amos.D2base.casese\endcsname{0.14}
\expandafter\gdef\csname R@an.cv.hetero.amos.D2base.ratio\endcsname{0.77}
\expandafter\gdef\csname R@an.cv.hetero.amos.D2base.sdfold\endcsname{0.20}
\expandafter\gdef\csname R@an.cv.hetero.amos.D2base.seedexp\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.hetero.amos.D2base.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.amos.L1base.casese\endcsname{0.16}
\expandafter\gdef\csname R@an.cv.hetero.amos.L1base.ratio\endcsname{3.24}
\expandafter\gdef\csname R@an.cv.hetero.amos.L1base.sdfold\endcsname{0.43}
\expandafter\gdef\csname R@an.cv.hetero.amos.L1base.seedexp\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.hetero.amos.L1base.verdict\endcsname{adds spread beyond one seed per arm and case sampling}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3L1.casese\endcsname{0.14}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3L1.ratio\endcsname{2.63}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3L1.sdfold\endcsname{0.36}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3L1.seedexp\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3L1.verdict\endcsname{adds spread beyond one seed per arm and case sampling}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3base.casese\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3base.ratio\endcsname{0.62}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3base.sdfold\endcsname{0.19}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3base.seedexp\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3base.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.kits.D2base.casese\endcsname{0.74}
\expandafter\gdef\csname R@an.cv.hetero.kits.D2base.ratio\endcsname{0.25}
\expandafter\gdef\csname R@an.cv.hetero.kits.D2base.sdfold\endcsname{0.68}
\expandafter\gdef\csname R@an.cv.hetero.kits.D2base.seedexp\endcsname{1.12}
\expandafter\gdef\csname R@an.cv.hetero.kits.D2base.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.kits.L1base.casese\endcsname{0.86}
\expandafter\gdef\csname R@an.cv.hetero.kits.L1base.ratio\endcsname{0.27}
\expandafter\gdef\csname R@an.cv.hetero.kits.L1base.sdfold\endcsname{0.74}
\expandafter\gdef\csname R@an.cv.hetero.kits.L1base.seedexp\endcsname{1.12}
\expandafter\gdef\csname R@an.cv.hetero.kits.L1base.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3L1.casese\endcsname{0.90}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3L1.ratio\endcsname{0.55}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3L1.sdfold\endcsname{1.07}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3L1.seedexp\endcsname{1.12}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3L1.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3base.casese\endcsname{0.84}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3base.ratio\endcsname{0.62}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3base.sdfold\endcsname{1.11}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3base.seedexp\endcsname{1.12}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3base.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.premise\endcsname{$\sqrt{2}\times$ the training-seed SD of that dataset's frozen DEFAULT pool, applied to each arm of the contrast: the frozen default pool is the registered source of a training-seed SD, so the same expectation is used for every contrast of a dataset, HyReX $-$ ResEnc-M included, where neither arm is the default}
\expandafter\gdef\csname R@an.cv.kfold\endcsname{five-fold}
\expandafter\gdef\csname R@an.cv.kits.D2.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.D2.cbs.clause\endcsname{LeanDec minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+1.05}\,pp, 95\,\% interval \ensuremath{+0.32} to \ensuremath{+1.79}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.kits.D2.cbs.est\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.cv.kits.D2.cbs.hi\endcsname{\ensuremath{+1.79}}
\expandafter\gdef\csname R@an.cv.kits.D2.cbs.lo\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.cv.kits.D2.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.D2.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.D2.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.D2.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.D2.f0\endcsname{85.27}
\expandafter\gdef\csname R@an.cv.kits.D2.f1\endcsname{84.58}
\expandafter\gdef\csname R@an.cv.kits.D2.f2\endcsname{84.62}
\expandafter\gdef\csname R@an.cv.kits.D2.f3\endcsname{87.94}
\expandafter\gdef\csname R@an.cv.kits.D2.f4\endcsname{83.01}
\expandafter\gdef\csname R@an.cv.kits.D2.max14\endcsname{87.94}
\expandafter\gdef\csname R@an.cv.kits.D2.mean14\endcsname{85.04}
\expandafter\gdef\csname R@an.cv.kits.D2.mean5\endcsname{85.08}
\expandafter\gdef\csname R@an.cv.kits.D2.min14\endcsname{83.01}
\expandafter\gdef\csname R@an.cv.kits.D2.params\endcsname{26.08}
\expandafter\gdef\csname R@an.cv.kits.D2.params1\endcsname{26.1}
\expandafter\gdef\csname R@an.cv.kits.D2.span14\endcsname{4.93}
\expandafter\gdef\csname R@an.cv.kits.D2.src0\endcsname{fresh s1-2}
\expandafter\gdef\csname R@an.cv.kits.D2.src0long\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.cv.kits.D2.src0mark\endcsname{b}
\expandafter\gdef\csname R@an.cv.kits.D2.src0n\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.cbs.clause\endcsname{LeanDec minus the function-identical control, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.48}\,pp, 95\,\% interval \ensuremath{-0.33} to \ensuremath{+1.29}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.cbs.est\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.cbs.hi\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.cbs.lo\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.ctloffset\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.dcv\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.f1\endcsname{\ensuremath{-0.67}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.f2\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.f3\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.f4\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.hi\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.lo\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.loo.max\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.loo.min\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.share.word\endcsname{fold 2 alone carries 62\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.share_max\endcsname{62}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.span14\endcsname{1.88}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.split\endcsname{LeanDec minus the default is \ensuremath{+1.04}\,pp over the four folds; the control's own offset from the default is \ensuremath{+0.56}\,pp, so the margin over the function-identical control is \ensuremath{+0.49}\,pp}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.vsdefault\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.word\endcsname{improves on it on average (3 of 4 folds)}
\expandafter\gdef\csname R@an.cv.kits.D2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.D2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.D2base.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.kits.D2base.boot.casewidth\endcsname{1.40}
\expandafter\gdef\csname R@an.cv.kits.D2base.boot.foldwidth\endcsname{2.15}
\expandafter\gdef\csname R@an.cv.kits.D2base.boot.hi\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.cv.kits.D2base.boot.lo\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.kits.D2base.boot.mean\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.cv.kits.D2base.boot.n\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.D2base.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.kits.D2base.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.36} to \ensuremath{+1.76}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.kits.D2base.d5\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.cv.kits.D2base.d5alt\endcsname{\ensuremath{+1.16}}
\expandafter\gdef\csname R@an.cv.kits.D2base.dcv\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@an.cv.kits.D2base.f0\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.cv.kits.D2base.f0alt\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.cv.kits.D2base.f0band\endcsname{1.45}
\expandafter\gdef\csname R@an.cv.kits.D2base.f0band.note\endcsname{two null SDs of this fold-0 difference, each the frozen default pool's training-seed SD of 0.795\,pp times $\sqrt{1/2 + 1/3}$ for the mean of two runs against the mean of the three-run pool: a locating band, not a test}
\expandafter\gdef\csname R@an.cv.kits.D2base.f0bandword\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.kits.D2base.f0gap\endcsname{1.89}
\expandafter\gdef\csname R@an.cv.kits.D2base.f0rev\endcsname{\ensuremath{-1.89}}
\expandafter\gdef\csname R@an.cv.kits.D2base.f0se\endcsname{0.726}
\expandafter\gdef\csname R@an.cv.kits.D2base.f1\endcsname{\ensuremath{+1.72}}
\expandafter\gdef\csname R@an.cv.kits.D2base.f2\endcsname{\ensuremath{+1.31}}
\expandafter\gdef\csname R@an.cv.kits.D2base.f3\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.cv.kits.D2base.f4\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.kits.D2base.hi\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.cv.kits.D2base.lo\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.kits.D2base.loo.max\endcsname{\ensuremath{+1.35}}
\expandafter\gdef\csname R@an.cv.kits.D2base.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.D2base.loo.min\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.cv.kits.D2base.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.D2base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.D2base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.D2base.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.D2base.share.word\endcsname{fold 1 alone carries 41\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.D2base.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.D2base.share_max\endcsname{41}
\expandafter\gdef\csname R@an.cv.kits.D2base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.D2base.span14\endcsname{1.60}
\expandafter\gdef\csname R@an.cv.kits.D2base.src0\endcsname{fresh s1-2 for LeanDec and frozen pool for default}
\expandafter\gdef\csname R@an.cv.kits.D2base.src0mark\endcsname{b/a}
\expandafter\gdef\csname R@an.cv.kits.D2base.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.kits.L1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.L1.cbs.clause\endcsname{ResEnc-M minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+2.15}\,pp, 95\,\% interval \ensuremath{+1.28} to \ensuremath{+3.06}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.kits.L1.cbs.est\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.cv.kits.L1.cbs.hi\endcsname{\ensuremath{+3.06}}
\expandafter\gdef\csname R@an.cv.kits.L1.cbs.lo\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.cv.kits.L1.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.L1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.L1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L1.f0\endcsname{86.85}
\expandafter\gdef\csname R@an.cv.kits.L1.f1\endcsname{85.44}
\expandafter\gdef\csname R@an.cv.kits.L1.f2\endcsname{86.25}
\expandafter\gdef\csname R@an.cv.kits.L1.f3\endcsname{88.27}
\expandafter\gdef\csname R@an.cv.kits.L1.f4\endcsname{84.60}
\expandafter\gdef\csname R@an.cv.kits.L1.max14\endcsname{88.27}
\expandafter\gdef\csname R@an.cv.kits.L1.mean14\endcsname{86.14}
\expandafter\gdef\csname R@an.cv.kits.L1.mean5\endcsname{86.28}
\expandafter\gdef\csname R@an.cv.kits.L1.min14\endcsname{84.60}
\expandafter\gdef\csname R@an.cv.kits.L1.params\endcsname{102.35}
\expandafter\gdef\csname R@an.cv.kits.L1.params1\endcsname{102.4}
\expandafter\gdef\csname R@an.cv.kits.L1.span14\endcsname{3.66}
\expandafter\gdef\csname R@an.cv.kits.L1.src0\endcsname{fresh s1-2}
\expandafter\gdef\csname R@an.cv.kits.L1.src0long\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.cv.kits.L1.src0mark\endcsname{b}
\expandafter\gdef\csname R@an.cv.kits.L1.src0n\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.dcv\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.f1\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.f2\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.f3\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.f4\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.hi\endcsname{\ensuremath{+1.66}}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.lo\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.loo.max\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.loo.min\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.share.word\endcsname{fold 2 alone carries 53\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.share_max\endcsname{53}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.span14\endcsname{1.41}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.kits.L1L3.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.kits.L1L3.boot.casewidth\endcsname{1.84}
\expandafter\gdef\csname R@an.cv.kits.L1L3.boot.foldwidth\endcsname{3.41}
\expandafter\gdef\csname R@an.cv.kits.L1L3.boot.hi\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.boot.lo\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.boot.mean\endcsname{\ensuremath{+1.46}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.boot.n\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.L1L3.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.kits.L1L3.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.52} to \ensuremath{+2.36}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.kits.L1L3.dcv\endcsname{\ensuremath{+1.47}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.f1\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.f2\endcsname{\ensuremath{+2.74}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.f3\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.f4\endcsname{\ensuremath{+1.87}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.hi\endcsname{\ensuremath{+3.17}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.lo\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.loo.max\endcsname{\ensuremath{+1.86}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L1L3.loo.min\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1L3.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L1L3.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.L1L3.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L1L3.share.word\endcsname{fold 2 alone carries 47\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.L1L3.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1L3.share_max\endcsname{47}
\expandafter\gdef\csname R@an.cv.kits.L1L3.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.L1L3.span14\endcsname{2.47}
\expandafter\gdef\csname R@an.cv.kits.L1L3.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.cbs.clause\endcsname{ResEnc-M minus the function-identical control, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+1.59}\,pp, 95\,\% interval \ensuremath{+0.68} to \ensuremath{+2.52}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.cbs.est\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.cbs.hi\endcsname{\ensuremath{+2.52}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.cbs.lo\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.ctloffset\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.dcv\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.f1\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.f2\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.f3\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.f4\endcsname{\ensuremath{+2.73}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.hi\endcsname{\ensuremath{+3.80}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.lo\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.loo.max\endcsname{\ensuremath{+2.05}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.loo.min\endcsname{\ensuremath{+1.17}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.share.word\endcsname{fold 2 alone carries 45\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.share_max\endcsname{45}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.span14\endcsname{2.64}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.split\endcsname{ResEnc-M minus the default is \ensuremath{+2.15}\,pp over the four folds; the control's own offset from the default is \ensuremath{+0.56}\,pp, so the margin over the function-identical control is \ensuremath{+1.59}\,pp}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.vsdefault\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.word\endcsname{improves on the control in every fold}
\expandafter\gdef\csname R@an.cv.kits.L1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.L1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.L1b.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.L1b.cbs.clause\endcsname{ResEnc-matched minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+1.55}\,pp, 95\,\% interval \ensuremath{+0.66} to \ensuremath{+2.42}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.kits.L1b.cbs.est\endcsname{\ensuremath{+1.55}}
\expandafter\gdef\csname R@an.cv.kits.L1b.cbs.hi\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.cv.kits.L1b.cbs.lo\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.cv.kits.L1b.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.L1b.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.L1b.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L1b.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L1b.f1\endcsname{85.21}
\expandafter\gdef\csname R@an.cv.kits.L1b.f2\endcsname{84.96}
\expandafter\gdef\csname R@an.cv.kits.L1b.f3\endcsname{88.40}
\expandafter\gdef\csname R@an.cv.kits.L1b.f4\endcsname{83.58}
\expandafter\gdef\csname R@an.cv.kits.L1b.mean14\endcsname{85.54}
\expandafter\gdef\csname R@an.cv.kits.L1b.params\endcsname{102.43}
\expandafter\gdef\csname R@an.cv.kits.L1b.params1\endcsname{102.4}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.dcv\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.f1\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.f2\endcsname{\ensuremath{+1.46}}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.f3\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.f4\endcsname{\ensuremath{+0.84}}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.hi\endcsname{\ensuremath{+1.82}}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.lo\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.loo.max\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.loo.min\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.share.word\endcsname{fold 2 alone carries 42\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.share_max\endcsname{42}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.span14\endcsname{1.41}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.kits.L1base.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.kits.L1base.boot.casewidth\endcsname{1.80}
\expandafter\gdef\csname R@an.cv.kits.L1base.boot.foldwidth\endcsname{2.34}
\expandafter\gdef\csname R@an.cv.kits.L1base.boot.hi\endcsname{\ensuremath{+3.08}}
\expandafter\gdef\csname R@an.cv.kits.L1base.boot.lo\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.cv.kits.L1base.boot.mean\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.cv.kits.L1base.boot.n\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.L1base.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.kits.L1base.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+1.28} to \ensuremath{+3.08}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.kits.L1base.d5\endcsname{\ensuremath{+2.41}}
\expandafter\gdef\csname R@an.cv.kits.L1base.d5alt\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.cv.kits.L1base.dcv\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.cv.kits.L1base.f0\endcsname{\ensuremath{+3.48}}
\expandafter\gdef\csname R@an.cv.kits.L1base.f0alt\endcsname{\ensuremath{+3.23}}
\expandafter\gdef\csname R@an.cv.kits.L1base.f0band\endcsname{1.45}
\expandafter\gdef\csname R@an.cv.kits.L1base.f0band.note\endcsname{two null SDs of this fold-0 difference, each the frozen default pool's training-seed SD of 0.795\,pp times $\sqrt{1/2 + 1/3}$ for the mean of two runs against the mean of the three-run pool: a locating band, not a test}
\expandafter\gdef\csname R@an.cv.kits.L1base.f0bandword\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.kits.L1base.f0gap\endcsname{3.48}
\expandafter\gdef\csname R@an.cv.kits.L1base.f0rev\endcsname{\ensuremath{-3.48}}
\expandafter\gdef\csname R@an.cv.kits.L1base.f0se\endcsname{0.726}
\expandafter\gdef\csname R@an.cv.kits.L1base.f1\endcsname{\ensuremath{+2.58}}
\expandafter\gdef\csname R@an.cv.kits.L1base.f2\endcsname{\ensuremath{+2.94}}
\expandafter\gdef\csname R@an.cv.kits.L1base.f3\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.cv.kits.L1base.f4\endcsname{\ensuremath{+1.71}}
\expandafter\gdef\csname R@an.cv.kits.L1base.hi\endcsname{\ensuremath{+3.32}}
\expandafter\gdef\csname R@an.cv.kits.L1base.lo\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.cv.kits.L1base.loo.max\endcsname{\ensuremath{+2.41}}
\expandafter\gdef\csname R@an.cv.kits.L1base.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.kits.L1base.loo.min\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@an.cv.kits.L1base.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L1base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.L1base.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L1base.share.word\endcsname{fold 2 alone carries 34\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.L1base.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1base.share_max\endcsname{34}
\expandafter\gdef\csname R@an.cv.kits.L1base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.L1base.span14\endcsname{1.58}
\expandafter\gdef\csname R@an.cv.kits.L1base.src0\endcsname{fresh s1-2 for ResEnc-M and frozen pool for default}
\expandafter\gdef\csname R@an.cv.kits.L1base.src0mark\endcsname{b/a}
\expandafter\gdef\csname R@an.cv.kits.L1base.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.kits.L3.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.L3.cbs.clause\endcsname{HyReX minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.68}\,pp, 95\,\% interval \ensuremath{-0.16} to \ensuremath{+1.55}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.kits.L3.cbs.est\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.cv.kits.L3.cbs.hi\endcsname{\ensuremath{+1.55}}
\expandafter\gdef\csname R@an.cv.kits.L3.cbs.lo\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.cv.kits.L3.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.L3.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.L3.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L3.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L3.f0\endcsname{85.47}
\expandafter\gdef\csname R@an.cv.kits.L3.f1\endcsname{85.17}
\expandafter\gdef\csname R@an.cv.kits.L3.f2\endcsname{83.51}
\expandafter\gdef\csname R@an.cv.kits.L3.f3\endcsname{87.29}
\expandafter\gdef\csname R@an.cv.kits.L3.f4\endcsname{82.74}
\expandafter\gdef\csname R@an.cv.kits.L3.max14\endcsname{87.29}
\expandafter\gdef\csname R@an.cv.kits.L3.mean14\endcsname{84.67}
\expandafter\gdef\csname R@an.cv.kits.L3.mean5\endcsname{84.83}
\expandafter\gdef\csname R@an.cv.kits.L3.min14\endcsname{82.74}
\expandafter\gdef\csname R@an.cv.kits.L3.params\endcsname{29.66}
\expandafter\gdef\csname R@an.cv.kits.L3.params1\endcsname{29.7}
\expandafter\gdef\csname R@an.cv.kits.L3.span14\endcsname{4.55}
\expandafter\gdef\csname R@an.cv.kits.L3.src0\endcsname{fresh s1-2}
\expandafter\gdef\csname R@an.cv.kits.L3.src0long\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.cv.kits.L3.src0mark\endcsname{b}
\expandafter\gdef\csname R@an.cv.kits.L3.src0n\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L3L1.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.kits.L3L1.boot.casewidth\endcsname{1.82}
\expandafter\gdef\csname R@an.cv.kits.L3L1.boot.foldwidth\endcsname{3.41}
\expandafter\gdef\csname R@an.cv.kits.L3L1.boot.hi\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.boot.lo\endcsname{\ensuremath{-2.42}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.boot.mean\endcsname{\ensuremath{-1.46}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.boot.n\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.L3L1.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.kits.L3L1.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-2.42} to \ensuremath{-0.59}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.kits.L3L1.d5\endcsname{\ensuremath{-1.45}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.dcv\endcsname{\ensuremath{-1.47}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.f0\endcsname{\ensuremath{-1.38}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.f0gap\endcsname{1.38}
\expandafter\gdef\csname R@an.cv.kits.L3L1.f0lead\endcsname{ResEnc-M is ahead of HyReX}
\expandafter\gdef\csname R@an.cv.kits.L3L1.f0rev\endcsname{\ensuremath{+1.38}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.f1\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.f2\endcsname{\ensuremath{-2.74}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.f3\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.f4\endcsname{\ensuremath{-1.87}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.hi\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.lo\endcsname{\ensuremath{-3.17}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.loo.max\endcsname{\ensuremath{-1.04}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L3L1.loo.min\endcsname{\ensuremath{-1.86}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L3L1.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.L3L1.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.L3L1.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.L3L1.share.word\endcsname{fold 2 alone carries 47\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.kits.L3L1.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L3L1.share_max\endcsname{47}
\expandafter\gdef\csname R@an.cv.kits.L3L1.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.kits.L3L1.span14\endcsname{2.47}
\expandafter\gdef\csname R@an.cv.kits.L3L1.src0\endcsname{fresh s1-2 for HyReX and for ResEnc-M}
\expandafter\gdef\csname R@an.cv.kits.L3L1.src0mark\endcsname{b/b}
\expandafter\gdef\csname R@an.cv.kits.L3L1.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.kits.L3L1.wordrev\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.cbs.clause\endcsname{HyReX minus the function-identical control, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.12}\,pp, 95\,\% interval \ensuremath{-0.70} to \ensuremath{+0.96}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.cbs.est\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.cbs.hi\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.cbs.lo\endcsname{\ensuremath{-0.70}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.dcv\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.f1\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.f2\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.f3\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.f4\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.hi\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.lo\endcsname{\ensuremath{-0.73}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.loo.max\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.loo.min\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.loo.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.loo.word\endcsname{changes sign when a single fold is dropped (three of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.share.word\endcsname{fold 4 alone carries 175\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.share_max\endcsname{175}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.span14\endcsname{1.26}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.word\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.cv.kits.L3base.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.kits.L3base.boot.casewidth\endcsname{1.69}
\expandafter\gdef\csname R@an.cv.kits.L3base.boot.foldwidth\endcsname{3.52}
\expandafter\gdef\csname R@an.cv.kits.L3base.boot.hi\endcsname{\ensuremath{+1.54}}
\expandafter\gdef\csname R@an.cv.kits.L3base.boot.lo\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.cv.kits.L3base.boot.mean\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.cv.kits.L3base.boot.n\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.L3base.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.kits.L3base.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.16} to \ensuremath{+1.54}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.kits.L3base.d5\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@an.cv.kits.L3base.d5alt\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.cv.kits.L3base.dcv\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.cv.kits.L3base.f0\endcsname{\ensuremath{+2.09}}
\expandafter\gdef\csname R@an.cv.kits.L3base.f0alt\endcsname{\ensuremath{+1.85}}
\expandafter\gdef\csname R@an.cv.kits.L3base.f0band\endcsname{1.45}
\expandafter\gdef\csname R@an.cv.kits.L3base.f0band.note\endcsname{two null SDs of this fold-0 difference, each the frozen default pool's training-seed SD of 0.795\,pp times $\sqrt{1/2 + 1/3}$ for the mean of two runs against the mean of the three-run pool: a locating band, not a test}
\expandafter\gdef\csname R@an.cv.kits.L3base.f0bandword\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.kits.L3base.f0gap\endcsname{2.09}
\expandafter\gdef\csname R@an.cv.kits.L3base.f0rev\endcsname{\ensuremath{-2.09}}
\expandafter\gdef\csname R@an.cv.kits.L3base.f0se\endcsname{0.726}
\expandafter\gdef\csname R@an.cv.kits.L3base.f1\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.cv.kits.L3base.f2\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.kits.L3base.f3\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.cv.kits.L3base.f4\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.kits.L3base.hi\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@an.cv.kits.L3base.lo\endcsname{\ensuremath{-1.08}}
\expandafter\gdef\csname R@an.cv.kits.L3base.loo.max\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@an.cv.kits.L3base.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.L3base.loo.min\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.cv.kits.L3base.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L3base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L3base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.L3base.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.L3base.share.word\endcsname{fold 1 alone carries 85\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.L3base.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L3base.share_max\endcsname{85}
\expandafter\gdef\csname R@an.cv.kits.L3base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.L3base.span14\endcsname{2.46}
\expandafter\gdef\csname R@an.cv.kits.L3base.src0\endcsname{fresh s1-2 for HyReX and frozen pool for default}
\expandafter\gdef\csname R@an.cv.kits.L3base.src0mark\endcsname{b/a}
\expandafter\gdef\csname R@an.cv.kits.L3base.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.kits.P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.P3c.cbs.clause\endcsname{the function-identical control minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.56}\,pp, 95\,\% interval \ensuremath{-0.18} to \ensuremath{+1.29}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.kits.P3c.cbs.est\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.P3c.cbs.hi\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.cv.kits.P3c.cbs.lo\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.kits.P3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.P3c.f1\endcsname{85.24}
\expandafter\gdef\csname R@an.cv.kits.P3c.f2\endcsname{83.41}
\expandafter\gdef\csname R@an.cv.kits.P3c.f3\endcsname{87.68}
\expandafter\gdef\csname R@an.cv.kits.P3c.f4\endcsname{81.87}
\expandafter\gdef\csname R@an.cv.kits.P3c.max14\endcsname{87.68}
\expandafter\gdef\csname R@an.cv.kits.P3c.mean14\endcsname{84.55}
\expandafter\gdef\csname R@an.cv.kits.P3c.min14\endcsname{81.87}
\expandafter\gdef\csname R@an.cv.kits.P3c.params\endcsname{31.20}
\expandafter\gdef\csname R@an.cv.kits.P3c.params1\endcsname{31.2}
\expandafter\gdef\csname R@an.cv.kits.P3c.span14\endcsname{5.81}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.dcv\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.f1\endcsname{\ensuremath{+2.38}}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.f2\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.f3\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.f4\endcsname{\ensuremath{-1.02}}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.hi\endcsname{\ensuremath{+2.82}}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.lo\endcsname{\ensuremath{-1.71}}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.loo.max\endcsname{\ensuremath{+1.08}}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.loo.min\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.loo.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.loo.word\endcsname{changes sign when a single fold is dropped (three of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.share.word\endcsname{fold 1 alone carries 107\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.share_max\endcsname{107}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.span14\endcsname{3.40}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.kits.V5B1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V5B1.cbs.clause\endcsname{LeanAdd minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+1.00}\,pp, 95\,\% interval \ensuremath{+0.18} to \ensuremath{+1.82}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.kits.V5B1.cbs.est\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.cv.kits.V5B1.cbs.hi\endcsname{\ensuremath{+1.82}}
\expandafter\gdef\csname R@an.cv.kits.V5B1.cbs.lo\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.kits.V5B1.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V5B1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B1.f1\endcsname{84.58}
\expandafter\gdef\csname R@an.cv.kits.V5B1.f2\endcsname{85.20}
\expandafter\gdef\csname R@an.cv.kits.V5B1.f3\endcsname{87.50}
\expandafter\gdef\csname R@an.cv.kits.V5B1.f4\endcsname{82.66}
\expandafter\gdef\csname R@an.cv.kits.V5B1.mean14\endcsname{84.99}
\expandafter\gdef\csname R@an.cv.kits.V5B1.params\endcsname{20.96}
\expandafter\gdef\csname R@an.cv.kits.V5B1.params1\endcsname{21.0}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.dcv\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.f1\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.f2\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.f3\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.f4\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.hi\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.lo\endcsname{\ensuremath{-0.79}}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.loo.max\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.loo.min\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.loo.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.loo.word\endcsname{changes sign when a single fold is dropped (two of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.share.word\endcsname{fold 3 alone carries 220\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.share_max\endcsname{220}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.span14\endcsname{1.03}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.cbs.clause\endcsname{LeanAdd minus the function-identical control, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.44}\,pp, 95\,\% interval \ensuremath{-0.34} to \ensuremath{+1.22}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.cbs.est\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.cbs.hi\endcsname{\ensuremath{+1.22}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.cbs.lo\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.ctloffset\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.dcv\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.f1\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.f2\endcsname{\ensuremath{+1.80}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.f3\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.f4\endcsname{\ensuremath{+0.79}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.hi\endcsname{\ensuremath{+2.17}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.lo\endcsname{\ensuremath{-1.30}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.loo.max\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.loo.min\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.loo.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.loo.word\endcsname{changes sign when a single fold is dropped (three of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.share.word\endcsname{fold 2 alone carries 103\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.share_max\endcsname{103}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.span14\endcsname{2.46}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.split\endcsname{LeanAdd minus the default is \ensuremath{+0.99}\,pp over the four folds; the control's own offset from the default is \ensuremath{+0.56}\,pp, so the margin over the function-identical control is \ensuremath{+0.44}\,pp}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.vsdefault\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.word\endcsname{improves on it on average (2 of 4 folds)}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.dcv\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.f1\endcsname{\ensuremath{+1.72}}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.f2\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.f3\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.f4\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.hi\endcsname{\ensuremath{+2.58}}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.lo\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.loo.max\endcsname{\ensuremath{+1.40}}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.loo.min\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.share.word\endcsname{fold 2 alone carries 48\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.share_max\endcsname{48}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.span14\endcsname{2.12}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.kits.V5B2.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V5B2.cbs.clause\endcsname{LeanAdd-NeXt minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.75}\,pp, 95\,\% interval \ensuremath{-1.56} to \ensuremath{+0.01}\,pp, which reaches just above zero}
\expandafter\gdef\csname R@an.cv.kits.V5B2.cbs.est\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.cv.kits.V5B2.cbs.hi\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.kits.V5B2.cbs.lo\endcsname{\ensuremath{-1.56}}
\expandafter\gdef\csname R@an.cv.kits.V5B2.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V5B2.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B2.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B2.f1\endcsname{83.53}
\expandafter\gdef\csname R@an.cv.kits.V5B2.f2\endcsname{82.53}
\expandafter\gdef\csname R@an.cv.kits.V5B2.f3\endcsname{86.32}
\expandafter\gdef\csname R@an.cv.kits.V5B2.f4\endcsname{80.59}
\expandafter\gdef\csname R@an.cv.kits.V5B2.mean14\endcsname{83.24}
\expandafter\gdef\csname R@an.cv.kits.V5B2.params\endcsname{21.26}
\expandafter\gdef\csname R@an.cv.kits.V5B2.params1\endcsname{21.3}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.dcv\endcsname{\ensuremath{-1.43}}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.f1\endcsname{\ensuremath{-1.64}}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.f2\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.f3\endcsname{\ensuremath{-0.97}}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.f4\endcsname{\ensuremath{-2.15}}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.hi\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.lo\endcsname{\ensuremath{-2.34}}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.loo.max\endcsname{\ensuremath{-1.20}}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.loo.min\endcsname{\ensuremath{-1.59}}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.loo.minfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.share.word\endcsname{fold 4 alone carries 37\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.share_max\endcsname{37}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.span14\endcsname{1.18}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.cbs.clause\endcsname{LeanAdd-NeXt minus the function-identical control, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-1.31}\,pp, 95\,\% interval \ensuremath{-2.09} to \ensuremath{-0.58}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.cbs.est\endcsname{\ensuremath{-1.31}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.cbs.hi\endcsname{\ensuremath{-0.58}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.cbs.lo\endcsname{\ensuremath{-2.09}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.ctloffset\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.dcv\endcsname{\ensuremath{-1.31}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.f1\endcsname{\ensuremath{-1.72}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.f2\endcsname{\ensuremath{-0.88}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.f3\endcsname{\ensuremath{-1.36}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.f4\endcsname{\ensuremath{-1.28}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.hi\endcsname{\ensuremath{-0.76}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.lo\endcsname{\ensuremath{-1.86}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.loo.max\endcsname{\ensuremath{-1.17}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.loo.min\endcsname{\ensuremath{-1.45}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.share.word\endcsname{fold 1 alone carries 33\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.share_max\endcsname{33}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.span14\endcsname{0.84}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.split\endcsname{LeanAdd-NeXt minus the default is \ensuremath{-0.75}\,pp over the four folds; the control's own offset from the default is \ensuremath{+0.56}\,pp, so the margin over the function-identical control is \ensuremath{-1.31}\,pp}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.vsdefault\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.word\endcsname{does not improve on it}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.dcv\endcsname{\ensuremath{-1.75}}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.f1\endcsname{\ensuremath{-1.05}}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.f2\endcsname{\ensuremath{-2.68}}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.f3\endcsname{\ensuremath{-1.18}}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.f4\endcsname{\ensuremath{-2.07}}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.hi\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.lo\endcsname{\ensuremath{-2.97}}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.loo.max\endcsname{\ensuremath{-1.44}}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.loo.min\endcsname{\ensuremath{-1.98}}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.share.word\endcsname{fold 2 alone carries 38\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.share_max\endcsname{38}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.span14\endcsname{1.63}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.dcv\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.f1\endcsname{\ensuremath{+0.67}}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.f2\endcsname{\ensuremath{-0.78}}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.f3\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.f4\endcsname{\ensuremath{-2.30}}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.hi\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.lo\endcsname{\ensuremath{-2.69}}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.loo.max\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.loo.min\endcsname{\ensuremath{-1.22}}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.share.word\endcsname{fold 4 alone carries 76\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.share_max\endcsname{76}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.span14\endcsname{2.97}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.cbs.clause\endcsname{HyReX-k9 minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.28}\,pp, 95\,\% interval \ensuremath{-0.62} to \ensuremath{+1.17}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.cbs.est\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.cbs.hi\endcsname{\ensuremath{+1.17}}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.cbs.lo\endcsname{\ensuremath{-0.62}}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.f1\endcsname{84.22}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.f2\endcsname{82.53}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.f3\endcsname{87.94}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.f4\endcsname{82.41}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.mean14\endcsname{84.27}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.params\endcsname{30.78}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.params1\endcsname{30.8}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.dcv\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.f1\endcsname{\ensuremath{-0.95}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.f2\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.f3\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.f4\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.hi\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.lo\endcsname{\ensuremath{-1.62}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.loo.max\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.loo.min\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.loo.minfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.share.word\endcsname{fold 2 alone carries 61\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.share_max\endcsname{61}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.span14\endcsname{1.63}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.cbs.clause\endcsname{HyReX-k9 minus the function-identical control, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.28}\,pp, 95\,\% interval \ensuremath{-1.13} to \ensuremath{+0.60}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.cbs.est\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.cbs.hi\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.cbs.lo\endcsname{\ensuremath{-1.13}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.ctloffset\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.dcv\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.f1\endcsname{\ensuremath{-1.02}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.f2\endcsname{\ensuremath{-0.88}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.f3\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.f4\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.hi\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.lo\endcsname{\ensuremath{-1.53}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.loo.max\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.loo.min\endcsname{\ensuremath{-0.55}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.share.word\endcsname{fold 1 alone carries 92\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.share_max\endcsname{92}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.span14\endcsname{1.56}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.split\endcsname{HyReX-k9 minus the default is \ensuremath{+0.28}\,pp over the four folds; the control's own offset from the default is \ensuremath{+0.56}\,pp, so the margin over the function-identical control is \ensuremath{-0.28}\,pp}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.vsdefault\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.word\endcsname{does not improve on it}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.dcv\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.f1\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.f2\endcsname{\ensuremath{-0.78}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.f3\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.f4\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.hi\endcsname{\ensuremath{+1.98}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.lo\endcsname{\ensuremath{-1.42}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.loo.max\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.loo.min\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.loo.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.loo.word\endcsname{changes sign when a single fold is dropped (three of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.share.word\endcsname{fold 1 alone carries 121\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.share_max\endcsname{121}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.span14\endcsname{2.14}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.word\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.cv.kits.V7A1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V7A1.cbs.clause\endcsname{LeanDeepMid minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+1.64}\,pp, 95\,\% interval \ensuremath{+0.89} to \ensuremath{+2.42}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.kits.V7A1.cbs.est\endcsname{\ensuremath{+1.64}}
\expandafter\gdef\csname R@an.cv.kits.V7A1.cbs.hi\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.cv.kits.V7A1.cbs.lo\endcsname{\ensuremath{+0.89}}
\expandafter\gdef\csname R@an.cv.kits.V7A1.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V7A1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7A1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A1.f1\endcsname{84.89}
\expandafter\gdef\csname R@an.cv.kits.V7A1.f2\endcsname{85.71}
\expandafter\gdef\csname R@an.cv.kits.V7A1.f3\endcsname{88.89}
\expandafter\gdef\csname R@an.cv.kits.V7A1.f4\endcsname{83.01}
\expandafter\gdef\csname R@an.cv.kits.V7A1.mean14\endcsname{85.63}
\expandafter\gdef\csname R@an.cv.kits.V7A1.params\endcsname{31.04}
\expandafter\gdef\csname R@an.cv.kits.V7A1.params1\endcsname{31.0}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.cbs.clause\endcsname{LeanDeepMid minus the function-identical control, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+1.08}\,pp, 95\,\% interval \ensuremath{+0.41} to \ensuremath{+1.78}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.cbs.est\endcsname{\ensuremath{+1.08}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.cbs.hi\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.cbs.lo\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.ctloffset\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.dcv\endcsname{\ensuremath{+1.08}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.f1\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.f2\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.f3\endcsname{\ensuremath{+1.20}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.f4\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.hi\endcsname{\ensuremath{+2.81}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.lo\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.loo.max\endcsname{\ensuremath{+1.55}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.loo.min\endcsname{\ensuremath{+0.67}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.share.word\endcsname{fold 2 alone carries 54\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.share_max\endcsname{54}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.span14\endcsname{2.66}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.split\endcsname{LeanDeepMid minus the default is \ensuremath{+1.63}\,pp over the four folds; the control's own offset from the default is \ensuremath{+0.56}\,pp, so the margin over the function-identical control is \ensuremath{+1.08}\,pp}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.vsdefault\endcsname{\ensuremath{+1.63}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.word\endcsname{improves on it on average (3 of 4 folds)}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.dcv\endcsname{\ensuremath{+2.39}}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.f1\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.f2\endcsname{\ensuremath{+3.19}}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.f3\endcsname{\ensuremath{+2.57}}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.f4\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.hi\endcsname{\ensuremath{+3.59}}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.lo\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.loo.max\endcsname{\ensuremath{+2.72}}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.loo.min\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.share.word\endcsname{fold 2 alone carries 33\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.share_max\endcsname{33}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.span14\endcsname{1.82}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.dcv\endcsname{\ensuremath{+1.63}}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.f1\endcsname{\ensuremath{+2.03}}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.f2\endcsname{\ensuremath{+2.40}}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.f3\endcsname{\ensuremath{+1.98}}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.f4\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.hi\endcsname{\ensuremath{+3.27}}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.lo\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.loo.max\endcsname{\ensuremath{+2.14}}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.loo.min\endcsname{\ensuremath{+1.38}}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.share.word\endcsname{fold 2 alone carries 37\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.share_max\endcsname{37}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.span14\endcsname{2.28}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.kits.V7A2.cbs.clause\endcsname{LeanDeepMid+FD minus the default, case-level paired bootstrap: one of the four folds has a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.kits.V7A2.cbs.nfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A2.f1\endcsname{84.67}
\expandafter\gdef\csname R@an.cv.kits.V7A2.params\endcsname{31.18}
\expandafter\gdef\csname R@an.cv.kits.V7A2.params1\endcsname{31.2}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.cbs.clause\endcsname{LeanDeepMid+FD minus the function-identical control, case-level paired bootstrap: one of the four folds has a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.cbs.nfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.f1\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.nfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.nfold.word\endcsname{one}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.f1\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.nfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.nfold.word\endcsname{one}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.f1\endcsname{\ensuremath{+1.81}}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.nfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.nfold.word\endcsname{one}
\expandafter\gdef\csname R@an.cv.kits.V7B1.cbs.clause\endcsname{LeanSep minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.kits.V7B1.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B1.params\endcsname{20.43}
\expandafter\gdef\csname R@an.cv.kits.V7B1.params1\endcsname{20.4}
\expandafter\gdef\csname R@an.cv.kits.V7B1P3c.cbs.clause\endcsname{LeanSep minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.kits.V7B1P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B1P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B1P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7B1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7B1V5B2.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B1V5B2.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7B1base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B1base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7B2.cbs.clause\endcsname{LeanDil minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.kits.V7B2.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B2.params\endcsname{20.45}
\expandafter\gdef\csname R@an.cv.kits.V7B2.params1\endcsname{20.5}
\expandafter\gdef\csname R@an.cv.kits.V7B2P3c.cbs.clause\endcsname{LeanDil minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.kits.V7B2P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B2P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B2P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7B2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7B2V5B2.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B2V5B2.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7B2base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B2base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7C1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V7C1.cbs.clause\endcsname{LeanNeXt-s5 minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.79}\,pp, 95\,\% interval \ensuremath{+0.07} to \ensuremath{+1.51}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.kits.V7C1.cbs.est\endcsname{\ensuremath{+0.79}}
\expandafter\gdef\csname R@an.cv.kits.V7C1.cbs.hi\endcsname{\ensuremath{+1.51}}
\expandafter\gdef\csname R@an.cv.kits.V7C1.cbs.lo\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.kits.V7C1.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V7C1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7C1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7C1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7C1.f1\endcsname{85.00}
\expandafter\gdef\csname R@an.cv.kits.V7C1.f2\endcsname{84.05}
\expandafter\gdef\csname R@an.cv.kits.V7C1.f3\endcsname{87.64}
\expandafter\gdef\csname R@an.cv.kits.V7C1.f4\endcsname{82.42}
\expandafter\gdef\csname R@an.cv.kits.V7C1.mean14\endcsname{84.78}
\expandafter\gdef\csname R@an.cv.kits.V7C1.params\endcsname{21.11}
\expandafter\gdef\csname R@an.cv.kits.V7C1.params1\endcsname{21.1}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.cbs.clause\endcsname{LeanNeXt-s5 minus the function-identical control, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.22}\,pp, 95\,\% interval \ensuremath{-0.49} to \ensuremath{+0.96}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.cbs.est\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.cbs.hi\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.cbs.lo\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.ctloffset\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.dcv\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.f1\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.f2\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.f3\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.f4\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.hi\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.lo\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.loo.max\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.loo.min\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.share.word\endcsname{fold 2 alone carries 71\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.share_max\endcsname{71}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.span14\endcsname{0.89}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.split\endcsname{LeanNeXt-s5 minus the default is \ensuremath{+0.78}\,pp over the four folds; the control's own offset from the default is \ensuremath{+0.56}\,pp, so the margin over the function-identical control is \ensuremath{+0.23}\,pp}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.vsdefault\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.word\endcsname{improves on it on average (2 of 4 folds)}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.dcv\endcsname{\ensuremath{+1.54}}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.f1\endcsname{\ensuremath{+1.47}}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.f2\endcsname{\ensuremath{+1.52}}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.f3\endcsname{\ensuremath{+1.32}}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.f4\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.hi\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.lo\endcsname{\ensuremath{+1.20}}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.loo.max\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.loo.min\endcsname{\ensuremath{+1.44}}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.share.word\endcsname{fold 4 alone carries 30\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.share_max\endcsname{30}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.span14\endcsname{0.51}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.dcv\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.f1\endcsname{\ensuremath{+2.14}}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.f2\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.f3\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.f4\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.hi\endcsname{\ensuremath{+2.48}}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.lo\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.loo.max\endcsname{\ensuremath{+1.20}}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.loo.min\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.share.word\endcsname{fold 1 alone carries 68\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.share_max\endcsname{68}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.span14\endcsname{2.61}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.kits.V8B2.cbs.clause\endcsname{Stem1 minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.kits.V8B2.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V8B2.params\endcsname{21.08}
\expandafter\gdef\csname R@an.cv.kits.V8B2.params1\endcsname{21.1}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.cbs.clause\endcsname{Stem1 minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.base.f0\endcsname{83.38}
\expandafter\gdef\csname R@an.cv.kits.base.f1\endcsname{82.86}
\expandafter\gdef\csname R@an.cv.kits.base.f2\endcsname{83.31}
\expandafter\gdef\csname R@an.cv.kits.base.f3\endcsname{86.91}
\expandafter\gdef\csname R@an.cv.kits.base.f4\endcsname{82.89}
\expandafter\gdef\csname R@an.cv.kits.base.max14\endcsname{86.91}
\expandafter\gdef\csname R@an.cv.kits.base.mean14\endcsname{83.99}
\expandafter\gdef\csname R@an.cv.kits.base.mean5\endcsname{83.87}
\expandafter\gdef\csname R@an.cv.kits.base.min14\endcsname{82.86}
\expandafter\gdef\csname R@an.cv.kits.base.params\endcsname{31.20}
\expandafter\gdef\csname R@an.cv.kits.base.params1\endcsname{31.2}
\expandafter\gdef\csname R@an.cv.kits.base.span14\endcsname{4.05}
\expandafter\gdef\csname R@an.cv.kits.base.src0\endcsname{frozen pool}
\expandafter\gdef\csname R@an.cv.kits.base.src0long\endcsname{the frozen default pool}
\expandafter\gdef\csname R@an.cv.kits.base.src0mark\endcsname{a}
\expandafter\gdef\csname R@an.cv.kits.base.src0n\endcsname{3}
\expandafter\gdef\csname R@an.cv.kits.recovery.L3\endcsname{0.32}
\expandafter\gdef\csname R@an.cv.kits.recovery.L3.hi\endcsname{1.09}
\expandafter\gdef\csname R@an.cv.kits.recovery.L3.lo\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.cv.kits.recovery.L3.method\endcsname{the delta method applied to the two four-fold mean margins, HyReX minus the default and ResEnc-M minus the default, which are differences from the same default runs, so their covariance over the folds enters the variance of the ratio; the interval takes the t quantile on three degrees of freedom of the registered paired-t intervals of the margins; it is descriptive, a description of four folds of one seed each and not a test, and it is withheld when ResEnc-M's own interval over the folds includes zero}
\expandafter\gdef\csname R@an.cv.kits.recovery.L3.sentence\endcsname{On KiTS23, HyReX's mean margin over the default on the four folds that entered no decision, \ensuremath{+0.68}\,pp, is 0.32 of ResEnc-M's, \ensuremath{+2.15}\,pp; the 95\,\% interval of that ratio, \ensuremath{-0.45} to 1.09, comes from the delta method on the two fold-mean margins and describes the four folds without testing anything}
\expandafter\gdef\csname R@an.cv.kits.recovery.L3.state\endcsname{complete}
\expandafter\gdef\csname R@an.cv.l1b.def\endcsname{the ResEnc-M preset re-implemented through the plan-aware family in which every agent design and every other control is built (it differs from the library preset in the default stem, the shortcut form and the zero-initialisation)}
\expandafter\gdef\csname R@an.cv.l1b.name\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.cv.line.acdc.D2P3c\endcsname{LeanDec (25.28\,M parameters) minus the function-identical control (30.38\,M): \ensuremath{+0.02}\,pp over the four folds, improves on it on average (2 of 4 folds), 95\,\% over folds \ensuremath{-0.23} to \ensuremath{+0.27}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.D2P3c3\endcsname{LeanDec (25.28\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.D2base\endcsname{LeanDec (25.28\,M parameters) minus the default (30.38\,M): \ensuremath{-0.05}\,pp over the four folds, does not improve in cross-validation (1/4 folds positive), 95\,\% over folds \ensuremath{-0.18} to \ensuremath{+0.07}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.L1L1b\endcsname{ResEnc-M (101.53\,M parameters) minus ResEnc-matched (101.63\,M): \ensuremath{+0.18}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.02} to \ensuremath{+0.33}\,pp, which lies inside $\pm$0.50\,pp and above zero}
\expandafter\gdef\csname R@an.cv.line.acdc.L1L3\endcsname{ResEnc-M (101.53\,M parameters) minus HyReX (28.85\,M): \ensuremath{+0.04}\,pp over the four folds, improves on average (2/4 folds), 95\,\% over folds \ensuremath{-0.24} to \ensuremath{+0.31}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.L1P3c\endcsname{ResEnc-M (101.53\,M parameters) minus the function-identical control (30.38\,M): \ensuremath{+0.45}\,pp over the four folds, improves on the control in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.34} to \ensuremath{+0.56}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.acdc.L1P3c3\endcsname{ResEnc-M (101.53\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.L1bL3\endcsname{ResEnc-matched (101.63\,M parameters) minus HyReX (28.85\,M): \ensuremath{-0.14}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.27} to \ensuremath{-0.01}\,pp, which lies inside $\pm$0.50\,pp and below zero}
\expandafter\gdef\csname R@an.cv.line.acdc.L1base\endcsname{ResEnc-M (101.53\,M parameters) minus the default (30.38\,M): \ensuremath{+0.37}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.26} to \ensuremath{+0.48}\,pp, which lies inside $\pm$0.50\,pp and above zero}
\expandafter\gdef\csname R@an.cv.line.acdc.L3P3c\endcsname{HyReX (28.85\,M parameters) minus the function-identical control (30.38\,M): \ensuremath{+0.41}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.06} to \ensuremath{+0.76}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.acdc.L3base\endcsname{HyReX (28.85\,M parameters) minus the default (30.38\,M): \ensuremath{+0.33}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.10} to \ensuremath{+0.56}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.acdc.P3cbase\endcsname{the function-identical control (30.38\,M parameters) minus the default (30.38\,M): \ensuremath{-0.08}\,pp over the four folds, does not improve in cross-validation (1/4 folds positive), 95\,\% over folds \ensuremath{-0.22} to \ensuremath{+0.06}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V5B1D2\endcsname{LeanAdd (20.18\,M parameters) minus LeanDec (25.28\,M): \ensuremath{-0.06}\,pp over the four folds, does not improve in cross-validation (1/4 folds positive), 95\,\% over folds \ensuremath{-0.20} to \ensuremath{+0.07}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V5B1P3c\endcsname{LeanAdd (20.18\,M parameters) minus the function-identical control (30.38\,M): \ensuremath{-0.04}\,pp over the four folds, does not improve on it (2/4 folds positive), 95\,\% over folds \ensuremath{-0.34} to \ensuremath{+0.27}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V5B1P3c3\endcsname{LeanAdd (20.18\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.V5B1base\endcsname{LeanAdd (20.18\,M parameters) minus the default (30.38\,M): \ensuremath{-0.12}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.32} to \ensuremath{+0.08}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V5B2L3\endcsname{LeanAdd-NeXt (20.48\,M parameters) minus HyReX (28.85\,M): \ensuremath{-0.45}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.69} to \ensuremath{-0.20}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.acdc.V5B2P3c\endcsname{LeanAdd-NeXt (20.48\,M parameters) minus the function-identical control (30.38\,M): \ensuremath{-0.04}\,pp over the four folds, does not improve on it (1/4 folds positive), 95\,\% over folds \ensuremath{-0.27} to \ensuremath{+0.20}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V5B2P3c3\endcsname{LeanAdd-NeXt (20.48\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.V5B2V5B1\endcsname{LeanAdd-NeXt (20.48\,M parameters) minus LeanAdd (20.18\,M): \ensuremath{0.00}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.29} to \ensuremath{+0.30}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V5B2base\endcsname{LeanAdd-NeXt (20.48\,M parameters) minus the default (30.38\,M): \ensuremath{-0.11}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.30} to \ensuremath{+0.07}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V6A1rL3\endcsname{HyReX-k9 (29.96\,M parameters) minus HyReX (28.85\,M): \ensuremath{-0.03}\,pp over the four folds, does not improve in cross-validation (3/4 folds positive), 95\,\% over folds \ensuremath{-0.28} to \ensuremath{+0.22}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V6A1rP3c\endcsname{HyReX-k9 (29.96\,M parameters) minus the function-identical control (30.38\,M): \ensuremath{+0.38}\,pp over the four folds, improves on the control in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.18} to \ensuremath{+0.59}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.acdc.V6A1rP3c3\endcsname{HyReX-k9 (29.96\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.V6A1rbase\endcsname{HyReX-k9 (29.96\,M parameters) minus the default (30.38\,M): \ensuremath{+0.31}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.13} to \ensuremath{+0.49}\,pp, which lies inside $\pm$0.50\,pp and above zero}
\expandafter\gdef\csname R@an.cv.line.acdc.V7A1P3c\endcsname{LeanDeepMid (30.26\,M parameters) minus the function-identical control (30.38\,M): \ensuremath{+0.16}\,pp over the four folds, improves on it on average (3 of 4 folds), 95\,\% over folds \ensuremath{-0.29} to \ensuremath{+0.60}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.acdc.V7A1P3c3\endcsname{LeanDeepMid (30.26\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.V7A1V5B2\endcsname{LeanDeepMid (30.26\,M parameters) minus LeanAdd-NeXt (20.48\,M): \ensuremath{+0.19}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.23} to \ensuremath{+0.62}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.acdc.V7A1base\endcsname{LeanDeepMid (30.26\,M parameters) minus the default (30.38\,M): \ensuremath{+0.08}\,pp over the four folds, improves on average (2/4 folds), 95\,\% over folds \ensuremath{-0.38} to \ensuremath{+0.54}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.acdc.V7A2P3c\endcsname{LeanDeepMid+FD (30.38\,M parameters) minus the function-identical control (30.38\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V7A2P3c3\endcsname{LeanDeepMid+FD (30.38\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.V7A2V7A1\endcsname{LeanDeepMid+FD (30.38\,M parameters) minus LeanDeepMid (30.26\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V7A2base\endcsname{LeanDeepMid+FD (30.38\,M parameters) minus the default (30.38\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V7B1P3c\endcsname{LeanSep (19.65\,M parameters) minus the function-identical control (30.38\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V7B1P3c3\endcsname{LeanSep (19.65\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.V7B1V5B2\endcsname{LeanSep (19.65\,M parameters) minus LeanAdd-NeXt (20.48\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V7B1base\endcsname{LeanSep (19.65\,M parameters) minus the default (30.38\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V7B2P3c\endcsname{LeanDil (19.67\,M parameters) minus the function-identical control (30.38\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V7B2P3c3\endcsname{LeanDil (19.67\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.V7B2V5B2\endcsname{LeanDil (19.67\,M parameters) minus LeanAdd-NeXt (20.48\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V7B2base\endcsname{LeanDil (19.67\,M parameters) minus the default (30.38\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V7C1P3c\endcsname{LeanNeXt-s5 (20.33\,M parameters) minus the function-identical control (30.38\,M): \ensuremath{-0.11}\,pp over the four folds, does not improve on it (1/4 folds positive), 95\,\% over folds \ensuremath{-0.32} to \ensuremath{+0.10}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V7C1P3c3\endcsname{LeanNeXt-s5 (20.33\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.V7C1V5B2\endcsname{LeanNeXt-s5 (20.33\,M parameters) minus LeanAdd-NeXt (20.48\,M): \ensuremath{-0.07}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.15} to \ensuremath{0.00}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V7C1base\endcsname{LeanNeXt-s5 (20.33\,M parameters) minus the default (30.38\,M): \ensuremath{-0.19}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.31} to \ensuremath{-0.07}\,pp, which lies inside $\pm$0.50\,pp and below zero}
\expandafter\gdef\csname R@an.cv.line.acdc.V8B2P3c\endcsname{Stem1 (20.32\,M parameters) minus the function-identical control (30.38\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V8B2P3c3\endcsname{Stem1 (20.32\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.V8B2base\endcsname{Stem1 (20.32\,M parameters) minus the default (30.38\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.D2P3c\endcsname{LeanDec (26.03\,M parameters) minus the function-identical control (31.12\,M): \ensuremath{-0.41}\,pp over the four folds, does not improve on it (1/4 folds positive), 95\,\% over folds \ensuremath{-0.95} to \ensuremath{+0.14}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.D2P3c3\endcsname{LeanDec (26.03\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.D2base\endcsname{LeanDec (26.03\,M parameters) minus the default (31.12\,M): \ensuremath{-0.44}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.75} to \ensuremath{-0.12}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.amos.L1L1b\endcsname{ResEnc-M (102.28\,M parameters) minus ResEnc-matched (102.37\,M): \ensuremath{-0.02}\,pp over the four folds, does not improve in cross-validation (1/4 folds positive), 95\,\% over folds \ensuremath{-0.28} to \ensuremath{+0.24}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.amos.L1L3\endcsname{ResEnc-M (102.28\,M parameters) minus HyReX (29.59\,M): \ensuremath{+0.18}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.40} to \ensuremath{+0.76}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.L1P3c\endcsname{ResEnc-M (102.28\,M parameters) minus the function-identical control (31.12\,M): \ensuremath{+0.44}\,pp over the four folds, improves on the control in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.01} to \ensuremath{+0.86}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.amos.L1P3c3\endcsname{ResEnc-M (102.28\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.L1bL3\endcsname{ResEnc-matched (102.37\,M parameters) minus HyReX (29.59\,M): \ensuremath{+0.20}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.38} to \ensuremath{+0.78}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.L1base\endcsname{ResEnc-M (102.28\,M parameters) minus the default (31.12\,M): \ensuremath{+0.41}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.27} to \ensuremath{+1.09}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.L3P3c\endcsname{HyReX (29.59\,M parameters) minus the function-identical control (31.12\,M): \ensuremath{+0.26}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{-0.03} to \ensuremath{+0.55}\,pp, which reaches just below zero}
\expandafter\gdef\csname R@an.cv.line.amos.L3base\endcsname{HyReX (29.59\,M parameters) minus the default (31.12\,M): \ensuremath{+0.23}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.08} to \ensuremath{+0.54}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.P3cbase\endcsname{the function-identical control (31.12\,M parameters) minus the default (31.12\,M): \ensuremath{-0.03}\,pp over the four folds, does not improve in cross-validation (2/4 folds positive), 95\,\% over folds \ensuremath{-0.57} to \ensuremath{+0.51}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.V5B1D2\endcsname{LeanAdd (20.93\,M parameters) minus LeanDec (26.03\,M): \ensuremath{-0.02}\,pp over the four folds, does not improve in cross-validation (2/4 folds positive), 95\,\% over folds \ensuremath{-0.28} to \ensuremath{+0.24}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.amos.V5B1P3c\endcsname{LeanAdd (20.93\,M parameters) minus the function-identical control (31.12\,M): \ensuremath{-0.43}\,pp over the four folds, does not improve on it (0/4 folds positive), 95\,\% over folds \ensuremath{-0.77} to \ensuremath{-0.09}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.amos.V5B1P3c3\endcsname{LeanAdd (20.93\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.V5B1base\endcsname{LeanAdd (20.93\,M parameters) minus the default (31.12\,M): \ensuremath{-0.46}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.82} to \ensuremath{-0.10}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.amos.V5B2L3\endcsname{LeanAdd-NeXt (21.22\,M parameters) minus HyReX (29.59\,M): \ensuremath{-0.48}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.85} to \ensuremath{-0.12}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.amos.V5B2P3c\endcsname{LeanAdd-NeXt (21.22\,M parameters) minus the function-identical control (31.12\,M): \ensuremath{-0.22}\,pp over the four folds, does not improve on it (0/4 folds positive), 95\,\% over folds \ensuremath{-0.38} to \ensuremath{-0.07}\,pp, which lies inside $\pm$0.50\,pp and below zero}
\expandafter\gdef\csname R@an.cv.line.amos.V5B2P3c3\endcsname{LeanAdd-NeXt (21.22\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.V5B2V5B1\endcsname{LeanAdd-NeXt (21.22\,M parameters) minus LeanAdd (20.93\,M): \ensuremath{+0.21}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.17} to \ensuremath{+0.58}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.V5B2base\endcsname{LeanAdd-NeXt (21.22\,M parameters) minus the default (31.12\,M): \ensuremath{-0.25}\,pp over the four folds, does not improve in cross-validation (1/4 folds positive), 95\,\% over folds \ensuremath{-0.83} to \ensuremath{+0.32}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.V6A1rL3\endcsname{HyReX-k9 (30.70\,M parameters) minus HyReX (29.59\,M): \ensuremath{-0.03}\,pp over the four folds, does not improve in cross-validation (1/4 folds positive), 95\,\% over folds \ensuremath{-0.37} to \ensuremath{+0.32}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.amos.V6A1rP3c\endcsname{HyReX-k9 (30.70\,M parameters) minus the function-identical control (31.12\,M): \ensuremath{+0.23}\,pp over the four folds, improves on the control in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.03} to \ensuremath{+0.44}\,pp, which lies inside $\pm$0.50\,pp and above zero}
\expandafter\gdef\csname R@an.cv.line.amos.V6A1rP3c3\endcsname{HyReX-k9 (30.70\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.V6A1rbase\endcsname{HyReX-k9 (30.70\,M parameters) minus the default (31.12\,M): \ensuremath{+0.20}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.34} to \ensuremath{+0.74}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.V7A1P3c\endcsname{LeanDeepMid (31.00\,M parameters) minus the function-identical control (31.12\,M): \ensuremath{+0.29}\,pp over the four folds, improves on the control in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.06} to \ensuremath{+0.52}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.amos.V7A1P3c3\endcsname{LeanDeepMid (31.00\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.V7A1V5B2\endcsname{LeanDeepMid (31.00\,M parameters) minus LeanAdd-NeXt (21.22\,M): \ensuremath{+0.51}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.26} to \ensuremath{+0.77}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.amos.V7A1base\endcsname{LeanDeepMid (31.00\,M parameters) minus the default (31.12\,M): \ensuremath{+0.26}\,pp over the four folds, improves on average (2/4 folds), 95\,\% over folds \ensuremath{-0.50} to \ensuremath{+1.02}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.V7A2P3c\endcsname{LeanDeepMid+FD (31.12\,M parameters) minus the function-identical control (31.12\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V7A2P3c3\endcsname{LeanDeepMid+FD (31.12\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.V7A2V7A1\endcsname{LeanDeepMid+FD (31.12\,M parameters) minus LeanDeepMid (31.00\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V7A2base\endcsname{LeanDeepMid+FD (31.12\,M parameters) minus the default (31.12\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V7B1P3c\endcsname{LeanSep (20.40\,M parameters) minus the function-identical control (31.12\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V7B1P3c3\endcsname{LeanSep (20.40\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.V7B1V5B2\endcsname{LeanSep (20.40\,M parameters) minus LeanAdd-NeXt (21.22\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V7B1base\endcsname{LeanSep (20.40\,M parameters) minus the default (31.12\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V7B2P3c\endcsname{LeanDil (20.42\,M parameters) minus the function-identical control (31.12\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V7B2P3c3\endcsname{LeanDil (20.42\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.V7B2V5B2\endcsname{LeanDil (20.42\,M parameters) minus LeanAdd-NeXt (21.22\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V7B2base\endcsname{LeanDil (20.42\,M parameters) minus the default (31.12\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V7C1P3c\endcsname{LeanNeXt-s5 (21.08\,M parameters) minus the function-identical control (31.12\,M): \ensuremath{-0.43}\,pp over the four folds, does not improve on it (0/4 folds positive), 95\,\% over folds \ensuremath{-0.69} to \ensuremath{-0.17}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.amos.V7C1P3c3\endcsname{LeanNeXt-s5 (21.08\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.V7C1V5B2\endcsname{LeanNeXt-s5 (21.08\,M parameters) minus LeanAdd-NeXt (21.22\,M): \ensuremath{-0.20}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.56} to \ensuremath{+0.15}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.V7C1base\endcsname{LeanNeXt-s5 (21.08\,M parameters) minus the default (31.12\,M): \ensuremath{-0.46}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.81} to \ensuremath{-0.11}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.amos.V8B2P3c\endcsname{Stem1 (21.07\,M parameters) minus the function-identical control (31.12\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V8B2P3c3\endcsname{Stem1 (21.07\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.V8B2base\endcsname{Stem1 (21.07\,M parameters) minus the default (31.12\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.kits.D2P3c\endcsname{LeanDec (26.08\,M parameters) minus the function-identical control (31.20\,M): \ensuremath{+0.49}\,pp over the four folds, improves on it on average (3 of 4 folds), 95\,\% over folds \ensuremath{-0.92} to \ensuremath{+1.89}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.D2P3c3\endcsname{LeanDec (26.08\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.D2base\endcsname{LeanDec (26.08\,M parameters) minus the default (31.20\,M): \ensuremath{+1.04}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{-0.03} to \ensuremath{+2.12}\,pp, which reaches just below zero}
\expandafter\gdef\csname R@an.cv.line.kits.L1L1b\endcsname{ResEnc-M (102.35\,M parameters) minus ResEnc-matched (102.43\,M): \ensuremath{+0.60}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.45} to \ensuremath{+1.66}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.L1L3\endcsname{ResEnc-M (102.35\,M parameters) minus HyReX (29.66\,M): \ensuremath{+1.47}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{-0.24} to \ensuremath{+3.17}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.L1P3c\endcsname{ResEnc-M (102.35\,M parameters) minus the function-identical control (31.20\,M): \ensuremath{+1.59}\,pp over the four folds, improves on the control in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{-0.63} to \ensuremath{+3.80}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.L1P3c3\endcsname{ResEnc-M (102.35\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.L1bL3\endcsname{ResEnc-matched (102.43\,M parameters) minus HyReX (29.66\,M): \ensuremath{+0.86}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{-0.10} to \ensuremath{+1.82}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.L1base\endcsname{ResEnc-M (102.35\,M parameters) minus the default (31.20\,M): \ensuremath{+2.15}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.98} to \ensuremath{+3.32}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.kits.L3P3c\endcsname{HyReX (29.66\,M parameters) minus the function-identical control (31.20\,M): \ensuremath{+0.12}\,pp over the four folds, improves on average (2/4 folds), 95\,\% over folds \ensuremath{-0.73} to \ensuremath{+0.98}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.L3base\endcsname{HyReX (29.66\,M parameters) minus the default (31.20\,M): \ensuremath{+0.68}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-1.08} to \ensuremath{+2.44}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.P3cbase\endcsname{the function-identical control (31.20\,M parameters) minus the default (31.20\,M): \ensuremath{+0.56}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-1.71} to \ensuremath{+2.82}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V5B1D2\endcsname{LeanAdd (20.96\,M parameters) minus LeanDec (26.08\,M): \ensuremath{-0.05}\,pp over the four folds, does not improve in cross-validation (2/4 folds positive), 95\,\% over folds \ensuremath{-0.79} to \ensuremath{+0.69}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V5B1P3c\endcsname{LeanAdd (20.96\,M parameters) minus the function-identical control (31.20\,M): \ensuremath{+0.44}\,pp over the four folds, improves on it on average (2 of 4 folds), 95\,\% over folds \ensuremath{-1.30} to \ensuremath{+2.17}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V5B1P3c3\endcsname{LeanAdd (20.96\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.V5B1base\endcsname{LeanAdd (20.96\,M parameters) minus the default (31.20\,M): \ensuremath{+0.99}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.59} to \ensuremath{+2.58}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V5B2L3\endcsname{LeanAdd-NeXt (21.26\,M parameters) minus HyReX (29.66\,M): \ensuremath{-1.43}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-2.34} to \ensuremath{-0.52}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.kits.V5B2P3c\endcsname{LeanAdd-NeXt (21.26\,M parameters) minus the function-identical control (31.20\,M): \ensuremath{-1.31}\,pp over the four folds, does not improve on it (0/4 folds positive), 95\,\% over folds \ensuremath{-1.86} to \ensuremath{-0.76}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.kits.V5B2P3c3\endcsname{LeanAdd-NeXt (21.26\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.V5B2V5B1\endcsname{LeanAdd-NeXt (21.26\,M parameters) minus LeanAdd (20.96\,M): \ensuremath{-1.75}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-2.97} to \ensuremath{-0.52}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.kits.V5B2base\endcsname{LeanAdd-NeXt (21.26\,M parameters) minus the default (31.20\,M): \ensuremath{-0.75}\,pp over the four folds, does not improve in cross-validation (1/4 folds positive), 95\,\% over folds \ensuremath{-2.69} to \ensuremath{+1.18}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V6A1rL3\endcsname{HyReX-k9 (30.78\,M parameters) minus HyReX (29.66\,M): \ensuremath{-0.40}\,pp over the four folds, does not improve in cross-validation (1/4 folds positive), 95\,\% over folds \ensuremath{-1.62} to \ensuremath{+0.82}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V6A1rP3c\endcsname{HyReX-k9 (30.78\,M parameters) minus the function-identical control (31.20\,M): \ensuremath{-0.28}\,pp over the four folds, does not improve on it (2/4 folds positive), 95\,\% over folds \ensuremath{-1.53} to \ensuremath{+0.98}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V6A1rP3c3\endcsname{HyReX-k9 (30.78\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.V6A1rbase\endcsname{HyReX-k9 (30.78\,M parameters) minus the default (31.20\,M): \ensuremath{+0.28}\,pp over the four folds, improves on average (2/4 folds), 95\,\% over folds \ensuremath{-1.42} to \ensuremath{+1.98}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V7A1P3c\endcsname{LeanDeepMid (31.04\,M parameters) minus the function-identical control (31.20\,M): \ensuremath{+1.08}\,pp over the four folds, improves on it on average (3 of 4 folds), 95\,\% over folds \ensuremath{-0.66} to \ensuremath{+2.81}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V7A1P3c3\endcsname{LeanDeepMid (31.04\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.V7A1V5B2\endcsname{LeanDeepMid (31.04\,M parameters) minus LeanAdd-NeXt (21.26\,M): \ensuremath{+2.39}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+1.18} to \ensuremath{+3.59}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.kits.V7A1base\endcsname{LeanDeepMid (31.04\,M parameters) minus the default (31.20\,M): \ensuremath{+1.63}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{0.00} to \ensuremath{+3.27}\,pp, which touches zero}
\expandafter\gdef\csname R@an.cv.line.kits.V7A2P3c\endcsname{LeanDeepMid+FD (31.18\,M parameters) minus the function-identical control (31.20\,M): one of the four per-fold differences are finished}
\expandafter\gdef\csname R@an.cv.line.kits.V7A2P3c3\endcsname{LeanDeepMid+FD (31.18\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.V7A2V7A1\endcsname{LeanDeepMid+FD (31.18\,M parameters) minus LeanDeepMid (31.04\,M): one of the four per-fold differences are finished}
\expandafter\gdef\csname R@an.cv.line.kits.V7A2base\endcsname{LeanDeepMid+FD (31.18\,M parameters) minus the default (31.20\,M): one of the four per-fold differences are finished}
\expandafter\gdef\csname R@an.cv.line.kits.V7B1P3c\endcsname{LeanSep (20.43\,M parameters) minus the function-identical control (31.20\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.kits.V7B1P3c3\endcsname{LeanSep (20.43\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.V7B1V5B2\endcsname{LeanSep (20.43\,M parameters) minus LeanAdd-NeXt (21.26\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.kits.V7B1base\endcsname{LeanSep (20.43\,M parameters) minus the default (31.20\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.kits.V7B2P3c\endcsname{LeanDil (20.45\,M parameters) minus the function-identical control (31.20\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.kits.V7B2P3c3\endcsname{LeanDil (20.45\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.V7B2V5B2\endcsname{LeanDil (20.45\,M parameters) minus LeanAdd-NeXt (21.26\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.kits.V7B2base\endcsname{LeanDil (20.45\,M parameters) minus the default (31.20\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.kits.V7C1P3c\endcsname{LeanNeXt-s5 (21.11\,M parameters) minus the function-identical control (31.20\,M): \ensuremath{+0.23}\,pp over the four folds, improves on it on average (2 of 4 folds), 95\,\% over folds \ensuremath{-0.47} to \ensuremath{+0.92}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V7C1P3c3\endcsname{LeanNeXt-s5 (21.11\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.V7C1V5B2\endcsname{LeanNeXt-s5 (21.11\,M parameters) minus LeanAdd-NeXt (21.26\,M): \ensuremath{+1.54}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+1.20} to \ensuremath{+1.88}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.kits.V7C1base\endcsname{LeanNeXt-s5 (21.11\,M parameters) minus the default (31.20\,M): \ensuremath{+0.78}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.92} to \ensuremath{+2.48}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V8B2P3c\endcsname{Stem1 (21.08\,M parameters) minus the function-identical control (31.20\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.kits.V8B2P3c3\endcsname{Stem1 (21.08\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.V8B2base\endcsname{Stem1 (21.08\,M parameters) minus the default (31.20\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.lit.acdc.nnunet\endcsname{91.54}
\expandafter\gdef\csname R@an.cv.lit.acdc.resencm\endcsname{91.99}
\expandafter\gdef\csname R@an.cv.lit.acdc.resencm_minus_nnunet\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.lit.amos.nnunet\endcsname{88.64}
\expandafter\gdef\csname R@an.cv.lit.amos.resencm\endcsname{88.77}
\expandafter\gdef\csname R@an.cv.lit.amos.resencm_minus_nnunet\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.cv.lit.kits.nnunet\endcsname{86.04}
\expandafter\gdef\csname R@an.cv.lit.kits.resencm\endcsname{86.79}
\expandafter\gdef\csname R@an.cv.lit.kits.resencm_minus_nnunet\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.cv.n.acdc\endcsname{200}
\expandafter\gdef\csname R@an.cv.n.amos\endcsname{200}
\expandafter\gdef\csname R@an.cv.n.kits\endcsname{489}
\expandafter\gdef\csname R@an.cv.nfolds\endcsname{4}
\expandafter\gdef\csname R@an.cv.nfolds.total\endcsname{5}
\expandafter\gdef\csname R@an.cv.nfolds.total.word\endcsname{five}
\expandafter\gdef\csname R@an.cv.nfolds.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.nval.acdc.f1\endcsname{40}
\expandafter\gdef\csname R@an.cv.nval.acdc.f2\endcsname{40}
\expandafter\gdef\csname R@an.cv.nval.acdc.f3\endcsname{40}
\expandafter\gdef\csname R@an.cv.nval.acdc.f4\endcsname{40}
\expandafter\gdef\csname R@an.cv.nval.amos.f1\endcsname{40}
\expandafter\gdef\csname R@an.cv.nval.amos.f2\endcsname{40}
\expandafter\gdef\csname R@an.cv.nval.amos.f3\endcsname{40}
\expandafter\gdef\csname R@an.cv.nval.amos.f4\endcsname{40}
\expandafter\gdef\csname R@an.cv.nval.kits.f1\endcsname{98}
\expandafter\gdef\csname R@an.cv.nval.kits.f2\endcsname{98}
\expandafter\gdef\csname R@an.cv.nval.kits.f3\endcsname{98}
\expandafter\gdef\csname R@an.cv.nval.kits.f4\endcsname{97}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.boot14.hi\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.boot14.lo\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{-0.11} to \ensuremath{+0.19}\,pp}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.11} to \ensuremath{+0.19}\,pp over the 160 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.fracpos\endcsname{47.0}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.fracpos14\endcsname{50.6}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.half14\endcsname{7}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.halfshare14\endcsname{9}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.mean\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.mean14\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.measured\endcsname{ResEnc-M improves on HyReX in 50.6\,\% of the 160 held-out cases (median \ensuremath{+0.01}\,pp), and the 10 largest gains carry 59\,\% of all gains}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.median\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.median14\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.n\endcsname{200}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.n0\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.n14\endcsname{160}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.npos\endcsname{94}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.npos14\endcsname{81}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.topshare\endcsname{54}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.topshare14\endcsname{59}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.topuniform14\endcsname{12.3}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.trim\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.trim14\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.boot14.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.boot14.lo\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{+0.20} to \ensuremath{+0.54}\,pp}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.20} to \ensuremath{+0.54}\,pp over the 160 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.fracpos\endcsname{66.0}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.fracpos14\endcsname{61.9}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.half14\endcsname{14}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.halfshare14\endcsname{14}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.mean\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.mean14\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.measured\endcsname{ResEnc-M improves on the default in 61.9\,\% of the 160 held-out cases (median \ensuremath{+0.13}\,pp), and the 10 largest gains carry 42\,\% of all gains}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.median\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.median14\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.n\endcsname{200}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.n0\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.n14\endcsname{160}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.npos\endcsname{132}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.npos14\endcsname{99}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.scope\endcsname{one held-out value per development case over folds 0--4; the 40-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for ResEnc-M and frozen pool for default), a 2- and 6-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.topshare\endcsname{37}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.topshare14\endcsname{42}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.topuniform14\endcsname{10.1}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.trim\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.trim14\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.boot14.hi\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.boot14.lo\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{-0.20} to \ensuremath{+0.11}\,pp}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.20} to \ensuremath{+0.11}\,pp over the 160 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.fracpos\endcsname{53.0}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.fracpos14\endcsname{49.4}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.half14\endcsname{11}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.halfshare14\endcsname{14}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.mean\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.mean14\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.measured\endcsname{HyReX improves on ResEnc-M in 49.4\,\% of the 160 held-out cases (median \ensuremath{-0.01}\,pp), and the 10 largest gains carry 50\,\% of all gains}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.median\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.median14\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.n\endcsname{200}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.n0\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.n14\endcsname{160}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.npos\endcsname{106}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.npos14\endcsname{79}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.scope\endcsname{one held-out value per development case over folds 0--4; the 40-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for HyReX and for ResEnc-M), a 2-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.topshare\endcsname{43}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.topshare14\endcsname{50}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.topuniform14\endcsname{12.7}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.trim\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.trim14\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.boot14.hi\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.boot14.lo\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{+0.18} to \ensuremath{+0.48}\,pp}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.18} to \ensuremath{+0.48}\,pp over the 160 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.fracpos\endcsname{68.5}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.fracpos14\endcsname{65.6}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.half14\endcsname{14}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.halfshare14\endcsname{13}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.mean\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.mean14\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.measured\endcsname{HyReX improves on the default in 65.6\,\% of the 160 held-out cases (median \ensuremath{+0.15}\,pp), and the 10 largest gains carry 41\,\% of all gains}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.median\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.median14\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.n\endcsname{200}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.n0\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.n14\endcsname{160}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.npos\endcsname{137}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.npos14\endcsname{105}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.scope\endcsname{one held-out value per development case over folds 0--4; the 40-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for HyReX and frozen pool for default), a 2- and 6-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.topshare\endcsname{34}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.topshare14\endcsname{41}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.topuniform14\endcsname{9.5}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.trim\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.trim14\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.boot14.hi\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.boot14.lo\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{-0.51} to \ensuremath{-0.23}\,pp}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.51} to \ensuremath{-0.23}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.fracpos\endcsname{28.0}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.fracpos14\endcsname{27.5}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.half14\endcsname{7}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.halfshare14\endcsname{16}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.mean\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.mean14\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.measured\endcsname{LeanDec improves on the default in 27.5\,\% of the 160 held-out cases (median \ensuremath{-0.26}\,pp), and the 10 largest gains carry 62\,\% of all gains (scored over non-empty-reference pairs)}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.median\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.median14\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.n\endcsname{200}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.n0\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.n14\endcsname{160}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.npos\endcsname{56}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.npos14\endcsname{44}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.scope\endcsname{one held-out value per development case over folds 0--4; the 40-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (seed 0 for LeanDec and frozen pool for default), a 1- and 6-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.topshare\endcsname{51}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.topshare14\endcsname{62}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.topuniform14\endcsname{22.7}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.trim\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.trim14\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.boot14.hi\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.boot14.lo\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{-0.08} to \ensuremath{+0.21}\,pp}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.08} to \ensuremath{+0.21}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.fracpos\endcsname{57.5}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.fracpos14\endcsname{56.2}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.half14\endcsname{15}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.halfshare14\endcsname{17}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.mean\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.mean14\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.measured\endcsname{ResEnc-M improves on HyReX in 56.2\,\% of the 160 held-out cases (median \ensuremath{+0.05}\,pp), and the 10 largest gains carry 40\,\% of all gains (scored over non-empty-reference pairs)}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.median\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.median14\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.n\endcsname{200}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.n0\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.n14\endcsname{160}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.npos\endcsname{115}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.npos14\endcsname{90}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.topshare\endcsname{34}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.topshare14\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.topuniform14\endcsname{11.1}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.trim\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.trim14\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.boot14.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.boot14.lo\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{+0.20} to \ensuremath{+0.54}\,pp}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.20} to \ensuremath{+0.54}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.fracpos\endcsname{72.0}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.fracpos14\endcsname{68.8}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.half14\endcsname{16}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.halfshare14\endcsname{15}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.mean\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.mean14\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.measured\endcsname{ResEnc-M improves on the default in 68.8\,\% of the 160 held-out cases (median \ensuremath{+0.20}\,pp), and the 10 largest gains carry 39\,\% of all gains (scored over non-empty-reference pairs)}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.median\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.median14\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.n\endcsname{200}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.n0\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.n14\endcsname{160}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.npos\endcsname{144}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.npos14\endcsname{110}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.scope\endcsname{one held-out value per development case over folds 0--4; the 40-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for ResEnc-M and frozen pool for default), a 2- and 6-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.topshare\endcsname{32}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.topshare14\endcsname{39}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.topuniform14\endcsname{9.1}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.trim\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.trim14\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.boot14.hi\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.boot14.lo\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{-0.21} to \ensuremath{+0.08}\,pp}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.21} to \ensuremath{+0.08}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.fracpos\endcsname{42.5}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.fracpos14\endcsname{43.8}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.half14\endcsname{11}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.halfshare14\endcsname{16}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.mean\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.mean14\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.measured\endcsname{HyReX improves on ResEnc-M in 43.8\,\% of the 160 held-out cases (median \ensuremath{-0.05}\,pp), and the 10 largest gains carry 49\,\% of all gains (scored over non-empty-reference pairs)}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.median\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.median14\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.n\endcsname{200}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.n0\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.n14\endcsname{160}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.npos\endcsname{85}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.npos14\endcsname{70}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.scope\endcsname{one held-out value per development case over folds 0--4; the 40-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for HyReX and for ResEnc-M), a 2-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.topshare\endcsname{45}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.topshare14\endcsname{49}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.topuniform14\endcsname{14.3}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.trim\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.trim14\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.boot14.hi\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.boot14.lo\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{+0.12} to \ensuremath{+0.47}\,pp}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.12} to \ensuremath{+0.47}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.fracpos\endcsname{69.0}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.fracpos14\endcsname{68.1}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.half14\endcsname{16}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.halfshare14\endcsname{15}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.mean\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.mean14\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.measured\endcsname{HyReX improves on the default in 68.1\,\% of the 160 held-out cases (median \ensuremath{+0.23}\,pp), and the 10 largest gains carry 38\,\% of all gains (scored over non-empty-reference pairs)}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.median\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.median14\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.n\endcsname{200}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.n0\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.n14\endcsname{160}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.npos\endcsname{138}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.npos14\endcsname{109}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.scope\endcsname{one held-out value per development case over folds 0--4; the 40-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for HyReX and frozen pool for default), a 2- and 6-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.topshare\endcsname{32}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.topshare14\endcsname{38}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.topuniform14\endcsname{9.2}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.trim\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.trim14\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.cv.oof.amos.estimand\endcsname{the AMOS22 case-level scores are taken over the (case, class) pairs whose reference is non-empty, a different estimand from the headline Dice that the cross-validated difference averages, so a case-level mean and the cross-validated difference differ by estimand and not only by sampling}
\expandafter\gdef\csname R@an.cv.oof.gainfrac\endcsname{50\,\%}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.boot14.hi\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.boot14.lo\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{+0.36} to \ensuremath{+1.76}\,pp}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.36} to \ensuremath{+1.76}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.fracpos\endcsname{53.0}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.fracpos14\endcsname{50.6}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.half14\endcsname{20}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.halfshare14\endcsname{10}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.mean\endcsname{\ensuremath{+1.22}}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.mean14\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.measured\endcsname{LeanDec improves on the default in 50.6\,\% of the 391 held-out cases (median \ensuremath{+0.01}\,pp), and the 10 largest gains carry 32\,\% of all gains}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.median\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.median14\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.n\endcsname{489}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.n0\endcsname{98}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.n14\endcsname{391}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.npos\endcsname{259}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.npos14\endcsname{198}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.scope\endcsname{one held-out value per development case over folds 0--4; the 98-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for LeanDec and frozen pool for default), a 2- and 3-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.topshare\endcsname{26}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.topshare14\endcsname{32}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.topuniform14\endcsname{5.1}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.trim\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.trim14\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.boot14.hi\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.boot14.lo\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{+0.52} to \ensuremath{+2.36}\,pp}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.52} to \ensuremath{+2.36}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.fracpos\endcsname{55.8}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.fracpos14\endcsname{54.5}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.half14\endcsname{20}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.halfshare14\endcsname{9}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.mean\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.mean14\endcsname{\ensuremath{+1.46}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.measured\endcsname{ResEnc-M improves on HyReX in 54.5\,\% of the 391 held-out cases (median \ensuremath{+0.12}\,pp), and the 10 largest gains carry 32\,\% of all gains}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.median\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.median14\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.n\endcsname{489}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.n0\endcsname{98}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.n14\endcsname{391}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.npos\endcsname{273}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.npos14\endcsname{213}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.topshare\endcsname{28}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.topshare14\endcsname{32}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.topuniform14\endcsname{4.7}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.trim\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.trim14\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.boot14.hi\endcsname{\ensuremath{+3.08}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.boot14.lo\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{+1.28} to \ensuremath{+3.08}\,pp}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+1.28} to \ensuremath{+3.08}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.fracpos\endcsname{64.8}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.fracpos14\endcsname{61.4}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.half14\endcsname{21}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.halfshare14\endcsname{9}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.mean\endcsname{\ensuremath{+2.41}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.mean14\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.measured\endcsname{ResEnc-M improves on the default in 61.4\,\% of the 391 held-out cases (median \ensuremath{+0.30}\,pp), and the 10 largest gains carry 31\,\% of all gains}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.median\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.median14\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.n\endcsname{489}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.n0\endcsname{98}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.n14\endcsname{391}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.npos\endcsname{317}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.npos14\endcsname{240}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.scope\endcsname{one held-out value per development case over folds 0--4; the 98-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for ResEnc-M and frozen pool for default), a 2- and 3-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.topshare\endcsname{25}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.topshare14\endcsname{31}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.topuniform14\endcsname{4.2}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.trim\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.trim14\endcsname{\ensuremath{+0.91}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.boot14.hi\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.boot14.lo\endcsname{\ensuremath{-2.42}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{-2.42} to \ensuremath{-0.59}\,pp}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-2.42} to \ensuremath{-0.59}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.fracpos\endcsname{44.2}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.fracpos14\endcsname{45.5}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.half14\endcsname{11}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.halfshare14\endcsname{6}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.mean\endcsname{\ensuremath{-1.45}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.mean14\endcsname{\ensuremath{-1.46}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.measured\endcsname{HyReX improves on ResEnc-M in 45.5\,\% of the 391 held-out cases (median \ensuremath{-0.12}\,pp), and the 10 largest gains carry 48\,\% of all gains}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.median\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.median14\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.n\endcsname{489}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.n0\endcsname{98}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.n14\endcsname{391}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.npos\endcsname{216}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.npos14\endcsname{178}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.scope\endcsname{one held-out value per development case over folds 0--4; the 98-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for HyReX and for ResEnc-M), a 2-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.topshare\endcsname{42}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.topshare14\endcsname{48}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.topuniform14\endcsname{5.6}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.trim\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.trim14\endcsname{\ensuremath{-0.65}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.boot14.hi\endcsname{\ensuremath{+1.54}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.boot14.lo\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{-0.16} to \ensuremath{+1.54}\,pp}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.16} to \ensuremath{+1.54}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.fracpos\endcsname{58.3}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.fracpos14\endcsname{55.8}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.half14\endcsname{19}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.halfshare14\endcsname{9}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.mean\endcsname{\ensuremath{+0.97}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.mean14\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.measured\endcsname{HyReX improves on the default in 55.8\,\% of the 391 held-out cases (median \ensuremath{+0.16}\,pp), and the 10 largest gains carry 34\,\% of all gains}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.median\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.median14\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.n\endcsname{489}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.n0\endcsname{98}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.n14\endcsname{391}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.npos\endcsname{285}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.npos14\endcsname{218}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q1\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q1n\endcsname{98}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q2\endcsname{\ensuremath{+2.38}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q2n\endcsname{98}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q3\endcsname{\ensuremath{-1.36}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q3n\endcsname{98}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q4\endcsname{\ensuremath{+1.54}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q4n\endcsname{98}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q5\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q5n\endcsname{97}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.scope\endcsname{one held-out value per development case over folds 0--4; the 98-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for HyReX and frozen pool for default), a 2- and 3-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.topshare\endcsname{28}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.topshare14\endcsname{34}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.topuniform14\endcsname{4.6}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.trim\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.trim14\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.oof.kits.quintile.basis\endcsname{physical tumour volume}
\expandafter\gdef\csname R@an.cv.oof.kits.quintile.unit\endcsname{mL}
\expandafter\gdef\csname R@an.cv.oof.top\endcsname{10}
\expandafter\gdef\csname R@an.cv.oof.topword\endcsname{ten}
\expandafter\gdef\csname R@an.cv.p3c.bandnote\endcsname{The grey band marks two standard deviations of a one-seed pair difference of that dataset and locates each per-fold difference on the seed-noise scale of that dataset}
\expandafter\gdef\csname R@an.cv.p3c.def\endcsname{the nnU-Net default network rebuilt through the plan-aware family in which every agent design and every other control is built (the same function as the default, a different implementation)}
\expandafter\gdef\csname R@an.cv.p3c.name\endcsname{function-identical control}
\expandafter\gdef\csname R@an.cv.p6.condition\endcsname{AMOS22 \ensuremath{-0.36}\,pp; KiTS23 \ensuremath{+2.36}\,pp}
\expandafter\gdef\csname R@an.cv.p6.condition.state\endcsname{fails}
\expandafter\gdef\csname R@an.cv.p6.deviation.limit\endcsname{The cross-validation of LeanDec departs from a registered clause: Addendum P6's condition failed (AMOS22 \ensuremath{-0.36}\,pp; KiTS23 \ensuremath{+2.36}\,pp against a \ensuremath{-0.15}\,pp line) and the runs were queued afterwards under Addendum AB and Addendum AA, whose own margin, \ensuremath{-0.50}\,pp, is looser than P6's and was fixed after the failing result was known. Both readings are printed: LeanDec minus the default is \ensuremath{+0.30}\,pp on average over the two co-primary benchmarks, at or above the \ensuremath{-0.15}\,pp margin of Addendum P6; LeanDec minus the default is \ensuremath{+0.30}\,pp on average over the two co-primary benchmarks, at or above the \ensuremath{-0.50}\,pp margin of Addendum AA target T2.}
\expandafter\gdef\csname R@an.cv.p6.deviation.limit.both\endcsname{The cross-validation of LeanDec departs from a registered clause: Addendum P6's condition failed (AMOS22 \ensuremath{-0.36}\,pp; KiTS23 \ensuremath{+2.36}\,pp against a \ensuremath{-0.15}\,pp line) and the runs were queued afterwards under Addendum AB and Addendum AA, whose own margin, \ensuremath{-0.50}\,pp, is looser than P6's and was fixed after the failing result was known. Both readings are printed: LeanDec minus the default is \ensuremath{+0.30}\,pp on average over the two co-primary benchmarks (AMOS22 and KiTS23; the registered reading of Addendum AB4), at or above the \ensuremath{-0.15}\,pp margin of Addendum P6 and at or above the \ensuremath{-0.50}\,pp margin of Addendum AA target T2.}
\expandafter\gdef\csname R@an.cv.p6.deviation.registered\endcsname{Addendum AB and Addendum AA}
\expandafter\gdef\csname R@an.cv.p6.deviation.sentence\endcsname{The registered condition of Addendum P6 for a cross-validation of LeanDec -- a fold-0 seed-0 Dice at least \ensuremath{-0.15}\,pp from the frozen default pool on every co-primary benchmark -- failed (AMOS22 \ensuremath{-0.36}\,pp; KiTS23 \ensuremath{+2.36}\,pp), so Addendum P6 owed it none; the cross-validation was nevertheless run, under Addendum AB and Addendum AA, by a decision of the lead taken after that failure was known, and is reported here with the failure.}
\expandafter\gdef\csname R@an.cv.p6.floor\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.p6.margin.both.clause\endcsname{LeanDec minus the default is \ensuremath{+0.30}\,pp on average over the two co-primary benchmarks (AMOS22 and KiTS23; the registered reading of Addendum AB4), at or above the \ensuremath{-0.15}\,pp margin of Addendum P6 and at or above the \ensuremath{-0.50}\,pp margin of Addendum AA target T2}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.acdc\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.acdc.met\endcsname{met}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.amos\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.amos.met\endcsname{not met}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.clause\endcsname{LeanDec minus the default is \ensuremath{+0.30}\,pp on average over the two co-primary benchmarks, at or above the \ensuremath{-0.15}\,pp margin of Addendum P6}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.kits\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.kits.met\endcsname{met}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.mean\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.mean.met\endcsname{met}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.ndone\endcsname{2}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.src\endcsname{Addendum P6}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.value\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.acdc\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.acdc.met\endcsname{met}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.amos\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.amos.met\endcsname{met}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.clause\endcsname{LeanDec minus the default is \ensuremath{+0.30}\,pp on average over the two co-primary benchmarks, at or above the \ensuremath{-0.50}\,pp margin of Addendum AA target T2}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.kits\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.kits.met\endcsname{met}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.mean\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.mean.met\endcsname{met}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.ndone\endcsname{2}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.src\endcsname{Addendum AA target T2}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.value\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.cv.p6.note\endcsname{Addendum P6 is queued: the twelve ai\_benchcvD2 runs add the (LeanDec, default) pair under the same estimands, and their per-fold Dice is in the LeanDec per-fold table}
\expandafter\gdef\csname R@an.cv.pairsd.acdc\endcsname{0.14}
\expandafter\gdef\csname R@an.cv.pairsd.amos\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.pairsd.kits\endcsname{1.12}
\expandafter\gdef\csname R@an.cv.pool.acdc.mean\endcsname{92.009}
\expandafter\gdef\csname R@an.cv.pool.acdc.n\endcsname{6}
\expandafter\gdef\csname R@an.cv.pool.acdc.sd\endcsname{0.099}
\expandafter\gdef\csname R@an.cv.pool.amos.mean\endcsname{87.701}
\expandafter\gdef\csname R@an.cv.pool.amos.n\endcsname{6}
\expandafter\gdef\csname R@an.cv.pool.amos.sd\endcsname{0.122}
\expandafter\gdef\csname R@an.cv.pool.kits.mean\endcsname{83.378}
\expandafter\gdef\csname R@an.cv.pool.kits.n\endcsname{3}
\expandafter\gdef\csname R@an.cv.pool.kits.sd\endcsname{0.795}
\expandafter\gdef\csname R@an.cv.pos.acdc.measured\endcsname{our ResEnc-M five-fold margin over our own default is \ensuremath{+0.34}\,pp (\ensuremath{+0.34}\,pp against the uncompiled sub-pool; fold-0 fifth: fresh s1-2 for ResEnc-M and frozen pool for default), against the published \ensuremath{+0.45}\,pp over the published default, a gap of 0.11\,pp}
\expandafter\gdef\csname R@an.cv.pos.acdc.reprogap\endcsname{0.11}
\expandafter\gdef\csname R@an.cv.pos.all\endcsname{yes}
\expandafter\gdef\csname R@an.cv.pos.amos.measured\endcsname{our ResEnc-M five-fold margin over our own default is \ensuremath{+0.42}\,pp (\ensuremath{+0.42}\,pp against the contemporaneous default runs; fold-0 fifth: fresh s1-2 for ResEnc-M and frozen pool for default), against the published \ensuremath{+0.13}\,pp over the published default, a gap of 0.29\,pp}
\expandafter\gdef\csname R@an.cv.pos.amos.reprogap\endcsname{0.29}
\expandafter\gdef\csname R@an.cv.pos.everynames\endcsname{ACDC}
\expandafter\gdef\csname R@an.cv.pos.kits.measured\endcsname{our ResEnc-M five-fold margin over our own default is \ensuremath{+2.41}\,pp (\ensuremath{+2.36}\,pp against the six-run pool; fold-0 fifth: fresh s1-2 for ResEnc-M and frozen pool for default), against the published \ensuremath{+0.75}\,pp over the published default, a gap of 1.66\,pp}
\expandafter\gdef\csname R@an.cv.pos.kits.reprogap\endcsname{1.66}
\expandafter\gdef\csname R@an.cv.pos.n\endcsname{3}
\expandafter\gdef\csname R@an.cv.pos.n.word\endcsname{three}
\expandafter\gdef\csname R@an.cv.pos.names\endcsname{AMOS22, KiTS23 and ACDC}
\expandafter\gdef\csname R@an.cv.pos.nds\endcsname{3}
\expandafter\gdef\csname R@an.cv.pos.nds.word\endcsname{three}
\expandafter\gdef\csname R@an.cv.pos.nevery\endcsname{1}
\expandafter\gdef\csname R@an.cv.pos.notnames\endcsname{none}
\expandafter\gdef\csname R@an.cv.pos.pendnames\endcsname{none}
\expandafter\gdef\csname R@an.cv.pos.sentence\endcsname{HyReX's selection-free mean contrast with the stock default is positive on all three development datasets (AMOS22, KiTS23 and ACDC); the registered wording per dataset, with its interval over folds and its fold count, is in the cross-validation summary table}
\expandafter\gdef\csname R@an.cv.pos.short\endcsname{positive on all three development datasets (AMOS22, KiTS23 and ACDC)}
\expandafter\gdef\csname R@an.cv.pos.total\endcsname{3}
\expandafter\gdef\csname R@an.cv.posctl.all\endcsname{yes}
\expandafter\gdef\csname R@an.cv.posctl.everynames\endcsname{AMOS22 and ACDC}
\expandafter\gdef\csname R@an.cv.posctl.n\endcsname{3}
\expandafter\gdef\csname R@an.cv.posctl.n.word\endcsname{three}
\expandafter\gdef\csname R@an.cv.posctl.names\endcsname{AMOS22, KiTS23 and ACDC}
\expandafter\gdef\csname R@an.cv.posctl.nds\endcsname{3}
\expandafter\gdef\csname R@an.cv.posctl.nds.word\endcsname{three}
\expandafter\gdef\csname R@an.cv.posctl.nevery\endcsname{2}
\expandafter\gdef\csname R@an.cv.posctl.notnames\endcsname{none}
\expandafter\gdef\csname R@an.cv.posctl.pendnames\endcsname{none}
\expandafter\gdef\csname R@an.cv.posctl.sentence\endcsname{HyReX's selection-free mean contrast with its function-identical control is positive in the mean on all three development datasets (AMOS22, KiTS23 and ACDC) and in every fold on two (AMOS22 and ACDC); the registered wording per dataset, with its interval over folds and its fold count, is in the table of the control's cross-validation lines}
\expandafter\gdef\csname R@an.cv.posctl.short\endcsname{positive in the mean on all three development datasets (AMOS22, KiTS23 and ACDC) and in every fold on two (AMOS22 and ACDC)}
\expandafter\gdef\csname R@an.cv.posctl.total\endcsname{3}
\expandafter\gdef\csname R@an.cv.ref.acdc.alt\endcsname{uncompiled sub-pool, 3 runs, \ensuremath{+0.007} pp against the frozen pool}
\expandafter\gdef\csname R@an.cv.ref.acdc.altkey\endcsname{uncompiled}
\expandafter\gdef\csname R@an.cv.ref.acdc.frozen.mean\endcsname{92.009}
\expandafter\gdef\csname R@an.cv.ref.acdc.frozen.n\endcsname{6}
\expandafter\gdef\csname R@an.cv.ref.acdc.frozen.shift\endcsname{\ensuremath{0.000}}
\expandafter\gdef\csname R@an.cv.ref.acdc.frozen.short\endcsname{frozen pool}
\expandafter\gdef\csname R@an.cv.ref.acdc.frozen.state\endcsname{available}
\expandafter\gdef\csname R@an.cv.ref.acdc.uncompiled.mean\endcsname{92.016}
\expandafter\gdef\csname R@an.cv.ref.acdc.uncompiled.n\endcsname{3}
\expandafter\gdef\csname R@an.cv.ref.acdc.uncompiled.shift\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.cv.ref.acdc.uncompiled.short\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.cv.ref.acdc.uncompiled.state\endcsname{available}
\expandafter\gdef\csname R@an.cv.ref.amos.alt\endcsname{contemporaneous default runs, 3 runs, \ensuremath{+0.011} pp against the frozen pool}
\expandafter\gdef\csname R@an.cv.ref.amos.altkey\endcsname{contemporaneous}
\expandafter\gdef\csname R@an.cv.ref.amos.contemporaneous.mean\endcsname{87.712}
\expandafter\gdef\csname R@an.cv.ref.amos.contemporaneous.n\endcsname{3}
\expandafter\gdef\csname R@an.cv.ref.amos.contemporaneous.shift\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.cv.ref.amos.contemporaneous.short\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.cv.ref.amos.contemporaneous.state\endcsname{available}
\expandafter\gdef\csname R@an.cv.ref.amos.frozen.mean\endcsname{87.701}
\expandafter\gdef\csname R@an.cv.ref.amos.frozen.n\endcsname{6}
\expandafter\gdef\csname R@an.cv.ref.amos.frozen.shift\endcsname{\ensuremath{0.000}}
\expandafter\gdef\csname R@an.cv.ref.amos.frozen.short\endcsname{frozen pool}
\expandafter\gdef\csname R@an.cv.ref.amos.frozen.state\endcsname{available}
\expandafter\gdef\csname R@an.cv.ref.amos.uncompiled.mean\endcsname{87.730}
\expandafter\gdef\csname R@an.cv.ref.amos.uncompiled.n\endcsname{3}
\expandafter\gdef\csname R@an.cv.ref.amos.uncompiled.shift\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.cv.ref.amos.uncompiled.short\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.cv.ref.amos.uncompiled.state\endcsname{available}
\expandafter\gdef\csname R@an.cv.ref.kits.alt\endcsname{six-run pool, \ensuremath{+0.244} pp against the frozen pool}
\expandafter\gdef\csname R@an.cv.ref.kits.altkey\endcsname{union}
\expandafter\gdef\csname R@an.cv.ref.kits.contemporaneous.mean\endcsname{83.866}
\expandafter\gdef\csname R@an.cv.ref.kits.contemporaneous.n\endcsname{3}
\expandafter\gdef\csname R@an.cv.ref.kits.contemporaneous.shift\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.cv.ref.kits.contemporaneous.short\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.cv.ref.kits.contemporaneous.state\endcsname{available}
\expandafter\gdef\csname R@an.cv.ref.kits.frozen.mean\endcsname{83.378}
\expandafter\gdef\csname R@an.cv.ref.kits.frozen.n\endcsname{3}
\expandafter\gdef\csname R@an.cv.ref.kits.frozen.shift\endcsname{\ensuremath{0.000}}
\expandafter\gdef\csname R@an.cv.ref.kits.frozen.short\endcsname{frozen pool}
\expandafter\gdef\csname R@an.cv.ref.kits.frozen.state\endcsname{available}
\expandafter\gdef\csname R@an.cv.ref.kits.union.mean\endcsname{83.622}
\expandafter\gdef\csname R@an.cv.ref.kits.union.n\endcsname{6}
\expandafter\gdef\csname R@an.cv.ref.kits.union.shift\endcsname{\ensuremath{+0.244}}
\expandafter\gdef\csname R@an.cv.ref.kits.union.short\endcsname{six-run pool}
\expandafter\gdef\csname R@an.cv.ref.kits.union.state\endcsname{available}
\expandafter\gdef\csname R@an.cv.resencm.stock\endcsname{ResEnc-M is the stock library preset and has no function-identical control: the ResEnc-matched re-implementation differs from the preset in the default stem, the shortcut form and the zero-initialisation, so its contrasts with HyReX are read beside each network's contrast with the stock default and, where the like-for-like set has finished, beside the re-implementation, whose own difference from the preset is reported as a re-implementation difference}
\expandafter\gdef\csname R@an.cv.robust.sect\endcsname{\textsuperscript{\S}}
\expandafter\gdef\csname R@an.cv.sec.acdc.D2base.dl\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.sec.acdc.D2base.dlhi\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.sec.acdc.D2base.dllo\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.sec.acdc.L1base.dl\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.sec.acdc.L1base.dlhi\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.cv.sec.acdc.L1base.dllo\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.sec.acdc.L3L1.dl\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cv.sec.acdc.L3L1.dlhi\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.cv.sec.acdc.L3L1.dllo\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.sec.acdc.L3base.dl\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.cv.sec.acdc.L3base.dlhi\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.cv.sec.acdc.L3base.dllo\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.sec.amos.D2base.dl\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.cv.sec.amos.D2base.dlhi\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.sec.amos.D2base.dllo\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.cv.sec.amos.L1base.dl\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.cv.sec.amos.L1base.dlhi\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.cv.sec.amos.L1base.dllo\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.sec.amos.L3L1.dl\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.sec.amos.L3L1.dlhi\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.sec.amos.L3L1.dllo\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.cv.sec.amos.L3base.dl\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.cv.sec.amos.L3base.dlhi\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.sec.amos.L3base.dllo\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.sec.kits.D2base.dl\endcsname{\ensuremath{+1.08}}
\expandafter\gdef\csname R@an.cv.sec.kits.D2base.dlhi\endcsname{\ensuremath{+1.75}}
\expandafter\gdef\csname R@an.cv.sec.kits.D2base.dllo\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv.sec.kits.L1base.dl\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.cv.sec.kits.L1base.dlhi\endcsname{\ensuremath{+2.52}}
\expandafter\gdef\csname R@an.cv.sec.kits.L1base.dllo\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.cv.sec.kits.L3L1.dl\endcsname{\ensuremath{-1.35}}
\expandafter\gdef\csname R@an.cv.sec.kits.L3L1.dlhi\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@an.cv.sec.kits.L3L1.dllo\endcsname{\ensuremath{-2.18}}
\expandafter\gdef\csname R@an.cv.sec.kits.L3base.dl\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cv.sec.kits.L3base.dlhi\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.cv.sec.kits.L3base.dllo\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.cv.span.acdc.band\endcsname{0.14}
\expandafter\gdef\csname R@an.cv.span.acdc.base\endcsname{1.36}
\expandafter\gdef\csname R@an.cv.span.acdc.contrast\endcsname{0.39}
\expandafter\gdef\csname R@an.cv.span.acdc.nc\endcsname{4}
\expandafter\gdef\csname R@an.cv.span.acdc.runnerup\endcsname{HyReX $-$ default}
\expandafter\gdef\csname R@an.cv.span.acdc.widest\endcsname{HyReX $-$ ResEnc-M}
\expandafter\gdef\csname R@an.cv.span.acdc.widestmargin\endcsname{0.04}
\expandafter\gdef\csname R@an.cv.span.acdc.widestword\endcsname{the largest of the four architecture-contrast spans measured here, which the 0.14 pp seed-noise scale of a one-seed pair difference does not resolve between HyReX $-$ ResEnc-M and HyReX $-$ default (0.39 pp against 0.35 pp)}
\expandafter\gdef\csname R@an.cv.span.acdc.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.span.amos.band\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.span.amos.base\endcsname{2.12}
\expandafter\gdef\csname R@an.cv.span.amos.contrast\endcsname{0.94}
\expandafter\gdef\csname R@an.cv.span.amos.nc\endcsname{4}
\expandafter\gdef\csname R@an.cv.span.amos.runnerup\endcsname{HyReX $-$ ResEnc-M}
\expandafter\gdef\csname R@an.cv.span.amos.widest\endcsname{ResEnc-M $-$ default}
\expandafter\gdef\csname R@an.cv.span.amos.widestmargin\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.span.amos.widestword\endcsname{the largest of the four architecture-contrast spans measured here, which the 0.17 pp seed-noise scale of a one-seed pair difference does not resolve between ResEnc-M $-$ default and HyReX $-$ ResEnc-M (0.94 pp against 0.77 pp)}
\expandafter\gdef\csname R@an.cv.span.amos.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.span.kits.band\endcsname{1.12}
\expandafter\gdef\csname R@an.cv.span.kits.base\endcsname{4.05}
\expandafter\gdef\csname R@an.cv.span.kits.contrast\endcsname{2.47}
\expandafter\gdef\csname R@an.cv.span.kits.nc\endcsname{4}
\expandafter\gdef\csname R@an.cv.span.kits.runnerup\endcsname{HyReX $-$ default}
\expandafter\gdef\csname R@an.cv.span.kits.widest\endcsname{HyReX $-$ ResEnc-M}
\expandafter\gdef\csname R@an.cv.span.kits.widestmargin\endcsname{0.01}
\expandafter\gdef\csname R@an.cv.span.kits.widestword\endcsname{the largest of the four architecture-contrast spans measured here, which the 1.12 pp seed-noise scale of a one-seed pair difference does not resolve between HyReX $-$ ResEnc-M and HyReX $-$ default (2.47 pp against 2.46 pp)}
\expandafter\gdef\csname R@an.cv.span.kits.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.src0.a\endcsname{the frozen default pool}
\expandafter\gdef\csname R@an.cv.src0.b\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.cv.src0.c\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.cv.src0.legend\endcsname{a frozen pool, b fresh s1-2, c seed 0}
\expandafter\gdef\csname R@an.cv.src0.legendlong\endcsname{a: the frozen default pool; b: the mean of fresh seeds 1 and 2; c: discovery seed 0}
\expandafter\gdef\csname R@an.cv.status.acdc\endcsname{16 of 16 runs finished}
\expandafter\gdef\csname R@an.cv.status.all\endcsname{48 of 48 runs finished}
\expandafter\gdef\csname R@an.cv.status.amos\endcsname{16 of 16 runs finished}
\expandafter\gdef\csname R@an.cv.status.failed\endcsname{no Addendum-P run has failed}
\expandafter\gdef\csname R@an.cv.status.kits\endcsname{16 of 16 runs finished}
\expandafter\gdef\csname R@an.cv.status.l1b\endcsname{12 of 12 runs finished}
\expandafter\gdef\csname R@an.cv.status.l1b.acdc\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.l1b.amos\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.l1b.failed\endcsname{no Addendum-X cross-validation run has failed}
\expandafter\gdef\csname R@an.cv.status.l1b.kits\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.l1b.n\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.l1b.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.l1b.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.n\endcsname{48}
\expandafter\gdef\csname R@an.cv.status.p3c\endcsname{12 of 12 runs finished}
\expandafter\gdef\csname R@an.cv.status.p3c.acdc\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.p3c.amos\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.p3c.failed\endcsname{no Addendum-W cross-validation run has failed}
\expandafter\gdef\csname R@an.cv.status.p3c.kits\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.p3c.n\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.p3c.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.p3c.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.p6\endcsname{P6 queued (12 runs)}
\expandafter\gdef\csname R@an.cv.status.p6.sentence\endcsname{the cross-validation of LeanDec was queued although Addendum P6 owed it none (Addendum AB); 12 of its 12 seed-0 runs have finished (and the 24 extension runs of Addendum AH2: 0 finished)}
\expandafter\gdef\csname R@an.cv.status.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.total\endcsname{48}
\expandafter\gdef\csname R@an.cv.status.v5b1\endcsname{12 of 12 runs finished}
\expandafter\gdef\csname R@an.cv.status.v5b1.acdc\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v5b1.amos\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v5b1.failed\endcsname{no cross-validation run of LeanAdd has failed}
\expandafter\gdef\csname R@an.cv.status.v5b1.kits\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v5b1.n\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v5b1.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.v5b1.sentence\endcsname{the cross-validation of LeanAdd (Addendum AM) has 12 of its 12 runs finished (AMOS22 4 of 4, KiTS23 4 of 4, ACDC 4 of 4)}
\expandafter\gdef\csname R@an.cv.status.v5b1.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v5b2\endcsname{12 of 12 runs finished}
\expandafter\gdef\csname R@an.cv.status.v5b2.acdc\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v5b2.amos\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v5b2.failed\endcsname{no cross-validation run of LeanAdd-NeXt has failed}
\expandafter\gdef\csname R@an.cv.status.v5b2.kits\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v5b2.n\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v5b2.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.v5b2.sentence\endcsname{the cross-validation of LeanAdd-NeXt (Addendum AM) has 12 of its 12 runs finished (AMOS22 4 of 4, KiTS23 4 of 4, ACDC 4 of 4)}
\expandafter\gdef\csname R@an.cv.status.v5b2.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v6a1r\endcsname{12 of 12 runs finished}
\expandafter\gdef\csname R@an.cv.status.v6a1r.acdc\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v6a1r.amos\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v6a1r.failed\endcsname{no cross-validation run of HyReX-k9 has failed}
\expandafter\gdef\csname R@an.cv.status.v6a1r.kits\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v6a1r.n\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v6a1r.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.v6a1r.sentence\endcsname{the cross-validation of HyReX-k9 (Addendum AO) has 12 of its 12 runs finished (AMOS22 4 of 4, KiTS23 4 of 4, ACDC 4 of 4)}
\expandafter\gdef\csname R@an.cv.status.v6a1r.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v7a1\endcsname{12 of 12 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7a1.acdc\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7a1.amos\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7a1.failed\endcsname{no cross-validation run of LeanDeepMid has failed}
\expandafter\gdef\csname R@an.cv.status.v7a1.kits\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7a1.n\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v7a1.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.v7a1.sentence\endcsname{the cross-validation of LeanDeepMid (Addendum AP) has 12 of its 12 runs finished (AMOS22 4 of 4, KiTS23 4 of 4, ACDC 4 of 4)}
\expandafter\gdef\csname R@an.cv.status.v7a1.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v7a2\endcsname{1 of 12 runs finished, 11 running}
\expandafter\gdef\csname R@an.cv.status.v7a2.acdc\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7a2.amos\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7a2.failed\endcsname{no cross-validation run of LeanDeepMid+FD has failed}
\expandafter\gdef\csname R@an.cv.status.v7a2.kits\endcsname{1 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7a2.n\endcsname{1}
\expandafter\gdef\csname R@an.cv.status.v7a2.running\endcsname{11}
\expandafter\gdef\csname R@an.cv.status.v7a2.sentence\endcsname{the cross-validation of LeanDeepMid+FD (Addendum AW) has 1 of its 12 runs finished (AMOS22 0 of 4, KiTS23 1 of 4, ACDC 0 of 4)}
\expandafter\gdef\csname R@an.cv.status.v7a2.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v7b1\endcsname{0 of 12 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7b1.acdc\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7b1.amos\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7b1.failed\endcsname{no cross-validation run of LeanSep has failed}
\expandafter\gdef\csname R@an.cv.status.v7b1.kits\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7b1.n\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.v7b1.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.v7b1.sentence\endcsname{the cross-validation of LeanSep (Addendum AQ) has 0 of its 12 runs finished (AMOS22 0 of 4, KiTS23 0 of 4, ACDC 0 of 4)}
\expandafter\gdef\csname R@an.cv.status.v7b1.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v7b2\endcsname{0 of 12 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7b2.acdc\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7b2.amos\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7b2.failed\endcsname{no cross-validation run of LeanDil has failed}
\expandafter\gdef\csname R@an.cv.status.v7b2.kits\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7b2.n\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.v7b2.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.v7b2.sentence\endcsname{the cross-validation of LeanDil (Addendum AQ) has 0 of its 12 runs finished (AMOS22 0 of 4, KiTS23 0 of 4, ACDC 0 of 4)}
\expandafter\gdef\csname R@an.cv.status.v7b2.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v7c1\endcsname{12 of 12 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7c1.acdc\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7c1.amos\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7c1.failed\endcsname{no cross-validation run of LeanNeXt-s5 has failed}
\expandafter\gdef\csname R@an.cv.status.v7c1.kits\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7c1.n\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v7c1.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.v7c1.sentence\endcsname{the cross-validation of LeanNeXt-s5 (Addendum AP) has 12 of its 12 runs finished (AMOS22 4 of 4, KiTS23 4 of 4, ACDC 4 of 4)}
\expandafter\gdef\csname R@an.cv.status.v7c1.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v8b2\endcsname{0 of 12 runs finished, 9 running}
\expandafter\gdef\csname R@an.cv.status.v8b2.acdc\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v8b2.amos\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v8b2.failed\endcsname{no cross-validation run of Stem1 has failed}
\expandafter\gdef\csname R@an.cv.status.v8b2.kits\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v8b2.n\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.v8b2.running\endcsname{9}
\expandafter\gdef\csname R@an.cv.status.v8b2.sentence\endcsname{the cross-validation of Stem1 (Addendum AY) has 0 of its 12 runs finished (AMOS22 0 of 4, KiTS23 0 of 4, ACDC 0 of 4)}
\expandafter\gdef\csname R@an.cv.status.v8b2.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.tta.acdc\endcsname{with}
\expandafter\gdef\csname R@an.cv.tta.amos\endcsname{without}
\expandafter\gdef\csname R@an.cv.tta.kits\endcsname{without}
\expandafter\gdef\csname R@an.cv.tta.note\endcsname{inference without test-time mirroring on AMOS22 and KiTS23 and with it on ACDC}
\expandafter\gdef\csname R@an.cv.vram.cap\endcsname{12}
\expandafter\gdef\csname R@an.cv.vram.capnote\endcsname{the registered 12\,GB training-memory cap, read from the profile entries of the cross-validation arms and not a measured peak}
\expandafter\gdef\csname R@an.cv.xarm.V5B1.file\endcsname{cand\_V5B1\_leanadd.py}
\expandafter\gdef\csname R@an.cv.xarm.V5B1.name\endcsname{LeanDec with additive skips}
\expandafter\gdef\csname R@an.cv.xarm.V5B1.parents\endcsname{LeanDec}
\expandafter\gdef\csname R@an.cv.xarm.V5B1.registration\endcsname{Addendum AM}
\expandafter\gdef\csname R@an.cv.xarm.V5B2.file\endcsname{cand\_V5B2\_leanaddnext.py}
\expandafter\gdef\csname R@an.cv.xarm.V5B2.name\endcsname{LeanAdd with coarse large kernels}
\expandafter\gdef\csname R@an.cv.xarm.V5B2.parents\endcsname{LeanAdd and HyReX}
\expandafter\gdef\csname R@an.cv.xarm.V5B2.registration\endcsname{Addendum AM}
\expandafter\gdef\csname R@an.cv.xarm.V6A1r.file\endcsname{cand\_V6A1r\_k9coarse.py}
\expandafter\gdef\csname R@an.cv.xarm.V6A1r.name\endcsname{HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cv.xarm.V6A1r.parents\endcsname{HyReX}
\expandafter\gdef\csname R@an.cv.xarm.V6A1r.registration\endcsname{Addendum AO}
\expandafter\gdef\csname R@an.cv.xarm.V7A1.file\endcsname{cand\_V7A1\_deepmid.py}
\expandafter\gdef\csname R@an.cv.xarm.V7A1.name\endcsname{LeanAdd-NeXt with a deeper middle encoder}
\expandafter\gdef\csname R@an.cv.xarm.V7A1.parents\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.cv.xarm.V7A1.registration\endcsname{Addendum AP}
\expandafter\gdef\csname R@an.cv.xarm.V7A2.file\endcsname{cand\_V7A2\_finedec.py}
\expandafter\gdef\csname R@an.cv.xarm.V7A2.name\endcsname{LeanDeepMid with the finest decoder convolutions}
\expandafter\gdef\csname R@an.cv.xarm.V7A2.parents\endcsname{LeanDeepMid}
\expandafter\gdef\csname R@an.cv.xarm.V7A2.registration\endcsname{Addendum AW}
\expandafter\gdef\csname R@an.cv.xarm.V7B1.file\endcsname{cand\_V7B1\_leansep.py}
\expandafter\gdef\csname R@an.cv.xarm.V7B1.name\endcsname{LeanAdd-NeXt with separable coarse kernels}
\expandafter\gdef\csname R@an.cv.xarm.V7B1.parents\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.cv.xarm.V7B1.registration\endcsname{Addendum AQ}
\expandafter\gdef\csname R@an.cv.xarm.V7B2.file\endcsname{cand\_V7B2\_leandil.py}
\expandafter\gdef\csname R@an.cv.xarm.V7B2.name\endcsname{LeanAdd-NeXt with dilated coarse kernels}
\expandafter\gdef\csname R@an.cv.xarm.V7B2.parents\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.cv.xarm.V7B2.registration\endcsname{Addendum AQ}
\expandafter\gdef\csname R@an.cv.xarm.V7C1.file\endcsname{cand\_V7C1\_s5only.py}
\expandafter\gdef\csname R@an.cv.xarm.V7C1.name\endcsname{LeanAdd-NeXt with the coarse operator at stage 5 only}
\expandafter\gdef\csname R@an.cv.xarm.V7C1.parents\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.cv.xarm.V7C1.registration\endcsname{Addendum AP}
\expandafter\gdef\csname R@an.cv.xarm.V8B2.file\endcsname{cand\_V8B2\_stem1.py}
\expandafter\gdef\csname R@an.cv.xarm.V8B2.name\endcsname{LeanNeXt-s5 with one convolution at encoder stage 0}
\expandafter\gdef\csname R@an.cv.xarm.V8B2.parents\endcsname{none}
\expandafter\gdef\csname R@an.cv.xarm.V8B2.registration\endcsname{Addendum AY}
\expandafter\gdef\csname R@an.cv.xarms.n\endcsname{9}
\expandafter\gdef\csname R@an.cv.xarms.names\endcsname{LeanAdd, LeanAdd-NeXt, HyReX-k9, LeanDeepMid, LeanNeXt-s5, LeanSep, LeanDil, LeanDeepMid+FD and Stem1}
\expandafter\gdef\csname R@an.cv.xarms.tags\endcsname{V5B1, V5B2, V6A1r, V7A1, V7C1, V7B1, V7B2, V7A2, V8B2}
\makeatother


==> an_extra_hyp.tex <==
%% AUTO-GENERATED by paper_v2_8p/hyp_keys.py -- do not edit by hand
\makeatletter
\expandafter\gdef\csname R@hyp.abs.d2.eso\endcsname{1.05}
\expandafter\gdef\csname R@hyp.abs.d2.liv\endcsname{0.02}
\expandafter\gdef\csname R@hyp.abs.kits.M\endcsname{1.63}
\expandafter\gdef\csname R@hyp.abs.r4.inc\endcsname{0.94}
\expandafter\gdef\csname R@hyp.abs.r4.inc.s0\endcsname{1.07}
\expandafter\gdef\csname R@hyp.acc.post.dk.med\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@hyp.acc.post.inb\endcsname{8}
\expandafter\gdef\csname R@hyp.acc.post.n\endcsname{13}
\expandafter\gdef\csname R@hyp.acc.post.step.med\endcsname{0.84}
\expandafter\gdef\csname R@hyp.acc.pre.dk.med\endcsname{\ensuremath{+1.84}}
\expandafter\gdef\csname R@hyp.acc.pre.inb\endcsname{0}
\expandafter\gdef\csname R@hyp.acc.pre.n\endcsname{10}
\expandafter\gdef\csname R@hyp.acc.pre.step.med\endcsname{1.21}
\expandafter\gdef\csname R@hyp.bm.acdc.L1.d\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@hyp.bm.acdc.L1.dhd95\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@hyp.bm.acdc.L1.dice\endcsname{91.38}
\expandafter\gdef\csname R@hyp.bm.acdc.L1.dmax\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@hyp.bm.acdc.L1.dnsd1\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@hyp.bm.acdc.L1.dnsd2\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@hyp.bm.acdc.L1.hd95\endcsname{4.1}
\expandafter\gdef\csname R@hyp.bm.acdc.L1.hi\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@hyp.bm.acdc.L1.lo\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@hyp.bm.acdc.L1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.acdc.L1.nsd1\endcsname{78.33}
\expandafter\gdef\csname R@hyp.bm.acdc.L1.nsd2\endcsname{93.06}
\expandafter\gdef\csname R@hyp.bm.acdc.L1.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.acdc.L1.se\endcsname{0.04}
\expandafter\gdef\csname R@hyp.bm.acdc.L1S.d\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@hyp.bm.acdc.L1S.dhd95\endcsname{0.0}
\expandafter\gdef\csname R@hyp.bm.acdc.L1S.dice\endcsname{91.01}
\expandafter\gdef\csname R@hyp.bm.acdc.L1S.dmax\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@hyp.bm.acdc.L1S.dnsd1\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@hyp.bm.acdc.L1S.dnsd2\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@hyp.bm.acdc.L1S.hd95\endcsname{4.0}
\expandafter\gdef\csname R@hyp.bm.acdc.L1S.hi\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@hyp.bm.acdc.L1S.lo\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@hyp.bm.acdc.L1S.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.acdc.L1S.nsd1\endcsname{77.49}
\expandafter\gdef\csname R@hyp.bm.acdc.L1S.nsd2\endcsname{92.39}
\expandafter\gdef\csname R@hyp.bm.acdc.L1S.nup\endcsname{2}
\expandafter\gdef\csname R@hyp.bm.acdc.L1S.se\endcsname{0.07}
\expandafter\gdef\csname R@hyp.bm.acdc.L3.d\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@hyp.bm.acdc.L3.dhd95\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@hyp.bm.acdc.L3.dice\endcsname{91.28}
\expandafter\gdef\csname R@hyp.bm.acdc.L3.dmax\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@hyp.bm.acdc.L3.dnsd1\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@hyp.bm.acdc.L3.dnsd2\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@hyp.bm.acdc.L3.hd95\endcsname{3.9}
\expandafter\gdef\csname R@hyp.bm.acdc.L3.hi\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@hyp.bm.acdc.L3.lo\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@hyp.bm.acdc.L3.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.acdc.L3.nsd1\endcsname{78.07}
\expandafter\gdef\csname R@hyp.bm.acdc.L3.nsd2\endcsname{92.73}
\expandafter\gdef\csname R@hyp.bm.acdc.L3.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.acdc.L3.se\endcsname{0.05}
\expandafter\gdef\csname R@hyp.bm.acdc.P3c.d\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@hyp.bm.acdc.P3c.dhd95\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@hyp.bm.acdc.P3c.dice\endcsname{90.85}
\expandafter\gdef\csname R@hyp.bm.acdc.P3c.dmax\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@hyp.bm.acdc.P3c.dnsd1\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@hyp.bm.acdc.P3c.dnsd2\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@hyp.bm.acdc.P3c.hd95\endcsname{3.9}
\expandafter\gdef\csname R@hyp.bm.acdc.P3c.hi\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@hyp.bm.acdc.P3c.lo\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@hyp.bm.acdc.P3c.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.acdc.P3c.nsd1\endcsname{77.20}
\expandafter\gdef\csname R@hyp.bm.acdc.P3c.nsd2\endcsname{92.07}
\expandafter\gdef\csname R@hyp.bm.acdc.P3c.nup\endcsname{2}
\expandafter\gdef\csname R@hyp.bm.acdc.P3c.se\endcsname{0.08}
\expandafter\gdef\csname R@hyp.bm.acdc.V5B1.d\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@hyp.bm.acdc.V5B1.dhd95\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@hyp.bm.acdc.V5B1.dice\endcsname{90.82}
\expandafter\gdef\csname R@hyp.bm.acdc.V5B1.dmax\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@hyp.bm.acdc.V5B1.dnsd1\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@hyp.bm.acdc.V5B1.dnsd2\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@hyp.bm.acdc.V5B1.hd95\endcsname{4.4}
\expandafter\gdef\csname R@hyp.bm.acdc.V5B1.hi\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@hyp.bm.acdc.V5B1.lo\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@hyp.bm.acdc.V5B1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.acdc.V5B1.nsd1\endcsname{77.06}
\expandafter\gdef\csname R@hyp.bm.acdc.V5B1.nsd2\endcsname{92.05}
\expandafter\gdef\csname R@hyp.bm.acdc.V5B1.nup\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.acdc.V5B1.se\endcsname{0.08}
\expandafter\gdef\csname R@hyp.bm.acdc.V7A1.d\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@hyp.bm.acdc.V7A1.dhd95\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@hyp.bm.acdc.V7A1.dice\endcsname{91.11}
\expandafter\gdef\csname R@hyp.bm.acdc.V7A1.dmax\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@hyp.bm.acdc.V7A1.dnsd1\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@hyp.bm.acdc.V7A1.dnsd2\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@hyp.bm.acdc.V7A1.hd95\endcsname{4.6}
\expandafter\gdef\csname R@hyp.bm.acdc.V7A1.hi\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@hyp.bm.acdc.V7A1.lo\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@hyp.bm.acdc.V7A1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.acdc.V7A1.nsd1\endcsname{77.72}
\expandafter\gdef\csname R@hyp.bm.acdc.V7A1.nsd2\endcsname{92.69}
\expandafter\gdef\csname R@hyp.bm.acdc.V7A1.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.acdc.V7A1.se\endcsname{0.15}
\expandafter\gdef\csname R@hyp.bm.acdc.V7C1.d\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@hyp.bm.acdc.V7C1.dhd95\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@hyp.bm.acdc.V7C1.dice\endcsname{90.83}
\expandafter\gdef\csname R@hyp.bm.acdc.V7C1.dmax\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@hyp.bm.acdc.V7C1.dnsd1\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@hyp.bm.acdc.V7C1.dnsd2\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@hyp.bm.acdc.V7C1.hd95\endcsname{4.3}
\expandafter\gdef\csname R@hyp.bm.acdc.V7C1.hi\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@hyp.bm.acdc.V7C1.lo\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@hyp.bm.acdc.V7C1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.acdc.V7C1.nsd1\endcsname{77.22}
\expandafter\gdef\csname R@hyp.bm.acdc.V7C1.nsd2\endcsname{92.21}
\expandafter\gdef\csname R@hyp.bm.acdc.V7C1.nup\endcsname{0}
\expandafter\gdef\csname R@hyp.bm.acdc.V7C1.se\endcsname{0.03}
\expandafter\gdef\csname R@hyp.bm.acdc.V9R2.d\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@hyp.bm.acdc.V9R2.dhd95\endcsname{0.0}
\expandafter\gdef\csname R@hyp.bm.acdc.V9R2.dice\endcsname{91.07}
\expandafter\gdef\csname R@hyp.bm.acdc.V9R2.dmax\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@hyp.bm.acdc.V9R2.dnsd1\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@hyp.bm.acdc.V9R2.dnsd2\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@hyp.bm.acdc.V9R2.hd95\endcsname{3.9}
\expandafter\gdef\csname R@hyp.bm.acdc.V9R2.hi\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@hyp.bm.acdc.V9R2.lo\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@hyp.bm.acdc.V9R2.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.acdc.V9R2.nsd1\endcsname{77.56}
\expandafter\gdef\csname R@hyp.bm.acdc.V9R2.nsd2\endcsname{92.59}
\expandafter\gdef\csname R@hyp.bm.acdc.V9R2.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.acdc.V9R2.se\endcsname{0.12}
\expandafter\gdef\csname R@hyp.bm.acdc.base.dice\endcsname{90.94}
\expandafter\gdef\csname R@hyp.bm.acdc.base.hd95\endcsname{4.0}
\expandafter\gdef\csname R@hyp.bm.acdc.base.nsd1\endcsname{77.37}
\expandafter\gdef\csname R@hyp.bm.acdc.base.nsd2\endcsname{92.24}
\expandafter\gdef\csname R@hyp.bm.amos.H1.d\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@hyp.bm.amos.H1.dhd95\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@hyp.bm.amos.H1.dice\endcsname{88.63}
\expandafter\gdef\csname R@hyp.bm.amos.H1.dmax\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@hyp.bm.amos.H1.dnsd1\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@hyp.bm.amos.H1.dnsd2\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@hyp.bm.amos.H1.hd95\endcsname{11.5}
\expandafter\gdef\csname R@hyp.bm.amos.H1.hi\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@hyp.bm.amos.H1.lo\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@hyp.bm.amos.H1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.amos.H1.nsd1\endcsname{82.09}
\expandafter\gdef\csname R@hyp.bm.amos.H1.nsd2\endcsname{89.90}
\expandafter\gdef\csname R@hyp.bm.amos.H1.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.amos.H1.se\endcsname{0.24}
\expandafter\gdef\csname R@hyp.bm.amos.L1.d\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@hyp.bm.amos.L1.dhd95\endcsname{\ensuremath{-1.1}}
\expandafter\gdef\csname R@hyp.bm.amos.L1.dice\endcsname{88.75}
\expandafter\gdef\csname R@hyp.bm.amos.L1.dmax\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@hyp.bm.amos.L1.dnsd1\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@hyp.bm.amos.L1.dnsd2\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@hyp.bm.amos.L1.hd95\endcsname{11.0}
\expandafter\gdef\csname R@hyp.bm.amos.L1.hi\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@hyp.bm.amos.L1.lo\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@hyp.bm.amos.L1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.amos.L1.nsd1\endcsname{82.26}
\expandafter\gdef\csname R@hyp.bm.amos.L1.nsd2\endcsname{90.08}
\expandafter\gdef\csname R@hyp.bm.amos.L1.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.amos.L1.se\endcsname{0.21}
\expandafter\gdef\csname R@hyp.bm.amos.L1S.d\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@hyp.bm.amos.L1S.dice\endcsname{88.11}
\expandafter\gdef\csname R@hyp.bm.amos.L1S.dmax\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@hyp.bm.amos.L1S.hi\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@hyp.bm.amos.L1S.lo\endcsname{\ensuremath{-0.82}}
\expandafter\gdef\csname R@hyp.bm.amos.L1S.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.amos.L1S.nup\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.amos.L1S.se\endcsname{0.18}
\expandafter\gdef\csname R@hyp.bm.amos.L3.d\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@hyp.bm.amos.L3.dhd95\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@hyp.bm.amos.L3.dice\endcsname{88.58}
\expandafter\gdef\csname R@hyp.bm.amos.L3.dmax\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@hyp.bm.amos.L3.dnsd1\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@hyp.bm.amos.L3.dnsd2\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@hyp.bm.amos.L3.hd95\endcsname{12.6}
\expandafter\gdef\csname R@hyp.bm.amos.L3.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@hyp.bm.amos.L3.lo\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@hyp.bm.amos.L3.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.amos.L3.nsd1\endcsname{81.97}
\expandafter\gdef\csname R@hyp.bm.amos.L3.nsd2\endcsname{89.79}
\expandafter\gdef\csname R@hyp.bm.amos.L3.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.amos.L3.se\endcsname{0.10}
\expandafter\gdef\csname R@hyp.bm.amos.MedNeXtM.d\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@hyp.bm.amos.MedNeXtM.dhd95\endcsname{\ensuremath{-0.4}}
\expandafter\gdef\csname R@hyp.bm.amos.MedNeXtM.dice\endcsname{88.89}
\expandafter\gdef\csname R@hyp.bm.amos.MedNeXtM.dmax\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@hyp.bm.amos.MedNeXtM.dnsd1\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@hyp.bm.amos.MedNeXtM.dnsd2\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@hyp.bm.amos.MedNeXtM.hd95\endcsname{11.6}
\expandafter\gdef\csname R@hyp.bm.amos.MedNeXtM.hi\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@hyp.bm.amos.MedNeXtM.lo\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@hyp.bm.amos.MedNeXtM.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.amos.MedNeXtM.nsd1\endcsname{82.39}
\expandafter\gdef\csname R@hyp.bm.amos.MedNeXtM.nsd2\endcsname{90.20}
\expandafter\gdef\csname R@hyp.bm.amos.MedNeXtM.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.amos.MedNeXtM.se\endcsname{0.16}
\expandafter\gdef\csname R@hyp.bm.amos.P3c.d\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@hyp.bm.amos.P3c.dice\endcsname{88.32}
\expandafter\gdef\csname R@hyp.bm.amos.P3c.dmax\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@hyp.bm.amos.P3c.hi\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@hyp.bm.amos.P3c.lo\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@hyp.bm.amos.P3c.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.amos.P3c.nup\endcsname{2}
\expandafter\gdef\csname R@hyp.bm.amos.P3c.se\endcsname{0.17}
\expandafter\gdef\csname R@hyp.bm.amos.V10B.d\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@hyp.bm.amos.V10B.dhd95\endcsname{\ensuremath{-0.5}}
\expandafter\gdef\csname R@hyp.bm.amos.V10B.dice\endcsname{88.56}
\expandafter\gdef\csname R@hyp.bm.amos.V10B.dmax\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@hyp.bm.amos.V10B.dnsd1\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@hyp.bm.amos.V10B.dnsd2\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@hyp.bm.amos.V10B.hd95\endcsname{11.6}
\expandafter\gdef\csname R@hyp.bm.amos.V10B.hi\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@hyp.bm.amos.V10B.lo\endcsname{\ensuremath{-0.55}}
\expandafter\gdef\csname R@hyp.bm.amos.V10B.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.amos.V10B.nsd1\endcsname{81.73}
\expandafter\gdef\csname R@hyp.bm.amos.V10B.nsd2\endcsname{89.72}
\expandafter\gdef\csname R@hyp.bm.amos.V10B.nup\endcsname{2}
\expandafter\gdef\csname R@hyp.bm.amos.V10B.se\endcsname{0.24}
\expandafter\gdef\csname R@hyp.bm.amos.V5B1.d\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@hyp.bm.amos.V5B1.dice\endcsname{87.89}
\expandafter\gdef\csname R@hyp.bm.amos.V5B1.dmax\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@hyp.bm.amos.V5B1.hi\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@hyp.bm.amos.V5B1.lo\endcsname{\ensuremath{-0.82}}
\expandafter\gdef\csname R@hyp.bm.amos.V5B1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.amos.V5B1.nup\endcsname{0}
\expandafter\gdef\csname R@hyp.bm.amos.V5B1.se\endcsname{0.11}
\expandafter\gdef\csname R@hyp.bm.amos.V7A1.d\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@hyp.bm.amos.V7A1.dhd95\endcsname{\ensuremath{-1.7}}
\expandafter\gdef\csname R@hyp.bm.amos.V7A1.dice\endcsname{88.61}
\expandafter\gdef\csname R@hyp.bm.amos.V7A1.dmax\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@hyp.bm.amos.V7A1.dnsd1\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@hyp.bm.amos.V7A1.dnsd2\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@hyp.bm.amos.V7A1.hd95\endcsname{10.4}
\expandafter\gdef\csname R@hyp.bm.amos.V7A1.hi\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@hyp.bm.amos.V7A1.lo\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@hyp.bm.amos.V7A1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.amos.V7A1.nsd1\endcsname{81.86}
\expandafter\gdef\csname R@hyp.bm.amos.V7A1.nsd2\endcsname{89.85}
\expandafter\gdef\csname R@hyp.bm.amos.V7A1.nup\endcsname{2}
\expandafter\gdef\csname R@hyp.bm.amos.V7A1.se\endcsname{0.24}
\expandafter\gdef\csname R@hyp.bm.amos.V7C1.d\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@hyp.bm.amos.V7C1.dhd95\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@hyp.bm.amos.V7C1.dice\endcsname{87.89}
\expandafter\gdef\csname R@hyp.bm.amos.V7C1.dmax\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@hyp.bm.amos.V7C1.dnsd1\endcsname{\ensuremath{-0.71}}
\expandafter\gdef\csname R@hyp.bm.amos.V7C1.dnsd2\endcsname{\ensuremath{-0.54}}
\expandafter\gdef\csname R@hyp.bm.amos.V7C1.hd95\endcsname{12.5}
\expandafter\gdef\csname R@hyp.bm.amos.V7C1.hi\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@hyp.bm.amos.V7C1.lo\endcsname{\ensuremath{-0.81}}
\expandafter\gdef\csname R@hyp.bm.amos.V7C1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.amos.V7C1.nsd1\endcsname{80.83}
\expandafter\gdef\csname R@hyp.bm.amos.V7C1.nsd2\endcsname{88.90}
\expandafter\gdef\csname R@hyp.bm.amos.V7C1.nup\endcsname{0}
\expandafter\gdef\csname R@hyp.bm.amos.V7C1.se\endcsname{0.11}
\expandafter\gdef\csname R@hyp.bm.amos.V7L.d\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@hyp.bm.amos.V7L.dhd95\endcsname{\ensuremath{-1.4}}
\expandafter\gdef\csname R@hyp.bm.amos.V7L.dice\endcsname{88.77}
\expandafter\gdef\csname R@hyp.bm.amos.V7L.dmax\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@hyp.bm.amos.V7L.dnsd1\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@hyp.bm.amos.V7L.dnsd2\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@hyp.bm.amos.V7L.hd95\endcsname{10.7}
\expandafter\gdef\csname R@hyp.bm.amos.V7L.hi\endcsname{\ensuremath{+1.20}}
\expandafter\gdef\csname R@hyp.bm.amos.V7L.lo\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@hyp.bm.amos.V7L.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.amos.V7L.nsd1\endcsname{82.17}
\expandafter\gdef\csname R@hyp.bm.amos.V7L.nsd2\endcsname{90.08}
\expandafter\gdef\csname R@hyp.bm.amos.V7L.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.amos.V7L.se\endcsname{0.24}
\expandafter\gdef\csname R@hyp.bm.amos.V9R2.d\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@hyp.bm.amos.V9R2.dhd95\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@hyp.bm.amos.V9R2.dice\endcsname{88.51}
\expandafter\gdef\csname R@hyp.bm.amos.V9R2.dmax\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@hyp.bm.amos.V9R2.dnsd1\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@hyp.bm.amos.V9R2.dnsd2\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@hyp.bm.amos.V9R2.hd95\endcsname{11.5}
\expandafter\gdef\csname R@hyp.bm.amos.V9R2.hi\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@hyp.bm.amos.V9R2.lo\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@hyp.bm.amos.V9R2.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.amos.V9R2.nsd1\endcsname{81.69}
\expandafter\gdef\csname R@hyp.bm.amos.V9R2.nsd2\endcsname{89.69}
\expandafter\gdef\csname R@hyp.bm.amos.V9R2.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.amos.V9R2.se\endcsname{0.19}
\expandafter\gdef\csname R@hyp.bm.amos.Y13.d\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@hyp.bm.amos.Y13.dhd95\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@hyp.bm.amos.Y13.dice\endcsname{88.56}
\expandafter\gdef\csname R@hyp.bm.amos.Y13.dmax\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@hyp.bm.amos.Y13.dnsd1\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@hyp.bm.amos.Y13.dnsd2\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@hyp.bm.amos.Y13.hd95\endcsname{13.0}
\expandafter\gdef\csname R@hyp.bm.amos.Y13.hi\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@hyp.bm.amos.Y13.lo\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@hyp.bm.amos.Y13.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.amos.Y13.nsd1\endcsname{81.84}
\expandafter\gdef\csname R@hyp.bm.amos.Y13.nsd2\endcsname{89.77}
\expandafter\gdef\csname R@hyp.bm.amos.Y13.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.amos.Y13.se\endcsname{0.22}
\expandafter\gdef\csname R@hyp.bm.amos.Y2.d\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@hyp.bm.amos.Y2.dhd95\endcsname{\ensuremath{-1.0}}
\expandafter\gdef\csname R@hyp.bm.amos.Y2.dice\endcsname{88.57}
\expandafter\gdef\csname R@hyp.bm.amos.Y2.dmax\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@hyp.bm.amos.Y2.dnsd1\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@hyp.bm.amos.Y2.dnsd2\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@hyp.bm.amos.Y2.hd95\endcsname{11.1}
\expandafter\gdef\csname R@hyp.bm.amos.Y2.hi\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@hyp.bm.amos.Y2.lo\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@hyp.bm.amos.Y2.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.amos.Y2.nsd1\endcsname{81.84}
\expandafter\gdef\csname R@hyp.bm.amos.Y2.nsd2\endcsname{89.78}
\expandafter\gdef\csname R@hyp.bm.amos.Y2.nup\endcsname{2}
\expandafter\gdef\csname R@hyp.bm.amos.Y2.se\endcsname{0.22}
\expandafter\gdef\csname R@hyp.bm.amos.base.dice\endcsname{88.35}
\expandafter\gdef\csname R@hyp.bm.amos.base.hd95\endcsname{12.1}
\expandafter\gdef\csname R@hyp.bm.amos.base.nsd1\endcsname{81.54}
\expandafter\gdef\csname R@hyp.bm.amos.base.nsd2\endcsname{89.44}
\expandafter\gdef\csname R@hyp.bm.brats.L1.d\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@hyp.bm.brats.L1.dice\endcsname{82.95}
\expandafter\gdef\csname R@hyp.bm.brats.L1.dmax\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@hyp.bm.brats.L1.n\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.L1.nup\endcsname{0}
\expandafter\gdef\csname R@hyp.bm.brats.L1S.d\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@hyp.bm.brats.L1S.dhd95\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@hyp.bm.brats.L1S.dice\endcsname{82.80}
\expandafter\gdef\csname R@hyp.bm.brats.L1S.dmax\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@hyp.bm.brats.L1S.dnsd1\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@hyp.bm.brats.L1S.dnsd2\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@hyp.bm.brats.L1S.hd95\endcsname{11.4}
\expandafter\gdef\csname R@hyp.bm.brats.L1S.n\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.L1S.nsd1\endcsname{75.14}
\expandafter\gdef\csname R@hyp.bm.brats.L1S.nsd2\endcsname{84.92}
\expandafter\gdef\csname R@hyp.bm.brats.L1S.nup\endcsname{0}
\expandafter\gdef\csname R@hyp.bm.brats.L3.d\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@hyp.bm.brats.L3.dice\endcsname{83.05}
\expandafter\gdef\csname R@hyp.bm.brats.L3.dmax\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@hyp.bm.brats.L3.n\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.L3.nup\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.V10B.d\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@hyp.bm.brats.V10B.dhd95\endcsname{\ensuremath{-1.5}}
\expandafter\gdef\csname R@hyp.bm.brats.V10B.dice\endcsname{83.19}
\expandafter\gdef\csname R@hyp.bm.brats.V10B.dmax\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@hyp.bm.brats.V10B.dnsd1\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@hyp.bm.brats.V10B.dnsd2\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@hyp.bm.brats.V10B.hd95\endcsname{10.1}
\expandafter\gdef\csname R@hyp.bm.brats.V10B.n\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.V10B.nsd1\endcsname{75.74}
\expandafter\gdef\csname R@hyp.bm.brats.V10B.nsd2\endcsname{85.45}
\expandafter\gdef\csname R@hyp.bm.brats.V10B.nup\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.V11.d\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@hyp.bm.brats.V11.dhd95\endcsname{\ensuremath{-0.7}}
\expandafter\gdef\csname R@hyp.bm.brats.V11.dice\endcsname{83.10}
\expandafter\gdef\csname R@hyp.bm.brats.V11.dmax\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@hyp.bm.brats.V11.dnsd1\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@hyp.bm.brats.V11.dnsd2\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@hyp.bm.brats.V11.hd95\endcsname{10.8}
\expandafter\gdef\csname R@hyp.bm.brats.V11.n\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.V11.nsd1\endcsname{75.36}
\expandafter\gdef\csname R@hyp.bm.brats.V11.nsd2\endcsname{85.28}
\expandafter\gdef\csname R@hyp.bm.brats.V11.nup\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.V7A1.d\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@hyp.bm.brats.V7A1.dhd95\endcsname{\ensuremath{-1.7}}
\expandafter\gdef\csname R@hyp.bm.brats.V7A1.dice\endcsname{83.21}
\expandafter\gdef\csname R@hyp.bm.brats.V7A1.dmax\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@hyp.bm.brats.V7A1.dnsd1\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@hyp.bm.brats.V7A1.dnsd2\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@hyp.bm.brats.V7A1.hd95\endcsname{9.9}
\expandafter\gdef\csname R@hyp.bm.brats.V7A1.n\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.V7A1.nsd1\endcsname{75.64}
\expandafter\gdef\csname R@hyp.bm.brats.V7A1.nsd2\endcsname{85.45}
\expandafter\gdef\csname R@hyp.bm.brats.V7A1.nup\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.V7C1.d\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@hyp.bm.brats.V7C1.dice\endcsname{83.12}
\expandafter\gdef\csname R@hyp.bm.brats.V7C1.dmax\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@hyp.bm.brats.V7C1.n\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.V7C1.nup\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.Y11.d\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@hyp.bm.brats.Y11.dhd95\endcsname{\ensuremath{-1.8}}
\expandafter\gdef\csname R@hyp.bm.brats.Y11.dice\endcsname{82.95}
\expandafter\gdef\csname R@hyp.bm.brats.Y11.dmax\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@hyp.bm.brats.Y11.dnsd1\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@hyp.bm.brats.Y11.dnsd2\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@hyp.bm.brats.Y11.hd95\endcsname{9.7}
\expandafter\gdef\csname R@hyp.bm.brats.Y11.n\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.Y11.nsd1\endcsname{75.15}
\expandafter\gdef\csname R@hyp.bm.brats.Y11.nsd2\endcsname{85.05}
\expandafter\gdef\csname R@hyp.bm.brats.Y11.nup\endcsname{0}
\expandafter\gdef\csname R@hyp.bm.brats.Y12.d\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@hyp.bm.brats.Y12.dhd95\endcsname{\ensuremath{+3.8}}
\expandafter\gdef\csname R@hyp.bm.brats.Y12.dice\endcsname{82.74}
\expandafter\gdef\csname R@hyp.bm.brats.Y12.dmax\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@hyp.bm.brats.Y12.dnsd1\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@hyp.bm.brats.Y12.dnsd2\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@hyp.bm.brats.Y12.hd95\endcsname{15.4}
\expandafter\gdef\csname R@hyp.bm.brats.Y12.n\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.Y12.nsd1\endcsname{75.08}
\expandafter\gdef\csname R@hyp.bm.brats.Y12.nsd2\endcsname{84.74}
\expandafter\gdef\csname R@hyp.bm.brats.Y12.nup\endcsname{0}
\expandafter\gdef\csname R@hyp.bm.brats.Y13.d\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@hyp.bm.brats.Y13.dhd95\endcsname{\ensuremath{-1.6}}
\expandafter\gdef\csname R@hyp.bm.brats.Y13.dice\endcsname{82.87}
\expandafter\gdef\csname R@hyp.bm.brats.Y13.dmax\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@hyp.bm.brats.Y13.dnsd1\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@hyp.bm.brats.Y13.dnsd2\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@hyp.bm.brats.Y13.hd95\endcsname{9.9}
\expandafter\gdef\csname R@hyp.bm.brats.Y13.n\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.Y13.nsd1\endcsname{75.29}
\expandafter\gdef\csname R@hyp.bm.brats.Y13.nsd2\endcsname{84.88}
\expandafter\gdef\csname R@hyp.bm.brats.Y13.nup\endcsname{0}
\expandafter\gdef\csname R@hyp.bm.brats.Y14.d\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@hyp.bm.brats.Y14.dice\endcsname{83.12}
\expandafter\gdef\csname R@hyp.bm.brats.Y14.dmax\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@hyp.bm.brats.Y14.n\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.Y14.nup\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.Y2.d\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@hyp.bm.brats.Y2.dhd95\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@hyp.bm.brats.Y2.dice\endcsname{82.95}
\expandafter\gdef\csname R@hyp.bm.brats.Y2.dmax\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@hyp.bm.brats.Y2.dnsd1\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@hyp.bm.brats.Y2.dnsd2\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@hyp.bm.brats.Y2.hd95\endcsname{11.8}
\expandafter\gdef\csname R@hyp.bm.brats.Y2.n\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.Y2.nsd1\endcsname{75.30}
\expandafter\gdef\csname R@hyp.bm.brats.Y2.nsd2\endcsname{85.06}
\expandafter\gdef\csname R@hyp.bm.brats.Y2.nup\endcsname{0}
\expandafter\gdef\csname R@hyp.bm.brats.Y6.d\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@hyp.bm.brats.Y6.dhd95\endcsname{\ensuremath{-2.6}}
\expandafter\gdef\csname R@hyp.bm.brats.Y6.dice\endcsname{82.87}
\expandafter\gdef\csname R@hyp.bm.brats.Y6.dmax\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@hyp.bm.brats.Y6.dnsd1\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@hyp.bm.brats.Y6.dnsd2\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@hyp.bm.brats.Y6.hd95\endcsname{9.0}
\expandafter\gdef\csname R@hyp.bm.brats.Y6.n\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.Y6.nsd1\endcsname{75.10}
\expandafter\gdef\csname R@hyp.bm.brats.Y6.nsd2\endcsname{84.98}
\expandafter\gdef\csname R@hyp.bm.brats.Y6.nup\endcsname{0}
\expandafter\gdef\csname R@hyp.bm.brats.Y7.d\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@hyp.bm.brats.Y7.dhd95\endcsname{\ensuremath{-1.6}}
\expandafter\gdef\csname R@hyp.bm.brats.Y7.dice\endcsname{83.31}
\expandafter\gdef\csname R@hyp.bm.brats.Y7.dmax\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@hyp.bm.brats.Y7.dnsd1\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@hyp.bm.brats.Y7.dnsd2\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@hyp.bm.brats.Y7.hd95\endcsname{10.0}
\expandafter\gdef\csname R@hyp.bm.brats.Y7.n\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.Y7.nsd1\endcsname{75.65}
\expandafter\gdef\csname R@hyp.bm.brats.Y7.nsd2\endcsname{85.58}
\expandafter\gdef\csname R@hyp.bm.brats.Y7.nup\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.brats.base.dice\endcsname{82.98}
\expandafter\gdef\csname R@hyp.bm.brats.base.hd95\endcsname{11.6}
\expandafter\gdef\csname R@hyp.bm.brats.base.nsd1\endcsname{75.38}
\expandafter\gdef\csname R@hyp.bm.brats.base.nsd2\endcsname{85.12}
\expandafter\gdef\csname R@hyp.bm.btcv.L1.d\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@hyp.bm.btcv.L1.dhd95\endcsname{\ensuremath{-2.5}}
\expandafter\gdef\csname R@hyp.bm.btcv.L1.dice\endcsname{78.52}
\expandafter\gdef\csname R@hyp.bm.btcv.L1.dmax\endcsname{\ensuremath{+1.67}}
\expandafter\gdef\csname R@hyp.bm.btcv.L1.dnsd1\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@hyp.bm.btcv.L1.dnsd2\endcsname{\ensuremath{+0.95}}
\expandafter\gdef\csname R@hyp.bm.btcv.L1.hd95\endcsname{34.9}
\expandafter\gdef\csname R@hyp.bm.btcv.L1.hi\endcsname{\ensuremath{+2.80}}
\expandafter\gdef\csname R@hyp.bm.btcv.L1.lo\endcsname{\ensuremath{-1.39}}
\expandafter\gdef\csname R@hyp.bm.btcv.L1.n\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.btcv.L1.nsd1\endcsname{70.20}
\expandafter\gdef\csname R@hyp.bm.btcv.L1.nsd2\endcsname{78.59}
\expandafter\gdef\csname R@hyp.bm.btcv.L1.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.btcv.L1.se\endcsname{0.49}
\expandafter\gdef\csname R@hyp.bm.btcv.L3.d\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@hyp.bm.btcv.L3.dice\endcsname{78.53}
\expandafter\gdef\csname R@hyp.bm.btcv.L3.dmax\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@hyp.bm.btcv.L3.hi\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@hyp.bm.btcv.L3.lo\endcsname{\ensuremath{-1.18}}
\expandafter\gdef\csname R@hyp.bm.btcv.L3.n\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.btcv.L3.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.btcv.L3.se\endcsname{0.44}
\expandafter\gdef\csname R@hyp.bm.btcv.V7A1.d\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@hyp.bm.btcv.V7A1.dhd95\endcsname{\ensuremath{+1.7}}
\expandafter\gdef\csname R@hyp.bm.btcv.V7A1.dice\endcsname{78.30}
\expandafter\gdef\csname R@hyp.bm.btcv.V7A1.dmax\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@hyp.bm.btcv.V7A1.dnsd1\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@hyp.bm.btcv.V7A1.dnsd2\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@hyp.bm.btcv.V7A1.hd95\endcsname{39.0}
\expandafter\gdef\csname R@hyp.bm.btcv.V7A1.hi\endcsname{\ensuremath{+1.42}}
\expandafter\gdef\csname R@hyp.bm.btcv.V7A1.lo\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@hyp.bm.btcv.V7A1.n\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.btcv.V7A1.nsd1\endcsname{69.67}
\expandafter\gdef\csname R@hyp.bm.btcv.V7A1.nsd2\endcsname{78.21}
\expandafter\gdef\csname R@hyp.bm.btcv.V7A1.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.btcv.V7A1.panc.d\endcsname{\ensuremath{+5.85}}
\expandafter\gdef\csname R@hyp.bm.btcv.V7A1.se\endcsname{0.22}
\expandafter\gdef\csname R@hyp.bm.btcv.V7C1.d\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@hyp.bm.btcv.V7C1.dhd95\endcsname{\ensuremath{-10.6}}
\expandafter\gdef\csname R@hyp.bm.btcv.V7C1.dice\endcsname{77.50}
\expandafter\gdef\csname R@hyp.bm.btcv.V7C1.dmax\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@hyp.bm.btcv.V7C1.dnsd1\endcsname{\ensuremath{-0.72}}
\expandafter\gdef\csname R@hyp.bm.btcv.V7C1.dnsd2\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@hyp.bm.btcv.V7C1.hd95\endcsname{26.7}
\expandafter\gdef\csname R@hyp.bm.btcv.V7C1.hi\endcsname{\ensuremath{+0.91}}
\expandafter\gdef\csname R@hyp.bm.btcv.V7C1.lo\endcsname{\ensuremath{-1.55}}
\expandafter\gdef\csname R@hyp.bm.btcv.V7C1.n\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.btcv.V7C1.nsd1\endcsname{68.73}
\expandafter\gdef\csname R@hyp.bm.btcv.V7C1.nsd2\endcsname{77.34}
\expandafter\gdef\csname R@hyp.bm.btcv.V7C1.nup\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.btcv.V7C1.se\endcsname{0.29}
\expandafter\gdef\csname R@hyp.bm.btcv.Y13.d\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@hyp.bm.btcv.Y13.dhd95\endcsname{\ensuremath{-1.7}}
\expandafter\gdef\csname R@hyp.bm.btcv.Y13.dice\endcsname{78.43}
\expandafter\gdef\csname R@hyp.bm.btcv.Y13.dmax\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@hyp.bm.btcv.Y13.dnsd1\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@hyp.bm.btcv.Y13.dnsd2\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@hyp.bm.btcv.Y13.hd95\endcsname{35.6}
\expandafter\gdef\csname R@hyp.bm.btcv.Y13.hi\endcsname{\ensuremath{+2.46}}
\expandafter\gdef\csname R@hyp.bm.btcv.Y13.lo\endcsname{\ensuremath{-1.23}}
\expandafter\gdef\csname R@hyp.bm.btcv.Y13.n\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.btcv.Y13.nsd1\endcsname{69.79}
\expandafter\gdef\csname R@hyp.bm.btcv.Y13.nsd2\endcsname{78.33}
\expandafter\gdef\csname R@hyp.bm.btcv.Y13.nup\endcsname{2}
\expandafter\gdef\csname R@hyp.bm.btcv.Y13.se\endcsname{0.43}
\expandafter\gdef\csname R@hyp.bm.btcv.base.dice\endcsname{77.82}
\expandafter\gdef\csname R@hyp.bm.btcv.base.hd95\endcsname{37.4}
\expandafter\gdef\csname R@hyp.bm.btcv.base.nsd1\endcsname{69.45}
\expandafter\gdef\csname R@hyp.bm.btcv.base.nsd2\endcsname{77.64}
\expandafter\gdef\csname R@hyp.bm.heart.V5B1g.d\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@hyp.bm.heart.V5B1g.dhd95\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@hyp.bm.heart.V5B1g.dice\endcsname{93.22}
\expandafter\gdef\csname R@hyp.bm.heart.V5B1g.dmax\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@hyp.bm.heart.V5B1g.dnsd1\endcsname{\ensuremath{-0.90}}
\expandafter\gdef\csname R@hyp.bm.heart.V5B1g.dnsd2\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@hyp.bm.heart.V5B1g.hd95\endcsname{4.0}
\expandafter\gdef\csname R@hyp.bm.heart.V5B1g.hi\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@hyp.bm.heart.V5B1g.lo\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@hyp.bm.heart.V5B1g.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.heart.V5B1g.nsd1\endcsname{45.05}
\expandafter\gdef\csname R@hyp.bm.heart.V5B1g.nsd2\endcsname{90.45}
\expandafter\gdef\csname R@hyp.bm.heart.V5B1g.nup\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.heart.V5B1g.se\endcsname{0.08}
\expandafter\gdef\csname R@hyp.bm.heart.V7A1.d\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@hyp.bm.heart.V7A1.dhd95\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@hyp.bm.heart.V7A1.dice\endcsname{93.23}
\expandafter\gdef\csname R@hyp.bm.heart.V7A1.dmax\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@hyp.bm.heart.V7A1.dnsd1\endcsname{\ensuremath{-0.82}}
\expandafter\gdef\csname R@hyp.bm.heart.V7A1.dnsd2\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@hyp.bm.heart.V7A1.hd95\endcsname{4.0}
\expandafter\gdef\csname R@hyp.bm.heart.V7A1.hi\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@hyp.bm.heart.V7A1.lo\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@hyp.bm.heart.V7A1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.heart.V7A1.nsd1\endcsname{45.13}
\expandafter\gdef\csname R@hyp.bm.heart.V7A1.nsd2\endcsname{90.27}
\expandafter\gdef\csname R@hyp.bm.heart.V7A1.nup\endcsname{2}
\expandafter\gdef\csname R@hyp.bm.heart.V7A1.se\endcsname{0.06}
\expandafter\gdef\csname R@hyp.bm.heart.V7C1.d\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@hyp.bm.heart.V7C1.dhd95\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@hyp.bm.heart.V7C1.dice\endcsname{93.34}
\expandafter\gdef\csname R@hyp.bm.heart.V7C1.dmax\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@hyp.bm.heart.V7C1.dnsd1\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@hyp.bm.heart.V7C1.dnsd2\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@hyp.bm.heart.V7C1.hd95\endcsname{3.9}
\expandafter\gdef\csname R@hyp.bm.heart.V7C1.hi\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@hyp.bm.heart.V7C1.lo\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@hyp.bm.heart.V7C1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.heart.V7C1.nsd1\endcsname{45.63}
\expandafter\gdef\csname R@hyp.bm.heart.V7C1.nsd2\endcsname{90.68}
\expandafter\gdef\csname R@hyp.bm.heart.V7C1.nup\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.heart.V7C1.se\endcsname{0.11}
\expandafter\gdef\csname R@hyp.bm.heart.V9R2g.d\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@hyp.bm.heart.V9R2g.dhd95\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@hyp.bm.heart.V9R2g.dice\endcsname{93.30}
\expandafter\gdef\csname R@hyp.bm.heart.V9R2g.dmax\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@hyp.bm.heart.V9R2g.dnsd1\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@hyp.bm.heart.V9R2g.dnsd2\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@hyp.bm.heart.V9R2g.hd95\endcsname{3.8}
\expandafter\gdef\csname R@hyp.bm.heart.V9R2g.hi\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@hyp.bm.heart.V9R2g.lo\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@hyp.bm.heart.V9R2g.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.heart.V9R2g.nsd1\endcsname{45.73}
\expandafter\gdef\csname R@hyp.bm.heart.V9R2g.nsd2\endcsname{90.53}
\expandafter\gdef\csname R@hyp.bm.heart.V9R2g.nup\endcsname{2}
\expandafter\gdef\csname R@hyp.bm.heart.V9R2g.se\endcsname{0.07}
\expandafter\gdef\csname R@hyp.bm.heart.base.dice\endcsname{93.29}
\expandafter\gdef\csname R@hyp.bm.heart.base.hd95\endcsname{3.8}
\expandafter\gdef\csname R@hyp.bm.heart.base.nsd1\endcsname{45.95}
\expandafter\gdef\csname R@hyp.bm.heart.base.nsd2\endcsname{90.74}
\expandafter\gdef\csname R@hyp.bm.hepv.Rule.d\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@hyp.bm.hepv.Rule.hi\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@hyp.bm.hepv.Rule.lo\endcsname{\ensuremath{-0.65}}
\expandafter\gdef\csname R@hyp.bm.hepv.Rule.tumour.d\endcsname{\ensuremath{+1.22}}
\expandafter\gdef\csname R@hyp.bm.hepv.V10B.d\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@hyp.bm.hepv.V10B.dhd95\endcsname{\ensuremath{-0.3}}
\expandafter\gdef\csname R@hyp.bm.hepv.V10B.dice\endcsname{66.36}
\expandafter\gdef\csname R@hyp.bm.hepv.V10B.dmax\endcsname{\ensuremath{+1.06}}
\expandafter\gdef\csname R@hyp.bm.hepv.V10B.dnsd1\endcsname{0.00}
\expandafter\gdef\csname R@hyp.bm.hepv.V10B.dnsd2\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@hyp.bm.hepv.V10B.hd95\endcsname{30.6}
\expandafter\gdef\csname R@hyp.bm.hepv.V10B.hi\endcsname{\ensuremath{+1.58}}
\expandafter\gdef\csname R@hyp.bm.hepv.V10B.lo\endcsname{\ensuremath{-1.15}}
\expandafter\gdef\csname R@hyp.bm.hepv.V10B.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.hepv.V10B.nsd1\endcsname{59.09}
\expandafter\gdef\csname R@hyp.bm.hepv.V10B.nsd2\endcsname{68.41}
\expandafter\gdef\csname R@hyp.bm.hepv.V10B.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.hepv.V10B.se\endcsname{0.43}
\expandafter\gdef\csname R@hyp.bm.hepv.V7A1.d\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@hyp.bm.hepv.V7A1.dhd95\endcsname{\ensuremath{-3.9}}
\expandafter\gdef\csname R@hyp.bm.hepv.V7A1.dice\endcsname{66.22}
\expandafter\gdef\csname R@hyp.bm.hepv.V7A1.dmax\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@hyp.bm.hepv.V7A1.dnsd1\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@hyp.bm.hepv.V7A1.dnsd2\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@hyp.bm.hepv.V7A1.hd95\endcsname{27.0}
\expandafter\gdef\csname R@hyp.bm.hepv.V7A1.hi\endcsname{\ensuremath{+1.33}}
\expandafter\gdef\csname R@hyp.bm.hepv.V7A1.lo\endcsname{\ensuremath{-1.20}}
\expandafter\gdef\csname R@hyp.bm.hepv.V7A1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.hepv.V7A1.nsd1\endcsname{59.37}
\expandafter\gdef\csname R@hyp.bm.hepv.V7A1.nsd2\endcsname{68.65}
\expandafter\gdef\csname R@hyp.bm.hepv.V7A1.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.hepv.V7A1.se\endcsname{0.40}
\expandafter\gdef\csname R@hyp.bm.hepv.V7A1.tumour.d\endcsname{\ensuremath{+1.32}}
\expandafter\gdef\csname R@hyp.bm.hepv.V7C1.d\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@hyp.bm.hepv.V7C1.dhd95\endcsname{\ensuremath{-1.4}}
\expandafter\gdef\csname R@hyp.bm.hepv.V7C1.dice\endcsname{66.01}
\expandafter\gdef\csname R@hyp.bm.hepv.V7C1.dmax\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@hyp.bm.hepv.V7C1.dnsd1\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@hyp.bm.hepv.V7C1.dnsd2\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@hyp.bm.hepv.V7C1.hd95\endcsname{29.4}
\expandafter\gdef\csname R@hyp.bm.hepv.V7C1.hi\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@hyp.bm.hepv.V7C1.lo\endcsname{\ensuremath{-1.27}}
\expandafter\gdef\csname R@hyp.bm.hepv.V7C1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.hepv.V7C1.nsd1\endcsname{59.13}
\expandafter\gdef\csname R@hyp.bm.hepv.V7C1.nsd2\endcsname{68.36}
\expandafter\gdef\csname R@hyp.bm.hepv.V7C1.nup\endcsname{2}
\expandafter\gdef\csname R@hyp.bm.hepv.V7C1.se\endcsname{0.36}
\expandafter\gdef\csname R@hyp.bm.hepv.Y11.d\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@hyp.bm.hepv.Y11.dhd95\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@hyp.bm.hepv.Y11.dice\endcsname{66.38}
\expandafter\gdef\csname R@hyp.bm.hepv.Y11.dmax\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@hyp.bm.hepv.Y11.dnsd1\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@hyp.bm.hepv.Y11.dnsd2\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@hyp.bm.hepv.Y11.hd95\endcsname{30.8}
\expandafter\gdef\csname R@hyp.bm.hepv.Y11.hi\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@hyp.bm.hepv.Y11.lo\endcsname{\ensuremath{-0.65}}
\expandafter\gdef\csname R@hyp.bm.hepv.Y11.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.hepv.Y11.nsd1\endcsname{59.28}
\expandafter\gdef\csname R@hyp.bm.hepv.Y11.nsd2\endcsname{68.62}
\expandafter\gdef\csname R@hyp.bm.hepv.Y11.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.hepv.Y11.se\endcsname{0.28}
\expandafter\gdef\csname R@hyp.bm.hepv.Y11.tumour.d\endcsname{\ensuremath{+1.22}}
\expandafter\gdef\csname R@hyp.bm.hepv.Y2.d\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@hyp.bm.hepv.Y2.dhd95\endcsname{\ensuremath{+7.6}}
\expandafter\gdef\csname R@hyp.bm.hepv.Y2.dice\endcsname{65.83}
\expandafter\gdef\csname R@hyp.bm.hepv.Y2.dmax\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@hyp.bm.hepv.Y2.dnsd1\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@hyp.bm.hepv.Y2.dnsd2\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@hyp.bm.hepv.Y2.hd95\endcsname{38.5}
\expandafter\gdef\csname R@hyp.bm.hepv.Y2.hi\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@hyp.bm.hepv.Y2.lo\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@hyp.bm.hepv.Y2.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.hepv.Y2.nsd1\endcsname{58.74}
\expandafter\gdef\csname R@hyp.bm.hepv.Y2.nsd2\endcsname{67.94}
\expandafter\gdef\csname R@hyp.bm.hepv.Y2.nup\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.hepv.Y2.se\endcsname{0.21}
\expandafter\gdef\csname R@hyp.bm.hepv.base.dice\endcsname{66.15}
\expandafter\gdef\csname R@hyp.bm.hepv.base.hd95\endcsname{30.9}
\expandafter\gdef\csname R@hyp.bm.hepv.base.nsd1\endcsname{59.09}
\expandafter\gdef\csname R@hyp.bm.hepv.base.nsd2\endcsname{68.26}
\expandafter\gdef\csname R@hyp.bm.kipa22.J2.d\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@hyp.bm.kipa22.J2.dhd95\endcsname{\ensuremath{-1.8}}
\expandafter\gdef\csname R@hyp.bm.kipa22.J2.dice\endcsname{88.96}
\expandafter\gdef\csname R@hyp.bm.kipa22.J2.dmax\endcsname{\ensuremath{+0.94}}
\expandafter\gdef\csname R@hyp.bm.kipa22.J2.dnsd1\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@hyp.bm.kipa22.J2.dnsd2\endcsname{\ensuremath{+0.97}}
\expandafter\gdef\csname R@hyp.bm.kipa22.J2.hd95\endcsname{4.6}
\expandafter\gdef\csname R@hyp.bm.kipa22.J2.hi\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@hyp.bm.kipa22.J2.lo\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@hyp.bm.kipa22.J2.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kipa22.J2.nsd1\endcsname{84.37}
\expandafter\gdef\csname R@hyp.bm.kipa22.J2.nsd2\endcsname{93.12}
\expandafter\gdef\csname R@hyp.bm.kipa22.J2.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kipa22.J2.se\endcsname{0.20}
\expandafter\gdef\csname R@hyp.bm.kipa22.V11.d\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V11.dhd95\endcsname{\ensuremath{-1.7}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V11.dice\endcsname{88.70}
\expandafter\gdef\csname R@hyp.bm.kipa22.V11.dmax\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V11.dnsd1\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V11.dnsd2\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V11.hd95\endcsname{4.7}
\expandafter\gdef\csname R@hyp.bm.kipa22.V11.hi\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V11.lo\endcsname{\ensuremath{-0.97}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V11.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kipa22.V11.nsd1\endcsname{84.24}
\expandafter\gdef\csname R@hyp.bm.kipa22.V11.nsd2\endcsname{92.85}
\expandafter\gdef\csname R@hyp.bm.kipa22.V11.nup\endcsname{2}
\expandafter\gdef\csname R@hyp.bm.kipa22.V11.se\endcsname{0.33}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7A1.d\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7A1.dhd95\endcsname{\ensuremath{-1.5}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7A1.dice\endcsname{88.80}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7A1.dmax\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7A1.dnsd1\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7A1.dnsd2\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7A1.hd95\endcsname{4.9}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7A1.hi\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7A1.lo\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7A1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7A1.nsd1\endcsname{84.13}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7A1.nsd2\endcsname{92.84}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7A1.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7A1.r2nsd1\endcsname{\ensuremath{+1.20}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7A1.se\endcsname{0.02}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7A1.tumour.d\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7C1.d\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7C1.dhd95\endcsname{\ensuremath{-0.7}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7C1.dice\endcsname{88.32}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7C1.dmax\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7C1.dnsd1\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7C1.dnsd2\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7C1.hd95\endcsname{5.7}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7C1.hi\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7C1.lo\endcsname{\ensuremath{-1.29}}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7C1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7C1.nsd1\endcsname{82.93}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7C1.nsd2\endcsname{91.86}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7C1.nup\endcsname{2}
\expandafter\gdef\csname R@hyp.bm.kipa22.V7C1.se\endcsname{0.31}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y11.d\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y11.dhd95\endcsname{\ensuremath{-1.5}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y11.dice\endcsname{88.95}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y11.dmax\endcsname{\ensuremath{+0.95}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y11.dnsd1\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y11.dnsd2\endcsname{\ensuremath{+0.90}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y11.hd95\endcsname{4.9}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y11.hi\endcsname{\ensuremath{+1.06}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y11.lo\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y11.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y11.nsd1\endcsname{84.43}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y11.nsd2\endcsname{93.05}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y11.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y11.se\endcsname{0.23}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y2.d\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y2.dhd95\endcsname{\ensuremath{-1.6}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y2.dice\endcsname{88.79}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y2.dmax\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y2.dnsd1\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y2.dnsd2\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y2.hd95\endcsname{4.8}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y2.hi\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y2.lo\endcsname{\ensuremath{-0.41}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y2.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y2.nsd1\endcsname{84.32}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y2.nsd2\endcsname{92.96}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y2.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y2.se\endcsname{0.18}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y3.d\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y3.dhd95\endcsname{\ensuremath{-0.3}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y3.dice\endcsname{89.02}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y3.dmax\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y3.dnsd1\endcsname{\ensuremath{+0.91}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y3.dnsd2\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y3.hd95\endcsname{6.1}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y3.hi\endcsname{\ensuremath{+0.67}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y3.lo\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y3.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y3.nsd1\endcsname{84.35}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y3.nsd2\endcsname{93.02}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y3.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y3.se\endcsname{0.09}
\expandafter\gdef\csname R@hyp.bm.kipa22.Y3.tumour.d\endcsname{\ensuremath{+1.34}}
\expandafter\gdef\csname R@hyp.bm.kipa22.base.dice\endcsname{88.62}
\expandafter\gdef\csname R@hyp.bm.kipa22.base.hd95\endcsname{6.4}
\expandafter\gdef\csname R@hyp.bm.kipa22.base.nsd1\endcsname{83.45}
\expandafter\gdef\csname R@hyp.bm.kipa22.base.nsd2\endcsname{92.15}
\expandafter\gdef\csname R@hyp.bm.kits.H1.d\endcsname{\ensuremath{+2.01}}
\expandafter\gdef\csname R@hyp.bm.kits.H1.dhd95\endcsname{\ensuremath{-18.0}}
\expandafter\gdef\csname R@hyp.bm.kits.H1.dice\endcsname{86.00}
\expandafter\gdef\csname R@hyp.bm.kits.H1.dmax\endcsname{\ensuremath{+3.65}}
\expandafter\gdef\csname R@hyp.bm.kits.H1.dnsd1\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@hyp.bm.kits.H1.dnsd2\endcsname{\ensuremath{+2.48}}
\expandafter\gdef\csname R@hyp.bm.kits.H1.hd95\endcsname{32.6}
\expandafter\gdef\csname R@hyp.bm.kits.H1.hi\endcsname{\ensuremath{+4.00}}
\expandafter\gdef\csname R@hyp.bm.kits.H1.lo\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@hyp.bm.kits.H1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.H1.nsd1\endcsname{72.95}
\expandafter\gdef\csname R@hyp.bm.kits.H1.nsd2\endcsname{80.83}
\expandafter\gdef\csname R@hyp.bm.kits.H1.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.H1.se\endcsname{0.63}
\expandafter\gdef\csname R@hyp.bm.kits.J1.d\endcsname{\ensuremath{+2.25}}
\expandafter\gdef\csname R@hyp.bm.kits.J1.dhd95\endcsname{\ensuremath{-18.9}}
\expandafter\gdef\csname R@hyp.bm.kits.J1.dice\endcsname{86.25}
\expandafter\gdef\csname R@hyp.bm.kits.J1.dmax\endcsname{\ensuremath{+3.56}}
\expandafter\gdef\csname R@hyp.bm.kits.J1.dnsd1\endcsname{\ensuremath{+2.64}}
\expandafter\gdef\csname R@hyp.bm.kits.J1.dnsd2\endcsname{\ensuremath{+2.78}}
\expandafter\gdef\csname R@hyp.bm.kits.J1.hd95\endcsname{31.7}
\expandafter\gdef\csname R@hyp.bm.kits.J1.hi\endcsname{\ensuremath{+4.16}}
\expandafter\gdef\csname R@hyp.bm.kits.J1.lo\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@hyp.bm.kits.J1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.J1.nsd1\endcsname{73.28}
\expandafter\gdef\csname R@hyp.bm.kits.J1.nsd2\endcsname{81.13}
\expandafter\gdef\csname R@hyp.bm.kits.J1.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.J1.se\endcsname{0.60}
\expandafter\gdef\csname R@hyp.bm.kits.J2.d\endcsname{\ensuremath{+2.32}}
\expandafter\gdef\csname R@hyp.bm.kits.J2.dhd95\endcsname{\ensuremath{-16.3}}
\expandafter\gdef\csname R@hyp.bm.kits.J2.dice\endcsname{86.31}
\expandafter\gdef\csname R@hyp.bm.kits.J2.dmax\endcsname{\ensuremath{+4.28}}
\expandafter\gdef\csname R@hyp.bm.kits.J2.dnsd1\endcsname{\ensuremath{+2.48}}
\expandafter\gdef\csname R@hyp.bm.kits.J2.dnsd2\endcsname{\ensuremath{+2.68}}
\expandafter\gdef\csname R@hyp.bm.kits.J2.hd95\endcsname{34.4}
\expandafter\gdef\csname R@hyp.bm.kits.J2.hi\endcsname{\ensuremath{+4.45}}
\expandafter\gdef\csname R@hyp.bm.kits.J2.lo\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@hyp.bm.kits.J2.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.J2.nsd1\endcsname{73.12}
\expandafter\gdef\csname R@hyp.bm.kits.J2.nsd2\endcsname{81.03}
\expandafter\gdef\csname R@hyp.bm.kits.J2.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.J2.se\endcsname{0.67}
\expandafter\gdef\csname R@hyp.bm.kits.J4.d\endcsname{\ensuremath{+1.93}}
\expandafter\gdef\csname R@hyp.bm.kits.J4.dhd95\endcsname{\ensuremath{-12.4}}
\expandafter\gdef\csname R@hyp.bm.kits.J4.dice\endcsname{85.92}
\expandafter\gdef\csname R@hyp.bm.kits.J4.dmax\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@hyp.bm.kits.J4.dnsd1\endcsname{\ensuremath{+2.11}}
\expandafter\gdef\csname R@hyp.bm.kits.J4.dnsd2\endcsname{\ensuremath{+2.30}}
\expandafter\gdef\csname R@hyp.bm.kits.J4.hd95\endcsname{38.3}
\expandafter\gdef\csname R@hyp.bm.kits.J4.hi\endcsname{\ensuremath{+2.70}}
\expandafter\gdef\csname R@hyp.bm.kits.J4.lo\endcsname{\ensuremath{+1.16}}
\expandafter\gdef\csname R@hyp.bm.kits.J4.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.J4.nsd1\endcsname{72.75}
\expandafter\gdef\csname R@hyp.bm.kits.J4.nsd2\endcsname{80.66}
\expandafter\gdef\csname R@hyp.bm.kits.J4.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.J4.se\endcsname{0.24}
\expandafter\gdef\csname R@hyp.bm.kits.L1.d\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@hyp.bm.kits.L1.dhd95\endcsname{\ensuremath{-18.0}}
\expandafter\gdef\csname R@hyp.bm.kits.L1.dice\endcsname{86.14}
\expandafter\gdef\csname R@hyp.bm.kits.L1.dmax\endcsname{\ensuremath{+2.94}}
\expandafter\gdef\csname R@hyp.bm.kits.L1.dnsd1\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@hyp.bm.kits.L1.dnsd2\endcsname{\ensuremath{+2.49}}
\expandafter\gdef\csname R@hyp.bm.kits.L1.hd95\endcsname{32.7}
\expandafter\gdef\csname R@hyp.bm.kits.L1.hi\endcsname{\ensuremath{+3.32}}
\expandafter\gdef\csname R@hyp.bm.kits.L1.lo\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@hyp.bm.kits.L1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.L1.nsd1\endcsname{72.93}
\expandafter\gdef\csname R@hyp.bm.kits.L1.nsd2\endcsname{80.84}
\expandafter\gdef\csname R@hyp.bm.kits.L1.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.L1.se\endcsname{0.37}
\expandafter\gdef\csname R@hyp.bm.kits.L1S.d\endcsname{\ensuremath{+1.54}}
\expandafter\gdef\csname R@hyp.bm.kits.L1S.dice\endcsname{85.53}
\expandafter\gdef\csname R@hyp.bm.kits.L1S.dmax\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@hyp.bm.kits.L1S.hi\endcsname{\ensuremath{+3.58}}
\expandafter\gdef\csname R@hyp.bm.kits.L1S.lo\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@hyp.bm.kits.L1S.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.L1S.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.kits.L1S.se\endcsname{0.64}
\expandafter\gdef\csname R@hyp.bm.kits.L3.d\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@hyp.bm.kits.L3.dhd95\endcsname{\ensuremath{-3.7}}
\expandafter\gdef\csname R@hyp.bm.kits.L3.dice\endcsname{84.67}
\expandafter\gdef\csname R@hyp.bm.kits.L3.dmax\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@hyp.bm.kits.L3.dnsd1\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@hyp.bm.kits.L3.dnsd2\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@hyp.bm.kits.L3.hd95\endcsname{46.9}
\expandafter\gdef\csname R@hyp.bm.kits.L3.hi\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@hyp.bm.kits.L3.lo\endcsname{\ensuremath{-1.08}}
\expandafter\gdef\csname R@hyp.bm.kits.L3.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.L3.nsd1\endcsname{71.51}
\expandafter\gdef\csname R@hyp.bm.kits.L3.nsd2\endcsname{79.19}
\expandafter\gdef\csname R@hyp.bm.kits.L3.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.kits.L3.se\endcsname{0.55}
\expandafter\gdef\csname R@hyp.bm.kits.MedNeXtM.d\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@hyp.bm.kits.MedNeXtM.dhd95\endcsname{\ensuremath{-2.5}}
\expandafter\gdef\csname R@hyp.bm.kits.MedNeXtM.dice\endcsname{83.24}
\expandafter\gdef\csname R@hyp.bm.kits.MedNeXtM.dmax\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@hyp.bm.kits.MedNeXtM.dnsd1\endcsname{\ensuremath{-0.84}}
\expandafter\gdef\csname R@hyp.bm.kits.MedNeXtM.dnsd2\endcsname{\ensuremath{-0.82}}
\expandafter\gdef\csname R@hyp.bm.kits.MedNeXtM.hd95\endcsname{48.2}
\expandafter\gdef\csname R@hyp.bm.kits.MedNeXtM.hi\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@hyp.bm.kits.MedNeXtM.lo\endcsname{\ensuremath{-1.46}}
\expandafter\gdef\csname R@hyp.bm.kits.MedNeXtM.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.MedNeXtM.nsd1\endcsname{69.80}
\expandafter\gdef\csname R@hyp.bm.kits.MedNeXtM.nsd2\endcsname{77.54}
\expandafter\gdef\csname R@hyp.bm.kits.MedNeXtM.nup\endcsname{0}
\expandafter\gdef\csname R@hyp.bm.kits.MedNeXtM.se\endcsname{0.22}
\expandafter\gdef\csname R@hyp.bm.kits.P3c.d\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@hyp.bm.kits.P3c.dice\endcsname{84.55}
\expandafter\gdef\csname R@hyp.bm.kits.P3c.dmax\endcsname{\ensuremath{+2.38}}
\expandafter\gdef\csname R@hyp.bm.kits.P3c.hi\endcsname{\ensuremath{+2.82}}
\expandafter\gdef\csname R@hyp.bm.kits.P3c.lo\endcsname{\ensuremath{-1.71}}
\expandafter\gdef\csname R@hyp.bm.kits.P3c.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.P3c.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.kits.P3c.se\endcsname{0.71}
\expandafter\gdef\csname R@hyp.bm.kits.R5.arm\endcsname{J2}
\expandafter\gdef\csname R@hyp.bm.kits.R5.d\endcsname{\ensuremath{+2.32}}
\expandafter\gdef\csname R@hyp.bm.kits.R5.dice\endcsname{86.31}
\expandafter\gdef\csname R@hyp.bm.kits.R5.hi\endcsname{\ensuremath{+4.45}}
\expandafter\gdef\csname R@hyp.bm.kits.R5.lo\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@hyp.bm.kits.R5.se\endcsname{0.67}
\expandafter\gdef\csname R@hyp.bm.kits.V11.d\endcsname{\ensuremath{+0.90}}
\expandafter\gdef\csname R@hyp.bm.kits.V11.dhd95\endcsname{\ensuremath{-7.9}}
\expandafter\gdef\csname R@hyp.bm.kits.V11.dice\endcsname{84.89}
\expandafter\gdef\csname R@hyp.bm.kits.V11.dmax\endcsname{\ensuremath{+2.75}}
\expandafter\gdef\csname R@hyp.bm.kits.V11.dnsd1\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@hyp.bm.kits.V11.dnsd2\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@hyp.bm.kits.V11.hd95\endcsname{42.8}
\expandafter\gdef\csname R@hyp.bm.kits.V11.hi\endcsname{\ensuremath{+3.18}}
\expandafter\gdef\csname R@hyp.bm.kits.V11.lo\endcsname{\ensuremath{-1.38}}
\expandafter\gdef\csname R@hyp.bm.kits.V11.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.V11.nsd1\endcsname{71.35}
\expandafter\gdef\csname R@hyp.bm.kits.V11.nsd2\endcsname{79.23}
\expandafter\gdef\csname R@hyp.bm.kits.V11.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.kits.V11.se\endcsname{0.72}
\expandafter\gdef\csname R@hyp.bm.kits.V5B1.d\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@hyp.bm.kits.V5B1.dice\endcsname{84.99}
\expandafter\gdef\csname R@hyp.bm.kits.V5B1.dmax\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@hyp.bm.kits.V5B1.hi\endcsname{\ensuremath{+2.58}}
\expandafter\gdef\csname R@hyp.bm.kits.V5B1.lo\endcsname{\ensuremath{-0.60}}
\expandafter\gdef\csname R@hyp.bm.kits.V5B1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.V5B1.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.kits.V5B1.se\endcsname{0.50}
\expandafter\gdef\csname R@hyp.bm.kits.V7A1.d\endcsname{\ensuremath{+1.63}}
\expandafter\gdef\csname R@hyp.bm.kits.V7A1.dhd95\endcsname{\ensuremath{-8.0}}
\expandafter\gdef\csname R@hyp.bm.kits.V7A1.dice\endcsname{85.63}
\expandafter\gdef\csname R@hyp.bm.kits.V7A1.dmax\endcsname{\ensuremath{+2.40}}
\expandafter\gdef\csname R@hyp.bm.kits.V7A1.dnsd1\endcsname{\ensuremath{+1.39}}
\expandafter\gdef\csname R@hyp.bm.kits.V7A1.dnsd2\endcsname{\ensuremath{+1.66}}
\expandafter\gdef\csname R@hyp.bm.kits.V7A1.hd95\endcsname{42.7}
\expandafter\gdef\csname R@hyp.bm.kits.V7A1.hi\endcsname{\ensuremath{+3.27}}
\expandafter\gdef\csname R@hyp.bm.kits.V7A1.lo\endcsname{0.00}
\expandafter\gdef\csname R@hyp.bm.kits.V7A1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.V7A1.nsd1\endcsname{72.03}
\expandafter\gdef\csname R@hyp.bm.kits.V7A1.nsd2\endcsname{80.01}
\expandafter\gdef\csname R@hyp.bm.kits.V7A1.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.V7A1.se\endcsname{0.51}
\expandafter\gdef\csname R@hyp.bm.kits.V7C1.d\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@hyp.bm.kits.V7C1.dhd95\endcsname{\ensuremath{-7.6}}
\expandafter\gdef\csname R@hyp.bm.kits.V7C1.dice\endcsname{84.78}
\expandafter\gdef\csname R@hyp.bm.kits.V7C1.dmax\endcsname{\ensuremath{+2.14}}
\expandafter\gdef\csname R@hyp.bm.kits.V7C1.dnsd1\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@hyp.bm.kits.V7C1.dnsd2\endcsname{\ensuremath{+0.72}}
\expandafter\gdef\csname R@hyp.bm.kits.V7C1.hd95\endcsname{43.0}
\expandafter\gdef\csname R@hyp.bm.kits.V7C1.hi\endcsname{\ensuremath{+2.48}}
\expandafter\gdef\csname R@hyp.bm.kits.V7C1.lo\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@hyp.bm.kits.V7C1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.V7C1.nsd1\endcsname{71.14}
\expandafter\gdef\csname R@hyp.bm.kits.V7C1.nsd2\endcsname{79.07}
\expandafter\gdef\csname R@hyp.bm.kits.V7C1.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.kits.V7C1.se\endcsname{0.53}
\expandafter\gdef\csname R@hyp.bm.kits.V9R2.d\endcsname{\ensuremath{+1.33}}
\expandafter\gdef\csname R@hyp.bm.kits.V9R2.dhd95\endcsname{\ensuremath{-8.9}}
\expandafter\gdef\csname R@hyp.bm.kits.V9R2.dice\endcsname{85.32}
\expandafter\gdef\csname R@hyp.bm.kits.V9R2.dmax\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@hyp.bm.kits.V9R2.dnsd1\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@hyp.bm.kits.V9R2.dnsd2\endcsname{\ensuremath{+1.38}}
\expandafter\gdef\csname R@hyp.bm.kits.V9R2.hd95\endcsname{41.8}
\expandafter\gdef\csname R@hyp.bm.kits.V9R2.hi\endcsname{\ensuremath{+3.42}}
\expandafter\gdef\csname R@hyp.bm.kits.V9R2.lo\endcsname{\ensuremath{-0.76}}
\expandafter\gdef\csname R@hyp.bm.kits.V9R2.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.V9R2.nsd1\endcsname{71.82}
\expandafter\gdef\csname R@hyp.bm.kits.V9R2.nsd2\endcsname{79.73}
\expandafter\gdef\csname R@hyp.bm.kits.V9R2.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.kits.V9R2.se\endcsname{0.66}
\expandafter\gdef\csname R@hyp.bm.kits.Y2.d\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@hyp.bm.kits.Y2.dhd95\endcsname{\ensuremath{-20.8}}
\expandafter\gdef\csname R@hyp.bm.kits.Y2.dice\endcsname{86.70}
\expandafter\gdef\csname R@hyp.bm.kits.Y2.dmax\endcsname{\ensuremath{+3.47}}
\expandafter\gdef\csname R@hyp.bm.kits.Y2.dnsd1\endcsname{\ensuremath{+2.76}}
\expandafter\gdef\csname R@hyp.bm.kits.Y2.dnsd2\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@hyp.bm.kits.Y2.hd95\endcsname{29.8}
\expandafter\gdef\csname R@hyp.bm.kits.Y2.hi\endcsname{\ensuremath{+3.73}}
\expandafter\gdef\csname R@hyp.bm.kits.Y2.lo\endcsname{\ensuremath{+1.68}}
\expandafter\gdef\csname R@hyp.bm.kits.Y2.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.Y2.nsd1\endcsname{73.40}
\expandafter\gdef\csname R@hyp.bm.kits.Y2.nsd2\endcsname{81.37}
\expandafter\gdef\csname R@hyp.bm.kits.Y2.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.Y2.se\endcsname{0.32}
\expandafter\gdef\csname R@hyp.bm.kits.Y3.d\endcsname{\ensuremath{+2.21}}
\expandafter\gdef\csname R@hyp.bm.kits.Y3.dhd95\endcsname{\ensuremath{-17.1}}
\expandafter\gdef\csname R@hyp.bm.kits.Y3.dice\endcsname{86.21}
\expandafter\gdef\csname R@hyp.bm.kits.Y3.dmax\endcsname{\ensuremath{+3.69}}
\expandafter\gdef\csname R@hyp.bm.kits.Y3.dnsd1\endcsname{\ensuremath{+2.33}}
\expandafter\gdef\csname R@hyp.bm.kits.Y3.dnsd2\endcsname{\ensuremath{+2.58}}
\expandafter\gdef\csname R@hyp.bm.kits.Y3.hd95\endcsname{33.6}
\expandafter\gdef\csname R@hyp.bm.kits.Y3.hi\endcsname{\ensuremath{+4.19}}
\expandafter\gdef\csname R@hyp.bm.kits.Y3.lo\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@hyp.bm.kits.Y3.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.Y3.nsd1\endcsname{72.97}
\expandafter\gdef\csname R@hyp.bm.kits.Y3.nsd2\endcsname{80.94}
\expandafter\gdef\csname R@hyp.bm.kits.Y3.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.Y3.se\endcsname{0.62}
\expandafter\gdef\csname R@hyp.bm.kits.Y4.d\endcsname{\ensuremath{+2.11}}
\expandafter\gdef\csname R@hyp.bm.kits.Y4.dhd95\endcsname{\ensuremath{-15.6}}
\expandafter\gdef\csname R@hyp.bm.kits.Y4.dice\endcsname{86.11}
\expandafter\gdef\csname R@hyp.bm.kits.Y4.dmax\endcsname{\ensuremath{+4.03}}
\expandafter\gdef\csname R@hyp.bm.kits.Y4.dnsd1\endcsname{\ensuremath{+2.30}}
\expandafter\gdef\csname R@hyp.bm.kits.Y4.dnsd2\endcsname{\ensuremath{+2.46}}
\expandafter\gdef\csname R@hyp.bm.kits.Y4.hd95\endcsname{35.0}
\expandafter\gdef\csname R@hyp.bm.kits.Y4.hi\endcsname{\ensuremath{+4.51}}
\expandafter\gdef\csname R@hyp.bm.kits.Y4.lo\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@hyp.bm.kits.Y4.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.Y4.nsd1\endcsname{72.94}
\expandafter\gdef\csname R@hyp.bm.kits.Y4.nsd2\endcsname{80.81}
\expandafter\gdef\csname R@hyp.bm.kits.Y4.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.kits.Y4.se\endcsname{0.75}
\expandafter\gdef\csname R@hyp.bm.kits.base.dice\endcsname{83.99}
\expandafter\gdef\csname R@hyp.bm.kits.base.hd95\endcsname{50.6}
\expandafter\gdef\csname R@hyp.bm.kits.base.nsd1\endcsname{70.64}
\expandafter\gdef\csname R@hyp.bm.kits.base.nsd2\endcsname{78.35}
\expandafter\gdef\csname R@hyp.bm.lacdc.L1.d\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@hyp.bm.lacdc.L1.dhd95\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@hyp.bm.lacdc.L1.dice\endcsname{91.90}
\expandafter\gdef\csname R@hyp.bm.lacdc.L1.dmax\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@hyp.bm.lacdc.L1.dnsd1\endcsname{\ensuremath{+1.32}}
\expandafter\gdef\csname R@hyp.bm.lacdc.L1.dnsd2\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@hyp.bm.lacdc.L1.hd95\endcsname{3.7}
\expandafter\gdef\csname R@hyp.bm.lacdc.L1.hi\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@hyp.bm.lacdc.L1.lo\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@hyp.bm.lacdc.L1.n\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.lacdc.L1.nsd1\endcsname{78.28}
\expandafter\gdef\csname R@hyp.bm.lacdc.L1.nsd2\endcsname{93.25}
\expandafter\gdef\csname R@hyp.bm.lacdc.L1.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.lacdc.L1.se\endcsname{0.05}
\expandafter\gdef\csname R@hyp.bm.lacdc.V7A1.d\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@hyp.bm.lacdc.V7A1.dhd95\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@hyp.bm.lacdc.V7A1.dice\endcsname{91.58}
\expandafter\gdef\csname R@hyp.bm.lacdc.V7A1.dmax\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@hyp.bm.lacdc.V7A1.dnsd1\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@hyp.bm.lacdc.V7A1.dnsd2\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@hyp.bm.lacdc.V7A1.hd95\endcsname{4.6}
\expandafter\gdef\csname R@hyp.bm.lacdc.V7A1.hi\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@hyp.bm.lacdc.V7A1.lo\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@hyp.bm.lacdc.V7A1.n\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.lacdc.V7A1.nsd1\endcsname{77.44}
\expandafter\gdef\csname R@hyp.bm.lacdc.V7A1.nsd2\endcsname{92.79}
\expandafter\gdef\csname R@hyp.bm.lacdc.V7A1.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.lacdc.V7A1.se\endcsname{0.09}
\expandafter\gdef\csname R@hyp.bm.lacdc.base.dice\endcsname{91.37}
\expandafter\gdef\csname R@hyp.bm.lacdc.base.hd95\endcsname{4.3}
\expandafter\gdef\csname R@hyp.bm.lacdc.base.nsd1\endcsname{76.96}
\expandafter\gdef\csname R@hyp.bm.lacdc.base.nsd2\endcsname{92.14}
\expandafter\gdef\csname R@hyp.bm.lamos.L1.d\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@hyp.bm.lamos.L1.dhd95\endcsname{\ensuremath{-0.5}}
\expandafter\gdef\csname R@hyp.bm.lamos.L1.dice\endcsname{90.02}
\expandafter\gdef\csname R@hyp.bm.lamos.L1.dmax\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@hyp.bm.lamos.L1.dnsd1\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@hyp.bm.lamos.L1.dnsd2\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@hyp.bm.lamos.L1.hd95\endcsname{12.2}
\expandafter\gdef\csname R@hyp.bm.lamos.L1.hi\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@hyp.bm.lamos.L1.lo\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@hyp.bm.lamos.L1.n\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.lamos.L1.nsd1\endcsname{83.28}
\expandafter\gdef\csname R@hyp.bm.lamos.L1.nsd2\endcsname{91.60}
\expandafter\gdef\csname R@hyp.bm.lamos.L1.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.lamos.L1.se\endcsname{0.04}
\expandafter\gdef\csname R@hyp.bm.lamos.V7A1.d\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@hyp.bm.lamos.V7A1.dhd95\endcsname{\ensuremath{-0.8}}
\expandafter\gdef\csname R@hyp.bm.lamos.V7A1.dice\endcsname{89.91}
\expandafter\gdef\csname R@hyp.bm.lamos.V7A1.dmax\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@hyp.bm.lamos.V7A1.dnsd1\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@hyp.bm.lamos.V7A1.dnsd2\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@hyp.bm.lamos.V7A1.hd95\endcsname{11.9}
\expandafter\gdef\csname R@hyp.bm.lamos.V7A1.hi\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@hyp.bm.lamos.V7A1.lo\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@hyp.bm.lamos.V7A1.n\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.lamos.V7A1.nsd1\endcsname{82.96}
\expandafter\gdef\csname R@hyp.bm.lamos.V7A1.nsd2\endcsname{91.42}
\expandafter\gdef\csname R@hyp.bm.lamos.V7A1.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.lamos.V7A1.se\endcsname{0.08}
\expandafter\gdef\csname R@hyp.bm.lamos.base.dice\endcsname{89.74}
\expandafter\gdef\csname R@hyp.bm.lamos.base.hd95\endcsname{12.6}
\expandafter\gdef\csname R@hyp.bm.lamos.base.nsd1\endcsname{82.76}
\expandafter\gdef\csname R@hyp.bm.lamos.base.nsd2\endcsname{91.14}
\expandafter\gdef\csname R@hyp.bm.lits.H1.d\endcsname{\ensuremath{+1.22}}
\expandafter\gdef\csname R@hyp.bm.lits.H1.dhd95\endcsname{\ensuremath{-8.2}}
\expandafter\gdef\csname R@hyp.bm.lits.H1.dice\endcsname{82.02}
\expandafter\gdef\csname R@hyp.bm.lits.H1.dmax\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@hyp.bm.lits.H1.dnsd1\endcsname{\ensuremath{+1.47}}
\expandafter\gdef\csname R@hyp.bm.lits.H1.dnsd2\endcsname{\ensuremath{+1.77}}
\expandafter\gdef\csname R@hyp.bm.lits.H1.hd95\endcsname{49.2}
\expandafter\gdef\csname R@hyp.bm.lits.H1.hi\endcsname{\ensuremath{+3.96}}
\expandafter\gdef\csname R@hyp.bm.lits.H1.lo\endcsname{\ensuremath{-1.51}}
\expandafter\gdef\csname R@hyp.bm.lits.H1.n\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.lits.H1.nsd1\endcsname{62.94}
\expandafter\gdef\csname R@hyp.bm.lits.H1.nsd2\endcsname{79.08}
\expandafter\gdef\csname R@hyp.bm.lits.H1.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.lits.H1.se\endcsname{0.64}
\expandafter\gdef\csname R@hyp.bm.lits.L1.d\endcsname{\ensuremath{+1.13}}
\expandafter\gdef\csname R@hyp.bm.lits.L1.dhd95\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@hyp.bm.lits.L1.dice\endcsname{81.93}
\expandafter\gdef\csname R@hyp.bm.lits.L1.dmax\endcsname{\ensuremath{+1.93}}
\expandafter\gdef\csname R@hyp.bm.lits.L1.dnsd1\endcsname{\ensuremath{+1.38}}
\expandafter\gdef\csname R@hyp.bm.lits.L1.dnsd2\endcsname{\ensuremath{+1.26}}
\expandafter\gdef\csname R@hyp.bm.lits.L1.hd95\endcsname{58.8}
\expandafter\gdef\csname R@hyp.bm.lits.L1.hi\endcsname{\ensuremath{+4.27}}
\expandafter\gdef\csname R@hyp.bm.lits.L1.lo\endcsname{\ensuremath{-2.01}}
\expandafter\gdef\csname R@hyp.bm.lits.L1.n\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.lits.L1.nsd1\endcsname{62.85}
\expandafter\gdef\csname R@hyp.bm.lits.L1.nsd2\endcsname{78.57}
\expandafter\gdef\csname R@hyp.bm.lits.L1.nup\endcsname{2}
\expandafter\gdef\csname R@hyp.bm.lits.L1.se\endcsname{0.73}
\expandafter\gdef\csname R@hyp.bm.lits.L3.d\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@hyp.bm.lits.L3.dice\endcsname{81.29}
\expandafter\gdef\csname R@hyp.bm.lits.L3.dmax\endcsname{\ensuremath{+2.20}}
\expandafter\gdef\csname R@hyp.bm.lits.L3.hi\endcsname{\ensuremath{+5.35}}
\expandafter\gdef\csname R@hyp.bm.lits.L3.lo\endcsname{\ensuremath{-4.36}}
\expandafter\gdef\csname R@hyp.bm.lits.L3.n\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.lits.L3.nup\endcsname{2}
\expandafter\gdef\csname R@hyp.bm.lits.L3.se\endcsname{1.13}
\expandafter\gdef\csname R@hyp.bm.lits.V7A1.d\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@hyp.bm.lits.V7A1.dhd95\endcsname{\ensuremath{-14.2}}
\expandafter\gdef\csname R@hyp.bm.lits.V7A1.dice\endcsname{82.44}
\expandafter\gdef\csname R@hyp.bm.lits.V7A1.dmax\endcsname{\ensuremath{+4.18}}
\expandafter\gdef\csname R@hyp.bm.lits.V7A1.dnsd1\endcsname{\ensuremath{+2.20}}
\expandafter\gdef\csname R@hyp.bm.lits.V7A1.dnsd2\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@hyp.bm.lits.V7A1.hd95\endcsname{43.2}
\expandafter\gdef\csname R@hyp.bm.lits.V7A1.hi\endcsname{\ensuremath{+8.37}}
\expandafter\gdef\csname R@hyp.bm.lits.V7A1.lo\endcsname{\ensuremath{-5.07}}
\expandafter\gdef\csname R@hyp.bm.lits.V7A1.n\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.lits.V7A1.nsd1\endcsname{63.67}
\expandafter\gdef\csname R@hyp.bm.lits.V7A1.nsd2\endcsname{79.65}
\expandafter\gdef\csname R@hyp.bm.lits.V7A1.nup\endcsname{2}
\expandafter\gdef\csname R@hyp.bm.lits.V7A1.se\endcsname{1.56}
\expandafter\gdef\csname R@hyp.bm.lits.V7A1.tumour.d\endcsname{\ensuremath{+3.28}}
\expandafter\gdef\csname R@hyp.bm.lits.V7C1.d\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@hyp.bm.lits.V7C1.dhd95\endcsname{\ensuremath{-8.6}}
\expandafter\gdef\csname R@hyp.bm.lits.V7C1.dice\endcsname{81.65}
\expandafter\gdef\csname R@hyp.bm.lits.V7C1.dmax\endcsname{\ensuremath{+2.78}}
\expandafter\gdef\csname R@hyp.bm.lits.V7C1.dnsd1\endcsname{\ensuremath{+0.72}}
\expandafter\gdef\csname R@hyp.bm.lits.V7C1.dnsd2\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@hyp.bm.lits.V7C1.hd95\endcsname{48.8}
\expandafter\gdef\csname R@hyp.bm.lits.V7C1.hi\endcsname{\ensuremath{+5.03}}
\expandafter\gdef\csname R@hyp.bm.lits.V7C1.lo\endcsname{\ensuremath{-3.33}}
\expandafter\gdef\csname R@hyp.bm.lits.V7C1.n\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.lits.V7C1.nsd1\endcsname{62.19}
\expandafter\gdef\csname R@hyp.bm.lits.V7C1.nsd2\endcsname{78.09}
\expandafter\gdef\csname R@hyp.bm.lits.V7C1.nup\endcsname{2}
\expandafter\gdef\csname R@hyp.bm.lits.V7C1.se\endcsname{0.97}
\expandafter\gdef\csname R@hyp.bm.lits.Y2.d\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@hyp.bm.lits.Y2.dhd95\endcsname{\ensuremath{-9.7}}
\expandafter\gdef\csname R@hyp.bm.lits.Y2.dice\endcsname{82.45}
\expandafter\gdef\csname R@hyp.bm.lits.Y2.dmax\endcsname{\ensuremath{+3.30}}
\expandafter\gdef\csname R@hyp.bm.lits.Y2.dnsd1\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@hyp.bm.lits.Y2.dnsd2\endcsname{\ensuremath{+2.37}}
\expandafter\gdef\csname R@hyp.bm.lits.Y2.hd95\endcsname{47.8}
\expandafter\gdef\csname R@hyp.bm.lits.Y2.hi\endcsname{\ensuremath{+5.60}}
\expandafter\gdef\csname R@hyp.bm.lits.Y2.lo\endcsname{\ensuremath{-2.30}}
\expandafter\gdef\csname R@hyp.bm.lits.Y2.n\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.lits.Y2.nsd1\endcsname{63.35}
\expandafter\gdef\csname R@hyp.bm.lits.Y2.nsd2\endcsname{79.68}
\expandafter\gdef\csname R@hyp.bm.lits.Y2.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.lits.Y2.se\endcsname{0.92}
\expandafter\gdef\csname R@hyp.bm.lits.base.dice\endcsname{80.79}
\expandafter\gdef\csname R@hyp.bm.lits.base.hd95\endcsname{57.5}
\expandafter\gdef\csname R@hyp.bm.lits.base.nsd1\endcsname{61.47}
\expandafter\gdef\csname R@hyp.bm.lits.base.nsd2\endcsname{77.31}
\expandafter\gdef\csname R@hyp.bm.lkipa.V7A1.d\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@hyp.bm.lkipa.V7A1.dnsd1\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@hyp.bm.lkipa.V7A1.dnsd2\endcsname{\ensuremath{+0.90}}
\expandafter\gdef\csname R@hyp.bm.lkipa.V7A1.tumour.d\endcsname{\ensuremath{+3.06}}
\expandafter\gdef\csname R@hyp.bm.lpanc.V7A1.cancer.d\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@hyp.bm.lpanc.V7A1.d\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@hyp.bm.lpanc.V7A1.dhd95\endcsname{\ensuremath{+8.7}}
\expandafter\gdef\csname R@hyp.bm.lpanc.V7A1.dice\endcsname{65.89}
\expandafter\gdef\csname R@hyp.bm.lpanc.V7A1.dmax\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@hyp.bm.lpanc.V7A1.dnsd1\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@hyp.bm.lpanc.V7A1.dnsd2\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@hyp.bm.lpanc.V7A1.hd95\endcsname{49.2}
\expandafter\gdef\csname R@hyp.bm.lpanc.V7A1.hi\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@hyp.bm.lpanc.V7A1.lo\endcsname{\ensuremath{-1.22}}
\expandafter\gdef\csname R@hyp.bm.lpanc.V7A1.n\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.lpanc.V7A1.nsd1\endcsname{46.75}
\expandafter\gdef\csname R@hyp.bm.lpanc.V7A1.nsd2\endcsname{59.18}
\expandafter\gdef\csname R@hyp.bm.lpanc.V7A1.nup\endcsname{2}
\expandafter\gdef\csname R@hyp.bm.lpanc.V7A1.se\endcsname{0.39}
\expandafter\gdef\csname R@hyp.bm.lpanc.base.dice\endcsname{65.42}
\expandafter\gdef\csname R@hyp.bm.lpanc.base.hd95\endcsname{40.5}
\expandafter\gdef\csname R@hyp.bm.lpanc.base.nsd1\endcsname{46.00}
\expandafter\gdef\csname R@hyp.bm.lpanc.base.nsd2\endcsname{58.42}
\expandafter\gdef\csname R@hyp.bm.panc.V7A1.cancer.d\endcsname{\ensuremath{+2.56}}
\expandafter\gdef\csname R@hyp.bm.panc.V7A1.d\endcsname{\ensuremath{+1.40}}
\expandafter\gdef\csname R@hyp.bm.panc.V7A1.dhd95\endcsname{\ensuremath{-7.3}}
\expandafter\gdef\csname R@hyp.bm.panc.V7A1.dice\endcsname{66.39}
\expandafter\gdef\csname R@hyp.bm.panc.V7A1.dmax\endcsname{\ensuremath{+3.06}}
\expandafter\gdef\csname R@hyp.bm.panc.V7A1.dnsd1\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@hyp.bm.panc.V7A1.dnsd2\endcsname{\ensuremath{+1.46}}
\expandafter\gdef\csname R@hyp.bm.panc.V7A1.hd95\endcsname{50.5}
\expandafter\gdef\csname R@hyp.bm.panc.V7A1.hi\endcsname{\ensuremath{+3.61}}
\expandafter\gdef\csname R@hyp.bm.panc.V7A1.lo\endcsname{\ensuremath{-0.81}}
\expandafter\gdef\csname R@hyp.bm.panc.V7A1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.panc.V7A1.nsd1\endcsname{46.03}
\expandafter\gdef\csname R@hyp.bm.panc.V7A1.nsd2\endcsname{58.80}
\expandafter\gdef\csname R@hyp.bm.panc.V7A1.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.panc.V7A1.se\endcsname{0.69}
\expandafter\gdef\csname R@hyp.bm.panc.V7C1.d\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@hyp.bm.panc.V7C1.dhd95\endcsname{\ensuremath{-14.4}}
\expandafter\gdef\csname R@hyp.bm.panc.V7C1.dice\endcsname{65.47}
\expandafter\gdef\csname R@hyp.bm.panc.V7C1.dmax\endcsname{\ensuremath{+1.66}}
\expandafter\gdef\csname R@hyp.bm.panc.V7C1.dnsd1\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@hyp.bm.panc.V7C1.dnsd2\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@hyp.bm.panc.V7C1.hd95\endcsname{43.4}
\expandafter\gdef\csname R@hyp.bm.panc.V7C1.hi\endcsname{\ensuremath{+2.33}}
\expandafter\gdef\csname R@hyp.bm.panc.V7C1.lo\endcsname{\ensuremath{-1.38}}
\expandafter\gdef\csname R@hyp.bm.panc.V7C1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.panc.V7C1.nsd1\endcsname{45.52}
\expandafter\gdef\csname R@hyp.bm.panc.V7C1.nsd2\endcsname{58.22}
\expandafter\gdef\csname R@hyp.bm.panc.V7C1.nup\endcsname{2}
\expandafter\gdef\csname R@hyp.bm.panc.V7C1.se\endcsname{0.58}
\expandafter\gdef\csname R@hyp.bm.panc.Y2.d\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@hyp.bm.panc.Y2.dhd95\endcsname{\ensuremath{+4.2}}
\expandafter\gdef\csname R@hyp.bm.panc.Y2.dice\endcsname{65.04}
\expandafter\gdef\csname R@hyp.bm.panc.Y2.dmax\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@hyp.bm.panc.Y2.dnsd1\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@hyp.bm.panc.Y2.dnsd2\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@hyp.bm.panc.Y2.hd95\endcsname{62.0}
\expandafter\gdef\csname R@hyp.bm.panc.Y2.hi\endcsname{\ensuremath{+2.47}}
\expandafter\gdef\csname R@hyp.bm.panc.Y2.lo\endcsname{\ensuremath{-2.38}}
\expandafter\gdef\csname R@hyp.bm.panc.Y2.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.panc.Y2.nsd1\endcsname{45.72}
\expandafter\gdef\csname R@hyp.bm.panc.Y2.nsd2\endcsname{58.12}
\expandafter\gdef\csname R@hyp.bm.panc.Y2.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.panc.Y2.se\endcsname{0.76}
\expandafter\gdef\csname R@hyp.bm.panc.base.dice\endcsname{64.99}
\expandafter\gdef\csname R@hyp.bm.panc.base.hd95\endcsname{57.8}
\expandafter\gdef\csname R@hyp.bm.panc.base.nsd1\endcsname{45.03}
\expandafter\gdef\csname R@hyp.bm.panc.base.nsd2\endcsname{57.34}
\expandafter\gdef\csname R@hyp.bm.spleen.V7A1.d\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@hyp.bm.spleen.V7A1.dhd95\endcsname{\ensuremath{-27.8}}
\expandafter\gdef\csname R@hyp.bm.spleen.V7A1.dice\endcsname{96.95}
\expandafter\gdef\csname R@hyp.bm.spleen.V7A1.dmax\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@hyp.bm.spleen.V7A1.dnsd1\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@hyp.bm.spleen.V7A1.dnsd2\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@hyp.bm.spleen.V7A1.hd95\endcsname{5.1}
\expandafter\gdef\csname R@hyp.bm.spleen.V7A1.hi\endcsname{\ensuremath{+0.89}}
\expandafter\gdef\csname R@hyp.bm.spleen.V7A1.lo\endcsname{\ensuremath{-0.71}}
\expandafter\gdef\csname R@hyp.bm.spleen.V7A1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.spleen.V7A1.nsd1\endcsname{91.62}
\expandafter\gdef\csname R@hyp.bm.spleen.V7A1.nsd2\endcsname{97.24}
\expandafter\gdef\csname R@hyp.bm.spleen.V7A1.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.bm.spleen.V7A1.se\endcsname{0.25}
\expandafter\gdef\csname R@hyp.bm.spleen.V7C1.d\endcsname{\ensuremath{-1.23}}
\expandafter\gdef\csname R@hyp.bm.spleen.V7C1.dhd95\endcsname{\ensuremath{-9.3}}
\expandafter\gdef\csname R@hyp.bm.spleen.V7C1.dice\endcsname{95.63}
\expandafter\gdef\csname R@hyp.bm.spleen.V7C1.dmax\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@hyp.bm.spleen.V7C1.dnsd1\endcsname{\ensuremath{-1.73}}
\expandafter\gdef\csname R@hyp.bm.spleen.V7C1.dnsd2\endcsname{\ensuremath{-1.75}}
\expandafter\gdef\csname R@hyp.bm.spleen.V7C1.hd95\endcsname{23.7}
\expandafter\gdef\csname R@hyp.bm.spleen.V7C1.hi\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@hyp.bm.spleen.V7C1.lo\endcsname{\ensuremath{-3.59}}
\expandafter\gdef\csname R@hyp.bm.spleen.V7C1.n\endcsname{4}
\expandafter\gdef\csname R@hyp.bm.spleen.V7C1.nsd1\endcsname{88.89}
\expandafter\gdef\csname R@hyp.bm.spleen.V7C1.nsd2\endcsname{94.71}
\expandafter\gdef\csname R@hyp.bm.spleen.V7C1.nup\endcsname{1}
\expandafter\gdef\csname R@hyp.bm.spleen.V7C1.se\endcsname{0.74}
\expandafter\gdef\csname R@hyp.bm.spleen.base.dice\endcsname{96.86}
\expandafter\gdef\csname R@hyp.bm.spleen.base.hd95\endcsname{32.9}
\expandafter\gdef\csname R@hyp.bm.spleen.base.nsd1\endcsname{90.62}
\expandafter\gdef\csname R@hyp.bm.spleen.base.nsd2\endcsname{96.46}
\expandafter\gdef\csname R@hyp.cls.lesion.mean\endcsname{\ensuremath{+1.31}}
\expandafter\gdef\csname R@hyp.cls.lesion.n\endcsname{7}
\expandafter\gdef\csname R@hyp.cls.lesion.npos\endcsname{6}
\expandafter\gdef\csname R@hyp.cls.organ.mean\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@hyp.cls.organ.n\endcsname{21}
\expandafter\gdef\csname R@hyp.cls.organ.npos\endcsname{17}
\expandafter\gdef\csname R@hyp.cost.J2.gmac\endcsname{373.6}
\expandafter\gdef\csname R@hyp.cost.J2.mem\endcsname{7.77}
\expandafter\gdef\csname R@hyp.cost.J2.par\endcsname{31.04}
\expandafter\gdef\csname R@hyp.cost.J2.step\endcsname{118.7}
\expandafter\gdef\csname R@hyp.cost.Y3.gmac\endcsname{373.6}
\expandafter\gdef\csname R@hyp.cost.Y3.mem\endcsname{7.77}
\expandafter\gdef\csname R@hyp.cost.Y3.par\endcsname{31.04}
\expandafter\gdef\csname R@hyp.cost.Y3.step\endcsname{115.7}
\expandafter\gdef\csname R@hyp.cyst.bear.Y2\endcsname{75.67}
\expandafter\gdef\csname R@hyp.cyst.free.Y2\endcsname{84.13}
\expandafter\gdef\csname R@hyp.cyst.gain.bear.Y2\endcsname{\ensuremath{+3.45}}
\expandafter\gdef\csname R@hyp.ev.mean\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@hyp.ev.n\endcsname{14}
\expandafter\gdef\csname R@hyp.ev.npos\endcsname{14}
\expandafter\gdef\csname R@hyp.ev.p\endcsname{0.0001}
\expandafter\gdef\csname R@hyp.ev.rule.n\endcsname{15}
\expandafter\gdef\csname R@hyp.l3.n\endcsname{6}
\expandafter\gdef\csname R@hyp.l3.nwin\endcsname{4}
\expandafter\gdef\csname R@hyp.lkipa.ncase\endcsname{14}
\expandafter\gdef\csname R@hyp.lkipa.on\endcsname{1}
\expandafter\gdef\csname R@hyp.lock.d\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@hyp.lock.kipa.d\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@hyp.lock.kipa.hi\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@hyp.lock.kipa.lo\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@hyp.lock.n\endcsname{10}
\expandafter\gdef\csname R@hyp.lock.npos\endcsname{9}
\expandafter\gdef\csname R@hyp.lock.nsets.word\endcsname{four}
\expandafter\gdef\csname R@hyp.lock.p\endcsname{0.011}
\expandafter\gdef\csname R@hyp.lock.panc.d\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@hyp.lock.panc.hi\endcsname{\ensuremath{+2.77}}
\expandafter\gdef\csname R@hyp.lock.panc.lo\endcsname{\ensuremath{-1.88}}
\expandafter\gdef\csname R@hyp.lpanc.ncase\endcsname{56}
\expandafter\gdef\csname R@hyp.mri.amos13.M.d\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@hyp.mri.amos13.M.dL1\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@hyp.mri.amos13.M.dL1S\endcsname{\ensuremath{+1.22}}
\expandafter\gdef\csname R@hyp.mri.amos13.M.dice\endcsname{81.19}
\expandafter\gdef\csname R@hyp.mri.brats.L1.d\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@hyp.mri.brats.M.d\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@hyp.mri.brats.M.dL1\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@hyp.mri.brats.M.dL3\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@hyp.mri.brats.M.dice\endcsname{83.21}
\expandafter\gdef\csname R@hyp.mri.brats.M.hi\endcsname{\ensuremath{+1.31}}
\expandafter\gdef\csname R@hyp.mri.brats.M.lo\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@hyp.mri.brats.Rule.d\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@hyp.mri.brats.Rule.hi\endcsname{\ensuremath{+1.47}}
\expandafter\gdef\csname R@hyp.mri.brats.Rule.lo\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@hyp.mri.heart.S.d\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@hyp.mri.heart.S.dM\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@hyp.mri.heart.S.peak\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@hyp.mri.heart.bf\endcsname{0.15}
\expandafter\gdef\csname R@hyp.mri.hippo.r1.d\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@hyp.mri.hippo.r1.nup\endcsname{3}
\expandafter\gdef\csname R@hyp.next.kits.H1.dM\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@hyp.next.kits.H1.dbase\endcsname{\ensuremath{+2.01}}
\expandafter\gdef\csname R@hyp.next.kits.H1.dice\endcsname{86.00}
\expandafter\gdef\csname R@hyp.next.kits.H1.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.next.kits.J1.dM\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@hyp.next.kits.J1.dbase\endcsname{\ensuremath{+2.25}}
\expandafter\gdef\csname R@hyp.next.kits.J1.dice\endcsname{86.25}
\expandafter\gdef\csname R@hyp.next.kits.J1.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.next.kits.J2.dM\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@hyp.next.kits.J2.dbase\endcsname{\ensuremath{+2.32}}
\expandafter\gdef\csname R@hyp.next.kits.J2.dice\endcsname{86.31}
\expandafter\gdef\csname R@hyp.next.kits.J2.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.next.kits.J4.dM\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@hyp.next.kits.J4.dbase\endcsname{\ensuremath{+1.93}}
\expandafter\gdef\csname R@hyp.next.kits.J4.dice\endcsname{85.92}
\expandafter\gdef\csname R@hyp.next.kits.J4.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.next.kits.Y3.dM\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@hyp.next.kits.Y3.dbase\endcsname{\ensuremath{+2.21}}
\expandafter\gdef\csname R@hyp.next.kits.Y3.dice\endcsname{86.21}
\expandafter\gdef\csname R@hyp.next.kits.Y3.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.next.kits.Y4.dM\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@hyp.next.kits.Y4.dbase\endcsname{\ensuremath{+2.11}}
\expandafter\gdef\csname R@hyp.next.kits.Y4.dice\endcsname{86.11}
\expandafter\gdef\csname R@hyp.next.kits.Y4.nup\endcsname{4}
\expandafter\gdef\csname R@hyp.peak.acdc.L1.d\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@hyp.peak.acdc.L1.dice\endcsname{90.53}
\expandafter\gdef\csname R@hyp.peak.acdc.L1S.d\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@hyp.peak.acdc.L1S.dice\endcsname{90.13}
\expandafter\gdef\csname R@hyp.peak.acdc.L3.d\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@hyp.peak.acdc.L3.dice\endcsname{90.29}
\expandafter\gdef\csname R@hyp.peak.acdc.Rule.d\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@hyp.peak.acdc.Rule.dice\endcsname{90.54}
\expandafter\gdef\csname R@hyp.peak.acdc.V11.d\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@hyp.peak.acdc.V11.dice\endcsname{90.36}
\expandafter\gdef\csname R@hyp.peak.acdc.V7A1.d\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@hyp.peak.acdc.V7A1.dice\endcsname{90.53}
\expandafter\gdef\csname R@hyp.peak.acdc.V7C1.d\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@hyp.peak.acdc.V7C1.dice\endcsname{89.91}
\expandafter\gdef\csname R@hyp.peak.acdc.Y11.d\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@hyp.peak.acdc.Y11.dice\endcsname{90.03}
\expandafter\gdef\csname R@hyp.peak.acdc.Y12.d\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@hyp.peak.acdc.Y12.dice\endcsname{90.13}
\expandafter\gdef\csname R@hyp.peak.acdc.Y13.d\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@hyp.peak.acdc.Y13.dice\endcsname{90.54}
\expandafter\gdef\csname R@hyp.peak.acdc.Y7.d\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@hyp.peak.acdc.Y7.dice\endcsname{90.21}
\expandafter\gdef\csname R@hyp.peak.acdc.base.dice\endcsname{89.97}
\expandafter\gdef\csname R@hyp.peak.acdc.split\endcsname{fold~4}
\expandafter\gdef\csname R@hyp.peak.amos.H1.d\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@hyp.peak.amos.H1.dice\endcsname{87.62}
\expandafter\gdef\csname R@hyp.peak.amos.L1.d\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@hyp.peak.amos.L1.dice\endcsname{87.68}
\expandafter\gdef\csname R@hyp.peak.amos.L1S.d\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@hyp.peak.amos.L1S.dice\endcsname{87.12}
\expandafter\gdef\csname R@hyp.peak.amos.L3.d\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@hyp.peak.amos.L3.dice\endcsname{87.38}
\expandafter\gdef\csname R@hyp.peak.amos.MedNeXtM.d\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@hyp.peak.amos.MedNeXtM.dice\endcsname{87.82}
\expandafter\gdef\csname R@hyp.peak.amos.Rule.d\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@hyp.peak.amos.Rule.dice\endcsname{87.88}
\expandafter\gdef\csname R@hyp.peak.amos.V10B.d\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@hyp.peak.amos.V10B.dice\endcsname{87.88}
\expandafter\gdef\csname R@hyp.peak.amos.V11.d\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@hyp.peak.amos.V11.dice\endcsname{87.56}
\expandafter\gdef\csname R@hyp.peak.amos.V7A1.d\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@hyp.peak.amos.V7A1.dice\endcsname{87.80}
\expandafter\gdef\csname R@hyp.peak.amos.V7C1.d\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@hyp.peak.amos.V7C1.dice\endcsname{86.72}
\expandafter\gdef\csname R@hyp.peak.amos.Y11.d\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@hyp.peak.amos.Y11.dice\endcsname{87.76}
\expandafter\gdef\csname R@hyp.peak.amos.Y12.d\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@hyp.peak.amos.Y12.dice\endcsname{87.59}
\expandafter\gdef\csname R@hyp.peak.amos.Y13.d\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@hyp.peak.amos.Y13.dice\endcsname{87.86}
\expandafter\gdef\csname R@hyp.peak.amos.Y14.d\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@hyp.peak.amos.Y14.dice\endcsname{87.63}
\expandafter\gdef\csname R@hyp.peak.amos.Y2.d\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@hyp.peak.amos.Y2.dice\endcsname{87.65}
\expandafter\gdef\csname R@hyp.peak.amos.Y3.d\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@hyp.peak.amos.Y3.dice\endcsname{87.68}
\expandafter\gdef\csname R@hyp.peak.amos.base.dice\endcsname{87.00}
\expandafter\gdef\csname R@hyp.peak.amos.split\endcsname{fold~4}
\expandafter\gdef\csname R@hyp.peak.brats.L1.d\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@hyp.peak.brats.L1.dice\endcsname{82.95}
\expandafter\gdef\csname R@hyp.peak.brats.L1S.d\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@hyp.peak.brats.L1S.dice\endcsname{82.80}
\expandafter\gdef\csname R@hyp.peak.brats.L3.d\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@hyp.peak.brats.L3.dice\endcsname{83.05}
\expandafter\gdef\csname R@hyp.peak.brats.Rule.d\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@hyp.peak.brats.Rule.dL1\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@hyp.peak.brats.Rule.dice\endcsname{83.31}
\expandafter\gdef\csname R@hyp.peak.brats.V10B.d\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@hyp.peak.brats.V10B.dice\endcsname{83.19}
\expandafter\gdef\csname R@hyp.peak.brats.V11.d\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@hyp.peak.brats.V11.dice\endcsname{83.10}
\expandafter\gdef\csname R@hyp.peak.brats.V7A1.d\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@hyp.peak.brats.V7A1.dice\endcsname{83.21}
\expandafter\gdef\csname R@hyp.peak.brats.V7C1.d\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@hyp.peak.brats.V7C1.dice\endcsname{83.12}
\expandafter\gdef\csname R@hyp.peak.brats.Y11.d\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@hyp.peak.brats.Y11.dice\endcsname{82.95}
\expandafter\gdef\csname R@hyp.peak.brats.Y12.d\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@hyp.peak.brats.Y12.dice\endcsname{82.74}
\expandafter\gdef\csname R@hyp.peak.brats.Y13.d\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@hyp.peak.brats.Y13.dice\endcsname{82.87}
\expandafter\gdef\csname R@hyp.peak.brats.Y14.d\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@hyp.peak.brats.Y14.dice\endcsname{83.12}
\expandafter\gdef\csname R@hyp.peak.brats.Y2.d\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@hyp.peak.brats.Y2.dice\endcsname{82.95}
\expandafter\gdef\csname R@hyp.peak.brats.Y6.d\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@hyp.peak.brats.Y6.dice\endcsname{82.87}
\expandafter\gdef\csname R@hyp.peak.brats.Y7.d\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@hyp.peak.brats.Y7.dice\endcsname{83.31}
\expandafter\gdef\csname R@hyp.peak.brats.base.dice\endcsname{82.98}
\expandafter\gdef\csname R@hyp.peak.brats.split\endcsname{run~1}
\expandafter\gdef\csname R@hyp.peak.btcv.J1.d\endcsname{\ensuremath{-77.57}}
\expandafter\gdef\csname R@hyp.peak.btcv.J1.dice\endcsname{0.00}
\expandafter\gdef\csname R@hyp.peak.btcv.J2.d\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@hyp.peak.btcv.J2.dice\endcsname{78.10}
\expandafter\gdef\csname R@hyp.peak.btcv.L1.d\endcsname{\ensuremath{+1.67}}
\expandafter\gdef\csname R@hyp.peak.btcv.L1.dice\endcsname{79.24}
\expandafter\gdef\csname R@hyp.peak.btcv.L1S.d\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@hyp.peak.btcv.L1S.dice\endcsname{77.85}
\expandafter\gdef\csname R@hyp.peak.btcv.L3.d\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@hyp.peak.btcv.L3.dice\endcsname{77.85}
\expandafter\gdef\csname R@hyp.peak.btcv.Rule.d\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@hyp.peak.btcv.Rule.dice\endcsname{78.94}
\expandafter\gdef\csname R@hyp.peak.btcv.V10B.d\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@hyp.peak.btcv.V10B.dice\endcsname{77.88}
\expandafter\gdef\csname R@hyp.peak.btcv.V11.d\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@hyp.peak.btcv.V11.dice\endcsname{78.02}
\expandafter\gdef\csname R@hyp.peak.btcv.V7A1.d\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@hyp.peak.btcv.V7A1.dice\endcsname{78.43}
\expandafter\gdef\csname R@hyp.peak.btcv.V7C1.d\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@hyp.peak.btcv.V7C1.dice\endcsname{77.67}
\expandafter\gdef\csname R@hyp.peak.btcv.Y11.d\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@hyp.peak.btcv.Y11.dice\endcsname{78.30}
\expandafter\gdef\csname R@hyp.peak.btcv.Y12.d\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@hyp.peak.btcv.Y12.dice\endcsname{78.19}
\expandafter\gdef\csname R@hyp.peak.btcv.Y13.d\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@hyp.peak.btcv.Y13.dice\endcsname{78.94}
\expandafter\gdef\csname R@hyp.peak.btcv.Y14.d\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@hyp.peak.btcv.Y14.dice\endcsname{78.25}
\expandafter\gdef\csname R@hyp.peak.btcv.Y3.d\endcsname{\ensuremath{+0.72}}
\expandafter\gdef\csname R@hyp.peak.btcv.Y3.dice\endcsname{78.29}
\expandafter\gdef\csname R@hyp.peak.btcv.base.dice\endcsname{77.57}
\expandafter\gdef\csname R@hyp.peak.btcv.split\endcsname{run~1}
\expandafter\gdef\csname R@hyp.peak.heart.L1.d\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@hyp.peak.heart.L1.dice\endcsname{92.55}
\expandafter\gdef\csname R@hyp.peak.heart.L1S.d\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@hyp.peak.heart.L1S.dice\endcsname{92.51}
\expandafter\gdef\csname R@hyp.peak.heart.L3.d\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@hyp.peak.heart.L3.dice\endcsname{92.56}
\expandafter\gdef\csname R@hyp.peak.heart.Rule.d\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@hyp.peak.heart.Rule.dice\endcsname{92.84}
\expandafter\gdef\csname R@hyp.peak.heart.V10B.d\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@hyp.peak.heart.V10B.dice\endcsname{92.61}
\expandafter\gdef\csname R@hyp.peak.heart.V7A1.d\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@hyp.peak.heart.V7A1.dice\endcsname{92.55}
\expandafter\gdef\csname R@hyp.peak.heart.V7C1.d\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@hyp.peak.heart.V7C1.dice\endcsname{92.84}
\expandafter\gdef\csname R@hyp.peak.heart.base.dice\endcsname{92.48}
\expandafter\gdef\csname R@hyp.peak.heart.split\endcsname{fold~2}
\expandafter\gdef\csname R@hyp.peak.hepv.J1.d\endcsname{\ensuremath{-0.54}}
\expandafter\gdef\csname R@hyp.peak.hepv.J1.dice\endcsname{63.18}
\expandafter\gdef\csname R@hyp.peak.hepv.J2.d\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@hyp.peak.hepv.J2.dice\endcsname{63.70}
\expandafter\gdef\csname R@hyp.peak.hepv.L1.d\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@hyp.peak.hepv.L1.dice\endcsname{63.26}
\expandafter\gdef\csname R@hyp.peak.hepv.L1S.d\endcsname{\ensuremath{+0.79}}
\expandafter\gdef\csname R@hyp.peak.hepv.L1S.dice\endcsname{64.50}
\expandafter\gdef\csname R@hyp.peak.hepv.L3.d\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@hyp.peak.hepv.L3.dice\endcsname{63.37}
\expandafter\gdef\csname R@hyp.peak.hepv.Rule.d\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@hyp.peak.hepv.Rule.dice\endcsname{64.47}
\expandafter\gdef\csname R@hyp.peak.hepv.V10B.d\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@hyp.peak.hepv.V10B.dice\endcsname{64.29}
\expandafter\gdef\csname R@hyp.peak.hepv.V11.d\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@hyp.peak.hepv.V11.dice\endcsname{63.93}
\expandafter\gdef\csname R@hyp.peak.hepv.V7A1.d\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@hyp.peak.hepv.V7A1.dice\endcsname{64.27}
\expandafter\gdef\csname R@hyp.peak.hepv.V7C1.d\endcsname{\ensuremath{-1.03}}
\expandafter\gdef\csname R@hyp.peak.hepv.V7C1.dice\endcsname{62.69}
\expandafter\gdef\csname R@hyp.peak.hepv.Y11.d\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@hyp.peak.hepv.Y11.dice\endcsname{64.47}
\expandafter\gdef\csname R@hyp.peak.hepv.Y12.d\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@hyp.peak.hepv.Y12.dice\endcsname{64.00}
\expandafter\gdef\csname R@hyp.peak.hepv.Y13.d\endcsname{\ensuremath{-1.06}}
\expandafter\gdef\csname R@hyp.peak.hepv.Y13.dice\endcsname{62.65}
\expandafter\gdef\csname R@hyp.peak.hepv.Y14.d\endcsname{0.00}
\expandafter\gdef\csname R@hyp.peak.hepv.Y14.dice\endcsname{63.72}
\expandafter\gdef\csname R@hyp.peak.hepv.Y2.d\endcsname{\ensuremath{-0.88}}
\expandafter\gdef\csname R@hyp.peak.hepv.Y2.dice\endcsname{62.84}
\expandafter\gdef\csname R@hyp.peak.hepv.Y3.d\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@hyp.peak.hepv.Y3.dice\endcsname{63.53}
\expandafter\gdef\csname R@hyp.peak.hepv.Y4.d\endcsname{\ensuremath{-1.06}}
\expandafter\gdef\csname R@hyp.peak.hepv.Y4.dice\endcsname{62.65}
\expandafter\gdef\csname R@hyp.peak.hepv.base.dice\endcsname{63.72}
\expandafter\gdef\csname R@hyp.peak.hepv.split\endcsname{fold~2}
\expandafter\gdef\csname R@hyp.peak.kipa22.J1.d\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@hyp.peak.kipa22.J1.dice\endcsname{90.35}
\expandafter\gdef\csname R@hyp.peak.kipa22.J1.tumour.dice\endcsname{93.45}
\expandafter\gdef\csname R@hyp.peak.kipa22.J2.d\endcsname{\ensuremath{+0.94}}
\expandafter\gdef\csname R@hyp.peak.kipa22.J2.dice\endcsname{90.53}
\expandafter\gdef\csname R@hyp.peak.kipa22.J2.tumour.dice\endcsname{93.41}
\expandafter\gdef\csname R@hyp.peak.kipa22.L1.d\endcsname{\ensuremath{+0.79}}
\expandafter\gdef\csname R@hyp.peak.kipa22.L1.dice\endcsname{90.37}
\expandafter\gdef\csname R@hyp.peak.kipa22.L1S.d\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@hyp.peak.kipa22.L1S.dice\endcsname{89.10}
\expandafter\gdef\csname R@hyp.peak.kipa22.L3.d\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@hyp.peak.kipa22.L3.dice\endcsname{90.27}
\expandafter\gdef\csname R@hyp.peak.kipa22.Rule.d\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@hyp.peak.kipa22.Rule.dice\endcsname{90.59}
\expandafter\gdef\csname R@hyp.peak.kipa22.V10B.d\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@hyp.peak.kipa22.V10B.dice\endcsname{90.01}
\expandafter\gdef\csname R@hyp.peak.kipa22.V10B.tumour.dice\endcsname{92.03}
\expandafter\gdef\csname R@hyp.peak.kipa22.V11.d\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@hyp.peak.kipa22.V11.dice\endcsname{90.59}
\expandafter\gdef\csname R@hyp.peak.kipa22.V11.tumour.dice\endcsname{93.81}
\expandafter\gdef\csname R@hyp.peak.kipa22.V7A1.d\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@hyp.peak.kipa22.V7A1.dice\endcsname{89.82}
\expandafter\gdef\csname R@hyp.peak.kipa22.V7C1.d\endcsname{\ensuremath{-1.17}}
\expandafter\gdef\csname R@hyp.peak.kipa22.V7C1.dice\endcsname{88.42}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y11.d\endcsname{\ensuremath{+0.95}}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y11.dice\endcsname{90.53}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y11.tumour.dice\endcsname{93.40}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y12.d\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y12.dice\endcsname{90.51}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y12.tumour.dice\endcsname{93.85}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y13.d\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y13.dice\endcsname{90.55}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y13.tumour.dice\endcsname{93.29}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y14.d\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y14.dice\endcsname{90.59}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y14.tumour.dice\endcsname{93.38}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y2.d\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y2.dice\endcsname{89.94}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y3.d\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y3.dice\endcsname{90.21}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y3.tumour.dice\endcsname{93.23}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y4.d\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y4.dice\endcsname{89.62}
\expandafter\gdef\csname R@hyp.peak.kipa22.Y4.tumour.dice\endcsname{89.18}
\expandafter\gdef\csname R@hyp.peak.kipa22.base.dice\endcsname{89.59}
\expandafter\gdef\csname R@hyp.peak.kipa22.split\endcsname{fold~4}
\expandafter\gdef\csname R@hyp.peak.kits.H1.d\endcsname{\ensuremath{+3.65}}
\expandafter\gdef\csname R@hyp.peak.kits.H1.dice\endcsname{86.51}
\expandafter\gdef\csname R@hyp.peak.kits.J1.d\endcsname{\ensuremath{+3.56}}
\expandafter\gdef\csname R@hyp.peak.kits.J1.dice\endcsname{86.42}
\expandafter\gdef\csname R@hyp.peak.kits.J2.d\endcsname{\ensuremath{+4.28}}
\expandafter\gdef\csname R@hyp.peak.kits.J2.dice\endcsname{87.14}
\expandafter\gdef\csname R@hyp.peak.kits.J4.d\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@hyp.peak.kits.J4.dice\endcsname{85.17}
\expandafter\gdef\csname R@hyp.peak.kits.L1.d\endcsname{\ensuremath{+2.58}}
\expandafter\gdef\csname R@hyp.peak.kits.L1.dice\endcsname{85.44}
\expandafter\gdef\csname R@hyp.peak.kits.L1S.d\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@hyp.peak.kits.L1S.dice\endcsname{84.98}
\expandafter\gdef\csname R@hyp.peak.kits.L3.d\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@hyp.peak.kits.L3.dice\endcsname{85.17}
\expandafter\gdef\csname R@hyp.peak.kits.MedNeXtM.d\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@hyp.peak.kits.MedNeXtM.dice\endcsname{82.43}
\expandafter\gdef\csname R@hyp.peak.kits.R5.arm\endcsname{J2}
\expandafter\gdef\csname R@hyp.peak.kits.R5.d\endcsname{\ensuremath{+4.28}}
\expandafter\gdef\csname R@hyp.peak.kits.R5.dL1\endcsname{\ensuremath{+1.70}}
\expandafter\gdef\csname R@hyp.peak.kits.R5.dice\endcsname{87.14}
\expandafter\gdef\csname R@hyp.peak.kits.Rule.d\endcsname{\ensuremath{+3.47}}
\expandafter\gdef\csname R@hyp.peak.kits.Rule.dice\endcsname{86.33}
\expandafter\gdef\csname R@hyp.peak.kits.V11.d\endcsname{\ensuremath{+2.75}}
\expandafter\gdef\csname R@hyp.peak.kits.V11.dice\endcsname{85.61}
\expandafter\gdef\csname R@hyp.peak.kits.V7A1.d\endcsname{\ensuremath{+2.03}}
\expandafter\gdef\csname R@hyp.peak.kits.V7A1.dice\endcsname{84.89}
\expandafter\gdef\csname R@hyp.peak.kits.V7C1.d\endcsname{\ensuremath{+2.14}}
\expandafter\gdef\csname R@hyp.peak.kits.V7C1.dice\endcsname{85.00}
\expandafter\gdef\csname R@hyp.peak.kits.Y11.d\endcsname{\ensuremath{+2.47}}
\expandafter\gdef\csname R@hyp.peak.kits.Y11.dice\endcsname{85.33}
\expandafter\gdef\csname R@hyp.peak.kits.Y12.d\endcsname{\ensuremath{+2.19}}
\expandafter\gdef\csname R@hyp.peak.kits.Y12.dice\endcsname{85.05}
\expandafter\gdef\csname R@hyp.peak.kits.Y13.d\endcsname{\ensuremath{+2.66}}
\expandafter\gdef\csname R@hyp.peak.kits.Y13.dice\endcsname{85.52}
\expandafter\gdef\csname R@hyp.peak.kits.Y14.d\endcsname{\ensuremath{+2.98}}
\expandafter\gdef\csname R@hyp.peak.kits.Y14.dice\endcsname{85.84}
\expandafter\gdef\csname R@hyp.peak.kits.Y2.d\endcsname{\ensuremath{+3.47}}
\expandafter\gdef\csname R@hyp.peak.kits.Y2.dL1\endcsname{\ensuremath{+0.89}}
\expandafter\gdef\csname R@hyp.peak.kits.Y2.dice\endcsname{86.33}
\expandafter\gdef\csname R@hyp.peak.kits.Y3.d\endcsname{\ensuremath{+3.69}}
\expandafter\gdef\csname R@hyp.peak.kits.Y3.dice\endcsname{86.55}
\expandafter\gdef\csname R@hyp.peak.kits.Y4.d\endcsname{\ensuremath{+4.03}}
\expandafter\gdef\csname R@hyp.peak.kits.Y4.dice\endcsname{86.89}
\expandafter\gdef\csname R@hyp.peak.kits.Y5.d\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@hyp.peak.kits.Y5.dice\endcsname{84.31}
\expandafter\gdef\csname R@hyp.peak.kits.base.dice\endcsname{82.86}
\expandafter\gdef\csname R@hyp.peak.kits.split\endcsname{fold~1}
\expandafter\gdef\csname R@hyp.peak.lacdc.L1.d\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@hyp.peak.lacdc.L1.dice\endcsname{91.91}
\expandafter\gdef\csname R@hyp.peak.lacdc.L1S.d\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@hyp.peak.lacdc.L1S.dice\endcsname{91.48}
\expandafter\gdef\csname R@hyp.peak.lacdc.Rule.d\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@hyp.peak.lacdc.Rule.dice\endcsname{91.67}
\expandafter\gdef\csname R@hyp.peak.lacdc.V7A1.d\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@hyp.peak.lacdc.V7A1.dice\endcsname{91.67}
\expandafter\gdef\csname R@hyp.peak.lacdc.base.dice\endcsname{91.35}
\expandafter\gdef\csname R@hyp.peak.lacdc.split\endcsname{run~2}
\expandafter\gdef\csname R@hyp.peak.lamos.L1.d\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@hyp.peak.lamos.L1.dice\endcsname{90.02}
\expandafter\gdef\csname R@hyp.peak.lamos.L1S.d\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@hyp.peak.lamos.L1S.dice\endcsname{89.32}
\expandafter\gdef\csname R@hyp.peak.lamos.Rule.d\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@hyp.peak.lamos.Rule.dice\endcsname{90.06}
\expandafter\gdef\csname R@hyp.peak.lamos.V7A1.d\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@hyp.peak.lamos.V7A1.dice\endcsname{90.06}
\expandafter\gdef\csname R@hyp.peak.lamos.base.dice\endcsname{89.72}
\expandafter\gdef\csname R@hyp.peak.lamos.split\endcsname{run~2}
\expandafter\gdef\csname R@hyp.peak.lits.H1.d\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@hyp.peak.lits.H1.dice\endcsname{80.28}
\expandafter\gdef\csname R@hyp.peak.lits.L1.d\endcsname{\ensuremath{+1.79}}
\expandafter\gdef\csname R@hyp.peak.lits.L1.dice\endcsname{81.76}
\expandafter\gdef\csname R@hyp.peak.lits.L1S.d\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@hyp.peak.lits.L1S.dice\endcsname{80.91}
\expandafter\gdef\csname R@hyp.peak.lits.L3.d\endcsname{\ensuremath{+2.20}}
\expandafter\gdef\csname R@hyp.peak.lits.L3.dice\endcsname{82.17}
\expandafter\gdef\csname R@hyp.peak.lits.Rule.d\endcsname{\ensuremath{+4.18}}
\expandafter\gdef\csname R@hyp.peak.lits.Rule.dice\endcsname{84.16}
\expandafter\gdef\csname R@hyp.peak.lits.V10B.d\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@hyp.peak.lits.V10B.dice\endcsname{82.51}
\expandafter\gdef\csname R@hyp.peak.lits.V11.d\endcsname{\ensuremath{+1.81}}
\expandafter\gdef\csname R@hyp.peak.lits.V11.dice\endcsname{81.79}
\expandafter\gdef\csname R@hyp.peak.lits.V7A1.d\endcsname{\ensuremath{+4.18}}
\expandafter\gdef\csname R@hyp.peak.lits.V7A1.dice\endcsname{84.16}
\expandafter\gdef\csname R@hyp.peak.lits.V7C1.d\endcsname{\ensuremath{+2.78}}
\expandafter\gdef\csname R@hyp.peak.lits.V7C1.dice\endcsname{82.76}
\expandafter\gdef\csname R@hyp.peak.lits.Y11.d\endcsname{\ensuremath{+2.00}}
\expandafter\gdef\csname R@hyp.peak.lits.Y11.dice\endcsname{81.97}
\expandafter\gdef\csname R@hyp.peak.lits.Y12.d\endcsname{\ensuremath{+2.65}}
\expandafter\gdef\csname R@hyp.peak.lits.Y12.dice\endcsname{82.62}
\expandafter\gdef\csname R@hyp.peak.lits.Y13.d\endcsname{\ensuremath{+1.87}}
\expandafter\gdef\csname R@hyp.peak.lits.Y13.dice\endcsname{81.85}
\expandafter\gdef\csname R@hyp.peak.lits.Y14.d\endcsname{\ensuremath{+2.96}}
\expandafter\gdef\csname R@hyp.peak.lits.Y14.dice\endcsname{82.94}
\expandafter\gdef\csname R@hyp.peak.lits.Y2.d\endcsname{\ensuremath{+3.30}}
\expandafter\gdef\csname R@hyp.peak.lits.Y2.dice\endcsname{83.27}
\expandafter\gdef\csname R@hyp.peak.lits.Y3.d\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@hyp.peak.lits.Y3.dice\endcsname{81.46}
\expandafter\gdef\csname R@hyp.peak.lits.Y7.d\endcsname{\ensuremath{+2.62}}
\expandafter\gdef\csname R@hyp.peak.lits.Y7.dice\endcsname{82.60}
\expandafter\gdef\csname R@hyp.peak.lits.base.dice\endcsname{79.98}
\expandafter\gdef\csname R@hyp.peak.lits.split\endcsname{run~2}
\expandafter\gdef\csname R@hyp.peak.lkipa.L1.d\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@hyp.peak.lkipa.L1.dice\endcsname{87.66}
\expandafter\gdef\csname R@hyp.peak.lkipa.L1S.d\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@hyp.peak.lkipa.L1S.dice\endcsname{87.44}
\expandafter\gdef\csname R@hyp.peak.lkipa.Rule.d\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@hyp.peak.lkipa.Rule.dice\endcsname{88.07}
\expandafter\gdef\csname R@hyp.peak.lkipa.V7A1.d\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@hyp.peak.lkipa.V7A1.dice\endcsname{88.07}
\expandafter\gdef\csname R@hyp.peak.lkipa.base.dice\endcsname{87.44}
\expandafter\gdef\csname R@hyp.peak.lkipa.split\endcsname{run~1}
\expandafter\gdef\csname R@hyp.peak.lpanc.L1.d\endcsname{\ensuremath{+2.24}}
\expandafter\gdef\csname R@hyp.peak.lpanc.L1.dice\endcsname{67.20}
\expandafter\gdef\csname R@hyp.peak.lpanc.L1S.d\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@hyp.peak.lpanc.L1S.dice\endcsname{66.54}
\expandafter\gdef\csname R@hyp.peak.lpanc.Rule.d\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@hyp.peak.lpanc.Rule.dice\endcsname{66.17}
\expandafter\gdef\csname R@hyp.peak.lpanc.V7A1.d\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@hyp.peak.lpanc.V7A1.dice\endcsname{66.17}
\expandafter\gdef\csname R@hyp.peak.lpanc.base.dice\endcsname{64.95}
\expandafter\gdef\csname R@hyp.peak.lpanc.split\endcsname{run~1}
\expandafter\gdef\csname R@hyp.peak.other.max\endcsname{\ensuremath{+4.18}}
\expandafter\gdef\csname R@hyp.peak.other.min\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@hyp.peak.other.n\endcsname{13}
\expandafter\gdef\csname R@hyp.peak.panc.H1.d\endcsname{\ensuremath{+2.17}}
\expandafter\gdef\csname R@hyp.peak.panc.H1.dice\endcsname{62.49}
\expandafter\gdef\csname R@hyp.peak.panc.J1.d\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@hyp.peak.panc.J1.dice\endcsname{60.62}
\expandafter\gdef\csname R@hyp.peak.panc.J2.d\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@hyp.peak.panc.J2.dice\endcsname{61.10}
\expandafter\gdef\csname R@hyp.peak.panc.L1.d\endcsname{\ensuremath{+3.04}}
\expandafter\gdef\csname R@hyp.peak.panc.L1.dice\endcsname{63.36}
\expandafter\gdef\csname R@hyp.peak.panc.L1S.d\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@hyp.peak.panc.L1S.dice\endcsname{61.14}
\expandafter\gdef\csname R@hyp.peak.panc.L3.d\endcsname{\ensuremath{-1.42}}
\expandafter\gdef\csname R@hyp.peak.panc.L3.dice\endcsname{58.90}
\expandafter\gdef\csname R@hyp.peak.panc.Rule.d\endcsname{\ensuremath{+3.06}}
\expandafter\gdef\csname R@hyp.peak.panc.Rule.dice\endcsname{63.38}
\expandafter\gdef\csname R@hyp.peak.panc.V10B.d\endcsname{\ensuremath{+2.26}}
\expandafter\gdef\csname R@hyp.peak.panc.V10B.dice\endcsname{62.58}
\expandafter\gdef\csname R@hyp.peak.panc.V11.d\endcsname{\ensuremath{+2.79}}
\expandafter\gdef\csname R@hyp.peak.panc.V11.dice\endcsname{63.11}
\expandafter\gdef\csname R@hyp.peak.panc.V7A1.d\endcsname{\ensuremath{+3.06}}
\expandafter\gdef\csname R@hyp.peak.panc.V7A1.dice\endcsname{63.38}
\expandafter\gdef\csname R@hyp.peak.panc.V7C1.d\endcsname{\ensuremath{+1.20}}
\expandafter\gdef\csname R@hyp.peak.panc.V7C1.dice\endcsname{61.52}
\expandafter\gdef\csname R@hyp.peak.panc.Y11.d\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@hyp.peak.panc.Y11.dice\endcsname{60.97}
\expandafter\gdef\csname R@hyp.peak.panc.Y12.d\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@hyp.peak.panc.Y12.dice\endcsname{60.75}
\expandafter\gdef\csname R@hyp.peak.panc.Y13.d\endcsname{\ensuremath{+2.30}}
\expandafter\gdef\csname R@hyp.peak.panc.Y13.dice\endcsname{62.62}
\expandafter\gdef\csname R@hyp.peak.panc.Y14.d\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@hyp.peak.panc.Y14.dice\endcsname{61.69}
\expandafter\gdef\csname R@hyp.peak.panc.Y2.d\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@hyp.peak.panc.Y2.dice\endcsname{61.30}
\expandafter\gdef\csname R@hyp.peak.panc.Y3.d\endcsname{\ensuremath{-1.14}}
\expandafter\gdef\csname R@hyp.peak.panc.Y3.dice\endcsname{59.18}
\expandafter\gdef\csname R@hyp.peak.panc.base.dice\endcsname{60.32}
\expandafter\gdef\csname R@hyp.peak.panc.split\endcsname{fold~2}
\expandafter\gdef\csname R@hyp.peak.spleen.L1.d\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@hyp.peak.spleen.L1.dice\endcsname{97.26}
\expandafter\gdef\csname R@hyp.peak.spleen.L1S.d\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@hyp.peak.spleen.L1S.dice\endcsname{97.31}
\expandafter\gdef\csname R@hyp.peak.spleen.L3.d\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@hyp.peak.spleen.L3.dice\endcsname{97.31}
\expandafter\gdef\csname R@hyp.peak.spleen.Rule.d\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@hyp.peak.spleen.Rule.dice\endcsname{97.35}
\expandafter\gdef\csname R@hyp.peak.spleen.V10B.d\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@hyp.peak.spleen.V10B.dice\endcsname{97.31}
\expandafter\gdef\csname R@hyp.peak.spleen.V11.d\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@hyp.peak.spleen.V11.dice\endcsname{97.30}
\expandafter\gdef\csname R@hyp.peak.spleen.V7A1.d\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@hyp.peak.spleen.V7A1.dice\endcsname{97.35}
\expandafter\gdef\csname R@hyp.peak.spleen.V7C1.d\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@hyp.peak.spleen.V7C1.dice\endcsname{96.47}
\expandafter\gdef\csname R@hyp.peak.spleen.Y12.d\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@hyp.peak.spleen.Y12.dice\endcsname{97.21}
\expandafter\gdef\csname R@hyp.peak.spleen.Y13.d\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@hyp.peak.spleen.Y13.dice\endcsname{97.23}
\expandafter\gdef\csname R@hyp.peak.spleen.Y14.d\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@hyp.peak.spleen.Y14.dice\endcsname{97.22}
\expandafter\gdef\csname R@hyp.peak.spleen.base.dice\endcsname{96.90}
\expandafter\gdef\csname R@hyp.peak.spleen.split\endcsname{fold~1}
\expandafter\gdef\csname R@hyp.peak.vsL1.ntot\endcsname{15}
\expandafter\gdef\csname R@hyp.peak.vsL1.nwin\endcsname{12}
\expandafter\gdef\csname R@hyp.peak.vsL1S.ntot\endcsname{15}
\expandafter\gdef\csname R@hyp.peak.vsL1S.nwin\endcsname{13}
\expandafter\gdef\csname R@hyp.peakown.kits.L1.d\endcsname{\ensuremath{+2.58}}
\expandafter\gdef\csname R@hyp.peakown.kits.L1.dice\endcsname{85.44}
\expandafter\gdef\csname R@hyp.peakown.kits.Y2.d\endcsname{\ensuremath{+3.47}}
\expandafter\gdef\csname R@hyp.peakown.kits.Y2.dice\endcsname{86.33}
\expandafter\gdef\csname R@hyp.peakown.kits.Y2.fold\endcsname{1}
\expandafter\gdef\csname R@hyp.peakown.kits.base.dice\endcsname{82.86}
\expandafter\gdef\csname R@hyp.r5.H1.dist\endcsname{40}
\expandafter\gdef\csname R@hyp.r5.H1.gross.d\endcsname{\ensuremath{+12.79}}
\expandafter\gdef\csname R@hyp.r5.H1.gross.dice\endcsname{61.07}
\expandafter\gdef\csname R@hyp.r5.H1.small5.d\endcsname{\ensuremath{+8.11}}
\expandafter\gdef\csname R@hyp.r5.H1.small5.dice\endcsname{66.49}
\expandafter\gdef\csname R@hyp.r5.H1.small5.vb\endcsname{1.16}
\expandafter\gdef\csname R@hyp.r5.J1.dist\endcsname{35}
\expandafter\gdef\csname R@hyp.r5.J1.gross.d\endcsname{\ensuremath{+14.28}}
\expandafter\gdef\csname R@hyp.r5.J1.gross.dice\endcsname{62.56}
\expandafter\gdef\csname R@hyp.r5.J1.small5.d\endcsname{\ensuremath{+9.08}}
\expandafter\gdef\csname R@hyp.r5.J1.small5.dice\endcsname{67.46}
\expandafter\gdef\csname R@hyp.r5.J1.small5.vb\endcsname{0.72}
\expandafter\gdef\csname R@hyp.r5.J2.dist\endcsname{42}
\expandafter\gdef\csname R@hyp.r5.J2.gross.d\endcsname{\ensuremath{+15.17}}
\expandafter\gdef\csname R@hyp.r5.J2.gross.dice\endcsname{63.46}
\expandafter\gdef\csname R@hyp.r5.J2.small5.d\endcsname{\ensuremath{+4.55}}
\expandafter\gdef\csname R@hyp.r5.J2.small5.dice\endcsname{62.93}
\expandafter\gdef\csname R@hyp.r5.J2.small5.vb\endcsname{1.01}
\expandafter\gdef\csname R@hyp.r5.J4.dist\endcsname{46}
\expandafter\gdef\csname R@hyp.r5.J4.gross.d\endcsname{\ensuremath{+12.98}}
\expandafter\gdef\csname R@hyp.r5.J4.gross.dice\endcsname{61.26}
\expandafter\gdef\csname R@hyp.r5.J4.small5.d\endcsname{\ensuremath{+6.91}}
\expandafter\gdef\csname R@hyp.r5.J4.small5.dice\endcsname{65.29}
\expandafter\gdef\csname R@hyp.r5.J4.small5.vb\endcsname{1.17}
\expandafter\gdef\csname R@hyp.r5.L1.dist\endcsname{41}
\expandafter\gdef\csname R@hyp.r5.L1.gross.d\endcsname{\ensuremath{+12.16}}
\expandafter\gdef\csname R@hyp.r5.L1.gross.dice\endcsname{60.44}
\expandafter\gdef\csname R@hyp.r5.L1.small5.d\endcsname{\ensuremath{+6.32}}
\expandafter\gdef\csname R@hyp.r5.L1.small5.dice\endcsname{64.70}
\expandafter\gdef\csname R@hyp.r5.L1.small5.vb\endcsname{1.43}
\expandafter\gdef\csname R@hyp.r5.V7A1.dist\endcsname{44}
\expandafter\gdef\csname R@hyp.r5.V7A1.gross.d\endcsname{\ensuremath{+10.26}}
\expandafter\gdef\csname R@hyp.r5.V7A1.gross.dice\endcsname{58.54}
\expandafter\gdef\csname R@hyp.r5.V7A1.small5.d\endcsname{\ensuremath{+8.27}}
\expandafter\gdef\csname R@hyp.r5.V7A1.small5.dice\endcsname{66.65}
\expandafter\gdef\csname R@hyp.r5.V7A1.small5.vb\endcsname{1.25}
\expandafter\gdef\csname R@hyp.r5.Y2.dist\endcsname{40}
\expandafter\gdef\csname R@hyp.r5.Y2.gross.d\endcsname{\ensuremath{+15.13}}
\expandafter\gdef\csname R@hyp.r5.Y2.gross.dice\endcsname{63.41}
\expandafter\gdef\csname R@hyp.r5.Y2.small5.d\endcsname{\ensuremath{+8.20}}
\expandafter\gdef\csname R@hyp.r5.Y2.small5.dice\endcsname{66.58}
\expandafter\gdef\csname R@hyp.r5.Y2.small5.vb\endcsname{1.13}
\expandafter\gdef\csname R@hyp.r5.Y3.dist\endcsname{39}
\expandafter\gdef\csname R@hyp.r5.Y3.gross.d\endcsname{\ensuremath{+15.69}}
\expandafter\gdef\csname R@hyp.r5.Y3.gross.dice\endcsname{63.97}
\expandafter\gdef\csname R@hyp.r5.Y3.small5.d\endcsname{\ensuremath{+8.41}}
\expandafter\gdef\csname R@hyp.r5.Y3.small5.dice\endcsname{66.79}
\expandafter\gdef\csname R@hyp.r5.Y3.small5.vb\endcsname{0.82}
\expandafter\gdef\csname R@hyp.r5.base.dist\endcsname{57}
\expandafter\gdef\csname R@hyp.r5.base.gross.dice\endcsname{48.28}
\expandafter\gdef\csname R@hyp.r5.base.small5.dice\endcsname{58.38}
\expandafter\gdef\csname R@hyp.r5.base.small5.vb\endcsname{1.73}
\expandafter\gdef\csname R@hyp.rule.all7.M.d\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@hyp.rule.all7.S.d\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@hyp.rule.all7.d\endcsname{\ensuremath{+0.72}}
\expandafter\gdef\csname R@hyp.rule.all7.n\endcsname{10}
\expandafter\gdef\csname R@hyp.rule.all7.npos\endcsname{10}
\expandafter\gdef\csname R@hyp.rule.ct5.M.d\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@hyp.rule.ct5.Y2.d\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@hyp.rule.ct5.rule.d\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@hyp.rule.unseen4.M.d\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@hyp.rule.unseen4.S.d\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@hyp.rule.unseen4.d\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@hyp.rule.unseen4.n\endcsname{5}
\expandafter\gdef\csname R@hyp.rule.unseen4.npos\endcsname{5}
\expandafter\gdef\csname R@hyp.sc.dec.M\endcsname{118}
\expandafter\gdef\csname R@hyp.sc.dec.base\endcsname{338}
\expandafter\gdef\csname R@hyp.sc.dec2.M\endcsname{93}
\expandafter\gdef\csname R@hyp.sc.dec2.base\endcsname{267}
\expandafter\gdef\csname R@hyp.sc.e23.M\endcsname{149}
\expandafter\gdef\csname R@hyp.sc.e23.base\endcsname{33}
\expandafter\gdef\csname R@hyp.sc.tot.M\endcsname{374}
\expandafter\gdef\csname R@hyp.sc.tot.base\endcsname{477}
\expandafter\gdef\csname R@hyp.split.n\endcsname{45}
\expandafter\gdef\csname R@hyp.split.npos\endcsname{38}
\expandafter\gdef\csname R@hyp.split.p\endcsname{<10^{-5}}
\expandafter\gdef\csname R@hyp.trig.hepv.r1\endcsname{56.0}
\expandafter\gdef\csname R@hyp.trig.hepv.r2\endcsname{2/2}
\expandafter\gdef\csname R@hyp.trig.hepv.r3\endcsname{$4{\times}6{\times}6$}
\expandafter\gdef\csname R@hyp.trig.hepv.r4\endcsname{0}
\expandafter\gdef\csname R@hyp.trig.kipa22.art.bf\endcsname{0.60}
\expandafter\gdef\csname R@hyp.trig.kipa22.r1\endcsname{55.9}
\expandafter\gdef\csname R@hyp.trig.kipa22.r2\endcsname{1/4}
\expandafter\gdef\csname R@hyp.trig.kipa22.r3\endcsname{$5{\times}4{\times}7$}
\expandafter\gdef\csname R@hyp.trig.kipa22.r4\endcsname{0}
\expandafter\gdef\csname R@hyp.trig.panc.canc.bf\endcsname{0.45}
\expandafter\gdef\csname R@hyp.trig.panc.r1\endcsname{42.8}
\expandafter\gdef\csname R@hyp.trig.panc.r2\endcsname{1/2}
\expandafter\gdef\csname R@hyp.trig.panc.r3\endcsname{$5{\times}7{\times}7$}
\expandafter\gdef\csname R@hyp.trig.panc.r4\endcsname{0}
\expandafter\gdef\csname R@hyp.trig.r2.above.d\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@hyp.trig.r2.above.nup\endcsname{9}
\expandafter\gdef\csname R@hyp.trig.r2.below.d\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@hyp.trig.r2.nabove\endcsname{12}
\expandafter\gdef\csname R@hyp.trig.r2.nbelow\endcsname{16}
\expandafter\gdef\csname R@hyp.trig.r2.nclass\endcsname{28}
\expandafter\gdef\csname R@hyp.trig.r2.nds\endcsname{eight}
\expandafter\gdef\csname R@hyp.trig.r4.brats.dM\endcsname{-0.13}
\expandafter\gdef\csname R@hyp.trig.r4.hepv.dM\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@hyp.trig.r4.kipa22.dM\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@hyp.trig.r4.lits.dM\endcsname{0.00}
\expandafter\gdef\csname R@hyp.trig.r4.nsilent\endcsname{5}
\expandafter\gdef\csname R@hyp.trig.r4.panc.dM\endcsname{\ensuremath{-1.35}}
\expandafter\gdef\csname R@hyp.trig.r4.silent.mean\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@hyp.trig.spleen.bf\endcsname{0.22}
\expandafter\gdef\csname R@hyp.trig.spleen.r1\endcsname{42.9}
\expandafter\gdef\csname R@hyp.trig.spleen.r2\endcsname{0/1}
\expandafter\gdef\csname R@hyp.trig.spleen.r3\endcsname{$4{\times}6{\times}5$}
\expandafter\gdef\csname R@hyp.trig.spleen.r4\endcsname{0}
\expandafter\gdef\csname R@hyp.y13.amos.cv.dL1S\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@hyp.y13.amos.cv.dice\endcsname{88.56}
\expandafter\gdef\csname R@hyp.y13.amos.f4.dY14\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@hyp.y13.btcv.d\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@hyp.y13.btcv.mean\endcsname{78.43}
\expandafter\gdef\csname R@hyp.y13.btcv.s0.dY14\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@hyp.y14.kits.dY13\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@hyp.y14.lits.dY13\endcsname{\ensuremath{+1.09}}
\makeatother


==> an_extra_perclass_stock.tex <==
% AUTO-GENERATED by paper_v1/dump_module.py from scripts/an_perclass_stock.py -- do not edit by hand
\makeatletter
\expandafter\gdef\csname R@an.perclass_stock.all.delta\endcsname{\ensuremath{+1.56}}
\expandafter\gdef\csname R@an.perclass_stock.all.delta_xa\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.perclass_stock.all.name\endcsname{Mean of the three regions}
\expandafter\gdef\csname R@an.perclass_stock.all.pool\endcsname{83.38}
\expandafter\gdef\csname R@an.perclass_stock.all.se\endcsname{0.49}
\expandafter\gdef\csname R@an.perclass_stock.all.se_xa\endcsname{0.49}
\expandafter\gdef\csname R@an.perclass_stock.all.stock\endcsname{84.26}
\expandafter\gdef\csname R@an.perclass_stock.all.stock.sd\endcsname{0.63}
\expandafter\gdef\csname R@an.perclass_stock.all.vspool\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.perclass_stock.all.xa\endcsname{86.04}
\expandafter\gdef\csname R@an.perclass_stock.all.xl\endcsname{85.82}
\expandafter\gdef\csname R@an.perclass_stock.c123.delta\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.perclass_stock.c123.delta_xa\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@an.perclass_stock.c123.name\endcsname{Kidney region}
\expandafter\gdef\csname R@an.perclass_stock.c123.pool\endcsname{96.02}
\expandafter\gdef\csname R@an.perclass_stock.c123.se\endcsname{0.26}
\expandafter\gdef\csname R@an.perclass_stock.c123.se_xa\endcsname{0.26}
\expandafter\gdef\csname R@an.perclass_stock.c123.stock\endcsname{96.34}
\expandafter\gdef\csname R@an.perclass_stock.c123.stock.sd\endcsname{0.33}
\expandafter\gdef\csname R@an.perclass_stock.c123.vspool\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.perclass_stock.c123.xa\endcsname{97.17}
\expandafter\gdef\csname R@an.perclass_stock.c123.xl\endcsname{97.27}
\expandafter\gdef\csname R@an.perclass_stock.c2.delta\endcsname{\ensuremath{+1.87}}
\expandafter\gdef\csname R@an.perclass_stock.c2.delta_xa\endcsname{\ensuremath{+2.21}}
\expandafter\gdef\csname R@an.perclass_stock.c2.name\endcsname{Tumour}
\expandafter\gdef\csname R@an.perclass_stock.c2.pool\endcsname{74.27}
\expandafter\gdef\csname R@an.perclass_stock.c2.se\endcsname{0.74}
\expandafter\gdef\csname R@an.perclass_stock.c2.se_xa\endcsname{0.74}
\expandafter\gdef\csname R@an.perclass_stock.c2.stock\endcsname{75.46}
\expandafter\gdef\csname R@an.perclass_stock.c2.stock.sd\endcsname{0.95}
\expandafter\gdef\csname R@an.perclass_stock.c2.vspool\endcsname{\ensuremath{+1.19}}
\expandafter\gdef\csname R@an.perclass_stock.c2.xa\endcsname{77.67}
\expandafter\gdef\csname R@an.perclass_stock.c2.xl\endcsname{77.33}
\expandafter\gdef\csname R@an.perclass_stock.c23.delta\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@an.perclass_stock.c23.delta_xa\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.perclass_stock.c23.name\endcsname{Masses}
\expandafter\gdef\csname R@an.perclass_stock.c23.pool\endcsname{79.84}
\expandafter\gdef\csname R@an.perclass_stock.c23.se\endcsname{0.71}
\expandafter\gdef\csname R@an.perclass_stock.c23.se_xa\endcsname{0.71}
\expandafter\gdef\csname R@an.perclass_stock.c23.stock\endcsname{80.97}
\expandafter\gdef\csname R@an.perclass_stock.c23.stock.sd\endcsname{0.90}
\expandafter\gdef\csname R@an.perclass_stock.c23.vspool\endcsname{\ensuremath{+1.13}}
\expandafter\gdef\csname R@an.perclass_stock.c23.xa\endcsname{83.28}
\expandafter\gdef\csname R@an.perclass_stock.c23.xl\endcsname{82.85}
\expandafter\gdef\csname R@an.perclass_stock.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.perclass_stock.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.perclass_stock.rule\endcsname{the standard error is the Welch standard error of a difference of two means: the square root of s squared over the number of arm runs plus s squared over the number of stock runs, with s the SD of the stock runs in that region for both terms (an arm's own SD of two runs is not a run-level SD); it describes how far a mean of two runs can differ from a mean of the stock runs through run-to-run variation of the recipe alone, and states no inference}
\expandafter\gdef\csname R@an.perclass_stock.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of {\ifdefined\archL\archL\else XX-Net-L\fi} differs from the mean of nnU-Net's nine stock runs by \ensuremath{+0.93}\,pp on the kidney region (SE 0.26), \ensuremath{+1.88}\,pp on the masses (SE 0.71) and \ensuremath{+1.87}\,pp on the tumour (SE 0.74), and that of {\ifdefined\archA\archA\else XX-Net-A\fi} by \ensuremath{+0.83}\,pp on the kidney region (SE 0.26), \ensuremath{+2.31}\,pp on the masses (SE 0.71) and \ensuremath{+2.21}\,pp on the tumour (SE 0.74)}
\expandafter\gdef\csname R@an.perclass_stock.state\endcsname{9 stock runs, XX-Net-L fresh pair complete, XX-Net-A fresh pair complete}
\expandafter\gdef\csname R@an.perclass_stock.stock.seeds\endcsname{3--11}
\expandafter\gdef\csname R@an.perclass_stock.xa.tag\endcsname{V7A1}
\expandafter\gdef\csname R@an.perclass_stock.xl.tag\endcsname{V7C1}
\makeatother


==> an_extra_qual.tex <==
%% AUTO-GENERATED by paper_v2_8p/qual_keys.py -- do not edit by hand
%% Fig. 4 values from figs/qual_v9/ (the experimenter's selection records, rules sha checked). qual.on is the gate.
\makeatletter
\expandafter\gdef\csname R@qual.A.case\endcsname{00461}
\expandafter\gdef\csname R@qual.A.dice.V7A1\endcsname{6.0}
\expandafter\gdef\csname R@qual.A.dice.Y2\endcsname{21.9}
\expandafter\gdef\csname R@qual.A.dice.base\endcsname{6.0}
\expandafter\gdef\csname R@qual.A.fold\endcsname{2}
\expandafter\gdef\csname R@qual.A.fp.V7A1\endcsname{421}
\expandafter\gdef\csname R@qual.A.fp.Y2\endcsname{89}
\expandafter\gdef\csname R@qual.A.fp.base\endcsname{422}
\expandafter\gdef\csname R@qual.A.pool\endcsname{198}
\expandafter\gdef\csname R@qual.A.refcyst\endcsname{488}
\expandafter\gdef\csname R@qual.B.case\endcsname{00227}
\expandafter\gdef\csname R@qual.B.dice.V7A1\endcsname{5.3}
\expandafter\gdef\csname R@qual.B.dice.Y2\endcsname{72.0}
\expandafter\gdef\csname R@qual.B.dice.base\endcsname{5.1}
\expandafter\gdef\csname R@qual.B.extr.V7A1\endcsname{358}
\expandafter\gdef\csname R@qual.B.extr.Y2\endcsname{1}
\expandafter\gdef\csname R@qual.B.extr.base\endcsname{365}
\expandafter\gdef\csname R@qual.B.fold\endcsname{4}
\expandafter\gdef\csname R@qual.B.pool\endcsname{8}
\expandafter\gdef\csname R@qual.C.case\endcsname{0281}
\expandafter\gdef\csname R@qual.C.dice.D2\endcsname{14.7}
\expandafter\gdef\csname R@qual.C.dice.V7A1\endcsname{59.3}
\expandafter\gdef\csname R@qual.C.dice.base\endcsname{48.8}
\expandafter\gdef\csname R@qual.C.eligible\endcsname{111}
\expandafter\gdef\csname R@qual.C.fold\endcsname{1}
\expandafter\gdef\csname R@qual.C.organ\endcsname{oesophagus}
\expandafter\gdef\csname R@qual.C.pool\endcsname{479}
\expandafter\gdef\csname R@qual.on\endcsname{1}
\makeatother


==> an_extra_rscost.tex <==
% AUTO-GENERATED by paper_v1/rs_costs.py -- do not edit by hand
\makeatletter
\expandafter\gdef\csname R@s1.rs.01.gmac\endcsname{1.65}
\expandafter\gdef\csname R@s1.rs.01.params\endcsname{3.04}
\expandafter\gdef\csname R@s1.rs.01.step\endcsname{3.05}
\expandafter\gdef\csname R@s1.rs.02.gmac\endcsname{1.63}
\expandafter\gdef\csname R@s1.rs.02.params\endcsname{2.07}
\expandafter\gdef\csname R@s1.rs.02.step\endcsname{2.27}
\expandafter\gdef\csname R@s1.rs.05.gmac\endcsname{1.19}
\expandafter\gdef\csname R@s1.rs.05.params\endcsname{2.97}
\expandafter\gdef\csname R@s1.rs.05.step\endcsname{3.51}
\expandafter\gdef\csname R@s1.rs.07.gmac\endcsname{1.22}
\expandafter\gdef\csname R@s1.rs.07.params\endcsname{1.21}
\expandafter\gdef\csname R@s1.rs.07.step\endcsname{1.75}
\expandafter\gdef\csname R@s1.rs.08.gmac\endcsname{1.28}
\expandafter\gdef\csname R@s1.rs.08.params\endcsname{1.33}
\expandafter\gdef\csname R@s1.rs.08.step\endcsname{2.65}
\expandafter\gdef\csname R@s1.rs.09.gmac\endcsname{0.81}
\expandafter\gdef\csname R@s1.rs.09.params\endcsname{1.78}
\expandafter\gdef\csname R@s1.rs.09.step\endcsname{3.02}
\expandafter\gdef\csname R@s1.rs.11.gmac\endcsname{1.77}
\expandafter\gdef\csname R@s1.rs.11.params\endcsname{1.45}
\expandafter\gdef\csname R@s1.rs.11.step\endcsname{5.24}
\expandafter\gdef\csname R@s1.rs.12.gmac\endcsname{1.28}
\expandafter\gdef\csname R@s1.rs.12.params\endcsname{1.67}
\expandafter\gdef\csname R@s1.rs.12.step\endcsname{5.27}
\expandafter\gdef\csname R@s1.rs.13.gmac\endcsname{1.05}
\expandafter\gdef\csname R@s1.rs.13.params\endcsname{1.74}
\expandafter\gdef\csname R@s1.rs.13.step\endcsname{3.83}
\expandafter\gdef\csname R@s1.rs.15.gmac\endcsname{1.70}
\expandafter\gdef\csname R@s1.rs.15.params\endcsname{1.62}
\expandafter\gdef\csname R@s1.rs.15.step\endcsname{2.34}
\expandafter\gdef\csname R@s1.rs.19.gmac\endcsname{1.97}
\expandafter\gdef\csname R@s1.rs.19.params\endcsname{0.81}
\expandafter\gdef\csname R@s1.rs.19.step\endcsname{3.46}
\expandafter\gdef\csname R@s1.rs.20.gmac\endcsname{1.06}
\expandafter\gdef\csname R@s1.rs.20.params\endcsname{3.01}
\expandafter\gdef\csname R@s1.rs.20.step\endcsname{2.93}
\expandafter\gdef\csname R@s1.rs.22.gmac\endcsname{1.43}
\expandafter\gdef\csname R@s1.rs.22.params\endcsname{1.40}
\expandafter\gdef\csname R@s1.rs.22.step\endcsname{4.06}
\expandafter\gdef\csname R@s1.rs.23.gmac\endcsname{1.40}
\expandafter\gdef\csname R@s1.rs.23.params\endcsname{2.64}
\expandafter\gdef\csname R@s1.rs.23.step\endcsname{3.18}
\expandafter\gdef\csname R@s1.rs.24.gmac\endcsname{1.59}
\expandafter\gdef\csname R@s1.rs.24.params\endcsname{2.17}
\expandafter\gdef\csname R@s1.rs.24.step\endcsname{3.12}
\expandafter\gdef\csname R@s1.sp.1.gmac\endcsname{1.63}
\expandafter\gdef\csname R@s1.sp.1.params\endcsname{3.46}
\expandafter\gdef\csname R@s1.sp.1.step\endcsname{1.69}
\expandafter\gdef\csname R@s1.sp.2.gmac\endcsname{1.74}
\expandafter\gdef\csname R@s1.sp.2.params\endcsname{3.46}
\expandafter\gdef\csname R@s1.sp.2.step\endcsname{1.91}
\makeatother


==> an_extra_s6.tex <==
%% AUTO-GENERATED by paper_v2_8p/s6_keys.py -- do not edit by hand
%% R4's two fold-0 seeds (score_d1d2_s6.json, PREREG_D1D2 s6.3), gates recomputed from the full-precision values.
\makeatletter
\expandafter\gdef\csname R@an.s6.fresh.V7A1\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.s6.fresh.Y2\endcsname{\ensuremath{+2.69}}
\expandafter\gdef\csname R@an.s6.g1.dM\endcsname{\ensuremath{+0.057}}
\expandafter\gdef\csname R@an.s6.g1.prec\endcsname{0.751}
\expandafter\gdef\csname R@an.s6.g1.thr\endcsname{0.726}
\expandafter\gdef\csname R@an.s6.g2.dM\endcsname{\ensuremath{-0.005}}
\expandafter\gdef\csname R@an.s6.g2.recall\endcsname{0.842}
\expandafter\gdef\csname R@an.s6.g2.thr\endcsname{0.832}
\expandafter\gdef\csname R@an.s6.on\endcsname{1}
\expandafter\gdef\csname R@an.s6.pass\endcsname{1}
\expandafter\gdef\csname R@an.s6.s1.dice\endcsname{86.76}
\expandafter\gdef\csname R@an.s6.s1.prec\endcsname{0.770}
\expandafter\gdef\csname R@an.s6.s1.recall\endcsname{0.841}
\expandafter\gdef\csname R@an.s6.s2.dice\endcsname{87.13}
\expandafter\gdef\csname R@an.s6.s2.prec\endcsname{0.732}
\expandafter\gdef\csname R@an.s6.s2.recall\endcsname{0.842}
\makeatother


==> an_extra_sc15.tex <==
%% AUTO-GENERATED by paper_v2_8p/stagecost_v15_keys.py -- do not edit by hand
\makeatletter
\expandafter\gdef\csname R@sc15.V7A1.D0.gmac\endcsname{1.5}
\expandafter\gdef\csname R@sc15.V7A1.D0.params\endcsname{3.59}
\expandafter\gdef\csname R@sc15.V7A1.D1.gmac\endcsname{7.6}
\expandafter\gdef\csname R@sc15.V7A1.D1.params\endcsname{2.43}
\expandafter\gdef\csname R@sc15.V7A1.D2.gmac\endcsname{15.6}
\expandafter\gdef\csname R@sc15.V7A1.D2.params\endcsname{0.71}
\expandafter\gdef\csname R@sc15.V7A1.D3.gmac\endcsname{31.1}
\expandafter\gdef\csname R@sc15.V7A1.D3.params\endcsname{0.18}
\expandafter\gdef\csname R@sc15.V7A1.D4.gmac\endcsname{62.3}
\expandafter\gdef\csname R@sc15.V7A1.D4.params\endcsname{0.04}
\expandafter\gdef\csname R@sc15.V7A1.E0.gmac\endcsname{59.8}
\expandafter\gdef\csname R@sc15.V7A1.E0.params\endcsname{0.03}
\expandafter\gdef\csname R@sc15.V7A1.E1.gmac\endcsname{43.5}
\expandafter\gdef\csname R@sc15.V7A1.E1.params\endcsname{0.17}
\expandafter\gdef\csname R@sc15.V7A1.E2.gmac\endcsname{109.0}
\expandafter\gdef\csname R@sc15.V7A1.E2.params\endcsname{3.33}
\expandafter\gdef\csname R@sc15.V7A1.E3.gmac\endcsname{40.0}
\expandafter\gdef\csname R@sc15.V7A1.E3.params\endcsname{9.77}
\expandafter\gdef\csname R@sc15.V7A1.E4.gmac\endcsname{2.6}
\expandafter\gdef\csname R@sc15.V7A1.E4.params\endcsname{5.13}
\expandafter\gdef\csname R@sc15.V7A1.E5.gmac\endcsname{0.4}
\expandafter\gdef\csname R@sc15.V7A1.E5.params\endcsname{5.68}
\expandafter\gdef\csname R@sc15.V7A1.heads.gmac\endcsname{0.3}
\expandafter\gdef\csname R@sc15.V7A1.heads.params\endcsname{0.00}
\expandafter\gdef\csname R@sc15.V7A1.total.gmac\endcsname{373.5}
\expandafter\gdef\csname R@sc15.V7A1.total.params\endcsname{31.04}
\expandafter\gdef\csname R@sc15.base.D0.gmac\endcsname{4.3}
\expandafter\gdef\csname R@sc15.base.D0.params\endcsname{9.12}
\expandafter\gdef\csname R@sc15.base.D1.gmac\endcsname{22.1}
\expandafter\gdef\csname R@sc15.base.D1.params\endcsname{5.97}
\expandafter\gdef\csname R@sc15.base.D2.gmac\endcsname{44.6}
\expandafter\gdef\csname R@sc15.base.D2.params\endcsname{1.59}
\expandafter\gdef\csname R@sc15.base.D3.gmac\endcsname{89.1}
\expandafter\gdef\csname R@sc15.base.D3.params\endcsname{0.40}
\expandafter\gdef\csname R@sc15.base.D4.gmac\endcsname{178.2}
\expandafter\gdef\csname R@sc15.base.D4.params\endcsname{0.10}
\expandafter\gdef\csname R@sc15.base.E0.gmac\endcsname{59.8}
\expandafter\gdef\csname R@sc15.base.E0.params\endcsname{0.03}
\expandafter\gdef\csname R@sc15.base.E1.gmac\endcsname{43.5}
\expandafter\gdef\csname R@sc15.base.E1.params\endcsname{0.17}
\expandafter\gdef\csname R@sc15.base.E2.gmac\endcsname{21.7}
\expandafter\gdef\csname R@sc15.base.E2.params\endcsname{0.66}
\expandafter\gdef\csname R@sc15.base.E3.gmac\endcsname{10.9}
\expandafter\gdef\csname R@sc15.base.E3.params\endcsname{2.66}
\expandafter\gdef\csname R@sc15.base.E4.gmac\endcsname{2.5}
\expandafter\gdef\csname R@sc15.base.E4.params\endcsname{4.98}
\expandafter\gdef\csname R@sc15.base.E5.gmac\endcsname{0.4}
\expandafter\gdef\csname R@sc15.base.E5.params\endcsname{5.53}
\expandafter\gdef\csname R@sc15.base.heads.gmac\endcsname{0.3}
\expandafter\gdef\csname R@sc15.base.heads.params\endcsname{0.00}
\expandafter\gdef\csname R@sc15.base.total.gmac\endcsname{477.4}
\expandafter\gdef\csname R@sc15.base.total.params\endcsname{31.20}
\makeatother


==> an_extra_stockref.tex <==
% AUTO-GENERATED by paper_v1/dump_module.py from scripts/an_stockref.py -- do not edit by hand
\makeatletter
\expandafter\gdef\csname R@an.stockref.amos.L1.delta_pool\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.stockref.amos.L1.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L1.delta_stock\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.stockref.amos.L1.incl0.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L1.incl0.delta_stock\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.stockref.amos.L1.incl0.mean\endcsname{88.23}
\expandafter\gdef\csname R@an.stockref.amos.L1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L1.incl0.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L1.incl0.se_stock\endcsname{0.10}
\expandafter\gdef\csname R@an.stockref.amos.L1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of ResEnc-M on AMOS22 fold 0 is 88.23 Dice: \ensuremath{+0.51}\,pp from the stock mean (SE 0.10, 3 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.L1.mean\endcsname{88.17}
\expandafter\gdef\csname R@an.stockref.amos.L1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.amos.L1.n_reb\endcsname{0}
\expandafter\gdef\csname R@an.stockref.amos.L1.n_stock\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L1.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L1.se_stock\endcsname{0.11}
\expandafter\gdef\csname R@an.stockref.amos.L1.sentence\endcsname{on AMOS22 fold 0 the mean of fresh seeds 1 and 2 of ResEnc-M is 88.17 Dice: \ensuremath{+0.45}\,pp from the stock mean (SE 0.11, 2 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.L1b.delta_pool\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.stockref.amos.L1b.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L1b.delta_stock\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.stockref.amos.L1b.incl0.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L1b.incl0.delta_stock\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.stockref.amos.L1b.incl0.mean\endcsname{87.95}
\expandafter\gdef\csname R@an.stockref.amos.L1b.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L1b.incl0.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L1b.incl0.se_stock\endcsname{0.10}
\expandafter\gdef\csname R@an.stockref.amos.L1b.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of ResEnc-matched on AMOS22 fold 0 is 87.95 Dice: \ensuremath{+0.23}\,pp from the stock mean (SE 0.10, 3 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.L1b.mean\endcsname{88.00}
\expandafter\gdef\csname R@an.stockref.amos.L1b.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.amos.L1b.n_reb\endcsname{0}
\expandafter\gdef\csname R@an.stockref.amos.L1b.n_stock\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L1b.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L1b.se_stock\endcsname{0.11}
\expandafter\gdef\csname R@an.stockref.amos.L1b.sentence\endcsname{on AMOS22 fold 0 the mean of fresh seeds 1 and 2 of ResEnc-matched is 88.00 Dice: \ensuremath{+0.29}\,pp from the stock mean (SE 0.11, 2 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.L2.delta_pool\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.stockref.amos.L2.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L2.delta_stock\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.stockref.amos.L2.incl0.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L2.incl0.delta_stock\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.stockref.amos.L2.incl0.mean\endcsname{87.95}
\expandafter\gdef\csname R@an.stockref.amos.L2.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L2.incl0.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L2.incl0.se_stock\endcsname{0.10}
\expandafter\gdef\csname R@an.stockref.amos.L2.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of ConvNeXt-k3 on AMOS22 fold 0 is 87.95 Dice: \ensuremath{+0.24}\,pp from the stock mean (SE 0.10, 3 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.L2.mean\endcsname{87.90}
\expandafter\gdef\csname R@an.stockref.amos.L2.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.amos.L2.n_reb\endcsname{0}
\expandafter\gdef\csname R@an.stockref.amos.L2.n_stock\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L2.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L2.se_stock\endcsname{0.11}
\expandafter\gdef\csname R@an.stockref.amos.L2.sentence\endcsname{on AMOS22 fold 0 the mean of fresh seeds 1 and 2 of ConvNeXt-k3 is 87.90 Dice: \ensuremath{+0.18}\,pp from the stock mean (SE 0.11, 2 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.L3.delta_pool\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.stockref.amos.L3.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L3.delta_stock\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.stockref.amos.L3.incl0.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L3.incl0.delta_stock\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.stockref.amos.L3.incl0.mean\endcsname{87.92}
\expandafter\gdef\csname R@an.stockref.amos.L3.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L3.incl0.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L3.incl0.se_stock\endcsname{0.10}
\expandafter\gdef\csname R@an.stockref.amos.L3.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of HyReX on AMOS22 fold 0 is 87.92 Dice: \ensuremath{+0.20}\,pp from the stock mean (SE 0.10, 3 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.L3.mean\endcsname{87.83}
\expandafter\gdef\csname R@an.stockref.amos.L3.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.amos.L3.n_reb\endcsname{0}
\expandafter\gdef\csname R@an.stockref.amos.L3.n_stock\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L3.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L3.se_stock\endcsname{0.11}
\expandafter\gdef\csname R@an.stockref.amos.L3.sentence\endcsname{on AMOS22 fold 0 the mean of fresh seeds 1 and 2 of HyReX is 87.83 Dice: \ensuremath{+0.12}\,pp from the stock mean (SE 0.11, 2 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.L4.delta_pool\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.stockref.amos.L4.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L4.delta_stock\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.stockref.amos.L4.incl0.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L4.incl0.delta_stock\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.stockref.amos.L4.incl0.mean\endcsname{88.15}
\expandafter\gdef\csname R@an.stockref.amos.L4.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L4.incl0.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L4.incl0.se_stock\endcsname{0.10}
\expandafter\gdef\csname R@an.stockref.amos.L4.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of ResEnc+context on AMOS22 fold 0 is 88.15 Dice: \ensuremath{+0.44}\,pp from the stock mean (SE 0.10, 3 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.L4.mean\endcsname{88.16}
\expandafter\gdef\csname R@an.stockref.amos.L4.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.amos.L4.n_reb\endcsname{0}
\expandafter\gdef\csname R@an.stockref.amos.L4.n_stock\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L4.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L4.se_stock\endcsname{0.11}
\expandafter\gdef\csname R@an.stockref.amos.L4.sentence\endcsname{on AMOS22 fold 0 the mean of fresh seeds 1 and 2 of ResEnc+context is 88.16 Dice: \ensuremath{+0.44}\,pp from the stock mean (SE 0.11, 2 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.arms\endcsname{L1, L1b, L2, L3, L4}
\expandafter\gdef\csname R@an.stockref.amos.pool.mean\endcsname{87.70}
\expandafter\gdef\csname R@an.stockref.amos.pool.n\endcsname{6}
\expandafter\gdef\csname R@an.stockref.amos.reb.n\endcsname{0}
\expandafter\gdef\csname R@an.stockref.amos.stock.mean\endcsname{87.71}
\expandafter\gdef\csname R@an.stockref.amos.stock.n\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.stock.sd\endcsname{0.12}
\expandafter\gdef\csname R@an.stockref.amos.stock.seeds\endcsname{3--5}
\expandafter\gdef\csname R@an.stockref.amos.stock.sentence\endcsname{the stock reference of AMOS22 fold 0 is the mean of the 3 finished plain-default runs (seeds 3--5) of the harness, 87.71 Dice (SD 0.12), \ensuremath{+0.01}\,pp from the frozen pool of 6 runs (87.70); the pool and its sub-pools are not part of it}
\expandafter\gdef\csname R@an.stockref.amos.stock.vspool\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.stockref.kits.C1.delta_pool\endcsname{\ensuremath{+2.40}}
\expandafter\gdef\csname R@an.stockref.kits.C1.delta_reb\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.stockref.kits.C1.delta_stock\endcsname{\ensuremath{+1.52}}
\expandafter\gdef\csname R@an.stockref.kits.C1.incl0.delta_reb\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.stockref.kits.C1.incl0.delta_stock\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.stockref.kits.C1.incl0.mean\endcsname{86.15}
\expandafter\gdef\csname R@an.stockref.kits.C1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.C1.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.C1.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.C1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of HyReX+dec. capacity on KiTS23 fold 0 is 86.15 Dice: \ensuremath{+1.89}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+1.48}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.C1.mean\endcsname{85.78}
\expandafter\gdef\csname R@an.stockref.kits.C1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.C1.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.C1.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.C1.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.C1.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.C1.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of HyReX+dec. capacity is 85.78 Dice: \ensuremath{+1.52}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+1.11}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.D1.delta_pool\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.stockref.kits.D1.delta_reb\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.stockref.kits.D1.delta_stock\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.stockref.kits.D1.incl0.delta_reb\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.stockref.kits.D1.incl0.delta_stock\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.stockref.kits.D1.incl0.mean\endcsname{84.90}
\expandafter\gdef\csname R@an.stockref.kits.D1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.D1.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.D1.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.D1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of HyReX point-fuse on KiTS23 fold 0 is 84.90 Dice: \ensuremath{+0.64}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.23}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.D1.mean\endcsname{84.85}
\expandafter\gdef\csname R@an.stockref.kits.D1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.D1.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.D1.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.D1.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.D1.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.D1.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of HyReX point-fuse is 84.85 Dice: \ensuremath{+0.60}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.18}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.D2.delta_pool\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.stockref.kits.D2.delta_reb\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.stockref.kits.D2.delta_stock\endcsname{\ensuremath{+1.01}}
\expandafter\gdef\csname R@an.stockref.kits.D2.incl0.delta_reb\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.stockref.kits.D2.incl0.delta_stock\endcsname{\ensuremath{+1.17}}
\expandafter\gdef\csname R@an.stockref.kits.D2.incl0.mean\endcsname{85.42}
\expandafter\gdef\csname R@an.stockref.kits.D2.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.D2.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.D2.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.D2.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of LeanDec on KiTS23 fold 0 is 85.42 Dice: \ensuremath{+1.17}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.75}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.D2.mean\endcsname{85.27}
\expandafter\gdef\csname R@an.stockref.kits.D2.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.D2.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.D2.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.D2.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.D2.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.D2.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of LeanDec is 85.27 Dice: \ensuremath{+1.01}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.60}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L1.delta_pool\endcsname{\ensuremath{+3.48}}
\expandafter\gdef\csname R@an.stockref.kits.L1.delta_reb\endcsname{\ensuremath{+2.18}}
\expandafter\gdef\csname R@an.stockref.kits.L1.delta_stock\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@an.stockref.kits.L1.incl0.delta_reb\endcsname{\ensuremath{+1.80}}
\expandafter\gdef\csname R@an.stockref.kits.L1.incl0.delta_stock\endcsname{\ensuremath{+2.21}}
\expandafter\gdef\csname R@an.stockref.kits.L1.incl0.mean\endcsname{86.47}
\expandafter\gdef\csname R@an.stockref.kits.L1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.L1.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L1.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.L1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of ResEnc-M on KiTS23 fold 0 is 86.47 Dice: \ensuremath{+2.21}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+1.80}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L1.mean\endcsname{86.85}
\expandafter\gdef\csname R@an.stockref.kits.L1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.L1.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.L1.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.L1.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.L1.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L1.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of ResEnc-M is 86.85 Dice: \ensuremath{+2.60}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+2.18}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L1b.delta_pool\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.stockref.kits.L1b.delta_reb\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.stockref.kits.L1b.delta_stock\endcsname{\ensuremath{+1.43}}
\expandafter\gdef\csname R@an.stockref.kits.L1b.incl0.delta_reb\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@an.stockref.kits.L1b.incl0.delta_stock\endcsname{\ensuremath{+1.24}}
\expandafter\gdef\csname R@an.stockref.kits.L1b.incl0.mean\endcsname{85.50}
\expandafter\gdef\csname R@an.stockref.kits.L1b.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.L1b.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L1b.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.L1b.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of ResEnc-matched on KiTS23 fold 0 is 85.50 Dice: \ensuremath{+1.24}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.83}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L1b.mean\endcsname{85.69}
\expandafter\gdef\csname R@an.stockref.kits.L1b.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.L1b.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.L1b.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.L1b.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.L1b.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L1b.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of ResEnc-matched is 85.69 Dice: \ensuremath{+1.43}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+1.02}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L2.delta_pool\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.stockref.kits.L2.delta_reb\endcsname{\ensuremath{-1.18}}
\expandafter\gdef\csname R@an.stockref.kits.L2.delta_stock\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.stockref.kits.L2.incl0.delta_reb\endcsname{\ensuremath{-1.00}}
\expandafter\gdef\csname R@an.stockref.kits.L2.incl0.delta_stock\endcsname{\ensuremath{-0.58}}
\expandafter\gdef\csname R@an.stockref.kits.L2.incl0.mean\endcsname{83.67}
\expandafter\gdef\csname R@an.stockref.kits.L2.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.L2.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L2.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.L2.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of ConvNeXt-k3 on KiTS23 fold 0 is 83.67 Dice: \ensuremath{-0.58}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{-1.00}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L2.mean\endcsname{83.49}
\expandafter\gdef\csname R@an.stockref.kits.L2.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.L2.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.L2.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.L2.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.L2.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L2.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of ConvNeXt-k3 is 83.49 Dice: \ensuremath{-0.77}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{-1.18}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L3.delta_pool\endcsname{\ensuremath{+2.09}}
\expandafter\gdef\csname R@an.stockref.kits.L3.delta_reb\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.stockref.kits.L3.delta_stock\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.stockref.kits.L3.incl0.delta_reb\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.stockref.kits.L3.incl0.delta_stock\endcsname{\ensuremath{+1.46}}
\expandafter\gdef\csname R@an.stockref.kits.L3.incl0.mean\endcsname{85.72}
\expandafter\gdef\csname R@an.stockref.kits.L3.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.L3.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L3.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.L3.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of HyReX on KiTS23 fold 0 is 85.72 Dice: \ensuremath{+1.46}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+1.05}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L3.mean\endcsname{85.47}
\expandafter\gdef\csname R@an.stockref.kits.L3.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.L3.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.L3.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.L3.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.L3.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L3.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of HyReX is 85.47 Dice: \ensuremath{+1.21}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.80}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L4.delta_pool\endcsname{\ensuremath{+2.25}}
\expandafter\gdef\csname R@an.stockref.kits.L4.delta_reb\endcsname{\ensuremath{+0.95}}
\expandafter\gdef\csname R@an.stockref.kits.L4.delta_stock\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.stockref.kits.L4.incl0.delta_reb\endcsname{\ensuremath{+0.94}}
\expandafter\gdef\csname R@an.stockref.kits.L4.incl0.delta_stock\endcsname{\ensuremath{+1.35}}
\expandafter\gdef\csname R@an.stockref.kits.L4.incl0.mean\endcsname{85.61}
\expandafter\gdef\csname R@an.stockref.kits.L4.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.L4.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L4.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.L4.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of ResEnc+context on KiTS23 fold 0 is 85.61 Dice: \ensuremath{+1.35}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.94}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L4.mean\endcsname{85.62}
\expandafter\gdef\csname R@an.stockref.kits.L4.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.L4.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.L4.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.L4.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.L4.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L4.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of ResEnc+context is 85.62 Dice: \ensuremath{+1.37}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.95}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L6.delta_pool\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.stockref.kits.L6.delta_reb\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.stockref.kits.L6.delta_stock\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.stockref.kits.L6.incl0.delta_reb\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.stockref.kits.L6.incl0.delta_stock\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.stockref.kits.L6.incl0.mean\endcsname{85.28}
\expandafter\gdef\csname R@an.stockref.kits.L6.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.L6.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L6.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.L6.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of HyReX+context on KiTS23 fold 0 is 85.28 Dice: \ensuremath{+1.02}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.61}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L6.mean\endcsname{84.97}
\expandafter\gdef\csname R@an.stockref.kits.L6.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.L6.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.L6.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.L6.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.L6.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L6.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of HyReX+context is 84.97 Dice: \ensuremath{+0.71}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.30}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.P3c.delta_pool\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.stockref.kits.P3c.delta_reb\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.stockref.kits.P3c.delta_stock\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.stockref.kits.P3c.incl0.delta_reb\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.stockref.kits.P3c.incl0.delta_stock\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.stockref.kits.P3c.incl0.mean\endcsname{84.62}
\expandafter\gdef\csname R@an.stockref.kits.P3c.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.P3c.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.P3c.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.P3c.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of fn.-identical control on KiTS23 fold 0 is 84.62 Dice: \ensuremath{+0.36}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{-0.05}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.P3c.mean\endcsname{84.55}
\expandafter\gdef\csname R@an.stockref.kits.P3c.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.P3c.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.P3c.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.P3c.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.P3c.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.P3c.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of fn.-identical control is 84.55 Dice: \ensuremath{+0.30}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{-0.12}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.S2.delta_pool\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.stockref.kits.S2.delta_reb\endcsname{\ensuremath{-0.72}}
\expandafter\gdef\csname R@an.stockref.kits.S2.delta_stock\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.stockref.kits.S2.incl0.delta_reb\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.stockref.kits.S2.incl0.delta_stock\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.stockref.kits.S2.incl0.mean\endcsname{84.21}
\expandafter\gdef\csname R@an.stockref.kits.S2.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.S2.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.S2.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.S2.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of HyReX, finer ConvNeXt on KiTS23 fold 0 is 84.21 Dice: \ensuremath{-0.05}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{-0.47}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.S2.mean\endcsname{83.95}
\expandafter\gdef\csname R@an.stockref.kits.S2.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.S2.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.S2.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.S2.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.S2.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.S2.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of HyReX, finer ConvNeXt is 83.95 Dice: \ensuremath{-0.31}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{-0.72}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.delta_pool\endcsname{\ensuremath{+2.17}}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.delta_reb\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.delta_stock\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.incl0.delta_reb\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.incl0.delta_stock\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.incl0.mean\endcsname{85.47}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of HyReX-LeanDec on KiTS23 fold 0 is 85.47 Dice: \ensuremath{+1.21}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.80}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.mean\endcsname{85.54}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of HyReX-LeanDec is 85.54 Dice: \ensuremath{+1.29}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.87}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.delta_pool\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.delta_reb\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.delta_stock\endcsname{\ensuremath{+1.41}}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.incl0.delta_reb\endcsname{\ensuremath{+0.95}}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.incl0.delta_stock\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.incl0.mean\endcsname{85.62}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of LeanAdd on KiTS23 fold 0 is 85.62 Dice: \ensuremath{+1.37}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.95}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.mean\endcsname{85.66}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of LeanAdd is 85.66 Dice: \ensuremath{+1.41}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.99}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.delta_pool\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.delta_reb\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.delta_stock\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.incl0.delta_reb\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.incl0.delta_stock\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.incl0.mean\endcsname{84.77}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of LeanAdd-NeXt on KiTS23 fold 0 is 84.77 Dice: \ensuremath{+0.51}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.09}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.mean\endcsname{84.83}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of LeanAdd-NeXt is 84.83 Dice: \ensuremath{+0.57}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.16}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.delta_pool\endcsname{\ensuremath{+1.70}}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.delta_reb\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.delta_stock\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.incl0.delta_reb\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.incl0.delta_stock\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.incl0.mean\endcsname{85.26}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of HyReX-k9 on KiTS23 fold 0 is 85.26 Dice: \ensuremath{+1.00}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.59}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.mean\endcsname{85.08}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of HyReX-k9 is 85.08 Dice: \ensuremath{+0.82}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.41}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.delta_pool\endcsname{\ensuremath{+2.66}}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.delta_reb\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.delta_stock\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.incl0.delta_reb\endcsname{\ensuremath{+1.33}}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.incl0.delta_stock\endcsname{\ensuremath{+1.74}}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.incl0.mean\endcsname{86.00}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of {\ifdefined\archA\archA\else XX-Net-A\fi} on KiTS23 fold 0 is 86.00 Dice: \ensuremath{+1.74}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+1.33}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.mean\endcsname{86.04}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of {\ifdefined\archA\archA\else XX-Net-A\fi} is 86.04 Dice: \ensuremath{+1.78}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+1.37}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.delta_pool\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.delta_reb\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.delta_stock\endcsname{\ensuremath{+1.41}}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.incl0.delta_reb\endcsname{\ensuremath{+1.20}}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.incl0.delta_stock\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.incl0.mean\endcsname{85.87}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of LeanDeepMid+FD on KiTS23 fold 0 is 85.87 Dice: \ensuremath{+1.61}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+1.20}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.mean\endcsname{85.67}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of LeanDeepMid+FD is 85.67 Dice: \ensuremath{+1.41}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+1.00}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.delta_pool\endcsname{\ensuremath{+2.38}}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.delta_reb\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.delta_stock\endcsname{\ensuremath{+1.50}}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.incl0.delta_reb\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.incl0.delta_stock\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.incl0.mean\endcsname{85.54}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of LeanSep on KiTS23 fold 0 is 85.54 Dice: \ensuremath{+1.28}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.87}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.mean\endcsname{85.76}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of LeanSep is 85.76 Dice: \ensuremath{+1.50}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+1.09}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.delta_pool\endcsname{\ensuremath{+1.84}}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.delta_reb\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.delta_stock\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.incl0.delta_reb\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.incl0.delta_stock\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.incl0.mean\endcsname{85.55}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of LeanDil on KiTS23 fold 0 is 85.55 Dice: \ensuremath{+1.29}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.87}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.mean\endcsname{85.22}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of LeanDil is 85.22 Dice: \ensuremath{+0.96}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.55}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.delta_pool\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.delta_reb\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.delta_stock\endcsname{\ensuremath{+1.56}}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.incl0.delta_reb\endcsname{\ensuremath{+1.24}}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.incl0.delta_stock\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.incl0.mean\endcsname{85.91}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of {\ifdefined\archL\archL\else XX-Net-L\fi} on KiTS23 fold 0 is 85.91 Dice: \ensuremath{+1.65}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+1.24}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.mean\endcsname{85.82}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of {\ifdefined\archL\archL\else XX-Net-L\fi} is 85.82 Dice: \ensuremath{+1.56}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+1.15}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.delta_pool\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.delta_reb\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.delta_stock\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.incl0.delta_reb\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.incl0.delta_stock\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.incl0.mean\endcsname{84.80}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of CoarseStack on KiTS23 fold 0 is 84.80 Dice: \ensuremath{+0.54}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.13}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.mean\endcsname{84.63}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of CoarseStack is 84.63 Dice: \ensuremath{+0.37}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{-0.04}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.delta_pool\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.delta_reb\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.delta_stock\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.incl0.delta_reb\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.incl0.delta_stock\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.incl0.mean\endcsname{85.08}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of StackDec on KiTS23 fold 0 is 85.08 Dice: \ensuremath{+0.82}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.41}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.mean\endcsname{85.26}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of StackDec is 85.26 Dice: \ensuremath{+1.00}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.58}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.delta_pool\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.delta_reb\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.delta_stock\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.incl0.delta_reb\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.incl0.delta_stock\endcsname{\ensuremath{+1.01}}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.incl0.mean\endcsname{85.26}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of LeanTrunk on KiTS23 fold 0 is 85.26 Dice: \ensuremath{+1.01}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.59}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.mean\endcsname{84.75}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of LeanTrunk is 84.75 Dice: \ensuremath{+0.50}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.08}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.delta_pool\endcsname{\ensuremath{+1.73}}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.delta_reb\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.delta_stock\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.incl0.delta_reb\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.incl0.delta_stock\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.incl0.mean\endcsname{85.08}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of Stem1 on KiTS23 fold 0 is 85.08 Dice: \ensuremath{+0.82}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.41}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.mean\endcsname{85.11}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of Stem1 is 85.11 Dice: \ensuremath{+0.85}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.44}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.W1c.delta_pool\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.stockref.kits.W1c.delta_reb\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.stockref.kits.W1c.delta_stock\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.stockref.kits.W1c.incl0.delta_reb\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.stockref.kits.W1c.incl0.delta_stock\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.stockref.kits.W1c.incl0.mean\endcsname{84.97}
\expandafter\gdef\csname R@an.stockref.kits.W1c.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.W1c.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.W1c.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.W1c.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of branch control on KiTS23 fold 0 is 84.97 Dice: \ensuremath{+0.71}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.30}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.W1c.mean\endcsname{84.44}
\expandafter\gdef\csname R@an.stockref.kits.W1c.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.W1c.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.W1c.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.W1c.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.W1c.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.W1c.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of branch control is 84.44 Dice: \ensuremath{+0.19}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{-0.23}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.arms\endcsname{C1, D1, D2, L1, L1b, L2, L3, L4, L6, P3c, S2, V5A5, V5B1, V5B2, V6A1r, V7A1, V7A2, V7B1, V7B2, V7C1, V8A1, V8A2, V8B1, V8B2, W1c}
\expandafter\gdef\csname R@an.stockref.kits.pool.mean\endcsname{83.38}
\expandafter\gdef\csname R@an.stockref.kits.pool.n\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.reb.mean\endcsname{84.67}
\expandafter\gdef\csname R@an.stockref.kits.reb.n\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.reb.sd\endcsname{0.72}
\expandafter\gdef\csname R@an.stockref.kits.reb.seeds\endcsname{3--7}
\expandafter\gdef\csname R@an.stockref.kits.reb.vspool\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.stockref.kits.reb.vsstock\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.stockref.kits.stock.mean\endcsname{84.26}
\expandafter\gdef\csname R@an.stockref.kits.stock.n\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.stock.sd\endcsname{0.63}
\expandafter\gdef\csname R@an.stockref.kits.stock.seeds\endcsname{3--11}
\expandafter\gdef\csname R@an.stockref.kits.stock.sentence\endcsname{the stock reference of KiTS23 fold 0 is the mean of the 9 finished plain-default runs (seeds 3--11) of the harness, 84.26 Dice (SD 0.63), \ensuremath{+0.88}\,pp from the frozen pool of 3 runs (83.38); the pool and its sub-pools are not part of it}
\expandafter\gdef\csname R@an.stockref.kits.stock.vspool\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.stockref.rule\endcsname{the standard error is the Welch form sqrt(s_arm^2/n_arm + s_ref^2/n_ref) of a difference of two means, with the arm's SD taken as the SD of the stock runs (an arm's own SD of two or three runs, one of them the selected discovery run, is not a run-level SD) and the reference's SD its own; it describes how far two means of that many runs can differ through run-to-run variation of the recipe alone, and states no inference}
\expandafter\gdef\csname R@an.stockref.state\endcsname{KiTS23: 25 of 46 arms with a fresh pair, 9 stock runs, 5 rebuild runs, AMOS22: 5 of 46 arms with a fresh pair, 3 stock runs, 0 rebuild runs}
\makeatother


==> an_extra_v6review.tex <==
%% AUTO-GENERATED by paper_v2_8p/v6review_keys.py -- do not edit by hand
%% From paper_v2/analysis_insight/review_v6_keys.json (checked there) and sat_keys.json.
\makeatletter
\expandafter\gdef\csname R@an.v6.amos.wo30.Y2\endcsname{7.2}
\expandafter\gdef\csname R@an.v6.amos.wo30.max\endcsname{7.3}
\expandafter\gdef\csname R@an.v6.amos.wo30.min\endcsname{6.9}
\expandafter\gdef\csname R@an.v6.amos.wo50.Y2\endcsname{12.5}
\expandafter\gdef\csname R@an.v6.amos.wo50.max\endcsname{13.2}
\expandafter\gdef\csname R@an.v6.amos.wo50.min\endcsname{12.3}
\expandafter\gdef\csname R@an.v6.amos.wo70.Y2\endcsname{25.6}
\expandafter\gdef\csname R@an.v6.amos.wo70.max\endcsname{27.6}
\expandafter\gdef\csname R@an.v6.amos.wo70.min\endcsname{25.5}
\expandafter\gdef\csname R@an.v6.kits.larger.allcuts\endcsname{1}
\expandafter\gdef\csname R@an.v6.kits.wo30.Y2\endcsname{29.9}
\expandafter\gdef\csname R@an.v6.kits.wo30.max\endcsname{33.6}
\expandafter\gdef\csname R@an.v6.kits.wo30.min\endcsname{26.8}
\expandafter\gdef\csname R@an.v6.kits.wo50.Y2\endcsname{42.6}
\expandafter\gdef\csname R@an.v6.kits.wo50.max\endcsname{47.1}
\expandafter\gdef\csname R@an.v6.kits.wo50.min\endcsname{39.2}
\expandafter\gdef\csname R@an.v6.kits.wo70.Y2\endcsname{51.9}
\expandafter\gdef\csname R@an.v6.kits.wo70.max\endcsname{61.0}
\expandafter\gdef\csname R@an.v6.kits.wo70.min\endcsname{51.9}
\expandafter\gdef\csname R@r18.sign.n\endcsname{6}
\expandafter\gdef\csname R@r18.sign.n.word\endcsname{six}
\expandafter\gdef\csname R@r18.sign.npos\endcsname{6}
\expandafter\gdef\csname R@r18.sign.p\endcsname{0.016}
\makeatother


==> an_extra_wave.tex <==
% AUTO-GENERATED by paper_v1_lit/supp_wave_keys.py from results/an_macros.tex and runs/trials/*/result.json -- do not edit by hand
\makeatletter
\expandafter\gdef\csname R@wv.1.bestfast\endcsname{--}
\expandafter\gdef\csname R@wv.1.built\endcsname{0}
\expandafter\gdef\csname R@wv.1.clear\endcsname{4}
\expandafter\gdef\csname R@wv.1.fast\endcsname{0}
\expandafter\gdef\csname R@wv.1.fresh\endcsname{4}
\expandafter\gdef\csname R@wv.1.front\endcsname{--}
\expandafter\gdef\csname R@wv.1.steperr\endcsname{--}
\expandafter\gdef\csname R@wv.1.trained\endcsname{4}
\expandafter\gdef\csname R@wv.2.bestfast\endcsname{--}
\expandafter\gdef\csname R@wv.2.built\endcsname{0}
\expandafter\gdef\csname R@wv.2.clear\endcsname{0}
\expandafter\gdef\csname R@wv.2.fast\endcsname{0}
\expandafter\gdef\csname R@wv.2.fresh\endcsname{0}
\expandafter\gdef\csname R@wv.2.front\endcsname{--}
\expandafter\gdef\csname R@wv.2.steperr\endcsname{--}
\expandafter\gdef\csname R@wv.2.trained\endcsname{3}
\expandafter\gdef\csname R@wv.3.bestfast\endcsname{--}
\expandafter\gdef\csname R@wv.3.built\endcsname{3}
\expandafter\gdef\csname R@wv.3.clear\endcsname{0}
\expandafter\gdef\csname R@wv.3.fast\endcsname{0}
\expandafter\gdef\csname R@wv.3.fresh\endcsname{0}
\expandafter\gdef\csname R@wv.3.front\endcsname{--}
\expandafter\gdef\csname R@wv.3.steperr\endcsname{--}
\expandafter\gdef\csname R@wv.3.trained\endcsname{0}
\expandafter\gdef\csname R@wv.4.bestfast\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@wv.4.built\endcsname{0}
\expandafter\gdef\csname R@wv.4.clear\endcsname{4}
\expandafter\gdef\csname R@wv.4.fast\endcsname{1}
\expandafter\gdef\csname R@wv.4.fresh\endcsname{4}
\expandafter\gdef\csname R@wv.4.front\endcsname{--}
\expandafter\gdef\csname R@wv.4.steperr\endcsname{--}
\expandafter\gdef\csname R@wv.4.trained\endcsname{5}
\expandafter\gdef\csname R@wv.5.bestfast\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@wv.5.built\endcsname{0}
\expandafter\gdef\csname R@wv.5.clear\endcsname{3}
\expandafter\gdef\csname R@wv.5.fast\endcsname{2}
\expandafter\gdef\csname R@wv.5.fresh\endcsname{3}
\expandafter\gdef\csname R@wv.5.front\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@wv.5.steperr\endcsname{12.6}
\expandafter\gdef\csname R@wv.5.trained\endcsname{3}
\expandafter\gdef\csname R@wv.6.bestfast\endcsname{--}
\expandafter\gdef\csname R@wv.6.built\endcsname{0}
\expandafter\gdef\csname R@wv.6.clear\endcsname{1}
\expandafter\gdef\csname R@wv.6.fast\endcsname{0}
\expandafter\gdef\csname R@wv.6.fresh\endcsname{1}
\expandafter\gdef\csname R@wv.6.front\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@wv.6.steperr\endcsname{--}
\expandafter\gdef\csname R@wv.6.trained\endcsname{1}
\expandafter\gdef\csname R@wv.7.bestfast\endcsname{\ensuremath{+1.95}}
\expandafter\gdef\csname R@wv.7.built\endcsname{0}
\expandafter\gdef\csname R@wv.7.clear\endcsname{5}
\expandafter\gdef\csname R@wv.7.fast\endcsname{4}
\expandafter\gdef\csname R@wv.7.fresh\endcsname{5}
\expandafter\gdef\csname R@wv.7.front\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@wv.7.steperr\endcsname{2.0}
\expandafter\gdef\csname R@wv.7.trained\endcsname{5}
\expandafter\gdef\csname R@wv.8.bestfast\endcsname{\ensuremath{+2.03}}
\expandafter\gdef\csname R@wv.8.built\endcsname{0}
\expandafter\gdef\csname R@wv.8.clear\endcsname{4}
\expandafter\gdef\csname R@wv.8.fast\endcsname{4}
\expandafter\gdef\csname R@wv.8.fresh\endcsname{4}
\expandafter\gdef\csname R@wv.8.front\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@wv.8.steperr\endcsname{2.8}
\expandafter\gdef\csname R@wv.8.trained\endcsname{4}
\expandafter\gdef\csname R@wv.clear_eq_fresh\endcsname{1}
\expandafter\gdef\csname R@wv.stock.amos.n\endcsname{3}
\expandafter\gdef\csname R@wv.stock.kits.n\endcsname{9}
\expandafter\gdef\csname R@wv.tot.built\endcsname{3}
\expandafter\gdef\csname R@wv.tot.clear\endcsname{21}
\expandafter\gdef\csname R@wv.tot.fast\endcsname{11}
\expandafter\gdef\csname R@wv.tot.fresh\endcsname{21}
\expandafter\gdef\csname R@wv.tot.trained\endcsname{25}
\makeatother


==> results/an_macros.tex <==
%% AUTO-GENERATED by scripts/run_analyses.py -- do not edit by hand.
\makeatletter
\expandafter\gdef\csname R@an.ablation.C1.acdc_fit\endcsname{fits}
\expandafter\gdef\csname R@an.ablation.C1.amos.band\endcsname{KILL the decoder side of the budget: C1 - HyReX below the Tier-1 gap (+0.265 pp); no decoder-capacity follow-up}
\expandafter\gdef\csname R@an.ablation.C1.amos.d\endcsname{+0.008}
\expandafter\gdef\csname R@an.ablation.C1.amos.dice\endcsname{88.091}
\expandafter\gdef\csname R@an.ablation.C1.amos.dsec\endcsname{+0.174}
\expandafter\gdef\csname R@an.ablation.C1.amos.edge_gap\endcsname{+0.008}
\expandafter\gdef\csname R@an.ablation.C1.amos.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.C1.amos.fresh_dunion\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.C1.amos.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.C1.amos.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.C1.amos.fresh_rel_floor\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.C1.amos.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.C1.amos.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.C1.amos.fresh_se\endcsname{0.122}
\expandafter\gdef\csname R@an.ablation.C1.amos.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.C1.amos.fresh_vs_parent_fresh\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.C1.amos.inspan\endcsname{above}
\expandafter\gdef\csname R@an.ablation.C1.amos.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.C1.amos.parent_all\endcsname{87.916}
\expandafter\gdef\csname R@an.ablation.C1.amos.parent_fresh\endcsname{87.833}
\expandafter\gdef\csname R@an.ablation.C1.amos.parent_max\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.C1.amos.parent_min\endcsname{87.686}
\expandafter\gdef\csname R@an.ablation.C1.amos.parent_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.C1.amos.parent_s0\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.C1.amos.parent_span\endcsname{0.397}
\expandafter\gdef\csname R@an.ablation.C1.amos.rel_floor\endcsname{within}
\expandafter\gdef\csname R@an.ablation.C1.amos.se\endcsname{0.173}
\expandafter\gdef\csname R@an.ablation.C1.amos.se_parent_all\endcsname{0.141}
\expandafter\gdef\csname R@an.ablation.C1.amos.se_parent_fresh\endcsname{0.150}
\expandafter\gdef\csname R@an.ablation.C1.amos.se_parent_s0\endcsname{0.173}
\expandafter\gdef\csname R@an.ablation.C1.amos.sesec\endcsname{0.141}
\expandafter\gdef\csname R@an.ablation.C1.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.C1.amos.verdict\endcsname{KILL (decoder budget)}
\expandafter\gdef\csname R@an.ablation.C1.amos.vs_contemp\endcsname{+0.379}
\expandafter\gdef\csname R@an.ablation.C1.amos.vs_parent_all\endcsname{+0.174}
\expandafter\gdef\csname R@an.ablation.C1.amos.vs_parent_fresh\endcsname{+0.257}
\expandafter\gdef\csname R@an.ablation.C1.amos.vs_parent_s0\endcsname{+0.008}
\expandafter\gdef\csname R@an.ablation.C1.amos.vs_pool\endcsname{+0.390}
\expandafter\gdef\csname R@an.ablation.C1.amos.vs_unc\endcsname{+0.361}
\expandafter\gdef\csname R@an.ablation.C1.amos.vs_union\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.C1.control\endcsname{HyReX seed 0}
\expandafter\gdef\csname R@an.ablation.C1.dparams\endcsname{+22.75}
\expandafter\gdef\csname R@an.ablation.C1.dparams_pct\endcsname{+76.9}
\expandafter\gdef\csname R@an.ablation.C1.kits.band\endcsname{run for the co-primary rule, not read as a guard (O4)}
\expandafter\gdef\csname R@an.ablation.C1.kits.d\endcsname{+0.665}
\expandafter\gdef\csname R@an.ablation.C1.kits.dice\endcsname{86.885}
\expandafter\gdef\csname R@an.ablation.C1.kits.dsec\endcsname{+1.164}
\expandafter\gdef\csname R@an.ablation.C1.kits.edge_gap\endcsname{+0.665}
\expandafter\gdef\csname R@an.ablation.C1.kits.fresh_d\endcsname{+2.401}
\expandafter\gdef\csname R@an.ablation.C1.kits.fresh_dunion\endcsname{+2.157}
\expandafter\gdef\csname R@an.ablation.C1.kits.fresh_mean\endcsname{85.779}
\expandafter\gdef\csname R@an.ablation.C1.kits.fresh_n\endcsname{2}
\expandafter\gdef\csname R@an.ablation.C1.kits.fresh_rel_floor\endcsname{within}
\expandafter\gdef\csname R@an.ablation.C1.kits.fresh_s1\endcsname{85.506}
\expandafter\gdef\csname R@an.ablation.C1.kits.fresh_s2\endcsname{86.052}
\expandafter\gdef\csname R@an.ablation.C1.kits.fresh_se\endcsname{0.795}
\expandafter\gdef\csname R@an.ablation.C1.kits.fresh_state\endcsname{finished}
\expandafter\gdef\csname R@an.ablation.C1.kits.fresh_vs_parent_fresh\endcsname{+0.307}
\expandafter\gdef\csname R@an.ablation.C1.kits.inspan\endcsname{above}
\expandafter\gdef\csname R@an.ablation.C1.kits.move\endcsname{-1.106}
\expandafter\gdef\csname R@an.ablation.C1.kits.parent_all\endcsname{85.721}
\expandafter\gdef\csname R@an.ablation.C1.kits.parent_fresh\endcsname{85.472}
\expandafter\gdef\csname R@an.ablation.C1.kits.parent_max\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.C1.kits.parent_min\endcsname{85.176}
\expandafter\gdef\csname R@an.ablation.C1.kits.parent_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.C1.kits.parent_s0\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.C1.kits.parent_span\endcsname{1.044}
\expandafter\gdef\csname R@an.ablation.C1.kits.rel_floor\endcsname{above}
\expandafter\gdef\csname R@an.ablation.C1.kits.se\endcsname{1.124}
\expandafter\gdef\csname R@an.ablation.C1.kits.se_parent_all\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.C1.kits.se_parent_fresh\endcsname{0.974}
\expandafter\gdef\csname R@an.ablation.C1.kits.se_parent_s0\endcsname{1.124}
\expandafter\gdef\csname R@an.ablation.C1.kits.sesec\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.C1.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.C1.kits.v4.center\endcsname{-1.006}
\expandafter\gdef\csname R@an.ablation.C1.kits.v4.dist\endcsname{-0.100}
\expandafter\gdef\csname R@an.ablation.C1.kits.v4.hi\endcsname{+0.267}
\expandafter\gdef\csname R@an.ablation.C1.kits.v4.lo\endcsname{-5.436}
\expandafter\gdef\csname R@an.ablation.C1.kits.v4.word\endcsname{inside}
\expandafter\gdef\csname R@an.ablation.C1.kits.verdict\endcsname{co-primary run only}
\expandafter\gdef\csname R@an.ablation.C1.kits.vs_contemp\endcsname{+3.020}
\expandafter\gdef\csname R@an.ablation.C1.kits.vs_parent_all\endcsname{+1.164}
\expandafter\gdef\csname R@an.ablation.C1.kits.vs_parent_fresh\endcsname{+1.414}
\expandafter\gdef\csname R@an.ablation.C1.kits.vs_parent_s0\endcsname{+0.665}
\expandafter\gdef\csname R@an.ablation.C1.kits.vs_pool\endcsname{+3.507}
\expandafter\gdef\csname R@an.ablation.C1.kits.vs_unc\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.C1.kits.vs_union\endcsname{+3.264}
\expandafter\gdef\csname R@an.ablation.C1.param_match\endcsname{unmatched}
\expandafter\gdef\csname R@an.ablation.C1.param_ratio\endcsname{1.769}
\expandafter\gdef\csname R@an.ablation.C1.params_m\endcsname{52.34}
\expandafter\gdef\csname R@an.ablation.C1.role\endcsname{child}
\expandafter\gdef\csname R@an.ablation.C1.step_ratio\endcsname{1.108}
\expandafter\gdef\csname R@an.ablation.C1.step_ratio_kits\endcsname{1.128}
\expandafter\gdef\csname R@an.ablation.D1.acdc_fit\endcsname{fits}
\expandafter\gdef\csname R@an.ablation.D1.amos.band\endcsname{within $\pm$0.50 of HyReX while the coarse fusion convolution is removed: not resolvable at one seed}
\expandafter\gdef\csname R@an.ablation.D1.amos.d\endcsname{-0.104}
\expandafter\gdef\csname R@an.ablation.D1.amos.dice\endcsname{87.979}
\expandafter\gdef\csname R@an.ablation.D1.amos.dsec\endcsname{+0.063}
\expandafter\gdef\csname R@an.ablation.D1.amos.edge_gap\endcsname{0.000}
\expandafter\gdef\csname R@an.ablation.D1.amos.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.D1.amos.fresh_dunion\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.D1.amos.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.D1.amos.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.D1.amos.fresh_rel_floor\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.D1.amos.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.D1.amos.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.D1.amos.fresh_se\endcsname{0.122}
\expandafter\gdef\csname R@an.ablation.D1.amos.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.D1.amos.fresh_vs_parent_fresh\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.D1.amos.inspan\endcsname{inside}
\expandafter\gdef\csname R@an.ablation.D1.amos.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.D1.amos.parent_all\endcsname{87.916}
\expandafter\gdef\csname R@an.ablation.D1.amos.parent_fresh\endcsname{87.833}
\expandafter\gdef\csname R@an.ablation.D1.amos.parent_max\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.D1.amos.parent_min\endcsname{87.686}
\expandafter\gdef\csname R@an.ablation.D1.amos.parent_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.D1.amos.parent_s0\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.D1.amos.parent_span\endcsname{0.397}
\expandafter\gdef\csname R@an.ablation.D1.amos.rel_floor\endcsname{within}
\expandafter\gdef\csname R@an.ablation.D1.amos.se\endcsname{0.173}
\expandafter\gdef\csname R@an.ablation.D1.amos.se_parent_all\endcsname{0.141}
\expandafter\gdef\csname R@an.ablation.D1.amos.se_parent_fresh\endcsname{0.150}
\expandafter\gdef\csname R@an.ablation.D1.amos.se_parent_s0\endcsname{0.173}
\expandafter\gdef\csname R@an.ablation.D1.amos.sesec\endcsname{0.141}
\expandafter\gdef\csname R@an.ablation.D1.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.D1.amos.verdict\endcsname{not resolved at one seed}
\expandafter\gdef\csname R@an.ablation.D1.amos.vs_contemp\endcsname{+0.267}
\expandafter\gdef\csname R@an.ablation.D1.amos.vs_parent_all\endcsname{+0.063}
\expandafter\gdef\csname R@an.ablation.D1.amos.vs_parent_fresh\endcsname{+0.146}
\expandafter\gdef\csname R@an.ablation.D1.amos.vs_parent_s0\endcsname{-0.104}
\expandafter\gdef\csname R@an.ablation.D1.amos.vs_pool\endcsname{+0.278}
\expandafter\gdef\csname R@an.ablation.D1.amos.vs_unc\endcsname{+0.249}
\expandafter\gdef\csname R@an.ablation.D1.amos.vs_union\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.D1.control\endcsname{HyReX seed 0}
\expandafter\gdef\csname R@an.ablation.D1.dparams\endcsname{-8.73}
\expandafter\gdef\csname R@an.ablation.D1.dparams_pct\endcsname{-29.5}
\expandafter\gdef\csname R@an.ablation.D1.kits.band\endcsname{not read as a loss above $-$2.25}
\expandafter\gdef\csname R@an.ablation.D1.kits.d\endcsname{-1.235}
\expandafter\gdef\csname R@an.ablation.D1.kits.dice\endcsname{84.985}
\expandafter\gdef\csname R@an.ablation.D1.kits.dsec\endcsname{-0.736}
\expandafter\gdef\csname R@an.ablation.D1.kits.edge_gap\endcsname{-0.191}
\expandafter\gdef\csname R@an.ablation.D1.kits.fresh_d\endcsname{+1.477}
\expandafter\gdef\csname R@an.ablation.D1.kits.fresh_dunion\endcsname{+1.233}
\expandafter\gdef\csname R@an.ablation.D1.kits.fresh_mean\endcsname{84.855}
\expandafter\gdef\csname R@an.ablation.D1.kits.fresh_n\endcsname{2}
\expandafter\gdef\csname R@an.ablation.D1.kits.fresh_rel_floor\endcsname{below}
\expandafter\gdef\csname R@an.ablation.D1.kits.fresh_s1\endcsname{85.137}
\expandafter\gdef\csname R@an.ablation.D1.kits.fresh_s2\endcsname{84.572}
\expandafter\gdef\csname R@an.ablation.D1.kits.fresh_se\endcsname{0.795}
\expandafter\gdef\csname R@an.ablation.D1.kits.fresh_state\endcsname{finished}
\expandafter\gdef\csname R@an.ablation.D1.kits.fresh_vs_parent_fresh\endcsname{-0.617}
\expandafter\gdef\csname R@an.ablation.D1.kits.inspan\endcsname{below}
\expandafter\gdef\csname R@an.ablation.D1.kits.move\endcsname{-0.131}
\expandafter\gdef\csname R@an.ablation.D1.kits.parent_all\endcsname{85.721}
\expandafter\gdef\csname R@an.ablation.D1.kits.parent_fresh\endcsname{85.472}
\expandafter\gdef\csname R@an.ablation.D1.kits.parent_max\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.D1.kits.parent_min\endcsname{85.176}
\expandafter\gdef\csname R@an.ablation.D1.kits.parent_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.D1.kits.parent_s0\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.D1.kits.parent_span\endcsname{1.044}
\expandafter\gdef\csname R@an.ablation.D1.kits.rel_floor\endcsname{below}
\expandafter\gdef\csname R@an.ablation.D1.kits.se\endcsname{1.124}
\expandafter\gdef\csname R@an.ablation.D1.kits.se_parent_all\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.D1.kits.se_parent_fresh\endcsname{0.974}
\expandafter\gdef\csname R@an.ablation.D1.kits.se_parent_s0\endcsname{1.124}
\expandafter\gdef\csname R@an.ablation.D1.kits.sesec\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.D1.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.D1.kits.verdict\endcsname{not read as a loss}
\expandafter\gdef\csname R@an.ablation.D1.kits.vs_contemp\endcsname{+1.120}
\expandafter\gdef\csname R@an.ablation.D1.kits.vs_parent_all\endcsname{-0.736}
\expandafter\gdef\csname R@an.ablation.D1.kits.vs_parent_fresh\endcsname{-0.486}
\expandafter\gdef\csname R@an.ablation.D1.kits.vs_parent_s0\endcsname{-1.235}
\expandafter\gdef\csname R@an.ablation.D1.kits.vs_pool\endcsname{+1.607}
\expandafter\gdef\csname R@an.ablation.D1.kits.vs_unc\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.D1.kits.vs_union\endcsname{+1.363}
\expandafter\gdef\csname R@an.ablation.D1.param_match\endcsname{unmatched}
\expandafter\gdef\csname R@an.ablation.D1.param_ratio\endcsname{0.705}
\expandafter\gdef\csname R@an.ablation.D1.params_m\endcsname{20.86}
\expandafter\gdef\csname R@an.ablation.D1.role\endcsname{child}
\expandafter\gdef\csname R@an.ablation.D1.step_ratio\endcsname{0.995}
\expandafter\gdef\csname R@an.ablation.D1.step_ratio_kits\endcsname{1.001}
\expandafter\gdef\csname R@an.ablation.D2.acdc_fit\endcsname{fits}
\expandafter\gdef\csname R@an.ablation.D2.amos.band\endcsname{in the registered undefined band ($-$0.50, $-$0.35): reported, not killed, not non-inferior}
\expandafter\gdef\csname R@an.ablation.D2.amos.d\endcsname{-0.362}
\expandafter\gdef\csname R@an.ablation.D2.amos.d_unc\endcsname{-0.391}
\expandafter\gdef\csname R@an.ablation.D2.amos.dice\endcsname{87.339}
\expandafter\gdef\csname R@an.ablation.D2.amos.dne\endcsname{-0.220}
\expandafter\gdef\csname R@an.ablation.D2.amos.edge_gap\endcsname{-0.347}
\expandafter\gdef\csname R@an.ablation.D2.amos.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.D2.amos.fresh_dunion\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.D2.amos.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.D2.amos.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.D2.amos.fresh_rel_floor\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.D2.amos.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.D2.amos.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.D2.amos.fresh_se\endcsname{0.122}
\expandafter\gdef\csname R@an.ablation.D2.amos.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.D2.amos.fresh_vs_parent_fresh\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.D2.amos.inspan\endcsname{below}
\expandafter\gdef\csname R@an.ablation.D2.amos.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.D2.amos.parent_all\endcsname{87.916}
\expandafter\gdef\csname R@an.ablation.D2.amos.parent_fresh\endcsname{87.833}
\expandafter\gdef\csname R@an.ablation.D2.amos.parent_max\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.D2.amos.parent_min\endcsname{87.686}
\expandafter\gdef\csname R@an.ablation.D2.amos.parent_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.D2.amos.parent_s0\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.D2.amos.parent_span\endcsname{0.397}
\expandafter\gdef\csname R@an.ablation.D2.amos.rel_floor\endcsname{below}
\expandafter\gdef\csname R@an.ablation.D2.amos.se\endcsname{0.132}
\expandafter\gdef\csname R@an.ablation.D2.amos.se_parent_all\endcsname{0.141}
\expandafter\gdef\csname R@an.ablation.D2.amos.se_parent_fresh\endcsname{0.150}
\expandafter\gdef\csname R@an.ablation.D2.amos.se_parent_s0\endcsname{0.173}
\expandafter\gdef\csname R@an.ablation.D2.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.D2.amos.verdict\endcsname{registered undefined band}
\expandafter\gdef\csname R@an.ablation.D2.amos.vs_contemp\endcsname{-0.373}
\expandafter\gdef\csname R@an.ablation.D2.amos.vs_parent_all\endcsname{-0.578}
\expandafter\gdef\csname R@an.ablation.D2.amos.vs_parent_fresh\endcsname{-0.495}
\expandafter\gdef\csname R@an.ablation.D2.amos.vs_parent_s0\endcsname{-0.744}
\expandafter\gdef\csname R@an.ablation.D2.amos.vs_pool\endcsname{-0.362}
\expandafter\gdef\csname R@an.ablation.D2.amos.vs_unc\endcsname{-0.391}
\expandafter\gdef\csname R@an.ablation.D2.amos.vs_union\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.D2.control\endcsname{the frozen default pool}
\expandafter\gdef\csname R@an.ablation.D2.dparams\endcsname{-5.10}
\expandafter\gdef\csname R@an.ablation.D2.dparams_pct\endcsname{-16.4}
\expandafter\gdef\csname R@an.ablation.D2.kits.band\endcsname{within $-$0.80 of the default}
\expandafter\gdef\csname R@an.ablation.D2.kits.d\endcsname{+2.355}
\expandafter\gdef\csname R@an.ablation.D2.kits.d_unc\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.D2.kits.dice\endcsname{85.734}
\expandafter\gdef\csname R@an.ablation.D2.kits.dne\endcsname{+2.355}
\expandafter\gdef\csname R@an.ablation.D2.kits.edge_gap\endcsname{0.000}
\expandafter\gdef\csname R@an.ablation.D2.kits.fresh_d\endcsname{+1.892}
\expandafter\gdef\csname R@an.ablation.D2.kits.fresh_dunion\endcsname{+1.648}
\expandafter\gdef\csname R@an.ablation.D2.kits.fresh_mean\endcsname{85.270}
\expandafter\gdef\csname R@an.ablation.D2.kits.fresh_n\endcsname{2}
\expandafter\gdef\csname R@an.ablation.D2.kits.fresh_rel_floor\endcsname{within}
\expandafter\gdef\csname R@an.ablation.D2.kits.fresh_s1\endcsname{85.357}
\expandafter\gdef\csname R@an.ablation.D2.kits.fresh_s2\endcsname{85.182}
\expandafter\gdef\csname R@an.ablation.D2.kits.fresh_se\endcsname{0.795}
\expandafter\gdef\csname R@an.ablation.D2.kits.fresh_state\endcsname{finished}
\expandafter\gdef\csname R@an.ablation.D2.kits.fresh_vs_parent_fresh\endcsname{-0.202}
\expandafter\gdef\csname R@an.ablation.D2.kits.inspan\endcsname{inside}
\expandafter\gdef\csname R@an.ablation.D2.kits.move\endcsname{-0.464}
\expandafter\gdef\csname R@an.ablation.D2.kits.parent_all\endcsname{85.721}
\expandafter\gdef\csname R@an.ablation.D2.kits.parent_fresh\endcsname{85.472}
\expandafter\gdef\csname R@an.ablation.D2.kits.parent_max\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.D2.kits.parent_min\endcsname{85.176}
\expandafter\gdef\csname R@an.ablation.D2.kits.parent_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.D2.kits.parent_s0\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.D2.kits.parent_span\endcsname{1.044}
\expandafter\gdef\csname R@an.ablation.D2.kits.rel_floor\endcsname{within}
\expandafter\gdef\csname R@an.ablation.D2.kits.se\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.D2.kits.se_parent_all\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.D2.kits.se_parent_fresh\endcsname{0.974}
\expandafter\gdef\csname R@an.ablation.D2.kits.se_parent_s0\endcsname{1.124}
\expandafter\gdef\csname R@an.ablation.D2.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.D2.kits.verdict\endcsname{within $-$0.80 of the default}
\expandafter\gdef\csname R@an.ablation.D2.kits.vs_contemp\endcsname{+1.868}
\expandafter\gdef\csname R@an.ablation.D2.kits.vs_parent_all\endcsname{+0.012}
\expandafter\gdef\csname R@an.ablation.D2.kits.vs_parent_fresh\endcsname{+0.262}
\expandafter\gdef\csname R@an.ablation.D2.kits.vs_parent_s0\endcsname{-0.486}
\expandafter\gdef\csname R@an.ablation.D2.kits.vs_pool\endcsname{+2.355}
\expandafter\gdef\csname R@an.ablation.D2.kits.vs_unc\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.D2.kits.vs_union\endcsname{+2.112}
\expandafter\gdef\csname R@an.ablation.D2.param_match\endcsname{unmatched}
\expandafter\gdef\csname R@an.ablation.D2.param_ratio\endcsname{0.836}
\expandafter\gdef\csname R@an.ablation.D2.params_m\endcsname{26.03}
\expandafter\gdef\csname R@an.ablation.D2.role\endcsname{decoder-depth control}
\expandafter\gdef\csname R@an.ablation.D2.step_ratio\endcsname{0.812}
\expandafter\gdef\csname R@an.ablation.D2.step_ratio_kits\endcsname{0.808}
\expandafter\gdef\csname R@an.ablation.I1.acdc_fit\endcsname{fits}
\expandafter\gdef\csname R@an.ablation.I1.amos.band\endcsname{aggregate NOT RESOLVABLE AT ONE SEED ($<$ 0.50 pp)}
\expandafter\gdef\csname R@an.ablation.I1.amos.d\endcsname{-0.087}
\expandafter\gdef\csname R@an.ablation.I1.amos.dice\endcsname{87.995}
\expandafter\gdef\csname R@an.ablation.I1.amos.dsec\endcsname{+0.079}
\expandafter\gdef\csname R@an.ablation.I1.amos.edge_gap\endcsname{0.000}
\expandafter\gdef\csname R@an.ablation.I1.amos.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.I1.amos.fresh_dunion\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.I1.amos.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.I1.amos.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.I1.amos.fresh_rel_floor\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.I1.amos.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.I1.amos.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.I1.amos.fresh_se\endcsname{0.122}
\expandafter\gdef\csname R@an.ablation.I1.amos.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.I1.amos.fresh_vs_parent_fresh\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.I1.amos.inspan\endcsname{inside}
\expandafter\gdef\csname R@an.ablation.I1.amos.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.I1.amos.parent_all\endcsname{87.916}
\expandafter\gdef\csname R@an.ablation.I1.amos.parent_fresh\endcsname{87.833}
\expandafter\gdef\csname R@an.ablation.I1.amos.parent_max\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.I1.amos.parent_min\endcsname{87.686}
\expandafter\gdef\csname R@an.ablation.I1.amos.parent_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.I1.amos.parent_s0\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.I1.amos.parent_span\endcsname{0.397}
\expandafter\gdef\csname R@an.ablation.I1.amos.rel_floor\endcsname{within}
\expandafter\gdef\csname R@an.ablation.I1.amos.se\endcsname{0.173}
\expandafter\gdef\csname R@an.ablation.I1.amos.se_parent_all\endcsname{0.141}
\expandafter\gdef\csname R@an.ablation.I1.amos.se_parent_fresh\endcsname{0.150}
\expandafter\gdef\csname R@an.ablation.I1.amos.se_parent_s0\endcsname{0.173}
\expandafter\gdef\csname R@an.ablation.I1.amos.sesec\endcsname{0.141}
\expandafter\gdef\csname R@an.ablation.I1.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.I1.amos.verdict\endcsname{not resolved at one seed}
\expandafter\gdef\csname R@an.ablation.I1.amos.vs_contemp\endcsname{+0.283}
\expandafter\gdef\csname R@an.ablation.I1.amos.vs_parent_all\endcsname{+0.079}
\expandafter\gdef\csname R@an.ablation.I1.amos.vs_parent_fresh\endcsname{+0.162}
\expandafter\gdef\csname R@an.ablation.I1.amos.vs_parent_s0\endcsname{-0.087}
\expandafter\gdef\csname R@an.ablation.I1.amos.vs_pool\endcsname{+0.294}
\expandafter\gdef\csname R@an.ablation.I1.amos.vs_unc\endcsname{+0.266}
\expandafter\gdef\csname R@an.ablation.I1.amos.vs_union\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.I1.control\endcsname{HyReX seed 0}
\expandafter\gdef\csname R@an.ablation.I1.dparams\endcsname{0.00}
\expandafter\gdef\csname R@an.ablation.I1.dparams_pct\endcsname{0.0}
\expandafter\gdef\csname R@an.ablation.I1.imp4.d\endcsname{+0.103}
\expandafter\gdef\csname R@an.ablation.I1.imp4.se\endcsname{0.0901}
\expandafter\gdef\csname R@an.ablation.I1.kits.band\endcsname{at or beyond the 0.50 pp one-seed floor from HyReX's selected seed, inside the range of HyReX's own seeds}
\expandafter\gdef\csname R@an.ablation.I1.kits.d\endcsname{-0.949}
\expandafter\gdef\csname R@an.ablation.I1.kits.dice\endcsname{85.271}
\expandafter\gdef\csname R@an.ablation.I1.kits.dsec\endcsname{-0.450}
\expandafter\gdef\csname R@an.ablation.I1.kits.edge_gap\endcsname{0.000}
\expandafter\gdef\csname R@an.ablation.I1.kits.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.I1.kits.fresh_dunion\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.I1.kits.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.I1.kits.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.I1.kits.fresh_rel_floor\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.I1.kits.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.I1.kits.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.I1.kits.fresh_se\endcsname{0.795}
\expandafter\gdef\csname R@an.ablation.I1.kits.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.I1.kits.fresh_vs_parent_fresh\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.I1.kits.inspan\endcsname{inside}
\expandafter\gdef\csname R@an.ablation.I1.kits.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.I1.kits.parent_all\endcsname{85.721}
\expandafter\gdef\csname R@an.ablation.I1.kits.parent_fresh\endcsname{85.472}
\expandafter\gdef\csname R@an.ablation.I1.kits.parent_max\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.I1.kits.parent_min\endcsname{85.176}
\expandafter\gdef\csname R@an.ablation.I1.kits.parent_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.I1.kits.parent_s0\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.I1.kits.parent_span\endcsname{1.044}
\expandafter\gdef\csname R@an.ablation.I1.kits.rel_floor\endcsname{below}
\expandafter\gdef\csname R@an.ablation.I1.kits.se\endcsname{1.124}
\expandafter\gdef\csname R@an.ablation.I1.kits.se_parent_all\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.I1.kits.se_parent_fresh\endcsname{0.974}
\expandafter\gdef\csname R@an.ablation.I1.kits.se_parent_s0\endcsname{1.124}
\expandafter\gdef\csname R@an.ablation.I1.kits.sesec\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.I1.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.I1.kits.verdict\endcsname{beyond the floor, inside HyReX's seed range}
\expandafter\gdef\csname R@an.ablation.I1.kits.vs_contemp\endcsname{+1.406}
\expandafter\gdef\csname R@an.ablation.I1.kits.vs_parent_all\endcsname{-0.450}
\expandafter\gdef\csname R@an.ablation.I1.kits.vs_parent_fresh\endcsname{-0.201}
\expandafter\gdef\csname R@an.ablation.I1.kits.vs_parent_s0\endcsname{-0.949}
\expandafter\gdef\csname R@an.ablation.I1.kits.vs_pool\endcsname{+1.893}
\expandafter\gdef\csname R@an.ablation.I1.kits.vs_unc\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.I1.kits.vs_union\endcsname{+1.649}
\expandafter\gdef\csname R@an.ablation.I1.param_match\endcsname{unmatched}
\expandafter\gdef\csname R@an.ablation.I1.param_ratio\endcsname{1.000}
\expandafter\gdef\csname R@an.ablation.I1.params_m\endcsname{29.59}
\expandafter\gdef\csname R@an.ablation.I1.role\endcsname{child}
\expandafter\gdef\csname R@an.ablation.I1.step_ratio\endcsname{1.005}
\expandafter\gdef\csname R@an.ablation.I1.step_ratio_kits\endcsname{1.005}
\expandafter\gdef\csname R@an.ablation.L3.acdc_fit\endcsname{fits}
\expandafter\gdef\csname R@an.ablation.L3.amos.band\endcsname{screen fired on the primary bar and the non-empty-GT secondary}
\expandafter\gdef\csname R@an.ablation.L3.amos.d\endcsname{+0.382}
\expandafter\gdef\csname R@an.ablation.L3.amos.d_unc\endcsname{+0.353}
\expandafter\gdef\csname R@an.ablation.L3.amos.dice\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.L3.amos.dne\endcsname{+0.385}
\expandafter\gdef\csname R@an.ablation.L3.amos.fresh_d\endcsname{+0.132}
\expandafter\gdef\csname R@an.ablation.L3.amos.fresh_dunion\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.L3.amos.fresh_mean\endcsname{87.833}
\expandafter\gdef\csname R@an.ablation.L3.amos.fresh_n\endcsname{2}
\expandafter\gdef\csname R@an.ablation.L3.amos.fresh_rel_floor\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.L3.amos.fresh_s1\endcsname{87.981}
\expandafter\gdef\csname R@an.ablation.L3.amos.fresh_s2\endcsname{87.686}
\expandafter\gdef\csname R@an.ablation.L3.amos.fresh_se\endcsname{0.122}
\expandafter\gdef\csname R@an.ablation.L3.amos.fresh_state\endcsname{finished}
\expandafter\gdef\csname R@an.ablation.L3.amos.fresh_vs_parent_fresh\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.L3.amos.move\endcsname{-0.249}
\expandafter\gdef\csname R@an.ablation.L3.amos.se\endcsname{0.132}
\expandafter\gdef\csname R@an.ablation.L3.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.L3.amos.verdict\endcsname{screen fired}
\expandafter\gdef\csname R@an.ablation.L3.amos.vs_contemp\endcsname{+0.371}
\expandafter\gdef\csname R@an.ablation.L3.amos.vs_pool\endcsname{+0.382}
\expandafter\gdef\csname R@an.ablation.L3.amos.vs_unc\endcsname{+0.353}
\expandafter\gdef\csname R@an.ablation.L3.amos.vs_union\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.L3.control\endcsname{the frozen default pool}
\expandafter\gdef\csname R@an.ablation.L3.dparams\endcsname{-1.53}
\expandafter\gdef\csname R@an.ablation.L3.dparams_pct\endcsname{-4.9}
\expandafter\gdef\csname R@an.ablation.L3.kits.band\endcsname{screen fired}
\expandafter\gdef\csname R@an.ablation.L3.kits.d\endcsname{+2.842}
\expandafter\gdef\csname R@an.ablation.L3.kits.d_unc\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.L3.kits.dice\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.L3.kits.dne\endcsname{+2.842}
\expandafter\gdef\csname R@an.ablation.L3.kits.fresh_d\endcsname{+2.094}
\expandafter\gdef\csname R@an.ablation.L3.kits.fresh_dunion\endcsname{+1.850}
\expandafter\gdef\csname R@an.ablation.L3.kits.fresh_mean\endcsname{85.472}
\expandafter\gdef\csname R@an.ablation.L3.kits.fresh_n\endcsname{2}
\expandafter\gdef\csname R@an.ablation.L3.kits.fresh_rel_floor\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.L3.kits.fresh_s1\endcsname{85.176}
\expandafter\gdef\csname R@an.ablation.L3.kits.fresh_s2\endcsname{85.768}
\expandafter\gdef\csname R@an.ablation.L3.kits.fresh_se\endcsname{0.795}
\expandafter\gdef\csname R@an.ablation.L3.kits.fresh_state\endcsname{finished}
\expandafter\gdef\csname R@an.ablation.L3.kits.fresh_vs_parent_fresh\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.L3.kits.move\endcsname{-0.748}
\expandafter\gdef\csname R@an.ablation.L3.kits.se\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.L3.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.L3.kits.verdict\endcsname{screen fired}
\expandafter\gdef\csname R@an.ablation.L3.kits.vs_contemp\endcsname{+2.355}
\expandafter\gdef\csname R@an.ablation.L3.kits.vs_pool\endcsname{+2.842}
\expandafter\gdef\csname R@an.ablation.L3.kits.vs_unc\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.L3.kits.vs_union\endcsname{+2.598}
\expandafter\gdef\csname R@an.ablation.L3.param_match\endcsname{unmatched}
\expandafter\gdef\csname R@an.ablation.L3.param_ratio\endcsname{0.951}
\expandafter\gdef\csname R@an.ablation.L3.params_m\endcsname{29.59}
\expandafter\gdef\csname R@an.ablation.L3.role\endcsname{parent}
\expandafter\gdef\csname R@an.ablation.L3.step_ratio\endcsname{1.528}
\expandafter\gdef\csname R@an.ablation.L3.step_ratio_kits\endcsname{1.401}
\expandafter\gdef\csname R@an.ablation.L3k3.acdc_fit\endcsname{fits}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.band\endcsname{not resolvable at one seed ($|\Delta|$ $<$ 0.50 pp)}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.d\endcsname{+0.078}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.dice\endcsname{88.160}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.dsec\endcsname{+0.244}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.edge_gap\endcsname{+0.078}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.fresh_dunion\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.fresh_rel_floor\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.fresh_se\endcsname{0.122}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.fresh_vs_parent_fresh\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.inspan\endcsname{above}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.parent_all\endcsname{87.916}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.parent_fresh\endcsname{87.833}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.parent_max\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.parent_min\endcsname{87.686}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.parent_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.parent_s0\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.parent_span\endcsname{0.397}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.rel_floor\endcsname{within}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.se\endcsname{0.173}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.se_parent_all\endcsname{0.141}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.se_parent_fresh\endcsname{0.150}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.se_parent_s0\endcsname{0.173}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.sesec\endcsname{0.141}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.verdict\endcsname{not resolved at one seed}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.vs_contemp\endcsname{+0.448}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.vs_parent_all\endcsname{+0.244}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.vs_parent_fresh\endcsname{+0.327}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.vs_parent_s0\endcsname{+0.078}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.vs_pool\endcsname{+0.459}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.vs_unc\endcsname{+0.430}
\expandafter\gdef\csname R@an.ablation.L3k3.amos.vs_union\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.L3k3.control\endcsname{HyReX seed 0}
\expandafter\gdef\csname R@an.ablation.L3k3.dparams\endcsname{-1.01}
\expandafter\gdef\csname R@an.ablation.L3k3.dparams_pct\endcsname{-3.4}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.band\endcsname{resolvable at the 0.50 pp one-seed floor (HyReX above); reported as ``kernel size or the 3.4\% capacity that comes with it'', never kernel alone}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.d\endcsname{-1.475}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.dice\endcsname{84.745}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.dsec\endcsname{-0.977}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.edge_gap\endcsname{-0.431}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.fresh_dunion\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.fresh_rel_floor\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.fresh_se\endcsname{0.795}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.fresh_vs_parent_fresh\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.inspan\endcsname{below}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.parent_all\endcsname{85.721}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.parent_fresh\endcsname{85.472}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.parent_max\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.parent_min\endcsname{85.176}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.parent_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.parent_s0\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.parent_span\endcsname{1.044}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.rel_floor\endcsname{below}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.se\endcsname{1.124}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.se_parent_all\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.se_parent_fresh\endcsname{0.974}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.se_parent_s0\endcsname{1.124}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.sesec\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.verdict\endcsname{resolved (HyReX above)}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.vs_contemp\endcsname{+0.879}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.vs_parent_all\endcsname{-0.977}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.vs_parent_fresh\endcsname{-0.727}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.vs_parent_s0\endcsname{-1.475}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.vs_pool\endcsname{+1.366}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.vs_unc\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.L3k3.kits.vs_union\endcsname{+1.123}
\expandafter\gdef\csname R@an.ablation.L3k3.param_match\endcsname{unmatched}
\expandafter\gdef\csname R@an.ablation.L3k3.param_ratio\endcsname{0.966}
\expandafter\gdef\csname R@an.ablation.L3k3.params_m\endcsname{28.58}
\expandafter\gdef\csname R@an.ablation.L3k3.role\endcsname{child}
\expandafter\gdef\csname R@an.ablation.L3k3.step_ratio\endcsname{0.881}
\expandafter\gdef\csname R@an.ablation.L3k3.step_ratio_kits\endcsname{0.909}
\expandafter\gdef\csname R@an.ablation.L3ng.acdc_fit\endcsname{does not fit}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.band\endcsname{not resolvable at one seed ($|\Delta|$ $<$ 0.50 pp)}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.d\endcsname{-0.114}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.dice\endcsname{87.969}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.dsec\endcsname{+0.052}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.edge_gap\endcsname{0.000}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.fresh_dunion\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.fresh_rel_floor\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.fresh_se\endcsname{0.122}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.fresh_vs_parent_fresh\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.inspan\endcsname{inside}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.parent_all\endcsname{87.916}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.parent_fresh\endcsname{87.833}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.parent_max\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.parent_min\endcsname{87.686}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.parent_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.parent_s0\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.parent_span\endcsname{0.397}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.rel_floor\endcsname{within}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.se\endcsname{0.173}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.se_parent_all\endcsname{0.141}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.se_parent_fresh\endcsname{0.150}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.se_parent_s0\endcsname{0.173}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.sesec\endcsname{0.141}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.verdict\endcsname{not resolved at one seed}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.vs_contemp\endcsname{+0.257}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.vs_parent_all\endcsname{+0.052}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.vs_parent_fresh\endcsname{+0.135}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.vs_parent_s0\endcsname{-0.114}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.vs_pool\endcsname{+0.268}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.vs_unc\endcsname{+0.239}
\expandafter\gdef\csname R@an.ablation.L3ng.amos.vs_union\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.L3ng.control\endcsname{HyReX seed 0}
\expandafter\gdef\csname R@an.ablation.L3ng.dparams\endcsname{-0.02}
\expandafter\gdef\csname R@an.ablation.L3ng.dparams_pct\endcsname{-0.1}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.band\endcsname{not resolvable at one seed ($|\Delta|$ $<$ 0.50 pp)}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.d\endcsname{-0.281}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.dice\endcsname{85.939}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.dsec\endcsname{+0.218}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.edge_gap\endcsname{0.000}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.fresh_dunion\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.fresh_rel_floor\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.fresh_se\endcsname{0.795}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.fresh_vs_parent_fresh\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.inspan\endcsname{inside}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.parent_all\endcsname{85.721}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.parent_fresh\endcsname{85.472}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.parent_max\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.parent_min\endcsname{85.176}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.parent_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.parent_s0\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.parent_span\endcsname{1.044}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.rel_floor\endcsname{within}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.se\endcsname{1.124}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.se_parent_all\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.se_parent_fresh\endcsname{0.974}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.se_parent_s0\endcsname{1.124}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.sesec\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.verdict\endcsname{not resolved at one seed}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.vs_contemp\endcsname{+2.074}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.vs_parent_all\endcsname{+0.218}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.vs_parent_fresh\endcsname{+0.468}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.vs_parent_s0\endcsname{-0.281}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.vs_pool\endcsname{+2.561}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.vs_unc\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.L3ng.kits.vs_union\endcsname{+2.317}
\expandafter\gdef\csname R@an.ablation.L3ng.param_match\endcsname{unmatched}
\expandafter\gdef\csname R@an.ablation.L3ng.param_ratio\endcsname{0.999}
\expandafter\gdef\csname R@an.ablation.L3ng.params_m\endcsname{29.57}
\expandafter\gdef\csname R@an.ablation.L3ng.role\endcsname{child}
\expandafter\gdef\csname R@an.ablation.L3ng.step_ratio\endcsname{0.976}
\expandafter\gdef\csname R@an.ablation.L3ng.step_ratio_kits\endcsname{0.983}
\expandafter\gdef\csname R@an.ablation.L6.acdc_fit\endcsname{fits}
\expandafter\gdef\csname R@an.ablation.L6.amos.band\endcsname{not resolvable at one seed ($|\Delta|$ $<$ 0.50 pp)}
\expandafter\gdef\csname R@an.ablation.L6.amos.d\endcsname{-0.366}
\expandafter\gdef\csname R@an.ablation.L6.amos.dice\endcsname{87.717}
\expandafter\gdef\csname R@an.ablation.L6.amos.dsec\endcsname{-0.200}
\expandafter\gdef\csname R@an.ablation.L6.amos.edge_gap\endcsname{0.000}
\expandafter\gdef\csname R@an.ablation.L6.amos.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L6.amos.fresh_dunion\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.L6.amos.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L6.amos.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.L6.amos.fresh_rel_floor\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L6.amos.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L6.amos.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L6.amos.fresh_se\endcsname{0.122}
\expandafter\gdef\csname R@an.ablation.L6.amos.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.L6.amos.fresh_vs_parent_fresh\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L6.amos.inspan\endcsname{inside}
\expandafter\gdef\csname R@an.ablation.L6.amos.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.L6.amos.parent_all\endcsname{87.916}
\expandafter\gdef\csname R@an.ablation.L6.amos.parent_fresh\endcsname{87.833}
\expandafter\gdef\csname R@an.ablation.L6.amos.parent_max\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.L6.amos.parent_min\endcsname{87.686}
\expandafter\gdef\csname R@an.ablation.L6.amos.parent_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.L6.amos.parent_s0\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.L6.amos.parent_span\endcsname{0.397}
\expandafter\gdef\csname R@an.ablation.L6.amos.rel_floor\endcsname{within}
\expandafter\gdef\csname R@an.ablation.L6.amos.se\endcsname{0.173}
\expandafter\gdef\csname R@an.ablation.L6.amos.se_parent_all\endcsname{0.141}
\expandafter\gdef\csname R@an.ablation.L6.amos.se_parent_fresh\endcsname{0.150}
\expandafter\gdef\csname R@an.ablation.L6.amos.se_parent_s0\endcsname{0.173}
\expandafter\gdef\csname R@an.ablation.L6.amos.sesec\endcsname{0.141}
\expandafter\gdef\csname R@an.ablation.L6.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.L6.amos.verdict\endcsname{not resolved at one seed}
\expandafter\gdef\csname R@an.ablation.L6.amos.vs_contemp\endcsname{+0.005}
\expandafter\gdef\csname R@an.ablation.L6.amos.vs_parent_all\endcsname{-0.200}
\expandafter\gdef\csname R@an.ablation.L6.amos.vs_parent_fresh\endcsname{-0.117}
\expandafter\gdef\csname R@an.ablation.L6.amos.vs_parent_s0\endcsname{-0.366}
\expandafter\gdef\csname R@an.ablation.L6.amos.vs_pool\endcsname{+0.016}
\expandafter\gdef\csname R@an.ablation.L6.amos.vs_unc\endcsname{-0.013}
\expandafter\gdef\csname R@an.ablation.L6.amos.vs_union\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.L6.control\endcsname{HyReX seed 0}
\expandafter\gdef\csname R@an.ablation.L6.dparams\endcsname{+1.50}
\expandafter\gdef\csname R@an.ablation.L6.dparams_pct\endcsname{+5.1}
\expandafter\gdef\csname R@an.ablation.L6.kits.band\endcsname{not resolvable at one seed ($|\Delta|$ $<$ 0.50 pp)}
\expandafter\gdef\csname R@an.ablation.L6.kits.d\endcsname{-0.316}
\expandafter\gdef\csname R@an.ablation.L6.kits.dfresh\endcsname{-0.502}
\expandafter\gdef\csname R@an.ablation.L6.kits.dfresh_in_sd\endcsname{0.63}
\expandafter\gdef\csname R@an.ablation.L6.kits.dice\endcsname{85.904}
\expandafter\gdef\csname R@an.ablation.L6.kits.dsec\endcsname{+0.183}
\expandafter\gdef\csname R@an.ablation.L6.kits.edge_gap\endcsname{0.000}
\expandafter\gdef\csname R@an.ablation.L6.kits.fresh_d\endcsname{+1.591}
\expandafter\gdef\csname R@an.ablation.L6.kits.fresh_dunion\endcsname{+1.348}
\expandafter\gdef\csname R@an.ablation.L6.kits.fresh_mean\endcsname{84.970}
\expandafter\gdef\csname R@an.ablation.L6.kits.fresh_n\endcsname{2}
\expandafter\gdef\csname R@an.ablation.L6.kits.fresh_rel_floor\endcsname{below}
\expandafter\gdef\csname R@an.ablation.L6.kits.fresh_s1\endcsname{84.577}
\expandafter\gdef\csname R@an.ablation.L6.kits.fresh_s2\endcsname{85.363}
\expandafter\gdef\csname R@an.ablation.L6.kits.fresh_se\endcsname{0.795}
\expandafter\gdef\csname R@an.ablation.L6.kits.fresh_state\endcsname{finished}
\expandafter\gdef\csname R@an.ablation.L6.kits.fresh_vs_parent_fresh\endcsname{-0.502}
\expandafter\gdef\csname R@an.ablation.L6.kits.inspan\endcsname{inside}
\expandafter\gdef\csname R@an.ablation.L6.kits.move\endcsname{-0.935}
\expandafter\gdef\csname R@an.ablation.L6.kits.parent_all\endcsname{85.721}
\expandafter\gdef\csname R@an.ablation.L6.kits.parent_fresh\endcsname{85.472}
\expandafter\gdef\csname R@an.ablation.L6.kits.parent_max\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.L6.kits.parent_min\endcsname{85.176}
\expandafter\gdef\csname R@an.ablation.L6.kits.parent_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.L6.kits.parent_s0\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.L6.kits.parent_span\endcsname{1.044}
\expandafter\gdef\csname R@an.ablation.L6.kits.rel_floor\endcsname{within}
\expandafter\gdef\csname R@an.ablation.L6.kits.se\endcsname{1.124}
\expandafter\gdef\csname R@an.ablation.L6.kits.se_parent_all\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.L6.kits.se_parent_fresh\endcsname{0.974}
\expandafter\gdef\csname R@an.ablation.L6.kits.se_parent_s0\endcsname{1.124}
\expandafter\gdef\csname R@an.ablation.L6.kits.sefresh\endcsname{0.795}
\expandafter\gdef\csname R@an.ablation.L6.kits.sesec\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.L6.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.L6.kits.verdict\endcsname{not resolved at one seed}
\expandafter\gdef\csname R@an.ablation.L6.kits.vs_contemp\endcsname{+2.039}
\expandafter\gdef\csname R@an.ablation.L6.kits.vs_parent_all\endcsname{+0.183}
\expandafter\gdef\csname R@an.ablation.L6.kits.vs_parent_fresh\endcsname{+0.433}
\expandafter\gdef\csname R@an.ablation.L6.kits.vs_parent_s0\endcsname{-0.316}
\expandafter\gdef\csname R@an.ablation.L6.kits.vs_pool\endcsname{+2.526}
\expandafter\gdef\csname R@an.ablation.L6.kits.vs_unc\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.L6.kits.vs_union\endcsname{+2.283}
\expandafter\gdef\csname R@an.ablation.L6.param_match\endcsname{matched}
\expandafter\gdef\csname R@an.ablation.L6.param_ratio\endcsname{1.051}
\expandafter\gdef\csname R@an.ablation.L6.params_m\endcsname{31.09}
\expandafter\gdef\csname R@an.ablation.L6.role\endcsname{child}
\expandafter\gdef\csname R@an.ablation.L6.step_ratio\endcsname{1.228}
\expandafter\gdef\csname R@an.ablation.L6.step_ratio_kits\endcsname{1.167}
\expandafter\gdef\csname R@an.ablation.N1.acdc_fit\endcsname{fits}
\expandafter\gdef\csname R@an.ablation.N1.amos.band\endcsname{KILL: channel grouping does not help in this harness (AMOS22 $\le$ 87.701 AND KiTS23 $\le$ 83.378, the two frozen pool means); no placement follow-up}
\expandafter\gdef\csname R@an.ablation.N1.amos.d\endcsname{-0.923}
\expandafter\gdef\csname R@an.ablation.N1.amos.d_unc\endcsname{-0.952}
\expandafter\gdef\csname R@an.ablation.N1.amos.dice\endcsname{86.778}
\expandafter\gdef\csname R@an.ablation.N1.amos.dne\endcsname{-0.796}
\expandafter\gdef\csname R@an.ablation.N1.amos.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.N1.amos.fresh_dunion\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.N1.amos.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.N1.amos.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.N1.amos.fresh_rel_floor\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.N1.amos.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.N1.amos.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.N1.amos.fresh_se\endcsname{0.122}
\expandafter\gdef\csname R@an.ablation.N1.amos.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.N1.amos.fresh_vs_parent_fresh\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.N1.amos.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.N1.amos.se\endcsname{0.132}
\expandafter\gdef\csname R@an.ablation.N1.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.N1.amos.verdict\endcsname{KILL}
\expandafter\gdef\csname R@an.ablation.N1.amos.vs_contemp\endcsname{-0.934}
\expandafter\gdef\csname R@an.ablation.N1.amos.vs_pool\endcsname{-0.923}
\expandafter\gdef\csname R@an.ablation.N1.amos.vs_unc\endcsname{-0.952}
\expandafter\gdef\csname R@an.ablation.N1.amos.vs_union\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.N1.control\endcsname{the frozen default pool}
\expandafter\gdef\csname R@an.ablation.N1.dparams\endcsname{0.00}
\expandafter\gdef\csname R@an.ablation.N1.dparams_pct\endcsname{0.0}
\expandafter\gdef\csname R@an.ablation.N1.kits.band\endcsname{at or below the frozen pool mean: the KiTS23 leg of the registered kill rule is met}
\expandafter\gdef\csname R@an.ablation.N1.kits.d\endcsname{-6.492}
\expandafter\gdef\csname R@an.ablation.N1.kits.d_unc\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.N1.kits.dice\endcsname{76.886}
\expandafter\gdef\csname R@an.ablation.N1.kits.dne\endcsname{-6.492}
\expandafter\gdef\csname R@an.ablation.N1.kits.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.N1.kits.fresh_dunion\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.N1.kits.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.N1.kits.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.N1.kits.fresh_rel_floor\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.N1.kits.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.N1.kits.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.N1.kits.fresh_se\endcsname{0.795}
\expandafter\gdef\csname R@an.ablation.N1.kits.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.N1.kits.fresh_vs_parent_fresh\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.N1.kits.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.N1.kits.se\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.N1.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.N1.kits.verdict\endcsname{kill-rule leg met}
\expandafter\gdef\csname R@an.ablation.N1.kits.vs_contemp\endcsname{-6.979}
\expandafter\gdef\csname R@an.ablation.N1.kits.vs_pool\endcsname{-6.492}
\expandafter\gdef\csname R@an.ablation.N1.kits.vs_unc\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.N1.kits.vs_union\endcsname{-6.736}
\expandafter\gdef\csname R@an.ablation.N1.param_match\endcsname{matched}
\expandafter\gdef\csname R@an.ablation.N1.param_ratio\endcsname{1.000}
\expandafter\gdef\csname R@an.ablation.N1.params_m\endcsname{31.12}
\expandafter\gdef\csname R@an.ablation.N1.role\endcsname{registered variant}
\expandafter\gdef\csname R@an.ablation.N1.step_ratio\endcsname{2.059}
\expandafter\gdef\csname R@an.ablation.N1.step_ratio_kits\endcsname{2.142}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.acdc_fit\endcsname{fits}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.band\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.d_unc\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.dice\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.dne\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.fresh_dunion\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.fresh_rel_floor\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.fresh_se\endcsname{0.122}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.fresh_vs_parent_fresh\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.se\endcsname{0.132}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.state\endcsname{not started}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.verdict\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.vs_contemp\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.vs_pool\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.vs_unc\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.amos.vs_union\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.control\endcsname{the frozen default pool}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.dparams\endcsname{+0.07}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.dparams_pct\endcsname{+0.2}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.band\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.d_unc\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.dice\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.dne\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.fresh_dunion\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.fresh_rel_floor\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.fresh_se\endcsname{0.795}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.fresh_vs_parent_fresh\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.se\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.state\endcsname{not started}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.verdict\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.vs_contemp\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.vs_pool\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.vs_unc\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.kits.vs_union\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.param_match\endcsname{unmatched}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.param_ratio\endcsname{1.002}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.params_m\endcsname{31.20}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.role\endcsname{registered variant}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.step_ratio\endcsname{2.145}
\expandafter\gdef\csname R@an.ablation.P1_frcap32.step_ratio_kits\endcsname{2.647}
\expandafter\gdef\csname R@an.ablation.P1b.acdc_fit\endcsname{fits}
\expandafter\gdef\csname R@an.ablation.P1b.amos.band\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1b.amos.d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1b.amos.d_unc\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1b.amos.dice\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1b.amos.dne\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1b.amos.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1b.amos.fresh_dunion\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1b.amos.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1b.amos.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.P1b.amos.fresh_rel_floor\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1b.amos.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1b.amos.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1b.amos.fresh_se\endcsname{0.122}
\expandafter\gdef\csname R@an.ablation.P1b.amos.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.P1b.amos.fresh_vs_parent_fresh\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1b.amos.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1b.amos.se\endcsname{0.132}
\expandafter\gdef\csname R@an.ablation.P1b.amos.state\endcsname{not started}
\expandafter\gdef\csname R@an.ablation.P1b.amos.verdict\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1b.amos.vs_contemp\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1b.amos.vs_pool\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1b.amos.vs_unc\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1b.amos.vs_union\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1b.control\endcsname{the frozen default pool}
\expandafter\gdef\csname R@an.ablation.P1b.dparams\endcsname{+0.07}
\expandafter\gdef\csname R@an.ablation.P1b.dparams_pct\endcsname{+0.2}
\expandafter\gdef\csname R@an.ablation.P1b.param_match\endcsname{matched}
\expandafter\gdef\csname R@an.ablation.P1b.param_ratio\endcsname{1.002}
\expandafter\gdef\csname R@an.ablation.P1b.params_m\endcsname{31.20}
\expandafter\gdef\csname R@an.ablation.P1b.role\endcsname{registered variant}
\expandafter\gdef\csname R@an.ablation.P1b.step_ratio\endcsname{1.074}
\expandafter\gdef\csname R@an.ablation.P1b.step_ratio_kits\endcsname{1.008}
\expandafter\gdef\csname R@an.ablation.P1c.acdc_fit\endcsname{fits}
\expandafter\gdef\csname R@an.ablation.P1c.amos.band\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.amos.d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.amos.d_unc\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.amos.dice\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.amos.dne\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.amos.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.amos.fresh_dunion\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1c.amos.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.amos.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.P1c.amos.fresh_rel_floor\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1c.amos.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.amos.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.amos.fresh_se\endcsname{0.122}
\expandafter\gdef\csname R@an.ablation.P1c.amos.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.P1c.amos.fresh_vs_parent_fresh\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1c.amos.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.amos.se\endcsname{0.132}
\expandafter\gdef\csname R@an.ablation.P1c.amos.state\endcsname{not started}
\expandafter\gdef\csname R@an.ablation.P1c.amos.verdict\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.amos.vs_contemp\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.amos.vs_pool\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.amos.vs_unc\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.amos.vs_union\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1c.control\endcsname{the frozen default pool}
\expandafter\gdef\csname R@an.ablation.P1c.dparams\endcsname{+0.44}
\expandafter\gdef\csname R@an.ablation.P1c.dparams_pct\endcsname{+1.4}
\expandafter\gdef\csname R@an.ablation.P1c.kits.band\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.kits.d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.kits.d_unc\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1c.kits.dice\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.kits.dne\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.kits.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.kits.fresh_dunion\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.kits.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.kits.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.P1c.kits.fresh_rel_floor\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1c.kits.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.kits.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.kits.fresh_se\endcsname{0.795}
\expandafter\gdef\csname R@an.ablation.P1c.kits.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.P1c.kits.fresh_vs_parent_fresh\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1c.kits.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.kits.se\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.P1c.kits.state\endcsname{not started}
\expandafter\gdef\csname R@an.ablation.P1c.kits.verdict\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.kits.vs_contemp\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.kits.vs_pool\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.kits.vs_unc\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P1c.kits.vs_union\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P1c.param_match\endcsname{unmatched}
\expandafter\gdef\csname R@an.ablation.P1c.param_ratio\endcsname{1.014}
\expandafter\gdef\csname R@an.ablation.P1c.params_m\endcsname{31.57}
\expandafter\gdef\csname R@an.ablation.P1c.role\endcsname{registered variant}
\expandafter\gdef\csname R@an.ablation.P1c.step_ratio\endcsname{1.018}
\expandafter\gdef\csname R@an.ablation.P1c.step_ratio_kits\endcsname{1.007}
\expandafter\gdef\csname R@an.ablation.P3c.amos.valid\endcsname{valid}
\expandafter\gdef\csname R@an.ablation.P3c.kits.valid\endcsname{valid}
\expandafter\gdef\csname R@an.ablation.P3lite.acdc_fit\endcsname{fits}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.band\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.dice\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.fresh_dunion\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.fresh_rel_floor\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.fresh_se\endcsname{0.122}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.fresh_vs_parent_fresh\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.se\endcsname{0.173}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.state\endcsname{not started}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.verdict\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.vs_contemp\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.vs_pool\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.vs_unc\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.amos.vs_union\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P3lite.control\endcsname{the function-identical control}
\expandafter\gdef\csname R@an.ablation.P3lite.dparams\endcsname{0.00}
\expandafter\gdef\csname R@an.ablation.P3lite.dparams_pct\endcsname{0.0}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.band\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.dice\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.fresh_dunion\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.fresh_rel_floor\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.fresh_se\endcsname{0.795}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.fresh_vs_parent_fresh\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.se\endcsname{1.124}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.state\endcsname{not started}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.verdict\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.vs_contemp\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.vs_pool\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.vs_unc\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.P3lite.kits.vs_union\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.P3lite.param_match\endcsname{matched}
\expandafter\gdef\csname R@an.ablation.P3lite.param_ratio\endcsname{1.000}
\expandafter\gdef\csname R@an.ablation.P3lite.params_m\endcsname{31.12}
\expandafter\gdef\csname R@an.ablation.P3lite.role\endcsname{registered variant}
\expandafter\gdef\csname R@an.ablation.P3lite.step_ratio\endcsname{1.001}
\expandafter\gdef\csname R@an.ablation.P3lite.step_ratio_kits\endcsname{0.998}
\expandafter\gdef\csname R@an.ablation.S2.acdc_fit\endcsname{does not fit}
\expandafter\gdef\csname R@an.ablation.S2.amos.band\endcsname{KILL: S2 - HyReX over HMS $\le$ 0 on AMOS22}
\expandafter\gdef\csname R@an.ablation.S2.amos.d\endcsname{-0.004}
\expandafter\gdef\csname R@an.ablation.S2.amos.dice\endcsname{88.079}
\expandafter\gdef\csname R@an.ablation.S2.amos.dsec\endcsname{+0.163}
\expandafter\gdef\csname R@an.ablation.S2.amos.edge_gap\endcsname{0.000}
\expandafter\gdef\csname R@an.ablation.S2.amos.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.S2.amos.fresh_dunion\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.S2.amos.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.S2.amos.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.S2.amos.fresh_rel_floor\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.S2.amos.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.S2.amos.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.S2.amos.fresh_se\endcsname{0.122}
\expandafter\gdef\csname R@an.ablation.S2.amos.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.S2.amos.fresh_vs_parent_fresh\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.S2.amos.inspan\endcsname{inside}
\expandafter\gdef\csname R@an.ablation.S2.amos.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.S2.amos.parent_all\endcsname{87.916}
\expandafter\gdef\csname R@an.ablation.S2.amos.parent_fresh\endcsname{87.833}
\expandafter\gdef\csname R@an.ablation.S2.amos.parent_max\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.S2.amos.parent_min\endcsname{87.686}
\expandafter\gdef\csname R@an.ablation.S2.amos.parent_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.S2.amos.parent_s0\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.S2.amos.parent_span\endcsname{0.397}
\expandafter\gdef\csname R@an.ablation.S2.amos.rel_floor\endcsname{within}
\expandafter\gdef\csname R@an.ablation.S2.amos.se\endcsname{0.173}
\expandafter\gdef\csname R@an.ablation.S2.amos.se_parent_all\endcsname{0.141}
\expandafter\gdef\csname R@an.ablation.S2.amos.se_parent_fresh\endcsname{0.150}
\expandafter\gdef\csname R@an.ablation.S2.amos.se_parent_s0\endcsname{0.173}
\expandafter\gdef\csname R@an.ablation.S2.amos.sesec\endcsname{0.141}
\expandafter\gdef\csname R@an.ablation.S2.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.S2.amos.verdict\endcsname{KILL (HMS)}
\expandafter\gdef\csname R@an.ablation.S2.amos.vs_contemp\endcsname{+0.367}
\expandafter\gdef\csname R@an.ablation.S2.amos.vs_parent_all\endcsname{+0.163}
\expandafter\gdef\csname R@an.ablation.S2.amos.vs_parent_fresh\endcsname{+0.246}
\expandafter\gdef\csname R@an.ablation.S2.amos.vs_parent_s0\endcsname{-0.004}
\expandafter\gdef\csname R@an.ablation.S2.amos.vs_pool\endcsname{+0.378}
\expandafter\gdef\csname R@an.ablation.S2.amos.vs_unc\endcsname{+0.349}
\expandafter\gdef\csname R@an.ablation.S2.amos.vs_union\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.S2.control\endcsname{HyReX seed 0}
\expandafter\gdef\csname R@an.ablation.S2.dparams\endcsname{-1.87}
\expandafter\gdef\csname R@an.ablation.S2.dparams_pct\endcsname{-6.3}
\expandafter\gdef\csname R@an.ablation.S2.hms.d\endcsname{-0.163}
\expandafter\gdef\csname R@an.ablation.S2.hms.se\endcsname{0.266}
\expandafter\gdef\csname R@an.ablation.S2.kits.band\endcsname{resolvable at the 0.50 pp one-seed floor (HyReX above)}
\expandafter\gdef\csname R@an.ablation.S2.kits.d\endcsname{-1.500}
\expandafter\gdef\csname R@an.ablation.S2.kits.dice\endcsname{84.720}
\expandafter\gdef\csname R@an.ablation.S2.kits.dsec\endcsname{-1.002}
\expandafter\gdef\csname R@an.ablation.S2.kits.edge_gap\endcsname{-0.456}
\expandafter\gdef\csname R@an.ablation.S2.kits.fresh_d\endcsname{+0.570}
\expandafter\gdef\csname R@an.ablation.S2.kits.fresh_dunion\endcsname{+0.326}
\expandafter\gdef\csname R@an.ablation.S2.kits.fresh_mean\endcsname{83.948}
\expandafter\gdef\csname R@an.ablation.S2.kits.fresh_n\endcsname{2}
\expandafter\gdef\csname R@an.ablation.S2.kits.fresh_rel_floor\endcsname{below}
\expandafter\gdef\csname R@an.ablation.S2.kits.fresh_s1\endcsname{84.161}
\expandafter\gdef\csname R@an.ablation.S2.kits.fresh_s2\endcsname{83.736}
\expandafter\gdef\csname R@an.ablation.S2.kits.fresh_se\endcsname{0.795}
\expandafter\gdef\csname R@an.ablation.S2.kits.fresh_state\endcsname{finished}
\expandafter\gdef\csname R@an.ablation.S2.kits.fresh_vs_parent_fresh\endcsname{-1.523}
\expandafter\gdef\csname R@an.ablation.S2.kits.inspan\endcsname{below}
\expandafter\gdef\csname R@an.ablation.S2.kits.move\endcsname{-0.771}
\expandafter\gdef\csname R@an.ablation.S2.kits.parent_all\endcsname{85.721}
\expandafter\gdef\csname R@an.ablation.S2.kits.parent_fresh\endcsname{85.472}
\expandafter\gdef\csname R@an.ablation.S2.kits.parent_max\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.S2.kits.parent_min\endcsname{85.176}
\expandafter\gdef\csname R@an.ablation.S2.kits.parent_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.S2.kits.parent_s0\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.S2.kits.parent_span\endcsname{1.044}
\expandafter\gdef\csname R@an.ablation.S2.kits.rel_floor\endcsname{below}
\expandafter\gdef\csname R@an.ablation.S2.kits.se\endcsname{1.124}
\expandafter\gdef\csname R@an.ablation.S2.kits.se_parent_all\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.S2.kits.se_parent_fresh\endcsname{0.974}
\expandafter\gdef\csname R@an.ablation.S2.kits.se_parent_s0\endcsname{1.124}
\expandafter\gdef\csname R@an.ablation.S2.kits.sesec\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.S2.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.S2.kits.verdict\endcsname{resolved (HyReX above)}
\expandafter\gdef\csname R@an.ablation.S2.kits.vs_contemp\endcsname{+0.854}
\expandafter\gdef\csname R@an.ablation.S2.kits.vs_parent_all\endcsname{-1.002}
\expandafter\gdef\csname R@an.ablation.S2.kits.vs_parent_fresh\endcsname{-0.752}
\expandafter\gdef\csname R@an.ablation.S2.kits.vs_parent_s0\endcsname{-1.500}
\expandafter\gdef\csname R@an.ablation.S2.kits.vs_pool\endcsname{+1.341}
\expandafter\gdef\csname R@an.ablation.S2.kits.vs_unc\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.S2.kits.vs_union\endcsname{+1.098}
\expandafter\gdef\csname R@an.ablation.S2.param_match\endcsname{unmatched}
\expandafter\gdef\csname R@an.ablation.S2.param_ratio\endcsname{0.937}
\expandafter\gdef\csname R@an.ablation.S2.params_m\endcsname{27.72}
\expandafter\gdef\csname R@an.ablation.S2.role\endcsname{child}
\expandafter\gdef\csname R@an.ablation.S2.step_ratio\endcsname{1.283}
\expandafter\gdef\csname R@an.ablation.S2.step_ratio_kits\endcsname{1.197}
\expandafter\gdef\csname R@an.ablation.W1c.acdc_fit\endcsname{fits}
\expandafter\gdef\csname R@an.ablation.W1c.amos.band\endcsname{not resolvable at one seed ($|\Delta|$ $<$ 0.50 pp)}
\expandafter\gdef\csname R@an.ablation.W1c.amos.d\endcsname{-0.019}
\expandafter\gdef\csname R@an.ablation.W1c.amos.dice\endcsname{88.064}
\expandafter\gdef\csname R@an.ablation.W1c.amos.dsec\endcsname{+0.148}
\expandafter\gdef\csname R@an.ablation.W1c.amos.edge_gap\endcsname{0.000}
\expandafter\gdef\csname R@an.ablation.W1c.amos.fresh_d\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.W1c.amos.fresh_dunion\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.W1c.amos.fresh_mean\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.W1c.amos.fresh_n\endcsname{0}
\expandafter\gdef\csname R@an.ablation.W1c.amos.fresh_rel_floor\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.W1c.amos.fresh_s1\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.W1c.amos.fresh_s2\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.W1c.amos.fresh_se\endcsname{0.122}
\expandafter\gdef\csname R@an.ablation.W1c.amos.fresh_state\endcsname{not registered}
\expandafter\gdef\csname R@an.ablation.W1c.amos.fresh_vs_parent_fresh\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.W1c.amos.inspan\endcsname{inside}
\expandafter\gdef\csname R@an.ablation.W1c.amos.move\endcsname{pending}
\expandafter\gdef\csname R@an.ablation.W1c.amos.parent_all\endcsname{87.916}
\expandafter\gdef\csname R@an.ablation.W1c.amos.parent_fresh\endcsname{87.833}
\expandafter\gdef\csname R@an.ablation.W1c.amos.parent_max\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.W1c.amos.parent_min\endcsname{87.686}
\expandafter\gdef\csname R@an.ablation.W1c.amos.parent_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.W1c.amos.parent_s0\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.W1c.amos.parent_span\endcsname{0.397}
\expandafter\gdef\csname R@an.ablation.W1c.amos.rel_floor\endcsname{within}
\expandafter\gdef\csname R@an.ablation.W1c.amos.se\endcsname{0.173}
\expandafter\gdef\csname R@an.ablation.W1c.amos.se_parent_all\endcsname{0.141}
\expandafter\gdef\csname R@an.ablation.W1c.amos.se_parent_fresh\endcsname{0.150}
\expandafter\gdef\csname R@an.ablation.W1c.amos.se_parent_s0\endcsname{0.173}
\expandafter\gdef\csname R@an.ablation.W1c.amos.sesec\endcsname{0.141}
\expandafter\gdef\csname R@an.ablation.W1c.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.W1c.amos.verdict\endcsname{not resolved at one seed}
\expandafter\gdef\csname R@an.ablation.W1c.amos.vs_contemp\endcsname{+0.352}
\expandafter\gdef\csname R@an.ablation.W1c.amos.vs_parent_all\endcsname{+0.148}
\expandafter\gdef\csname R@an.ablation.W1c.amos.vs_parent_fresh\endcsname{+0.231}
\expandafter\gdef\csname R@an.ablation.W1c.amos.vs_parent_s0\endcsname{-0.019}
\expandafter\gdef\csname R@an.ablation.W1c.amos.vs_pool\endcsname{+0.363}
\expandafter\gdef\csname R@an.ablation.W1c.amos.vs_unc\endcsname{+0.334}
\expandafter\gdef\csname R@an.ablation.W1c.amos.vs_union\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.W1c.control\endcsname{HyReX seed 0}
\expandafter\gdef\csname R@an.ablation.W1c.dparams\endcsname{+1.54}
\expandafter\gdef\csname R@an.ablation.W1c.dparams_pct\endcsname{+5.2}
\expandafter\gdef\csname R@an.ablation.W1c.kits.band\endcsname{not resolvable at one seed ($|\Delta|$ $<$ 0.50 pp)}
\expandafter\gdef\csname R@an.ablation.W1c.kits.d\endcsname{-0.206}
\expandafter\gdef\csname R@an.ablation.W1c.kits.dice\endcsname{86.014}
\expandafter\gdef\csname R@an.ablation.W1c.kits.dsec\endcsname{+0.293}
\expandafter\gdef\csname R@an.ablation.W1c.kits.edge_gap\endcsname{0.000}
\expandafter\gdef\csname R@an.ablation.W1c.kits.fresh_d\endcsname{+1.067}
\expandafter\gdef\csname R@an.ablation.W1c.kits.fresh_dunion\endcsname{+0.823}
\expandafter\gdef\csname R@an.ablation.W1c.kits.fresh_mean\endcsname{84.445}
\expandafter\gdef\csname R@an.ablation.W1c.kits.fresh_n\endcsname{2}
\expandafter\gdef\csname R@an.ablation.W1c.kits.fresh_rel_floor\endcsname{below}
\expandafter\gdef\csname R@an.ablation.W1c.kits.fresh_s1\endcsname{85.112}
\expandafter\gdef\csname R@an.ablation.W1c.kits.fresh_s2\endcsname{83.777}
\expandafter\gdef\csname R@an.ablation.W1c.kits.fresh_se\endcsname{0.795}
\expandafter\gdef\csname R@an.ablation.W1c.kits.fresh_state\endcsname{finished}
\expandafter\gdef\csname R@an.ablation.W1c.kits.fresh_vs_parent_fresh\endcsname{-1.027}
\expandafter\gdef\csname R@an.ablation.W1c.kits.inspan\endcsname{inside}
\expandafter\gdef\csname R@an.ablation.W1c.kits.move\endcsname{-1.569}
\expandafter\gdef\csname R@an.ablation.W1c.kits.parent_all\endcsname{85.721}
\expandafter\gdef\csname R@an.ablation.W1c.kits.parent_fresh\endcsname{85.472}
\expandafter\gdef\csname R@an.ablation.W1c.kits.parent_max\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.W1c.kits.parent_min\endcsname{85.176}
\expandafter\gdef\csname R@an.ablation.W1c.kits.parent_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.W1c.kits.parent_s0\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.W1c.kits.parent_span\endcsname{1.044}
\expandafter\gdef\csname R@an.ablation.W1c.kits.rel_floor\endcsname{within}
\expandafter\gdef\csname R@an.ablation.W1c.kits.se\endcsname{1.124}
\expandafter\gdef\csname R@an.ablation.W1c.kits.se_parent_all\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.W1c.kits.se_parent_fresh\endcsname{0.974}
\expandafter\gdef\csname R@an.ablation.W1c.kits.se_parent_s0\endcsname{1.124}
\expandafter\gdef\csname R@an.ablation.W1c.kits.sesec\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.W1c.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.ablation.W1c.kits.v4.center\endcsname{+0.000}
\expandafter\gdef\csname R@an.ablation.W1c.kits.v4.dist\endcsname{-1.569}
\expandafter\gdef\csname R@an.ablation.W1c.kits.v4.hi\endcsname{+2.834}
\expandafter\gdef\csname R@an.ablation.W1c.kits.v4.lo\endcsname{-2.837}
\expandafter\gdef\csname R@an.ablation.W1c.kits.v4.word\endcsname{inside}
\expandafter\gdef\csname R@an.ablation.W1c.kits.verdict\endcsname{not resolved at one seed}
\expandafter\gdef\csname R@an.ablation.W1c.kits.vs_contemp\endcsname{+2.148}
\expandafter\gdef\csname R@an.ablation.W1c.kits.vs_parent_all\endcsname{+0.293}
\expandafter\gdef\csname R@an.ablation.W1c.kits.vs_parent_fresh\endcsname{+0.542}
\expandafter\gdef\csname R@an.ablation.W1c.kits.vs_parent_s0\endcsname{-0.206}
\expandafter\gdef\csname R@an.ablation.W1c.kits.vs_pool\endcsname{+2.636}
\expandafter\gdef\csname R@an.ablation.W1c.kits.vs_unc\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.W1c.kits.vs_union\endcsname{+2.392}
\expandafter\gdef\csname R@an.ablation.W1c.param_match\endcsname{matched}
\expandafter\gdef\csname R@an.ablation.W1c.param_ratio\endcsname{1.052}
\expandafter\gdef\csname R@an.ablation.W1c.params_m\endcsname{31.14}
\expandafter\gdef\csname R@an.ablation.W1c.role\endcsname{parameter-matched control}
\expandafter\gdef\csname R@an.ablation.W1c.step_ratio\endcsname{0.750}
\expandafter\gdef\csname R@an.ablation.W1c.step_ratio_kits\endcsname{0.807}
\expandafter\gdef\csname R@an.ablation.bands.rows.amos\endcsname{15}
\expandafter\gdef\csname R@an.ablation.bands.rows.kits\endcsname{14}
\expandafter\gdef\csname R@an.ablation.count.children\endcsname{7}
\expandafter\gdef\csname R@an.ablation.count.controls\endcsname{1}
\expandafter\gdef\csname R@an.ablation.count.ctlref\endcsname{1}
\expandafter\gdef\csname R@an.ablation.count.directional\endcsname{3}
\expandafter\gdef\csname R@an.ablation.count.groups\endcsname{6}
\expandafter\gdef\csname R@an.ablation.count.killed\endcsname{3}
\expandafter\gdef\csname R@an.ablation.count.pending\endcsname{4}
\expandafter\gdef\csname R@an.ablation.count.poolref\endcsname{5}
\expandafter\gdef\csname R@an.ablation.count.pr_rows\endcsname{9}
\expandafter\gdef\csname R@an.ablation.count.read\endcsname{9}
\expandafter\gdef\csname R@an.ablation.count.rows\endcsname{13}
\expandafter\gdef\csname R@an.ablation.default.params_m\endcsname{31.12}
\expandafter\gdef\csname R@an.ablation.fig.ci_text\endcsname{an interval of $\pm$1.96 standard errors of that row's null (the normal approximation; the SD behind it is the frozen pool's, 6 runs on AMOS22 and 3 on KiTS23)}
\expandafter\gdef\csname R@an.ablation.fig.ci_z\endcsname{1.96}
\expandafter\gdef\csname R@an.ablation.fig.ribbon_sd\endcsname{2}
\expandafter\gdef\csname R@an.ablation.floor\endcsname{0.50}
\expandafter\gdef\csname R@an.ablation.lineage.dparams_max\endcsname{+76.9}
\expandafter\gdef\csname R@an.ablation.lineage.dparams_min\endcsname{-29.5}
\expandafter\gdef\csname R@an.ablation.lineage.step_max\endcsname{1.28}
\expandafter\gdef\csname R@an.ablation.lineage.step_min\endcsname{0.88}
\expandafter\gdef\csname R@an.ablation.parent.amos.all\endcsname{87.916}
\expandafter\gdef\csname R@an.ablation.parent.amos.fresh\endcsname{87.833}
\expandafter\gdef\csname R@an.ablation.parent.amos.fresh_d\endcsname{+0.132}
\expandafter\gdef\csname R@an.ablation.parent.amos.fresh_dunion\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.parent.amos.hi\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.parent.amos.lo\endcsname{87.686}
\expandafter\gdef\csname R@an.ablation.parent.amos.n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.parent.amos.s0\endcsname{88.083}
\expandafter\gdef\csname R@an.ablation.parent.amos.s0_minus_fresh\endcsname{+0.249}
\expandafter\gdef\csname R@an.ablation.parent.amos.s1\endcsname{87.981}
\expandafter\gdef\csname R@an.ablation.parent.amos.s2\endcsname{87.686}
\expandafter\gdef\csname R@an.ablation.parent.amos.se_all\endcsname{0.141}
\expandafter\gdef\csname R@an.ablation.parent.amos.se_fresh\endcsname{0.150}
\expandafter\gdef\csname R@an.ablation.parent.amos.span\endcsname{0.397}
\expandafter\gdef\csname R@an.ablation.parent.amos.top\endcsname{yes}
\expandafter\gdef\csname R@an.ablation.parent.kits.all\endcsname{85.721}
\expandafter\gdef\csname R@an.ablation.parent.kits.fresh\endcsname{85.472}
\expandafter\gdef\csname R@an.ablation.parent.kits.fresh_d\endcsname{+2.094}
\expandafter\gdef\csname R@an.ablation.parent.kits.fresh_dunion\endcsname{+1.850}
\expandafter\gdef\csname R@an.ablation.parent.kits.hi\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.parent.kits.lo\endcsname{85.176}
\expandafter\gdef\csname R@an.ablation.parent.kits.n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.parent.kits.s0\endcsname{86.220}
\expandafter\gdef\csname R@an.ablation.parent.kits.s0_minus_fresh\endcsname{+0.748}
\expandafter\gdef\csname R@an.ablation.parent.kits.s1\endcsname{85.176}
\expandafter\gdef\csname R@an.ablation.parent.kits.s2\endcsname{85.768}
\expandafter\gdef\csname R@an.ablation.parent.kits.se_all\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.parent.kits.se_fresh\endcsname{0.974}
\expandafter\gdef\csname R@an.ablation.parent.kits.span\endcsname{1.044}
\expandafter\gdef\csname R@an.ablation.parent.kits.top\endcsname{yes}
\expandafter\gdef\csname R@an.ablation.pr.amos.count.above\endcsname{2}
\expandafter\gdef\csname R@an.ablation.pr.amos.count.below\endcsname{0}
\expandafter\gdef\csname R@an.ablation.pr.amos.count.inside\endcsname{5}
\expandafter\gdef\csname R@an.ablation.pr.amos.count.n\endcsname{7}
\expandafter\gdef\csname R@an.ablation.pr.amos.count.pending\endcsname{0}
\expandafter\gdef\csname R@an.ablation.pr.amos.count.read\endcsname{7}
\expandafter\gdef\csname R@an.ablation.pr.amos.far.gap\endcsname{+0.078}
\expandafter\gdef\csname R@an.ablation.pr.amos.far.tag\endcsname{HyReX-k3}
\expandafter\gdef\csname R@an.ablation.pr.kits.count.above\endcsname{1}
\expandafter\gdef\csname R@an.ablation.pr.kits.count.below\endcsname{3}
\expandafter\gdef\csname R@an.ablation.pr.kits.count.inside\endcsname{3}
\expandafter\gdef\csname R@an.ablation.pr.kits.count.n\endcsname{7}
\expandafter\gdef\csname R@an.ablation.pr.kits.count.pending\endcsname{0}
\expandafter\gdef\csname R@an.ablation.pr.kits.count.read\endcsname{7}
\expandafter\gdef\csname R@an.ablation.pr.kits.far.gap\endcsname{+0.665}
\expandafter\gdef\csname R@an.ablation.pr.kits.far.tag\endcsname{C1}
\expandafter\gdef\csname R@an.ablation.ref.amos.contemp_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.ref.amos.contemp_shift\endcsname{+0.011}
\expandafter\gdef\csname R@an.ablation.ref.amos.floor_cross_p\endcsname{0.4}
\expandafter\gdef\csname R@an.ablation.ref.amos.floor_cross_p.def\endcsname{the probability that two networks of identical function, each trained at one seed, differ by more than the registered 0.50\,pp one-seed floor in either direction: the two-sided tail of a normal distribution centred on zero with standard deviation 0.173\,pp, which is the seed SD of the 6 frozen default runs of AMOS22 (0.122\,pp, 5 degrees of freedom, treated as known) times the square root of two}
\expandafter\gdef\csname R@an.ablation.ref.amos.floor_in_sepair\endcsname{2.89}
\expandafter\gdef\csname R@an.ablation.ref.amos.l3_3seed\endcsname{87.916}
\expandafter\gdef\csname R@an.ablation.ref.amos.mean\endcsname{87.701}
\expandafter\gdef\csname R@an.ablation.ref.amos.n\endcsname{6}
\expandafter\gdef\csname R@an.ablation.ref.amos.sd\endcsname{0.122}
\expandafter\gdef\csname R@an.ablation.ref.amos.sepair\endcsname{0.173}
\expandafter\gdef\csname R@an.ablation.ref.amos.sepool\endcsname{0.132}
\expandafter\gdef\csname R@an.ablation.ref.amos.unc_shift\endcsname{+0.029}
\expandafter\gdef\csname R@an.ablation.ref.amos.union_mean\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.ref.amos.union_n\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.ref.amos.union_sd\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.ref.amos.union_shift\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.ref.kits.contemp_n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.ref.kits.contemp_shift\endcsname{+0.487}
\expandafter\gdef\csname R@an.ablation.ref.kits.floor_cross_p\endcsname{66}
\expandafter\gdef\csname R@an.ablation.ref.kits.floor_cross_p.def\endcsname{the probability that two networks of identical function, each trained at one seed, differ by more than the registered 0.50\,pp one-seed floor in either direction: the two-sided tail of a normal distribution centred on zero with standard deviation 1.124\,pp, which is the seed SD of the 3 frozen default runs of KiTS23 (0.795\,pp, 2 degrees of freedom, treated as known) times the square root of two}
\expandafter\gdef\csname R@an.ablation.ref.kits.floor_in_sepair\endcsname{0.44}
\expandafter\gdef\csname R@an.ablation.ref.kits.l3_3seed\endcsname{85.721}
\expandafter\gdef\csname R@an.ablation.ref.kits.mean\endcsname{83.378}
\expandafter\gdef\csname R@an.ablation.ref.kits.n\endcsname{3}
\expandafter\gdef\csname R@an.ablation.ref.kits.sd\endcsname{0.795}
\expandafter\gdef\csname R@an.ablation.ref.kits.sepair\endcsname{1.124}
\expandafter\gdef\csname R@an.ablation.ref.kits.sepool\endcsname{0.918}
\expandafter\gdef\csname R@an.ablation.ref.kits.unc_shift\endcsname{n/a}
\expandafter\gdef\csname R@an.ablation.ref.kits.union_mean\endcsname{83.622}
\expandafter\gdef\csname R@an.ablation.ref.kits.union_n\endcsname{6}
\expandafter\gdef\csname R@an.ablation.ref.kits.union_sd\endcsname{0.722}
\expandafter\gdef\csname R@an.ablation.ref.kits.union_shift\endcsname{+0.244}
\expandafter\gdef\csname R@an.ablation.reg.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.ablation.screen\endcsname{+0.35}
\expandafter\gdef\csname R@an.ablation.sent.C1\endcsname{C1 (HyReX with a dense-residual coarse decoder) scores 88.09 on AMOS22 at seed 0, \ensuremath{+0.01}\,pp from HyReX's seed 0 (below the registered \ensuremath{+0.265}\,pp Tier-1 line), and 86.89 on KiTS23 at seed 0 (\ensuremath{+3.51}\,pp over the frozen 3-run pool, \ensuremath{+3.26}\,pp over the 6-run default reference), 0.67\,pp above the 85.18 to 86.22 range of HyReX's 3 seeds. C1 differs from HyReX in coarse-decoder composition and in parameter count together (52.34 M against HyReX's 29.59 M, \ensuremath{+76.9}\,\%), so no sign of the difference is attributed to a single factor.}
\expandafter\gdef\csname R@an.ablation.sent.C1.followup\endcsname{The registered kind-preserving follow-up of Addendum O4 applies to a difference from \ensuremath{+0.265}\,pp to 0.50\,pp, and C1's difference at seed 0 (\ensuremath{+0.01}\,pp) lies outside that band, so the follow-up is not triggered.}
\expandafter\gdef\csname R@an.ablation.sent.D2\endcsname{LeanDec, the nnU-Net default with one convolution per decoder stage (0.84$\times$ its parameters) scores 85.27 on KiTS23 over 2 fresh seeds, \ensuremath{+1.89}\,pp over the frozen 3-run pool (\ensuremath{+1.65}\,pp over the 6-run default reference) and \ensuremath{-0.20}\,pp against HyReX's fresh-seed mean, inside the 0.50\,pp resolution line; on AMOS22 its seed 0 scores 87.34, \ensuremath{-0.36}\,pp against the frozen pool, 0.35\,pp below the 87.69 to 88.08 range of HyReX's 3 seeds.}
\expandafter\gdef\csname R@an.ablation.sent.D2.attr\endcsname{LeanDec, a default-topology network with a thinned decoder and no new operator, scores 0.20\,pp below HyReX's fresh-seed mean on KiTS23, inside the 0.50\,pp resolution line; the KiTS23 gain therefore does not identify the operator assignment as its source.}
\expandafter\gdef\csname R@an.ablation.sent.L6\endcsname{HyReX+context scores 87.72 on AMOS22 at seed 0, inside the 87.69 to 88.08 range of HyReX's 3 seeds: \ensuremath{-0.37}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{-0.12}\,pp against its fresh-seed mean and \ensuremath{-0.20}\,pp against its 3-seed mean. HyReX+context scores 85.90 on KiTS23 at seed 0, inside the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{-0.32}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.43}\,pp against its fresh-seed mean and \ensuremath{+0.18}\,pp against its 3-seed mean. Over 2 fresh seeds on KiTS23 its mean is 84.97, \ensuremath{-0.50}\,pp against HyReX's fresh-seed mean, at 0.63 of the 0.795\,pp null SD of a difference between 2-seed means.}
\expandafter\gdef\csname R@an.ablation.sent.W1c\endcsname{The branch control (31.14 M parameters, the default network's size) scores 86.01 on KiTS23 at seed 0, inside the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{-0.21}\,pp against HyReX's seed 0 and \ensuremath{+0.54}\,pp against its fresh-seed mean; its fresh-seed mean is 84.44, \ensuremath{+1.07}\,pp over the frozen pool (\ensuremath{+0.82}\,pp over the 6-run default reference) and \ensuremath{-1.03}\,pp against HyReX's fresh-seed mean, beyond the 0.50\,pp resolution line (Addendum V3); on AMOS22 it scores 88.06 at seed 0, inside the 87.69 to 88.08 range of HyReX's 3 seeds.}
\expandafter\gdef\csname R@an.ablation.sent.attr\endcsname{HyReX w/o GRN reads \ensuremath{-0.11}\,pp against HyReX's seed 0 on AMOS22, inside the 87.69 to 88.08 range of HyReX's 3 seeds, inside the registered 0.50\,pp one-seed floor; HyReX-k3 reads \ensuremath{+0.08}\,pp against HyReX's seed 0 on AMOS22, 0.08\,pp above the 87.69 to 88.08 range of HyReX's 3 seeds, inside the registered 0.50\,pp one-seed floor. HyReX w/o GRN scores 85.94 on KiTS23 at seed 0, inside the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{-0.28}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.47}\,pp against its fresh-seed mean and \ensuremath{+0.22}\,pp against its 3-seed mean. HyReX-k3 scores 84.74 on KiTS23 at seed 0, 0.43\,pp below the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{-1.48}\,pp against HyReX's seed 0 (beyond the registered 0.50\,pp one-seed floor), \ensuremath{-0.73}\,pp against its fresh-seed mean and \ensuremath{-0.98}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.C1\endcsname{C1 (HyReX with a dense-residual coarse decoder) scores 88.09 on AMOS22 at seed 0, 0.01\,pp above the 87.69 to 88.08 range of HyReX's 3 seeds: \ensuremath{+0.01}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.26}\,pp against its fresh-seed mean and \ensuremath{+0.17}\,pp against its 3-seed mean. C1 (HyReX with a dense-residual coarse decoder) scores 86.89 on KiTS23 at seed 0, 0.67\,pp above the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{+0.67}\,pp against HyReX's seed 0 (beyond the registered 0.50\,pp one-seed floor), \ensuremath{+1.41}\,pp against its fresh-seed mean and \ensuremath{+1.16}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.C1.amos\endcsname{C1 (HyReX with a dense-residual coarse decoder) scores 88.09 on AMOS22 at seed 0, 0.01\,pp above the 87.69 to 88.08 range of HyReX's 3 seeds: \ensuremath{+0.01}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.26}\,pp against its fresh-seed mean and \ensuremath{+0.17}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.C1.amos.short\endcsname{C1 scores 88.09 on AMOS22 at seed 0, 0.01\,pp above HyReX's seed range: \ensuremath{+0.01}\,pp against seed 0 (inside the registered 0.50\,pp one-seed floor) and \ensuremath{+0.26}\,pp against HyReX's fresh-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.C1.kits\endcsname{C1 (HyReX with a dense-residual coarse decoder) scores 86.89 on KiTS23 at seed 0, 0.67\,pp above the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{+0.67}\,pp against HyReX's seed 0 (beyond the registered 0.50\,pp one-seed floor), \ensuremath{+1.41}\,pp against its fresh-seed mean and \ensuremath{+1.16}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.C1.kits.short\endcsname{C1 scores 86.89 on KiTS23 at seed 0, 0.67\,pp above HyReX's seed range: \ensuremath{+0.67}\,pp against seed 0 (beyond the registered 0.50\,pp one-seed floor) and \ensuremath{+1.41}\,pp against HyReX's fresh-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.C1.short\endcsname{At seed 0, C1 reads \ensuremath{+0.01}\,pp on AMOS22 (0.01\,pp above HyReX's seed range) and \ensuremath{+0.67}\,pp on KiTS23 (0.67\,pp above it) against HyReX's seed 0, inside the registered 0.50\,pp one-seed floor on AMOS22 and beyond it on KiTS23.}
\expandafter\gdef\csname R@an.ablation.sent.child.D1\endcsname{HyReX point-fuse decoder scores 87.98 on AMOS22 at seed 0, inside the 87.69 to 88.08 range of HyReX's 3 seeds: \ensuremath{-0.10}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.15}\,pp against its fresh-seed mean and \ensuremath{+0.06}\,pp against its 3-seed mean. HyReX point-fuse decoder scores 84.99 on KiTS23 at seed 0, 0.19\,pp below the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{-1.23}\,pp against HyReX's seed 0 (beyond the registered 0.50\,pp one-seed floor), \ensuremath{-0.49}\,pp against its fresh-seed mean and \ensuremath{-0.74}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.D1.amos\endcsname{HyReX point-fuse decoder scores 87.98 on AMOS22 at seed 0, inside the 87.69 to 88.08 range of HyReX's 3 seeds: \ensuremath{-0.10}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.15}\,pp against its fresh-seed mean and \ensuremath{+0.06}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.D1.amos.short\endcsname{HyReX point-fuse decoder scores 87.98 on AMOS22 at seed 0, inside HyReX's seed range: \ensuremath{-0.10}\,pp against seed 0 (inside the registered 0.50\,pp one-seed floor) and \ensuremath{+0.15}\,pp against HyReX's fresh-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.D1.kits\endcsname{HyReX point-fuse decoder scores 84.99 on KiTS23 at seed 0, 0.19\,pp below the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{-1.23}\,pp against HyReX's seed 0 (beyond the registered 0.50\,pp one-seed floor), \ensuremath{-0.49}\,pp against its fresh-seed mean and \ensuremath{-0.74}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.D1.kits.short\endcsname{HyReX point-fuse decoder scores 84.99 on KiTS23 at seed 0, 0.19\,pp below HyReX's seed range: \ensuremath{-1.23}\,pp against seed 0 (beyond the registered 0.50\,pp one-seed floor) and \ensuremath{-0.49}\,pp against HyReX's fresh-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.D1.short\endcsname{At seed 0, HyReX point-fuse decoder reads \ensuremath{-0.10}\,pp on AMOS22 (inside HyReX's seed range) and \ensuremath{-1.23}\,pp on KiTS23 (0.19\,pp below it) against HyReX's seed 0, inside the registered 0.50\,pp one-seed floor on AMOS22 and beyond it on KiTS23.}
\expandafter\gdef\csname R@an.ablation.sent.child.D2.amos\endcsname{LeanDec scores 87.34 on AMOS22 at seed 0, 0.35\,pp below the 87.69 to 88.08 range of HyReX's 3 seeds: \ensuremath{-0.74}\,pp against HyReX's seed 0 (beyond the registered 0.50\,pp one-seed floor), \ensuremath{-0.49}\,pp against its fresh-seed mean and \ensuremath{-0.58}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.D2.amos.short\endcsname{LeanDec scores 87.34 on AMOS22 at seed 0, 0.35\,pp below HyReX's seed range: \ensuremath{-0.74}\,pp against seed 0 (beyond the registered 0.50\,pp one-seed floor) and \ensuremath{-0.49}\,pp against HyReX's fresh-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.D2.kits\endcsname{LeanDec scores 85.73 on KiTS23 at seed 0, inside the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{-0.49}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.26}\,pp against its fresh-seed mean and \ensuremath{+0.01}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.D2.kits.short\endcsname{LeanDec scores 85.73 on KiTS23 at seed 0, inside HyReX's seed range: \ensuremath{-0.49}\,pp against seed 0 (inside the registered 0.50\,pp one-seed floor) and \ensuremath{+0.26}\,pp against HyReX's fresh-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.I1\endcsname{HyReX + pooled skip scores 88.00 on AMOS22 at seed 0, inside the 87.69 to 88.08 range of HyReX's 3 seeds: \ensuremath{-0.09}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.16}\,pp against its fresh-seed mean and \ensuremath{+0.08}\,pp against its 3-seed mean. HyReX + pooled skip scores 85.27 on KiTS23 at seed 0, inside the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{-0.95}\,pp against HyReX's seed 0 (beyond the registered 0.50\,pp one-seed floor), \ensuremath{-0.20}\,pp against its fresh-seed mean and \ensuremath{-0.45}\,pp against its 3-seed mean. The skip type is not separated from HyReX's own seeds at one seed on every co-primary read (2 of 2).}
\expandafter\gdef\csname R@an.ablation.sent.child.I1.amos\endcsname{HyReX + pooled skip scores 88.00 on AMOS22 at seed 0, inside the 87.69 to 88.08 range of HyReX's 3 seeds: \ensuremath{-0.09}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.16}\,pp against its fresh-seed mean and \ensuremath{+0.08}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.I1.amos.short\endcsname{HyReX + pooled skip scores 88.00 on AMOS22 at seed 0, inside HyReX's seed range: \ensuremath{-0.09}\,pp against seed 0 (inside the registered 0.50\,pp one-seed floor) and \ensuremath{+0.16}\,pp against HyReX's fresh-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.I1.kits\endcsname{HyReX + pooled skip scores 85.27 on KiTS23 at seed 0, inside the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{-0.95}\,pp against HyReX's seed 0 (beyond the registered 0.50\,pp one-seed floor), \ensuremath{-0.20}\,pp against its fresh-seed mean and \ensuremath{-0.45}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.I1.kits.short\endcsname{HyReX + pooled skip scores 85.27 on KiTS23 at seed 0, inside HyReX's seed range: \ensuremath{-0.95}\,pp against seed 0 (beyond the registered 0.50\,pp one-seed floor) and \ensuremath{-0.20}\,pp against HyReX's fresh-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.I1.short\endcsname{At seed 0, HyReX + pooled skip reads \ensuremath{-0.09}\,pp on AMOS22 and \ensuremath{-0.95}\,pp on KiTS23 against HyReX's seed 0, inside HyReX's seed range; inside the registered 0.50\,pp one-seed floor on AMOS22 and beyond it on KiTS23.}
\expandafter\gdef\csname R@an.ablation.sent.child.L3k3\endcsname{HyReX-k3 scores 88.16 on AMOS22 at seed 0, 0.08\,pp above the 87.69 to 88.08 range of HyReX's 3 seeds: \ensuremath{+0.08}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.33}\,pp against its fresh-seed mean and \ensuremath{+0.24}\,pp against its 3-seed mean. HyReX-k3 scores 84.74 on KiTS23 at seed 0, 0.43\,pp below the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{-1.48}\,pp against HyReX's seed 0 (beyond the registered 0.50\,pp one-seed floor), \ensuremath{-0.73}\,pp against its fresh-seed mean and \ensuremath{-0.98}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.L3k3.amos\endcsname{HyReX-k3 scores 88.16 on AMOS22 at seed 0, 0.08\,pp above the 87.69 to 88.08 range of HyReX's 3 seeds: \ensuremath{+0.08}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.33}\,pp against its fresh-seed mean and \ensuremath{+0.24}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.L3k3.amos.short\endcsname{HyReX-k3 scores 88.16 on AMOS22 at seed 0, 0.08\,pp above HyReX's seed range: \ensuremath{+0.08}\,pp against seed 0 (inside the registered 0.50\,pp one-seed floor) and \ensuremath{+0.33}\,pp against HyReX's fresh-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.L3k3.kits\endcsname{HyReX-k3 scores 84.74 on KiTS23 at seed 0, 0.43\,pp below the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{-1.48}\,pp against HyReX's seed 0 (beyond the registered 0.50\,pp one-seed floor), \ensuremath{-0.73}\,pp against its fresh-seed mean and \ensuremath{-0.98}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.L3k3.kits.short\endcsname{HyReX-k3 scores 84.74 on KiTS23 at seed 0, 0.43\,pp below HyReX's seed range: \ensuremath{-1.48}\,pp against seed 0 (beyond the registered 0.50\,pp one-seed floor) and \ensuremath{-0.73}\,pp against HyReX's fresh-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.L3k3.short\endcsname{At seed 0, HyReX-k3 reads \ensuremath{+0.08}\,pp on AMOS22 (0.08\,pp above HyReX's seed range) and \ensuremath{-1.48}\,pp on KiTS23 (0.43\,pp below it) against HyReX's seed 0, inside the registered 0.50\,pp one-seed floor on AMOS22 and beyond it on KiTS23.}
\expandafter\gdef\csname R@an.ablation.sent.child.L3ng\endcsname{HyReX w/o GRN scores 87.97 on AMOS22 at seed 0, inside the 87.69 to 88.08 range of HyReX's 3 seeds: \ensuremath{-0.11}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.14}\,pp against its fresh-seed mean and \ensuremath{+0.05}\,pp against its 3-seed mean. HyReX w/o GRN scores 85.94 on KiTS23 at seed 0, inside the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{-0.28}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.47}\,pp against its fresh-seed mean and \ensuremath{+0.22}\,pp against its 3-seed mean. The GRN factor is not separated from HyReX's own seeds at one seed on every co-primary read (2 of 2).}
\expandafter\gdef\csname R@an.ablation.sent.child.L3ng.amos\endcsname{HyReX w/o GRN scores 87.97 on AMOS22 at seed 0, inside the 87.69 to 88.08 range of HyReX's 3 seeds: \ensuremath{-0.11}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.14}\,pp against its fresh-seed mean and \ensuremath{+0.05}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.L3ng.amos.short\endcsname{HyReX w/o GRN scores 87.97 on AMOS22 at seed 0, inside HyReX's seed range: \ensuremath{-0.11}\,pp against seed 0 (inside the registered 0.50\,pp one-seed floor) and \ensuremath{+0.14}\,pp against HyReX's fresh-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.L3ng.kits\endcsname{HyReX w/o GRN scores 85.94 on KiTS23 at seed 0, inside the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{-0.28}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.47}\,pp against its fresh-seed mean and \ensuremath{+0.22}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.L3ng.kits.short\endcsname{HyReX w/o GRN scores 85.94 on KiTS23 at seed 0, inside HyReX's seed range: \ensuremath{-0.28}\,pp against seed 0 (inside the registered 0.50\,pp one-seed floor) and \ensuremath{+0.47}\,pp against HyReX's fresh-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.L3ng.short\endcsname{At seed 0, HyReX w/o GRN reads \ensuremath{-0.11}\,pp on AMOS22 and \ensuremath{-0.28}\,pp on KiTS23 against HyReX's seed 0, inside HyReX's seed range and the registered 0.50\,pp one-seed floor on each.}
\expandafter\gdef\csname R@an.ablation.sent.child.L6\endcsname{HyReX+context scores 87.72 on AMOS22 at seed 0, inside the 87.69 to 88.08 range of HyReX's 3 seeds: \ensuremath{-0.37}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{-0.12}\,pp against its fresh-seed mean and \ensuremath{-0.20}\,pp against its 3-seed mean. HyReX+context scores 85.90 on KiTS23 at seed 0, inside the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{-0.32}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.43}\,pp against its fresh-seed mean and \ensuremath{+0.18}\,pp against its 3-seed mean. The context bundle is not separated from HyReX's own seeds at one seed on every co-primary read (2 of 2).}
\expandafter\gdef\csname R@an.ablation.sent.child.L6.amos\endcsname{HyReX+context scores 87.72 on AMOS22 at seed 0, inside the 87.69 to 88.08 range of HyReX's 3 seeds: \ensuremath{-0.37}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{-0.12}\,pp against its fresh-seed mean and \ensuremath{-0.20}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.L6.amos.short\endcsname{HyReX+context scores 87.72 on AMOS22 at seed 0, inside HyReX's seed range: \ensuremath{-0.37}\,pp against seed 0 (inside the registered 0.50\,pp one-seed floor) and \ensuremath{-0.12}\,pp against HyReX's fresh-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.L6.kits\endcsname{HyReX+context scores 85.90 on KiTS23 at seed 0, inside the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{-0.32}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.43}\,pp against its fresh-seed mean and \ensuremath{+0.18}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.L6.kits.short\endcsname{HyReX+context scores 85.90 on KiTS23 at seed 0, inside HyReX's seed range: \ensuremath{-0.32}\,pp against seed 0 (inside the registered 0.50\,pp one-seed floor) and \ensuremath{+0.43}\,pp against HyReX's fresh-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.L6.short\endcsname{At seed 0, HyReX+context reads \ensuremath{-0.37}\,pp on AMOS22 and \ensuremath{-0.32}\,pp on KiTS23 against HyReX's seed 0, inside HyReX's seed range and the registered 0.50\,pp one-seed floor on each.}
\expandafter\gdef\csname R@an.ablation.sent.child.S2\endcsname{HyReX, ConvNeXt one stage finer scores 88.08 on AMOS22 at seed 0, inside the 87.69 to 88.08 range of HyReX's 3 seeds: \ensuremath{0.00}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.25}\,pp against its fresh-seed mean and \ensuremath{+0.16}\,pp against its 3-seed mean. HyReX, ConvNeXt one stage finer scores 84.72 on KiTS23 at seed 0, 0.46\,pp below the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{-1.50}\,pp against HyReX's seed 0 (beyond the registered 0.50\,pp one-seed floor), \ensuremath{-0.75}\,pp against its fresh-seed mean and \ensuremath{-1.00}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.S2.amos\endcsname{HyReX, ConvNeXt one stage finer scores 88.08 on AMOS22 at seed 0, inside the 87.69 to 88.08 range of HyReX's 3 seeds: \ensuremath{0.00}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.25}\,pp against its fresh-seed mean and \ensuremath{+0.16}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.S2.amos.short\endcsname{HyReX, ConvNeXt one stage finer scores 88.08 on AMOS22 at seed 0, inside HyReX's seed range: \ensuremath{0.00}\,pp against seed 0 (inside the registered 0.50\,pp one-seed floor) and \ensuremath{+0.25}\,pp against HyReX's fresh-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.S2.kits\endcsname{HyReX, ConvNeXt one stage finer scores 84.72 on KiTS23 at seed 0, 0.46\,pp below the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{-1.50}\,pp against HyReX's seed 0 (beyond the registered 0.50\,pp one-seed floor), \ensuremath{-0.75}\,pp against its fresh-seed mean and \ensuremath{-1.00}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.S2.kits.short\endcsname{HyReX, ConvNeXt one stage finer scores 84.72 on KiTS23 at seed 0, 0.46\,pp below HyReX's seed range: \ensuremath{-1.50}\,pp against seed 0 (beyond the registered 0.50\,pp one-seed floor) and \ensuremath{-0.75}\,pp against HyReX's fresh-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.S2.short\endcsname{At seed 0, HyReX, ConvNeXt one stage finer reads \ensuremath{0.00}\,pp on AMOS22 (inside HyReX's seed range) and \ensuremath{-1.50}\,pp on KiTS23 (0.46\,pp below it) against HyReX's seed 0, inside the registered 0.50\,pp one-seed floor on AMOS22 and beyond it on KiTS23.}
\expandafter\gdef\csname R@an.ablation.sent.child.W1c.amos\endcsname{The branch control scores 88.06 on AMOS22 at seed 0, inside the 87.69 to 88.08 range of HyReX's 3 seeds: \ensuremath{-0.02}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.23}\,pp against its fresh-seed mean and \ensuremath{+0.15}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.W1c.amos.short\endcsname{The branch control scores 88.06 on AMOS22 at seed 0, inside HyReX's seed range: \ensuremath{-0.02}\,pp against seed 0 (inside the registered 0.50\,pp one-seed floor) and \ensuremath{+0.23}\,pp against HyReX's fresh-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.W1c.kits\endcsname{The branch control scores 86.01 on KiTS23 at seed 0, inside the 85.18 to 86.22 range of HyReX's 3 seeds: \ensuremath{-0.21}\,pp against HyReX's seed 0 (inside the registered 0.50\,pp one-seed floor), \ensuremath{+0.54}\,pp against its fresh-seed mean and \ensuremath{+0.29}\,pp against its 3-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.child.W1c.kits.short\endcsname{The branch control scores 86.01 on KiTS23 at seed 0, inside HyReX's seed range: \ensuremath{-0.21}\,pp against seed 0 (inside the registered 0.50\,pp one-seed floor) and \ensuremath{+0.54}\,pp against HyReX's fresh-seed mean.}
\expandafter\gdef\csname R@an.ablation.sent.parent.amos\endcsname{On AMOS22, HyReX's 3 seeds span 87.69 to 88.08; the discovery seed, 88.08, is the highest of them and 0.25\,pp above the fresh-seed mean, 87.83.}
\expandafter\gdef\csname R@an.ablation.sent.parent.kits\endcsname{On KiTS23, HyReX's 3 seeds span 85.18 to 86.22; the discovery seed, 86.22, is the highest of them and 0.75\,pp above the fresh-seed mean, 85.47.}
\expandafter\gdef\csname R@an.ablation.sent.pool.C1.amos\endcsname{C1 (HyReX with a dense-residual coarse decoder) at seed 0 is \ensuremath{+0.39}\,pp over the frozen 6-run AMOS22 pool, \ensuremath{+0.36}\,pp over its uncompiled 3-run sub-pool and \ensuremath{+0.38}\,pp over the 3 contemporaneous default runs.}
\expandafter\gdef\csname R@an.ablation.sent.pool.C1.kits\endcsname{C1 (HyReX with a dense-residual coarse decoder) at seed 0 is \ensuremath{+3.51}\,pp over the frozen 3-run KiTS23 pool and \ensuremath{+3.26}\,pp over the 6-run default reference; the mean of its 2 fresh seeds is \ensuremath{+2.40}\,pp over the frozen pool and \ensuremath{+2.16}\,pp over the 6-run default reference.}
\expandafter\gdef\csname R@an.ablation.sent.pool.D1.amos\endcsname{HyReX point-fuse decoder at seed 0 is \ensuremath{+0.28}\,pp over the frozen 6-run AMOS22 pool, \ensuremath{+0.25}\,pp over its uncompiled 3-run sub-pool and \ensuremath{+0.27}\,pp over the 3 contemporaneous default runs.}
\expandafter\gdef\csname R@an.ablation.sent.pool.D1.kits\endcsname{HyReX point-fuse decoder at seed 0 is \ensuremath{+1.61}\,pp over the frozen 3-run KiTS23 pool and \ensuremath{+1.36}\,pp over the 6-run default reference; the mean of its 2 fresh seeds is \ensuremath{+1.48}\,pp over the frozen pool and \ensuremath{+1.23}\,pp over the 6-run default reference.}
\expandafter\gdef\csname R@an.ablation.sent.pool.D2.amos\endcsname{LeanDec at seed 0 is \ensuremath{-0.36}\,pp over the frozen 6-run AMOS22 pool, \ensuremath{-0.39}\,pp over its uncompiled 3-run sub-pool and \ensuremath{-0.37}\,pp over the 3 contemporaneous default runs.}
\expandafter\gdef\csname R@an.ablation.sent.pool.D2.kits\endcsname{LeanDec at seed 0 is \ensuremath{+2.36}\,pp over the frozen 3-run KiTS23 pool and \ensuremath{+2.11}\,pp over the 6-run default reference; the mean of its 2 fresh seeds is \ensuremath{+1.89}\,pp over the frozen pool and \ensuremath{+1.65}\,pp over the 6-run default reference.}
\expandafter\gdef\csname R@an.ablation.sent.pool.I1.amos\endcsname{HyReX + pooled skip at seed 0 is \ensuremath{+0.29}\,pp over the frozen 6-run AMOS22 pool, \ensuremath{+0.27}\,pp over its uncompiled 3-run sub-pool and \ensuremath{+0.28}\,pp over the 3 contemporaneous default runs.}
\expandafter\gdef\csname R@an.ablation.sent.pool.I1.kits\endcsname{HyReX + pooled skip at seed 0 is \ensuremath{+1.89}\,pp over the frozen 3-run KiTS23 pool and \ensuremath{+1.65}\,pp over the 6-run default reference.}
\expandafter\gdef\csname R@an.ablation.sent.pool.L3k3.amos\endcsname{HyReX-k3 at seed 0 is \ensuremath{+0.46}\,pp over the frozen 6-run AMOS22 pool, \ensuremath{+0.43}\,pp over its uncompiled 3-run sub-pool and \ensuremath{+0.45}\,pp over the 3 contemporaneous default runs.}
\expandafter\gdef\csname R@an.ablation.sent.pool.L3k3.kits\endcsname{HyReX-k3 at seed 0 is \ensuremath{+1.37}\,pp over the frozen 3-run KiTS23 pool and \ensuremath{+1.12}\,pp over the 6-run default reference.}
\expandafter\gdef\csname R@an.ablation.sent.pool.L3ng.amos\endcsname{HyReX w/o GRN at seed 0 is \ensuremath{+0.27}\,pp over the frozen 6-run AMOS22 pool, \ensuremath{+0.24}\,pp over its uncompiled 3-run sub-pool and \ensuremath{+0.26}\,pp over the 3 contemporaneous default runs.}
\expandafter\gdef\csname R@an.ablation.sent.pool.L3ng.kits\endcsname{HyReX w/o GRN at seed 0 is \ensuremath{+2.56}\,pp over the frozen 3-run KiTS23 pool and \ensuremath{+2.32}\,pp over the 6-run default reference.}
\expandafter\gdef\csname R@an.ablation.sent.pool.L6.amos\endcsname{HyReX+context at seed 0 is \ensuremath{+0.02}\,pp over the frozen 6-run AMOS22 pool, \ensuremath{-0.01}\,pp over its uncompiled 3-run sub-pool and \ensuremath{0.00}\,pp over the 3 contemporaneous default runs.}
\expandafter\gdef\csname R@an.ablation.sent.pool.L6.kits\endcsname{HyReX+context at seed 0 is \ensuremath{+2.53}\,pp over the frozen 3-run KiTS23 pool and \ensuremath{+2.28}\,pp over the 6-run default reference; the mean of its 2 fresh seeds is \ensuremath{+1.59}\,pp over the frozen pool and \ensuremath{+1.35}\,pp over the 6-run default reference.}
\expandafter\gdef\csname R@an.ablation.sent.pool.S2.amos\endcsname{HyReX, ConvNeXt one stage finer at seed 0 is \ensuremath{+0.38}\,pp over the frozen 6-run AMOS22 pool, \ensuremath{+0.35}\,pp over its uncompiled 3-run sub-pool and \ensuremath{+0.37}\,pp over the 3 contemporaneous default runs.}
\expandafter\gdef\csname R@an.ablation.sent.pool.S2.kits\endcsname{HyReX, ConvNeXt one stage finer at seed 0 is \ensuremath{+1.34}\,pp over the frozen 3-run KiTS23 pool and \ensuremath{+1.10}\,pp over the 6-run default reference; the mean of its 2 fresh seeds is \ensuremath{+0.57}\,pp over the frozen pool and \ensuremath{+0.33}\,pp over the 6-run default reference.}
\expandafter\gdef\csname R@an.ablation.sent.pool.W1c.amos\endcsname{The branch control at seed 0 is \ensuremath{+0.36}\,pp over the frozen 6-run AMOS22 pool, \ensuremath{+0.33}\,pp over its uncompiled 3-run sub-pool and \ensuremath{+0.35}\,pp over the 3 contemporaneous default runs.}
\expandafter\gdef\csname R@an.ablation.sent.pool.W1c.kits\endcsname{The branch control at seed 0 is \ensuremath{+2.64}\,pp over the frozen 3-run KiTS23 pool and \ensuremath{+2.39}\,pp over the 6-run default reference; the mean of its 2 fresh seeds is \ensuremath{+1.07}\,pp over the frozen pool and \ensuremath{+0.82}\,pp over the 6-run default reference.}
\expandafter\gdef\csname R@an.ablation.sent.summary.amos\endcsname{Of the 7 HyReX children read on AMOS22, 5 lie inside the range of HyReX's own seeds, 2 above it and 0 below it; the farthest outside is HyReX-k3 (0.08\,pp above the range).}
\expandafter\gdef\csname R@an.ablation.sent.summary.amos.short\endcsname{Of 7 HyReX children read on AMOS22, 5 lie inside the range of HyReX's own seeds, 2 above and 0 below; the farthest is HyReX-k3 (0.08\,pp above).}
\expandafter\gdef\csname R@an.ablation.sent.summary.kits\endcsname{Of the 7 HyReX children read on KiTS23, 3 lie inside the range of HyReX's own seeds, 1 above it and 3 below it; the farthest outside is C1 (0.67\,pp above the range).}
\expandafter\gdef\csname R@an.ablation.sent.summary.kits.short\endcsname{Of 7 HyReX children read on KiTS23, 3 lie inside the range of HyReX's own seeds, 1 above and 3 below; the farthest is C1 (0.67\,pp above).}
\expandafter\gdef\csname R@an.ablation.sent.v4.C1\endcsname{C1 (HyReX with a dense-residual coarse decoder) moved \ensuremath{-1.106}\,pp from its discovery seed to its fresh-seed mean on KiTS23, \ensuremath{-0.100}\,pp from the registered plug-in value \ensuremath{-1.006}\,pp, inside the registered band from \ensuremath{-5.436}\,pp to \ensuremath{+0.267}\,pp: it moved as the registered model predicts.}
\expandafter\gdef\csname R@an.ablation.sent.v4.W1c\endcsname{The branch control moved \ensuremath{-1.569}\,pp from its discovery seed to its fresh-seed mean on KiTS23, \ensuremath{-1.569}\,pp from the registered centre of the model, inside the registered band from \ensuremath{-2.837}\,pp to \ensuremath{+2.834}\,pp: it moved as the registered model predicts.}
\expandafter\gdef\csname R@an.ablation.sent.wh.c1_over_hyrex\endcsname{withheld}
\expandafter\gdef\csname R@an.ablation.sent.wh.component_below\endcsname{Below the range of HyReX's own seeds at one seed: HyReX-k3 on KiTS23; HyReX, ConvNeXt one stage finer on KiTS23; HyReX point-fuse decoder on KiTS23.}
\expandafter\gdef\csname R@an.ablation.sent.wh.leandec_label\endcsname{withheld}
\expandafter\gdef\csname R@an.ablation.sent.wh.operator_source\endcsname{withheld}
\expandafter\gdef\csname R@an.ablation.sent.wh.skip_load_bearing\endcsname{withheld}
\expandafter\gdef\csname R@an.ablation.tier1_gap\endcsname{+0.265}
\expandafter\gdef\csname R@an.ablation.v4.elig.hi\endcsname{+0.267}
\expandafter\gdef\csname R@an.ablation.v4.elig.lo\endcsname{-5.436}
\expandafter\gdef\csname R@an.ablation.v4.m\endcsname{6}
\expandafter\gdef\csname R@an.ablation.v4.never.hi\endcsname{+2.834}
\expandafter\gdef\csname R@an.ablation.v4.never.lo\endcsname{-2.837}
\expandafter\gdef\csname R@an.ablation.v4.plugin\endcsname{-1.006}
\expandafter\gdef\csname R@an.acdc_guard.acdc.fresh.L1.clause\endcsname{On the two fresh seeds, ResEnc-M's ACDC Dice is 92.268 and 92.234, a mean of 0.242 pp above the frozen default pool, so the ACDC gain is retained on fresh seeds.}
\expandafter\gdef\csname R@an.acdc_guard.acdc.fresh.L1.delta\endcsname{\ensuremath{+0.242}}
\expandafter\gdef\csname R@an.acdc_guard.acdc.fresh.L1.direction\endcsname{above}
\expandafter\gdef\csname R@an.acdc_guard.acdc.fresh.L1.mean\endcsname{92.251}
\expandafter\gdef\csname R@an.acdc_guard.acdc.fresh.L1.retained\endcsname{yes}
\expandafter\gdef\csname R@an.acdc_guard.acdc.fresh.L1.seed1\endcsname{92.268}
\expandafter\gdef\csname R@an.acdc_guard.acdc.fresh.L1.seed2\endcsname{92.234}
\expandafter\gdef\csname R@an.acdc_guard.acdc.fresh.L1.state\endcsname{landed}
\expandafter\gdef\csname R@an.acdc_guard.acdc.fresh.L3.clause\endcsname{On the two fresh seeds, HyReX's ACDC Dice is 92.426 and 92.493, a mean of 0.450 pp above the frozen default pool, so the ACDC gain is retained on fresh seeds.}
\expandafter\gdef\csname R@an.acdc_guard.acdc.fresh.L3.delta\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.acdc_guard.acdc.fresh.L3.direction\endcsname{above}
\expandafter\gdef\csname R@an.acdc_guard.acdc.fresh.L3.mean\endcsname{92.460}
\expandafter\gdef\csname R@an.acdc_guard.acdc.fresh.L3.retained\endcsname{yes}
\expandafter\gdef\csname R@an.acdc_guard.acdc.fresh.L3.seed1\endcsname{92.426}
\expandafter\gdef\csname R@an.acdc_guard.acdc.fresh.L3.seed2\endcsname{92.493}
\expandafter\gdef\csname R@an.acdc_guard.acdc.fresh.L3.state\endcsname{landed}
\expandafter\gdef\csname R@an.acdc_guard.acdc.fresh.all_landed\endcsname{yes}
\expandafter\gdef\csname R@an.acdc_guard.acdc.fresh.n_landed\endcsname{2}
\expandafter\gdef\csname R@an.acdc_guard.acdc.fresh.n_registered\endcsname{2}
\expandafter\gdef\csname R@an.acdc_guard.arm.L1.above_poolmax\endcsname{yes}
\expandafter\gdef\csname R@an.acdc_guard.arm.L1.delta\endcsname{\ensuremath{+0.336}}
\expandafter\gdef\csname R@an.acdc_guard.arm.L1.dice\endcsname{92.345}
\expandafter\gdef\csname R@an.acdc_guard.arm.L1.margin_poolmax\endcsname{\ensuremath{+0.217}}
\expandafter\gdef\csname R@an.acdc_guard.arm.L1.n_exceeded\endcsname{6}
\expandafter\gdef\csname R@an.acdc_guard.arm.L1b.above_poolmax\endcsname{yes}
\expandafter\gdef\csname R@an.acdc_guard.arm.L1b.delta\endcsname{\ensuremath{+0.283}}
\expandafter\gdef\csname R@an.acdc_guard.arm.L1b.dice\endcsname{92.293}
\expandafter\gdef\csname R@an.acdc_guard.arm.L1b.margin_poolmax\endcsname{\ensuremath{+0.164}}
\expandafter\gdef\csname R@an.acdc_guard.arm.L1b.n_exceeded\endcsname{6}
\expandafter\gdef\csname R@an.acdc_guard.arm.L2.above_poolmax\endcsname{no}
\expandafter\gdef\csname R@an.acdc_guard.arm.L2.delta\endcsname{\ensuremath{-0.015}}
\expandafter\gdef\csname R@an.acdc_guard.arm.L2.dice\endcsname{91.995}
\expandafter\gdef\csname R@an.acdc_guard.arm.L2.margin_poolmax\endcsname{\ensuremath{-0.134}}
\expandafter\gdef\csname R@an.acdc_guard.arm.L2.n_exceeded\endcsname{3}
\expandafter\gdef\csname R@an.acdc_guard.arm.L3.above_poolmax\endcsname{yes}
\expandafter\gdef\csname R@an.acdc_guard.arm.L3.delta\endcsname{\ensuremath{+0.616}}
\expandafter\gdef\csname R@an.acdc_guard.arm.L3.dice\endcsname{92.626}
\expandafter\gdef\csname R@an.acdc_guard.arm.L3.margin_poolmax\endcsname{\ensuremath{+0.497}}
\expandafter\gdef\csname R@an.acdc_guard.arm.L3.n_exceeded\endcsname{6}
\expandafter\gdef\csname R@an.acdc_guard.arm.L4.above_poolmax\endcsname{yes}
\expandafter\gdef\csname R@an.acdc_guard.arm.L4.delta\endcsname{\ensuremath{+0.315}}
\expandafter\gdef\csname R@an.acdc_guard.arm.L4.dice\endcsname{92.325}
\expandafter\gdef\csname R@an.acdc_guard.arm.L4.margin_poolmax\endcsname{\ensuremath{+0.196}}
\expandafter\gdef\csname R@an.acdc_guard.arm.L4.n_exceeded\endcsname{6}
\expandafter\gdef\csname R@an.acdc_guard.arm.L6.above_poolmax\endcsname{yes}
\expandafter\gdef\csname R@an.acdc_guard.arm.L6.delta\endcsname{\ensuremath{+0.451}}
\expandafter\gdef\csname R@an.acdc_guard.arm.L6.dice\endcsname{92.461}
\expandafter\gdef\csname R@an.acdc_guard.arm.L6.margin_poolmax\endcsname{\ensuremath{+0.332}}
\expandafter\gdef\csname R@an.acdc_guard.arm.L6.n_exceeded\endcsname{6}
\expandafter\gdef\csname R@an.acdc_guard.arm.P3c.above_poolmax\endcsname{no}
\expandafter\gdef\csname R@an.acdc_guard.arm.P3c.delta\endcsname{\ensuremath{-0.013}}
\expandafter\gdef\csname R@an.acdc_guard.arm.P3c.dice\endcsname{91.997}
\expandafter\gdef\csname R@an.acdc_guard.arm.P3c.margin_poolmax\endcsname{\ensuremath{-0.132}}
\expandafter\gdef\csname R@an.acdc_guard.arm.P3c.n_exceeded\endcsname{3}
\expandafter\gdef\csname R@an.acdc_guard.arm.V5B2.above_poolmax\endcsname{no}
\expandafter\gdef\csname R@an.acdc_guard.arm.V5B2.delta\endcsname{\ensuremath{-0.181}}
\expandafter\gdef\csname R@an.acdc_guard.arm.V5B2.dice\endcsname{91.828}
\expandafter\gdef\csname R@an.acdc_guard.arm.V5B2.margin_poolmax\endcsname{\ensuremath{-0.300}}
\expandafter\gdef\csname R@an.acdc_guard.arm.V5B2.n_exceeded\endcsname{0}
\expandafter\gdef\csname R@an.acdc_guard.arm.V6A1r.above_poolmax\endcsname{yes}
\expandafter\gdef\csname R@an.acdc_guard.arm.V6A1r.delta\endcsname{\ensuremath{+0.573}}
\expandafter\gdef\csname R@an.acdc_guard.arm.V6A1r.dice\endcsname{92.582}
\expandafter\gdef\csname R@an.acdc_guard.arm.V6A1r.margin_poolmax\endcsname{\ensuremath{+0.454}}
\expandafter\gdef\csname R@an.acdc_guard.arm.V6A1r.n_exceeded\endcsname{6}
\expandafter\gdef\csname R@an.acdc_guard.arm.V7A1.above_poolmax\endcsname{yes}
\expandafter\gdef\csname R@an.acdc_guard.arm.V7A1.delta\endcsname{\ensuremath{+0.229}}
\expandafter\gdef\csname R@an.acdc_guard.arm.V7A1.dice\endcsname{92.238}
\expandafter\gdef\csname R@an.acdc_guard.arm.V7A1.margin_poolmax\endcsname{\ensuremath{+0.110}}
\expandafter\gdef\csname R@an.acdc_guard.arm.V7A1.n_exceeded\endcsname{6}
\expandafter\gdef\csname R@an.acdc_guard.arm.V7A2.above_poolmax\endcsname{yes}
\expandafter\gdef\csname R@an.acdc_guard.arm.V7A2.delta\endcsname{\ensuremath{+0.362}}
\expandafter\gdef\csname R@an.acdc_guard.arm.V7A2.dice\endcsname{92.371}
\expandafter\gdef\csname R@an.acdc_guard.arm.V7A2.margin_poolmax\endcsname{\ensuremath{+0.243}}
\expandafter\gdef\csname R@an.acdc_guard.arm.V7A2.n_exceeded\endcsname{6}
\expandafter\gdef\csname R@an.acdc_guard.arm.V7C1.above_poolmax\endcsname{no}
\expandafter\gdef\csname R@an.acdc_guard.arm.V7C1.delta\endcsname{\ensuremath{-0.252}}
\expandafter\gdef\csname R@an.acdc_guard.arm.V7C1.dice\endcsname{91.757}
\expandafter\gdef\csname R@an.acdc_guard.arm.V7C1.margin_poolmax\endcsname{\ensuremath{-0.372}}
\expandafter\gdef\csname R@an.acdc_guard.arm.V7C1.n_exceeded\endcsname{0}
\expandafter\gdef\csname R@an.acdc_guard.d\endcsname{+0.616}
\expandafter\gdef\csname R@an.acdc_guard.dice\endcsname{92.626}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.arms_above\endcsname{HyReX, ResEnc-M, ResEnc-matched, ResEnc+context, HyReX+context, LeanDeepMid+FD, LeanDeepMid and HyReX-k9}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.arms_not_above\endcsname{ConvNeXt-k3, fn.-identical control, LeanAdd-NeXt and LeanNeXt-s5}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.clause\endcsname{On ACDC, HyReX's seed-0 Dice, 92.626, is above the largest of the 6 frozen default runs (91.853 to 92.128), outside the default's run-to-run range. 7 of the other 11 evaluated arms (ResEnc-M, ResEnc-matched, ResEnc+context, HyReX+context, LeanDeepMid+FD, LeanDeepMid and HyReX-k9) are above every default run on ACDC as well.}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.clause.range\endcsname{On ACDC, HyReX's seed-0 Dice, 92.626, is above the largest of the 6 frozen default runs (91.853 to 92.128), outside the default's run-to-run range.}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.clause.shared\endcsname{7 of the other 11 evaluated arms (ResEnc-M, ResEnc-matched, ResEnc+context, HyReX+context, LeanDeepMid+FD, LeanDeepMid and HyReX-k9) are above every default run on ACDC as well.}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.clause.unc\endcsname{HyReX's ACDC seed-0 Dice is also above the largest of the 3 uncompiled default runs (92.097), the like-for-like reference for an uncompiled design.}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.hero_above\endcsname{yes}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.max\endcsname{92.128}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.min\endcsname{91.853}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.n_above\endcsname{8}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.n_arms\endcsname{12}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.n_not_above\endcsname{4}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.n_others\endcsname{11}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.n_others_above\endcsname{7}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.n_pool\endcsname{6}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.others_above\endcsname{ResEnc-M, ResEnc-matched, ResEnc+context, HyReX+context, LeanDeepMid+FD, LeanDeepMid and HyReX-k9}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.range\endcsname{0.275}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.unc.hero_above\endcsname{yes}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.unc.max\endcsname{92.097}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.unc.n\endcsname{3}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.unc.n_above\endcsname{8}
\expandafter\gdef\csname R@an.acdc_guard.poolmax.unique_to_L3\endcsname{no}
\expandafter\gdef\csname R@an.acdc_guard.struct.all_largest\endcsname{no}
\expandafter\gdef\csname R@an.acdc_guard.struct.c1.largest\endcsname{no}
\expandafter\gdef\csname R@an.acdc_guard.struct.c1.margin\endcsname{\ensuremath{-0.130}}
\expandafter\gdef\csname R@an.acdc_guard.struct.c1.name\endcsname{RV}
\expandafter\gdef\csname R@an.acdc_guard.struct.c1.rank\endcsname{2}
\expandafter\gdef\csname R@an.acdc_guard.struct.c1.runner\endcsname{HyReX-k9}
\expandafter\gdef\csname R@an.acdc_guard.struct.c1.runner_pp\endcsname{\ensuremath{+1.397}}
\expandafter\gdef\csname R@an.acdc_guard.struct.c2.largest\endcsname{yes}
\expandafter\gdef\csname R@an.acdc_guard.struct.c2.margin\endcsname{0.050}
\expandafter\gdef\csname R@an.acdc_guard.struct.c2.name\endcsname{MLV}
\expandafter\gdef\csname R@an.acdc_guard.struct.c2.rank\endcsname{1}
\expandafter\gdef\csname R@an.acdc_guard.struct.c2.runner\endcsname{HyReX-k9}
\expandafter\gdef\csname R@an.acdc_guard.struct.c2.runner_pp\endcsname{\ensuremath{+0.307}}
\expandafter\gdef\csname R@an.acdc_guard.struct.c3.largest\endcsname{yes}
\expandafter\gdef\csname R@an.acdc_guard.struct.c3.margin\endcsname{0.119}
\expandafter\gdef\csname R@an.acdc_guard.struct.c3.name\endcsname{LVC}
\expandafter\gdef\csname R@an.acdc_guard.struct.c3.rank\endcsname{1}
\expandafter\gdef\csname R@an.acdc_guard.struct.c3.runner\endcsname{LeanDeepMid}
\expandafter\gdef\csname R@an.acdc_guard.struct.c3.runner_pp\endcsname{\ensuremath{+0.106}}
\expandafter\gdef\csname R@an.acdc_guard.struct.clause\endcsname{HyReX records the largest discovery-seed gain of the 12 arms with a finished ACDC run on 2 of the 3 ACDC structures (MLV and LVC) and ranks second on RV}
\expandafter\gdef\csname R@an.acdc_guard.struct.n\endcsname{3}
\expandafter\gdef\csname R@an.acdc_guard.struct.n_largest\endcsname{2}
\expandafter\gdef\csname R@an.acdc_guard.struct.names\endcsname{RV, MLV and LVC}
\expandafter\gdef\csname R@an.acdc_guard.struct.runners\endcsname{LeanDeepMid and HyReX-k9}
\expandafter\gdef\csname R@an.arch_profile.C1.acdc.act\endcsname{857}
\expandafter\gdef\csname R@an.arch_profile.C1.acdc.dwshare\endcsname{0.20}
\expandafter\gdef\csname R@an.arch_profile.C1.acdc.gmac\endcsname{518.8}
\expandafter\gdef\csname R@an.arch_profile.C1.acdc.params\endcsname{51.59}
\expandafter\gdef\csname R@an.arch_profile.C1.acdc.paramsexact\endcsname{51\,591\,636}
\expandafter\gdef\csname R@an.arch_profile.C1.acdc.peak\endcsname{10.26}
\expandafter\gdef\csname R@an.arch_profile.C1.acdc.step\endcsname{256.2}
\expandafter\gdef\csname R@an.arch_profile.C1.amos.act\endcsname{1483}
\expandafter\gdef\csname R@an.arch_profile.C1.amos.dwshare\endcsname{0.14}
\expandafter\gdef\csname R@an.arch_profile.C1.amos.gmac\endcsname{864.9}
\expandafter\gdef\csname R@an.arch_profile.C1.amos.params\endcsname{52.34}
\expandafter\gdef\csname R@an.arch_profile.C1.amos.paramsexact\endcsname{52\,338\,576}
\expandafter\gdef\csname R@an.arch_profile.C1.amos.peak\endcsname{11.14}
\expandafter\gdef\csname R@an.arch_profile.C1.amos.step\endcsname{237.7}
\expandafter\gdef\csname R@an.arch_profile.C1.kits.act\endcsname{1146}
\expandafter\gdef\csname R@an.arch_profile.C1.kits.dwshare\endcsname{0.10}
\expandafter\gdef\csname R@an.arch_profile.C1.kits.gmac\endcsname{657.6}
\expandafter\gdef\csname R@an.arch_profile.C1.kits.params\endcsname{52.41}
\expandafter\gdef\csname R@an.arch_profile.C1.kits.paramsexact\endcsname{52\,410\,607}
\expandafter\gdef\csname R@an.arch_profile.C1.kits.peak\endcsname{9.08}
\expandafter\gdef\csname R@an.arch_profile.C1.kits.step\endcsname{194.8}
\expandafter\gdef\csname R@an.arch_profile.D1.acdc.act\endcsname{829}
\expandafter\gdef\csname R@an.arch_profile.D1.acdc.dwshare\endcsname{0.32}
\expandafter\gdef\csname R@an.arch_profile.D1.acdc.gmac\endcsname{412.7}
\expandafter\gdef\csname R@an.arch_profile.D1.acdc.params\endcsname{20.11}
\expandafter\gdef\csname R@an.arch_profile.D1.acdc.paramsexact\endcsname{20\,112\,724}
\expandafter\gdef\csname R@an.arch_profile.D1.acdc.peak\endcsname{10.37}
\expandafter\gdef\csname R@an.arch_profile.D1.acdc.step\endcsname{232.0}
\expandafter\gdef\csname R@an.arch_profile.D1.amos.act\endcsname{1438}
\expandafter\gdef\csname R@an.arch_profile.D1.amos.dwshare\endcsname{0.22}
\expandafter\gdef\csname R@an.arch_profile.D1.amos.gmac\endcsname{700.8}
\expandafter\gdef\csname R@an.arch_profile.D1.amos.params\endcsname{20.86}
\expandafter\gdef\csname R@an.arch_profile.D1.amos.paramsexact\endcsname{20\,859\,664}
\expandafter\gdef\csname R@an.arch_profile.D1.amos.peak\endcsname{10.69}
\expandafter\gdef\csname R@an.arch_profile.D1.amos.step\endcsname{213.4}
\expandafter\gdef\csname R@an.arch_profile.D1.kits.act\endcsname{1122}
\expandafter\gdef\csname R@an.arch_profile.D1.kits.dwshare\endcsname{0.15}
\expandafter\gdef\csname R@an.arch_profile.D1.kits.gmac\endcsname{570.1}
\expandafter\gdef\csname R@an.arch_profile.D1.kits.params\endcsname{20.93}
\expandafter\gdef\csname R@an.arch_profile.D1.kits.paramsexact\endcsname{20\,931\,695}
\expandafter\gdef\csname R@an.arch_profile.D1.kits.peak\endcsname{9.51}
\expandafter\gdef\csname R@an.arch_profile.D1.kits.step\endcsname{172.8}
\expandafter\gdef\csname R@an.arch_profile.D2.acdc.act\endcsname{434}
\expandafter\gdef\csname R@an.arch_profile.D2.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.D2.acdc.gmac\endcsname{246.2}
\expandafter\gdef\csname R@an.arch_profile.D2.acdc.params\endcsname{25.28}
\expandafter\gdef\csname R@an.arch_profile.D2.acdc.paramsexact\endcsname{25\,278\,580}
\expandafter\gdef\csname R@an.arch_profile.D2.acdc.peak\endcsname{9.45}
\expandafter\gdef\csname R@an.arch_profile.D2.acdc.step\endcsname{114.4}
\expandafter\gdef\csname R@an.arch_profile.D2.amos.act\endcsname{772}
\expandafter\gdef\csname R@an.arch_profile.D2.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.D2.amos.gmac\endcsname{411.1}
\expandafter\gdef\csname R@an.arch_profile.D2.amos.params\endcsname{26.03}
\expandafter\gdef\csname R@an.arch_profile.D2.amos.paramsexact\endcsname{26\,025\,520}
\expandafter\gdef\csname R@an.arch_profile.D2.amos.peak\endcsname{8.14}
\expandafter\gdef\csname R@an.arch_profile.D2.amos.step\endcsname{114.0}
\expandafter\gdef\csname R@an.arch_profile.D2.kits.act\endcsname{632}
\expandafter\gdef\csname R@an.arch_profile.D2.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.D2.kits.gmac\endcsname{367.2}
\expandafter\gdef\csname R@an.arch_profile.D2.kits.params\endcsname{26.08}
\expandafter\gdef\csname R@an.arch_profile.D2.kits.paramsexact\endcsname{26\,079\,119}
\expandafter\gdef\csname R@an.arch_profile.D2.kits.peak\endcsname{7.76}
\expandafter\gdef\csname R@an.arch_profile.D2.kits.step\endcsname{99.6}
\expandafter\gdef\csname R@an.arch_profile.I1.acdc.act\endcsname{829}
\expandafter\gdef\csname R@an.arch_profile.I1.acdc.dwshare\endcsname{0.30}
\expandafter\gdef\csname R@an.arch_profile.I1.acdc.gmac\endcsname{433.9}
\expandafter\gdef\csname R@an.arch_profile.I1.acdc.params\endcsname{28.85}
\expandafter\gdef\csname R@an.arch_profile.I1.acdc.paramsexact\endcsname{28\,845\,396}
\expandafter\gdef\csname R@an.arch_profile.I1.acdc.peak\endcsname{10.52}
\expandafter\gdef\csname R@an.arch_profile.I1.acdc.step\endcsname{233.3}
\expandafter\gdef\csname R@an.arch_profile.I1.amos.act\endcsname{1438}
\expandafter\gdef\csname R@an.arch_profile.I1.amos.dwshare\endcsname{0.21}
\expandafter\gdef\csname R@an.arch_profile.I1.amos.gmac\endcsname{732.1}
\expandafter\gdef\csname R@an.arch_profile.I1.amos.params\endcsname{29.59}
\expandafter\gdef\csname R@an.arch_profile.I1.amos.paramsexact\endcsname{29\,592\,336}
\expandafter\gdef\csname R@an.arch_profile.I1.amos.peak\endcsname{10.83}
\expandafter\gdef\csname R@an.arch_profile.I1.amos.step\endcsname{215.5}
\expandafter\gdef\csname R@an.arch_profile.I1.kits.act\endcsname{1122}
\expandafter\gdef\csname R@an.arch_profile.I1.kits.dwshare\endcsname{0.14}
\expandafter\gdef\csname R@an.arch_profile.I1.kits.gmac\endcsname{586.8}
\expandafter\gdef\csname R@an.arch_profile.I1.kits.params\endcsname{29.66}
\expandafter\gdef\csname R@an.arch_profile.I1.kits.paramsexact\endcsname{29\,664\,367}
\expandafter\gdef\csname R@an.arch_profile.I1.kits.peak\endcsname{9.61}
\expandafter\gdef\csname R@an.arch_profile.I1.kits.step\endcsname{173.5}
\expandafter\gdef\csname R@an.arch_profile.L1.acdc.act\endcsname{790}
\expandafter\gdef\csname R@an.arch_profile.L1.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.L1.acdc.gmac\endcsname{597.8}
\expandafter\gdef\csname R@an.arch_profile.L1.acdc.params\endcsname{101.53}
\expandafter\gdef\csname R@an.arch_profile.L1.acdc.paramsexact\endcsname{101\,531\,604}
\expandafter\gdef\csname R@an.arch_profile.L1.acdc.peak\endcsname{10.46}
\expandafter\gdef\csname R@an.arch_profile.L1.acdc.step\endcsname{214.2}
\expandafter\gdef\csname R@an.arch_profile.L1.amos.act\endcsname{1373}
\expandafter\gdef\csname R@an.arch_profile.L1.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.L1.amos.gmac\endcsname{977.3}
\expandafter\gdef\csname R@an.arch_profile.L1.amos.params\endcsname{102.28}
\expandafter\gdef\csname R@an.arch_profile.L1.amos.paramsexact\endcsname{102\,278\,544}
\expandafter\gdef\csname R@an.arch_profile.L1.amos.peak\endcsname{10.93}
\expandafter\gdef\csname R@an.arch_profile.L1.amos.step\endcsname{205.3}
\expandafter\gdef\csname R@an.arch_profile.L1.kits.act\endcsname{1020}
\expandafter\gdef\csname R@an.arch_profile.L1.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.L1.kits.gmac\endcsname{717.5}
\expandafter\gdef\csname R@an.arch_profile.L1.kits.params\endcsname{102.35}
\expandafter\gdef\csname R@an.arch_profile.L1.kits.paramsexact\endcsname{102\,350\,575}
\expandafter\gdef\csname R@an.arch_profile.L1.kits.peak\endcsname{9.73}
\expandafter\gdef\csname R@an.arch_profile.L1.kits.step\endcsname{164.6}
\expandafter\gdef\csname R@an.arch_profile.L1b.acdc.act\endcsname{790}
\expandafter\gdef\csname R@an.arch_profile.L1b.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.L1b.acdc.gmac\endcsname{587.3}
\expandafter\gdef\csname R@an.arch_profile.L1b.acdc.params\endcsname{101.63}
\expandafter\gdef\csname R@an.arch_profile.L1b.acdc.paramsexact\endcsname{101\,626\,548}
\expandafter\gdef\csname R@an.arch_profile.L1b.acdc.peak\endcsname{10.56}
\expandafter\gdef\csname R@an.arch_profile.L1b.acdc.step\endcsname{200.1}
\expandafter\gdef\csname R@an.arch_profile.L1b.amos.act\endcsname{1374}
\expandafter\gdef\csname R@an.arch_profile.L1b.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.L1b.amos.gmac\endcsname{959.3}
\expandafter\gdef\csname R@an.arch_profile.L1b.amos.params\endcsname{102.37}
\expandafter\gdef\csname R@an.arch_profile.L1b.amos.paramsexact\endcsname{102\,373\,488}
\expandafter\gdef\csname R@an.arch_profile.L1b.amos.peak\endcsname{10.60}
\expandafter\gdef\csname R@an.arch_profile.L1b.amos.step\endcsname{193.8}
\expandafter\gdef\csname R@an.arch_profile.L1b.kits.act\endcsname{1020}
\expandafter\gdef\csname R@an.arch_profile.L1b.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.L1b.kits.gmac\endcsname{659.6}
\expandafter\gdef\csname R@an.arch_profile.L1b.kits.params\endcsname{102.43}
\expandafter\gdef\csname R@an.arch_profile.L1b.kits.paramsexact\endcsname{102\,427\,087}
\expandafter\gdef\csname R@an.arch_profile.L1b.kits.peak\endcsname{9.43}
\expandafter\gdef\csname R@an.arch_profile.L1b.kits.step\endcsname{151.3}
\expandafter\gdef\csname R@an.arch_profile.L2.acdc.act\endcsname{914}
\expandafter\gdef\csname R@an.arch_profile.L2.acdc.dwshare\endcsname{0.88}
\expandafter\gdef\csname R@an.arch_profile.L2.acdc.gmac\endcsname{230.9}
\expandafter\gdef\csname R@an.arch_profile.L2.acdc.params\endcsname{23.68}
\expandafter\gdef\csname R@an.arch_profile.L2.acdc.paramsexact\endcsname{23\,682\,132}
\expandafter\gdef\csname R@an.arch_profile.L2.acdc.peak\endcsname{11.42}
\expandafter\gdef\csname R@an.arch_profile.L2.acdc.step\endcsname{213.3}
\expandafter\gdef\csname R@an.arch_profile.L2.amos.act\endcsname{1586}
\expandafter\gdef\csname R@an.arch_profile.L2.amos.dwshare\endcsname{0.89}
\expandafter\gdef\csname R@an.arch_profile.L2.amos.gmac\endcsname{385.5}
\expandafter\gdef\csname R@an.arch_profile.L2.amos.params\endcsname{24.43}
\expandafter\gdef\csname R@an.arch_profile.L2.amos.paramsexact\endcsname{24\,429\,072}
\expandafter\gdef\csname R@an.arch_profile.L2.amos.peak\endcsname{9.93}
\expandafter\gdef\csname R@an.arch_profile.L2.amos.step\endcsname{205.4}
\expandafter\gdef\csname R@an.arch_profile.L2.kits.act\endcsname{1200}
\expandafter\gdef\csname R@an.arch_profile.L2.kits.dwshare\endcsname{0.46}
\expandafter\gdef\csname R@an.arch_profile.L2.kits.gmac\endcsname{401.9}
\expandafter\gdef\csname R@an.arch_profile.L2.kits.params\endcsname{24.50}
\expandafter\gdef\csname R@an.arch_profile.L2.kits.paramsexact\endcsname{24\,501\,103}
\expandafter\gdef\csname R@an.arch_profile.L2.kits.peak\endcsname{9.12}
\expandafter\gdef\csname R@an.arch_profile.L2.kits.step\endcsname{164.0}
\expandafter\gdef\csname R@an.arch_profile.L3.acdc.act\endcsname{829}
\expandafter\gdef\csname R@an.arch_profile.L3.acdc.dwshare\endcsname{0.30}
\expandafter\gdef\csname R@an.arch_profile.L3.acdc.gmac\endcsname{433.9}
\expandafter\gdef\csname R@an.arch_profile.L3.acdc.params\endcsname{28.85}
\expandafter\gdef\csname R@an.arch_profile.L3.acdc.paramsexact\endcsname{28\,845\,396}
\expandafter\gdef\csname R@an.arch_profile.L3.acdc.peak\endcsname{10.43}
\expandafter\gdef\csname R@an.arch_profile.L3.acdc.step\endcsname{233.1}
\expandafter\gdef\csname R@an.arch_profile.L3.amos.act\endcsname{1438}
\expandafter\gdef\csname R@an.arch_profile.L3.amos.dwshare\endcsname{0.21}
\expandafter\gdef\csname R@an.arch_profile.L3.amos.gmac\endcsname{732.1}
\expandafter\gdef\csname R@an.arch_profile.L3.amos.params\endcsname{29.59}
\expandafter\gdef\csname R@an.arch_profile.L3.amos.paramsexact\endcsname{29\,592\,336}
\expandafter\gdef\csname R@an.arch_profile.L3.amos.peak\endcsname{10.74}
\expandafter\gdef\csname R@an.arch_profile.L3.amos.step\endcsname{214.5}
\expandafter\gdef\csname R@an.arch_profile.L3.kits.act\endcsname{1122}
\expandafter\gdef\csname R@an.arch_profile.L3.kits.dwshare\endcsname{0.14}
\expandafter\gdef\csname R@an.arch_profile.L3.kits.gmac\endcsname{586.8}
\expandafter\gdef\csname R@an.arch_profile.L3.kits.params\endcsname{29.66}
\expandafter\gdef\csname R@an.arch_profile.L3.kits.paramsexact\endcsname{29\,664\,367}
\expandafter\gdef\csname R@an.arch_profile.L3.kits.peak\endcsname{9.56}
\expandafter\gdef\csname R@an.arch_profile.L3.kits.step\endcsname{172.7}
\expandafter\gdef\csname R@an.arch_profile.L3k3.acdc.act\endcsname{829}
\expandafter\gdef\csname R@an.arch_profile.L3k3.acdc.dwshare\endcsname{0.04}
\expandafter\gdef\csname R@an.arch_profile.L3k3.acdc.gmac\endcsname{432.8}
\expandafter\gdef\csname R@an.arch_profile.L3k3.acdc.params\endcsname{27.83}
\expandafter\gdef\csname R@an.arch_profile.L3k3.acdc.paramsexact\endcsname{27\,834\,964}
\expandafter\gdef\csname R@an.arch_profile.L3k3.acdc.peak\endcsname{10.42}
\expandafter\gdef\csname R@an.arch_profile.L3k3.acdc.step\endcsname{196.5}
\expandafter\gdef\csname R@an.arch_profile.L3k3.amos.act\endcsname{1438}
\expandafter\gdef\csname R@an.arch_profile.L3k3.amos.dwshare\endcsname{0.04}
\expandafter\gdef\csname R@an.arch_profile.L3k3.amos.gmac\endcsname{730.8}
\expandafter\gdef\csname R@an.arch_profile.L3k3.amos.params\endcsname{28.58}
\expandafter\gdef\csname R@an.arch_profile.L3k3.amos.paramsexact\endcsname{28\,581\,904}
\expandafter\gdef\csname R@an.arch_profile.L3k3.amos.peak\endcsname{10.74}
\expandafter\gdef\csname R@an.arch_profile.L3k3.amos.step\endcsname{189.0}
\expandafter\gdef\csname R@an.arch_profile.L3k3.kits.act\endcsname{1122}
\expandafter\gdef\csname R@an.arch_profile.L3k3.kits.dwshare\endcsname{0.02}
\expandafter\gdef\csname R@an.arch_profile.L3k3.kits.gmac\endcsname{586.1}
\expandafter\gdef\csname R@an.arch_profile.L3k3.kits.params\endcsname{28.65}
\expandafter\gdef\csname R@an.arch_profile.L3k3.kits.paramsexact\endcsname{28\,653\,935}
\expandafter\gdef\csname R@an.arch_profile.L3k3.kits.peak\endcsname{9.56}
\expandafter\gdef\csname R@an.arch_profile.L3k3.kits.step\endcsname{157.0}
\expandafter\gdef\csname R@an.arch_profile.L3ng.acdc.act\endcsname{829}
\expandafter\gdef\csname R@an.arch_profile.L3ng.acdc.dwshare\endcsname{0.30}
\expandafter\gdef\csname R@an.arch_profile.L3ng.acdc.gmac\endcsname{433.9}
\expandafter\gdef\csname R@an.arch_profile.L3ng.acdc.params\endcsname{28.82}
\expandafter\gdef\csname R@an.arch_profile.L3ng.acdc.paramsexact\endcsname{28\,821\,972}
\expandafter\gdef\csname R@an.arch_profile.L3ng.acdc.peak\endcsname{11.70}
\expandafter\gdef\csname R@an.arch_profile.L3ng.acdc.step\endcsname{225.8}
\expandafter\gdef\csname R@an.arch_profile.L3ng.amos.act\endcsname{1438}
\expandafter\gdef\csname R@an.arch_profile.L3ng.amos.dwshare\endcsname{0.21}
\expandafter\gdef\csname R@an.arch_profile.L3ng.amos.gmac\endcsname{732.1}
\expandafter\gdef\csname R@an.arch_profile.L3ng.amos.params\endcsname{29.57}
\expandafter\gdef\csname R@an.arch_profile.L3ng.amos.paramsexact\endcsname{29\,568\,912}
\expandafter\gdef\csname R@an.arch_profile.L3ng.amos.peak\endcsname{10.51}
\expandafter\gdef\csname R@an.arch_profile.L3ng.amos.step\endcsname{209.4}
\expandafter\gdef\csname R@an.arch_profile.L3ng.kits.act\endcsname{1122}
\expandafter\gdef\csname R@an.arch_profile.L3ng.kits.dwshare\endcsname{0.14}
\expandafter\gdef\csname R@an.arch_profile.L3ng.kits.gmac\endcsname{586.8}
\expandafter\gdef\csname R@an.arch_profile.L3ng.kits.params\endcsname{29.64}
\expandafter\gdef\csname R@an.arch_profile.L3ng.kits.paramsexact\endcsname{29\,640\,943}
\expandafter\gdef\csname R@an.arch_profile.L3ng.kits.peak\endcsname{9.44}
\expandafter\gdef\csname R@an.arch_profile.L3ng.kits.step\endcsname{169.7}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.acdc.act\endcsname{877}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.acdc.dwshare\endcsname{0.48}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.acdc.gmac\endcsname{551.2}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.acdc.params\endcsname{96.82}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.acdc.paramsexact\endcsname{96\,820\,948}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.acdc.peak\endcsname{11.72}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.acdc.step\endcsname{299.8}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.amos.act\endcsname{1507}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.amos.dwshare\endcsname{0.35}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.amos.gmac\endcsname{895.5}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.amos.params\endcsname{99.79}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.amos.paramsexact\endcsname{99\,786\,640}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.amos.peak\endcsname{11.30}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.amos.step\endcsname{261.9}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.kits.act\endcsname{1158}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.kits.dwshare\endcsname{0.25}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.kits.gmac\endcsname{673.9}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.kits.params\endcsname{99.85}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.kits.paramsexact\endcsname{99\,851\,183}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.kits.peak\endcsname{10.33}
\expandafter\gdef\csname R@an.arch_profile.L3w_L.kits.step\endcsname{204.4}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.acdc.act\endcsname{853}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.acdc.dwshare\endcsname{0.41}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.acdc.gmac\endcsname{483.3}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.acdc.params\endcsname{57.36}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.acdc.paramsexact\endcsname{57\,361\,940}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.acdc.peak\endcsname{11.06}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.acdc.step\endcsname{267.0}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.amos.act\endcsname{1473}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.amos.dwshare\endcsname{0.29}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.amos.gmac\endcsname{801.0}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.amos.params\endcsname{59.03}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.amos.paramsexact\endcsname{59\,033\,936}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.amos.peak\endcsname{11.24}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.amos.step\endcsname{239.1}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.kits.act\endcsname{1140}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.kits.dwshare\endcsname{0.20}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.kits.gmac\endcsname{623.5}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.kits.params\endcsname{59.10}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.kits.paramsexact\endcsname{59\,102\,223}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.kits.peak\endcsname{9.91}
\expandafter\gdef\csname R@an.arch_profile.L3w_M.kits.step\endcsname{189.8}
\expandafter\gdef\csname R@an.arch_profile.L4.acdc.act\endcsname{791}
\expandafter\gdef\csname R@an.arch_profile.L4.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.L4.acdc.gmac\endcsname{587.3}
\expandafter\gdef\csname R@an.arch_profile.L4.acdc.params\endcsname{102.02}
\expandafter\gdef\csname R@an.arch_profile.L4.acdc.paramsexact\endcsname{102\,021\,383}
\expandafter\gdef\csname R@an.arch_profile.L4.acdc.peak\endcsname{10.27}
\expandafter\gdef\csname R@an.arch_profile.L4.acdc.step\endcsname{215.7}
\expandafter\gdef\csname R@an.arch_profile.L4.amos.act\endcsname{1374}
\expandafter\gdef\csname R@an.arch_profile.L4.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.L4.amos.gmac\endcsname{959.3}
\expandafter\gdef\csname R@an.arch_profile.L4.amos.params\endcsname{102.77}
\expandafter\gdef\csname R@an.arch_profile.L4.amos.paramsexact\endcsname{102\,768\,323}
\expandafter\gdef\csname R@an.arch_profile.L4.amos.peak\endcsname{10.75}
\expandafter\gdef\csname R@an.arch_profile.L4.amos.step\endcsname{204.9}
\expandafter\gdef\csname R@an.arch_profile.L4.kits.act\endcsname{1020}
\expandafter\gdef\csname R@an.arch_profile.L4.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.L4.kits.gmac\endcsname{659.6}
\expandafter\gdef\csname R@an.arch_profile.L4.kits.params\endcsname{102.82}
\expandafter\gdef\csname R@an.arch_profile.L4.kits.paramsexact\endcsname{102\,821\,922}
\expandafter\gdef\csname R@an.arch_profile.L4.kits.peak\endcsname{9.52}
\expandafter\gdef\csname R@an.arch_profile.L4.kits.step\endcsname{160.1}
\expandafter\gdef\csname R@an.arch_profile.L6.acdc.act\endcsname{921}
\expandafter\gdef\csname R@an.arch_profile.L6.acdc.dwshare\endcsname{0.25}
\expandafter\gdef\csname R@an.arch_profile.L6.acdc.gmac\endcsname{529.1}
\expandafter\gdef\csname R@an.arch_profile.L6.acdc.params\endcsname{30.35}
\expandafter\gdef\csname R@an.arch_profile.L6.acdc.paramsexact\endcsname{30\,347\,303}
\expandafter\gdef\csname R@an.arch_profile.L6.acdc.peak\endcsname{11.49}
\expandafter\gdef\csname R@an.arch_profile.L6.acdc.step\endcsname{288.4}
\expandafter\gdef\csname R@an.arch_profile.L6.amos.act\endcsname{1596}
\expandafter\gdef\csname R@an.arch_profile.L6.amos.dwshare\endcsname{0.17}
\expandafter\gdef\csname R@an.arch_profile.L6.amos.gmac\endcsname{895.2}
\expandafter\gdef\csname R@an.arch_profile.L6.amos.params\endcsname{31.09}
\expandafter\gdef\csname R@an.arch_profile.L6.amos.paramsexact\endcsname{31\,094\,243}
\expandafter\gdef\csname R@an.arch_profile.L6.amos.peak\endcsname{10.27}
\expandafter\gdef\csname R@an.arch_profile.L6.amos.step\endcsname{263.5}
\expandafter\gdef\csname R@an.arch_profile.L6.kits.act\endcsname{1206}
\expandafter\gdef\csname R@an.arch_profile.L6.kits.dwshare\endcsname{0.12}
\expandafter\gdef\csname R@an.arch_profile.L6.kits.gmac\endcsname{673.8}
\expandafter\gdef\csname R@an.arch_profile.L6.kits.params\endcsname{31.17}
\expandafter\gdef\csname R@an.arch_profile.L6.kits.paramsexact\endcsname{31\,166\,274}
\expandafter\gdef\csname R@an.arch_profile.L6.kits.peak\endcsname{9.33}
\expandafter\gdef\csname R@an.arch_profile.L6.kits.step\endcsname{201.5}
\expandafter\gdef\csname R@an.arch_profile.N1.acdc.act\endcsname{557}
\expandafter\gdef\csname R@an.arch_profile.N1.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.N1.acdc.gmac\endcsname{315.3}
\expandafter\gdef\csname R@an.arch_profile.N1.acdc.params\endcsname{30.38}
\expandafter\gdef\csname R@an.arch_profile.N1.acdc.paramsexact\endcsname{30\,377\,428}
\expandafter\gdef\csname R@an.arch_profile.N1.acdc.peak\endcsname{10.27}
\expandafter\gdef\csname R@an.arch_profile.N1.acdc.step\endcsname{227.3}
\expandafter\gdef\csname R@an.arch_profile.N1.amos.act\endcsname{981}
\expandafter\gdef\csname R@an.arch_profile.N1.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.N1.amos.gmac\endcsname{527.0}
\expandafter\gdef\csname R@an.arch_profile.N1.amos.params\endcsname{31.12}
\expandafter\gdef\csname R@an.arch_profile.N1.amos.paramsexact\endcsname{31\,124\,368}
\expandafter\gdef\csname R@an.arch_profile.N1.amos.peak\endcsname{9.01}
\expandafter\gdef\csname R@an.arch_profile.N1.amos.step\endcsname{289.1}
\expandafter\gdef\csname R@an.arch_profile.N1.kits.act\endcsname{811}
\expandafter\gdef\csname R@an.arch_profile.N1.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.N1.kits.gmac\endcsname{477.4}
\expandafter\gdef\csname R@an.arch_profile.N1.kits.params\endcsname{31.20}
\expandafter\gdef\csname R@an.arch_profile.N1.kits.paramsexact\endcsname{31\,196\,399}
\expandafter\gdef\csname R@an.arch_profile.N1.kits.peak\endcsname{8.51}
\expandafter\gdef\csname R@an.arch_profile.N1.kits.step\endcsname{264.1}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.acdc.act\endcsname{1217}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.acdc.gmac\endcsname{399.9}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.acdc.params\endcsname{30.45}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.acdc.paramsexact\endcsname{30\,452\,052}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.acdc.peak\endcsname{11.05}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.acdc.step\endcsname{304.7}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.amos.act\endcsname{2114}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.amos.gmac\endcsname{672.0}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.amos.params\endcsname{31.20}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.amos.paramsexact\endcsname{31\,198\,992}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.amos.peak\endcsname{10.94}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.amos.step\endcsname{301.2}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.kits.act\endcsname{2019}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.kits.gmac\endcsname{941.3}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.kits.params\endcsname{31.42}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.kits.paramsexact\endcsname{31\,418\,479}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.kits.peak\endcsname{9.59}
\expandafter\gdef\csname R@an.arch_profile.P1_frcap32.kits.step\endcsname{326.4}
\expandafter\gdef\csname R@an.arch_profile.P1b.acdc.act\endcsname{557}
\expandafter\gdef\csname R@an.arch_profile.P1b.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.P1b.acdc.gmac\endcsname{400.5}
\expandafter\gdef\csname R@an.arch_profile.P1b.acdc.params\endcsname{30.45}
\expandafter\gdef\csname R@an.arch_profile.P1b.acdc.paramsexact\endcsname{30\,451\,732}
\expandafter\gdef\csname R@an.arch_profile.P1b.acdc.peak\endcsname{10.27}
\expandafter\gdef\csname R@an.arch_profile.P1b.acdc.step\endcsname{154.5}
\expandafter\gdef\csname R@an.arch_profile.P1b.amos.act\endcsname{981}
\expandafter\gdef\csname R@an.arch_profile.P1b.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.P1b.amos.gmac\endcsname{673.1}
\expandafter\gdef\csname R@an.arch_profile.P1b.amos.params\endcsname{31.20}
\expandafter\gdef\csname R@an.arch_profile.P1b.amos.paramsexact\endcsname{31\,198\,672}
\expandafter\gdef\csname R@an.arch_profile.P1b.amos.peak\endcsname{9.01}
\expandafter\gdef\csname R@an.arch_profile.P1b.amos.step\endcsname{150.8}
\expandafter\gdef\csname R@an.arch_profile.P1b.kits.act\endcsname{811}
\expandafter\gdef\csname R@an.arch_profile.P1b.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.P1b.kits.gmac\endcsname{477.4}
\expandafter\gdef\csname R@an.arch_profile.P1b.kits.params\endcsname{31.20}
\expandafter\gdef\csname R@an.arch_profile.P1b.kits.paramsexact\endcsname{31\,196\,399}
\expandafter\gdef\csname R@an.arch_profile.P1b.kits.peak\endcsname{8.51}
\expandafter\gdef\csname R@an.arch_profile.P1b.kits.step\endcsname{124.3}
\expandafter\gdef\csname R@an.arch_profile.P1c.acdc.act\endcsname{566}
\expandafter\gdef\csname R@an.arch_profile.P1c.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.P1c.acdc.gmac\endcsname{331.2}
\expandafter\gdef\csname R@an.arch_profile.P1c.acdc.params\endcsname{30.82}
\expandafter\gdef\csname R@an.arch_profile.P1c.acdc.paramsexact\endcsname{30\,820\,180}
\expandafter\gdef\csname R@an.arch_profile.P1c.acdc.peak\endcsname{10.35}
\expandafter\gdef\csname R@an.arch_profile.P1c.acdc.step\endcsname{144.7}
\expandafter\gdef\csname R@an.arch_profile.P1c.amos.act\endcsname{997}
\expandafter\gdef\csname R@an.arch_profile.P1c.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.P1c.amos.gmac\endcsname{554.2}
\expandafter\gdef\csname R@an.arch_profile.P1c.amos.params\endcsname{31.57}
\expandafter\gdef\csname R@an.arch_profile.P1c.amos.paramsexact\endcsname{31\,567\,120}
\expandafter\gdef\csname R@an.arch_profile.P1c.amos.peak\endcsname{9.07}
\expandafter\gdef\csname R@an.arch_profile.P1c.amos.step\endcsname{142.9}
\expandafter\gdef\csname R@an.arch_profile.P1c.kits.act\endcsname{819}
\expandafter\gdef\csname R@an.arch_profile.P1c.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.P1c.kits.gmac\endcsname{491.9}
\expandafter\gdef\csname R@an.arch_profile.P1c.kits.params\endcsname{31.64}
\expandafter\gdef\csname R@an.arch_profile.P1c.kits.paramsexact\endcsname{31\,639\,151}
\expandafter\gdef\csname R@an.arch_profile.P1c.kits.peak\endcsname{8.54}
\expandafter\gdef\csname R@an.arch_profile.P1c.kits.step\endcsname{124.2}
\expandafter\gdef\csname R@an.arch_profile.P3c.acdc.act\endcsname{559}
\expandafter\gdef\csname R@an.arch_profile.P3c.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.P3c.acdc.gmac\endcsname{315.4}
\expandafter\gdef\csname R@an.arch_profile.P3c.acdc.params\endcsname{30.38}
\expandafter\gdef\csname R@an.arch_profile.P3c.acdc.paramsexact\endcsname{30\,377\,492}
\expandafter\gdef\csname R@an.arch_profile.P3c.acdc.peak\endcsname{10.29}
\expandafter\gdef\csname R@an.arch_profile.P3c.acdc.step\endcsname{147.1}
\expandafter\gdef\csname R@an.arch_profile.P3c.amos.act\endcsname{985}
\expandafter\gdef\csname R@an.arch_profile.P3c.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.P3c.amos.gmac\endcsname{527.1}
\expandafter\gdef\csname R@an.arch_profile.P3c.amos.params\endcsname{31.12}
\expandafter\gdef\csname R@an.arch_profile.P3c.amos.paramsexact\endcsname{31\,124\,432}
\expandafter\gdef\csname R@an.arch_profile.P3c.amos.peak\endcsname{9.01}
\expandafter\gdef\csname R@an.arch_profile.P3c.amos.step\endcsname{146.9}
\expandafter\gdef\csname R@an.arch_profile.P3c.kits.act\endcsname{815}
\expandafter\gdef\csname R@an.arch_profile.P3c.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.P3c.kits.gmac\endcsname{477.5}
\expandafter\gdef\csname R@an.arch_profile.P3c.kits.params\endcsname{31.20}
\expandafter\gdef\csname R@an.arch_profile.P3c.kits.paramsexact\endcsname{31\,196\,463}
\expandafter\gdef\csname R@an.arch_profile.P3c.kits.peak\endcsname{8.52}
\expandafter\gdef\csname R@an.arch_profile.P3c.kits.step\endcsname{127.5}
\expandafter\gdef\csname R@an.arch_profile.P3lite.acdc.act\endcsname{559}
\expandafter\gdef\csname R@an.arch_profile.P3lite.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.P3lite.acdc.gmac\endcsname{315.4}
\expandafter\gdef\csname R@an.arch_profile.P3lite.acdc.params\endcsname{30.38}
\expandafter\gdef\csname R@an.arch_profile.P3lite.acdc.paramsexact\endcsname{30\,377\,492}
\expandafter\gdef\csname R@an.arch_profile.P3lite.acdc.peak\endcsname{10.29}
\expandafter\gdef\csname R@an.arch_profile.P3lite.acdc.step\endcsname{146.1}
\expandafter\gdef\csname R@an.arch_profile.P3lite.amos.act\endcsname{985}
\expandafter\gdef\csname R@an.arch_profile.P3lite.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.P3lite.amos.gmac\endcsname{527.1}
\expandafter\gdef\csname R@an.arch_profile.P3lite.amos.params\endcsname{31.12}
\expandafter\gdef\csname R@an.arch_profile.P3lite.amos.paramsexact\endcsname{31\,124\,432}
\expandafter\gdef\csname R@an.arch_profile.P3lite.amos.peak\endcsname{9.01}
\expandafter\gdef\csname R@an.arch_profile.P3lite.amos.step\endcsname{147.1}
\expandafter\gdef\csname R@an.arch_profile.P3lite.kits.act\endcsname{815}
\expandafter\gdef\csname R@an.arch_profile.P3lite.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.P3lite.kits.gmac\endcsname{477.5}
\expandafter\gdef\csname R@an.arch_profile.P3lite.kits.params\endcsname{31.20}
\expandafter\gdef\csname R@an.arch_profile.P3lite.kits.paramsexact\endcsname{31\,196\,463}
\expandafter\gdef\csname R@an.arch_profile.P3lite.kits.peak\endcsname{8.52}
\expandafter\gdef\csname R@an.arch_profile.P3lite.kits.step\endcsname{127.3}
\expandafter\gdef\csname R@an.arch_profile.S2.acdc.act\endcsname{857}
\expandafter\gdef\csname R@an.arch_profile.S2.acdc.dwshare\endcsname{0.83}
\expandafter\gdef\csname R@an.arch_profile.S2.acdc.gmac\endcsname{366.6}
\expandafter\gdef\csname R@an.arch_profile.S2.acdc.params\endcsname{26.97}
\expandafter\gdef\csname R@an.arch_profile.S2.acdc.paramsexact\endcsname{26\,970\,964}
\expandafter\gdef\csname R@an.arch_profile.S2.acdc.peak\endcsname{11.72}
\expandafter\gdef\csname R@an.arch_profile.S2.acdc.step\endcsname{299.8}
\expandafter\gdef\csname R@an.arch_profile.S2.amos.act\endcsname{1485}
\expandafter\gdef\csname R@an.arch_profile.S2.amos.dwshare\endcsname{0.73}
\expandafter\gdef\csname R@an.arch_profile.S2.amos.gmac\endcsname{616.7}
\expandafter\gdef\csname R@an.arch_profile.S2.amos.params\endcsname{27.72}
\expandafter\gdef\csname R@an.arch_profile.S2.amos.paramsexact\endcsname{27\,717\,904}
\expandafter\gdef\csname R@an.arch_profile.S2.amos.peak\endcsname{10.48}
\expandafter\gdef\csname R@an.arch_profile.S2.amos.step\endcsname{275.3}
\expandafter\gdef\csname R@an.arch_profile.S2.kits.act\endcsname{1147}
\expandafter\gdef\csname R@an.arch_profile.S2.kits.dwshare\endcsname{0.46}
\expandafter\gdef\csname R@an.arch_profile.S2.kits.gmac\endcsname{525.3}
\expandafter\gdef\csname R@an.arch_profile.S2.kits.params\endcsname{27.79}
\expandafter\gdef\csname R@an.arch_profile.S2.kits.paramsexact\endcsname{27\,789\,935}
\expandafter\gdef\csname R@an.arch_profile.S2.kits.peak\endcsname{9.42}
\expandafter\gdef\csname R@an.arch_profile.S2.kits.step\endcsname{206.8}
\expandafter\gdef\csname R@an.arch_profile.SP1.acdc.act\endcsname{1035}
\expandafter\gdef\csname R@an.arch_profile.SP1.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.SP1.acdc.gmac\endcsname{663.1}
\expandafter\gdef\csname R@an.arch_profile.SP1.acdc.params\endcsname{107.11}
\expandafter\gdef\csname R@an.arch_profile.SP1.acdc.paramsexact\endcsname{107\,106\,676}
\expandafter\gdef\csname R@an.arch_profile.SP1.acdc.peak\endcsname{10.37}
\expandafter\gdef\csname R@an.arch_profile.SP1.acdc.step\endcsname{279.8}
\expandafter\gdef\csname R@an.arch_profile.SP1.amos.act\endcsname{1792}
\expandafter\gdef\csname R@an.arch_profile.SP1.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.SP1.amos.gmac\endcsname{1086.4}
\expandafter\gdef\csname R@an.arch_profile.SP1.amos.params\endcsname{107.85}
\expandafter\gdef\csname R@an.arch_profile.SP1.amos.paramsexact\endcsname{107\,853\,616}
\expandafter\gdef\csname R@an.arch_profile.SP1.amos.peak\endcsname{9.98}
\expandafter\gdef\csname R@an.arch_profile.SP1.amos.step\endcsname{268.2}
\expandafter\gdef\csname R@an.arch_profile.SP1.kits.act\endcsname{1377}
\expandafter\gdef\csname R@an.arch_profile.SP1.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.SP1.kits.gmac\endcsname{777.9}
\expandafter\gdef\csname R@an.arch_profile.SP1.kits.params\endcsname{107.93}
\expandafter\gdef\csname R@an.arch_profile.SP1.kits.paramsexact\endcsname{107\,925\,647}
\expandafter\gdef\csname R@an.arch_profile.SP1.kits.peak\endcsname{9.82}
\expandafter\gdef\csname R@an.arch_profile.SP1.kits.step\endcsname{208.6}
\expandafter\gdef\csname R@an.arch_profile.SP2.acdc.act\endcsname{962}
\expandafter\gdef\csname R@an.arch_profile.SP2.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.SP2.acdc.gmac\endcsname{671.3}
\expandafter\gdef\csname R@an.arch_profile.SP2.acdc.params\endcsname{107.11}
\expandafter\gdef\csname R@an.arch_profile.SP2.acdc.paramsexact\endcsname{107\,113\,716}
\expandafter\gdef\csname R@an.arch_profile.SP2.acdc.peak\endcsname{10.57}
\expandafter\gdef\csname R@an.arch_profile.SP2.acdc.step\endcsname{306.0}
\expandafter\gdef\csname R@an.arch_profile.SP2.amos.act\endcsname{1666}
\expandafter\gdef\csname R@an.arch_profile.SP2.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.SP2.amos.gmac\endcsname{1100.5}
\expandafter\gdef\csname R@an.arch_profile.SP2.amos.params\endcsname{107.86}
\expandafter\gdef\csname R@an.arch_profile.SP2.amos.paramsexact\endcsname{107\,860\,656}
\expandafter\gdef\csname R@an.arch_profile.SP2.amos.peak\endcsname{9.25}
\expandafter\gdef\csname R@an.arch_profile.SP2.amos.step\endcsname{291.2}
\expandafter\gdef\csname R@an.arch_profile.SP2.kits.act\endcsname{1243}
\expandafter\gdef\csname R@an.arch_profile.SP2.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.SP2.kits.gmac\endcsname{831.5}
\expandafter\gdef\csname R@an.arch_profile.SP2.kits.params\endcsname{107.95}
\expandafter\gdef\csname R@an.arch_profile.SP2.kits.paramsexact\endcsname{107\,951\,119}
\expandafter\gdef\csname R@an.arch_profile.SP2.kits.peak\endcsname{8.13}
\expandafter\gdef\csname R@an.arch_profile.SP2.kits.step\endcsname{235.8}
\expandafter\gdef\csname R@an.arch_profile.V5A5.acdc.act\endcsname{719}
\expandafter\gdef\csname R@an.arch_profile.V5A5.acdc.dwshare\endcsname{0.33}
\expandafter\gdef\csname R@an.arch_profile.V5A5.acdc.gmac\endcsname{391.6}
\expandafter\gdef\csname R@an.arch_profile.V5A5.acdc.params\endcsname{28.73}
\expandafter\gdef\csname R@an.arch_profile.V5A5.acdc.paramsexact\endcsname{28\,725\,300}
\expandafter\gdef\csname R@an.arch_profile.V5A5.acdc.peak\endcsname{11.74}
\expandafter\gdef\csname R@an.arch_profile.V5A5.acdc.step\endcsname{212.1}
\expandafter\gdef\csname R@an.arch_profile.V5A5.amos.act\endcsname{1250}
\expandafter\gdef\csname R@an.arch_profile.V5A5.amos.dwshare\endcsname{0.24}
\expandafter\gdef\csname R@an.arch_profile.V5A5.amos.gmac\endcsname{659.6}
\expandafter\gdef\csname R@an.arch_profile.V5A5.amos.params\endcsname{29.47}
\expandafter\gdef\csname R@an.arch_profile.V5A5.amos.paramsexact\endcsname{29\,472\,240}
\expandafter\gdef\csname R@an.arch_profile.V5A5.amos.peak\endcsname{9.99}
\expandafter\gdef\csname R@an.arch_profile.V5A5.amos.step\endcsname{195.6}
\expandafter\gdef\csname R@an.arch_profile.V5A5.kits.act\endcsname{954}
\expandafter\gdef\csname R@an.arch_profile.V5A5.kits.dwshare\endcsname{0.17}
\expandafter\gdef\csname R@an.arch_profile.V5A5.kits.gmac\endcsname{499.8}
\expandafter\gdef\csname R@an.arch_profile.V5A5.kits.params\endcsname{29.53}
\expandafter\gdef\csname R@an.arch_profile.V5A5.kits.paramsexact\endcsname{29\,525\,839}
\expandafter\gdef\csname R@an.arch_profile.V5A5.kits.peak\endcsname{8.89}
\expandafter\gdef\csname R@an.arch_profile.V5A5.kits.step\endcsname{152.3}
\expandafter\gdef\csname R@an.arch_profile.V5B1.acdc.act\endcsname{434}
\expandafter\gdef\csname R@an.arch_profile.V5B1.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.V5B1.acdc.gmac\endcsname{177.0}
\expandafter\gdef\csname R@an.arch_profile.V5B1.acdc.params\endcsname{20.18}
\expandafter\gdef\csname R@an.arch_profile.V5B1.acdc.paramsexact\endcsname{20\,182\,132}
\expandafter\gdef\csname R@an.arch_profile.V5B1.acdc.peak\endcsname{9.03}
\expandafter\gdef\csname R@an.arch_profile.V5B1.acdc.step\endcsname{102.1}
\expandafter\gdef\csname R@an.arch_profile.V5B1.amos.act\endcsname{772}
\expandafter\gdef\csname R@an.arch_profile.V5B1.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.V5B1.amos.gmac\endcsname{295.2}
\expandafter\gdef\csname R@an.arch_profile.V5B1.amos.params\endcsname{20.93}
\expandafter\gdef\csname R@an.arch_profile.V5B1.amos.paramsexact\endcsname{20\,929\,072}
\expandafter\gdef\csname R@an.arch_profile.V5B1.amos.peak\endcsname{7.94}
\expandafter\gdef\csname R@an.arch_profile.V5B1.amos.step\endcsname{103.9}
\expandafter\gdef\csname R@an.arch_profile.V5B1.kits.act\endcsname{632}
\expandafter\gdef\csname R@an.arch_profile.V5B1.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.V5B1.kits.gmac\endcsname{257.1}
\expandafter\gdef\csname R@an.arch_profile.V5B1.kits.params\endcsname{20.96}
\expandafter\gdef\csname R@an.arch_profile.V5B1.kits.paramsexact\endcsname{20\,964\,239}
\expandafter\gdef\csname R@an.arch_profile.V5B1.kits.peak\endcsname{7.64}
\expandafter\gdef\csname R@an.arch_profile.V5B1.kits.step\endcsname{89.6}
\expandafter\gdef\csname R@an.arch_profile.V5B2.acdc.act\endcsname{444}
\expandafter\gdef\csname R@an.arch_profile.V5B2.acdc.dwshare\endcsname{0.35}
\expandafter\gdef\csname R@an.arch_profile.V5B2.acdc.gmac\endcsname{177.2}
\expandafter\gdef\csname R@an.arch_profile.V5B2.acdc.params\endcsname{20.48}
\expandafter\gdef\csname R@an.arch_profile.V5B2.acdc.paramsexact\endcsname{20\,477\,172}
\expandafter\gdef\csname R@an.arch_profile.V5B2.acdc.peak\endcsname{9.25}
\expandafter\gdef\csname R@an.arch_profile.V5B2.acdc.step\endcsname{130.0}
\expandafter\gdef\csname R@an.arch_profile.V5B2.amos.act\endcsname{780}
\expandafter\gdef\csname R@an.arch_profile.V5B2.amos.dwshare\endcsname{0.16}
\expandafter\gdef\csname R@an.arch_profile.V5B2.amos.gmac\endcsname{295.3}
\expandafter\gdef\csname R@an.arch_profile.V5B2.amos.params\endcsname{21.22}
\expandafter\gdef\csname R@an.arch_profile.V5B2.amos.paramsexact\endcsname{21\,224\,112}
\expandafter\gdef\csname R@an.arch_profile.V5B2.amos.peak\endcsname{8.02}
\expandafter\gdef\csname R@an.arch_profile.V5B2.amos.step\endcsname{119.8}
\expandafter\gdef\csname R@an.arch_profile.V5B2.kits.act\endcsname{636}
\expandafter\gdef\csname R@an.arch_profile.V5B2.kits.dwshare\endcsname{0.10}
\expandafter\gdef\csname R@an.arch_profile.V5B2.kits.gmac\endcsname{257.2}
\expandafter\gdef\csname R@an.arch_profile.V5B2.kits.params\endcsname{21.26}
\expandafter\gdef\csname R@an.arch_profile.V5B2.kits.paramsexact\endcsname{21\,259\,279}
\expandafter\gdef\csname R@an.arch_profile.V5B2.kits.peak\endcsname{7.68}
\expandafter\gdef\csname R@an.arch_profile.V5B2.kits.step\endcsname{103.1}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.acdc.act\endcsname{829}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.acdc.dwshare\endcsname{0.49}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.acdc.gmac\endcsname{434.7}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.acdc.params\endcsname{29.96}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.acdc.paramsexact\endcsname{29\,957\,076}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.acdc.peak\endcsname{10.43}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.acdc.step\endcsname{257.2}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.amos.act\endcsname{1438}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.amos.dwshare\endcsname{0.30}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.amos.gmac\endcsname{732.7}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.amos.params\endcsname{30.70}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.amos.paramsexact\endcsname{30\,704\,016}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.amos.peak\endcsname{10.75}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.amos.step\endcsname{228.9}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.kits.act\endcsname{1122}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.kits.dwshare\endcsname{0.20}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.kits.gmac\endcsname{587.1}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.kits.params\endcsname{30.78}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.kits.paramsexact\endcsname{30\,776\,047}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.kits.peak\endcsname{9.57}
\expandafter\gdef\csname R@an.arch_profile.V6A1r.kits.step\endcsname{183.7}
\expandafter\gdef\csname R@an.arch_profile.V7A1.acdc.act\endcsname{520}
\expandafter\gdef\csname R@an.arch_profile.V7A1.acdc.dwshare\endcsname{0.20}
\expandafter\gdef\csname R@an.arch_profile.V7A1.acdc.gmac\endcsname{304.5}
\expandafter\gdef\csname R@an.arch_profile.V7A1.acdc.params\endcsname{30.26}
\expandafter\gdef\csname R@an.arch_profile.V7A1.acdc.paramsexact\endcsname{30\,256\,756}
\expandafter\gdef\csname R@an.arch_profile.V7A1.acdc.peak\endcsname{9.89}
\expandafter\gdef\csname R@an.arch_profile.V7A1.acdc.step\endcsname{151.8}
\expandafter\gdef\csname R@an.arch_profile.V7A1.amos.act\endcsname{910}
\expandafter\gdef\csname R@an.arch_profile.V7A1.amos.dwshare\endcsname{0.09}
\expandafter\gdef\csname R@an.arch_profile.V7A1.amos.gmac\endcsname{513.5}
\expandafter\gdef\csname R@an.arch_profile.V7A1.amos.params\endcsname{31.00}
\expandafter\gdef\csname R@an.arch_profile.V7A1.amos.paramsexact\endcsname{31\,003\,696}
\expandafter\gdef\csname R@an.arch_profile.V7A1.amos.peak\endcsname{8.59}
\expandafter\gdef\csname R@an.arch_profile.V7A1.amos.step\endcsname{140.3}
\expandafter\gdef\csname R@an.arch_profile.V7A1.kits.act\endcsname{706}
\expandafter\gdef\csname R@an.arch_profile.V7A1.kits.dwshare\endcsname{0.07}
\expandafter\gdef\csname R@an.arch_profile.V7A1.kits.gmac\endcsname{373.5}
\expandafter\gdef\csname R@an.arch_profile.V7A1.kits.params\endcsname{31.04}
\expandafter\gdef\csname R@an.arch_profile.V7A1.kits.paramsexact\endcsname{31\,038\,863}
\expandafter\gdef\csname R@an.arch_profile.V7A1.kits.peak\endcsname{8.02}
\expandafter\gdef\csname R@an.arch_profile.V7A1.kits.step\endcsname{113.1}
\expandafter\gdef\csname R@an.arch_profile.V7A2.acdc.act\endcsname{630}
\expandafter\gdef\csname R@an.arch_profile.V7A2.acdc.dwshare\endcsname{0.18}
\expandafter\gdef\csname R@an.arch_profile.V7A2.acdc.gmac\endcsname{346.8}
\expandafter\gdef\csname R@an.arch_profile.V7A2.acdc.params\endcsname{30.38}
\expandafter\gdef\csname R@an.arch_profile.V7A2.acdc.paramsexact\endcsname{30\,376\,852}
\expandafter\gdef\csname R@an.arch_profile.V7A2.acdc.peak\endcsname{10.78}
\expandafter\gdef\csname R@an.arch_profile.V7A2.acdc.step\endcsname{174.3}
\expandafter\gdef\csname R@an.arch_profile.V7A2.amos.act\endcsname{1098}
\expandafter\gdef\csname R@an.arch_profile.V7A2.amos.dwshare\endcsname{0.08}
\expandafter\gdef\csname R@an.arch_profile.V7A2.amos.gmac\endcsname{586.0}
\expandafter\gdef\csname R@an.arch_profile.V7A2.amos.params\endcsname{31.12}
\expandafter\gdef\csname R@an.arch_profile.V7A2.amos.paramsexact\endcsname{31\,123\,792}
\expandafter\gdef\csname R@an.arch_profile.V7A2.amos.peak\endcsname{9.34}
\expandafter\gdef\csname R@an.arch_profile.V7A2.amos.step\endcsname{161.0}
\expandafter\gdef\csname R@an.arch_profile.V7A2.kits.act\endcsname{873}
\expandafter\gdef\csname R@an.arch_profile.V7A2.kits.dwshare\endcsname{0.05}
\expandafter\gdef\csname R@an.arch_profile.V7A2.kits.gmac\endcsname{460.5}
\expandafter\gdef\csname R@an.arch_profile.V7A2.kits.params\endcsname{31.18}
\expandafter\gdef\csname R@an.arch_profile.V7A2.kits.paramsexact\endcsname{31\,177\,391}
\expandafter\gdef\csname R@an.arch_profile.V7A2.kits.peak\endcsname{8.69}
\expandafter\gdef\csname R@an.arch_profile.V7A2.kits.step\endcsname{134.7}
\expandafter\gdef\csname R@an.arch_profile.V7A3.acdc.act\endcsname{566}
\expandafter\gdef\csname R@an.arch_profile.V7A3.acdc.dwshare\endcsname{0.25}
\expandafter\gdef\csname R@an.arch_profile.V7A3.acdc.gmac\endcsname{246.4}
\expandafter\gdef\csname R@an.arch_profile.V7A3.acdc.params\endcsname{25.58}
\expandafter\gdef\csname R@an.arch_profile.V7A3.acdc.paramsexact\endcsname{25\,576\,020}
\expandafter\gdef\csname R@an.arch_profile.V7A3.acdc.peak\endcsname{10.26}
\expandafter\gdef\csname R@an.arch_profile.V7A3.acdc.step\endcsname{156.5}
\expandafter\gdef\csname R@an.arch_profile.V7A3.amos.act\endcsname{989}
\expandafter\gdef\csname R@an.arch_profile.V7A3.amos.dwshare\endcsname{0.12}
\expandafter\gdef\csname R@an.arch_profile.V7A3.amos.gmac\endcsname{411.2}
\expandafter\gdef\csname R@an.arch_profile.V7A3.amos.params\endcsname{26.32}
\expandafter\gdef\csname R@an.arch_profile.V7A3.amos.paramsexact\endcsname{26\,322\,960}
\expandafter\gdef\csname R@an.arch_profile.V7A3.amos.peak\endcsname{8.89}
\expandafter\gdef\csname R@an.arch_profile.V7A3.amos.step\endcsname{145.0}
\expandafter\gdef\csname R@an.arch_profile.V7A3.kits.act\endcsname{815}
\expandafter\gdef\csname R@an.arch_profile.V7A3.kits.dwshare\endcsname{0.07}
\expandafter\gdef\csname R@an.arch_profile.V7A3.kits.gmac\endcsname{367.3}
\expandafter\gdef\csname R@an.arch_profile.V7A3.kits.params\endcsname{26.38}
\expandafter\gdef\csname R@an.arch_profile.V7A3.kits.paramsexact\endcsname{26\,376\,559}
\expandafter\gdef\csname R@an.arch_profile.V7A3.kits.peak\endcsname{8.43}
\expandafter\gdef\csname R@an.arch_profile.V7A3.kits.step\endcsname{125.5}
\expandafter\gdef\csname R@an.arch_profile.V7B1.acdc.act\endcsname{448}
\expandafter\gdef\csname R@an.arch_profile.V7B1.acdc.dwshare\endcsname{0.02}
\expandafter\gdef\csname R@an.arch_profile.V7B1.acdc.gmac\endcsname{176.6}
\expandafter\gdef\csname R@an.arch_profile.V7B1.acdc.params\endcsname{19.65}
\expandafter\gdef\csname R@an.arch_profile.V7B1.acdc.paramsexact\endcsname{19\,652\,852}
\expandafter\gdef\csname R@an.arch_profile.V7B1.acdc.peak\endcsname{9.28}
\expandafter\gdef\csname R@an.arch_profile.V7B1.acdc.step\endcsname{111.5}
\expandafter\gdef\csname R@an.arch_profile.V7B1.amos.act\endcsname{783}
\expandafter\gdef\csname R@an.arch_profile.V7B1.amos.dwshare\endcsname{0.01}
\expandafter\gdef\csname R@an.arch_profile.V7B1.amos.gmac\endcsname{294.9}
\expandafter\gdef\csname R@an.arch_profile.V7B1.amos.params\endcsname{20.40}
\expandafter\gdef\csname R@an.arch_profile.V7B1.amos.paramsexact\endcsname{20\,399\,792}
\expandafter\gdef\csname R@an.arch_profile.V7B1.amos.peak\endcsname{8.03}
\expandafter\gdef\csname R@an.arch_profile.V7B1.amos.step\endcsname{109.4}
\expandafter\gdef\csname R@an.arch_profile.V7B1.kits.act\endcsname{638}
\expandafter\gdef\csname R@an.arch_profile.V7B1.kits.dwshare\endcsname{0.01}
\expandafter\gdef\csname R@an.arch_profile.V7B1.kits.gmac\endcsname{256.9}
\expandafter\gdef\csname R@an.arch_profile.V7B1.kits.params\endcsname{20.43}
\expandafter\gdef\csname R@an.arch_profile.V7B1.kits.paramsexact\endcsname{20\,434\,959}
\expandafter\gdef\csname R@an.arch_profile.V7B1.kits.peak\endcsname{7.69}
\expandafter\gdef\csname R@an.arch_profile.V7B1.kits.step\endcsname{95.3}
\expandafter\gdef\csname R@an.arch_profile.V7B2.acdc.act\endcsname{444}
\expandafter\gdef\csname R@an.arch_profile.V7B2.acdc.dwshare\endcsname{0.03}
\expandafter\gdef\csname R@an.arch_profile.V7B2.acdc.gmac\endcsname{176.6}
\expandafter\gdef\csname R@an.arch_profile.V7B2.acdc.params\endcsname{19.67}
\expandafter\gdef\csname R@an.arch_profile.V7B2.acdc.paramsexact\endcsname{19\,668\,212}
\expandafter\gdef\csname R@an.arch_profile.V7B2.acdc.peak\endcsname{9.25}
\expandafter\gdef\csname R@an.arch_profile.V7B2.acdc.step\endcsname{108.6}
\expandafter\gdef\csname R@an.arch_profile.V7B2.amos.act\endcsname{780}
\expandafter\gdef\csname R@an.arch_profile.V7B2.amos.dwshare\endcsname{0.01}
\expandafter\gdef\csname R@an.arch_profile.V7B2.amos.gmac\endcsname{294.9}
\expandafter\gdef\csname R@an.arch_profile.V7B2.amos.params\endcsname{20.42}
\expandafter\gdef\csname R@an.arch_profile.V7B2.amos.paramsexact\endcsname{20\,415\,152}
\expandafter\gdef\csname R@an.arch_profile.V7B2.amos.peak\endcsname{8.02}
\expandafter\gdef\csname R@an.arch_profile.V7B2.amos.step\endcsname{109.7}
\expandafter\gdef\csname R@an.arch_profile.V7B2.kits.act\endcsname{636}
\expandafter\gdef\csname R@an.arch_profile.V7B2.kits.dwshare\endcsname{0.01}
\expandafter\gdef\csname R@an.arch_profile.V7B2.kits.gmac\endcsname{256.9}
\expandafter\gdef\csname R@an.arch_profile.V7B2.kits.params\endcsname{20.45}
\expandafter\gdef\csname R@an.arch_profile.V7B2.kits.paramsexact\endcsname{20\,450\,319}
\expandafter\gdef\csname R@an.arch_profile.V7B2.kits.peak\endcsname{7.68}
\expandafter\gdef\csname R@an.arch_profile.V7B2.kits.step\endcsname{94.0}
\expandafter\gdef\csname R@an.arch_profile.V7C1.acdc.act\endcsname{436}
\expandafter\gdef\csname R@an.arch_profile.V7C1.acdc.dwshare\endcsname{0.07}
\expandafter\gdef\csname R@an.arch_profile.V7C1.acdc.gmac\endcsname{177.1}
\expandafter\gdef\csname R@an.arch_profile.V7C1.acdc.params\endcsname{20.33}
\expandafter\gdef\csname R@an.arch_profile.V7C1.acdc.paramsexact\endcsname{20\,329\,652}
\expandafter\gdef\csname R@an.arch_profile.V7C1.acdc.peak\endcsname{9.08}
\expandafter\gdef\csname R@an.arch_profile.V7C1.acdc.step\endcsname{111.5}
\expandafter\gdef\csname R@an.arch_profile.V7C1.amos.act\endcsname{773}
\expandafter\gdef\csname R@an.arch_profile.V7C1.amos.dwshare\endcsname{0.02}
\expandafter\gdef\csname R@an.arch_profile.V7C1.amos.gmac\endcsname{295.2}
\expandafter\gdef\csname R@an.arch_profile.V7C1.amos.params\endcsname{21.08}
\expandafter\gdef\csname R@an.arch_profile.V7C1.amos.paramsexact\endcsname{21\,076\,592}
\expandafter\gdef\csname R@an.arch_profile.V7C1.amos.peak\endcsname{7.95}
\expandafter\gdef\csname R@an.arch_profile.V7C1.amos.step\endcsname{108.9}
\expandafter\gdef\csname R@an.arch_profile.V7C1.kits.act\endcsname{633}
\expandafter\gdef\csname R@an.arch_profile.V7C1.kits.dwshare\endcsname{0.01}
\expandafter\gdef\csname R@an.arch_profile.V7C1.kits.gmac\endcsname{257.1}
\expandafter\gdef\csname R@an.arch_profile.V7C1.kits.params\endcsname{21.11}
\expandafter\gdef\csname R@an.arch_profile.V7C1.kits.paramsexact\endcsname{21\,111\,759}
\expandafter\gdef\csname R@an.arch_profile.V7C1.kits.peak\endcsname{7.65}
\expandafter\gdef\csname R@an.arch_profile.V7C1.kits.step\endcsname{95.1}
\expandafter\gdef\csname R@an.arch_profile.V7C2.acdc.act\endcsname{444}
\expandafter\gdef\csname R@an.arch_profile.V7C2.acdc.dwshare\endcsname{0.03}
\expandafter\gdef\csname R@an.arch_profile.V7C2.acdc.gmac\endcsname{176.6}
\expandafter\gdef\csname R@an.arch_profile.V7C2.acdc.params\endcsname{19.67}
\expandafter\gdef\csname R@an.arch_profile.V7C2.acdc.paramsexact\endcsname{19\,668\,212}
\expandafter\gdef\csname R@an.arch_profile.V7C2.acdc.peak\endcsname{9.25}
\expandafter\gdef\csname R@an.arch_profile.V7C2.acdc.step\endcsname{110.0}
\expandafter\gdef\csname R@an.arch_profile.V7C2.amos.act\endcsname{780}
\expandafter\gdef\csname R@an.arch_profile.V7C2.amos.dwshare\endcsname{0.01}
\expandafter\gdef\csname R@an.arch_profile.V7C2.amos.gmac\endcsname{294.9}
\expandafter\gdef\csname R@an.arch_profile.V7C2.amos.params\endcsname{20.42}
\expandafter\gdef\csname R@an.arch_profile.V7C2.amos.paramsexact\endcsname{20\,415\,152}
\expandafter\gdef\csname R@an.arch_profile.V7C2.amos.peak\endcsname{8.02}
\expandafter\gdef\csname R@an.arch_profile.V7C2.amos.step\endcsname{108.4}
\expandafter\gdef\csname R@an.arch_profile.V7C2.kits.act\endcsname{636}
\expandafter\gdef\csname R@an.arch_profile.V7C2.kits.dwshare\endcsname{0.01}
\expandafter\gdef\csname R@an.arch_profile.V7C2.kits.gmac\endcsname{256.9}
\expandafter\gdef\csname R@an.arch_profile.V7C2.kits.params\endcsname{20.45}
\expandafter\gdef\csname R@an.arch_profile.V7C2.kits.paramsexact\endcsname{20\,450\,319}
\expandafter\gdef\csname R@an.arch_profile.V7C2.kits.peak\endcsname{7.68}
\expandafter\gdef\csname R@an.arch_profile.V7C2.kits.step\endcsname{94.2}
\expandafter\gdef\csname R@an.arch_profile.V8A1.acdc.act\endcsname{444}
\expandafter\gdef\csname R@an.arch_profile.V8A1.acdc.dwshare\endcsname{0.31}
\expandafter\gdef\csname R@an.arch_profile.V8A1.acdc.gmac\endcsname{179.9}
\expandafter\gdef\csname R@an.arch_profile.V8A1.acdc.params\endcsname{30.53}
\expandafter\gdef\csname R@an.arch_profile.V8A1.acdc.paramsexact\endcsname{30\,526\,132}
\expandafter\gdef\csname R@an.arch_profile.V8A1.acdc.peak\endcsname{9.29}
\expandafter\gdef\csname R@an.arch_profile.V8A1.acdc.step\endcsname{141.6}
\expandafter\gdef\csname R@an.arch_profile.V8A1.amos.act\endcsname{776}
\expandafter\gdef\csname R@an.arch_profile.V8A1.amos.dwshare\endcsname{0.08}
\expandafter\gdef\csname R@an.arch_profile.V8A1.amos.gmac\endcsname{296.4}
\expandafter\gdef\csname R@an.arch_profile.V8A1.amos.params\endcsname{31.27}
\expandafter\gdef\csname R@an.arch_profile.V8A1.amos.paramsexact\endcsname{31\,273\,072}
\expandafter\gdef\csname R@an.arch_profile.V8A1.amos.peak\endcsname{8.04}
\expandafter\gdef\csname R@an.arch_profile.V8A1.amos.step\endcsname{125.7}
\expandafter\gdef\csname R@an.arch_profile.V8A1.kits.act\endcsname{634}
\expandafter\gdef\csname R@an.arch_profile.V8A1.kits.dwshare\endcsname{0.05}
\expandafter\gdef\csname R@an.arch_profile.V8A1.kits.gmac\endcsname{257.8}
\expandafter\gdef\csname R@an.arch_profile.V8A1.kits.params\endcsname{31.31}
\expandafter\gdef\csname R@an.arch_profile.V8A1.kits.paramsexact\endcsname{31\,308\,239}
\expandafter\gdef\csname R@an.arch_profile.V8A1.kits.peak\endcsname{7.72}
\expandafter\gdef\csname R@an.arch_profile.V8A1.kits.step\endcsname{112.4}
\expandafter\gdef\csname R@an.arch_profile.V8A2.acdc.act\endcsname{444}
\expandafter\gdef\csname R@an.arch_profile.V8A2.acdc.dwshare\endcsname{0.19}
\expandafter\gdef\csname R@an.arch_profile.V8A2.acdc.gmac\endcsname{189.7}
\expandafter\gdef\csname R@an.arch_profile.V8A2.acdc.params\endcsname{30.69}
\expandafter\gdef\csname R@an.arch_profile.V8A2.acdc.paramsexact\endcsname{30\,692\,212}
\expandafter\gdef\csname R@an.arch_profile.V8A2.acdc.peak\endcsname{9.25}
\expandafter\gdef\csname R@an.arch_profile.V8A2.acdc.step\endcsname{130.7}
\expandafter\gdef\csname R@an.arch_profile.V8A2.amos.act\endcsname{779}
\expandafter\gdef\csname R@an.arch_profile.V8A2.amos.dwshare\endcsname{0.05}
\expandafter\gdef\csname R@an.arch_profile.V8A2.amos.gmac\endcsname{312.1}
\expandafter\gdef\csname R@an.arch_profile.V8A2.amos.params\endcsname{31.44}
\expandafter\gdef\csname R@an.arch_profile.V8A2.amos.paramsexact\endcsname{31\,439\,152}
\expandafter\gdef\csname R@an.arch_profile.V8A2.amos.peak\endcsname{8.05}
\expandafter\gdef\csname R@an.arch_profile.V8A2.amos.step\endcsname{120.4}
\expandafter\gdef\csname R@an.arch_profile.V8A2.kits.act\endcsname{636}
\expandafter\gdef\csname R@an.arch_profile.V8A2.kits.dwshare\endcsname{0.03}
\expandafter\gdef\csname R@an.arch_profile.V8A2.kits.gmac\endcsname{266.1}
\expandafter\gdef\csname R@an.arch_profile.V8A2.kits.params\endcsname{31.47}
\expandafter\gdef\csname R@an.arch_profile.V8A2.kits.paramsexact\endcsname{31\,474\,319}
\expandafter\gdef\csname R@an.arch_profile.V8A2.kits.peak\endcsname{7.73}
\expandafter\gdef\csname R@an.arch_profile.V8A2.kits.step\endcsname{105.3}
\expandafter\gdef\csname R@an.arch_profile.V8B1.acdc.act\endcsname{325}
\expandafter\gdef\csname R@an.arch_profile.V8B1.acdc.dwshare\endcsname{0.09}
\expandafter\gdef\csname R@an.arch_profile.V8B1.acdc.gmac\endcsname{131.7}
\expandafter\gdef\csname R@an.arch_profile.V8B1.acdc.params\endcsname{17.44}
\expandafter\gdef\csname R@an.arch_profile.V8B1.acdc.paramsexact\endcsname{17\,443\,796}
\expandafter\gdef\csname R@an.arch_profile.V8B1.acdc.peak\endcsname{8.17}
\expandafter\gdef\csname R@an.arch_profile.V8B1.acdc.step\endcsname{88.6}
\expandafter\gdef\csname R@an.arch_profile.V8B1.amos.act\endcsname{584}
\expandafter\gdef\csname R@an.arch_profile.V8B1.amos.dwshare\endcsname{0.02}
\expandafter\gdef\csname R@an.arch_profile.V8B1.amos.gmac\endcsname{220.1}
\expandafter\gdef\csname R@an.arch_profile.V8B1.amos.params\endcsname{18.19}
\expandafter\gdef\csname R@an.arch_profile.V8B1.amos.paramsexact\endcsname{18\,190\,736}
\expandafter\gdef\csname R@an.arch_profile.V8B1.amos.peak\endcsname{7.17}
\expandafter\gdef\csname R@an.arch_profile.V8B1.amos.step\endcsname{86.4}
\expandafter\gdef\csname R@an.arch_profile.V8B1.kits.act\endcsname{465}
\expandafter\gdef\csname R@an.arch_profile.V8B1.kits.dwshare\endcsname{0.02}
\expandafter\gdef\csname R@an.arch_profile.V8B1.kits.gmac\endcsname{168.7}
\expandafter\gdef\csname R@an.arch_profile.V8B1.kits.params\endcsname{18.21}
\expandafter\gdef\csname R@an.arch_profile.V8B1.kits.paramsexact\endcsname{18\,207\,471}
\expandafter\gdef\csname R@an.arch_profile.V8B1.kits.peak\endcsname{6.96}
\expandafter\gdef\csname R@an.arch_profile.V8B1.kits.step\endcsname{72.5}
\expandafter\gdef\csname R@an.arch_profile.V8B2.acdc.act\endcsname{363}
\expandafter\gdef\csname R@an.arch_profile.V8B2.acdc.dwshare\endcsname{0.07}
\expandafter\gdef\csname R@an.arch_profile.V8B2.acdc.gmac\endcsname{166.5}
\expandafter\gdef\csname R@an.arch_profile.V8B2.acdc.params\endcsname{20.32}
\expandafter\gdef\csname R@an.arch_profile.V8B2.acdc.paramsexact\endcsname{20\,320\,340}
\expandafter\gdef\csname R@an.arch_profile.V8B2.acdc.peak\endcsname{8.49}
\expandafter\gdef\csname R@an.arch_profile.V8B2.acdc.step\endcsname{97.0}
\expandafter\gdef\csname R@an.arch_profile.V8B2.amos.act\endcsname{647}
\expandafter\gdef\csname R@an.arch_profile.V8B2.amos.dwshare\endcsname{0.02}
\expandafter\gdef\csname R@an.arch_profile.V8B2.amos.gmac\endcsname{277.1}
\expandafter\gdef\csname R@an.arch_profile.V8B2.amos.params\endcsname{21.07}
\expandafter\gdef\csname R@an.arch_profile.V8B2.amos.paramsexact\endcsname{21\,067\,280}
\expandafter\gdef\csname R@an.arch_profile.V8B2.amos.peak\endcsname{7.45}
\expandafter\gdef\csname R@an.arch_profile.V8B2.amos.step\endcsname{94.3}
\expandafter\gdef\csname R@an.arch_profile.V8B2.kits.act\endcsname{499}
\expandafter\gdef\csname R@an.arch_profile.V8B2.kits.dwshare\endcsname{0.01}
\expandafter\gdef\csname R@an.arch_profile.V8B2.kits.gmac\endcsname{199.1}
\expandafter\gdef\csname R@an.arch_profile.V8B2.kits.params\endcsname{21.08}
\expandafter\gdef\csname R@an.arch_profile.V8B2.kits.paramsexact\endcsname{21\,084\,015}
\expandafter\gdef\csname R@an.arch_profile.V8B2.kits.peak\endcsname{7.11}
\expandafter\gdef\csname R@an.arch_profile.V8B2.kits.step\endcsname{77.6}
\expandafter\gdef\csname R@an.arch_profile.V8X1.acdc.act\endcsname{435}
\expandafter\gdef\csname R@an.arch_profile.V8X1.acdc.dwshare\endcsname{0.06}
\expandafter\gdef\csname R@an.arch_profile.V8X1.acdc.gmac\endcsname{174.1}
\expandafter\gdef\csname R@an.arch_profile.V8X1.acdc.params\endcsname{17.58}
\expandafter\gdef\csname R@an.arch_profile.V8X1.acdc.paramsexact\endcsname{17\,583\,780}
\expandafter\gdef\csname R@an.arch_profile.V8X1.acdc.peak\endcsname{9.05}
\expandafter\gdef\csname R@an.arch_profile.V8X1.acdc.step\endcsname{110.3}
\expandafter\gdef\csname R@an.arch_profile.V8X1.amos.act\endcsname{772}
\expandafter\gdef\csname R@an.arch_profile.V8X1.amos.dwshare\endcsname{0.02}
\expandafter\gdef\csname R@an.arch_profile.V8X1.amos.gmac\endcsname{291.7}
\expandafter\gdef\csname R@an.arch_profile.V8X1.amos.params\endcsname{18.21}
\expandafter\gdef\csname R@an.arch_profile.V8X1.amos.paramsexact\endcsname{18\,210\,432}
\expandafter\gdef\csname R@an.arch_profile.V8X1.amos.peak\endcsname{7.93}
\expandafter\gdef\csname R@an.arch_profile.V8X1.amos.step\endcsname{108.7}
\expandafter\gdef\csname R@an.arch_profile.V8X1.kits.act\endcsname{632}
\expandafter\gdef\csname R@an.arch_profile.V8X1.kits.dwshare\endcsname{0.01}
\expandafter\gdef\csname R@an.arch_profile.V8X1.kits.gmac\endcsname{255.3}
\expandafter\gdef\csname R@an.arch_profile.V8X1.kits.params\endcsname{18.25}
\expandafter\gdef\csname R@an.arch_profile.V8X1.kits.paramsexact\endcsname{18\,246\,119}
\expandafter\gdef\csname R@an.arch_profile.V8X1.kits.peak\endcsname{7.63}
\expandafter\gdef\csname R@an.arch_profile.V8X1.kits.step\endcsname{94.6}
\expandafter\gdef\csname R@an.arch_profile.W1.acdc.act\endcsname{602}
\expandafter\gdef\csname R@an.arch_profile.W1.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.W1.acdc.gmac\endcsname{316.2}
\expandafter\gdef\csname R@an.arch_profile.W1.acdc.params\endcsname{30.39}
\expandafter\gdef\csname R@an.arch_profile.W1.acdc.paramsexact\endcsname{30\,388\,244}
\expandafter\gdef\csname R@an.arch_profile.W1.acdc.peak\endcsname{10.73}
\expandafter\gdef\csname R@an.arch_profile.W1.acdc.step\endcsname{163.2}
\expandafter\gdef\csname R@an.arch_profile.W1.amos.act\endcsname{1060}
\expandafter\gdef\csname R@an.arch_profile.W1.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.W1.amos.gmac\endcsname{528.5}
\expandafter\gdef\csname R@an.arch_profile.W1.amos.params\endcsname{31.14}
\expandafter\gdef\csname R@an.arch_profile.W1.amos.paramsexact\endcsname{31\,135\,184}
\expandafter\gdef\csname R@an.arch_profile.W1.amos.peak\endcsname{9.40}
\expandafter\gdef\csname R@an.arch_profile.W1.amos.step\endcsname{160.3}
\expandafter\gdef\csname R@an.arch_profile.W1.kits.act\endcsname{853}
\expandafter\gdef\csname R@an.arch_profile.W1.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.W1.kits.gmac\endcsname{478.2}
\expandafter\gdef\csname R@an.arch_profile.W1.kits.params\endcsname{31.21}
\expandafter\gdef\csname R@an.arch_profile.W1.kits.paramsexact\endcsname{31\,207\,215}
\expandafter\gdef\csname R@an.arch_profile.W1.kits.peak\endcsname{8.72}
\expandafter\gdef\csname R@an.arch_profile.W1.kits.step\endcsname{138.6}
\expandafter\gdef\csname R@an.arch_profile.W1c.acdc.act\endcsname{602}
\expandafter\gdef\csname R@an.arch_profile.W1c.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.W1c.acdc.gmac\endcsname{316.2}
\expandafter\gdef\csname R@an.arch_profile.W1c.acdc.params\endcsname{30.39}
\expandafter\gdef\csname R@an.arch_profile.W1c.acdc.paramsexact\endcsname{30\,388\,244}
\expandafter\gdef\csname R@an.arch_profile.W1c.acdc.peak\endcsname{10.73}
\expandafter\gdef\csname R@an.arch_profile.W1c.acdc.step\endcsname{163.8}
\expandafter\gdef\csname R@an.arch_profile.W1c.amos.act\endcsname{1060}
\expandafter\gdef\csname R@an.arch_profile.W1c.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.W1c.amos.gmac\endcsname{528.5}
\expandafter\gdef\csname R@an.arch_profile.W1c.amos.params\endcsname{31.14}
\expandafter\gdef\csname R@an.arch_profile.W1c.amos.paramsexact\endcsname{31\,135\,184}
\expandafter\gdef\csname R@an.arch_profile.W1c.amos.peak\endcsname{9.40}
\expandafter\gdef\csname R@an.arch_profile.W1c.amos.step\endcsname{160.8}
\expandafter\gdef\csname R@an.arch_profile.W1c.kits.act\endcsname{853}
\expandafter\gdef\csname R@an.arch_profile.W1c.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.W1c.kits.gmac\endcsname{478.2}
\expandafter\gdef\csname R@an.arch_profile.W1c.kits.params\endcsname{31.21}
\expandafter\gdef\csname R@an.arch_profile.W1c.kits.paramsexact\endcsname{31\,207\,215}
\expandafter\gdef\csname R@an.arch_profile.W1c.kits.peak\endcsname{8.72}
\expandafter\gdef\csname R@an.arch_profile.W1c.kits.step\endcsname{139.4}
\expandafter\gdef\csname R@an.arch_profile.W2.acdc.act\endcsname{602}
\expandafter\gdef\csname R@an.arch_profile.W2.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.W2.acdc.gmac\endcsname{316.2}
\expandafter\gdef\csname R@an.arch_profile.W2.acdc.params\endcsname{30.39}
\expandafter\gdef\csname R@an.arch_profile.W2.acdc.paramsexact\endcsname{30\,388\,474}
\expandafter\gdef\csname R@an.arch_profile.W2.acdc.peak\endcsname{10.74}
\expandafter\gdef\csname R@an.arch_profile.W2.acdc.step\endcsname{165.2}
\expandafter\gdef\csname R@an.arch_profile.W2.amos.act\endcsname{1060}
\expandafter\gdef\csname R@an.arch_profile.W2.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.W2.amos.gmac\endcsname{528.5}
\expandafter\gdef\csname R@an.arch_profile.W2.amos.params\endcsname{31.14}
\expandafter\gdef\csname R@an.arch_profile.W2.amos.paramsexact\endcsname{31\,135\,414}
\expandafter\gdef\csname R@an.arch_profile.W2.amos.peak\endcsname{9.41}
\expandafter\gdef\csname R@an.arch_profile.W2.amos.step\endcsname{161.6}
\expandafter\gdef\csname R@an.arch_profile.W2.kits.act\endcsname{853}
\expandafter\gdef\csname R@an.arch_profile.W2.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.W2.kits.gmac\endcsname{478.2}
\expandafter\gdef\csname R@an.arch_profile.W2.kits.params\endcsname{31.21}
\expandafter\gdef\csname R@an.arch_profile.W2.kits.paramsexact\endcsname{31\,207\,445}
\expandafter\gdef\csname R@an.arch_profile.W2.kits.peak\endcsname{8.73}
\expandafter\gdef\csname R@an.arch_profile.W2.kits.step\endcsname{139.6}
\expandafter\gdef\csname R@an.arch_profile.W3.acdc.act\endcsname{512}
\expandafter\gdef\csname R@an.arch_profile.W3.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.W3.acdc.gmac\endcsname{310.5}
\expandafter\gdef\csname R@an.arch_profile.W3.acdc.params\endcsname{29.55}
\expandafter\gdef\csname R@an.arch_profile.W3.acdc.paramsexact\endcsname{29\,549\,352}
\expandafter\gdef\csname R@an.arch_profile.W3.acdc.peak\endcsname{10.61}
\expandafter\gdef\csname R@an.arch_profile.W3.acdc.step\endcsname{155.8}
\expandafter\gdef\csname R@an.arch_profile.W3.amos.act\endcsname{905}
\expandafter\gdef\csname R@an.arch_profile.W3.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.W3.amos.gmac\endcsname{518.7}
\expandafter\gdef\csname R@an.arch_profile.W3.amos.params\endcsname{29.57}
\expandafter\gdef\csname R@an.arch_profile.W3.amos.paramsexact\endcsname{29\,566\,716}
\expandafter\gdef\csname R@an.arch_profile.W3.amos.peak\endcsname{9.29}
\expandafter\gdef\csname R@an.arch_profile.W3.amos.step\endcsname{152.1}
\expandafter\gdef\csname R@an.arch_profile.W3.kits.act\endcsname{740}
\expandafter\gdef\csname R@an.arch_profile.W3.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.W3.kits.gmac\endcsname{471.0}
\expandafter\gdef\csname R@an.arch_profile.W3.kits.params\endcsname{29.63}
\expandafter\gdef\csname R@an.arch_profile.W3.kits.paramsexact\endcsname{29\,631\,335}
\expandafter\gdef\csname R@an.arch_profile.W3.kits.peak\endcsname{8.70}
\expandafter\gdef\csname R@an.arch_profile.W3.kits.step\endcsname{133.7}
\expandafter\gdef\csname R@an.arch_profile.W3c.acdc.act\endcsname{508}
\expandafter\gdef\csname R@an.arch_profile.W3c.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.W3c.acdc.gmac\endcsname{310.1}
\expandafter\gdef\csname R@an.arch_profile.W3c.acdc.params\endcsname{29.53}
\expandafter\gdef\csname R@an.arch_profile.W3c.acdc.paramsexact\endcsname{29\,531\,604}
\expandafter\gdef\csname R@an.arch_profile.W3c.acdc.peak\endcsname{11.04}
\expandafter\gdef\csname R@an.arch_profile.W3c.acdc.step\endcsname{155.3}
\expandafter\gdef\csname R@an.arch_profile.W3c.amos.act\endcsname{898}
\expandafter\gdef\csname R@an.arch_profile.W3c.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.W3c.amos.gmac\endcsname{518.0}
\expandafter\gdef\csname R@an.arch_profile.W3c.amos.params\endcsname{29.54}
\expandafter\gdef\csname R@an.arch_profile.W3c.amos.paramsexact\endcsname{29\,541\,264}
\expandafter\gdef\csname R@an.arch_profile.W3c.amos.peak\endcsname{9.50}
\expandafter\gdef\csname R@an.arch_profile.W3c.amos.step\endcsname{150.2}
\expandafter\gdef\csname R@an.arch_profile.W3c.kits.act\endcsname{733}
\expandafter\gdef\csname R@an.arch_profile.W3c.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.W3c.kits.gmac\endcsname{470.4}
\expandafter\gdef\csname R@an.arch_profile.W3c.kits.params\endcsname{29.61}
\expandafter\gdef\csname R@an.arch_profile.W3c.kits.paramsexact\endcsname{29\,605\,103}
\expandafter\gdef\csname R@an.arch_profile.W3c.kits.peak\endcsname{8.50}
\expandafter\gdef\csname R@an.arch_profile.W3c.kits.step\endcsname{130.6}
\expandafter\gdef\csname R@an.arch_profile.W4.acdc.act\endcsname{1284}
\expandafter\gdef\csname R@an.arch_profile.W4.acdc.dwshare\endcsname{2.16}
\expandafter\gdef\csname R@an.arch_profile.W4.acdc.gmac\endcsname{289.0}
\expandafter\gdef\csname R@an.arch_profile.W4.acdc.params\endcsname{33.48}
\expandafter\gdef\csname R@an.arch_profile.W4.acdc.paramsexact\endcsname{33\,479\,252}
\expandafter\gdef\csname R@an.arch_profile.W4.acdc.peak\endcsname{10.76}
\expandafter\gdef\csname R@an.arch_profile.W4.acdc.step\endcsname{544.8}
\expandafter\gdef\csname R@an.arch_profile.W4.amos.act\endcsname{2210}
\expandafter\gdef\csname R@an.arch_profile.W4.amos.dwshare\endcsname{2.15}
\expandafter\gdef\csname R@an.arch_profile.W4.amos.gmac\endcsname{480.5}
\expandafter\gdef\csname R@an.arch_profile.W4.amos.params\endcsname{34.23}
\expandafter\gdef\csname R@an.arch_profile.W4.amos.paramsexact\endcsname{34\,226\,192}
\expandafter\gdef\csname R@an.arch_profile.W4.amos.peak\endcsname{10.51}
\expandafter\gdef\csname R@an.arch_profile.W4.amos.step\endcsname{493.2}
\expandafter\gdef\csname R@an.arch_profile.W4.kits.act\endcsname{1533}
\expandafter\gdef\csname R@an.arch_profile.W4.kits.dwshare\endcsname{1.22}
\expandafter\gdef\csname R@an.arch_profile.W4.kits.gmac\endcsname{452.6}
\expandafter\gdef\csname R@an.arch_profile.W4.kits.params\endcsname{34.30}
\expandafter\gdef\csname R@an.arch_profile.W4.kits.paramsexact\endcsname{34\,298\,223}
\expandafter\gdef\csname R@an.arch_profile.W4.kits.peak\endcsname{9.45}
\expandafter\gdef\csname R@an.arch_profile.W4.kits.step\endcsname{323.5}
\expandafter\gdef\csname R@an.arch_profile.W5.acdc.act\endcsname{790}
\expandafter\gdef\csname R@an.arch_profile.W5.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.W5.acdc.gmac\endcsname{587.3}
\expandafter\gdef\csname R@an.arch_profile.W5.acdc.params\endcsname{101.63}
\expandafter\gdef\csname R@an.arch_profile.W5.acdc.paramsexact\endcsname{101\,626\,548}
\expandafter\gdef\csname R@an.arch_profile.W5.acdc.peak\endcsname{10.66}
\expandafter\gdef\csname R@an.arch_profile.W5.acdc.step\endcsname{200.4}
\expandafter\gdef\csname R@an.arch_profile.W5.amos.act\endcsname{1374}
\expandafter\gdef\csname R@an.arch_profile.W5.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.W5.amos.gmac\endcsname{959.3}
\expandafter\gdef\csname R@an.arch_profile.W5.amos.params\endcsname{102.37}
\expandafter\gdef\csname R@an.arch_profile.W5.amos.paramsexact\endcsname{102\,373\,488}
\expandafter\gdef\csname R@an.arch_profile.W5.amos.peak\endcsname{10.69}
\expandafter\gdef\csname R@an.arch_profile.W5.amos.step\endcsname{192.8}
\expandafter\gdef\csname R@an.arch_profile.W5.kits.act\endcsname{1020}
\expandafter\gdef\csname R@an.arch_profile.W5.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.W5.kits.gmac\endcsname{659.6}
\expandafter\gdef\csname R@an.arch_profile.W5.kits.params\endcsname{102.43}
\expandafter\gdef\csname R@an.arch_profile.W5.kits.paramsexact\endcsname{102\,427\,087}
\expandafter\gdef\csname R@an.arch_profile.W5.kits.peak\endcsname{9.47}
\expandafter\gdef\csname R@an.arch_profile.W5.kits.step\endcsname{150.8}
\expandafter\gdef\csname R@an.arch_profile.band.acdc.all3structures.hi\endcsname{73}
\expandafter\gdef\csname R@an.arch_profile.band.acdc.all3structures.lo\endcsname{44}
\expandafter\gdef\csname R@an.arch_profile.band.amos.largest3organs.hi\endcsname{135}
\expandafter\gdef\csname R@an.arch_profile.band.amos.largest3organs.lo\endcsname{59}
\expandafter\gdef\csname R@an.arch_profile.band.amos.smallest3organs.hi\endcsname{31}
\expandafter\gdef\csname R@an.arch_profile.band.amos.smallest3organs.lo\endcsname{17}
\expandafter\gdef\csname R@an.arch_profile.band.kits.kidney.hi\endcsname{112}
\expandafter\gdef\csname R@an.arch_profile.band.kits.kidney.lo\endcsname{82}
\expandafter\gdef\csname R@an.arch_profile.band.kits.tumour.hi\endcsname{72}
\expandafter\gdef\csname R@an.arch_profile.band.kits.tumour.lo\endcsname{18}
\expandafter\gdef\csname R@an.arch_profile.bar.allocated.gb\endcsname{11.6}
\expandafter\gdef\csname R@an.arch_profile.bar.reserved.gb\endcsname{12}
\expandafter\gdef\csname R@an.arch_profile.base.acdc.act\endcsname{557}
\expandafter\gdef\csname R@an.arch_profile.base.acdc.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.base.acdc.gmac\endcsname{315.3}
\expandafter\gdef\csname R@an.arch_profile.base.acdc.params\endcsname{30.38}
\expandafter\gdef\csname R@an.arch_profile.base.acdc.paramsexact\endcsname{30\,377\,428}
\expandafter\gdef\csname R@an.arch_profile.base.acdc.peak\endcsname{10.27}
\expandafter\gdef\csname R@an.arch_profile.base.acdc.step\endcsname{142.0}
\expandafter\gdef\csname R@an.arch_profile.base.amos.act\endcsname{981}
\expandafter\gdef\csname R@an.arch_profile.base.amos.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.base.amos.gmac\endcsname{527.0}
\expandafter\gdef\csname R@an.arch_profile.base.amos.params\endcsname{31.12}
\expandafter\gdef\csname R@an.arch_profile.base.amos.paramsexact\endcsname{31\,124\,368}
\expandafter\gdef\csname R@an.arch_profile.base.amos.peak\endcsname{9.01}
\expandafter\gdef\csname R@an.arch_profile.base.amos.step\endcsname{140.4}
\expandafter\gdef\csname R@an.arch_profile.base.kits.act\endcsname{811}
\expandafter\gdef\csname R@an.arch_profile.base.kits.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.base.kits.gmac\endcsname{477.4}
\expandafter\gdef\csname R@an.arch_profile.base.kits.params\endcsname{31.20}
\expandafter\gdef\csname R@an.arch_profile.base.kits.paramsexact\endcsname{31\,196\,399}
\expandafter\gdef\csname R@an.arch_profile.base.kits.peak\endcsname{8.51}
\expandafter\gdef\csname R@an.arch_profile.base.kits.step\endcsname{123.3}
\expandafter\gdef\csname R@an.arch_profile.batch.acdc\endcsname{4}
\expandafter\gdef\csname R@an.arch_profile.batch.amos\endcsname{2}
\expandafter\gdef\csname R@an.arch_profile.batch.kits\endcsname{2}
\expandafter\gdef\csname R@an.arch_profile.cap.gb\endcsname{12}
\expandafter\gdef\csname R@an.arch_profile.cover.D1.amos.level\endcsname{4}
\expandafter\gdef\csname R@an.arch_profile.cover.D1.amos.margin.mm\endcsname{63.0}
\expandafter\gdef\csname R@an.arch_profile.cover.D1.amos.rf.mm\endcsname{114.3}
\expandafter\gdef\csname R@an.arch_profile.cover.D1.kits.level\endcsname{3}
\expandafter\gdef\csname R@an.arch_profile.cover.D1.kits.margin.mm\endcsname{13.0}
\expandafter\gdef\csname R@an.arch_profile.cover.D1.kits.rf.mm\endcsname{49.2}
\expandafter\gdef\csname R@an.arch_profile.cover.D2.amos.level\endcsname{5}
\expandafter\gdef\csname R@an.arch_profile.cover.D2.amos.margin.mm\endcsname{13.7}
\expandafter\gdef\csname R@an.arch_profile.cover.D2.amos.rf.mm\endcsname{65.0}
\expandafter\gdef\csname R@an.arch_profile.cover.D2.kits.level\endcsname{4}
\expandafter\gdef\csname R@an.arch_profile.cover.D2.kits.margin.mm\endcsname{0.5}
\expandafter\gdef\csname R@an.arch_profile.cover.D2.kits.rf.mm\endcsname{36.7}
\expandafter\gdef\csname R@an.arch_profile.cover.L1.amos.level\endcsname{3}
\expandafter\gdef\csname R@an.arch_profile.cover.L1.amos.margin.mm\endcsname{9.6}
\expandafter\gdef\csname R@an.arch_profile.cover.L1.amos.rf.mm\endcsname{60.9}
\expandafter\gdef\csname R@an.arch_profile.cover.L1.kits.level\endcsname{3}
\expandafter\gdef\csname R@an.arch_profile.cover.L1.kits.margin.mm\endcsname{33.3}
\expandafter\gdef\csname R@an.arch_profile.cover.L1.kits.rf.mm\endcsname{69.5}
\expandafter\gdef\csname R@an.arch_profile.cover.L2.amos.level\endcsname{4}
\expandafter\gdef\csname R@an.arch_profile.cover.L2.amos.margin.mm\endcsname{11.0}
\expandafter\gdef\csname R@an.arch_profile.cover.L2.amos.rf.mm\endcsname{62.3}
\expandafter\gdef\csname R@an.arch_profile.cover.L2.kits.level\endcsname{4}
\expandafter\gdef\csname R@an.arch_profile.cover.L2.kits.margin.mm\endcsname{34.9}
\expandafter\gdef\csname R@an.arch_profile.cover.L2.kits.rf.mm\endcsname{71.1}
\expandafter\gdef\csname R@an.arch_profile.cover.L3.amos.level\endcsname{4}
\expandafter\gdef\csname R@an.arch_profile.cover.L3.amos.margin.mm\endcsname{63.0}
\expandafter\gdef\csname R@an.arch_profile.cover.L3.amos.rf.mm\endcsname{114.3}
\expandafter\gdef\csname R@an.arch_profile.cover.L3.kits.level\endcsname{3}
\expandafter\gdef\csname R@an.arch_profile.cover.L3.kits.margin.mm\endcsname{13.0}
\expandafter\gdef\csname R@an.arch_profile.cover.L3.kits.rf.mm\endcsname{49.2}
\expandafter\gdef\csname R@an.arch_profile.cover.L3k3.amos.level\endcsname{4}
\expandafter\gdef\csname R@an.arch_profile.cover.L3k3.amos.margin.mm\endcsname{30.1}
\expandafter\gdef\csname R@an.arch_profile.cover.L3k3.amos.rf.mm\endcsname{81.5}
\expandafter\gdef\csname R@an.arch_profile.cover.L3k3.kits.level\endcsname{3}
\expandafter\gdef\csname R@an.arch_profile.cover.L3k3.kits.margin.mm\endcsname{13.0}
\expandafter\gdef\csname R@an.arch_profile.cover.L3k3.kits.rf.mm\endcsname{49.2}
\expandafter\gdef\csname R@an.arch_profile.cover.S2.amos.level\endcsname{4}
\expandafter\gdef\csname R@an.arch_profile.cover.S2.amos.margin.mm\endcsname{68.5}
\expandafter\gdef\csname R@an.arch_profile.cover.S2.amos.rf.mm\endcsname{119.8}
\expandafter\gdef\csname R@an.arch_profile.cover.S2.kits.level\endcsname{3}
\expandafter\gdef\csname R@an.arch_profile.cover.S2.kits.margin.mm\endcsname{19.3}
\expandafter\gdef\csname R@an.arch_profile.cover.S2.kits.rf.mm\endcsname{55.5}
\expandafter\gdef\csname R@an.arch_profile.cover.base.amos.level\endcsname{5}
\expandafter\gdef\csname R@an.arch_profile.cover.base.amos.margin.mm\endcsname{13.7}
\expandafter\gdef\csname R@an.arch_profile.cover.base.amos.rf.mm\endcsname{65.0}
\expandafter\gdef\csname R@an.arch_profile.cover.base.kits.level\endcsname{4}
\expandafter\gdef\csname R@an.arch_profile.cover.base.kits.margin.mm\endcsname{0.5}
\expandafter\gdef\csname R@an.arch_profile.cover.base.kits.rf.mm\endcsname{36.7}
\expandafter\gdef\csname R@an.arch_profile.fit.gmac_params.n\endcsname{136}
\expandafter\gdef\csname R@an.arch_profile.fit.gmac_params.r2\endcsname{0.476}
\expandafter\gdef\csname R@an.arch_profile.fit.gmac_params.r2.dp2\endcsname{0.48}
\expandafter\gdef\csname R@an.arch_profile.fit.gmac_params.slope\endcsname{0.65}
\expandafter\gdef\csname R@an.arch_profile.fit.n_designs\endcsname{47}
\expandafter\gdef\csname R@an.arch_profile.fit.n_points\endcsname{136}
\expandafter\gdef\csname R@an.arch_profile.fit.peak_act.acdc.r2\endcsname{0.614}
\expandafter\gdef\csname R@an.arch_profile.fit.peak_act.amos.r2\endcsname{0.817}
\expandafter\gdef\csname R@an.arch_profile.fit.peak_act.kits.r2\endcsname{0.778}
\expandafter\gdef\csname R@an.arch_profile.fit.peak_act.linear.gb_per_Gelem\endcsname{1.08}
\expandafter\gdef\csname R@an.arch_profile.fit.peak_act.linear.intercept\endcsname{6.96}
\expandafter\gdef\csname R@an.arch_profile.fit.peak_act.linear.r2\endcsname{0.638}
\expandafter\gdef\csname R@an.arch_profile.fit.peak_act.n\endcsname{136}
\expandafter\gdef\csname R@an.arch_profile.fit.peak_act.r2\endcsname{0.756}
\expandafter\gdef\csname R@an.arch_profile.fit.peak_act.r2.dp2\endcsname{0.76}
\expandafter\gdef\csname R@an.arch_profile.fit.peak_act.slope\endcsname{0.30}
\expandafter\gdef\csname R@an.arch_profile.fit.peak_act1.n\endcsname{136}
\expandafter\gdef\csname R@an.arch_profile.fit.peak_act1.r2\endcsname{0.163}
\expandafter\gdef\csname R@an.arch_profile.fit.peak_act1.r2.dp2\endcsname{0.16}
\expandafter\gdef\csname R@an.arch_profile.fit.peak_act1.slope\endcsname{0.12}
\expandafter\gdef\csname R@an.arch_profile.fit.resid_dwshare.step_act.r\endcsname{0.30}
\expandafter\gdef\csname R@an.arch_profile.fit.resid_dwshare.step_gmac.r\endcsname{0.70}
\expandafter\gdef\csname R@an.arch_profile.fit.resid_dwshare.step_gmac_batch.r\endcsname{0.79}
\expandafter\gdef\csname R@an.arch_profile.fit.step_act.n\endcsname{136}
\expandafter\gdef\csname R@an.arch_profile.fit.step_act.r2\endcsname{0.854}
\expandafter\gdef\csname R@an.arch_profile.fit.step_act.r2.dp2\endcsname{0.85}
\expandafter\gdef\csname R@an.arch_profile.fit.step_act.slope\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.fit.step_gmac.acdc.r2\endcsname{0.577}
\expandafter\gdef\csname R@an.arch_profile.fit.step_gmac.amos.r2\endcsname{0.571}
\expandafter\gdef\csname R@an.arch_profile.fit.step_gmac.kits.r2\endcsname{0.690}
\expandafter\gdef\csname R@an.arch_profile.fit.step_gmac.n\endcsname{136}
\expandafter\gdef\csname R@an.arch_profile.fit.step_gmac.r2\endcsname{0.417}
\expandafter\gdef\csname R@an.arch_profile.fit.step_gmac.r2.dp2\endcsname{0.42}
\expandafter\gdef\csname R@an.arch_profile.fit.step_gmac.slope\endcsname{0.50}
\expandafter\gdef\csname R@an.arch_profile.fit.step_gmac_batch.n\endcsname{136}
\expandafter\gdef\csname R@an.arch_profile.fit.step_gmac_batch.r2\endcsname{0.620}
\expandafter\gdef\csname R@an.arch_profile.fit.step_gmac_batch.r2.dp2\endcsname{0.62}
\expandafter\gdef\csname R@an.arch_profile.fit.step_gmac_batch.slope\endcsname{0.67}
\expandafter\gdef\csname R@an.arch_profile.fit.step_params.n\endcsname{136}
\expandafter\gdef\csname R@an.arch_profile.fit.step_params.r2\endcsname{0.254}
\expandafter\gdef\csname R@an.arch_profile.fit.step_params.r2.dp2\endcsname{0.25}
\expandafter\gdef\csname R@an.arch_profile.fit.step_params.slope\endcsname{0.37}
\expandafter\gdef\csname R@an.arch_profile.fits.C1.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.C1.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.C1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.C1.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.C1.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.C1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.C1.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.D1.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.D1.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.D1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.D1.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.D1.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.D1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.D1.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.D2.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.D2.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.D2.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.D2.brats\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.D2.btcv\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.D2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.D2.lits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.I1.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.I1.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.I1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.I1.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.I1.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.I1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.I1.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L1.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L1.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L1.brats\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L1.btcv\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L1.lits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L1b.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L1b.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L1b.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L1b.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L1b.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L1b.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L1b.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L2.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L2.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L2.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L2.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L2.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L2.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L3.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L3.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L3.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L3.brats\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L3.btcv\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L3.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L3.lits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L3k3.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L3k3.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L3k3.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L3k3.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L3k3.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L3k3.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L3k3.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L3ng.acdc\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.fits.L3ng.all\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.fits.L3ng.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L3ng.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L3ng.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L3ng.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L3ng.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L3w_L.acdc\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.fits.L3w_L.all\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.fits.L3w_L.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L3w_L.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L3w_L.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L3w_L.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L3w_L.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L3w_M.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L3w_M.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L3w_M.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L3w_M.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L3w_M.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L3w_M.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L3w_M.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L4.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L4.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L4.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L4.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L4.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L4.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L4.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L6.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L6.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L6.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L6.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L6.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.L6.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.L6.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.N1.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.N1.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.N1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.N1.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.N1.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.N1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.N1.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.P1_frcap32.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P1_frcap32.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P1_frcap32.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P1_frcap32.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.P1_frcap32.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.P1_frcap32.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P1_frcap32.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.P1b.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P1b.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P1b.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P1b.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.P1b.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.P1b.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P1b.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.P1c.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P1c.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P1c.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P1c.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.P1c.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.P1c.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P1c.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.P3c.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P3c.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P3c.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P3c.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.P3c.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.P3c.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P3c.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.P3lite.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P3lite.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P3lite.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P3lite.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.P3lite.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.P3lite.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.P3lite.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.S2.acdc\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.fits.S2.all\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.fits.S2.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.S2.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.S2.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.S2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.S2.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.SP1.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.SP1.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.SP1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.SP1.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.SP1.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.SP1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.SP1.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.SP2.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.SP2.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.SP2.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.SP2.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.SP2.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.SP2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.SP2.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.V5A5.acdc\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.fits.V5A5.all\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.fits.V5A5.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V5A5.brats\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V5A5.btcv\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V5A5.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V5A5.lits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V5B1.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V5B1.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V5B1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V5B1.brats\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V5B1.btcv\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V5B1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V5B1.lits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V5B2.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V5B2.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V5B2.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V5B2.brats\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V5B2.btcv\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V5B2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V5B2.lits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V6A1r.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V6A1r.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V6A1r.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V6A1r.brats\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V6A1r.btcv\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V6A1r.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V6A1r.lits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A1.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A1.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A1.brats\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A1.btcv\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A1.lits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A2.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A2.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A2.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A2.brats\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A2.btcv\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A2.lits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A3.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A3.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A3.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A3.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A3.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A3.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7A3.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.V7B1.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7B1.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7B1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7B1.brats\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7B1.btcv\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7B1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7B1.lits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7B2.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7B2.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7B2.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7B2.brats\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7B2.btcv\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7B2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7B2.lits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7C1.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7C1.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7C1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7C1.brats\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7C1.btcv\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7C1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7C1.lits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7C2.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7C2.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7C2.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7C2.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.V7C2.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.V7C2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V7C2.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.V8A1.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8A1.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8A1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8A1.brats\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8A1.btcv\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8A1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8A1.lits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8A2.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8A2.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8A2.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8A2.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.V8A2.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.V8A2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8A2.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.V8B1.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8B1.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8B1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8B1.brats\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8B1.btcv\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8B1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8B1.lits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8B2.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8B2.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8B2.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8B2.brats\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8B2.btcv\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8B2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8B2.lits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8X1.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8X1.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8X1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8X1.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.V8X1.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.V8X1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.V8X1.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W1.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W1.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W1.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W1.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W1.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W1c.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W1c.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W1c.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W1c.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W1c.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W1c.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W1c.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W2.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W2.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W2.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W2.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W2.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W2.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W3.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W3.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W3.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W3.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W3.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W3.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W3.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W3c.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W3c.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W3c.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W3c.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W3c.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W3c.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W3c.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W4.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W4.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W4.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W4.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W4.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W4.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W4.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W5.acdc\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.fits.W5.all\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.fits.W5.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W5.brats\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W5.btcv\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.W5.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.W5.lits\endcsname{\pend}
\expandafter\gdef\csname R@an.arch_profile.fits.base.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.base.all\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.base.amos\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.base.brats\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.base.btcv\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.base.kits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.fits.base.lits\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.frag.max.gb\endcsname{1.60}
\expandafter\gdef\csname R@an.arch_profile.heads.D1.amos.params\endcsname{12\,880}
\expandafter\gdef\csname R@an.arch_profile.heads.D2.amos.params\endcsname{12\,880}
\expandafter\gdef\csname R@an.arch_profile.heads.L1.amos.params\endcsname{12\,880}
\expandafter\gdef\csname R@an.arch_profile.heads.L3.amos.params\endcsname{12\,880}
\expandafter\gdef\csname R@an.arch_profile.heads.base.amos.params\endcsname{12\,880}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.1.act\endcsname{692}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.1.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.1.gmac\endcsname{77.1}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.1.params\endcsname{0.046}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.2.act\endcsname{472}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.2.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.2.gmac\endcsname{358.4}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.2.params\endcsname{0.788}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.3.act\endcsname{165}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.3.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.3.gmac\endcsname{235.6}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.3.params\endcsname{4.067}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.4.act\endcsname{57}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.4.dwshare\endcsname{4.57}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.4.gmac\endcsname{21.5}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.4.params\endcsname{3.387}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.5.act\endcsname{11}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.5.dwshare\endcsname{8.94}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.5.gmac\endcsname{5.9}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.5.params\endcsname{6.880}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.6.act\endcsname{1.0}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.6.dwshare\endcsname{7.75}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.6.gmac\endcsname{0.7}
\expandafter\gdef\csname R@an.arch_profile.lvl.D1.amos.6.params\endcsname{5.679}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.1.act\endcsname{440}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.1.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.1.gmac\endcsname{59.0}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.1.params\endcsname{0.036}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.2.act\endcsname{220}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.2.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.2.gmac\endcsname{194.3}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.2.params\endcsname{0.453}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.3.act\endcsname{55}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.3.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.3.gmac\endcsname{97.1}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.3.params\endcsname{1.812}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.4.act\endcsname{14}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.4.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.4.gmac\endcsname{48.2}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.4.params\endcsname{6.851}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.5.act\endcsname{2.2}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.5.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.5.gmac\endcsname{10.2}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.5.params\endcsname{11.329}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.6.act\endcsname{0.2}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.6.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.6.gmac\endcsname{0.7}
\expandafter\gdef\csname R@an.arch_profile.lvl.D2.amos.6.params\endcsname{5.532}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.1.act\endcsname{566}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.1.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.1.gmac\endcsname{77.1}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.1.params\endcsname{0.046}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.2.act\endcsname{535}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.2.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.2.gmac\endcsname{412.7}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.2.params\endcsname{0.899}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.3.act\endcsname{165}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.3.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.3.gmac\endcsname{260.7}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.3.params\endcsname{4.477}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.4.act\endcsname{57}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.4.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.4.gmac\endcsname{184.3}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.4.params\endcsname{24.587}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.5.act\endcsname{8.9}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.5.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.5.gmac\endcsname{36.8}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.5.params\endcsname{39.069}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.6.act\endcsname{0.9}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.6.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.6.gmac\endcsname{4.0}
\expandafter\gdef\csname R@an.arch_profile.lvl.L1.amos.6.params\endcsname{33.189}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.1.act\endcsname{692}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.1.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.1.gmac\endcsname{77.1}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.1.params\endcsname{0.046}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.2.act\endcsname{472}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.2.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.2.gmac\endcsname{358.4}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.2.params\endcsname{0.788}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.3.act\endcsname{165}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.3.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.3.gmac\endcsname{235.6}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.3.params\endcsname{4.067}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.4.act\endcsname{57}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.4.dwshare\endcsname{2.06}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.4.gmac\endcsname{47.7}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.4.params\endcsname{6.795}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.5.act\endcsname{11}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.5.dwshare\endcsname{4.79}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.5.gmac\endcsname{11.0}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.5.params\endcsname{12.204}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.6.act\endcsname{1.0}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.6.dwshare\endcsname{7.75}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.6.gmac\endcsname{0.7}
\expandafter\gdef\csname R@an.arch_profile.lvl.L3.amos.6.params\endcsname{5.679}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.1.act\endcsname{566}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.1.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.1.gmac\endcsname{77.1}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.1.params\endcsname{0.046}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.2.act\endcsname{283}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.2.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.2.gmac\endcsname{248.6}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.2.params\endcsname{0.564}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.3.act\endcsname{71}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.3.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.3.gmac\endcsname{124.3}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.3.params\endcsname{2.254}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.4.act\endcsname{18}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.4.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.4.gmac\endcsname{61.8}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.4.params\endcsname{8.621}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.5.act\endcsname{2.8}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.5.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.5.gmac\endcsname{12.8}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.5.params\endcsname{14.094}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.6.act\endcsname{0.2}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.6.dwshare\endcsname{0.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.6.gmac\endcsname{0.7}
\expandafter\gdef\csname R@an.arch_profile.lvl.base.amos.6.params\endcsname{5.532}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D1.amos.1.act\endcsname{+22}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D1.amos.1.gmac\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D1.amos.1.params\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D1.amos.2.act\endcsname{+67}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D1.amos.2.gmac\endcsname{+44}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D1.amos.2.params\endcsname{+40}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D1.amos.3.act\endcsname{+133}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D1.amos.3.gmac\endcsname{+89}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D1.amos.3.params\endcsname{+80}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D1.amos.4.act\endcsname{+222}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D1.amos.4.gmac\endcsname{$-$65}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D1.amos.4.params\endcsname{$-$61}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D1.amos.5.act\endcsname{+289}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D1.amos.5.gmac\endcsname{$-$54}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D1.amos.5.params\endcsname{$-$51}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D1.amos.6.act\endcsname{+550}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D1.amos.6.gmac\endcsname{+2}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D1.amos.6.params\endcsname{+3}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D2.amos.1.act\endcsname{$-$22}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D2.amos.1.gmac\endcsname{$-$24}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D2.amos.1.params\endcsname{$-$20}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D2.amos.2.act\endcsname{$-$22}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D2.amos.2.gmac\endcsname{$-$22}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D2.amos.2.params\endcsname{$-$20}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D2.amos.3.act\endcsname{$-$22}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D2.amos.3.gmac\endcsname{$-$22}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D2.amos.3.params\endcsname{$-$20}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D2.amos.4.act\endcsname{$-$22}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D2.amos.4.gmac\endcsname{$-$22}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D2.amos.4.params\endcsname{$-$21}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D2.amos.5.act\endcsname{$-$22}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D2.amos.5.gmac\endcsname{$-$21}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D2.amos.5.params\endcsname{$-$20}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D2.amos.6.act\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D2.amos.6.gmac\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.D2.amos.6.params\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L1.amos.1.act\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L1.amos.1.gmac\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L1.amos.1.params\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L1.amos.2.act\endcsname{+89}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L1.amos.2.gmac\endcsname{+66}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L1.amos.2.params\endcsname{+59}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L1.amos.3.act\endcsname{+133}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L1.amos.3.gmac\endcsname{+110}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L1.amos.3.params\endcsname{+99}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L1.amos.4.act\endcsname{+222}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L1.amos.4.gmac\endcsname{+198}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L1.amos.4.params\endcsname{+185}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L1.amos.5.act\endcsname{+222}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L1.amos.5.gmac\endcsname{+187}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L1.amos.5.params\endcsname{+177}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L1.amos.6.act\endcsname{+500}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L1.amos.6.gmac\endcsname{+500}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L1.amos.6.params\endcsname{+500}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L3.amos.1.act\endcsname{+22}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L3.amos.1.gmac\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L3.amos.1.params\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L3.amos.2.act\endcsname{+67}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L3.amos.2.gmac\endcsname{+44}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L3.amos.2.params\endcsname{+40}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L3.amos.3.act\endcsname{+133}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L3.amos.3.gmac\endcsname{+89}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L3.amos.3.params\endcsname{+80}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L3.amos.4.act\endcsname{+222}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L3.amos.4.gmac\endcsname{$-$23}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L3.amos.4.params\endcsname{$-$21}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L3.amos.5.act\endcsname{+289}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L3.amos.5.gmac\endcsname{$-$14}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L3.amos.5.params\endcsname{$-$13}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L3.amos.6.act\endcsname{+550}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L3.amos.6.gmac\endcsname{+2}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.L3.amos.6.params\endcsname{+3}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.base.amos.1.act\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.base.amos.1.gmac\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.base.amos.1.params\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.base.amos.2.act\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.base.amos.2.gmac\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.base.amos.2.params\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.base.amos.3.act\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.base.amos.3.gmac\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.base.amos.3.params\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.base.amos.4.act\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.base.amos.4.gmac\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.base.amos.4.params\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.base.amos.5.act\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.base.amos.5.gmac\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.base.amos.5.params\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.base.amos.6.act\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.base.amos.6.gmac\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.pct.base.amos.6.params\endcsname{+0}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D1.amos.1.act\endcsname{1.22}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D1.amos.1.gmac\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D1.amos.1.params\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D1.amos.2.act\endcsname{1.67}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D1.amos.2.gmac\endcsname{1.44}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D1.amos.2.params\endcsname{1.40}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D1.amos.3.act\endcsname{2.33}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D1.amos.3.gmac\endcsname{1.89}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D1.amos.3.params\endcsname{1.80}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D1.amos.4.act\endcsname{3.22}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D1.amos.4.gmac\endcsname{0.35}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D1.amos.4.params\endcsname{0.39}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D1.amos.5.act\endcsname{3.89}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D1.amos.5.gmac\endcsname{0.46}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D1.amos.5.params\endcsname{0.49}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D1.amos.6.act\endcsname{6.50}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D1.amos.6.gmac\endcsname{1.02}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D1.amos.6.params\endcsname{1.03}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D2.amos.1.act\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D2.amos.1.gmac\endcsname{0.76}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D2.amos.1.params\endcsname{0.80}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D2.amos.2.act\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D2.amos.2.gmac\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D2.amos.2.params\endcsname{0.80}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D2.amos.3.act\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D2.amos.3.gmac\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D2.amos.3.params\endcsname{0.80}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D2.amos.4.act\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D2.amos.4.gmac\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D2.amos.4.params\endcsname{0.79}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D2.amos.5.act\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D2.amos.5.gmac\endcsname{0.79}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D2.amos.5.params\endcsname{0.80}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D2.amos.6.act\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D2.amos.6.gmac\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.D2.amos.6.params\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L1.amos.1.act\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L1.amos.1.gmac\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L1.amos.1.params\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L1.amos.2.act\endcsname{1.89}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L1.amos.2.gmac\endcsname{1.66}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L1.amos.2.params\endcsname{1.59}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L1.amos.3.act\endcsname{2.33}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L1.amos.3.gmac\endcsname{2.10}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L1.amos.3.params\endcsname{1.99}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L1.amos.4.act\endcsname{3.22}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L1.amos.4.gmac\endcsname{2.98}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L1.amos.4.params\endcsname{2.85}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L1.amos.5.act\endcsname{3.22}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L1.amos.5.gmac\endcsname{2.87}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L1.amos.5.params\endcsname{2.77}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L1.amos.6.act\endcsname{6.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L1.amos.6.gmac\endcsname{6.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L1.amos.6.params\endcsname{6.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L3.amos.1.act\endcsname{1.22}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L3.amos.1.gmac\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L3.amos.1.params\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L3.amos.2.act\endcsname{1.67}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L3.amos.2.gmac\endcsname{1.44}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L3.amos.2.params\endcsname{1.40}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L3.amos.3.act\endcsname{2.33}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L3.amos.3.gmac\endcsname{1.89}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L3.amos.3.params\endcsname{1.80}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L3.amos.4.act\endcsname{3.22}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L3.amos.4.gmac\endcsname{0.77}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L3.amos.4.params\endcsname{0.79}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L3.amos.5.act\endcsname{3.89}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L3.amos.5.gmac\endcsname{0.86}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L3.amos.5.params\endcsname{0.87}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L3.amos.6.act\endcsname{6.50}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L3.amos.6.gmac\endcsname{1.02}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.L3.amos.6.params\endcsname{1.03}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.base.amos.1.act\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.base.amos.1.gmac\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.base.amos.1.params\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.base.amos.2.act\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.base.amos.2.gmac\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.base.amos.2.params\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.base.amos.3.act\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.base.amos.3.gmac\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.base.amos.3.params\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.base.amos.4.act\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.base.amos.4.gmac\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.base.amos.4.params\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.base.amos.5.act\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.base.amos.5.gmac\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.base.amos.5.params\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.base.amos.6.act\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.base.amos.6.gmac\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.lvl.ratio.base.amos.6.params\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.n.cloud\endcsname{21}
\expandafter\gdef\csname R@an.arch_profile.n.cloud.points\endcsname{41}
\expandafter\gdef\csname R@an.arch_profile.n.cloud.sampled\endcsname{24}
\expandafter\gdef\csname R@an.arch_profile.n.cloud.skipped\endcsname{31}
\expandafter\gdef\csname R@an.arch_profile.n.designs\endcsname{47}
\expandafter\gdef\csname R@an.arch_profile.n.plans\endcsname{3}
\expandafter\gdef\csname R@an.arch_profile.nfits\endcsname{136}
\expandafter\gdef\csname R@an.arch_profile.nfits.n.word\endcsname{136}
\expandafter\gdef\csname R@an.arch_profile.nfits.total\endcsname{141}
\expandafter\gdef\csname R@an.arch_profile.nofit.allocated.n\endcsname{4}
\expandafter\gdef\csname R@an.arch_profile.nofit.n\endcsname{5}
\expandafter\gdef\csname R@an.arch_profile.nofit.n.word\endcsname{five}
\expandafter\gdef\csname R@an.arch_profile.nofit.names\endcsname{HyReX w/o GRN on ACDC; HyReX-L (scaled) on ACDC; HyReX, finer ConvNeXt on ACDC; HyReX-LeanDec on ACDC; pooled-skip control on ACDC}
\expandafter\gdef\csname R@an.arch_profile.nofit.plans\endcsname{ACDC}
\expandafter\gdef\csname R@an.arch_profile.nofit.reserved.n\endcsname{2}
\expandafter\gdef\csname R@an.arch_profile.nofit.why\endcsname{HyReX w/o GRN on ACDC (allocated 11.70 GB over the 11.6 GB bar); HyReX-L (scaled) on ACDC (allocated 11.72 GB over the 11.6 GB bar and reserved 12.00 GB over the 12 GB cap); HyReX, finer ConvNeXt on ACDC (allocated 11.72 GB over the 11.6 GB bar); HyReX-LeanDec on ACDC (allocated 11.74 GB over the 11.6 GB bar); pooled-skip control on ACDC (reserved 12.00 GB over the 12 GB cap)}
\expandafter\gdef\csname R@an.arch_profile.op.axial_dw13.s1.ms\endcsname{36.04}
\expandafter\gdef\csname R@an.arch_profile.op.axial_dw13.s1.ratio\endcsname{5.7}
\expandafter\gdef\csname R@an.arch_profile.op.axial_dw13.s2.ms\endcsname{9.40}
\expandafter\gdef\csname R@an.arch_profile.op.axial_dw13.s2.ratio\endcsname{4.5}
\expandafter\gdef\csname R@an.arch_profile.op.axial_dw13.s3.ms\endcsname{2.42}
\expandafter\gdef\csname R@an.arch_profile.op.axial_dw13.s3.ratio\endcsname{2.5}
\expandafter\gdef\csname R@an.arch_profile.op.axial_dw13.s4.ms\endcsname{0.56}
\expandafter\gdef\csname R@an.arch_profile.op.axial_dw13.s4.ratio\endcsname{1.5}
\expandafter\gdef\csname R@an.arch_profile.op.axial_dw7.s1.ms\endcsname{26.16}
\expandafter\gdef\csname R@an.arch_profile.op.axial_dw7.s1.ratio\endcsname{4.2}
\expandafter\gdef\csname R@an.arch_profile.op.axial_dw7.s2.ms\endcsname{6.81}
\expandafter\gdef\csname R@an.arch_profile.op.axial_dw7.s2.ratio\endcsname{3.2}
\expandafter\gdef\csname R@an.arch_profile.op.axial_dw7.s3.ms\endcsname{1.66}
\expandafter\gdef\csname R@an.arch_profile.op.axial_dw7.s3.ratio\endcsname{1.7}
\expandafter\gdef\csname R@an.arch_profile.op.axial_dw7.s4.ms\endcsname{0.50}
\expandafter\gdef\csname R@an.arch_profile.op.axial_dw7.s4.ratio\endcsname{1.3}
\expandafter\gdef\csname R@an.arch_profile.op.bottleneck_r4.s1.ms\endcsname{8.20}
\expandafter\gdef\csname R@an.arch_profile.op.bottleneck_r4.s1.ratio\endcsname{1.3}
\expandafter\gdef\csname R@an.arch_profile.op.bottleneck_r4.s2.ms\endcsname{1.71}
\expandafter\gdef\csname R@an.arch_profile.op.bottleneck_r4.s2.ratio\endcsname{0.8}
\expandafter\gdef\csname R@an.arch_profile.op.bottleneck_r4.s3.ms\endcsname{1.24}
\expandafter\gdef\csname R@an.arch_profile.op.bottleneck_r4.s3.ratio\endcsname{1.3}
\expandafter\gdef\csname R@an.arch_profile.op.bottleneck_r4.s4.ms\endcsname{1.11}
\expandafter\gdef\csname R@an.arch_profile.op.bottleneck_r4.s4.ratio\endcsname{2.9}
\expandafter\gdef\csname R@an.arch_profile.op.convnext_k3_e2.s1.ms\endcsname{19.90}
\expandafter\gdef\csname R@an.arch_profile.op.convnext_k3_e2.s1.ratio\endcsname{3.2}
\expandafter\gdef\csname R@an.arch_profile.op.convnext_k3_e2.s2.ms\endcsname{5.11}
\expandafter\gdef\csname R@an.arch_profile.op.convnext_k3_e2.s2.ratio\endcsname{2.4}
\expandafter\gdef\csname R@an.arch_profile.op.convnext_k3_e2.s3.ms\endcsname{1.38}
\expandafter\gdef\csname R@an.arch_profile.op.convnext_k3_e2.s3.ratio\endcsname{1.4}
\expandafter\gdef\csname R@an.arch_profile.op.convnext_k3_e2.s4.ms\endcsname{0.84}
\expandafter\gdef\csname R@an.arch_profile.op.convnext_k3_e2.s4.ratio\endcsname{2.2}
\expandafter\gdef\csname R@an.arch_profile.op.convnext_k5_e2.s1.ms\endcsname{68.60}
\expandafter\gdef\csname R@an.arch_profile.op.convnext_k5_e2.s1.ratio\endcsname{10.9}
\expandafter\gdef\csname R@an.arch_profile.op.convnext_k5_e2.s2.ms\endcsname{17.40}
\expandafter\gdef\csname R@an.arch_profile.op.convnext_k5_e2.s2.ratio\endcsname{8.3}
\expandafter\gdef\csname R@an.arch_profile.op.convnext_k5_e2.s3.ms\endcsname{4.58}
\expandafter\gdef\csname R@an.arch_profile.op.convnext_k5_e2.s3.ratio\endcsname{4.7}
\expandafter\gdef\csname R@an.arch_profile.op.convnext_k5_e2.s4.ms\endcsname{1.21}
\expandafter\gdef\csname R@an.arch_profile.op.convnext_k5_e2.s4.ratio\endcsname{3.2}
\expandafter\gdef\csname R@an.arch_profile.op.dense3x3x3.s1.ms\endcsname{6.27}
\expandafter\gdef\csname R@an.arch_profile.op.dense3x3x3.s1.ratio\endcsname{1.0}
\expandafter\gdef\csname R@an.arch_profile.op.dense3x3x3.s2.ms\endcsname{2.10}
\expandafter\gdef\csname R@an.arch_profile.op.dense3x3x3.s2.ratio\endcsname{1.0}
\expandafter\gdef\csname R@an.arch_profile.op.dense3x3x3.s3.ms\endcsname{0.98}
\expandafter\gdef\csname R@an.arch_profile.op.dense3x3x3.s3.ratio\endcsname{1.0}
\expandafter\gdef\csname R@an.arch_profile.op.dense3x3x3.s4.ms\endcsname{0.38}
\expandafter\gdef\csname R@an.arch_profile.op.dense3x3x3.s4.ratio\endcsname{1.0}
\expandafter\gdef\csname R@an.arch_profile.op.dense3x3x3_IN_lrelu.s1.ms\endcsname{9.42}
\expandafter\gdef\csname R@an.arch_profile.op.dense3x3x3_IN_lrelu.s1.ratio\endcsname{1.5}
\expandafter\gdef\csname R@an.arch_profile.op.dense3x3x3_IN_lrelu.s2.ms\endcsname{2.46}
\expandafter\gdef\csname R@an.arch_profile.op.dense3x3x3_IN_lrelu.s2.ratio\endcsname{1.2}
\expandafter\gdef\csname R@an.arch_profile.op.dense3x3x3_IN_lrelu.s3.ms\endcsname{1.07}
\expandafter\gdef\csname R@an.arch_profile.op.dense3x3x3_IN_lrelu.s3.ratio\endcsname{1.1}
\expandafter\gdef\csname R@an.arch_profile.op.dense3x3x3_IN_lrelu.s4.ms\endcsname{0.63}
\expandafter\gdef\csname R@an.arch_profile.op.dense3x3x3_IN_lrelu.s4.ratio\endcsname{1.7}
\expandafter\gdef\csname R@an.arch_profile.op.device\endcsname{A100-SXM4-80GB}
\expandafter\gdef\csname R@an.arch_profile.op.dilated3x3x3_d2.s1.ms\endcsname{20.28}
\expandafter\gdef\csname R@an.arch_profile.op.dilated3x3x3_d2.s1.ratio\endcsname{3.2}
\expandafter\gdef\csname R@an.arch_profile.op.dilated3x3x3_d2.s2.ms\endcsname{2.09}
\expandafter\gdef\csname R@an.arch_profile.op.dilated3x3x3_d2.s2.ratio\endcsname{1.0}
\expandafter\gdef\csname R@an.arch_profile.op.dilated3x3x3_d2.s3.ms\endcsname{0.97}
\expandafter\gdef\csname R@an.arch_profile.op.dilated3x3x3_d2.s3.ratio\endcsname{1.0}
\expandafter\gdef\csname R@an.arch_profile.op.dilated3x3x3_d2.s4.ms\endcsname{0.41}
\expandafter\gdef\csname R@an.arch_profile.op.dilated3x3x3_d2.s4.ratio\endcsname{1.1}
\expandafter\gdef\csname R@an.arch_profile.op.dw3.s1.ms\endcsname{10.69}
\expandafter\gdef\csname R@an.arch_profile.op.dw3.s1.ratio\endcsname{1.7}
\expandafter\gdef\csname R@an.arch_profile.op.dw3.s2.ms\endcsname{2.85}
\expandafter\gdef\csname R@an.arch_profile.op.dw3.s2.ratio\endcsname{1.4}
\expandafter\gdef\csname R@an.arch_profile.op.dw3.s3.ms\endcsname{0.75}
\expandafter\gdef\csname R@an.arch_profile.op.dw3.s3.ratio\endcsname{0.8}
\expandafter\gdef\csname R@an.arch_profile.op.dw3.s4.ms\endcsname{0.26}
\expandafter\gdef\csname R@an.arch_profile.op.dw3.s4.ratio\endcsname{0.7}
\expandafter\gdef\csname R@an.arch_profile.op.dw5.s1.ms\endcsname{59.41}
\expandafter\gdef\csname R@an.arch_profile.op.dw5.s1.ratio\endcsname{9.5}
\expandafter\gdef\csname R@an.arch_profile.op.dw5.s2.ms\endcsname{15.14}
\expandafter\gdef\csname R@an.arch_profile.op.dw5.s2.ratio\endcsname{7.2}
\expandafter\gdef\csname R@an.arch_profile.op.dw5.s3.ms\endcsname{3.95}
\expandafter\gdef\csname R@an.arch_profile.op.dw5.s3.ratio\endcsname{4.0}
\expandafter\gdef\csname R@an.arch_profile.op.dw5.s4.ms\endcsname{0.92}
\expandafter\gdef\csname R@an.arch_profile.op.dw5.s4.ratio\endcsname{2.4}
\expandafter\gdef\csname R@an.arch_profile.op.dw7.s1.ms\endcsname{143.91}
\expandafter\gdef\csname R@an.arch_profile.op.dw7.s1.ratio\endcsname{23.0}
\expandafter\gdef\csname R@an.arch_profile.op.dw7.s2.ms\endcsname{36.62}
\expandafter\gdef\csname R@an.arch_profile.op.dw7.s2.ratio\endcsname{17.4}
\expandafter\gdef\csname R@an.arch_profile.op.dw7.s3.ms\endcsname{9.59}
\expandafter\gdef\csname R@an.arch_profile.op.dw7.s3.ratio\endcsname{9.8}
\expandafter\gdef\csname R@an.arch_profile.op.dw7.s4.ms\endcsname{2.23}
\expandafter\gdef\csname R@an.arch_profile.op.dw7.s4.ratio\endcsname{5.9}
\expandafter\gdef\csname R@an.arch_profile.op.dw7_vs_dense.s1\endcsname{23}
\expandafter\gdef\csname R@an.arch_profile.op.dw7_vs_dense.s4\endcsname{5.9}
\expandafter\gdef\csname R@an.arch_profile.op.grouped3x3x3_g8.s1.ms\endcsname{6.66}
\expandafter\gdef\csname R@an.arch_profile.op.grouped3x3x3_g8.s1.ratio\endcsname{1.1}
\expandafter\gdef\csname R@an.arch_profile.op.grouped3x3x3_g8.s2.ms\endcsname{1.81}
\expandafter\gdef\csname R@an.arch_profile.op.grouped3x3x3_g8.s2.ratio\endcsname{0.9}
\expandafter\gdef\csname R@an.arch_profile.op.grouped3x3x3_g8.s3.ms\endcsname{0.51}
\expandafter\gdef\csname R@an.arch_profile.op.grouped3x3x3_g8.s3.ratio\endcsname{0.5}
\expandafter\gdef\csname R@an.arch_profile.op.grouped3x3x3_g8.s4.ms\endcsname{0.41}
\expandafter\gdef\csname R@an.arch_profile.op.grouped3x3x3_g8.s4.ratio\endcsname{1.1}
\expandafter\gdef\csname R@an.arch_profile.op.pw_1x1_c_to_2c.s1.ms\endcsname{4.19}
\expandafter\gdef\csname R@an.arch_profile.op.pw_1x1_c_to_2c.s1.ratio\endcsname{0.7}
\expandafter\gdef\csname R@an.arch_profile.op.pw_1x1_c_to_2c.s2.ms\endcsname{1.14}
\expandafter\gdef\csname R@an.arch_profile.op.pw_1x1_c_to_2c.s2.ratio\endcsname{0.5}
\expandafter\gdef\csname R@an.arch_profile.op.pw_1x1_c_to_2c.s3.ms\endcsname{0.51}
\expandafter\gdef\csname R@an.arch_profile.op.pw_1x1_c_to_2c.s3.ratio\endcsname{0.5}
\expandafter\gdef\csname R@an.arch_profile.op.pw_1x1_c_to_2c.s4.ms\endcsname{0.34}
\expandafter\gdef\csname R@an.arch_profile.op.pw_1x1_c_to_2c.s4.ratio\endcsname{0.9}
\expandafter\gdef\csname R@an.arch_profile.op.stage.s1.level\endcsname{2}
\expandafter\gdef\csname R@an.arch_profile.op.stage.s2.level\endcsname{3}
\expandafter\gdef\csname R@an.arch_profile.op.stage.s3.level\endcsname{4}
\expandafter\gdef\csname R@an.arch_profile.op.stage.s4.level\endcsname{5}
\expandafter\gdef\csname R@an.arch_profile.patch.acdc.xy.mm\endcsname{390}
\expandafter\gdef\csname R@an.arch_profile.patch.acdc.z.mm\endcsname{100}
\expandafter\gdef\csname R@an.arch_profile.patch.amos.xy.mm\endcsname{131}
\expandafter\gdef\csname R@an.arch_profile.patch.amos.z.mm\endcsname{128}
\expandafter\gdef\csname R@an.arch_profile.patch.kits.xy.mm\endcsname{100}
\expandafter\gdef\csname R@an.arch_profile.patch.kits.z.mm\endcsname{128}
\expandafter\gdef\csname R@an.arch_profile.peak.max.gb\endcsname{11.74}
\expandafter\gdef\csname R@an.arch_profile.peak.min.gb\endcsname{6.96}
\expandafter\gdef\csname R@an.arch_profile.pub.mednextl3.vram\endcsname{17.3}
\expandafter\gdef\csname R@an.arch_profile.pub.mednextl5.vram\endcsname{18.0}
\expandafter\gdef\csname R@an.arch_profile.pub.n.over_cap\endcsname{7}
\expandafter\gdef\csname R@an.arch_profile.pub.n.total\endcsname{10}
\expandafter\gdef\csname R@an.arch_profile.pub.nnformer.vram\endcsname{5.7}
\expandafter\gdef\csname R@an.arch_profile.pub.nnunet.vram\endcsname{7.7}
\expandafter\gdef\csname R@an.arch_profile.pub.over_cap.names\endcsname{nnU-Net ResEnc-XL; STU-Net-L; nnU-Net ResEnc-L; MedNeXt-L, $k{=}5$; MedNeXt-L, $k{=}3$; SwinUNETR-V2; U-Mamba-Bot}
\expandafter\gdef\csname R@an.arch_profile.pub.resencl.vram\endcsname{22.7}
\expandafter\gdef\csname R@an.arch_profile.pub.resencm.vram\endcsname{9.1}
\expandafter\gdef\csname R@an.arch_profile.pub.resencxl.vram\endcsname{36.6}
\expandafter\gdef\csname R@an.arch_profile.pub.stunetl.vram\endcsname{26.5}
\expandafter\gdef\csname R@an.arch_profile.pub.swinunetrv2.vram\endcsname{13.4}
\expandafter\gdef\csname R@an.arch_profile.pub.umambabot.vram\endcsname{12.4}
\expandafter\gdef\csname R@an.arch_profile.pub10.best.names\endcsname{STU-Net-L, SwinUNETR-V2 and U-Mamba-Bot}
\expandafter\gdef\csname R@an.arch_profile.pub10.n\endcsname{10}
\expandafter\gdef\csname R@an.arch_profile.pub10.n.families.best\endcsname{3}
\expandafter\gdef\csname R@an.arch_profile.pub10.n.families.omitted\endcsname{3}
\expandafter\gdef\csname R@an.arch_profile.pub10.n.families.whole\endcsname{4}
\expandafter\gdef\csname R@an.arch_profile.pub10.n.omitted\endcsname{9}
\expandafter\gdef\csname R@an.arch_profile.pub10.n.omitted.over_cap\endcsname{5}
\expandafter\gdef\csname R@an.arch_profile.pub10.n.omitted.within_cap\endcsname{4}
\expandafter\gdef\csname R@an.arch_profile.pub10.n.over_cap\endcsname{7}
\expandafter\gdef\csname R@an.arch_profile.pub10.n.within_cap\endcsname{3}
\expandafter\gdef\csname R@an.arch_profile.pub10.omitted.families\endcsname{CoTr, No-Mamba Base, A3DS SegResNet, A3DS DiNTS and A3DS SwinUNETR}
\expandafter\gdef\csname R@an.arch_profile.pub10.omitted.names\endcsname{STU-Net-S, STU-Net-B, SwinUNETR, CoTr, No-Mamba Base, U-Mamba-Enc, A3DS SegResNet, A3DS DiNTS and A3DS SwinUNETR}
\expandafter\gdef\csname R@an.arch_profile.pub10.omitted.variants\endcsname{STU-Net-S, STU-Net-B, SwinUNETR and U-Mamba-Enc}
\expandafter\gdef\csname R@an.arch_profile.pub10.rule\endcsname{every row of the families nnU-Net, ResEnc, MedNeXt and nnFormer and, of each other family with several variants, the variant with the highest mean Dice over ACDC, AMOS22 and KiTS23 (STU-Net-L, SwinUNETR-V2 and U-Mamba-Bot)}
\expandafter\gdef\csname R@an.arch_profile.pub10.score\endcsname{mean Dice over ACDC, AMOS22 and KiTS23}
\expandafter\gdef\csname R@an.arch_profile.pub10.whole.families\endcsname{nnU-Net, ResEnc, MedNeXt and nnFormer}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsdints.acdc\endcsname{82.97}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsdints.amos\endcsname{82.35}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsdints.arch\endcsname{CNN}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsdints.class\endcsname{above}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsdints.dicetable\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsdints.hours\endcsname{16}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsdints.kits\endcsname{65.28}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsdints.label\endcsname{A3DS DiNTS}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsdints.margin\endcsname{+17.2}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsdints.nnu\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsdints.short\endcsname{A3DS DiNTS}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsdints.vram\endcsname{29.2}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dssegresnet.acdc\endcsname{90.69}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dssegresnet.amos\endcsname{87.27}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dssegresnet.arch\endcsname{CNN}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dssegresnet.class\endcsname{above}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dssegresnet.dicetable\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dssegresnet.hours\endcsname{22}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dssegresnet.kits\endcsname{81.11}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dssegresnet.label\endcsname{A3DS SegResNet}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dssegresnet.margin\endcsname{+8.0}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dssegresnet.nnu\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dssegresnet.short\endcsname{A3DS SegResNet}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dssegresnet.vram\endcsname{20.0}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsswinunetr.acdc\endcsname{82.68}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsswinunetr.amos\endcsname{85.05}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsswinunetr.arch\endcsname{TF}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsswinunetr.class\endcsname{above}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsswinunetr.dicetable\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsswinunetr.hours\endcsname{9}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsswinunetr.kits\endcsname{52.82}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsswinunetr.label\endcsname{A3DS SwinUNETR}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsswinunetr.margin\endcsname{+22.5}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsswinunetr.nnu\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsswinunetr.short\endcsname{A3DS SwinUNETR}
\expandafter\gdef\csname R@an.arch_profile.pub19.a3dsswinunetr.vram\endcsname{34.5}
\expandafter\gdef\csname R@an.arch_profile.pub19.arch.cnn.at_cap\endcsname{1}
\expandafter\gdef\csname R@an.arch_profile.pub19.arch.cnn.below_cap\endcsname{4}
\expandafter\gdef\csname R@an.arch_profile.pub19.arch.cnn.over_cap\endcsname{7}
\expandafter\gdef\csname R@an.arch_profile.pub19.arch.cnn.total\endcsname{12}
\expandafter\gdef\csname R@an.arch_profile.pub19.arch.cnn.within_cap\endcsname{5}
\expandafter\gdef\csname R@an.arch_profile.pub19.arch.mam.at_cap\endcsname{0}
\expandafter\gdef\csname R@an.arch_profile.pub19.arch.mam.below_cap\endcsname{0}
\expandafter\gdef\csname R@an.arch_profile.pub19.arch.mam.over_cap\endcsname{2}
\expandafter\gdef\csname R@an.arch_profile.pub19.arch.mam.total\endcsname{2}
\expandafter\gdef\csname R@an.arch_profile.pub19.arch.mam.within_cap\endcsname{0}
\expandafter\gdef\csname R@an.arch_profile.pub19.arch.tf.at_cap\endcsname{0}
\expandafter\gdef\csname R@an.arch_profile.pub19.arch.tf.below_cap\endcsname{2}
\expandafter\gdef\csname R@an.arch_profile.pub19.arch.tf.over_cap\endcsname{3}
\expandafter\gdef\csname R@an.arch_profile.pub19.arch.tf.total\endcsname{5}
\expandafter\gdef\csname R@an.arch_profile.pub19.arch.tf.within_cap\endcsname{2}
\expandafter\gdef\csname R@an.arch_profile.pub19.at_cap.names\endcsname{No-Mamba Base}
\expandafter\gdef\csname R@an.arch_profile.pub19.below_cap.names\endcsname{ResEnc-M, STU-Net-B, CoTr, nnU-Net, nnFormer and STU-Net-S}
\expandafter\gdef\csname R@an.arch_profile.pub19.cap.gb\endcsname{12}
\expandafter\gdef\csname R@an.arch_profile.pub19.cotr.acdc\endcsname{90.56}
\expandafter\gdef\csname R@an.arch_profile.pub19.cotr.amos\endcsname{88.02}
\expandafter\gdef\csname R@an.arch_profile.pub19.cotr.arch\endcsname{TF}
\expandafter\gdef\csname R@an.arch_profile.pub19.cotr.class\endcsname{within}
\expandafter\gdef\csname R@an.arch_profile.pub19.cotr.dicetable\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.pub19.cotr.hours\endcsname{18}
\expandafter\gdef\csname R@an.arch_profile.pub19.cotr.kits\endcsname{84.59}
\expandafter\gdef\csname R@an.arch_profile.pub19.cotr.label\endcsname{CoTr}
\expandafter\gdef\csname R@an.arch_profile.pub19.cotr.margin\endcsname{$-$3.8}
\expandafter\gdef\csname R@an.arch_profile.pub19.cotr.nnu\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.cotr.short\endcsname{CoTr}
\expandafter\gdef\csname R@an.arch_profile.pub19.cotr.vram\endcsname{8.2}
\expandafter\gdef\csname R@an.arch_profile.pub19.cv.folds\endcsname{5}
\expandafter\gdef\csname R@an.arch_profile.pub19.gain.l.acdc\endcsname{$-$0.30}
\expandafter\gdef\csname R@an.arch_profile.pub19.gain.l.amos\endcsname{+0.64}
\expandafter\gdef\csname R@an.arch_profile.pub19.gain.l.kits\endcsname{+1.38}
\expandafter\gdef\csname R@an.arch_profile.pub19.gain.xl.acdc\endcsname{$-$0.51}
\expandafter\gdef\csname R@an.arch_profile.pub19.gain.xl.amos\endcsname{+0.91}
\expandafter\gdef\csname R@an.arch_profile.pub19.gain.xl.kits\endcsname{+1.88}
\expandafter\gdef\csname R@an.arch_profile.pub19.gpu.resencl\endcsname{24}
\expandafter\gdef\csname R@an.arch_profile.pub19.gpu.resencm.hi\endcsname{11}
\expandafter\gdef\csname R@an.arch_profile.pub19.gpu.resencm.lo\endcsname{9}
\expandafter\gdef\csname R@an.arch_profile.pub19.gpu.resencxl\endcsname{40}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl3.acdc\endcsname{92.65}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl3.amos\endcsname{89.62}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl3.arch\endcsname{CNN}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl3.class\endcsname{above}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl3.dicetable\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl3.hours\endcsname{68}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl3.kits\endcsname{88.25}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl3.label\endcsname{MedNeXt-L, $k{=}3$}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl3.margin\endcsname{+5.3}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl3.nnu\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl3.short\endcsname{MedNeXt-L k3}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl3.vram\endcsname{17.3}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl5.acdc\endcsname{92.62}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl5.amos\endcsname{89.73}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl5.arch\endcsname{CNN}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl5.class\endcsname{above}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl5.dicetable\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl5.hours\endcsname{233}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl5.kits\endcsname{87.74}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl5.label\endcsname{MedNeXt-L, $k{=}5$}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl5.margin\endcsname{+6.0}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl5.nnu\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl5.short\endcsname{MedNeXt-L k5}
\expandafter\gdef\csname R@an.arch_profile.pub19.mednextl5.vram\endcsname{18.0}
\expandafter\gdef\csname R@an.arch_profile.pub19.n.at_cap\endcsname{1}
\expandafter\gdef\csname R@an.arch_profile.pub19.n.below_cap\endcsname{6}
\expandafter\gdef\csname R@an.arch_profile.pub19.n.dicecols\endcsname{6}
\expandafter\gdef\csname R@an.arch_profile.pub19.n.no_vram\endcsname{0}
\expandafter\gdef\csname R@an.arch_profile.pub19.n.over_cap\endcsname{12}
\expandafter\gdef\csname R@an.arch_profile.pub19.n.total\endcsname{19}
\expandafter\gdef\csname R@an.arch_profile.pub19.n.with_vram\endcsname{19}
\expandafter\gdef\csname R@an.arch_profile.pub19.n.within_cap\endcsname{7}
\expandafter\gdef\csname R@an.arch_profile.pub19.ncases.acdc\endcsname{200}
\expandafter\gdef\csname R@an.arch_profile.pub19.ncases.amos\endcsname{360}
\expandafter\gdef\csname R@an.arch_profile.pub19.ncases.kits\endcsname{489}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnformer.acdc\endcsname{92.40}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnformer.amos\endcsname{81.55}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnformer.arch\endcsname{TF}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnformer.class\endcsname{within}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnformer.dicetable\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnformer.hours\endcsname{8}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnformer.kits\endcsname{75.85}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnformer.label\endcsname{nnFormer}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnformer.margin\endcsname{$-$6.3}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnformer.nnu\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnformer.short\endcsname{nnFormer}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnformer.vram\endcsname{5.7}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnu.at_cap\endcsname{1}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnu.below_cap\endcsname{6}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnu.over_cap\endcsname{9}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnu.total\endcsname{16}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnu.within_cap\endcsname{7}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnunet.acdc\endcsname{91.54}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnunet.amos\endcsname{88.64}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnunet.arch\endcsname{CNN}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnunet.class\endcsname{within}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnunet.dicetable\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnunet.hours\endcsname{9}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnunet.kits\endcsname{86.04}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnunet.label\endcsname{nnU-Net (orig.)}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnunet.margin\endcsname{$-$4.3}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnunet.nnu\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnunet.short\endcsname{nnU-Net}
\expandafter\gdef\csname R@an.arch_profile.pub19.nnunet.vram\endcsname{7.7}
\expandafter\gdef\csname R@an.arch_profile.pub19.nomambabase.acdc\endcsname{91.89}
\expandafter\gdef\csname R@an.arch_profile.pub19.nomambabase.amos\endcsname{89.04}
\expandafter\gdef\csname R@an.arch_profile.pub19.nomambabase.arch\endcsname{CNN}
\expandafter\gdef\csname R@an.arch_profile.pub19.nomambabase.class\endcsname{within}
\expandafter\gdef\csname R@an.arch_profile.pub19.nomambabase.dicetable\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.pub19.nomambabase.hours\endcsname{24}
\expandafter\gdef\csname R@an.arch_profile.pub19.nomambabase.kits\endcsname{85.98}
\expandafter\gdef\csname R@an.arch_profile.pub19.nomambabase.label\endcsname{No-Mamba Base}
\expandafter\gdef\csname R@an.arch_profile.pub19.nomambabase.margin\endcsname{0.0}
\expandafter\gdef\csname R@an.arch_profile.pub19.nomambabase.nnu\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.nomambabase.short\endcsname{No-Mamba Base}
\expandafter\gdef\csname R@an.arch_profile.pub19.nomambabase.vram\endcsname{12.0}
\expandafter\gdef\csname R@an.arch_profile.pub19.nonnu.at_cap\endcsname{0}
\expandafter\gdef\csname R@an.arch_profile.pub19.nonnu.below_cap\endcsname{0}
\expandafter\gdef\csname R@an.arch_profile.pub19.nonnu.over_cap\endcsname{3}
\expandafter\gdef\csname R@an.arch_profile.pub19.nonnu.total\endcsname{3}
\expandafter\gdef\csname R@an.arch_profile.pub19.nonnu.within_cap\endcsname{0}
\expandafter\gdef\csname R@an.arch_profile.pub19.over_cap.names\endcsname{ResEnc-XL, A3DS SwinUNETR, A3DS DiNTS, STU-Net-L, U-Mamba-Enc, ResEnc-L, A3DS SegResNet, MedNeXt-L k5, MedNeXt-L k3, SwinUNETR-V2, SwinUNETR and U-Mamba-Bot}
\expandafter\gdef\csname R@an.arch_profile.pub19.paper.n_match\endcsname{19}
\expandafter\gdef\csname R@an.arch_profile.pub19.paper.n_rows\endcsname{19}
\expandafter\gdef\csname R@an.arch_profile.pub19.pin.kind\endcsname{a transcription of the text the fetch tool returned}
\expandafter\gdef\csname R@an.arch_profile.pub19.price.l.hours\endcsname{2.9}
\expandafter\gdef\csname R@an.arch_profile.pub19.price.l.vram\endcsname{2.5}
\expandafter\gdef\csname R@an.arch_profile.pub19.price.xl.hours\endcsname{5.5}
\expandafter\gdef\csname R@an.arch_profile.pub19.price.xl.vram\endcsname{4.0}
\expandafter\gdef\csname R@an.arch_profile.pub19.reco.class\endcsname{above}
\expandafter\gdef\csname R@an.arch_profile.pub19.reco.preset\endcsname{ResEnc-L}
\expandafter\gdef\csname R@an.arch_profile.pub19.reco.vram\endcsname{22.7}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencl.acdc\endcsname{91.69}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencl.amos\endcsname{89.41}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencl.arch\endcsname{CNN}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencl.class\endcsname{above}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencl.dicetable\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencl.hours\endcsname{35}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencl.kits\endcsname{88.17}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencl.label\endcsname{nnU-Net ResEnc-L}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencl.margin\endcsname{+10.7}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencl.nnu\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencl.short\endcsname{ResEnc-L}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencl.vram\endcsname{22.7}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencm.acdc\endcsname{91.99}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencm.amos\endcsname{88.77}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencm.arch\endcsname{CNN}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencm.class\endcsname{within}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencm.dicetable\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencm.hours\endcsname{12}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencm.kits\endcsname{86.79}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencm.label\endcsname{nnU-Net ResEnc-M}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencm.margin\endcsname{$-$2.9}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencm.nnu\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencm.short\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencm.vram\endcsname{9.1}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencxl.acdc\endcsname{91.48}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencxl.amos\endcsname{89.68}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencxl.arch\endcsname{CNN}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencxl.class\endcsname{above}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencxl.dicetable\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencxl.hours\endcsname{66}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencxl.kits\endcsname{88.67}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencxl.label\endcsname{nnU-Net ResEnc-XL}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencxl.margin\endcsname{+24.6}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencxl.nnu\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencxl.short\endcsname{ResEnc-XL}
\expandafter\gdef\csname R@an.arch_profile.pub19.resencxl.vram\endcsname{36.6}
\expandafter\gdef\csname R@an.arch_profile.pub19.retrieved\endcsname{2026-10-07}
\expandafter\gdef\csname R@an.arch_profile.pub19.rt_vs_vram.n\endcsname{19}
\expandafter\gdef\csname R@an.arch_profile.pub19.rt_vs_vram.n_nnu\endcsname{16}
\expandafter\gdef\csname R@an.arch_profile.pub19.rt_vs_vram.r2\endcsname{0.265}
\expandafter\gdef\csname R@an.arch_profile.pub19.rt_vs_vram.r2_nnu\endcsname{0.605}
\expandafter\gdef\csname R@an.arch_profile.pub19.rt_vs_vram.slope\endcsname{0.76}
\expandafter\gdef\csname R@an.arch_profile.pub19.rt_vs_vram.slope_nnu\endcsname{1.26}
\expandafter\gdef\csname R@an.arch_profile.pub19.sha12\endcsname{848a81b32cb0}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetb.acdc\endcsname{91.30}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetb.amos\endcsname{88.46}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetb.arch\endcsname{CNN}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetb.class\endcsname{within}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetb.dicetable\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetb.hours\endcsname{15}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetb.kits\endcsname{86.32}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetb.label\endcsname{STU-Net-B}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetb.margin\endcsname{$-$3.2}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetb.nnu\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetb.short\endcsname{STU-Net-B}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetb.vram\endcsname{8.8}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetl.acdc\endcsname{91.31}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetl.amos\endcsname{89.34}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetl.arch\endcsname{CNN}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetl.class\endcsname{above}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetl.dicetable\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetl.hours\endcsname{51}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetl.kits\endcsname{85.84}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetl.label\endcsname{STU-Net-L}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetl.margin\endcsname{+14.5}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetl.nnu\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetl.short\endcsname{STU-Net-L}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunetl.vram\endcsname{26.5}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunets.acdc\endcsname{91.04}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunets.amos\endcsname{88.08}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunets.arch\endcsname{CNN}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunets.class\endcsname{within}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunets.dicetable\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunets.hours\endcsname{10}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunets.kits\endcsname{84.93}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunets.label\endcsname{STU-Net-S}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunets.margin\endcsname{$-$6.8}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunets.nnu\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunets.short\endcsname{STU-Net-S}
\expandafter\gdef\csname R@an.arch_profile.pub19.stunets.vram\endcsname{5.2}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetr.acdc\endcsname{91.29}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetr.amos\endcsname{83.81}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetr.arch\endcsname{TF}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetr.class\endcsname{above}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetr.dicetable\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetr.hours\endcsname{15}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetr.kits\endcsname{81.27}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetr.label\endcsname{SwinUNETR}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetr.margin\endcsname{+1.1}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetr.nnu\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetr.short\endcsname{SwinUNETR}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetr.vram\endcsname{13.1}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetrv2.acdc\endcsname{92.01}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetrv2.amos\endcsname{86.24}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetrv2.arch\endcsname{TF}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetrv2.class\endcsname{above}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetrv2.dicetable\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetrv2.hours\endcsname{15}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetrv2.kits\endcsname{84.14}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetrv2.label\endcsname{SwinUNETR-V2}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetrv2.margin\endcsname{+1.4}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetrv2.nnu\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetrv2.short\endcsname{SwinUNETR-V2}
\expandafter\gdef\csname R@an.arch_profile.pub19.swinunetrv2.vram\endcsname{13.4}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambabot.acdc\endcsname{91.79}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambabot.amos\endcsname{89.13}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambabot.arch\endcsname{Mam}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambabot.class\endcsname{above}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambabot.dicetable\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambabot.hours\endcsname{24}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambabot.kits\endcsname{86.22}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambabot.label\endcsname{U-Mamba-Bot}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambabot.margin\endcsname{+0.4}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambabot.nnu\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambabot.short\endcsname{U-Mamba-Bot}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambabot.vram\endcsname{12.4}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambaenc.acdc\endcsname{91.22}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambaenc.amos\endcsname{88.38}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambaenc.arch\endcsname{Mam}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambaenc.class\endcsname{above}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambaenc.dicetable\endcsname{no}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambaenc.hours\endcsname{47}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambaenc.kits\endcsname{86.34}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambaenc.label\endcsname{U-Mamba-Enc}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambaenc.margin\endcsname{+12.9}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambaenc.nnu\endcsname{yes}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambaenc.short\endcsname{U-Mamba-Enc}
\expandafter\gdef\csname R@an.arch_profile.pub19.umambaenc.vram\endcsname{24.9}
\expandafter\gdef\csname R@an.arch_profile.pub19.vram.tool\endcsname{nvidia-smi}
\expandafter\gdef\csname R@an.arch_profile.pub19.within_cap.names\endcsname{No-Mamba Base, ResEnc-M, STU-Net-B, CoTr, nnU-Net, nnFormer and STU-Net-S}
\expandafter\gdef\csname R@an.arch_profile.ratio.C1.acdc.act_vs_default\endcsname{1.54}
\expandafter\gdef\csname R@an.arch_profile.ratio.C1.acdc.gmac_vs_default\endcsname{1.65}
\expandafter\gdef\csname R@an.arch_profile.ratio.C1.acdc.params_vs_default\endcsname{1.70}
\expandafter\gdef\csname R@an.arch_profile.ratio.C1.acdc.step_vs_default\endcsname{1.80}
\expandafter\gdef\csname R@an.arch_profile.ratio.C1.amos.act_vs_default\endcsname{1.51}
\expandafter\gdef\csname R@an.arch_profile.ratio.C1.amos.gmac_vs_default\endcsname{1.64}
\expandafter\gdef\csname R@an.arch_profile.ratio.C1.amos.params_vs_default\endcsname{1.68}
\expandafter\gdef\csname R@an.arch_profile.ratio.C1.amos.step_vs_default\endcsname{1.69}
\expandafter\gdef\csname R@an.arch_profile.ratio.C1.kits.act_vs_default\endcsname{1.41}
\expandafter\gdef\csname R@an.arch_profile.ratio.C1.kits.gmac_vs_default\endcsname{1.38}
\expandafter\gdef\csname R@an.arch_profile.ratio.C1.kits.params_vs_default\endcsname{1.68}
\expandafter\gdef\csname R@an.arch_profile.ratio.C1.kits.step_vs_default\endcsname{1.58}
\expandafter\gdef\csname R@an.arch_profile.ratio.D1.acdc.act_vs_default\endcsname{1.49}
\expandafter\gdef\csname R@an.arch_profile.ratio.D1.acdc.gmac_vs_default\endcsname{1.31}
\expandafter\gdef\csname R@an.arch_profile.ratio.D1.acdc.params_vs_default\endcsname{0.66}
\expandafter\gdef\csname R@an.arch_profile.ratio.D1.acdc.step_vs_default\endcsname{1.63}
\expandafter\gdef\csname R@an.arch_profile.ratio.D1.amos.act_vs_default\endcsname{1.47}
\expandafter\gdef\csname R@an.arch_profile.ratio.D1.amos.gmac_vs_default\endcsname{1.33}
\expandafter\gdef\csname R@an.arch_profile.ratio.D1.amos.params_vs_default\endcsname{0.67}
\expandafter\gdef\csname R@an.arch_profile.ratio.D1.amos.step_vs_default\endcsname{1.52}
\expandafter\gdef\csname R@an.arch_profile.ratio.D1.kits.act_vs_default\endcsname{1.38}
\expandafter\gdef\csname R@an.arch_profile.ratio.D1.kits.gmac_vs_default\endcsname{1.19}
\expandafter\gdef\csname R@an.arch_profile.ratio.D1.kits.params_vs_default\endcsname{0.67}
\expandafter\gdef\csname R@an.arch_profile.ratio.D1.kits.step_vs_default\endcsname{1.40}
\expandafter\gdef\csname R@an.arch_profile.ratio.D2.acdc.act_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.D2.acdc.gmac_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.D2.acdc.params_vs_default\endcsname{0.83}
\expandafter\gdef\csname R@an.arch_profile.ratio.D2.acdc.step_vs_default\endcsname{0.81}
\expandafter\gdef\csname R@an.arch_profile.ratio.D2.amos.act_vs_default\endcsname{0.79}
\expandafter\gdef\csname R@an.arch_profile.ratio.D2.amos.gmac_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.D2.amos.params_vs_default\endcsname{0.84}
\expandafter\gdef\csname R@an.arch_profile.ratio.D2.amos.step_vs_default\endcsname{0.81}
\expandafter\gdef\csname R@an.arch_profile.ratio.D2.kits.act_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.D2.kits.gmac_vs_default\endcsname{0.77}
\expandafter\gdef\csname R@an.arch_profile.ratio.D2.kits.params_vs_default\endcsname{0.84}
\expandafter\gdef\csname R@an.arch_profile.ratio.D2.kits.step_vs_default\endcsname{0.81}
\expandafter\gdef\csname R@an.arch_profile.ratio.I1.acdc.act_vs_default\endcsname{1.49}
\expandafter\gdef\csname R@an.arch_profile.ratio.I1.acdc.gmac_vs_default\endcsname{1.38}
\expandafter\gdef\csname R@an.arch_profile.ratio.I1.acdc.params_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.arch_profile.ratio.I1.acdc.step_vs_default\endcsname{1.64}
\expandafter\gdef\csname R@an.arch_profile.ratio.I1.amos.act_vs_default\endcsname{1.47}
\expandafter\gdef\csname R@an.arch_profile.ratio.I1.amos.gmac_vs_default\endcsname{1.39}
\expandafter\gdef\csname R@an.arch_profile.ratio.I1.amos.params_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.arch_profile.ratio.I1.amos.step_vs_default\endcsname{1.53}
\expandafter\gdef\csname R@an.arch_profile.ratio.I1.kits.act_vs_default\endcsname{1.38}
\expandafter\gdef\csname R@an.arch_profile.ratio.I1.kits.gmac_vs_default\endcsname{1.23}
\expandafter\gdef\csname R@an.arch_profile.ratio.I1.kits.params_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.arch_profile.ratio.I1.kits.step_vs_default\endcsname{1.41}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1.acdc.act_vs_default\endcsname{1.42}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1.acdc.gmac_vs_default\endcsname{1.90}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1.acdc.params_vs_default\endcsname{3.34}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1.acdc.step_vs_default\endcsname{1.51}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1.amos.act_vs_default\endcsname{1.40}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1.amos.gmac_vs_default\endcsname{1.85}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1.amos.params_vs_default\endcsname{3.29}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1.amos.step_vs_default\endcsname{1.46}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1.kits.act_vs_default\endcsname{1.26}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1.kits.gmac_vs_default\endcsname{1.50}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1.kits.params_vs_default\endcsname{3.28}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1.kits.step_vs_default\endcsname{1.33}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1b.acdc.act_vs_default\endcsname{1.42}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1b.acdc.gmac_vs_default\endcsname{1.86}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1b.acdc.params_vs_default\endcsname{3.35}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1b.acdc.step_vs_default\endcsname{1.41}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1b.amos.act_vs_default\endcsname{1.40}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1b.amos.gmac_vs_default\endcsname{1.82}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1b.amos.params_vs_default\endcsname{3.29}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1b.amos.step_vs_default\endcsname{1.38}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1b.kits.act_vs_default\endcsname{1.26}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1b.kits.gmac_vs_default\endcsname{1.38}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1b.kits.params_vs_default\endcsname{3.28}
\expandafter\gdef\csname R@an.arch_profile.ratio.L1b.kits.step_vs_default\endcsname{1.23}
\expandafter\gdef\csname R@an.arch_profile.ratio.L2.acdc.act_vs_default\endcsname{1.64}
\expandafter\gdef\csname R@an.arch_profile.ratio.L2.acdc.gmac_vs_default\endcsname{0.73}
\expandafter\gdef\csname R@an.arch_profile.ratio.L2.acdc.params_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.L2.acdc.step_vs_default\endcsname{1.50}
\expandafter\gdef\csname R@an.arch_profile.ratio.L2.amos.act_vs_default\endcsname{1.62}
\expandafter\gdef\csname R@an.arch_profile.ratio.L2.amos.gmac_vs_default\endcsname{0.73}
\expandafter\gdef\csname R@an.arch_profile.ratio.L2.amos.params_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.L2.amos.step_vs_default\endcsname{1.46}
\expandafter\gdef\csname R@an.arch_profile.ratio.L2.kits.act_vs_default\endcsname{1.48}
\expandafter\gdef\csname R@an.arch_profile.ratio.L2.kits.gmac_vs_default\endcsname{0.84}
\expandafter\gdef\csname R@an.arch_profile.ratio.L2.kits.params_vs_default\endcsname{0.79}
\expandafter\gdef\csname R@an.arch_profile.ratio.L2.kits.step_vs_default\endcsname{1.33}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3.acdc.act_vs_default\endcsname{1.49}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3.acdc.gmac_vs_default\endcsname{1.38}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3.acdc.params_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3.acdc.step_vs_default\endcsname{1.64}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3.amos.act_vs_default\endcsname{1.47}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3.amos.gmac_vs_default\endcsname{1.39}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3.amos.params_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3.amos.step_vs_default\endcsname{1.53}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3.kits.act_vs_default\endcsname{1.38}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3.kits.gmac_vs_default\endcsname{1.23}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3.kits.params_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3.kits.step_vs_default\endcsname{1.40}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3k3.acdc.act_vs_default\endcsname{1.49}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3k3.acdc.gmac_vs_default\endcsname{1.37}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3k3.acdc.params_vs_default\endcsname{0.92}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3k3.acdc.step_vs_default\endcsname{1.38}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3k3.amos.act_vs_default\endcsname{1.47}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3k3.amos.gmac_vs_default\endcsname{1.39}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3k3.amos.params_vs_default\endcsname{0.92}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3k3.amos.step_vs_default\endcsname{1.35}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3k3.kits.act_vs_default\endcsname{1.38}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3k3.kits.gmac_vs_default\endcsname{1.23}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3k3.kits.params_vs_default\endcsname{0.92}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3k3.kits.step_vs_default\endcsname{1.27}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3ng.acdc.act_vs_default\endcsname{1.49}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3ng.acdc.gmac_vs_default\endcsname{1.38}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3ng.acdc.params_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3ng.acdc.step_vs_default\endcsname{1.59}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3ng.amos.act_vs_default\endcsname{1.47}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3ng.amos.gmac_vs_default\endcsname{1.39}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3ng.amos.params_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3ng.amos.step_vs_default\endcsname{1.49}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3ng.kits.act_vs_default\endcsname{1.38}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3ng.kits.gmac_vs_default\endcsname{1.23}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3ng.kits.params_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3ng.kits.step_vs_default\endcsname{1.38}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_L.acdc.act_vs_default\endcsname{1.58}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_L.acdc.gmac_vs_default\endcsname{1.75}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_L.acdc.params_vs_default\endcsname{3.19}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_L.acdc.step_vs_default\endcsname{2.11}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_L.amos.act_vs_default\endcsname{1.54}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_L.amos.gmac_vs_default\endcsname{1.70}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_L.amos.params_vs_default\endcsname{3.21}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_L.amos.step_vs_default\endcsname{1.87}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_L.kits.act_vs_default\endcsname{1.43}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_L.kits.gmac_vs_default\endcsname{1.41}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_L.kits.params_vs_default\endcsname{3.20}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_L.kits.step_vs_default\endcsname{1.66}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_M.acdc.act_vs_default\endcsname{1.53}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_M.acdc.gmac_vs_default\endcsname{1.53}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_M.acdc.params_vs_default\endcsname{1.89}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_M.acdc.step_vs_default\endcsname{1.88}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_M.amos.act_vs_default\endcsname{1.50}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_M.amos.gmac_vs_default\endcsname{1.52}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_M.amos.params_vs_default\endcsname{1.90}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_M.amos.step_vs_default\endcsname{1.70}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_M.kits.act_vs_default\endcsname{1.41}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_M.kits.gmac_vs_default\endcsname{1.31}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_M.kits.params_vs_default\endcsname{1.89}
\expandafter\gdef\csname R@an.arch_profile.ratio.L3w_M.kits.step_vs_default\endcsname{1.54}
\expandafter\gdef\csname R@an.arch_profile.ratio.L4.acdc.act_vs_default\endcsname{1.42}
\expandafter\gdef\csname R@an.arch_profile.ratio.L4.acdc.gmac_vs_default\endcsname{1.86}
\expandafter\gdef\csname R@an.arch_profile.ratio.L4.acdc.params_vs_default\endcsname{3.36}
\expandafter\gdef\csname R@an.arch_profile.ratio.L4.acdc.step_vs_default\endcsname{1.52}
\expandafter\gdef\csname R@an.arch_profile.ratio.L4.amos.act_vs_default\endcsname{1.40}
\expandafter\gdef\csname R@an.arch_profile.ratio.L4.amos.gmac_vs_default\endcsname{1.82}
\expandafter\gdef\csname R@an.arch_profile.ratio.L4.amos.params_vs_default\endcsname{3.30}
\expandafter\gdef\csname R@an.arch_profile.ratio.L4.amos.step_vs_default\endcsname{1.46}
\expandafter\gdef\csname R@an.arch_profile.ratio.L4.kits.act_vs_default\endcsname{1.26}
\expandafter\gdef\csname R@an.arch_profile.ratio.L4.kits.gmac_vs_default\endcsname{1.38}
\expandafter\gdef\csname R@an.arch_profile.ratio.L4.kits.params_vs_default\endcsname{3.30}
\expandafter\gdef\csname R@an.arch_profile.ratio.L4.kits.step_vs_default\endcsname{1.30}
\expandafter\gdef\csname R@an.arch_profile.ratio.L6.acdc.act_vs_default\endcsname{1.66}
\expandafter\gdef\csname R@an.arch_profile.ratio.L6.acdc.gmac_vs_default\endcsname{1.68}
\expandafter\gdef\csname R@an.arch_profile.ratio.L6.acdc.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.L6.acdc.step_vs_default\endcsname{2.03}
\expandafter\gdef\csname R@an.arch_profile.ratio.L6.amos.act_vs_default\endcsname{1.63}
\expandafter\gdef\csname R@an.arch_profile.ratio.L6.amos.gmac_vs_default\endcsname{1.70}
\expandafter\gdef\csname R@an.arch_profile.ratio.L6.amos.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.L6.amos.step_vs_default\endcsname{1.88}
\expandafter\gdef\csname R@an.arch_profile.ratio.L6.kits.act_vs_default\endcsname{1.49}
\expandafter\gdef\csname R@an.arch_profile.ratio.L6.kits.gmac_vs_default\endcsname{1.41}
\expandafter\gdef\csname R@an.arch_profile.ratio.L6.kits.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.L6.kits.step_vs_default\endcsname{1.63}
\expandafter\gdef\csname R@an.arch_profile.ratio.N1.acdc.act_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.N1.acdc.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.N1.acdc.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.N1.acdc.step_vs_default\endcsname{1.60}
\expandafter\gdef\csname R@an.arch_profile.ratio.N1.amos.act_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.N1.amos.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.N1.amos.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.N1.amos.step_vs_default\endcsname{2.06}
\expandafter\gdef\csname R@an.arch_profile.ratio.N1.kits.act_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.N1.kits.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.N1.kits.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.N1.kits.step_vs_default\endcsname{2.14}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1_frcap32.acdc.act_vs_default\endcsname{2.19}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1_frcap32.acdc.gmac_vs_default\endcsname{1.27}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1_frcap32.acdc.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1_frcap32.acdc.step_vs_default\endcsname{2.15}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1_frcap32.amos.act_vs_default\endcsname{2.15}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1_frcap32.amos.gmac_vs_default\endcsname{1.28}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1_frcap32.amos.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1_frcap32.amos.step_vs_default\endcsname{2.15}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1_frcap32.kits.act_vs_default\endcsname{2.49}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1_frcap32.kits.gmac_vs_default\endcsname{1.97}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1_frcap32.kits.params_vs_default\endcsname{1.01}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1_frcap32.kits.step_vs_default\endcsname{2.65}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1b.acdc.act_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1b.acdc.gmac_vs_default\endcsname{1.27}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1b.acdc.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1b.acdc.step_vs_default\endcsname{1.09}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1b.amos.act_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1b.amos.gmac_vs_default\endcsname{1.28}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1b.amos.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1b.amos.step_vs_default\endcsname{1.07}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1b.kits.act_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1b.kits.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1b.kits.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1b.kits.step_vs_default\endcsname{1.01}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1c.acdc.act_vs_default\endcsname{1.02}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1c.acdc.gmac_vs_default\endcsname{1.05}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1c.acdc.params_vs_default\endcsname{1.01}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1c.acdc.step_vs_default\endcsname{1.02}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1c.amos.act_vs_default\endcsname{1.02}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1c.amos.gmac_vs_default\endcsname{1.05}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1c.amos.params_vs_default\endcsname{1.01}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1c.amos.step_vs_default\endcsname{1.02}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1c.kits.act_vs_default\endcsname{1.01}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1c.kits.gmac_vs_default\endcsname{1.03}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1c.kits.params_vs_default\endcsname{1.01}
\expandafter\gdef\csname R@an.arch_profile.ratio.P1c.kits.step_vs_default\endcsname{1.01}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3c.acdc.act_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3c.acdc.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3c.acdc.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3c.acdc.step_vs_default\endcsname{1.04}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3c.amos.act_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3c.amos.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3c.amos.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3c.amos.step_vs_default\endcsname{1.05}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3c.kits.act_vs_default\endcsname{1.01}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3c.kits.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3c.kits.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3c.kits.step_vs_default\endcsname{1.03}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3lite.acdc.act_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3lite.acdc.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3lite.acdc.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3lite.acdc.step_vs_default\endcsname{1.03}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3lite.amos.act_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3lite.amos.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3lite.amos.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3lite.amos.step_vs_default\endcsname{1.05}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3lite.kits.act_vs_default\endcsname{1.01}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3lite.kits.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3lite.kits.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.P3lite.kits.step_vs_default\endcsname{1.03}
\expandafter\gdef\csname R@an.arch_profile.ratio.S2.acdc.act_vs_default\endcsname{1.54}
\expandafter\gdef\csname R@an.arch_profile.ratio.S2.acdc.gmac_vs_default\endcsname{1.16}
\expandafter\gdef\csname R@an.arch_profile.ratio.S2.acdc.params_vs_default\endcsname{0.89}
\expandafter\gdef\csname R@an.arch_profile.ratio.S2.acdc.step_vs_default\endcsname{2.11}
\expandafter\gdef\csname R@an.arch_profile.ratio.S2.amos.act_vs_default\endcsname{1.51}
\expandafter\gdef\csname R@an.arch_profile.ratio.S2.amos.gmac_vs_default\endcsname{1.17}
\expandafter\gdef\csname R@an.arch_profile.ratio.S2.amos.params_vs_default\endcsname{0.89}
\expandafter\gdef\csname R@an.arch_profile.ratio.S2.amos.step_vs_default\endcsname{1.96}
\expandafter\gdef\csname R@an.arch_profile.ratio.S2.kits.act_vs_default\endcsname{1.41}
\expandafter\gdef\csname R@an.arch_profile.ratio.S2.kits.gmac_vs_default\endcsname{1.10}
\expandafter\gdef\csname R@an.arch_profile.ratio.S2.kits.params_vs_default\endcsname{0.89}
\expandafter\gdef\csname R@an.arch_profile.ratio.S2.kits.step_vs_default\endcsname{1.68}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP1.acdc.act_vs_default\endcsname{1.86}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP1.acdc.gmac_vs_default\endcsname{2.10}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP1.acdc.params_vs_default\endcsname{3.53}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP1.acdc.step_vs_default\endcsname{1.97}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP1.amos.act_vs_default\endcsname{1.83}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP1.amos.gmac_vs_default\endcsname{2.06}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP1.amos.params_vs_default\endcsname{3.47}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP1.amos.step_vs_default\endcsname{1.91}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP1.kits.act_vs_default\endcsname{1.70}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP1.kits.gmac_vs_default\endcsname{1.63}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP1.kits.params_vs_default\endcsname{3.46}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP1.kits.step_vs_default\endcsname{1.69}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP2.acdc.act_vs_default\endcsname{1.73}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP2.acdc.gmac_vs_default\endcsname{2.13}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP2.acdc.params_vs_default\endcsname{3.53}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP2.acdc.step_vs_default\endcsname{2.15}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP2.amos.act_vs_default\endcsname{1.70}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP2.amos.gmac_vs_default\endcsname{2.09}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP2.amos.params_vs_default\endcsname{3.47}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP2.amos.step_vs_default\endcsname{2.07}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP2.kits.act_vs_default\endcsname{1.53}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP2.kits.gmac_vs_default\endcsname{1.74}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP2.kits.params_vs_default\endcsname{3.46}
\expandafter\gdef\csname R@an.arch_profile.ratio.SP2.kits.step_vs_default\endcsname{1.91}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5A5.acdc.act_vs_default\endcsname{1.29}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5A5.acdc.gmac_vs_default\endcsname{1.24}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5A5.acdc.params_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5A5.acdc.step_vs_default\endcsname{1.49}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5A5.amos.act_vs_default\endcsname{1.27}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5A5.amos.gmac_vs_default\endcsname{1.25}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5A5.amos.params_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5A5.amos.step_vs_default\endcsname{1.39}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5A5.kits.act_vs_default\endcsname{1.18}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5A5.kits.gmac_vs_default\endcsname{1.05}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5A5.kits.params_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5A5.kits.step_vs_default\endcsname{1.24}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B1.acdc.act_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B1.acdc.gmac_vs_default\endcsname{0.56}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B1.acdc.params_vs_default\endcsname{0.66}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B1.acdc.step_vs_default\endcsname{0.72}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B1.amos.act_vs_default\endcsname{0.79}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B1.amos.gmac_vs_default\endcsname{0.56}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B1.amos.params_vs_default\endcsname{0.67}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B1.amos.step_vs_default\endcsname{0.74}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B1.kits.act_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B1.kits.gmac_vs_default\endcsname{0.54}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B1.kits.params_vs_default\endcsname{0.67}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B1.kits.step_vs_default\endcsname{0.73}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B2.acdc.act_vs_default\endcsname{0.80}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B2.acdc.gmac_vs_default\endcsname{0.56}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B2.acdc.params_vs_default\endcsname{0.67}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B2.acdc.step_vs_default\endcsname{0.92}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B2.amos.act_vs_default\endcsname{0.79}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B2.amos.gmac_vs_default\endcsname{0.56}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B2.amos.params_vs_default\endcsname{0.68}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B2.amos.step_vs_default\endcsname{0.85}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B2.kits.act_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B2.kits.gmac_vs_default\endcsname{0.54}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B2.kits.params_vs_default\endcsname{0.68}
\expandafter\gdef\csname R@an.arch_profile.ratio.V5B2.kits.step_vs_default\endcsname{0.84}
\expandafter\gdef\csname R@an.arch_profile.ratio.V6A1r.acdc.act_vs_default\endcsname{1.49}
\expandafter\gdef\csname R@an.arch_profile.ratio.V6A1r.acdc.gmac_vs_default\endcsname{1.38}
\expandafter\gdef\csname R@an.arch_profile.ratio.V6A1r.acdc.params_vs_default\endcsname{0.99}
\expandafter\gdef\csname R@an.arch_profile.ratio.V6A1r.acdc.step_vs_default\endcsname{1.81}
\expandafter\gdef\csname R@an.arch_profile.ratio.V6A1r.amos.act_vs_default\endcsname{1.47}
\expandafter\gdef\csname R@an.arch_profile.ratio.V6A1r.amos.gmac_vs_default\endcsname{1.39}
\expandafter\gdef\csname R@an.arch_profile.ratio.V6A1r.amos.params_vs_default\endcsname{0.99}
\expandafter\gdef\csname R@an.arch_profile.ratio.V6A1r.amos.step_vs_default\endcsname{1.63}
\expandafter\gdef\csname R@an.arch_profile.ratio.V6A1r.kits.act_vs_default\endcsname{1.38}
\expandafter\gdef\csname R@an.arch_profile.ratio.V6A1r.kits.gmac_vs_default\endcsname{1.23}
\expandafter\gdef\csname R@an.arch_profile.ratio.V6A1r.kits.params_vs_default\endcsname{0.99}
\expandafter\gdef\csname R@an.arch_profile.ratio.V6A1r.kits.step_vs_default\endcsname{1.49}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A1.acdc.act_vs_default\endcsname{0.93}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A1.acdc.gmac_vs_default\endcsname{0.97}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A1.acdc.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A1.acdc.step_vs_default\endcsname{1.07}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A1.amos.act_vs_default\endcsname{0.93}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A1.amos.gmac_vs_default\endcsname{0.97}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A1.amos.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A1.amos.step_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A1.kits.act_vs_default\endcsname{0.87}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A1.kits.gmac_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A1.kits.params_vs_default\endcsname{0.99}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A1.kits.step_vs_default\endcsname{0.92}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A2.acdc.act_vs_default\endcsname{1.13}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A2.acdc.gmac_vs_default\endcsname{1.10}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A2.acdc.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A2.acdc.step_vs_default\endcsname{1.23}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A2.amos.act_vs_default\endcsname{1.12}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A2.amos.gmac_vs_default\endcsname{1.11}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A2.amos.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A2.amos.step_vs_default\endcsname{1.15}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A2.kits.act_vs_default\endcsname{1.08}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A2.kits.gmac_vs_default\endcsname{0.96}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A2.kits.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A2.kits.step_vs_default\endcsname{1.09}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A3.acdc.act_vs_default\endcsname{1.02}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A3.acdc.gmac_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A3.acdc.params_vs_default\endcsname{0.84}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A3.acdc.step_vs_default\endcsname{1.10}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A3.amos.act_vs_default\endcsname{1.01}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A3.amos.gmac_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A3.amos.params_vs_default\endcsname{0.85}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A3.amos.step_vs_default\endcsname{1.03}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A3.kits.act_vs_default\endcsname{1.01}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A3.kits.gmac_vs_default\endcsname{0.77}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A3.kits.params_vs_default\endcsname{0.85}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7A3.kits.step_vs_default\endcsname{1.02}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B1.acdc.act_vs_default\endcsname{0.80}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B1.acdc.gmac_vs_default\endcsname{0.56}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B1.acdc.params_vs_default\endcsname{0.65}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B1.acdc.step_vs_default\endcsname{0.79}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B1.amos.act_vs_default\endcsname{0.80}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B1.amos.gmac_vs_default\endcsname{0.56}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B1.amos.params_vs_default\endcsname{0.66}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B1.amos.step_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B1.kits.act_vs_default\endcsname{0.79}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B1.kits.gmac_vs_default\endcsname{0.54}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B1.kits.params_vs_default\endcsname{0.66}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B1.kits.step_vs_default\endcsname{0.77}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B2.acdc.act_vs_default\endcsname{0.80}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B2.acdc.gmac_vs_default\endcsname{0.56}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B2.acdc.params_vs_default\endcsname{0.65}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B2.acdc.step_vs_default\endcsname{0.76}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B2.amos.act_vs_default\endcsname{0.79}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B2.amos.gmac_vs_default\endcsname{0.56}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B2.amos.params_vs_default\endcsname{0.66}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B2.amos.step_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B2.kits.act_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B2.kits.gmac_vs_default\endcsname{0.54}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B2.kits.params_vs_default\endcsname{0.66}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7B2.kits.step_vs_default\endcsname{0.76}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C1.acdc.act_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C1.acdc.gmac_vs_default\endcsname{0.56}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C1.acdc.params_vs_default\endcsname{0.67}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C1.acdc.step_vs_default\endcsname{0.79}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C1.amos.act_vs_default\endcsname{0.79}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C1.amos.gmac_vs_default\endcsname{0.56}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C1.amos.params_vs_default\endcsname{0.68}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C1.amos.step_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C1.kits.act_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C1.kits.gmac_vs_default\endcsname{0.54}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C1.kits.params_vs_default\endcsname{0.68}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C1.kits.step_vs_default\endcsname{0.77}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C2.acdc.act_vs_default\endcsname{0.80}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C2.acdc.gmac_vs_default\endcsname{0.56}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C2.acdc.params_vs_default\endcsname{0.65}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C2.acdc.step_vs_default\endcsname{0.77}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C2.amos.act_vs_default\endcsname{0.79}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C2.amos.gmac_vs_default\endcsname{0.56}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C2.amos.params_vs_default\endcsname{0.66}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C2.amos.step_vs_default\endcsname{0.77}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C2.kits.act_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C2.kits.gmac_vs_default\endcsname{0.54}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C2.kits.params_vs_default\endcsname{0.66}
\expandafter\gdef\csname R@an.arch_profile.ratio.V7C2.kits.step_vs_default\endcsname{0.76}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A1.acdc.act_vs_default\endcsname{0.80}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A1.acdc.gmac_vs_default\endcsname{0.57}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A1.acdc.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A1.acdc.step_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A1.amos.act_vs_default\endcsname{0.79}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A1.amos.gmac_vs_default\endcsname{0.56}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A1.amos.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A1.amos.step_vs_default\endcsname{0.90}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A1.kits.act_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A1.kits.gmac_vs_default\endcsname{0.54}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A1.kits.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A1.kits.step_vs_default\endcsname{0.91}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A2.acdc.act_vs_default\endcsname{0.80}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A2.acdc.gmac_vs_default\endcsname{0.60}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A2.acdc.params_vs_default\endcsname{1.01}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A2.acdc.step_vs_default\endcsname{0.92}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A2.amos.act_vs_default\endcsname{0.79}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A2.amos.gmac_vs_default\endcsname{0.59}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A2.amos.params_vs_default\endcsname{1.01}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A2.amos.step_vs_default\endcsname{0.86}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A2.kits.act_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A2.kits.gmac_vs_default\endcsname{0.56}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A2.kits.params_vs_default\endcsname{1.01}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8A2.kits.step_vs_default\endcsname{0.85}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B1.acdc.act_vs_default\endcsname{0.58}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B1.acdc.gmac_vs_default\endcsname{0.42}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B1.acdc.params_vs_default\endcsname{0.57}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B1.acdc.step_vs_default\endcsname{0.62}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B1.amos.act_vs_default\endcsname{0.59}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B1.amos.gmac_vs_default\endcsname{0.42}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B1.amos.params_vs_default\endcsname{0.58}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B1.amos.step_vs_default\endcsname{0.62}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B1.kits.act_vs_default\endcsname{0.57}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B1.kits.gmac_vs_default\endcsname{0.35}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B1.kits.params_vs_default\endcsname{0.58}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B1.kits.step_vs_default\endcsname{0.59}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B2.acdc.act_vs_default\endcsname{0.65}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B2.acdc.gmac_vs_default\endcsname{0.53}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B2.acdc.params_vs_default\endcsname{0.67}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B2.acdc.step_vs_default\endcsname{0.68}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B2.amos.act_vs_default\endcsname{0.66}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B2.amos.gmac_vs_default\endcsname{0.53}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B2.amos.params_vs_default\endcsname{0.68}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B2.amos.step_vs_default\endcsname{0.67}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B2.kits.act_vs_default\endcsname{0.61}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B2.kits.gmac_vs_default\endcsname{0.42}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B2.kits.params_vs_default\endcsname{0.68}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8B2.kits.step_vs_default\endcsname{0.63}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8X1.acdc.act_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8X1.acdc.gmac_vs_default\endcsname{0.55}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8X1.acdc.params_vs_default\endcsname{0.58}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8X1.acdc.step_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8X1.amos.act_vs_default\endcsname{0.79}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8X1.amos.gmac_vs_default\endcsname{0.55}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8X1.amos.params_vs_default\endcsname{0.59}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8X1.amos.step_vs_default\endcsname{0.77}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8X1.kits.act_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8X1.kits.gmac_vs_default\endcsname{0.53}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8X1.kits.params_vs_default\endcsname{0.58}
\expandafter\gdef\csname R@an.arch_profile.ratio.V8X1.kits.step_vs_default\endcsname{0.77}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1.acdc.act_vs_default\endcsname{1.08}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1.acdc.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1.acdc.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1.acdc.step_vs_default\endcsname{1.15}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1.amos.act_vs_default\endcsname{1.08}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1.amos.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1.amos.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1.amos.step_vs_default\endcsname{1.14}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1.kits.act_vs_default\endcsname{1.05}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1.kits.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1.kits.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1.kits.step_vs_default\endcsname{1.12}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1c.acdc.act_vs_default\endcsname{1.08}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1c.acdc.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1c.acdc.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1c.acdc.step_vs_default\endcsname{1.15}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1c.amos.act_vs_default\endcsname{1.08}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1c.amos.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1c.amos.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1c.amos.step_vs_default\endcsname{1.15}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1c.kits.act_vs_default\endcsname{1.05}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1c.kits.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1c.kits.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.W1c.kits.step_vs_default\endcsname{1.13}
\expandafter\gdef\csname R@an.arch_profile.ratio.W2.acdc.act_vs_default\endcsname{1.08}
\expandafter\gdef\csname R@an.arch_profile.ratio.W2.acdc.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.W2.acdc.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.W2.acdc.step_vs_default\endcsname{1.16}
\expandafter\gdef\csname R@an.arch_profile.ratio.W2.amos.act_vs_default\endcsname{1.08}
\expandafter\gdef\csname R@an.arch_profile.ratio.W2.amos.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.W2.amos.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.W2.amos.step_vs_default\endcsname{1.15}
\expandafter\gdef\csname R@an.arch_profile.ratio.W2.kits.act_vs_default\endcsname{1.05}
\expandafter\gdef\csname R@an.arch_profile.ratio.W2.kits.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.W2.kits.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.W2.kits.step_vs_default\endcsname{1.13}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3.acdc.act_vs_default\endcsname{0.92}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3.acdc.gmac_vs_default\endcsname{0.98}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3.acdc.params_vs_default\endcsname{0.97}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3.acdc.step_vs_default\endcsname{1.10}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3.amos.act_vs_default\endcsname{0.92}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3.amos.gmac_vs_default\endcsname{0.98}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3.amos.params_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3.amos.step_vs_default\endcsname{1.08}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3.kits.act_vs_default\endcsname{0.91}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3.kits.gmac_vs_default\endcsname{0.99}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3.kits.params_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3.kits.step_vs_default\endcsname{1.08}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3c.acdc.act_vs_default\endcsname{0.91}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3c.acdc.gmac_vs_default\endcsname{0.98}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3c.acdc.params_vs_default\endcsname{0.97}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3c.acdc.step_vs_default\endcsname{1.09}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3c.amos.act_vs_default\endcsname{0.91}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3c.amos.gmac_vs_default\endcsname{0.98}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3c.amos.params_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3c.amos.step_vs_default\endcsname{1.07}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3c.kits.act_vs_default\endcsname{0.90}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3c.kits.gmac_vs_default\endcsname{0.99}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3c.kits.params_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.arch_profile.ratio.W3c.kits.step_vs_default\endcsname{1.06}
\expandafter\gdef\csname R@an.arch_profile.ratio.W4.acdc.act_vs_default\endcsname{2.31}
\expandafter\gdef\csname R@an.arch_profile.ratio.W4.acdc.gmac_vs_default\endcsname{0.92}
\expandafter\gdef\csname R@an.arch_profile.ratio.W4.acdc.params_vs_default\endcsname{1.10}
\expandafter\gdef\csname R@an.arch_profile.ratio.W4.acdc.step_vs_default\endcsname{3.84}
\expandafter\gdef\csname R@an.arch_profile.ratio.W4.amos.act_vs_default\endcsname{2.25}
\expandafter\gdef\csname R@an.arch_profile.ratio.W4.amos.gmac_vs_default\endcsname{0.91}
\expandafter\gdef\csname R@an.arch_profile.ratio.W4.amos.params_vs_default\endcsname{1.10}
\expandafter\gdef\csname R@an.arch_profile.ratio.W4.amos.step_vs_default\endcsname{3.51}
\expandafter\gdef\csname R@an.arch_profile.ratio.W4.kits.act_vs_default\endcsname{1.89}
\expandafter\gdef\csname R@an.arch_profile.ratio.W4.kits.gmac_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.arch_profile.ratio.W4.kits.params_vs_default\endcsname{1.10}
\expandafter\gdef\csname R@an.arch_profile.ratio.W4.kits.step_vs_default\endcsname{2.62}
\expandafter\gdef\csname R@an.arch_profile.ratio.W5.acdc.act_vs_default\endcsname{1.42}
\expandafter\gdef\csname R@an.arch_profile.ratio.W5.acdc.gmac_vs_default\endcsname{1.86}
\expandafter\gdef\csname R@an.arch_profile.ratio.W5.acdc.params_vs_default\endcsname{3.35}
\expandafter\gdef\csname R@an.arch_profile.ratio.W5.acdc.step_vs_default\endcsname{1.41}
\expandafter\gdef\csname R@an.arch_profile.ratio.W5.amos.act_vs_default\endcsname{1.40}
\expandafter\gdef\csname R@an.arch_profile.ratio.W5.amos.gmac_vs_default\endcsname{1.82}
\expandafter\gdef\csname R@an.arch_profile.ratio.W5.amos.params_vs_default\endcsname{3.29}
\expandafter\gdef\csname R@an.arch_profile.ratio.W5.amos.step_vs_default\endcsname{1.37}
\expandafter\gdef\csname R@an.arch_profile.ratio.W5.kits.act_vs_default\endcsname{1.26}
\expandafter\gdef\csname R@an.arch_profile.ratio.W5.kits.gmac_vs_default\endcsname{1.38}
\expandafter\gdef\csname R@an.arch_profile.ratio.W5.kits.params_vs_default\endcsname{3.28}
\expandafter\gdef\csname R@an.arch_profile.ratio.W5.kits.step_vs_default\endcsname{1.22}
\expandafter\gdef\csname R@an.arch_profile.ratio.base.acdc.act_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.base.acdc.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.base.acdc.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.base.acdc.step_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.base.amos.act_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.base.amos.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.base.amos.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.base.amos.step_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.base.kits.act_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.base.kits.gmac_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.base.kits.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.ratio.base.kits.step_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.arch_profile.rf.D1.acdc.xy.enc4.mm\endcsname{254}
\expandafter\gdef\csname R@an.arch_profile.rf.D1.acdc.xy.mm\endcsname{2320}
\expandafter\gdef\csname R@an.arch_profile.rf.D1.acdc.xy.vox\endcsname{1523}
\expandafter\gdef\csname R@an.arch_profile.rf.D1.acdc.z.enc4.mm\endcsname{415}
\expandafter\gdef\csname R@an.arch_profile.rf.D1.acdc.z.mm\endcsname{1715}
\expandafter\gdef\csname R@an.arch_profile.rf.D1.acdc.z.vox\endcsname{343}
\expandafter\gdef\csname R@an.arch_profile.rf.D1.amos.xy.enc4.mm\endcsname{114}
\expandafter\gdef\csname R@an.arch_profile.rf.D1.amos.xy.mm\endcsname{1043}
\expandafter\gdef\csname R@an.arch_profile.rf.D1.amos.xy.vox\endcsname{1523}
\expandafter\gdef\csname R@an.arch_profile.rf.D1.amos.z.enc4.mm\endcsname{166}
\expandafter\gdef\csname R@an.arch_profile.rf.D1.amos.z.mm\endcsname{1518}
\expandafter\gdef\csname R@an.arch_profile.rf.D1.amos.z.vox\endcsname{759}
\expandafter\gdef\csname R@an.arch_profile.rf.D1.kits.xy.enc4.mm\endcsname{130}
\expandafter\gdef\csname R@an.arch_profile.rf.D1.kits.xy.mm\endcsname{1190}
\expandafter\gdef\csname R@an.arch_profile.rf.D1.kits.xy.vox\endcsname{1523}
\expandafter\gdef\csname R@an.arch_profile.rf.D1.kits.z.enc4.mm\endcsname{167}
\expandafter\gdef\csname R@an.arch_profile.rf.D1.kits.z.mm\endcsname{1523}
\expandafter\gdef\csname R@an.arch_profile.rf.D1.kits.z.vox\endcsname{1523}
\expandafter\gdef\csname R@an.arch_profile.rf.D2.acdc.xy.enc4.mm\endcsname{72}
\expandafter\gdef\csname R@an.arch_profile.rf.D2.acdc.xy.mm\endcsname{385}
\expandafter\gdef\csname R@an.arch_profile.rf.D2.acdc.xy.vox\endcsname{253}
\expandafter\gdef\csname R@an.arch_profile.rf.D2.acdc.z.enc4.mm\endcsname{115}
\expandafter\gdef\csname R@an.arch_profile.rf.D2.acdc.z.mm\endcsname{385}
\expandafter\gdef\csname R@an.arch_profile.rf.D2.acdc.z.vox\endcsname{77}
\expandafter\gdef\csname R@an.arch_profile.rf.D2.amos.xy.enc4.mm\endcsname{32}
\expandafter\gdef\csname R@an.arch_profile.rf.D2.amos.xy.mm\endcsname{173}
\expandafter\gdef\csname R@an.arch_profile.rf.D2.amos.xy.vox\endcsname{253}
\expandafter\gdef\csname R@an.arch_profile.rf.D2.amos.z.enc4.mm\endcsname{46}
\expandafter\gdef\csname R@an.arch_profile.rf.D2.amos.z.mm\endcsname{250}
\expandafter\gdef\csname R@an.arch_profile.rf.D2.amos.z.vox\endcsname{125}
\expandafter\gdef\csname R@an.arch_profile.rf.D2.kits.xy.enc4.mm\endcsname{37}
\expandafter\gdef\csname R@an.arch_profile.rf.D2.kits.xy.mm\endcsname{198}
\expandafter\gdef\csname R@an.arch_profile.rf.D2.kits.xy.vox\endcsname{253}
\expandafter\gdef\csname R@an.arch_profile.rf.D2.kits.z.enc4.mm\endcsname{47}
\expandafter\gdef\csname R@an.arch_profile.rf.D2.kits.z.mm\endcsname{253}
\expandafter\gdef\csname R@an.arch_profile.rf.D2.kits.z.vox\endcsname{253}
\expandafter\gdef\csname R@an.arch_profile.rf.L1.acdc.xy.enc4.mm\endcsname{416}
\expandafter\gdef\csname R@an.arch_profile.rf.L1.acdc.xy.mm\endcsname{2192}
\expandafter\gdef\csname R@an.arch_profile.rf.L1.acdc.xy.vox\endcsname{1439}
\expandafter\gdef\csname R@an.arch_profile.rf.L1.acdc.z.enc4.mm\endcsname{675}
\expandafter\gdef\csname R@an.arch_profile.rf.L1.acdc.z.mm\endcsname{1745}
\expandafter\gdef\csname R@an.arch_profile.rf.L1.acdc.z.vox\endcsname{349}
\expandafter\gdef\csname R@an.arch_profile.rf.L1.amos.xy.enc4.mm\endcsname{187}
\expandafter\gdef\csname R@an.arch_profile.rf.L1.amos.xy.mm\endcsname{985}
\expandafter\gdef\csname R@an.arch_profile.rf.L1.amos.xy.vox\endcsname{1439}
\expandafter\gdef\csname R@an.arch_profile.rf.L1.amos.z.enc4.mm\endcsname{270}
\expandafter\gdef\csname R@an.arch_profile.rf.L1.amos.z.mm\endcsname{1434}
\expandafter\gdef\csname R@an.arch_profile.rf.L1.amos.z.vox\endcsname{717}
\expandafter\gdef\csname R@an.arch_profile.rf.L1.kits.xy.enc4.mm\endcsname{213}
\expandafter\gdef\csname R@an.arch_profile.rf.L1.kits.xy.mm\endcsname{1124}
\expandafter\gdef\csname R@an.arch_profile.rf.L1.kits.xy.vox\endcsname{1439}
\expandafter\gdef\csname R@an.arch_profile.rf.L1.kits.z.enc4.mm\endcsname{273}
\expandafter\gdef\csname R@an.arch_profile.rf.L1.kits.z.mm\endcsname{1439}
\expandafter\gdef\csname R@an.arch_profile.rf.L1.kits.z.vox\endcsname{1439}
\expandafter\gdef\csname R@an.arch_profile.rf.L2.acdc.xy.enc4.mm\endcsname{139}
\expandafter\gdef\csname R@an.arch_profile.rf.L2.acdc.xy.mm\endcsname{839}
\expandafter\gdef\csname R@an.arch_profile.rf.L2.acdc.xy.vox\endcsname{551}
\expandafter\gdef\csname R@an.arch_profile.rf.L2.acdc.z.enc4.mm\endcsname{225}
\expandafter\gdef\csname R@an.arch_profile.rf.L2.acdc.z.mm\endcsname{765}
\expandafter\gdef\csname R@an.arch_profile.rf.L2.acdc.z.vox\endcsname{153}
\expandafter\gdef\csname R@an.arch_profile.rf.L2.amos.xy.enc4.mm\endcsname{62}
\expandafter\gdef\csname R@an.arch_profile.rf.L2.amos.xy.mm\endcsname{377}
\expandafter\gdef\csname R@an.arch_profile.rf.L2.amos.xy.vox\endcsname{551}
\expandafter\gdef\csname R@an.arch_profile.rf.L2.amos.z.enc4.mm\endcsname{90}
\expandafter\gdef\csname R@an.arch_profile.rf.L2.amos.z.mm\endcsname{546}
\expandafter\gdef\csname R@an.arch_profile.rf.L2.amos.z.vox\endcsname{273}
\expandafter\gdef\csname R@an.arch_profile.rf.L2.kits.xy.enc4.mm\endcsname{71}
\expandafter\gdef\csname R@an.arch_profile.rf.L2.kits.xy.mm\endcsname{430}
\expandafter\gdef\csname R@an.arch_profile.rf.L2.kits.xy.vox\endcsname{551}
\expandafter\gdef\csname R@an.arch_profile.rf.L2.kits.z.enc4.mm\endcsname{91}
\expandafter\gdef\csname R@an.arch_profile.rf.L2.kits.z.mm\endcsname{551}
\expandafter\gdef\csname R@an.arch_profile.rf.L2.kits.z.vox\endcsname{551}
\expandafter\gdef\csname R@an.arch_profile.rf.L3.acdc.xy.enc4.mm\endcsname{254}
\expandafter\gdef\csname R@an.arch_profile.rf.L3.acdc.xy.mm\endcsname{2393}
\expandafter\gdef\csname R@an.arch_profile.rf.L3.acdc.xy.vox\endcsname{1571}
\expandafter\gdef\csname R@an.arch_profile.rf.L3.acdc.z.enc4.mm\endcsname{415}
\expandafter\gdef\csname R@an.arch_profile.rf.L3.acdc.z.mm\endcsname{1795}
\expandafter\gdef\csname R@an.arch_profile.rf.L3.acdc.z.vox\endcsname{359}
\expandafter\gdef\csname R@an.arch_profile.rf.L3.amos.xy.enc4.mm\endcsname{114}
\expandafter\gdef\csname R@an.arch_profile.rf.L3.amos.xy.mm\endcsname{1075}
\expandafter\gdef\csname R@an.arch_profile.rf.L3.amos.xy.vox\endcsname{1571}
\expandafter\gdef\csname R@an.arch_profile.rf.L3.amos.z.enc4.mm\endcsname{166}
\expandafter\gdef\csname R@an.arch_profile.rf.L3.amos.z.mm\endcsname{1566}
\expandafter\gdef\csname R@an.arch_profile.rf.L3.amos.z.vox\endcsname{783}
\expandafter\gdef\csname R@an.arch_profile.rf.L3.kits.xy.enc4.mm\endcsname{130}
\expandafter\gdef\csname R@an.arch_profile.rf.L3.kits.xy.mm\endcsname{1227}
\expandafter\gdef\csname R@an.arch_profile.rf.L3.kits.xy.vox\endcsname{1571}
\expandafter\gdef\csname R@an.arch_profile.rf.L3.kits.z.enc4.mm\endcsname{167}
\expandafter\gdef\csname R@an.arch_profile.rf.L3.kits.z.mm\endcsname{1571}
\expandafter\gdef\csname R@an.arch_profile.rf.L3.kits.z.vox\endcsname{1571}
\expandafter\gdef\csname R@an.arch_profile.rf.L3k3.acdc.xy.enc4.mm\endcsname{181}
\expandafter\gdef\csname R@an.arch_profile.rf.L3k3.acdc.xy.mm\endcsname{1028}
\expandafter\gdef\csname R@an.arch_profile.rf.L3k3.acdc.xy.vox\endcsname{675}
\expandafter\gdef\csname R@an.arch_profile.rf.L3k3.acdc.z.enc4.mm\endcsname{295}
\expandafter\gdef\csname R@an.arch_profile.rf.L3k3.acdc.z.mm\endcsname{915}
\expandafter\gdef\csname R@an.arch_profile.rf.L3k3.acdc.z.vox\endcsname{183}
\expandafter\gdef\csname R@an.arch_profile.rf.L3k3.amos.xy.enc4.mm\endcsname{81}
\expandafter\gdef\csname R@an.arch_profile.rf.L3k3.amos.xy.mm\endcsname{462}
\expandafter\gdef\csname R@an.arch_profile.rf.L3k3.amos.xy.vox\endcsname{675}
\expandafter\gdef\csname R@an.arch_profile.rf.L3k3.amos.z.enc4.mm\endcsname{118}
\expandafter\gdef\csname R@an.arch_profile.rf.L3k3.amos.z.mm\endcsname{670}
\expandafter\gdef\csname R@an.arch_profile.rf.L3k3.amos.z.vox\endcsname{335}
\expandafter\gdef\csname R@an.arch_profile.rf.L3k3.kits.xy.enc4.mm\endcsname{93}
\expandafter\gdef\csname R@an.arch_profile.rf.L3k3.kits.xy.mm\endcsname{527}
\expandafter\gdef\csname R@an.arch_profile.rf.L3k3.kits.xy.vox\endcsname{675}
\expandafter\gdef\csname R@an.arch_profile.rf.L3k3.kits.z.enc4.mm\endcsname{119}
\expandafter\gdef\csname R@an.arch_profile.rf.L3k3.kits.z.mm\endcsname{675}
\expandafter\gdef\csname R@an.arch_profile.rf.L3k3.kits.z.vox\endcsname{675}
\expandafter\gdef\csname R@an.arch_profile.rf.S2.acdc.xy.enc4.mm\endcsname{267}
\expandafter\gdef\csname R@an.arch_profile.rf.S2.acdc.xy.mm\endcsname{2406}
\expandafter\gdef\csname R@an.arch_profile.rf.S2.acdc.xy.vox\endcsname{1579}
\expandafter\gdef\csname R@an.arch_profile.rf.S2.acdc.z.enc4.mm\endcsname{435}
\expandafter\gdef\csname R@an.arch_profile.rf.S2.acdc.z.mm\endcsname{1815}
\expandafter\gdef\csname R@an.arch_profile.rf.S2.acdc.z.vox\endcsname{363}
\expandafter\gdef\csname R@an.arch_profile.rf.S2.amos.xy.enc4.mm\endcsname{120}
\expandafter\gdef\csname R@an.arch_profile.rf.S2.amos.xy.mm\endcsname{1081}
\expandafter\gdef\csname R@an.arch_profile.rf.S2.amos.xy.vox\endcsname{1579}
\expandafter\gdef\csname R@an.arch_profile.rf.S2.amos.z.enc4.mm\endcsname{174}
\expandafter\gdef\csname R@an.arch_profile.rf.S2.amos.z.mm\endcsname{1574}
\expandafter\gdef\csname R@an.arch_profile.rf.S2.amos.z.vox\endcsname{787}
\expandafter\gdef\csname R@an.arch_profile.rf.S2.kits.xy.enc4.mm\endcsname{137}
\expandafter\gdef\csname R@an.arch_profile.rf.S2.kits.xy.mm\endcsname{1234}
\expandafter\gdef\csname R@an.arch_profile.rf.S2.kits.xy.vox\endcsname{1579}
\expandafter\gdef\csname R@an.arch_profile.rf.S2.kits.z.enc4.mm\endcsname{175}
\expandafter\gdef\csname R@an.arch_profile.rf.S2.kits.z.mm\endcsname{1579}
\expandafter\gdef\csname R@an.arch_profile.rf.S2.kits.z.vox\endcsname{1579}
\expandafter\gdef\csname R@an.arch_profile.rf.base.acdc.xy.enc4.mm\endcsname{72}
\expandafter\gdef\csname R@an.arch_profile.rf.base.acdc.xy.mm\endcsname{480}
\expandafter\gdef\csname R@an.arch_profile.rf.base.acdc.xy.vox\endcsname{315}
\expandafter\gdef\csname R@an.arch_profile.rf.base.acdc.z.enc4.mm\endcsname{115}
\expandafter\gdef\csname R@an.arch_profile.rf.base.acdc.z.mm\endcsname{495}
\expandafter\gdef\csname R@an.arch_profile.rf.base.acdc.z.vox\endcsname{99}
\expandafter\gdef\csname R@an.arch_profile.rf.base.amos.xy.enc4.mm\endcsname{32}
\expandafter\gdef\csname R@an.arch_profile.rf.base.amos.xy.mm\endcsname{216}
\expandafter\gdef\csname R@an.arch_profile.rf.base.amos.xy.vox\endcsname{315}
\expandafter\gdef\csname R@an.arch_profile.rf.base.amos.z.enc4.mm\endcsname{46}
\expandafter\gdef\csname R@an.arch_profile.rf.base.amos.z.mm\endcsname{310}
\expandafter\gdef\csname R@an.arch_profile.rf.base.amos.z.vox\endcsname{155}
\expandafter\gdef\csname R@an.arch_profile.rf.base.kits.xy.enc4.mm\endcsname{37}
\expandafter\gdef\csname R@an.arch_profile.rf.base.kits.xy.mm\endcsname{246}
\expandafter\gdef\csname R@an.arch_profile.rf.base.kits.xy.vox\endcsname{315}
\expandafter\gdef\csname R@an.arch_profile.rf.base.kits.z.enc4.mm\endcsname{47}
\expandafter\gdef\csname R@an.arch_profile.rf.base.kits.z.mm\endcsname{315}
\expandafter\gdef\csname R@an.arch_profile.rf.base.kits.z.vox\endcsname{315}
\expandafter\gdef\csname R@an.arch_profile.rf.outpatch.drawn.min\endcsname{1.32}
\expandafter\gdef\csname R@an.arch_profile.rf.outpatch.drawn.min.where\endcsname{LeanDec on AMOS22 in-plane}
\expandafter\gdef\csname R@an.arch_profile.rf.outpatch.min\endcsname{0.99}
\expandafter\gdef\csname R@an.arch_profile.rf.outpatch.min.where\endcsname{LeanDec on ACDC in-plane}
\expandafter\gdef\csname R@an.arch_profile.size.acdc.LVC.d10\endcsname{40}
\expandafter\gdef\csname R@an.arch_profile.size.acdc.LVC.d50\endcsname{53}
\expandafter\gdef\csname R@an.arch_profile.size.acdc.LVC.d90\endcsname{73}
\expandafter\gdef\csname R@an.arch_profile.size.acdc.LVC.n\endcsname{40}
\expandafter\gdef\csname R@an.arch_profile.size.acdc.MLV.d10\endcsname{50}
\expandafter\gdef\csname R@an.arch_profile.size.acdc.MLV.d50\endcsname{59}
\expandafter\gdef\csname R@an.arch_profile.size.acdc.MLV.d90\endcsname{72}
\expandafter\gdef\csname R@an.arch_profile.size.acdc.MLV.n\endcsname{40}
\expandafter\gdef\csname R@an.arch_profile.size.acdc.RV.d10\endcsname{45}
\expandafter\gdef\csname R@an.arch_profile.size.acdc.RV.d50\endcsname{61}
\expandafter\gdef\csname R@an.arch_profile.size.acdc.RV.d90\endcsname{73}
\expandafter\gdef\csname R@an.arch_profile.size.acdc.RV.n\endcsname{40}
\expandafter\gdef\csname R@an.arch_profile.size.amos.aorta.d10\endcsname{45}
\expandafter\gdef\csname R@an.arch_profile.size.amos.aorta.d50\endcsname{56}
\expandafter\gdef\csname R@an.arch_profile.size.amos.aorta.d90\endcsname{73}
\expandafter\gdef\csname R@an.arch_profile.size.amos.aorta.n\endcsname{40}
\expandafter\gdef\csname R@an.arch_profile.size.amos.bladder.d10\endcsname{43}
\expandafter\gdef\csname R@an.arch_profile.size.amos.bladder.d50\endcsname{57}
\expandafter\gdef\csname R@an.arch_profile.size.amos.bladder.d90\endcsname{85}
\expandafter\gdef\csname R@an.arch_profile.size.amos.bladder.n\endcsname{40}
\expandafter\gdef\csname R@an.arch_profile.size.amos.duodenum.d10\endcsname{40}
\expandafter\gdef\csname R@an.arch_profile.size.amos.duodenum.d50\endcsname{46}
\expandafter\gdef\csname R@an.arch_profile.size.amos.duodenum.d90\endcsname{56}
\expandafter\gdef\csname R@an.arch_profile.size.amos.duodenum.n\endcsname{40}
\expandafter\gdef\csname R@an.arch_profile.size.amos.esophagus.d10\endcsname{23}
\expandafter\gdef\csname R@an.arch_profile.size.amos.esophagus.d50\endcsname{29}
\expandafter\gdef\csname R@an.arch_profile.size.amos.esophagus.d90\endcsname{38}
\expandafter\gdef\csname R@an.arch_profile.size.amos.esophagus.n\endcsname{40}
\expandafter\gdef\csname R@an.arch_profile.size.amos.gallbladder.d10\endcsname{29}
\expandafter\gdef\csname R@an.arch_profile.size.amos.gallbladder.d50\endcsname{36}
\expandafter\gdef\csname R@an.arch_profile.size.amos.gallbladder.d90\endcsname{45}
\expandafter\gdef\csname R@an.arch_profile.size.amos.gallbladder.n\endcsname{38}
\expandafter\gdef\csname R@an.arch_profile.size.amos.leftadrenalgland.d10\endcsname{17}
\expandafter\gdef\csname R@an.arch_profile.size.amos.leftadrenalgland.d50\endcsname{19}
\expandafter\gdef\csname R@an.arch_profile.size.amos.leftadrenalgland.d90\endcsname{23}
\expandafter\gdef\csname R@an.arch_profile.size.amos.leftadrenalgland.n\endcsname{40}
\expandafter\gdef\csname R@an.arch_profile.size.amos.leftkidney.d10\endcsname{56}
\expandafter\gdef\csname R@an.arch_profile.size.amos.leftkidney.d50\endcsname{63}
\expandafter\gdef\csname R@an.arch_profile.size.amos.leftkidney.d90\endcsname{74}
\expandafter\gdef\csname R@an.arch_profile.size.amos.leftkidney.n\endcsname{40}
\expandafter\gdef\csname R@an.arch_profile.size.amos.liver.d10\endcsname{119}
\expandafter\gdef\csname R@an.arch_profile.size.amos.liver.d50\endcsname{130}
\expandafter\gdef\csname R@an.arch_profile.size.amos.liver.d90\endcsname{149}
\expandafter\gdef\csname R@an.arch_profile.size.amos.liver.n\endcsname{40}
\expandafter\gdef\csname R@an.arch_profile.size.amos.pancreas.d10\endcsname{43}
\expandafter\gdef\csname R@an.arch_profile.size.amos.pancreas.d50\endcsname{50}
\expandafter\gdef\csname R@an.arch_profile.size.amos.pancreas.d90\endcsname{58}
\expandafter\gdef\csname R@an.arch_profile.size.amos.pancreas.n\endcsname{40}
\expandafter\gdef\csname R@an.arch_profile.size.amos.postcava.d10\endcsname{43}
\expandafter\gdef\csname R@an.arch_profile.size.amos.postcava.d50\endcsname{51}
\expandafter\gdef\csname R@an.arch_profile.size.amos.postcava.d90\endcsname{56}
\expandafter\gdef\csname R@an.arch_profile.size.amos.postcava.n\endcsname{40}
\expandafter\gdef\csname R@an.arch_profile.size.amos.prostateuterus.d10\endcsname{33}
\expandafter\gdef\csname R@an.arch_profile.size.amos.prostateuterus.d50\endcsname{40}
\expandafter\gdef\csname R@an.arch_profile.size.amos.prostateuterus.d90\endcsname{62}
\expandafter\gdef\csname R@an.arch_profile.size.amos.prostateuterus.n\endcsname{39}
\expandafter\gdef\csname R@an.arch_profile.size.amos.rightadrenalgland.d10\endcsname{16}
\expandafter\gdef\csname R@an.arch_profile.size.amos.rightadrenalgland.d50\endcsname{18}
\expandafter\gdef\csname R@an.arch_profile.size.amos.rightadrenalgland.d90\endcsname{21}
\expandafter\gdef\csname R@an.arch_profile.size.amos.rightadrenalgland.n\endcsname{39}
\expandafter\gdef\csname R@an.arch_profile.size.amos.rightkidney.d10\endcsname{56}
\expandafter\gdef\csname R@an.arch_profile.size.amos.rightkidney.d50\endcsname{62}
\expandafter\gdef\csname R@an.arch_profile.size.amos.rightkidney.d90\endcsname{72}
\expandafter\gdef\csname R@an.arch_profile.size.amos.rightkidney.n\endcsname{40}
\expandafter\gdef\csname R@an.arch_profile.size.amos.spleen.d10\endcsname{53}
\expandafter\gdef\csname R@an.arch_profile.size.amos.spleen.d50\endcsname{70}
\expandafter\gdef\csname R@an.arch_profile.size.amos.spleen.d90\endcsname{86}
\expandafter\gdef\csname R@an.arch_profile.size.amos.spleen.n\endcsname{38}
\expandafter\gdef\csname R@an.arch_profile.size.amos.stomach.d10\endcsname{65}
\expandafter\gdef\csname R@an.arch_profile.size.amos.stomach.d50\endcsname{76}
\expandafter\gdef\csname R@an.arch_profile.size.amos.stomach.d90\endcsname{105}
\expandafter\gdef\csname R@an.arch_profile.size.amos.stomach.n\endcsname{40}
\expandafter\gdef\csname R@an.arch_profile.size.kits.kidney.d10\endcsname{82}
\expandafter\gdef\csname R@an.arch_profile.size.kits.kidney.d50\endcsname{95}
\expandafter\gdef\csname R@an.arch_profile.size.kits.kidney.d90\endcsname{112}
\expandafter\gdef\csname R@an.arch_profile.size.kits.kidney.n\endcsname{98}
\expandafter\gdef\csname R@an.arch_profile.size.kits.masses.d10\endcsname{21}
\expandafter\gdef\csname R@an.arch_profile.size.kits.masses.d50\endcsname{41}
\expandafter\gdef\csname R@an.arch_profile.size.kits.masses.d90\endcsname{80}
\expandafter\gdef\csname R@an.arch_profile.size.kits.masses.n\endcsname{98}
\expandafter\gdef\csname R@an.arch_profile.size.kits.tumor.d10\endcsname{18}
\expandafter\gdef\csname R@an.arch_profile.size.kits.tumor.d50\endcsname{36}
\expandafter\gdef\csname R@an.arch_profile.size.kits.tumor.d90\endcsname{72}
\expandafter\gdef\csname R@an.arch_profile.size.kits.tumor.n\endcsname{98}
\expandafter\gdef\csname R@an.arch_profile.switch.L3.level\endcsname{4}
\expandafter\gdef\csname R@an.arch_profile.typ.amos.d50\endcsname{51}
\expandafter\gdef\csname R@an.arch_profile.typ.amos.d50.mm1\endcsname{51.3}
\expandafter\gdef\csname R@an.arch_profile.typ.kits.d50\endcsname{36}
\expandafter\gdef\csname R@an.arch_profile.typ.kits.d50.mm1\endcsname{36.2}
\expandafter\gdef\csname R@an.archspec.default.name\endcsname{nnU-Net default}
\expandafter\gdef\csname R@an.archspec.default.params\endcsname{31\,196\,399}
\expandafter\gdef\csname R@an.archspec.default.tag\endcsname{base}
\expandafter\gdef\csname R@an.archspec.rows\endcsname{22}
\expandafter\gdef\csname R@an.archspec.stem1.name\endcsname{Stem1 ({\ifdefined\archL\archL\else XX-Net-L\fi}, one-convolution stem)}
\expandafter\gdef\csname R@an.archspec.stem1.params\endcsname{21\,084\,015}
\expandafter\gdef\csname R@an.archspec.stem1.tag\endcsname{V8B2}
\expandafter\gdef\csname R@an.archspec.xa.name\endcsname{{\ifdefined\archA\archA\else XX-Net-A\fi}}
\expandafter\gdef\csname R@an.archspec.xa.params\endcsname{31\,038\,863}
\expandafter\gdef\csname R@an.archspec.xa.tag\endcsname{V7A1}
\expandafter\gdef\csname R@an.archspec.xl.name\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi}}
\expandafter\gdef\csname R@an.archspec.xl.params\endcsname{21\,111\,759}
\expandafter\gdef\csname R@an.archspec.xl.tag\endcsname{V7C1}
\expandafter\gdef\csname R@an.baseline_compile.L1.frozen\endcsname{+0.647}
\expandafter\gdef\csname R@an.baseline_compile.L1.unc\endcsname{+0.618}
\expandafter\gdef\csname R@an.baseline_compile.L1b.frozen\endcsname{+0.138}
\expandafter\gdef\csname R@an.baseline_compile.L1b.unc\endcsname{+0.109}
\expandafter\gdef\csname R@an.baseline_compile.L2.frozen\endcsname{+0.362}
\expandafter\gdef\csname R@an.baseline_compile.L2.unc\endcsname{+0.333}
\expandafter\gdef\csname R@an.baseline_compile.L3.frozen\endcsname{+0.382}
\expandafter\gdef\csname R@an.baseline_compile.L3.unc\endcsname{+0.353}
\expandafter\gdef\csname R@an.baseline_compile.L4.frozen\endcsname{+0.430}
\expandafter\gdef\csname R@an.baseline_compile.L4.unc\endcsname{+0.401}
\expandafter\gdef\csname R@an.baseline_compile.L6.frozen\endcsname{+0.016}
\expandafter\gdef\csname R@an.baseline_compile.L6.unc\endcsname{-0.013}
\expandafter\gdef\csname R@an.baseline_compile.W1.frozen\endcsname{+0.099}
\expandafter\gdef\csname R@an.baseline_compile.W1.unc\endcsname{+0.071}
\expandafter\gdef\csname R@an.baseline_compile.W1c.frozen\endcsname{+0.363}
\expandafter\gdef\csname R@an.baseline_compile.W1c.unc\endcsname{+0.334}
\expandafter\gdef\csname R@an.baseline_compile.W2.frozen\endcsname{+0.211}
\expandafter\gdef\csname R@an.baseline_compile.W2.unc\endcsname{+0.182}
\expandafter\gdef\csname R@an.baseline_compile.W3.frozen\endcsname{+0.270}
\expandafter\gdef\csname R@an.baseline_compile.W3.unc\endcsname{+0.241}
\expandafter\gdef\csname R@an.baseline_compile.W3c.frozen\endcsname{+0.162}
\expandafter\gdef\csname R@an.baseline_compile.W3c.unc\endcsname{+0.133}
\expandafter\gdef\csname R@an.baseline_compile.acdc.d\endcsname{-0.014}
\expandafter\gdef\csname R@an.baseline_compile.acdc.ncomp\endcsname{3}
\expandafter\gdef\csname R@an.baseline_compile.acdc.nunc\endcsname{3}
\expandafter\gdef\csname R@an.baseline_compile.amos.d\endcsname{-0.058}
\expandafter\gdef\csname R@an.baseline_compile.amos.ncomp\endcsname{3}
\expandafter\gdef\csname R@an.baseline_compile.amos.nunc\endcsname{3}
\expandafter\gdef\csname R@an.baseline_compile.amos.ref.frozen\endcsname{87.701}
\expandafter\gdef\csname R@an.baseline_compile.amos.ref.shift\endcsname{+0.029}
\expandafter\gdef\csname R@an.baseline_compile.amos.ref.unc\endcsname{87.730}
\expandafter\gdef\csname R@an.baseline_compile.design.ncomp\endcsname{0}
\expandafter\gdef\csname R@an.baseline_compile.design.nscan\endcsname{40}
\expandafter\gdef\csname R@an.baseline_compile.flips\endcsname{L2 and W1c}
\expandafter\gdef\csname R@an.baseline_compile.flips.n\endcsname{2}
\expandafter\gdef\csname R@an.baseline_compile.kits.ncomp\endcsname{0}
\expandafter\gdef\csname R@an.baseline_compile.kits.nunc\endcsname{3}
\expandafter\gdef\csname R@an.buildpath.buildpath.def\endcsname{the build path is how a network is built -- the library path it is constructed and trained through. The rebuild offset is the contrast of a function-identical rebuild against the stock network it rebuilds, measured, with no mechanism attributed to it}
\expandafter\gdef\csname R@an.buildpath.claim.direction\endcsname{the plan-aware build is better (or worse)}
\expandafter\gdef\csname R@an.buildpath.claim.direction.def\endcsname{the rebuild offset of the plain family and the re-implementation difference of the residual family have the SAME sign on a dataset (withdrawn by CLAIM_FRAME 33: only the plain family has a function-identical control)}
\expandafter\gdef\csname R@an.buildpath.claim.direction.measured\endcsname{KiTS23: +1.18 and \ensuremath{-}1.16 pp, OPPOSITE signs; AMOS22: pending; ACDC: +0.12 and +0.08 pp, the SAME signs}
\expandafter\gdef\csname R@an.buildpath.claim.direction.state\endcsname{true}
\expandafter\gdef\csname R@an.buildpath.claim.mechanism\endcsname{a mechanism for the rebuild offset or the re-implementation difference (initialisation, padding, normalisation placement, ...)}
\expandafter\gdef\csname R@an.buildpath.claim.mechanism.def\endcsname{no run in this study varies any single library-versus-plan-aware difference, so nothing here identifies a mechanism and the claim is false whatever the data show}
\expandafter\gdef\csname R@an.buildpath.claim.mechanism.measured\endcsname{no run of this study varies a single library-versus-plan-aware difference, so nothing here identifies a mechanism}
\expandafter\gdef\csname R@an.buildpath.claim.mechanism.state\endcsname{false}
\expandafter\gdef\csname R@an.buildpath.claim.mostly\endcsname{HyReX's margin is mostly implementation (or mostly design)}
\expandafter\gdef\csname R@an.buildpath.claim.mostly.def\endcsname{one of the two parts of the decomposition carries at least 66.7 \% of their sum, both parts pointing the same way}
\expandafter\gdef\csname R@an.buildpath.claim.mostly.measured\endcsname{KiTS23: +1.18 pp and +0.92 pp, larger part 56.2 \% of the sum; AMOS22: pending; ACDC: +0.12 pp and +0.33 pp, larger part 74.1 \% of the sum}
\expandafter\gdef\csname R@an.buildpath.claim.mostly.state\endcsname{true}
\expandafter\gdef\csname R@an.buildpath.claim.parity\endcsname{HyReX matches / is on par with / is equivalent to the residual-encoder topology}
\expandafter\gdef\csname R@an.buildpath.claim.parity.def\endcsname{no outcome licenses it: a like-for-like difference inside the 0.50 pp floor is NOT RESOLVED, never an equivalence (Addendum X5), so this claim is false whatever the data show}
\expandafter\gdef\csname R@an.buildpath.claim.parity.measured\endcsname{no outcome licenses it; the measured like-for-like difference on KiTS23 is +0.22 pp, inside the 0.50 pp floor, which is NOT RESOLVED and not an equivalence}
\expandafter\gdef\csname R@an.buildpath.claim.parity.state\endcsname{false}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.buildre.ci\endcsname{\ensuremath{[+0.02,\,+0.33]}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.buildre.clause\endcsname{ResEnc-M minus ResEnc-matched is +0.18 pp over the four confirmation folds (improves in every fold; per fold +0.11, +0.08, +0.28, +0.23; 95 \% interval [+0.02, +0.33])}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.buildre.dcv\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.buildre.f1\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.buildre.f2\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.buildre.f3\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.buildre.f4\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.buildre.hi\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.buildre.label\endcsname{re-implementation difference, the stock preset minus the ResEnc-matched re-implementation}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.buildre.lo\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.buildre.name\endcsname{ResEnc-M $-$ ResEnc-matched}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.buildre.nfull\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.buildre.npos\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.buildre.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.buildre.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvplain.ci\endcsname{\ensuremath{[+0.10,\,+0.56]}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvplain.clause\endcsname{HyReX minus default is +0.33 pp over the four confirmation folds (improves in every fold; per fold +0.34, +0.51, +0.15, +0.33; 95 \% interval [+0.10, +0.56])}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvplain.dcv\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvplain.f1\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvplain.f2\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvplain.f3\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvplain.f4\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvplain.hi\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvplain.label\endcsname{the registered contrast HyReX minus the default}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvplain.lo\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvplain.name\endcsname{HyReX $-$ default}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvplain.nfull\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvplain.npos\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvplain.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvplain.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvre.ci\endcsname{\ensuremath{[-0.24,\,+0.31]}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvre.clause\endcsname{ResEnc-M minus HyReX is +0.04 pp over the four confirmation folds (improves on average (2/4 folds); per fold \ensuremath{-}0.06, \ensuremath{-}0.15, +0.24, +0.11; 95 \% interval [\ensuremath{-}0.24, +0.31])}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvre.dcv\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvre.f1\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvre.f2\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvre.f3\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvre.f4\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvre.hi\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvre.label\endcsname{the registered contrast ResEnc-M minus HyReX}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvre.lo\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvre.name\endcsname{ResEnc-M $-$ HyReX}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvre.nfull\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvre.npos\endcsname{2}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvre.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.cvre.word\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.design.ci\endcsname{\ensuremath{[+0.06,\,+0.76]}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.design.clause\endcsname{HyReX minus function-identical control is +0.41 pp over the four confirmation folds (improves in every fold; per fold +0.45, +0.70, +0.17, +0.33; 95 \% interval [+0.06, +0.76])}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.design.dcv\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.design.f1\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.design.f2\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.design.f3\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.design.f4\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.design.hi\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.design.label\endcsname{design margin, HyReX minus the function-identical control}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.design.lo\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.design.name\endcsname{HyReX $-$ function-identical control}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.design.nfull\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.design.npos\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.design.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.design.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.id.plain.gap\endcsname{0.0e+00}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.id.plain.nfolds\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.id.plain.state\endcsname{holds}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.id.re.gap\endcsname{0.0e+00}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.id.re.nfolds\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.id.re.state\endcsname{holds}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.impl.ci\endcsname{\ensuremath{[-0.22,\,+0.06]}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.impl.clause\endcsname{function-identical control minus default is \ensuremath{-}0.08 pp over the four confirmation folds (does not improve in cross-validation; per fold \ensuremath{-}0.11, \ensuremath{-}0.19, \ensuremath{-}0.02, 0.00; 95 \% interval [\ensuremath{-}0.22, +0.06])}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.impl.dcv\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.impl.f1\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.impl.f2\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.impl.f3\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.impl.f4\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.impl.hi\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.impl.label\endcsname{control offset, the function-identical control minus the default}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.impl.lo\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.impl.name\endcsname{function-identical control $-$ default}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.impl.nfull\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.impl.npos\endcsname{1}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.impl.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.impl.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.likere.ci\endcsname{\ensuremath{[-0.27,\,-0.01]}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.likere.clause\endcsname{ResEnc-matched minus HyReX is \ensuremath{-}0.14 pp over the four confirmation folds (does not improve in cross-validation; per fold \ensuremath{-}0.16, \ensuremath{-}0.23, \ensuremath{-}0.04, \ensuremath{-}0.12; 95 \% interval [\ensuremath{-}0.27, \ensuremath{-}0.01])}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.likere.dcv\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.likere.f1\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.likere.f2\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.likere.f3\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.likere.f4\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.likere.hi\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.likere.label\endcsname{like-for-like, the ResEnc-matched re-implementation minus HyReX}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.likere.lo\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.likere.name\endcsname{ResEnc-matched $-$ HyReX}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.likere.nfull\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.likere.npos\endcsname{0}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.likere.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.cv.acdc.likere.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.buildpath.cv.amos.buildre.ci\endcsname{\ensuremath{[-0.28,\,+0.24]}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.buildre.clause\endcsname{ResEnc-M minus ResEnc-matched is \ensuremath{-}0.02 pp over the four confirmation folds (does not improve in cross-validation; per fold \ensuremath{-}0.18, +0.21, \ensuremath{-}0.06, \ensuremath{-}0.06; 95 \% interval [\ensuremath{-}0.28, +0.24])}
\expandafter\gdef\csname R@an.buildpath.cv.amos.buildre.dcv\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.buildre.f1\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.buildre.f2\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.buildre.f3\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.buildre.f4\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.buildre.hi\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.buildre.label\endcsname{re-implementation difference, the stock preset minus the ResEnc-matched re-implementation}
\expandafter\gdef\csname R@an.buildpath.cv.amos.buildre.lo\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.buildre.name\endcsname{ResEnc-M $-$ ResEnc-matched}
\expandafter\gdef\csname R@an.buildpath.cv.amos.buildre.nfull\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.amos.buildre.npos\endcsname{1}
\expandafter\gdef\csname R@an.buildpath.cv.amos.buildre.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.cv.amos.buildre.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvplain.ci\endcsname{\ensuremath{[-0.08,\,+0.54]}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvplain.clause\endcsname{HyReX minus default is +0.23 pp over the four confirmation folds (improves on average (3/4 folds); per fold \ensuremath{-}0.03, +0.36, +0.19, +0.39; 95 \% interval [\ensuremath{-}0.08, +0.54])}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvplain.dcv\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvplain.f1\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvplain.f2\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvplain.f3\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvplain.f4\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvplain.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvplain.label\endcsname{the registered contrast HyReX minus the default}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvplain.lo\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvplain.name\endcsname{HyReX $-$ default}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvplain.nfull\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvplain.npos\endcsname{3}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvplain.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvplain.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvre.ci\endcsname{\ensuremath{[-0.40,\,+0.76]}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvre.clause\endcsname{ResEnc-M minus HyReX is +0.18 pp over the four confirmation folds (improves on average (3/4 folds); per fold +0.37, +0.41, \ensuremath{-}0.37, +0.30; 95 \% interval [\ensuremath{-}0.40, +0.76])}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvre.dcv\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvre.f1\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvre.f2\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvre.f3\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvre.f4\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvre.hi\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvre.label\endcsname{the registered contrast ResEnc-M minus HyReX}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvre.lo\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvre.name\endcsname{ResEnc-M $-$ HyReX}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvre.nfull\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvre.npos\endcsname{3}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvre.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.cv.amos.cvre.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.buildpath.cv.amos.design.ci\endcsname{\ensuremath{[-0.03,\,+0.55]}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.design.clause\endcsname{HyReX minus function-identical control is +0.26 pp over the four confirmation folds (improves in every fold; per fold +0.32, +0.21, +0.47, +0.04; 95 \% interval [\ensuremath{-}0.03, +0.55])}
\expandafter\gdef\csname R@an.buildpath.cv.amos.design.dcv\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.design.f1\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.design.f2\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.design.f3\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.design.f4\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.design.hi\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.design.label\endcsname{design margin, HyReX minus the function-identical control}
\expandafter\gdef\csname R@an.buildpath.cv.amos.design.lo\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.design.name\endcsname{HyReX $-$ function-identical control}
\expandafter\gdef\csname R@an.buildpath.cv.amos.design.nfull\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.amos.design.npos\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.amos.design.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.cv.amos.design.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.buildpath.cv.amos.id.plain.gap\endcsname{0.0e+00}
\expandafter\gdef\csname R@an.buildpath.cv.amos.id.plain.nfolds\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.amos.id.plain.state\endcsname{holds}
\expandafter\gdef\csname R@an.buildpath.cv.amos.id.re.gap\endcsname{0.0e+00}
\expandafter\gdef\csname R@an.buildpath.cv.amos.id.re.nfolds\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.amos.id.re.state\endcsname{holds}
\expandafter\gdef\csname R@an.buildpath.cv.amos.impl.ci\endcsname{\ensuremath{[-0.57,\,+0.51]}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.impl.clause\endcsname{function-identical control minus default is \ensuremath{-}0.03 pp over the four confirmation folds (does not improve in cross-validation; per fold \ensuremath{-}0.35, +0.16, \ensuremath{-}0.28, +0.35; 95 \% interval [\ensuremath{-}0.57, +0.51])}
\expandafter\gdef\csname R@an.buildpath.cv.amos.impl.dcv\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.impl.f1\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.impl.f2\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.impl.f3\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.impl.f4\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.impl.hi\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.impl.label\endcsname{control offset, the function-identical control minus the default}
\expandafter\gdef\csname R@an.buildpath.cv.amos.impl.lo\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.impl.name\endcsname{function-identical control $-$ default}
\expandafter\gdef\csname R@an.buildpath.cv.amos.impl.nfull\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.amos.impl.npos\endcsname{2}
\expandafter\gdef\csname R@an.buildpath.cv.amos.impl.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.cv.amos.impl.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.buildpath.cv.amos.likere.ci\endcsname{\ensuremath{[-0.38,\,+0.78]}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.likere.clause\endcsname{ResEnc-matched minus HyReX is +0.20 pp over the four confirmation folds (improves on average (3/4 folds); per fold +0.55, +0.19, \ensuremath{-}0.30, +0.36; 95 \% interval [\ensuremath{-}0.38, +0.78])}
\expandafter\gdef\csname R@an.buildpath.cv.amos.likere.dcv\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.likere.f1\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.likere.f2\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.likere.f3\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.likere.f4\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.likere.hi\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.likere.label\endcsname{like-for-like, the ResEnc-matched re-implementation minus HyReX}
\expandafter\gdef\csname R@an.buildpath.cv.amos.likere.lo\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.buildpath.cv.amos.likere.name\endcsname{ResEnc-matched $-$ HyReX}
\expandafter\gdef\csname R@an.buildpath.cv.amos.likere.nfull\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.amos.likere.npos\endcsname{3}
\expandafter\gdef\csname R@an.buildpath.cv.amos.likere.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.cv.amos.likere.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.buildpath.cv.kits.buildre.ci\endcsname{\ensuremath{[-0.45,\,+1.66]}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.buildre.clause\endcsname{ResEnc-M minus ResEnc-matched is +0.60 pp over the four confirmation folds (improves on average (3/4 folds); per fold +0.23, +1.28, \ensuremath{-}0.13, +1.03; 95 \% interval [\ensuremath{-}0.45, +1.66])}
\expandafter\gdef\csname R@an.buildpath.cv.kits.buildre.dcv\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.buildre.f1\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.buildre.f2\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.buildre.f3\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.buildre.f4\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.buildre.hi\endcsname{\ensuremath{+1.66}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.buildre.label\endcsname{re-implementation difference, the stock preset minus the ResEnc-matched re-implementation}
\expandafter\gdef\csname R@an.buildpath.cv.kits.buildre.lo\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.buildre.name\endcsname{ResEnc-M $-$ ResEnc-matched}
\expandafter\gdef\csname R@an.buildpath.cv.kits.buildre.nfull\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.kits.buildre.npos\endcsname{3}
\expandafter\gdef\csname R@an.buildpath.cv.kits.buildre.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.cv.kits.buildre.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvplain.ci\endcsname{\ensuremath{[-1.08,\,+2.44]}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvplain.clause\endcsname{HyReX minus default is +0.68 pp over the four confirmation folds (improves on average (3/4 folds); per fold +2.31, +0.20, +0.38, \ensuremath{-}0.15; 95 \% interval [\ensuremath{-}1.08, +2.44])}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvplain.dcv\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvplain.f1\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvplain.f2\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvplain.f3\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvplain.f4\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvplain.hi\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvplain.label\endcsname{the registered contrast HyReX minus the default}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvplain.lo\endcsname{\ensuremath{-1.08}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvplain.name\endcsname{HyReX $-$ default}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvplain.nfull\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvplain.npos\endcsname{3}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvplain.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvplain.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvre.ci\endcsname{\ensuremath{[-0.24,\,+3.17]}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvre.clause\endcsname{ResEnc-M minus HyReX is +1.47 pp over the four confirmation folds (improves in every fold; per fold +0.27, +2.74, +0.98, +1.87; 95 \% interval [\ensuremath{-}0.24, +3.17])}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvre.dcv\endcsname{\ensuremath{+1.47}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvre.f1\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvre.f2\endcsname{\ensuremath{+2.74}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvre.f3\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvre.f4\endcsname{\ensuremath{+1.87}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvre.hi\endcsname{\ensuremath{+3.17}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvre.label\endcsname{the registered contrast ResEnc-M minus HyReX}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvre.lo\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvre.name\endcsname{ResEnc-M $-$ HyReX}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvre.nfull\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvre.npos\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvre.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.cv.kits.cvre.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.buildpath.cv.kits.design.ci\endcsname{\ensuremath{[-0.73,\,+0.98]}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.design.clause\endcsname{HyReX minus function-identical control is +0.12 pp over the four confirmation folds (improves on average (2/4 folds); per fold \ensuremath{-}0.07, +0.10, \ensuremath{-}0.40, +0.87; 95 \% interval [\ensuremath{-}0.73, +0.98])}
\expandafter\gdef\csname R@an.buildpath.cv.kits.design.dcv\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.design.f1\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.design.f2\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.design.f3\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.design.f4\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.design.hi\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.design.label\endcsname{design margin, HyReX minus the function-identical control}
\expandafter\gdef\csname R@an.buildpath.cv.kits.design.lo\endcsname{\ensuremath{-0.73}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.design.name\endcsname{HyReX $-$ function-identical control}
\expandafter\gdef\csname R@an.buildpath.cv.kits.design.nfull\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.kits.design.npos\endcsname{2}
\expandafter\gdef\csname R@an.buildpath.cv.kits.design.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.cv.kits.design.word\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.buildpath.cv.kits.id.plain.gap\endcsname{0.0e+00}
\expandafter\gdef\csname R@an.buildpath.cv.kits.id.plain.nfolds\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.kits.id.plain.state\endcsname{holds}
\expandafter\gdef\csname R@an.buildpath.cv.kits.id.re.gap\endcsname{0.0e+00}
\expandafter\gdef\csname R@an.buildpath.cv.kits.id.re.nfolds\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.kits.id.re.state\endcsname{holds}
\expandafter\gdef\csname R@an.buildpath.cv.kits.impl.ci\endcsname{\ensuremath{[-1.71,\,+2.82]}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.impl.clause\endcsname{function-identical control minus default is +0.56 pp over the four confirmation folds (improves on average (3/4 folds); per fold +2.38, +0.10, +0.77, \ensuremath{-}1.02; 95 \% interval [\ensuremath{-}1.71, +2.82])}
\expandafter\gdef\csname R@an.buildpath.cv.kits.impl.dcv\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.impl.f1\endcsname{\ensuremath{+2.38}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.impl.f2\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.impl.f3\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.impl.f4\endcsname{\ensuremath{-1.02}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.impl.hi\endcsname{\ensuremath{+2.82}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.impl.label\endcsname{control offset, the function-identical control minus the default}
\expandafter\gdef\csname R@an.buildpath.cv.kits.impl.lo\endcsname{\ensuremath{-1.71}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.impl.name\endcsname{function-identical control $-$ default}
\expandafter\gdef\csname R@an.buildpath.cv.kits.impl.nfull\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.kits.impl.npos\endcsname{3}
\expandafter\gdef\csname R@an.buildpath.cv.kits.impl.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.cv.kits.impl.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.buildpath.cv.kits.likere.ci\endcsname{\ensuremath{[-0.10,\,+1.82]}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.likere.clause\endcsname{ResEnc-matched minus HyReX is +0.86 pp over the four confirmation folds (improves in every fold; per fold +0.04, +1.46, +1.11, +0.84; 95 \% interval [\ensuremath{-}0.10, +1.82])}
\expandafter\gdef\csname R@an.buildpath.cv.kits.likere.dcv\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.likere.f1\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.likere.f2\endcsname{\ensuremath{+1.46}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.likere.f3\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.likere.f4\endcsname{\ensuremath{+0.84}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.likere.hi\endcsname{\ensuremath{+1.82}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.likere.label\endcsname{like-for-like, the ResEnc-matched re-implementation minus HyReX}
\expandafter\gdef\csname R@an.buildpath.cv.kits.likere.lo\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.buildpath.cv.kits.likere.name\endcsname{ResEnc-matched $-$ HyReX}
\expandafter\gdef\csname R@an.buildpath.cv.kits.likere.nfull\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.kits.likere.npos\endcsname{4}
\expandafter\gdef\csname R@an.buildpath.cv.kits.likere.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.cv.kits.likere.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.buildpath.cv.nall\endcsname{60}
\expandafter\gdef\csname R@an.buildpath.cv.ndone\endcsname{60}
\expandafter\gdef\csname R@an.buildpath.cv.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L1.dice\endcsname{92.251}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L1.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L1.params\endcsname{101.53}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L1.s0\endcsname{92.345}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L1.s1\endcsname{92.268}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L1.s2\endcsname{92.234}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L1.src\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L1.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L1b.dice\endcsname{92.328}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L1b.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L1b.params\endcsname{101.63}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L1b.s0\endcsname{92.293}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L1b.s1\endcsname{92.296}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L1b.s2\endcsname{92.361}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L1b.src\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L1b.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L3.dice\endcsname{92.460}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L3.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L3.params\endcsname{28.85}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L3.s0\endcsname{92.626}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L3.s1\endcsname{92.426}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L3.s2\endcsname{92.493}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L3.src\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.L3.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.P3c.dice\endcsname{92.126}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.P3c.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.P3c.params\endcsname{30.38}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.P3c.s0\endcsname{91.997}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.P3c.s1\endcsname{92.134}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.P3c.s2\endcsname{92.118}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.P3c.src\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.P3c.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.W1c.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.W1c.src\endcsname{pending}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.W1c.state\endcsname{pending}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.base.dice\endcsname{92.009}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.base.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.base.params\endcsname{30.38}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.base.src\endcsname{the frozen default pool}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.base.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildplain.abs\endcsname{0.12}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildplain.alt.uncompiled\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildplain.clause\endcsname{on ACDC fold 0, function-identical control minus default is +0.12 pp over two fresh seeds each (0.23 times the 0.50 pp one-seed pair floor; 0.34 times the ACDC resolution yardstick; 1.45 standard errors of a two-seed mean against the six-run frozen pool; the runs of the function-identical control and the frozen six-run default pool interleave)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildplain.floor\endcsname{0.23}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildplain.gap\endcsname{0.000}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildplain.label\endcsname{rebuild offset, plain family}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildplain.name\endcsname{function-identical control $-$ default}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildplain.nse\endcsname{1.45}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildplain.resolved\endcsname{inside}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildplain.se\endcsname{0.081}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildplain.sep\endcsname{the runs of the function-identical control and the frozen six-run default pool interleave}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildplain.sepref\endcsname{the frozen six-run default pool}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildplain.sepword\endcsname{interleaved}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildplain.short\endcsname{on ACDC fold 0, function-identical control minus default is +0.12 pp over two fresh seeds each (0.23 times the 0.50 pp one-seed pair floor) and \ensuremath{-}0.01 pp at seed 0}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildplain.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildplain.val\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildplain.yard\endcsname{0.34}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre.abs\endcsname{0.08}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre.clause\endcsname{on ACDC fold 0, ResEnc-matched minus ResEnc-M is +0.08 pp over two fresh seeds each (0.15 times the 0.50 pp one-seed pair floor; 0.22 times the ACDC resolution yardstick; 0.78 standard errors of a two-versus-two difference at the ACDC pool SD of 0.099; every run of ResEnc-matched lies above every run of ResEnc-M (fresh seeds 1 and 2), smallest gap 0.027 pp)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre.floor\endcsname{0.15}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre.gap\endcsname{0.027}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre.label\endcsname{re-implementation difference, residual-encoder family}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre.name\endcsname{ResEnc-matched $-$ ResEnc-M}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre.nse\endcsname{0.78}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre.resolved\endcsname{inside}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre.se\endcsname{0.099}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre.sep\endcsname{every run of ResEnc-matched lies above every run of ResEnc-M (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre.sepref\endcsname{ResEnc-M (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre.sepword\endcsname{separated}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre.short\endcsname{on ACDC fold 0, ResEnc-matched minus ResEnc-M is +0.08 pp over two fresh seeds each (0.15 times the 0.50 pp one-seed pair floor)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre.val\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre.yard\endcsname{0.22}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre_rev.abs\endcsname{0.08}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre_rev.clause\endcsname{on ACDC fold 0, ResEnc-M minus ResEnc-matched is \ensuremath{-}0.08 pp over two fresh seeds each (0.15 times the 0.50 pp one-seed pair floor; 0.22 times the ACDC resolution yardstick; 0.78 standard errors of a two-versus-two difference at the ACDC pool SD of 0.099; every run of ResEnc-M lies below every run of ResEnc-matched (fresh seeds 1 and 2), smallest gap 0.027 pp)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre_rev.floor\endcsname{0.15}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre_rev.gap\endcsname{0.027}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre_rev.label\endcsname{the stock preset minus the ResEnc-matched re-implementation}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre_rev.name\endcsname{ResEnc-M $-$ ResEnc-matched}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre_rev.nse\endcsname{0.78}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre_rev.resolved\endcsname{inside}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre_rev.se\endcsname{0.099}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre_rev.sep\endcsname{every run of ResEnc-M lies below every run of ResEnc-matched (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre_rev.sepref\endcsname{ResEnc-matched (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre_rev.sepword\endcsname{separated (the other way)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre_rev.short\endcsname{on ACDC fold 0, ResEnc-M minus ResEnc-matched is \ensuremath{-}0.08 pp over two fresh seeds each (0.15 times the 0.50 pp one-seed pair floor)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre_rev.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre_rev.val\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.buildre_rev.yard\endcsname{0.22}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.decomp.plain\endcsname{On ACDC, the registered fresh-seed margin of HyReX over the stock default pool is +0.45 pp and splits exactly into rebuild offset, plain family of +0.12 pp and design margin over the function-identical control of +0.33 pp}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.decomp.re\endcsname{On ACDC, the stock preset against HyReX is \ensuremath{-}0.21 pp and splits exactly into the stock preset minus the ResEnc-matched re-implementation of \ensuremath{-}0.08 pp and like-for-like, both plan-aware builds of \ensuremath{-}0.13 pp}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.design.abs\endcsname{0.33}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.design.clause\endcsname{on ACDC fold 0, HyReX minus function-identical control is +0.33 pp over two fresh seeds each (0.67 times the 0.50 pp one-seed pair floor; 0.96 times the ACDC resolution yardstick; 3.37 standard errors of a two-versus-two difference at the ACDC pool SD of 0.099; every run of HyReX lies above every run of the function-identical control (fresh seeds 1 and 2), smallest gap 0.292 pp)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.design.floor\endcsname{0.67}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.design.gap\endcsname{0.292}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.design.label\endcsname{design margin over the function-identical control}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.design.name\endcsname{HyReX $-$ function-identical control}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.design.nse\endcsname{3.37}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.design.resolved\endcsname{inside}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.design.se\endcsname{0.099}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.design.sep\endcsname{every run of HyReX lies above every run of the function-identical control (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.design.sepref\endcsname{the function-identical control (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.design.sepword\endcsname{separated}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.design.short\endcsname{on ACDC fold 0, HyReX minus function-identical control is +0.33 pp over two fresh seeds each (0.67 times the 0.50 pp one-seed pair floor)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.design.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.design.val\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.design.yard\endcsname{0.96}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.hyrex.abs\endcsname{0.45}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.hyrex.alt.uncompiled\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.hyrex.clause\endcsname{on ACDC fold 0, HyReX minus default is +0.45 pp over two fresh seeds each (0.90 times the 0.50 pp one-seed pair floor; 1.30 times the ACDC resolution yardstick; 5.58 standard errors of a two-seed mean against the six-run frozen pool; every run of HyReX lies above every run of the frozen six-run default pool, smallest gap 0.298 pp)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.hyrex.floor\endcsname{0.90}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.hyrex.gap\endcsname{0.298}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.hyrex.label\endcsname{the registered fresh-seed margin}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.hyrex.name\endcsname{HyReX $-$ default}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.hyrex.nse\endcsname{5.58}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.hyrex.resolved\endcsname{inside}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.hyrex.se\endcsname{0.081}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.hyrex.sep\endcsname{every run of HyReX lies above every run of the frozen six-run default pool}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.hyrex.sepref\endcsname{the frozen six-run default pool}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.hyrex.sepword\endcsname{separated}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.hyrex.short\endcsname{on ACDC fold 0, HyReX minus default is +0.45 pp over two fresh seeds each (0.90 times the 0.50 pp one-seed pair floor) and +0.62 pp at seed 0}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.hyrex.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.hyrex.val\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.hyrex.yard\endcsname{1.30}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.id.plain.gap\endcsname{0.0e+00}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.id.plain.state\endcsname{holds}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.id.re.gap\endcsname{0.0e+00}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.id.re.state\endcsname{holds}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.like.abs\endcsname{0.13}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.like.clause\endcsname{on ACDC fold 0, ResEnc-matched minus HyReX is \ensuremath{-}0.13 pp over two fresh seeds each (0.26 times the 0.50 pp one-seed pair floor; 0.38 times the ACDC resolution yardstick; 1.33 standard errors of a two-versus-two difference at the ACDC pool SD of 0.099; every run of ResEnc-matched lies below every run of HyReX (fresh seeds 1 and 2), smallest gap 0.065 pp)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.like.floor\endcsname{0.26}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.like.gap\endcsname{0.065}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.like.label\endcsname{like-for-like, both plan-aware builds}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.like.name\endcsname{ResEnc-matched $-$ HyReX}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.like.nse\endcsname{1.33}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.like.resolved\endcsname{inside}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.like.se\endcsname{0.099}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.like.sep\endcsname{every run of ResEnc-matched lies below every run of HyReX (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.like.sepref\endcsname{HyReX (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.like.sepword\endcsname{separated (the other way)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.like.short\endcsname{on ACDC fold 0, ResEnc-matched minus HyReX is \ensuremath{-}0.13 pp over two fresh seeds each (0.26 times the 0.50 pp one-seed pair floor)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.like.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.like.val\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.like.yard\endcsname{0.38}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.pool\endcsname{92.009}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.pooln\endcsname{6}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.pooln.word\endcsname{six}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.poolsd\endcsname{0.099}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.ref.uncompiled.label\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.ref.uncompiled.mean\endcsname{92.016}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.ref.uncompiled.n\endcsname{3}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.ref.uncompiled.shift\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.ref.uncompiled.state\endcsname{landed}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.stockre.abs\endcsname{0.21}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.stockre.clause\endcsname{on ACDC fold 0, ResEnc-M minus HyReX is \ensuremath{-}0.21 pp over two fresh seeds each (0.42 times the 0.50 pp one-seed pair floor; 0.60 times the ACDC resolution yardstick; 2.11 standard errors of a two-versus-two difference at the ACDC pool SD of 0.099; every run of ResEnc-M lies below every run of HyReX (fresh seeds 1 and 2), smallest gap 0.158 pp)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.stockre.floor\endcsname{0.42}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.stockre.gap\endcsname{0.158}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.stockre.label\endcsname{the stock preset against HyReX}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.stockre.name\endcsname{ResEnc-M $-$ HyReX}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.stockre.nse\endcsname{2.11}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.stockre.resolved\endcsname{inside}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.stockre.se\endcsname{0.099}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.stockre.sep\endcsname{every run of ResEnc-M lies below every run of HyReX (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.stockre.sepref\endcsname{HyReX (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.stockre.sepword\endcsname{separated (the other way)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.stockre.short\endcsname{on ACDC fold 0, ResEnc-M minus HyReX is \ensuremath{-}0.21 pp over two fresh seeds each (0.42 times the 0.50 pp one-seed pair floor)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.stockre.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.stockre.val\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.stockre.yard\endcsname{0.60}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.w1cpool.clause\endcsname{branch control minus default is pending on ACDC (branch control is not complete at two fresh seeds)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.w1cpool.label\endcsname{a second default-sized plan-aware design}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.w1cpool.name\endcsname{branch control $-$ default}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.w1cpool.se\endcsname{0.081}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.w1cpool.short\endcsname{branch control minus default is pending on ACDC (branch control is not complete at two fresh seeds)}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.w1cpool.state\endcsname{pending}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.w1cpool.val\endcsname{\leavevmode\pend}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.yard\endcsname{0.35}
\expandafter\gdef\csname R@an.buildpath.f0.acdc.yard.def\endcsname{the ACDC resolution yardstick of Addendum R: the smallest pair difference a two-seed contrast resolves at that benchmark's own pool SD (two-sided, 5 \% level, 80 \% power)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L1.dice\endcsname{88.166}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L1.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L1.params\endcsname{102.28}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L1.s0\endcsname{88.348}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L1.s1\endcsname{88.363}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L1.s2\endcsname{87.969}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L1.src\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L1.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L1b.dice\endcsname{87.999}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L1b.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L1b.params\endcsname{102.37}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L1b.s0\endcsname{87.839}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L1b.s1\endcsname{88.127}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L1b.s2\endcsname{87.870}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L1b.src\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L1b.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L3.dice\endcsname{87.833}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L3.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L3.params\endcsname{29.59}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L3.s0\endcsname{88.083}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L3.s1\endcsname{87.981}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L3.s2\endcsname{87.686}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L3.src\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.buildpath.f0.amos.L3.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.amos.P3c.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.buildpath.f0.amos.P3c.params\endcsname{31.12}
\expandafter\gdef\csname R@an.buildpath.f0.amos.P3c.s0\endcsname{87.708}
\expandafter\gdef\csname R@an.buildpath.f0.amos.P3c.src\endcsname{pending}
\expandafter\gdef\csname R@an.buildpath.f0.amos.P3c.state\endcsname{pending}
\expandafter\gdef\csname R@an.buildpath.f0.amos.W1c.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.buildpath.f0.amos.W1c.params\endcsname{31.14}
\expandafter\gdef\csname R@an.buildpath.f0.amos.W1c.s0\endcsname{88.064}
\expandafter\gdef\csname R@an.buildpath.f0.amos.W1c.src\endcsname{pending}
\expandafter\gdef\csname R@an.buildpath.f0.amos.W1c.state\endcsname{pending}
\expandafter\gdef\csname R@an.buildpath.f0.amos.base.dice\endcsname{87.701}
\expandafter\gdef\csname R@an.buildpath.f0.amos.base.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.buildpath.f0.amos.base.params\endcsname{31.12}
\expandafter\gdef\csname R@an.buildpath.f0.amos.base.src\endcsname{the frozen default pool}
\expandafter\gdef\csname R@an.buildpath.f0.amos.base.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildplain.clause\endcsname{function-identical control minus default is pending on AMOS22 (function-identical control is not complete at two fresh seeds)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildplain.label\endcsname{rebuild offset, plain family}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildplain.name\endcsname{function-identical control $-$ default}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildplain.se\endcsname{0.100}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildplain.short\endcsname{function-identical control minus default is pending on AMOS22 (function-identical control is not complete at two fresh seeds)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildplain.state\endcsname{pending}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildplain.val\endcsname{\leavevmode\pend}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre.abs\endcsname{0.17}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre.clause\endcsname{on AMOS22 fold 0, ResEnc-matched minus ResEnc-M is \ensuremath{-}0.17 pp over two fresh seeds each (0.33 times the 0.50 pp one-seed pair floor; 1.37 standard errors of a two-versus-two difference at the AMOS22 pool SD of 0.122; the runs of ResEnc-matched and ResEnc-M (fresh seeds 1 and 2) interleave)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre.floor\endcsname{0.33}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre.gap\endcsname{0.000}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre.label\endcsname{re-implementation difference, residual-encoder family}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre.name\endcsname{ResEnc-matched $-$ ResEnc-M}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre.nse\endcsname{1.37}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre.resolved\endcsname{inside}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre.se\endcsname{0.122}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre.sep\endcsname{the runs of ResEnc-matched and ResEnc-M (fresh seeds 1 and 2) interleave}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre.sepref\endcsname{ResEnc-M (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre.sepword\endcsname{interleaved}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre.short\endcsname{on AMOS22 fold 0, ResEnc-matched minus ResEnc-M is \ensuremath{-}0.17 pp over two fresh seeds each (0.33 times the 0.50 pp one-seed pair floor)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre.val\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre_rev.abs\endcsname{0.17}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre_rev.clause\endcsname{on AMOS22 fold 0, ResEnc-M minus ResEnc-matched is +0.17 pp over two fresh seeds each (0.33 times the 0.50 pp one-seed pair floor; 1.37 standard errors of a two-versus-two difference at the AMOS22 pool SD of 0.122; the runs of ResEnc-M and ResEnc-matched (fresh seeds 1 and 2) interleave)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre_rev.floor\endcsname{0.33}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre_rev.gap\endcsname{0.000}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre_rev.label\endcsname{the stock preset minus the ResEnc-matched re-implementation}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre_rev.name\endcsname{ResEnc-M $-$ ResEnc-matched}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre_rev.nse\endcsname{1.37}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre_rev.resolved\endcsname{inside}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre_rev.se\endcsname{0.122}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre_rev.sep\endcsname{the runs of ResEnc-M and ResEnc-matched (fresh seeds 1 and 2) interleave}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre_rev.sepref\endcsname{ResEnc-matched (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre_rev.sepword\endcsname{interleaved}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre_rev.short\endcsname{on AMOS22 fold 0, ResEnc-M minus ResEnc-matched is +0.17 pp over two fresh seeds each (0.33 times the 0.50 pp one-seed pair floor)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre_rev.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.amos.buildre_rev.val\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.buildpath.f0.amos.decomp.plain\endcsname{On AMOS22 the decomposition is pending (function-identical control not complete at two fresh seeds)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.decomp.re\endcsname{On AMOS22, the stock preset against HyReX is +0.33 pp and splits exactly into the stock preset minus the ResEnc-matched re-implementation of +0.17 pp and like-for-like, both plan-aware builds of +0.17 pp}
\expandafter\gdef\csname R@an.buildpath.f0.amos.design.clause\endcsname{HyReX minus function-identical control is pending on AMOS22 (function-identical control is not complete at two fresh seeds)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.design.label\endcsname{design margin over the function-identical control}
\expandafter\gdef\csname R@an.buildpath.f0.amos.design.name\endcsname{HyReX $-$ function-identical control}
\expandafter\gdef\csname R@an.buildpath.f0.amos.design.se\endcsname{0.122}
\expandafter\gdef\csname R@an.buildpath.f0.amos.design.short\endcsname{HyReX minus function-identical control is pending on AMOS22 (function-identical control is not complete at two fresh seeds)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.design.state\endcsname{pending}
\expandafter\gdef\csname R@an.buildpath.f0.amos.design.val\endcsname{\leavevmode\pend}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.abs\endcsname{0.13}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.alt.contemporaneous\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.alt.uncompiled\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.clause\endcsname{on AMOS22 fold 0, HyReX minus default is +0.13 pp over two fresh seeds each (0.26 times the 0.50 pp one-seed pair floor; 1.33 standard errors of a two-seed mean against the six-run frozen pool; the runs of HyReX and the frozen six-run default pool interleave; the runs of HyReX and the nine-run reference interleave)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.floor\endcsname{0.26}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.gap\endcsname{0.000}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.gap.union\endcsname{0.000}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.label\endcsname{the registered fresh-seed margin}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.name\endcsname{HyReX $-$ default}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.nse\endcsname{1.33}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.resolved\endcsname{inside}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.se\endcsname{0.100}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.sep\endcsname{the runs of HyReX and the frozen six-run default pool interleave}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.sep.union\endcsname{the runs of HyReX and the nine-run reference interleave}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.sepref\endcsname{the frozen six-run default pool}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.sepref.union\endcsname{the nine-run reference}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.sepword\endcsname{interleaved}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.sepword.union\endcsname{interleaved}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.short\endcsname{on AMOS22 fold 0, HyReX minus default is +0.13 pp over two fresh seeds each (0.26 times the 0.50 pp one-seed pair floor) and +0.38 pp at seed 0}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.amos.hyrex.val\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.buildpath.f0.amos.id.plain.state\endcsname{pending}
\expandafter\gdef\csname R@an.buildpath.f0.amos.id.re.gap\endcsname{0.0e+00}
\expandafter\gdef\csname R@an.buildpath.f0.amos.id.re.state\endcsname{holds}
\expandafter\gdef\csname R@an.buildpath.f0.amos.like.abs\endcsname{0.17}
\expandafter\gdef\csname R@an.buildpath.f0.amos.like.clause\endcsname{on AMOS22 fold 0, ResEnc-matched minus HyReX is +0.17 pp over two fresh seeds each (0.33 times the 0.50 pp one-seed pair floor; 1.35 standard errors of a two-versus-two difference at the AMOS22 pool SD of 0.122; the runs of ResEnc-matched and HyReX (fresh seeds 1 and 2) interleave)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.like.floor\endcsname{0.33}
\expandafter\gdef\csname R@an.buildpath.f0.amos.like.gap\endcsname{0.000}
\expandafter\gdef\csname R@an.buildpath.f0.amos.like.label\endcsname{like-for-like, both plan-aware builds}
\expandafter\gdef\csname R@an.buildpath.f0.amos.like.name\endcsname{ResEnc-matched $-$ HyReX}
\expandafter\gdef\csname R@an.buildpath.f0.amos.like.nse\endcsname{1.35}
\expandafter\gdef\csname R@an.buildpath.f0.amos.like.resolved\endcsname{inside}
\expandafter\gdef\csname R@an.buildpath.f0.amos.like.se\endcsname{0.122}
\expandafter\gdef\csname R@an.buildpath.f0.amos.like.sep\endcsname{the runs of ResEnc-matched and HyReX (fresh seeds 1 and 2) interleave}
\expandafter\gdef\csname R@an.buildpath.f0.amos.like.sepref\endcsname{HyReX (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.like.sepword\endcsname{interleaved}
\expandafter\gdef\csname R@an.buildpath.f0.amos.like.short\endcsname{on AMOS22 fold 0, ResEnc-matched minus HyReX is +0.17 pp over two fresh seeds each (0.33 times the 0.50 pp one-seed pair floor)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.like.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.amos.like.val\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.buildpath.f0.amos.pool\endcsname{87.701}
\expandafter\gdef\csname R@an.buildpath.f0.amos.pooln\endcsname{6}
\expandafter\gdef\csname R@an.buildpath.f0.amos.pooln.word\endcsname{six}
\expandafter\gdef\csname R@an.buildpath.f0.amos.poolsd\endcsname{0.122}
\expandafter\gdef\csname R@an.buildpath.f0.amos.ref.contemporaneous.label\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.buildpath.f0.amos.ref.contemporaneous.mean\endcsname{87.712}
\expandafter\gdef\csname R@an.buildpath.f0.amos.ref.contemporaneous.n\endcsname{3}
\expandafter\gdef\csname R@an.buildpath.f0.amos.ref.contemporaneous.shift\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.buildpath.f0.amos.ref.contemporaneous.state\endcsname{landed}
\expandafter\gdef\csname R@an.buildpath.f0.amos.ref.uncompiled.label\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.buildpath.f0.amos.ref.uncompiled.mean\endcsname{87.730}
\expandafter\gdef\csname R@an.buildpath.f0.amos.ref.uncompiled.n\endcsname{3}
\expandafter\gdef\csname R@an.buildpath.f0.amos.ref.uncompiled.shift\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.buildpath.f0.amos.ref.uncompiled.state\endcsname{landed}
\expandafter\gdef\csname R@an.buildpath.f0.amos.stockre.abs\endcsname{0.33}
\expandafter\gdef\csname R@an.buildpath.f0.amos.stockre.clause\endcsname{on AMOS22 fold 0, ResEnc-M minus HyReX is +0.33 pp over two fresh seeds each (0.66 times the 0.50 pp one-seed pair floor; 2.72 standard errors of a two-versus-two difference at the AMOS22 pool SD of 0.122; the runs of ResEnc-M and HyReX (fresh seeds 1 and 2) interleave)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.stockre.floor\endcsname{0.66}
\expandafter\gdef\csname R@an.buildpath.f0.amos.stockre.gap\endcsname{0.000}
\expandafter\gdef\csname R@an.buildpath.f0.amos.stockre.label\endcsname{the stock preset against HyReX}
\expandafter\gdef\csname R@an.buildpath.f0.amos.stockre.name\endcsname{ResEnc-M $-$ HyReX}
\expandafter\gdef\csname R@an.buildpath.f0.amos.stockre.nse\endcsname{2.72}
\expandafter\gdef\csname R@an.buildpath.f0.amos.stockre.resolved\endcsname{inside}
\expandafter\gdef\csname R@an.buildpath.f0.amos.stockre.se\endcsname{0.122}
\expandafter\gdef\csname R@an.buildpath.f0.amos.stockre.sep\endcsname{the runs of ResEnc-M and HyReX (fresh seeds 1 and 2) interleave}
\expandafter\gdef\csname R@an.buildpath.f0.amos.stockre.sepref\endcsname{HyReX (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.stockre.sepword\endcsname{interleaved}
\expandafter\gdef\csname R@an.buildpath.f0.amos.stockre.short\endcsname{on AMOS22 fold 0, ResEnc-M minus HyReX is +0.33 pp over two fresh seeds each (0.66 times the 0.50 pp one-seed pair floor)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.stockre.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.amos.stockre.val\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.buildpath.f0.amos.w1cpool.clause\endcsname{branch control minus default is pending on AMOS22 (branch control is not complete at two fresh seeds)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.w1cpool.label\endcsname{a second default-sized plan-aware design}
\expandafter\gdef\csname R@an.buildpath.f0.amos.w1cpool.name\endcsname{branch control $-$ default}
\expandafter\gdef\csname R@an.buildpath.f0.amos.w1cpool.se\endcsname{0.100}
\expandafter\gdef\csname R@an.buildpath.f0.amos.w1cpool.short\endcsname{branch control minus default is pending on AMOS22 (branch control is not complete at two fresh seeds)}
\expandafter\gdef\csname R@an.buildpath.f0.amos.w1cpool.state\endcsname{pending}
\expandafter\gdef\csname R@an.buildpath.f0.amos.w1cpool.val\endcsname{\leavevmode\pend}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L1.dice\endcsname{86.853}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L1.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L1.params\endcsname{102.35}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L1.s0\endcsname{85.704}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L1.s1\endcsname{86.512}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L1.s2\endcsname{87.195}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L1.src\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L1.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L1b.dice\endcsname{85.691}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L1b.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L1b.params\endcsname{102.43}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L1b.s0\endcsname{85.121}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L1b.s1\endcsname{85.942}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L1b.s2\endcsname{85.441}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L1b.src\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L1b.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L3.dice\endcsname{85.472}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L3.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L3.params\endcsname{29.66}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L3.s0\endcsname{86.220}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L3.s1\endcsname{85.176}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L3.s2\endcsname{85.768}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L3.src\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.buildpath.f0.kits.L3.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.kits.P3c.dice\endcsname{84.554}
\expandafter\gdef\csname R@an.buildpath.f0.kits.P3c.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.buildpath.f0.kits.P3c.params\endcsname{31.20}
\expandafter\gdef\csname R@an.buildpath.f0.kits.P3c.s0\endcsname{84.743}
\expandafter\gdef\csname R@an.buildpath.f0.kits.P3c.s1\endcsname{84.529}
\expandafter\gdef\csname R@an.buildpath.f0.kits.P3c.s2\endcsname{84.579}
\expandafter\gdef\csname R@an.buildpath.f0.kits.P3c.src\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.buildpath.f0.kits.P3c.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.kits.W1c.dice\endcsname{84.445}
\expandafter\gdef\csname R@an.buildpath.f0.kits.W1c.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.buildpath.f0.kits.W1c.params\endcsname{31.21}
\expandafter\gdef\csname R@an.buildpath.f0.kits.W1c.s0\endcsname{86.014}
\expandafter\gdef\csname R@an.buildpath.f0.kits.W1c.s1\endcsname{85.112}
\expandafter\gdef\csname R@an.buildpath.f0.kits.W1c.s2\endcsname{83.777}
\expandafter\gdef\csname R@an.buildpath.f0.kits.W1c.src\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.buildpath.f0.kits.W1c.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.kits.base.dice\endcsname{83.378}
\expandafter\gdef\csname R@an.buildpath.f0.kits.base.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.buildpath.f0.kits.base.params\endcsname{31.20}
\expandafter\gdef\csname R@an.buildpath.f0.kits.base.src\endcsname{the frozen default pool}
\expandafter\gdef\csname R@an.buildpath.f0.kits.base.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.abs\endcsname{1.18}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.alt.contemporaneous\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.alt.union\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.clause\endcsname{on KiTS23 fold 0, function-identical control minus default is +1.18 pp over two fresh seeds each (2.35 times the 0.50 pp one-seed pair floor; 1.62 standard errors of a two-seed mean against the three-run frozen pool; every run of the function-identical control lies above every run of the frozen three-run default pool, smallest gap 0.257 pp; the runs of the function-identical control and the six-run reference interleave)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.floor\endcsname{2.35}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.gap\endcsname{0.257}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.gap.union\endcsname{0.000}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.label\endcsname{rebuild offset, plain family}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.name\endcsname{function-identical control $-$ default}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.nse\endcsname{1.62}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.resolved\endcsname{above}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.se\endcsname{0.726}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.sep\endcsname{every run of the function-identical control lies above every run of the frozen three-run default pool}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.sep.union\endcsname{the runs of the function-identical control and the six-run reference interleave}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.sepref\endcsname{the frozen three-run default pool}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.sepref.union\endcsname{the six-run reference}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.sepword\endcsname{separated}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.sepword.union\endcsname{interleaved}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.short\endcsname{on KiTS23 fold 0, function-identical control minus default is +1.18 pp over two fresh seeds each (2.35 times the 0.50 pp one-seed pair floor) and +1.36 pp at seed 0}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildplain.val\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre.abs\endcsname{1.16}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre.clause\endcsname{on KiTS23 fold 0, ResEnc-matched minus ResEnc-M is \ensuremath{-}1.16 pp over two fresh seeds each (2.32 times the 0.50 pp one-seed pair floor; 1.46 standard errors of a two-versus-two difference at the KiTS23 pool SD of 0.795; every run of ResEnc-matched lies below every run of ResEnc-M (fresh seeds 1 and 2), smallest gap 0.570 pp)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre.floor\endcsname{2.32}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre.gap\endcsname{0.570}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre.label\endcsname{re-implementation difference, residual-encoder family}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre.name\endcsname{ResEnc-matched $-$ ResEnc-M}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre.nse\endcsname{1.46}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre.resolved\endcsname{above}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre.se\endcsname{0.795}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre.sep\endcsname{every run of ResEnc-matched lies below every run of ResEnc-M (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre.sepref\endcsname{ResEnc-M (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre.sepword\endcsname{separated (the other way)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre.short\endcsname{on KiTS23 fold 0, ResEnc-matched minus ResEnc-M is \ensuremath{-}1.16 pp over two fresh seeds each (2.32 times the 0.50 pp one-seed pair floor)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre.val\endcsname{\ensuremath{-1.16}}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre_rev.abs\endcsname{1.16}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre_rev.clause\endcsname{on KiTS23 fold 0, ResEnc-M minus ResEnc-matched is +1.16 pp over two fresh seeds each (2.32 times the 0.50 pp one-seed pair floor; 1.46 standard errors of a two-versus-two difference at the KiTS23 pool SD of 0.795; every run of ResEnc-M lies above every run of ResEnc-matched (fresh seeds 1 and 2), smallest gap 0.570 pp)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre_rev.floor\endcsname{2.32}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre_rev.gap\endcsname{0.570}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre_rev.label\endcsname{the stock preset minus the ResEnc-matched re-implementation}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre_rev.name\endcsname{ResEnc-M $-$ ResEnc-matched}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre_rev.nse\endcsname{1.46}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre_rev.resolved\endcsname{above}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre_rev.se\endcsname{0.795}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre_rev.sep\endcsname{every run of ResEnc-M lies above every run of ResEnc-matched (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre_rev.sepref\endcsname{ResEnc-matched (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre_rev.sepword\endcsname{separated}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre_rev.short\endcsname{on KiTS23 fold 0, ResEnc-M minus ResEnc-matched is +1.16 pp over two fresh seeds each (2.32 times the 0.50 pp one-seed pair floor)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre_rev.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.kits.buildre_rev.val\endcsname{\ensuremath{+1.16}}
\expandafter\gdef\csname R@an.buildpath.f0.kits.decomp.plain\endcsname{On KiTS23, the registered fresh-seed margin of HyReX over the stock default pool is +2.09 pp and splits exactly into rebuild offset, plain family of +1.18 pp and design margin over the function-identical control of +0.92 pp}
\expandafter\gdef\csname R@an.buildpath.f0.kits.decomp.re\endcsname{On KiTS23, the stock preset against HyReX is +1.38 pp and splits exactly into the stock preset minus the ResEnc-matched re-implementation of +1.16 pp and like-for-like, both plan-aware builds of +0.22 pp}
\expandafter\gdef\csname R@an.buildpath.f0.kits.design.abs\endcsname{0.92}
\expandafter\gdef\csname R@an.buildpath.f0.kits.design.clause\endcsname{on KiTS23 fold 0, HyReX minus function-identical control is +0.92 pp over two fresh seeds each (1.84 times the 0.50 pp one-seed pair floor; 1.15 standard errors of a two-versus-two difference at the KiTS23 pool SD of 0.795; every run of HyReX lies above every run of the function-identical control (fresh seeds 1 and 2), smallest gap 0.597 pp)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.design.floor\endcsname{1.84}
\expandafter\gdef\csname R@an.buildpath.f0.kits.design.gap\endcsname{0.597}
\expandafter\gdef\csname R@an.buildpath.f0.kits.design.label\endcsname{design margin over the function-identical control}
\expandafter\gdef\csname R@an.buildpath.f0.kits.design.name\endcsname{HyReX $-$ function-identical control}
\expandafter\gdef\csname R@an.buildpath.f0.kits.design.nse\endcsname{1.15}
\expandafter\gdef\csname R@an.buildpath.f0.kits.design.resolved\endcsname{above}
\expandafter\gdef\csname R@an.buildpath.f0.kits.design.se\endcsname{0.795}
\expandafter\gdef\csname R@an.buildpath.f0.kits.design.sep\endcsname{every run of HyReX lies above every run of the function-identical control (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.design.sepref\endcsname{the function-identical control (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.design.sepword\endcsname{separated}
\expandafter\gdef\csname R@an.buildpath.f0.kits.design.short\endcsname{on KiTS23 fold 0, HyReX minus function-identical control is +0.92 pp over two fresh seeds each (1.84 times the 0.50 pp one-seed pair floor)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.design.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.kits.design.val\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.abs\endcsname{2.09}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.alt.contemporaneous\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.alt.union\endcsname{\ensuremath{+1.85}}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.clause\endcsname{on KiTS23 fold 0, HyReX minus default is +2.09 pp over two fresh seeds each (4.19 times the 0.50 pp one-seed pair floor; 2.89 standard errors of a two-seed mean against the three-run frozen pool; every run of HyReX lies above every run of the frozen three-run default pool, smallest gap 0.904 pp; every run of HyReX lies above every run of the six-run reference, smallest gap 0.555 pp)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.floor\endcsname{4.19}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.gap\endcsname{0.904}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.gap.union\endcsname{0.555}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.label\endcsname{the registered fresh-seed margin}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.name\endcsname{HyReX $-$ default}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.nse\endcsname{2.89}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.resolved\endcsname{above}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.se\endcsname{0.726}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.sep\endcsname{every run of HyReX lies above every run of the frozen three-run default pool}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.sep.union\endcsname{every run of HyReX lies above every run of the six-run reference}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.sepref\endcsname{the frozen three-run default pool}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.sepref.union\endcsname{the six-run reference}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.sepword\endcsname{separated}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.sepword.union\endcsname{separated}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.short\endcsname{on KiTS23 fold 0, HyReX minus default is +2.09 pp over two fresh seeds each (4.19 times the 0.50 pp one-seed pair floor) and +2.84 pp at seed 0}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.kits.hyrex.val\endcsname{\ensuremath{+2.09}}
\expandafter\gdef\csname R@an.buildpath.f0.kits.id.plain.gap\endcsname{0.0e+00}
\expandafter\gdef\csname R@an.buildpath.f0.kits.id.plain.state\endcsname{holds}
\expandafter\gdef\csname R@an.buildpath.f0.kits.id.re.gap\endcsname{0.0e+00}
\expandafter\gdef\csname R@an.buildpath.f0.kits.id.re.state\endcsname{holds}
\expandafter\gdef\csname R@an.buildpath.f0.kits.like.abs\endcsname{0.22}
\expandafter\gdef\csname R@an.buildpath.f0.kits.like.clause\endcsname{on KiTS23 fold 0, ResEnc-matched minus HyReX is +0.22 pp over two fresh seeds each (0.44 times the 0.50 pp one-seed pair floor; 0.28 standard errors of a two-versus-two difference at the KiTS23 pool SD of 0.795; the runs of ResEnc-matched and HyReX (fresh seeds 1 and 2) interleave)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.like.floor\endcsname{0.44}
\expandafter\gdef\csname R@an.buildpath.f0.kits.like.gap\endcsname{0.000}
\expandafter\gdef\csname R@an.buildpath.f0.kits.like.label\endcsname{like-for-like, both plan-aware builds}
\expandafter\gdef\csname R@an.buildpath.f0.kits.like.name\endcsname{ResEnc-matched $-$ HyReX}
\expandafter\gdef\csname R@an.buildpath.f0.kits.like.nse\endcsname{0.28}
\expandafter\gdef\csname R@an.buildpath.f0.kits.like.resolved\endcsname{inside}
\expandafter\gdef\csname R@an.buildpath.f0.kits.like.se\endcsname{0.795}
\expandafter\gdef\csname R@an.buildpath.f0.kits.like.sep\endcsname{the runs of ResEnc-matched and HyReX (fresh seeds 1 and 2) interleave}
\expandafter\gdef\csname R@an.buildpath.f0.kits.like.sepref\endcsname{HyReX (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.like.sepword\endcsname{interleaved}
\expandafter\gdef\csname R@an.buildpath.f0.kits.like.short\endcsname{on KiTS23 fold 0, ResEnc-matched minus HyReX is +0.22 pp over two fresh seeds each (0.44 times the 0.50 pp one-seed pair floor)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.like.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.kits.like.val\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.buildpath.f0.kits.pool\endcsname{83.378}
\expandafter\gdef\csname R@an.buildpath.f0.kits.pooln\endcsname{3}
\expandafter\gdef\csname R@an.buildpath.f0.kits.pooln.word\endcsname{three}
\expandafter\gdef\csname R@an.buildpath.f0.kits.poolsd\endcsname{0.795}
\expandafter\gdef\csname R@an.buildpath.f0.kits.ref.contemporaneous.label\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.buildpath.f0.kits.ref.contemporaneous.mean\endcsname{83.866}
\expandafter\gdef\csname R@an.buildpath.f0.kits.ref.contemporaneous.n\endcsname{3}
\expandafter\gdef\csname R@an.buildpath.f0.kits.ref.contemporaneous.shift\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.buildpath.f0.kits.ref.contemporaneous.state\endcsname{landed}
\expandafter\gdef\csname R@an.buildpath.f0.kits.ref.union.label\endcsname{six-run reference}
\expandafter\gdef\csname R@an.buildpath.f0.kits.ref.union.mean\endcsname{83.622}
\expandafter\gdef\csname R@an.buildpath.f0.kits.ref.union.n\endcsname{6}
\expandafter\gdef\csname R@an.buildpath.f0.kits.ref.union.shift\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.buildpath.f0.kits.ref.union.state\endcsname{landed}
\expandafter\gdef\csname R@an.buildpath.f0.kits.stockre.abs\endcsname{1.38}
\expandafter\gdef\csname R@an.buildpath.f0.kits.stockre.clause\endcsname{on KiTS23 fold 0, ResEnc-M minus HyReX is +1.38 pp over two fresh seeds each (2.76 times the 0.50 pp one-seed pair floor; 1.74 standard errors of a two-versus-two difference at the KiTS23 pool SD of 0.795; every run of ResEnc-M lies above every run of HyReX (fresh seeds 1 and 2), smallest gap 0.744 pp)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.stockre.floor\endcsname{2.76}
\expandafter\gdef\csname R@an.buildpath.f0.kits.stockre.gap\endcsname{0.744}
\expandafter\gdef\csname R@an.buildpath.f0.kits.stockre.label\endcsname{the stock preset against HyReX}
\expandafter\gdef\csname R@an.buildpath.f0.kits.stockre.name\endcsname{ResEnc-M $-$ HyReX}
\expandafter\gdef\csname R@an.buildpath.f0.kits.stockre.nse\endcsname{1.74}
\expandafter\gdef\csname R@an.buildpath.f0.kits.stockre.resolved\endcsname{above}
\expandafter\gdef\csname R@an.buildpath.f0.kits.stockre.se\endcsname{0.795}
\expandafter\gdef\csname R@an.buildpath.f0.kits.stockre.sep\endcsname{every run of ResEnc-M lies above every run of HyReX (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.stockre.sepref\endcsname{HyReX (fresh seeds 1 and 2)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.stockre.sepword\endcsname{separated}
\expandafter\gdef\csname R@an.buildpath.f0.kits.stockre.short\endcsname{on KiTS23 fold 0, ResEnc-M minus HyReX is +1.38 pp over two fresh seeds each (2.76 times the 0.50 pp one-seed pair floor)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.stockre.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.kits.stockre.val\endcsname{\ensuremath{+1.38}}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.abs\endcsname{1.07}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.alt.contemporaneous\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.alt.union\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.clause\endcsname{on KiTS23 fold 0, branch control minus default is +1.07 pp over two fresh seeds each (2.13 times the 0.50 pp one-seed pair floor; 1.47 standard errors of a two-seed mean against the three-run frozen pool; the runs of the branch control and the frozen three-run default pool interleave; the runs of the branch control and the six-run reference interleave)}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.floor\endcsname{2.13}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.gap\endcsname{0.000}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.gap.union\endcsname{0.000}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.label\endcsname{a second default-sized plan-aware design}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.name\endcsname{branch control $-$ default}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.nse\endcsname{1.47}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.resolved\endcsname{above}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.se\endcsname{0.726}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.sep\endcsname{the runs of the branch control and the frozen three-run default pool interleave}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.sep.union\endcsname{the runs of the branch control and the six-run reference interleave}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.sepref\endcsname{the frozen three-run default pool}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.sepref.union\endcsname{the six-run reference}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.sepword\endcsname{interleaved}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.sepword.union\endcsname{interleaved}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.short\endcsname{on KiTS23 fold 0, branch control minus default is +1.07 pp over two fresh seeds each (2.13 times the 0.50 pp one-seed pair floor) and +2.64 pp at seed 0}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.state\endcsname{done}
\expandafter\gdef\csname R@an.buildpath.f0.kits.w1cpool.val\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.buildpath.floor\endcsname{0.50}
\expandafter\gdef\csname R@an.buildpath.floor.word\endcsname{0.50 pp one-seed pair floor}
\expandafter\gdef\csname R@an.buildpath.l1b.def\endcsname{the ResEnc-matched re-implementation: the ResEnc-M topology built through the path every agent design is built in, differing from the stock library preset in its stem, its shortcut form and its zero-initialisation}
\expandafter\gdef\csname R@an.buildpath.l1b.name\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.buildpath.nds\endcsname{3}
\expandafter\gdef\csname R@an.buildpath.nds.word\endcsname{three}
\expandafter\gdef\csname R@an.buildpath.nfolds.word\endcsname{four}
\expandafter\gdef\csname R@an.buildpath.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.buildpath.nfresh.word\endcsname{two}
\expandafter\gdef\csname R@an.buildpath.offset.kits.hi\endcsname{+0.97}
\expandafter\gdef\csname R@an.buildpath.offset.kits.lo\endcsname{\ensuremath{-}0.18}
\expandafter\gdef\csname R@an.buildpath.offset.kits.np3c\endcsname{8}
\expandafter\gdef\csname R@an.buildpath.offset.kits.nstock\endcsname{9}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.abs\endcsname{0.88}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.band\endcsname{inside}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.dir\endcsname{below}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.hi\endcsname{+0.13}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.lo\endcsname{\ensuremath{-}1.89}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.mean\endcsname{84.257}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.n\endcsname{9}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.n.word\endcsname{nine}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.nfail\endcsname{0}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.nofn\endcsname{9 of 9}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.nreg\endcsname{9}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.nreg.word\endcsname{nine}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.nse\endcsname{1.7}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.poolmean\endcsname{83.378}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.pooln\endcsname{3}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.pooln.word\endcsname{three}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.poolsd\endcsname{0.795}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.sd\endcsname{0.632}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.se\endcsname{0.50}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.sentence\endcsname{The three runs of the frozen pool read 0.88 pp below the nine later default runs of this study's conditions, about 1.7 standard errors of a three-versus-nine difference of means (empirical standard error 0.50 pp); every difference against the pool is read with that in mind.}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.offset.kits.poolshift.val\endcsname{\ensuremath{-}0.88}
\expandafter\gdef\csname R@an.buildpath.offset.kits.sd.p3c\endcsname{0.55}
\expandafter\gdef\csname R@an.buildpath.offset.kits.sd.stock\endcsname{0.63}
\expandafter\gdef\csname R@an.buildpath.offset.kits.sdratio\endcsname{0.87}
\expandafter\gdef\csname R@an.buildpath.offset.kits.se\endcsname{0.29}
\expandafter\gdef\csname R@an.buildpath.offset.kits.sentence\endcsname{The KiTS23 rebuild offset of the plain family is +0.39 pp over 8 rebuild runs against 9 stock runs of this study's conditions, with an empirical two-sample standard error of 0.29 pp; the interval of plus or minus two standard errors runs \ensuremath{-}0.18 to +0.97 pp, so by the registered rule of Addendum AC it is within the reference's seed noise.}
\expandafter\gdef\csname R@an.buildpath.offset.kits.state\endcsname{complete}
\expandafter\gdef\csname R@an.buildpath.offset.kits.val\endcsname{+0.39}
\expandafter\gdef\csname R@an.buildpath.offset.kits.vsall12\endcsname{+0.61}
\expandafter\gdef\csname R@an.buildpath.offset.kits.vspool\endcsname{+1.27}
\expandafter\gdef\csname R@an.buildpath.offset.kits.vssix\endcsname{+1.03}
\expandafter\gdef\csname R@an.buildpath.offset.kits.word\endcsname{within the reference's seed noise}
\expandafter\gdef\csname R@an.buildpath.p3c.def\endcsname{the plan-aware rebuild of the nnU-Net default network: the same function as the default, built through the library path every agent design and every control of this study is built in}
\expandafter\gdef\csname R@an.buildpath.p3c.name\endcsname{function-identical control}
\expandafter\gdef\csname R@an.buildpath.planet.n\endcsname{four}
\expandafter\gdef\csname R@an.buildpath.planet.names\endcsname{function-identical control, branch control, HyReX and ResEnc-matched}
\expandafter\gdef\csname R@an.buildpath.refnote\endcsname{A within-fold or arm-versus-arm contrast touches no frozen pool; only a contrast against the default pool does, and each of those is printed beside the registered sensitivity reference of its dataset.}
\expandafter\gdef\csname R@an.buildpath.sent.design\endcsname{Measured against its function-identical control rather than the stock default, HyReX's KiTS23 fold-0 margin at two fresh seeds each is +0.92 pp, above the 0.50 pp one-seed pair floor, and the control's own offset reads +1.18 pp of the registered +2.09 pp. The registered cross-validation decomposition (Addendum W3, Addendum X) gives the selection-free version on the four confirmation folds.}
\expandafter\gdef\csname R@an.buildpath.sent.design.state\endcsname{holds}
\expandafter\gdef\csname R@an.buildpath.sent.like\endcsname{Built through the same library path, the residual-encoder control reads +0.22 pp above HyReX on the KiTS23 fold-0 fresh seeds (two fresh seeds each), inside the 0.50 pp one-seed pair floor, and +0.17 pp above it on AMOS22 fold 0 at two fresh seeds each (also inside), at 3.45 times the parameters.}
\expandafter\gdef\csname R@an.buildpath.sent.like.state\endcsname{holds}
\expandafter\gdef\csname R@an.buildpath.sent.protocol\endcsname{A function-identical rebuild of the default network, trained through the same library as the agent designs, reads +1.18 pp against the stock default on KiTS23 fold 0 at two fresh seeds each: the control's own offset, between two networks that compute the same function. It is at least as large as the design margin under study (+0.92 pp). The ResEnc-M contrast reads \ensuremath{-}1.16 pp on the same fold and seeds; those two networks differ in their stem, their shortcut form and their initialisation, so that difference is a re-implementation difference and not a second reading of the rebuild offset. That is one fold of one dataset: the registered cross-validation decomposition (Addendum W3, Addendum X) reads this contrast on the four confirmation folds of each co-primary.}
\expandafter\gdef\csname R@an.buildpath.sent.protocol.state\endcsname{holds}
\expandafter\gdef\csname R@an.buildpath.sent.sized\endcsname{The two default-sized plan-aware designs read 84.554 and 84.445 on KiTS23 fold 0 at two fresh seeds each, so a plan-aware network at the default's size reads +1.07 to +1.18 pp over the stock pool, whichever of the two designs it is, and both values lie above the 0.50 pp one-seed pair floor.}
\expandafter\gdef\csname R@an.buildpath.sent.sized.state\endcsname{holds}
\expandafter\gdef\csname R@an.buildpath.stock.names\endcsname{default and ResEnc-M}
\expandafter\gdef\csname R@an.buildpath.tab.cv.env\endcsname{LAYOUT NOTE (not caption prose): table* spanning \texttt{\textbackslash{}textwidth}, column spec l r r r r r c l}
\expandafter\gdef\csname R@an.buildpath.tab.fold0.env\endcsname{LAYOUT NOTE (not caption prose): table* spanning \texttt{\textbackslash{}textwidth}, column spec @{}lrrlrll@{} at footnotesize with \texttt{\textbackslash{}tabcolsep} 4pt (42 body rows)}
\expandafter\gdef\csname R@an.buildpath.tab.fold0.split.env\endcsname{LAYOUT NOTE (not caption prose): one table* per dataset, the same column spec and size (14 body rows each); the per-dataset bodies are tab_an_buildpath_fold0<dataset>.tex}
\expandafter\gdef\csname R@an.buildpath.tab.fold0.width\endcsname{LAYOUT NOTE (not caption prose): both forms are FULL WIDTH -- in a single column the block overruns the column by about two pp of its own width, so neither is offered as a single-column float}
\expandafter\gdef\csname R@an.case_seedmean.B\endcsname{2000}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1.consistent\endcsname{25}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1.consistent_shift\endcsname{13}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1.fracpos\endcsname{82.5}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1.mean\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1.mean_sens\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1.mean_unc\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1.median\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1.npos\endcsname{33}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1.top5\endcsname{110}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1.top5_cell\endcsname{110}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1.trim\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1.vsnull\endcsname{above both nulls}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1b.consistent\endcsname{15}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1b.consistent_shift\endcsname{8}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1b.fracpos\endcsname{60.0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1b.mean\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1b.mean_sens\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1b.mean_unc\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1b.median\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1b.npos\endcsname{24}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1b.top5\endcsname{106}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1b.top5_cell\endcsname{106}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1b.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1b.trim\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L1b.vsnull\endcsname{inside both nulls}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L3.consistent\endcsname{30}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L3.consistent_shift\endcsname{12}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L3.fracpos\endcsname{80.0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L3.mean\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L3.mean_sens\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L3.mean_unc\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L3.median\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L3.npos\endcsname{32}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L3.top5\endcsname{65}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L3.top5_cell\endcsname{65}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L3.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L3.trim\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.L3.vsnull\endcsname{above both nulls}
\expandafter\gdef\csname R@an.case_seedmean.acdc.cons.max\endcsname{30}
\expandafter\gdef\csname R@an.case_seedmean.acdc.cons.maxarm\endcsname{HyReX}
\expandafter\gdef\csname R@an.case_seedmean.acdc.cons.min\endcsname{15}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.L1_L1b\endcsname{0.84}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.L1_L1b.ceil\endcsname{0.91}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.L3_L1\endcsname{0.83}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.L3_L1.ceil\endcsname{0.96}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.L3_L1b\endcsname{0.88}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.L3_L1b.ceil\endcsname{0.93}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.ceiling\endcsname{0.88}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.ceiling_adj\endcsname{0.94}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.ceiling_hi\endcsname{0.96}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.ceiling_lo\endcsname{0.91}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.cross\endcsname{0.80}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.dismax\endcsname{0.94}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.dismax_hi\endcsname{1.05}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.dismax_lo\endcsname{0.78}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.dismaxpair\endcsname{HyReX--ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.dismean\endcsname{0.91}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.max\endcsname{0.88}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.maxceil\endcsname{0.93}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.maxpair\endcsname{HyReX--ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.nabove\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.nabove_boot\endcsname{0.1}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.nabove_hi\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.nabove_lo\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.nabove_pnone\endcsname{92}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.npairs\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.sb.L1\endcsname{0.94}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.sb.L1b\endcsname{0.89}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.sb.L3\endcsname{0.98}
\expandafter\gdef\csname R@an.case_seedmean.acdc.corr.shared\endcsname{91}
\expandafter\gdef\csname R@an.case_seedmean.acdc.loo.consistent\endcsname{13.3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.loo.max\endcsname{21}
\expandafter\gdef\csname R@an.case_seedmean.acdc.loo.mean\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.acdc.loo.min\endcsname{7}
\expandafter\gdef\csname R@an.case_seedmean.acdc.loo.ncombo\endcsname{60}
\expandafter\gdef\csname R@an.case_seedmean.acdc.loo.p\endcsname{1/3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1.consistent\endcsname{19}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1.consistent_shift\endcsname{27}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1.fracpos\endcsname{65.0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1.mean\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1.mean_sens\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1.mean_unc\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1.median\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1.npos\endcsname{26}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1.top5\endcsname{355}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1.top5_cell\endcsname{355$^{\dagger}$}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1.top5_interp\endcsname{no}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1.trim\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1.vsnull\endcsname{above both nulls}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1b.consistent\endcsname{12}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1b.consistent_shift\endcsname{19}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1b.fracpos\endcsname{47.5}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1b.mean\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1b.mean_sens\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1b.mean_unc\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1b.median\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1b.npos\endcsname{19}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1b.top5\endcsname{155}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1b.top5_cell\endcsname{155$^{\dagger}$}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1b.top5_interp\endcsname{no}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1b.trim\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L1b.vsnull\endcsname{inside both nulls}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L3.consistent\endcsname{22}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L3.consistent_shift\endcsname{26}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L3.fracpos\endcsname{65.0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L3.mean\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L3.mean_sens\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L3.mean_unc\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L3.median\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L3.npos\endcsname{26}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L3.top5\endcsname{400}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L3.top5_cell\endcsname{400$^{\dagger}$}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L3.top5_interp\endcsname{no}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L3.trim\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.L3.vsnull\endcsname{above both nulls}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.cons.max\endcsname{22}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.cons.maxarm\endcsname{HyReX}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.cons.min\endcsname{12}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.L1_L1b\endcsname{0.94}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.L1_L1b.ceil\endcsname{0.94}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.L3_L1\endcsname{0.93}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.L3_L1.ceil\endcsname{0.98}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.L3_L1b\endcsname{0.95}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.L3_L1b.ceil\endcsname{0.94}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.ceiling\endcsname{0.91}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.ceiling_adj\endcsname{0.95}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.ceiling_hi\endcsname{0.98}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.ceiling_lo\endcsname{0.94}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.cross\endcsname{0.89}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.dismax\endcsname{1.00}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.dismax_hi\endcsname{1.76}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.dismax_lo\endcsname{0.13}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.dismaxpair\endcsname{ResEnc-M (library preset)--ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.dismean\endcsname{0.99}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.max\endcsname{0.95}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.maxceil\endcsname{0.94}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.maxpair\endcsname{HyReX--ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.nabove\endcsname{2}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.nabove_boot\endcsname{1.0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.nabove_hi\endcsname{2}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.nabove_lo\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.nabove_pnone\endcsname{38}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.npairs\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.sb.L1\endcsname{0.97}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.sb.L1b\endcsname{0.91}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.sb.L3\endcsname{0.99}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.corr.shared\endcsname{97}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.loo.consistent\endcsname{13.3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.loo.max\endcsname{19}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.loo.mean\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.loo.min\endcsname{8}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.oracle.best\endcsname{HyReX}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.oracle.best_mean\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.oracle.gain\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.oracle.gain_cv\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.oracle.mean\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.shift.max\endcsname{27}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.shift.maxarm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.shift.min\endcsname{19}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.shift.minarm\endcsname{ResEnc-matched}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.shift.nabove\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.lvc.shift.ndrop\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1.consistent\endcsname{21}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1.consistent_shift\endcsname{15}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1.fracpos\endcsname{72.5}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1.mean\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1.mean_sens\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1.mean_unc\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1.median\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1.npos\endcsname{29}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1.top5\endcsname{66}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1.top5_cell\endcsname{66}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1.trim\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1.vsnull\endcsname{above both nulls}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1b.consistent\endcsname{9}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1b.consistent_shift\endcsname{10}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1b.fracpos\endcsname{45.0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1b.mean\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1b.mean_sens\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1b.mean_unc\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1b.median\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1b.npos\endcsname{18}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1b.top5\endcsname{\ensuremath{>}999}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1b.top5_cell\endcsname{\ensuremath{>}999$^{\dagger}$}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1b.top5_interp\endcsname{no}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1b.trim\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L1b.vsnull\endcsname{inside both nulls}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L3.consistent\endcsname{26}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L3.consistent_shift\endcsname{12}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L3.fracpos\endcsname{77.5}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L3.mean\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L3.mean_sens\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L3.mean_unc\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L3.median\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L3.npos\endcsname{31}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L3.top5\endcsname{55}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L3.top5_cell\endcsname{55}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L3.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L3.trim\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.L3.vsnull\endcsname{above both nulls}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.cons.max\endcsname{26}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.cons.maxarm\endcsname{HyReX}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.cons.min\endcsname{9}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.L1_L1b\endcsname{0.62}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.L1_L1b.ceil\endcsname{0.67}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.L3_L1\endcsname{0.47}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.L3_L1.ceil\endcsname{0.74}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.L3_L1b\endcsname{0.61}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.L3_L1b.ceil\endcsname{0.76}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.ceiling\endcsname{0.58}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.ceiling_adj\endcsname{0.73}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.ceiling_hi\endcsname{0.76}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.ceiling_lo\endcsname{0.67}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.cross\endcsname{0.44}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.dismax\endcsname{0.92}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.dismax_hi\endcsname{1.89}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.dismax_lo\endcsname{0.64}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.dismaxpair\endcsname{ResEnc-M (library preset)--ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.dismean\endcsname{0.79}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.max\endcsname{0.62}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.maxceil\endcsname{0.67}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.maxpair\endcsname{ResEnc-M (library preset)--ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.nabove\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.nabove_boot\endcsname{0.6}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.nabove_hi\endcsname{2}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.nabove_lo\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.nabove_pnone\endcsname{55}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.npairs\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.sb.L1\endcsname{0.65}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.sb.L1b\endcsname{0.70}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.sb.L3\endcsname{0.83}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.corr.shared\endcsname{76}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.loo.consistent\endcsname{13.3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.loo.max\endcsname{20}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.loo.mean\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.loo.min\endcsname{7}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.oracle.best\endcsname{HyReX}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.oracle.best_mean\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.oracle.gain\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.oracle.gain_cv\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.oracle.mean\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.shift.max\endcsname{15}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.shift.maxarm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.shift.min\endcsname{10}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.shift.minarm\endcsname{ResEnc-matched}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.shift.nabove\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.mlv.shift.ndrop\endcsname{2}
\expandafter\gdef\csname R@an.case_seedmean.acdc.n\endcsname{40}
\expandafter\gdef\csname R@an.case_seedmean.acdc.narms\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.nempty\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.npending\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.null.consistent_exp\endcsname{10.9}
\expandafter\gdef\csname R@an.case_seedmean.acdc.null.hi\endcsname{17}
\expandafter\gdef\csname R@an.case_seedmean.acdc.null.lo\endcsname{6}
\expandafter\gdef\csname R@an.case_seedmean.acdc.null.npool\endcsname{6}
\expandafter\gdef\csname R@an.case_seedmean.acdc.null.p\endcsname{0.2728}
\expandafter\gdef\csname R@an.case_seedmean.acdc.null.rho\endcsname{0.143}
\expandafter\gdef\csname R@an.case_seedmean.acdc.oracle.best\endcsname{HyReX}
\expandafter\gdef\csname R@an.case_seedmean.acdc.oracle.best_mean\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.oracle.gain\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.oracle.gain_cv\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.oracle.mean\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.ref.contemp.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.case_seedmean.acdc.ref.contemp.n\endcsname{\pend}
\expandafter\gdef\csname R@an.case_seedmean.acdc.ref.contemp.sd\endcsname{\pend}
\expandafter\gdef\csname R@an.case_seedmean.acdc.ref.contemp.shift\endcsname{\pend}
\expandafter\gdef\csname R@an.case_seedmean.acdc.ref.contemp.short\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.case_seedmean.acdc.ref.frozen.mean\endcsname{92.009}
\expandafter\gdef\csname R@an.case_seedmean.acdc.ref.frozen.n\endcsname{6}
\expandafter\gdef\csname R@an.case_seedmean.acdc.ref.frozen.sd\endcsname{0.099}
\expandafter\gdef\csname R@an.case_seedmean.acdc.ref.frozen.shift\endcsname{0.000}
\expandafter\gdef\csname R@an.case_seedmean.acdc.ref.frozen.short\endcsname{frozen pool}
\expandafter\gdef\csname R@an.case_seedmean.acdc.ref.nfin\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.acdc.ref.npend\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.acdc.ref.pendnames\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.case_seedmean.acdc.ref.unc.mean\endcsname{92.016}
\expandafter\gdef\csname R@an.case_seedmean.acdc.ref.unc.n\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.ref.unc.sd\endcsname{0.071}
\expandafter\gdef\csname R@an.case_seedmean.acdc.ref.unc.shift\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.ref.unc.short\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1.bar\endcsname{not applicable}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1.casegap\endcsname{0.000}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1.casemean\endcsname{\ensuremath{+0.242}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1.delta\endcsname{\ensuremath{+0.242}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1.mean\endcsname{92.251}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1.runs\endcsname{above}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1.s1\endcsname{92.268}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1.s2\endcsname{92.234}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1.se_pool\endcsname{0.081}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1.se_seed\endcsname{0.017}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1.spread\endcsname{0.034}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1.state\endcsname{separated above}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1b.bar\endcsname{not applicable}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1b.casegap\endcsname{0.000}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1b.casemean\endcsname{\ensuremath{+0.319}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1b.delta\endcsname{\ensuremath{+0.319}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1b.mean\endcsname{92.328}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1b.runs\endcsname{above}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1b.s1\endcsname{92.296}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1b.s2\endcsname{92.361}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1b.se_pool\endcsname{0.081}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1b.se_seed\endcsname{0.033}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1b.spread\endcsname{0.065}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L1b.state\endcsname{separated above}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L3.bar\endcsname{not applicable}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L3.casegap\endcsname{0.000}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L3.casemean\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L3.delta\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L3.mean\endcsname{92.460}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L3.runs\endcsname{above}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L3.s1\endcsname{92.426}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L3.s2\endcsname{92.493}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L3.se_pool\endcsname{0.081}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L3.se_seed\endcsname{0.033}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L3.spread\endcsname{0.067}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.L3.state\endcsname{separated above}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.arms\endcsname{HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.narms\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.nnosep\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.nosepnames\endcsname{none}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.nsep\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.sepdef\endcsname{both fresh runs above every one of the 6 frozen-pool runs, or both below every one}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.sepnames\endcsname{HyReX, ResEnc-matched, ResEnc-M}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.sepsentence\endcsname{At two fresh seeds ACDC separates HyReX (\ensuremath{+0.450}\,pp), ResEnc-M (\ensuremath{+0.242}\,pp) and ResEnc-matched (\ensuremath{+0.319}\,pp).}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rep.state\endcsname{separated above}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1.consistent\endcsname{22}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1.consistent_shift\endcsname{7}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1.fracpos\endcsname{70.0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1.mean\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1.mean_sens\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1.mean_unc\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1.median\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1.npos\endcsname{28}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1.top5\endcsname{114}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1.top5_cell\endcsname{114}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1.trim\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1.vsnull\endcsname{above both nulls}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1b.consistent\endcsname{25}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1b.consistent_shift\endcsname{8}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1b.fracpos\endcsname{67.5}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1b.mean\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1b.mean_sens\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1b.mean_unc\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1b.median\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1b.npos\endcsname{27}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1b.top5\endcsname{83}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1b.top5_cell\endcsname{83}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1b.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1b.trim\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L1b.vsnull\endcsname{above both nulls}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L3.consistent\endcsname{22}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L3.consistent_shift\endcsname{8}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L3.fracpos\endcsname{75.0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L3.mean\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L3.mean_sens\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L3.mean_unc\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L3.median\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L3.npos\endcsname{30}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L3.top5\endcsname{73}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L3.top5_cell\endcsname{73}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L3.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L3.trim\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.L3.vsnull\endcsname{above both nulls}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.cons.max\endcsname{25}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.cons.maxarm\endcsname{ResEnc-matched}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.cons.min\endcsname{22}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.L1_L1b\endcsname{0.89}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.L1_L1b.ceil\endcsname{0.94}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.L3_L1\endcsname{0.85}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.L3_L1.ceil\endcsname{0.95}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.L3_L1b\endcsname{0.93}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.L3_L1b.ceil\endcsname{0.97}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.ceiling\endcsname{0.91}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.ceiling_adj\endcsname{0.95}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.ceiling_hi\endcsname{0.97}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.ceiling_lo\endcsname{0.94}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.cross\endcsname{0.85}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.dismax\endcsname{0.96}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.dismax_hi\endcsname{1.02}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.dismax_lo\endcsname{0.83}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.dismaxpair\endcsname{HyReX--ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.dismean\endcsname{0.93}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.max\endcsname{0.93}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.maxceil\endcsname{0.97}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.maxpair\endcsname{HyReX--ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.nabove\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.nabove_boot\endcsname{0.1}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.nabove_hi\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.nabove_lo\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.nabove_pnone\endcsname{95}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.npairs\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.sb.L1\endcsname{0.93}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.sb.L1b\endcsname{0.96}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.sb.L3\endcsname{0.98}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.corr.shared\endcsname{93}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.loo.consistent\endcsname{13.3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.loo.max\endcsname{22}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.loo.mean\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.loo.min\endcsname{7}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.oracle.best\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.oracle.best_mean\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.oracle.gain\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.oracle.gain_cv\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.oracle.mean\endcsname{\ensuremath{+1.58}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.shift.max\endcsname{8}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.shift.maxarm\endcsname{HyReX}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.shift.min\endcsname{7}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.shift.minarm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.shift.nabove\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.rv.shift.ndrop\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.sens.key\endcsname{unc}
\expandafter\gdef\csname R@an.case_seedmean.acdc.sens.n\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.sens.shift\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.case_seedmean.acdc.sens.short\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.case_seedmean.acdc.sens.state\endcsname{ready}
\expandafter\gdef\csname R@an.case_seedmean.acdc.shift.max\endcsname{13}
\expandafter\gdef\csname R@an.case_seedmean.acdc.shift.maxarm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.case_seedmean.acdc.shift.min\endcsname{8}
\expandafter\gdef\csname R@an.case_seedmean.acdc.shift.minarm\endcsname{ResEnc-matched}
\expandafter\gdef\csname R@an.case_seedmean.acdc.shift.nabove\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.shift.ndrop\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.sim.hi\endcsname{21}
\expandafter\gdef\csname R@an.case_seedmean.acdc.sim.lo\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.sim.mean\endcsname{10.9}
\expandafter\gdef\csname R@an.case_seedmean.acdc.sim.scasehi\endcsname{1.44}
\expandafter\gdef\csname R@an.case_seedmean.acdc.sim.scaselo\endcsname{0.08}
\expandafter\gdef\csname R@an.case_seedmean.acdc.sim.scasemed\endcsname{0.24}
\expandafter\gdef\csname R@an.case_seedmean.acdc.sim.sdrun\endcsname{0.072}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ak.sd\endcsname{0.71}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ak.share\endcsname{4.07}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.arm.sd\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.arm.share\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.arms\endcsname{nnU-Net default, HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.case.sd\endcsname{3.41}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.case.share\endcsname{92.71}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.excl\endcsname{none}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.narm\endcsname{4}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.nboot\endcsname{2000}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ncase\endcsname{40}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.negnames\endcsname{seed(arm), arm}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.nexcl\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.nfresh_subsets\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.nneg\endcsname{2}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.nseed\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio\endcsname{1.27}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_arm\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_arm_ci\endcsname{not defined}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_arm_fresh\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_arm_fresh_ndef\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_arm_hi\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_arm_lo\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_arm_ndef\endcsname{1652}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_arm_sd\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_arm_sd_hi\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_arm_sd_lo\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_arm_support\endcsname{82.6}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_arm_txt\endcsname{not defined (the seed(arm) component is not resolved from zero)}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_ci\endcsname{printed}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_fresh\endcsname{2.72}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_fresh_ndef\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_hi\endcsname{1.67}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_lo\endcsname{0.15}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_ndef\endcsname{2000}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_sd\endcsname{1.13}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_sd_hi\endcsname{1.29}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_sd_lo\endcsname{0.38}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_support\endcsname{100.0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.ratio_txt\endcsname{1.27 [0.15, 1.67]}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.resid.sd\endcsname{0.64}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.resid.share\endcsname{3.22}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.seed.sd\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.lvc.seed.share\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ak.sd\endcsname{0.59}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ak.share\endcsname{4.81}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.arm.sd\endcsname{0.18}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.arm.share\endcsname{0.44}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.arms\endcsname{nnU-Net default, HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.case.sd\endcsname{2.57}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.case.share\endcsname{91.79}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.excl\endcsname{none}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.narm\endcsname{4}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.nboot\endcsname{2000}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ncase\endcsname{40}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.negnames\endcsname{seed(arm)}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.nexcl\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.nfresh_subsets\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.nneg\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.nseed\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio\endcsname{1.63}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_arm\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_arm_ci\endcsname{not defined}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_arm_fresh\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_arm_fresh_ndef\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_arm_hi\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_arm_lo\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_arm_ndef\endcsname{1712}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_arm_sd\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_arm_sd_hi\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_arm_sd_lo\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_arm_support\endcsname{85.6}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_arm_txt\endcsname{not defined (the seed(arm) component is not resolved from zero)}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_ci\endcsname{printed}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_fresh\endcsname{1.83}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_fresh_ndef\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_hi\endcsname{3.13}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_lo\endcsname{0.73}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_ndef\endcsname{2000}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_sd\endcsname{1.28}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_sd_hi\endcsname{1.77}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_sd_lo\endcsname{0.85}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_support\endcsname{100.0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.ratio_txt\endcsname{1.63 [0.73, 3.13]}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.resid.sd\endcsname{0.46}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.resid.share\endcsname{2.96}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.seed.sd\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mean.seed.share\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ak.sd\endcsname{0.26}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ak.share\endcsname{0.64}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.arm.sd\endcsname{0.16}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.arm.share\endcsname{0.24}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.arms\endcsname{nnU-Net default, HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.case.sd\endcsname{3.18}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.case.share\endcsname{97.59}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.excl\endcsname{none}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.narm\endcsname{4}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.nboot\endcsname{2000}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ncase\endcsname{40}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.negnames\endcsname{none}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.nexcl\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.nfresh_subsets\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.nneg\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.nseed\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio\endcsname{0.43}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_arm\endcsname{14.66}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_arm_ci\endcsname{printed}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_arm_fresh\endcsname{4.03}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_arm_fresh_ndef\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_arm_hi\endcsname{45.36}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_arm_lo\endcsname{1.54}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_arm_ndef\endcsname{1952}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_arm_sd\endcsname{3.83}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_arm_sd_hi\endcsname{6.73}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_arm_sd_lo\endcsname{1.24}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_arm_support\endcsname{97.6}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_arm_txt\endcsname{14.66 [1.54, 45.36]}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_ci\endcsname{printed}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_fresh\endcsname{0.50}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_fresh_ndef\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_hi\endcsname{0.87}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_lo\endcsname{0.13}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_ndef\endcsname{2000}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_sd\endcsname{0.65}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_sd_hi\endcsname{0.93}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_sd_lo\endcsname{0.36}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_support\endcsname{100.0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.ratio_txt\endcsname{0.43 [0.13, 0.87]}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.resid.sd\endcsname{0.40}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.resid.share\endcsname{1.51}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.seed.sd\endcsname{0.04}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.mlv.seed.share\endcsname{0.02}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ak.sd\endcsname{1.42}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ak.share\endcsname{8.86}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.arm.sd\endcsname{0.47}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.arm.share\endcsname{0.96}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.arms\endcsname{nnU-Net default, HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.case.sd\endcsname{4.42}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.case.share\endcsname{85.96}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.excl\endcsname{none}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.narm\endcsname{4}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.nboot\endcsname{2000}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ncase\endcsname{40}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.negnames\endcsname{seed(arm)}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.nexcl\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.nfresh_subsets\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.nneg\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.nseed\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio\endcsname{2.10}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_arm\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_arm_ci\endcsname{not defined}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_arm_fresh\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_arm_fresh_ndef\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_arm_hi\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_arm_lo\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_arm_ndef\endcsname{1662}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_arm_sd\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_arm_sd_hi\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_arm_sd_lo\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_arm_support\endcsname{83.1}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_arm_txt\endcsname{not defined (the seed(arm) component is not resolved from zero)}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_ci\endcsname{printed}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_fresh\endcsname{2.02}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_fresh_ndef\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_hi\endcsname{4.91}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_lo\endcsname{0.55}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_ndef\endcsname{2000}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_sd\endcsname{1.45}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_sd_hi\endcsname{2.22}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_sd_lo\endcsname{0.74}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_support\endcsname{100.0}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.ratio_txt\endcsname{2.10 [0.55, 4.91]}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.resid.sd\endcsname{0.98}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.resid.share\endcsname{4.23}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.seed.sd\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.acdc.var.rv.seed.share\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1.consistent\endcsname{23}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1.consistent_shift\endcsname{10}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1.fracpos\endcsname{85.0}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1.mean\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1.mean_sens\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1.mean_unc\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1.median\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1.npos\endcsname{34}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1.top5\endcsname{40}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1.top5_cell\endcsname{40}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1.trim\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1.vsnull\endcsname{above both nulls}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1b.consistent\endcsname{24}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1b.consistent_shift\endcsname{15}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1b.fracpos\endcsname{80.0}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1b.mean\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1b.mean_sens\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1b.mean_unc\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1b.median\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1b.npos\endcsname{32}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1b.top5\endcsname{59}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1b.top5_cell\endcsname{59}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1b.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1b.trim\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L1b.vsnull\endcsname{above both nulls}
\expandafter\gdef\csname R@an.case_seedmean.amos.L2.consistent\endcsname{17}
\expandafter\gdef\csname R@an.case_seedmean.amos.L2.consistent_shift\endcsname{12}
\expandafter\gdef\csname R@an.case_seedmean.amos.L2.fracpos\endcsname{65.0}
\expandafter\gdef\csname R@an.case_seedmean.amos.L2.mean\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L2.mean_sens\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L2.mean_unc\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L2.median\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L2.npos\endcsname{26}
\expandafter\gdef\csname R@an.case_seedmean.amos.L2.top5\endcsname{89}
\expandafter\gdef\csname R@an.case_seedmean.amos.L2.top5_cell\endcsname{89}
\expandafter\gdef\csname R@an.case_seedmean.amos.L2.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.amos.L2.trim\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L2.vsnull\endcsname{inside the analytic null and above the simulated one}
\expandafter\gdef\csname R@an.case_seedmean.amos.L3.consistent\endcsname{22}
\expandafter\gdef\csname R@an.case_seedmean.amos.L3.consistent_shift\endcsname{17}
\expandafter\gdef\csname R@an.case_seedmean.amos.L3.fracpos\endcsname{72.5}
\expandafter\gdef\csname R@an.case_seedmean.amos.L3.mean\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L3.mean_sens\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L3.mean_unc\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L3.median\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L3.npos\endcsname{29}
\expandafter\gdef\csname R@an.case_seedmean.amos.L3.top5\endcsname{69}
\expandafter\gdef\csname R@an.case_seedmean.amos.L3.top5_cell\endcsname{69}
\expandafter\gdef\csname R@an.case_seedmean.amos.L3.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.amos.L3.trim\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L3.vsnull\endcsname{above both nulls}
\expandafter\gdef\csname R@an.case_seedmean.amos.L4.consistent\endcsname{22}
\expandafter\gdef\csname R@an.case_seedmean.amos.L4.consistent_shift\endcsname{12}
\expandafter\gdef\csname R@an.case_seedmean.amos.L4.fracpos\endcsname{65.0}
\expandafter\gdef\csname R@an.case_seedmean.amos.L4.mean\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L4.mean_sens\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L4.mean_unc\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L4.median\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L4.npos\endcsname{26}
\expandafter\gdef\csname R@an.case_seedmean.amos.L4.top5\endcsname{50}
\expandafter\gdef\csname R@an.case_seedmean.amos.L4.top5_cell\endcsname{50}
\expandafter\gdef\csname R@an.case_seedmean.amos.L4.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.amos.L4.trim\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.case_seedmean.amos.L4.vsnull\endcsname{above both nulls}
\expandafter\gdef\csname R@an.case_seedmean.amos.cons.max\endcsname{24}
\expandafter\gdef\csname R@an.case_seedmean.amos.cons.maxarm\endcsname{ResEnc-matched}
\expandafter\gdef\csname R@an.case_seedmean.amos.cons.min\endcsname{17}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L1_L1b\endcsname{0.77}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L1_L1b.ceil\endcsname{0.34}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L1_L2\endcsname{0.44}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L1_L2.ceil\endcsname{0.32}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L1_L4\endcsname{0.48}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L1_L4.ceil\endcsname{0.32}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L1b_L2\endcsname{0.52}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L1b_L2.ceil\endcsname{0.74}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L1b_L4\endcsname{0.39}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L1b_L4.ceil\endcsname{0.76}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L3_L1\endcsname{0.44}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L3_L1.ceil\endcsname{0.26}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L3_L1b\endcsname{0.57}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L3_L1b.ceil\endcsname{0.62}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L3_L2\endcsname{0.50}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L3_L2.ceil\endcsname{0.58}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L3_L4\endcsname{0.41}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L3_L4.ceil\endcsname{0.59}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L4_L2\endcsname{0.18}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.L4_L2.ceil\endcsname{0.71}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.ceiling\endcsname{0.43}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.ceiling_adj\endcsname{0.60}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.ceiling_hi\endcsname{0.76}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.ceiling_lo\endcsname{0.26}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.cross\endcsname{0.32}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.dismax\endcsname{2.27}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.dismax_hi\endcsname{7.25}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.dismax_lo\endcsname{0.42}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.dismaxpair\endcsname{ResEnc-M (library preset)--ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.dismean\endcsname{1.07}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.max\endcsname{0.77}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.maxceil\endcsname{0.34}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.maxpair\endcsname{ResEnc-M (library preset)--ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.nabove\endcsname{4}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.nabove_boot\endcsname{2.7}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.nabove_hi\endcsname{7}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.nabove_lo\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.nabove_pnone\endcsname{17}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.npairs\endcsname{10}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.sb.L1\endcsname{0.14}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.sb.L1b\endcsname{0.79}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.sb.L2\endcsname{0.69}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.sb.L3\endcsname{0.48}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.sb.L4\endcsname{0.73}
\expandafter\gdef\csname R@an.case_seedmean.amos.corr.shared\endcsname{75}
\expandafter\gdef\csname R@an.case_seedmean.amos.loo.consistent\endcsname{13.3}
\expandafter\gdef\csname R@an.case_seedmean.amos.loo.max\endcsname{17}
\expandafter\gdef\csname R@an.case_seedmean.amos.loo.mean\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.amos.loo.min\endcsname{9}
\expandafter\gdef\csname R@an.case_seedmean.amos.loo.ncombo\endcsname{60}
\expandafter\gdef\csname R@an.case_seedmean.amos.loo.p\endcsname{1/3}
\expandafter\gdef\csname R@an.case_seedmean.amos.n\endcsname{40}
\expandafter\gdef\csname R@an.case_seedmean.amos.narms\endcsname{5}
\expandafter\gdef\csname R@an.case_seedmean.amos.nempty\endcsname{6}
\expandafter\gdef\csname R@an.case_seedmean.amos.npending\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.amos.null.consistent_exp\endcsname{10.9}
\expandafter\gdef\csname R@an.case_seedmean.amos.null.hi\endcsname{17}
\expandafter\gdef\csname R@an.case_seedmean.amos.null.lo\endcsname{6}
\expandafter\gdef\csname R@an.case_seedmean.amos.null.npool\endcsname{6}
\expandafter\gdef\csname R@an.case_seedmean.amos.null.p\endcsname{0.2728}
\expandafter\gdef\csname R@an.case_seedmean.amos.null.rho\endcsname{0.143}
\expandafter\gdef\csname R@an.case_seedmean.amos.oracle.best\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.case_seedmean.amos.oracle.best_mean\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.case_seedmean.amos.oracle.gain\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.case_seedmean.amos.oracle.gain_cv\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.case_seedmean.amos.oracle.mean\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.case_seedmean.amos.ref.contemp.mean\endcsname{87.712}
\expandafter\gdef\csname R@an.case_seedmean.amos.ref.contemp.n\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.amos.ref.contemp.sd\endcsname{0.125}
\expandafter\gdef\csname R@an.case_seedmean.amos.ref.contemp.shift\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.case_seedmean.amos.ref.contemp.short\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.case_seedmean.amos.ref.frozen.mean\endcsname{87.701}
\expandafter\gdef\csname R@an.case_seedmean.amos.ref.frozen.n\endcsname{6}
\expandafter\gdef\csname R@an.case_seedmean.amos.ref.frozen.sd\endcsname{0.122}
\expandafter\gdef\csname R@an.case_seedmean.amos.ref.frozen.shift\endcsname{0.000}
\expandafter\gdef\csname R@an.case_seedmean.amos.ref.frozen.short\endcsname{frozen pool}
\expandafter\gdef\csname R@an.case_seedmean.amos.ref.nfin\endcsname{2}
\expandafter\gdef\csname R@an.case_seedmean.amos.ref.npend\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.amos.ref.pendnames\endcsname{none}
\expandafter\gdef\csname R@an.case_seedmean.amos.ref.unc.mean\endcsname{87.730}
\expandafter\gdef\csname R@an.case_seedmean.amos.ref.unc.n\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.amos.ref.unc.sd\endcsname{0.143}
\expandafter\gdef\csname R@an.case_seedmean.amos.ref.unc.shift\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.case_seedmean.amos.ref.unc.short\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1.bar\endcsname{clears}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1.casegap\endcsname{\ensuremath{+0.001}}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1.casemean\endcsname{\ensuremath{+0.466}}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1.delta\endcsname{\ensuremath{+0.465}}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1.mean\endcsname{88.166}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1.runs\endcsname{above}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1.s1\endcsname{88.363}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1.s2\endcsname{87.969}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1.se_pool\endcsname{0.100}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1.se_seed\endcsname{0.197}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1.spread\endcsname{0.394}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1.state\endcsname{separated above}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1b.bar\endcsname{below}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1b.casegap\endcsname{\ensuremath{+0.147}}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1b.casemean\endcsname{\ensuremath{+0.444}}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1b.delta\endcsname{\ensuremath{+0.298}}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1b.mean\endcsname{87.999}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1b.runs\endcsname{overlaps}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1b.s1\endcsname{88.127}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1b.s2\endcsname{87.870}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1b.se_pool\endcsname{0.100}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1b.se_seed\endcsname{0.129}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1b.spread\endcsname{0.257}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L1b.state\endcsname{not separated}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L2.bar\endcsname{below}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L2.casegap\endcsname{\ensuremath{+0.071}}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L2.casemean\endcsname{\ensuremath{+0.266}}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L2.delta\endcsname{\ensuremath{+0.194}}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L2.mean\endcsname{87.895}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L2.runs\endcsname{overlaps}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L2.s1\endcsname{87.956}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L2.s2\endcsname{87.835}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L2.se_pool\endcsname{0.100}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L2.se_seed\endcsname{0.061}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L2.spread\endcsname{0.121}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L2.state\endcsname{not separated}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L3.bar\endcsname{below}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L3.casegap\endcsname{\ensuremath{+0.071}}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L3.casemean\endcsname{\ensuremath{+0.203}}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L3.delta\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L3.mean\endcsname{87.833}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L3.runs\endcsname{overlaps}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L3.s1\endcsname{87.981}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L3.s2\endcsname{87.686}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L3.se_pool\endcsname{0.100}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L3.se_seed\endcsname{0.148}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L3.spread\endcsname{0.296}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L3.state\endcsname{not separated}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L4.bar\endcsname{clears}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L4.casegap\endcsname{\ensuremath{-0.078}}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L4.casemean\endcsname{\ensuremath{+0.376}}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L4.delta\endcsname{\ensuremath{+0.455}}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L4.mean\endcsname{88.156}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L4.runs\endcsname{above}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L4.s1\endcsname{88.053}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L4.s2\endcsname{88.258}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L4.se_pool\endcsname{0.100}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L4.se_seed\endcsname{0.102}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L4.spread\endcsname{0.205}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.L4.state\endcsname{separated above}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.arms\endcsname{HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.bar.value\endcsname{0.35}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.gaphero\endcsname{\ensuremath{+0.332}}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.herorank\endcsname{5}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.herosentence\endcsname{On AMOS22 HyReX's fresh-mean delta, \ensuremath{+0.132}\,pp, ranks 5th of the 5 complete pairs, 0.332\,pp behind ResEnc-M's.}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.lead\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.lead_vs\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.leadcons\endcsname{23}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.leadgap\endcsname{\ensuremath{+0.010}}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.leadishero\endcsname{no}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.leadsentence\endcsname{On AMOS22 the largest fresh-mean delta of the 5 complete pairs is ResEnc-M's, \ensuremath{+0.465}\,pp, which is 0.010\,pp ahead of ResEnc+context's.}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.narms\endcsname{5}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.nlead\endcsname{5}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.nnosep\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.nosepnames\endcsname{ResEnc-matched, ConvNeXt-k3, HyReX}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.nsep\endcsname{2}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.order\endcsname{ResEnc-M (library preset) \ensuremath{+0.465}, ResEnc+context \ensuremath{+0.455}, ResEnc-matched (re-implemented) \ensuremath{+0.298}, ConvNeXt-k3 \ensuremath{+0.194}, HyReX \ensuremath{+0.132}}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.sepdef\endcsname{both fresh runs above every one of the 6 frozen-pool runs, or both below every one}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.sepnames\endcsname{ResEnc-M, ResEnc+context}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.sepsentence\endcsname{At two fresh seeds AMOS22 separates ResEnc-M (\ensuremath{+0.465}\,pp) and ResEnc+context (\ensuremath{+0.455}\,pp); does not separate ResEnc-matched (\ensuremath{+0.298}\,pp), ConvNeXt-k3 (\ensuremath{+0.194}\,pp) and HyReX (\ensuremath{+0.132}\,pp).}
\expandafter\gdef\csname R@an.case_seedmean.amos.rep.state\endcsname{not separated}
\expandafter\gdef\csname R@an.case_seedmean.amos.sens.key\endcsname{unc}
\expandafter\gdef\csname R@an.case_seedmean.amos.sens.n\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.amos.sens.shift\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.case_seedmean.amos.sens.short\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.case_seedmean.amos.sens.state\endcsname{ready}
\expandafter\gdef\csname R@an.case_seedmean.amos.shift.max\endcsname{17}
\expandafter\gdef\csname R@an.case_seedmean.amos.shift.maxarm\endcsname{HyReX}
\expandafter\gdef\csname R@an.case_seedmean.amos.shift.min\endcsname{10}
\expandafter\gdef\csname R@an.case_seedmean.amos.shift.minarm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.case_seedmean.amos.shift.nabove\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.amos.shift.ndrop\endcsname{5}
\expandafter\gdef\csname R@an.case_seedmean.amos.sim.hi\endcsname{16}
\expandafter\gdef\csname R@an.case_seedmean.amos.sim.lo\endcsname{6}
\expandafter\gdef\csname R@an.case_seedmean.amos.sim.mean\endcsname{10.8}
\expandafter\gdef\csname R@an.case_seedmean.amos.sim.scasehi\endcsname{1.69}
\expandafter\gdef\csname R@an.case_seedmean.amos.sim.scaselo\endcsname{0.07}
\expandafter\gdef\csname R@an.case_seedmean.amos.sim.scasemed\endcsname{0.43}
\expandafter\gdef\csname R@an.case_seedmean.amos.sim.sdrun\endcsname{0.000}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ak.sd\endcsname{0.29}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ak.share\endcsname{0.20}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.arm.sd\endcsname{0.11}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.arm.share\endcsname{0.03}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.arms\endcsname{nnU-Net default, HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented), ResEnc+context, ConvNeXt-k3}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.case.sd\endcsname{6.44}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.case.share\endcsname{98.69}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.excl\endcsname{none}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.narm\endcsname{6}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.nboot\endcsname{2000}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ncase\endcsname{40}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.negnames\endcsname{seed(arm)}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.nexcl\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.nfresh_subsets\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.nneg\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.nseed\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio\endcsname{0.19}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_arm\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_arm_ci\endcsname{not defined}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_arm_fresh\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_arm_fresh_ndef\endcsname{2}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_arm_hi\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_arm_lo\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_arm_ndef\endcsname{1856}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_arm_sd\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_arm_sd_hi\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_arm_sd_lo\endcsname{--}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_arm_support\endcsname{92.8}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_arm_txt\endcsname{not defined (the seed(arm) component is not resolved from zero)}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_ci\endcsname{printed}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_fresh\endcsname{0.30}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_fresh_ndef\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_hi\endcsname{0.38}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_lo\endcsname{0.06}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_ndef\endcsname{2000}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_sd\endcsname{0.44}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_sd_hi\endcsname{0.62}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_sd_lo\endcsname{0.24}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_support\endcsname{100.0}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.ratio_txt\endcsname{0.19 [0.06, 0.38]}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.resid.sd\endcsname{0.67}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.resid.share\endcsname{1.07}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.seed.sd\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.amos.var.mean.seed.share\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.cimin\endcsname{97.5}
\expandafter\gdef\csname R@an.case_seedmean.easycut\endcsname{90.0}
\expandafter\gdef\csname R@an.case_seedmean.fixture.nadded\endcsname{4}
\expandafter\gdef\csname R@an.case_seedmean.fixture.nchecks\endcsname{48}
\expandafter\gdef\csname R@an.case_seedmean.fixture.ncontrol\endcsname{18}
\expandafter\gdef\csname R@an.case_seedmean.fixture.nforced\endcsname{6}
\expandafter\gdef\csname R@an.case_seedmean.fixture.nkeys\endcsname{2089}
\expandafter\gdef\csname R@an.case_seedmean.fixture.nland\endcsname{32}
\expandafter\gdef\csname R@an.case_seedmean.fixture.nscen\endcsname{80}
\expandafter\gdef\csname R@an.case_seedmean.fixture.nworlds\endcsname{2}
\expandafter\gdef\csname R@an.case_seedmean.hardcut\endcsname{50.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1.consistent\endcsname{57}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1.consistent_shift\endcsname{17}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1.fracpos\endcsname{78.6}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1.mean\endcsname{\ensuremath{+3.48}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1.mean_contemp\endcsname{\ensuremath{+2.99}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1.mean_sens\endcsname{\ensuremath{+2.99}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1.median\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1.npos\endcsname{77}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1.top5\endcsname{41}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1.top5_cell\endcsname{41}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1.trim\endcsname{\ensuremath{+1.91}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1.vsnull\endcsname{above the analytic null and inside the simulated one}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1b.consistent\endcsname{55}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1b.consistent_shift\endcsname{20}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1b.fracpos\endcsname{70.4}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1b.mean\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1b.mean_contemp\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1b.mean_sens\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1b.median\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1b.npos\endcsname{69}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1b.top5\endcsname{57}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1b.top5_cell\endcsname{57}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1b.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1b.trim\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L1b.vsnull\endcsname{above the analytic null and inside the simulated one}
\expandafter\gdef\csname R@an.case_seedmean.kits.L2.consistent\endcsname{38}
\expandafter\gdef\csname R@an.case_seedmean.kits.L2.consistent_shift\endcsname{34}
\expandafter\gdef\csname R@an.case_seedmean.kits.L2.fracpos\endcsname{50.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.L2.mean\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L2.mean_contemp\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L2.mean_sens\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L2.median\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.kits.L2.npos\endcsname{49}
\expandafter\gdef\csname R@an.case_seedmean.kits.L2.top5\endcsname{\ensuremath{>}999}
\expandafter\gdef\csname R@an.case_seedmean.kits.L2.top5_cell\endcsname{\ensuremath{>}999$^{\dagger}$}
\expandafter\gdef\csname R@an.case_seedmean.kits.L2.top5_interp\endcsname{no}
\expandafter\gdef\csname R@an.case_seedmean.kits.L2.trim\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L2.vsnull\endcsname{above the analytic null and inside the simulated one}
\expandafter\gdef\csname R@an.case_seedmean.kits.L3.consistent\endcsname{54}
\expandafter\gdef\csname R@an.case_seedmean.kits.L3.consistent_shift\endcsname{24}
\expandafter\gdef\csname R@an.case_seedmean.kits.L3.fracpos\endcsname{68.4}
\expandafter\gdef\csname R@an.case_seedmean.kits.L3.mean\endcsname{\ensuremath{+2.09}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L3.mean_contemp\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L3.mean_sens\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L3.median\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L3.npos\endcsname{67}
\expandafter\gdef\csname R@an.case_seedmean.kits.L3.top5\endcsname{61}
\expandafter\gdef\csname R@an.case_seedmean.kits.L3.top5_cell\endcsname{61}
\expandafter\gdef\csname R@an.case_seedmean.kits.L3.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.L3.trim\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L3.vsnull\endcsname{above the analytic null and inside the simulated one}
\expandafter\gdef\csname R@an.case_seedmean.kits.L4.consistent\endcsname{54}
\expandafter\gdef\csname R@an.case_seedmean.kits.L4.consistent_shift\endcsname{23}
\expandafter\gdef\csname R@an.case_seedmean.kits.L4.fracpos\endcsname{67.3}
\expandafter\gdef\csname R@an.case_seedmean.kits.L4.mean\endcsname{\ensuremath{+2.25}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L4.mean_contemp\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L4.mean_sens\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L4.median\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L4.npos\endcsname{66}
\expandafter\gdef\csname R@an.case_seedmean.kits.L4.top5\endcsname{48}
\expandafter\gdef\csname R@an.case_seedmean.kits.L4.top5_cell\endcsname{48}
\expandafter\gdef\csname R@an.case_seedmean.kits.L4.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.L4.trim\endcsname{\ensuremath{+1.47}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L4.vsnull\endcsname{above the analytic null and inside the simulated one}
\expandafter\gdef\csname R@an.case_seedmean.kits.L6.consistent\endcsname{45}
\expandafter\gdef\csname R@an.case_seedmean.kits.L6.consistent_shift\endcsname{21}
\expandafter\gdef\csname R@an.case_seedmean.kits.L6.fracpos\endcsname{62.2}
\expandafter\gdef\csname R@an.case_seedmean.kits.L6.mean\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L6.mean_contemp\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L6.mean_sens\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L6.median\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L6.npos\endcsname{61}
\expandafter\gdef\csname R@an.case_seedmean.kits.L6.top5\endcsname{76}
\expandafter\gdef\csname R@an.case_seedmean.kits.L6.top5_cell\endcsname{76}
\expandafter\gdef\csname R@an.case_seedmean.kits.L6.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.L6.trim\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.case_seedmean.kits.L6.vsnull\endcsname{above the analytic null and inside the simulated one}
\expandafter\gdef\csname R@an.case_seedmean.kits.cons.max\endcsname{57}
\expandafter\gdef\csname R@an.case_seedmean.kits.cons.maxarm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.case_seedmean.kits.cons.min\endcsname{38}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L1_L1b\endcsname{0.64}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L1_L1b.ceil\endcsname{0.83}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L1_L2\endcsname{0.35}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L1_L2.ceil\endcsname{0.77}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L1_L4\endcsname{0.70}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L1_L4.ceil\endcsname{0.70}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L1_L6\endcsname{0.56}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L1_L6.ceil\endcsname{0.79}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L1b_L2\endcsname{0.60}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L1b_L2.ceil\endcsname{0.77}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L1b_L4\endcsname{0.65}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L1b_L4.ceil\endcsname{0.70}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L1b_L6\endcsname{0.65}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L1b_L6.ceil\endcsname{0.80}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L3_L1\endcsname{0.61}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L3_L1.ceil\endcsname{0.76}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L3_L1b\endcsname{0.52}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L3_L1b.ceil\endcsname{0.76}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L3_L2\endcsname{0.43}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L3_L2.ceil\endcsname{0.70}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L3_L4\endcsname{0.76}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L3_L4.ceil\endcsname{0.63}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L3_L6\endcsname{0.66}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L3_L6.ceil\endcsname{0.72}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L4_L2\endcsname{0.36}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L4_L2.ceil\endcsname{0.65}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L4_L6\endcsname{0.77}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L4_L6.ceil\endcsname{0.66}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L6_L2\endcsname{0.38}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.L6_L2.ceil\endcsname{0.74}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.ceiling\endcsname{0.59}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.ceiling_adj\endcsname{0.74}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.ceiling_hi\endcsname{0.83}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.ceiling_lo\endcsname{0.63}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.cross\endcsname{0.46}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.dismax\endcsname{1.21}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.dismax_hi\endcsname{2.60}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.dismax_lo\endcsname{0.99}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.dismaxpair\endcsname{HyReX--ResEnc+context}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.dismean\endcsname{0.79}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.max\endcsname{0.77}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.maxceil\endcsname{0.66}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.maxpair\endcsname{ResEnc+context--HyReX+context}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.nabove\endcsname{2}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.nabove_boot\endcsname{3.5}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.nabove_hi\endcsname{7}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.nabove_lo\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.nabove_pnone\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.npairs\endcsname{15}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.sb.L1\endcsname{0.83}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.sb.L1b\endcsname{0.84}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.sb.L2\endcsname{0.72}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.sb.L3\endcsname{0.69}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.sb.L4\endcsname{0.58}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.sb.L6\endcsname{0.76}
\expandafter\gdef\csname R@an.case_seedmean.kits.corr.shared\endcsname{79}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1.consistent\endcsname{73}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1.consistent_shift\endcsname{17}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1.fracpos\endcsname{83.7}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1.mean\endcsname{\ensuremath{+1.19}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1.mean_contemp\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1.mean_sens\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1.median\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1.npos\endcsname{82}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1.top5\endcsname{55}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1.top5_cell\endcsname{55}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1.trim\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1.vsnull\endcsname{above both nulls}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1b.consistent\endcsname{69}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1b.consistent_shift\endcsname{20}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1b.fracpos\endcsname{78.6}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1b.mean\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1b.mean_contemp\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1b.mean_sens\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1b.median\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1b.npos\endcsname{77}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1b.top5\endcsname{65}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1b.top5_cell\endcsname{65}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1b.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1b.trim\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L1b.vsnull\endcsname{above both nulls}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L2.consistent\endcsname{33}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L2.consistent_shift\endcsname{64}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L2.fracpos\endcsname{40.8}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L2.mean\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L2.mean_contemp\endcsname{\ensuremath{-0.74}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L2.mean_sens\endcsname{\ensuremath{-0.74}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L2.median\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L2.npos\endcsname{40}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L2.top5\endcsname{197}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L2.top5_cell\endcsname{197$^{\dagger}$}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L2.top5_interp\endcsname{no}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L2.trim\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L2.vsnull\endcsname{inside both nulls}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L3.consistent\endcsname{60}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L3.consistent_shift\endcsname{18}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L3.fracpos\endcsname{69.4}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L3.mean\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L3.mean_contemp\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L3.mean_sens\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L3.median\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L3.npos\endcsname{68}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L3.top5\endcsname{64}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L3.top5_cell\endcsname{64}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L3.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L3.trim\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L3.vsnull\endcsname{above the analytic null and inside the simulated one}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L4.consistent\endcsname{65}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L4.consistent_shift\endcsname{18}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L4.fracpos\endcsname{79.6}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L4.mean\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L4.mean_contemp\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L4.mean_sens\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L4.median\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L4.npos\endcsname{78}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L4.top5\endcsname{55}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L4.top5_cell\endcsname{55}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L4.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L4.trim\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L4.vsnull\endcsname{above both nulls}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L6.consistent\endcsname{50}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L6.consistent_shift\endcsname{18}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L6.fracpos\endcsname{63.3}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L6.mean\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L6.mean_contemp\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L6.mean_sens\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L6.median\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L6.npos\endcsname{62}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L6.top5\endcsname{84}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L6.top5_cell\endcsname{84}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L6.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L6.trim\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.L6.vsnull\endcsname{above the analytic null and inside the simulated one}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.cons.max\endcsname{73}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.cons.maxarm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.cons.min\endcsname{33}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L1_L1b\endcsname{0.65}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L1_L1b.ceil\endcsname{0.85}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L1_L2\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L1_L2.ceil\endcsname{0.82}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L1_L4\endcsname{0.83}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L1_L4.ceil\endcsname{0.44}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L1_L6\endcsname{0.81}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L1_L6.ceil\endcsname{0.84}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L1b_L2\endcsname{0.62}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L1b_L2.ceil\endcsname{0.81}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L1b_L4\endcsname{0.87}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L1b_L4.ceil\endcsname{0.43}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L1b_L6\endcsname{0.43}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L1b_L6.ceil\endcsname{0.83}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L3_L1\endcsname{0.82}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L3_L1.ceil\endcsname{0.78}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L3_L1b\endcsname{0.61}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L3_L1b.ceil\endcsname{0.77}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L3_L2\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L3_L2.ceil\endcsname{0.74}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L3_L4\endcsname{0.87}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L3_L4.ceil\endcsname{0.40}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L3_L6\endcsname{0.87}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L3_L6.ceil\endcsname{0.76}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L4_L2\endcsname{0.23}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L4_L2.ceil\endcsname{0.42}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L4_L6\endcsname{0.71}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L4_L6.ceil\endcsname{0.43}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L6_L2\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.L6_L2.ceil\endcsname{0.80}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.ceiling\endcsname{0.58}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.ceiling_adj\endcsname{0.73}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.ceiling_hi\endcsname{0.85}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.ceiling_lo\endcsname{0.40}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.cross\endcsname{0.43}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.dismax\endcsname{2.19}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.dismax_hi\endcsname{4.71}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.dismax_lo\endcsname{1.07}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.dismaxpair\endcsname{HyReX--ResEnc+context}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.dismean\endcsname{0.93}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.max\endcsname{0.87}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.maxceil\endcsname{0.40}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.maxpair\endcsname{HyReX--ResEnc+context}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.nabove\endcsname{6}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.nabove_boot\endcsname{5.2}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.nabove_hi\endcsname{10}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.nabove_lo\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.nabove_pnone\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.npairs\endcsname{15}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.sb.L1\endcsname{0.86}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.sb.L1b\endcsname{0.84}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.sb.L2\endcsname{0.78}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.sb.L3\endcsname{0.71}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.sb.L4\endcsname{0.22}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.sb.L6\endcsname{0.82}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.corr.shared\endcsname{74}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.loo.consistent\endcsname{32.7}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.loo.max\endcsname{34}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.loo.mean\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.loo.min\endcsname{31}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.oracle.best\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.oracle.best_mean\endcsname{\ensuremath{+1.19}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.oracle.gain\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.oracle.gain_cv\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.oracle.mean\endcsname{\ensuremath{+1.46}}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.shift.max\endcsname{64}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.shift.maxarm\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.shift.min\endcsname{17}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.shift.minarm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.shift.nabove\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.kits.kidney.shift.ndrop\endcsname{5}
\expandafter\gdef\csname R@an.case_seedmean.kits.loo.consistent\endcsname{32.7}
\expandafter\gdef\csname R@an.case_seedmean.kits.loo.max\endcsname{34}
\expandafter\gdef\csname R@an.case_seedmean.kits.loo.mean\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.kits.loo.min\endcsname{30}
\expandafter\gdef\csname R@an.case_seedmean.kits.loo.ncombo\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.loo.p\endcsname{1/3}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1.consistent\endcsname{54}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1.consistent_shift\endcsname{17}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1.fracpos\endcsname{73.5}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1.mean\endcsname{\ensuremath{+4.15}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1.mean_contemp\endcsname{\ensuremath{+3.66}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1.mean_sens\endcsname{\ensuremath{+3.66}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1.median\endcsname{\ensuremath{+0.91}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1.npos\endcsname{72}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1.top5\endcsname{51}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1.top5_cell\endcsname{51}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1.trim\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1.vsnull\endcsname{above the analytic null and inside the simulated one}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1b.consistent\endcsname{52}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1b.consistent_shift\endcsname{17}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1b.fracpos\endcsname{70.4}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1b.mean\endcsname{\ensuremath{+3.26}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1b.mean_contemp\endcsname{\ensuremath{+2.77}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1b.mean_sens\endcsname{\ensuremath{+2.77}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1b.median\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1b.npos\endcsname{69}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1b.top5\endcsname{62}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1b.top5_cell\endcsname{62}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1b.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1b.trim\endcsname{\ensuremath{+1.50}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L1b.vsnull\endcsname{above the analytic null and inside the simulated one}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L2.consistent\endcsname{37}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L2.consistent_shift\endcsname{30}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L2.fracpos\endcsname{53.1}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L2.mean\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L2.mean_contemp\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L2.mean_sens\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L2.median\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L2.npos\endcsname{52}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L2.top5\endcsname{265}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L2.top5_cell\endcsname{265$^{\dagger}$}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L2.top5_interp\endcsname{no}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L2.trim\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L2.vsnull\endcsname{inside both nulls}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L3.consistent\endcsname{56}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L3.consistent_shift\endcsname{21}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L3.fracpos\endcsname{70.4}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L3.mean\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L3.mean_contemp\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L3.mean_sens\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L3.median\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L3.npos\endcsname{69}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L3.top5\endcsname{54}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L3.top5_cell\endcsname{54}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L3.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L3.trim\endcsname{\ensuremath{+1.68}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L3.vsnull\endcsname{above the analytic null and inside the simulated one}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L4.consistent\endcsname{51}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L4.consistent_shift\endcsname{16}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L4.fracpos\endcsname{66.3}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L4.mean\endcsname{\ensuremath{+2.73}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L4.mean_contemp\endcsname{\ensuremath{+2.25}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L4.mean_sens\endcsname{\ensuremath{+2.25}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L4.median\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L4.npos\endcsname{65}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L4.top5\endcsname{58}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L4.top5_cell\endcsname{58}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L4.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L4.trim\endcsname{\ensuremath{+1.22}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L4.vsnull\endcsname{above the analytic null and inside the simulated one}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L6.consistent\endcsname{40}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L6.consistent_shift\endcsname{21}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L6.fracpos\endcsname{55.1}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L6.mean\endcsname{\ensuremath{+1.72}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L6.mean_contemp\endcsname{\ensuremath{+1.24}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L6.mean_sens\endcsname{\ensuremath{+1.24}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L6.median\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L6.npos\endcsname{54}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L6.top5\endcsname{97}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L6.top5_cell\endcsname{97}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L6.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L6.trim\endcsname{\ensuremath{+0.90}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.L6.vsnull\endcsname{above the analytic null and inside the simulated one}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.cons.max\endcsname{56}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.cons.maxarm\endcsname{HyReX}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.cons.min\endcsname{37}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L1_L1b\endcsname{0.77}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L1_L1b.ceil\endcsname{0.87}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L1_L2\endcsname{0.52}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L1_L2.ceil\endcsname{0.72}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L1_L4\endcsname{0.80}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L1_L4.ceil\endcsname{0.75}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L1_L6\endcsname{0.58}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L1_L6.ceil\endcsname{0.79}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L1b_L2\endcsname{0.69}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L1b_L2.ceil\endcsname{0.75}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L1b_L4\endcsname{0.78}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L1b_L4.ceil\endcsname{0.79}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L1b_L6\endcsname{0.70}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L1b_L6.ceil\endcsname{0.82}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L3_L1\endcsname{0.67}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L3_L1.ceil\endcsname{0.73}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L3_L1b\endcsname{0.69}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L3_L1b.ceil\endcsname{0.76}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L3_L2\endcsname{0.55}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L3_L2.ceil\endcsname{0.63}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L3_L4\endcsname{0.75}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L3_L4.ceil\endcsname{0.66}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L3_L6\endcsname{0.64}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L3_L6.ceil\endcsname{0.69}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L4_L2\endcsname{0.51}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L4_L2.ceil\endcsname{0.65}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L4_L6\endcsname{0.79}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L4_L6.ceil\endcsname{0.71}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L6_L2\endcsname{0.54}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.L6_L2.ceil\endcsname{0.68}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.ceiling\endcsname{0.60}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.ceiling_adj\endcsname{0.75}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.ceiling_hi\endcsname{0.87}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.ceiling_lo\endcsname{0.63}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.cross\endcsname{0.53}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.dismax\endcsname{1.14}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.dismax_hi\endcsname{2.05}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.dismax_lo\endcsname{1.01}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.dismaxpair\endcsname{HyReX--ResEnc+context}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.dismean\endcsname{0.91}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.max\endcsname{0.80}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.maxceil\endcsname{0.75}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.maxpair\endcsname{ResEnc-M (library preset)--ResEnc+context}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.nabove\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.nabove_boot\endcsname{5.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.nabove_hi\endcsname{11}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.nabove_lo\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.nabove_pnone\endcsname{2}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.npairs\endcsname{15}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.sb.L1\endcsname{0.83}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.sb.L1b\endcsname{0.92}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.sb.L2\endcsname{0.62}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.sb.L3\endcsname{0.64}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.sb.L4\endcsname{0.68}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.sb.L6\endcsname{0.74}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.corr.shared\endcsname{90}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.loo.consistent\endcsname{32.3}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.loo.max\endcsname{35}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.loo.mean\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.loo.min\endcsname{31}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.oracle.best\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.oracle.best_mean\endcsname{\ensuremath{+4.15}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.oracle.gain\endcsname{\ensuremath{+2.07}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.oracle.gain_cv\endcsname{\ensuremath{-0.69}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.oracle.mean\endcsname{\ensuremath{+6.22}}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.shift.max\endcsname{30}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.shift.maxarm\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.shift.min\endcsname{16}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.shift.minarm\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.shift.nabove\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.kits.masses.shift.ndrop\endcsname{6}
\expandafter\gdef\csname R@an.case_seedmean.kits.n\endcsname{98}
\expandafter\gdef\csname R@an.case_seedmean.kits.narms\endcsname{6}
\expandafter\gdef\csname R@an.case_seedmean.kits.nempty\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.kits.npending\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.kits.null.consistent_exp\endcsname{28.4}
\expandafter\gdef\csname R@an.case_seedmean.kits.null.hi\endcsname{37}
\expandafter\gdef\csname R@an.case_seedmean.kits.null.lo\endcsname{20}
\expandafter\gdef\csname R@an.case_seedmean.kits.null.npool\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.null.p\endcsname{0.2902}
\expandafter\gdef\csname R@an.case_seedmean.kits.null.rho\endcsname{0.250}
\expandafter\gdef\csname R@an.case_seedmean.kits.oracle.best\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.case_seedmean.kits.oracle.best_mean\endcsname{\ensuremath{+3.48}}
\expandafter\gdef\csname R@an.case_seedmean.kits.oracle.gain\endcsname{\ensuremath{+1.56}}
\expandafter\gdef\csname R@an.case_seedmean.kits.oracle.gain_cv\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.case_seedmean.kits.oracle.mean\endcsname{\ensuremath{+5.03}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1.dprec\endcsname{\ensuremath{+6.57}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1.drec\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1.prec\endcsname{78.3}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1.prec_hi\endcsname{80.1}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1.prec_lo\endcsname{77.4}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1.prec_micro\endcsname{87.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1.rec\endcsname{84.6}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1.rec_hi\endcsname{84.7}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1.rec_lo\endcsname{84.6}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1.rec_micro\endcsname{93.3}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1.sephalf\endcsname{recall}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1.sepmargin\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1.vol\endcsname{\ensuremath{+0.075}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1b.dprec\endcsname{\ensuremath{+4.21}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1b.drec\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1b.prec\endcsname{75.9}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1b.prec_hi\endcsname{76.3}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1b.prec_lo\endcsname{75.4}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1b.prec_micro\endcsname{82.6}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1b.rec\endcsname{84.5}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1b.rec_hi\endcsname{85.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1b.rec_lo\endcsname{84.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1b.rec_micro\endcsname{93.5}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1b.sephalf\endcsname{recall}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1b.sepmargin\endcsname{\ensuremath{-0.69}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L1b.vol\endcsname{\ensuremath{+0.096}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L2.dprec\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L2.drec\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L2.prec\endcsname{71.6}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L2.prec_hi\endcsname{72.8}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L2.prec_lo\endcsname{70.8}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L2.prec_micro\endcsname{76.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L2.rec\endcsname{85.3}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L2.rec_hi\endcsname{86.1}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L2.rec_lo\endcsname{84.6}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L2.rec_micro\endcsname{93.3}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L2.sephalf\endcsname{precision}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L2.sepmargin\endcsname{\ensuremath{-2.32}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L2.vol\endcsname{\ensuremath{+0.139}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L3.dprec\endcsname{\ensuremath{+2.74}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L3.drec\endcsname{\ensuremath{+1.41}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L3.prec\endcsname{74.5}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L3.prec_hi\endcsname{75.1}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L3.prec_lo\endcsname{73.8}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L3.prec_micro\endcsname{82.9}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L3.rec\endcsname{85.6}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L3.rec_hi\endcsname{86.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L3.rec_lo\endcsname{85.3}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L3.rec_micro\endcsname{93.4}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L3.sephalf\endcsname{recall}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L3.sepmargin\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L3.vol\endcsname{\ensuremath{+0.146}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L4.dprec\endcsname{\ensuremath{+5.34}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L4.drec\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L4.prec\endcsname{77.1}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L4.prec_hi\endcsname{78.1}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L4.prec_lo\endcsname{76.6}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L4.prec_micro\endcsname{84.1}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L4.rec\endcsname{83.8}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L4.rec_hi\endcsname{84.2}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L4.rec_lo\endcsname{83.4}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L4.rec_micro\endcsname{93.6}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L4.sephalf\endcsname{recall}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L4.sepmargin\endcsname{\ensuremath{-1.33}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L4.vol\endcsname{\ensuremath{+0.079}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L6.dprec\endcsname{\ensuremath{+3.67}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L6.drec\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L6.prec\endcsname{75.4}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L6.prec_hi\endcsname{76.7}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L6.prec_lo\endcsname{74.1}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L6.prec_micro\endcsname{82.1}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L6.rec\endcsname{84.4}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L6.rec_hi\endcsname{85.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L6.rec_lo\endcsname{83.7}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L6.rec_micro\endcsname{93.3}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L6.sephalf\endcsname{recall}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L6.sepmargin\endcsname{\ensuremath{-1.02}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.L6.vol\endcsname{\ensuremath{+0.098}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.default.prec\endcsname{71.7}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.default.prec_hi\endcsname{73.1}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.default.prec_lo\endcsname{70.5}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.default.prec_micro\endcsname{77.7}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.default.rec\endcsname{84.2}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.default.rec_hi\endcsname{84.7}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.default.rec_lo\endcsname{83.6}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.default.rec_micro\endcsname{93.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.default.vol\endcsname{\ensuremath{+0.110}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.herosep\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.npos\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.nruns\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.nsep\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.sep\endcsname{HyReX}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.sepmargin\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.sepmargin_next\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.sepmargin_nextarm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.sepmargin_nextgap\endcsname{0.12}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.sepmargin_nexthalf\endcsname{recall}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.sepmargin_nextword\endcsname{misses}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr.sepmarginarm\endcsname{HyReX}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1.dprec\endcsname{\ensuremath{+5.57}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1.drec\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1.prec\endcsname{83.7}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1.prec_hi\endcsname{84.5}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1.prec_lo\endcsname{82.8}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1.prec_micro\endcsname{88.6}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1.rec\endcsname{87.8}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1.rec_hi\endcsname{88.2}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1.rec_lo\endcsname{87.5}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1.rec_micro\endcsname{93.6}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1.sephalf\endcsname{recall}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1.sepmargin\endcsname{\ensuremath{-0.94}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1.vol\endcsname{\ensuremath{+0.036}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1b.dprec\endcsname{\ensuremath{+4.40}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1b.drec\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1b.prec\endcsname{82.5}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1b.prec_hi\endcsname{82.6}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1b.prec_lo\endcsname{82.4}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1b.prec_micro\endcsname{85.7}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1b.rec\endcsname{88.2}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1b.rec_hi\endcsname{88.2}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1b.rec_lo\endcsname{88.1}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1b.rec_micro\endcsname{94.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1b.sephalf\endcsname{recall}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1b.sepmargin\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L1b.vol\endcsname{\ensuremath{+0.059}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L2.dprec\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L2.drec\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L2.prec\endcsname{78.8}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L2.prec_hi\endcsname{80.2}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L2.prec_lo\endcsname{77.4}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L2.prec_micro\endcsname{79.3}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L2.rec\endcsname{87.7}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L2.rec_hi\endcsname{87.8}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L2.rec_lo\endcsname{87.6}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L2.rec_micro\endcsname{92.8}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L2.sephalf\endcsname{precision}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L2.sepmargin\endcsname{\ensuremath{-1.64}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L2.vol\endcsname{\ensuremath{+0.100}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L3.dprec\endcsname{\ensuremath{+3.53}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L3.drec\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L3.prec\endcsname{81.6}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L3.prec_hi\endcsname{81.9}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L3.prec_lo\endcsname{81.4}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L3.prec_micro\endcsname{85.7}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L3.rec\endcsname{88.7}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L3.rec_hi\endcsname{89.2}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L3.rec_lo\endcsname{88.2}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L3.rec_micro\endcsname{93.9}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L3.sephalf\endcsname{recall}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L3.sepmargin\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L3.vol\endcsname{\ensuremath{+0.067}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L4.dprec\endcsname{\ensuremath{+3.83}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L4.drec\endcsname{\ensuremath{-0.67}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L4.prec\endcsname{81.9}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L4.prec_hi\endcsname{83.1}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L4.prec_lo\endcsname{80.8}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L4.prec_micro\endcsname{87.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L4.rec\endcsname{87.3}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L4.rec_hi\endcsname{87.5}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L4.rec_lo\endcsname{87.1}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L4.rec_micro\endcsname{94.1}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L4.sephalf\endcsname{recall}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L4.sepmargin\endcsname{\ensuremath{-1.32}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L4.vol\endcsname{\ensuremath{+0.054}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L6.dprec\endcsname{\ensuremath{+2.37}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L6.drec\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L6.prec\endcsname{80.5}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L6.prec_hi\endcsname{81.1}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L6.prec_lo\endcsname{79.8}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L6.prec_micro\endcsname{83.4}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L6.rec\endcsname{88.1}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L6.rec_hi\endcsname{88.2}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L6.rec_lo\endcsname{87.9}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L6.rec_micro\endcsname{93.7}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L6.sephalf\endcsname{recall}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L6.sepmargin\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.L6.vol\endcsname{\ensuremath{+0.077}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.default.prec\endcsname{78.1}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.default.prec_hi\endcsname{79.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.default.prec_lo\endcsname{76.9}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.default.prec_micro\endcsname{80.6}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.default.rec\endcsname{88.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.default.rec_hi\endcsname{88.4}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.default.rec_lo\endcsname{87.3}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.default.rec_micro\endcsname{93.9}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.default.vol\endcsname{\ensuremath{+0.085}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.herosep\endcsname{no}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.npos\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.nruns\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.nsep\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.sep\endcsname{none}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.sepmargin\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.sepmargin_next\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.sepmargin_nextarm\endcsname{ResEnc-matched}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.sepmargin_nextgap\endcsname{0.29}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.sepmargin_nexthalf\endcsname{recall}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.sepmargin_nextword\endcsname{misses}
\expandafter\gdef\csname R@an.case_seedmean.kits.pr_masses.sepmarginarm\endcsname{HyReX}
\expandafter\gdef\csname R@an.case_seedmean.kits.ref.contemp.mean\endcsname{83.866}
\expandafter\gdef\csname R@an.case_seedmean.kits.ref.contemp.n\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.ref.contemp.sd\endcsname{0.703}
\expandafter\gdef\csname R@an.case_seedmean.kits.ref.contemp.shift\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.case_seedmean.kits.ref.contemp.short\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.case_seedmean.kits.ref.frozen.mean\endcsname{83.378}
\expandafter\gdef\csname R@an.case_seedmean.kits.ref.frozen.n\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.ref.frozen.sd\endcsname{0.795}
\expandafter\gdef\csname R@an.case_seedmean.kits.ref.frozen.shift\endcsname{0.000}
\expandafter\gdef\csname R@an.case_seedmean.kits.ref.frozen.short\endcsname{frozen pool}
\expandafter\gdef\csname R@an.case_seedmean.kits.ref.nfin\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.kits.ref.npend\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.kits.ref.pendnames\endcsname{none}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1.bar\endcsname{clears}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1.casegap\endcsname{0.000}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1.casemean\endcsname{\ensuremath{+3.475}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1.delta\endcsname{\ensuremath{+3.475}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1.mean\endcsname{86.853}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1.runs\endcsname{above}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1.s1\endcsname{86.512}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1.s2\endcsname{87.195}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1.se_pool\endcsname{0.726}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1.se_seed\endcsname{0.342}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1.spread\endcsname{0.683}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1.state\endcsname{separated above}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1b.bar\endcsname{clears}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1b.casegap\endcsname{0.000}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1b.casemean\endcsname{\ensuremath{+2.313}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1b.delta\endcsname{\ensuremath{+2.313}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1b.mean\endcsname{85.691}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1b.runs\endcsname{above}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1b.s1\endcsname{85.942}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1b.s2\endcsname{85.441}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1b.se_pool\endcsname{0.726}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1b.se_seed\endcsname{0.251}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1b.spread\endcsname{0.501}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L1b.state\endcsname{separated above}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L2.bar\endcsname{below}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L2.casegap\endcsname{0.000}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L2.casemean\endcsname{\ensuremath{+0.110}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L2.delta\endcsname{\ensuremath{+0.110}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L2.mean\endcsname{83.489}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L2.runs\endcsname{overlaps}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L2.s1\endcsname{82.573}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L2.s2\endcsname{84.404}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L2.se_pool\endcsname{0.726}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L2.se_seed\endcsname{0.915}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L2.spread\endcsname{1.831}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L2.state\endcsname{not separated}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L3.bar\endcsname{clears}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L3.casegap\endcsname{0.000}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L3.casemean\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L3.delta\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L3.mean\endcsname{85.472}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L3.runs\endcsname{above}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L3.s1\endcsname{85.176}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L3.s2\endcsname{85.768}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L3.se_pool\endcsname{0.726}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L3.se_seed\endcsname{0.296}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L3.spread\endcsname{0.592}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L3.state\endcsname{separated above}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L4.bar\endcsname{clears}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L4.casegap\endcsname{0.000}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L4.casemean\endcsname{\ensuremath{+2.246}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L4.delta\endcsname{\ensuremath{+2.246}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L4.mean\endcsname{85.625}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L4.runs\endcsname{above}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L4.s1\endcsname{86.055}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L4.s2\endcsname{85.194}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L4.se_pool\endcsname{0.726}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L4.se_seed\endcsname{0.431}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L4.spread\endcsname{0.862}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L4.state\endcsname{separated above}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L6.bar\endcsname{clears}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L6.casegap\endcsname{0.000}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L6.casemean\endcsname{\ensuremath{+1.591}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L6.delta\endcsname{\ensuremath{+1.591}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L6.mean\endcsname{84.970}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L6.runs\endcsname{above}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L6.s1\endcsname{84.577}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L6.s2\endcsname{85.363}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L6.se_pool\endcsname{0.726}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L6.se_seed\endcsname{0.393}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L6.spread\endcsname{0.786}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.L6.state\endcsname{separated above}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.arms\endcsname{HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context, HyReX+context}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.bar.value\endcsname{0.35}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.gaphero\endcsname{\ensuremath{+1.382}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.herorank\endcsname{4}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.herosentence\endcsname{On KiTS23 HyReX's fresh-mean delta, \ensuremath{+2.094}\,pp (\ensuremath{+1.850}\,pp against the six-run reference), ranks 4th of the 6 complete pairs, 1.382\,pp behind ResEnc-M's.}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.lead\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.lead_vs\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.leadcons\endcsname{57}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.leadgap\endcsname{\ensuremath{+1.162}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.leadishero\endcsname{no}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.leadsentence\endcsname{On KiTS23 the largest fresh-mean delta of the 6 complete pairs is ResEnc-M's, \ensuremath{+3.475}\,pp (\ensuremath{+3.232}\,pp against the six-run reference), which is 1.162\,pp ahead of ResEnc-matched's.}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.narms\endcsname{6}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.nlead\endcsname{6}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.nnosep\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.nosepnames\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.nsep\endcsname{5}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.order\endcsname{ResEnc-M (library preset) \ensuremath{+3.475}, ResEnc-matched (re-implemented) \ensuremath{+2.313}, ResEnc+context \ensuremath{+2.246}, HyReX \ensuremath{+2.094}, HyReX+context \ensuremath{+1.591}, ConvNeXt-k3 \ensuremath{+0.110}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.sepdef\endcsname{both fresh runs above every one of the 3 frozen-pool runs, or both below every one}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.sepnames\endcsname{ResEnc-M, ResEnc-matched, ResEnc+context, HyReX, HyReX+context}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.sepsentence\endcsname{At two fresh seeds KiTS23 separates ResEnc-M (\ensuremath{+3.475}\,pp against the frozen pool, \ensuremath{+3.232}\,pp against the six-run reference), ResEnc-matched (\ensuremath{+2.313}\,pp, \ensuremath{+2.070}\,pp), ResEnc+context (\ensuremath{+2.246}\,pp, \ensuremath{+2.003}\,pp), HyReX (\ensuremath{+2.094}\,pp, \ensuremath{+1.850}\,pp) and HyReX+context (\ensuremath{+1.591}\,pp, \ensuremath{+1.348}\,pp); does not separate ConvNeXt-k3 (\ensuremath{+0.110}\,pp, \ensuremath{-0.133}\,pp).}
\expandafter\gdef\csname R@an.case_seedmean.kits.rep.state\endcsname{separated above}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L1.hardgain\endcsname{\ensuremath{+14.22}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L1.lost\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L1.nhard\endcsname{13}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L1.rate\endcsname{38.5}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L1.rescued\endcsname{5}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L1.vsnull\endcsname{above}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L1b.hardgain\endcsname{\ensuremath{+4.68}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L1b.lost\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L1b.nhard\endcsname{13}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L1b.rate\endcsname{7.7}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L1b.rescued\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L1b.vsnull\endcsname{below}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L2.hardgain\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L2.lost\endcsname{4}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L2.nhard\endcsname{13}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L2.rate\endcsname{7.7}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L2.rescued\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L2.vsnull\endcsname{below}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L3.hardgain\endcsname{\ensuremath{+8.18}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L3.lost\endcsname{2}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L3.nhard\endcsname{13}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L3.rate\endcsname{15.4}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L3.rescued\endcsname{2}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L3.vsnull\endcsname{inside}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L4.hardgain\endcsname{\ensuremath{+8.54}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L4.lost\endcsname{2}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L4.nhard\endcsname{13}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L4.rate\endcsname{7.7}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L4.rescued\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L4.vsnull\endcsname{below}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L6.hardgain\endcsname{\ensuremath{+5.02}}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L6.lost\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L6.nhard\endcsname{13}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L6.rate\endcsname{23.1}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L6.rescued\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.L6.vsnull\endcsname{inside}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.abovenames\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.nabove\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.neasy\endcsname{31}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.nhard\endcsname{13}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.null.lost\endcsname{3.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.null.lost_max\endcsname{4}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.null.lost_min\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.null.ndraw\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.null.nhard\endcsname{15.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.null.nhard_max\endcsname{16}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.null.nhard_min\endcsname{14}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.null.rate\endcsname{19.9}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.null.rate_max\endcsname{25.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.null.rate_min\endcsname{13.3}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.null.rescued\endcsname{3.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.null.rescued_max\endcsname{4}
\expandafter\gdef\csname R@an.case_seedmean.kits.rescue.null.rescued_min\endcsname{2}
\expandafter\gdef\csname R@an.case_seedmean.kits.sens.key\endcsname{contemp}
\expandafter\gdef\csname R@an.case_seedmean.kits.sens.n\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.sens.shift\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.case_seedmean.kits.sens.short\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.case_seedmean.kits.sens.state\endcsname{ready}
\expandafter\gdef\csname R@an.case_seedmean.kits.shift.max\endcsname{34}
\expandafter\gdef\csname R@an.case_seedmean.kits.shift.maxarm\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.case_seedmean.kits.shift.min\endcsname{17}
\expandafter\gdef\csname R@an.case_seedmean.kits.shift.minarm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.case_seedmean.kits.shift.nabove\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.kits.shift.ndrop\endcsname{6}
\expandafter\gdef\csname R@an.case_seedmean.kits.sim.hi\endcsname{58}
\expandafter\gdef\csname R@an.case_seedmean.kits.sim.lo\endcsname{8}
\expandafter\gdef\csname R@an.case_seedmean.kits.sim.mean\endcsname{28.5}
\expandafter\gdef\csname R@an.case_seedmean.kits.sim.scasehi\endcsname{26.96}
\expandafter\gdef\csname R@an.case_seedmean.kits.sim.scaselo\endcsname{0.39}
\expandafter\gdef\csname R@an.case_seedmean.kits.sim.scasemed\endcsname{1.30}
\expandafter\gdef\csname R@an.case_seedmean.kits.sim.sdrun\endcsname{0.584}
\expandafter\gdef\csname R@an.case_seedmean.kits.six.adj\endcsname{six-run}
\expandafter\gdef\csname R@an.case_seedmean.kits.six.n\endcsname{6}
\expandafter\gdef\csname R@an.case_seedmean.kits.six.shift\endcsname{\ensuremath{+0.244}}
\expandafter\gdef\csname R@an.case_seedmean.kits.six.state\endcsname{ready}
\expandafter\gdef\csname R@an.case_seedmean.kits.tert.source\endcsname{physical tumour volume}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1.consistent\endcsname{56}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1.consistent_shift\endcsname{22}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1.fracpos\endcsname{75.5}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1.mean\endcsname{\ensuremath{+5.09}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1.mean_contemp\endcsname{\ensuremath{+4.61}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1.mean_sens\endcsname{\ensuremath{+4.61}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1.median\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1.npos\endcsname{74}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1.top5\endcsname{36}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1.top5_cell\endcsname{36}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1.trim\endcsname{\ensuremath{+3.39}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1.vsnull\endcsname{above both nulls}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1b.consistent\endcsname{53}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1b.consistent_shift\endcsname{19}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1b.fracpos\endcsname{67.3}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1b.mean\endcsname{\ensuremath{+2.80}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1b.mean_contemp\endcsname{\ensuremath{+2.32}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1b.mean_sens\endcsname{\ensuremath{+2.32}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1b.median\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1b.npos\endcsname{66}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1b.top5\endcsname{55}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1b.top5_cell\endcsname{55}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1b.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1b.trim\endcsname{\ensuremath{+2.03}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L1b.vsnull\endcsname{above the analytic null and inside the simulated one}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L2.consistent\endcsname{38}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L2.consistent_shift\endcsname{39}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L2.fracpos\endcsname{52.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L2.mean\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L2.mean_contemp\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L2.mean_sens\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L2.median\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L2.npos\endcsname{51}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L2.top5\endcsname{\ensuremath{>}999}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L2.top5_cell\endcsname{\ensuremath{>}999$^{\dagger}$}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L2.top5_interp\endcsname{no}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L2.trim\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L2.vsnull\endcsname{above the analytic null and inside the simulated one}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L3.consistent\endcsname{48}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L3.consistent_shift\endcsname{23}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L3.fracpos\endcsname{63.3}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L3.mean\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L3.mean_contemp\endcsname{\ensuremath{+1.85}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L3.mean_sens\endcsname{\ensuremath{+1.85}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L3.median\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L3.npos\endcsname{62}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L3.top5\endcsname{75}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L3.top5_cell\endcsname{75}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L3.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L3.trim\endcsname{\ensuremath{+1.55}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L3.vsnull\endcsname{above the analytic null and inside the simulated one}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L4.consistent\endcsname{54}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L4.consistent_shift\endcsname{23}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L4.fracpos\endcsname{61.2}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L4.mean\endcsname{\ensuremath{+3.14}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L4.mean_contemp\endcsname{\ensuremath{+2.66}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L4.mean_sens\endcsname{\ensuremath{+2.66}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L4.median\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L4.npos\endcsname{60}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L4.top5\endcsname{51}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L4.top5_cell\endcsname{51}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L4.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L4.trim\endcsname{\ensuremath{+2.35}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L4.vsnull\endcsname{above both nulls}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L6.consistent\endcsname{42}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L6.consistent_shift\endcsname{20}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L6.fracpos\endcsname{61.2}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L6.mean\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L6.mean_contemp\endcsname{\ensuremath{+1.93}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L6.mean_sens\endcsname{\ensuremath{+1.93}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L6.median\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L6.npos\endcsname{60}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L6.top5\endcsname{65}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L6.top5_cell\endcsname{65}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L6.top5_interp\endcsname{yes}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L6.trim\endcsname{\ensuremath{+1.81}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.L6.vsnull\endcsname{above the analytic null and inside the simulated one}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.cons.max\endcsname{56}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.cons.maxarm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.cons.min\endcsname{38}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L1_L1b\endcsname{0.47}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L1_L1b.ceil\endcsname{0.73}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L1_L2\endcsname{0.24}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L1_L2.ceil\endcsname{0.82}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L1_L4\endcsname{0.44}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L1_L4.ceil\endcsname{0.77}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L1_L6\endcsname{0.46}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L1_L6.ceil\endcsname{0.72}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L1b_L2\endcsname{0.37}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L1b_L2.ceil\endcsname{0.72}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L1b_L4\endcsname{0.41}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L1b_L4.ceil\endcsname{0.67}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L1b_L6\endcsname{0.58}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L1b_L6.ceil\endcsname{0.63}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L3_L1\endcsname{0.40}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L3_L1.ceil\endcsname{0.80}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L3_L1b\endcsname{0.26}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L3_L1b.ceil\endcsname{0.70}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L3_L2\endcsname{0.49}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L3_L2.ceil\endcsname{0.79}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L3_L4\endcsname{0.69}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L3_L4.ceil\endcsname{0.74}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L3_L6\endcsname{0.53}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L3_L6.ceil\endcsname{0.69}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L4_L2\endcsname{0.27}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L4_L2.ceil\endcsname{0.75}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L4_L6\endcsname{0.62}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L4_L6.ceil\endcsname{0.66}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L6_L2\endcsname{0.26}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.L6_L2.ceil\endcsname{0.71}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.ceiling\endcsname{0.58}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.ceiling_adj\endcsname{0.73}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.ceiling_hi\endcsname{0.82}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.ceiling_lo\endcsname{0.63}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.cross\endcsname{0.35}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.dismax\endcsname{0.95}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.dismax_hi\endcsname{1.71}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.dismax_lo\endcsname{0.94}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.dismaxpair\endcsname{ResEnc+context--HyReX+context}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.dismean\endcsname{0.61}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.max\endcsname{0.69}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.maxceil\endcsname{0.74}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.maxpair\endcsname{HyReX--ResEnc+context}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.nabove\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.nabove_boot\endcsname{2.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.nabove_hi\endcsname{5}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.nabove_lo\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.nabove_pnone\endcsname{11}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.npairs\endcsname{15}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.sb.L1\endcsname{0.83}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.sb.L1b\endcsname{0.63}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.sb.L2\endcsname{0.81}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.sb.L3\endcsname{0.77}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.sb.L4\endcsname{0.70}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.sb.L6\endcsname{0.62}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.corr.shared\endcsname{60}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.loo.consistent\endcsname{32.3}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.loo.max\endcsname{36}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.loo.mean\endcsname{0.00}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.loo.min\endcsname{30}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.oracle.best\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.oracle.best_mean\endcsname{\ensuremath{+5.09}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.oracle.gain\endcsname{\ensuremath{+2.98}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.oracle.gain_cv\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.oracle.mean\endcsname{\ensuremath{+8.07}}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.shift.max\endcsname{39}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.shift.maxarm\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.shift.min\endcsname{19}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.shift.minarm\endcsname{ResEnc-matched}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.shift.nabove\endcsname{1}
\expandafter\gdef\csname R@an.case_seedmean.kits.tumor.shift.ndrop\endcsname{5}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ak.sd\endcsname{1.54}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ak.share\endcsname{10.86}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.arm.sd\endcsname{0.39}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.arm.share\endcsname{0.68}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.arms\endcsname{nnU-Net default, HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented), ResEnc+context, HyReX+context, ConvNeXt-k3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.case.sd\endcsname{3.78}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.case.share\endcsname{64.97}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.excl\endcsname{none}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.narm\endcsname{7}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.nboot\endcsname{2000}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ncase\endcsname{98}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.negnames\endcsname{none}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.nexcl\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.nfresh_subsets\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.nneg\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.nseed\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio\endcsname{0.47}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_arm\endcsname{2.90}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_arm_ci\endcsname{printed}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_arm_fresh\endcsname{9.08}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_arm_fresh_ndef\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_arm_hi\endcsname{11.29}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_arm_lo\endcsname{0.54}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_arm_ndef\endcsname{1995}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_arm_sd\endcsname{1.70}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_arm_sd_hi\endcsname{3.36}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_arm_sd_lo\endcsname{0.73}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_arm_support\endcsname{99.8}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_arm_txt\endcsname{2.90 [0.54, 11.29]}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_ci\endcsname{printed}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_fresh\endcsname{0.34}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_fresh_ndef\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_hi\endcsname{0.71}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_lo\endcsname{0.02}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_ndef\endcsname{2000}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_sd\endcsname{0.68}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_sd_hi\endcsname{0.84}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_sd_lo\endcsname{0.12}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_support\endcsname{100.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.ratio_txt\endcsname{0.47 [0.02, 0.71]}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.resid.sd\endcsname{2.26}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.resid.share\endcsname{23.25}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.seed.sd\endcsname{0.23}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.kidney.seed.share\endcsname{0.24}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ak.sd\endcsname{3.47}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ak.share\endcsname{3.11}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.arm.sd\endcsname{1.19}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.arm.share\endcsname{0.37}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.arms\endcsname{nnU-Net default, HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented), ResEnc+context, HyReX+context, ConvNeXt-k3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.case.sd\endcsname{17.96}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.case.share\endcsname{83.48}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.excl\endcsname{none}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.narm\endcsname{7}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.nboot\endcsname{2000}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ncase\endcsname{98}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.negnames\endcsname{none}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.nexcl\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.nfresh_subsets\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.nneg\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.nseed\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio\endcsname{0.24}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_arm\endcsname{6.63}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_arm_ci\endcsname{printed}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_arm_fresh\endcsname{7.28}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_arm_fresh_ndef\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_arm_hi\endcsname{17.69}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_arm_lo\endcsname{0.37}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_arm_ndef\endcsname{1965}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_arm_sd\endcsname{2.58}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_arm_sd_hi\endcsname{4.21}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_arm_sd_lo\endcsname{0.61}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_arm_support\endcsname{98.2}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_arm_txt\endcsname{6.63 [0.37, 17.69]}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_ci\endcsname{printed}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_fresh\endcsname{0.26}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_fresh_ndef\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_hi\endcsname{0.40}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_lo\endcsname{0.11}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_ndef\endcsname{2000}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_sd\endcsname{0.49}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_sd_hi\endcsname{0.63}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_sd_lo\endcsname{0.33}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_support\endcsname{100.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.ratio_txt\endcsname{0.24 [0.11, 0.40]}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.resid.sd\endcsname{7.08}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.resid.share\endcsname{12.98}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.seed.sd\endcsname{0.46}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.masses.seed.share\endcsname{0.06}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ak.sd\endcsname{2.82}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ak.share\endcsname{3.82}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.arm.sd\endcsname{1.03}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.arm.share\endcsname{0.51}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.arms\endcsname{nnU-Net default, HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented), ResEnc+context, HyReX+context, ConvNeXt-k3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.case.sd\endcsname{13.07}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.case.share\endcsname{82.14}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.excl\endcsname{none}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.narm\endcsname{7}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.nboot\endcsname{2000}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ncase\endcsname{98}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.negnames\endcsname{none}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.nexcl\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.nfresh_subsets\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.nneg\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.nseed\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio\endcsname{0.28}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_arm\endcsname{6.10}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_arm_ci\endcsname{printed}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_arm_fresh\endcsname{6.03}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_arm_fresh_ndef\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_arm_hi\endcsname{20.73}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_arm_lo\endcsname{0.49}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_arm_ndef\endcsname{1975}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_arm_sd\endcsname{2.47}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_arm_sd_hi\endcsname{4.55}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_arm_sd_lo\endcsname{0.70}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_arm_support\endcsname{98.8}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_arm_txt\endcsname{6.10 [0.49, 20.73]}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_ci\endcsname{printed}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_fresh\endcsname{0.35}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_fresh_ndef\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_hi\endcsname{0.53}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_lo\endcsname{0.10}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_ndef\endcsname{2000}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_sd\endcsname{0.53}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_sd_hi\endcsname{0.73}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_sd_lo\endcsname{0.32}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_support\endcsname{100.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.ratio_txt\endcsname{0.28 [0.10, 0.53]}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.resid.sd\endcsname{5.29}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.resid.share\endcsname{13.45}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.seed.sd\endcsname{0.42}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.mean.seed.share\endcsname{0.08}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ak.sd\endcsname{4.39}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ak.share\endcsname{2.96}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.arm.sd\endcsname{1.48}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.arm.share\endcsname{0.34}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.arms\endcsname{nnU-Net default, HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented), ResEnc+context, HyReX+context, ConvNeXt-k3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.case.sd\endcsname{23.63}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.case.share\endcsname{85.83}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.excl\endcsname{none}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.narm\endcsname{7}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.nboot\endcsname{2000}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ncase\endcsname{98}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.negnames\endcsname{none}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.nexcl\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.nfresh_subsets\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.nneg\endcsname{0}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.nseed\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio\endcsname{0.27}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_arm\endcsname{6.13}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_arm_ci\endcsname{printed}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_arm_fresh\endcsname{7.21}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_arm_fresh_ndef\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_arm_hi\endcsname{19.89}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_arm_lo\endcsname{0.31}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_arm_ndef\endcsname{1972}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_arm_sd\endcsname{2.48}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_arm_sd_hi\endcsname{4.46}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_arm_sd_lo\endcsname{0.56}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_arm_support\endcsname{98.6}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_arm_txt\endcsname{6.13 [0.31, 19.89]}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_ci\endcsname{printed}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_fresh\endcsname{0.48}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_fresh_ndef\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_hi\endcsname{0.49}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_lo\endcsname{0.13}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_ndef\endcsname{2000}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_sd\endcsname{0.52}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_sd_hi\endcsname{0.70}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_sd_lo\endcsname{0.36}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_support\endcsname{100.0}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.ratio_txt\endcsname{0.27 [0.13, 0.49]}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.resid.sd\endcsname{8.39}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.resid.share\endcsname{10.82}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.seed.sd\endcsname{0.60}
\expandafter\gdef\csname R@an.case_seedmean.kits.var.tumor.seed.share\endcsname{0.06}
\expandafter\gdef\csname R@an.case_seedmean.kits.w1c.clause\endcsname{has its fresh pair, seeds~1 and~2 finished, with a fresh-mean delta of \ensuremath{+1.067}\,pp against the same frozen 3-run pool (\ensuremath{+0.823}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.case_seedmean.kits.w1c.delta_fresh\endcsname{\ensuremath{+1.067}}
\expandafter\gdef\csname R@an.case_seedmean.kits.w1c.delta_fresh_six\endcsname{\ensuremath{+0.823}}
\expandafter\gdef\csname R@an.case_seedmean.kits.w1c.delta_s0\endcsname{\ensuremath{+2.636}}
\expandafter\gdef\csname R@an.case_seedmean.kits.w1c.delta_s0_six\endcsname{\ensuremath{+2.392}}
\expandafter\gdef\csname R@an.case_seedmean.kits.w1c.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.case_seedmean.kits.w1c.nseed\endcsname{3}
\expandafter\gdef\csname R@an.case_seedmean.kits.w1c.state\endcsname{fresh pair}
\expandafter\gdef\csname R@an.case_seedmean.pairfloor\endcsname{0.50}
\expandafter\gdef\csname R@an.case_seedmean.primarybar\endcsname{0.35}
\expandafter\gdef\csname R@an.case_seedmean.topcap\endcsname{999}
\expandafter\gdef\csname R@an.case_seedmean.topk\endcsname{5}
\expandafter\gdef\csname R@an.case_seedmean.trimpct\endcsname{10}
\expandafter\gdef\csname R@an.compiled_efficiency.acdc.D2.ms\endcsname{89.4}
\expandafter\gdef\csname R@an.compiled_efficiency.acdc.change\endcsname{\ensuremath{-17.8}}
\expandafter\gdef\csname R@an.compiled_efficiency.acdc.default.ms\endcsname{108.7}
\expandafter\gdef\csname R@an.compiled_efficiency.acdc.dice.state\endcsname{not registered}
\expandafter\gdef\csname R@an.compiled_efficiency.acdc.params.d2\endcsname{25.28}
\expandafter\gdef\csname R@an.compiled_efficiency.acdc.params.default\endcsname{30.38}
\expandafter\gdef\csname R@an.compiled_efficiency.acdc.params.pct\endcsname{16.8}
\expandafter\gdef\csname R@an.compiled_efficiency.acdc.params.ratio\endcsname{0.832}
\expandafter\gdef\csname R@an.compiled_efficiency.acdc.ratio\endcsname{0.822}
\expandafter\gdef\csname R@an.compiled_efficiency.acdc.reduction\endcsname{17.8}
\expandafter\gdef\csname R@an.compiled_efficiency.acdc.saved.ms\endcsname{19.3}
\expandafter\gdef\csname R@an.compiled_efficiency.acdc.scope\endcsname{same-job isolated pair}
\expandafter\gdef\csname R@an.compiled_efficiency.amos.D2.ms\endcsname{84.5}
\expandafter\gdef\csname R@an.compiled_efficiency.amos.change\endcsname{\ensuremath{-16.1}}
\expandafter\gdef\csname R@an.compiled_efficiency.amos.default.ms\endcsname{100.7}
\expandafter\gdef\csname R@an.compiled_efficiency.amos.dice.state\endcsname{read}
\expandafter\gdef\csname R@an.compiled_efficiency.amos.params.d2\endcsname{26.03}
\expandafter\gdef\csname R@an.compiled_efficiency.amos.params.default\endcsname{31.12}
\expandafter\gdef\csname R@an.compiled_efficiency.amos.params.pct\endcsname{16.4}
\expandafter\gdef\csname R@an.compiled_efficiency.amos.params.ratio\endcsname{0.836}
\expandafter\gdef\csname R@an.compiled_efficiency.amos.ratio\endcsname{0.839}
\expandafter\gdef\csname R@an.compiled_efficiency.amos.reduction\endcsname{16.1}
\expandafter\gdef\csname R@an.compiled_efficiency.amos.saved.ms\endcsname{16.2}
\expandafter\gdef\csname R@an.compiled_efficiency.amos.scope\endcsname{separate profile jobs}
\expandafter\gdef\csname R@an.compiled_efficiency.change.max\endcsname{\ensuremath{-16.1}}
\expandafter\gdef\csname R@an.compiled_efficiency.change.min\endcsname{\ensuremath{-18.4}}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.amos.alt.contemporaneous\endcsname{\ensuremath{-0.373}}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.amos.alt.contemporaneous.name\endcsname{the contemporaneous default runs}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.amos.alt.uncompiled\endcsname{\ensuremath{-0.391}}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.amos.alt.uncompiled.name\endcsname{its uncompiled sub-pool}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.amos.cv.nqueued\endcsname{12}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.amos.cv.nruns\endcsname{4}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.amos.delta\endcsname{\ensuremath{-0.362}}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.amos.dir\endcsname{down}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.amos.fresh.delta\endcsname{\pend}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.amos.fresh.state\endcsname{none}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.amos.refs.pending\endcsname{none}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.cv.deviation\endcsname{LeanDec's cross-validation is run under a registered deviation from Addendum P6 (Addendum AB, Addendum AA and Addendum AJ): the P6 condition failed on AMOS22 and the runs were queued after that was known, so every reading of them is reported against both margins}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.cv.ncovered\endcsname{24}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.cv.nqueued\endcsname{24}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.cv.nregistered\endcsname{8}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.cv.nruns\endcsname{8}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.cv.nuncovered\endcsname{0}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.cv.registration\endcsname{Addendum AB, Addendum AA and Addendum AJ}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.cv.state\endcsname{deviation}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.kits.alt.union\endcsname{\ensuremath{+2.112}}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.kits.alt.union.name\endcsname{the six-run reference}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.kits.cv.nqueued\endcsname{12}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.kits.cv.nruns\endcsname{4}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.kits.delta\endcsname{\ensuremath{+2.355}}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.kits.dir\endcsname{up}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.kits.fresh.delta\endcsname{\ensuremath{+1.892}}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.kits.fresh.state\endcsname{complete}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.kits.nseed\endcsname{3}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.kits.refs.pending\endcsname{none}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.p6.below\endcsname{AMOS22}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.p6.fold\endcsname{0}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.p6.line\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.p6.pending\endcsname{none}
\expandafter\gdef\csname R@an.compiled_efficiency.d2.p6.state\endcsname{does not fire}
\expandafter\gdef\csname R@an.compiled_efficiency.dice.notregistered\endcsname{ACDC}
\expandafter\gdef\csname R@an.compiled_efficiency.dice.npending\endcsname{0}
\expandafter\gdef\csname R@an.compiled_efficiency.dice.nread\endcsname{2}
\expandafter\gdef\csname R@an.compiled_efficiency.dice.nregistered\endcsname{2}
\expandafter\gdef\csname R@an.compiled_efficiency.dice.pending\endcsname{none}
\expandafter\gdef\csname R@an.compiled_efficiency.dice.registered\endcsname{AMOS22, KiTS23}
\expandafter\gdef\csname R@an.compiled_efficiency.isolated.ds\endcsname{ACDC, KiTS23}
\expandafter\gdef\csname R@an.compiled_efficiency.isolated.interpretation\endcsname{isolated outcomes; no causal conclusion about previous cross-shape failures}
\expandafter\gdef\csname R@an.compiled_efficiency.isolated.separate\endcsname{AMOS22}
\expandafter\gdef\csname R@an.compiled_efficiency.kits.D2.ms\endcsname{72.1}
\expandafter\gdef\csname R@an.compiled_efficiency.kits.change\endcsname{\ensuremath{-18.4}}
\expandafter\gdef\csname R@an.compiled_efficiency.kits.default.ms\endcsname{88.4}
\expandafter\gdef\csname R@an.compiled_efficiency.kits.dice.state\endcsname{read}
\expandafter\gdef\csname R@an.compiled_efficiency.kits.params.d2\endcsname{26.08}
\expandafter\gdef\csname R@an.compiled_efficiency.kits.params.default\endcsname{31.20}
\expandafter\gdef\csname R@an.compiled_efficiency.kits.params.pct\endcsname{16.4}
\expandafter\gdef\csname R@an.compiled_efficiency.kits.params.ratio\endcsname{0.836}
\expandafter\gdef\csname R@an.compiled_efficiency.kits.ratio\endcsname{0.816}
\expandafter\gdef\csname R@an.compiled_efficiency.kits.reduction\endcsname{18.4}
\expandafter\gdef\csname R@an.compiled_efficiency.kits.saved.ms\endcsname{16.3}
\expandafter\gdef\csname R@an.compiled_efficiency.kits.scope\endcsname{same-job isolated pair}
\expandafter\gdef\csname R@an.compiled_efficiency.nfaster\endcsname{3}
\expandafter\gdef\csname R@an.compiled_efficiency.nplans\endcsname{3}
\expandafter\gdef\csname R@an.compiled_efficiency.params.pct.max\endcsname{16.8}
\expandafter\gdef\csname R@an.compiled_efficiency.params.pct.min\endcsname{16.4}
\expandafter\gdef\csname R@an.compiled_efficiency.reduction.max\endcsname{18.4}
\expandafter\gdef\csname R@an.compiled_efficiency.reduction.min\endcsname{16.1}
\expandafter\gdef\csname R@an.compiled_efficiency.saved.max.ms\endcsname{19.3}
\expandafter\gdef\csname R@an.compiled_efficiency.saved.min.ms\endcsname{16.2}
\expandafter\gdef\csname R@an.compiled_efficiency.sent.accuracy\endcsname{At seed 0 its Dice is 0.362\,pp below the frozen default pool (0.391\,pp below its uncompiled sub-pool; 0.373\,pp below the contemporaneous default runs) on AMOS22 (one finished run) and 2.355\,pp above the frozen default pool (2.112\,pp above the six-run reference) on KiTS23 (three finished runs); the mean of its fresh seeds 1 and 2 on KiTS23 is 1.892\,pp above the frozen default pool (1.648\,pp above the six-run reference)}
\expandafter\gdef\csname R@an.compiled_efficiency.sent.caption_alt\endcsname{against the registered alternative references the same readings are \ensuremath{-0.391}\,pp on AMOS22 (its uncompiled sub-pool), \ensuremath{-0.373}\,pp on AMOS22 (the contemporaneous default runs) and \ensuremath{+2.112}\,pp on KiTS23 (the six-run reference)}
\expandafter\gdef\csname R@an.compiled_efficiency.sent.caption_dice\endcsname{its seed-0 Dice reads \ensuremath{-0.362}\,pp on AMOS22 and \ensuremath{+2.355}\,pp on KiTS23 against the frozen default pools (\ensuremath{-0.391}\,pp against its uncompiled sub-pool on AMOS22, \ensuremath{-0.373}\,pp against the contemporaneous default runs on AMOS22 and \ensuremath{+2.112}\,pp against the six-run reference on KiTS23)}
\expandafter\gdef\csname R@an.compiled_efficiency.sent.cost\endcsname{With compilation on and the plan fixed, LeanDec's synthetic training step is 16.1 to 18.4\,\% shorter than the default's on all three plans, and its parameter count is 16.4 to 16.8\,\% lower}
\expandafter\gdef\csname R@an.compiled_efficiency.sent.direction\endcsname{at seed 0, down on AMOS22 and up on KiTS23; on the mean of fresh seeds 1 and 2, up on KiTS23}
\expandafter\gdef\csname R@an.compiled_efficiency.sent.p6\endcsname{Addendum P6 queues LeanDec's cross-validation only when its seed-0 Dice is at most 0.15\,pp below the frozen pool on every co-primary; it falls past that line on AMOS22, so Addendum P6 owed it no cross-validation; the cross-validation was nevertheless run under a registered deviation (Addendum AB, Addendum AA and Addendum AJ), by a decision of the lead taken after that failure was known, and LeanDec's cross-validation accuracy is reported against both margins -- Addendum P6's 0.15\,pp line and the 0.50\,pp margin of Addendum AA target T2 (\R{an.cv.p6.margin.p6.clause}; \R{an.cv.p6.margin.t2.clause})}
\expandafter\gdef\csname R@an.compiled_efficiency.sent.tradeoff\endcsname{With compilation on and the plan fixed, LeanDec's synthetic training step is 16.1 to 18.4\,\% shorter than the default's on all three plans, and its parameter count is 16.4 to 16.8\,\% lower. At seed 0 its Dice is 0.362\,pp below the frozen default pool (0.391\,pp below its uncompiled sub-pool; 0.373\,pp below the contemporaneous default runs) on AMOS22 (one finished run) and 2.355\,pp above the frozen default pool (2.112\,pp above the six-run reference) on KiTS23 (three finished runs); the mean of its fresh seeds 1 and 2 on KiTS23 is 1.892\,pp above the frozen default pool (1.648\,pp above the six-run reference). Addendum P6 queues LeanDec's cross-validation only when its seed-0 Dice is at most 0.15\,pp below the frozen pool on every co-primary; it falls past that line on AMOS22, so Addendum P6 owed it no cross-validation; the cross-validation was nevertheless run under a registered deviation (Addendum AB, Addendum AA and Addendum AJ), by a decision of the lead taken after that failure was known, and LeanDec's cross-validation accuracy is reported against both margins -- Addendum P6's 0.15\,pp line and the 0.50\,pp margin of Addendum AA target T2 (\R{an.cv.p6.margin.p6.clause}; \R{an.cv.p6.margin.t2.clause}).}
\expandafter\gdef\csname R@an.compiled_efficiency.stepsdice.state\endcsname{built by the manuscript}
\expandafter\gdef\csname R@an.convergence.above.acdc.100\endcsname{3}
\expandafter\gdef\csname R@an.convergence.above.acdc.1000\endcsname{5}
\expandafter\gdef\csname R@an.convergence.above.acdc.250\endcsname{3}
\expandafter\gdef\csname R@an.convergence.above.acdc.500\endcsname{4}
\expandafter\gdef\csname R@an.convergence.above.acdc.750\endcsname{5}
\expandafter\gdef\csname R@an.convergence.above.amos.100\endcsname{6}
\expandafter\gdef\csname R@an.convergence.above.amos.1000\endcsname{5}
\expandafter\gdef\csname R@an.convergence.above.amos.250\endcsname{4}
\expandafter\gdef\csname R@an.convergence.above.amos.500\endcsname{4}
\expandafter\gdef\csname R@an.convergence.above.amos.750\endcsname{5}
\expandafter\gdef\csname R@an.convergence.above.chance.acdc\endcsname{0.9}
\expandafter\gdef\csname R@an.convergence.above.chance.amos\endcsname{0.9}
\expandafter\gdef\csname R@an.convergence.above.chance.kits\endcsname{1.5}
\expandafter\gdef\csname R@an.convergence.above.kits.100\endcsname{5}
\expandafter\gdef\csname R@an.convergence.above.kits.1000\endcsname{5}
\expandafter\gdef\csname R@an.convergence.above.kits.250\endcsname{1}
\expandafter\gdef\csname R@an.convergence.above.kits.500\endcsname{3}
\expandafter\gdef\csname R@an.convergence.above.kits.750\endcsname{0}
\expandafter\gdef\csname R@an.convergence.armsd.acdc.100\endcsname{0.22}
\expandafter\gdef\csname R@an.convergence.armsd.acdc.1000\endcsname{0.17}
\expandafter\gdef\csname R@an.convergence.armsd.acdc.250\endcsname{0.14}
\expandafter\gdef\csname R@an.convergence.armsd.acdc.500\endcsname{0.16}
\expandafter\gdef\csname R@an.convergence.armsd.acdc.750\endcsname{0.11}
\expandafter\gdef\csname R@an.convergence.armsd.amos.100\endcsname{0.87}
\expandafter\gdef\csname R@an.convergence.armsd.amos.1000\endcsname{0.33}
\expandafter\gdef\csname R@an.convergence.armsd.amos.250\endcsname{0.41}
\expandafter\gdef\csname R@an.convergence.armsd.amos.500\endcsname{0.56}
\expandafter\gdef\csname R@an.convergence.armsd.amos.750\endcsname{0.51}
\expandafter\gdef\csname R@an.convergence.armsd.kits.100\endcsname{2.26}
\expandafter\gdef\csname R@an.convergence.armsd.kits.1000\endcsname{0.36}
\expandafter\gdef\csname R@an.convergence.armsd.kits.250\endcsname{1.02}
\expandafter\gdef\csname R@an.convergence.armsd.kits.500\endcsname{1.75}
\expandafter\gdef\csname R@an.convergence.armsd.kits.750\endcsname{0.49}
\expandafter\gdef\csname R@an.convergence.auc.acdc.L1\endcsname{91.79}
\expandafter\gdef\csname R@an.convergence.auc.acdc.L1b\endcsname{91.94}
\expandafter\gdef\csname R@an.convergence.auc.acdc.L2\endcsname{91.29}
\expandafter\gdef\csname R@an.convergence.auc.acdc.L3\endcsname{91.87}
\expandafter\gdef\csname R@an.convergence.auc.acdc.L4\endcsname{91.73}
\expandafter\gdef\csname R@an.convergence.auc.acdc.L6\endcsname{91.70}
\expandafter\gdef\csname R@an.convergence.auc.acdc.designs.mean\endcsname{91.72}
\expandafter\gdef\csname R@an.convergence.auc.acdc.designs.sd\endcsname{0.23}
\expandafter\gdef\csname R@an.convergence.auc.acdc.diff\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.convergence.auc.acdc.earlier\endcsname{1}
\expandafter\gdef\csname R@an.convergence.auc.acdc.inside\endcsname{3}
\expandafter\gdef\csname R@an.convergence.auc.acdc.later\endcsname{2}
\expandafter\gdef\csname R@an.convergence.auc.acdc.pool.max\endcsname{91.81}
\expandafter\gdef\csname R@an.convergence.auc.acdc.pool.mean\endcsname{91.60}
\expandafter\gdef\csname R@an.convergence.auc.acdc.pool.min\endcsname{91.40}
\expandafter\gdef\csname R@an.convergence.auc.acdc.pool.sd\endcsname{0.16}
\expandafter\gdef\csname R@an.convergence.auc.acdc.se\endcsname{0.11}
\expandafter\gdef\csname R@an.convergence.auc.acdc.z\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.convergence.auc.amos.L1\endcsname{79.77}
\expandafter\gdef\csname R@an.convergence.auc.amos.L1b\endcsname{78.80}
\expandafter\gdef\csname R@an.convergence.auc.amos.L2\endcsname{79.06}
\expandafter\gdef\csname R@an.convergence.auc.amos.L3\endcsname{79.57}
\expandafter\gdef\csname R@an.convergence.auc.amos.L4\endcsname{78.94}
\expandafter\gdef\csname R@an.convergence.auc.amos.L6\endcsname{79.30}
\expandafter\gdef\csname R@an.convergence.auc.amos.W1\endcsname{78.39}
\expandafter\gdef\csname R@an.convergence.auc.amos.W1c\endcsname{78.64}
\expandafter\gdef\csname R@an.convergence.auc.amos.W2\endcsname{78.23}
\expandafter\gdef\csname R@an.convergence.auc.amos.W3\endcsname{77.70}
\expandafter\gdef\csname R@an.convergence.auc.amos.W3c\endcsname{77.14}
\expandafter\gdef\csname R@an.convergence.auc.amos.W4\endcsname{79.51}
\expandafter\gdef\csname R@an.convergence.auc.amos.W5\endcsname{79.25}
\expandafter\gdef\csname R@an.convergence.auc.amos.designs.mean\endcsname{79.24}
\expandafter\gdef\csname R@an.convergence.auc.amos.designs.sd\endcsname{0.37}
\expandafter\gdef\csname R@an.convergence.auc.amos.diff\endcsname{\ensuremath{+1.52}}
\expandafter\gdef\csname R@an.convergence.auc.amos.earlier\endcsname{0}
\expandafter\gdef\csname R@an.convergence.auc.amos.inside\endcsname{0}
\expandafter\gdef\csname R@an.convergence.auc.amos.later\endcsname{6}
\expandafter\gdef\csname R@an.convergence.auc.amos.pool.max\endcsname{78.21}
\expandafter\gdef\csname R@an.convergence.auc.amos.pool.mean\endcsname{77.72}
\expandafter\gdef\csname R@an.convergence.auc.amos.pool.min\endcsname{77.41}
\expandafter\gdef\csname R@an.convergence.auc.amos.pool.sd\endcsname{0.29}
\expandafter\gdef\csname R@an.convergence.auc.amos.se\endcsname{0.19}
\expandafter\gdef\csname R@an.convergence.auc.amos.z\endcsname{\ensuremath{+7.9}}
\expandafter\gdef\csname R@an.convergence.auc.kits.L1\endcsname{87.36}
\expandafter\gdef\csname R@an.convergence.auc.kits.L1b\endcsname{86.69}
\expandafter\gdef\csname R@an.convergence.auc.kits.L2\endcsname{85.26}
\expandafter\gdef\csname R@an.convergence.auc.kits.L3\endcsname{85.86}
\expandafter\gdef\csname R@an.convergence.auc.kits.L4\endcsname{86.47}
\expandafter\gdef\csname R@an.convergence.auc.kits.L6\endcsname{86.42}
\expandafter\gdef\csname R@an.convergence.auc.kits.W1c\endcsname{85.96}
\expandafter\gdef\csname R@an.convergence.auc.kits.designs.mean\endcsname{86.35}
\expandafter\gdef\csname R@an.convergence.auc.kits.designs.sd\endcsname{0.72}
\expandafter\gdef\csname R@an.convergence.auc.kits.diff\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.convergence.auc.kits.earlier\endcsname{1}
\expandafter\gdef\csname R@an.convergence.auc.kits.inside\endcsname{1}
\expandafter\gdef\csname R@an.convergence.auc.kits.later\endcsname{4}
\expandafter\gdef\csname R@an.convergence.auc.kits.pool.max\endcsname{85.89}
\expandafter\gdef\csname R@an.convergence.auc.kits.pool.mean\endcsname{85.71}
\expandafter\gdef\csname R@an.convergence.auc.kits.pool.min\endcsname{85.47}
\expandafter\gdef\csname R@an.convergence.auc.kits.pool.sd\endcsname{0.21}
\expandafter\gdef\csname R@an.convergence.auc.kits.se\endcsname{0.32}
\expandafter\gdef\csname R@an.convergence.auc.kits.z\endcsname{\ensuremath{+2.0}}
\expandafter\gdef\csname R@an.convergence.aucr.acdc.L1\endcsname{0.9903}
\expandafter\gdef\csname R@an.convergence.aucr.acdc.L1b\endcsname{0.9907}
\expandafter\gdef\csname R@an.convergence.aucr.acdc.L2\endcsname{0.9875}
\expandafter\gdef\csname R@an.convergence.aucr.acdc.L3\endcsname{0.9883}
\expandafter\gdef\csname R@an.convergence.aucr.acdc.L4\endcsname{0.9895}
\expandafter\gdef\csname R@an.convergence.aucr.acdc.L6\endcsname{0.9891}
\expandafter\gdef\csname R@an.convergence.aucr.acdc.designs.mean\endcsname{0.9892}
\expandafter\gdef\csname R@an.convergence.aucr.acdc.designs.sd\endcsname{0.0012}
\expandafter\gdef\csname R@an.convergence.aucr.acdc.diff\endcsname{\ensuremath{-0.0014}}
\expandafter\gdef\csname R@an.convergence.aucr.acdc.earlier\endcsname{1}
\expandafter\gdef\csname R@an.convergence.aucr.acdc.inside\endcsname{5}
\expandafter\gdef\csname R@an.convergence.aucr.acdc.later\endcsname{0}
\expandafter\gdef\csname R@an.convergence.aucr.acdc.pool.max\endcsname{0.9934}
\expandafter\gdef\csname R@an.convergence.aucr.acdc.pool.mean\endcsname{0.9907}
\expandafter\gdef\csname R@an.convergence.aucr.acdc.pool.min\endcsname{0.9880}
\expandafter\gdef\csname R@an.convergence.aucr.acdc.pool.sd\endcsname{0.0020}
\expandafter\gdef\csname R@an.convergence.aucr.acdc.se\endcsname{0.0010}
\expandafter\gdef\csname R@an.convergence.aucr.acdc.z\endcsname{\ensuremath{-1.5}}
\expandafter\gdef\csname R@an.convergence.aucr.amos.L1\endcsname{0.9012}
\expandafter\gdef\csname R@an.convergence.aucr.amos.L1b\endcsname{0.8877}
\expandafter\gdef\csname R@an.convergence.aucr.amos.L2\endcsname{0.8979}
\expandafter\gdef\csname R@an.convergence.aucr.amos.L3\endcsname{0.8972}
\expandafter\gdef\csname R@an.convergence.aucr.amos.L4\endcsname{0.8884}
\expandafter\gdef\csname R@an.convergence.aucr.amos.L6\endcsname{0.8991}
\expandafter\gdef\csname R@an.convergence.aucr.amos.W1\endcsname{0.8962}
\expandafter\gdef\csname R@an.convergence.aucr.amos.W1c\endcsname{0.8946}
\expandafter\gdef\csname R@an.convergence.aucr.amos.W2\endcsname{0.8864}
\expandafter\gdef\csname R@an.convergence.aucr.amos.W3\endcsname{0.8790}
\expandafter\gdef\csname R@an.convergence.aucr.amos.W3c\endcsname{0.8754}
\expandafter\gdef\csname R@an.convergence.aucr.amos.W4\endcsname{0.8998}
\expandafter\gdef\csname R@an.convergence.aucr.amos.W5\endcsname{0.8979}
\expandafter\gdef\csname R@an.convergence.aucr.amos.designs.mean\endcsname{0.8952}
\expandafter\gdef\csname R@an.convergence.aucr.amos.designs.sd\endcsname{0.0057}
\expandafter\gdef\csname R@an.convergence.aucr.amos.diff\endcsname{\ensuremath{+0.0093}}
\expandafter\gdef\csname R@an.convergence.aucr.amos.earlier\endcsname{0}
\expandafter\gdef\csname R@an.convergence.aucr.amos.inside\endcsname{2}
\expandafter\gdef\csname R@an.convergence.aucr.amos.later\endcsname{4}
\expandafter\gdef\csname R@an.convergence.aucr.amos.pool.max\endcsname{0.8897}
\expandafter\gdef\csname R@an.convergence.aucr.amos.pool.mean\endcsname{0.8859}
\expandafter\gdef\csname R@an.convergence.aucr.amos.pool.min\endcsname{0.8811}
\expandafter\gdef\csname R@an.convergence.aucr.amos.pool.sd\endcsname{0.0031}
\expandafter\gdef\csname R@an.convergence.aucr.amos.se\endcsname{0.0027}
\expandafter\gdef\csname R@an.convergence.aucr.amos.z\endcsname{\ensuremath{+3.5}}
\expandafter\gdef\csname R@an.convergence.aucr.kits.L1\endcsname{0.9360}
\expandafter\gdef\csname R@an.convergence.aucr.kits.L1b\endcsname{0.9232}
\expandafter\gdef\csname R@an.convergence.aucr.kits.L2\endcsname{0.9185}
\expandafter\gdef\csname R@an.convergence.aucr.kits.L3\endcsname{0.9183}
\expandafter\gdef\csname R@an.convergence.aucr.kits.L4\endcsname{0.9278}
\expandafter\gdef\csname R@an.convergence.aucr.kits.L6\endcsname{0.9250}
\expandafter\gdef\csname R@an.convergence.aucr.kits.W1c\endcsname{0.9288}
\expandafter\gdef\csname R@an.convergence.aucr.kits.designs.mean\endcsname{0.9248}
\expandafter\gdef\csname R@an.convergence.aucr.kits.designs.sd\endcsname{0.0066}
\expandafter\gdef\csname R@an.convergence.aucr.kits.diff\endcsname{\ensuremath{+0.0008}}
\expandafter\gdef\csname R@an.convergence.aucr.kits.earlier\endcsname{2}
\expandafter\gdef\csname R@an.convergence.aucr.kits.inside\endcsname{2}
\expandafter\gdef\csname R@an.convergence.aucr.kits.later\endcsname{2}
\expandafter\gdef\csname R@an.convergence.aucr.kits.pool.max\endcsname{0.9262}
\expandafter\gdef\csname R@an.convergence.aucr.kits.pool.mean\endcsname{0.9240}
\expandafter\gdef\csname R@an.convergence.aucr.kits.pool.min\endcsname{0.9223}
\expandafter\gdef\csname R@an.convergence.aucr.kits.pool.sd\endcsname{0.0020}
\expandafter\gdef\csname R@an.convergence.aucr.kits.se\endcsname{0.0029}
\expandafter\gdef\csname R@an.convergence.aucr.kits.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.convergence.betweenarm.acdc.max\endcsname{0.31}
\expandafter\gdef\csname R@an.convergence.betweenarm.acdc.median\endcsname{0.05}
\expandafter\gdef\csname R@an.convergence.betweenarm.acdc.nbelow\endcsname{15}
\expandafter\gdef\csname R@an.convergence.betweenarm.acdc.npairs\endcsname{15}
\expandafter\gdef\csname R@an.convergence.betweenarm.amos.max\endcsname{1.26}
\expandafter\gdef\csname R@an.convergence.betweenarm.amos.median\endcsname{0.23}
\expandafter\gdef\csname R@an.convergence.betweenarm.amos.nbelow\endcsname{75}
\expandafter\gdef\csname R@an.convergence.betweenarm.amos.npairs\endcsname{78}
\expandafter\gdef\csname R@an.convergence.betweenarm.kits.max\endcsname{0.91}
\expandafter\gdef\csname R@an.convergence.betweenarm.kits.median\endcsname{0.35}
\expandafter\gdef\csname R@an.convergence.betweenarm.kits.nbelow\endcsname{21}
\expandafter\gdef\csname R@an.convergence.betweenarm.kits.npairs\endcsname{21}
\expandafter\gdef\csname R@an.convergence.chance.acdc\endcsname{98.3}
\expandafter\gdef\csname R@an.convergence.chance.amos\endcsname{98.3}
\expandafter\gdef\csname R@an.convergence.chance.kits\endcsname{98.3}
\expandafter\gdef\csname R@an.convergence.conc.acdc.n\endcsname{901}
\expandafter\gdef\csname R@an.convergence.conc.acdc.nabove\endcsname{826}
\expandafter\gdef\csname R@an.convergence.conc.acdc.nbelow\endcsname{0}
\expandafter\gdef\csname R@an.convergence.conc.acdc.phrase\endcsname{stays at or above the chance level}
\expandafter\gdef\csname R@an.convergence.conc.amos.n\endcsname{901}
\expandafter\gdef\csname R@an.convergence.conc.amos.nabove\endcsname{566}
\expandafter\gdef\csname R@an.convergence.conc.amos.nbelow\endcsname{335}
\expandafter\gdef\csname R@an.convergence.conc.amos.phrase\endcsname{crosses the chance level}
\expandafter\gdef\csname R@an.convergence.conc.kits.n\endcsname{901}
\expandafter\gdef\csname R@an.convergence.conc.kits.nabove\endcsname{721}
\expandafter\gdef\csname R@an.convergence.conc.kits.nbelow\endcsname{45}
\expandafter\gdef\csname R@an.convergence.conc.kits.phrase\endcsname{crosses the chance level}
\expandafter\gdef\csname R@an.convergence.conchead\endcsname{crosses the chance level on AMOS22 and KiTS23 and stays at or above the chance level on ACDC}
\expandafter\gdef\csname R@an.convergence.curves.e0\endcsname{100}
\expandafter\gdef\csname R@an.convergence.curves.zoom\endcsname{60}
\expandafter\gdef\csname R@an.convergence.defgap90.acdc\endcsname{0}
\expandafter\gdef\csname R@an.convergence.defgap90.amos\endcsname{43}
\expandafter\gdef\csname R@an.convergence.defgap90.kits\endcsname{124}
\expandafter\gdef\csname R@an.convergence.defgap95.acdc\endcsname{0}
\expandafter\gdef\csname R@an.convergence.defgap95.amos\endcsname{93}
\expandafter\gdef\csname R@an.convergence.defgap95.kits\endcsname{252}
\expandafter\gdef\csname R@an.convergence.defgap98.acdc\endcsname{0}
\expandafter\gdef\csname R@an.convergence.defgap98.amos\endcsname{55}
\expandafter\gdef\csname R@an.convergence.defgap98.kits\endcsname{129}
\expandafter\gdef\csname R@an.convergence.dlead.acdc\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.convergence.dlead.amos\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.convergence.dlead.kits\endcsname{\ensuremath{+2.05}}
\expandafter\gdef\csname R@an.convergence.e90.acdc.L1\endcsname{24}
\expandafter\gdef\csname R@an.convergence.e90.acdc.L1b\endcsname{23}
\expandafter\gdef\csname R@an.convergence.e90.acdc.L2\endcsname{26}
\expandafter\gdef\csname R@an.convergence.e90.acdc.L3\endcsname{23}
\expandafter\gdef\csname R@an.convergence.e90.acdc.L4\endcsname{24}
\expandafter\gdef\csname R@an.convergence.e90.acdc.L6\endcsname{24}
\expandafter\gdef\csname R@an.convergence.e90.acdc.designs.max\endcsname{26}
\expandafter\gdef\csname R@an.convergence.e90.acdc.designs.mean\endcsname{24.0}
\expandafter\gdef\csname R@an.convergence.e90.acdc.designs.median\endcsname{24.0}
\expandafter\gdef\csname R@an.convergence.e90.acdc.designs.min\endcsname{23}
\expandafter\gdef\csname R@an.convergence.e90.acdc.designs.sd\endcsname{1.1}
\expandafter\gdef\csname R@an.convergence.e90.acdc.diff\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.convergence.e90.acdc.earlier\endcsname{0}
\expandafter\gdef\csname R@an.convergence.e90.acdc.inside\endcsname{6}
\expandafter\gdef\csname R@an.convergence.e90.acdc.later\endcsname{0}
\expandafter\gdef\csname R@an.convergence.e90.acdc.pool.max\endcsname{26}
\expandafter\gdef\csname R@an.convergence.e90.acdc.pool.mean\endcsname{22.8}
\expandafter\gdef\csname R@an.convergence.e90.acdc.pool.min\endcsname{19}
\expandafter\gdef\csname R@an.convergence.e90.acdc.pool.sd\endcsname{3.1}
\expandafter\gdef\csname R@an.convergence.e90.acdc.se\endcsname{1.3}
\expandafter\gdef\csname R@an.convergence.e90.acdc.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.convergence.e90.amos.L1\endcsname{183}
\expandafter\gdef\csname R@an.convergence.e90.amos.L1b\endcsname{239}
\expandafter\gdef\csname R@an.convergence.e90.amos.L2\endcsname{224}
\expandafter\gdef\csname R@an.convergence.e90.amos.L3\endcsname{207}
\expandafter\gdef\csname R@an.convergence.e90.amos.L4\endcsname{223}
\expandafter\gdef\csname R@an.convergence.e90.amos.L6\endcsname{200}
\expandafter\gdef\csname R@an.convergence.e90.amos.W1\endcsname{210}
\expandafter\gdef\csname R@an.convergence.e90.amos.W1c\endcsname{236}
\expandafter\gdef\csname R@an.convergence.e90.amos.W2\endcsname{225}
\expandafter\gdef\csname R@an.convergence.e90.amos.W3\endcsname{268}
\expandafter\gdef\csname R@an.convergence.e90.amos.W3c\endcsname{304}
\expandafter\gdef\csname R@an.convergence.e90.amos.W4\endcsname{198}
\expandafter\gdef\csname R@an.convergence.e90.amos.W5\endcsname{204}
\expandafter\gdef\csname R@an.convergence.e90.amos.designs.max\endcsname{239}
\expandafter\gdef\csname R@an.convergence.e90.amos.designs.mean\endcsname{212.7}
\expandafter\gdef\csname R@an.convergence.e90.amos.designs.median\endcsname{215.0}
\expandafter\gdef\csname R@an.convergence.e90.amos.designs.min\endcsname{183}
\expandafter\gdef\csname R@an.convergence.e90.amos.designs.sd\endcsname{20.0}
\expandafter\gdef\csname R@an.convergence.e90.amos.diff\endcsname{\ensuremath{-31.8}}
\expandafter\gdef\csname R@an.convergence.e90.amos.earlier\endcsname{3}
\expandafter\gdef\csname R@an.convergence.e90.amos.inside\endcsname{3}
\expandafter\gdef\csname R@an.convergence.e90.amos.later\endcsname{0}
\expandafter\gdef\csname R@an.convergence.e90.amos.pool.max\endcsname{258}
\expandafter\gdef\csname R@an.convergence.e90.amos.pool.mean\endcsname{244.5}
\expandafter\gdef\csname R@an.convergence.e90.amos.pool.min\endcsname{221}
\expandafter\gdef\csname R@an.convergence.e90.amos.pool.sd\endcsname{15.3}
\expandafter\gdef\csname R@an.convergence.e90.amos.se\endcsname{10.3}
\expandafter\gdef\csname R@an.convergence.e90.amos.z\endcsname{\ensuremath{-3.1}}
\expandafter\gdef\csname R@an.convergence.e90.kits.L1\endcsname{97}
\expandafter\gdef\csname R@an.convergence.e90.kits.L1b\endcsname{98}
\expandafter\gdef\csname R@an.convergence.e90.kits.L2\endcsname{137}
\expandafter\gdef\csname R@an.convergence.e90.kits.L3\endcsname{168}
\expandafter\gdef\csname R@an.convergence.e90.kits.L4\endcsname{102}
\expandafter\gdef\csname R@an.convergence.e90.kits.L6\endcsname{138}
\expandafter\gdef\csname R@an.convergence.e90.kits.W1c\endcsname{164}
\expandafter\gdef\csname R@an.convergence.e90.kits.designs.max\endcsname{168}
\expandafter\gdef\csname R@an.convergence.e90.kits.designs.mean\endcsname{123.3}
\expandafter\gdef\csname R@an.convergence.e90.kits.designs.median\endcsname{119.5}
\expandafter\gdef\csname R@an.convergence.e90.kits.designs.min\endcsname{97}
\expandafter\gdef\csname R@an.convergence.e90.kits.designs.sd\endcsname{28.9}
\expandafter\gdef\csname R@an.convergence.e90.kits.diff\endcsname{\ensuremath{-34.3}}
\expandafter\gdef\csname R@an.convergence.e90.kits.earlier\endcsname{3}
\expandafter\gdef\csname R@an.convergence.e90.kits.inside\endcsname{3}
\expandafter\gdef\csname R@an.convergence.e90.kits.later\endcsname{0}
\expandafter\gdef\csname R@an.convergence.e90.kits.pool.max\endcsname{191}
\expandafter\gdef\csname R@an.convergence.e90.kits.pool.mean\endcsname{157.7}
\expandafter\gdef\csname R@an.convergence.e90.kits.pool.min\endcsname{135}
\expandafter\gdef\csname R@an.convergence.e90.kits.pool.sd\endcsname{29.5}
\expandafter\gdef\csname R@an.convergence.e90.kits.se\endcsname{20.7}
\expandafter\gdef\csname R@an.convergence.e90.kits.z\endcsname{\ensuremath{-1.7}}
\expandafter\gdef\csname R@an.convergence.e95.acdc.L1\endcsname{32}
\expandafter\gdef\csname R@an.convergence.e95.acdc.L1b\endcsname{31}
\expandafter\gdef\csname R@an.convergence.e95.acdc.L2\endcsname{34}
\expandafter\gdef\csname R@an.convergence.e95.acdc.L3\endcsname{32}
\expandafter\gdef\csname R@an.convergence.e95.acdc.L4\endcsname{32}
\expandafter\gdef\csname R@an.convergence.e95.acdc.L6\endcsname{32}
\expandafter\gdef\csname R@an.convergence.e95.acdc.designs.max\endcsname{34}
\expandafter\gdef\csname R@an.convergence.e95.acdc.designs.mean\endcsname{32.2}
\expandafter\gdef\csname R@an.convergence.e95.acdc.designs.median\endcsname{32.0}
\expandafter\gdef\csname R@an.convergence.e95.acdc.designs.min\endcsname{31}
\expandafter\gdef\csname R@an.convergence.e95.acdc.designs.sd\endcsname{1.0}
\expandafter\gdef\csname R@an.convergence.e95.acdc.diff\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.convergence.e95.acdc.earlier\endcsname{0}
\expandafter\gdef\csname R@an.convergence.e95.acdc.inside\endcsname{6}
\expandafter\gdef\csname R@an.convergence.e95.acdc.later\endcsname{0}
\expandafter\gdef\csname R@an.convergence.e95.acdc.pool.max\endcsname{34}
\expandafter\gdef\csname R@an.convergence.e95.acdc.pool.mean\endcsname{31.3}
\expandafter\gdef\csname R@an.convergence.e95.acdc.pool.min\endcsname{28}
\expandafter\gdef\csname R@an.convergence.e95.acdc.pool.sd\endcsname{2.3}
\expandafter\gdef\csname R@an.convergence.e95.acdc.se\endcsname{1.0}
\expandafter\gdef\csname R@an.convergence.e95.acdc.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.convergence.e95.amos.L1\endcsname{476}
\expandafter\gdef\csname R@an.convergence.e95.amos.L1b\endcsname{655}
\expandafter\gdef\csname R@an.convergence.e95.amos.L2\endcsname{504}
\expandafter\gdef\csname R@an.convergence.e95.amos.L3\endcsname{558}
\expandafter\gdef\csname R@an.convergence.e95.amos.L4\endcsname{616}
\expandafter\gdef\csname R@an.convergence.e95.amos.L6\endcsname{488}
\expandafter\gdef\csname R@an.convergence.e95.amos.W1\endcsname{526}
\expandafter\gdef\csname R@an.convergence.e95.amos.W1c\endcsname{590}
\expandafter\gdef\csname R@an.convergence.e95.amos.W2\endcsname{616}
\expandafter\gdef\csname R@an.convergence.e95.amos.W3\endcsname{597}
\expandafter\gdef\csname R@an.convergence.e95.amos.W3c\endcsname{683}
\expandafter\gdef\csname R@an.convergence.e95.amos.W4\endcsname{503}
\expandafter\gdef\csname R@an.convergence.e95.amos.W5\endcsname{494}
\expandafter\gdef\csname R@an.convergence.e95.amos.designs.max\endcsname{655}
\expandafter\gdef\csname R@an.convergence.e95.amos.designs.mean\endcsname{549.5}
\expandafter\gdef\csname R@an.convergence.e95.amos.designs.median\endcsname{531.0}
\expandafter\gdef\csname R@an.convergence.e95.amos.designs.min\endcsname{476}
\expandafter\gdef\csname R@an.convergence.e95.amos.designs.sd\endcsname{73.3}
\expandafter\gdef\csname R@an.convergence.e95.amos.diff\endcsname{\ensuremath{-39.0}}
\expandafter\gdef\csname R@an.convergence.e95.amos.earlier\endcsname{3}
\expandafter\gdef\csname R@an.convergence.e95.amos.inside\endcsname{2}
\expandafter\gdef\csname R@an.convergence.e95.amos.later\endcsname{1}
\expandafter\gdef\csname R@an.convergence.e95.amos.pool.max\endcsname{636}
\expandafter\gdef\csname R@an.convergence.e95.amos.pool.mean\endcsname{588.5}
\expandafter\gdef\csname R@an.convergence.e95.amos.pool.min\endcsname{517}
\expandafter\gdef\csname R@an.convergence.e95.amos.pool.sd\endcsname{45.3}
\expandafter\gdef\csname R@an.convergence.e95.amos.se\endcsname{35.2}
\expandafter\gdef\csname R@an.convergence.e95.amos.z\endcsname{\ensuremath{-1.1}}
\expandafter\gdef\csname R@an.convergence.e95.kits.L1\endcsname{226}
\expandafter\gdef\csname R@an.convergence.e95.kits.L1b\endcsname{476}
\expandafter\gdef\csname R@an.convergence.e95.kits.L2\endcsname{313}
\expandafter\gdef\csname R@an.convergence.e95.kits.L3\endcsname{536}
\expandafter\gdef\csname R@an.convergence.e95.kits.L4\endcsname{311}
\expandafter\gdef\csname R@an.convergence.e95.kits.L6\endcsname{371}
\expandafter\gdef\csname R@an.convergence.e95.kits.W1c\endcsname{323}
\expandafter\gdef\csname R@an.convergence.e95.kits.designs.max\endcsname{536}
\expandafter\gdef\csname R@an.convergence.e95.kits.designs.mean\endcsname{372.2}
\expandafter\gdef\csname R@an.convergence.e95.kits.designs.median\endcsname{342.0}
\expandafter\gdef\csname R@an.convergence.e95.kits.designs.min\endcsname{226}
\expandafter\gdef\csname R@an.convergence.e95.kits.designs.sd\endcsname{115.1}
\expandafter\gdef\csname R@an.convergence.e95.kits.diff\endcsname{\ensuremath{-86.8}}
\expandafter\gdef\csname R@an.convergence.e95.kits.earlier\endcsname{4}
\expandafter\gdef\csname R@an.convergence.e95.kits.inside\endcsname{1}
\expandafter\gdef\csname R@an.convergence.e95.kits.later\endcsname{1}
\expandafter\gdef\csname R@an.convergence.e95.kits.pool.max\endcsname{483}
\expandafter\gdef\csname R@an.convergence.e95.kits.pool.mean\endcsname{459.0}
\expandafter\gdef\csname R@an.convergence.e95.kits.pool.min\endcsname{432}
\expandafter\gdef\csname R@an.convergence.e95.kits.pool.sd\endcsname{25.6}
\expandafter\gdef\csname R@an.convergence.e95.kits.se\endcsname{49.3}
\expandafter\gdef\csname R@an.convergence.e95.kits.z\endcsname{\ensuremath{-1.8}}
\expandafter\gdef\csname R@an.convergence.e98.acdc.L1\endcsname{45}
\expandafter\gdef\csname R@an.convergence.e98.acdc.L1b\endcsname{43}
\expandafter\gdef\csname R@an.convergence.e98.acdc.L2\endcsname{48}
\expandafter\gdef\csname R@an.convergence.e98.acdc.L3\endcsname{45}
\expandafter\gdef\csname R@an.convergence.e98.acdc.L4\endcsname{44}
\expandafter\gdef\csname R@an.convergence.e98.acdc.L6\endcsname{44}
\expandafter\gdef\csname R@an.convergence.e98.acdc.designs.max\endcsname{48}
\expandafter\gdef\csname R@an.convergence.e98.acdc.designs.mean\endcsname{44.8}
\expandafter\gdef\csname R@an.convergence.e98.acdc.designs.median\endcsname{44.5}
\expandafter\gdef\csname R@an.convergence.e98.acdc.designs.min\endcsname{43}
\expandafter\gdef\csname R@an.convergence.e98.acdc.designs.sd\endcsname{1.7}
\expandafter\gdef\csname R@an.convergence.e98.acdc.diff\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.convergence.e98.acdc.earlier\endcsname{0}
\expandafter\gdef\csname R@an.convergence.e98.acdc.inside\endcsname{5}
\expandafter\gdef\csname R@an.convergence.e98.acdc.later\endcsname{1}
\expandafter\gdef\csname R@an.convergence.e98.acdc.pool.max\endcsname{47}
\expandafter\gdef\csname R@an.convergence.e98.acdc.pool.mean\endcsname{44.7}
\expandafter\gdef\csname R@an.convergence.e98.acdc.pool.min\endcsname{42}
\expandafter\gdef\csname R@an.convergence.e98.acdc.pool.sd\endcsname{1.8}
\expandafter\gdef\csname R@an.convergence.e98.acdc.se\endcsname{1.0}
\expandafter\gdef\csname R@an.convergence.e98.acdc.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.convergence.e98.amos.L1\endcsname{790}
\expandafter\gdef\csname R@an.convergence.e98.amos.L1b\endcsname{874}
\expandafter\gdef\csname R@an.convergence.e98.amos.L2\endcsname{799}
\expandafter\gdef\csname R@an.convergence.e98.amos.L3\endcsname{813}
\expandafter\gdef\csname R@an.convergence.e98.amos.L4\endcsname{819}
\expandafter\gdef\csname R@an.convergence.e98.amos.L6\endcsname{747}
\expandafter\gdef\csname R@an.convergence.e98.amos.W1\endcsname{788}
\expandafter\gdef\csname R@an.convergence.e98.amos.W1c\endcsname{830}
\expandafter\gdef\csname R@an.convergence.e98.amos.W2\endcsname{876}
\expandafter\gdef\csname R@an.convergence.e98.amos.W3\endcsname{855}
\expandafter\gdef\csname R@an.convergence.e98.amos.W3c\endcsname{885}
\expandafter\gdef\csname R@an.convergence.e98.amos.W4\endcsname{847}
\expandafter\gdef\csname R@an.convergence.e98.amos.W5\endcsname{832}
\expandafter\gdef\csname R@an.convergence.e98.amos.designs.max\endcsname{874}
\expandafter\gdef\csname R@an.convergence.e98.amos.designs.mean\endcsname{807.0}
\expandafter\gdef\csname R@an.convergence.e98.amos.designs.median\endcsname{806.0}
\expandafter\gdef\csname R@an.convergence.e98.amos.designs.min\endcsname{747}
\expandafter\gdef\csname R@an.convergence.e98.amos.designs.sd\endcsname{41.5}
\expandafter\gdef\csname R@an.convergence.e98.amos.diff\endcsname{\ensuremath{-31.8}}
\expandafter\gdef\csname R@an.convergence.e98.amos.earlier\endcsname{3}
\expandafter\gdef\csname R@an.convergence.e98.amos.inside\endcsname{2}
\expandafter\gdef\csname R@an.convergence.e98.amos.later\endcsname{1}
\expandafter\gdef\csname R@an.convergence.e98.amos.pool.max\endcsname{862}
\expandafter\gdef\csname R@an.convergence.e98.amos.pool.mean\endcsname{838.8}
\expandafter\gdef\csname R@an.convergence.e98.amos.pool.min\endcsname{812}
\expandafter\gdef\csname R@an.convergence.e98.amos.pool.sd\endcsname{19.8}
\expandafter\gdef\csname R@an.convergence.e98.amos.se\endcsname{18.8}
\expandafter\gdef\csname R@an.convergence.e98.amos.z\endcsname{\ensuremath{-1.7}}
\expandafter\gdef\csname R@an.convergence.e98.kits.L1\endcsname{638}
\expandafter\gdef\csname R@an.convergence.e98.kits.L1b\endcsname{785}
\expandafter\gdef\csname R@an.convergence.e98.kits.L2\endcsname{847}
\expandafter\gdef\csname R@an.convergence.e98.kits.L3\endcsname{801}
\expandafter\gdef\csname R@an.convergence.e98.kits.L4\endcsname{625}
\expandafter\gdef\csname R@an.convergence.e98.kits.L6\endcsname{801}
\expandafter\gdef\csname R@an.convergence.e98.kits.W1c\endcsname{678}
\expandafter\gdef\csname R@an.convergence.e98.kits.designs.max\endcsname{847}
\expandafter\gdef\csname R@an.convergence.e98.kits.designs.mean\endcsname{749.5}
\expandafter\gdef\csname R@an.convergence.e98.kits.designs.median\endcsname{793.0}
\expandafter\gdef\csname R@an.convergence.e98.kits.designs.min\endcsname{625}
\expandafter\gdef\csname R@an.convergence.e98.kits.designs.sd\endcsname{93.8}
\expandafter\gdef\csname R@an.convergence.e98.kits.diff\endcsname{\ensuremath{-5.5}}
\expandafter\gdef\csname R@an.convergence.e98.kits.earlier\endcsname{2}
\expandafter\gdef\csname R@an.convergence.e98.kits.inside\endcsname{0}
\expandafter\gdef\csname R@an.convergence.e98.kits.later\endcsname{4}
\expandafter\gdef\csname R@an.convergence.e98.kits.pool.max\endcsname{780}
\expandafter\gdef\csname R@an.convergence.e98.kits.pool.mean\endcsname{755.0}
\expandafter\gdef\csname R@an.convergence.e98.kits.pool.min\endcsname{740}
\expandafter\gdef\csname R@an.convergence.e98.kits.pool.sd\endcsname{21.8}
\expandafter\gdef\csname R@an.convergence.e98.kits.se\endcsname{40.3}
\expandafter\gdef\csname R@an.convergence.e98.kits.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.convergence.final.acdc.L1\endcsname{92.69}
\expandafter\gdef\csname R@an.convergence.final.acdc.L1b\endcsname{92.80}
\expandafter\gdef\csname R@an.convergence.final.acdc.L2\endcsname{92.45}
\expandafter\gdef\csname R@an.convergence.final.acdc.L3\endcsname{92.96}
\expandafter\gdef\csname R@an.convergence.final.acdc.L4\endcsname{92.71}
\expandafter\gdef\csname R@an.convergence.final.acdc.L6\endcsname{92.72}
\expandafter\gdef\csname R@an.convergence.final.acdc.pool.max\endcsname{92.55}
\expandafter\gdef\csname R@an.convergence.final.acdc.pool.mean\endcsname{92.47}
\expandafter\gdef\csname R@an.convergence.final.acdc.pool.min\endcsname{92.37}
\expandafter\gdef\csname R@an.convergence.final.acdc.pool.sd\endcsname{0.07}
\expandafter\gdef\csname R@an.convergence.final.amos.L1\endcsname{88.51}
\expandafter\gdef\csname R@an.convergence.final.amos.L1b\endcsname{88.77}
\expandafter\gdef\csname R@an.convergence.final.amos.L2\endcsname{88.05}
\expandafter\gdef\csname R@an.convergence.final.amos.L3\endcsname{88.69}
\expandafter\gdef\csname R@an.convergence.final.amos.L4\endcsname{88.86}
\expandafter\gdef\csname R@an.convergence.final.amos.L6\endcsname{88.20}
\expandafter\gdef\csname R@an.convergence.final.amos.W1\endcsname{87.47}
\expandafter\gdef\csname R@an.convergence.final.amos.W1c\endcsname{87.91}
\expandafter\gdef\csname R@an.convergence.final.amos.W2\endcsname{88.25}
\expandafter\gdef\csname R@an.convergence.final.amos.W3\endcsname{88.39}
\expandafter\gdef\csname R@an.convergence.final.amos.W3c\endcsname{88.12}
\expandafter\gdef\csname R@an.convergence.final.amos.W4\endcsname{88.36}
\expandafter\gdef\csname R@an.convergence.final.amos.W5\endcsname{88.26}
\expandafter\gdef\csname R@an.convergence.final.amos.pool.max\endcsname{88.11}
\expandafter\gdef\csname R@an.convergence.final.amos.pool.mean\endcsname{87.74}
\expandafter\gdef\csname R@an.convergence.final.amos.pool.min\endcsname{87.45}
\expandafter\gdef\csname R@an.convergence.final.amos.pool.sd\endcsname{0.22}
\expandafter\gdef\csname R@an.convergence.final.kits.L1\endcsname{93.33}
\expandafter\gdef\csname R@an.convergence.final.kits.L1b\endcsname{93.90}
\expandafter\gdef\csname R@an.convergence.final.kits.L2\endcsname{92.82}
\expandafter\gdef\csname R@an.convergence.final.kits.L3\endcsname{93.50}
\expandafter\gdef\csname R@an.convergence.final.kits.L4\endcsname{93.20}
\expandafter\gdef\csname R@an.convergence.final.kits.L6\endcsname{93.43}
\expandafter\gdef\csname R@an.convergence.final.kits.W1c\endcsname{92.54}
\expandafter\gdef\csname R@an.convergence.final.kits.pool.max\endcsname{92.99}
\expandafter\gdef\csname R@an.convergence.final.kits.pool.mean\endcsname{92.76}
\expandafter\gdef\csname R@an.convergence.final.kits.pool.min\endcsname{92.55}
\expandafter\gdef\csname R@an.convergence.final.kits.pool.sd\endcsname{0.22}
\expandafter\gdef\csname R@an.convergence.finalspread.acdc.L1\endcsname{0.13}
\expandafter\gdef\csname R@an.convergence.finalspread.acdc.L1b\endcsname{0.14}
\expandafter\gdef\csname R@an.convergence.finalspread.acdc.L3\endcsname{0.35}
\expandafter\gdef\csname R@an.convergence.finalspread.acdc.max\endcsname{0.35}
\expandafter\gdef\csname R@an.convergence.finalspread.acdc.min\endcsname{0.13}
\expandafter\gdef\csname R@an.convergence.finalspread.acdc.n\endcsname{3}
\expandafter\gdef\csname R@an.convergence.finalspread.amos.L1\endcsname{0.36}
\expandafter\gdef\csname R@an.convergence.finalspread.amos.L1b\endcsname{0.34}
\expandafter\gdef\csname R@an.convergence.finalspread.amos.L2\endcsname{0.45}
\expandafter\gdef\csname R@an.convergence.finalspread.amos.L3\endcsname{0.68}
\expandafter\gdef\csname R@an.convergence.finalspread.amos.L4\endcsname{0.95}
\expandafter\gdef\csname R@an.convergence.finalspread.amos.max\endcsname{0.95}
\expandafter\gdef\csname R@an.convergence.finalspread.amos.min\endcsname{0.34}
\expandafter\gdef\csname R@an.convergence.finalspread.amos.n\endcsname{5}
\expandafter\gdef\csname R@an.convergence.finalspread.kits.L1\endcsname{0.70}
\expandafter\gdef\csname R@an.convergence.finalspread.kits.L1b\endcsname{1.25}
\expandafter\gdef\csname R@an.convergence.finalspread.kits.L2\endcsname{1.27}
\expandafter\gdef\csname R@an.convergence.finalspread.kits.L3\endcsname{0.55}
\expandafter\gdef\csname R@an.convergence.finalspread.kits.L4\endcsname{0.13}
\expandafter\gdef\csname R@an.convergence.finalspread.kits.L6\endcsname{1.00}
\expandafter\gdef\csname R@an.convergence.finalspread.kits.W1c\endcsname{0.65}
\expandafter\gdef\csname R@an.convergence.finalspread.kits.max\endcsname{1.27}
\expandafter\gdef\csname R@an.convergence.finalspread.kits.min\endcsname{0.13}
\expandafter\gdef\csname R@an.convergence.finalspread.kits.n\endcsname{7}
\expandafter\gdef\csname R@an.convergence.gap.acdc\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.convergence.gap.amos\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.convergence.gap.kits\endcsname{\ensuremath{+7.94}}
\expandafter\gdef\csname R@an.convergence.gapp.acdc\endcsname{0.031}
\expandafter\gdef\csname R@an.convergence.gapp.amos\endcsname{0.18}
\expandafter\gdef\csname R@an.convergence.gapp.kits\endcsname{0.67}
\expandafter\gdef\csname R@an.convergence.gapsd.acdc\endcsname{0.09}
\expandafter\gdef\csname R@an.convergence.gapsd.amos\endcsname{0.35}
\expandafter\gdef\csname R@an.convergence.gapsd.kits\endcsname{0.67}
\expandafter\gdef\csname R@an.convergence.lead.acdc.100\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.convergence.lead.acdc.100.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.lead.acdc.1000\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.convergence.lead.acdc.1000.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.lead.acdc.250\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.convergence.lead.acdc.250.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.lead.acdc.500\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.convergence.lead.acdc.500.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.lead.acdc.750\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.convergence.lead.acdc.750.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.lead.acdc.absmax\endcsname{0.25}
\expandafter\gdef\csname R@an.convergence.lead.acdc.dir\endcsname{rises}
\expandafter\gdef\csname R@an.convergence.lead.acdc.nfall\endcsname{0}
\expandafter\gdef\csname R@an.convergence.lead.acdc.nflat\endcsname{1}
\expandafter\gdef\csname R@an.convergence.lead.acdc.nneg\endcsname{0}
\expandafter\gdef\csname R@an.convergence.lead.acdc.nrise\endcsname{3}
\expandafter\gdef\csname R@an.convergence.lead.acdc.nsign\endcsname{0}
\expandafter\gdef\csname R@an.convergence.lead.acdc.nsteps\endcsname{4}
\expandafter\gdef\csname R@an.convergence.lead.acdc.path\endcsname{over the 4 steps between read epochs it rises at 3 and stays level to two decimals at 1}
\expandafter\gdef\csname R@an.convergence.lead.acdc.pop\endcsname{the 6 registered designs}
\expandafter\gdef\csname R@an.convergence.lead.amos.100\endcsname{\ensuremath{+4.15}}
\expandafter\gdef\csname R@an.convergence.lead.amos.100.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.lead.amos.1000\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.convergence.lead.amos.1000.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.lead.amos.250\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.convergence.lead.amos.250.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.lead.amos.500\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.convergence.lead.amos.500.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.lead.amos.750\endcsname{\ensuremath{+1.01}}
\expandafter\gdef\csname R@an.convergence.lead.amos.750.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.lead.amos.absmax\endcsname{4.15}
\expandafter\gdef\csname R@an.convergence.lead.amos.dir\endcsname{falls}
\expandafter\gdef\csname R@an.convergence.lead.amos.nfall\endcsname{3}
\expandafter\gdef\csname R@an.convergence.lead.amos.nflat\endcsname{0}
\expandafter\gdef\csname R@an.convergence.lead.amos.nneg\endcsname{0}
\expandafter\gdef\csname R@an.convergence.lead.amos.nrise\endcsname{1}
\expandafter\gdef\csname R@an.convergence.lead.amos.nsign\endcsname{0}
\expandafter\gdef\csname R@an.convergence.lead.amos.nsteps\endcsname{4}
\expandafter\gdef\csname R@an.convergence.lead.amos.path\endcsname{over the 4 steps between read epochs it rises at 1 and falls at 3}
\expandafter\gdef\csname R@an.convergence.lead.amos.pop\endcsname{the 6 registered designs}
\expandafter\gdef\csname R@an.convergence.lead.kits.100\endcsname{\ensuremath{+2.99}}
\expandafter\gdef\csname R@an.convergence.lead.kits.100.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.lead.kits.1000\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.convergence.lead.kits.1000.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.lead.kits.250\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.convergence.lead.kits.250.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.lead.kits.500\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.convergence.lead.kits.500.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.lead.kits.750\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.convergence.lead.kits.750.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.lead.kits.absmax\endcsname{2.99}
\expandafter\gdef\csname R@an.convergence.lead.kits.dir\endcsname{falls}
\expandafter\gdef\csname R@an.convergence.lead.kits.nfall\endcsname{2}
\expandafter\gdef\csname R@an.convergence.lead.kits.nflat\endcsname{0}
\expandafter\gdef\csname R@an.convergence.lead.kits.nneg\endcsname{2}
\expandafter\gdef\csname R@an.convergence.lead.kits.nrise\endcsname{2}
\expandafter\gdef\csname R@an.convergence.lead.kits.nsign\endcsname{4}
\expandafter\gdef\csname R@an.convergence.lead.kits.nsteps\endcsname{4}
\expandafter\gdef\csname R@an.convergence.lead.kits.path\endcsname{over the 4 steps between read epochs it rises at 2 and falls at 2}
\expandafter\gdef\csname R@an.convergence.lead.kits.pop\endcsname{the 6 registered designs}
\expandafter\gdef\csname R@an.convergence.leadcover.acdc.100\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.convergence.leadcover.acdc.100.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.leadcover.acdc.1000\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.convergence.leadcover.acdc.1000.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.leadcover.acdc.250\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.convergence.leadcover.acdc.250.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.leadcover.acdc.500\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.convergence.leadcover.acdc.500.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.leadcover.acdc.750\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.convergence.leadcover.acdc.750.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence.leadcover.amos.100\endcsname{\ensuremath{+3.11}}
\expandafter\gdef\csname R@an.convergence.leadcover.amos.100.n\endcsname{13}
\expandafter\gdef\csname R@an.convergence.leadcover.amos.1000\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.convergence.leadcover.amos.1000.n\endcsname{13}
\expandafter\gdef\csname R@an.convergence.leadcover.amos.250\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.convergence.leadcover.amos.250.n\endcsname{13}
\expandafter\gdef\csname R@an.convergence.leadcover.amos.500\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.convergence.leadcover.amos.500.n\endcsname{13}
\expandafter\gdef\csname R@an.convergence.leadcover.amos.750\endcsname{\ensuremath{+0.72}}
\expandafter\gdef\csname R@an.convergence.leadcover.amos.750.n\endcsname{13}
\expandafter\gdef\csname R@an.convergence.leadcover.kits.100\endcsname{\ensuremath{+2.88}}
\expandafter\gdef\csname R@an.convergence.leadcover.kits.100.n\endcsname{7}
\expandafter\gdef\csname R@an.convergence.leadcover.kits.1000\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.convergence.leadcover.kits.1000.n\endcsname{7}
\expandafter\gdef\csname R@an.convergence.leadcover.kits.250\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.convergence.leadcover.kits.250.n\endcsname{7}
\expandafter\gdef\csname R@an.convergence.leadcover.kits.500\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.convergence.leadcover.kits.500.n\endcsname{7}
\expandafter\gdef\csname R@an.convergence.leadcover.kits.750\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.convergence.leadcover.kits.750.n\endcsname{7}
\expandafter\gdef\csname R@an.convergence.leadmax.acdc.100\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.convergence.leadmax.acdc.1000\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.convergence.leadmax.acdc.250\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.convergence.leadmax.acdc.500\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.convergence.leadmax.acdc.750\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.convergence.leadmax.amos.100\endcsname{\ensuremath{+5.57}}
\expandafter\gdef\csname R@an.convergence.leadmax.amos.1000\endcsname{\ensuremath{+1.13}}
\expandafter\gdef\csname R@an.convergence.leadmax.amos.250\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.convergence.leadmax.amos.500\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@an.convergence.leadmax.amos.750\endcsname{\ensuremath{+1.71}}
\expandafter\gdef\csname R@an.convergence.leadmax.kits.100\endcsname{\ensuremath{+5.67}}
\expandafter\gdef\csname R@an.convergence.leadmax.kits.1000\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@an.convergence.leadmax.kits.250\endcsname{\ensuremath{+1.49}}
\expandafter\gdef\csname R@an.convergence.leadmax.kits.500\endcsname{\ensuremath{+2.96}}
\expandafter\gdef\csname R@an.convergence.leadmax.kits.750\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.convergence.leadmin.acdc.100\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.convergence.leadmin.acdc.1000\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.convergence.leadmin.acdc.250\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.convergence.leadmin.acdc.500\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.convergence.leadmin.acdc.750\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.convergence.leadmin.amos.100\endcsname{\ensuremath{+3.38}}
\expandafter\gdef\csname R@an.convergence.leadmin.amos.1000\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.convergence.leadmin.amos.250\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.convergence.leadmin.amos.500\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.convergence.leadmin.amos.750\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.convergence.leadmin.kits.100\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.convergence.leadmin.kits.1000\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.convergence.leadmin.kits.250\endcsname{\ensuremath{-1.51}}
\expandafter\gdef\csname R@an.convergence.leadmin.kits.500\endcsname{\ensuremath{-1.60}}
\expandafter\gdef\csname R@an.convergence.leadmin.kits.750\endcsname{\ensuremath{-1.29}}
\expandafter\gdef\csname R@an.convergence.lrfrac.100\endcsname{91}
\expandafter\gdef\csname R@an.convergence.lrfrac.1000\endcsname{0}
\expandafter\gdef\csname R@an.convergence.lrfrac.250\endcsname{77}
\expandafter\gdef\csname R@an.convergence.lrfrac.500\endcsname{54}
\expandafter\gdef\csname R@an.convergence.lrfrac.750\endcsname{29}
\expandafter\gdef\csname R@an.convergence.multiarms.acdc\endcsname{ResEnc-M (library preset), ResEnc-matched (re-implemented) and HyReX}
\expandafter\gdef\csname R@an.convergence.multiarms.acdc.max\endcsname{HyReX}
\expandafter\gdef\csname R@an.convergence.multiarms.amos\endcsname{ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, HyReX and ResEnc+context}
\expandafter\gdef\csname R@an.convergence.multiarms.amos.max\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.convergence.multiarms.kits\endcsname{ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context and branch control}
\expandafter\gdef\csname R@an.convergence.multiarms.kits.max\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.convergence.n.acdc\endcsname{6}
\expandafter\gdef\csname R@an.convergence.n.amos\endcsname{6}
\expandafter\gdef\csname R@an.convergence.n.kits\endcsname{6}
\expandafter\gdef\csname R@an.convergence.ncover.acdc\endcsname{6}
\expandafter\gdef\csname R@an.convergence.ncover.amos\endcsname{13}
\expandafter\gdef\csname R@an.convergence.ncover.kits\endcsname{7}
\expandafter\gdef\csname R@an.convergence.npair.acdc\endcsname{3}
\expandafter\gdef\csname R@an.convergence.npair.amos\endcsname{5}
\expandafter\gdef\csname R@an.convergence.npair.kits\endcsname{7}
\expandafter\gdef\csname R@an.convergence.npool.acdc\endcsname{6}
\expandafter\gdef\csname R@an.convergence.npool.amos\endcsname{6}
\expandafter\gdef\csname R@an.convergence.npool.kits\endcsname{3}
\expandafter\gdef\csname R@an.convergence.nrep.acdc\endcsname{6}
\expandafter\gdef\csname R@an.convergence.nrep.amos\endcsname{10}
\expandafter\gdef\csname R@an.convergence.nrep.kits\endcsname{14}
\expandafter\gdef\csname R@an.convergence.nruns.acdc\endcsname{12}
\expandafter\gdef\csname R@an.convergence.nruns.amos\endcsname{23}
\expandafter\gdef\csname R@an.convergence.nruns.kits\endcsname{21}
\expandafter\gdef\csname R@an.convergence.nrunsfam.acdc.reg\endcsname{6}
\expandafter\gdef\csname R@an.convergence.nrunsfam.acdc.rep\endcsname{6}
\expandafter\gdef\csname R@an.convergence.nrunsfam.acdc.twin\endcsname{0}
\expandafter\gdef\csname R@an.convergence.nrunsfam.amos.reg\endcsname{21}
\expandafter\gdef\csname R@an.convergence.nrunsfam.amos.rep\endcsname{2}
\expandafter\gdef\csname R@an.convergence.nrunsfam.amos.twin\endcsname{0}
\expandafter\gdef\csname R@an.convergence.nrunsfam.kits.reg\endcsname{21}
\expandafter\gdef\csname R@an.convergence.nrunsfam.kits.rep\endcsname{0}
\expandafter\gdef\csname R@an.convergence.nrunsfam.kits.twin\endcsname{0}
\expandafter\gdef\csname R@an.convergence.nseeds.acdc.L1\endcsname{3}
\expandafter\gdef\csname R@an.convergence.nseeds.acdc.L1b\endcsname{3}
\expandafter\gdef\csname R@an.convergence.nseeds.acdc.L2\endcsname{1}
\expandafter\gdef\csname R@an.convergence.nseeds.acdc.L3\endcsname{3}
\expandafter\gdef\csname R@an.convergence.nseeds.acdc.L4\endcsname{1}
\expandafter\gdef\csname R@an.convergence.nseeds.acdc.L6\endcsname{1}
\expandafter\gdef\csname R@an.convergence.nseeds.amos.L1\endcsname{3}
\expandafter\gdef\csname R@an.convergence.nseeds.amos.L1b\endcsname{3}
\expandafter\gdef\csname R@an.convergence.nseeds.amos.L2\endcsname{3}
\expandafter\gdef\csname R@an.convergence.nseeds.amos.L3\endcsname{3}
\expandafter\gdef\csname R@an.convergence.nseeds.amos.L4\endcsname{3}
\expandafter\gdef\csname R@an.convergence.nseeds.amos.L6\endcsname{1}
\expandafter\gdef\csname R@an.convergence.nseeds.amos.W1\endcsname{1}
\expandafter\gdef\csname R@an.convergence.nseeds.amos.W1c\endcsname{1}
\expandafter\gdef\csname R@an.convergence.nseeds.amos.W2\endcsname{1}
\expandafter\gdef\csname R@an.convergence.nseeds.amos.W3\endcsname{1}
\expandafter\gdef\csname R@an.convergence.nseeds.amos.W3c\endcsname{1}
\expandafter\gdef\csname R@an.convergence.nseeds.amos.W4\endcsname{1}
\expandafter\gdef\csname R@an.convergence.nseeds.amos.W5\endcsname{1}
\expandafter\gdef\csname R@an.convergence.nseeds.kits.L1\endcsname{3}
\expandafter\gdef\csname R@an.convergence.nseeds.kits.L1b\endcsname{3}
\expandafter\gdef\csname R@an.convergence.nseeds.kits.L2\endcsname{3}
\expandafter\gdef\csname R@an.convergence.nseeds.kits.L3\endcsname{3}
\expandafter\gdef\csname R@an.convergence.nseeds.kits.L4\endcsname{3}
\expandafter\gdef\csname R@an.convergence.nseeds.kits.L6\endcsname{3}
\expandafter\gdef\csname R@an.convergence.nseeds.kits.W1c\endcsname{3}
\expandafter\gdef\csname R@an.convergence.nswap.acdc\endcsname{6}
\expandafter\gdef\csname R@an.convergence.nswap.amos\endcsname{10}
\expandafter\gdef\csname R@an.convergence.nswap.kits\endcsname{12}
\expandafter\gdef\csname R@an.convergence.order.dice.acdc\endcsname{HyReX $>$ HyReX+context $>$ ResEnc-M (library preset) $>$ ResEnc+context $>$ ResEnc-matched (re-implemented) $>$ ConvNeXt-k3}
\expandafter\gdef\csname R@an.convergence.order.dice.amos\endcsname{ResEnc-M (library preset) $>$ ResEnc+context $>$ HyReX $>$ ConvNeXt-k3 $>$ ResEnc-matched (re-implemented) $>$ HyReX+context}
\expandafter\gdef\csname R@an.convergence.order.dice.kits\endcsname{HyReX $>$ HyReX+context $>$ ResEnc-M (library preset) $>$ ResEnc+context $>$ ResEnc-matched (re-implemented) $>$ ConvNeXt-k3}
\expandafter\gdef\csname R@an.convergence.order.ema.acdc.100\endcsname{ResEnc-matched (re-implemented) $>$ ResEnc+context $>$ ResEnc-M (library preset) $>$ HyReX $>$ HyReX+context $>$ ConvNeXt-k3}
\expandafter\gdef\csname R@an.convergence.order.ema.acdc.1000\endcsname{HyReX $>$ ResEnc-matched (re-implemented) $>$ HyReX+context $>$ ResEnc+context $>$ ResEnc-M (library preset) $>$ ConvNeXt-k3}
\expandafter\gdef\csname R@an.convergence.order.ema.acdc.250\endcsname{ResEnc-matched (re-implemented) $>$ HyReX $>$ ResEnc-M (library preset) $>$ HyReX+context $>$ ConvNeXt-k3 $>$ ResEnc+context}
\expandafter\gdef\csname R@an.convergence.order.ema.acdc.500\endcsname{HyReX $>$ ResEnc-M (library preset) $>$ ResEnc-matched (re-implemented) $>$ HyReX+context $>$ ResEnc+context $>$ ConvNeXt-k3}
\expandafter\gdef\csname R@an.convergence.order.ema.acdc.750\endcsname{HyReX $>$ ResEnc-matched (re-implemented) $>$ ResEnc+context $>$ ResEnc-M (library preset) $>$ HyReX+context $>$ ConvNeXt-k3}
\expandafter\gdef\csname R@an.convergence.order.ema.amos.100\endcsname{ResEnc-M (library preset) $>$ ConvNeXt-k3 $>$ HyReX $>$ ResEnc+context $>$ ResEnc-matched (re-implemented) $>$ HyReX+context}
\expandafter\gdef\csname R@an.convergence.order.ema.amos.1000\endcsname{ResEnc+context $>$ ResEnc-matched (re-implemented) $>$ HyReX $>$ ResEnc-M (library preset) $>$ HyReX+context $>$ ConvNeXt-k3}
\expandafter\gdef\csname R@an.convergence.order.ema.amos.250\endcsname{ResEnc-matched (re-implemented) $>$ HyReX $>$ ResEnc-M (library preset) $>$ HyReX+context $>$ ResEnc+context $>$ ConvNeXt-k3}
\expandafter\gdef\csname R@an.convergence.order.ema.amos.500\endcsname{HyReX+context $>$ HyReX $>$ ConvNeXt-k3 $>$ ResEnc+context $>$ ResEnc-matched (re-implemented) $>$ ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.convergence.order.ema.amos.750\endcsname{HyReX+context $>$ ResEnc-M (library preset) $>$ HyReX $>$ ResEnc-matched (re-implemented) $>$ ConvNeXt-k3 $>$ ResEnc+context}
\expandafter\gdef\csname R@an.convergence.order.ema.kits.100\endcsname{ResEnc-M (library preset) $>$ ResEnc-matched (re-implemented) $>$ ResEnc+context $>$ HyReX+context $>$ HyReX $>$ ConvNeXt-k3}
\expandafter\gdef\csname R@an.convergence.order.ema.kits.1000\endcsname{ResEnc-matched (re-implemented) $>$ HyReX $>$ HyReX+context $>$ ResEnc-M (library preset) $>$ ResEnc+context $>$ ConvNeXt-k3}
\expandafter\gdef\csname R@an.convergence.order.ema.kits.250\endcsname{HyReX+context $>$ ResEnc-M (library preset) $>$ ResEnc+context $>$ ResEnc-matched (re-implemented) $>$ ConvNeXt-k3 $>$ HyReX}
\expandafter\gdef\csname R@an.convergence.order.ema.kits.500\endcsname{ResEnc-M (library preset) $>$ ResEnc+context $>$ ResEnc-matched (re-implemented) $>$ HyReX+context $>$ ConvNeXt-k3 $>$ HyReX}
\expandafter\gdef\csname R@an.convergence.order.ema.kits.750\endcsname{ResEnc-matched (re-implemented) $>$ ResEnc-M (library preset) $>$ ConvNeXt-k3 $>$ ResEnc+context $>$ HyReX $>$ HyReX+context}
\expandafter\gdef\csname R@an.convergence.pairarms.acdc\endcsname{ResEnc-M (library preset), ResEnc-matched (re-implemented) and HyReX}
\expandafter\gdef\csname R@an.convergence.pairarms.amos\endcsname{ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, HyReX and ResEnc+context}
\expandafter\gdef\csname R@an.convergence.pairarms.kits\endcsname{ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context and branch control}
\expandafter\gdef\csname R@an.convergence.pdnoise.acdc.lvc\endcsname{0.2}
\expandafter\gdef\csname R@an.convergence.pdnoise.acdc.mlv\endcsname{0.2}
\expandafter\gdef\csname R@an.convergence.pdnoise.acdc.rv\endcsname{0.4}
\expandafter\gdef\csname R@an.convergence.pdnoise.amos.aorta\endcsname{0.9}
\expandafter\gdef\csname R@an.convergence.pdnoise.amos.bladder\endcsname{11.2}
\expandafter\gdef\csname R@an.convergence.pdnoise.amos.duodenum\endcsname{3.3}
\expandafter\gdef\csname R@an.convergence.pdnoise.amos.esophagus\endcsname{2.4}
\expandafter\gdef\csname R@an.convergence.pdnoise.amos.gall_bladder\endcsname{5.0}
\expandafter\gdef\csname R@an.convergence.pdnoise.amos.left_adrenal_gland\endcsname{3.8}
\expandafter\gdef\csname R@an.convergence.pdnoise.amos.left_kidney\endcsname{3.6}
\expandafter\gdef\csname R@an.convergence.pdnoise.amos.liver\endcsname{1.3}
\expandafter\gdef\csname R@an.convergence.pdnoise.amos.pancreas\endcsname{2.4}
\expandafter\gdef\csname R@an.convergence.pdnoise.amos.postcava\endcsname{1.7}
\expandafter\gdef\csname R@an.convergence.pdnoise.amos.prostate_uterus\endcsname{7.2}
\expandafter\gdef\csname R@an.convergence.pdnoise.amos.right_adrenal_gland\endcsname{3.6}
\expandafter\gdef\csname R@an.convergence.pdnoise.amos.right_kidney\endcsname{3.3}
\expandafter\gdef\csname R@an.convergence.pdnoise.amos.spleen\endcsname{3.5}
\expandafter\gdef\csname R@an.convergence.pdnoise.amos.stomach\endcsname{2.6}
\expandafter\gdef\csname R@an.convergence.pdnoise.kits.kidney\endcsname{1.3}
\expandafter\gdef\csname R@an.convergence.pdnoise.kits.masses\endcsname{4.1}
\expandafter\gdef\csname R@an.convergence.pdnoise.kits.tumor\endcsname{5.2}
\expandafter\gdef\csname R@an.convergence.pgap.acdc\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.convergence.pgap.amos\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.convergence.pgap.kits\endcsname{\ensuremath{+9.38}}
\expandafter\gdef\csname R@an.convergence.pgapsd.acdc\endcsname{0.04}
\expandafter\gdef\csname R@an.convergence.pgapsd.amos\endcsname{0.23}
\expandafter\gdef\csname R@an.convergence.pgapsd.kits\endcsname{0.79}
\expandafter\gdef\csname R@an.convergence.poolsd.acdc.100\endcsname{0.13}
\expandafter\gdef\csname R@an.convergence.poolsd.acdc.1000\endcsname{0.07}
\expandafter\gdef\csname R@an.convergence.poolsd.acdc.250\endcsname{0.13}
\expandafter\gdef\csname R@an.convergence.poolsd.acdc.500\endcsname{0.14}
\expandafter\gdef\csname R@an.convergence.poolsd.acdc.750\endcsname{0.08}
\expandafter\gdef\csname R@an.convergence.poolsd.amos.100\endcsname{1.17}
\expandafter\gdef\csname R@an.convergence.poolsd.amos.1000\endcsname{0.22}
\expandafter\gdef\csname R@an.convergence.poolsd.amos.250\endcsname{0.52}
\expandafter\gdef\csname R@an.convergence.poolsd.amos.500\endcsname{0.45}
\expandafter\gdef\csname R@an.convergence.poolsd.amos.750\endcsname{0.45}
\expandafter\gdef\csname R@an.convergence.poolsd.kits.100\endcsname{1.35}
\expandafter\gdef\csname R@an.convergence.poolsd.kits.1000\endcsname{0.22}
\expandafter\gdef\csname R@an.convergence.poolsd.kits.250\endcsname{1.11}
\expandafter\gdef\csname R@an.convergence.poolsd.kits.500\endcsname{0.60}
\expandafter\gdef\csname R@an.convergence.poolsd.kits.750\endcsname{0.47}
\expandafter\gdef\csname R@an.convergence.prem.F.acdc\endcsname{4.46}
\expandafter\gdef\csname R@an.convergence.prem.F.amos\endcsname{3.34}
\expandafter\gdef\csname R@an.convergence.prem.F.kits\endcsname{0.94}
\expandafter\gdef\csname R@an.convergence.prem.npairs.acdc\endcsname{15}
\expandafter\gdef\csname R@an.convergence.prem.npairs.amos\endcsname{15}
\expandafter\gdef\csname R@an.convergence.prem.npairs.kits\endcsname{15}
\expandafter\gdef\csname R@an.convergence.prem.nres.acdc\endcsname{2}
\expandafter\gdef\csname R@an.convergence.prem.nres.amos\endcsname{2}
\expandafter\gdef\csname R@an.convergence.prem.nres.kits\endcsname{0}
\expandafter\gdef\csname R@an.convergence.prem.p.acdc\endcsname{0.063}
\expandafter\gdef\csname R@an.convergence.prem.p.amos\endcsname{0.11}
\expandafter\gdef\csname R@an.convergence.prem.p.kits\endcsname{0.59}
\expandafter\gdef\csname R@an.convergence.prem.ratio.acdc\endcsname{2.11}
\expandafter\gdef\csname R@an.convergence.prem.ratio.amos\endcsname{1.83}
\expandafter\gdef\csname R@an.convergence.prem.ratio.kits\endcsname{0.97}
\expandafter\gdef\csname R@an.convergence.prem.sdarms.acdc\endcsname{0.209}
\expandafter\gdef\csname R@an.convergence.prem.sdarms.amos\endcsname{0.223}
\expandafter\gdef\csname R@an.convergence.prem.sdarms.kits\endcsname{0.770}
\expandafter\gdef\csname R@an.convergence.prem.sdpool.acdc\endcsname{0.099}
\expandafter\gdef\csname R@an.convergence.prem.sdpool.amos\endcsname{0.122}
\expandafter\gdef\csname R@an.convergence.prem.sdpool.kits\endcsname{0.795}
\expandafter\gdef\csname R@an.convergence.prem.thr.acdc\endcsname{0.36}
\expandafter\gdef\csname R@an.convergence.prem.thr.amos\endcsname{0.44}
\expandafter\gdef\csname R@an.convergence.prem.thr.kits\endcsname{4.84}
\expandafter\gdef\csname R@an.convergence.ptau.acdc.100\endcsname{0.72}
\expandafter\gdef\csname R@an.convergence.ptau.acdc.1000\endcsname{0.27}
\expandafter\gdef\csname R@an.convergence.ptau.acdc.250\endcsname{0.72}
\expandafter\gdef\csname R@an.convergence.ptau.acdc.500\endcsname{0.14}
\expandafter\gdef\csname R@an.convergence.ptau.acdc.750\endcsname{0.72}
\expandafter\gdef\csname R@an.convergence.ptau.amos.100\endcsname{0.14}
\expandafter\gdef\csname R@an.convergence.ptau.amos.1000\endcsname{0.72}
\expandafter\gdef\csname R@an.convergence.ptau.amos.250\endcsname{1.00}
\expandafter\gdef\csname R@an.convergence.ptau.amos.500\endcsname{0.27}
\expandafter\gdef\csname R@an.convergence.ptau.amos.750\endcsname{0.72}
\expandafter\gdef\csname R@an.convergence.ptau.kits.100\endcsname{1.00}
\expandafter\gdef\csname R@an.convergence.ptau.kits.1000\endcsname{0.27}
\expandafter\gdef\csname R@an.convergence.ptau.kits.250\endcsname{0.47}
\expandafter\gdef\csname R@an.convergence.ptau.kits.500\endcsname{1.00}
\expandafter\gdef\csname R@an.convergence.ptau.kits.750\endcsname{0.27}
\expandafter\gdef\csname R@an.convergence.ptau.min.all\endcsname{0.14}
\expandafter\gdef\csname R@an.convergence.ptau.min.all.where\endcsname{AMOS22 at epoch 100}
\expandafter\gdef\csname R@an.convergence.ptau.min.tab\endcsname{0.14}
\expandafter\gdef\csname R@an.convergence.ptaul.acdc.100\endcsname{0.47}
\expandafter\gdef\csname R@an.convergence.ptaul.acdc.1000\endcsname{1.00}
\expandafter\gdef\csname R@an.convergence.ptaul.acdc.250\endcsname{0.47}
\expandafter\gdef\csname R@an.convergence.ptaul.acdc.500\endcsname{0.14}
\expandafter\gdef\csname R@an.convergence.ptaul.acdc.750\endcsname{1.00}
\expandafter\gdef\csname R@an.convergence.ptaul.amos.100\endcsname{1.00}
\expandafter\gdef\csname R@an.convergence.ptaul.amos.1000\endcsname{1.00}
\expandafter\gdef\csname R@an.convergence.ptaul.amos.250\endcsname{0.72}
\expandafter\gdef\csname R@an.convergence.ptaul.amos.500\endcsname{0.72}
\expandafter\gdef\csname R@an.convergence.ptaul.amos.750\endcsname{0.72}
\expandafter\gdef\csname R@an.convergence.ptaul.kits.100\endcsname{1.00}
\expandafter\gdef\csname R@an.convergence.ptaul.kits.1000\endcsname{1.00}
\expandafter\gdef\csname R@an.convergence.ptaul.kits.250\endcsname{1.00}
\expandafter\gdef\csname R@an.convergence.ptaul.kits.500\endcsname{0.72}
\expandafter\gdef\csname R@an.convergence.ptaul.kits.750\endcsname{0.27}
\expandafter\gdef\csname R@an.convergence.s90.acdc.L1\endcsname{24}
\expandafter\gdef\csname R@an.convergence.s90.acdc.L1b\endcsname{23}
\expandafter\gdef\csname R@an.convergence.s90.acdc.L2\endcsname{26}
\expandafter\gdef\csname R@an.convergence.s90.acdc.L3\endcsname{23}
\expandafter\gdef\csname R@an.convergence.s90.acdc.L4\endcsname{24}
\expandafter\gdef\csname R@an.convergence.s90.acdc.L6\endcsname{24}
\expandafter\gdef\csname R@an.convergence.s90.acdc.designs.max\endcsname{26}
\expandafter\gdef\csname R@an.convergence.s90.acdc.designs.mean\endcsname{24.0}
\expandafter\gdef\csname R@an.convergence.s90.acdc.designs.median\endcsname{24.0}
\expandafter\gdef\csname R@an.convergence.s90.acdc.designs.min\endcsname{23}
\expandafter\gdef\csname R@an.convergence.s90.acdc.designs.sd\endcsname{1.1}
\expandafter\gdef\csname R@an.convergence.s90.acdc.diff\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.convergence.s90.acdc.earlier\endcsname{0}
\expandafter\gdef\csname R@an.convergence.s90.acdc.inside\endcsname{6}
\expandafter\gdef\csname R@an.convergence.s90.acdc.later\endcsname{0}
\expandafter\gdef\csname R@an.convergence.s90.acdc.pool.max\endcsname{26}
\expandafter\gdef\csname R@an.convergence.s90.acdc.pool.mean\endcsname{22.8}
\expandafter\gdef\csname R@an.convergence.s90.acdc.pool.min\endcsname{19}
\expandafter\gdef\csname R@an.convergence.s90.acdc.pool.sd\endcsname{3.1}
\expandafter\gdef\csname R@an.convergence.s90.acdc.se\endcsname{1.3}
\expandafter\gdef\csname R@an.convergence.s90.acdc.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.convergence.s90.amos.L1\endcsname{263}
\expandafter\gdef\csname R@an.convergence.s90.amos.L1b\endcsname{297}
\expandafter\gdef\csname R@an.convergence.s90.amos.L2\endcsname{265}
\expandafter\gdef\csname R@an.convergence.s90.amos.L3\endcsname{250}
\expandafter\gdef\csname R@an.convergence.s90.amos.L4\endcsname{286}
\expandafter\gdef\csname R@an.convergence.s90.amos.L6\endcsname{203}
\expandafter\gdef\csname R@an.convergence.s90.amos.W1\endcsname{224}
\expandafter\gdef\csname R@an.convergence.s90.amos.W1c\endcsname{256}
\expandafter\gdef\csname R@an.convergence.s90.amos.W2\endcsname{368}
\expandafter\gdef\csname R@an.convergence.s90.amos.W3\endcsname{271}
\expandafter\gdef\csname R@an.convergence.s90.amos.W3c\endcsname{404}
\expandafter\gdef\csname R@an.convergence.s90.amos.W4\endcsname{227}
\expandafter\gdef\csname R@an.convergence.s90.amos.W5\endcsname{299}
\expandafter\gdef\csname R@an.convergence.s90.amos.designs.max\endcsname{297}
\expandafter\gdef\csname R@an.convergence.s90.amos.designs.mean\endcsname{260.7}
\expandafter\gdef\csname R@an.convergence.s90.amos.designs.median\endcsname{264.0}
\expandafter\gdef\csname R@an.convergence.s90.amos.designs.min\endcsname{203}
\expandafter\gdef\csname R@an.convergence.s90.amos.designs.sd\endcsname{32.9}
\expandafter\gdef\csname R@an.convergence.s90.amos.diff\endcsname{\ensuremath{-26.7}}
\expandafter\gdef\csname R@an.convergence.s90.amos.earlier\endcsname{4}
\expandafter\gdef\csname R@an.convergence.s90.amos.inside\endcsname{2}
\expandafter\gdef\csname R@an.convergence.s90.amos.later\endcsname{0}
\expandafter\gdef\csname R@an.convergence.s90.amos.pool.max\endcsname{317}
\expandafter\gdef\csname R@an.convergence.s90.amos.pool.mean\endcsname{287.3}
\expandafter\gdef\csname R@an.convergence.s90.amos.pool.min\endcsname{268}
\expandafter\gdef\csname R@an.convergence.s90.amos.pool.sd\endcsname{20.0}
\expandafter\gdef\csname R@an.convergence.s90.amos.se\endcsname{15.7}
\expandafter\gdef\csname R@an.convergence.s90.amos.z\endcsname{\ensuremath{-1.7}}
\expandafter\gdef\csname R@an.convergence.s90.kits.L1\endcsname{119}
\expandafter\gdef\csname R@an.convergence.s90.kits.L1b\endcsname{277}
\expandafter\gdef\csname R@an.convergence.s90.kits.L2\endcsname{267}
\expandafter\gdef\csname R@an.convergence.s90.kits.L3\endcsname{382}
\expandafter\gdef\csname R@an.convergence.s90.kits.L4\endcsname{221}
\expandafter\gdef\csname R@an.convergence.s90.kits.L6\endcsname{297}
\expandafter\gdef\csname R@an.convergence.s90.kits.W1c\endcsname{247}
\expandafter\gdef\csname R@an.convergence.s90.kits.designs.max\endcsname{382}
\expandafter\gdef\csname R@an.convergence.s90.kits.designs.mean\endcsname{260.5}
\expandafter\gdef\csname R@an.convergence.s90.kits.designs.median\endcsname{272.0}
\expandafter\gdef\csname R@an.convergence.s90.kits.designs.min\endcsname{119}
\expandafter\gdef\csname R@an.convergence.s90.kits.designs.sd\endcsname{87.2}
\expandafter\gdef\csname R@an.convergence.s90.kits.diff\endcsname{\ensuremath{-49.5}}
\expandafter\gdef\csname R@an.convergence.s90.kits.earlier\endcsname{2}
\expandafter\gdef\csname R@an.convergence.s90.kits.inside\endcsname{4}
\expandafter\gdef\csname R@an.convergence.s90.kits.later\endcsname{0}
\expandafter\gdef\csname R@an.convergence.s90.kits.pool.max\endcsname{406}
\expandafter\gdef\csname R@an.convergence.s90.kits.pool.mean\endcsname{310.0}
\expandafter\gdef\csname R@an.convergence.s90.kits.pool.min\endcsname{229}
\expandafter\gdef\csname R@an.convergence.s90.kits.pool.sd\endcsname{89.4}
\expandafter\gdef\csname R@an.convergence.s90.kits.se\endcsname{62.7}
\expandafter\gdef\csname R@an.convergence.s90.kits.z\endcsname{\ensuremath{-0.8}}
\expandafter\gdef\csname R@an.convergence.s95.acdc.L1\endcsname{32}
\expandafter\gdef\csname R@an.convergence.s95.acdc.L1b\endcsname{31}
\expandafter\gdef\csname R@an.convergence.s95.acdc.L2\endcsname{34}
\expandafter\gdef\csname R@an.convergence.s95.acdc.L3\endcsname{32}
\expandafter\gdef\csname R@an.convergence.s95.acdc.L4\endcsname{32}
\expandafter\gdef\csname R@an.convergence.s95.acdc.L6\endcsname{32}
\expandafter\gdef\csname R@an.convergence.s95.acdc.designs.max\endcsname{34}
\expandafter\gdef\csname R@an.convergence.s95.acdc.designs.mean\endcsname{32.2}
\expandafter\gdef\csname R@an.convergence.s95.acdc.designs.median\endcsname{32.0}
\expandafter\gdef\csname R@an.convergence.s95.acdc.designs.min\endcsname{31}
\expandafter\gdef\csname R@an.convergence.s95.acdc.designs.sd\endcsname{1.0}
\expandafter\gdef\csname R@an.convergence.s95.acdc.diff\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.convergence.s95.acdc.earlier\endcsname{0}
\expandafter\gdef\csname R@an.convergence.s95.acdc.inside\endcsname{6}
\expandafter\gdef\csname R@an.convergence.s95.acdc.later\endcsname{0}
\expandafter\gdef\csname R@an.convergence.s95.acdc.pool.max\endcsname{34}
\expandafter\gdef\csname R@an.convergence.s95.acdc.pool.mean\endcsname{31.3}
\expandafter\gdef\csname R@an.convergence.s95.acdc.pool.min\endcsname{28}
\expandafter\gdef\csname R@an.convergence.s95.acdc.pool.sd\endcsname{2.3}
\expandafter\gdef\csname R@an.convergence.s95.acdc.se\endcsname{1.0}
\expandafter\gdef\csname R@an.convergence.s95.acdc.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.convergence.s95.amos.L1\endcsname{611}
\expandafter\gdef\csname R@an.convergence.s95.amos.L1b\endcsname{664}
\expandafter\gdef\csname R@an.convergence.s95.amos.L2\endcsname{627}
\expandafter\gdef\csname R@an.convergence.s95.amos.L3\endcsname{640}
\expandafter\gdef\csname R@an.convergence.s95.amos.L4\endcsname{749}
\expandafter\gdef\csname R@an.convergence.s95.amos.L6\endcsname{566}
\expandafter\gdef\csname R@an.convergence.s95.amos.W1\endcsname{654}
\expandafter\gdef\csname R@an.convergence.s95.amos.W1c\endcsname{623}
\expandafter\gdef\csname R@an.convergence.s95.amos.W2\endcsname{718}
\expandafter\gdef\csname R@an.convergence.s95.amos.W3\endcsname{701}
\expandafter\gdef\csname R@an.convergence.s95.amos.W3c\endcsname{757}
\expandafter\gdef\csname R@an.convergence.s95.amos.W4\endcsname{663}
\expandafter\gdef\csname R@an.convergence.s95.amos.W5\endcsname{648}
\expandafter\gdef\csname R@an.convergence.s95.amos.designs.max\endcsname{749}
\expandafter\gdef\csname R@an.convergence.s95.amos.designs.mean\endcsname{642.8}
\expandafter\gdef\csname R@an.convergence.s95.amos.designs.median\endcsname{633.5}
\expandafter\gdef\csname R@an.convergence.s95.amos.designs.min\endcsname{566}
\expandafter\gdef\csname R@an.convergence.s95.amos.designs.sd\endcsname{61.5}
\expandafter\gdef\csname R@an.convergence.s95.amos.diff\endcsname{\ensuremath{-17.3}}
\expandafter\gdef\csname R@an.convergence.s95.amos.earlier\endcsname{1}
\expandafter\gdef\csname R@an.convergence.s95.amos.inside\endcsname{4}
\expandafter\gdef\csname R@an.convergence.s95.amos.later\endcsname{1}
\expandafter\gdef\csname R@an.convergence.s95.amos.pool.max\endcsname{681}
\expandafter\gdef\csname R@an.convergence.s95.amos.pool.mean\endcsname{660.2}
\expandafter\gdef\csname R@an.convergence.s95.amos.pool.min\endcsname{610}
\expandafter\gdef\csname R@an.convergence.s95.amos.pool.sd\endcsname{25.4}
\expandafter\gdef\csname R@an.convergence.s95.amos.se\endcsname{27.2}
\expandafter\gdef\csname R@an.convergence.s95.amos.z\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.convergence.s95.kits.L1\endcsname{672}
\expandafter\gdef\csname R@an.convergence.s95.kits.L1b\endcsname{634}
\expandafter\gdef\csname R@an.convergence.s95.kits.L2\endcsname{767}
\expandafter\gdef\csname R@an.convergence.s95.kits.L3\endcsname{737}
\expandafter\gdef\csname R@an.convergence.s95.kits.L4\endcsname{655}
\expandafter\gdef\csname R@an.convergence.s95.kits.L6\endcsname{749}
\expandafter\gdef\csname R@an.convergence.s95.kits.W1c\endcsname{613}
\expandafter\gdef\csname R@an.convergence.s95.kits.designs.max\endcsname{767}
\expandafter\gdef\csname R@an.convergence.s95.kits.designs.mean\endcsname{702.3}
\expandafter\gdef\csname R@an.convergence.s95.kits.designs.median\endcsname{704.5}
\expandafter\gdef\csname R@an.convergence.s95.kits.designs.min\endcsname{634}
\expandafter\gdef\csname R@an.convergence.s95.kits.designs.sd\endcsname{55.5}
\expandafter\gdef\csname R@an.convergence.s95.kits.diff\endcsname{\ensuremath{+73.0}}
\expandafter\gdef\csname R@an.convergence.s95.kits.earlier\endcsname{0}
\expandafter\gdef\csname R@an.convergence.s95.kits.inside\endcsname{1}
\expandafter\gdef\csname R@an.convergence.s95.kits.later\endcsname{5}
\expandafter\gdef\csname R@an.convergence.s95.kits.pool.max\endcsname{647}
\expandafter\gdef\csname R@an.convergence.s95.kits.pool.mean\endcsname{629.3}
\expandafter\gdef\csname R@an.convergence.s95.kits.pool.min\endcsname{600}
\expandafter\gdef\csname R@an.convergence.s95.kits.pool.sd\endcsname{25.6}
\expandafter\gdef\csname R@an.convergence.s95.kits.se\endcsname{27.0}
\expandafter\gdef\csname R@an.convergence.s95.kits.z\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.convergence.s98.acdc.L1\endcsname{45}
\expandafter\gdef\csname R@an.convergence.s98.acdc.L1b\endcsname{43}
\expandafter\gdef\csname R@an.convergence.s98.acdc.L2\endcsname{48}
\expandafter\gdef\csname R@an.convergence.s98.acdc.L3\endcsname{45}
\expandafter\gdef\csname R@an.convergence.s98.acdc.L4\endcsname{44}
\expandafter\gdef\csname R@an.convergence.s98.acdc.L6\endcsname{44}
\expandafter\gdef\csname R@an.convergence.s98.acdc.designs.max\endcsname{48}
\expandafter\gdef\csname R@an.convergence.s98.acdc.designs.mean\endcsname{44.8}
\expandafter\gdef\csname R@an.convergence.s98.acdc.designs.median\endcsname{44.5}
\expandafter\gdef\csname R@an.convergence.s98.acdc.designs.min\endcsname{43}
\expandafter\gdef\csname R@an.convergence.s98.acdc.designs.sd\endcsname{1.7}
\expandafter\gdef\csname R@an.convergence.s98.acdc.diff\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.convergence.s98.acdc.earlier\endcsname{0}
\expandafter\gdef\csname R@an.convergence.s98.acdc.inside\endcsname{5}
\expandafter\gdef\csname R@an.convergence.s98.acdc.later\endcsname{1}
\expandafter\gdef\csname R@an.convergence.s98.acdc.pool.max\endcsname{47}
\expandafter\gdef\csname R@an.convergence.s98.acdc.pool.mean\endcsname{44.7}
\expandafter\gdef\csname R@an.convergence.s98.acdc.pool.min\endcsname{42}
\expandafter\gdef\csname R@an.convergence.s98.acdc.pool.sd\endcsname{1.8}
\expandafter\gdef\csname R@an.convergence.s98.acdc.se\endcsname{1.0}
\expandafter\gdef\csname R@an.convergence.s98.acdc.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.convergence.s98.amos.L1\endcsname{911}
\expandafter\gdef\csname R@an.convergence.s98.amos.L1b\endcsname{920}
\expandafter\gdef\csname R@an.convergence.s98.amos.L2\endcsname{887}
\expandafter\gdef\csname R@an.convergence.s98.amos.L3\endcsname{901}
\expandafter\gdef\csname R@an.convergence.s98.amos.L4\endcsname{925}
\expandafter\gdef\csname R@an.convergence.s98.amos.L6\endcsname{815}
\expandafter\gdef\csname R@an.convergence.s98.amos.W1\endcsname{858}
\expandafter\gdef\csname R@an.convergence.s98.amos.W1c\endcsname{885}
\expandafter\gdef\csname R@an.convergence.s98.amos.W2\endcsname{898}
\expandafter\gdef\csname R@an.convergence.s98.amos.W3\endcsname{941}
\expandafter\gdef\csname R@an.convergence.s98.amos.W3c\endcsname{917}
\expandafter\gdef\csname R@an.convergence.s98.amos.W4\endcsname{852}
\expandafter\gdef\csname R@an.convergence.s98.amos.W5\endcsname{856}
\expandafter\gdef\csname R@an.convergence.s98.amos.designs.max\endcsname{925}
\expandafter\gdef\csname R@an.convergence.s98.amos.designs.mean\endcsname{893.2}
\expandafter\gdef\csname R@an.convergence.s98.amos.designs.median\endcsname{906.0}
\expandafter\gdef\csname R@an.convergence.s98.amos.designs.min\endcsname{815}
\expandafter\gdef\csname R@an.convergence.s98.amos.designs.sd\endcsname{40.6}
\expandafter\gdef\csname R@an.convergence.s98.amos.diff\endcsname{\ensuremath{+10.0}}
\expandafter\gdef\csname R@an.convergence.s98.amos.earlier\endcsname{1}
\expandafter\gdef\csname R@an.convergence.s98.amos.inside\endcsname{2}
\expandafter\gdef\csname R@an.convergence.s98.amos.later\endcsname{3}
\expandafter\gdef\csname R@an.convergence.s98.amos.pool.max\endcsname{902}
\expandafter\gdef\csname R@an.convergence.s98.amos.pool.mean\endcsname{883.2}
\expandafter\gdef\csname R@an.convergence.s98.amos.pool.min\endcsname{858}
\expandafter\gdef\csname R@an.convergence.s98.amos.pool.sd\endcsname{16.8}
\expandafter\gdef\csname R@an.convergence.s98.amos.se\endcsname{18.0}
\expandafter\gdef\csname R@an.convergence.s98.amos.z\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.convergence.s98.kits.L1\endcsname{864}
\expandafter\gdef\csname R@an.convergence.s98.kits.L1b\endcsname{878}
\expandafter\gdef\csname R@an.convergence.s98.kits.L2\endcsname{948}
\expandafter\gdef\csname R@an.convergence.s98.kits.L3\endcsname{942}
\expandafter\gdef\csname R@an.convergence.s98.kits.L4\endcsname{855}
\expandafter\gdef\csname R@an.convergence.s98.kits.L6\endcsname{936}
\expandafter\gdef\csname R@an.convergence.s98.kits.W1c\endcsname{845}
\expandafter\gdef\csname R@an.convergence.s98.kits.designs.max\endcsname{948}
\expandafter\gdef\csname R@an.convergence.s98.kits.designs.mean\endcsname{903.8}
\expandafter\gdef\csname R@an.convergence.s98.kits.designs.median\endcsname{907.0}
\expandafter\gdef\csname R@an.convergence.s98.kits.designs.min\endcsname{855}
\expandafter\gdef\csname R@an.convergence.s98.kits.designs.sd\endcsname{42.6}
\expandafter\gdef\csname R@an.convergence.s98.kits.diff\endcsname{\ensuremath{+31.2}}
\expandafter\gdef\csname R@an.convergence.s98.kits.earlier\endcsname{0}
\expandafter\gdef\csname R@an.convergence.s98.kits.inside\endcsname{3}
\expandafter\gdef\csname R@an.convergence.s98.kits.later\endcsname{3}
\expandafter\gdef\csname R@an.convergence.s98.kits.pool.max\endcsname{902}
\expandafter\gdef\csname R@an.convergence.s98.kits.pool.mean\endcsname{872.7}
\expandafter\gdef\csname R@an.convergence.s98.kits.pool.min\endcsname{853}
\expandafter\gdef\csname R@an.convergence.s98.kits.pool.sd\endcsname{25.9}
\expandafter\gdef\csname R@an.convergence.s98.kits.se\endcsname{22.9}
\expandafter\gdef\csname R@an.convergence.s98.kits.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.convergence.scalehead\endcsname{on the scale of the differences between arms on AMOS22 and larger than every difference between two arms on KiTS23 and ACDC}
\expandafter\gdef\csname R@an.convergence.scalephrase.acdc\endcsname{larger than every difference between two arms}
\expandafter\gdef\csname R@an.convergence.scalephrase.amos\endcsname{on the scale of the differences between arms}
\expandafter\gdef\csname R@an.convergence.scalephrase.kits\endcsname{larger than every difference between two arms}
\expandafter\gdef\csname R@an.convergence.sdratio.acdc.100\endcsname{1.68}
\expandafter\gdef\csname R@an.convergence.sdratio.acdc.1000\endcsname{2.39}
\expandafter\gdef\csname R@an.convergence.sdratio.acdc.250\endcsname{1.04}
\expandafter\gdef\csname R@an.convergence.sdratio.acdc.500\endcsname{1.12}
\expandafter\gdef\csname R@an.convergence.sdratio.acdc.750\endcsname{1.31}
\expandafter\gdef\csname R@an.convergence.sdratio.amos.100\endcsname{0.74}
\expandafter\gdef\csname R@an.convergence.sdratio.amos.1000\endcsname{1.45}
\expandafter\gdef\csname R@an.convergence.sdratio.amos.250\endcsname{0.79}
\expandafter\gdef\csname R@an.convergence.sdratio.amos.500\endcsname{1.23}
\expandafter\gdef\csname R@an.convergence.sdratio.amos.750\endcsname{1.13}
\expandafter\gdef\csname R@an.convergence.sdratio.kits.100\endcsname{1.68}
\expandafter\gdef\csname R@an.convergence.sdratio.kits.1000\endcsname{1.60}
\expandafter\gdef\csname R@an.convergence.sdratio.kits.250\endcsname{0.92}
\expandafter\gdef\csname R@an.convergence.sdratio.kits.500\endcsname{2.95}
\expandafter\gdef\csname R@an.convergence.sdratio.kits.750\endcsname{1.05}
\expandafter\gdef\csname R@an.convergence.sep.clear.list\endcsname{AMOS22 at epoch 100}
\expandafter\gdef\csname R@an.convergence.sep.conc.acdc.100\endcsname{6}
\expandafter\gdef\csname R@an.convergence.sep.conc.acdc.1000\endcsname{9}
\expandafter\gdef\csname R@an.convergence.sep.conc.acdc.250\endcsname{7}
\expandafter\gdef\csname R@an.convergence.sep.conc.acdc.500\endcsname{9}
\expandafter\gdef\csname R@an.convergence.sep.conc.acdc.750\endcsname{9}
\expandafter\gdef\csname R@an.convergence.sep.conc.amos.100\endcsname{11}
\expandafter\gdef\csname R@an.convergence.sep.conc.amos.1000\endcsname{5}
\expandafter\gdef\csname R@an.convergence.sep.conc.amos.250\endcsname{4}
\expandafter\gdef\csname R@an.convergence.sep.conc.amos.500\endcsname{3}
\expandafter\gdef\csname R@an.convergence.sep.conc.amos.750\endcsname{5}
\expandafter\gdef\csname R@an.convergence.sep.conc.kits.100\endcsname{4}
\expandafter\gdef\csname R@an.convergence.sep.conc.kits.1000\endcsname{4}
\expandafter\gdef\csname R@an.convergence.sep.conc.kits.250\endcsname{3}
\expandafter\gdef\csname R@an.convergence.sep.conc.kits.500\endcsname{3}
\expandafter\gdef\csname R@an.convergence.sep.conc.kits.750\endcsname{1}
\expandafter\gdef\csname R@an.convergence.sep.late.acdc\endcsname{9 of its 10 separated pairs at each of epochs 500, 750 and 1000 (exact one-sided $p=0.067$ at each)}
\expandafter\gdef\csname R@an.convergence.sep.late.amos\endcsname{3 at epoch 500, 5 at epoch 750 and 5 at epoch 1000 of its 11 separated pairs (exact one-sided $p=0.88$, 0.65 and 0.65)}
\expandafter\gdef\csname R@an.convergence.sep.late.kits\endcsname{3 at epoch 500, 1 at epoch 750 and 4 at epoch 1000 of its 4 separated pairs (exact one-sided $p=0.40$, 0.80 and 0.20)}
\expandafter\gdef\csname R@an.convergence.sep.n.acdc\endcsname{10}
\expandafter\gdef\csname R@an.convergence.sep.n.amos\endcsname{11}
\expandafter\gdef\csname R@an.convergence.sep.n.kits\endcsname{4}
\expandafter\gdef\csname R@an.convergence.sep.nclear\endcsname{1}
\expandafter\gdef\csname R@an.convergence.sep.nreads\endcsname{15}
\expandafter\gdef\csname R@an.convergence.sep.nreads.tab\endcsname{10}
\expandafter\gdef\csname R@an.convergence.sep.p.acdc.100\endcsname{0.42}
\expandafter\gdef\csname R@an.convergence.sep.p.acdc.1000\endcsname{0.067}
\expandafter\gdef\csname R@an.convergence.sep.p.acdc.250\endcsname{0.27}
\expandafter\gdef\csname R@an.convergence.sep.p.acdc.500\endcsname{0.067}
\expandafter\gdef\csname R@an.convergence.sep.p.acdc.750\endcsname{0.067}
\expandafter\gdef\csname R@an.convergence.sep.p.amos.100\endcsname{0.017}
\expandafter\gdef\csname R@an.convergence.sep.p.amos.1000\endcsname{0.65}
\expandafter\gdef\csname R@an.convergence.sep.p.amos.250\endcsname{0.78}
\expandafter\gdef\csname R@an.convergence.sep.p.amos.500\endcsname{0.88}
\expandafter\gdef\csname R@an.convergence.sep.p.amos.750\endcsname{0.65}
\expandafter\gdef\csname R@an.convergence.sep.p.kits.100\endcsname{0.20}
\expandafter\gdef\csname R@an.convergence.sep.p.kits.1000\endcsname{0.20}
\expandafter\gdef\csname R@an.convergence.sep.p.kits.250\endcsname{0.40}
\expandafter\gdef\csname R@an.convergence.sep.p.kits.500\endcsname{0.40}
\expandafter\gdef\csname R@an.convergence.sep.p.kits.750\endcsname{0.80}
\expandafter\gdef\csname R@an.convergence.sep.se.acdc\endcsname{0.14}
\expandafter\gdef\csname R@an.convergence.sep.se.amos\endcsname{0.17}
\expandafter\gdef\csname R@an.convergence.sep.se.kits\endcsname{1.12}
\expandafter\gdef\csname R@an.convergence.spreadclause.acdc\endcsname{on ACDC the within-arm final-EMA spread is read for 3 of the 6 arms drawn, namely ResEnc-M (library preset), ResEnc-matched (re-implemented) and HyReX; the largest of those spreads, that of HyReX, is 0.35 pseudo-Dice points, larger than every difference between two arms: it exceeds all 15 differences between two arms' mean final EMA in the same panel (median 0.05)}
\expandafter\gdef\csname R@an.convergence.spreadclause.amos\endcsname{on AMOS22 the within-arm final-EMA spread is read for 5 of the 13 arms drawn, namely ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, HyReX and ResEnc+context; the largest of those spreads, that of ResEnc+context, is 0.95 pseudo-Dice points, on the scale of the differences between arms: it exceeds 75 of the 78 differences between two arms' mean final EMA in the same panel (median 0.23)}
\expandafter\gdef\csname R@an.convergence.spreadclause.kits\endcsname{on KiTS23 the within-arm final-EMA spread is read for 7 of the 7 arms drawn, namely ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context and branch control; the largest of those spreads, that of ConvNeXt-k3, is 1.27 pseudo-Dice points, larger than every difference between two arms: it exceeds all 21 differences between two arms' mean final EMA in the same panel (median 0.35)}
\expandafter\gdef\csname R@an.convergence.swap.max.acdc.100\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.convergence.swap.max.acdc.1000\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.convergence.swap.max.acdc.250\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.convergence.swap.max.acdc.500\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.convergence.swap.max.acdc.750\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.convergence.swap.max.amos.100\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.convergence.swap.max.amos.1000\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.convergence.swap.max.amos.250\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.convergence.swap.max.amos.500\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.convergence.swap.max.amos.750\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.convergence.swap.max.kits.100\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.convergence.swap.max.kits.1000\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.convergence.swap.max.kits.250\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.convergence.swap.max.kits.500\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.convergence.swap.max.kits.750\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.convergence.swap.min.acdc.100\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.convergence.swap.min.acdc.1000\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.convergence.swap.min.acdc.250\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.convergence.swap.min.acdc.500\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.convergence.swap.min.acdc.750\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.convergence.swap.min.amos.100\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.convergence.swap.min.amos.1000\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.convergence.swap.min.amos.250\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.convergence.swap.min.amos.500\endcsname{\ensuremath{-0.73}}
\expandafter\gdef\csname R@an.convergence.swap.min.amos.750\endcsname{\ensuremath{-0.60}}
\expandafter\gdef\csname R@an.convergence.swap.min.kits.100\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.convergence.swap.min.kits.1000\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.convergence.swap.min.kits.250\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.convergence.swap.min.kits.500\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.convergence.swap.min.kits.750\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.convergence.tau.acdc.100\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.convergence.tau.acdc.1000\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.convergence.tau.acdc.250\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.convergence.tau.acdc.500\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.convergence.tau.acdc.750\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.convergence.tau.amos.100\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.convergence.tau.amos.1000\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.convergence.tau.amos.250\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.convergence.tau.amos.500\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.convergence.tau.amos.750\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.convergence.tau.kits.100\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.convergence.tau.kits.1000\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.convergence.tau.kits.250\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.convergence.tau.kits.500\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.convergence.tau.kits.750\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.convergence.tauall.mean.acdc\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.convergence.tauall.mean.amos\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.convergence.tauall.mean.kits\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.convergence.tauall.n.acdc\endcsname{901}
\expandafter\gdef\csname R@an.convergence.tauall.n.amos\endcsname{901}
\expandafter\gdef\csname R@an.convergence.tauall.n.kits\endcsname{901}
\expandafter\gdef\csname R@an.convergence.tauall.pos.acdc\endcsname{88}
\expandafter\gdef\csname R@an.convergence.tauall.pos.amos\endcsname{61}
\expandafter\gdef\csname R@an.convergence.tauall.pos.kits\endcsname{61}
\expandafter\gdef\csname R@an.convergence.tauall.sd.acdc\endcsname{0.24}
\expandafter\gdef\csname R@an.convergence.tauall.sd.amos\endcsname{0.36}
\expandafter\gdef\csname R@an.convergence.tauall.sd.kits\endcsname{0.27}
\expandafter\gdef\csname R@an.convergence.tauedge.acdc\endcsname{0.87}
\expandafter\gdef\csname R@an.convergence.tauedge.amos\endcsname{0.87}
\expandafter\gdef\csname R@an.convergence.tauedge.both\endcsname{0.87}
\expandafter\gdef\csname R@an.convergence.tauedge.kits\endcsname{0.87}
\expandafter\gdef\csname R@an.convergence.taul.acdc.100\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.convergence.taul.acdc.1000\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.convergence.taul.acdc.250\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.convergence.taul.acdc.500\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.convergence.taul.acdc.750\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.convergence.taul.amos.100\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.convergence.taul.amos.1000\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.convergence.taul.amos.250\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.convergence.taul.amos.500\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.convergence.taul.amos.750\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.convergence.taul.kits.100\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.convergence.taul.kits.1000\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.convergence.taul.kits.250\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.convergence.taul.kits.500\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.convergence.taul.kits.750\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.convergence.taulall.mean.acdc\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.convergence.taulall.mean.amos\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.convergence.taulall.mean.kits\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.convergence.taulall.n.acdc\endcsname{901}
\expandafter\gdef\csname R@an.convergence.taulall.n.amos\endcsname{901}
\expandafter\gdef\csname R@an.convergence.taulall.n.kits\endcsname{901}
\expandafter\gdef\csname R@an.convergence.taulall.pos.acdc\endcsname{95}
\expandafter\gdef\csname R@an.convergence.taulall.pos.amos\endcsname{73}
\expandafter\gdef\csname R@an.convergence.taulall.pos.kits\endcsname{71}
\expandafter\gdef\csname R@an.convergence.taulall.sd.acdc\endcsname{0.18}
\expandafter\gdef\csname R@an.convergence.taulall.sd.amos\endcsname{0.28}
\expandafter\gdef\csname R@an.convergence.taulall.sd.kits\endcsname{0.25}
\expandafter\gdef\csname R@an.convergence.taumax.acdc\endcsname{0.60}
\expandafter\gdef\csname R@an.convergence.taumax.amos\endcsname{0.60}
\expandafter\gdef\csname R@an.convergence.taumax.both\endcsname{0.60}
\expandafter\gdef\csname R@an.convergence.taumax.kits\endcsname{0.47}
\expandafter\gdef\csname R@an.convergence.taumaxs.acdc\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.convergence.taumaxs.amos\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.convergence.taumaxs.kits\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.convergence.taumin.acdc\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.convergence.taumin.amos\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.convergence.taumin.kits\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.convergence.tauwin.acdc.cmax\endcsname{8}
\expandafter\gdef\csname R@an.convergence.tauwin.acdc.cmin\endcsname{5}
\expandafter\gdef\csname R@an.convergence.tauwin.acdc.max\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.convergence.tauwin.acdc.mean\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.convergence.tauwin.acdc.min\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.convergence.tauwin.acdc.n\endcsname{41}
\expandafter\gdef\csname R@an.convergence.tauwin.acdc.nall\endcsname{0}
\expandafter\gdef\csname R@an.convergence.tauwin.acdc.nge100\endcsname{30}
\expandafter\gdef\csname R@an.convergence.tauwin.amos.cmax\endcsname{11}
\expandafter\gdef\csname R@an.convergence.tauwin.amos.cmin\endcsname{5}
\expandafter\gdef\csname R@an.convergence.tauwin.amos.max\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.convergence.tauwin.amos.mean\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.convergence.tauwin.amos.min\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.convergence.tauwin.amos.n\endcsname{41}
\expandafter\gdef\csname R@an.convergence.tauwin.amos.nall\endcsname{8}
\expandafter\gdef\csname R@an.convergence.tauwin.amos.nge100\endcsname{5}
\expandafter\gdef\csname R@an.convergence.tauwin.kits.cmax\endcsname{4}
\expandafter\gdef\csname R@an.convergence.tauwin.kits.cmin\endcsname{1}
\expandafter\gdef\csname R@an.convergence.tauwin.kits.max\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.convergence.tauwin.kits.mean\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.convergence.tauwin.kits.min\endcsname{\ensuremath{-0.60}}
\expandafter\gdef\csname R@an.convergence.tauwin.kits.n\endcsname{41}
\expandafter\gdef\csname R@an.convergence.tauwin.kits.nall\endcsname{26}
\expandafter\gdef\csname R@an.convergence.tauwin.kits.nge100\endcsname{24}
\expandafter\gdef\csname R@an.convergence_xx.amos.def.at250\endcsname{78.94}
\expandafter\gdef\csname R@an.convergence_xx.amos.def.at500\endcsname{82.11}
\expandafter\gdef\csname R@an.convergence_xx.amos.def.e95\endcsname{617}
\expandafter\gdef\csname R@an.convergence_xx.amos.def.e98\endcsname{849}
\expandafter\gdef\csname R@an.convergence_xx.amos.def.final\endcsname{87.74}
\expandafter\gdef\csname R@an.convergence_xx.amos.def.n\endcsname{6}
\expandafter\gdef\csname R@an.convergence_xx.amos.sentence\endcsname{on AMOS22 the run-mean EMA pseudo-Dice of {\ifdefined\archL\archL\else XX-Net-L\fi} reaches 98\,\% of its final value at epoch 804 against 849 for the default (1 and 6 runs), and is \ensuremath{-0.29}\,pp from the default's at epoch 250}
\expandafter\gdef\csname R@an.convergence_xx.amos.xa.at250\endcsname{80.41}
\expandafter\gdef\csname R@an.convergence_xx.amos.xa.at500\endcsname{83.13}
\expandafter\gdef\csname R@an.convergence_xx.amos.xa.e95\endcsname{611}
\expandafter\gdef\csname R@an.convergence_xx.amos.xa.e98\endcsname{873}
\expandafter\gdef\csname R@an.convergence_xx.amos.xa.final\endcsname{88.67}
\expandafter\gdef\csname R@an.convergence_xx.amos.xa.n\endcsname{1}
\expandafter\gdef\csname R@an.convergence_xx.amos.xl.at250\endcsname{78.65}
\expandafter\gdef\csname R@an.convergence_xx.amos.xl.at500\endcsname{81.85}
\expandafter\gdef\csname R@an.convergence_xx.amos.xl.d.at250\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.convergence_xx.amos.xl.d.at500\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.convergence_xx.amos.xl.d.final\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.convergence_xx.amos.xl.e95\endcsname{539}
\expandafter\gdef\csname R@an.convergence_xx.amos.xl.e98\endcsname{804}
\expandafter\gdef\csname R@an.convergence_xx.amos.xl.final\endcsname{87.56}
\expandafter\gdef\csname R@an.convergence_xx.amos.xl.n\endcsname{1}
\expandafter\gdef\csname R@an.convergence_xx.caption\endcsname{Training curves on fold 0: EMA pseudo-Dice of the validation patches (top) and validation loss (bottom) of {\ifdefined\archL\archL\else XX-Net-L\fi}, {\ifdefined\archA\archA\else XX-Net-A\fi} and the nnU-Net default on KiTS23 and AMOS22; lines are the mean over runs (the default's frozen pool, the candidates' finished seeds), bands their range, both drawn as a 25-epoch running mean. The EMA pseudo-Dice is a training-time proxy, not the final validation Dice}
\expandafter\gdef\csname R@an.convergence_xx.kits.def.at250\endcsname{85.79}
\expandafter\gdef\csname R@an.convergence_xx.kits.def.at500\endcsname{87.64}
\expandafter\gdef\csname R@an.convergence_xx.kits.def.e95\endcsname{486}
\expandafter\gdef\csname R@an.convergence_xx.kits.def.e98\endcsname{749}
\expandafter\gdef\csname R@an.convergence_xx.kits.def.final\endcsname{92.76}
\expandafter\gdef\csname R@an.convergence_xx.kits.def.n\endcsname{3}
\expandafter\gdef\csname R@an.convergence_xx.kits.sentence\endcsname{on KiTS23 the run-mean EMA pseudo-Dice of {\ifdefined\archL\archL\else XX-Net-L\fi} reaches 98\,\% of its final value at epoch 752 against 749 for the default (3 and 3 runs), and is \ensuremath{-0.59}\,pp from the default's at epoch 250}
\expandafter\gdef\csname R@an.convergence_xx.kits.xa.at250\endcsname{85.59}
\expandafter\gdef\csname R@an.convergence_xx.kits.xa.at500\endcsname{88.91}
\expandafter\gdef\csname R@an.convergence_xx.kits.xa.e95\endcsname{436}
\expandafter\gdef\csname R@an.convergence_xx.kits.xa.e98\endcsname{771}
\expandafter\gdef\csname R@an.convergence_xx.kits.xa.final\endcsname{93.12}
\expandafter\gdef\csname R@an.convergence_xx.kits.xa.n\endcsname{3}
\expandafter\gdef\csname R@an.convergence_xx.kits.xl.at250\endcsname{85.19}
\expandafter\gdef\csname R@an.convergence_xx.kits.xl.at500\endcsname{88.58}
\expandafter\gdef\csname R@an.convergence_xx.kits.xl.d.at250\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.convergence_xx.kits.xl.d.at500\endcsname{\ensuremath{+0.94}}
\expandafter\gdef\csname R@an.convergence_xx.kits.xl.d.final\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.convergence_xx.kits.xl.e95\endcsname{468}
\expandafter\gdef\csname R@an.convergence_xx.kits.xl.e98\endcsname{752}
\expandafter\gdef\csname R@an.convergence_xx.kits.xl.final\endcsname{92.50}
\expandafter\gdef\csname R@an.convergence_xx.kits.xl.n\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.atdefault.best\endcsname{HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.atdefault.best.pp\endcsname{\ensuremath{+0.616}}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.atdefault.clause\endcsname{the largest ACDC seed-0 gain among the 9 registered arms with a finished run at or below the default's 30.38 M parameters on the ACDC plan is that of HyReX, \ensuremath{+0.616} pp, then that of HyReX with 9-kernel coarse stages, \ensuremath{+0.573} pp (0.043 pp behind, 0.31 SD of a one-seed pair difference, inside its 0.50 pp edge)}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.atdefault.hero.behind\endcsname{0.000}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.atdefault.hero.pp\endcsname{\ensuremath{+0.616}}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.atdefault.hero.rank\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.atdefault.licence\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.atdefault.margin\endcsname{0.043}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.atdefault.n\endcsname{9}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.atdefault.names\endcsname{HyReX, HyReX with 9-kernel coarse stages, HyReX+context, LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), function-identical control, ConvNeXt-k3, LeanAdd with coarse large kernels (LeanAdd-NeXt), LeanAdd-NeXt with the coarse operator at stage 5 alone}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.atdefault.second\endcsname{HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.atdefault.universe\endcsname{the 9 registered arms with a finished run at or below the default's 30.38 M parameters on the ACDC plan}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.best\endcsname{HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.best.clause\endcsname{HyReX, the highest seed-0 delta among the 12 registered arms with a finished ACDC run (the library preset and the matched controls included), 0.043 pp ahead of HyReX with 9-kernel coarse stages, a margin inside the registered 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.floor.arms\endcsname{HyReX, HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.floor.clause\endcsname{2 of the 12 evaluated ACDC arms have a seed-0 margin over the default that clears the registered 0.5 pp one-seed pair floor: HyReX, HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.floor.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.floor.of\endcsname{12}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.fresh.best\endcsname{HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.fresh.best.pp\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.fresh.clause\endcsname{HyReX's ACDC gain is retained on the fresh seeds, \ensuremath{+0.450} pp against the frozen pool and \ensuremath{+0.242} pp for ResEnc-M (library preset); HyReX is 0.208 pp above ResEnc-M (library preset) on ACDC, measured on the fresh-seed mean (seeds 1--2) of both arms: 2.11 times the 0.099 pp null SD of a two-seed difference; at the discovery seed HyReX is ahead by 0.281 pp, below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.fresh.landed\endcsname{HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented), function-identical control}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.fresh.margin\endcsname{0.131}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.fresh.pending\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.fresh.second\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.fresh.second.pp\endcsname{\ensuremath{+0.319}}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.fresh.super\endcsname{over the 4 of 12 finished arms that have a fresh mean}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.fresh.top.clause\endcsname{HyReX records the largest ACDC fresh-seed mean, \ensuremath{+0.450} pp, against \ensuremath{+0.319} pp for ResEnc-matched (re-implemented) (0.131 pp apart), over the 4 of 12 finished arms that have a fresh mean}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.hero.gap\endcsname{0.043}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.hero.gap.dir\endcsname{ahead}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.hero.gap.floor\endcsname{inside}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.hero.gap.sepair\endcsname{0.31}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.hero.place\endcsname{the largest discovery-seed gain of the 12 arms with a finished ACDC run}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.hero.pp\endcsname{\ensuremath{+0.616}}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.hero.rank\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.leader\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.leader.clause\endcsname{the top two seed-0 deltas, HyReX and HyReX with 9-kernel coarse stages, are 0.043 pp apart, a margin inside the registered 0.5 pp one-seed pair floor; ACDC is the registered guard dataset}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.margin\endcsname{0.043}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.margin.pair\endcsname{HyReX over HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.margin.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.order\endcsname{HyReX, HyReX with 9-kernel coarse stages, HyReX+context, LeanDeepMid with the two finest decoder convolutions restored, ResEnc-M (library preset), ResEnc+context, ResEnc-matched (re-implemented), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), function-identical control, ConvNeXt-k3, LeanAdd with coarse large kernels (LeanAdd-NeXt), LeanAdd-NeXt with the coarse operator at stage 5 alone}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.order.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.order.n\endcsname{12}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.order.universe\endcsname{every registered arm with a finished ACDC run, the library preset and the matched controls included}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.others.n\endcsname{11}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.others.top\endcsname{HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.others.top.pp\endcsname{\ensuremath{+0.573}}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.rank.clause\endcsname{HyReX records the largest seed-0 gain of the 12 evaluated arms, \ensuremath{+0.616} pp, 0.043 pp ahead of HyReX with 9-kernel coarse stages; that gap is inside the registered 0.5 pp floor and 0.31 of the one-seed pair SD of ACDC (0.14 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.second\endcsname{HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.second.clause\endcsname{HyReX with 9-kernel coarse stages, the second-largest delta at \ensuremath{+0.573} pp, is also a HyReX design}
\expandafter\gdef\csname R@an.cost_accuracy.acdc.second.family\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.C1.acdc\endcsname{10.26}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.C1.amos\endcsname{11.14}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.C1.kits\endcsname{9.08}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.D1.acdc\endcsname{10.37}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.D1.amos\endcsname{10.69}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.D1.kits\endcsname{9.51}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.D2.acdc\endcsname{9.45}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.D2.amos\endcsname{8.14}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.D2.kits\endcsname{7.76}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.L1.acdc\endcsname{10.46}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.L1.amos\endcsname{10.93}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.L1.kits\endcsname{9.73}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.L1b.acdc\endcsname{10.56}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.L1b.amos\endcsname{10.60}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.L1b.kits\endcsname{9.43}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.L2.acdc\endcsname{11.42}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.L2.amos\endcsname{9.93}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.L2.kits\endcsname{9.12}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.L3.acdc\endcsname{10.43}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.L3.amos\endcsname{10.74}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.L3.kits\endcsname{9.56}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.L4.acdc\endcsname{10.27}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.L4.amos\endcsname{10.75}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.L4.kits\endcsname{9.52}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.L6.acdc\endcsname{11.49}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.L6.amos\endcsname{10.27}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.L6.kits\endcsname{9.33}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.P3c.acdc\endcsname{10.29}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.P3c.amos\endcsname{9.01}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.P3c.kits\endcsname{8.52}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.S2.acdc\endcsname{11.72}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.S2.amos\endcsname{10.48}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.S2.kits\endcsname{9.42}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V5A5.acdc\endcsname{11.74}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V5A5.amos\endcsname{9.99}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V5A5.kits\endcsname{8.89}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V5B1.acdc\endcsname{9.03}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V5B1.amos\endcsname{7.94}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V5B1.kits\endcsname{7.64}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V5B2.acdc\endcsname{9.25}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V5B2.amos\endcsname{8.02}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V5B2.kits\endcsname{7.68}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V6A1r.acdc\endcsname{10.43}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V6A1r.amos\endcsname{10.75}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V6A1r.kits\endcsname{9.57}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V7A1.acdc\endcsname{9.89}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V7A1.amos\endcsname{8.59}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V7A1.kits\endcsname{8.02}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V7A2.acdc\endcsname{10.78}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V7A2.amos\endcsname{9.34}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V7A2.kits\endcsname{8.69}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V7B1.acdc\endcsname{9.28}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V7B1.amos\endcsname{8.03}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V7B1.kits\endcsname{7.69}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V7B2.acdc\endcsname{9.25}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V7B2.amos\endcsname{8.02}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V7B2.kits\endcsname{7.68}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V7C1.acdc\endcsname{9.08}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V7C1.amos\endcsname{7.95}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V7C1.kits\endcsname{7.65}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V8A1.acdc\endcsname{9.29}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V8A1.amos\endcsname{8.04}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V8A1.kits\endcsname{7.72}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V8A2.acdc\endcsname{9.25}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V8A2.amos\endcsname{8.05}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V8A2.kits\endcsname{7.73}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V8B1.acdc\endcsname{8.17}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V8B1.amos\endcsname{7.17}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V8B1.kits\endcsname{6.96}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V8B2.acdc\endcsname{8.49}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V8B2.amos\endcsname{7.45}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.V8B2.kits\endcsname{7.11}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W1.acdc\endcsname{10.73}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W1.amos\endcsname{9.40}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W1.kits\endcsname{8.72}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W1c.acdc\endcsname{10.73}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W1c.amos\endcsname{9.40}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W1c.kits\endcsname{8.72}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W2.acdc\endcsname{10.74}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W2.amos\endcsname{9.41}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W2.kits\endcsname{8.73}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W3.acdc\endcsname{10.61}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W3.amos\endcsname{9.29}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W3.kits\endcsname{8.70}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W3c.acdc\endcsname{11.04}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W3c.amos\endcsname{9.50}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W3c.kits\endcsname{8.50}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W4.acdc\endcsname{10.76}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W4.amos\endcsname{10.51}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W4.kits\endcsname{9.45}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W5.acdc\endcsname{10.66}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W5.amos\endcsname{10.69}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.W5.kits\endcsname{9.47}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.base.acdc\endcsname{10.27}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.base.amos\endcsname{9.01}
\expandafter\gdef\csname R@an.cost_accuracy.alloc.base.kits\endcsname{8.51}
\expandafter\gdef\csname R@an.cost_accuracy.amos.atdefault.best\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.cost_accuracy.amos.atdefault.best.pp\endcsname{\ensuremath{+0.194}}
\expandafter\gdef\csname R@an.cost_accuracy.amos.atdefault.clause\endcsname{the largest AMOS22 fresh-seed gain among the 2 registered arms with a complete fresh pair at or below the default's 31.12 M parameters on the AMOS22 plan is that of ConvNeXt-k3, \ensuremath{+0.194} pp, then that of HyReX, \ensuremath{+0.132} pp (0.062 pp behind, 0.51 SD of the null of a difference of two-seed means, inside its 0.24 pp edge)}
\expandafter\gdef\csname R@an.cost_accuracy.amos.atdefault.hero.behind\endcsname{0.062}
\expandafter\gdef\csname R@an.cost_accuracy.amos.atdefault.hero.pp\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.cost_accuracy.amos.atdefault.hero.rank\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.amos.atdefault.licence\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.amos.atdefault.margin\endcsname{0.062}
\expandafter\gdef\csname R@an.cost_accuracy.amos.atdefault.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.amos.atdefault.names\endcsname{ConvNeXt-k3, HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.amos.atdefault.second\endcsname{HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.amos.atdefault.universe\endcsname{the 2 registered arms with a complete fresh pair at or below the default's 31.12 M parameters on the AMOS22 plan}
\expandafter\gdef\csname R@an.cost_accuracy.amos.best\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.amos.best.clause\endcsname{ResEnc-M (library preset), the highest seed-0 delta among the 31 registered arms with a finished AMOS22 run (the library preset and the matched controls included), 0.055 pp ahead of pooled-skip control, a margin inside the registered 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.amos.floor.arms\endcsname{ResEnc-M (library preset), pooled-skip control}
\expandafter\gdef\csname R@an.cost_accuracy.amos.floor.clause\endcsname{2 of the 31 evaluated AMOS22 arms have a seed-0 margin over the default that clears the registered 0.5 pp one-seed pair floor: ResEnc-M (library preset), pooled-skip control}
\expandafter\gdef\csname R@an.cost_accuracy.amos.floor.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.amos.floor.of\endcsname{31}
\expandafter\gdef\csname R@an.cost_accuracy.amos.fresh.best\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.amos.fresh.best.pp\endcsname{\ensuremath{+0.465}}
\expandafter\gdef\csname R@an.cost_accuracy.amos.fresh.leader\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.amos.fresh.licence\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.amos.fresh.margin\endcsname{0.010}
\expandafter\gdef\csname R@an.cost_accuracy.amos.fresh.margin.edge\endcsname{0.24}
\expandafter\gdef\csname R@an.cost_accuracy.amos.fresh.margin.sd\endcsname{0.08}
\expandafter\gdef\csname R@an.cost_accuracy.amos.fresh.second\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.cost_accuracy.amos.fresh.second.pp\endcsname{\ensuremath{+0.455}}
\expandafter\gdef\csname R@an.cost_accuracy.amos.fresh.super\endcsname{over the 5 of 31 finished arms that have a fresh mean}
\expandafter\gdef\csname R@an.cost_accuracy.amos.fresh.top.clause\endcsname{the two highest AMOS22 fresh means are ResEnc-M (library preset) at \ensuremath{+0.465} pp and ResEnc+context at \ensuremath{+0.455} pp, 0.010 pp apart (0.08 SD of the null of a difference of two-seed means, inside its 0.24 pp edge), over the 5 of 31 finished arms that have a fresh mean}
\expandafter\gdef\csname R@an.cost_accuracy.amos.leader\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.amos.leader.clause\endcsname{the top two seed-0 deltas, ResEnc-M (library preset) and pooled-skip control, are 0.055 pp apart, a margin inside the registered 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.amos.margin\endcsname{0.055}
\expandafter\gdef\csname R@an.cost_accuracy.amos.margin.pair\endcsname{ResEnc-M (library preset) over pooled-skip control}
\expandafter\gdef\csname R@an.cost_accuracy.amos.margin.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.amos.order\endcsname{ResEnc-M (library preset), pooled-skip control, HyReX with 9-kernel coarse stages, ResEnc+context, HyReX + decoder capacity, HyReX, HyReX, ConvNeXt one stage finer, branch control, ConvNeXt-k3, LeanDeepMid with the two finest decoder convolutions restored, HyReX point-fuse decoder, offset upsampling, thickness-gated mixing, trilinear-decoder control, ResEnc-matched (re-implemented), LeanAdd with coarse large kernels (LeanAdd-NeXt), $z$-dilation mixing, ConvNeXt-4$\times$-GRN (MedNeXt-like reference), HyReX with LeanDec fine decoder stages, HyReX+context, function-identical control, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanDec (default with one conv per decoder stage), LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk)}
\expandafter\gdef\csname R@an.cost_accuracy.amos.order.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.amos.order.n\endcsname{31}
\expandafter\gdef\csname R@an.cost_accuracy.amos.order.universe\endcsname{every registered arm with a finished AMOS22 run, the library preset and the matched controls included}
\expandafter\gdef\csname R@an.cost_accuracy.amos.second\endcsname{pooled-skip control}
\expandafter\gdef\csname R@an.cost_accuracy.amos.second.clause\endcsname{pooled-skip control is second, at \ensuremath{+0.591} pp}
\expandafter\gdef\csname R@an.cost_accuracy.amos.second.family\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.C1.acdc\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.C1.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.C1.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.D1.acdc\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.D1.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.D1.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.D2.acdc\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.D2.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.D2.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.L1.acdc\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.L1.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.L1.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.L1b.acdc\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.L1b.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.L1b.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.L2.acdc\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.L2.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.L2.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.L3.acdc\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.L3.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.L3.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.L4.acdc\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.L4.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.L4.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.L6.acdc\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.L6.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.L6.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.P3c.acdc\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.P3c.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.P3c.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.S2.acdc\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.S2.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.S2.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V5A5.acdc\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V5A5.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V5A5.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V5B1.acdc\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V5B1.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V5B1.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V5B2.acdc\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V5B2.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V5B2.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V6A1r.acdc\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V6A1r.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V6A1r.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V7A1.acdc\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V7A1.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V7A1.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V7A2.acdc\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V7A2.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V7A2.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V7B1.acdc\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V7B1.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V7B1.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V7B2.acdc\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V7B2.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V7B2.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V7C1.acdc\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V7C1.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V7C1.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V8A1.acdc\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V8A1.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V8A1.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V8A2.acdc\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V8A2.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V8A2.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V8B1.acdc\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V8B1.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V8B1.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V8B2.acdc\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V8B2.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.V8B2.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W1.acdc\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W1.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W1.kits\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W1c.acdc\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W1c.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W1c.kits\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W2.acdc\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W2.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W2.kits\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W3.acdc\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W3.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W3.kits\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W3c.acdc\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W3c.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W3c.kits\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W4.acdc\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W4.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W4.kits\endcsname{registered, queued}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W5.acdc\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W5.amos\endcsname{finished}
\expandafter\gdef\csname R@an.cost_accuracy.armstate.W5.kits\endcsname{not run on this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.band.acdc\endcsname{0.21}
\expandafter\gdef\csname R@an.cost_accuracy.band.amos\endcsname{0.26}
\expandafter\gdef\csname R@an.cost_accuracy.band.kits\endcsname{1.84}
\expandafter\gdef\csname R@an.cost_accuracy.breakeven.L1.acdc\endcsname{1.585}
\expandafter\gdef\csname R@an.cost_accuracy.breakeven.L1.amos\endcsname{0.457}
\expandafter\gdef\csname R@an.cost_accuracy.breakeven.L1.kits\endcsname{7.223}
\expandafter\gdef\csname R@an.cost_accuracy.breakeven.acdc\endcsname{0.069}
\expandafter\gdef\csname R@an.cost_accuracy.breakeven.acdc.clause\endcsname{on ACDC ResEnc-M would need 1.585 pp to reach HyReX's return per parameter, and HyReX's return exceeds ResEnc-M's for any HyReX gain above 0.069 pp}
\expandafter\gdef\csname R@an.cost_accuracy.breakeven.amos\endcsname{0.134}
\expandafter\gdef\csname R@an.cost_accuracy.breakeven.argument.clause\endcsname{on KiTS23 ResEnc-M would need 7.223 pp to reach HyReX's return per parameter, and HyReX's return exceeds ResEnc-M's for any HyReX gain above 1.007 pp; on ACDC ResEnc-M would need 1.585 pp to reach HyReX's return per parameter, and HyReX's return exceeds ResEnc-M's for any HyReX gain above 0.069 pp}
\expandafter\gdef\csname R@an.cost_accuracy.breakeven.argument.datasets\endcsname{KiTS23 and ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.breakeven.kits\endcsname{1.007}
\expandafter\gdef\csname R@an.cost_accuracy.breakeven.kits.clause\endcsname{on KiTS23 ResEnc-M would need 7.223 pp to reach HyReX's return per parameter, and HyReX's return exceeds ResEnc-M's for any HyReX gain above 1.007 pp}
\expandafter\gdef\csname R@an.cost_accuracy.bubblekey\endcsname{25 / 50 / 100}
\expandafter\gdef\csname R@an.cost_accuracy.c30.acdc.moved\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.c30.acdc.n\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.c30.acdc.shift\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.cost_accuracy.c30.acdc.shiftabs\endcsname{0.007}
\expandafter\gdef\csname R@an.cost_accuracy.c30.amos.moved\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.c30.amos.n\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.c30.amos.shift\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.cost_accuracy.c30.amos.shiftabs\endcsname{0.029}
\expandafter\gdef\csname R@an.cost_accuracy.c30.kits.moved\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.c30.kits.n\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.c30.kits.shift\endcsname{\ensuremath{0.000}}
\expandafter\gdef\csname R@an.cost_accuracy.c30.kits.shiftabs\endcsname{0.000}
\expandafter\gdef\csname R@an.cost_accuracy.cap.acdc\endcsname{12}
\expandafter\gdef\csname R@an.cost_accuracy.cap.amos\endcsname{12}
\expandafter\gdef\csname R@an.cost_accuracy.cap.kits\endcsname{12}
\expandafter\gdef\csname R@an.cost_accuracy.caption.encoding\endcsname{Hollow marks are the discovery seed (seed 0), small dots the finished fresh seeds and filled marks the fresh mean of seeds 1--2; two filled marks that share ink are drawn translucent, and an arm whose step lies far beyond the others is named in the panel's note and left off the axis}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.C1.kits.par\endcsname{0.51}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.C1.kits.step\endcsname{1.18}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.D2.kits.par\endcsname{0.25}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.D2.kits.step\endcsname{0.61}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.L3.acdc.par\endcsname{0.28}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.L3.acdc.step\endcsname{1.09}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.L3.kits.par\endcsname{0.29}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.L3.kits.step\endcsname{1.05}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.L6.acdc.par\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.L6.acdc.step\endcsname{1.35}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.L6.kits.par\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.L6.kits.step\endcsname{1.22}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.V6A1r.acdc.par\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.V6A1r.acdc.step\endcsname{1.20}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.V7A1.kits.par\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.V7A1.kits.step\endcsname{0.69}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.V7A2.acdc.par\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.V7A2.acdc.step\endcsname{0.81}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.V7A2.kits.par\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.V7A2.kits.step\endcsname{0.82}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.V7B2.kits.par\endcsname{0.20}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.V7B2.kits.step\endcsname{0.57}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.V7C1.kits.par\endcsname{0.21}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.V7C1.kits.step\endcsname{0.58}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.V8B1.kits.par\endcsname{0.18}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.V8B1.kits.step\endcsname{0.44}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.acdc.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.acdc.below\endcsname{ConvNeXt-k3, ResEnc+context, LeanAdd with coarse large kernels (LeanAdd-NeXt), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with the coarse operator at stage 5 alone}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.acdc.fresh.basis\endcsname{fresh-seed mean (seeds 1--2) of both arms}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.acdc.fresh.below\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.acdc.fresh.matched\endcsname{HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.acdc.fresh.n\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.acdc.highest\endcsname{HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.acdc.highest.basis\endcsname{seed 0, the discovery seed, relative to the library preset}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.acdc.highest.clause\endcsname{HyReX, the largest seed-0 delta among the 9 candidate designs with a finished ACDC run (the candidate set excludes the library preset and the matched controls), at \ensuremath{+0.281} pp relative to the preset and 0.043 pp ahead of HyReX with 9-kernel coarse stages, a margin inside the registered 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.acdc.highest.gap\endcsname{\ensuremath{+0.281}}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.acdc.highest.n\endcsname{9}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.acdc.highest.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.acdc.highest.universe\endcsname{the 9 candidate designs with a finished ACDC run -- the arms a selection decision could have picked, which excludes the library preset and the matched controls}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.acdc.matched\endcsname{HyReX, HyReX+context, HyReX with 9-kernel coarse stages, LeanDeepMid with the two finest decoder convolutions restored}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.acdc.nreversed\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.acdc.pending\endcsname{$z$-dilation mixing, thickness-gated mixing, offset upsampling, HyReX + decoder capacity, HyReX point-fuse decoder, LeanDec (default with one conv per decoder stage), HyReX, ConvNeXt one stage finer, HyReX with LeanDec fine decoder stages, LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1)}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.acdc.reversed\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.amos.below\endcsname{ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context, $z$-dilation mixing, thickness-gated mixing, offset upsampling, HyReX + decoder capacity, HyReX point-fuse decoder, LeanDec (default with one conv per decoder stage), HyReX, ConvNeXt one stage finer, HyReX with LeanDec fine decoder stages, LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with 9-kernel coarse stages, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1)}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.amos.fresh.basis\endcsname{fresh-seed mean (seeds 1--2) of both arms}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.amos.fresh.below\endcsname{ConvNeXt-k3, HyReX, ResEnc+context}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.amos.fresh.matched\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.amos.fresh.n\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.amos.highest\endcsname{HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.amos.highest.basis\endcsname{seed 0, the discovery seed, relative to the library preset}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.amos.highest.clause\endcsname{HyReX with 9-kernel coarse stages, the largest seed-0 delta among the 24 candidate designs with a finished AMOS22 run (the candidate set excludes the library preset and the matched controls), at \ensuremath{-0.160} pp relative to the preset and 0.057 pp ahead of ResEnc+context, a margin inside the registered 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.amos.highest.gap\endcsname{\ensuremath{-0.160}}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.amos.highest.n\endcsname{24}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.amos.highest.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.amos.highest.universe\endcsname{the 24 candidate designs with a finished AMOS22 run -- the arms a selection decision could have picked, which excludes the library preset and the matched controls}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.amos.matched\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.amos.nreversed\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.amos.pending\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.amos.reversed\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.kits.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.kits.below\endcsname{ConvNeXt-k3, ResEnc+context, HyReX point-fuse decoder, HyReX, ConvNeXt one stage finer, HyReX with LeanDec fine decoder stages, LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with 9-kernel coarse stages, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1)}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.kits.fresh.basis\endcsname{fresh-seed mean (seeds 1--2) of both arms}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.kits.fresh.below\endcsname{ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context, HyReX + decoder capacity, HyReX point-fuse decoder, LeanDec (default with one conv per decoder stage), HyReX, ConvNeXt one stage finer, HyReX with LeanDec fine decoder stages, LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with 9-kernel coarse stages, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1)}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.kits.fresh.matched\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.kits.fresh.n\endcsname{21}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.kits.highest\endcsname{HyReX + decoder capacity}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.kits.highest.basis\endcsname{seed 0, the discovery seed, relative to the library preset}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.kits.highest.clause\endcsname{HyReX + decoder capacity, the largest seed-0 delta among the 21 candidate designs with a finished KiTS23 run (the candidate set excludes the library preset and the matched controls), at \ensuremath{+1.181} pp relative to the preset and 0.596 pp ahead of LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), a margin above the registered 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.kits.highest.gap\endcsname{\ensuremath{+1.181}}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.kits.highest.n\endcsname{21}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.kits.highest.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.kits.highest.universe\endcsname{the 21 candidate designs with a finished KiTS23 run -- the arms a selection decision could have picked, which excludes the library preset and the matched controls}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.kits.matched\endcsname{HyReX, HyReX+context, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk)}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.kits.nreversed\endcsname{9}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.kits.pending\endcsname{$z$-dilation mixing, thickness-gated mixing, offset upsampling}
\expandafter\gdef\csname R@an.cost_accuracy.ctm.kits.reversed\endcsname{HyReX, HyReX+context, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk)}
\expandafter\gdef\csname R@an.cost_accuracy.delta.C1.amos\endcsname{\ensuremath{+0.390}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.C1.kits\endcsname{\ensuremath{+3.507}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.D1.amos\endcsname{\ensuremath{+0.278}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.D1.kits\endcsname{\ensuremath{+1.607}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.D2.amos\endcsname{\ensuremath{-0.362}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.D2.kits\endcsname{\ensuremath{+2.355}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.L1.acdc\endcsname{\ensuremath{+0.336}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.L1.amos\endcsname{\ensuremath{+0.647}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.L1.kits\endcsname{\ensuremath{+2.326}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.L1b.acdc\endcsname{\ensuremath{+0.283}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.L1b.amos\endcsname{\ensuremath{+0.138}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.L1b.kits\endcsname{\ensuremath{+1.743}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.L2.acdc\endcsname{\ensuremath{-0.015}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.L2.amos\endcsname{\ensuremath{+0.362}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.L2.kits\endcsname{\ensuremath{+0.664}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.L3.acdc\endcsname{\ensuremath{+0.616}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.L3.amos\endcsname{\ensuremath{+0.382}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.L3.kits\endcsname{\ensuremath{+2.842}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.L4.acdc\endcsname{\ensuremath{+0.315}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.L4.amos\endcsname{\ensuremath{+0.430}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.L4.kits\endcsname{\ensuremath{+2.198}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.L6.acdc\endcsname{\ensuremath{+0.451}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.L6.amos\endcsname{\ensuremath{+0.016}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.L6.kits\endcsname{\ensuremath{+2.526}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.P3c.acdc\endcsname{\ensuremath{-0.013}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.P3c.amos\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.P3c.kits\endcsname{\ensuremath{+1.364}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.S2.amos\endcsname{\ensuremath{+0.378}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.S2.kits\endcsname{\ensuremath{+1.341}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V5A5.amos\endcsname{\ensuremath{+0.041}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V5A5.kits\endcsname{\ensuremath{+1.949}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V5B1.amos\endcsname{\ensuremath{-0.261}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V5B1.kits\endcsname{\ensuremath{+2.162}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V5B2.acdc\endcsname{\ensuremath{-0.181}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V5B2.amos\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V5B2.kits\endcsname{\ensuremath{+1.264}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V6A1r.acdc\endcsname{\ensuremath{+0.573}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V6A1r.amos\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V6A1r.kits\endcsname{\ensuremath{+2.236}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V7A1.acdc\endcsname{\ensuremath{+0.229}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V7A1.amos\endcsname{\ensuremath{-0.045}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V7A1.kits\endcsname{\ensuremath{+2.548}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V7A2.acdc\endcsname{\ensuremath{+0.362}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V7A2.amos\endcsname{\ensuremath{+0.359}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V7A2.kits\endcsname{\ensuremath{+2.886}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V7B1.amos\endcsname{\ensuremath{-0.436}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V7B1.kits\endcsname{\ensuremath{+1.721}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V7B2.amos\endcsname{\ensuremath{-0.267}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V7B2.kits\endcsname{\ensuremath{+2.824}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V7C1.acdc\endcsname{\ensuremath{-0.252}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V7C1.amos\endcsname{\ensuremath{-0.106}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V7C1.kits\endcsname{\ensuremath{+2.707}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V8A1.amos\endcsname{\ensuremath{-0.505}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V8A1.kits\endcsname{\ensuremath{+1.760}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V8A2.amos\endcsname{\ensuremath{-0.312}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V8A2.kits\endcsname{\ensuremath{+1.353}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V8B1.amos\endcsname{\ensuremath{-0.751}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V8B1.kits\endcsname{\ensuremath{+2.911}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V8B2.amos\endcsname{\ensuremath{-0.287}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.V8B2.kits\endcsname{\ensuremath{+1.646}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.W1.amos\endcsname{\ensuremath{+0.099}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.W1c.amos\endcsname{\ensuremath{+0.363}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.W1c.kits\endcsname{\ensuremath{+2.636}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.W2.amos\endcsname{\ensuremath{+0.211}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.W3.amos\endcsname{\ensuremath{+0.270}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.W3c.amos\endcsname{\ensuremath{+0.162}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.W4.amos\endcsname{\ensuremath{+0.076}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.W5.amos\endcsname{\ensuremath{+0.591}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.base.acdc\endcsname{\ensuremath{0.000}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.base.amos\endcsname{\ensuremath{0.000}}
\expandafter\gdef\csname R@an.cost_accuracy.delta.base.kits\endcsname{\ensuremath{0.000}}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.C1.amos\endcsname{3.2}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.C1.kits\endcsname{4.4}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.D1.amos\endcsname{2.3}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.D1.kits\endcsname{2.0}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.D2.amos\endcsname{-3.0}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.D2.kits\endcsname{3.0}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.L1.acdc\endcsname{3.4}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.L1.amos\endcsname{5.3}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.L1.kits\endcsname{2.9}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.L1b.acdc\endcsname{2.9}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.L1b.amos\endcsname{1.1}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.L1b.kits\endcsname{2.2}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.L2.acdc\endcsname{-0.1}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.L2.amos\endcsname{3.0}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.L2.kits\endcsname{0.8}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.L3.acdc\endcsname{6.2}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.L3.amos\endcsname{3.1}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.L3.kits\endcsname{3.6}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.L4.acdc\endcsname{3.2}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.L4.amos\endcsname{3.5}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.L4.kits\endcsname{2.8}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.L6.acdc\endcsname{4.6}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.L6.amos\endcsname{0.1}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.L6.kits\endcsname{3.2}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.P3c.acdc\endcsname{-0.1}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.P3c.amos\endcsname{0.1}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.P3c.kits\endcsname{1.7}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.S2.amos\endcsname{3.1}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.S2.kits\endcsname{1.7}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V5A5.amos\endcsname{0.3}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V5A5.kits\endcsname{2.5}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V5B1.amos\endcsname{-2.1}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V5B1.kits\endcsname{2.7}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V5B2.acdc\endcsname{-1.8}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V5B2.amos\endcsname{1.1}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V5B2.kits\endcsname{1.6}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V6A1r.acdc\endcsname{5.8}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V6A1r.amos\endcsname{4.0}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V6A1r.kits\endcsname{2.8}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V7A1.acdc\endcsname{2.3}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V7A1.amos\endcsname{-0.4}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V7A1.kits\endcsname{3.2}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V7A2.acdc\endcsname{3.7}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V7A2.amos\endcsname{2.9}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V7A2.kits\endcsname{3.6}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V7B1.amos\endcsname{-3.6}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V7B1.kits\endcsname{2.2}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V7B2.amos\endcsname{-2.2}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V7B2.kits\endcsname{3.6}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V7C1.acdc\endcsname{-2.6}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V7C1.amos\endcsname{-0.9}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V7C1.kits\endcsname{3.4}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V8A1.amos\endcsname{-4.1}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V8A1.kits\endcsname{2.2}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V8A2.amos\endcsname{-2.6}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V8A2.kits\endcsname{1.7}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V8B1.amos\endcsname{-6.1}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V8B1.kits\endcsname{3.7}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V8B2.amos\endcsname{-2.4}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.V8B2.kits\endcsname{2.1}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.W1.amos\endcsname{0.8}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.W1c.amos\endcsname{3.0}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.W1c.kits\endcsname{3.3}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.W2.amos\endcsname{1.7}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.W3.amos\endcsname{2.2}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.W3c.amos\endcsname{1.3}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.W4.amos\endcsname{0.6}
\expandafter\gdef\csname R@an.cost_accuracy.deltasd.W5.amos\endcsname{4.8}
\expandafter\gdef\csname R@an.cost_accuracy.floor.acdc.basis\endcsname{fresh mean (seeds 1-2)}
\expandafter\gdef\csname R@an.cost_accuracy.floor.acdc.kind\endcsname{no resolution band, the guard dataset being read descriptively}
\expandafter\gdef\csname R@an.cost_accuracy.floor.amos.basis\endcsname{fresh mean (seeds 1-2)}
\expandafter\gdef\csname R@an.cost_accuracy.floor.amos.half\endcsname{0.24}
\expandafter\gdef\csname R@an.cost_accuracy.floor.amos.kind\endcsname{two-seed null of this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.floor.device.summary\endcsname{(a) the two-seed null of AMOS22, $\pm$0.24 pp; (b) the two-seed null of KiTS23, $\pm$1.56 pp; (c) no resolution band, the guard dataset being read descriptively}
\expandafter\gdef\csname R@an.cost_accuracy.floor.kits.basis\endcsname{fresh mean (seeds 1-2)}
\expandafter\gdef\csname R@an.cost_accuracy.floor.kits.half\endcsname{1.56}
\expandafter\gdef\csname R@an.cost_accuracy.floor.kits.kind\endcsname{two-seed null of this dataset}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.C1.kits\endcsname{\ensuremath{+2.401}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.C1.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.C1.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.C1.kits.se\endcsname{0.273}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.C1.kits.seeds\endcsname{\ensuremath{+2.128} and \ensuremath{+2.674}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.C1.kits.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.C1.kits.spread\endcsname{0.546}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.C1.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.C1.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.C1.kits.z\endcsname{3.31}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D1.kits\endcsname{\ensuremath{+1.477}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D1.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D1.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D1.kits.se\endcsname{0.283}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D1.kits.seeds\endcsname{\ensuremath{+1.759} and \ensuremath{+1.194}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D1.kits.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D1.kits.spread\endcsname{0.565}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D1.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D1.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D1.kits.z\endcsname{2.03}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D2.kits\endcsname{\ensuremath{+1.892}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D2.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D2.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D2.kits.se\endcsname{0.088}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D2.kits.seeds\endcsname{\ensuremath{+1.979} and \ensuremath{+1.804}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D2.kits.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D2.kits.spread\endcsname{0.175}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D2.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D2.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.D2.kits.z\endcsname{2.61}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.acdc\endcsname{\ensuremath{+0.242}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.acdc.nullsd\endcsname{0.081}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.acdc.z\endcsname{3.00}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.amos\endcsname{\ensuremath{+0.465}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.amos.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.amos.nullsd\endcsname{0.100}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.amos.se\endcsname{0.197}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.amos.seeds\endcsname{\ensuremath{+0.662} and \ensuremath{+0.268}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.amos.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.amos.spread\endcsname{0.394}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.amos.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.amos.unc\endcsname{\ensuremath{+0.436}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.amos.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.amos.z\endcsname{4.66}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.kits\endcsname{\ensuremath{+3.475}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.kits.se\endcsname{0.342}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.kits.seeds\endcsname{\ensuremath{+3.134} and \ensuremath{+3.817}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.kits.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.kits.spread\endcsname{0.683}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1.kits.z\endcsname{4.79}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.acdc\endcsname{\ensuremath{+0.319}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.acdc.nullsd\endcsname{0.081}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.acdc.z\endcsname{3.95}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.amos\endcsname{\ensuremath{+0.298}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.amos.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.amos.nullsd\endcsname{0.100}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.amos.se\endcsname{0.129}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.amos.seeds\endcsname{\ensuremath{+0.426} and \ensuremath{+0.169}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.amos.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.amos.spread\endcsname{0.257}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.amos.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.amos.unc\endcsname{\ensuremath{+0.269}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.amos.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.amos.z\endcsname{2.98}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.kits\endcsname{\ensuremath{+2.313}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.kits.se\endcsname{0.251}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.kits.seeds\endcsname{\ensuremath{+2.564} and \ensuremath{+2.062}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.kits.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.kits.spread\endcsname{0.501}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L1b.kits.z\endcsname{3.19}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.amos\endcsname{\ensuremath{+0.194}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.amos.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.amos.nullsd\endcsname{0.100}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.amos.se\endcsname{0.061}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.amos.seeds\endcsname{\ensuremath{+0.255} and \ensuremath{+0.134}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.amos.sep\endcsname{not separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.amos.spread\endcsname{0.121}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.amos.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.amos.unc\endcsname{\ensuremath{+0.166}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.amos.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.amos.z\endcsname{1.95}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.kits\endcsname{\ensuremath{+0.110}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.kits.se\endcsname{0.915}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.kits.seeds\endcsname{\ensuremath{-0.805} and \ensuremath{+1.026}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.kits.sep\endcsname{not separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.kits.spread\endcsname{1.831}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.kits.straddle\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.kits.vsse\endcsname{smaller}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L2.kits.z\endcsname{0.15}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.acdc\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.acdc.nullsd\endcsname{0.081}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.acdc.z\endcsname{5.58}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.amos\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.amos.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.amos.nullsd\endcsname{0.100}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.amos.se\endcsname{0.148}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.amos.seeds\endcsname{\ensuremath{+0.280} and \ensuremath{-0.016}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.amos.sep\endcsname{not separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.amos.spread\endcsname{0.296}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.amos.straddle\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.amos.unc\endcsname{\ensuremath{+0.104}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.amos.vsse\endcsname{smaller}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.amos.z\endcsname{1.33}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.kits\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.kits.se\endcsname{0.296}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.kits.seeds\endcsname{\ensuremath{+1.798} and \ensuremath{+2.390}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.kits.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.kits.spread\endcsname{0.592}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L3.kits.z\endcsname{2.89}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.amos\endcsname{\ensuremath{+0.455}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.amos.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.amos.nullsd\endcsname{0.100}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.amos.se\endcsname{0.102}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.amos.seeds\endcsname{\ensuremath{+0.352} and \ensuremath{+0.557}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.amos.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.amos.spread\endcsname{0.205}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.amos.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.amos.unc\endcsname{\ensuremath{+0.426}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.amos.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.amos.z\endcsname{4.56}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.kits\endcsname{\ensuremath{+2.246}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.kits.se\endcsname{0.431}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.kits.seeds\endcsname{\ensuremath{+2.677} and \ensuremath{+1.815}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.kits.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.kits.spread\endcsname{0.862}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L4.kits.z\endcsname{3.10}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L6.kits\endcsname{\ensuremath{+1.591}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L6.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L6.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L6.kits.se\endcsname{0.393}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L6.kits.seeds\endcsname{\ensuremath{+1.198} and \ensuremath{+1.984}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L6.kits.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L6.kits.spread\endcsname{0.786}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L6.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L6.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.L6.kits.z\endcsname{2.19}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.P3c.acdc\endcsname{\ensuremath{+0.117}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.P3c.acdc.nullsd\endcsname{0.081}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.P3c.acdc.z\endcsname{1.45}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.P3c.kits\endcsname{\ensuremath{+1.176}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.P3c.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.P3c.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.P3c.kits.se\endcsname{0.025}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.P3c.kits.seeds\endcsname{\ensuremath{+1.151} and \ensuremath{+1.201}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.P3c.kits.sep\endcsname{not separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.P3c.kits.spread\endcsname{0.050}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.P3c.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.P3c.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.P3c.kits.z\endcsname{1.62}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.S2.kits\endcsname{\ensuremath{+0.570}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.S2.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.S2.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.S2.kits.se\endcsname{0.212}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.S2.kits.seeds\endcsname{\ensuremath{+0.782} and \ensuremath{+0.358}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.S2.kits.sep\endcsname{not separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.S2.kits.spread\endcsname{0.425}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.S2.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.S2.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.S2.kits.z\endcsname{0.79}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5A5.kits\endcsname{\ensuremath{+2.165}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5A5.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5A5.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5A5.kits.se\endcsname{0.182}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5A5.kits.seeds\endcsname{\ensuremath{+2.348} and \ensuremath{+1.983}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5A5.kits.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5A5.kits.spread\endcsname{0.365}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5A5.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5A5.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5A5.kits.z\endcsname{2.98}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B1.kits\endcsname{\ensuremath{+2.285}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B1.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B1.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B1.kits.se\endcsname{0.043}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B1.kits.seeds\endcsname{\ensuremath{+2.242} and \ensuremath{+2.328}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B1.kits.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B1.kits.spread\endcsname{0.087}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B1.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B1.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B1.kits.z\endcsname{3.15}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B2.kits\endcsname{\ensuremath{+1.448}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B2.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B2.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B2.kits.se\endcsname{0.049}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B2.kits.seeds\endcsname{\ensuremath{+1.498} and \ensuremath{+1.399}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B2.kits.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B2.kits.spread\endcsname{0.099}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B2.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B2.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V5B2.kits.z\endcsname{2.00}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V6A1r.kits\endcsname{\ensuremath{+1.704}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V6A1r.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V6A1r.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V6A1r.kits.se\endcsname{0.009}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V6A1r.kits.seeds\endcsname{\ensuremath{+1.695} and \ensuremath{+1.713}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V6A1r.kits.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V6A1r.kits.spread\endcsname{0.018}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V6A1r.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V6A1r.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V6A1r.kits.z\endcsname{2.35}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A1.kits\endcsname{\ensuremath{+2.662}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A1.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A1.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A1.kits.se\endcsname{0.335}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A1.kits.seeds\endcsname{\ensuremath{+2.326} and \ensuremath{+2.997}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A1.kits.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A1.kits.spread\endcsname{0.671}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A1.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A1.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A1.kits.z\endcsname{3.67}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A2.kits\endcsname{\ensuremath{+2.289}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A2.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A2.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A2.kits.se\endcsname{0.316}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A2.kits.seeds\endcsname{\ensuremath{+1.973} and \ensuremath{+2.606}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A2.kits.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A2.kits.spread\endcsname{0.633}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A2.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A2.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7A2.kits.z\endcsname{3.15}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B1.kits\endcsname{\ensuremath{+2.382}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B1.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B1.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B1.kits.se\endcsname{0.329}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B1.kits.seeds\endcsname{\ensuremath{+2.053} and \ensuremath{+2.710}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B1.kits.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B1.kits.spread\endcsname{0.657}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B1.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B1.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B1.kits.z\endcsname{3.28}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B2.kits\endcsname{\ensuremath{+1.838}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B2.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B2.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B2.kits.se\endcsname{0.557}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B2.kits.seeds\endcsname{\ensuremath{+2.395} and \ensuremath{+1.282}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B2.kits.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B2.kits.spread\endcsname{1.113}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B2.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B2.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7B2.kits.z\endcsname{2.53}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7C1.amos\endcsname{pending}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7C1.kits\endcsname{\ensuremath{+2.440}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7C1.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7C1.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7C1.kits.se\endcsname{0.318}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7C1.kits.seeds\endcsname{\ensuremath{+2.758} and \ensuremath{+2.121}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7C1.kits.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7C1.kits.spread\endcsname{0.637}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7C1.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7C1.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V7C1.kits.z\endcsname{3.36}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A1.kits\endcsname{\ensuremath{+1.249}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A1.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A1.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A1.kits.se\endcsname{0.172}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A1.kits.seeds\endcsname{\ensuremath{+1.077} and \ensuremath{+1.421}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A1.kits.sep\endcsname{not separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A1.kits.spread\endcsname{0.343}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A1.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A1.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A1.kits.z\endcsname{1.72}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A2.kits\endcsname{\ensuremath{+1.877}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A2.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A2.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A2.kits.se\endcsname{0.284}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A2.kits.seeds\endcsname{\ensuremath{+1.593} and \ensuremath{+2.162}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A2.kits.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A2.kits.spread\endcsname{0.569}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A2.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A2.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8A2.kits.z\endcsname{2.59}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B1.kits\endcsname{\ensuremath{+1.375}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B1.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B1.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B1.kits.se\endcsname{0.704}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B1.kits.seeds\endcsname{\ensuremath{+2.079} and \ensuremath{+0.670}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B1.kits.sep\endcsname{not separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B1.kits.spread\endcsname{1.409}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B1.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B1.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B1.kits.z\endcsname{1.89}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B2.amos\endcsname{pending}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B2.kits\endcsname{\ensuremath{+1.731}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B2.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B2.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B2.kits.se\endcsname{0.161}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B2.kits.seeds\endcsname{\ensuremath{+1.892} and \ensuremath{+1.570}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B2.kits.sep\endcsname{separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B2.kits.spread\endcsname{0.321}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B2.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B2.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.V8B2.kits.z\endcsname{2.39}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.W1c.kits\endcsname{\ensuremath{+1.067}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.W1c.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.W1c.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.W1c.kits.se\endcsname{0.667}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.W1c.kits.seeds\endcsname{\ensuremath{+1.734} and \ensuremath{+0.399}}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.W1c.kits.sep\endcsname{not separated}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.W1c.kits.spread\endcsname{1.335}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.W1c.kits.straddle\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.W1c.kits.vsse\endcsname{larger}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.W1c.kits.z\endcsname{1.47}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.acdc.n\endcsname{4}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.acdc.npending\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.acdc.pending\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.amos.n\endcsname{5}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.amos.npending\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.amos.pending\endcsname{LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanAdd-NeXt with the coarse operator at stage 5 alone}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.kits.n\endcsname{25}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.kits.npending\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.fresh.kits.pending\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.freshnull.edge.amos\endcsname{0.24}
\expandafter\gdef\csname R@an.cost_accuracy.freshnull.edge.kits\endcsname{1.56}
\expandafter\gdef\csname R@an.cost_accuracy.freshnull.sd.acdc\endcsname{0.099}
\expandafter\gdef\csname R@an.cost_accuracy.freshnull.sd.amos\endcsname{0.122}
\expandafter\gdef\csname R@an.cost_accuracy.freshnull.sd.kits\endcsname{0.795}
\expandafter\gdef\csname R@an.cost_accuracy.freshnull.z\endcsname{1.96}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.C1.kits\endcsname{\ensuremath{-1.106}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.C1.kits.abs\endcsname{1.106}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.C1.kits.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.D1.kits\endcsname{\ensuremath{-0.131}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.D1.kits.abs\endcsname{0.131}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.D1.kits.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.D2.kits\endcsname{\ensuremath{-0.464}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.D2.kits.abs\endcsname{0.464}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.D2.kits.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L1.acdc\endcsname{\ensuremath{-0.094}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L1.acdc.abs\endcsname{0.094}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L1.acdc.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L1.amos\endcsname{\ensuremath{-0.182}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L1.amos.abs\endcsname{0.182}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L1.amos.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L1.kits\endcsname{\ensuremath{+1.149}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L1.kits.abs\endcsname{1.149}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L1.kits.dir\endcsname{up}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L1b.acdc\endcsname{\ensuremath{+0.036}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L1b.acdc.abs\endcsname{0.036}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L1b.acdc.dir\endcsname{up}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L1b.amos\endcsname{\ensuremath{+0.160}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L1b.amos.abs\endcsname{0.160}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L1b.amos.dir\endcsname{up}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L1b.kits\endcsname{\ensuremath{+0.571}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L1b.kits.abs\endcsname{0.571}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L1b.kits.dir\endcsname{up}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L2.amos\endcsname{\ensuremath{-0.168}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L2.amos.abs\endcsname{0.168}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L2.amos.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L2.kits\endcsname{\ensuremath{-0.554}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L2.kits.abs\endcsname{0.554}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L2.kits.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L3.acdc\endcsname{\ensuremath{-0.166}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L3.acdc.abs\endcsname{0.166}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L3.acdc.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L3.amos\endcsname{\ensuremath{-0.249}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L3.amos.abs\endcsname{0.249}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L3.amos.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L3.kits\endcsname{\ensuremath{-0.748}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L3.kits.abs\endcsname{0.748}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L3.kits.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L4.amos\endcsname{\ensuremath{+0.025}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L4.amos.abs\endcsname{0.025}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L4.amos.dir\endcsname{up}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L4.kits\endcsname{\ensuremath{+0.048}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L4.kits.abs\endcsname{0.048}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L4.kits.dir\endcsname{up}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L6.kits\endcsname{\ensuremath{-0.935}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L6.kits.abs\endcsname{0.935}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.L6.kits.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.P3c.acdc\endcsname{\ensuremath{+0.129}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.P3c.acdc.abs\endcsname{0.129}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.P3c.acdc.dir\endcsname{up}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.P3c.kits\endcsname{\ensuremath{-0.189}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.P3c.kits.abs\endcsname{0.189}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.P3c.kits.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.S2.kits\endcsname{\ensuremath{-0.771}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.S2.kits.abs\endcsname{0.771}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.S2.kits.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V5A5.kits\endcsname{\ensuremath{+0.216}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V5A5.kits.abs\endcsname{0.216}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V5A5.kits.dir\endcsname{up}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V5B1.kits\endcsname{\ensuremath{+0.123}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V5B1.kits.abs\endcsname{0.123}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V5B1.kits.dir\endcsname{up}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V5B2.kits\endcsname{\ensuremath{+0.184}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V5B2.kits.abs\endcsname{0.184}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V5B2.kits.dir\endcsname{up}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V6A1r.kits\endcsname{\ensuremath{-0.532}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V6A1r.kits.abs\endcsname{0.532}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V6A1r.kits.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V7A1.kits\endcsname{\ensuremath{+0.113}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V7A1.kits.abs\endcsname{0.113}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V7A1.kits.dir\endcsname{up}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V7A2.kits\endcsname{\ensuremath{-0.597}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V7A2.kits.abs\endcsname{0.597}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V7A2.kits.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V7B1.kits\endcsname{\ensuremath{+0.660}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V7B1.kits.abs\endcsname{0.660}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V7B1.kits.dir\endcsname{up}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V7B2.kits\endcsname{\ensuremath{-0.986}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V7B2.kits.abs\endcsname{0.986}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V7B2.kits.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V7C1.kits\endcsname{\ensuremath{-0.267}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V7C1.kits.abs\endcsname{0.267}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V7C1.kits.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V8A1.kits\endcsname{\ensuremath{-0.511}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V8A1.kits.abs\endcsname{0.511}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V8A1.kits.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V8A2.kits\endcsname{\ensuremath{+0.524}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V8A2.kits.abs\endcsname{0.524}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V8A2.kits.dir\endcsname{up}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V8B1.kits\endcsname{\ensuremath{-1.536}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V8B1.kits.abs\endcsname{1.536}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V8B1.kits.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V8B2.kits\endcsname{\ensuremath{+0.085}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V8B2.kits.abs\endcsname{0.085}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.V8B2.kits.dir\endcsname{up}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.W1c.kits\endcsname{\ensuremath{-1.569}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.W1c.kits.abs\endcsname{1.569}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.W1c.kits.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.acdc.absmax\endcsname{0.166}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.acdc.absmax.arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.acdc.absmax.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.acdc.absmax.scope\endcsname{every one of the 4 arms with a fresh ACDC mean, in either direction}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.acdc.max\endcsname{\ensuremath{+0.129}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.acdc.min\endcsname{\ensuremath{-0.166}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.acdc.n\endcsname{4}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.acdc.ndown\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.amos.absmax\endcsname{0.249}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.amos.absmax.arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.amos.absmax.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.amos.absmax.scope\endcsname{every one of the 5 arms with a fresh AMOS22 mean, in either direction}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.amos.max\endcsname{\ensuremath{+0.160}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.amos.min\endcsname{\ensuremath{-0.249}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.amos.n\endcsname{5}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.amos.ndown\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.kits.absmax\endcsname{1.569}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.kits.absmax.arm\endcsname{branch control}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.kits.absmax.dir\endcsname{down}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.kits.absmax.scope\endcsname{every one of the 25 arms with a fresh KiTS23 mean, in either direction}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.kits.max\endcsname{\ensuremath{+1.149}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.kits.min\endcsname{\ensuremath{-1.569}}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.kits.n\endcsname{25}
\expandafter\gdef\csname R@an.cost_accuracy.freshshift.kits.ndown\endcsname{15}
\expandafter\gdef\csname R@an.cost_accuracy.front.acdc\endcsname{LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd with coarse large kernels (LeanAdd-NeXt), nnU-Net default, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.front.acdc.ai\endcsname{LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd with coarse large kernels (LeanAdd-NeXt), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.front.acdc.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.front.acdc.cheapest\endcsname{LeanAdd-NeXt with the coarse operator at stage 5 alone}
\expandafter\gdef\csname R@an.cost_accuracy.front.acdc.clause\endcsname{The drawn ACDC 2-D front is built on seed 0, the discovery seed, for all 12 drawn arms, with the default at the origin, and holds LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd with coarse large kernels (LeanAdd-NeXt), nnU-Net default, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, HyReX; the fresh-seed mean of ResEnc-M (library preset), ResEnc-matched (re-implemented), HyReX, function-identical control, drawn beside their ring, takes no part in it}
\expandafter\gdef\csname R@an.cost_accuracy.front.acdc.fresh\endcsname{nnU-Net default, function-identical control, ResEnc-matched (re-implemented), HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.front.acdc.fresh.n\endcsname{4}
\expandafter\gdef\csname R@an.cost_accuracy.front.acdc.n\endcsname{6}
\expandafter\gdef\csname R@an.cost_accuracy.front.acdc.narms\endcsname{5}
\expandafter\gdef\csname R@an.cost_accuracy.front.acdc.nfresh\endcsname{4}
\expandafter\gdef\csname R@an.cost_accuracy.front.acdc.nunrep\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.front.acdc.s0\endcsname{LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd with coarse large kernels (LeanAdd-NeXt), nnU-Net default, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.front.acdc.unrep\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.front.amos\endcsname{nnU-Net default, ResEnc-matched (re-implemented), ResEnc+context, ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.front.amos.ai\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.cost_accuracy.front.amos.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.front.amos.cheapest\endcsname{nnU-Net default}
\expandafter\gdef\csname R@an.cost_accuracy.front.amos.clause\endcsname{The drawn AMOS22 2-D front is built on the fresh-seed mean (seeds 1--2) of the 5 arms that have one, with the default at the origin, and holds nnU-Net default, ResEnc-matched (re-implemented), ResEnc+context, ResEnc-M (library preset); the 26 arms drawn as rings at their discovery seed take no part in it}
\expandafter\gdef\csname R@an.cost_accuracy.front.amos.fresh\endcsname{nnU-Net default, ResEnc-matched (re-implemented), ResEnc+context, ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.front.amos.fresh.n\endcsname{4}
\expandafter\gdef\csname R@an.cost_accuracy.front.amos.n\endcsname{4}
\expandafter\gdef\csname R@an.cost_accuracy.front.amos.narms\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.front.amos.nfresh\endcsname{5}
\expandafter\gdef\csname R@an.cost_accuracy.front.amos.nunrep\endcsname{26}
\expandafter\gdef\csname R@an.cost_accuracy.front.amos.s0\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd with coarse large kernels (LeanAdd-NeXt), trilinear-decoder control, offset upsampling, branch control, pooled-skip control, ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.front.amos.unrep\endcsname{HyReX+context, $z$-dilation mixing, branch control, thickness-gated mixing, offset upsampling, trilinear-decoder control, ConvNeXt-4$\times$-GRN (MedNeXt-like reference), pooled-skip control, HyReX, ConvNeXt one stage finer, HyReX point-fuse decoder, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), function-identical control, LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with LeanDec fine decoder stages, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with the coarse operator at stage 5 alone, HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.front.cheapest.clause\endcsname{the cheapest points of the 2-D fronts are nnU-Net default on AMOS22, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk) on KiTS23 and LeanAdd-NeXt with the coarse operator at stage 5 alone on ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.front.kits\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.front.kits.ai\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid)}
\expandafter\gdef\csname R@an.cost_accuracy.front.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.front.kits.cheapest\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk)}
\expandafter\gdef\csname R@an.cost_accuracy.front.kits.clause\endcsname{The drawn KiTS23 2-D front is built on the fresh-seed mean (seeds 1--2) of the 25 arms that have one, with the default at the origin, and holds LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.front.kits.fresh\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.front.kits.fresh.n\endcsname{6}
\expandafter\gdef\csname R@an.cost_accuracy.front.kits.n\endcsname{6}
\expandafter\gdef\csname R@an.cost_accuracy.front.kits.narms\endcsname{6}
\expandafter\gdef\csname R@an.cost_accuracy.front.kits.nfresh\endcsname{25}
\expandafter\gdef\csname R@an.cost_accuracy.front.kits.nunrep\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.front.kits.s0\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), HyReX + decoder capacity}
\expandafter\gdef\csname R@an.cost_accuracy.front.kits.unrep\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all\endcsname{LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd with coarse large kernels (LeanAdd-NeXt), ConvNeXt-k3, HyReX, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, nnU-Net default}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.clause\endcsname{On seed 0, the discovery seed, over the 12 registered arms with a finished ACDC run and the default at the origin, the (parameters, profiled step time, gain) front on ACDC holds LeanAdd-NeXt with the coarse operator at stage 5 alone as the fewest-parameter and cheapest-step endpoint, LeanAdd with coarse large kernels (LeanAdd-NeXt) as an interior point, ConvNeXt-k3 as an interior point, HyReX as the largest-gain endpoint, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid) as an interior point, LeanDeepMid with the two finest decoder convolutions restored as an interior point and nnU-Net default as an interior point; ResEnc-M (library preset), ResEnc-matched (re-implemented), ResEnc+context, HyReX+context, function-identical control and HyReX with 9-kernel coarse stages are dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.dom.L1.margin\endcsname{0.026}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.dom.L1.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.dom.L1b.margin\endcsname{0.078}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.dom.L1b.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.dom.L4.margin\endcsname{0.046}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.dom.L4.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.dom.L6.margin\endcsname{0.165}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.dom.L6.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.dom.P3c.margin\endcsname{0.013}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.dom.P3c.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.dom.V6A1r.margin\endcsname{0.043}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.dom.V6A1r.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.dominated\endcsname{ResEnc-M (library preset), ResEnc-matched (re-implemented), ResEnc+context, HyReX+context, function-identical control, HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.endpoints\endcsname{LeanAdd-NeXt with the coarse operator at stage 5 alone, HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.hero\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.hero.clause\endcsname{HyReX is on the ACDC (parameters, profiled step time, gain) front as the largest-gain endpoint and dominates HyReX+context and HyReX with 9-kernel coarse stages (2 of the 12 other points)}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.hero.dominates\endcsname{HyReX+context, HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.hero.ndominates\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.hero.notdominated\endcsname{nnU-Net default, ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context, function-identical control, LeanAdd with coarse large kernels (LeanAdd-NeXt), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with the coarse operator at stage 5 alone}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.interior\endcsname{LeanAdd with coarse large kernels (LeanAdd-NeXt), ConvNeXt-k3, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, nnU-Net default}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.n\endcsname{7}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.ndominated\endcsname{6}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.nendpoints\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.ninterior\endcsname{5}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.role.L1\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.role.L1b\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.role.L2\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.role.L3\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.role.L3.ext\endcsname{the largest-gain endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.role.L4\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.role.L6\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.role.P3c\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.role.V5B2\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.role.V6A1r\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.role.V7A1\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.role.V7A2\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.role.V7C1\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.role.V7C1.ext\endcsname{the fewest-parameter and cheapest-step endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.all.role.base\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.basis.short\endcsname{seed 0}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.edge\endcsname{0.50}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.n\endcsname{12}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params\endcsname{LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd with coarse large kernels (LeanAdd-NeXt), ConvNeXt-k3, HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.clause\endcsname{On seed 0, the discovery seed, over the 12 registered arms with a finished ACDC run and the default at the origin, the (parameters, gain) front on ACDC holds LeanAdd-NeXt with the coarse operator at stage 5 alone as the fewest-parameter endpoint, LeanAdd with coarse large kernels (LeanAdd-NeXt) as an interior point, ConvNeXt-k3 as an interior point and HyReX as the largest-gain endpoint; nnU-Net default, ResEnc-M (library preset), ResEnc-matched (re-implemented), ResEnc+context, HyReX+context, function-identical control, LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid) and HyReX with 9-kernel coarse stages are dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.dom.L1.margin\endcsname{0.281}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.dom.L1.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.dom.L1b.margin\endcsname{0.333}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.dom.L1b.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.dom.L4.margin\endcsname{0.301}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.dom.L4.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.dom.L6.margin\endcsname{0.165}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.dom.L6.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.dom.P3c.margin\endcsname{0.629}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.dom.P3c.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.dom.V6A1r.margin\endcsname{0.043}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.dom.V6A1r.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.dom.V7A1.margin\endcsname{0.387}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.dom.V7A1.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.dom.V7A2.margin\endcsname{0.255}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.dom.V7A2.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.dom.base.margin\endcsname{0.616}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.dom.base.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.dominated\endcsname{nnU-Net default, ResEnc-M (library preset), ResEnc-matched (re-implemented), ResEnc+context, HyReX+context, function-identical control, LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.endpoints\endcsname{LeanAdd-NeXt with the coarse operator at stage 5 alone, HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.hero\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.hero.clause\endcsname{HyReX is on the ACDC (parameters, gain) front as the largest-gain endpoint: no arm is above and left of it, and it dominates 9 of the 12 other points, all except ConvNeXt-k3, LeanAdd with coarse large kernels (LeanAdd-NeXt) and LeanAdd-NeXt with the coarse operator at stage 5 alone}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.hero.dominates\endcsname{nnU-Net default, ResEnc-M (library preset), ResEnc-matched (re-implemented), ResEnc+context, HyReX+context, function-identical control, LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.hero.dominators\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.hero.ndominates\endcsname{9}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.hero.ndominators\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.hero.notdominated\endcsname{ConvNeXt-k3, LeanAdd with coarse large kernels (LeanAdd-NeXt), LeanAdd-NeXt with the coarse operator at stage 5 alone}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.interior\endcsname{LeanAdd with coarse large kernels (LeanAdd-NeXt), ConvNeXt-k3}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.n\endcsname{4}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.ndominated\endcsname{9}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.nendpoints\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.ninterior\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.role.L1\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.role.L1b\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.role.L2\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.role.L3\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.role.L3.ext\endcsname{the largest-gain endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.role.L4\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.role.L6\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.role.P3c\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.role.V5B2\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.role.V6A1r\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.role.V7A1\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.role.V7A2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.role.V7C1\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.role.V7C1.ext\endcsname{the fewest-parameter endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.params.role.base\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step\endcsname{LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd with coarse large kernels (LeanAdd-NeXt), nnU-Net default, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.clause\endcsname{On seed 0, the discovery seed, over the 12 registered arms with a finished ACDC run and the default at the origin, the (profiled step time, gain) front on ACDC holds LeanAdd-NeXt with the coarse operator at stage 5 alone as the cheapest-step endpoint, LeanAdd with coarse large kernels (LeanAdd-NeXt) as an interior point, nnU-Net default as an interior point, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid) as an interior point, LeanDeepMid with the two finest decoder convolutions restored as an interior point and HyReX as the largest-gain endpoint; ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context, HyReX+context, function-identical control and HyReX with 9-kernel coarse stages are dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.dom.L1.margin\endcsname{0.026}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.dom.L1.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.dom.L1b.margin\endcsname{0.078}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.dom.L1b.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.dom.L2.margin\endcsname{0.376}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.dom.L2.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.dom.L4.margin\endcsname{0.046}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.dom.L4.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.dom.L6.margin\endcsname{0.165}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.dom.L6.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.dom.P3c.margin\endcsname{0.013}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.dom.P3c.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.dom.V6A1r.margin\endcsname{0.043}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.dom.V6A1r.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.dominated\endcsname{ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context, HyReX+context, function-identical control, HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.endpoints\endcsname{LeanAdd-NeXt with the coarse operator at stage 5 alone, HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.hero\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.hero.clause\endcsname{HyReX is on the ACDC (profiled step time, gain) front as the largest-gain endpoint and dominates HyReX+context and HyReX with 9-kernel coarse stages (2 of the 12 other points)}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.hero.dominates\endcsname{HyReX+context, HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.hero.ndominates\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.hero.notdominated\endcsname{nnU-Net default, ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context, function-identical control, LeanAdd with coarse large kernels (LeanAdd-NeXt), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with the coarse operator at stage 5 alone}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.interior\endcsname{LeanAdd with coarse large kernels (LeanAdd-NeXt), nnU-Net default, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.n\endcsname{6}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.ndominated\endcsname{7}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.nendpoints\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.ninterior\endcsname{4}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.role.L1\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.role.L1b\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.role.L2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.role.L3\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.role.L3.ext\endcsname{the largest-gain endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.role.L4\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.role.L6\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.role.P3c\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.role.V5B2\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.role.V6A1r\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.role.V7A1\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.role.V7A2\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.role.V7C1\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.role.V7C1.ext\endcsname{the cheapest-step endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.step.role.base\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.acdc.universe\endcsname{the 12 registered arms with a finished ACDC run and the default at the origin}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all\endcsname{ConvNeXt-k3, nnU-Net default, ResEnc-M (library preset), ResEnc-matched (re-implemented), ResEnc+context}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.clause\endcsname{On the fresh-seed mean of seeds 1--2, over the 5 arms with a complete fresh pair and the default at the origin, the (parameters, profiled step time, gain) front on AMOS22 holds ConvNeXt-k3 as the fewest-parameter endpoint, nnU-Net default as the cheapest-step endpoint, ResEnc-M (library preset) as the largest-gain endpoint, ResEnc-matched (re-implemented) as an interior point and ResEnc+context as an interior point; HyReX is dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.dom.L3.margin\endcsname{0.062}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.dom.L3.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.dominated\endcsname{HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.endpoints\endcsname{ConvNeXt-k3, nnU-Net default, ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.hero\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.hero.clause\endcsname{HyReX is dominated on the AMOS22 (parameters, profiled step time, gain) front by ConvNeXt-k3, 0.062 pp ahead in gain, inside the 0.24 pp edge of the null of a difference of two-seed means; its fresh-seed gain is not separated from the default at two seeds}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.hero.dominates\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.hero.ndominates\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.hero.notdominated\endcsname{nnU-Net default, ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.interior\endcsname{ResEnc-matched (re-implemented), ResEnc+context}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.n\endcsname{5}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.ndominated\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.nendpoints\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.ninterior\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.role.L1\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.role.L1.ext\endcsname{the largest-gain endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.role.L1b\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.role.L2\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.role.L2.ext\endcsname{the fewest-parameter endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.role.L3\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.role.L4\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.role.base\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.all.role.base.ext\endcsname{the cheapest-step endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.basis.short\endcsname{fresh}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.edge\endcsname{0.24}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.n\endcsname{5}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params\endcsname{ConvNeXt-k3, ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.clause\endcsname{On the fresh-seed mean of seeds 1--2, over the 5 arms with a complete fresh pair and the default at the origin, the (parameters, gain) front on AMOS22 holds ConvNeXt-k3 as the fewest-parameter endpoint and ResEnc-M (library preset) as the largest-gain endpoint; HyReX, nnU-Net default, ResEnc-matched (re-implemented) and ResEnc+context are dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.dom.L1b.margin\endcsname{0.167}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.dom.L1b.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.dom.L3.margin\endcsname{0.062}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.dom.L3.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.dom.L4.margin\endcsname{0.010}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.dom.L4.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.dom.base.margin\endcsname{0.194}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.dom.base.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.dominated\endcsname{HyReX, nnU-Net default, ResEnc-matched (re-implemented), ResEnc+context}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.endpoints\endcsname{ConvNeXt-k3, ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.hero\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.hero.clause\endcsname{ConvNeXt-k3 sits above and left of HyReX on the AMOS22 (parameters, gain) plane by 0.062 pp in gain, with 5.16 M fewer parameters; that gain gap is inside the registered 0.5 pp floor and 0.36 of the one-seed pair SD of AMOS22 (0.17 pp); the fresh-seed gain of HyReX is not separated from the default at two seeds}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.hero.dominates\endcsname{nnU-Net default}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.hero.dominators\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.hero.gap\endcsname{0.062}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.hero.gap.floor\endcsname{inside}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.hero.gap.sepair\endcsname{0.36}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.hero.ndominates\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.hero.ndominators\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.hero.notdominated\endcsname{ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.interior\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.ndominated\endcsname{4}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.nendpoints\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.ninterior\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.role.L1\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.role.L1.ext\endcsname{the largest-gain endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.role.L1b\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.role.L2\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.role.L2.ext\endcsname{the fewest-parameter endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.role.L3\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.role.L4\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.params.role.base\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step\endcsname{nnU-Net default, ResEnc-matched (re-implemented), ResEnc+context, ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.clause\endcsname{On the fresh-seed mean of seeds 1--2, over the 5 arms with a complete fresh pair and the default at the origin, the (profiled step time, gain) front on AMOS22 holds nnU-Net default as the cheapest-step endpoint, ResEnc-matched (re-implemented) as an interior point, ResEnc+context as an interior point and ResEnc-M (library preset) as the largest-gain endpoint; HyReX and ConvNeXt-k3 are dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.dom.L2.margin\endcsname{0.270}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.dom.L2.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.dom.L3.margin\endcsname{0.332}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.dom.L3.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.dominated\endcsname{HyReX, ConvNeXt-k3}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.endpoints\endcsname{nnU-Net default, ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.hero\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.hero.clause\endcsname{HyReX is dominated on the AMOS22 (profiled step time, gain) front by ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3 and ResEnc+context, up to 0.332 pp ahead in gain, above the 0.24 pp edge of the null of a difference of two-seed means; its fresh-seed gain is not separated from the default at two seeds}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.hero.dominates\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.hero.ndominates\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.hero.notdominated\endcsname{nnU-Net default, ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.interior\endcsname{ResEnc-matched (re-implemented), ResEnc+context}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.n\endcsname{4}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.ndominated\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.nendpoints\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.ninterior\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.role.L1\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.role.L1.ext\endcsname{the largest-gain endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.role.L1b\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.role.L2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.role.L3\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.role.L4\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.role.base\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.step.role.base.ext\endcsname{the cheapest-step endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.amos.universe\endcsname{the 5 arms with a complete fresh pair and the default at the origin}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanDec with additive skips (LeanAdd), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.clause\endcsname{On the fresh-seed mean of seeds 1--2, over the 25 arms with a complete fresh pair and the default at the origin, the (parameters, profiled step time, gain) front on KiTS23 holds LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk) as the fewest-parameter and cheapest-step endpoint, LeanAdd-NeXt with separable coarse kernels (LeanSep) as an interior point, LeanAdd-NeXt with dilated coarse kernels (LeanDil) as an interior point, LeanDec with additive skips (LeanAdd) as an interior point, LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1) as an interior point, LeanAdd-NeXt with the coarse operator at stage 5 alone as an interior point, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid) as an interior point and ResEnc-M (library preset) as the largest-gain endpoint; HyReX, nnU-Net default, ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context, HyReX+context, branch control, HyReX, ConvNeXt one stage finer, HyReX point-fuse decoder, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), function-identical control, LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with LeanDec fine decoder stages, LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanDeepMid with the two finest decoder convolutions restored and HyReX with 9-kernel coarse stages are dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.C1.margin\endcsname{0.261}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.C1.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.D1.margin\endcsname{0.905}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.D1.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.D2.margin\endcsname{0.548}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.D2.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.L1b.margin\endcsname{0.349}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.L1b.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.L2.margin\endcsname{2.330}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.L2.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.L3.margin\endcsname{0.346}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.L3.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.L4.margin\endcsname{0.415}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.L4.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.L6.margin\endcsname{1.070}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.L6.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.P3c.margin\endcsname{1.486}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.P3c.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.S2.margin\endcsname{1.870}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.S2.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.V5A5.margin\endcsname{0.275}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.V5A5.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.V5B2.margin\endcsname{0.992}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.V5B2.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.V6A1r.margin\endcsname{0.736}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.V6A1r.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.V7A2.margin\endcsname{0.373}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.V7A2.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.V8A1.margin\endcsname{1.191}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.V8A1.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.V8A2.margin\endcsname{0.563}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.V8A2.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.W1c.margin\endcsname{1.595}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.W1c.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.base.margin\endcsname{2.662}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dom.base.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.dominated\endcsname{HyReX, nnU-Net default, ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context, HyReX+context, branch control, HyReX, ConvNeXt one stage finer, HyReX point-fuse decoder, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), function-identical control, LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with LeanDec fine decoder stages, LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanDeepMid with the two finest decoder convolutions restored, HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.endpoints\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.hero\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.hero.clause\endcsname{HyReX is dominated on the KiTS23 (parameters, profiled step time, gain) front by HyReX with LeanDec fine decoder stages, LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with separable coarse kernels (LeanSep) and LeanAdd-NeXt with the coarse operator at stage 5 alone, up to 0.346 pp ahead in gain, inside the 1.56 pp edge of the null of a difference of two-seed means; its fresh-seed gain is separated from the default at two seeds}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.hero.dominates\endcsname{HyReX+context, HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.hero.ndominates\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.hero.notdominated\endcsname{nnU-Net default, ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context, branch control, HyReX, ConvNeXt one stage finer, HyReX point-fuse decoder, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), function-identical control, LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with LeanDec fine decoder stages, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with the coarse operator at stage 5 alone}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.interior\endcsname{LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanDec with additive skips (LeanAdd), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid)}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.n\endcsname{8}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.ndominated\endcsname{18}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.nendpoints\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.ninterior\endcsname{6}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.C1\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.D1\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.D2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.L1\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.L1.ext\endcsname{the largest-gain endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.L1b\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.L2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.L3\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.L4\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.L6\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.P3c\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.S2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.V5A5\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.V5B1\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.V5B2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.V6A1r\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.V7A1\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.V7A2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.V7B1\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.V7B2\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.V7C1\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.V8A1\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.V8A2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.V8B1\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.V8B1.ext\endcsname{the fewest-parameter and cheapest-step endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.V8B2\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.W1c\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.all.role.base\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.basis.short\endcsname{fresh}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.edge\endcsname{1.56}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.n\endcsname{25}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.clause\endcsname{On the fresh-seed mean of seeds 1--2, over the 25 arms with a complete fresh pair and the default at the origin, the (parameters, gain) front on KiTS23 holds LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk) as the fewest-parameter endpoint, LeanAdd-NeXt with separable coarse kernels (LeanSep) as an interior point, LeanAdd-NeXt with the coarse operator at stage 5 alone as an interior point, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid) as an interior point and ResEnc-M (library preset) as the largest-gain endpoint; HyReX, nnU-Net default, ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context, HyReX+context, branch control, HyReX, ConvNeXt one stage finer, HyReX point-fuse decoder, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), function-identical control, LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with LeanDec fine decoder stages, LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with dilated coarse kernels (LeanDil) and HyReX with 9-kernel coarse stages are dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.C1.margin\endcsname{0.261}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.C1.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.D1.margin\endcsname{0.905}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.D1.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.D2.margin\endcsname{0.548}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.D2.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.L1b.margin\endcsname{1.162}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.L1b.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.L2.margin\endcsname{2.330}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.L2.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.L3.margin\endcsname{0.346}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.L3.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.L4.margin\endcsname{1.229}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.L4.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.L6.margin\endcsname{1.070}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.L6.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.P3c.margin\endcsname{1.486}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.P3c.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.S2.margin\endcsname{1.870}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.S2.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.V5A5.margin\endcsname{0.275}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.V5A5.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.V5B1.margin\endcsname{0.096}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.V5B1.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.V5B2.margin\endcsname{0.992}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.V5B2.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.V6A1r.margin\endcsname{0.736}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.V6A1r.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.V7A2.margin\endcsname{0.373}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.V7A2.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.V7B2.margin\endcsname{0.543}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.V7B2.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.V8A1.margin\endcsname{1.413}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.V8A1.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.V8A2.margin\endcsname{0.785}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.V8A2.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.V8B2.margin\endcsname{0.650}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.V8B2.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.W1c.margin\endcsname{1.595}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.W1c.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.base.margin\endcsname{2.662}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dom.base.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.dominated\endcsname{HyReX, nnU-Net default, ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context, HyReX+context, branch control, HyReX, ConvNeXt one stage finer, HyReX point-fuse decoder, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), function-identical control, LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with LeanDec fine decoder stages, LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with dilated coarse kernels (LeanDil), HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.endpoints\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.hero\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.hero.clause\endcsname{LeanAdd-NeXt with the coarse operator at stage 5 alone by 0.346 pp in gain with 8.55 M fewer parameters, LeanAdd-NeXt with separable coarse kernels (LeanSep) by 0.288 pp in gain with 9.23 M fewer parameters, LeanDec with additive skips (LeanAdd) by 0.192 pp in gain with 8.70 M fewer parameters and HyReX with LeanDec fine decoder stages by 0.072 pp in gain with 0.13 M fewer parameters sit above and left of HyReX on the KiTS23 (parameters, gain) plane; the largest gain gap, 0.346 pp, is inside the registered 0.5 pp floor and 0.31 of the one-seed pair SD of KiTS23 (1.12 pp); the fresh-seed gain of HyReX is separated from the default at two seeds}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.hero.dominates\endcsname{nnU-Net default, HyReX+context, branch control, function-identical control, LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.hero.dominators\endcsname{LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanDec with additive skips (LeanAdd), HyReX with LeanDec fine decoder stages}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.hero.gap\endcsname{0.346}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.hero.gap.floor\endcsname{inside}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.hero.gap.sepair\endcsname{0.31}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.hero.ndominates\endcsname{7}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.hero.ndominators\endcsname{4}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.hero.notdominated\endcsname{ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context, HyReX, ConvNeXt one stage finer, HyReX point-fuse decoder, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with LeanDec fine decoder stages, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with the coarse operator at stage 5 alone}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.interior\endcsname{LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid)}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.n\endcsname{5}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.ndominated\endcsname{21}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.nendpoints\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.ninterior\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.C1\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.D1\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.D2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.L1\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.L1.ext\endcsname{the largest-gain endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.L1b\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.L2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.L3\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.L4\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.L6\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.P3c\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.S2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.V5A5\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.V5B1\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.V5B2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.V6A1r\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.V7A1\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.V7A2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.V7B1\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.V7B2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.V7C1\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.V8A1\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.V8A2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.V8B1\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.V8B1.ext\endcsname{the fewest-parameter endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.V8B2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.W1c\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.params.role.base\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.clause\endcsname{On the fresh-seed mean of seeds 1--2, over the 25 arms with a complete fresh pair and the default at the origin, the (profiled step time, gain) front on KiTS23 holds LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk) as the cheapest-step endpoint, LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1) as an interior point, LeanDec with additive skips (LeanAdd) as an interior point, LeanAdd-NeXt with the coarse operator at stage 5 alone as an interior point, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid) as an interior point and ResEnc-M (library preset) as the largest-gain endpoint; HyReX, nnU-Net default, ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context, HyReX+context, branch control, HyReX, ConvNeXt one stage finer, HyReX point-fuse decoder, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), function-identical control, LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with LeanDec fine decoder stages, LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil) and HyReX with 9-kernel coarse stages are dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.C1.margin\endcsname{1.074}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.C1.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.D1.margin\endcsname{1.999}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.D1.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.D2.margin\endcsname{0.548}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.D2.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.L1b.margin\endcsname{0.349}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.L1b.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.L2.margin\endcsname{2.551}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.L2.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.L3.margin\endcsname{1.382}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.L3.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.L4.margin\endcsname{0.415}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.L4.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.L6.margin\endcsname{1.884}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.L6.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.P3c.margin\endcsname{1.486}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.P3c.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.S2.margin\endcsname{2.905}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.S2.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.V5A5.margin\endcsname{0.496}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.V5A5.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.V5B2.margin\endcsname{0.992}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.V5B2.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.V6A1r.margin\endcsname{1.771}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.V6A1r.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.V7A2.margin\endcsname{0.373}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.V7A2.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.V7B1.margin\endcsname{0.058}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.V7B1.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.V7B2.margin\endcsname{0.447}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.V7B2.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.V8A1.margin\endcsname{1.191}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.V8A1.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.V8A2.margin\endcsname{0.563}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.V8A2.resolved\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.W1c.margin\endcsname{1.595}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.W1c.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.base.margin\endcsname{2.662}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dom.base.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.dominated\endcsname{HyReX, nnU-Net default, ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context, HyReX+context, branch control, HyReX, ConvNeXt one stage finer, HyReX point-fuse decoder, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), function-identical control, LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with LeanDec fine decoder stages, LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.endpoints\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.hero\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.hero.clause\endcsname{HyReX is dominated on the KiTS23 (profiled step time, gain) front by ResEnc-M (library preset), ResEnc-matched (re-implemented), ResEnc+context, HyReX with LeanDec fine decoder stages, LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep) and LeanAdd-NeXt with the coarse operator at stage 5 alone, up to 1.382 pp ahead in gain, inside the 1.56 pp edge of the null of a difference of two-seed means; its fresh-seed gain is separated from the default at two seeds}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.hero.dominates\endcsname{HyReX+context, HyReX, ConvNeXt one stage finer, HyReX point-fuse decoder, HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.hero.ndominates\endcsname{4}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.hero.notdominated\endcsname{nnU-Net default, ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context, branch control, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), function-identical control, LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with LeanDec fine decoder stages, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with the coarse operator at stage 5 alone}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.interior\endcsname{LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid)}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.n\endcsname{6}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.ndominated\endcsname{20}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.nendpoints\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.ninterior\endcsname{4}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.C1\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.D1\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.D2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.L1\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.L1.ext\endcsname{the largest-gain endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.L1b\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.L2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.L3\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.L4\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.L6\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.P3c\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.S2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.V5A5\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.V5B1\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.V5B2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.V6A1r\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.V7A1\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.V7A2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.V7B1\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.V7B2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.V7C1\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.V8A1\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.V8A2\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.V8B1\endcsname{endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.V8B1.ext\endcsname{the cheapest-step endpoint}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.V8B2\endcsname{interior}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.W1c\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.step.role.base\endcsname{dominated}
\expandafter\gdef\csname R@an.cost_accuracy.front3.kits.universe\endcsname{the 25 arms with a complete fresh pair and the default at the origin}
\expandafter\gdef\csname R@an.cost_accuracy.gppworst.acdc\endcsname{5.67}
\expandafter\gdef\csname R@an.cost_accuracy.gppworst.acdc.holds\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.gppworst.acdc.nseeds\endcsname{2 and 2}
\expandafter\gdef\csname R@an.cost_accuracy.gppworst.kits\endcsname{1.62}
\expandafter\gdef\csname R@an.cost_accuracy.gppworst.kits.holds\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.gppworst.kits.nseeds\endcsname{2 and 2}
\expandafter\gdef\csname R@an.cost_accuracy.head.C1.acdc\endcsname{0.21}
\expandafter\gdef\csname R@an.cost_accuracy.head.C1.amos\endcsname{0.36}
\expandafter\gdef\csname R@an.cost_accuracy.head.C1.kits\endcsname{2.27}
\expandafter\gdef\csname R@an.cost_accuracy.head.D1.acdc\endcsname{0.23}
\expandafter\gdef\csname R@an.cost_accuracy.head.D1.amos\endcsname{0.85}
\expandafter\gdef\csname R@an.cost_accuracy.head.D1.kits\endcsname{1.92}
\expandafter\gdef\csname R@an.cost_accuracy.head.D2.acdc\endcsname{2.02}
\expandafter\gdef\csname R@an.cost_accuracy.head.D2.amos\endcsname{3.25}
\expandafter\gdef\csname R@an.cost_accuracy.head.D2.kits\endcsname{3.57}
\expandafter\gdef\csname R@an.cost_accuracy.head.L1.acdc\endcsname{0.47}
\expandafter\gdef\csname R@an.cost_accuracy.head.L1.amos\endcsname{0.39}
\expandafter\gdef\csname R@an.cost_accuracy.head.L1.kits\endcsname{1.48}
\expandafter\gdef\csname R@an.cost_accuracy.head.L1b.acdc\endcsname{0.11}
\expandafter\gdef\csname R@an.cost_accuracy.head.L1b.amos\endcsname{0.71}
\expandafter\gdef\csname R@an.cost_accuracy.head.L1b.kits\endcsname{1.78}
\expandafter\gdef\csname R@an.cost_accuracy.head.L2.acdc\endcsname{0.34}
\expandafter\gdef\csname R@an.cost_accuracy.head.L2.amos\endcsname{1.56}
\expandafter\gdef\csname R@an.cost_accuracy.head.L2.kits\endcsname{2.15}
\expandafter\gdef\csname R@an.cost_accuracy.head.L3.acdc\endcsname{0.18}
\expandafter\gdef\csname R@an.cost_accuracy.head.L3.amos\endcsname{0.81}
\expandafter\gdef\csname R@an.cost_accuracy.head.L3.kits\endcsname{1.87}
\expandafter\gdef\csname R@an.cost_accuracy.head.L4.acdc\endcsname{0.71}
\expandafter\gdef\csname R@an.cost_accuracy.head.L4.amos\endcsname{0.57}
\expandafter\gdef\csname R@an.cost_accuracy.head.L4.kits\endcsname{1.74}
\expandafter\gdef\csname R@an.cost_accuracy.head.L6.acdc\endcsname{0.35}
\expandafter\gdef\csname R@an.cost_accuracy.head.L6.amos\endcsname{1.29}
\expandafter\gdef\csname R@an.cost_accuracy.head.L6.kits\endcsname{2.10}
\expandafter\gdef\csname R@an.cost_accuracy.head.P3c.acdc\endcsname{0.85}
\expandafter\gdef\csname R@an.cost_accuracy.head.P3c.amos\endcsname{2.57}
\expandafter\gdef\csname R@an.cost_accuracy.head.P3c.kits\endcsname{2.83}
\expandafter\gdef\csname R@an.cost_accuracy.head.S2.acdc\endcsname{0.12}
\expandafter\gdef\csname R@an.cost_accuracy.head.S2.amos\endcsname{1.06}
\expandafter\gdef\csname R@an.cost_accuracy.head.S2.kits\endcsname{2.02}
\expandafter\gdef\csname R@an.cost_accuracy.head.V5A5.acdc\endcsname{0.02}
\expandafter\gdef\csname R@an.cost_accuracy.head.V5A5.amos\endcsname{1.56}
\expandafter\gdef\csname R@an.cost_accuracy.head.V5A5.kits\endcsname{2.41}
\expandafter\gdef\csname R@an.cost_accuracy.head.V5B1.acdc\endcsname{2.13}
\expandafter\gdef\csname R@an.cost_accuracy.head.V5B1.amos\endcsname{3.43}
\expandafter\gdef\csname R@an.cost_accuracy.head.V5B1.kits\endcsname{3.84}
\expandafter\gdef\csname R@an.cost_accuracy.head.V5B2.acdc\endcsname{1.94}
\expandafter\gdef\csname R@an.cost_accuracy.head.V5B2.amos\endcsname{3.35}
\expandafter\gdef\csname R@an.cost_accuracy.head.V5B2.kits\endcsname{3.81}
\expandafter\gdef\csname R@an.cost_accuracy.head.V6A1r.acdc\endcsname{0.17}
\expandafter\gdef\csname R@an.cost_accuracy.head.V6A1r.amos\endcsname{0.80}
\expandafter\gdef\csname R@an.cost_accuracy.head.V6A1r.kits\endcsname{1.86}
\expandafter\gdef\csname R@an.cost_accuracy.head.V7A1.acdc\endcsname{1.27}
\expandafter\gdef\csname R@an.cost_accuracy.head.V7A1.amos\endcsname{2.80}
\expandafter\gdef\csname R@an.cost_accuracy.head.V7A1.kits\endcsname{3.48}
\expandafter\gdef\csname R@an.cost_accuracy.head.V7A2.acdc\endcsname{0.39}
\expandafter\gdef\csname R@an.cost_accuracy.head.V7A2.amos\endcsname{2.04}
\expandafter\gdef\csname R@an.cost_accuracy.head.V7A2.kits\endcsname{2.81}
\expandafter\gdef\csname R@an.cost_accuracy.head.V7B1.acdc\endcsname{1.89}
\expandafter\gdef\csname R@an.cost_accuracy.head.V7B1.amos\endcsname{3.36}
\expandafter\gdef\csname R@an.cost_accuracy.head.V7B1.kits\endcsname{3.81}
\expandafter\gdef\csname R@an.cost_accuracy.head.V7B2.acdc\endcsname{1.94}
\expandafter\gdef\csname R@an.cost_accuracy.head.V7B2.amos\endcsname{3.35}
\expandafter\gdef\csname R@an.cost_accuracy.head.V7B2.kits\endcsname{3.82}
\expandafter\gdef\csname R@an.cost_accuracy.head.V7C1.acdc\endcsname{2.11}
\expandafter\gdef\csname R@an.cost_accuracy.head.V7C1.amos\endcsname{3.42}
\expandafter\gdef\csname R@an.cost_accuracy.head.V7C1.kits\endcsname{3.83}
\expandafter\gdef\csname R@an.cost_accuracy.head.V8A1.acdc\endcsname{1.88}
\expandafter\gdef\csname R@an.cost_accuracy.head.V8A1.amos\endcsname{3.32}
\expandafter\gdef\csname R@an.cost_accuracy.head.V8A1.kits\endcsname{3.75}
\expandafter\gdef\csname R@an.cost_accuracy.head.V8A2.acdc\endcsname{1.93}
\expandafter\gdef\csname R@an.cost_accuracy.head.V8A2.amos\endcsname{3.32}
\expandafter\gdef\csname R@an.cost_accuracy.head.V8A2.kits\endcsname{3.77}
\expandafter\gdef\csname R@an.cost_accuracy.head.V8B1.acdc\endcsname{3.16}
\expandafter\gdef\csname R@an.cost_accuracy.head.V8B1.amos\endcsname{4.34}
\expandafter\gdef\csname R@an.cost_accuracy.head.V8B1.kits\endcsname{4.52}
\expandafter\gdef\csname R@an.cost_accuracy.head.V8B2.acdc\endcsname{2.85}
\expandafter\gdef\csname R@an.cost_accuracy.head.V8B2.amos\endcsname{4.07}
\expandafter\gdef\csname R@an.cost_accuracy.head.V8B2.kits\endcsname{4.43}
\expandafter\gdef\csname R@an.cost_accuracy.head.W1.acdc\endcsname{0.63}
\expandafter\gdef\csname R@an.cost_accuracy.head.W1.amos\endcsname{2.18}
\expandafter\gdef\csname R@an.cost_accuracy.head.W1.kits\endcsname{2.75}
\expandafter\gdef\csname R@an.cost_accuracy.head.W1c.acdc\endcsname{0.39}
\expandafter\gdef\csname R@an.cost_accuracy.head.W1c.amos\endcsname{2.18}
\expandafter\gdef\csname R@an.cost_accuracy.head.W1c.kits\endcsname{2.75}
\expandafter\gdef\csname R@an.cost_accuracy.head.W2.acdc\endcsname{0.60}
\expandafter\gdef\csname R@an.cost_accuracy.head.W2.amos\endcsname{2.16}
\expandafter\gdef\csname R@an.cost_accuracy.head.W2.kits\endcsname{2.73}
\expandafter\gdef\csname R@an.cost_accuracy.head.W3.acdc\endcsname{0.65}
\expandafter\gdef\csname R@an.cost_accuracy.head.W3.amos\endcsname{2.01}
\expandafter\gdef\csname R@an.cost_accuracy.head.W3.kits\endcsname{2.69}
\expandafter\gdef\csname R@an.cost_accuracy.head.W3c.acdc\endcsname{0.63}
\expandafter\gdef\csname R@an.cost_accuracy.head.W3c.amos\endcsname{1.35}
\expandafter\gdef\csname R@an.cost_accuracy.head.W3c.kits\endcsname{1.90}
\expandafter\gdef\csname R@an.cost_accuracy.head.W4.acdc\endcsname{0.23}
\expandafter\gdef\csname R@an.cost_accuracy.head.W4.amos\endcsname{0.12}
\expandafter\gdef\csname R@an.cost_accuracy.head.W4.kits\endcsname{1.93}
\expandafter\gdef\csname R@an.cost_accuracy.head.W5.acdc\endcsname{0.00}
\expandafter\gdef\csname R@an.cost_accuracy.head.W5.amos\endcsname{0.63}
\expandafter\gdef\csname R@an.cost_accuracy.head.W5.kits\endcsname{1.73}
\expandafter\gdef\csname R@an.cost_accuracy.head.base.acdc\endcsname{0.85}
\expandafter\gdef\csname R@an.cost_accuracy.head.base.amos\endcsname{2.57}
\expandafter\gdef\csname R@an.cost_accuracy.head.base.kits\endcsname{2.83}
\expandafter\gdef\csname R@an.cost_accuracy.kits.atdefault.best\endcsname{LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid)}
\expandafter\gdef\csname R@an.cost_accuracy.kits.atdefault.best.pp\endcsname{\ensuremath{+2.662}}
\expandafter\gdef\csname R@an.cost_accuracy.kits.atdefault.clause\endcsname{the largest KiTS23 fresh-seed gain among the 18 registered arms with a complete fresh pair at or below the default's 31.20 M parameters on the KiTS23 plan is that of LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), \ensuremath{+2.662} pp, then that of LeanAdd-NeXt with the coarse operator at stage 5 alone, \ensuremath{+2.440} pp (0.222 pp behind, 0.28 SD of the null of a difference of two-seed means, inside its 1.56 pp edge), then that of LeanAdd-NeXt with separable coarse kernels (LeanSep), \ensuremath{+2.382} pp, then that of LeanDeepMid with the two finest decoder convolutions restored, \ensuremath{+2.289} pp; HyReX stands seventh of the 18 at \ensuremath{+2.094} pp, 0.568 pp behind the largest}
\expandafter\gdef\csname R@an.cost_accuracy.kits.atdefault.hero.behind\endcsname{0.568}
\expandafter\gdef\csname R@an.cost_accuracy.kits.atdefault.hero.pp\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.cost_accuracy.kits.atdefault.hero.rank\endcsname{7}
\expandafter\gdef\csname R@an.cost_accuracy.kits.atdefault.licence\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.kits.atdefault.margin\endcsname{0.222}
\expandafter\gdef\csname R@an.cost_accuracy.kits.atdefault.n\endcsname{18}
\expandafter\gdef\csname R@an.cost_accuracy.kits.atdefault.names\endcsname{LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanDeepMid with the two finest decoder convolutions restored, LeanDec with additive skips (LeanAdd), HyReX with LeanDec fine decoder stages, HyReX, LeanDec (default with one conv per decoder stage), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), HyReX with 9-kernel coarse stages, HyReX+context, HyReX point-fuse decoder, LeanAdd with coarse large kernels (LeanAdd-NeXt), LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), function-identical control, HyReX, ConvNeXt one stage finer, ConvNeXt-k3}
\expandafter\gdef\csname R@an.cost_accuracy.kits.atdefault.second\endcsname{LeanAdd-NeXt with the coarse operator at stage 5 alone}
\expandafter\gdef\csname R@an.cost_accuracy.kits.atdefault.universe\endcsname{the 18 registered arms with a complete fresh pair at or below the default's 31.20 M parameters on the KiTS23 plan}
\expandafter\gdef\csname R@an.cost_accuracy.kits.best\endcsname{HyReX + decoder capacity}
\expandafter\gdef\csname R@an.cost_accuracy.kits.best.clause\endcsname{HyReX + decoder capacity, the highest seed-0 delta among the 25 registered arms with a finished KiTS23 run (the library preset and the matched controls included), 0.596 pp ahead of LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), a margin above the registered 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.kits.floor.arms\endcsname{HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context, HyReX+context, branch control, HyReX, ConvNeXt one stage finer, HyReX point-fuse decoder, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), function-identical control, LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with LeanDec fine decoder stages, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with the coarse operator at stage 5 alone, HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.kits.floor.clause\endcsname{25 of the 25 evaluated KiTS23 arms have a seed-0 margin over the default that clears the registered 0.5 pp one-seed pair floor: HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context, HyReX+context, branch control, HyReX, ConvNeXt one stage finer, HyReX point-fuse decoder, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), function-identical control, LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with LeanDec fine decoder stages, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with the coarse operator at stage 5 alone, HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.kits.floor.n\endcsname{25}
\expandafter\gdef\csname R@an.cost_accuracy.kits.floor.of\endcsname{25}
\expandafter\gdef\csname R@an.cost_accuracy.kits.fresh.best\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.kits.fresh.best.pp\endcsname{\ensuremath{+3.475}}
\expandafter\gdef\csname R@an.cost_accuracy.kits.fresh.leader\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.kits.fresh.licence\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.kits.fresh.margin\endcsname{0.814}
\expandafter\gdef\csname R@an.cost_accuracy.kits.fresh.margin.edge\endcsname{1.56}
\expandafter\gdef\csname R@an.cost_accuracy.kits.fresh.margin.sd\endcsname{1.02}
\expandafter\gdef\csname R@an.cost_accuracy.kits.fresh.second\endcsname{LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid)}
\expandafter\gdef\csname R@an.cost_accuracy.kits.fresh.second.pp\endcsname{\ensuremath{+2.662}}
\expandafter\gdef\csname R@an.cost_accuracy.kits.fresh.super\endcsname{over the 25 of 25 finished arms that have a fresh mean}
\expandafter\gdef\csname R@an.cost_accuracy.kits.fresh.top.clause\endcsname{the two highest KiTS23 fresh means are ResEnc-M (library preset) at \ensuremath{+3.475} pp and LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid) at \ensuremath{+2.662} pp, 0.814 pp apart (1.02 SD of the null of a difference of two-seed means, inside its 1.56 pp edge), over the 25 of 25 finished arms that have a fresh mean}
\expandafter\gdef\csname R@an.cost_accuracy.kits.leader\endcsname{HyReX + decoder capacity}
\expandafter\gdef\csname R@an.cost_accuracy.kits.leader.clause\endcsname{the top two seed-0 deltas, HyReX + decoder capacity and LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), are 0.596 pp apart, a margin above the registered 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.kits.margin\endcsname{0.596}
\expandafter\gdef\csname R@an.cost_accuracy.kits.margin.pair\endcsname{HyReX + decoder capacity over LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk)}
\expandafter\gdef\csname R@an.cost_accuracy.kits.margin.resolved\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.kits.order\endcsname{HyReX + decoder capacity, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanDeepMid with the two finest decoder convolutions restored, HyReX, LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, branch control, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), HyReX+context, LeanDec (default with one conv per decoder stage), ResEnc-M (library preset), HyReX with 9-kernel coarse stages, ResEnc+context, LeanDec with additive skips (LeanAdd), HyReX with LeanDec fine decoder stages, LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), ResEnc-matched (re-implemented), LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), HyReX point-fuse decoder, function-identical control, LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), HyReX, ConvNeXt one stage finer, LeanAdd with coarse large kernels (LeanAdd-NeXt), ConvNeXt-k3}
\expandafter\gdef\csname R@an.cost_accuracy.kits.order.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.kits.order.n\endcsname{25}
\expandafter\gdef\csname R@an.cost_accuracy.kits.order.universe\endcsname{every registered arm with a finished KiTS23 run, the library preset and the matched controls included}
\expandafter\gdef\csname R@an.cost_accuracy.kits.second\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk)}
\expandafter\gdef\csname R@an.cost_accuracy.kits.second.clause\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk) is second, at \ensuremath{+2.911} pp}
\expandafter\gdef\csname R@an.cost_accuracy.kits.second.family\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.mem.max.res.acdc\endcsname{12.00}
\expandafter\gdef\csname R@an.cost_accuracy.mem.max.res.acdc.arm\endcsname{pooled-skip control}
\expandafter\gdef\csname R@an.cost_accuracy.mem.max.res.amos\endcsname{11.88}
\expandafter\gdef\csname R@an.cost_accuracy.mem.max.res.amos.arm\endcsname{ConvNeXt-4$\times$-GRN (MedNeXt-like reference)}
\expandafter\gdef\csname R@an.cost_accuracy.mem.max.res.kits\endcsname{10.52}
\expandafter\gdef\csname R@an.cost_accuracy.mem.max.res.kits.arm\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.mem.nnear.acdc\endcsname{14}
\expandafter\gdef\csname R@an.cost_accuracy.mem.nnear.amos\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.mem.nnear.kits\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.mem.nover.acdc\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.mem.nover.amos\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.mem.nover.kits\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.C1.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.C1.head\endcsname{0.21}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.C1.hi\endcsname{11.79}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.C1.lo\endcsname{9.73}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.D1.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.D1.head\endcsname{0.23}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.D1.hi\endcsname{11.77}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.D1.lo\endcsname{10.08}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.D2.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.D2.head\endcsname{2.02}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.D2.hi\endcsname{9.98}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.D2.lo\endcsname{8.43}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L1.binding\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L1.head\endcsname{0.39}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L1.hi\endcsname{11.61}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L1.lo\endcsname{10.52}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L1b.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L1b.head\endcsname{0.11}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L1b.hi\endcsname{11.89}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L1b.lo\endcsname{10.22}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L2.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L2.head\endcsname{0.34}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L2.hi\endcsname{11.66}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L2.lo\endcsname{9.85}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L3.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L3.head\endcsname{0.18}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L3.hi\endcsname{11.82}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L3.lo\endcsname{10.13}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L4.binding\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L4.head\endcsname{0.57}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L4.hi\endcsname{11.43}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L4.lo\endcsname{10.26}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L6.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L6.head\endcsname{0.35}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L6.hi\endcsname{11.65}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.L6.lo\endcsname{9.90}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.P3c.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.P3c.head\endcsname{0.85}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.P3c.hi\endcsname{11.15}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.P3c.lo\endcsname{9.17}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.S2.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.S2.head\endcsname{0.12}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.S2.hi\endcsname{11.88}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.S2.lo\endcsname{9.98}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V5A5.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V5A5.head\endcsname{0.02}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V5A5.hi\endcsname{11.98}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V5A5.lo\endcsname{9.59}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V5B1.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V5B1.head\endcsname{2.13}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V5B1.hi\endcsname{9.87}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V5B1.lo\endcsname{8.16}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V5B2.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V5B2.head\endcsname{1.94}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V5B2.hi\endcsname{10.06}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V5B2.lo\endcsname{8.19}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V6A1r.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V6A1r.head\endcsname{0.17}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V6A1r.hi\endcsname{11.83}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V6A1r.lo\endcsname{10.14}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7A1.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7A1.head\endcsname{1.27}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7A1.hi\endcsname{10.73}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7A1.lo\endcsname{8.52}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7A2.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7A2.head\endcsname{0.39}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7A2.hi\endcsname{11.61}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7A2.lo\endcsname{9.19}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7B1.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7B1.head\endcsname{1.89}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7B1.hi\endcsname{10.11}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7B1.lo\endcsname{8.19}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7B2.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7B2.head\endcsname{1.94}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7B2.hi\endcsname{10.06}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7B2.lo\endcsname{8.18}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7C1.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7C1.head\endcsname{2.11}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7C1.hi\endcsname{9.89}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V7C1.lo\endcsname{8.17}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V8A1.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V8A1.head\endcsname{1.88}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V8A1.hi\endcsname{10.12}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V8A1.lo\endcsname{8.25}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V8A2.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V8A2.head\endcsname{1.93}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V8A2.hi\endcsname{10.07}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V8A2.lo\endcsname{8.23}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V8B1.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V8B1.head\endcsname{3.16}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V8B1.hi\endcsname{8.84}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V8B1.lo\endcsname{7.48}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V8B2.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V8B2.head\endcsname{2.85}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V8B2.hi\endcsname{9.15}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.V8B2.lo\endcsname{7.57}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W1.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W1.head\endcsname{0.63}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W1.hi\endcsname{11.37}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W1.lo\endcsname{9.25}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W1c.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W1c.head\endcsname{0.39}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W1c.hi\endcsname{11.61}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W1c.lo\endcsname{9.25}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W2.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W2.head\endcsname{0.60}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W2.hi\endcsname{11.40}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W2.lo\endcsname{9.27}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W3.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W3.head\endcsname{0.65}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W3.hi\endcsname{11.35}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W3.lo\endcsname{9.31}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W3c.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W3c.head\endcsname{0.63}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W3c.hi\endcsname{11.37}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W3c.lo\endcsname{10.10}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W4.binding\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W4.head\endcsname{0.12}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W4.hi\endcsname{11.88}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W4.lo\endcsname{10.07}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W5.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W5.head\endcsname{0.00}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W5.hi\endcsname{12.00}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.W5.lo\endcsname{10.27}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.base.binding\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.base.head\endcsname{0.85}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.base.hi\endcsname{11.15}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.base.lo\endcsname{9.17}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.nacdc\endcsname{29}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.nover\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.nover.arms\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.nrows\endcsname{32}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.over\endcsname{pooled-skip control, HyReX, ConvNeXt one stage finer, HyReX with LeanDec fine decoder stages}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.over.clause\endcsname{the profiler's fit rule rejects pooled-skip control (12.00 GB reserved on ACDC against the 12 GB cap), HyReX, ConvNeXt one stage finer (11.88 GB reserved on ACDC against the 12 GB cap) and HyReX with LeanDec fine decoder stages (11.98 GB reserved on ACDC against the 12 GB cap)}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.tightest\endcsname{pooled-skip control}
\expandafter\gdef\csname R@an.cost_accuracy.memspan.tightest.head\endcsname{0.00}
\expandafter\gdef\csname R@an.cost_accuracy.narms.acdc\endcsname{12}
\expandafter\gdef\csname R@an.cost_accuracy.narms.amos\endcsname{31}
\expandafter\gdef\csname R@an.cost_accuracy.narms.kits\endcsname{25}
\expandafter\gdef\csname R@an.cost_accuracy.notrun.acdc\endcsname{$z$-dilation mixing, branch control, thickness-gated mixing, offset upsampling, trilinear-decoder control, ConvNeXt-4$\times$-GRN (MedNeXt-like reference), pooled-skip control, HyReX, ConvNeXt one stage finer, HyReX point-fuse decoder, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), LeanDec with additive skips (LeanAdd), HyReX with LeanDec fine decoder stages, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil)}
\expandafter\gdef\csname R@an.cost_accuracy.notrun.acdc.n\endcsname{19}
\expandafter\gdef\csname R@an.cost_accuracy.notrun.amos\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.notrun.amos.n\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.notrun.kits\endcsname{$z$-dilation mixing, thickness-gated mixing, offset upsampling, trilinear-decoder control, pooled-skip control}
\expandafter\gdef\csname R@an.cost_accuracy.notrun.kits.n\endcsname{5}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.C1.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.C1.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.D1.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.D1.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.D2.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.D2.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.L1.acdc\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.L1.amos\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.L1.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.L1b.acdc\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.L1b.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.L1b.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.L2.acdc\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.L2.amos\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.L2.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.L3.acdc\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.L3.amos\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.L3.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.L4.acdc\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.L4.amos\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.L4.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.L6.acdc\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.L6.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.L6.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.P3c.acdc\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.P3c.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.P3c.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.S2.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.S2.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V5A5.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V5A5.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V5B1.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V5B1.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V5B2.acdc\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V5B2.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V5B2.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V6A1r.acdc\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V6A1r.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V6A1r.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V7A1.acdc\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V7A1.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V7A1.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V7A2.acdc\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V7A2.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V7A2.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V7B1.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V7B1.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V7B2.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V7B2.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V7C1.acdc\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V7C1.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V7C1.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V8A1.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V8A1.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V8A2.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V8A2.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V8B1.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V8B1.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V8B2.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.V8B2.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.W1.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.W1c.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.W1c.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.W2.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.W3.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.W3c.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.W4.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.nseed.W5.amos\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.offaxis.acdc\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.offaxis.acdc.n\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.offaxis.amos\endcsname{ConvNeXt-4$\times$-GRN (MedNeXt-like reference)}
\expandafter\gdef\csname R@an.cost_accuracy.offaxis.amos.clause\endcsname{ConvNeXt-4$\times$-GRN (MedNeXt-like reference) at 3.51$\times$ the default's step (\ensuremath{+0.08} pp)}
\expandafter\gdef\csname R@an.cost_accuracy.offaxis.amos.n\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.offaxis.kits\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.offaxis.kits.n\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.pairfloor\endcsname{0.5}
\expandafter\gdef\csname R@an.cost_accuracy.panel.acdc.basis\endcsname{seed 0, with the fresh mean for 4 of 12 arms}
\expandafter\gdef\csname R@an.cost_accuracy.panel.amos.basis\endcsname{seed 0, with the fresh mean for 5 of 31 arms}
\expandafter\gdef\csname R@an.cost_accuracy.panel.basis.summary\endcsname{(a) seed 0, with the fresh mean for 5 of 31 arms; (b) the fresh mean of seeds 1--2; (c) seed 0, with the fresh mean for 4 of 12 arms}
\expandafter\gdef\csname R@an.cost_accuracy.panel.kits.basis\endcsname{the fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.par.C1.acdc\endcsname{51.6}
\expandafter\gdef\csname R@an.cost_accuracy.par.C1.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.C1.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.C1.amos\endcsname{52.3}
\expandafter\gdef\csname R@an.cost_accuracy.par.C1.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.C1.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.C1.kits\endcsname{52.4}
\expandafter\gdef\csname R@an.cost_accuracy.par.C1.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.C1.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.D1.acdc\endcsname{20.1}
\expandafter\gdef\csname R@an.cost_accuracy.par.D1.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.D1.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.D1.amos\endcsname{20.9}
\expandafter\gdef\csname R@an.cost_accuracy.par.D1.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.D1.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.D1.kits\endcsname{20.9}
\expandafter\gdef\csname R@an.cost_accuracy.par.D1.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.D1.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.D2.acdc\endcsname{25.3}
\expandafter\gdef\csname R@an.cost_accuracy.par.D2.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.D2.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.D2.amos\endcsname{26.0}
\expandafter\gdef\csname R@an.cost_accuracy.par.D2.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.D2.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.D2.kits\endcsname{26.1}
\expandafter\gdef\csname R@an.cost_accuracy.par.D2.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.D2.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.L1.acdc\endcsname{101.5}
\expandafter\gdef\csname R@an.cost_accuracy.par.L1.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.L1.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.L1.amos\endcsname{102.3}
\expandafter\gdef\csname R@an.cost_accuracy.par.L1.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.L1.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.L1.kits\endcsname{102.4}
\expandafter\gdef\csname R@an.cost_accuracy.par.L1.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.L1.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.L1b.acdc\endcsname{101.6}
\expandafter\gdef\csname R@an.cost_accuracy.par.L1b.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.L1b.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.L1b.amos\endcsname{102.4}
\expandafter\gdef\csname R@an.cost_accuracy.par.L1b.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.L1b.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.L1b.kits\endcsname{102.4}
\expandafter\gdef\csname R@an.cost_accuracy.par.L1b.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.L1b.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.L2.acdc\endcsname{23.7}
\expandafter\gdef\csname R@an.cost_accuracy.par.L2.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.L2.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.L2.amos\endcsname{24.4}
\expandafter\gdef\csname R@an.cost_accuracy.par.L2.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.L2.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.L2.kits\endcsname{24.5}
\expandafter\gdef\csname R@an.cost_accuracy.par.L2.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.L2.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.L3.acdc\endcsname{28.8}
\expandafter\gdef\csname R@an.cost_accuracy.par.L3.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.L3.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.L3.amos\endcsname{29.6}
\expandafter\gdef\csname R@an.cost_accuracy.par.L3.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.L3.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.L3.kits\endcsname{29.7}
\expandafter\gdef\csname R@an.cost_accuracy.par.L3.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.L3.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.L4.acdc\endcsname{102.0}
\expandafter\gdef\csname R@an.cost_accuracy.par.L4.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.L4.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.L4.amos\endcsname{102.8}
\expandafter\gdef\csname R@an.cost_accuracy.par.L4.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.L4.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.L4.kits\endcsname{102.8}
\expandafter\gdef\csname R@an.cost_accuracy.par.L4.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.L4.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.L6.acdc\endcsname{30.3}
\expandafter\gdef\csname R@an.cost_accuracy.par.L6.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.L6.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.L6.amos\endcsname{31.1}
\expandafter\gdef\csname R@an.cost_accuracy.par.L6.amos.matchesbase\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.par.L6.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.L6.kits\endcsname{31.2}
\expandafter\gdef\csname R@an.cost_accuracy.par.L6.kits.matchesbase\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.par.L6.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.P3c.acdc\endcsname{30.4}
\expandafter\gdef\csname R@an.cost_accuracy.par.P3c.acdc.matchesbase\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.par.P3c.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.P3c.amos\endcsname{31.1}
\expandafter\gdef\csname R@an.cost_accuracy.par.P3c.amos.matchesbase\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.par.P3c.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.P3c.kits\endcsname{31.2}
\expandafter\gdef\csname R@an.cost_accuracy.par.P3c.kits.matchesbase\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.par.P3c.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.S2.acdc\endcsname{27.0}
\expandafter\gdef\csname R@an.cost_accuracy.par.S2.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.S2.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.S2.amos\endcsname{27.7}
\expandafter\gdef\csname R@an.cost_accuracy.par.S2.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.S2.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.S2.kits\endcsname{27.8}
\expandafter\gdef\csname R@an.cost_accuracy.par.S2.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.S2.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5A5.acdc\endcsname{28.7}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5A5.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5A5.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5A5.amos\endcsname{29.5}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5A5.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5A5.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5A5.kits\endcsname{29.5}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5A5.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5A5.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5B1.acdc\endcsname{20.2}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5B1.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5B1.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5B1.amos\endcsname{20.9}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5B1.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5B1.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5B1.kits\endcsname{21.0}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5B1.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5B1.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5B2.acdc\endcsname{20.5}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5B2.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5B2.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5B2.amos\endcsname{21.2}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5B2.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5B2.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5B2.kits\endcsname{21.3}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5B2.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V5B2.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.V6A1r.acdc\endcsname{30.0}
\expandafter\gdef\csname R@an.cost_accuracy.par.V6A1r.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V6A1r.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.V6A1r.amos\endcsname{30.7}
\expandafter\gdef\csname R@an.cost_accuracy.par.V6A1r.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V6A1r.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.V6A1r.kits\endcsname{30.8}
\expandafter\gdef\csname R@an.cost_accuracy.par.V6A1r.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V6A1r.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7A1.acdc\endcsname{30.3}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7A1.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7A1.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7A1.amos\endcsname{31.0}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7A1.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7A1.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7A1.kits\endcsname{31.0}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7A1.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7A1.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7A2.acdc\endcsname{30.4}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7A2.acdc.matchesbase\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7A2.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7A2.amos\endcsname{31.1}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7A2.amos.matchesbase\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7A2.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7A2.kits\endcsname{31.2}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7A2.kits.matchesbase\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7A2.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7B1.acdc\endcsname{19.6}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7B1.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7B1.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7B1.amos\endcsname{20.4}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7B1.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7B1.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7B1.kits\endcsname{20.4}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7B1.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7B1.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7B2.acdc\endcsname{19.7}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7B2.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7B2.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7B2.amos\endcsname{20.4}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7B2.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7B2.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7B2.kits\endcsname{20.5}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7B2.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7B2.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7C1.acdc\endcsname{20.3}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7C1.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7C1.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7C1.amos\endcsname{21.1}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7C1.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7C1.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7C1.kits\endcsname{21.1}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7C1.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V7C1.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8A1.acdc\endcsname{30.5}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8A1.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8A1.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8A1.amos\endcsname{31.3}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8A1.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8A1.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8A1.kits\endcsname{31.3}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8A1.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8A1.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8A2.acdc\endcsname{30.7}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8A2.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8A2.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8A2.amos\endcsname{31.4}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8A2.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8A2.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8A2.kits\endcsname{31.5}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8A2.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8A2.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8B1.acdc\endcsname{17.4}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8B1.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8B1.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8B1.amos\endcsname{18.2}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8B1.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8B1.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8B1.kits\endcsname{18.2}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8B1.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8B1.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8B2.acdc\endcsname{20.3}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8B2.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8B2.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8B2.amos\endcsname{21.1}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8B2.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8B2.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8B2.kits\endcsname{21.1}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8B2.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.V8B2.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.W1.acdc\endcsname{30.4}
\expandafter\gdef\csname R@an.cost_accuracy.par.W1.acdc.matchesbase\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.par.W1.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.W1.amos\endcsname{31.1}
\expandafter\gdef\csname R@an.cost_accuracy.par.W1.amos.matchesbase\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.par.W1.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.W1.kits\endcsname{31.2}
\expandafter\gdef\csname R@an.cost_accuracy.par.W1.kits.matchesbase\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.par.W1.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.W1c.acdc\endcsname{30.4}
\expandafter\gdef\csname R@an.cost_accuracy.par.W1c.acdc.matchesbase\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.par.W1c.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.W1c.amos\endcsname{31.1}
\expandafter\gdef\csname R@an.cost_accuracy.par.W1c.amos.matchesbase\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.par.W1c.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.W1c.kits\endcsname{31.2}
\expandafter\gdef\csname R@an.cost_accuracy.par.W1c.kits.matchesbase\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.par.W1c.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.W2.acdc\endcsname{30.4}
\expandafter\gdef\csname R@an.cost_accuracy.par.W2.acdc.matchesbase\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.par.W2.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.W2.amos\endcsname{31.1}
\expandafter\gdef\csname R@an.cost_accuracy.par.W2.amos.matchesbase\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.par.W2.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.W2.kits\endcsname{31.2}
\expandafter\gdef\csname R@an.cost_accuracy.par.W2.kits.matchesbase\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.par.W2.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.W3.acdc\endcsname{29.6}
\expandafter\gdef\csname R@an.cost_accuracy.par.W3.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.W3.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.W3.amos\endcsname{29.6}
\expandafter\gdef\csname R@an.cost_accuracy.par.W3.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.W3.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.W3.kits\endcsname{29.6}
\expandafter\gdef\csname R@an.cost_accuracy.par.W3.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.W3.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.W3c.acdc\endcsname{29.5}
\expandafter\gdef\csname R@an.cost_accuracy.par.W3c.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.W3c.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.W3c.amos\endcsname{29.5}
\expandafter\gdef\csname R@an.cost_accuracy.par.W3c.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.W3c.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.W3c.kits\endcsname{29.6}
\expandafter\gdef\csname R@an.cost_accuracy.par.W3c.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.W3c.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.W4.acdc\endcsname{33.5}
\expandafter\gdef\csname R@an.cost_accuracy.par.W4.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.W4.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.W4.amos\endcsname{34.2}
\expandafter\gdef\csname R@an.cost_accuracy.par.W4.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.W4.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.W4.kits\endcsname{34.3}
\expandafter\gdef\csname R@an.cost_accuracy.par.W4.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.W4.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.W5.acdc\endcsname{101.6}
\expandafter\gdef\csname R@an.cost_accuracy.par.W5.acdc.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.W5.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.W5.amos\endcsname{102.4}
\expandafter\gdef\csname R@an.cost_accuracy.par.W5.amos.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.W5.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.W5.kits\endcsname{102.4}
\expandafter\gdef\csname R@an.cost_accuracy.par.W5.kits.matchesbase\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.par.W5.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par.base.acdc\endcsname{30.4}
\expandafter\gdef\csname R@an.cost_accuracy.par.base.acdc.plan\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.par.base.amos\endcsname{31.1}
\expandafter\gdef\csname R@an.cost_accuracy.par.base.amos.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.par.base.kits\endcsname{31.2}
\expandafter\gdef\csname R@an.cost_accuracy.par.base.kits.plan\endcsname{KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.par2.C1.acdc\endcsname{51.59}
\expandafter\gdef\csname R@an.cost_accuracy.par2.C1.amos\endcsname{52.34}
\expandafter\gdef\csname R@an.cost_accuracy.par2.C1.kits\endcsname{52.41}
\expandafter\gdef\csname R@an.cost_accuracy.par2.D1.acdc\endcsname{20.11}
\expandafter\gdef\csname R@an.cost_accuracy.par2.D1.amos\endcsname{20.86}
\expandafter\gdef\csname R@an.cost_accuracy.par2.D1.kits\endcsname{20.93}
\expandafter\gdef\csname R@an.cost_accuracy.par2.D2.acdc\endcsname{25.28}
\expandafter\gdef\csname R@an.cost_accuracy.par2.D2.amos\endcsname{26.03}
\expandafter\gdef\csname R@an.cost_accuracy.par2.D2.kits\endcsname{26.08}
\expandafter\gdef\csname R@an.cost_accuracy.par2.L1.acdc\endcsname{101.53}
\expandafter\gdef\csname R@an.cost_accuracy.par2.L1.amos\endcsname{102.28}
\expandafter\gdef\csname R@an.cost_accuracy.par2.L1.kits\endcsname{102.35}
\expandafter\gdef\csname R@an.cost_accuracy.par2.L1b.acdc\endcsname{101.63}
\expandafter\gdef\csname R@an.cost_accuracy.par2.L1b.amos\endcsname{102.37}
\expandafter\gdef\csname R@an.cost_accuracy.par2.L1b.kits\endcsname{102.43}
\expandafter\gdef\csname R@an.cost_accuracy.par2.L2.acdc\endcsname{23.68}
\expandafter\gdef\csname R@an.cost_accuracy.par2.L2.amos\endcsname{24.43}
\expandafter\gdef\csname R@an.cost_accuracy.par2.L2.kits\endcsname{24.50}
\expandafter\gdef\csname R@an.cost_accuracy.par2.L3.acdc\endcsname{28.85}
\expandafter\gdef\csname R@an.cost_accuracy.par2.L3.amos\endcsname{29.59}
\expandafter\gdef\csname R@an.cost_accuracy.par2.L3.kits\endcsname{29.66}
\expandafter\gdef\csname R@an.cost_accuracy.par2.L4.acdc\endcsname{102.02}
\expandafter\gdef\csname R@an.cost_accuracy.par2.L4.amos\endcsname{102.77}
\expandafter\gdef\csname R@an.cost_accuracy.par2.L4.kits\endcsname{102.82}
\expandafter\gdef\csname R@an.cost_accuracy.par2.L6.acdc\endcsname{30.35}
\expandafter\gdef\csname R@an.cost_accuracy.par2.L6.amos\endcsname{31.09}
\expandafter\gdef\csname R@an.cost_accuracy.par2.L6.kits\endcsname{31.17}
\expandafter\gdef\csname R@an.cost_accuracy.par2.P3c.acdc\endcsname{30.38}
\expandafter\gdef\csname R@an.cost_accuracy.par2.P3c.amos\endcsname{31.12}
\expandafter\gdef\csname R@an.cost_accuracy.par2.P3c.kits\endcsname{31.20}
\expandafter\gdef\csname R@an.cost_accuracy.par2.S2.acdc\endcsname{26.97}
\expandafter\gdef\csname R@an.cost_accuracy.par2.S2.amos\endcsname{27.72}
\expandafter\gdef\csname R@an.cost_accuracy.par2.S2.kits\endcsname{27.79}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V5A5.acdc\endcsname{28.73}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V5A5.amos\endcsname{29.47}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V5A5.kits\endcsname{29.53}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V5B1.acdc\endcsname{20.18}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V5B1.amos\endcsname{20.93}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V5B1.kits\endcsname{20.96}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V5B2.acdc\endcsname{20.48}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V5B2.amos\endcsname{21.22}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V5B2.kits\endcsname{21.26}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V6A1r.acdc\endcsname{29.96}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V6A1r.amos\endcsname{30.70}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V6A1r.kits\endcsname{30.78}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V7A1.acdc\endcsname{30.26}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V7A1.amos\endcsname{31.00}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V7A1.kits\endcsname{31.04}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V7A2.acdc\endcsname{30.38}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V7A2.amos\endcsname{31.12}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V7A2.kits\endcsname{31.18}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V7B1.acdc\endcsname{19.65}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V7B1.amos\endcsname{20.40}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V7B1.kits\endcsname{20.43}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V7B2.acdc\endcsname{19.67}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V7B2.amos\endcsname{20.42}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V7B2.kits\endcsname{20.45}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V7C1.acdc\endcsname{20.33}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V7C1.amos\endcsname{21.08}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V7C1.kits\endcsname{21.11}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V8A1.acdc\endcsname{30.53}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V8A1.amos\endcsname{31.27}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V8A1.kits\endcsname{31.31}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V8A2.acdc\endcsname{30.69}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V8A2.amos\endcsname{31.44}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V8A2.kits\endcsname{31.47}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V8B1.acdc\endcsname{17.44}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V8B1.amos\endcsname{18.19}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V8B1.kits\endcsname{18.21}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V8B2.acdc\endcsname{20.32}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V8B2.amos\endcsname{21.07}
\expandafter\gdef\csname R@an.cost_accuracy.par2.V8B2.kits\endcsname{21.08}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W1.acdc\endcsname{30.39}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W1.amos\endcsname{31.14}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W1.kits\endcsname{31.21}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W1c.acdc\endcsname{30.39}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W1c.amos\endcsname{31.14}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W1c.kits\endcsname{31.21}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W2.acdc\endcsname{30.39}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W2.amos\endcsname{31.14}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W2.kits\endcsname{31.21}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W3.acdc\endcsname{29.55}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W3.amos\endcsname{29.57}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W3.kits\endcsname{29.63}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W3c.acdc\endcsname{29.53}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W3c.amos\endcsname{29.54}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W3c.kits\endcsname{29.61}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W4.acdc\endcsname{33.48}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W4.amos\endcsname{34.23}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W4.kits\endcsname{34.30}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W5.acdc\endcsname{101.63}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W5.amos\endcsname{102.37}
\expandafter\gdef\csname R@an.cost_accuracy.par2.W5.kits\endcsname{102.43}
\expandafter\gdef\csname R@an.cost_accuracy.par2.base.acdc\endcsname{30.38}
\expandafter\gdef\csname R@an.cost_accuracy.par2.base.amos\endcsname{31.12}
\expandafter\gdef\csname R@an.cost_accuracy.par2.base.kits\endcsname{31.20}
\expandafter\gdef\csname R@an.cost_accuracy.parclause.L6.amos\endcsname{the default's own parameter count on the AMOS22 plan (31.09 M against 31.12 M)}
\expandafter\gdef\csname R@an.cost_accuracy.parclause.L6.kits\endcsname{the default's own parameter count on the KiTS23 plan (31.17 M against 31.20 M)}
\expandafter\gdef\csname R@an.cost_accuracy.parclause.P3c.acdc\endcsname{the default's own parameter count on the ACDC plan (30.38 M against 30.38 M)}
\expandafter\gdef\csname R@an.cost_accuracy.parclause.P3c.amos\endcsname{the default's own parameter count on the AMOS22 plan (31.12 M against 31.12 M)}
\expandafter\gdef\csname R@an.cost_accuracy.parclause.P3c.kits\endcsname{the default's own parameter count on the KiTS23 plan (31.20 M against 31.20 M)}
\expandafter\gdef\csname R@an.cost_accuracy.parclause.V7A2.acdc\endcsname{the default's own parameter count on the ACDC plan (30.38 M against 30.38 M)}
\expandafter\gdef\csname R@an.cost_accuracy.parclause.V7A2.amos\endcsname{the default's own parameter count on the AMOS22 plan (31.12 M against 31.12 M)}
\expandafter\gdef\csname R@an.cost_accuracy.parclause.V7A2.kits\endcsname{the default's own parameter count on the KiTS23 plan (31.18 M against 31.20 M)}
\expandafter\gdef\csname R@an.cost_accuracy.parclause.W1.acdc\endcsname{the default's own parameter count on the ACDC plan (30.39 M against 30.38 M)}
\expandafter\gdef\csname R@an.cost_accuracy.parclause.W1.amos\endcsname{the default's own parameter count on the AMOS22 plan (31.14 M against 31.12 M)}
\expandafter\gdef\csname R@an.cost_accuracy.parclause.W1.kits\endcsname{the default's own parameter count on the KiTS23 plan (31.21 M against 31.20 M)}
\expandafter\gdef\csname R@an.cost_accuracy.parclause.W1c.acdc\endcsname{the default's own parameter count on the ACDC plan (30.39 M against 30.38 M)}
\expandafter\gdef\csname R@an.cost_accuracy.parclause.W1c.amos\endcsname{the default's own parameter count on the AMOS22 plan (31.14 M against 31.12 M)}
\expandafter\gdef\csname R@an.cost_accuracy.parclause.W1c.kits\endcsname{the default's own parameter count on the KiTS23 plan (31.21 M against 31.20 M)}
\expandafter\gdef\csname R@an.cost_accuracy.parclause.W2.acdc\endcsname{the default's own parameter count on the ACDC plan (30.39 M against 30.38 M)}
\expandafter\gdef\csname R@an.cost_accuracy.parclause.W2.amos\endcsname{the default's own parameter count on the AMOS22 plan (31.14 M against 31.12 M)}
\expandafter\gdef\csname R@an.cost_accuracy.parclause.W2.kits\endcsname{the default's own parameter count on the KiTS23 plan (31.21 M against 31.20 M)}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.acdc\endcsname{nnU-Net default, ConvNeXt-k3, HyReX, LeanAdd with coarse large kernels (LeanAdd-NeXt), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with the coarse operator at stage 5 alone}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.acdc.ai\endcsname{ConvNeXt-k3, HyReX, LeanAdd with coarse large kernels (LeanAdd-NeXt), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with the coarse operator at stage 5 alone}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.acdc.ai.dominated\endcsname{ResEnc+context, HyReX+context, HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.acdc.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.acdc.basis.clause\endcsname{every ACDC delta in this set is the discovery seed 0 of its arm, the one basis all 13 points share; the fresh-seed mean of seeds 1--2, available for 4 of them (HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented), function-identical control), moves by up to 0.166 pp, in both directions}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.acdc.dominated\endcsname{ResEnc-M (library preset), ResEnc-matched (re-implemented), ResEnc+context, HyReX+context, function-identical control, HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.acdc.marginal\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.acdc.n\endcsname{13}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.acdc.narms\endcsname{12}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.acdc.ndom\endcsname{6}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.acdc.nfresh\endcsname{4}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.acdc.nopt\endcsname{7}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.acdc.npend\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.acdc.nrobustdom\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.acdc.pending\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.acdc.robust\endcsname{nnU-Net default, ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, HyReX, ResEnc+context, function-identical control, LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with 9-kernel coarse stages, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with the coarse operator at stage 5 alone}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.acdc.robust.dominated\endcsname{HyReX+context}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos\endcsname{ResEnc-M (library preset), ConvNeXt-k3, HyReX, branch control, offset upsampling, trilinear-decoder control, pooled-skip control, HyReX point-fuse decoder, HyReX, ConvNeXt one stage finer, LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with 9-kernel coarse stages, LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1)}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.ai\endcsname{ConvNeXt-k3, HyReX, offset upsampling, HyReX point-fuse decoder, HyReX, ConvNeXt one stage finer, LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with 9-kernel coarse stages, LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1)}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.ai.dominated\endcsname{ResEnc+context, HyReX+context, $z$-dilation mixing, thickness-gated mixing, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), HyReX with LeanDec fine decoder stages, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec)}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.basis.clause\endcsname{every AMOS22 delta in this set is the discovery seed 0 of its arm, the one basis all 32 points share; the fresh-seed mean of seeds 1--2, available for 5 of them (HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context), moves by up to 0.249 pp, in both directions}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.dominated\endcsname{nnU-Net default, ResEnc-matched (re-implemented), ResEnc+context, HyReX+context, $z$-dilation mixing, thickness-gated mixing, ConvNeXt-4$\times$-GRN (MedNeXt-like reference), HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), function-identical control, HyReX with LeanDec fine decoder stages, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec)}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.fresh\endcsname{nnU-Net default, ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.fresh.ai\endcsname{ConvNeXt-k3, ResEnc+context}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.fresh.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.fresh.clause\endcsname{On the fresh-seed mean of seeds 1--2, over the 5 arms that have one and the default at the origin, the Pareto-optimal points in (parameters, profiled step time, $\Delta$Dice) on AMOS22 are nnU-Net default, ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context; HyReX is dominated by ConvNeXt-k3, 0.062 pp ahead in gain, inside the 0.24 pp edge of the null of a difference of two-seed means}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.fresh.dominated\endcsname{HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.fresh.n\endcsname{6}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.fresh.narms\endcsname{5}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.fresh.ndom\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.fresh.nopt\endcsname{5}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.marginal\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.n\endcsname{32}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.narms\endcsname{31}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.ndom\endcsname{14}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.nfresh\endcsname{5}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.nopt\endcsname{18}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.npend\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.nrobustdom\endcsname{7}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.pending\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.robust\endcsname{nnU-Net default, ResEnc-M (library preset), ConvNeXt-k3, HyReX, ResEnc+context, $z$-dilation mixing, branch control, thickness-gated mixing, offset upsampling, trilinear-decoder control, pooled-skip control, HyReX + decoder capacity, HyReX point-fuse decoder, function-identical control, HyReX, ConvNeXt one stage finer, HyReX with LeanDec fine decoder stages, LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with 9-kernel coarse stages, LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1)}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.amos.robust.dominated\endcsname{ResEnc-matched (re-implemented), HyReX+context, ConvNeXt-4$\times$-GRN (MedNeXt-like reference), LeanDec (default with one conv per decoder stage), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec)}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits\endcsname{HyReX + decoder capacity, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk)}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.ai\endcsname{HyReX + decoder capacity, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk)}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.ai.dominated\endcsname{ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context, HyReX point-fuse decoder, LeanDec (default with one conv per decoder stage), HyReX, ConvNeXt one stage finer, HyReX with LeanDec fine decoder stages, LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with 9-kernel coarse stages, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1)}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.basis.clause\endcsname{every KiTS23 delta in this set is the discovery seed 0 of its arm, the one basis all 26 points share; the fresh-seed mean of seeds 1--2, available for 25 of them (HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context, HyReX+context, branch control, HyReX, ConvNeXt one stage finer, HyReX point-fuse decoder, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), function-identical control, LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with LeanDec fine decoder stages, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with the coarse operator at stage 5 alone, HyReX with 9-kernel coarse stages), moves by up to 1.569 pp, in both directions}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.dominated\endcsname{nnU-Net default, ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context, branch control, HyReX point-fuse decoder, LeanDec (default with one conv per decoder stage), function-identical control, HyReX, ConvNeXt one stage finer, HyReX with LeanDec fine decoder stages, LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with 9-kernel coarse stages, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1)}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.fresh\endcsname{ResEnc-M (library preset), LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1)}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.fresh.ai\endcsname{LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1)}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.fresh.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.fresh.clause\endcsname{On the fresh-seed mean of seeds 1--2, over the 25 arms that have one and the default at the origin, the Pareto-optimal points in (parameters, profiled step time, $\Delta$Dice) on KiTS23 are ResEnc-M (library preset), LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1); nnU-Net default is dominated by LeanDec (default with one conv per decoder stage), LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk) and LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), up to 2.662 pp ahead in gain, above the 1.56 pp edge of the null of a difference of two-seed means; ResEnc-matched (re-implemented) is dominated by LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with separable coarse kernels (LeanSep) and LeanAdd-NeXt with the coarse operator at stage 5 alone, up to 0.349 pp ahead in gain, inside the 1.56 pp edge of the null of a difference of two-seed means; ConvNeXt-k3 is dominated by LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk) and LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), up to 2.330 pp ahead in gain, above the 1.56 pp edge of the null of a difference of two-seed means; HyReX is dominated by HyReX with LeanDec fine decoder stages, LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with separable coarse kernels (LeanSep) and LeanAdd-NeXt with the coarse operator at stage 5 alone, up to 0.346 pp ahead in gain, inside the 1.56 pp edge of the null of a difference of two-seed means; ResEnc+context is dominated by ResEnc-matched (re-implemented), LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep) and LeanAdd-NeXt with the coarse operator at stage 5 alone, up to 0.415 pp ahead in gain, inside the 1.56 pp edge of the null of a difference of two-seed means; HyReX+context is dominated by HyReX, LeanDec (default with one conv per decoder stage), HyReX with LeanDec fine decoder stages, LeanDec with additive skips (LeanAdd), HyReX with 9-kernel coarse stages, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone and LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), up to 1.070 pp ahead in gain, inside the 1.56 pp edge of the null of a difference of two-seed means; branch control is dominated by LeanDec (default with one conv per decoder stage), function-identical control, LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk) and LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), up to 1.595 pp ahead in gain, above the 1.56 pp edge of the null of a difference of two-seed means; HyReX + decoder capacity is dominated by LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid) and LeanAdd-NeXt with the coarse operator at stage 5 alone, up to 0.261 pp ahead in gain, inside the 1.56 pp edge of the null of a difference of two-seed means; HyReX point-fuse decoder is dominated by LeanAdd-NeXt with separable coarse kernels (LeanSep) and LeanAdd-NeXt with dilated coarse kernels (LeanDil), up to 0.905 pp ahead in gain, inside the 1.56 pp edge of the null of a difference of two-seed means; LeanDec (default with one conv per decoder stage) is dominated by LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with separable coarse kernels (LeanSep) and LeanAdd-NeXt with the coarse operator at stage 5 alone, up to 0.548 pp ahead in gain, inside the 1.56 pp edge of the null of a difference of two-seed means; function-identical control is dominated by LeanDec (default with one conv per decoder stage), LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk) and LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), up to 1.486 pp ahead in gain, inside the 1.56 pp edge of the null of a difference of two-seed means; HyReX, ConvNeXt one stage finer is dominated by HyReX point-fuse decoder, LeanDec (default with one conv per decoder stage), LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk) and LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), up to 1.870 pp ahead in gain, above the 1.56 pp edge of the null of a difference of two-seed means; HyReX with LeanDec fine decoder stages is dominated by LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with separable coarse kernels (LeanSep) and LeanAdd-NeXt with the coarse operator at stage 5 alone, up to 0.275 pp ahead in gain, inside the 1.56 pp edge of the null of a difference of two-seed means; LeanAdd with coarse large kernels (LeanAdd-NeXt) is dominated by LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone and LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), up to 0.992 pp ahead in gain, inside the 1.56 pp edge of the null of a difference of two-seed means; HyReX with 9-kernel coarse stages is dominated by HyReX, LeanDec (default with one conv per decoder stage), HyReX with LeanDec fine decoder stages, LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone and LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), up to 0.736 pp ahead in gain, inside the 1.56 pp edge of the null of a difference of two-seed means; LeanDeepMid with the two finest decoder convolutions restored is dominated by LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with separable coarse kernels (LeanSep) and LeanAdd-NeXt with the coarse operator at stage 5 alone, up to 0.373 pp ahead in gain, inside the 1.56 pp edge of the null of a difference of two-seed means; LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack) is dominated by LeanDec (default with one conv per decoder stage), LeanDec with additive skips (LeanAdd), LeanAdd with coarse large kernels (LeanAdd-NeXt), LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk) and LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), up to 1.191 pp ahead in gain, inside the 1.56 pp edge of the null of a difference of two-seed means; LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec) is dominated by LeanDec (default with one conv per decoder stage), LeanDec with additive skips (LeanAdd), LeanAdd-NeXt with separable coarse kernels (LeanSep) and LeanAdd-NeXt with the coarse operator at stage 5 alone, up to 0.563 pp ahead in gain, inside the 1.56 pp edge of the null of a difference of two-seed means}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.fresh.dominated\endcsname{nnU-Net default, ResEnc-matched (re-implemented), ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context, branch control, HyReX + decoder capacity, HyReX point-fuse decoder, LeanDec (default with one conv per decoder stage), function-identical control, HyReX, ConvNeXt one stage finer, HyReX with LeanDec fine decoder stages, LeanAdd with coarse large kernels (LeanAdd-NeXt), HyReX with 9-kernel coarse stages, LeanDeepMid with the two finest decoder convolutions restored, LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec)}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.fresh.n\endcsname{26}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.fresh.narms\endcsname{25}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.fresh.ndom\endcsname{18}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.fresh.nopt\endcsname{8}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.marginal\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.n\endcsname{26}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.narms\endcsname{25}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.ndom\endcsname{24}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.nfresh\endcsname{25}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.nopt\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.npend\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.nrobustdom\endcsname{11}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.pending\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.robust\endcsname{ResEnc-M (library preset), HyReX, ResEnc+context, HyReX+context, branch control, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), HyReX with LeanDec fine decoder stages, LeanDec with additive skips (LeanAdd), HyReX with 9-kernel coarse stages, LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk)}
\expandafter\gdef\csname R@an.cost_accuracy.pareto.kits.robust.dominated\endcsname{nnU-Net default, ResEnc-matched (re-implemented), ConvNeXt-k3, HyReX point-fuse decoder, function-identical control, HyReX, ConvNeXt one stage finer, LeanAdd with coarse large kernels (LeanAdd-NeXt), LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1)}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.C1.acdc\endcsname{170}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.C1.amos\endcsname{168}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.C1.kits\endcsname{168}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.D1.acdc\endcsname{66}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.D1.amos\endcsname{67}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.D1.kits\endcsname{67}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.D2.acdc\endcsname{83}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.D2.amos\endcsname{84}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.D2.kits\endcsname{84}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.L1.acdc\endcsname{334}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.L1.amos\endcsname{329}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.L1.kits\endcsname{328}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.L1b.acdc\endcsname{335}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.L1b.amos\endcsname{329}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.L1b.kits\endcsname{328}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.L2.acdc\endcsname{78}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.L2.amos\endcsname{78}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.L2.kits\endcsname{79}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.L3.acdc\endcsname{95}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.L3.amos\endcsname{95}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.L3.kits\endcsname{95}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.L4.acdc\endcsname{336}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.L4.amos\endcsname{330}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.L4.kits\endcsname{330}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.L6.acdc\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.L6.amos\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.L6.kits\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.P3c.acdc\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.P3c.amos\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.P3c.kits\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.S2.acdc\endcsname{89}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.S2.amos\endcsname{89}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.S2.kits\endcsname{89}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V5A5.acdc\endcsname{95}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V5A5.amos\endcsname{95}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V5A5.kits\endcsname{95}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V5B1.acdc\endcsname{66}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V5B1.amos\endcsname{67}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V5B1.kits\endcsname{67}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V5B2.acdc\endcsname{67}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V5B2.amos\endcsname{68}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V5B2.kits\endcsname{68}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V6A1r.acdc\endcsname{99}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V6A1r.amos\endcsname{99}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V6A1r.kits\endcsname{99}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V7A1.acdc\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V7A1.amos\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V7A1.kits\endcsname{99}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V7A2.acdc\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V7A2.amos\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V7A2.kits\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V7B1.acdc\endcsname{65}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V7B1.amos\endcsname{66}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V7B1.kits\endcsname{66}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V7B2.acdc\endcsname{65}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V7B2.amos\endcsname{66}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V7B2.kits\endcsname{66}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V7C1.acdc\endcsname{67}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V7C1.amos\endcsname{68}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V7C1.kits\endcsname{68}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V8A1.acdc\endcsname{101}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V8A1.amos\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V8A1.kits\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V8A2.acdc\endcsname{101}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V8A2.amos\endcsname{101}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V8A2.kits\endcsname{101}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V8B1.acdc\endcsname{57}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V8B1.amos\endcsname{58}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V8B1.kits\endcsname{58}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V8B2.acdc\endcsname{67}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V8B2.amos\endcsname{68}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.V8B2.kits\endcsname{68}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W1.acdc\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W1.amos\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W1.kits\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W1c.acdc\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W1c.amos\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W1c.kits\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W2.acdc\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W2.amos\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W2.kits\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W3.acdc\endcsname{97}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W3.amos\endcsname{95}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W3.kits\endcsname{95}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W3c.acdc\endcsname{97}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W3c.amos\endcsname{95}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W3c.kits\endcsname{95}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W4.acdc\endcsname{110}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W4.amos\endcsname{110}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W4.kits\endcsname{110}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W5.acdc\endcsname{335}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W5.amos\endcsname{329}
\expandafter\gdef\csname R@an.cost_accuracy.parpct.W5.kits\endcsname{328}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.C1.acdc\endcsname{69.8}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.C1.acdc.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.C1.amos\endcsname{68.2}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.C1.amos.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.C1.kits\endcsname{68.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.C1.kits.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.D1.acdc\endcsname{33.8}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.D1.acdc.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.D1.amos\endcsname{33.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.D1.amos.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.D1.kits\endcsname{32.9}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.D1.kits.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.D2.acdc\endcsname{16.8}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.D2.acdc.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.D2.amos\endcsname{16.4}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.D2.amos.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.D2.kits\endcsname{16.4}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.D2.kits.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L1.acdc\endcsname{234.2}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L1.acdc.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L1.amos\endcsname{228.6}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L1.amos.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L1.kits\endcsname{228.1}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L1.kits.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L1b.acdc\endcsname{234.5}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L1b.acdc.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L1b.amos\endcsname{228.9}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L1b.amos.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L1b.kits\endcsname{228.3}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L1b.kits.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L2.acdc\endcsname{22.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L2.acdc.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L2.amos\endcsname{21.5}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L2.amos.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L2.kits\endcsname{21.5}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L2.kits.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L3.acdc\endcsname{5.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L3.acdc.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L3.amos\endcsname{4.9}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L3.amos.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L3.kits\endcsname{4.9}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L3.kits.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L4.acdc\endcsname{235.8}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L4.acdc.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L4.amos\endcsname{230.2}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L4.amos.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L4.kits\endcsname{229.6}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L4.kits.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L6.acdc\endcsname{0.1}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L6.acdc.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L6.amos\endcsname{0.1}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L6.amos.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L6.kits\endcsname{0.1}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.L6.kits.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.P3c.acdc\endcsname{0.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.P3c.acdc.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.P3c.amos\endcsname{0.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.P3c.amos.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.P3c.kits\endcsname{0.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.P3c.kits.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.S2.acdc\endcsname{11.2}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.S2.acdc.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.S2.amos\endcsname{10.9}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.S2.amos.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.S2.kits\endcsname{10.9}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.S2.kits.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V5A5.acdc\endcsname{5.4}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V5A5.acdc.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V5A5.amos\endcsname{5.3}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V5A5.amos.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V5A5.kits\endcsname{5.4}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V5A5.kits.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V5B1.acdc\endcsname{33.6}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V5B1.acdc.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V5B1.amos\endcsname{32.8}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V5B1.amos.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V5B1.kits\endcsname{32.8}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V5B1.kits.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V5B2.acdc\endcsname{32.6}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V5B2.acdc.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V5B2.amos\endcsname{31.8}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V5B2.amos.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V5B2.kits\endcsname{31.9}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V5B2.kits.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V6A1r.acdc\endcsname{1.4}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V6A1r.acdc.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V6A1r.amos\endcsname{1.4}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V6A1r.amos.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V6A1r.kits\endcsname{1.3}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V6A1r.kits.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7A1.acdc\endcsname{0.4}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7A1.acdc.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7A1.amos\endcsname{0.4}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7A1.amos.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7A1.kits\endcsname{0.5}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7A1.kits.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7A2.acdc\endcsname{0.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7A2.acdc.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7A2.amos\endcsname{0.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7A2.amos.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7A2.kits\endcsname{0.1}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7A2.kits.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7B1.acdc\endcsname{35.3}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7B1.acdc.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7B1.amos\endcsname{34.5}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7B1.amos.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7B1.kits\endcsname{34.5}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7B1.kits.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7B2.acdc\endcsname{35.2}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7B2.acdc.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7B2.amos\endcsname{34.4}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7B2.amos.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7B2.kits\endcsname{34.4}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7B2.kits.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7C1.acdc\endcsname{33.1}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7C1.acdc.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7C1.amos\endcsname{32.3}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7C1.amos.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7C1.kits\endcsname{32.3}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V7C1.kits.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8A1.acdc\endcsname{0.5}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8A1.acdc.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8A1.amos\endcsname{0.5}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8A1.amos.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8A1.kits\endcsname{0.4}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8A1.kits.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8A2.acdc\endcsname{1.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8A2.acdc.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8A2.amos\endcsname{1.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8A2.amos.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8A2.kits\endcsname{0.9}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8A2.kits.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8B1.acdc\endcsname{42.6}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8B1.acdc.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8B1.amos\endcsname{41.6}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8B1.amos.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8B1.kits\endcsname{41.6}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8B1.kits.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8B2.acdc\endcsname{33.1}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8B2.acdc.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8B2.amos\endcsname{32.3}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8B2.amos.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8B2.kits\endcsname{32.4}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.V8B2.kits.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W1.acdc\endcsname{0.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W1.acdc.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W1.amos\endcsname{0.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W1.amos.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W1.kits\endcsname{0.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W1.kits.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W1c.acdc\endcsname{0.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W1c.acdc.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W1c.amos\endcsname{0.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W1c.amos.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W1c.kits\endcsname{0.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W1c.kits.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W2.acdc\endcsname{0.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W2.acdc.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W2.amos\endcsname{0.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W2.amos.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W2.kits\endcsname{0.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W2.kits.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W3.acdc\endcsname{2.7}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W3.acdc.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W3.amos\endcsname{5.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W3.amos.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W3.kits\endcsname{5.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W3.kits.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W3c.acdc\endcsname{2.8}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W3c.acdc.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W3c.amos\endcsname{5.1}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W3c.amos.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W3c.kits\endcsname{5.1}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W3c.kits.dir\endcsname{fewer}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W4.acdc\endcsname{10.2}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W4.acdc.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W4.amos\endcsname{10.0}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W4.amos.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W4.kits\endcsname{9.9}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W4.kits.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W5.acdc\endcsname{234.6}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W5.acdc.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W5.amos\endcsname{228.9}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W5.amos.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W5.kits\endcsname{228.3}
\expandafter\gdef\csname R@an.cost_accuracy.parpctless.W5.kits.dir\endcsname{more}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.C1.acdc\endcsname{\ensuremath{+69.8}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.C1.amos\endcsname{\ensuremath{+68.2}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.C1.kits\endcsname{\ensuremath{+68.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.D1.acdc\endcsname{\ensuremath{-33.8}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.D1.amos\endcsname{\ensuremath{-33.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.D1.kits\endcsname{\ensuremath{-32.9}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.D2.acdc\endcsname{\ensuremath{-16.8}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.D2.amos\endcsname{\ensuremath{-16.4}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.D2.kits\endcsname{\ensuremath{-16.4}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.L1.acdc\endcsname{\ensuremath{+234.2}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.L1.amos\endcsname{\ensuremath{+228.6}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.L1.kits\endcsname{\ensuremath{+228.1}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.L1b.acdc\endcsname{\ensuremath{+234.5}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.L1b.amos\endcsname{\ensuremath{+228.9}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.L1b.kits\endcsname{\ensuremath{+228.3}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.L2.acdc\endcsname{\ensuremath{-22.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.L2.amos\endcsname{\ensuremath{-21.5}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.L2.kits\endcsname{\ensuremath{-21.5}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.L3.acdc\endcsname{\ensuremath{-5.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.L3.amos\endcsname{\ensuremath{-4.9}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.L3.kits\endcsname{\ensuremath{-4.9}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.L4.acdc\endcsname{\ensuremath{+235.8}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.L4.amos\endcsname{\ensuremath{+230.2}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.L4.kits\endcsname{\ensuremath{+229.6}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.L6.acdc\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.L6.amos\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.L6.kits\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.P3c.acdc\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.P3c.amos\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.P3c.kits\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.S2.acdc\endcsname{\ensuremath{-11.2}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.S2.amos\endcsname{\ensuremath{-10.9}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.S2.kits\endcsname{\ensuremath{-10.9}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V5A5.acdc\endcsname{\ensuremath{-5.4}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V5A5.amos\endcsname{\ensuremath{-5.3}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V5A5.kits\endcsname{\ensuremath{-5.4}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V5B1.acdc\endcsname{\ensuremath{-33.6}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V5B1.amos\endcsname{\ensuremath{-32.8}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V5B1.kits\endcsname{\ensuremath{-32.8}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V5B2.acdc\endcsname{\ensuremath{-32.6}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V5B2.amos\endcsname{\ensuremath{-31.8}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V5B2.kits\endcsname{\ensuremath{-31.9}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V6A1r.acdc\endcsname{\ensuremath{-1.4}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V6A1r.amos\endcsname{\ensuremath{-1.4}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V6A1r.kits\endcsname{\ensuremath{-1.3}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V7A1.acdc\endcsname{\ensuremath{-0.4}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V7A1.amos\endcsname{\ensuremath{-0.4}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V7A1.kits\endcsname{\ensuremath{-0.5}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V7A2.acdc\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V7A2.amos\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V7A2.kits\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V7B1.acdc\endcsname{\ensuremath{-35.3}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V7B1.amos\endcsname{\ensuremath{-34.5}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V7B1.kits\endcsname{\ensuremath{-34.5}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V7B2.acdc\endcsname{\ensuremath{-35.2}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V7B2.amos\endcsname{\ensuremath{-34.4}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V7B2.kits\endcsname{\ensuremath{-34.4}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V7C1.acdc\endcsname{\ensuremath{-33.1}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V7C1.amos\endcsname{\ensuremath{-32.3}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V7C1.kits\endcsname{\ensuremath{-32.3}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V8A1.acdc\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V8A1.amos\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V8A1.kits\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V8A2.acdc\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V8A2.amos\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V8A2.kits\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V8B1.acdc\endcsname{\ensuremath{-42.6}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V8B1.amos\endcsname{\ensuremath{-41.6}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V8B1.kits\endcsname{\ensuremath{-41.6}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V8B2.acdc\endcsname{\ensuremath{-33.1}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V8B2.amos\endcsname{\ensuremath{-32.3}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.V8B2.kits\endcsname{\ensuremath{-32.4}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W1.acdc\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W1.amos\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W1.kits\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W1c.acdc\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W1c.amos\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W1c.kits\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W2.acdc\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W2.amos\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W2.kits\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W3.acdc\endcsname{\ensuremath{-2.7}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W3.amos\endcsname{\ensuremath{-5.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W3.kits\endcsname{\ensuremath{-5.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W3c.acdc\endcsname{\ensuremath{-2.8}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W3c.amos\endcsname{\ensuremath{-5.1}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W3c.kits\endcsname{\ensuremath{-5.1}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W4.acdc\endcsname{\ensuremath{+10.2}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W4.amos\endcsname{\ensuremath{+10.0}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W4.kits\endcsname{\ensuremath{+9.9}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W5.acdc\endcsname{\ensuremath{+234.6}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W5.amos\endcsname{\ensuremath{+228.9}}
\expandafter\gdef\csname R@an.cost_accuracy.parpctvsbase.W5.kits\endcsname{\ensuremath{+228.3}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.C1.acdc\endcsname{\ensuremath{+21.213}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.C1.amos\endcsname{\ensuremath{+21.214}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.C1.kits\endcsname{\ensuremath{+21.214}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.D1.acdc\endcsname{\ensuremath{-10.267}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.D1.amos\endcsname{\ensuremath{-10.265}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.D1.kits\endcsname{\ensuremath{-10.265}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.D2.acdc\endcsname{\ensuremath{-5.097}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.D2.amos\endcsname{\ensuremath{-5.099}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.D2.kits\endcsname{\ensuremath{-5.117}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.L1.acdc\endcsname{\ensuremath{+71.154}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.L1.amos\endcsname{\ensuremath{+71.154}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.L1.kits\endcsname{\ensuremath{+71.154}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.L1b.acdc\endcsname{\ensuremath{+71.249}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.L1b.amos\endcsname{\ensuremath{+71.249}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.L1b.kits\endcsname{\ensuremath{+71.231}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.L2.acdc\endcsname{\ensuremath{-6.695}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.L2.amos\endcsname{\ensuremath{-6.695}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.L2.kits\endcsname{\ensuremath{-6.695}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.L3.acdc\endcsname{\ensuremath{-1.532}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.L3.amos\endcsname{\ensuremath{-1.532}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.L3.kits\endcsname{\ensuremath{-1.532}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.L4.acdc\endcsname{\ensuremath{+71.644}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.L4.amos\endcsname{\ensuremath{+71.644}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.L4.kits\endcsname{\ensuremath{+71.626}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.L6.acdc\endcsname{\ensuremath{-0.030}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.L6.amos\endcsname{\ensuremath{-0.030}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.L6.kits\endcsname{\ensuremath{-0.030}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.P3c.acdc\endcsname{\ensuremath{0.000}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.P3c.amos\endcsname{\ensuremath{0.000}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.P3c.kits\endcsname{\ensuremath{0.000}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.S2.acdc\endcsname{\ensuremath{-3.407}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.S2.amos\endcsname{\ensuremath{-3.406}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.S2.kits\endcsname{\ensuremath{-3.406}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V5A5.acdc\endcsname{\ensuremath{-1.647}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V5A5.amos\endcsname{\ensuremath{-1.652}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V5A5.kits\endcsname{\ensuremath{-1.671}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V5B1.acdc\endcsname{\ensuremath{-10.197}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V5B1.amos\endcsname{\ensuremath{-10.195}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V5B1.kits\endcsname{\ensuremath{-10.232}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V5B2.acdc\endcsname{\ensuremath{-9.900}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V5B2.amos\endcsname{\ensuremath{-9.900}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V5B2.kits\endcsname{\ensuremath{-9.937}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V6A1r.acdc\endcsname{\ensuremath{-0.420}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V6A1r.amos\endcsname{\ensuremath{-0.420}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V6A1r.kits\endcsname{\ensuremath{-0.420}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V7A1.acdc\endcsname{\ensuremath{-0.121}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V7A1.amos\endcsname{\ensuremath{-0.121}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V7A1.kits\endcsname{\ensuremath{-0.158}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V7A2.acdc\endcsname{\ensuremath{-0.001}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V7A2.amos\endcsname{\ensuremath{-0.001}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V7A2.kits\endcsname{\ensuremath{-0.019}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V7B1.acdc\endcsname{\ensuremath{-10.727}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V7B1.amos\endcsname{\ensuremath{-10.725}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V7B1.kits\endcsname{\ensuremath{-10.761}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V7B2.acdc\endcsname{\ensuremath{-10.707}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V7B2.amos\endcsname{\ensuremath{-10.709}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V7B2.kits\endcsname{\ensuremath{-10.746}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V7C1.acdc\endcsname{\ensuremath{-10.048}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V7C1.amos\endcsname{\ensuremath{-10.048}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V7C1.kits\endcsname{\ensuremath{-10.085}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V8A1.acdc\endcsname{\ensuremath{+0.153}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V8A1.amos\endcsname{\ensuremath{+0.149}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V8A1.kits\endcsname{\ensuremath{+0.112}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V8A2.acdc\endcsname{\ensuremath{+0.313}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V8A2.amos\endcsname{\ensuremath{+0.315}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V8A2.kits\endcsname{\ensuremath{+0.278}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V8B1.acdc\endcsname{\ensuremath{-12.937}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V8B1.amos\endcsname{\ensuremath{-12.934}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V8B1.kits\endcsname{\ensuremath{-12.989}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V8B2.acdc\endcsname{\ensuremath{-10.057}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V8B2.amos\endcsname{\ensuremath{-10.057}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.V8B2.kits\endcsname{\ensuremath{-10.112}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W1.acdc\endcsname{\ensuremath{+0.013}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W1.amos\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W1.kits\endcsname{\ensuremath{+0.014}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W1c.acdc\endcsname{\ensuremath{+0.013}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W1c.amos\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W1c.kits\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W2.acdc\endcsname{\ensuremath{+0.013}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W2.amos\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W2.kits\endcsname{\ensuremath{+0.014}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W3.acdc\endcsname{\ensuremath{-0.827}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W3.amos\endcsname{\ensuremath{-1.558}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W3.kits\endcsname{\ensuremath{-1.566}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W3c.acdc\endcsname{\ensuremath{-0.847}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W3c.amos\endcsname{\ensuremath{-1.583}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W3c.kits\endcsname{\ensuremath{-1.586}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W4.acdc\endcsname{\ensuremath{+3.103}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W4.amos\endcsname{\ensuremath{+3.102}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W4.kits\endcsname{\ensuremath{+3.104}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W5.acdc\endcsname{\ensuremath{+71.253}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W5.amos\endcsname{\ensuremath{+71.249}}
\expandafter\gdef\csname R@an.cost_accuracy.parvsbase.W5.kits\endcsname{\ensuremath{+71.234}}
\expandafter\gdef\csname R@an.cost_accuracy.peak.acdc.n\endcsname{13}
\expandafter\gdef\csname R@an.cost_accuracy.peak.acdc.nhigh\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.peak.acdc.over\endcsname{0.44}
\expandafter\gdef\csname R@an.cost_accuracy.peak.acdc.worst\endcsname{0.44}
\expandafter\gdef\csname R@an.cost_accuracy.peak.amos.n\endcsname{32}
\expandafter\gdef\csname R@an.cost_accuracy.peak.amos.nhigh\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.peak.amos.over\endcsname{-0.02}
\expandafter\gdef\csname R@an.cost_accuracy.peak.amos.worst\endcsname{0.03}
\expandafter\gdef\csname R@an.cost_accuracy.peak.kits.n\endcsname{26}
\expandafter\gdef\csname R@an.cost_accuracy.peak.kits.nhigh\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.peak.kits.over\endcsname{-0.04}
\expandafter\gdef\csname R@an.cost_accuracy.peak.kits.worst\endcsname{0.05}
\expandafter\gdef\csname R@an.cost_accuracy.pool.n.acdc\endcsname{6}
\expandafter\gdef\csname R@an.cost_accuracy.pool.n.amos\endcsname{6}
\expandafter\gdef\csname R@an.cost_accuracy.pool.n.kits\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.pool.sd.acdc\endcsname{0.099}
\expandafter\gdef\csname R@an.cost_accuracy.pool.sd.amos\endcsname{0.122}
\expandafter\gdef\csname R@an.cost_accuracy.pool.sd.kits\endcsname{0.795}
\expandafter\gdef\csname R@an.cost_accuracy.pool.spread.acdc\endcsname{0.275}
\expandafter\gdef\csname R@an.cost_accuracy.pool.spread.acdc.bars\endcsname{0.79}
\expandafter\gdef\csname R@an.cost_accuracy.pool.spread.amos\endcsname{0.321}
\expandafter\gdef\csname R@an.cost_accuracy.pool.spread.amos.bars\endcsname{0.92}
\expandafter\gdef\csname R@an.cost_accuracy.pool.spread.kits\endcsname{1.522}
\expandafter\gdef\csname R@an.cost_accuracy.pool.spread.kits.bars\endcsname{4.35}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.C1.amos\endcsname{0.0074}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.C1.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.C1.kits\endcsname{0.0458}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.C1.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.D1.amos\endcsname{0.0133}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.D1.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.D1.kits\endcsname{0.0705}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.D1.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.D2.amos\endcsname{\ensuremath{-0.0139}}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.D2.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.D2.kits\endcsname{0.0725}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.D2.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L1.acdc\endcsname{0.0024}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L1.acdc.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L1.amos\endcsname{0.0045}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L1.amos.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L1.kits\endcsname{0.0340}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L1.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L1b.acdc\endcsname{0.0031}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L1b.acdc.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L1b.amos\endcsname{0.0029}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L1b.amos.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L1b.kits\endcsname{0.0226}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L1b.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L2.acdc\endcsname{\ensuremath{-0.0006}}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L2.acdc.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L2.amos\endcsname{0.0080}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L2.amos.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L2.kits\endcsname{0.0045}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L2.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L3.acdc\endcsname{0.0156}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L3.acdc.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L3.amos\endcsname{0.0045}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L3.amos.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L3.kits\endcsname{0.0706}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L3.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L4.acdc\endcsname{0.0031}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L4.acdc.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L4.amos\endcsname{0.0044}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L4.amos.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L4.kits\endcsname{0.0218}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L4.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L6.acdc\endcsname{0.0149}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L6.acdc.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L6.amos\endcsname{0.0005}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L6.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L6.kits\endcsname{0.0511}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.L6.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.P3c.acdc\endcsname{0.0038}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.P3c.acdc.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.P3c.amos\endcsname{0.0002}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.P3c.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.P3c.kits\endcsname{0.0377}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.P3c.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.S2.amos\endcsname{0.0136}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.S2.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.S2.kits\endcsname{0.0205}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.S2.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V5A5.amos\endcsname{0.0014}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V5A5.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V5A5.kits\endcsname{0.0733}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V5A5.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V5B1.amos\endcsname{\ensuremath{-0.0125}}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V5B1.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V5B1.kits\endcsname{0.1090}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V5B1.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V5B2.acdc\endcsname{\ensuremath{-0.0088}}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V5B2.acdc.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V5B2.amos\endcsname{0.0062}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V5B2.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V5B2.kits\endcsname{0.0681}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V5B2.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V6A1r.acdc\endcsname{0.0191}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V6A1r.acdc.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V6A1r.amos\endcsname{0.0159}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V6A1r.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V6A1r.kits\endcsname{0.0554}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V6A1r.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7A1.acdc\endcsname{0.0076}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7A1.acdc.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7A1.amos\endcsname{\ensuremath{-0.0014}}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7A1.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7A1.kits\endcsname{0.0858}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7A1.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7A2.acdc\endcsname{0.0119}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7A2.acdc.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7A2.amos\endcsname{0.0115}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7A2.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7A2.kits\endcsname{0.0734}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7A2.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7B1.amos\endcsname{\ensuremath{-0.0213}}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7B1.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7B1.kits\endcsname{0.1165}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7B1.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7B2.amos\endcsname{\ensuremath{-0.0131}}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7B2.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7B2.kits\endcsname{0.0899}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7B2.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7C1.acdc\endcsname{\ensuremath{-0.0124}}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7C1.acdc.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7C1.amos\endcsname{\ensuremath{-0.0050}}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7C1.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7C1.kits\endcsname{0.1156}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V7C1.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V8A1.amos\endcsname{\ensuremath{-0.0161}}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V8A1.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V8A1.kits\endcsname{0.0399}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V8A1.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V8A2.amos\endcsname{\ensuremath{-0.0099}}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V8A2.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V8A2.kits\endcsname{0.0596}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V8A2.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V8B1.amos\endcsname{\ensuremath{-0.0413}}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V8B1.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V8B1.kits\endcsname{0.0755}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V8B1.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V8B2.amos\endcsname{\ensuremath{-0.0136}}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V8B2.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V8B2.kits\endcsname{0.0821}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.V8B2.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.W1.amos\endcsname{0.0032}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.W1.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.W1c.amos\endcsname{0.0117}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.W1c.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.W1c.kits\endcsname{0.0342}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.W1c.kits.basis\endcsname{the fresh-seed mean of seeds 1--2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.W2.amos\endcsname{0.0068}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.W2.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.W3.amos\endcsname{0.0091}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.W3.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.W3c.amos\endcsname{0.0055}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.W3c.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.W4.amos\endcsname{0.0022}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.W4.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.W5.amos\endcsname{0.0058}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.W5.amos.basis\endcsname{seed 0, the discovery seed}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.acdc.clause\endcsname{HyReX gains 0.0156 pp per million parameters on ACDC and ResEnc-M (library preset) 0.0024, so HyReX gains 6.6 times as much per parameter (measured on the fresh-seed mean of seeds 1--2)}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.acdc.same\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.amos.clause\endcsname{HyReX and ResEnc-M (library preset) both gain 0.0045 pp per million parameters on AMOS22 (measured on the fresh-seed mean of seeds 1--2)}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.amos.same\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.argument.clause\endcsname{HyReX gains 0.0706 pp per million parameters on KiTS23 and ResEnc-M (library preset) 0.0340, so HyReX gains 2.1 times as much per parameter (measured on the fresh-seed mean of seeds 1--2). HyReX gains 0.0156 pp per million parameters on ACDC and ResEnc-M (library preset) 0.0024, so HyReX gains 6.6 times as much per parameter (measured on the fresh-seed mean of seeds 1--2)}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.argument.datasets\endcsname{KiTS23 and ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.argument.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.kits.clause\endcsname{HyReX gains 0.0706 pp per million parameters on KiTS23 and ResEnc-M (library preset) 0.0340, so HyReX gains 2.1 times as much per parameter (measured on the fresh-seed mean of seeds 1--2)}
\expandafter\gdef\csname R@an.cost_accuracy.ppm.kits.same\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.queued.acdc\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.queued.acdc.n\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.queued.amos\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.queued.amos.n\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.queued.kits\endcsname{ConvNeXt-4$\times$-GRN (MedNeXt-like reference)}
\expandafter\gdef\csname R@an.cost_accuracy.queued.kits.n\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.ref.acdc.contemporaneous\endcsname{pending}
\expandafter\gdef\csname R@an.cost_accuracy.ref.acdc.frozen\endcsname{\ensuremath{0.000}}
\expandafter\gdef\csname R@an.cost_accuracy.ref.acdc.frozen.n\endcsname{6}
\expandafter\gdef\csname R@an.cost_accuracy.ref.acdc.uncompiled\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.cost_accuracy.ref.acdc.uncompiled.n\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.ref.amos.contemporaneous\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.cost_accuracy.ref.amos.contemporaneous.n\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.ref.amos.frozen\endcsname{\ensuremath{0.000}}
\expandafter\gdef\csname R@an.cost_accuracy.ref.amos.frozen.n\endcsname{6}
\expandafter\gdef\csname R@an.cost_accuracy.ref.amos.uncompiled\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.cost_accuracy.ref.amos.uncompiled.n\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.ref.kits.contemporaneous\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.cost_accuracy.ref.kits.contemporaneous.n\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.ref.kits.frozen\endcsname{\ensuremath{0.000}}
\expandafter\gdef\csname R@an.cost_accuracy.ref.kits.frozen.n\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.regpend.acdc\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.regpend.acdc.n\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.regpend.amos\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.regpend.amos.n\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.regpend.kits\endcsname{ConvNeXt-4$\times$-GRN (MedNeXt-like reference)}
\expandafter\gdef\csname R@an.cost_accuracy.regpend.kits.n\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.res.C1.acdc\endcsname{11.79}
\expandafter\gdef\csname R@an.cost_accuracy.res.C1.amos\endcsname{11.64}
\expandafter\gdef\csname R@an.cost_accuracy.res.C1.kits\endcsname{9.73}
\expandafter\gdef\csname R@an.cost_accuracy.res.D1.acdc\endcsname{11.77}
\expandafter\gdef\csname R@an.cost_accuracy.res.D1.amos\endcsname{11.15}
\expandafter\gdef\csname R@an.cost_accuracy.res.D1.kits\endcsname{10.08}
\expandafter\gdef\csname R@an.cost_accuracy.res.D2.acdc\endcsname{9.98}
\expandafter\gdef\csname R@an.cost_accuracy.res.D2.amos\endcsname{8.75}
\expandafter\gdef\csname R@an.cost_accuracy.res.D2.kits\endcsname{8.43}
\expandafter\gdef\csname R@an.cost_accuracy.res.L1.acdc\endcsname{11.53}
\expandafter\gdef\csname R@an.cost_accuracy.res.L1.amos\endcsname{11.61}
\expandafter\gdef\csname R@an.cost_accuracy.res.L1.kits\endcsname{10.52}
\expandafter\gdef\csname R@an.cost_accuracy.res.L1b.acdc\endcsname{11.89}
\expandafter\gdef\csname R@an.cost_accuracy.res.L1b.amos\endcsname{11.29}
\expandafter\gdef\csname R@an.cost_accuracy.res.L1b.kits\endcsname{10.22}
\expandafter\gdef\csname R@an.cost_accuracy.res.L2.acdc\endcsname{11.66}
\expandafter\gdef\csname R@an.cost_accuracy.res.L2.amos\endcsname{10.44}
\expandafter\gdef\csname R@an.cost_accuracy.res.L2.kits\endcsname{9.85}
\expandafter\gdef\csname R@an.cost_accuracy.res.L3.acdc\endcsname{11.82}
\expandafter\gdef\csname R@an.cost_accuracy.res.L3.amos\endcsname{11.19}
\expandafter\gdef\csname R@an.cost_accuracy.res.L3.kits\endcsname{10.13}
\expandafter\gdef\csname R@an.cost_accuracy.res.L4.acdc\endcsname{11.29}
\expandafter\gdef\csname R@an.cost_accuracy.res.L4.amos\endcsname{11.43}
\expandafter\gdef\csname R@an.cost_accuracy.res.L4.kits\endcsname{10.26}
\expandafter\gdef\csname R@an.cost_accuracy.res.L6.acdc\endcsname{11.65}
\expandafter\gdef\csname R@an.cost_accuracy.res.L6.amos\endcsname{10.71}
\expandafter\gdef\csname R@an.cost_accuracy.res.L6.kits\endcsname{9.90}
\expandafter\gdef\csname R@an.cost_accuracy.res.P3c.acdc\endcsname{11.15}
\expandafter\gdef\csname R@an.cost_accuracy.res.P3c.amos\endcsname{9.43}
\expandafter\gdef\csname R@an.cost_accuracy.res.P3c.kits\endcsname{9.17}
\expandafter\gdef\csname R@an.cost_accuracy.res.S2.acdc\endcsname{11.88}
\expandafter\gdef\csname R@an.cost_accuracy.res.S2.amos\endcsname{10.94}
\expandafter\gdef\csname R@an.cost_accuracy.res.S2.kits\endcsname{9.98}
\expandafter\gdef\csname R@an.cost_accuracy.res.V5A5.acdc\endcsname{11.98}
\expandafter\gdef\csname R@an.cost_accuracy.res.V5A5.amos\endcsname{10.44}
\expandafter\gdef\csname R@an.cost_accuracy.res.V5A5.kits\endcsname{9.59}
\expandafter\gdef\csname R@an.cost_accuracy.res.V5B1.acdc\endcsname{9.87}
\expandafter\gdef\csname R@an.cost_accuracy.res.V5B1.amos\endcsname{8.57}
\expandafter\gdef\csname R@an.cost_accuracy.res.V5B1.kits\endcsname{8.16}
\expandafter\gdef\csname R@an.cost_accuracy.res.V5B2.acdc\endcsname{10.06}
\expandafter\gdef\csname R@an.cost_accuracy.res.V5B2.amos\endcsname{8.65}
\expandafter\gdef\csname R@an.cost_accuracy.res.V5B2.kits\endcsname{8.19}
\expandafter\gdef\csname R@an.cost_accuracy.res.V6A1r.acdc\endcsname{11.83}
\expandafter\gdef\csname R@an.cost_accuracy.res.V6A1r.amos\endcsname{11.20}
\expandafter\gdef\csname R@an.cost_accuracy.res.V6A1r.kits\endcsname{10.14}
\expandafter\gdef\csname R@an.cost_accuracy.res.V7A1.acdc\endcsname{10.73}
\expandafter\gdef\csname R@an.cost_accuracy.res.V7A1.amos\endcsname{9.20}
\expandafter\gdef\csname R@an.cost_accuracy.res.V7A1.kits\endcsname{8.52}
\expandafter\gdef\csname R@an.cost_accuracy.res.V7A2.acdc\endcsname{11.61}
\expandafter\gdef\csname R@an.cost_accuracy.res.V7A2.amos\endcsname{9.96}
\expandafter\gdef\csname R@an.cost_accuracy.res.V7A2.kits\endcsname{9.19}
\expandafter\gdef\csname R@an.cost_accuracy.res.V7B1.acdc\endcsname{10.11}
\expandafter\gdef\csname R@an.cost_accuracy.res.V7B1.amos\endcsname{8.64}
\expandafter\gdef\csname R@an.cost_accuracy.res.V7B1.kits\endcsname{8.19}
\expandafter\gdef\csname R@an.cost_accuracy.res.V7B2.acdc\endcsname{10.06}
\expandafter\gdef\csname R@an.cost_accuracy.res.V7B2.amos\endcsname{8.65}
\expandafter\gdef\csname R@an.cost_accuracy.res.V7B2.kits\endcsname{8.18}
\expandafter\gdef\csname R@an.cost_accuracy.res.V7C1.acdc\endcsname{9.89}
\expandafter\gdef\csname R@an.cost_accuracy.res.V7C1.amos\endcsname{8.58}
\expandafter\gdef\csname R@an.cost_accuracy.res.V7C1.kits\endcsname{8.17}
\expandafter\gdef\csname R@an.cost_accuracy.res.V8A1.acdc\endcsname{10.12}
\expandafter\gdef\csname R@an.cost_accuracy.res.V8A1.amos\endcsname{8.68}
\expandafter\gdef\csname R@an.cost_accuracy.res.V8A1.kits\endcsname{8.25}
\expandafter\gdef\csname R@an.cost_accuracy.res.V8A2.acdc\endcsname{10.07}
\expandafter\gdef\csname R@an.cost_accuracy.res.V8A2.amos\endcsname{8.68}
\expandafter\gdef\csname R@an.cost_accuracy.res.V8A2.kits\endcsname{8.23}
\expandafter\gdef\csname R@an.cost_accuracy.res.V8B1.acdc\endcsname{8.84}
\expandafter\gdef\csname R@an.cost_accuracy.res.V8B1.amos\endcsname{7.66}
\expandafter\gdef\csname R@an.cost_accuracy.res.V8B1.kits\endcsname{7.48}
\expandafter\gdef\csname R@an.cost_accuracy.res.V8B2.acdc\endcsname{9.15}
\expandafter\gdef\csname R@an.cost_accuracy.res.V8B2.amos\endcsname{7.93}
\expandafter\gdef\csname R@an.cost_accuracy.res.V8B2.kits\endcsname{7.57}
\expandafter\gdef\csname R@an.cost_accuracy.res.W1.acdc\endcsname{11.37}
\expandafter\gdef\csname R@an.cost_accuracy.res.W1.amos\endcsname{9.82}
\expandafter\gdef\csname R@an.cost_accuracy.res.W1.kits\endcsname{9.25}
\expandafter\gdef\csname R@an.cost_accuracy.res.W1c.acdc\endcsname{11.61}
\expandafter\gdef\csname R@an.cost_accuracy.res.W1c.amos\endcsname{9.82}
\expandafter\gdef\csname R@an.cost_accuracy.res.W1c.kits\endcsname{9.25}
\expandafter\gdef\csname R@an.cost_accuracy.res.W2.acdc\endcsname{11.40}
\expandafter\gdef\csname R@an.cost_accuracy.res.W2.amos\endcsname{9.84}
\expandafter\gdef\csname R@an.cost_accuracy.res.W2.kits\endcsname{9.27}
\expandafter\gdef\csname R@an.cost_accuracy.res.W3.acdc\endcsname{11.35}
\expandafter\gdef\csname R@an.cost_accuracy.res.W3.amos\endcsname{9.99}
\expandafter\gdef\csname R@an.cost_accuracy.res.W3.kits\endcsname{9.31}
\expandafter\gdef\csname R@an.cost_accuracy.res.W3c.acdc\endcsname{11.37}
\expandafter\gdef\csname R@an.cost_accuracy.res.W3c.amos\endcsname{10.65}
\expandafter\gdef\csname R@an.cost_accuracy.res.W3c.kits\endcsname{10.10}
\expandafter\gdef\csname R@an.cost_accuracy.res.W4.acdc\endcsname{11.77}
\expandafter\gdef\csname R@an.cost_accuracy.res.W4.amos\endcsname{11.88}
\expandafter\gdef\csname R@an.cost_accuracy.res.W4.kits\endcsname{10.07}
\expandafter\gdef\csname R@an.cost_accuracy.res.W5.acdc\endcsname{12.00}
\expandafter\gdef\csname R@an.cost_accuracy.res.W5.amos\endcsname{11.37}
\expandafter\gdef\csname R@an.cost_accuracy.res.W5.kits\endcsname{10.27}
\expandafter\gdef\csname R@an.cost_accuracy.res.base.acdc\endcsname{11.15}
\expandafter\gdef\csname R@an.cost_accuracy.res.base.amos\endcsname{9.43}
\expandafter\gdef\csname R@an.cost_accuracy.res.base.kits\endcsname{9.17}
\expandafter\gdef\csname R@an.cost_accuracy.res.gap.L3L1.acdc\endcsname{0.29}
\expandafter\gdef\csname R@an.cost_accuracy.res.gap.L3L1.amos\endcsname{0.42}
\expandafter\gdef\csname R@an.cost_accuracy.res.gap.L3L1.kits\endcsname{0.39}
\expandafter\gdef\csname R@an.cost_accuracy.res.maxgap.L3L1\endcsname{0.42}
\expandafter\gdef\csname R@an.cost_accuracy.res.maxgap.L3L1.exact\endcsname{0.420}
\expandafter\gdef\csname R@an.cost_accuracy.res.maxgap.L3L1.plan\endcsname{AMOS22}
\expandafter\gdef\csname R@an.cost_accuracy.retest.max\endcsname{1.5}
\expandafter\gdef\csname R@an.cost_accuracy.retest.n\endcsname{21}
\expandafter\gdef\csname R@an.cost_accuracy.retest.sd\endcsname{0.4}
\expandafter\gdef\csname R@an.cost_accuracy.running.acdc\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.running.acdc.n\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.running.amos\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.running.amos.n\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.running.kits\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.running.kits.n\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.screen.C1.amos.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.C1.amos.d0.margin\endcsname{\ensuremath{+0.040}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.C1.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.C1.kits.d0.margin\endcsname{\ensuremath{+3.157}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.C1.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.C1.kits.dfresh.margin\endcsname{\ensuremath{+2.051}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.C1.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+3.507} pp at the discovery seed and \ensuremath{+2.401} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+2.128} and \ensuremath{+2.674}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.D1.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.D1.amos.d0.margin\endcsname{\ensuremath{-0.072}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.D1.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.D1.kits.d0.margin\endcsname{\ensuremath{+1.257}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.D1.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.D1.kits.dfresh.margin\endcsname{\ensuremath{+1.127}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.D1.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+1.607} pp at the discovery seed and \ensuremath{+1.477} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+1.759} and \ensuremath{+1.194}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.D2.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.D2.amos.d0.margin\endcsname{\ensuremath{-0.712}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.D2.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.D2.kits.d0.margin\endcsname{\ensuremath{+2.005}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.D2.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.D2.kits.dfresh.margin\endcsname{\ensuremath{+1.542}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.D2.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+2.355} pp at the discovery seed and \ensuremath{+1.892} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+1.979} and \ensuremath{+1.804}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1.amos.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1.amos.d0.margin\endcsname{\ensuremath{+0.297}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1.amos.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1.amos.dfresh.margin\endcsname{\ensuremath{+0.115}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1.amos.reproduce\endcsname{the AMOS22 screen result reproduces on the registered replication estimand: \ensuremath{+0.647} pp at the discovery seed and \ensuremath{+0.465} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+0.662} and \ensuremath{+0.268}; every AMOS22 delta here is against the frozen 6-run pool whose own runs span 0.321 pp, and against the registered uncompiled sub-pool (3 of those 6 runs) the same fresh mean is \ensuremath{+0.436} pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1.kits.d0.margin\endcsname{\ensuremath{+1.976}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1.kits.dfresh.margin\endcsname{\ensuremath{+3.125}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+2.326} pp at the discovery seed and \ensuremath{+3.475} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+3.134} and \ensuremath{+3.817}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1b.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1b.amos.d0.margin\endcsname{\ensuremath{-0.212}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1b.amos.dfresh\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1b.amos.dfresh.margin\endcsname{\ensuremath{-0.052}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1b.amos.reproduce\endcsname{this arm never cleared the 0.35 pp AMOS22 screen bar at the discovery seed (\ensuremath{+0.138} pp), so there is no screen result to reproduce; its fresh mean is \ensuremath{+0.298} pp; every AMOS22 delta here is against the frozen 6-run pool whose own runs span 0.321 pp, and against the registered uncompiled sub-pool (3 of those 6 runs) the same fresh mean is \ensuremath{+0.269} pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1b.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1b.kits.d0.margin\endcsname{\ensuremath{+1.393}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1b.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1b.kits.dfresh.margin\endcsname{\ensuremath{+1.963}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L1b.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+1.743} pp at the discovery seed and \ensuremath{+2.313} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+2.564} and \ensuremath{+2.062}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L2.amos.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L2.amos.d0.margin\endcsname{\ensuremath{+0.012}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L2.amos.dfresh\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L2.amos.dfresh.margin\endcsname{\ensuremath{-0.156}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L2.amos.reproduce\endcsname{the AMOS22 screen result does not reproduce on the registered replication estimand: the discovery seed cleared the 0.35 pp bar at \ensuremath{+0.362} pp, and the fresh mean of seeds 1--2, from two seeds at \ensuremath{+0.255} and \ensuremath{+0.134}, is \ensuremath{+0.194} pp, inside the 0.26 pp single-seed band; the fresh-seed difference is larger than the standard error of its own two seeds (0.061 pp) and, at 1.95 times the 0.100 pp null SD of a two-seed mean delta, the design is not separated from the default at two seeds; every AMOS22 delta here is against the frozen 6-run pool whose own runs span 0.321 pp, and against the registered uncompiled sub-pool (3 of those 6 runs) the same fresh mean is \ensuremath{+0.166} pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L2.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L2.kits.d0.margin\endcsname{\ensuremath{+0.314}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L2.kits.dfresh\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L2.kits.dfresh.margin\endcsname{\ensuremath{-0.240}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L2.kits.reproduce\endcsname{the KiTS23 screen result does not reproduce on the registered replication estimand: the discovery seed cleared the 0.35 pp bar at \ensuremath{+0.664} pp, and the fresh mean of seeds 1--2, from two seeds at \ensuremath{-0.805} and \ensuremath{+1.026}, is \ensuremath{+0.110} pp, inside the 1.84 pp single-seed band; the fresh-seed difference is smaller than the standard error of its own two seeds (0.915 pp) and, at 0.15 times the 0.726 pp null SD of a two-seed mean delta, the design is not separated from the default at two seeds; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L3.amos.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L3.amos.d0.margin\endcsname{\ensuremath{+0.032}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L3.amos.dfresh\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L3.amos.dfresh.margin\endcsname{\ensuremath{-0.218}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L3.amos.reproduce\endcsname{the AMOS22 screen result does not reproduce on the registered replication estimand: the discovery seed cleared the 0.35 pp bar at \ensuremath{+0.382} pp, and the fresh mean of seeds 1--2, from two seeds at \ensuremath{+0.280} and \ensuremath{-0.016}, is \ensuremath{+0.132} pp, inside the 0.26 pp single-seed band; the fresh-seed difference is smaller than the standard error of its own two seeds (0.148 pp) and, at 1.33 times the 0.100 pp null SD of a two-seed mean delta, the design is not separated from the default at two seeds; every AMOS22 delta here is against the frozen 6-run pool whose own runs span 0.321 pp, and against the registered uncompiled sub-pool (3 of those 6 runs) the same fresh mean is \ensuremath{+0.104} pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L3.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L3.kits.d0.margin\endcsname{\ensuremath{+2.492}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L3.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L3.kits.dfresh.margin\endcsname{\ensuremath{+1.744}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L3.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+2.842} pp at the discovery seed and \ensuremath{+2.094} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+1.798} and \ensuremath{+2.390}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L4.amos.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L4.amos.d0.margin\endcsname{\ensuremath{+0.080}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L4.amos.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L4.amos.dfresh.margin\endcsname{\ensuremath{+0.105}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L4.amos.reproduce\endcsname{the AMOS22 screen result reproduces on the registered replication estimand: \ensuremath{+0.430} pp at the discovery seed and \ensuremath{+0.455} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+0.352} and \ensuremath{+0.557}; every AMOS22 delta here is against the frozen 6-run pool whose own runs span 0.321 pp, and against the registered uncompiled sub-pool (3 of those 6 runs) the same fresh mean is \ensuremath{+0.426} pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L4.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L4.kits.d0.margin\endcsname{\ensuremath{+1.848}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L4.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L4.kits.dfresh.margin\endcsname{\ensuremath{+1.896}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L4.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+2.198} pp at the discovery seed and \ensuremath{+2.246} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+2.677} and \ensuremath{+1.815}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L6.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L6.amos.d0.margin\endcsname{\ensuremath{-0.334}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L6.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L6.kits.d0.margin\endcsname{\ensuremath{+2.176}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L6.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L6.kits.dfresh.margin\endcsname{\ensuremath{+1.241}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.L6.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+2.526} pp at the discovery seed and \ensuremath{+1.591} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+1.198} and \ensuremath{+1.984}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.P3c.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.P3c.amos.d0.margin\endcsname{\ensuremath{-0.343}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.P3c.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.P3c.kits.d0.margin\endcsname{\ensuremath{+1.014}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.P3c.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.P3c.kits.dfresh.margin\endcsname{\ensuremath{+0.826}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.P3c.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+1.364} pp at the discovery seed and \ensuremath{+1.176} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+1.151} and \ensuremath{+1.201}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.S2.amos.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.S2.amos.d0.margin\endcsname{\ensuremath{+0.028}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.S2.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.S2.kits.d0.margin\endcsname{\ensuremath{+0.991}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.S2.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.S2.kits.dfresh.margin\endcsname{\ensuremath{+0.220}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.S2.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+1.341} pp at the discovery seed and \ensuremath{+0.570} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+0.782} and \ensuremath{+0.358}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5A5.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5A5.amos.d0.margin\endcsname{\ensuremath{-0.309}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5A5.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5A5.kits.d0.margin\endcsname{\ensuremath{+1.599}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5A5.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5A5.kits.dfresh.margin\endcsname{\ensuremath{+1.815}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5A5.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+1.949} pp at the discovery seed and \ensuremath{+2.165} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+2.348} and \ensuremath{+1.983}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5B1.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5B1.amos.d0.margin\endcsname{\ensuremath{-0.611}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5B1.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5B1.kits.d0.margin\endcsname{\ensuremath{+1.812}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5B1.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5B1.kits.dfresh.margin\endcsname{\ensuremath{+1.935}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5B1.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+2.162} pp at the discovery seed and \ensuremath{+2.285} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+2.242} and \ensuremath{+2.328}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5B2.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5B2.amos.d0.margin\endcsname{\ensuremath{-0.218}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5B2.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5B2.kits.d0.margin\endcsname{\ensuremath{+0.914}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5B2.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5B2.kits.dfresh.margin\endcsname{\ensuremath{+1.098}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V5B2.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+1.264} pp at the discovery seed and \ensuremath{+1.448} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+1.498} and \ensuremath{+1.399}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V6A1r.amos.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V6A1r.amos.d0.margin\endcsname{\ensuremath{+0.137}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V6A1r.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V6A1r.kits.d0.margin\endcsname{\ensuremath{+1.886}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V6A1r.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V6A1r.kits.dfresh.margin\endcsname{\ensuremath{+1.354}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V6A1r.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+2.236} pp at the discovery seed and \ensuremath{+1.704} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+1.695} and \ensuremath{+1.713}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7A1.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7A1.amos.d0.margin\endcsname{\ensuremath{-0.395}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7A1.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7A1.kits.d0.margin\endcsname{\ensuremath{+2.198}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7A1.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7A1.kits.dfresh.margin\endcsname{\ensuremath{+2.312}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7A1.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+2.548} pp at the discovery seed and \ensuremath{+2.662} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+2.326} and \ensuremath{+2.997}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7A2.amos.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7A2.amos.d0.margin\endcsname{\ensuremath{+0.009}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7A2.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7A2.kits.d0.margin\endcsname{\ensuremath{+2.536}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7A2.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7A2.kits.dfresh.margin\endcsname{\ensuremath{+1.939}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7A2.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+2.886} pp at the discovery seed and \ensuremath{+2.289} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+1.973} and \ensuremath{+2.606}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7B1.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7B1.amos.d0.margin\endcsname{\ensuremath{-0.786}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7B1.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7B1.kits.d0.margin\endcsname{\ensuremath{+1.371}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7B1.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7B1.kits.dfresh.margin\endcsname{\ensuremath{+2.032}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7B1.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+1.721} pp at the discovery seed and \ensuremath{+2.382} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+2.053} and \ensuremath{+2.710}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7B2.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7B2.amos.d0.margin\endcsname{\ensuremath{-0.617}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7B2.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7B2.kits.d0.margin\endcsname{\ensuremath{+2.474}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7B2.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7B2.kits.dfresh.margin\endcsname{\ensuremath{+1.488}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7B2.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+2.824} pp at the discovery seed and \ensuremath{+1.838} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+2.395} and \ensuremath{+1.282}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7C1.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7C1.amos.d0.margin\endcsname{\ensuremath{-0.456}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7C1.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7C1.kits.d0.margin\endcsname{\ensuremath{+2.357}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7C1.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7C1.kits.dfresh.margin\endcsname{\ensuremath{+2.090}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V7C1.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+2.707} pp at the discovery seed and \ensuremath{+2.440} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+2.758} and \ensuremath{+2.121}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8A1.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8A1.amos.d0.margin\endcsname{\ensuremath{-0.855}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8A1.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8A1.kits.d0.margin\endcsname{\ensuremath{+1.410}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8A1.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8A1.kits.dfresh.margin\endcsname{\ensuremath{+0.899}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8A1.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+1.760} pp at the discovery seed and \ensuremath{+1.249} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+1.077} and \ensuremath{+1.421}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8A2.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8A2.amos.d0.margin\endcsname{\ensuremath{-0.662}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8A2.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8A2.kits.d0.margin\endcsname{\ensuremath{+1.003}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8A2.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8A2.kits.dfresh.margin\endcsname{\ensuremath{+1.527}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8A2.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+1.353} pp at the discovery seed and \ensuremath{+1.877} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+1.593} and \ensuremath{+2.162}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8B1.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8B1.amos.d0.margin\endcsname{\ensuremath{-1.101}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8B1.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8B1.kits.d0.margin\endcsname{\ensuremath{+2.561}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8B1.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8B1.kits.dfresh.margin\endcsname{\ensuremath{+1.025}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8B1.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+2.911} pp at the discovery seed and \ensuremath{+1.375} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+2.079} and \ensuremath{+0.670}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8B2.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8B2.amos.d0.margin\endcsname{\ensuremath{-0.637}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8B2.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8B2.kits.d0.margin\endcsname{\ensuremath{+1.296}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8B2.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8B2.kits.dfresh.margin\endcsname{\ensuremath{+1.381}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.V8B2.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+1.646} pp at the discovery seed and \ensuremath{+1.731} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+1.892} and \ensuremath{+1.570}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.W1.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.W1.amos.d0.margin\endcsname{\ensuremath{-0.251}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.W1c.amos.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.W1c.amos.d0.margin\endcsname{\ensuremath{+0.013}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.W1c.kits.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.W1c.kits.d0.margin\endcsname{\ensuremath{+2.286}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.W1c.kits.dfresh\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.W1c.kits.dfresh.margin\endcsname{\ensuremath{+0.717}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.W1c.kits.reproduce\endcsname{the KiTS23 screen result reproduces on the registered replication estimand: \ensuremath{+2.636} pp at the discovery seed and \ensuremath{+1.067} pp on the fresh mean of seeds 1--2, both above the 0.35 pp bar, from two seeds at \ensuremath{+1.734} and \ensuremath{+0.399}; every KiTS23 delta here is against the frozen 3-run pool whose own runs span 1.522 pp}
\expandafter\gdef\csname R@an.cost_accuracy.screen.W2.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.W2.amos.d0.margin\endcsname{\ensuremath{-0.139}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.W3.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.W3.amos.d0.margin\endcsname{\ensuremath{-0.080}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.W3c.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.W3c.amos.d0.margin\endcsname{\ensuremath{-0.188}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.W4.amos.d0\endcsname{does not clear}
\expandafter\gdef\csname R@an.cost_accuracy.screen.W4.amos.d0.margin\endcsname{\ensuremath{-0.274}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.W5.amos.d0\endcsname{clears}
\expandafter\gdef\csname R@an.cost_accuracy.screen.W5.amos.d0.margin\endcsname{\ensuremath{+0.241}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.bar\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cost_accuracy.screen.basis\endcsname{discovery seed 0, the seed the registered screen acted on}
\expandafter\gdef\csname R@an.cost_accuracy.se.pair.acdc\endcsname{0.14}
\expandafter\gdef\csname R@an.cost_accuracy.se.pair.amos\endcsname{0.17}
\expandafter\gdef\csname R@an.cost_accuracy.se.pair.kits\endcsname{1.12}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.C1.amos.0\endcsname{\ensuremath{+0.390}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.C1.kits.0\endcsname{\ensuremath{+3.507}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.C1.kits.1\endcsname{\ensuremath{+2.128}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.C1.kits.2\endcsname{\ensuremath{+2.674}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.D1.amos.0\endcsname{\ensuremath{+0.278}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.D1.kits.0\endcsname{\ensuremath{+1.607}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.D1.kits.1\endcsname{\ensuremath{+1.759}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.D1.kits.2\endcsname{\ensuremath{+1.194}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.D2.amos.0\endcsname{\ensuremath{-0.362}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.D2.kits.0\endcsname{\ensuremath{+2.355}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.D2.kits.1\endcsname{\ensuremath{+1.979}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.D2.kits.2\endcsname{\ensuremath{+1.804}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L1.acdc.0\endcsname{\ensuremath{+0.336}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L1.amos.0\endcsname{\ensuremath{+0.647}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L1.amos.1\endcsname{\ensuremath{+0.662}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L1.amos.2\endcsname{\ensuremath{+0.268}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L1.kits.0\endcsname{\ensuremath{+2.326}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L1.kits.1\endcsname{\ensuremath{+3.134}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L1.kits.2\endcsname{\ensuremath{+3.817}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L1b.acdc.0\endcsname{\ensuremath{+0.283}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L1b.amos.0\endcsname{\ensuremath{+0.138}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L1b.kits.0\endcsname{\ensuremath{+1.743}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L1b.kits.1\endcsname{\ensuremath{+2.564}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L1b.kits.2\endcsname{\ensuremath{+2.062}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L2.acdc.0\endcsname{\ensuremath{-0.015}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L2.amos.0\endcsname{\ensuremath{+0.362}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L2.amos.1\endcsname{\ensuremath{+0.255}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L2.amos.2\endcsname{\ensuremath{+0.134}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L2.kits.0\endcsname{\ensuremath{+0.664}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L2.kits.1\endcsname{\ensuremath{-0.805}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L2.kits.2\endcsname{\ensuremath{+1.026}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L3.acdc.0\endcsname{\ensuremath{+0.616}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L3.amos.0\endcsname{\ensuremath{+0.382}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L3.amos.1\endcsname{\ensuremath{+0.280}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L3.amos.2\endcsname{\ensuremath{-0.016}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L3.kits.0\endcsname{\ensuremath{+2.842}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L3.kits.1\endcsname{\ensuremath{+1.798}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L3.kits.2\endcsname{\ensuremath{+2.390}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L4.acdc.0\endcsname{\ensuremath{+0.315}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L4.amos.0\endcsname{\ensuremath{+0.430}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L4.amos.1\endcsname{\ensuremath{+0.352}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L4.amos.2\endcsname{\ensuremath{+0.557}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L4.kits.0\endcsname{\ensuremath{+2.198}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L4.kits.1\endcsname{\ensuremath{+2.677}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L4.kits.2\endcsname{\ensuremath{+1.815}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L6.acdc.0\endcsname{\ensuremath{+0.451}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L6.amos.0\endcsname{\ensuremath{+0.016}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L6.kits.0\endcsname{\ensuremath{+2.526}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L6.kits.1\endcsname{\ensuremath{+1.198}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.L6.kits.2\endcsname{\ensuremath{+1.984}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.P3c.acdc.0\endcsname{\ensuremath{-0.013}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.P3c.amos.0\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.P3c.kits.0\endcsname{\ensuremath{+1.364}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.P3c.kits.1\endcsname{\ensuremath{+1.151}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.P3c.kits.2\endcsname{\ensuremath{+1.201}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.S2.amos.0\endcsname{\ensuremath{+0.378}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.S2.kits.0\endcsname{\ensuremath{+1.341}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.S2.kits.1\endcsname{\ensuremath{+0.782}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.S2.kits.2\endcsname{\ensuremath{+0.358}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V5A5.amos.0\endcsname{\ensuremath{+0.041}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V5A5.kits.0\endcsname{\ensuremath{+1.949}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V5A5.kits.1\endcsname{\ensuremath{+2.348}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V5A5.kits.2\endcsname{\ensuremath{+1.983}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V5B1.amos.0\endcsname{\ensuremath{-0.261}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V5B1.kits.0\endcsname{\ensuremath{+2.162}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V5B1.kits.1\endcsname{\ensuremath{+2.242}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V5B1.kits.2\endcsname{\ensuremath{+2.328}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V5B2.acdc.0\endcsname{\ensuremath{-0.181}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V5B2.amos.0\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V5B2.kits.0\endcsname{\ensuremath{+1.264}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V5B2.kits.1\endcsname{\ensuremath{+1.498}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V5B2.kits.2\endcsname{\ensuremath{+1.399}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V6A1r.acdc.0\endcsname{\ensuremath{+0.573}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V6A1r.amos.0\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V6A1r.kits.0\endcsname{\ensuremath{+2.236}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V6A1r.kits.1\endcsname{\ensuremath{+1.695}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V6A1r.kits.2\endcsname{\ensuremath{+1.713}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7A1.acdc.0\endcsname{\ensuremath{+0.229}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7A1.amos.0\endcsname{\ensuremath{-0.045}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7A1.kits.0\endcsname{\ensuremath{+2.548}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7A1.kits.1\endcsname{\ensuremath{+2.326}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7A1.kits.2\endcsname{\ensuremath{+2.997}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7A2.acdc.0\endcsname{\ensuremath{+0.362}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7A2.amos.0\endcsname{\ensuremath{+0.359}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7A2.kits.0\endcsname{\ensuremath{+2.886}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7A2.kits.1\endcsname{\ensuremath{+1.973}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7A2.kits.2\endcsname{\ensuremath{+2.606}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7B1.amos.0\endcsname{\ensuremath{-0.436}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7B1.kits.0\endcsname{\ensuremath{+1.721}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7B1.kits.1\endcsname{\ensuremath{+2.053}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7B1.kits.2\endcsname{\ensuremath{+2.710}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7B2.amos.0\endcsname{\ensuremath{-0.267}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7B2.kits.0\endcsname{\ensuremath{+2.824}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7B2.kits.1\endcsname{\ensuremath{+2.395}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7B2.kits.2\endcsname{\ensuremath{+1.282}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7C1.acdc.0\endcsname{\ensuremath{-0.252}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7C1.amos.0\endcsname{\ensuremath{-0.106}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7C1.kits.0\endcsname{\ensuremath{+2.707}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7C1.kits.1\endcsname{\ensuremath{+2.758}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V7C1.kits.2\endcsname{\ensuremath{+2.121}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V8A1.amos.0\endcsname{\ensuremath{-0.505}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V8A1.kits.0\endcsname{\ensuremath{+1.760}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V8A1.kits.1\endcsname{\ensuremath{+1.077}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V8A1.kits.2\endcsname{\ensuremath{+1.421}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V8A2.amos.0\endcsname{\ensuremath{-0.312}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V8A2.kits.0\endcsname{\ensuremath{+1.353}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V8A2.kits.1\endcsname{\ensuremath{+1.593}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V8A2.kits.2\endcsname{\ensuremath{+2.162}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V8B1.amos.0\endcsname{\ensuremath{-0.751}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V8B1.kits.0\endcsname{\ensuremath{+2.911}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V8B1.kits.1\endcsname{\ensuremath{+2.079}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V8B1.kits.2\endcsname{\ensuremath{+0.670}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V8B2.amos.0\endcsname{\ensuremath{-0.287}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V8B2.kits.0\endcsname{\ensuremath{+1.646}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V8B2.kits.1\endcsname{\ensuremath{+1.892}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.V8B2.kits.2\endcsname{\ensuremath{+1.570}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.W1.amos.0\endcsname{\ensuremath{+0.099}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.W1c.amos.0\endcsname{\ensuremath{+0.363}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.W1c.kits.0\endcsname{\ensuremath{+2.636}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.W1c.kits.1\endcsname{\ensuremath{+1.734}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.W1c.kits.2\endcsname{\ensuremath{+0.399}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.W2.amos.0\endcsname{\ensuremath{+0.211}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.W3.amos.0\endcsname{\ensuremath{+0.270}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.W3c.amos.0\endcsname{\ensuremath{+0.162}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.W4.amos.0\endcsname{\ensuremath{+0.076}}
\expandafter\gdef\csname R@an.cost_accuracy.seeddelta.W5.amos.0\endcsname{\ensuremath{+0.591}}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.C1.kits\endcsname{1.379}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.D1.kits\endcsname{0.565}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.D2.kits\endcsname{0.551}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.L1.amos\endcsname{0.394}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.L1.kits\endcsname{1.491}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.L1b.kits\endcsname{0.821}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.L2.amos\endcsname{0.228}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.L2.kits\endcsname{1.831}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.L3.amos\endcsname{0.397}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.L3.kits\endcsname{1.044}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.L4.amos\endcsname{0.205}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.L4.kits\endcsname{0.862}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.L6.kits\endcsname{1.328}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.P3c.kits\endcsname{0.214}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.S2.kits\endcsname{0.984}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.V5A5.kits\endcsname{0.398}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.V5B1.kits\endcsname{0.166}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.V5B2.kits\endcsname{0.233}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.V6A1r.kits\endcsname{0.541}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.V7A1.kits\endcsname{0.671}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.V7A2.kits\endcsname{0.913}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.V7B1.kits\endcsname{0.989}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.V7B2.kits\endcsname{1.543}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.V7C1.kits\endcsname{0.637}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.V8A1.kits\endcsname{0.683}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.V8A2.kits\endcsname{0.808}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.V8B1.kits\endcsname{2.241}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.V8B2.kits\endcsname{0.321}
\expandafter\gdef\csname R@an.cost_accuracy.seedspread.W1c.kits\endcsname{2.236}
\expandafter\gdef\csname R@an.cost_accuracy.sep.acdc.clause\endcsname{At two fresh seeds, against the frozen 6-run pool (null SD of a two-seed mean delta 0.081 pp), the ACDC fresh means are HyReX at \ensuremath{+0.450} pp (5.58 SD), ResEnc-matched (re-implemented) at \ensuremath{+0.319} pp (3.95 SD), ResEnc-M (library preset) at \ensuremath{+0.242} pp (3.00 SD) and function-identical control at \ensuremath{+0.117} pp (1.45 SD)}
\expandafter\gdef\csname R@an.cost_accuracy.sep.acdc.n\endcsname{4}
\expandafter\gdef\csname R@an.cost_accuracy.sep.acdc.nullsd\endcsname{0.081}
\expandafter\gdef\csname R@an.cost_accuracy.sep.amos.bracket.clause\endcsname{At two fresh seeds AMOS22 separates fresh means of 0.298 pp (ResEnc-matched (re-implemented)) and above and does not separate fresh means of 0.194 pp (ConvNeXt-k3) and below, against the 0.20 pp edge of its two-seed null (1.96 SD of 0.100 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.sep.amos.clause\endcsname{At two fresh seeds, against the frozen 6-run pool (null SD of a two-seed mean delta 0.100 pp), AMOS22 separates ResEnc-M (library preset) at \ensuremath{+0.465} pp (4.66 SD), ResEnc+context at \ensuremath{+0.455} pp (4.56 SD) and ResEnc-matched (re-implemented) at \ensuremath{+0.298} pp (2.98 SD); it does not separate ConvNeXt-k3 at \ensuremath{+0.194} pp (1.95 SD) and HyReX at \ensuremath{+0.132} pp (1.33 SD)}
\expandafter\gdef\csname R@an.cost_accuracy.sep.amos.edge\endcsname{0.20}
\expandafter\gdef\csname R@an.cost_accuracy.sep.amos.largestnot\endcsname{0.194}
\expandafter\gdef\csname R@an.cost_accuracy.sep.amos.largestnot.arm\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.cost_accuracy.sep.amos.n\endcsname{5}
\expandafter\gdef\csname R@an.cost_accuracy.sep.amos.nnot\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.sep.amos.notsep\endcsname{ConvNeXt-k3, HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.sep.amos.nsep\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.sep.amos.nullsd\endcsname{0.100}
\expandafter\gdef\csname R@an.cost_accuracy.sep.amos.sep\endcsname{ResEnc-M (library preset), ResEnc+context, ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.cost_accuracy.sep.amos.smallest\endcsname{0.298}
\expandafter\gdef\csname R@an.cost_accuracy.sep.amos.smallest.arm\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.cost_accuracy.sep.kits.bracket.clause\endcsname{At two fresh seeds KiTS23 separates fresh means of 1.448 pp (LeanAdd with coarse large kernels (LeanAdd-NeXt)) and above and does not separate fresh means of 1.375 pp (LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk)) and below, against the 1.42 pp edge of its two-seed null (1.96 SD of 0.726 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.sep.kits.clause\endcsname{At two fresh seeds, against the frozen 3-run pool (null SD of a two-seed mean delta 0.726 pp), KiTS23 separates ResEnc-M (library preset) at \ensuremath{+3.475} pp (4.79 SD), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid) at \ensuremath{+2.662} pp (3.67 SD), LeanAdd-NeXt with the coarse operator at stage 5 alone at \ensuremath{+2.440} pp (3.36 SD), HyReX + decoder capacity at \ensuremath{+2.401} pp (3.31 SD), LeanAdd-NeXt with separable coarse kernels (LeanSep) at \ensuremath{+2.382} pp (3.28 SD), ResEnc-matched (re-implemented) at \ensuremath{+2.313} pp (3.19 SD), LeanDeepMid with the two finest decoder convolutions restored at \ensuremath{+2.289} pp (3.15 SD), LeanDec with additive skips (LeanAdd) at \ensuremath{+2.285} pp (3.15 SD), ResEnc+context at \ensuremath{+2.246} pp (3.10 SD), HyReX with LeanDec fine decoder stages at \ensuremath{+2.165} pp (2.98 SD), HyReX at \ensuremath{+2.094} pp (2.89 SD), LeanDec (default with one conv per decoder stage) at \ensuremath{+1.892} pp (2.61 SD), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec) at \ensuremath{+1.877} pp (2.59 SD), LeanAdd-NeXt with dilated coarse kernels (LeanDil) at \ensuremath{+1.838} pp (2.53 SD), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1) at \ensuremath{+1.731} pp (2.39 SD), HyReX with 9-kernel coarse stages at \ensuremath{+1.704} pp (2.35 SD), HyReX+context at \ensuremath{+1.591} pp (2.19 SD), HyReX point-fuse decoder at \ensuremath{+1.477} pp (2.03 SD) and LeanAdd with coarse large kernels (LeanAdd-NeXt) at \ensuremath{+1.448} pp (2.00 SD); it does not separate LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk) at \ensuremath{+1.375} pp (1.89 SD), LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack) at \ensuremath{+1.249} pp (1.72 SD), function-identical control at \ensuremath{+1.176} pp (1.62 SD), branch control at \ensuremath{+1.067} pp (1.47 SD), HyReX, ConvNeXt one stage finer at \ensuremath{+0.570} pp (0.79 SD) and ConvNeXt-k3 at \ensuremath{+0.110} pp (0.15 SD)}
\expandafter\gdef\csname R@an.cost_accuracy.sep.kits.edge\endcsname{1.42}
\expandafter\gdef\csname R@an.cost_accuracy.sep.kits.largestnot\endcsname{1.375}
\expandafter\gdef\csname R@an.cost_accuracy.sep.kits.largestnot.arm\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk)}
\expandafter\gdef\csname R@an.cost_accuracy.sep.kits.n\endcsname{25}
\expandafter\gdef\csname R@an.cost_accuracy.sep.kits.nnot\endcsname{6}
\expandafter\gdef\csname R@an.cost_accuracy.sep.kits.notsep\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), function-identical control, branch control, HyReX, ConvNeXt one stage finer, ConvNeXt-k3}
\expandafter\gdef\csname R@an.cost_accuracy.sep.kits.nsep\endcsname{19}
\expandafter\gdef\csname R@an.cost_accuracy.sep.kits.nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.cost_accuracy.sep.kits.sep\endcsname{ResEnc-M (library preset), LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid), LeanAdd-NeXt with the coarse operator at stage 5 alone, HyReX + decoder capacity, LeanAdd-NeXt with separable coarse kernels (LeanSep), ResEnc-matched (re-implemented), LeanDeepMid with the two finest decoder convolutions restored, LeanDec with additive skips (LeanAdd), ResEnc+context, HyReX with LeanDec fine decoder stages, HyReX, LeanDec (default with one conv per decoder stage), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1), HyReX with 9-kernel coarse stages, HyReX+context, HyReX point-fuse decoder, LeanAdd with coarse large kernels (LeanAdd-NeXt)}
\expandafter\gdef\csname R@an.cost_accuracy.sep.kits.smallest\endcsname{1.448}
\expandafter\gdef\csname R@an.cost_accuracy.sep.kits.smallest.arm\endcsname{LeanAdd with coarse large kernels (LeanAdd-NeXt)}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.agent\endcsname{HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.agent.absdown\endcsname{0.166}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.agent.absdown.arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.agent.down\endcsname{HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.agent.n\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.agent.ndown\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.agent.up\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.down\endcsname{HyReX, ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.ndown\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.nup\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.other\endcsname{ResEnc-M (library preset), ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.other.absdown\endcsname{0.094}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.other.absdown.arm\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.other.absup\endcsname{0.036}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.other.absup.arm\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.other.down\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.other.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.other.ndown\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.other.up\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.acdc.up\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.agent\endcsname{HyReX, ConvNeXt-k3, ResEnc+context}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.agent.absdown\endcsname{0.249}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.agent.absdown.arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.agent.absup\endcsname{0.025}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.agent.absup.arm\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.agent.down\endcsname{HyReX, ConvNeXt-k3}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.agent.n\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.agent.ndown\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.agent.up\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.down\endcsname{HyReX, ResEnc-M (library preset), ConvNeXt-k3}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.ndown\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.nup\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.other\endcsname{ResEnc-M (library preset), ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.other.absdown\endcsname{0.182}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.other.absdown.arm\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.other.absup\endcsname{0.160}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.other.absup.arm\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.other.down\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.other.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.other.ndown\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.other.up\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.amos.up\endcsname{ResEnc-matched (re-implemented), ResEnc+context}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.agent\endcsname{HyReX, ConvNeXt-k3, ResEnc+context, HyReX+context}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.agent.absdown\endcsname{0.935}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.agent.absdown.arm\endcsname{HyReX+context}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.agent.absup\endcsname{0.048}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.agent.absup.arm\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.agent.down\endcsname{HyReX, ConvNeXt-k3, HyReX+context}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.agent.n\endcsname{4}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.agent.ndown\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.agent.up\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.down\endcsname{HyReX, ConvNeXt-k3, HyReX+context}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.ndown\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.nup\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.other\endcsname{ResEnc-M (library preset), ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.other.absup\endcsname{1.149}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.other.absup.arm\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.other.down\endcsname{none}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.other.n\endcsname{2}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.other.ndown\endcsname{0}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.other.up\endcsname{ResEnc-M (library preset), ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.cost_accuracy.shiftrole.kits.up\endcsname{ResEnc-M (library preset), ResEnc-matched (re-implemented), ResEnc+context}
\expandafter\gdef\csname R@an.cost_accuracy.step.C1.acdc\endcsname{1.80}
\expandafter\gdef\csname R@an.cost_accuracy.step.C1.amos\endcsname{1.69}
\expandafter\gdef\csname R@an.cost_accuracy.step.C1.kits\endcsname{1.58}
\expandafter\gdef\csname R@an.cost_accuracy.step.D1.acdc\endcsname{1.63}
\expandafter\gdef\csname R@an.cost_accuracy.step.D1.amos\endcsname{1.52}
\expandafter\gdef\csname R@an.cost_accuracy.step.D1.kits\endcsname{1.40}
\expandafter\gdef\csname R@an.cost_accuracy.step.D2.acdc\endcsname{0.81}
\expandafter\gdef\csname R@an.cost_accuracy.step.D2.amos\endcsname{0.81}
\expandafter\gdef\csname R@an.cost_accuracy.step.D2.kits\endcsname{0.81}
\expandafter\gdef\csname R@an.cost_accuracy.step.L1.acdc\endcsname{1.51}
\expandafter\gdef\csname R@an.cost_accuracy.step.L1.amos\endcsname{1.46}
\expandafter\gdef\csname R@an.cost_accuracy.step.L1.kits\endcsname{1.33}
\expandafter\gdef\csname R@an.cost_accuracy.step.L1b.acdc\endcsname{1.41}
\expandafter\gdef\csname R@an.cost_accuracy.step.L1b.amos\endcsname{1.38}
\expandafter\gdef\csname R@an.cost_accuracy.step.L1b.kits\endcsname{1.23}
\expandafter\gdef\csname R@an.cost_accuracy.step.L2.acdc\endcsname{1.50}
\expandafter\gdef\csname R@an.cost_accuracy.step.L2.amos\endcsname{1.46}
\expandafter\gdef\csname R@an.cost_accuracy.step.L2.kits\endcsname{1.33}
\expandafter\gdef\csname R@an.cost_accuracy.step.L3.acdc\endcsname{1.64}
\expandafter\gdef\csname R@an.cost_accuracy.step.L3.amos\endcsname{1.53}
\expandafter\gdef\csname R@an.cost_accuracy.step.L3.kits\endcsname{1.40}
\expandafter\gdef\csname R@an.cost_accuracy.step.L4.acdc\endcsname{1.52}
\expandafter\gdef\csname R@an.cost_accuracy.step.L4.amos\endcsname{1.46}
\expandafter\gdef\csname R@an.cost_accuracy.step.L4.kits\endcsname{1.30}
\expandafter\gdef\csname R@an.cost_accuracy.step.L6.acdc\endcsname{2.03}
\expandafter\gdef\csname R@an.cost_accuracy.step.L6.amos\endcsname{1.88}
\expandafter\gdef\csname R@an.cost_accuracy.step.L6.kits\endcsname{1.63}
\expandafter\gdef\csname R@an.cost_accuracy.step.P3c.acdc\endcsname{1.04}
\expandafter\gdef\csname R@an.cost_accuracy.step.P3c.amos\endcsname{1.05}
\expandafter\gdef\csname R@an.cost_accuracy.step.P3c.kits\endcsname{1.03}
\expandafter\gdef\csname R@an.cost_accuracy.step.S2.acdc\endcsname{2.11}
\expandafter\gdef\csname R@an.cost_accuracy.step.S2.amos\endcsname{1.96}
\expandafter\gdef\csname R@an.cost_accuracy.step.S2.kits\endcsname{1.68}
\expandafter\gdef\csname R@an.cost_accuracy.step.V5A5.acdc\endcsname{1.49}
\expandafter\gdef\csname R@an.cost_accuracy.step.V5A5.amos\endcsname{1.39}
\expandafter\gdef\csname R@an.cost_accuracy.step.V5A5.kits\endcsname{1.24}
\expandafter\gdef\csname R@an.cost_accuracy.step.V5B1.acdc\endcsname{0.72}
\expandafter\gdef\csname R@an.cost_accuracy.step.V5B1.amos\endcsname{0.74}
\expandafter\gdef\csname R@an.cost_accuracy.step.V5B1.kits\endcsname{0.73}
\expandafter\gdef\csname R@an.cost_accuracy.step.V5B2.acdc\endcsname{0.92}
\expandafter\gdef\csname R@an.cost_accuracy.step.V5B2.amos\endcsname{0.85}
\expandafter\gdef\csname R@an.cost_accuracy.step.V5B2.kits\endcsname{0.84}
\expandafter\gdef\csname R@an.cost_accuracy.step.V6A1r.acdc\endcsname{1.81}
\expandafter\gdef\csname R@an.cost_accuracy.step.V6A1r.amos\endcsname{1.63}
\expandafter\gdef\csname R@an.cost_accuracy.step.V6A1r.kits\endcsname{1.49}
\expandafter\gdef\csname R@an.cost_accuracy.step.V7A1.acdc\endcsname{1.07}
\expandafter\gdef\csname R@an.cost_accuracy.step.V7A1.amos\endcsname{1.00}
\expandafter\gdef\csname R@an.cost_accuracy.step.V7A1.kits\endcsname{0.92}
\expandafter\gdef\csname R@an.cost_accuracy.step.V7A2.acdc\endcsname{1.23}
\expandafter\gdef\csname R@an.cost_accuracy.step.V7A2.amos\endcsname{1.15}
\expandafter\gdef\csname R@an.cost_accuracy.step.V7A2.kits\endcsname{1.09}
\expandafter\gdef\csname R@an.cost_accuracy.step.V7B1.acdc\endcsname{0.79}
\expandafter\gdef\csname R@an.cost_accuracy.step.V7B1.amos\endcsname{0.78}
\expandafter\gdef\csname R@an.cost_accuracy.step.V7B1.kits\endcsname{0.77}
\expandafter\gdef\csname R@an.cost_accuracy.step.V7B2.acdc\endcsname{0.76}
\expandafter\gdef\csname R@an.cost_accuracy.step.V7B2.amos\endcsname{0.78}
\expandafter\gdef\csname R@an.cost_accuracy.step.V7B2.kits\endcsname{0.76}
\expandafter\gdef\csname R@an.cost_accuracy.step.V7C1.acdc\endcsname{0.79}
\expandafter\gdef\csname R@an.cost_accuracy.step.V7C1.amos\endcsname{0.78}
\expandafter\gdef\csname R@an.cost_accuracy.step.V7C1.kits\endcsname{0.77}
\expandafter\gdef\csname R@an.cost_accuracy.step.V8A1.acdc\endcsname{1.00}
\expandafter\gdef\csname R@an.cost_accuracy.step.V8A1.amos\endcsname{0.90}
\expandafter\gdef\csname R@an.cost_accuracy.step.V8A1.kits\endcsname{0.91}
\expandafter\gdef\csname R@an.cost_accuracy.step.V8A2.acdc\endcsname{0.92}
\expandafter\gdef\csname R@an.cost_accuracy.step.V8A2.amos\endcsname{0.86}
\expandafter\gdef\csname R@an.cost_accuracy.step.V8A2.kits\endcsname{0.85}
\expandafter\gdef\csname R@an.cost_accuracy.step.V8B1.acdc\endcsname{0.62}
\expandafter\gdef\csname R@an.cost_accuracy.step.V8B1.amos\endcsname{0.62}
\expandafter\gdef\csname R@an.cost_accuracy.step.V8B1.kits\endcsname{0.59}
\expandafter\gdef\csname R@an.cost_accuracy.step.V8B2.acdc\endcsname{0.68}
\expandafter\gdef\csname R@an.cost_accuracy.step.V8B2.amos\endcsname{0.67}
\expandafter\gdef\csname R@an.cost_accuracy.step.V8B2.kits\endcsname{0.63}
\expandafter\gdef\csname R@an.cost_accuracy.step.W1.acdc\endcsname{1.15}
\expandafter\gdef\csname R@an.cost_accuracy.step.W1.amos\endcsname{1.14}
\expandafter\gdef\csname R@an.cost_accuracy.step.W1.kits\endcsname{1.12}
\expandafter\gdef\csname R@an.cost_accuracy.step.W1c.acdc\endcsname{1.15}
\expandafter\gdef\csname R@an.cost_accuracy.step.W1c.amos\endcsname{1.15}
\expandafter\gdef\csname R@an.cost_accuracy.step.W1c.kits\endcsname{1.13}
\expandafter\gdef\csname R@an.cost_accuracy.step.W2.acdc\endcsname{1.16}
\expandafter\gdef\csname R@an.cost_accuracy.step.W2.amos\endcsname{1.15}
\expandafter\gdef\csname R@an.cost_accuracy.step.W2.kits\endcsname{1.13}
\expandafter\gdef\csname R@an.cost_accuracy.step.W3.acdc\endcsname{1.10}
\expandafter\gdef\csname R@an.cost_accuracy.step.W3.amos\endcsname{1.08}
\expandafter\gdef\csname R@an.cost_accuracy.step.W3.kits\endcsname{1.08}
\expandafter\gdef\csname R@an.cost_accuracy.step.W3c.acdc\endcsname{1.09}
\expandafter\gdef\csname R@an.cost_accuracy.step.W3c.amos\endcsname{1.07}
\expandafter\gdef\csname R@an.cost_accuracy.step.W3c.kits\endcsname{1.06}
\expandafter\gdef\csname R@an.cost_accuracy.step.W4.acdc\endcsname{3.84}
\expandafter\gdef\csname R@an.cost_accuracy.step.W4.amos\endcsname{3.51}
\expandafter\gdef\csname R@an.cost_accuracy.step.W4.kits\endcsname{2.62}
\expandafter\gdef\csname R@an.cost_accuracy.step.W5.acdc\endcsname{1.41}
\expandafter\gdef\csname R@an.cost_accuracy.step.W5.amos\endcsname{1.37}
\expandafter\gdef\csname R@an.cost_accuracy.step.W5.kits\endcsname{1.22}
\expandafter\gdef\csname R@an.cost_accuracy.step.cheapest.acdc\endcsname{0.79}
\expandafter\gdef\csname R@an.cost_accuracy.step.cheapest.acdc.arm\endcsname{LeanAdd-NeXt with the coarse operator at stage 5 alone}
\expandafter\gdef\csname R@an.cost_accuracy.step.cheapest.acdc.role\endcsname{agent}
\expandafter\gdef\csname R@an.cost_accuracy.step.cheapest.acdc.wave\endcsname{wave 2}
\expandafter\gdef\csname R@an.cost_accuracy.step.cheapest.acdc.what\endcsname{agent-designed arm}
\expandafter\gdef\csname R@an.cost_accuracy.step.cheapest.amos\endcsname{0.62}
\expandafter\gdef\csname R@an.cost_accuracy.step.cheapest.amos.arm\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk)}
\expandafter\gdef\csname R@an.cost_accuracy.step.cheapest.amos.role\endcsname{agent}
\expandafter\gdef\csname R@an.cost_accuracy.step.cheapest.amos.wave\endcsname{wave 2}
\expandafter\gdef\csname R@an.cost_accuracy.step.cheapest.amos.what\endcsname{agent-designed arm}
\expandafter\gdef\csname R@an.cost_accuracy.step.cheapest.kits\endcsname{0.59}
\expandafter\gdef\csname R@an.cost_accuracy.step.cheapest.kits.arm\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk)}
\expandafter\gdef\csname R@an.cost_accuracy.step.cheapest.kits.role\endcsname{agent}
\expandafter\gdef\csname R@an.cost_accuracy.step.cheapest.kits.wave\endcsname{wave 2}
\expandafter\gdef\csname R@an.cost_accuracy.step.cheapest.kits.what\endcsname{agent-designed arm}
\expandafter\gdef\csname R@an.cost_accuracy.step.w1.acdc.max\endcsname{2.03}
\expandafter\gdef\csname R@an.cost_accuracy.step.w1.acdc.max.arm\endcsname{HyReX+context}
\expandafter\gdef\csname R@an.cost_accuracy.step.w1.acdc.min\endcsname{1.41}
\expandafter\gdef\csname R@an.cost_accuracy.step.w1.acdc.min.arm\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.cost_accuracy.step.w1.acdc.n\endcsname{6}
\expandafter\gdef\csname R@an.cost_accuracy.step.w1.amos.max\endcsname{1.88}
\expandafter\gdef\csname R@an.cost_accuracy.step.w1.amos.max.arm\endcsname{HyReX+context}
\expandafter\gdef\csname R@an.cost_accuracy.step.w1.amos.min\endcsname{1.38}
\expandafter\gdef\csname R@an.cost_accuracy.step.w1.amos.min.arm\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.cost_accuracy.step.w1.amos.n\endcsname{6}
\expandafter\gdef\csname R@an.cost_accuracy.step.w1.kits.max\endcsname{1.63}
\expandafter\gdef\csname R@an.cost_accuracy.step.w1.kits.max.arm\endcsname{HyReX+context}
\expandafter\gdef\csname R@an.cost_accuracy.step.w1.kits.min\endcsname{1.23}
\expandafter\gdef\csname R@an.cost_accuracy.step.w1.kits.min.arm\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.cost_accuracy.step.w1.kits.n\endcsname{6}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.asym.clause\endcsname{on AMOS22 and KiTS23, reported on the fresh-seed mean of seeds 1--2 of both arms, ResEnc-M (library preset) is ahead of HyReX by 0.332 and 1.382 pp; on ACDC, reported on the fresh-seed mean of seeds 1--2 of both arms, HyReX is ahead of ResEnc-M (library preset) by 0.208 pp}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.asym.heroleads\endcsname{ACDC}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.asym.nfresh\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.asym.presetleads\endcsname{AMOS22, KiTS23}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.basis.acdc\endcsname{the fresh-seed mean of seeds 1--2 of both arms, the registered replication estimand}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.basis.amos\endcsname{the fresh-seed mean of seeds 1--2 of both arms, the registered replication estimand}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.basis.kits\endcsname{the fresh-seed mean of seeds 1--2 of both arms, the registered replication estimand}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.C1.amos\endcsname{ResEnc-M (library preset) is 0.257 pp above HyReX + decoder capacity on AMOS22, measured on seed 0, the discovery seed: a margin inside the registered 0.5 pp one-seed pair floor, not separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.C1.kits\endcsname{ResEnc-M (library preset) is 1.074 pp above HyReX + decoder capacity on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 1.35 times the 0.795 pp null SD of a two-seed difference, inside the 1.56 pp (1.96 SD) edge, not separated at two seeds; at the discovery seed HyReX + decoder capacity is ahead by 1.181 pp, above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.D1.amos\endcsname{ResEnc-M (library preset) is 0.369 pp above HyReX point-fuse decoder on AMOS22, measured on seed 0, the discovery seed: a margin inside the registered 0.5 pp one-seed pair floor, not separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.D1.kits\endcsname{ResEnc-M (library preset) is 1.999 pp above HyReX point-fuse decoder on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 2.51 times the 0.795 pp null SD of a two-seed difference, above the 1.56 pp (1.96 SD) edge, separated at two seeds; at the discovery seed ResEnc-M (library preset) is ahead by 0.719 pp, above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.D2.amos\endcsname{ResEnc-M (library preset) is 1.009 pp above LeanDec (default with one conv per decoder stage) on AMOS22, measured on seed 0, the discovery seed: a margin above the registered 0.5 pp one-seed pair floor, separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.D2.kits\endcsname{ResEnc-M (library preset) is 1.584 pp above LeanDec (default with one conv per decoder stage) on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 1.99 times the 0.795 pp null SD of a two-seed difference, above the 1.56 pp (1.96 SD) edge, separated at two seeds; at the discovery seed LeanDec (default with one conv per decoder stage) is ahead by 0.029 pp, below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.L2.acdc\endcsname{ResEnc-M (library preset) is 0.350 pp above ConvNeXt-k3 on ACDC, measured on seed 0, the discovery seed: a margin inside the registered 0.5 pp one-seed pair floor; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.L2.amos\endcsname{ResEnc-M (library preset) is 0.270 pp above ConvNeXt-k3 on AMOS22, measured on the fresh-seed mean (seeds 1--2) of both arms: 2.21 times the 0.122 pp null SD of a two-seed difference, above the 0.24 pp (1.96 SD) edge, separated at two seeds; at the discovery seed ResEnc-M (library preset) is ahead by 0.285 pp, below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.L2.kits\endcsname{ResEnc-M (library preset) is 3.365 pp above ConvNeXt-k3 on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 4.23 times the 0.795 pp null SD of a two-seed difference, above the 1.56 pp (1.96 SD) edge, separated at two seeds; at the discovery seed ResEnc-M (library preset) is ahead by 1.662 pp, above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.L3.acdc\endcsname{HyReX is 0.208 pp above ResEnc-M (library preset) on ACDC, measured on the fresh-seed mean (seeds 1--2) of both arms: 2.11 times the 0.099 pp null SD of a two-seed difference; at the discovery seed HyReX is ahead by 0.281 pp, below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.L3.amos\endcsname{ResEnc-M (library preset) is 0.332 pp above HyReX on AMOS22, measured on the fresh-seed mean (seeds 1--2) of both arms: 2.72 times the 0.122 pp null SD of a two-seed difference, above the 0.24 pp (1.96 SD) edge, separated at two seeds; at the discovery seed ResEnc-M (library preset) is ahead by 0.265 pp, below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.L3.kits\endcsname{ResEnc-M (library preset) is 1.382 pp above HyReX on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 1.74 times the 0.795 pp null SD of a two-seed difference, inside the 1.56 pp (1.96 SD) edge, not separated at two seeds; at the discovery seed HyReX is ahead by 0.516 pp, above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.L4.acdc\endcsname{ResEnc-M (library preset) is 0.020 pp above ResEnc+context on ACDC, measured on seed 0, the discovery seed: a margin inside the registered 0.5 pp one-seed pair floor; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.L4.amos\endcsname{ResEnc-M (library preset) is 0.010 pp above ResEnc+context on AMOS22, measured on the fresh-seed mean (seeds 1--2) of both arms: 0.08 times the 0.122 pp null SD of a two-seed difference, inside the 0.24 pp (1.96 SD) edge, not separated at two seeds; at the discovery seed ResEnc-M (library preset) is ahead by 0.217 pp, below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.L4.kits\endcsname{ResEnc-M (library preset) is 1.229 pp above ResEnc+context on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 1.55 times the 0.795 pp null SD of a two-seed difference, inside the 1.56 pp (1.96 SD) edge, not separated at two seeds; at the discovery seed ResEnc-M (library preset) is ahead by 0.128 pp, below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.L6.acdc\endcsname{HyReX+context is 0.116 pp above ResEnc-M (library preset) on ACDC, measured on seed 0, the discovery seed: a margin inside the registered 0.5 pp one-seed pair floor; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.L6.amos\endcsname{ResEnc-M (library preset) is 0.631 pp above HyReX+context on AMOS22, measured on seed 0, the discovery seed: a margin above the registered 0.5 pp one-seed pair floor, separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.L6.kits\endcsname{ResEnc-M (library preset) is 1.884 pp above HyReX+context on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 2.37 times the 0.795 pp null SD of a two-seed difference, above the 1.56 pp (1.96 SD) edge, separated at two seeds; at the discovery seed HyReX+context is ahead by 0.200 pp, below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.S2.amos\endcsname{ResEnc-M (library preset) is 0.269 pp above HyReX, ConvNeXt one stage finer on AMOS22, measured on seed 0, the discovery seed: a margin inside the registered 0.5 pp one-seed pair floor, not separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.S2.kits\endcsname{ResEnc-M (library preset) is 2.905 pp above HyReX, ConvNeXt one stage finer on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 3.65 times the 0.795 pp null SD of a two-seed difference, above the 1.56 pp (1.96 SD) edge, separated at two seeds; at the discovery seed ResEnc-M (library preset) is ahead by 0.985 pp, above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V5A5.amos\endcsname{ResEnc-M (library preset) is 0.606 pp above HyReX with LeanDec fine decoder stages on AMOS22, measured on seed 0, the discovery seed: a margin above the registered 0.5 pp one-seed pair floor, separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V5A5.kits\endcsname{ResEnc-M (library preset) is 1.310 pp above HyReX with LeanDec fine decoder stages on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 1.65 times the 0.795 pp null SD of a two-seed difference, inside the 1.56 pp (1.96 SD) edge, not separated at two seeds; at the discovery seed ResEnc-M (library preset) is ahead by 0.377 pp, below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V5B1.amos\endcsname{ResEnc-M (library preset) is 0.908 pp above LeanDec with additive skips (LeanAdd) on AMOS22, measured on seed 0, the discovery seed: a margin above the registered 0.5 pp one-seed pair floor, separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V5B1.kits\endcsname{ResEnc-M (library preset) is 1.190 pp above LeanDec with additive skips (LeanAdd) on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 1.50 times the 0.795 pp null SD of a two-seed difference, inside the 1.56 pp (1.96 SD) edge, not separated at two seeds; at the discovery seed ResEnc-M (library preset) is ahead by 0.164 pp, below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V5B2.acdc\endcsname{ResEnc-M (library preset) is 0.517 pp above LeanAdd with coarse large kernels (LeanAdd-NeXt) on ACDC, measured on seed 0, the discovery seed: a margin above the registered 0.5 pp one-seed pair floor; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V5B2.amos\endcsname{ResEnc-M (library preset) is 0.515 pp above LeanAdd with coarse large kernels (LeanAdd-NeXt) on AMOS22, measured on seed 0, the discovery seed: a margin above the registered 0.5 pp one-seed pair floor, separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V5B2.kits\endcsname{ResEnc-M (library preset) is 2.027 pp above LeanAdd with coarse large kernels (LeanAdd-NeXt) on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 2.55 times the 0.795 pp null SD of a two-seed difference, above the 1.56 pp (1.96 SD) edge, separated at two seeds; at the discovery seed ResEnc-M (library preset) is ahead by 1.062 pp, above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V6A1r.acdc\endcsname{HyReX with 9-kernel coarse stages is 0.237 pp above ResEnc-M (library preset) on ACDC, measured on seed 0, the discovery seed: a margin inside the registered 0.5 pp one-seed pair floor; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V6A1r.amos\endcsname{ResEnc-M (library preset) is 0.160 pp above HyReX with 9-kernel coarse stages on AMOS22, measured on seed 0, the discovery seed: a margin inside the registered 0.5 pp one-seed pair floor, not separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V6A1r.kits\endcsname{ResEnc-M (library preset) is 1.771 pp above HyReX with 9-kernel coarse stages on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 2.23 times the 0.795 pp null SD of a two-seed difference, above the 1.56 pp (1.96 SD) edge, separated at two seeds; at the discovery seed ResEnc-M (library preset) is ahead by 0.090 pp, below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V7A1.acdc\endcsname{ResEnc-M (library preset) is 0.107 pp above LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid) on ACDC, measured on seed 0, the discovery seed: a margin inside the registered 0.5 pp one-seed pair floor; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V7A1.amos\endcsname{ResEnc-M (library preset) is 0.691 pp above LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid) on AMOS22, measured on seed 0, the discovery seed: a margin above the registered 0.5 pp one-seed pair floor, separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V7A1.kits\endcsname{ResEnc-M (library preset) is 0.814 pp above LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid) on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 1.02 times the 0.795 pp null SD of a two-seed difference, inside the 1.56 pp (1.96 SD) edge, not separated at two seeds; at the discovery seed LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid) is ahead by 0.222 pp, below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V7A2.acdc\endcsname{LeanDeepMid with the two finest decoder convolutions restored is 0.026 pp above ResEnc-M (library preset) on ACDC, measured on seed 0, the discovery seed: a margin inside the registered 0.5 pp one-seed pair floor; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V7A2.amos\endcsname{ResEnc-M (library preset) is 0.287 pp above LeanDeepMid with the two finest decoder convolutions restored on AMOS22, measured on seed 0, the discovery seed: a margin inside the registered 0.5 pp one-seed pair floor, not separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V7A2.kits\endcsname{ResEnc-M (library preset) is 1.186 pp above LeanDeepMid with the two finest decoder convolutions restored on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 1.49 times the 0.795 pp null SD of a two-seed difference, inside the 1.56 pp (1.96 SD) edge, not separated at two seeds; at the discovery seed LeanDeepMid with the two finest decoder convolutions restored is ahead by 0.560 pp, above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V7B1.amos\endcsname{ResEnc-M (library preset) is 1.082 pp above LeanAdd-NeXt with separable coarse kernels (LeanSep) on AMOS22, measured on seed 0, the discovery seed: a margin above the registered 0.5 pp one-seed pair floor, separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V7B1.kits\endcsname{ResEnc-M (library preset) is 1.094 pp above LeanAdd-NeXt with separable coarse kernels (LeanSep) on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 1.38 times the 0.795 pp null SD of a two-seed difference, inside the 1.56 pp (1.96 SD) edge, not separated at two seeds; at the discovery seed ResEnc-M (library preset) is ahead by 0.605 pp, above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V7B2.amos\endcsname{ResEnc-M (library preset) is 0.913 pp above LeanAdd-NeXt with dilated coarse kernels (LeanDil) on AMOS22, measured on seed 0, the discovery seed: a margin above the registered 0.5 pp one-seed pair floor, separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V7B2.kits\endcsname{ResEnc-M (library preset) is 1.637 pp above LeanAdd-NeXt with dilated coarse kernels (LeanDil) on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 2.06 times the 0.795 pp null SD of a two-seed difference, above the 1.56 pp (1.96 SD) edge, separated at two seeds; at the discovery seed LeanAdd-NeXt with dilated coarse kernels (LeanDil) is ahead by 0.498 pp, below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V7C1.acdc\endcsname{ResEnc-M (library preset) is 0.588 pp above LeanAdd-NeXt with the coarse operator at stage 5 alone on ACDC, measured on seed 0, the discovery seed: a margin above the registered 0.5 pp one-seed pair floor; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V7C1.amos\endcsname{ResEnc-M (library preset) is 0.753 pp above LeanAdd-NeXt with the coarse operator at stage 5 alone on AMOS22, measured on seed 0, the discovery seed: a margin above the registered 0.5 pp one-seed pair floor, separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V7C1.kits\endcsname{ResEnc-M (library preset) is 1.035 pp above LeanAdd-NeXt with the coarse operator at stage 5 alone on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 1.30 times the 0.795 pp null SD of a two-seed difference, inside the 1.56 pp (1.96 SD) edge, not separated at two seeds; at the discovery seed LeanAdd-NeXt with the coarse operator at stage 5 alone is ahead by 0.381 pp, below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V8A1.amos\endcsname{ResEnc-M (library preset) is 1.152 pp above LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack) on AMOS22, measured on seed 0, the discovery seed: a margin above the registered 0.5 pp one-seed pair floor, separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V8A1.kits\endcsname{ResEnc-M (library preset) is 2.226 pp above LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack) on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 2.80 times the 0.795 pp null SD of a two-seed difference, above the 1.56 pp (1.96 SD) edge, separated at two seeds; at the discovery seed ResEnc-M (library preset) is ahead by 0.566 pp, above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V8A2.amos\endcsname{ResEnc-M (library preset) is 0.959 pp above LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec) on AMOS22, measured on seed 0, the discovery seed: a margin above the registered 0.5 pp one-seed pair floor, separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V8A2.kits\endcsname{ResEnc-M (library preset) is 1.598 pp above LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec) on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 2.01 times the 0.795 pp null SD of a two-seed difference, above the 1.56 pp (1.96 SD) edge, separated at two seeds; at the discovery seed ResEnc-M (library preset) is ahead by 0.973 pp, above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V8B1.amos\endcsname{ResEnc-M (library preset) is 1.397 pp above LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk) on AMOS22, measured on seed 0, the discovery seed: a margin above the registered 0.5 pp one-seed pair floor, separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V8B1.kits\endcsname{ResEnc-M (library preset) is 2.101 pp above LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk) on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 2.64 times the 0.795 pp null SD of a two-seed difference, above the 1.56 pp (1.96 SD) edge, separated at two seeds; at the discovery seed LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk) is ahead by 0.585 pp, above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V8B2.amos\endcsname{ResEnc-M (library preset) is 0.934 pp above LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1) on AMOS22, measured on seed 0, the discovery seed: a margin above the registered 0.5 pp one-seed pair floor, separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.V8B2.kits\endcsname{ResEnc-M (library preset) is 1.744 pp above LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1) on KiTS23, measured on the fresh-seed mean (seeds 1--2) of both arms: 2.19 times the 0.795 pp null SD of a two-seed difference, above the 1.56 pp (1.96 SD) edge, separated at two seeds; at the discovery seed ResEnc-M (library preset) is ahead by 0.680 pp, above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.W1.amos\endcsname{ResEnc-M (library preset) is 0.547 pp above $z$-dilation mixing on AMOS22, measured on seed 0, the discovery seed: a margin above the registered 0.5 pp one-seed pair floor, separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.W2.amos\endcsname{ResEnc-M (library preset) is 0.436 pp above thickness-gated mixing on AMOS22, measured on seed 0, the discovery seed: a margin inside the registered 0.5 pp one-seed pair floor, not separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.clause.W3.amos\endcsname{ResEnc-M (library preset) is 0.377 pp above offset upsampling on AMOS22, measured on seed 0, the discovery seed: a margin inside the registered 0.5 pp one-seed pair floor, not separated at one seed each; its registered fresh pair is pending}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.device.acdc\endcsname{no resolution band: the guard dataset is read descriptively}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.device.amos\endcsname{the 0.24 pp edge of this dataset's two-seed null (1.96 SD of 0.122 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.device.kits\endcsname{the 1.56 pp edge of this dataset's two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.C1.amos\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.C1.kits\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.D1.amos\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.D1.kits\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.D2.amos\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.D2.kits\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.L2.acdc\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.L2.amos\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.L2.kits\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.L3.acdc\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.L3.amos\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.L3.kits\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.L4.acdc\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.L4.amos\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.L4.kits\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.L6.acdc\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.L6.amos\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.L6.kits\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.S2.amos\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.S2.kits\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V5A5.amos\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V5A5.kits\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V5B1.amos\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V5B1.kits\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V5B2.acdc\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V5B2.amos\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V5B2.kits\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V6A1r.acdc\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V6A1r.amos\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V6A1r.kits\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V7A1.acdc\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V7A1.amos\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V7A1.kits\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V7A2.acdc\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V7A2.amos\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V7A2.kits\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V7B1.amos\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V7B1.kits\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V7B2.amos\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V7B2.kits\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V7C1.acdc\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V7C1.amos\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V7C1.kits\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V8A1.amos\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V8A1.kits\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V8A2.amos\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V8A2.kits\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V8B1.amos\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V8B1.kits\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V8B2.amos\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.V8B2.kits\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.W1.amos\endcsname{above the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.W2.amos\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.floor.W3.amos\endcsname{below the 0.5 pp one-seed pair floor}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.C1.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.D1.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.D2.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.L2.amos\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.L2.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.L3.acdc\endcsname{HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.L3.amos\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.L3.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.L4.amos\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.L4.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.L6.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.S2.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.V5A5.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.V5B1.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.V5B2.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.V6A1r.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.V7A1.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.V7A2.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.V7B1.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.V7B2.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.V7C1.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.V8A1.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.V8A2.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.V8B1.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshahead.V8B2.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.C1.kits\endcsname{below the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.D1.kits\endcsname{above the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.D2.kits\endcsname{above the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.L2.amos\endcsname{above the 0.24 pp edge of the two-seed null (1.96 SD of 0.122 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.L2.kits\endcsname{above the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.L3.amos\endcsname{above the 0.24 pp edge of the two-seed null (1.96 SD of 0.122 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.L3.kits\endcsname{below the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.L4.amos\endcsname{below the 0.24 pp edge of the two-seed null (1.96 SD of 0.122 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.L4.kits\endcsname{below the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.L6.kits\endcsname{above the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.S2.kits\endcsname{above the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.V5A5.kits\endcsname{below the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.V5B1.kits\endcsname{below the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.V5B2.kits\endcsname{above the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.V6A1r.kits\endcsname{above the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.V7A1.kits\endcsname{below the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.V7A2.kits\endcsname{below the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.V7B1.kits\endcsname{below the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.V7B2.kits\endcsname{above the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.V7C1.kits\endcsname{below the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.V8A1.kits\endcsname{above the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.V8A2.kits\endcsname{above the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.V8B1.kits\endcsname{above the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshfloor.V8B2.kits\endcsname{above the 1.56 pp edge of the two-seed null (1.96 SD of 0.795 pp)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.C1.kits\endcsname{\ensuremath{-1.074}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.D1.kits\endcsname{\ensuremath{-1.999}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.D2.kits\endcsname{\ensuremath{-1.584}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.L2.amos\endcsname{\ensuremath{-0.270}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.L2.kits\endcsname{\ensuremath{-3.365}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.L3.acdc\endcsname{\ensuremath{+0.208}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.L3.amos\endcsname{\ensuremath{-0.332}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.L3.kits\endcsname{\ensuremath{-1.382}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.L4.amos\endcsname{\ensuremath{-0.010}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.L4.kits\endcsname{\ensuremath{-1.229}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.L6.kits\endcsname{\ensuremath{-1.884}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.S2.kits\endcsname{\ensuremath{-2.905}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.V5A5.kits\endcsname{\ensuremath{-1.310}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.V5B1.kits\endcsname{\ensuremath{-1.190}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.V5B2.kits\endcsname{\ensuremath{-2.027}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.V6A1r.kits\endcsname{\ensuremath{-1.771}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.V7A1.kits\endcsname{\ensuremath{-0.814}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.V7A2.kits\endcsname{\ensuremath{-1.186}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.V7B1.kits\endcsname{\ensuremath{-1.094}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.V7B2.kits\endcsname{\ensuremath{-1.637}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.V7C1.kits\endcsname{\ensuremath{-1.035}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.V8A1.kits\endcsname{\ensuremath{-2.226}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.V8A2.kits\endcsname{\ensuremath{-1.598}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.V8B1.kits\endcsname{\ensuremath{-2.101}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgap.V8B2.kits\endcsname{\ensuremath{-1.744}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.C1.kits\endcsname{1.074}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.D1.kits\endcsname{1.999}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.D2.kits\endcsname{1.584}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.L2.amos\endcsname{0.270}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.L2.kits\endcsname{3.365}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.L3.acdc\endcsname{0.208}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.L3.amos\endcsname{0.332}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.L3.kits\endcsname{1.382}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.L4.amos\endcsname{0.010}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.L4.kits\endcsname{1.229}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.L6.kits\endcsname{1.884}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.S2.kits\endcsname{2.905}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.V5A5.kits\endcsname{1.310}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.V5B1.kits\endcsname{1.190}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.V5B2.kits\endcsname{2.027}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.V6A1r.kits\endcsname{1.771}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.V7A1.kits\endcsname{0.814}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.V7A2.kits\endcsname{1.186}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.V7B1.kits\endcsname{1.094}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.V7B2.kits\endcsname{1.637}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.V7C1.kits\endcsname{1.035}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.V8A1.kits\endcsname{2.226}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.V8A2.kits\endcsname{1.598}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.V8B1.kits\endcsname{2.101}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshgapabs.V8B2.kits\endcsname{1.744}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.C1.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.D1.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.D2.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.L2.amos\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.L2.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.L3.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.L3.amos\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.L3.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.L4.amos\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.L4.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.L6.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.S2.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.V5A5.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.V5B1.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.V5B2.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.V6A1r.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.V7A1.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.V7A2.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.V7B1.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.V7B2.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.V7C1.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.V8A1.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.V8A2.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.V8B1.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshreaches.V8B2.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.C1.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.D1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.D2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.L2.amos\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.L2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.L3.amos\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.L3.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.L4.amos\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.L4.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.L6.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.S2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.V5A5.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.V5B1.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.V5B2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.V6A1r.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.V7A1.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.V7A2.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.V7B1.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.V7B2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.V7C1.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.V8A1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.V8A2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.V8B1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshresolved.V8B2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.C1.kits\endcsname{1.35}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.D1.kits\endcsname{2.51}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.D2.kits\endcsname{1.99}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.L2.amos\endcsname{2.21}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.L2.kits\endcsname{4.23}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.L3.acdc\endcsname{2.11}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.L3.amos\endcsname{2.72}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.L3.kits\endcsname{1.74}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.L4.amos\endcsname{0.08}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.L4.kits\endcsname{1.55}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.L6.kits\endcsname{2.37}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.S2.kits\endcsname{3.65}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.V5A5.kits\endcsname{1.65}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.V5B1.kits\endcsname{1.50}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.V5B2.kits\endcsname{2.55}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.V6A1r.kits\endcsname{2.23}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.V7A1.kits\endcsname{1.02}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.V7A2.kits\endcsname{1.49}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.V7B1.kits\endcsname{1.38}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.V7B2.kits\endcsname{2.06}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.V7C1.kits\endcsname{1.30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.V8A1.kits\endcsname{2.80}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.V8A2.kits\endcsname{2.01}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.V8B1.kits\endcsname{2.64}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshse.V8B2.kits\endcsname{2.19}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.C1.kits\endcsname{1.35}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.D1.kits\endcsname{2.51}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.D2.kits\endcsname{1.99}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.L2.amos\endcsname{2.21}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.L2.kits\endcsname{4.23}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.L3.acdc\endcsname{2.11}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.L3.amos\endcsname{2.72}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.L3.kits\endcsname{1.74}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.L4.amos\endcsname{0.08}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.L4.kits\endcsname{1.55}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.L6.kits\endcsname{2.37}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.S2.kits\endcsname{3.65}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.V5A5.kits\endcsname{1.65}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.V5B1.kits\endcsname{1.50}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.V5B2.kits\endcsname{2.55}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.V6A1r.kits\endcsname{2.23}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.V7A1.kits\endcsname{1.02}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.V7A2.kits\endcsname{1.49}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.V7B1.kits\endcsname{1.38}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.V7B2.kits\endcsname{2.06}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.V7C1.kits\endcsname{1.30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.V8A1.kits\endcsname{2.80}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.V8A2.kits\endcsname{2.01}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.V8B1.kits\endcsname{2.64}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.freshsemult.V8B2.kits\endcsname{2.19}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.C1.amos\endcsname{\ensuremath{-0.257}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.C1.kits\endcsname{\ensuremath{+1.181}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.D1.amos\endcsname{\ensuremath{-0.369}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.D1.kits\endcsname{\ensuremath{-0.719}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.D2.amos\endcsname{\ensuremath{-1.009}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.D2.kits\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.L2.acdc\endcsname{\ensuremath{-0.350}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.L2.amos\endcsname{\ensuremath{-0.285}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.L2.kits\endcsname{\ensuremath{-1.662}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.L3.acdc\endcsname{\ensuremath{+0.281}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.L3.amos\endcsname{\ensuremath{-0.265}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.L3.kits\endcsname{\ensuremath{+0.516}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.L4.acdc\endcsname{\ensuremath{-0.020}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.L4.amos\endcsname{\ensuremath{-0.217}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.L4.kits\endcsname{\ensuremath{-0.128}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.L6.acdc\endcsname{\ensuremath{+0.116}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.L6.amos\endcsname{\ensuremath{-0.631}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.L6.kits\endcsname{\ensuremath{+0.200}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.S2.amos\endcsname{\ensuremath{-0.269}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.S2.kits\endcsname{\ensuremath{-0.985}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V5A5.amos\endcsname{\ensuremath{-0.606}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V5A5.kits\endcsname{\ensuremath{-0.377}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V5B1.amos\endcsname{\ensuremath{-0.908}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V5B1.kits\endcsname{\ensuremath{-0.164}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V5B2.acdc\endcsname{\ensuremath{-0.517}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V5B2.amos\endcsname{\ensuremath{-0.515}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V5B2.kits\endcsname{\ensuremath{-1.062}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V6A1r.acdc\endcsname{\ensuremath{+0.237}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V6A1r.amos\endcsname{\ensuremath{-0.160}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V6A1r.kits\endcsname{\ensuremath{-0.090}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V7A1.acdc\endcsname{\ensuremath{-0.107}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V7A1.amos\endcsname{\ensuremath{-0.691}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V7A1.kits\endcsname{\ensuremath{+0.222}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V7A2.acdc\endcsname{\ensuremath{+0.026}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V7A2.amos\endcsname{\ensuremath{-0.287}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V7A2.kits\endcsname{\ensuremath{+0.560}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V7B1.amos\endcsname{\ensuremath{-1.082}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V7B1.kits\endcsname{\ensuremath{-0.605}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V7B2.amos\endcsname{\ensuremath{-0.913}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V7B2.kits\endcsname{\ensuremath{+0.498}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V7C1.acdc\endcsname{\ensuremath{-0.588}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V7C1.amos\endcsname{\ensuremath{-0.753}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V7C1.kits\endcsname{\ensuremath{+0.381}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V8A1.amos\endcsname{\ensuremath{-1.152}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V8A1.kits\endcsname{\ensuremath{-0.566}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V8A2.amos\endcsname{\ensuremath{-0.959}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V8A2.kits\endcsname{\ensuremath{-0.973}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V8B1.amos\endcsname{\ensuremath{-1.397}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V8B1.kits\endcsname{\ensuremath{+0.585}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V8B2.amos\endcsname{\ensuremath{-0.934}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.V8B2.kits\endcsname{\ensuremath{-0.680}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.W1.amos\endcsname{\ensuremath{-0.547}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.W2.amos\endcsname{\ensuremath{-0.436}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gap.W3.amos\endcsname{\ensuremath{-0.377}}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.C1.amos\endcsname{0.257}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.C1.kits\endcsname{1.181}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.D1.amos\endcsname{0.369}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.D1.kits\endcsname{0.719}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.D2.amos\endcsname{1.009}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.D2.kits\endcsname{0.029}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.L2.acdc\endcsname{0.350}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.L2.amos\endcsname{0.285}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.L2.kits\endcsname{1.662}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.L3.acdc\endcsname{0.281}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.L3.amos\endcsname{0.265}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.L3.kits\endcsname{0.516}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.L4.acdc\endcsname{0.020}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.L4.amos\endcsname{0.217}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.L4.kits\endcsname{0.128}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.L6.acdc\endcsname{0.116}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.L6.amos\endcsname{0.631}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.L6.kits\endcsname{0.200}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.S2.amos\endcsname{0.269}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.S2.kits\endcsname{0.985}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V5A5.amos\endcsname{0.606}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V5A5.kits\endcsname{0.377}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V5B1.amos\endcsname{0.908}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V5B1.kits\endcsname{0.164}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V5B2.acdc\endcsname{0.517}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V5B2.amos\endcsname{0.515}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V5B2.kits\endcsname{1.062}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V6A1r.acdc\endcsname{0.237}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V6A1r.amos\endcsname{0.160}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V6A1r.kits\endcsname{0.090}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V7A1.acdc\endcsname{0.107}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V7A1.amos\endcsname{0.691}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V7A1.kits\endcsname{0.222}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V7A2.acdc\endcsname{0.026}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V7A2.amos\endcsname{0.287}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V7A2.kits\endcsname{0.560}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V7B1.amos\endcsname{1.082}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V7B1.kits\endcsname{0.605}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V7B2.amos\endcsname{0.913}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V7B2.kits\endcsname{0.498}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V7C1.acdc\endcsname{0.588}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V7C1.amos\endcsname{0.753}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V7C1.kits\endcsname{0.381}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V8A1.amos\endcsname{1.152}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V8A1.kits\endcsname{0.566}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V8A2.amos\endcsname{0.959}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V8A2.kits\endcsname{0.973}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V8B1.amos\endcsname{1.397}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V8B1.kits\endcsname{0.585}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V8B2.amos\endcsname{0.934}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.V8B2.kits\endcsname{0.680}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.W1.amos\endcsname{0.547}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.W2.amos\endcsname{0.436}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.gapabs.W3.amos\endcsname{0.377}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.lead.acdc\endcsname{HyReX}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.lead.amos\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.lead.kits\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.leadgap.acdc\endcsname{0.208}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.leadgap.amos\endcsname{0.332}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.leadgap.kits\endcsname{1.382}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.nfreshgap.acdc\endcsname{1}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.nfreshgap.amos\endcsname{3}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.nfreshgap.kits\endcsname{21}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.C1.amos\endcsname{0.51}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.C1.kits\endcsname{0.51}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.D1.amos\endcsname{0.20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.D1.kits\endcsname{0.20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.D2.amos\endcsname{0.25}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.D2.kits\endcsname{0.25}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.L2.acdc\endcsname{0.23}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.L2.amos\endcsname{0.24}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.L2.kits\endcsname{0.24}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.L3.acdc\endcsname{0.28}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.L3.amos\endcsname{0.29}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.L3.kits\endcsname{0.29}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.L4.acdc\endcsname{1.00}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.L4.amos\endcsname{1.00}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.L4.kits\endcsname{1.00}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.L6.acdc\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.L6.amos\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.L6.kits\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.S2.amos\endcsname{0.27}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.S2.kits\endcsname{0.27}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V5A5.amos\endcsname{0.29}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V5A5.kits\endcsname{0.29}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V5B1.amos\endcsname{0.20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V5B1.kits\endcsname{0.20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V5B2.acdc\endcsname{0.20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V5B2.amos\endcsname{0.21}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V5B2.kits\endcsname{0.21}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V6A1r.acdc\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V6A1r.amos\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V6A1r.kits\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V7A1.acdc\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V7A1.amos\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V7A1.kits\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V7A2.acdc\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V7A2.amos\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V7A2.kits\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V7B1.amos\endcsname{0.20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V7B1.kits\endcsname{0.20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V7B2.amos\endcsname{0.20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V7B2.kits\endcsname{0.20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V7C1.acdc\endcsname{0.20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V7C1.amos\endcsname{0.21}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V7C1.kits\endcsname{0.21}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V8A1.amos\endcsname{0.31}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V8A1.kits\endcsname{0.31}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V8A2.amos\endcsname{0.31}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V8A2.kits\endcsname{0.31}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V8B1.amos\endcsname{0.18}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V8B1.kits\endcsname{0.18}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V8B2.amos\endcsname{0.21}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.V8B2.kits\endcsname{0.21}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.W1.amos\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.W2.amos\endcsname{0.30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.par.W3.amos\endcsname{0.29}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.C1.amos\endcsname{2.0}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.C1.kits\endcsname{2.0}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.D1.amos\endcsname{4.9}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.D1.kits\endcsname{4.9}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.D2.amos\endcsname{3.9}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.D2.kits\endcsname{3.9}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.L2.acdc\endcsname{4.3}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.L2.amos\endcsname{4.2}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.L2.kits\endcsname{4.2}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.L3.acdc\endcsname{3.5}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.L3.amos\endcsname{3.5}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.L3.kits\endcsname{3.5}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.L4.acdc\endcsname{1.0}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.L4.amos\endcsname{1.0}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.L4.kits\endcsname{1.0}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.L6.acdc\endcsname{3.3}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.L6.amos\endcsname{3.3}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.L6.kits\endcsname{3.3}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.S2.amos\endcsname{3.7}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.S2.kits\endcsname{3.7}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V5A5.amos\endcsname{3.5}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V5A5.kits\endcsname{3.5}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V5B1.amos\endcsname{4.9}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V5B1.kits\endcsname{4.9}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V5B2.acdc\endcsname{5.0}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V5B2.amos\endcsname{4.8}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V5B2.kits\endcsname{4.8}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V6A1r.acdc\endcsname{3.4}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V6A1r.amos\endcsname{3.3}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V6A1r.kits\endcsname{3.3}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V7A1.acdc\endcsname{3.4}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V7A1.amos\endcsname{3.3}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V7A1.kits\endcsname{3.3}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V7A2.acdc\endcsname{3.3}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V7A2.amos\endcsname{3.3}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V7A2.kits\endcsname{3.3}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V7B1.amos\endcsname{5.0}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V7B1.kits\endcsname{5.0}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V7B2.amos\endcsname{5.0}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V7B2.kits\endcsname{5.0}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V7C1.acdc\endcsname{5.0}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V7C1.amos\endcsname{4.9}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V7C1.kits\endcsname{4.8}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V8A1.amos\endcsname{3.3}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V8A1.kits\endcsname{3.3}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V8A2.amos\endcsname{3.3}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V8A2.kits\endcsname{3.3}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V8B1.amos\endcsname{5.6}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V8B1.kits\endcsname{5.6}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V8B2.amos\endcsname{4.9}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.V8B2.kits\endcsname{4.9}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.W1.amos\endcsname{3.3}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.W2.amos\endcsname{3.3}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parfold.W3.amos\endcsname{3.5}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.C1.amos\endcsname{51}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.C1.kits\endcsname{51}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.D1.amos\endcsname{20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.D1.kits\endcsname{20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.D2.amos\endcsname{25}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.D2.kits\endcsname{25}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.L2.acdc\endcsname{23}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.L2.amos\endcsname{24}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.L2.kits\endcsname{24}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.L3.acdc\endcsname{28}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.L3.amos\endcsname{29}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.L3.kits\endcsname{29}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.L4.acdc\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.L4.amos\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.L4.kits\endcsname{100}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.L6.acdc\endcsname{30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.L6.amos\endcsname{30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.L6.kits\endcsname{30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.S2.amos\endcsname{27}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.S2.kits\endcsname{27}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V5A5.amos\endcsname{29}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V5A5.kits\endcsname{29}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V5B1.amos\endcsname{20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V5B1.kits\endcsname{20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V5B2.acdc\endcsname{20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V5B2.amos\endcsname{21}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V5B2.kits\endcsname{21}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V6A1r.acdc\endcsname{30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V6A1r.amos\endcsname{30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V6A1r.kits\endcsname{30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V7A1.acdc\endcsname{30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V7A1.amos\endcsname{30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V7A1.kits\endcsname{30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V7A2.acdc\endcsname{30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V7A2.amos\endcsname{30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V7A2.kits\endcsname{30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V7B1.amos\endcsname{20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V7B1.kits\endcsname{20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V7B2.amos\endcsname{20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V7B2.kits\endcsname{20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V7C1.acdc\endcsname{20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V7C1.amos\endcsname{21}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V7C1.kits\endcsname{21}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V8A1.amos\endcsname{31}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V8A1.kits\endcsname{31}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V8A2.amos\endcsname{31}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V8A2.kits\endcsname{31}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V8B1.amos\endcsname{18}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V8B1.kits\endcsname{18}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V8B2.amos\endcsname{21}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.V8B2.kits\endcsname{21}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.W1.amos\endcsname{30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.W2.amos\endcsname{30}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.parpct.W3.amos\endcsname{29}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.C1.amos\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.C1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.D1.amos\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.D1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.D2.amos\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.D2.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.L2.acdc\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.L2.amos\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.L2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.L3.acdc\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.L3.amos\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.L3.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.L4.acdc\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.L4.amos\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.L4.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.L6.acdc\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.L6.amos\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.L6.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.S2.amos\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.S2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V5A5.amos\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V5A5.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V5B1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V5B1.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V5B2.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V5B2.amos\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V5B2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V6A1r.acdc\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V6A1r.amos\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V6A1r.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V7A1.acdc\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V7A1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V7A1.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V7A2.acdc\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V7A2.amos\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V7A2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V7B1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V7B1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V7B2.amos\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V7B2.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V7C1.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V7C1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V7C1.kits\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V8A1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V8A1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V8A2.amos\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V8A2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V8B1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V8B1.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V8B2.amos\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.V8B2.kits\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.W1.amos\endcsname{yes}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.W2.amos\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.resolved.W3.amos\endcsname{no}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.C1.amos\endcsname{1.49}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.C1.kits\endcsname{1.05}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.D1.amos\endcsname{2.13}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.D1.kits\endcsname{0.64}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.D2.amos\endcsname{5.84}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.D2.kits\endcsname{0.03}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.L2.acdc\endcsname{2.51}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.L2.amos\endcsname{1.65}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.L2.kits\endcsname{1.48}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.L3.acdc\endcsname{2.01}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.L3.amos\endcsname{1.53}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.L3.kits\endcsname{0.46}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.L4.acdc\endcsname{0.15}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.L4.amos\endcsname{1.26}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.L4.kits\endcsname{0.11}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.L6.acdc\endcsname{0.83}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.L6.amos\endcsname{3.65}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.L6.kits\endcsname{0.18}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.S2.amos\endcsname{1.56}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.S2.kits\endcsname{0.88}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V5A5.amos\endcsname{3.51}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V5A5.kits\endcsname{0.34}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V5B1.amos\endcsname{5.25}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V5B1.kits\endcsname{0.15}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V5B2.acdc\endcsname{3.70}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V5B2.amos\endcsname{2.98}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V5B2.kits\endcsname{0.94}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V6A1r.acdc\endcsname{1.70}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V6A1r.amos\endcsname{0.93}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V6A1r.kits\endcsname{0.08}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V7A1.acdc\endcsname{0.76}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V7A1.amos\endcsname{4.00}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V7A1.kits\endcsname{0.20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V7A2.acdc\endcsname{0.19}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V7A2.amos\endcsname{1.66}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V7A2.kits\endcsname{0.50}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V7B1.amos\endcsname{6.26}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V7B1.kits\endcsname{0.54}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V7B2.amos\endcsname{5.28}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V7B2.kits\endcsname{0.44}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V7C1.acdc\endcsname{4.21}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V7C1.amos\endcsname{4.35}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V7C1.kits\endcsname{0.34}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V8A1.amos\endcsname{6.66}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V8A1.kits\endcsname{0.50}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V8A2.amos\endcsname{5.55}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V8A2.kits\endcsname{0.87}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V8B1.amos\endcsname{8.08}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V8B1.kits\endcsname{0.52}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V8B2.amos\endcsname{5.40}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.V8B2.kits\endcsname{0.61}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.W1.amos\endcsname{3.17}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.W2.amos\endcsname{2.52}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.se.W3.amos\endcsname{2.18}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.C1.amos\endcsname{1.49}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.C1.kits\endcsname{1.05}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.D1.amos\endcsname{2.13}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.D1.kits\endcsname{0.64}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.D2.amos\endcsname{5.84}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.D2.kits\endcsname{0.03}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.L2.acdc\endcsname{2.51}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.L2.amos\endcsname{1.65}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.L2.kits\endcsname{1.48}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.L3.acdc\endcsname{2.01}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.L3.amos\endcsname{1.53}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.L3.kits\endcsname{0.46}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.L4.acdc\endcsname{0.15}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.L4.amos\endcsname{1.26}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.L4.kits\endcsname{0.11}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.L6.acdc\endcsname{0.83}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.L6.amos\endcsname{3.65}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.L6.kits\endcsname{0.18}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.S2.amos\endcsname{1.56}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.S2.kits\endcsname{0.88}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V5A5.amos\endcsname{3.51}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V5A5.kits\endcsname{0.34}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V5B1.amos\endcsname{5.25}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V5B1.kits\endcsname{0.15}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V5B2.acdc\endcsname{3.70}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V5B2.amos\endcsname{2.98}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V5B2.kits\endcsname{0.94}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V6A1r.acdc\endcsname{1.70}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V6A1r.amos\endcsname{0.93}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V6A1r.kits\endcsname{0.08}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V7A1.acdc\endcsname{0.76}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V7A1.amos\endcsname{4.00}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V7A1.kits\endcsname{0.20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V7A2.acdc\endcsname{0.19}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V7A2.amos\endcsname{1.66}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V7A2.kits\endcsname{0.50}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V7B1.amos\endcsname{6.26}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V7B1.kits\endcsname{0.54}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V7B2.amos\endcsname{5.28}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V7B2.kits\endcsname{0.44}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V7C1.acdc\endcsname{4.21}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V7C1.amos\endcsname{4.35}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V7C1.kits\endcsname{0.34}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V8A1.amos\endcsname{6.66}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V8A1.kits\endcsname{0.50}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V8A2.amos\endcsname{5.55}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V8A2.kits\endcsname{0.87}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V8B1.amos\endcsname{8.08}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V8B1.kits\endcsname{0.52}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V8B2.amos\endcsname{5.40}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.V8B2.kits\endcsname{0.61}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.W1.amos\endcsname{3.17}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.W2.amos\endcsname{2.52}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.semult.W3.amos\endcsname{2.18}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.C1.amos\endcsname{1.16}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.C1.kits\endcsname{1.18}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.D1.amos\endcsname{1.04}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.D1.kits\endcsname{1.05}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.D2.amos\endcsname{0.56}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.D2.kits\endcsname{0.61}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.L2.acdc\endcsname{1.00}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.L2.amos\endcsname{1.00}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.L2.kits\endcsname{1.00}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.L3.acdc\endcsname{1.09}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.L3.amos\endcsname{1.04}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.L3.kits\endcsname{1.05}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.L4.acdc\endcsname{1.01}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.L4.amos\endcsname{1.00}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.L4.kits\endcsname{0.97}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.L6.acdc\endcsname{1.35}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.L6.amos\endcsname{1.28}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.L6.kits\endcsname{1.22}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.S2.amos\endcsname{1.34}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.S2.kits\endcsname{1.26}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V5A5.amos\endcsname{0.95}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V5A5.kits\endcsname{0.93}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V5B1.amos\endcsname{0.51}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V5B1.kits\endcsname{0.54}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V5B2.acdc\endcsname{0.61}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V5B2.amos\endcsname{0.58}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V5B2.kits\endcsname{0.63}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V6A1r.acdc\endcsname{1.20}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V6A1r.amos\endcsname{1.11}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V6A1r.kits\endcsname{1.12}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V7A1.acdc\endcsname{0.71}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V7A1.amos\endcsname{0.68}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V7A1.kits\endcsname{0.69}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V7A2.acdc\endcsname{0.81}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V7A2.amos\endcsname{0.78}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V7A2.kits\endcsname{0.82}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V7B1.amos\endcsname{0.53}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V7B1.kits\endcsname{0.58}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V7B2.amos\endcsname{0.53}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V7B2.kits\endcsname{0.57}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V7C1.acdc\endcsname{0.52}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V7C1.amos\endcsname{0.53}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V7C1.kits\endcsname{0.58}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V8A1.amos\endcsname{0.61}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V8A1.kits\endcsname{0.68}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V8A2.amos\endcsname{0.59}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V8A2.kits\endcsname{0.64}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V8B1.amos\endcsname{0.42}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V8B1.kits\endcsname{0.44}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V8B2.amos\endcsname{0.46}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.V8B2.kits\endcsname{0.47}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.W1.amos\endcsname{0.78}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.W2.amos\endcsname{0.79}
\expandafter\gdef\csname R@an.cost_accuracy.vsL1.step.W3.amos\endcsname{0.74}
\expandafter\gdef\csname R@an.cost_accuracy.wall.C1.kits\endcsname{1.56}
\expandafter\gdef\csname R@an.cost_accuracy.wall.D1.kits\endcsname{1.39}
\expandafter\gdef\csname R@an.cost_accuracy.wall.D2.kits\endcsname{0.83}
\expandafter\gdef\csname R@an.cost_accuracy.wall.L1.kits\endcsname{1.32}
\expandafter\gdef\csname R@an.cost_accuracy.wall.L1b.kits\endcsname{1.22}
\expandafter\gdef\csname R@an.cost_accuracy.wall.L2.kits\endcsname{1.31}
\expandafter\gdef\csname R@an.cost_accuracy.wall.L3.kits\endcsname{1.39}
\expandafter\gdef\csname R@an.cost_accuracy.wall.L4.kits\endcsname{1.29}
\expandafter\gdef\csname R@an.cost_accuracy.wall.L6.kits\endcsname{1.63}
\expandafter\gdef\csname R@an.cost_accuracy.wall.P3c.kits\endcsname{1.03}
\expandafter\gdef\csname R@an.cost_accuracy.wall.S2.kits\endcsname{1.66}
\expandafter\gdef\csname R@an.cost_accuracy.wall.V5A5.kits\endcsname{1.22}
\expandafter\gdef\csname R@an.cost_accuracy.wall.V5B1.kits\endcsname{0.93}
\expandafter\gdef\csname R@an.cost_accuracy.wall.V5B2.kits\endcsname{0.83}
\expandafter\gdef\csname R@an.cost_accuracy.wall.V6A1r.kits\endcsname{1.49}
\expandafter\gdef\csname R@an.cost_accuracy.wall.V7A1.kits\endcsname{0.96}
\expandafter\gdef\csname R@an.cost_accuracy.wall.V7A2.kits\endcsname{1.16}
\expandafter\gdef\csname R@an.cost_accuracy.wall.V7B1.kits\endcsname{0.99}
\expandafter\gdef\csname R@an.cost_accuracy.wall.V7B2.kits\endcsname{0.99}
\expandafter\gdef\csname R@an.cost_accuracy.wall.V7C1.kits\endcsname{1.00}
\expandafter\gdef\csname R@an.cost_accuracy.wall.V8A1.kits\endcsname{0.99}
\expandafter\gdef\csname R@an.cost_accuracy.wall.V8A2.kits\endcsname{0.90}
\expandafter\gdef\csname R@an.cost_accuracy.wall.V8B1.kits\endcsname{0.95}
\expandafter\gdef\csname R@an.cost_accuracy.wall.V8B2.kits\endcsname{0.90}
\expandafter\gdef\csname R@an.cost_accuracy.wall.W1c.kits\endcsname{1.10}
\expandafter\gdef\csname R@an.cost_accuracy.wallprof.bound\endcsname{61.7}
\expandafter\gdef\csname R@an.cost_accuracy.wallprof.bound.core\endcsname{4.2}
\expandafter\gdef\csname R@an.cost_accuracy.wallprof.max\endcsname{1.62}
\expandafter\gdef\csname R@an.cost_accuracy.wallprof.maxdev\endcsname{61.68}
\expandafter\gdef\csname R@an.cost_accuracy.wallprof.maxdev.core\endcsname{4.17}
\expandafter\gdef\csname R@an.cost_accuracy.wallprof.min\endcsname{0.97}
\expandafter\gdef\csname R@an.cost_accuracy.wallprof.n\endcsname{25}
\expandafter\gdef\csname R@an.cost_accuracy.wallprof.n.core\endcsname{16}
\expandafter\gdef\csname R@an.cost_accuracy.wallprof.outliers\endcsname{LeanDec with additive skips (LeanAdd), LeanDeepMid with the two finest decoder convolutions restored, LeanAdd-NeXt with separable coarse kernels (LeanSep), LeanAdd-NeXt with dilated coarse kernels (LeanDil), LeanAdd-NeXt with the coarse operator at stage 5 alone, LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack), LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec), LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk), LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1)}
\expandafter\gdef\csname R@an.cost_accuracy.wallprof.outliers.n\endcsname{9}
\expandafter\gdef\csname R@an.cost_accuracy.wallprof.sentence\endcsname{the measured wall-clock ratio of each of the 25 arms with a run and a profile reproduces its profiled ratio within 4.2\,\% for 16 of them (largest deviation 4.17\,\%); LeanDec with additive skips (LeanAdd) trained at 0.93$\times$ the stock default's wall-clock against a profiled 0.73$\times$; LeanDeepMid with the two finest decoder convolutions restored trained at 1.16$\times$ the stock default's wall-clock against a profiled 1.09$\times$; LeanAdd-NeXt with separable coarse kernels (LeanSep) trained at 0.99$\times$ the stock default's wall-clock against a profiled 0.77$\times$; LeanAdd-NeXt with dilated coarse kernels (LeanDil) trained at 0.99$\times$ the stock default's wall-clock against a profiled 0.76$\times$; LeanAdd-NeXt with the coarse operator at stage 5 alone trained at 1.00$\times$ the stock default's wall-clock against a profiled 0.77$\times$; LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack) trained at 0.99$\times$ the stock default's wall-clock against a profiled 0.91$\times$; LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec) trained at 0.90$\times$ the stock default's wall-clock against a profiled 0.85$\times$; LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk) trained at 0.95$\times$ the stock default's wall-clock against a profiled 0.59$\times$; LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1) trained at 0.90$\times$ the stock default's wall-clock against a profiled 0.63$\times$ (one run each: the cause is not established)}
\expandafter\gdef\csname R@an.cost_accuracy.wallprof.tol\endcsname{5}
\expandafter\gdef\csname R@an.counts.built\endcsname{51}
\expandafter\gdef\csname R@an.counts.built.def\endcsname{design source files built for waves 1 to 8, one per candidate file}
\expandafter\gdef\csname R@an.counts.built.outside\endcsname{9}
\expandafter\gdef\csname R@an.counts.built.outside.def\endcsname{built designs without a row in the verdict table; built minus registered}
\expandafter\gdef\csname R@an.counts.designs\endcsname{28}
\expandafter\gdef\csname R@an.counts.designs.agent\endcsname{25}
\expandafter\gdef\csname R@an.counts.designs.agent.def\endcsname{designs that are agent-designed arms; a subset of designs}
\expandafter\gdef\csname R@an.counts.designs.def\endcsname{trained arms whose discovery screen ran as a design of the search loop; a subset of trained (the other 10 trained arms are controls, reference designs and attribution arms that judge them)}
\expandafter\gdef\csname R@an.counts.gpudays.alloc\endcsname{140}
\expandafter\gdef\csname R@an.counts.gpudays.alloc.def\endcsname{GPU-days of those runs as allocated (queue duration times the 2 GPUs a run holds)}
\expandafter\gdef\csname R@an.counts.gpudays.eff\endcsname{49}
\expandafter\gdef\csname R@an.counts.gpudays.eff.def\endcsname{GPU-days used as a percentage of those allocated}
\expandafter\gdef\csname R@an.counts.gpudays.used\endcsname{68}
\expandafter\gdef\csname R@an.counts.gpudays.used.def\endcsname{GPU-days of those runs on the one device the network trains on (training seconds); 49 percent of the allocated}
\expandafter\gdef\csname R@an.counts.gpus\endcsname{2}
\expandafter\gdef\csname R@an.counts.gpus.def\endcsname{the GPUs one run of the search holds in the queue}
\expandafter\gdef\csname R@an.counts.hierarchy\endcsname{the loop proposed 111 ideas and built 51 designs; 42 of the built designs are rows of the verdict table (the lineage), 38 of those were trained at full budget, 28 as designs of the search and 10 as controls, reference designs and attribution arms that judge them; 25 of the trained arms were replicated on fresh seeds; the 28 designs took 138 full-budget runs, 140 GPU-days as allocated and 68 on the training device}
\expandafter\gdef\csname R@an.counts.ideas\endcsname{111}
\expandafter\gdef\csname R@an.counts.ideas.def\endcsname{ideas named by an ideator agent or a wave brief (the ledger of waves 1 to 4 and the ideator documents of waves 5 to 8); not a superset of the rows below, since controls are built without an idea (44 ideas were funded as a design)}
\expandafter\gdef\csname R@an.counts.ideas.funded\endcsname{44}
\expandafter\gdef\csname R@an.counts.ideas.funded.def\endcsname{ideas funded as a design of the loop; a subset of ideas}
\expandafter\gdef\csname R@an.counts.judges\endcsname{10}
\expandafter\gdef\csname R@an.counts.judges.def\endcsname{trained arms that are not designs; trained minus designs}
\expandafter\gdef\csname R@an.counts.registered\endcsname{42}
\expandafter\gdef\csname R@an.counts.registered.def\endcsname{built designs with a row in the verdict table, the nodes of the lineage; a subset of built (the 9 built designs outside the table were profiled and never run as arms)}
\expandafter\gdef\csname R@an.counts.replicated\endcsname{25}
\expandafter\gdef\csname R@an.counts.replicated.def\endcsname{trained arms with a finished fresh-seed pair (seeds 1 and 2) on some dataset, controls included; a subset of trained (21 of them are designs)}
\expandafter\gdef\csname R@an.counts.replicated.designs\endcsname{21}
\expandafter\gdef\csname R@an.counts.replicated.designs.def\endcsname{replicated arms that are designs; a subset of replicated and of designs}
\expandafter\gdef\csname R@an.counts.reviewed\endcsname{38}
\expandafter\gdef\csname R@an.counts.reviewed.def\endcsname{ideas of the waves with a per-idea review record that carry a recorded verdict; a subset of ideas}
\expandafter\gdef\csname R@an.counts.runs\endcsname{138}
\expandafter\gdef\csname R@an.counts.runs.def\endcsname{finished full-budget runs of the designs (53 discovery screens, 11 ACDC guard runs, 74 fresh-seed replications); controls, baselines, cross-validation and held-out runs are not counted}
\expandafter\gdef\csname R@an.counts.runs.fresh\endcsname{74}
\expandafter\gdef\csname R@an.counts.runs.fresh.def\endcsname{finished fresh-seed replication runs of the designs; a subset of runs}
\expandafter\gdef\csname R@an.counts.runs.guard\endcsname{11}
\expandafter\gdef\csname R@an.counts.runs.guard.def\endcsname{finished ACDC guard runs of the designs; a subset of runs}
\expandafter\gdef\csname R@an.counts.runs.screen\endcsname{53}
\expandafter\gdef\csname R@an.counts.runs.screen.def\endcsname{finished discovery-screen runs of the designs; a subset of runs}
\expandafter\gdef\csname R@an.counts.sentence.funnel\endcsname{over the feedback waves the agents proposed 111 ideas, built 51 designs, registered 42 of them, trained 38 at full budget and replicated 25 on fresh seeds}
\expandafter\gdef\csname R@an.counts.sentence.search\endcsname{the search trained 28 designs at full budget in 138 runs, about 68 GPU-days on the device the network trains on (140 GPU-days as allocated, each run holding 2 GPUs)}
\expandafter\gdef\csname R@an.counts.trained\endcsname{38}
\expandafter\gdef\csname R@an.counts.trained.def\endcsname{registered arms trained at full budget (1000 epochs) at fold 0 with a Dice on a co-primary; a subset of registered (4 registered arms were not trained)}
\expandafter\gdef\csname R@an.counts.untrained\endcsname{4}
\expandafter\gdef\csname R@an.counts.untrained.def\endcsname{registered arms without a full-budget result; registered minus trained}
\expandafter\gdef\csname R@an.cv.B\endcsname{2000}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.clause\endcsname{LeanDec minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.05}\,pp, 95\,\% interval \ensuremath{-0.19} to \ensuremath{+0.08}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.est\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.hi\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.lo\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.D2.f1\endcsname{91.51}
\expandafter\gdef\csname R@an.cv.acdc.D2.f2\endcsname{91.71}
\expandafter\gdef\csname R@an.cv.acdc.D2.f3\endcsname{91.66}
\expandafter\gdef\csname R@an.cv.acdc.D2.f4\endcsname{90.41}
\expandafter\gdef\csname R@an.cv.acdc.D2.max14\endcsname{91.71}
\expandafter\gdef\csname R@an.cv.acdc.D2.min14\endcsname{90.41}
\expandafter\gdef\csname R@an.cv.acdc.D2.params\endcsname{25.28}
\expandafter\gdef\csname R@an.cv.acdc.D2.params1\endcsname{25.3}
\expandafter\gdef\csname R@an.cv.acdc.D2.span14\endcsname{1.30}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.clause\endcsname{LeanDec minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.02}\,pp, 95\,\% interval \ensuremath{-0.11} to \ensuremath{+0.18}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.est\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.hi\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.lo\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.ctloffset\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.dcv\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.f1\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.f2\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.f3\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.f4\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.hi\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.lo\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.loo.max\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.loo.min\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.loo.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.loo.word\endcsname{changes sign when a single fold is dropped (three of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.share.word\endcsname{fold 2 alone carries 242\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.share_max\endcsname{242}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.span14\endcsname{0.37}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.split\endcsname{LeanDec minus the default is \ensuremath{-0.05}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.08}\,pp, so the margin over the function-identical control is \ensuremath{+0.02}\,pp}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.vsdefault\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.word\endcsname{improves on it on average (2 of 4 folds)}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.D2base.dcv\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.acdc.D2base.f1\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.acdc.D2base.f2\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.D2base.f3\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.acdc.D2base.f4\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.D2base.hi\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.acdc.D2base.lo\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.acdc.D2base.loo.max\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cv.acdc.D2base.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.D2base.loo.min\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.acdc.D2base.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.D2base.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.D2base.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.D2base.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.D2base.share.word\endcsname{fold 3 alone carries 69\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.D2base.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.D2base.share_max\endcsname{69}
\expandafter\gdef\csname R@an.cv.acdc.D2base.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.D2base.span14\endcsname{0.20}
\expandafter\gdef\csname R@an.cv.acdc.D2base.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.clause\endcsname{ResEnc-M minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.37}\,pp, 95\,\% interval \ensuremath{+0.21} to \ensuremath{+0.55}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.est\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.hi\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.lo\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L1.f0\endcsname{92.25}
\expandafter\gdef\csname R@an.cv.acdc.L1.f1\endcsname{91.87}
\expandafter\gdef\csname R@an.cv.acdc.L1.f2\endcsname{92.03}
\expandafter\gdef\csname R@an.cv.acdc.L1.f3\endcsname{92.21}
\expandafter\gdef\csname R@an.cv.acdc.L1.f4\endcsname{90.90}
\expandafter\gdef\csname R@an.cv.acdc.L1.max14\endcsname{92.21}
\expandafter\gdef\csname R@an.cv.acdc.L1.mean14\endcsname{91.75}
\expandafter\gdef\csname R@an.cv.acdc.L1.mean5\endcsname{91.85}
\expandafter\gdef\csname R@an.cv.acdc.L1.min14\endcsname{90.90}
\expandafter\gdef\csname R@an.cv.acdc.L1.params\endcsname{101.53}
\expandafter\gdef\csname R@an.cv.acdc.L1.params1\endcsname{101.5}
\expandafter\gdef\csname R@an.cv.acdc.L1.span14\endcsname{1.32}
\expandafter\gdef\csname R@an.cv.acdc.L1.src0\endcsname{fresh s1-2}
\expandafter\gdef\csname R@an.cv.acdc.L1.src0long\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.cv.acdc.L1.src0mark\endcsname{b}
\expandafter\gdef\csname R@an.cv.acdc.L1.src0n\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.dcv\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.f1\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.f2\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.f3\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.f4\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.hi\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.lo\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.loo.max\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.loo.min\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.loo.minfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.share.word\endcsname{fold 3 alone carries 40\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.share_max\endcsname{40}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.span14\endcsname{0.20}
\expandafter\gdef\csname R@an.cv.acdc.L1L1b.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.boot.casewidth\endcsname{0.30}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.boot.foldwidth\endcsname{0.55}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.boot.hi\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.boot.lo\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.boot.mean\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.boot.n\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.11} to \ensuremath{+0.19}\,pp over the 160 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.dcv\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.f1\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.f2\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.f3\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.f4\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.hi\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.lo\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.loo.max\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.loo.min\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.loo.minfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.loo.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.loo.word\endcsname{changes sign when a single fold is dropped (three of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.share.word\endcsname{fold 3 alone carries 165\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.share_max\endcsname{165}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.span14\endcsname{0.39}
\expandafter\gdef\csname R@an.cv.acdc.L1L3.word\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.clause\endcsname{ResEnc-M minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.45}\,pp, 95\,\% interval \ensuremath{+0.26} to \ensuremath{+0.66}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.est\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.hi\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.lo\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.ctloffset\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.dcv\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.f1\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.f2\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.f3\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.f4\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.hi\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.lo\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.loo.max\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.loo.min\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.share.word\endcsname{fold 2 alone carries 31\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.share_max\endcsname{31}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.span14\endcsname{0.16}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.split\endcsname{ResEnc-M minus the default is \ensuremath{+0.37}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.08}\,pp, so the margin over the function-identical control is \ensuremath{+0.45}\,pp}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.vsdefault\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.word\endcsname{improves on the control in every fold}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.clause\endcsname{ResEnc-matched minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.19}\,pp, 95\,\% interval \ensuremath{+0.04} to \ensuremath{+0.37}\,pp, which lies inside $\pm$0.50\,pp and above zero}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.est\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.hi\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.lo\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L1b.f1\endcsname{91.76}
\expandafter\gdef\csname R@an.cv.acdc.L1b.f2\endcsname{91.94}
\expandafter\gdef\csname R@an.cv.acdc.L1b.f3\endcsname{91.93}
\expandafter\gdef\csname R@an.cv.acdc.L1b.f4\endcsname{90.67}
\expandafter\gdef\csname R@an.cv.acdc.L1b.mean14\endcsname{91.57}
\expandafter\gdef\csname R@an.cv.acdc.L1b.params\endcsname{101.63}
\expandafter\gdef\csname R@an.cv.acdc.L1b.params1\endcsname{101.6}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.dcv\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.f1\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.f2\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.f3\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.f4\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.hi\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.lo\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.loo.max\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.loo.min\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.loo.minfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.share.word\endcsname{fold 2 alone carries 42\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.share_max\endcsname{42}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.span14\endcsname{0.19}
\expandafter\gdef\csname R@an.cv.acdc.L1bL3.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.L1base.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.acdc.L1base.boot.casewidth\endcsname{0.34}
\expandafter\gdef\csname R@an.cv.acdc.L1base.boot.foldwidth\endcsname{0.21}
\expandafter\gdef\csname R@an.cv.acdc.L1base.boot.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.boot.lo\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.boot.mean\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.boot.n\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L1base.boot.vsfold\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.acdc.L1base.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.20} to \ensuremath{+0.54}\,pp over the 160 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.acdc.L1base.d5\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.d5alt\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.dcv\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f0\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f0alt\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f0band\endcsname{0.16}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f0band.note\endcsname{two null SDs of this fold-0 difference, each the frozen default pool's training-seed SD of 0.099\,pp times $\sqrt{1/2 + 1/6}$ for the mean of two runs against the mean of the six-run pool: a locating band, not a test}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f0bandword\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f0gap\endcsname{0.24}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f0rev\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f0se\endcsname{0.081}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f1\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f2\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f3\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.f4\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.hi\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.lo\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.loo.max\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L1base.loo.min\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.acdc.L1base.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.L1base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L1base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.L1base.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L1base.share.word\endcsname{fold 4 alone carries 30\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.L1base.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.L1base.share_max\endcsname{30}
\expandafter\gdef\csname R@an.cv.acdc.L1base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.L1base.span14\endcsname{0.16}
\expandafter\gdef\csname R@an.cv.acdc.L1base.src0\endcsname{fresh s1-2 for ResEnc-M and frozen pool for default}
\expandafter\gdef\csname R@an.cv.acdc.L1base.src0mark\endcsname{b/a}
\expandafter\gdef\csname R@an.cv.acdc.L1base.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.clause\endcsname{HyReX minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.33}\,pp, 95\,\% interval \ensuremath{+0.19} to \ensuremath{+0.49}\,pp, which lies inside $\pm$0.50\,pp and above zero}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.est\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.hi\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.lo\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L3.f0\endcsname{92.46}
\expandafter\gdef\csname R@an.cv.acdc.L3.f1\endcsname{91.92}
\expandafter\gdef\csname R@an.cv.acdc.L3.f2\endcsname{92.18}
\expandafter\gdef\csname R@an.cv.acdc.L3.f3\endcsname{91.97}
\expandafter\gdef\csname R@an.cv.acdc.L3.f4\endcsname{90.79}
\expandafter\gdef\csname R@an.cv.acdc.L3.max14\endcsname{92.18}
\expandafter\gdef\csname R@an.cv.acdc.L3.mean14\endcsname{91.71}
\expandafter\gdef\csname R@an.cv.acdc.L3.mean5\endcsname{91.86}
\expandafter\gdef\csname R@an.cv.acdc.L3.min14\endcsname{90.79}
\expandafter\gdef\csname R@an.cv.acdc.L3.params\endcsname{28.85}
\expandafter\gdef\csname R@an.cv.acdc.L3.params1\endcsname{28.8}
\expandafter\gdef\csname R@an.cv.acdc.L3.span14\endcsname{1.39}
\expandafter\gdef\csname R@an.cv.acdc.L3.src0\endcsname{fresh s1-2}
\expandafter\gdef\csname R@an.cv.acdc.L3.src0long\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.cv.acdc.L3.src0mark\endcsname{b}
\expandafter\gdef\csname R@an.cv.acdc.L3.src0n\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.boot.casewidth\endcsname{0.31}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.boot.foldwidth\endcsname{0.55}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.boot.hi\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.boot.lo\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.boot.mean\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.boot.n\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.20} to \ensuremath{+0.11}\,pp over the 160 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.d5\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.dcv\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.f0\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.f0gap\endcsname{0.21}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.f0lead\endcsname{the 0.50 pp registered pair floor does not resolve HyReX against ResEnc-M}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.f0rev\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.f1\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.f2\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.f3\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.f4\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.hi\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.lo\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.loo.max\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.loo.min\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.loo.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.loo.word\endcsname{changes sign when a single fold is dropped (one of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.share.word\endcsname{fold 3 alone carries 165\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.share_max\endcsname{165}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.span14\endcsname{0.39}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.src0\endcsname{fresh s1-2 for HyReX and for ResEnc-M}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.src0mark\endcsname{b/b}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.L3L1.wordrev\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.clause\endcsname{HyReX minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.41}\,pp, 95\,\% interval \ensuremath{+0.22} to \ensuremath{+0.62}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.est\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.hi\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.lo\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.dcv\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.f1\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.f2\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.f3\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.f4\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.hi\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.lo\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.loo.max\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.loo.min\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.share.word\endcsname{fold 2 alone carries 42\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.share_max\endcsname{42}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.span14\endcsname{0.53}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.acdc.L3base.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.acdc.L3base.boot.casewidth\endcsname{0.30}
\expandafter\gdef\csname R@an.cv.acdc.L3base.boot.foldwidth\endcsname{0.46}
\expandafter\gdef\csname R@an.cv.acdc.L3base.boot.hi\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.boot.lo\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.boot.mean\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.boot.n\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L3base.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.acdc.L3base.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.18} to \ensuremath{+0.48}\,pp over the 160 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.acdc.L3base.d5\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.d5alt\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.dcv\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f0\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f0alt\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f0band\endcsname{0.16}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f0band.note\endcsname{two null SDs of this fold-0 difference, each the frozen default pool's training-seed SD of 0.099\,pp times $\sqrt{1/2 + 1/6}$ for the mean of two runs against the mean of the six-run pool: a locating band, not a test}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f0bandword\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f0gap\endcsname{0.45}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f0rev\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f0se\endcsname{0.081}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f1\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f2\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f3\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.f4\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.hi\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.lo\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.loo.max\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.L3base.loo.min\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.cv.acdc.L3base.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L3base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L3base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.L3base.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.L3base.share.word\endcsname{fold 2 alone carries 38\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.L3base.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.L3base.share_max\endcsname{38}
\expandafter\gdef\csname R@an.cv.acdc.L3base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.L3base.span14\endcsname{0.35}
\expandafter\gdef\csname R@an.cv.acdc.L3base.src0\endcsname{fresh s1-2 for HyReX and frozen pool for default}
\expandafter\gdef\csname R@an.cv.acdc.L3base.src0mark\endcsname{b/a}
\expandafter\gdef\csname R@an.cv.acdc.L3base.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.clause\endcsname{the function-identical control minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.08}\,pp, 95\,\% interval \ensuremath{-0.20} to \ensuremath{+0.04}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.est\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.hi\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.lo\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.P3c.f1\endcsname{91.47}
\expandafter\gdef\csname R@an.cv.acdc.P3c.f2\endcsname{91.48}
\expandafter\gdef\csname R@an.cv.acdc.P3c.f3\endcsname{91.80}
\expandafter\gdef\csname R@an.cv.acdc.P3c.f4\endcsname{90.46}
\expandafter\gdef\csname R@an.cv.acdc.P3c.max14\endcsname{91.80}
\expandafter\gdef\csname R@an.cv.acdc.P3c.mean14\endcsname{91.30}
\expandafter\gdef\csname R@an.cv.acdc.P3c.min14\endcsname{90.46}
\expandafter\gdef\csname R@an.cv.acdc.P3c.params\endcsname{30.38}
\expandafter\gdef\csname R@an.cv.acdc.P3c.params1\endcsname{30.4}
\expandafter\gdef\csname R@an.cv.acdc.P3c.span14\endcsname{1.34}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.dcv\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.f1\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.f2\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.f3\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.f4\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.hi\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.lo\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.loo.max\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.loo.min\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.share.word\endcsname{fold 2 alone carries 60\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.share_max\endcsname{60}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.span14\endcsname{0.19}
\expandafter\gdef\csname R@an.cv.acdc.P3cbase.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.clause\endcsname{LeanAdd minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.12}\,pp, 95\,\% interval \ensuremath{-0.25} to \ensuremath{+0.01}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.est\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.hi\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.lo\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.f1\endcsname{91.56}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.f2\endcsname{91.61}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.f3\endcsname{91.51}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.f4\endcsname{90.37}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.mean14\endcsname{91.26}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.params\endcsname{20.18}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.params1\endcsname{20.2}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.dcv\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.f1\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.f2\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.f3\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.f4\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.hi\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.lo\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.loo.max\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.loo.min\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.share.word\endcsname{fold 3 alone carries 60\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.share_max\endcsname{60}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.span14\endcsname{0.20}
\expandafter\gdef\csname R@an.cv.acdc.V5B1D2.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.clause\endcsname{LeanAdd minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.04}\,pp, 95\,\% interval \ensuremath{-0.17} to \ensuremath{+0.10}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.est\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.hi\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.lo\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.ctloffset\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.dcv\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.f1\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.f2\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.f3\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.f4\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.hi\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.lo\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.loo.max\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.loo.min\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.loo.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.loo.word\endcsname{changes sign when a single fold is dropped (one of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.share.word\endcsname{fold 3 alone carries 184\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.share_max\endcsname{184}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.span14\endcsname{0.42}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.split\endcsname{LeanAdd minus the default is \ensuremath{-0.12}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.08}\,pp, so the margin over the function-identical control is \ensuremath{-0.04}\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.vsdefault\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.word\endcsname{does not improve on it}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.dcv\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.f1\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.f2\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.f3\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.f4\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.hi\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.lo\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.loo.max\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.loo.min\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.share.word\endcsname{fold 3 alone carries 65\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.share_max\endcsname{65}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.span14\endcsname{0.28}
\expandafter\gdef\csname R@an.cv.acdc.V5B1base.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.clause\endcsname{LeanAdd-NeXt minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.11}\,pp, 95\,\% interval \ensuremath{-0.27} to \ensuremath{+0.04}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.est\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.hi\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.lo\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.f1\endcsname{91.31}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.f2\endcsname{91.65}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.f3\endcsname{91.70}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.f4\endcsname{90.41}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.mean14\endcsname{91.27}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.params\endcsname{20.48}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.params1\endcsname{20.5}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.dcv\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.f1\endcsname{\ensuremath{-0.62}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.f2\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.f3\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.f4\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.hi\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.lo\endcsname{\ensuremath{-0.69}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.loo.max\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.loo.min\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.loo.minfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.share.word\endcsname{fold 1 alone carries 34\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.share_max\endcsname{34}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.span14\endcsname{0.35}
\expandafter\gdef\csname R@an.cv.acdc.V5B2L3.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.clause\endcsname{LeanAdd-NeXt minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.04}\,pp, 95\,\% interval \ensuremath{-0.19} to \ensuremath{+0.13}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.est\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.hi\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.lo\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.ctloffset\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.dcv\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.f1\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.f2\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.f3\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.f4\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.hi\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.lo\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.loo.max\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.loo.min\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.loo.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.loo.word\endcsname{changes sign when a single fold is dropped (one of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.share.word\endcsname{fold 1 alone carries 118\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.share_max\endcsname{118}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.span14\endcsname{0.34}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.split\endcsname{LeanAdd-NeXt minus the default is \ensuremath{-0.11}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.08}\,pp, so the margin over the function-identical control is \ensuremath{-0.04}\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.vsdefault\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.word\endcsname{does not improve on it}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.dcv\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.f1\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.f2\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.f3\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.f4\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.hi\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.lo\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.loo.max\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.loo.min\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.loo.minfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.loo.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.loo.word\endcsname{changes sign when a single fold is dropped (one of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.share.word\endcsname{fold 3 alone carries 1368\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.share_max\endcsname{1368}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.span14\endcsname{0.44}
\expandafter\gdef\csname R@an.cv.acdc.V5B2V5B1.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.dcv\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.f1\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.f2\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.f3\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.f4\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.hi\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.lo\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.loo.max\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.loo.min\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.share.word\endcsname{fold 1 alone carries 60\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.share_max\endcsname{60}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.span14\endcsname{0.26}
\expandafter\gdef\csname R@an.cv.acdc.V5B2base.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.clause\endcsname{HyReX-k9 minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.31}\,pp, 95\,\% interval \ensuremath{+0.18} to \ensuremath{+0.44}\,pp, which lies inside $\pm$0.50\,pp and above zero}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.est\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.hi\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.lo\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.f1\endcsname{91.95}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.f2\endcsname{91.92}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.f3\endcsname{91.99}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.f4\endcsname{90.88}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.mean14\endcsname{91.69}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.params\endcsname{29.96}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.params1\endcsname{30.0}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.dcv\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.f1\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.f2\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.f3\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.f4\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.hi\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.lo\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.loo.max\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.loo.min\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.loo.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.loo.word\endcsname{changes sign when a single fold is dropped (one of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.share.word\endcsname{fold 2 alone carries 239\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.share_max\endcsname{239}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.span14\endcsname{0.35}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rL3.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.clause\endcsname{HyReX-k9 minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.38}\,pp, 95\,\% interval \ensuremath{+0.22} to \ensuremath{+0.56}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.est\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.hi\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.lo\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.ctloffset\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.dcv\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.f1\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.f2\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.f3\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.f4\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.hi\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.lo\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.loo.max\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.loo.min\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.share.word\endcsname{fold 1 alone carries 31\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.share_max\endcsname{31}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.span14\endcsname{0.29}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.split\endcsname{HyReX-k9 minus the default is \ensuremath{+0.31}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.08}\,pp, so the margin over the function-identical control is \ensuremath{+0.38}\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.vsdefault\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.word\endcsname{improves on the control in every fold}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.dcv\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.f1\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.f2\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.f3\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.f4\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.hi\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.lo\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.loo.max\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.loo.min\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.share.word\endcsname{fold 4 alone carries 35\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.share_max\endcsname{35}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.span14\endcsname{0.25}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rbase.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.clause\endcsname{LeanDeepMid minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.08}\,pp, 95\,\% interval \ensuremath{-0.09} to \ensuremath{+0.24}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.est\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.hi\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.lo\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.f1\endcsname{91.57}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.f2\endcsname{91.72}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.f3\endcsname{91.61}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.f4\endcsname{90.94}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.mean14\endcsname{91.46}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.params\endcsname{30.26}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.params1\endcsname{30.3}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.clause\endcsname{LeanDeepMid minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.16}\,pp, 95\,\% interval \ensuremath{-0.02} to \ensuremath{+0.35}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.est\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.hi\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.lo\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.ctloffset\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.dcv\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.f1\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.f2\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.f3\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.f4\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.hi\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.lo\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.loo.max\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.loo.min\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.share.word\endcsname{fold 4 alone carries 76\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.share_max\endcsname{76}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.span14\endcsname{0.67}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.split\endcsname{LeanDeepMid minus the default is \ensuremath{+0.08}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.08}\,pp, so the margin over the function-identical control is \ensuremath{+0.16}\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.vsdefault\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.word\endcsname{improves on it on average (3 of 4 folds)}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.dcv\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.f1\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.f2\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.f3\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.f4\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.hi\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.lo\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.loo.max\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.loo.min\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.share.word\endcsname{fold 4 alone carries 68\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.share_max\endcsname{68}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.span14\endcsname{0.62}
\expandafter\gdef\csname R@an.cv.acdc.V7A1V5B2.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.dcv\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.f1\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.f2\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.f3\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.f4\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.lo\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.loo.max\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.loo.min\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.loo.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.loo.word\endcsname{changes sign when a single fold is dropped (three of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.share.word\endcsname{fold 4 alone carries 152\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.share_max\endcsname{152}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.span14\endcsname{0.69}
\expandafter\gdef\csname R@an.cv.acdc.V7A1base.word\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.cv.acdc.V7A2.cbs.clause\endcsname{LeanDeepMid+FD minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.acdc.V7A2.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7A2.params\endcsname{30.38}
\expandafter\gdef\csname R@an.cv.acdc.V7A2.params1\endcsname{30.4}
\expandafter\gdef\csname R@an.cv.acdc.V7A2P3c.cbs.clause\endcsname{LeanDeepMid+FD minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.acdc.V7A2P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7A2P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7A2P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7A2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7A2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7A2V7A1.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7A2V7A1.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7A2base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7A2base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7B1.cbs.clause\endcsname{LeanSep minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.acdc.V7B1.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B1.params\endcsname{19.65}
\expandafter\gdef\csname R@an.cv.acdc.V7B1.params1\endcsname{19.6}
\expandafter\gdef\csname R@an.cv.acdc.V7B1P3c.cbs.clause\endcsname{LeanSep minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.acdc.V7B1P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B1P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B1P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7B1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7B1V5B2.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B1V5B2.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7B1base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B1base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7B2.cbs.clause\endcsname{LeanDil minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.acdc.V7B2.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B2.params\endcsname{19.67}
\expandafter\gdef\csname R@an.cv.acdc.V7B2.params1\endcsname{19.7}
\expandafter\gdef\csname R@an.cv.acdc.V7B2P3c.cbs.clause\endcsname{LeanDil minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.acdc.V7B2P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B2P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B2P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7B2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7B2V5B2.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B2V5B2.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7B2base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7B2base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.clause\endcsname{LeanNeXt-s5 minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.19}\,pp, 95\,\% interval \ensuremath{-0.34} to \ensuremath{-0.04}\,pp, which lies inside $\pm$0.50\,pp and below zero}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.est\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.hi\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.lo\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.f1\endcsname{91.30}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.f2\endcsname{91.56}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.f3\endcsname{91.61}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.f4\endcsname{90.29}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.mean14\endcsname{91.19}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.params\endcsname{20.33}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.params1\endcsname{20.3}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.clause\endcsname{LeanNeXt-s5 minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.11}\,pp, 95\,\% interval \ensuremath{-0.25} to \ensuremath{+0.04}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.est\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.hi\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.lo\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.ctloffset\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.dcv\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.f1\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.f2\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.f3\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.f4\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.hi\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.lo\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.loo.max\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.loo.min\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.share.word\endcsname{fold 3 alone carries 43\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.share_max\endcsname{43}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.span14\endcsname{0.27}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.split\endcsname{LeanNeXt-s5 minus the default is \ensuremath{-0.19}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.08}\,pp, so the margin over the function-identical control is \ensuremath{-0.11}\,pp}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.vsdefault\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.word\endcsname{does not improve on it}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.dcv\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.f1\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.f2\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.f3\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.f4\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.hi\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.lo\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.loo.max\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.loo.min\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.share.word\endcsname{fold 4 alone carries 39\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.share_max\endcsname{39}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.span14\endcsname{0.11}
\expandafter\gdef\csname R@an.cv.acdc.V7C1V5B2.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.dcv\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.f1\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.f2\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.f3\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.f4\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.hi\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.lo\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.loo.max\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.loo.min\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.share.word\endcsname{fold 1 alone carries 37\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.share_max\endcsname{37}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.span14\endcsname{0.18}
\expandafter\gdef\csname R@an.cv.acdc.V7C1base.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.acdc.V8B2.cbs.clause\endcsname{Stem1 minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.acdc.V8B2.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V8B2.params\endcsname{20.32}
\expandafter\gdef\csname R@an.cv.acdc.V8B2.params1\endcsname{20.3}
\expandafter\gdef\csname R@an.cv.acdc.V8B2P3c.cbs.clause\endcsname{Stem1 minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.acdc.V8B2P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V8B2P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V8B2P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V8B2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V8B2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.V8B2base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.acdc.V8B2base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.acdc.base.f0\endcsname{92.01}
\expandafter\gdef\csname R@an.cv.acdc.base.f1\endcsname{91.58}
\expandafter\gdef\csname R@an.cv.acdc.base.f2\endcsname{91.67}
\expandafter\gdef\csname R@an.cv.acdc.base.f3\endcsname{91.82}
\expandafter\gdef\csname R@an.cv.acdc.base.f4\endcsname{90.46}
\expandafter\gdef\csname R@an.cv.acdc.base.max14\endcsname{91.82}
\expandafter\gdef\csname R@an.cv.acdc.base.mean14\endcsname{91.38}
\expandafter\gdef\csname R@an.cv.acdc.base.mean5\endcsname{91.51}
\expandafter\gdef\csname R@an.cv.acdc.base.min14\endcsname{90.46}
\expandafter\gdef\csname R@an.cv.acdc.base.params\endcsname{30.38}
\expandafter\gdef\csname R@an.cv.acdc.base.params1\endcsname{30.4}
\expandafter\gdef\csname R@an.cv.acdc.base.span14\endcsname{1.36}
\expandafter\gdef\csname R@an.cv.acdc.base.src0\endcsname{frozen pool}
\expandafter\gdef\csname R@an.cv.acdc.base.src0long\endcsname{the frozen default pool}
\expandafter\gdef\csname R@an.cv.acdc.base.src0mark\endcsname{a}
\expandafter\gdef\csname R@an.cv.acdc.base.src0n\endcsname{6}
\expandafter\gdef\csname R@an.cv.acdc.recovery.L3\endcsname{0.90}
\expandafter\gdef\csname R@an.cv.acdc.recovery.L3.hi\endcsname{1.63}
\expandafter\gdef\csname R@an.cv.acdc.recovery.L3.lo\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.acdc.recovery.L3.method\endcsname{the delta method applied to the two four-fold mean margins, HyReX minus the default and ResEnc-M minus the default, which are differences from the same default runs, so their covariance over the folds enters the variance of the ratio; the interval takes the t quantile on three degrees of freedom of the registered paired-t intervals of the margins; it is descriptive, a description of four folds of one seed each and not a test, and it is withheld when ResEnc-M's own interval over the folds includes zero}
\expandafter\gdef\csname R@an.cv.acdc.recovery.L3.sentence\endcsname{On ACDC, HyReX's mean margin over the default on the four folds that entered no decision, \ensuremath{+0.33}\,pp, is 0.90 of ResEnc-M's, \ensuremath{+0.37}\,pp; the 95\,\% interval of that ratio, 0.17 to 1.63, comes from the delta method on the two fold-mean margins and describes the four folds without testing anything}
\expandafter\gdef\csname R@an.cv.acdc.recovery.L3.state\endcsname{complete}
\expandafter\gdef\csname R@an.cv.acdc.replication\endcsname{ACDC is a registered guard, not a co-primary; the registered ACDC fresh-seed replication has landed, so its fold-0 cells for HyReX and ResEnc-M are fresh seed-1-2 means, while the four confirmation folds remain one seed per arm}
\expandafter\gdef\csname R@an.cv.amos.D2.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.D2.cbs.clause\endcsname{LeanDec minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.43}\,pp, 95\,\% interval \ensuremath{-0.66} to \ensuremath{-0.22}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.amos.D2.cbs.est\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.cv.amos.D2.cbs.hi\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.cv.amos.D2.cbs.lo\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.cv.amos.D2.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.D2.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.D2.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.D2.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.D2.f0\endcsname{87.34}
\expandafter\gdef\csname R@an.cv.amos.D2.f1\endcsname{88.83}
\expandafter\gdef\csname R@an.cv.amos.D2.f2\endcsname{87.92}
\expandafter\gdef\csname R@an.cv.amos.D2.f3\endcsname{88.14}
\expandafter\gdef\csname R@an.cv.amos.D2.f4\endcsname{86.74}
\expandafter\gdef\csname R@an.cv.amos.D2.max14\endcsname{88.83}
\expandafter\gdef\csname R@an.cv.amos.D2.mean14\endcsname{87.91}
\expandafter\gdef\csname R@an.cv.amos.D2.mean5\endcsname{87.79}
\expandafter\gdef\csname R@an.cv.amos.D2.min14\endcsname{86.74}
\expandafter\gdef\csname R@an.cv.amos.D2.params\endcsname{26.03}
\expandafter\gdef\csname R@an.cv.amos.D2.params1\endcsname{26.0}
\expandafter\gdef\csname R@an.cv.amos.D2.span14\endcsname{2.08}
\expandafter\gdef\csname R@an.cv.amos.D2.src0\endcsname{seed 0}
\expandafter\gdef\csname R@an.cv.amos.D2.src0long\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.cv.amos.D2.src0mark\endcsname{c}
\expandafter\gdef\csname R@an.cv.amos.D2.src0n\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.cbs.clause\endcsname{LeanDec minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.40}\,pp, 95\,\% interval \ensuremath{-0.61} to \ensuremath{-0.18}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.cbs.est\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.cbs.hi\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.cbs.lo\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.ctloffset\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.dcv\endcsname{\ensuremath{-0.41}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.f1\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.f2\endcsname{\ensuremath{-0.72}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.f3\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.f4\endcsname{\ensuremath{-0.60}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.hi\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.lo\endcsname{\ensuremath{-0.95}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.loo.max\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.loo.min\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.share.word\endcsname{fold 2 alone carries 44\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.share_max\endcsname{44}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.span14\endcsname{0.78}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.split\endcsname{LeanDec minus the default is \ensuremath{-0.44}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.03}\,pp, so the margin over the function-identical control is \ensuremath{-0.41}\,pp}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.vsdefault\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.cv.amos.D2P3c.word\endcsname{does not improve on it}
\expandafter\gdef\csname R@an.cv.amos.D2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.D2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.D2base.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.amos.D2base.boot.casewidth\endcsname{0.28}
\expandafter\gdef\csname R@an.cv.amos.D2base.boot.foldwidth\endcsname{0.63}
\expandafter\gdef\csname R@an.cv.amos.D2base.boot.hi\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.cv.amos.D2base.boot.lo\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.cv.amos.D2base.boot.mean\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.cv.amos.D2base.boot.n\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.D2base.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.amos.D2base.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.51} to \ensuremath{-0.23}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.amos.D2base.d5\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.cv.amos.D2base.d5alt\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.cv.amos.D2base.dcv\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.cv.amos.D2base.f0\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.cv.amos.D2base.f0alt\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.cv.amos.D2base.f0band\endcsname{0.26}
\expandafter\gdef\csname R@an.cv.amos.D2base.f0band.note\endcsname{two null SDs of this fold-0 difference, each the frozen default pool's training-seed SD of 0.122\,pp times $\sqrt{1/1 + 1/6}$ for the mean of one run against the mean of the six-run pool: a locating band, not a test}
\expandafter\gdef\csname R@an.cv.amos.D2base.f0bandword\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.amos.D2base.f0gap\endcsname{0.36}
\expandafter\gdef\csname R@an.cv.amos.D2base.f0rev\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.amos.D2base.f0se\endcsname{0.132}
\expandafter\gdef\csname R@an.cv.amos.D2base.f1\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.cv.amos.D2base.f2\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.cv.amos.D2base.f3\endcsname{\ensuremath{-0.65}}
\expandafter\gdef\csname R@an.cv.amos.D2base.f4\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.amos.D2base.hi\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.amos.D2base.lo\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.cv.amos.D2base.loo.max\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.cv.amos.D2base.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.D2base.loo.min\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.cv.amos.D2base.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.D2base.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.D2base.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.D2base.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.D2base.share.word\endcsname{fold 3 alone carries 37\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.D2base.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.D2base.share_max\endcsname{37}
\expandafter\gdef\csname R@an.cv.amos.D2base.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.D2base.span14\endcsname{0.40}
\expandafter\gdef\csname R@an.cv.amos.D2base.src0\endcsname{seed 0 for LeanDec and frozen pool for default}
\expandafter\gdef\csname R@an.cv.amos.D2base.src0mark\endcsname{c/a}
\expandafter\gdef\csname R@an.cv.amos.D2base.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.L1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.L1.cbs.clause\endcsname{ResEnc-M minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.40}\,pp, 95\,\% interval \ensuremath{+0.16} to \ensuremath{+0.65}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.amos.L1.cbs.est\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.cv.amos.L1.cbs.hi\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.cv.amos.L1.cbs.lo\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.cv.amos.L1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.L1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.L1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1.f0\endcsname{88.17}
\expandafter\gdef\csname R@an.cv.amos.L1.f1\endcsname{89.46}
\expandafter\gdef\csname R@an.cv.amos.L1.f2\endcsname{89.25}
\expandafter\gdef\csname R@an.cv.amos.L1.f3\endcsname{88.63}
\expandafter\gdef\csname R@an.cv.amos.L1.f4\endcsname{87.68}
\expandafter\gdef\csname R@an.cv.amos.L1.max14\endcsname{89.46}
\expandafter\gdef\csname R@an.cv.amos.L1.mean14\endcsname{88.75}
\expandafter\gdef\csname R@an.cv.amos.L1.mean5\endcsname{88.64}
\expandafter\gdef\csname R@an.cv.amos.L1.min14\endcsname{87.68}
\expandafter\gdef\csname R@an.cv.amos.L1.params\endcsname{102.28}
\expandafter\gdef\csname R@an.cv.amos.L1.params1\endcsname{102.3}
\expandafter\gdef\csname R@an.cv.amos.L1.span14\endcsname{1.78}
\expandafter\gdef\csname R@an.cv.amos.L1.src0\endcsname{fresh s1-2}
\expandafter\gdef\csname R@an.cv.amos.L1.src0long\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.cv.amos.L1.src0mark\endcsname{b}
\expandafter\gdef\csname R@an.cv.amos.L1.src0n\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.dcv\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.f1\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.f2\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.f3\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.f4\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.hi\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.lo\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.loo.max\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.loo.min\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.loo.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.loo.word\endcsname{changes sign when a single fold is dropped (one of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.share.word\endcsname{fold 1 alone carries 202\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.share_max\endcsname{202}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.span14\endcsname{0.39}
\expandafter\gdef\csname R@an.cv.amos.L1L1b.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.L1L3.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.amos.L1L3.boot.casewidth\endcsname{0.28}
\expandafter\gdef\csname R@an.cv.amos.L1L3.boot.foldwidth\endcsname{1.16}
\expandafter\gdef\csname R@an.cv.amos.L1L3.boot.hi\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.boot.lo\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.boot.mean\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.boot.n\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.L1L3.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.amos.L1L3.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.08} to \ensuremath{+0.21}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.amos.L1L3.dcv\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.f1\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.f2\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.f3\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.f4\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.hi\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.lo\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.loo.max\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.L1L3.loo.min\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.amos.L1L3.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.L1L3.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.L1L3.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.L1L3.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.amos.L1L3.share.word\endcsname{fold 2 alone carries 57\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.L1L3.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.L1L3.share_max\endcsname{57}
\expandafter\gdef\csname R@an.cv.amos.L1L3.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.L1L3.span14\endcsname{0.77}
\expandafter\gdef\csname R@an.cv.amos.L1L3.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.cbs.clause\endcsname{ResEnc-M minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.44}\,pp, 95\,\% interval \ensuremath{+0.19} to \ensuremath{+0.71}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.cbs.est\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.cbs.hi\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.cbs.lo\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.ctloffset\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.dcv\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.f1\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.f2\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.f3\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.f4\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.hi\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.lo\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.loo.max\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.loo.min\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.share.word\endcsname{fold 1 alone carries 40\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.share_max\endcsname{40}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.span14\endcsname{0.59}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.split\endcsname{ResEnc-M minus the default is \ensuremath{+0.41}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.03}\,pp, so the margin over the function-identical control is \ensuremath{+0.44}\,pp}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.vsdefault\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv.amos.L1P3c.word\endcsname{improves on the control in every fold}
\expandafter\gdef\csname R@an.cv.amos.L1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.L1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.L1b.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.L1b.cbs.clause\endcsname{ResEnc-matched minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.43}\,pp, 95\,\% interval \ensuremath{+0.19} to \ensuremath{+0.68}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.amos.L1b.cbs.est\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.cv.amos.L1b.cbs.hi\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.cv.amos.L1b.cbs.lo\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.amos.L1b.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.L1b.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.L1b.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1b.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1b.f1\endcsname{89.63}
\expandafter\gdef\csname R@an.cv.amos.L1b.f2\endcsname{89.03}
\expandafter\gdef\csname R@an.cv.amos.L1b.f3\endcsname{88.69}
\expandafter\gdef\csname R@an.cv.amos.L1b.f4\endcsname{87.74}
\expandafter\gdef\csname R@an.cv.amos.L1b.mean14\endcsname{88.78}
\expandafter\gdef\csname R@an.cv.amos.L1b.params\endcsname{102.37}
\expandafter\gdef\csname R@an.cv.amos.L1b.params1\endcsname{102.4}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.dcv\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.f1\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.f2\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.f3\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.f4\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.hi\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.lo\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.loo.max\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.loo.min\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.share.word\endcsname{fold 1 alone carries 69\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.share_max\endcsname{69}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.span14\endcsname{0.85}
\expandafter\gdef\csname R@an.cv.amos.L1bL3.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.amos.L1base.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.amos.L1base.boot.casewidth\endcsname{0.34}
\expandafter\gdef\csname R@an.cv.amos.L1base.boot.foldwidth\endcsname{1.36}
\expandafter\gdef\csname R@an.cv.amos.L1base.boot.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.cv.amos.L1base.boot.lo\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.amos.L1base.boot.mean\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.amos.L1base.boot.n\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.L1base.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.amos.L1base.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.20} to \ensuremath{+0.54}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.amos.L1base.d5\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.cv.amos.L1base.d5alt\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.cv.amos.L1base.dcv\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv.amos.L1base.f0\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.cv.amos.L1base.f0alt\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.amos.L1base.f0band\endcsname{0.20}
\expandafter\gdef\csname R@an.cv.amos.L1base.f0band.note\endcsname{two null SDs of this fold-0 difference, each the frozen default pool's training-seed SD of 0.122\,pp times $\sqrt{1/2 + 1/6}$ for the mean of two runs against the mean of the six-run pool: a locating band, not a test}
\expandafter\gdef\csname R@an.cv.amos.L1base.f0bandword\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.amos.L1base.f0gap\endcsname{0.46}
\expandafter\gdef\csname R@an.cv.amos.L1base.f0rev\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.cv.amos.L1base.f0se\endcsname{0.100}
\expandafter\gdef\csname R@an.cv.amos.L1base.f1\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.cv.amos.L1base.f2\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.cv.amos.L1base.f3\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.amos.L1base.f4\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.cv.amos.L1base.hi\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.cv.amos.L1base.lo\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.cv.amos.L1base.loo.max\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.cv.amos.L1base.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.L1base.loo.min\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.cv.amos.L1base.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.L1base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.L1base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.L1base.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.amos.L1base.share.word\endcsname{fold 2 alone carries 47\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.L1base.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.L1base.share_max\endcsname{47}
\expandafter\gdef\csname R@an.cv.amos.L1base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.L1base.span14\endcsname{0.94}
\expandafter\gdef\csname R@an.cv.amos.L1base.src0\endcsname{fresh s1-2 for ResEnc-M and frozen pool for default}
\expandafter\gdef\csname R@an.cv.amos.L1base.src0mark\endcsname{b/a}
\expandafter\gdef\csname R@an.cv.amos.L1base.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.amos.L3.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.L3.cbs.clause\endcsname{HyReX minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.24}\,pp, 95\,\% interval \ensuremath{+0.01} to \ensuremath{+0.46}\,pp, which lies inside $\pm$0.50\,pp and above zero}
\expandafter\gdef\csname R@an.cv.amos.L3.cbs.est\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.amos.L3.cbs.hi\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.cv.amos.L3.cbs.lo\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.amos.L3.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.L3.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.L3.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L3.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L3.f0\endcsname{87.83}
\expandafter\gdef\csname R@an.cv.amos.L3.f1\endcsname{89.09}
\expandafter\gdef\csname R@an.cv.amos.L3.f2\endcsname{88.84}
\expandafter\gdef\csname R@an.cv.amos.L3.f3\endcsname{88.99}
\expandafter\gdef\csname R@an.cv.amos.L3.f4\endcsname{87.38}
\expandafter\gdef\csname R@an.cv.amos.L3.max14\endcsname{89.09}
\expandafter\gdef\csname R@an.cv.amos.L3.mean14\endcsname{88.58}
\expandafter\gdef\csname R@an.cv.amos.L3.mean5\endcsname{88.43}
\expandafter\gdef\csname R@an.cv.amos.L3.min14\endcsname{87.38}
\expandafter\gdef\csname R@an.cv.amos.L3.params\endcsname{29.59}
\expandafter\gdef\csname R@an.cv.amos.L3.params1\endcsname{29.6}
\expandafter\gdef\csname R@an.cv.amos.L3.span14\endcsname{1.70}
\expandafter\gdef\csname R@an.cv.amos.L3.src0\endcsname{fresh s1-2}
\expandafter\gdef\csname R@an.cv.amos.L3.src0long\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.cv.amos.L3.src0mark\endcsname{b}
\expandafter\gdef\csname R@an.cv.amos.L3.src0n\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.L3L1.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.amos.L3L1.boot.casewidth\endcsname{0.29}
\expandafter\gdef\csname R@an.cv.amos.L3L1.boot.foldwidth\endcsname{1.16}
\expandafter\gdef\csname R@an.cv.amos.L3L1.boot.hi\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.boot.lo\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.boot.mean\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.boot.n\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.L3L1.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.amos.L3L1.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.21} to \ensuremath{+0.08}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.amos.L3L1.d5\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.dcv\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.f0\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.f0gap\endcsname{0.33}
\expandafter\gdef\csname R@an.cv.amos.L3L1.f0lead\endcsname{the 0.50 pp registered pair floor does not resolve HyReX against ResEnc-M}
\expandafter\gdef\csname R@an.cv.amos.L3L1.f0rev\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.f1\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.f2\endcsname{\ensuremath{-0.41}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.f3\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.f4\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.hi\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.lo\endcsname{\ensuremath{-0.76}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.loo.max\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.L3L1.loo.min\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.cv.amos.L3L1.loo.minfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.L3L1.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.L3L1.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.L3L1.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.amos.L3L1.share.word\endcsname{fold 2 alone carries 57\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.L3L1.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.L3L1.share_max\endcsname{57}
\expandafter\gdef\csname R@an.cv.amos.L3L1.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.L3L1.span14\endcsname{0.77}
\expandafter\gdef\csname R@an.cv.amos.L3L1.src0\endcsname{fresh s1-2 for HyReX and for ResEnc-M}
\expandafter\gdef\csname R@an.cv.amos.L3L1.src0mark\endcsname{b/b}
\expandafter\gdef\csname R@an.cv.amos.L3L1.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.L3L1.wordrev\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.cbs.clause\endcsname{HyReX minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.27}\,pp, 95\,\% interval \ensuremath{+0.07} to \ensuremath{+0.48}\,pp, which lies inside $\pm$0.50\,pp and above zero}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.cbs.est\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.cbs.hi\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.cbs.lo\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.dcv\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.f1\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.f2\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.f3\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.f4\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.hi\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.lo\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.loo.max\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.loo.min\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.loo.minfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.share.word\endcsname{fold 3 alone carries 45\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.share_max\endcsname{45}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.span14\endcsname{0.43}
\expandafter\gdef\csname R@an.cv.amos.L3P3c.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.amos.L3base.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.amos.L3base.boot.casewidth\endcsname{0.35}
\expandafter\gdef\csname R@an.cv.amos.L3base.boot.foldwidth\endcsname{0.61}
\expandafter\gdef\csname R@an.cv.amos.L3base.boot.hi\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.cv.amos.L3base.boot.lo\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.amos.L3base.boot.mean\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.amos.L3base.boot.n\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.L3base.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.amos.L3base.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.12} to \ensuremath{+0.47}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.amos.L3base.d5\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.amos.L3base.d5alt\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.amos.L3base.dcv\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.amos.L3base.f0\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.cv.amos.L3base.f0alt\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.amos.L3base.f0band\endcsname{0.20}
\expandafter\gdef\csname R@an.cv.amos.L3base.f0band.note\endcsname{two null SDs of this fold-0 difference, each the frozen default pool's training-seed SD of 0.122\,pp times $\sqrt{1/2 + 1/6}$ for the mean of two runs against the mean of the six-run pool: a locating band, not a test}
\expandafter\gdef\csname R@an.cv.amos.L3base.f0bandword\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.amos.L3base.f0gap\endcsname{0.13}
\expandafter\gdef\csname R@an.cv.amos.L3base.f0rev\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.cv.amos.L3base.f0se\endcsname{0.100}
\expandafter\gdef\csname R@an.cv.amos.L3base.f1\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.L3base.f2\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.amos.L3base.f3\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.amos.L3base.f4\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.cv.amos.L3base.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.cv.amos.L3base.lo\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.amos.L3base.loo.max\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.cv.amos.L3base.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.L3base.loo.min\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.amos.L3base.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.L3base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.L3base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.L3base.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.amos.L3base.share.word\endcsname{fold 4 alone carries 42\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.L3base.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.L3base.share_max\endcsname{42}
\expandafter\gdef\csname R@an.cv.amos.L3base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.L3base.span14\endcsname{0.42}
\expandafter\gdef\csname R@an.cv.amos.L3base.src0\endcsname{fresh s1-2 for HyReX and frozen pool for default}
\expandafter\gdef\csname R@an.cv.amos.L3base.src0mark\endcsname{b/a}
\expandafter\gdef\csname R@an.cv.amos.L3base.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.amos.P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.P3c.cbs.clause\endcsname{the function-identical control minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.04}\,pp, 95\,\% interval \ensuremath{-0.25} to \ensuremath{+0.17}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.amos.P3c.cbs.est\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.amos.P3c.cbs.hi\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.cv.amos.P3c.cbs.lo\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.amos.P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.P3c.f1\endcsname{88.77}
\expandafter\gdef\csname R@an.cv.amos.P3c.f2\endcsname{88.64}
\expandafter\gdef\csname R@an.cv.amos.P3c.f3\endcsname{88.52}
\expandafter\gdef\csname R@an.cv.amos.P3c.f4\endcsname{87.34}
\expandafter\gdef\csname R@an.cv.amos.P3c.max14\endcsname{88.77}
\expandafter\gdef\csname R@an.cv.amos.P3c.mean14\endcsname{88.32}
\expandafter\gdef\csname R@an.cv.amos.P3c.min14\endcsname{87.34}
\expandafter\gdef\csname R@an.cv.amos.P3c.params\endcsname{31.12}
\expandafter\gdef\csname R@an.cv.amos.P3c.params1\endcsname{31.1}
\expandafter\gdef\csname R@an.cv.amos.P3c.span14\endcsname{1.42}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.dcv\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.f1\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.f2\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.f3\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.f4\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.hi\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.lo\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.loo.max\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.loo.min\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.loo.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.loo.word\endcsname{changes sign when a single fold is dropped (two of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.share.word\endcsname{fold 1 alone carries 281\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.share_max\endcsname{281}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.span14\endcsname{0.70}
\expandafter\gdef\csname R@an.cv.amos.P3cbase.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.V5B1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V5B1.cbs.clause\endcsname{LeanAdd minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.46}\,pp, 95\,\% interval \ensuremath{-0.67} to \ensuremath{-0.25}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.amos.V5B1.cbs.est\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.cv.amos.V5B1.cbs.hi\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.amos.V5B1.cbs.lo\endcsname{\ensuremath{-0.67}}
\expandafter\gdef\csname R@an.cv.amos.V5B1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V5B1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B1.f1\endcsname{88.65}
\expandafter\gdef\csname R@an.cv.amos.V5B1.f2\endcsname{88.11}
\expandafter\gdef\csname R@an.cv.amos.V5B1.f3\endcsname{88.03}
\expandafter\gdef\csname R@an.cv.amos.V5B1.f4\endcsname{86.76}
\expandafter\gdef\csname R@an.cv.amos.V5B1.mean14\endcsname{87.89}
\expandafter\gdef\csname R@an.cv.amos.V5B1.params\endcsname{20.93}
\expandafter\gdef\csname R@an.cv.amos.V5B1.params1\endcsname{20.9}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.dcv\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.f1\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.f2\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.f3\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.f4\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.hi\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.lo\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.loo.max\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.loo.min\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.loo.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.loo.word\endcsname{changes sign when a single fold is dropped (two of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.share.word\endcsname{fold 1 alone carries 201\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.share_max\endcsname{201}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.span14\endcsname{0.37}
\expandafter\gdef\csname R@an.cv.amos.V5B1D2.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.cbs.clause\endcsname{LeanAdd minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.42}\,pp, 95\,\% interval \ensuremath{-0.61} to \ensuremath{-0.23}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.cbs.est\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.cbs.hi\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.cbs.lo\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.ctloffset\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.dcv\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.f1\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.f2\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.f3\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.f4\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.hi\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.lo\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.loo.max\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.loo.min\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.share.word\endcsname{fold 4 alone carries 34\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.share_max\endcsname{34}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.span14\endcsname{0.47}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.split\endcsname{LeanAdd minus the default is \ensuremath{-0.46}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.03}\,pp, so the margin over the function-identical control is \ensuremath{-0.43}\,pp}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.vsdefault\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c.word\endcsname{does not improve on it}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V5B1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.dcv\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.f1\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.f2\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.f3\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.f4\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.hi\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.lo\endcsname{\ensuremath{-0.82}}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.loo.max\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.loo.min\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.share.word\endcsname{fold 3 alone carries 42\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.share_max\endcsname{42}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.span14\endcsname{0.52}
\expandafter\gdef\csname R@an.cv.amos.V5B1base.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.V5B2.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V5B2.cbs.clause\endcsname{LeanAdd-NeXt minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.25}\,pp, 95\,\% interval \ensuremath{-0.47} to \ensuremath{-0.04}\,pp, which lies inside $\pm$0.50\,pp and below zero}
\expandafter\gdef\csname R@an.cv.amos.V5B2.cbs.est\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.amos.V5B2.cbs.hi\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.amos.V5B2.cbs.lo\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.cv.amos.V5B2.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V5B2.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B2.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B2.f1\endcsname{88.56}
\expandafter\gdef\csname R@an.cv.amos.V5B2.f2\endcsname{88.28}
\expandafter\gdef\csname R@an.cv.amos.V5B2.f3\endcsname{88.30}
\expandafter\gdef\csname R@an.cv.amos.V5B2.f4\endcsname{87.23}
\expandafter\gdef\csname R@an.cv.amos.V5B2.mean14\endcsname{88.09}
\expandafter\gdef\csname R@an.cv.amos.V5B2.params\endcsname{21.22}
\expandafter\gdef\csname R@an.cv.amos.V5B2.params1\endcsname{21.2}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.dcv\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.f1\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.f2\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.f3\endcsname{\ensuremath{-0.69}}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.f4\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.hi\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.lo\endcsname{\ensuremath{-0.85}}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.loo.max\endcsname{\ensuremath{-0.41}}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.loo.min\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.share.word\endcsname{fold 3 alone carries 36\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.share_max\endcsname{36}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.span14\endcsname{0.53}
\expandafter\gdef\csname R@an.cv.amos.V5B2L3.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.cbs.clause\endcsname{LeanAdd-NeXt minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.21}\,pp, 95\,\% interval \ensuremath{-0.40} to \ensuremath{-0.03}\,pp, which lies inside $\pm$0.50\,pp and below zero}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.cbs.est\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.cbs.hi\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.cbs.lo\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.ctloffset\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.dcv\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.f1\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.f2\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.f3\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.f4\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.hi\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.lo\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.loo.max\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.loo.min\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.share.word\endcsname{fold 2 alone carries 39\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.share_max\endcsname{39}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.span14\endcsname{0.24}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.split\endcsname{LeanAdd-NeXt minus the default is \ensuremath{-0.25}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.03}\,pp, so the margin over the function-identical control is \ensuremath{-0.22}\,pp}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.vsdefault\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c.word\endcsname{does not improve on it}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V5B2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.dcv\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.f1\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.f2\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.f3\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.f4\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.hi\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.lo\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.loo.max\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.loo.min\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.share.word\endcsname{fold 4 alone carries 57\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.share_max\endcsname{57}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.span14\endcsname{0.57}
\expandafter\gdef\csname R@an.cv.amos.V5B2V5B1.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.dcv\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.f1\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.f2\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.f3\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.f4\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.hi\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.lo\endcsname{\ensuremath{-0.83}}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.loo.max\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.loo.min\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.share.word\endcsname{fold 1 alone carries 55\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.share_max\endcsname{55}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.span14\endcsname{0.79}
\expandafter\gdef\csname R@an.cv.amos.V5B2base.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.cbs.clause\endcsname{HyReX-k9 minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.21}\,pp, 95\,\% interval \ensuremath{-0.03} to \ensuremath{+0.45}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.cbs.est\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.cbs.hi\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.cbs.lo\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.f1\endcsname{89.02}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.f2\endcsname{88.68}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.f3\endcsname{88.82}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.f4\endcsname{87.67}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.mean14\endcsname{88.55}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.params\endcsname{30.70}
\expandafter\gdef\csname R@an.cv.amos.V6A1r.params1\endcsname{30.7}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.dcv\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.f1\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.f2\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.f3\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.f4\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.hi\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.lo\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.loo.max\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.loo.min\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.loo.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.loo.word\endcsname{changes sign when a single fold is dropped (two of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.share.word\endcsname{fold 3 alone carries 155\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.share_max\endcsname{155}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.span14\endcsname{0.46}
\expandafter\gdef\csname R@an.cv.amos.V6A1rL3.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.cbs.clause\endcsname{HyReX-k9 minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.25}\,pp, 95\,\% interval \ensuremath{-0.01} to \ensuremath{+0.51}\,pp, which reaches just below zero}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.cbs.est\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.cbs.hi\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.cbs.lo\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.ctloffset\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.dcv\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.f1\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.f2\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.f3\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.f4\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.hi\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.lo\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.loo.max\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.loo.min\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.share.word\endcsname{fold 4 alone carries 36\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.share_max\endcsname{36}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.span14\endcsname{0.29}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.split\endcsname{HyReX-k9 minus the default is \ensuremath{+0.20}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.03}\,pp, so the margin over the function-identical control is \ensuremath{+0.23}\,pp}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.vsdefault\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c.word\endcsname{improves on the control in every fold}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V6A1rP3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.dcv\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.f1\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.f2\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.f3\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.f4\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.hi\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.lo\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.loo.max\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.loo.min\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.share.word\endcsname{fold 4 alone carries 84\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.share_max\endcsname{84}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.span14\endcsname{0.78}
\expandafter\gdef\csname R@an.cv.amos.V6A1rbase.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.amos.V7A1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V7A1.cbs.clause\endcsname{LeanDeepMid minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.26}\,pp, 95\,\% interval \ensuremath{+0.01} to \ensuremath{+0.52}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.amos.V7A1.cbs.est\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.amos.V7A1.cbs.hi\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.cv.amos.V7A1.cbs.lo\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.amos.V7A1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V7A1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7A1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7A1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7A1.f1\endcsname{88.96}
\expandafter\gdef\csname R@an.cv.amos.V7A1.f2\endcsname{88.99}
\expandafter\gdef\csname R@an.cv.amos.V7A1.f3\endcsname{88.66}
\expandafter\gdef\csname R@an.cv.amos.V7A1.f4\endcsname{87.80}
\expandafter\gdef\csname R@an.cv.amos.V7A1.mean14\endcsname{88.61}
\expandafter\gdef\csname R@an.cv.amos.V7A1.params\endcsname{31.00}
\expandafter\gdef\csname R@an.cv.amos.V7A1.params1\endcsname{31.0}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.cbs.clause\endcsname{LeanDeepMid minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.30}\,pp, 95\,\% interval \ensuremath{+0.07} to \ensuremath{+0.55}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.cbs.est\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.cbs.hi\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.cbs.lo\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.ctloffset\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.dcv\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.f1\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.f2\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.f3\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.f4\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.hi\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.lo\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.loo.max\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.loo.min\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.share.word\endcsname{fold 4 alone carries 40\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.share_max\endcsname{40}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.span14\endcsname{0.32}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.split\endcsname{LeanDeepMid minus the default is \ensuremath{+0.26}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.03}\,pp, so the margin over the function-identical control is \ensuremath{+0.29}\,pp}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.vsdefault\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c.word\endcsname{improves on the control in every fold}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7A1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.dcv\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.f1\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.f2\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.f3\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.f4\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.hi\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.lo\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.loo.max\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.loo.min\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.share.word\endcsname{fold 2 alone carries 35\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.share_max\endcsname{35}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.span14\endcsname{0.35}
\expandafter\gdef\csname R@an.cv.amos.V7A1V5B2.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.dcv\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.f1\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.f2\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.f3\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.f4\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.hi\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.lo\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.loo.max\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.loo.min\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.share.word\endcsname{fold 4 alone carries 78\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.share_max\endcsname{78}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.span14\endcsname{0.96}
\expandafter\gdef\csname R@an.cv.amos.V7A1base.word\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.cv.amos.V7A2.cbs.clause\endcsname{LeanDeepMid+FD minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.amos.V7A2.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7A2.params\endcsname{31.12}
\expandafter\gdef\csname R@an.cv.amos.V7A2.params1\endcsname{31.1}
\expandafter\gdef\csname R@an.cv.amos.V7A2P3c.cbs.clause\endcsname{LeanDeepMid+FD minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.amos.V7A2P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7A2P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7A2P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7A2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7A2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7A2V7A1.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7A2V7A1.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7A2base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7A2base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7B1.cbs.clause\endcsname{LeanSep minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.amos.V7B1.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B1.params\endcsname{20.40}
\expandafter\gdef\csname R@an.cv.amos.V7B1.params1\endcsname{20.4}
\expandafter\gdef\csname R@an.cv.amos.V7B1P3c.cbs.clause\endcsname{LeanSep minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.amos.V7B1P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B1P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B1P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7B1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7B1V5B2.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B1V5B2.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7B1base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B1base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7B2.cbs.clause\endcsname{LeanDil minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.amos.V7B2.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B2.params\endcsname{20.42}
\expandafter\gdef\csname R@an.cv.amos.V7B2.params1\endcsname{20.4}
\expandafter\gdef\csname R@an.cv.amos.V7B2P3c.cbs.clause\endcsname{LeanDil minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.amos.V7B2P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B2P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B2P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7B2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7B2V5B2.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B2V5B2.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7B2base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7B2base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7C1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V7C1.cbs.clause\endcsname{LeanNeXt-s5 minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.46}\,pp, 95\,\% interval \ensuremath{-0.68} to \ensuremath{-0.25}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.amos.V7C1.cbs.est\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.cv.amos.V7C1.cbs.hi\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.amos.V7C1.cbs.lo\endcsname{\ensuremath{-0.68}}
\expandafter\gdef\csname R@an.cv.amos.V7C1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V7C1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7C1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7C1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7C1.f1\endcsname{88.54}
\expandafter\gdef\csname R@an.cv.amos.V7C1.f2\endcsname{88.20}
\expandafter\gdef\csname R@an.cv.amos.V7C1.f3\endcsname{88.09}
\expandafter\gdef\csname R@an.cv.amos.V7C1.f4\endcsname{86.72}
\expandafter\gdef\csname R@an.cv.amos.V7C1.mean14\endcsname{87.89}
\expandafter\gdef\csname R@an.cv.amos.V7C1.params\endcsname{21.08}
\expandafter\gdef\csname R@an.cv.amos.V7C1.params1\endcsname{21.1}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.cbs.clause\endcsname{LeanNeXt-s5 minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.43}\,pp, 95\,\% interval \ensuremath{-0.63} to \ensuremath{-0.25}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.cbs.est\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.cbs.hi\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.cbs.lo\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.ctloffset\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.dcv\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.f1\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.f2\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.f3\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.f4\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.hi\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.lo\endcsname{\ensuremath{-0.69}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.loo.max\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.loo.min\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.share.word\endcsname{fold 4 alone carries 37\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.share_max\endcsname{37}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.span14\endcsname{0.40}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.split\endcsname{LeanNeXt-s5 minus the default is \ensuremath{-0.46}\,pp over the four folds; the control's own offset from the default is \ensuremath{-0.03}\,pp, so the margin over the function-identical control is \ensuremath{-0.43}\,pp}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.vsdefault\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c.word\endcsname{does not improve on it}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V7C1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.dcv\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.f1\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.f2\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.f3\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.f4\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.hi\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.lo\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.loo.max\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.loo.min\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.share.word\endcsname{fold 4 alone carries 62\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.share_max\endcsname{62}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.span14\endcsname{0.50}
\expandafter\gdef\csname R@an.cv.amos.V7C1V5B2.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.dcv\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.f1\endcsname{\ensuremath{-0.58}}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.f2\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.f3\endcsname{\ensuremath{-0.71}}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.f4\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.hi\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.lo\endcsname{\ensuremath{-0.81}}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.loo.max\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.loo.min\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.share.word\endcsname{fold 3 alone carries 39\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.share_max\endcsname{39}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.span14\endcsname{0.44}
\expandafter\gdef\csname R@an.cv.amos.V7C1base.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.amos.V8B2.cbs.clause\endcsname{Stem1 minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.amos.V8B2.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V8B2.params\endcsname{21.07}
\expandafter\gdef\csname R@an.cv.amos.V8B2.params1\endcsname{21.1}
\expandafter\gdef\csname R@an.cv.amos.V8B2P3c.cbs.clause\endcsname{Stem1 minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.amos.V8B2P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V8B2P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V8B2P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V8B2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V8B2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.V8B2base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.amos.V8B2base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.amos.base.f0\endcsname{87.70}
\expandafter\gdef\csname R@an.cv.amos.base.f1\endcsname{89.12}
\expandafter\gdef\csname R@an.cv.amos.base.f2\endcsname{88.48}
\expandafter\gdef\csname R@an.cv.amos.base.f3\endcsname{88.80}
\expandafter\gdef\csname R@an.cv.amos.base.f4\endcsname{87.00}
\expandafter\gdef\csname R@an.cv.amos.base.max14\endcsname{89.12}
\expandafter\gdef\csname R@an.cv.amos.base.mean14\endcsname{88.35}
\expandafter\gdef\csname R@an.cv.amos.base.mean5\endcsname{88.22}
\expandafter\gdef\csname R@an.cv.amos.base.min14\endcsname{87.00}
\expandafter\gdef\csname R@an.cv.amos.base.params\endcsname{31.12}
\expandafter\gdef\csname R@an.cv.amos.base.params1\endcsname{31.1}
\expandafter\gdef\csname R@an.cv.amos.base.span14\endcsname{2.12}
\expandafter\gdef\csname R@an.cv.amos.base.src0\endcsname{frozen pool}
\expandafter\gdef\csname R@an.cv.amos.base.src0long\endcsname{the frozen default pool}
\expandafter\gdef\csname R@an.cv.amos.base.src0mark\endcsname{a}
\expandafter\gdef\csname R@an.cv.amos.base.src0n\endcsname{6}
\expandafter\gdef\csname R@an.cv.amos.recovery.L3\endcsname{0.56}
\expandafter\gdef\csname R@an.cv.amos.recovery.L3.method\endcsname{the delta method applied to the two four-fold mean margins, HyReX minus the default and ResEnc-M minus the default, which are differences from the same default runs, so their covariance over the folds enters the variance of the ratio; the interval takes the t quantile on three degrees of freedom of the registered paired-t intervals of the margins; it is descriptive, a description of four folds of one seed each and not a test, and it is withheld when ResEnc-M's own interval over the folds includes zero}
\expandafter\gdef\csname R@an.cv.amos.recovery.L3.sentence\endcsname{On AMOS22, HyReX's mean margin over the default on the four folds that entered no decision, \ensuremath{+0.23}\,pp, is 0.56 of ResEnc-M's, \ensuremath{+0.41}\,pp; ResEnc-M's own interval over the folds includes zero, so the ratio is given without an interval}
\expandafter\gdef\csname R@an.cv.amos.recovery.L3.state\endcsname{interval withheld}
\expandafter\gdef\csname R@an.cv.band.acdc.D2base.word\endcsname{\leavevmode\pend}
\expandafter\gdef\csname R@an.cv.band.acdc.L1base.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.band.acdc.L3L1.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.band.acdc.L3base.word\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.band.acdc.hw\endcsname{0.28}
\expandafter\gdef\csname R@an.cv.band.amos.D2base.word\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.band.amos.L1base.word\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.band.amos.L3L1.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.band.amos.L3base.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.band.amos.hw\endcsname{0.35}
\expandafter\gdef\csname R@an.cv.band.kits.D2base.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.band.kits.L1base.word\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.band.kits.L3L1.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.band.kits.L3base.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.band.kits.hw\endcsname{2.25}
\expandafter\gdef\csname R@an.cv.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.cbs.arms\endcsname{L3, L1, D2, P3c, L1b, V5B1, V5B2, V6A1r, V7A1, V7C1, V7B1, V7B2, V7A2, V8B2}
\expandafter\gdef\csname R@an.cv.cbs.label\endcsname{case-level paired bootstrap}
\expandafter\gdef\csname R@an.cv.cbs.method\endcsname{the unit is the validation case of folds 1 to 4 (every case once), the difference of an arm and its reference is averaged over the seeds available for the arm and its reference in the fold, and the interval is the percentile 95\,\% interval of the mean difference over 10000 resamples of the cases with replacement, stratified by fold, with random-number seed 20261011}
\expandafter\gdef\csname R@an.cv.cbs.n\endcsname{58}
\expandafter\gdef\csname R@an.cv.cbs.note\endcsname{the case-level interval carries case-sampling variance and the averaging over the seeds available for the arm and its reference, not the training-seed variance of a one-seed fold}
\expandafter\gdef\csname R@an.cv.cbs.reference\endcsname{the reference of a contrast is the nnU-Net default, or the function-identical rebuild, trained on the same fold (its cross-validation runs, seeds as available), not a pooled reference}
\expandafter\gdef\csname R@an.cv.cbs.registration\endcsname{Addendum AZ2}
\expandafter\gdef\csname R@an.cv.cbs.seed\endcsname{20261011}
\expandafter\gdef\csname R@an.cv.cbs.total\endcsname{78}
\expandafter\gdef\csname R@an.cv.ci.df\endcsname{3}
\expandafter\gdef\csname R@an.cv.ci.level\endcsname{95\,\%}
\expandafter\gdef\csname R@an.cv.claim.breadth.acdc\endcsname{On ACDC the HyReX-minus-default contrast is carried by the cohort and not by a handful of cases}
\expandafter\gdef\csname R@an.cv.claim.breadth.amos\endcsname{On AMOS22 the HyReX-minus-default contrast is carried by the cohort and not by a handful of cases}
\expandafter\gdef\csname R@an.cv.claim.breadth.def\endcsname{more than 50\,\% of the held-out cases improve and the 10 largest gains carry at most 25\,\% of all gains}
\expandafter\gdef\csname R@an.cv.claim.breadth.kits\endcsname{On KiTS23 the HyReX-minus-default contrast is carried by the cohort and not by a handful of cases}
\expandafter\gdef\csname R@an.cv.claim.repro.acdc\endcsname{On ACDC our ResEnc-M five-fold margin reproduces the published margin to within 1.00\,pp}
\expandafter\gdef\csname R@an.cv.claim.repro.amos\endcsname{On AMOS22 our ResEnc-M five-fold margin reproduces the published margin to within 1.00\,pp}
\expandafter\gdef\csname R@an.cv.claim.repro.def\endcsname{the five-fold ResEnc-M margin over the default differs from the published ResEnc-M margin by at most 1.00\,pp, a tolerance that is smaller than the published margin itself (a tolerance that is not would also hold for a margin of zero, and a sentence that holds whatever was measured reproduces nothing)}
\expandafter\gdef\csname R@an.cv.claim.repro.kits\endcsname{On KiTS23 our ResEnc-M five-fold margin reproduces the published margin to within 1.00\,pp}
\expandafter\gdef\csname R@an.cv.ctl.acdc.narms\endcsname{11}
\expandafter\gdef\csname R@an.cv.ctl.acdc.nready\endcsname{7}
\expandafter\gdef\csname R@an.cv.ctl.acdc.nready3\endcsname{0}
\expandafter\gdef\csname R@an.cv.ctl.amos.narms\endcsname{11}
\expandafter\gdef\csname R@an.cv.ctl.amos.nready\endcsname{7}
\expandafter\gdef\csname R@an.cv.ctl.amos.nready3\endcsname{0}
\expandafter\gdef\csname R@an.cv.ctl.kits.narms\endcsname{11}
\expandafter\gdef\csname R@an.cv.ctl.kits.nready\endcsname{9}
\expandafter\gdef\csname R@an.cv.ctl.kits.nready3\endcsname{0}
\expandafter\gdef\csname R@an.cv.ctl.label\endcsname{margin over the function-identical control}
\expandafter\gdef\csname R@an.cv.ctl.n\endcsname{11}
\expandafter\gdef\csname R@an.cv.ctl.names\endcsname{ResEnc-M, LeanDec, LeanAdd, LeanAdd-NeXt, HyReX-k9, LeanDeepMid, LeanNeXt-s5, LeanSep, LeanDil, LeanDeepMid+FD and Stem1}
\expandafter\gdef\csname R@an.cv.ctl.registration\endcsname{Addendum AV}
\expandafter\gdef\csname R@an.cv.ctl.seeds.n\endcsname{0}
\expandafter\gdef\csname R@an.cv.ctl.seeds.sentence\endcsname{the control's seed-1 and seed-2 runs of the cross-validation folds: none of the 24 have finished, so the secondary reading is pending}
\expandafter\gdef\csname R@an.cv.ctl.seeds.state\endcsname{pending}
\expandafter\gdef\csname R@an.cv.ctl.seeds.total\endcsname{24}
\expandafter\gdef\csname R@an.cv.ctl.tags\endcsname{L1, D2, V5B1, V5B2, V6A1r, V7A1, V7C1, V7B1, V7B2, V7A2, V8B2}
\expandafter\gdef\csname R@an.cv.cvseeds\endcsname{one}
\expandafter\gdef\csname R@an.cv.cvseeds.phrase\endcsname{one seed per arm}
\expandafter\gdef\csname R@an.cv.d5.src0\endcsname{AMOS22 HyReX fresh s1-2 (b); AMOS22 default frozen pool (a); AMOS22 ResEnc-M fresh s1-2 (b); AMOS22 LeanDec seed 0 (c); KiTS23 HyReX fresh s1-2 (b); KiTS23 default frozen pool (a); KiTS23 ResEnc-M fresh s1-2 (b); KiTS23 LeanDec fresh s1-2 (b); ACDC HyReX fresh s1-2 (b); ACDC default frozen pool (a); ACDC ResEnc-M fresh s1-2 (b)}
\expandafter\gdef\csname R@an.cv.d5.src0note\endcsname{the five-fold means published here do NOT all take their fold-0 fifth from the same estimand: fifth, so their fold-0 LeanDec enters from seed 0 on AMOS22, fresh s1-2 on KiTS23s are not like-for-like across datasets}
\expandafter\gdef\csname R@an.cv.decomp.acdc.clause\endcsname{On ACDC, HyReX minus the default is \ensuremath{+0.33}\,pp (95\,\% over folds \ensuremath{+0.10} to \ensuremath{+0.56}, which lies above zero; improves in every fold), and splits into the control's own offset, the function-identical control minus the default, of \ensuremath{-0.08}\,pp (95\,\% over folds \ensuremath{-0.22} to \ensuremath{+0.06}, which lies inside $\pm$0.50\,pp; does not improve in cross-validation) and a design margin over the control, HyReX minus the function-identical control, of \ensuremath{+0.41}\,pp (95\,\% over folds \ensuremath{+0.06} to \ensuremath{+0.76}, which lies above zero; improves in every fold); the two parts add to the registered contrast in every fold}
\expandafter\gdef\csname R@an.cv.decomp.acdc.done\endcsname{4}
\expandafter\gdef\csname R@an.cv.decomp.acdc.everyfold\endcsname{positive in every fold: HyReX minus the default and the design margin over the control}
\expandafter\gdef\csname R@an.cv.decomp.acdc.short\endcsname{ACDC: HyReX minus the default is \ensuremath{+0.33}\,pp and splits into the control's offset of \ensuremath{-0.08}\,pp and a design margin of \ensuremath{+0.41}\,pp}
\expandafter\gdef\csname R@an.cv.decomp.acdc.state\endcsname{complete}
\expandafter\gdef\csname R@an.cv.decomp.amos.clause\endcsname{On AMOS22, HyReX minus the default is \ensuremath{+0.23}\,pp (95\,\% over folds \ensuremath{-0.08} to \ensuremath{+0.54}, which includes zero; improves on average (3/4 folds)), and splits into the control's own offset, the function-identical control minus the default, of \ensuremath{-0.03}\,pp (95\,\% over folds \ensuremath{-0.57} to \ensuremath{+0.51}, which includes zero; does not improve in cross-validation) and a design margin over the control, HyReX minus the function-identical control, of \ensuremath{+0.26}\,pp (95\,\% over folds \ensuremath{-0.03} to \ensuremath{+0.55}, which reaches just below zero; improves in every fold); the two parts add to the registered contrast in every fold}
\expandafter\gdef\csname R@an.cv.decomp.amos.done\endcsname{4}
\expandafter\gdef\csname R@an.cv.decomp.amos.everyfold\endcsname{positive in every fold: the design margin over the control}
\expandafter\gdef\csname R@an.cv.decomp.amos.short\endcsname{AMOS22: HyReX minus the default is \ensuremath{+0.23}\,pp and splits into the control's offset of \ensuremath{-0.03}\,pp and a design margin of \ensuremath{+0.26}\,pp}
\expandafter\gdef\csname R@an.cv.decomp.amos.state\endcsname{complete}
\expandafter\gdef\csname R@an.cv.decomp.kits.clause\endcsname{On KiTS23, HyReX minus the default is \ensuremath{+0.68}\,pp (95\,\% over folds \ensuremath{-1.08} to \ensuremath{+2.44}, which includes zero; improves on average (3/4 folds)), and splits into the control's own offset, the function-identical control minus the default, of \ensuremath{+0.56}\,pp (95\,\% over folds \ensuremath{-1.71} to \ensuremath{+2.82}, which includes zero; improves on average (3/4 folds)) and a design margin over the control, HyReX minus the function-identical control, of \ensuremath{+0.12}\,pp (95\,\% over folds \ensuremath{-0.73} to \ensuremath{+0.98}, which includes zero; improves on average (2/4 folds)); the two parts add to the registered contrast in every fold}
\expandafter\gdef\csname R@an.cv.decomp.kits.done\endcsname{4}
\expandafter\gdef\csname R@an.cv.decomp.kits.everyfold\endcsname{none of the three differences is positive in every fold}
\expandafter\gdef\csname R@an.cv.decomp.kits.short\endcsname{KiTS23: HyReX minus the default is \ensuremath{+0.68}\,pp and splits into the control's offset of \ensuremath{+0.56}\,pp and a design margin of \ensuremath{+0.12}\,pp}
\expandafter\gdef\csname R@an.cv.decomp.kits.state\endcsname{complete}
\expandafter\gdef\csname R@an.cv.decomp.refnote\endcsname{The registered contrast and both of its parts are differences of two runs trained and scored on the same cases of the same fold, so no frozen default pool and no sensitivity reference enters them}
\expandafter\gdef\csname R@an.cv.decompre.acdc.clause\endcsname{On ACDC, ResEnc-M minus HyReX is \ensuremath{+0.04}\,pp (95\,\% over folds \ensuremath{-0.24} to \ensuremath{+0.31}, which lies inside $\pm$0.50\,pp; improves on average (2/4 folds)), and splits into a re-implementation difference, ResEnc-M minus the ResEnc-matched re-implementation, of \ensuremath{+0.18}\,pp (95\,\% over folds \ensuremath{+0.02} to \ensuremath{+0.33}, which lies inside $\pm$0.50\,pp and above zero; improves in every fold) and a like-for-like part, the ResEnc-matched re-implementation minus HyReX, of \ensuremath{-0.14}\,pp (95\,\% over folds \ensuremath{-0.27} to \ensuremath{-0.01}, which lies inside $\pm$0.50\,pp and below zero; does not improve in cross-validation); the two parts add to the registered contrast in every fold}
\expandafter\gdef\csname R@an.cv.decompre.acdc.done\endcsname{4}
\expandafter\gdef\csname R@an.cv.decompre.acdc.short\endcsname{ACDC: ResEnc-M minus HyReX is \ensuremath{+0.04}\,pp and splits into a re-implementation difference of \ensuremath{+0.18}\,pp and a like-for-like part of \ensuremath{-0.14}\,pp}
\expandafter\gdef\csname R@an.cv.decompre.acdc.state\endcsname{complete}
\expandafter\gdef\csname R@an.cv.decompre.amos.clause\endcsname{On AMOS22, ResEnc-M minus HyReX is \ensuremath{+0.18}\,pp (95\,\% over folds \ensuremath{-0.40} to \ensuremath{+0.76}, which includes zero; improves on average (3/4 folds)), and splits into a re-implementation difference, ResEnc-M minus the ResEnc-matched re-implementation, of \ensuremath{-0.02}\,pp (95\,\% over folds \ensuremath{-0.28} to \ensuremath{+0.24}, which lies inside $\pm$0.50\,pp; does not improve in cross-validation) and a like-for-like part, the ResEnc-matched re-implementation minus HyReX, of \ensuremath{+0.20}\,pp (95\,\% over folds \ensuremath{-0.38} to \ensuremath{+0.78}, which includes zero; improves on average (3/4 folds)); the two parts add to the registered contrast in every fold}
\expandafter\gdef\csname R@an.cv.decompre.amos.done\endcsname{4}
\expandafter\gdef\csname R@an.cv.decompre.amos.short\endcsname{AMOS22: ResEnc-M minus HyReX is \ensuremath{+0.18}\,pp and splits into a re-implementation difference of \ensuremath{-0.02}\,pp and a like-for-like part of \ensuremath{+0.20}\,pp}
\expandafter\gdef\csname R@an.cv.decompre.amos.state\endcsname{complete}
\expandafter\gdef\csname R@an.cv.decompre.kits.clause\endcsname{On KiTS23, ResEnc-M minus HyReX is \ensuremath{+1.47}\,pp (95\,\% over folds \ensuremath{-0.24} to \ensuremath{+3.17}, which includes zero; improves in every fold), and splits into a re-implementation difference, ResEnc-M minus the ResEnc-matched re-implementation, of \ensuremath{+0.60}\,pp (95\,\% over folds \ensuremath{-0.45} to \ensuremath{+1.66}, which includes zero; improves on average (3/4 folds)) and a like-for-like part, the ResEnc-matched re-implementation minus HyReX, of \ensuremath{+0.86}\,pp (95\,\% over folds \ensuremath{-0.10} to \ensuremath{+1.82}, which includes zero; improves in every fold); the two parts add to the registered contrast in every fold}
\expandafter\gdef\csname R@an.cv.decompre.kits.done\endcsname{4}
\expandafter\gdef\csname R@an.cv.decompre.kits.short\endcsname{KiTS23: ResEnc-M minus HyReX is \ensuremath{+1.47}\,pp and splits into a re-implementation difference of \ensuremath{+0.60}\,pp and a like-for-like part of \ensuremath{+0.86}\,pp}
\expandafter\gdef\csname R@an.cv.decompre.kits.state\endcsname{complete}
\expandafter\gdef\csname R@an.cv.decompre.refnote\endcsname{The registered contrast and both of its parts are differences of two runs trained and scored on the same cases of the same fold, so no frozen default pool and no sensitivity reference enters them}
\expandafter\gdef\csname R@an.cv.decompre.why\endcsname{ResEnc-M is the stock library network and HyReX is a plan-aware build, and the ResEnc-matched re-implementation (built through the plan-aware path; it differs from the library preset in the default stem, the shortcut form and the zero-initialisation) splits their registered contrast into a re-implementation difference, ResEnc-M minus the re-implementation, and a like-for-like part, the re-implementation minus HyReX}
\expandafter\gdef\csname R@an.cv.fold.fifth\endcsname{fifth}
\expandafter\gdef\csname R@an.cv.fold0.share\endcsname{one fifth}
\expandafter\gdef\csname R@an.cv.gate.sent1\endcsname{writable today: all 14 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent10\endcsname{writable today: all 7 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent11\endcsname{writable today: all 8 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent12\endcsname{writable today: all 5 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent13\endcsname{writable today: all 3 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent14\endcsname{writable today: all 1 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent2\endcsname{writable today: all 5 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent3\endcsname{writable today: all 6 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent4\endcsname{writable today: all 6 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent5\endcsname{writable today: all 16 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent6\endcsname{writable today: all 4 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent6c\endcsname{writable today: all 1 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent7\endcsname{writable today: all 6 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent8\endcsname{writable today: all 8 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sent9\endcsname{writable today: all 8 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sentTfolds\endcsname{writable today: all 4 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sentToof\endcsname{writable today: all 1 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sentTp3c\endcsname{writable today: all 4 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sentTpositioning\endcsname{writable today: all 6 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.sentTrobust\endcsname{writable today: all 6 macros it names are emitted}
\expandafter\gdef\csname R@an.cv.gate.summary\endcsname{20 of the 20 proposed sentences of the cv note are writable today (sentence 1, sentence 2, sentence 3, sentence 4, sentence 5, sentence 6, sentence 6c, sentence 7, sentence 8, sentence 9, sentence 10, sentence 11, sentence 12, sentence 13, sentence 14, takeaway folds, takeaway oof, takeaway p3c, takeaway positioning, takeaway robust)}
\expandafter\gdef\csname R@an.cv.hetero.acdc.D2base.casese\endcsname{0.13}
\expandafter\gdef\csname R@an.cv.hetero.acdc.D2base.ratio\endcsname{0.18}
\expandafter\gdef\csname R@an.cv.hetero.acdc.D2base.sdfold\endcsname{0.08}
\expandafter\gdef\csname R@an.cv.hetero.acdc.D2base.seedexp\endcsname{0.14}
\expandafter\gdef\csname R@an.cv.hetero.acdc.D2base.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L1base.casese\endcsname{0.18}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L1base.ratio\endcsname{0.09}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L1base.sdfold\endcsname{0.07}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L1base.seedexp\endcsname{0.14}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L1base.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3L1.casese\endcsname{0.15}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3L1.ratio\endcsname{0.72}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3L1.sdfold\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3L1.seedexp\endcsname{0.14}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3L1.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3base.casese\endcsname{0.15}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3base.ratio\endcsname{0.50}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3base.sdfold\endcsname{0.14}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3base.seedexp\endcsname{0.14}
\expandafter\gdef\csname R@an.cv.hetero.acdc.L3base.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.amos.D2base.casese\endcsname{0.14}
\expandafter\gdef\csname R@an.cv.hetero.amos.D2base.ratio\endcsname{0.77}
\expandafter\gdef\csname R@an.cv.hetero.amos.D2base.sdfold\endcsname{0.20}
\expandafter\gdef\csname R@an.cv.hetero.amos.D2base.seedexp\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.hetero.amos.D2base.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.amos.L1base.casese\endcsname{0.16}
\expandafter\gdef\csname R@an.cv.hetero.amos.L1base.ratio\endcsname{3.24}
\expandafter\gdef\csname R@an.cv.hetero.amos.L1base.sdfold\endcsname{0.43}
\expandafter\gdef\csname R@an.cv.hetero.amos.L1base.seedexp\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.hetero.amos.L1base.verdict\endcsname{adds spread beyond one seed per arm and case sampling}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3L1.casese\endcsname{0.14}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3L1.ratio\endcsname{2.63}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3L1.sdfold\endcsname{0.36}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3L1.seedexp\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3L1.verdict\endcsname{adds spread beyond one seed per arm and case sampling}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3base.casese\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3base.ratio\endcsname{0.62}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3base.sdfold\endcsname{0.19}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3base.seedexp\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.hetero.amos.L3base.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.kits.D2base.casese\endcsname{0.74}
\expandafter\gdef\csname R@an.cv.hetero.kits.D2base.ratio\endcsname{0.25}
\expandafter\gdef\csname R@an.cv.hetero.kits.D2base.sdfold\endcsname{0.68}
\expandafter\gdef\csname R@an.cv.hetero.kits.D2base.seedexp\endcsname{1.12}
\expandafter\gdef\csname R@an.cv.hetero.kits.D2base.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.kits.L1base.casese\endcsname{0.86}
\expandafter\gdef\csname R@an.cv.hetero.kits.L1base.ratio\endcsname{0.27}
\expandafter\gdef\csname R@an.cv.hetero.kits.L1base.sdfold\endcsname{0.74}
\expandafter\gdef\csname R@an.cv.hetero.kits.L1base.seedexp\endcsname{1.12}
\expandafter\gdef\csname R@an.cv.hetero.kits.L1base.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3L1.casese\endcsname{0.90}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3L1.ratio\endcsname{0.55}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3L1.sdfold\endcsname{1.07}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3L1.seedexp\endcsname{1.12}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3L1.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3base.casese\endcsname{0.84}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3base.ratio\endcsname{0.62}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3base.sdfold\endcsname{1.11}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3base.seedexp\endcsname{1.12}
\expandafter\gdef\csname R@an.cv.hetero.kits.L3base.verdict\endcsname{is smaller than one seed per arm and case sampling already predict}
\expandafter\gdef\csname R@an.cv.hetero.premise\endcsname{$\sqrt{2}\times$ the training-seed SD of that dataset's frozen DEFAULT pool, applied to each arm of the contrast: the frozen default pool is the registered source of a training-seed SD, so the same expectation is used for every contrast of a dataset, HyReX $-$ ResEnc-M included, where neither arm is the default}
\expandafter\gdef\csname R@an.cv.kfold\endcsname{five-fold}
\expandafter\gdef\csname R@an.cv.kits.D2.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.D2.cbs.clause\endcsname{LeanDec minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+1.05}\,pp, 95\,\% interval \ensuremath{+0.32} to \ensuremath{+1.79}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.kits.D2.cbs.est\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.cv.kits.D2.cbs.hi\endcsname{\ensuremath{+1.79}}
\expandafter\gdef\csname R@an.cv.kits.D2.cbs.lo\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.cv.kits.D2.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.D2.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.D2.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.D2.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.D2.f0\endcsname{85.27}
\expandafter\gdef\csname R@an.cv.kits.D2.f1\endcsname{84.58}
\expandafter\gdef\csname R@an.cv.kits.D2.f2\endcsname{84.62}
\expandafter\gdef\csname R@an.cv.kits.D2.f3\endcsname{87.94}
\expandafter\gdef\csname R@an.cv.kits.D2.f4\endcsname{83.01}
\expandafter\gdef\csname R@an.cv.kits.D2.max14\endcsname{87.94}
\expandafter\gdef\csname R@an.cv.kits.D2.mean14\endcsname{85.04}
\expandafter\gdef\csname R@an.cv.kits.D2.mean5\endcsname{85.08}
\expandafter\gdef\csname R@an.cv.kits.D2.min14\endcsname{83.01}
\expandafter\gdef\csname R@an.cv.kits.D2.params\endcsname{26.08}
\expandafter\gdef\csname R@an.cv.kits.D2.params1\endcsname{26.1}
\expandafter\gdef\csname R@an.cv.kits.D2.span14\endcsname{4.93}
\expandafter\gdef\csname R@an.cv.kits.D2.src0\endcsname{fresh s1-2}
\expandafter\gdef\csname R@an.cv.kits.D2.src0long\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.cv.kits.D2.src0mark\endcsname{b}
\expandafter\gdef\csname R@an.cv.kits.D2.src0n\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.cbs.clause\endcsname{LeanDec minus the function-identical control, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.48}\,pp, 95\,\% interval \ensuremath{-0.33} to \ensuremath{+1.29}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.cbs.est\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.cbs.hi\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.cbs.lo\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.ctloffset\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.dcv\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.f1\endcsname{\ensuremath{-0.67}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.f2\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.f3\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.f4\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.hi\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.lo\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.loo.max\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.loo.min\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.share.word\endcsname{fold 2 alone carries 62\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.share_max\endcsname{62}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.span14\endcsname{1.88}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.split\endcsname{LeanDec minus the default is \ensuremath{+1.04}\,pp over the four folds; the control's own offset from the default is \ensuremath{+0.56}\,pp, so the margin over the function-identical control is \ensuremath{+0.49}\,pp}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.vsdefault\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@an.cv.kits.D2P3c.word\endcsname{improves on it on average (3 of 4 folds)}
\expandafter\gdef\csname R@an.cv.kits.D2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.D2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.D2base.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.kits.D2base.boot.casewidth\endcsname{1.40}
\expandafter\gdef\csname R@an.cv.kits.D2base.boot.foldwidth\endcsname{2.15}
\expandafter\gdef\csname R@an.cv.kits.D2base.boot.hi\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.cv.kits.D2base.boot.lo\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.kits.D2base.boot.mean\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.cv.kits.D2base.boot.n\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.D2base.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.kits.D2base.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.36} to \ensuremath{+1.76}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.kits.D2base.d5\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.cv.kits.D2base.d5alt\endcsname{\ensuremath{+1.16}}
\expandafter\gdef\csname R@an.cv.kits.D2base.dcv\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@an.cv.kits.D2base.f0\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.cv.kits.D2base.f0alt\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.cv.kits.D2base.f0band\endcsname{1.45}
\expandafter\gdef\csname R@an.cv.kits.D2base.f0band.note\endcsname{two null SDs of this fold-0 difference, each the frozen default pool's training-seed SD of 0.795\,pp times $\sqrt{1/2 + 1/3}$ for the mean of two runs against the mean of the three-run pool: a locating band, not a test}
\expandafter\gdef\csname R@an.cv.kits.D2base.f0bandword\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.kits.D2base.f0gap\endcsname{1.89}
\expandafter\gdef\csname R@an.cv.kits.D2base.f0rev\endcsname{\ensuremath{-1.89}}
\expandafter\gdef\csname R@an.cv.kits.D2base.f0se\endcsname{0.726}
\expandafter\gdef\csname R@an.cv.kits.D2base.f1\endcsname{\ensuremath{+1.72}}
\expandafter\gdef\csname R@an.cv.kits.D2base.f2\endcsname{\ensuremath{+1.31}}
\expandafter\gdef\csname R@an.cv.kits.D2base.f3\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.cv.kits.D2base.f4\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.kits.D2base.hi\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.cv.kits.D2base.lo\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.kits.D2base.loo.max\endcsname{\ensuremath{+1.35}}
\expandafter\gdef\csname R@an.cv.kits.D2base.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.D2base.loo.min\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.cv.kits.D2base.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.D2base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.D2base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.D2base.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.D2base.share.word\endcsname{fold 1 alone carries 41\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.D2base.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.D2base.share_max\endcsname{41}
\expandafter\gdef\csname R@an.cv.kits.D2base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.D2base.span14\endcsname{1.60}
\expandafter\gdef\csname R@an.cv.kits.D2base.src0\endcsname{fresh s1-2 for LeanDec and frozen pool for default}
\expandafter\gdef\csname R@an.cv.kits.D2base.src0mark\endcsname{b/a}
\expandafter\gdef\csname R@an.cv.kits.D2base.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.kits.L1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.L1.cbs.clause\endcsname{ResEnc-M minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+2.15}\,pp, 95\,\% interval \ensuremath{+1.28} to \ensuremath{+3.06}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.kits.L1.cbs.est\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.cv.kits.L1.cbs.hi\endcsname{\ensuremath{+3.06}}
\expandafter\gdef\csname R@an.cv.kits.L1.cbs.lo\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.cv.kits.L1.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.L1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.L1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L1.f0\endcsname{86.85}
\expandafter\gdef\csname R@an.cv.kits.L1.f1\endcsname{85.44}
\expandafter\gdef\csname R@an.cv.kits.L1.f2\endcsname{86.25}
\expandafter\gdef\csname R@an.cv.kits.L1.f3\endcsname{88.27}
\expandafter\gdef\csname R@an.cv.kits.L1.f4\endcsname{84.60}
\expandafter\gdef\csname R@an.cv.kits.L1.max14\endcsname{88.27}
\expandafter\gdef\csname R@an.cv.kits.L1.mean14\endcsname{86.14}
\expandafter\gdef\csname R@an.cv.kits.L1.mean5\endcsname{86.28}
\expandafter\gdef\csname R@an.cv.kits.L1.min14\endcsname{84.60}
\expandafter\gdef\csname R@an.cv.kits.L1.params\endcsname{102.35}
\expandafter\gdef\csname R@an.cv.kits.L1.params1\endcsname{102.4}
\expandafter\gdef\csname R@an.cv.kits.L1.span14\endcsname{3.66}
\expandafter\gdef\csname R@an.cv.kits.L1.src0\endcsname{fresh s1-2}
\expandafter\gdef\csname R@an.cv.kits.L1.src0long\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.cv.kits.L1.src0mark\endcsname{b}
\expandafter\gdef\csname R@an.cv.kits.L1.src0n\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.dcv\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.f1\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.f2\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.f3\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.f4\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.hi\endcsname{\ensuremath{+1.66}}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.lo\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.loo.max\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.loo.min\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.share.word\endcsname{fold 2 alone carries 53\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.share_max\endcsname{53}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.span14\endcsname{1.41}
\expandafter\gdef\csname R@an.cv.kits.L1L1b.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.kits.L1L3.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.kits.L1L3.boot.casewidth\endcsname{1.84}
\expandafter\gdef\csname R@an.cv.kits.L1L3.boot.foldwidth\endcsname{3.41}
\expandafter\gdef\csname R@an.cv.kits.L1L3.boot.hi\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.boot.lo\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.boot.mean\endcsname{\ensuremath{+1.46}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.boot.n\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.L1L3.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.kits.L1L3.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.52} to \ensuremath{+2.36}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.kits.L1L3.dcv\endcsname{\ensuremath{+1.47}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.f1\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.f2\endcsname{\ensuremath{+2.74}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.f3\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.f4\endcsname{\ensuremath{+1.87}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.hi\endcsname{\ensuremath{+3.17}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.lo\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.loo.max\endcsname{\ensuremath{+1.86}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L1L3.loo.min\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@an.cv.kits.L1L3.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1L3.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L1L3.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.L1L3.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L1L3.share.word\endcsname{fold 2 alone carries 47\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.L1L3.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1L3.share_max\endcsname{47}
\expandafter\gdef\csname R@an.cv.kits.L1L3.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.L1L3.span14\endcsname{2.47}
\expandafter\gdef\csname R@an.cv.kits.L1L3.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.cbs.clause\endcsname{ResEnc-M minus the function-identical control, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+1.59}\,pp, 95\,\% interval \ensuremath{+0.68} to \ensuremath{+2.52}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.cbs.est\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.cbs.hi\endcsname{\ensuremath{+2.52}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.cbs.lo\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.ctloffset\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.dcv\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.f1\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.f2\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.f3\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.f4\endcsname{\ensuremath{+2.73}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.hi\endcsname{\ensuremath{+3.80}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.lo\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.loo.max\endcsname{\ensuremath{+2.05}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.loo.min\endcsname{\ensuremath{+1.17}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.share.word\endcsname{fold 2 alone carries 45\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.share_max\endcsname{45}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.span14\endcsname{2.64}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.split\endcsname{ResEnc-M minus the default is \ensuremath{+2.15}\,pp over the four folds; the control's own offset from the default is \ensuremath{+0.56}\,pp, so the margin over the function-identical control is \ensuremath{+1.59}\,pp}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.vsdefault\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.cv.kits.L1P3c.word\endcsname{improves on the control in every fold}
\expandafter\gdef\csname R@an.cv.kits.L1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.L1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.L1b.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.L1b.cbs.clause\endcsname{ResEnc-matched minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+1.55}\,pp, 95\,\% interval \ensuremath{+0.66} to \ensuremath{+2.42}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.kits.L1b.cbs.est\endcsname{\ensuremath{+1.55}}
\expandafter\gdef\csname R@an.cv.kits.L1b.cbs.hi\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.cv.kits.L1b.cbs.lo\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.cv.kits.L1b.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.L1b.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.L1b.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L1b.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L1b.f1\endcsname{85.21}
\expandafter\gdef\csname R@an.cv.kits.L1b.f2\endcsname{84.96}
\expandafter\gdef\csname R@an.cv.kits.L1b.f3\endcsname{88.40}
\expandafter\gdef\csname R@an.cv.kits.L1b.f4\endcsname{83.58}
\expandafter\gdef\csname R@an.cv.kits.L1b.mean14\endcsname{85.54}
\expandafter\gdef\csname R@an.cv.kits.L1b.params\endcsname{102.43}
\expandafter\gdef\csname R@an.cv.kits.L1b.params1\endcsname{102.4}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.dcv\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.f1\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.f2\endcsname{\ensuremath{+1.46}}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.f3\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.f4\endcsname{\ensuremath{+0.84}}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.hi\endcsname{\ensuremath{+1.82}}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.lo\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.loo.max\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.loo.min\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.share.word\endcsname{fold 2 alone carries 42\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.share_max\endcsname{42}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.span14\endcsname{1.41}
\expandafter\gdef\csname R@an.cv.kits.L1bL3.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.kits.L1base.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.kits.L1base.boot.casewidth\endcsname{1.80}
\expandafter\gdef\csname R@an.cv.kits.L1base.boot.foldwidth\endcsname{2.34}
\expandafter\gdef\csname R@an.cv.kits.L1base.boot.hi\endcsname{\ensuremath{+3.08}}
\expandafter\gdef\csname R@an.cv.kits.L1base.boot.lo\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.cv.kits.L1base.boot.mean\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.cv.kits.L1base.boot.n\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.L1base.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.kits.L1base.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+1.28} to \ensuremath{+3.08}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.kits.L1base.d5\endcsname{\ensuremath{+2.41}}
\expandafter\gdef\csname R@an.cv.kits.L1base.d5alt\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.cv.kits.L1base.dcv\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.cv.kits.L1base.f0\endcsname{\ensuremath{+3.48}}
\expandafter\gdef\csname R@an.cv.kits.L1base.f0alt\endcsname{\ensuremath{+3.23}}
\expandafter\gdef\csname R@an.cv.kits.L1base.f0band\endcsname{1.45}
\expandafter\gdef\csname R@an.cv.kits.L1base.f0band.note\endcsname{two null SDs of this fold-0 difference, each the frozen default pool's training-seed SD of 0.795\,pp times $\sqrt{1/2 + 1/3}$ for the mean of two runs against the mean of the three-run pool: a locating band, not a test}
\expandafter\gdef\csname R@an.cv.kits.L1base.f0bandword\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.kits.L1base.f0gap\endcsname{3.48}
\expandafter\gdef\csname R@an.cv.kits.L1base.f0rev\endcsname{\ensuremath{-3.48}}
\expandafter\gdef\csname R@an.cv.kits.L1base.f0se\endcsname{0.726}
\expandafter\gdef\csname R@an.cv.kits.L1base.f1\endcsname{\ensuremath{+2.58}}
\expandafter\gdef\csname R@an.cv.kits.L1base.f2\endcsname{\ensuremath{+2.94}}
\expandafter\gdef\csname R@an.cv.kits.L1base.f3\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.cv.kits.L1base.f4\endcsname{\ensuremath{+1.71}}
\expandafter\gdef\csname R@an.cv.kits.L1base.hi\endcsname{\ensuremath{+3.32}}
\expandafter\gdef\csname R@an.cv.kits.L1base.lo\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.cv.kits.L1base.loo.max\endcsname{\ensuremath{+2.41}}
\expandafter\gdef\csname R@an.cv.kits.L1base.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.kits.L1base.loo.min\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@an.cv.kits.L1base.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L1base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.L1base.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L1base.share.word\endcsname{fold 2 alone carries 34\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.L1base.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L1base.share_max\endcsname{34}
\expandafter\gdef\csname R@an.cv.kits.L1base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.L1base.span14\endcsname{1.58}
\expandafter\gdef\csname R@an.cv.kits.L1base.src0\endcsname{fresh s1-2 for ResEnc-M and frozen pool for default}
\expandafter\gdef\csname R@an.cv.kits.L1base.src0mark\endcsname{b/a}
\expandafter\gdef\csname R@an.cv.kits.L1base.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.kits.L3.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.L3.cbs.clause\endcsname{HyReX minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.68}\,pp, 95\,\% interval \ensuremath{-0.16} to \ensuremath{+1.55}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.kits.L3.cbs.est\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.cv.kits.L3.cbs.hi\endcsname{\ensuremath{+1.55}}
\expandafter\gdef\csname R@an.cv.kits.L3.cbs.lo\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.cv.kits.L3.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.L3.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.L3.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L3.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L3.f0\endcsname{85.47}
\expandafter\gdef\csname R@an.cv.kits.L3.f1\endcsname{85.17}
\expandafter\gdef\csname R@an.cv.kits.L3.f2\endcsname{83.51}
\expandafter\gdef\csname R@an.cv.kits.L3.f3\endcsname{87.29}
\expandafter\gdef\csname R@an.cv.kits.L3.f4\endcsname{82.74}
\expandafter\gdef\csname R@an.cv.kits.L3.max14\endcsname{87.29}
\expandafter\gdef\csname R@an.cv.kits.L3.mean14\endcsname{84.67}
\expandafter\gdef\csname R@an.cv.kits.L3.mean5\endcsname{84.83}
\expandafter\gdef\csname R@an.cv.kits.L3.min14\endcsname{82.74}
\expandafter\gdef\csname R@an.cv.kits.L3.params\endcsname{29.66}
\expandafter\gdef\csname R@an.cv.kits.L3.params1\endcsname{29.7}
\expandafter\gdef\csname R@an.cv.kits.L3.span14\endcsname{4.55}
\expandafter\gdef\csname R@an.cv.kits.L3.src0\endcsname{fresh s1-2}
\expandafter\gdef\csname R@an.cv.kits.L3.src0long\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.cv.kits.L3.src0mark\endcsname{b}
\expandafter\gdef\csname R@an.cv.kits.L3.src0n\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L3L1.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.kits.L3L1.boot.casewidth\endcsname{1.82}
\expandafter\gdef\csname R@an.cv.kits.L3L1.boot.foldwidth\endcsname{3.41}
\expandafter\gdef\csname R@an.cv.kits.L3L1.boot.hi\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.boot.lo\endcsname{\ensuremath{-2.42}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.boot.mean\endcsname{\ensuremath{-1.46}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.boot.n\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.L3L1.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.kits.L3L1.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-2.42} to \ensuremath{-0.59}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.kits.L3L1.d5\endcsname{\ensuremath{-1.45}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.dcv\endcsname{\ensuremath{-1.47}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.f0\endcsname{\ensuremath{-1.38}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.f0gap\endcsname{1.38}
\expandafter\gdef\csname R@an.cv.kits.L3L1.f0lead\endcsname{ResEnc-M is ahead of HyReX}
\expandafter\gdef\csname R@an.cv.kits.L3L1.f0rev\endcsname{\ensuremath{+1.38}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.f1\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.f2\endcsname{\ensuremath{-2.74}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.f3\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.f4\endcsname{\ensuremath{-1.87}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.hi\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.lo\endcsname{\ensuremath{-3.17}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.loo.max\endcsname{\ensuremath{-1.04}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L3L1.loo.min\endcsname{\ensuremath{-1.86}}
\expandafter\gdef\csname R@an.cv.kits.L3L1.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L3L1.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.L3L1.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.L3L1.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.L3L1.share.word\endcsname{fold 2 alone carries 47\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.kits.L3L1.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.L3L1.share_max\endcsname{47}
\expandafter\gdef\csname R@an.cv.kits.L3L1.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.kits.L3L1.span14\endcsname{2.47}
\expandafter\gdef\csname R@an.cv.kits.L3L1.src0\endcsname{fresh s1-2 for HyReX and for ResEnc-M}
\expandafter\gdef\csname R@an.cv.kits.L3L1.src0mark\endcsname{b/b}
\expandafter\gdef\csname R@an.cv.kits.L3L1.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.kits.L3L1.wordrev\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.cbs.clause\endcsname{HyReX minus the function-identical control, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.12}\,pp, 95\,\% interval \ensuremath{-0.70} to \ensuremath{+0.96}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.cbs.est\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.cbs.hi\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.cbs.lo\endcsname{\ensuremath{-0.70}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.dcv\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.f1\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.f2\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.f3\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.f4\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.hi\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.lo\endcsname{\ensuremath{-0.73}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.loo.max\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.loo.min\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.loo.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.loo.word\endcsname{changes sign when a single fold is dropped (three of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.share.word\endcsname{fold 4 alone carries 175\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.share_max\endcsname{175}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.span14\endcsname{1.26}
\expandafter\gdef\csname R@an.cv.kits.L3P3c.word\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.cv.kits.L3base.boot.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.kits.L3base.boot.casewidth\endcsname{1.69}
\expandafter\gdef\csname R@an.cv.kits.L3base.boot.foldwidth\endcsname{3.52}
\expandafter\gdef\csname R@an.cv.kits.L3base.boot.hi\endcsname{\ensuremath{+1.54}}
\expandafter\gdef\csname R@an.cv.kits.L3base.boot.lo\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.cv.kits.L3base.boot.mean\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.cv.kits.L3base.boot.n\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.L3base.boot.vsfold\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.kits.L3base.boot.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.16} to \ensuremath{+1.54}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.kits.L3base.d5\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@an.cv.kits.L3base.d5alt\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.cv.kits.L3base.dcv\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.cv.kits.L3base.f0\endcsname{\ensuremath{+2.09}}
\expandafter\gdef\csname R@an.cv.kits.L3base.f0alt\endcsname{\ensuremath{+1.85}}
\expandafter\gdef\csname R@an.cv.kits.L3base.f0band\endcsname{1.45}
\expandafter\gdef\csname R@an.cv.kits.L3base.f0band.note\endcsname{two null SDs of this fold-0 difference, each the frozen default pool's training-seed SD of 0.795\,pp times $\sqrt{1/2 + 1/3}$ for the mean of two runs against the mean of the three-run pool: a locating band, not a test}
\expandafter\gdef\csname R@an.cv.kits.L3base.f0bandword\endcsname{is narrower than}
\expandafter\gdef\csname R@an.cv.kits.L3base.f0gap\endcsname{2.09}
\expandafter\gdef\csname R@an.cv.kits.L3base.f0rev\endcsname{\ensuremath{-2.09}}
\expandafter\gdef\csname R@an.cv.kits.L3base.f0se\endcsname{0.726}
\expandafter\gdef\csname R@an.cv.kits.L3base.f1\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.cv.kits.L3base.f2\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.kits.L3base.f3\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.cv.kits.L3base.f4\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.kits.L3base.hi\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@an.cv.kits.L3base.lo\endcsname{\ensuremath{-1.08}}
\expandafter\gdef\csname R@an.cv.kits.L3base.loo.max\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@an.cv.kits.L3base.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.L3base.loo.min\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.cv.kits.L3base.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L3base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.L3base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.L3base.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.L3base.share.word\endcsname{fold 1 alone carries 85\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.L3base.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.L3base.share_max\endcsname{85}
\expandafter\gdef\csname R@an.cv.kits.L3base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.L3base.span14\endcsname{2.46}
\expandafter\gdef\csname R@an.cv.kits.L3base.src0\endcsname{fresh s1-2 for HyReX and frozen pool for default}
\expandafter\gdef\csname R@an.cv.kits.L3base.src0mark\endcsname{b/a}
\expandafter\gdef\csname R@an.cv.kits.L3base.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.kits.P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.P3c.cbs.clause\endcsname{the function-identical control minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.56}\,pp, 95\,\% interval \ensuremath{-0.18} to \ensuremath{+1.29}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.kits.P3c.cbs.est\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.P3c.cbs.hi\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.cv.kits.P3c.cbs.lo\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.kits.P3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.P3c.f1\endcsname{85.24}
\expandafter\gdef\csname R@an.cv.kits.P3c.f2\endcsname{83.41}
\expandafter\gdef\csname R@an.cv.kits.P3c.f3\endcsname{87.68}
\expandafter\gdef\csname R@an.cv.kits.P3c.f4\endcsname{81.87}
\expandafter\gdef\csname R@an.cv.kits.P3c.max14\endcsname{87.68}
\expandafter\gdef\csname R@an.cv.kits.P3c.mean14\endcsname{84.55}
\expandafter\gdef\csname R@an.cv.kits.P3c.min14\endcsname{81.87}
\expandafter\gdef\csname R@an.cv.kits.P3c.params\endcsname{31.20}
\expandafter\gdef\csname R@an.cv.kits.P3c.params1\endcsname{31.2}
\expandafter\gdef\csname R@an.cv.kits.P3c.span14\endcsname{5.81}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.dcv\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.f1\endcsname{\ensuremath{+2.38}}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.f2\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.f3\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.f4\endcsname{\ensuremath{-1.02}}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.hi\endcsname{\ensuremath{+2.82}}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.lo\endcsname{\ensuremath{-1.71}}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.loo.max\endcsname{\ensuremath{+1.08}}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.loo.min\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.loo.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.loo.word\endcsname{changes sign when a single fold is dropped (three of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.share.word\endcsname{fold 1 alone carries 107\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.share_max\endcsname{107}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.span14\endcsname{3.40}
\expandafter\gdef\csname R@an.cv.kits.P3cbase.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.kits.V5B1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V5B1.cbs.clause\endcsname{LeanAdd minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+1.00}\,pp, 95\,\% interval \ensuremath{+0.18} to \ensuremath{+1.82}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.kits.V5B1.cbs.est\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.cv.kits.V5B1.cbs.hi\endcsname{\ensuremath{+1.82}}
\expandafter\gdef\csname R@an.cv.kits.V5B1.cbs.lo\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.kits.V5B1.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V5B1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B1.f1\endcsname{84.58}
\expandafter\gdef\csname R@an.cv.kits.V5B1.f2\endcsname{85.20}
\expandafter\gdef\csname R@an.cv.kits.V5B1.f3\endcsname{87.50}
\expandafter\gdef\csname R@an.cv.kits.V5B1.f4\endcsname{82.66}
\expandafter\gdef\csname R@an.cv.kits.V5B1.mean14\endcsname{84.99}
\expandafter\gdef\csname R@an.cv.kits.V5B1.params\endcsname{20.96}
\expandafter\gdef\csname R@an.cv.kits.V5B1.params1\endcsname{21.0}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.dcv\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.f1\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.f2\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.f3\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.f4\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.hi\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.lo\endcsname{\ensuremath{-0.79}}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.loo.max\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.loo.min\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.loo.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.loo.word\endcsname{changes sign when a single fold is dropped (two of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.share.word\endcsname{fold 3 alone carries 220\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.share_fold\endcsname{3}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.share_max\endcsname{220}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.span14\endcsname{1.03}
\expandafter\gdef\csname R@an.cv.kits.V5B1D2.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.cbs.clause\endcsname{LeanAdd minus the function-identical control, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.44}\,pp, 95\,\% interval \ensuremath{-0.34} to \ensuremath{+1.22}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.cbs.est\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.cbs.hi\endcsname{\ensuremath{+1.22}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.cbs.lo\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.ctloffset\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.dcv\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.f1\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.f2\endcsname{\ensuremath{+1.80}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.f3\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.f4\endcsname{\ensuremath{+0.79}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.hi\endcsname{\ensuremath{+2.17}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.lo\endcsname{\ensuremath{-1.30}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.loo.max\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.loo.min\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.loo.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.loo.word\endcsname{changes sign when a single fold is dropped (three of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.share.word\endcsname{fold 2 alone carries 103\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.share_max\endcsname{103}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.span14\endcsname{2.46}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.split\endcsname{LeanAdd minus the default is \ensuremath{+0.99}\,pp over the four folds; the control's own offset from the default is \ensuremath{+0.56}\,pp, so the margin over the function-identical control is \ensuremath{+0.44}\,pp}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.vsdefault\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c.word\endcsname{improves on it on average (2 of 4 folds)}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V5B1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.dcv\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.f1\endcsname{\ensuremath{+1.72}}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.f2\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.f3\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.f4\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.hi\endcsname{\ensuremath{+2.58}}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.lo\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.loo.max\endcsname{\ensuremath{+1.40}}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.loo.min\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.share.word\endcsname{fold 2 alone carries 48\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.share_max\endcsname{48}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.span14\endcsname{2.12}
\expandafter\gdef\csname R@an.cv.kits.V5B1base.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.kits.V5B2.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V5B2.cbs.clause\endcsname{LeanAdd-NeXt minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.75}\,pp, 95\,\% interval \ensuremath{-1.56} to \ensuremath{+0.01}\,pp, which reaches just above zero}
\expandafter\gdef\csname R@an.cv.kits.V5B2.cbs.est\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.cv.kits.V5B2.cbs.hi\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.kits.V5B2.cbs.lo\endcsname{\ensuremath{-1.56}}
\expandafter\gdef\csname R@an.cv.kits.V5B2.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V5B2.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B2.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B2.f1\endcsname{83.53}
\expandafter\gdef\csname R@an.cv.kits.V5B2.f2\endcsname{82.53}
\expandafter\gdef\csname R@an.cv.kits.V5B2.f3\endcsname{86.32}
\expandafter\gdef\csname R@an.cv.kits.V5B2.f4\endcsname{80.59}
\expandafter\gdef\csname R@an.cv.kits.V5B2.mean14\endcsname{83.24}
\expandafter\gdef\csname R@an.cv.kits.V5B2.params\endcsname{21.26}
\expandafter\gdef\csname R@an.cv.kits.V5B2.params1\endcsname{21.3}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.dcv\endcsname{\ensuremath{-1.43}}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.f1\endcsname{\ensuremath{-1.64}}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.f2\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.f3\endcsname{\ensuremath{-0.97}}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.f4\endcsname{\ensuremath{-2.15}}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.hi\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.lo\endcsname{\ensuremath{-2.34}}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.loo.max\endcsname{\ensuremath{-1.20}}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.loo.min\endcsname{\ensuremath{-1.59}}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.loo.minfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.share.word\endcsname{fold 4 alone carries 37\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.share_max\endcsname{37}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.span14\endcsname{1.18}
\expandafter\gdef\csname R@an.cv.kits.V5B2L3.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.cbs.clause\endcsname{LeanAdd-NeXt minus the function-identical control, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-1.31}\,pp, 95\,\% interval \ensuremath{-2.09} to \ensuremath{-0.58}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.cbs.est\endcsname{\ensuremath{-1.31}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.cbs.hi\endcsname{\ensuremath{-0.58}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.cbs.lo\endcsname{\ensuremath{-2.09}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.ctloffset\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.dcv\endcsname{\ensuremath{-1.31}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.f1\endcsname{\ensuremath{-1.72}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.f2\endcsname{\ensuremath{-0.88}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.f3\endcsname{\ensuremath{-1.36}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.f4\endcsname{\ensuremath{-1.28}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.hi\endcsname{\ensuremath{-0.76}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.lo\endcsname{\ensuremath{-1.86}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.loo.max\endcsname{\ensuremath{-1.17}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.loo.min\endcsname{\ensuremath{-1.45}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.share.word\endcsname{fold 1 alone carries 33\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.share_max\endcsname{33}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.span14\endcsname{0.84}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.split\endcsname{LeanAdd-NeXt minus the default is \ensuremath{-0.75}\,pp over the four folds; the control's own offset from the default is \ensuremath{+0.56}\,pp, so the margin over the function-identical control is \ensuremath{-1.31}\,pp}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.vsdefault\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c.word\endcsname{does not improve on it}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V5B2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.dcv\endcsname{\ensuremath{-1.75}}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.f1\endcsname{\ensuremath{-1.05}}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.f2\endcsname{\ensuremath{-2.68}}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.f3\endcsname{\ensuremath{-1.18}}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.f4\endcsname{\ensuremath{-2.07}}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.hi\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.lo\endcsname{\ensuremath{-2.97}}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.loo.max\endcsname{\ensuremath{-1.44}}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.loo.min\endcsname{\ensuremath{-1.98}}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.share.word\endcsname{fold 2 alone carries 38\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.share_max\endcsname{38}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.span14\endcsname{1.63}
\expandafter\gdef\csname R@an.cv.kits.V5B2V5B1.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.dcv\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.f1\endcsname{\ensuremath{+0.67}}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.f2\endcsname{\ensuremath{-0.78}}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.f3\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.f4\endcsname{\ensuremath{-2.30}}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.hi\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.lo\endcsname{\ensuremath{-2.69}}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.loo.max\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.loo.min\endcsname{\ensuremath{-1.22}}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.share.word\endcsname{fold 4 alone carries 76\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.share_max\endcsname{76}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.span14\endcsname{2.97}
\expandafter\gdef\csname R@an.cv.kits.V5B2base.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.cbs.clause\endcsname{HyReX-k9 minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.28}\,pp, 95\,\% interval \ensuremath{-0.62} to \ensuremath{+1.17}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.cbs.est\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.cbs.hi\endcsname{\ensuremath{+1.17}}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.cbs.lo\endcsname{\ensuremath{-0.62}}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.f1\endcsname{84.22}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.f2\endcsname{82.53}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.f3\endcsname{87.94}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.f4\endcsname{82.41}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.mean14\endcsname{84.27}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.params\endcsname{30.78}
\expandafter\gdef\csname R@an.cv.kits.V6A1r.params1\endcsname{30.8}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.dcv\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.f1\endcsname{\ensuremath{-0.95}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.f2\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.f3\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.f4\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.hi\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.lo\endcsname{\ensuremath{-1.62}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.loo.max\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.loo.min\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.loo.minfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.share.word\endcsname{fold 2 alone carries 61\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.share_max\endcsname{61}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.span14\endcsname{1.63}
\expandafter\gdef\csname R@an.cv.kits.V6A1rL3.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.cbs.clause\endcsname{HyReX-k9 minus the function-identical control, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.28}\,pp, 95\,\% interval \ensuremath{-1.13} to \ensuremath{+0.60}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.cbs.est\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.cbs.hi\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.cbs.lo\endcsname{\ensuremath{-1.13}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.ctloffset\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.dcv\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.f1\endcsname{\ensuremath{-1.02}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.f2\endcsname{\ensuremath{-0.88}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.f3\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.f4\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.hi\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.lo\endcsname{\ensuremath{-1.53}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.loo.max\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.loo.min\endcsname{\ensuremath{-0.55}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.share.word\endcsname{fold 1 alone carries 92\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.share_max\endcsname{92}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.span14\endcsname{1.56}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.split\endcsname{HyReX-k9 minus the default is \ensuremath{+0.28}\,pp over the four folds; the control's own offset from the default is \ensuremath{+0.56}\,pp, so the margin over the function-identical control is \ensuremath{-0.28}\,pp}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.vsdefault\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c.word\endcsname{does not improve on it}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V6A1rP3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.dcv\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.f1\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.f2\endcsname{\ensuremath{-0.78}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.f3\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.f4\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.hi\endcsname{\ensuremath{+1.98}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.lo\endcsname{\ensuremath{-1.42}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.loo.max\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.loo.min\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.loo.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.loo.word\endcsname{changes sign when a single fold is dropped (three of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.share.word\endcsname{fold 1 alone carries 121\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.share_max\endcsname{121}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.span14\endcsname{2.14}
\expandafter\gdef\csname R@an.cv.kits.V6A1rbase.word\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.cv.kits.V7A1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V7A1.cbs.clause\endcsname{LeanDeepMid minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+1.64}\,pp, 95\,\% interval \ensuremath{+0.89} to \ensuremath{+2.42}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.kits.V7A1.cbs.est\endcsname{\ensuremath{+1.64}}
\expandafter\gdef\csname R@an.cv.kits.V7A1.cbs.hi\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.cv.kits.V7A1.cbs.lo\endcsname{\ensuremath{+0.89}}
\expandafter\gdef\csname R@an.cv.kits.V7A1.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V7A1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7A1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A1.f1\endcsname{84.89}
\expandafter\gdef\csname R@an.cv.kits.V7A1.f2\endcsname{85.71}
\expandafter\gdef\csname R@an.cv.kits.V7A1.f3\endcsname{88.89}
\expandafter\gdef\csname R@an.cv.kits.V7A1.f4\endcsname{83.01}
\expandafter\gdef\csname R@an.cv.kits.V7A1.mean14\endcsname{85.63}
\expandafter\gdef\csname R@an.cv.kits.V7A1.params\endcsname{31.04}
\expandafter\gdef\csname R@an.cv.kits.V7A1.params1\endcsname{31.0}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.cbs.clause\endcsname{LeanDeepMid minus the function-identical control, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+1.08}\,pp, 95\,\% interval \ensuremath{+0.41} to \ensuremath{+1.78}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.cbs.est\endcsname{\ensuremath{+1.08}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.cbs.hi\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.cbs.lo\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.ctloffset\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.dcv\endcsname{\ensuremath{+1.08}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.f1\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.f2\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.f3\endcsname{\ensuremath{+1.20}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.f4\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.hi\endcsname{\ensuremath{+2.81}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.lo\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.loo.max\endcsname{\ensuremath{+1.55}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.loo.min\endcsname{\ensuremath{+0.67}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.share.word\endcsname{fold 2 alone carries 54\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.share_max\endcsname{54}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.span14\endcsname{2.66}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.split\endcsname{LeanDeepMid minus the default is \ensuremath{+1.63}\,pp over the four folds; the control's own offset from the default is \ensuremath{+0.56}\,pp, so the margin over the function-identical control is \ensuremath{+1.08}\,pp}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.vsdefault\endcsname{\ensuremath{+1.63}}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c.word\endcsname{improves on it on average (3 of 4 folds)}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7A1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.dcv\endcsname{\ensuremath{+2.39}}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.f1\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.f2\endcsname{\ensuremath{+3.19}}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.f3\endcsname{\ensuremath{+2.57}}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.f4\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.hi\endcsname{\ensuremath{+3.59}}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.lo\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.loo.max\endcsname{\ensuremath{+2.72}}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.loo.min\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.share.word\endcsname{fold 2 alone carries 33\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.share_max\endcsname{33}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.span14\endcsname{1.82}
\expandafter\gdef\csname R@an.cv.kits.V7A1V5B2.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.dcv\endcsname{\ensuremath{+1.63}}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.f1\endcsname{\ensuremath{+2.03}}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.f2\endcsname{\ensuremath{+2.40}}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.f3\endcsname{\ensuremath{+1.98}}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.f4\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.hi\endcsname{\ensuremath{+3.27}}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.lo\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.loo.max\endcsname{\ensuremath{+2.14}}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.loo.min\endcsname{\ensuremath{+1.38}}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.share.word\endcsname{fold 2 alone carries 37\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.share_max\endcsname{37}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.span14\endcsname{2.28}
\expandafter\gdef\csname R@an.cv.kits.V7A1base.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.kits.V7A2.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V7A2.cbs.clause\endcsname{LeanDeepMid+FD minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.91}\,pp, 95\,\% interval \ensuremath{+0.17} to \ensuremath{+1.66}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.kits.V7A2.cbs.est\endcsname{\ensuremath{+0.91}}
\expandafter\gdef\csname R@an.cv.kits.V7A2.cbs.hi\endcsname{\ensuremath{+1.66}}
\expandafter\gdef\csname R@an.cv.kits.V7A2.cbs.lo\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.cv.kits.V7A2.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V7A2.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7A2.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A2.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A2.f1\endcsname{84.67}
\expandafter\gdef\csname R@an.cv.kits.V7A2.f2\endcsname{84.21}
\expandafter\gdef\csname R@an.cv.kits.V7A2.f3\endcsname{88.06}
\expandafter\gdef\csname R@an.cv.kits.V7A2.f4\endcsname{82.65}
\expandafter\gdef\csname R@an.cv.kits.V7A2.mean14\endcsname{84.90}
\expandafter\gdef\csname R@an.cv.kits.V7A2.params\endcsname{31.18}
\expandafter\gdef\csname R@an.cv.kits.V7A2.params1\endcsname{31.2}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.cbs.clause\endcsname{LeanDeepMid+FD minus the function-identical control, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.35}\,pp, 95\,\% interval \ensuremath{-0.29} to \ensuremath{+1.03}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.cbs.est\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.cbs.hi\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.cbs.lo\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.ctloffset\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.dcv\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.f1\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.f2\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.f3\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.f4\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.hi\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.lo\endcsname{\ensuremath{-0.67}}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.loo.max\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.loo.min\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.share.word\endcsname{fold 2 alone carries 57\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.share_max\endcsname{57}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.span14\endcsname{1.37}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.split\endcsname{LeanDeepMid+FD minus the default is \ensuremath{+0.91}\,pp over the four folds; the control's own offset from the default is \ensuremath{+0.56}\,pp, so the margin over the function-identical control is \ensuremath{+0.35}\,pp}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.vsdefault\endcsname{\ensuremath{+0.91}}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c.word\endcsname{improves on it on average (3 of 4 folds)}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7A2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.dcv\endcsname{\ensuremath{-0.73}}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.f1\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.f2\endcsname{\ensuremath{-1.50}}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.f3\endcsname{\ensuremath{-0.82}}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.f4\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.hi\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.lo\endcsname{\ensuremath{-1.65}}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.loo.max\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.loo.maxfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.loo.min\endcsname{\ensuremath{-0.89}}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.share.word\endcsname{fold 2 alone carries 52\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.share_max\endcsname{52}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.span14\endcsname{1.28}
\expandafter\gdef\csname R@an.cv.kits.V7A2V7A1.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.dcv\endcsname{\ensuremath{+0.91}}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.f1\endcsname{\ensuremath{+1.81}}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.f2\endcsname{\ensuremath{+0.90}}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.f3\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.f4\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.hi\endcsname{\ensuremath{+2.27}}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.lo\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.loo.max\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.loo.min\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.share.word\endcsname{fold 1 alone carries 50\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.share_max\endcsname{50}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.span14\endcsname{2.05}
\expandafter\gdef\csname R@an.cv.kits.V7A2base.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.kits.V7B1.cbs.clause\endcsname{LeanSep minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.kits.V7B1.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B1.params\endcsname{20.43}
\expandafter\gdef\csname R@an.cv.kits.V7B1.params1\endcsname{20.4}
\expandafter\gdef\csname R@an.cv.kits.V7B1P3c.cbs.clause\endcsname{LeanSep minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.kits.V7B1P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B1P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B1P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7B1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7B1V5B2.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B1V5B2.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7B1base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B1base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7B2.cbs.clause\endcsname{LeanDil minus the default, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.kits.V7B2.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B2.params\endcsname{20.45}
\expandafter\gdef\csname R@an.cv.kits.V7B2.params1\endcsname{20.5}
\expandafter\gdef\csname R@an.cv.kits.V7B2P3c.cbs.clause\endcsname{LeanDil minus the function-identical control, case-level paired bootstrap: none of the four folds have a finished run of the arm and its reference}
\expandafter\gdef\csname R@an.cv.kits.V7B2P3c.cbs.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B2P3c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B2P3c.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7B2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7B2V5B2.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B2V5B2.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7B2base.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7B2base.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7C1.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V7C1.cbs.clause\endcsname{LeanNeXt-s5 minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.79}\,pp, 95\,\% interval \ensuremath{+0.07} to \ensuremath{+1.51}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.kits.V7C1.cbs.est\endcsname{\ensuremath{+0.79}}
\expandafter\gdef\csname R@an.cv.kits.V7C1.cbs.hi\endcsname{\ensuremath{+1.51}}
\expandafter\gdef\csname R@an.cv.kits.V7C1.cbs.lo\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.kits.V7C1.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V7C1.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7C1.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7C1.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7C1.f1\endcsname{85.00}
\expandafter\gdef\csname R@an.cv.kits.V7C1.f2\endcsname{84.05}
\expandafter\gdef\csname R@an.cv.kits.V7C1.f3\endcsname{87.64}
\expandafter\gdef\csname R@an.cv.kits.V7C1.f4\endcsname{82.42}
\expandafter\gdef\csname R@an.cv.kits.V7C1.mean14\endcsname{84.78}
\expandafter\gdef\csname R@an.cv.kits.V7C1.params\endcsname{21.11}
\expandafter\gdef\csname R@an.cv.kits.V7C1.params1\endcsname{21.1}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.cbs.clause\endcsname{LeanNeXt-s5 minus the function-identical control, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{+0.22}\,pp, 95\,\% interval \ensuremath{-0.49} to \ensuremath{+0.96}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.cbs.est\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.cbs.hi\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.cbs.lo\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.ctloffset\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.dcv\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.f1\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.f2\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.f3\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.f4\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.hi\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.lo\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.loo.max\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.loo.maxfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.loo.min\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.share.word\endcsname{fold 2 alone carries 71\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.share_fold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.share_max\endcsname{71}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.span14\endcsname{0.89}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.split\endcsname{LeanNeXt-s5 minus the default is \ensuremath{+0.78}\,pp over the four folds; the control's own offset from the default is \ensuremath{+0.56}\,pp, so the margin over the function-identical control is \ensuremath{+0.23}\,pp}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.vsdefault\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c.word\endcsname{improves on it on average (2 of 4 folds)}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V7C1P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.dcv\endcsname{\ensuremath{+1.54}}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.f1\endcsname{\ensuremath{+1.47}}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.f2\endcsname{\ensuremath{+1.52}}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.f3\endcsname{\ensuremath{+1.32}}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.f4\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.hi\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.lo\endcsname{\ensuremath{+1.20}}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.loo.max\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.loo.maxfold\endcsname{3}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.loo.min\endcsname{\ensuremath{+1.44}}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.loo.minfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.share.word\endcsname{fold 4 alone carries 30\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.share_max\endcsname{30}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.span14\endcsname{0.51}
\expandafter\gdef\csname R@an.cv.kits.V7C1V5B2.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.dcv\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.f1\endcsname{\ensuremath{+2.14}}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.f2\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.f3\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.f4\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.hi\endcsname{\ensuremath{+2.48}}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.lo\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.loo.max\endcsname{\ensuremath{+1.20}}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.loo.min\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.loo.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.loo.word\endcsname{stays positive when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.share.word\endcsname{fold 1 alone carries 68\,\% of the summed per-fold differences}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.share_fold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.share_max\endcsname{68}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.sign\endcsname{positive}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.span14\endcsname{2.61}
\expandafter\gdef\csname R@an.cv.kits.V7C1base.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv.kits.V8B2.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V8B2.cbs.clause\endcsname{Stem1 minus the default, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.24}\,pp, 95\,\% interval \ensuremath{-1.09} to \ensuremath{+0.57}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.kits.V8B2.cbs.est\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.kits.V8B2.cbs.hi\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.cv.kits.V8B2.cbs.lo\endcsname{\ensuremath{-1.09}}
\expandafter\gdef\csname R@an.cv.kits.V8B2.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V8B2.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V8B2.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V8B2.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V8B2.f1\endcsname{84.09}
\expandafter\gdef\csname R@an.cv.kits.V8B2.f2\endcsname{83.33}
\expandafter\gdef\csname R@an.cv.kits.V8B2.f3\endcsname{87.02}
\expandafter\gdef\csname R@an.cv.kits.V8B2.f4\endcsname{80.56}
\expandafter\gdef\csname R@an.cv.kits.V8B2.mean14\endcsname{83.75}
\expandafter\gdef\csname R@an.cv.kits.V8B2.params\endcsname{21.08}
\expandafter\gdef\csname R@an.cv.kits.V8B2.params1\endcsname{21.1}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.cbs.B\endcsname{10000}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.cbs.clause\endcsname{Stem1 minus the function-identical control, case-level paired bootstrap over the 391 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold): \ensuremath{-0.80}\,pp, 95\,\% interval \ensuremath{-1.63} to \ensuremath{-0.02}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.cbs.est\endcsname{\ensuremath{-0.80}}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.cbs.hi\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.cbs.lo\endcsname{\ensuremath{-1.63}}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.cbs.ncases\endcsname{391}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.cbs.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.cbs.nseeds\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.cbs.nseeds.max\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.ctloffset\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.dcv\endcsname{\ensuremath{-0.80}}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.f1\endcsname{\ensuremath{-1.15}}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.f2\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.f3\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.f4\endcsname{\ensuremath{-1.31}}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.hi\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.lo\endcsname{\ensuremath{-1.68}}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.loo.max\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.loo.min\endcsname{\ensuremath{-1.04}}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.loo.minfold\endcsname{2}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.loo.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.loo.word\endcsname{stays at or below zero when any single fold is dropped}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.share.word\endcsname{fold 4 alone carries 41\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.share_max\endcsname{41}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.span14\endcsname{1.23}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.split\endcsname{Stem1 minus the default is \ensuremath{-0.24}\,pp over the four folds; the control's own offset from the default is \ensuremath{+0.56}\,pp, so the margin over the function-identical control is \ensuremath{-0.80}\,pp}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.vsdefault\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c.word\endcsname{does not improve on it}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c3.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv.kits.V8B2P3c3.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.dcv\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.f1\endcsname{\ensuremath{+1.23}}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.f2\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.f3\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.f4\endcsname{\ensuremath{-2.33}}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.hi\endcsname{\ensuremath{+2.13}}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.lo\endcsname{\ensuremath{-2.62}}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.loo.max\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.loo.maxfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.loo.min\endcsname{\ensuremath{-0.74}}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.loo.minfold\endcsname{1}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.loo.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.loo.word\endcsname{changes sign when a single fold is dropped (one of the four leave-one-fold-out means are positive)}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.nfold.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.share.word\endcsname{fold 4 alone carries 238\,\% of the summed per-fold deficits}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.share_fold\endcsname{4}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.share_max\endcsname{238}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.sign\endcsname{negative}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.span14\endcsname{3.56}
\expandafter\gdef\csname R@an.cv.kits.V8B2base.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv.kits.base.f0\endcsname{83.38}
\expandafter\gdef\csname R@an.cv.kits.base.f1\endcsname{82.86}
\expandafter\gdef\csname R@an.cv.kits.base.f2\endcsname{83.31}
\expandafter\gdef\csname R@an.cv.kits.base.f3\endcsname{86.91}
\expandafter\gdef\csname R@an.cv.kits.base.f4\endcsname{82.89}
\expandafter\gdef\csname R@an.cv.kits.base.max14\endcsname{86.91}
\expandafter\gdef\csname R@an.cv.kits.base.mean14\endcsname{83.99}
\expandafter\gdef\csname R@an.cv.kits.base.mean5\endcsname{83.87}
\expandafter\gdef\csname R@an.cv.kits.base.min14\endcsname{82.86}
\expandafter\gdef\csname R@an.cv.kits.base.params\endcsname{31.20}
\expandafter\gdef\csname R@an.cv.kits.base.params1\endcsname{31.2}
\expandafter\gdef\csname R@an.cv.kits.base.span14\endcsname{4.05}
\expandafter\gdef\csname R@an.cv.kits.base.src0\endcsname{frozen pool}
\expandafter\gdef\csname R@an.cv.kits.base.src0long\endcsname{the frozen default pool}
\expandafter\gdef\csname R@an.cv.kits.base.src0mark\endcsname{a}
\expandafter\gdef\csname R@an.cv.kits.base.src0n\endcsname{3}
\expandafter\gdef\csname R@an.cv.kits.recovery.L3\endcsname{0.32}
\expandafter\gdef\csname R@an.cv.kits.recovery.L3.hi\endcsname{1.09}
\expandafter\gdef\csname R@an.cv.kits.recovery.L3.lo\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.cv.kits.recovery.L3.method\endcsname{the delta method applied to the two four-fold mean margins, HyReX minus the default and ResEnc-M minus the default, which are differences from the same default runs, so their covariance over the folds enters the variance of the ratio; the interval takes the t quantile on three degrees of freedom of the registered paired-t intervals of the margins; it is descriptive, a description of four folds of one seed each and not a test, and it is withheld when ResEnc-M's own interval over the folds includes zero}
\expandafter\gdef\csname R@an.cv.kits.recovery.L3.sentence\endcsname{On KiTS23, HyReX's mean margin over the default on the four folds that entered no decision, \ensuremath{+0.68}\,pp, is 0.32 of ResEnc-M's, \ensuremath{+2.15}\,pp; the 95\,\% interval of that ratio, \ensuremath{-0.45} to 1.09, comes from the delta method on the two fold-mean margins and describes the four folds without testing anything}
\expandafter\gdef\csname R@an.cv.kits.recovery.L3.state\endcsname{complete}
\expandafter\gdef\csname R@an.cv.l1b.def\endcsname{the ResEnc-M preset re-implemented through the plan-aware family in which every agent design and every other control is built (it differs from the library preset in the default stem, the shortcut form and the zero-initialisation)}
\expandafter\gdef\csname R@an.cv.l1b.name\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.cv.line.acdc.D2P3c\endcsname{LeanDec (25.28\,M parameters) minus the function-identical control (30.38\,M): \ensuremath{+0.02}\,pp over the four folds, improves on it on average (2 of 4 folds), 95\,\% over folds \ensuremath{-0.23} to \ensuremath{+0.27}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.D2P3c3\endcsname{LeanDec (25.28\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.D2base\endcsname{LeanDec (25.28\,M parameters) minus the default (30.38\,M): \ensuremath{-0.05}\,pp over the four folds, does not improve in cross-validation (1/4 folds positive), 95\,\% over folds \ensuremath{-0.18} to \ensuremath{+0.07}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.L1L1b\endcsname{ResEnc-M (101.53\,M parameters) minus ResEnc-matched (101.63\,M): \ensuremath{+0.18}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.02} to \ensuremath{+0.33}\,pp, which lies inside $\pm$0.50\,pp and above zero}
\expandafter\gdef\csname R@an.cv.line.acdc.L1L3\endcsname{ResEnc-M (101.53\,M parameters) minus HyReX (28.85\,M): \ensuremath{+0.04}\,pp over the four folds, improves on average (2/4 folds), 95\,\% over folds \ensuremath{-0.24} to \ensuremath{+0.31}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.L1P3c\endcsname{ResEnc-M (101.53\,M parameters) minus the function-identical control (30.38\,M): \ensuremath{+0.45}\,pp over the four folds, improves on the control in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.34} to \ensuremath{+0.56}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.acdc.L1P3c3\endcsname{ResEnc-M (101.53\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.L1bL3\endcsname{ResEnc-matched (101.63\,M parameters) minus HyReX (28.85\,M): \ensuremath{-0.14}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.27} to \ensuremath{-0.01}\,pp, which lies inside $\pm$0.50\,pp and below zero}
\expandafter\gdef\csname R@an.cv.line.acdc.L1base\endcsname{ResEnc-M (101.53\,M parameters) minus the default (30.38\,M): \ensuremath{+0.37}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.26} to \ensuremath{+0.48}\,pp, which lies inside $\pm$0.50\,pp and above zero}
\expandafter\gdef\csname R@an.cv.line.acdc.L3P3c\endcsname{HyReX (28.85\,M parameters) minus the function-identical control (30.38\,M): \ensuremath{+0.41}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.06} to \ensuremath{+0.76}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.acdc.L3base\endcsname{HyReX (28.85\,M parameters) minus the default (30.38\,M): \ensuremath{+0.33}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.10} to \ensuremath{+0.56}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.acdc.P3cbase\endcsname{the function-identical control (30.38\,M parameters) minus the default (30.38\,M): \ensuremath{-0.08}\,pp over the four folds, does not improve in cross-validation (1/4 folds positive), 95\,\% over folds \ensuremath{-0.22} to \ensuremath{+0.06}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V5B1D2\endcsname{LeanAdd (20.18\,M parameters) minus LeanDec (25.28\,M): \ensuremath{-0.06}\,pp over the four folds, does not improve in cross-validation (1/4 folds positive), 95\,\% over folds \ensuremath{-0.20} to \ensuremath{+0.07}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V5B1P3c\endcsname{LeanAdd (20.18\,M parameters) minus the function-identical control (30.38\,M): \ensuremath{-0.04}\,pp over the four folds, does not improve on it (2/4 folds positive), 95\,\% over folds \ensuremath{-0.34} to \ensuremath{+0.27}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V5B1P3c3\endcsname{LeanAdd (20.18\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.V5B1base\endcsname{LeanAdd (20.18\,M parameters) minus the default (30.38\,M): \ensuremath{-0.12}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.32} to \ensuremath{+0.08}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V5B2L3\endcsname{LeanAdd-NeXt (20.48\,M parameters) minus HyReX (28.85\,M): \ensuremath{-0.45}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.69} to \ensuremath{-0.20}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.acdc.V5B2P3c\endcsname{LeanAdd-NeXt (20.48\,M parameters) minus the function-identical control (30.38\,M): \ensuremath{-0.04}\,pp over the four folds, does not improve on it (1/4 folds positive), 95\,\% over folds \ensuremath{-0.27} to \ensuremath{+0.20}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V5B2P3c3\endcsname{LeanAdd-NeXt (20.48\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.V5B2V5B1\endcsname{LeanAdd-NeXt (20.48\,M parameters) minus LeanAdd (20.18\,M): \ensuremath{0.00}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.29} to \ensuremath{+0.30}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V5B2base\endcsname{LeanAdd-NeXt (20.48\,M parameters) minus the default (30.38\,M): \ensuremath{-0.11}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.30} to \ensuremath{+0.07}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V6A1rL3\endcsname{HyReX-k9 (29.96\,M parameters) minus HyReX (28.85\,M): \ensuremath{-0.03}\,pp over the four folds, does not improve in cross-validation (3/4 folds positive), 95\,\% over folds \ensuremath{-0.28} to \ensuremath{+0.22}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V6A1rP3c\endcsname{HyReX-k9 (29.96\,M parameters) minus the function-identical control (30.38\,M): \ensuremath{+0.38}\,pp over the four folds, improves on the control in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.18} to \ensuremath{+0.59}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.acdc.V6A1rP3c3\endcsname{HyReX-k9 (29.96\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.V6A1rbase\endcsname{HyReX-k9 (29.96\,M parameters) minus the default (30.38\,M): \ensuremath{+0.31}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.13} to \ensuremath{+0.49}\,pp, which lies inside $\pm$0.50\,pp and above zero}
\expandafter\gdef\csname R@an.cv.line.acdc.V7A1P3c\endcsname{LeanDeepMid (30.26\,M parameters) minus the function-identical control (30.38\,M): \ensuremath{+0.16}\,pp over the four folds, improves on it on average (3 of 4 folds), 95\,\% over folds \ensuremath{-0.29} to \ensuremath{+0.60}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.acdc.V7A1P3c3\endcsname{LeanDeepMid (30.26\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.V7A1V5B2\endcsname{LeanDeepMid (30.26\,M parameters) minus LeanAdd-NeXt (20.48\,M): \ensuremath{+0.19}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.23} to \ensuremath{+0.62}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.acdc.V7A1base\endcsname{LeanDeepMid (30.26\,M parameters) minus the default (30.38\,M): \ensuremath{+0.08}\,pp over the four folds, improves on average (2/4 folds), 95\,\% over folds \ensuremath{-0.38} to \ensuremath{+0.54}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.acdc.V7A2P3c\endcsname{LeanDeepMid+FD (30.38\,M parameters) minus the function-identical control (30.38\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V7A2P3c3\endcsname{LeanDeepMid+FD (30.38\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.V7A2V7A1\endcsname{LeanDeepMid+FD (30.38\,M parameters) minus LeanDeepMid (30.26\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V7A2base\endcsname{LeanDeepMid+FD (30.38\,M parameters) minus the default (30.38\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V7B1P3c\endcsname{LeanSep (19.65\,M parameters) minus the function-identical control (30.38\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V7B1P3c3\endcsname{LeanSep (19.65\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.V7B1V5B2\endcsname{LeanSep (19.65\,M parameters) minus LeanAdd-NeXt (20.48\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V7B1base\endcsname{LeanSep (19.65\,M parameters) minus the default (30.38\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V7B2P3c\endcsname{LeanDil (19.67\,M parameters) minus the function-identical control (30.38\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V7B2P3c3\endcsname{LeanDil (19.67\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.V7B2V5B2\endcsname{LeanDil (19.67\,M parameters) minus LeanAdd-NeXt (20.48\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V7B2base\endcsname{LeanDil (19.67\,M parameters) minus the default (30.38\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V7C1P3c\endcsname{LeanNeXt-s5 (20.33\,M parameters) minus the function-identical control (30.38\,M): \ensuremath{-0.11}\,pp over the four folds, does not improve on it (1/4 folds positive), 95\,\% over folds \ensuremath{-0.32} to \ensuremath{+0.10}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V7C1P3c3\endcsname{LeanNeXt-s5 (20.33\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.V7C1V5B2\endcsname{LeanNeXt-s5 (20.33\,M parameters) minus LeanAdd-NeXt (20.48\,M): \ensuremath{-0.07}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.15} to \ensuremath{0.00}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.acdc.V7C1base\endcsname{LeanNeXt-s5 (20.33\,M parameters) minus the default (30.38\,M): \ensuremath{-0.19}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.31} to \ensuremath{-0.07}\,pp, which lies inside $\pm$0.50\,pp and below zero}
\expandafter\gdef\csname R@an.cv.line.acdc.V8B2P3c\endcsname{Stem1 (20.32\,M parameters) minus the function-identical control (30.38\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.acdc.V8B2P3c3\endcsname{Stem1 (20.32\,M parameters) minus the function-identical control's three-seed mean of the same fold (30.38\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.acdc.V8B2base\endcsname{Stem1 (20.32\,M parameters) minus the default (30.38\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.D2P3c\endcsname{LeanDec (26.03\,M parameters) minus the function-identical control (31.12\,M): \ensuremath{-0.41}\,pp over the four folds, does not improve on it (1/4 folds positive), 95\,\% over folds \ensuremath{-0.95} to \ensuremath{+0.14}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.D2P3c3\endcsname{LeanDec (26.03\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.D2base\endcsname{LeanDec (26.03\,M parameters) minus the default (31.12\,M): \ensuremath{-0.44}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.75} to \ensuremath{-0.12}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.amos.L1L1b\endcsname{ResEnc-M (102.28\,M parameters) minus ResEnc-matched (102.37\,M): \ensuremath{-0.02}\,pp over the four folds, does not improve in cross-validation (1/4 folds positive), 95\,\% over folds \ensuremath{-0.28} to \ensuremath{+0.24}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.amos.L1L3\endcsname{ResEnc-M (102.28\,M parameters) minus HyReX (29.59\,M): \ensuremath{+0.18}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.40} to \ensuremath{+0.76}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.L1P3c\endcsname{ResEnc-M (102.28\,M parameters) minus the function-identical control (31.12\,M): \ensuremath{+0.44}\,pp over the four folds, improves on the control in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.01} to \ensuremath{+0.86}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.amos.L1P3c3\endcsname{ResEnc-M (102.28\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.L1bL3\endcsname{ResEnc-matched (102.37\,M parameters) minus HyReX (29.59\,M): \ensuremath{+0.20}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.38} to \ensuremath{+0.78}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.L1base\endcsname{ResEnc-M (102.28\,M parameters) minus the default (31.12\,M): \ensuremath{+0.41}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.27} to \ensuremath{+1.09}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.L3P3c\endcsname{HyReX (29.59\,M parameters) minus the function-identical control (31.12\,M): \ensuremath{+0.26}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{-0.03} to \ensuremath{+0.55}\,pp, which reaches just below zero}
\expandafter\gdef\csname R@an.cv.line.amos.L3base\endcsname{HyReX (29.59\,M parameters) minus the default (31.12\,M): \ensuremath{+0.23}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.08} to \ensuremath{+0.54}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.P3cbase\endcsname{the function-identical control (31.12\,M parameters) minus the default (31.12\,M): \ensuremath{-0.03}\,pp over the four folds, does not improve in cross-validation (2/4 folds positive), 95\,\% over folds \ensuremath{-0.57} to \ensuremath{+0.51}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.V5B1D2\endcsname{LeanAdd (20.93\,M parameters) minus LeanDec (26.03\,M): \ensuremath{-0.02}\,pp over the four folds, does not improve in cross-validation (2/4 folds positive), 95\,\% over folds \ensuremath{-0.28} to \ensuremath{+0.24}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.amos.V5B1P3c\endcsname{LeanAdd (20.93\,M parameters) minus the function-identical control (31.12\,M): \ensuremath{-0.43}\,pp over the four folds, does not improve on it (0/4 folds positive), 95\,\% over folds \ensuremath{-0.77} to \ensuremath{-0.09}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.amos.V5B1P3c3\endcsname{LeanAdd (20.93\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.V5B1base\endcsname{LeanAdd (20.93\,M parameters) minus the default (31.12\,M): \ensuremath{-0.46}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.82} to \ensuremath{-0.10}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.amos.V5B2L3\endcsname{LeanAdd-NeXt (21.22\,M parameters) minus HyReX (29.59\,M): \ensuremath{-0.48}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.85} to \ensuremath{-0.12}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.amos.V5B2P3c\endcsname{LeanAdd-NeXt (21.22\,M parameters) minus the function-identical control (31.12\,M): \ensuremath{-0.22}\,pp over the four folds, does not improve on it (0/4 folds positive), 95\,\% over folds \ensuremath{-0.38} to \ensuremath{-0.07}\,pp, which lies inside $\pm$0.50\,pp and below zero}
\expandafter\gdef\csname R@an.cv.line.amos.V5B2P3c3\endcsname{LeanAdd-NeXt (21.22\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.V5B2V5B1\endcsname{LeanAdd-NeXt (21.22\,M parameters) minus LeanAdd (20.93\,M): \ensuremath{+0.21}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.17} to \ensuremath{+0.58}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.V5B2base\endcsname{LeanAdd-NeXt (21.22\,M parameters) minus the default (31.12\,M): \ensuremath{-0.25}\,pp over the four folds, does not improve in cross-validation (1/4 folds positive), 95\,\% over folds \ensuremath{-0.83} to \ensuremath{+0.32}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.V6A1rL3\endcsname{HyReX-k9 (30.70\,M parameters) minus HyReX (29.59\,M): \ensuremath{-0.03}\,pp over the four folds, does not improve in cross-validation (1/4 folds positive), 95\,\% over folds \ensuremath{-0.37} to \ensuremath{+0.32}\,pp, which lies inside $\pm$0.50\,pp}
\expandafter\gdef\csname R@an.cv.line.amos.V6A1rP3c\endcsname{HyReX-k9 (30.70\,M parameters) minus the function-identical control (31.12\,M): \ensuremath{+0.23}\,pp over the four folds, improves on the control in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.03} to \ensuremath{+0.44}\,pp, which lies inside $\pm$0.50\,pp and above zero}
\expandafter\gdef\csname R@an.cv.line.amos.V6A1rP3c3\endcsname{HyReX-k9 (30.70\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.V6A1rbase\endcsname{HyReX-k9 (30.70\,M parameters) minus the default (31.12\,M): \ensuremath{+0.20}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.34} to \ensuremath{+0.74}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.V7A1P3c\endcsname{LeanDeepMid (31.00\,M parameters) minus the function-identical control (31.12\,M): \ensuremath{+0.29}\,pp over the four folds, improves on the control in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.06} to \ensuremath{+0.52}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.amos.V7A1P3c3\endcsname{LeanDeepMid (31.00\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.V7A1V5B2\endcsname{LeanDeepMid (31.00\,M parameters) minus LeanAdd-NeXt (21.22\,M): \ensuremath{+0.51}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.26} to \ensuremath{+0.77}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.amos.V7A1base\endcsname{LeanDeepMid (31.00\,M parameters) minus the default (31.12\,M): \ensuremath{+0.26}\,pp over the four folds, improves on average (2/4 folds), 95\,\% over folds \ensuremath{-0.50} to \ensuremath{+1.02}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.V7A2P3c\endcsname{LeanDeepMid+FD (31.12\,M parameters) minus the function-identical control (31.12\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V7A2P3c3\endcsname{LeanDeepMid+FD (31.12\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.V7A2V7A1\endcsname{LeanDeepMid+FD (31.12\,M parameters) minus LeanDeepMid (31.00\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V7A2base\endcsname{LeanDeepMid+FD (31.12\,M parameters) minus the default (31.12\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V7B1P3c\endcsname{LeanSep (20.40\,M parameters) minus the function-identical control (31.12\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V7B1P3c3\endcsname{LeanSep (20.40\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.V7B1V5B2\endcsname{LeanSep (20.40\,M parameters) minus LeanAdd-NeXt (21.22\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V7B1base\endcsname{LeanSep (20.40\,M parameters) minus the default (31.12\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V7B2P3c\endcsname{LeanDil (20.42\,M parameters) minus the function-identical control (31.12\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V7B2P3c3\endcsname{LeanDil (20.42\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.V7B2V5B2\endcsname{LeanDil (20.42\,M parameters) minus LeanAdd-NeXt (21.22\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V7B2base\endcsname{LeanDil (20.42\,M parameters) minus the default (31.12\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V7C1P3c\endcsname{LeanNeXt-s5 (21.08\,M parameters) minus the function-identical control (31.12\,M): \ensuremath{-0.43}\,pp over the four folds, does not improve on it (0/4 folds positive), 95\,\% over folds \ensuremath{-0.69} to \ensuremath{-0.17}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.amos.V7C1P3c3\endcsname{LeanNeXt-s5 (21.08\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.V7C1V5B2\endcsname{LeanNeXt-s5 (21.08\,M parameters) minus LeanAdd-NeXt (21.22\,M): \ensuremath{-0.20}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.56} to \ensuremath{+0.15}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.amos.V7C1base\endcsname{LeanNeXt-s5 (21.08\,M parameters) minus the default (31.12\,M): \ensuremath{-0.46}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-0.81} to \ensuremath{-0.11}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.amos.V8B2P3c\endcsname{Stem1 (21.07\,M parameters) minus the function-identical control (31.12\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.amos.V8B2P3c3\endcsname{Stem1 (21.07\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.12\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.amos.V8B2base\endcsname{Stem1 (21.07\,M parameters) minus the default (31.12\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.kits.D2P3c\endcsname{LeanDec (26.08\,M parameters) minus the function-identical control (31.20\,M): \ensuremath{+0.49}\,pp over the four folds, improves on it on average (3 of 4 folds), 95\,\% over folds \ensuremath{-0.92} to \ensuremath{+1.89}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.D2P3c3\endcsname{LeanDec (26.08\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.D2base\endcsname{LeanDec (26.08\,M parameters) minus the default (31.20\,M): \ensuremath{+1.04}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{-0.03} to \ensuremath{+2.12}\,pp, which reaches just below zero}
\expandafter\gdef\csname R@an.cv.line.kits.L1L1b\endcsname{ResEnc-M (102.35\,M parameters) minus ResEnc-matched (102.43\,M): \ensuremath{+0.60}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.45} to \ensuremath{+1.66}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.L1L3\endcsname{ResEnc-M (102.35\,M parameters) minus HyReX (29.66\,M): \ensuremath{+1.47}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{-0.24} to \ensuremath{+3.17}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.L1P3c\endcsname{ResEnc-M (102.35\,M parameters) minus the function-identical control (31.20\,M): \ensuremath{+1.59}\,pp over the four folds, improves on the control in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{-0.63} to \ensuremath{+3.80}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.L1P3c3\endcsname{ResEnc-M (102.35\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.L1bL3\endcsname{ResEnc-matched (102.43\,M parameters) minus HyReX (29.66\,M): \ensuremath{+0.86}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{-0.10} to \ensuremath{+1.82}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.L1base\endcsname{ResEnc-M (102.35\,M parameters) minus the default (31.20\,M): \ensuremath{+2.15}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+0.98} to \ensuremath{+3.32}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.kits.L3P3c\endcsname{HyReX (29.66\,M parameters) minus the function-identical control (31.20\,M): \ensuremath{+0.12}\,pp over the four folds, improves on average (2/4 folds), 95\,\% over folds \ensuremath{-0.73} to \ensuremath{+0.98}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.L3base\endcsname{HyReX (29.66\,M parameters) minus the default (31.20\,M): \ensuremath{+0.68}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-1.08} to \ensuremath{+2.44}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.P3cbase\endcsname{the function-identical control (31.20\,M parameters) minus the default (31.20\,M): \ensuremath{+0.56}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-1.71} to \ensuremath{+2.82}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V5B1D2\endcsname{LeanAdd (20.96\,M parameters) minus LeanDec (26.08\,M): \ensuremath{-0.05}\,pp over the four folds, does not improve in cross-validation (2/4 folds positive), 95\,\% over folds \ensuremath{-0.79} to \ensuremath{+0.69}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V5B1P3c\endcsname{LeanAdd (20.96\,M parameters) minus the function-identical control (31.20\,M): \ensuremath{+0.44}\,pp over the four folds, improves on it on average (2 of 4 folds), 95\,\% over folds \ensuremath{-1.30} to \ensuremath{+2.17}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V5B1P3c3\endcsname{LeanAdd (20.96\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.V5B1base\endcsname{LeanAdd (20.96\,M parameters) minus the default (31.20\,M): \ensuremath{+0.99}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.59} to \ensuremath{+2.58}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V5B2L3\endcsname{LeanAdd-NeXt (21.26\,M parameters) minus HyReX (29.66\,M): \ensuremath{-1.43}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-2.34} to \ensuremath{-0.52}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.kits.V5B2P3c\endcsname{LeanAdd-NeXt (21.26\,M parameters) minus the function-identical control (31.20\,M): \ensuremath{-1.31}\,pp over the four folds, does not improve on it (0/4 folds positive), 95\,\% over folds \ensuremath{-1.86} to \ensuremath{-0.76}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.kits.V5B2P3c3\endcsname{LeanAdd-NeXt (21.26\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.V5B2V5B1\endcsname{LeanAdd-NeXt (21.26\,M parameters) minus LeanAdd (20.96\,M): \ensuremath{-1.75}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-2.97} to \ensuremath{-0.52}\,pp, which lies below zero}
\expandafter\gdef\csname R@an.cv.line.kits.V5B2base\endcsname{LeanAdd-NeXt (21.26\,M parameters) minus the default (31.20\,M): \ensuremath{-0.75}\,pp over the four folds, does not improve in cross-validation (1/4 folds positive), 95\,\% over folds \ensuremath{-2.69} to \ensuremath{+1.18}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V6A1rL3\endcsname{HyReX-k9 (30.78\,M parameters) minus HyReX (29.66\,M): \ensuremath{-0.40}\,pp over the four folds, does not improve in cross-validation (1/4 folds positive), 95\,\% over folds \ensuremath{-1.62} to \ensuremath{+0.82}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V6A1rP3c\endcsname{HyReX-k9 (30.78\,M parameters) minus the function-identical control (31.20\,M): \ensuremath{-0.28}\,pp over the four folds, does not improve on it (2/4 folds positive), 95\,\% over folds \ensuremath{-1.53} to \ensuremath{+0.98}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V6A1rP3c3\endcsname{HyReX-k9 (30.78\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.V6A1rbase\endcsname{HyReX-k9 (30.78\,M parameters) minus the default (31.20\,M): \ensuremath{+0.28}\,pp over the four folds, improves on average (2/4 folds), 95\,\% over folds \ensuremath{-1.42} to \ensuremath{+1.98}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V7A1P3c\endcsname{LeanDeepMid (31.04\,M parameters) minus the function-identical control (31.20\,M): \ensuremath{+1.08}\,pp over the four folds, improves on it on average (3 of 4 folds), 95\,\% over folds \ensuremath{-0.66} to \ensuremath{+2.81}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V7A1P3c3\endcsname{LeanDeepMid (31.04\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.V7A1V5B2\endcsname{LeanDeepMid (31.04\,M parameters) minus LeanAdd-NeXt (21.26\,M): \ensuremath{+2.39}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+1.18} to \ensuremath{+3.59}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.kits.V7A1base\endcsname{LeanDeepMid (31.04\,M parameters) minus the default (31.20\,M): \ensuremath{+1.63}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{0.00} to \ensuremath{+3.27}\,pp, which touches zero}
\expandafter\gdef\csname R@an.cv.line.kits.V7A2P3c\endcsname{LeanDeepMid+FD (31.18\,M parameters) minus the function-identical control (31.20\,M): \ensuremath{+0.35}\,pp over the four folds, improves on it on average (3 of 4 folds), 95\,\% over folds \ensuremath{-0.67} to \ensuremath{+1.37}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V7A2P3c3\endcsname{LeanDeepMid+FD (31.18\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.V7A2V7A1\endcsname{LeanDeepMid+FD (31.18\,M parameters) minus LeanDeepMid (31.04\,M): \ensuremath{-0.73}\,pp over the four folds, does not improve in cross-validation (0/4 folds positive), 95\,\% over folds \ensuremath{-1.65} to \ensuremath{+0.20}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V7A2base\endcsname{LeanDeepMid+FD (31.18\,M parameters) minus the default (31.20\,M): \ensuremath{+0.91}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.45} to \ensuremath{+2.27}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V7B1P3c\endcsname{LeanSep (20.43\,M parameters) minus the function-identical control (31.20\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.kits.V7B1P3c3\endcsname{LeanSep (20.43\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.V7B1V5B2\endcsname{LeanSep (20.43\,M parameters) minus LeanAdd-NeXt (21.26\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.kits.V7B1base\endcsname{LeanSep (20.43\,M parameters) minus the default (31.20\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.kits.V7B2P3c\endcsname{LeanDil (20.45\,M parameters) minus the function-identical control (31.20\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.kits.V7B2P3c3\endcsname{LeanDil (20.45\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.V7B2V5B2\endcsname{LeanDil (20.45\,M parameters) minus LeanAdd-NeXt (21.26\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.kits.V7B2base\endcsname{LeanDil (20.45\,M parameters) minus the default (31.20\,M): none of the four per-fold differences is finished}
\expandafter\gdef\csname R@an.cv.line.kits.V7C1P3c\endcsname{LeanNeXt-s5 (21.11\,M parameters) minus the function-identical control (31.20\,M): \ensuremath{+0.23}\,pp over the four folds, improves on it on average (2 of 4 folds), 95\,\% over folds \ensuremath{-0.47} to \ensuremath{+0.92}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V7C1P3c3\endcsname{LeanNeXt-s5 (21.11\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.V7C1V5B2\endcsname{LeanNeXt-s5 (21.11\,M parameters) minus LeanAdd-NeXt (21.26\,M): \ensuremath{+1.54}\,pp over the four folds, improves in every fold (4/4 folds positive), 95\,\% over folds \ensuremath{+1.20} to \ensuremath{+1.88}\,pp, which lies above zero}
\expandafter\gdef\csname R@an.cv.line.kits.V7C1base\endcsname{LeanNeXt-s5 (21.11\,M parameters) minus the default (31.20\,M): \ensuremath{+0.78}\,pp over the four folds, improves on average (3/4 folds), 95\,\% over folds \ensuremath{-0.92} to \ensuremath{+2.48}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V8B2P3c\endcsname{Stem1 (21.08\,M parameters) minus the function-identical control (31.20\,M): \ensuremath{-0.80}\,pp over the four folds, does not improve on it (0/4 folds positive), 95\,\% over folds \ensuremath{-1.68} to \ensuremath{+0.08}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.line.kits.V8B2P3c3\endcsname{Stem1 (21.08\,M parameters) minus the function-identical control's three-seed mean of the same fold (31.20\,M) (secondary reading): pending until the control's seed-1 and seed-2 runs of every fold have finished (none of the 24 are in)}
\expandafter\gdef\csname R@an.cv.line.kits.V8B2base\endcsname{Stem1 (21.08\,M parameters) minus the default (31.20\,M): \ensuremath{-0.24}\,pp over the four folds, does not improve in cross-validation (3/4 folds positive), 95\,\% over folds \ensuremath{-2.62} to \ensuremath{+2.13}\,pp, which includes zero}
\expandafter\gdef\csname R@an.cv.lit.acdc.nnunet\endcsname{91.54}
\expandafter\gdef\csname R@an.cv.lit.acdc.resencm\endcsname{91.99}
\expandafter\gdef\csname R@an.cv.lit.acdc.resencm_minus_nnunet\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.lit.amos.nnunet\endcsname{88.64}
\expandafter\gdef\csname R@an.cv.lit.amos.resencm\endcsname{88.77}
\expandafter\gdef\csname R@an.cv.lit.amos.resencm_minus_nnunet\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.cv.lit.kits.nnunet\endcsname{86.04}
\expandafter\gdef\csname R@an.cv.lit.kits.resencm\endcsname{86.79}
\expandafter\gdef\csname R@an.cv.lit.kits.resencm_minus_nnunet\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.cv.n.acdc\endcsname{200}
\expandafter\gdef\csname R@an.cv.n.amos\endcsname{200}
\expandafter\gdef\csname R@an.cv.n.kits\endcsname{489}
\expandafter\gdef\csname R@an.cv.nfolds\endcsname{4}
\expandafter\gdef\csname R@an.cv.nfolds.total\endcsname{5}
\expandafter\gdef\csname R@an.cv.nfolds.total.word\endcsname{five}
\expandafter\gdef\csname R@an.cv.nfolds.word\endcsname{four}
\expandafter\gdef\csname R@an.cv.nval.acdc.f1\endcsname{40}
\expandafter\gdef\csname R@an.cv.nval.acdc.f2\endcsname{40}
\expandafter\gdef\csname R@an.cv.nval.acdc.f3\endcsname{40}
\expandafter\gdef\csname R@an.cv.nval.acdc.f4\endcsname{40}
\expandafter\gdef\csname R@an.cv.nval.amos.f1\endcsname{40}
\expandafter\gdef\csname R@an.cv.nval.amos.f2\endcsname{40}
\expandafter\gdef\csname R@an.cv.nval.amos.f3\endcsname{40}
\expandafter\gdef\csname R@an.cv.nval.amos.f4\endcsname{40}
\expandafter\gdef\csname R@an.cv.nval.kits.f1\endcsname{98}
\expandafter\gdef\csname R@an.cv.nval.kits.f2\endcsname{98}
\expandafter\gdef\csname R@an.cv.nval.kits.f3\endcsname{98}
\expandafter\gdef\csname R@an.cv.nval.kits.f4\endcsname{97}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.boot14.hi\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.boot14.lo\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{-0.11} to \ensuremath{+0.19}\,pp}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.11} to \ensuremath{+0.19}\,pp over the 160 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.fracpos\endcsname{47.0}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.fracpos14\endcsname{50.6}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.half14\endcsname{7}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.halfshare14\endcsname{9}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.mean\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.mean14\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.measured\endcsname{ResEnc-M improves on HyReX in 50.6\,\% of the 160 held-out cases (median \ensuremath{+0.01}\,pp), and the 10 largest gains carry 59\,\% of all gains}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.median\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.median14\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.n\endcsname{200}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.n0\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.n14\endcsname{160}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.npos\endcsname{94}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.npos14\endcsname{81}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.topshare\endcsname{54}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.topshare14\endcsname{59}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.topuniform14\endcsname{12.3}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.trim\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1L3.trim14\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.boot14.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.boot14.lo\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{+0.20} to \ensuremath{+0.54}\,pp}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.20} to \ensuremath{+0.54}\,pp over the 160 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.fracpos\endcsname{66.0}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.fracpos14\endcsname{61.9}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.half14\endcsname{14}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.halfshare14\endcsname{14}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.mean\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.mean14\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.measured\endcsname{ResEnc-M improves on the default in 61.9\,\% of the 160 held-out cases (median \ensuremath{+0.13}\,pp), and the 10 largest gains carry 42\,\% of all gains}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.median\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.median14\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.n\endcsname{200}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.n0\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.n14\endcsname{160}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.npos\endcsname{132}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.npos14\endcsname{99}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.scope\endcsname{one held-out value per development case over folds 0--4; the 40-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for ResEnc-M and frozen pool for default), a 2- and 6-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.topshare\endcsname{37}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.topshare14\endcsname{42}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.topuniform14\endcsname{10.1}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.trim\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L1base.trim14\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.boot14.hi\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.boot14.lo\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{-0.20} to \ensuremath{+0.11}\,pp}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.20} to \ensuremath{+0.11}\,pp over the 160 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.fracpos\endcsname{53.0}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.fracpos14\endcsname{49.4}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.half14\endcsname{11}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.halfshare14\endcsname{14}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.mean\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.mean14\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.measured\endcsname{HyReX improves on ResEnc-M in 49.4\,\% of the 160 held-out cases (median \ensuremath{-0.01}\,pp), and the 10 largest gains carry 50\,\% of all gains}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.median\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.median14\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.n\endcsname{200}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.n0\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.n14\endcsname{160}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.npos\endcsname{106}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.npos14\endcsname{79}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.scope\endcsname{one held-out value per development case over folds 0--4; the 40-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for HyReX and for ResEnc-M), a 2-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.topshare\endcsname{43}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.topshare14\endcsname{50}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.topuniform14\endcsname{12.7}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.trim\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3L1.trim14\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.boot14.hi\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.boot14.lo\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{+0.18} to \ensuremath{+0.48}\,pp}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.18} to \ensuremath{+0.48}\,pp over the 160 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.fracpos\endcsname{68.5}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.fracpos14\endcsname{65.6}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.half14\endcsname{14}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.halfshare14\endcsname{13}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.mean\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.mean14\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.measured\endcsname{HyReX improves on the default in 65.6\,\% of the 160 held-out cases (median \ensuremath{+0.15}\,pp), and the 10 largest gains carry 41\,\% of all gains}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.median\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.median14\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.n\endcsname{200}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.n0\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.n14\endcsname{160}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.npos\endcsname{137}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.npos14\endcsname{105}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.scope\endcsname{one held-out value per development case over folds 0--4; the 40-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for HyReX and frozen pool for default), a 2- and 6-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.topshare\endcsname{34}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.topshare14\endcsname{41}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.topuniform14\endcsname{9.5}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.trim\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.oof.acdc.L3base.trim14\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.boot14.hi\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.boot14.lo\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{-0.51} to \ensuremath{-0.23}\,pp}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.51} to \ensuremath{-0.23}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.fracpos\endcsname{28.0}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.fracpos14\endcsname{27.5}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.half14\endcsname{7}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.halfshare14\endcsname{16}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.mean\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.mean14\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.measured\endcsname{LeanDec improves on the default in 27.5\,\% of the 160 held-out cases (median \ensuremath{-0.26}\,pp), and the 10 largest gains carry 62\,\% of all gains (scored over non-empty-reference pairs)}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.median\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.median14\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.n\endcsname{200}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.n0\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.n14\endcsname{160}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.npos\endcsname{56}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.npos14\endcsname{44}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.scope\endcsname{one held-out value per development case over folds 0--4; the 40-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (seed 0 for LeanDec and frozen pool for default), a 1- and 6-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.topshare\endcsname{51}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.topshare14\endcsname{62}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.topuniform14\endcsname{22.7}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.trim\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.cv.oof.amos.D2base.trim14\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.boot14.hi\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.boot14.lo\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{-0.08} to \ensuremath{+0.21}\,pp}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.08} to \ensuremath{+0.21}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.fracpos\endcsname{57.5}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.fracpos14\endcsname{56.2}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.half14\endcsname{15}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.halfshare14\endcsname{17}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.mean\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.mean14\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.measured\endcsname{ResEnc-M improves on HyReX in 56.2\,\% of the 160 held-out cases (median \ensuremath{+0.05}\,pp), and the 10 largest gains carry 40\,\% of all gains (scored over non-empty-reference pairs)}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.median\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.median14\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.n\endcsname{200}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.n0\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.n14\endcsname{160}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.npos\endcsname{115}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.npos14\endcsname{90}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.topshare\endcsname{34}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.topshare14\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.topuniform14\endcsname{11.1}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.trim\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1L3.trim14\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.boot14.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.boot14.lo\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{+0.20} to \ensuremath{+0.54}\,pp}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.20} to \ensuremath{+0.54}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.fracpos\endcsname{72.0}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.fracpos14\endcsname{68.8}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.half14\endcsname{16}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.halfshare14\endcsname{15}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.mean\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.mean14\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.measured\endcsname{ResEnc-M improves on the default in 68.8\,\% of the 160 held-out cases (median \ensuremath{+0.20}\,pp), and the 10 largest gains carry 39\,\% of all gains (scored over non-empty-reference pairs)}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.median\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.median14\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.n\endcsname{200}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.n0\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.n14\endcsname{160}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.npos\endcsname{144}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.npos14\endcsname{110}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.scope\endcsname{one held-out value per development case over folds 0--4; the 40-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for ResEnc-M and frozen pool for default), a 2- and 6-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.topshare\endcsname{32}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.topshare14\endcsname{39}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.topuniform14\endcsname{9.1}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.trim\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.cv.oof.amos.L1base.trim14\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.boot14.hi\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.boot14.lo\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{-0.21} to \ensuremath{+0.08}\,pp}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.21} to \ensuremath{+0.08}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.fracpos\endcsname{42.5}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.fracpos14\endcsname{43.8}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.half14\endcsname{11}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.halfshare14\endcsname{16}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.mean\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.mean14\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.measured\endcsname{HyReX improves on ResEnc-M in 43.8\,\% of the 160 held-out cases (median \ensuremath{-0.05}\,pp), and the 10 largest gains carry 49\,\% of all gains (scored over non-empty-reference pairs)}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.median\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.median14\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.n\endcsname{200}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.n0\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.n14\endcsname{160}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.npos\endcsname{85}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.npos14\endcsname{70}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.scope\endcsname{one held-out value per development case over folds 0--4; the 40-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for HyReX and for ResEnc-M), a 2-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.topshare\endcsname{45}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.topshare14\endcsname{49}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.topuniform14\endcsname{14.3}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.trim\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3L1.trim14\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.boot14.hi\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.boot14.lo\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{+0.12} to \ensuremath{+0.47}\,pp}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.12} to \ensuremath{+0.47}\,pp over the 160 held-out cases, scored over non-empty-reference pairs (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.fracpos\endcsname{69.0}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.fracpos14\endcsname{68.1}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.half14\endcsname{16}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.halfshare14\endcsname{15}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.mean\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.mean14\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.measured\endcsname{HyReX improves on the default in 68.1\,\% of the 160 held-out cases (median \ensuremath{+0.23}\,pp), and the 10 largest gains carry 38\,\% of all gains (scored over non-empty-reference pairs)}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.median\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.median14\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.n\endcsname{200}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.n0\endcsname{40}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.n14\endcsname{160}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.npos\endcsname{138}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.npos14\endcsname{109}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.scope\endcsname{one held-out value per development case over folds 0--4; the 40-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for HyReX and frozen pool for default), a 2- and 6-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.topshare\endcsname{32}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.topshare14\endcsname{38}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.topuniform14\endcsname{9.2}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.trim\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.cv.oof.amos.L3base.trim14\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.cv.oof.amos.estimand\endcsname{the AMOS22 case-level scores are taken over the (case, class) pairs whose reference is non-empty, a different estimand from the headline Dice that the cross-validated difference averages, so a case-level mean and the cross-validated difference differ by estimand and not only by sampling}
\expandafter\gdef\csname R@an.cv.oof.gainfrac\endcsname{50\,\%}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.boot14.hi\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.boot14.lo\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{+0.36} to \ensuremath{+1.76}\,pp}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.36} to \ensuremath{+1.76}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.fracpos\endcsname{53.0}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.fracpos14\endcsname{50.6}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.half14\endcsname{20}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.halfshare14\endcsname{10}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.mean\endcsname{\ensuremath{+1.22}}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.mean14\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.measured\endcsname{LeanDec improves on the default in 50.6\,\% of the 391 held-out cases (median \ensuremath{+0.01}\,pp), and the 10 largest gains carry 32\,\% of all gains}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.median\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.median14\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.n\endcsname{489}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.n0\endcsname{98}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.n14\endcsname{391}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.npos\endcsname{259}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.npos14\endcsname{198}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.scope\endcsname{one held-out value per development case over folds 0--4; the 98-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for LeanDec and frozen pool for default), a 2- and 3-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.topshare\endcsname{26}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.topshare14\endcsname{32}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.topuniform14\endcsname{5.1}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.trim\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.cv.oof.kits.D2base.trim14\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.boot14.hi\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.boot14.lo\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{+0.52} to \ensuremath{+2.36}\,pp}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+0.52} to \ensuremath{+2.36}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.fracpos\endcsname{55.8}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.fracpos14\endcsname{54.5}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.half14\endcsname{20}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.halfshare14\endcsname{9}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.mean\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.mean14\endcsname{\ensuremath{+1.46}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.measured\endcsname{ResEnc-M improves on HyReX in 54.5\,\% of the 391 held-out cases (median \ensuremath{+0.12}\,pp), and the 10 largest gains carry 32\,\% of all gains}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.median\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.median14\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.n\endcsname{489}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.n0\endcsname{98}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.n14\endcsname{391}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.npos\endcsname{273}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.npos14\endcsname{213}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.topshare\endcsname{28}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.topshare14\endcsname{32}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.topuniform14\endcsname{4.7}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.trim\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1L3.trim14\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.boot14.hi\endcsname{\ensuremath{+3.08}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.boot14.lo\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{+1.28} to \ensuremath{+3.08}\,pp}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{+1.28} to \ensuremath{+3.08}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.fracpos\endcsname{64.8}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.fracpos14\endcsname{61.4}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.half14\endcsname{21}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.halfshare14\endcsname{9}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.mean\endcsname{\ensuremath{+2.41}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.mean14\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.measured\endcsname{ResEnc-M improves on the default in 61.4\,\% of the 391 held-out cases (median \ensuremath{+0.30}\,pp), and the 10 largest gains carry 31\,\% of all gains}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.median\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.median14\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.n\endcsname{489}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.n0\endcsname{98}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.n14\endcsname{391}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.npos\endcsname{317}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.npos14\endcsname{240}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.scope\endcsname{one held-out value per development case over folds 0--4; the 98-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for ResEnc-M and frozen pool for default), a 2- and 3-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.topshare\endcsname{25}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.topshare14\endcsname{31}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.topuniform14\endcsname{4.2}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.trim\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@an.cv.oof.kits.L1base.trim14\endcsname{\ensuremath{+0.91}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.boot14.hi\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.boot14.lo\endcsname{\ensuremath{-2.42}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{-2.42} to \ensuremath{-0.59}\,pp}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-2.42} to \ensuremath{-0.59}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.fracpos\endcsname{44.2}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.fracpos14\endcsname{45.5}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.half14\endcsname{11}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.halfshare14\endcsname{6}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.mean\endcsname{\ensuremath{-1.45}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.mean14\endcsname{\ensuremath{-1.46}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.measured\endcsname{HyReX improves on ResEnc-M in 45.5\,\% of the 391 held-out cases (median \ensuremath{-0.12}\,pp), and the 10 largest gains carry 48\,\% of all gains}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.median\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.median14\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.n\endcsname{489}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.n0\endcsname{98}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.n14\endcsname{391}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.npos\endcsname{216}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.npos14\endcsname{178}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.scope\endcsname{one held-out value per development case over folds 0--4; the 98-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for HyReX and for ResEnc-M), a 2-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.topshare\endcsname{42}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.topshare14\endcsname{48}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.topuniform14\endcsname{5.6}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.trim\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3L1.trim14\endcsname{\ensuremath{-0.65}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.boot14.b\endcsname{2000}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.boot14.hi\endcsname{\ensuremath{+1.54}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.boot14.lo\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.boot14.short\endcsname{a case-bootstrap 95\,\% interval from \ensuremath{-0.16} to \ensuremath{+1.54}\,pp}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.boot14.word\endcsname{a case-bootstrap 95\,\% interval of the mean per-case difference from \ensuremath{-0.16} to \ensuremath{+1.54}\,pp over the 391 held-out cases (2000 resamples of the cases with the trained networks held fixed: case sampling only, no training-seed or fold-to-fold variation)}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.fracpos\endcsname{58.3}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.fracpos14\endcsname{55.8}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.half14\endcsname{19}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.halfshare14\endcsname{9}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.mean\endcsname{\ensuremath{+0.97}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.mean14\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.measured\endcsname{HyReX improves on the default in 55.8\,\% of the 391 held-out cases (median \ensuremath{+0.16}\,pp), and the 10 largest gains carry 34\,\% of all gains}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.median\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.median14\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.n\endcsname{489}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.n0\endcsname{98}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.n14\endcsname{391}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.npos\endcsname{285}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.npos14\endcsname{218}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q1\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q1n\endcsname{98}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q2\endcsname{\ensuremath{+2.38}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q2n\endcsname{98}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q3\endcsname{\ensuremath{-1.36}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q3n\endcsname{98}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q4\endcsname{\ensuremath{+1.54}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q4n\endcsname{98}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q5\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.q5n\endcsname{97}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.scope\endcsname{one held-out value per development case over folds 0--4; the 98-case fold-0 block is the selection fold and enters from the least-selected fold-0 estimate (fresh s1-2 for HyReX and frozen pool for default), a 2- and 3-run per-case average against the single runs of folds 1--4}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.topshare\endcsname{28}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.topshare14\endcsname{34}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.topuniform14\endcsname{4.6}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.trim\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.cv.oof.kits.L3base.trim14\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.oof.kits.quintile.basis\endcsname{physical tumour volume}
\expandafter\gdef\csname R@an.cv.oof.kits.quintile.unit\endcsname{mL}
\expandafter\gdef\csname R@an.cv.oof.top\endcsname{10}
\expandafter\gdef\csname R@an.cv.oof.topword\endcsname{ten}
\expandafter\gdef\csname R@an.cv.p3c.bandnote\endcsname{The grey band marks two standard deviations of a one-seed pair difference of that dataset and locates each per-fold difference on the seed-noise scale of that dataset}
\expandafter\gdef\csname R@an.cv.p3c.def\endcsname{the nnU-Net default network rebuilt through the plan-aware family in which every agent design and every other control is built (the same function as the default, a different implementation)}
\expandafter\gdef\csname R@an.cv.p3c.name\endcsname{function-identical control}
\expandafter\gdef\csname R@an.cv.p6.condition\endcsname{AMOS22 \ensuremath{-0.36}\,pp; KiTS23 \ensuremath{+2.36}\,pp}
\expandafter\gdef\csname R@an.cv.p6.condition.state\endcsname{fails}
\expandafter\gdef\csname R@an.cv.p6.deviation.limit\endcsname{The cross-validation of LeanDec departs from a registered clause: Addendum P6's condition failed (AMOS22 \ensuremath{-0.36}\,pp; KiTS23 \ensuremath{+2.36}\,pp against a \ensuremath{-0.15}\,pp line) and the runs were queued afterwards under Addendum AB and Addendum AA, whose own margin, \ensuremath{-0.50}\,pp, is looser than P6's and was fixed after the failing result was known. Both readings are printed: LeanDec minus the default is \ensuremath{+0.30}\,pp on average over the two co-primary benchmarks, at or above the \ensuremath{-0.15}\,pp margin of Addendum P6; LeanDec minus the default is \ensuremath{+0.30}\,pp on average over the two co-primary benchmarks, at or above the \ensuremath{-0.50}\,pp margin of Addendum AA target T2.}
\expandafter\gdef\csname R@an.cv.p6.deviation.limit.both\endcsname{The cross-validation of LeanDec departs from a registered clause: Addendum P6's condition failed (AMOS22 \ensuremath{-0.36}\,pp; KiTS23 \ensuremath{+2.36}\,pp against a \ensuremath{-0.15}\,pp line) and the runs were queued afterwards under Addendum AB and Addendum AA, whose own margin, \ensuremath{-0.50}\,pp, is looser than P6's and was fixed after the failing result was known. Both readings are printed: LeanDec minus the default is \ensuremath{+0.30}\,pp on average over the two co-primary benchmarks (AMOS22 and KiTS23; the registered reading of Addendum AB4), at or above the \ensuremath{-0.15}\,pp margin of Addendum P6 and at or above the \ensuremath{-0.50}\,pp margin of Addendum AA target T2.}
\expandafter\gdef\csname R@an.cv.p6.deviation.registered\endcsname{Addendum AB and Addendum AA}
\expandafter\gdef\csname R@an.cv.p6.deviation.sentence\endcsname{The registered condition of Addendum P6 for a cross-validation of LeanDec -- a fold-0 seed-0 Dice at least \ensuremath{-0.15}\,pp from the frozen default pool on every co-primary benchmark -- failed (AMOS22 \ensuremath{-0.36}\,pp; KiTS23 \ensuremath{+2.36}\,pp), so Addendum P6 owed it none; the cross-validation was nevertheless run, under Addendum AB and Addendum AA, by a decision of the lead taken after that failure was known, and is reported here with the failure.}
\expandafter\gdef\csname R@an.cv.p6.floor\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.p6.margin.both.clause\endcsname{LeanDec minus the default is \ensuremath{+0.30}\,pp on average over the two co-primary benchmarks (AMOS22 and KiTS23; the registered reading of Addendum AB4), at or above the \ensuremath{-0.15}\,pp margin of Addendum P6 and at or above the \ensuremath{-0.50}\,pp margin of Addendum AA target T2}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.acdc\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.acdc.met\endcsname{met}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.amos\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.amos.met\endcsname{not met}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.clause\endcsname{LeanDec minus the default is \ensuremath{+0.30}\,pp on average over the two co-primary benchmarks, at or above the \ensuremath{-0.15}\,pp margin of Addendum P6}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.kits\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.kits.met\endcsname{met}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.mean\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.mean.met\endcsname{met}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.ndone\endcsname{2}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.src\endcsname{Addendum P6}
\expandafter\gdef\csname R@an.cv.p6.margin.p6.value\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.acdc\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.acdc.met\endcsname{met}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.amos\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.amos.met\endcsname{met}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.clause\endcsname{LeanDec minus the default is \ensuremath{+0.30}\,pp on average over the two co-primary benchmarks, at or above the \ensuremath{-0.50}\,pp margin of Addendum AA target T2}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.kits\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.kits.met\endcsname{met}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.mean\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.mean.met\endcsname{met}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.ndone\endcsname{2}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.src\endcsname{Addendum AA target T2}
\expandafter\gdef\csname R@an.cv.p6.margin.t2.value\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.cv.p6.note\endcsname{Addendum P6 is queued: the twelve ai\_benchcvD2 runs add the (LeanDec, default) pair under the same estimands, and their per-fold Dice is in the LeanDec per-fold table}
\expandafter\gdef\csname R@an.cv.pairsd.acdc\endcsname{0.14}
\expandafter\gdef\csname R@an.cv.pairsd.amos\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.pairsd.kits\endcsname{1.12}
\expandafter\gdef\csname R@an.cv.pool.acdc.mean\endcsname{92.009}
\expandafter\gdef\csname R@an.cv.pool.acdc.n\endcsname{6}
\expandafter\gdef\csname R@an.cv.pool.acdc.sd\endcsname{0.099}
\expandafter\gdef\csname R@an.cv.pool.amos.mean\endcsname{87.701}
\expandafter\gdef\csname R@an.cv.pool.amos.n\endcsname{6}
\expandafter\gdef\csname R@an.cv.pool.amos.sd\endcsname{0.122}
\expandafter\gdef\csname R@an.cv.pool.kits.mean\endcsname{83.378}
\expandafter\gdef\csname R@an.cv.pool.kits.n\endcsname{3}
\expandafter\gdef\csname R@an.cv.pool.kits.sd\endcsname{0.795}
\expandafter\gdef\csname R@an.cv.pos.acdc.measured\endcsname{our ResEnc-M five-fold margin over our own default is \ensuremath{+0.34}\,pp (\ensuremath{+0.34}\,pp against the uncompiled sub-pool; fold-0 fifth: fresh s1-2 for ResEnc-M and frozen pool for default), against the published \ensuremath{+0.45}\,pp over the published default, a gap of 0.11\,pp}
\expandafter\gdef\csname R@an.cv.pos.acdc.reprogap\endcsname{0.11}
\expandafter\gdef\csname R@an.cv.pos.all\endcsname{yes}
\expandafter\gdef\csname R@an.cv.pos.amos.measured\endcsname{our ResEnc-M five-fold margin over our own default is \ensuremath{+0.42}\,pp (\ensuremath{+0.42}\,pp against the contemporaneous default runs; fold-0 fifth: fresh s1-2 for ResEnc-M and frozen pool for default), against the published \ensuremath{+0.13}\,pp over the published default, a gap of 0.29\,pp}
\expandafter\gdef\csname R@an.cv.pos.amos.reprogap\endcsname{0.29}
\expandafter\gdef\csname R@an.cv.pos.everynames\endcsname{ACDC}
\expandafter\gdef\csname R@an.cv.pos.kits.measured\endcsname{our ResEnc-M five-fold margin over our own default is \ensuremath{+2.41}\,pp (\ensuremath{+2.36}\,pp against the six-run pool; fold-0 fifth: fresh s1-2 for ResEnc-M and frozen pool for default), against the published \ensuremath{+0.75}\,pp over the published default, a gap of 1.66\,pp}
\expandafter\gdef\csname R@an.cv.pos.kits.reprogap\endcsname{1.66}
\expandafter\gdef\csname R@an.cv.pos.n\endcsname{3}
\expandafter\gdef\csname R@an.cv.pos.n.word\endcsname{three}
\expandafter\gdef\csname R@an.cv.pos.names\endcsname{AMOS22, KiTS23 and ACDC}
\expandafter\gdef\csname R@an.cv.pos.nds\endcsname{3}
\expandafter\gdef\csname R@an.cv.pos.nds.word\endcsname{three}
\expandafter\gdef\csname R@an.cv.pos.nevery\endcsname{1}
\expandafter\gdef\csname R@an.cv.pos.notnames\endcsname{none}
\expandafter\gdef\csname R@an.cv.pos.pendnames\endcsname{none}
\expandafter\gdef\csname R@an.cv.pos.sentence\endcsname{HyReX's selection-free mean contrast with the stock default is positive on all three development datasets (AMOS22, KiTS23 and ACDC); the registered wording per dataset, with its interval over folds and its fold count, is in the cross-validation summary table}
\expandafter\gdef\csname R@an.cv.pos.short\endcsname{positive on all three development datasets (AMOS22, KiTS23 and ACDC)}
\expandafter\gdef\csname R@an.cv.pos.total\endcsname{3}
\expandafter\gdef\csname R@an.cv.posctl.all\endcsname{yes}
\expandafter\gdef\csname R@an.cv.posctl.everynames\endcsname{AMOS22 and ACDC}
\expandafter\gdef\csname R@an.cv.posctl.n\endcsname{3}
\expandafter\gdef\csname R@an.cv.posctl.n.word\endcsname{three}
\expandafter\gdef\csname R@an.cv.posctl.names\endcsname{AMOS22, KiTS23 and ACDC}
\expandafter\gdef\csname R@an.cv.posctl.nds\endcsname{3}
\expandafter\gdef\csname R@an.cv.posctl.nds.word\endcsname{three}
\expandafter\gdef\csname R@an.cv.posctl.nevery\endcsname{2}
\expandafter\gdef\csname R@an.cv.posctl.notnames\endcsname{none}
\expandafter\gdef\csname R@an.cv.posctl.pendnames\endcsname{none}
\expandafter\gdef\csname R@an.cv.posctl.sentence\endcsname{HyReX's selection-free mean contrast with its function-identical control is positive in the mean on all three development datasets (AMOS22, KiTS23 and ACDC) and in every fold on two (AMOS22 and ACDC); the registered wording per dataset, with its interval over folds and its fold count, is in the table of the control's cross-validation lines}
\expandafter\gdef\csname R@an.cv.posctl.short\endcsname{positive in the mean on all three development datasets (AMOS22, KiTS23 and ACDC) and in every fold on two (AMOS22 and ACDC)}
\expandafter\gdef\csname R@an.cv.posctl.total\endcsname{3}
\expandafter\gdef\csname R@an.cv.ref.acdc.alt\endcsname{uncompiled sub-pool, 3 runs, \ensuremath{+0.007} pp against the frozen pool}
\expandafter\gdef\csname R@an.cv.ref.acdc.altkey\endcsname{uncompiled}
\expandafter\gdef\csname R@an.cv.ref.acdc.frozen.mean\endcsname{92.009}
\expandafter\gdef\csname R@an.cv.ref.acdc.frozen.n\endcsname{6}
\expandafter\gdef\csname R@an.cv.ref.acdc.frozen.shift\endcsname{\ensuremath{0.000}}
\expandafter\gdef\csname R@an.cv.ref.acdc.frozen.short\endcsname{frozen pool}
\expandafter\gdef\csname R@an.cv.ref.acdc.frozen.state\endcsname{available}
\expandafter\gdef\csname R@an.cv.ref.acdc.uncompiled.mean\endcsname{92.016}
\expandafter\gdef\csname R@an.cv.ref.acdc.uncompiled.n\endcsname{3}
\expandafter\gdef\csname R@an.cv.ref.acdc.uncompiled.shift\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.cv.ref.acdc.uncompiled.short\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.cv.ref.acdc.uncompiled.state\endcsname{available}
\expandafter\gdef\csname R@an.cv.ref.amos.alt\endcsname{contemporaneous default runs, 3 runs, \ensuremath{+0.011} pp against the frozen pool}
\expandafter\gdef\csname R@an.cv.ref.amos.altkey\endcsname{contemporaneous}
\expandafter\gdef\csname R@an.cv.ref.amos.contemporaneous.mean\endcsname{87.712}
\expandafter\gdef\csname R@an.cv.ref.amos.contemporaneous.n\endcsname{3}
\expandafter\gdef\csname R@an.cv.ref.amos.contemporaneous.shift\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.cv.ref.amos.contemporaneous.short\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.cv.ref.amos.contemporaneous.state\endcsname{available}
\expandafter\gdef\csname R@an.cv.ref.amos.frozen.mean\endcsname{87.701}
\expandafter\gdef\csname R@an.cv.ref.amos.frozen.n\endcsname{6}
\expandafter\gdef\csname R@an.cv.ref.amos.frozen.shift\endcsname{\ensuremath{0.000}}
\expandafter\gdef\csname R@an.cv.ref.amos.frozen.short\endcsname{frozen pool}
\expandafter\gdef\csname R@an.cv.ref.amos.frozen.state\endcsname{available}
\expandafter\gdef\csname R@an.cv.ref.amos.uncompiled.mean\endcsname{87.730}
\expandafter\gdef\csname R@an.cv.ref.amos.uncompiled.n\endcsname{3}
\expandafter\gdef\csname R@an.cv.ref.amos.uncompiled.shift\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.cv.ref.amos.uncompiled.short\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.cv.ref.amos.uncompiled.state\endcsname{available}
\expandafter\gdef\csname R@an.cv.ref.kits.alt\endcsname{six-run pool, \ensuremath{+0.244} pp against the frozen pool}
\expandafter\gdef\csname R@an.cv.ref.kits.altkey\endcsname{union}
\expandafter\gdef\csname R@an.cv.ref.kits.contemporaneous.mean\endcsname{83.866}
\expandafter\gdef\csname R@an.cv.ref.kits.contemporaneous.n\endcsname{3}
\expandafter\gdef\csname R@an.cv.ref.kits.contemporaneous.shift\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.cv.ref.kits.contemporaneous.short\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.cv.ref.kits.contemporaneous.state\endcsname{available}
\expandafter\gdef\csname R@an.cv.ref.kits.frozen.mean\endcsname{83.378}
\expandafter\gdef\csname R@an.cv.ref.kits.frozen.n\endcsname{3}
\expandafter\gdef\csname R@an.cv.ref.kits.frozen.shift\endcsname{\ensuremath{0.000}}
\expandafter\gdef\csname R@an.cv.ref.kits.frozen.short\endcsname{frozen pool}
\expandafter\gdef\csname R@an.cv.ref.kits.frozen.state\endcsname{available}
\expandafter\gdef\csname R@an.cv.ref.kits.union.mean\endcsname{83.622}
\expandafter\gdef\csname R@an.cv.ref.kits.union.n\endcsname{6}
\expandafter\gdef\csname R@an.cv.ref.kits.union.shift\endcsname{\ensuremath{+0.244}}
\expandafter\gdef\csname R@an.cv.ref.kits.union.short\endcsname{six-run pool}
\expandafter\gdef\csname R@an.cv.ref.kits.union.state\endcsname{available}
\expandafter\gdef\csname R@an.cv.resencm.stock\endcsname{ResEnc-M is the stock library preset and has no function-identical control: the ResEnc-matched re-implementation differs from the preset in the default stem, the shortcut form and the zero-initialisation, so its contrasts with HyReX are read beside each network's contrast with the stock default and, where the like-for-like set has finished, beside the re-implementation, whose own difference from the preset is reported as a re-implementation difference}
\expandafter\gdef\csname R@an.cv.robust.sect\endcsname{\textsuperscript{\S}}
\expandafter\gdef\csname R@an.cv.sec.acdc.D2base.dl\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.sec.acdc.D2base.dlhi\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.sec.acdc.D2base.dllo\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cv.sec.acdc.L1base.dl\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.sec.acdc.L1base.dlhi\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.cv.sec.acdc.L1base.dllo\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.cv.sec.acdc.L3L1.dl\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cv.sec.acdc.L3L1.dlhi\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.cv.sec.acdc.L3L1.dllo\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv.sec.acdc.L3base.dl\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.cv.sec.acdc.L3base.dlhi\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.cv.sec.acdc.L3base.dllo\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.sec.amos.D2base.dl\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.cv.sec.amos.D2base.dlhi\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.cv.sec.amos.D2base.dllo\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.cv.sec.amos.L1base.dl\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.cv.sec.amos.L1base.dlhi\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.cv.sec.amos.L1base.dllo\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.sec.amos.L3L1.dl\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cv.sec.amos.L3L1.dlhi\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.cv.sec.amos.L3L1.dllo\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.cv.sec.amos.L3base.dl\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.cv.sec.amos.L3base.dlhi\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv.sec.amos.L3base.dllo\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.sec.kits.D2base.dl\endcsname{\ensuremath{+1.08}}
\expandafter\gdef\csname R@an.cv.sec.kits.D2base.dlhi\endcsname{\ensuremath{+1.75}}
\expandafter\gdef\csname R@an.cv.sec.kits.D2base.dllo\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv.sec.kits.L1base.dl\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.cv.sec.kits.L1base.dlhi\endcsname{\ensuremath{+2.52}}
\expandafter\gdef\csname R@an.cv.sec.kits.L1base.dllo\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.cv.sec.kits.L3L1.dl\endcsname{\ensuremath{-1.35}}
\expandafter\gdef\csname R@an.cv.sec.kits.L3L1.dlhi\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@an.cv.sec.kits.L3L1.dllo\endcsname{\ensuremath{-2.18}}
\expandafter\gdef\csname R@an.cv.sec.kits.L3base.dl\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cv.sec.kits.L3base.dlhi\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.cv.sec.kits.L3base.dllo\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.cv.span.acdc.band\endcsname{0.14}
\expandafter\gdef\csname R@an.cv.span.acdc.base\endcsname{1.36}
\expandafter\gdef\csname R@an.cv.span.acdc.contrast\endcsname{0.39}
\expandafter\gdef\csname R@an.cv.span.acdc.nc\endcsname{4}
\expandafter\gdef\csname R@an.cv.span.acdc.runnerup\endcsname{HyReX $-$ default}
\expandafter\gdef\csname R@an.cv.span.acdc.widest\endcsname{HyReX $-$ ResEnc-M}
\expandafter\gdef\csname R@an.cv.span.acdc.widestmargin\endcsname{0.04}
\expandafter\gdef\csname R@an.cv.span.acdc.widestword\endcsname{the largest of the four architecture-contrast spans measured here, which the 0.14 pp seed-noise scale of a one-seed pair difference does not resolve between HyReX $-$ ResEnc-M and HyReX $-$ default (0.39 pp against 0.35 pp)}
\expandafter\gdef\csname R@an.cv.span.acdc.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.span.amos.band\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.span.amos.base\endcsname{2.12}
\expandafter\gdef\csname R@an.cv.span.amos.contrast\endcsname{0.94}
\expandafter\gdef\csname R@an.cv.span.amos.nc\endcsname{4}
\expandafter\gdef\csname R@an.cv.span.amos.runnerup\endcsname{HyReX $-$ ResEnc-M}
\expandafter\gdef\csname R@an.cv.span.amos.widest\endcsname{ResEnc-M $-$ default}
\expandafter\gdef\csname R@an.cv.span.amos.widestmargin\endcsname{0.17}
\expandafter\gdef\csname R@an.cv.span.amos.widestword\endcsname{the largest of the four architecture-contrast spans measured here, which the 0.17 pp seed-noise scale of a one-seed pair difference does not resolve between ResEnc-M $-$ default and HyReX $-$ ResEnc-M (0.94 pp against 0.77 pp)}
\expandafter\gdef\csname R@an.cv.span.amos.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.span.kits.band\endcsname{1.12}
\expandafter\gdef\csname R@an.cv.span.kits.base\endcsname{4.05}
\expandafter\gdef\csname R@an.cv.span.kits.contrast\endcsname{2.47}
\expandafter\gdef\csname R@an.cv.span.kits.nc\endcsname{4}
\expandafter\gdef\csname R@an.cv.span.kits.runnerup\endcsname{HyReX $-$ default}
\expandafter\gdef\csname R@an.cv.span.kits.widest\endcsname{HyReX $-$ ResEnc-M}
\expandafter\gdef\csname R@an.cv.span.kits.widestmargin\endcsname{0.01}
\expandafter\gdef\csname R@an.cv.span.kits.widestword\endcsname{the largest of the four architecture-contrast spans measured here, which the 1.12 pp seed-noise scale of a one-seed pair difference does not resolve between HyReX $-$ ResEnc-M and HyReX $-$ default (2.47 pp against 2.46 pp)}
\expandafter\gdef\csname R@an.cv.span.kits.word\endcsname{is wider than}
\expandafter\gdef\csname R@an.cv.src0.a\endcsname{the frozen default pool}
\expandafter\gdef\csname R@an.cv.src0.b\endcsname{the mean of fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.cv.src0.c\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.cv.src0.legend\endcsname{a frozen pool, b fresh s1-2, c seed 0}
\expandafter\gdef\csname R@an.cv.src0.legendlong\endcsname{a: the frozen default pool; b: the mean of fresh seeds 1 and 2; c: discovery seed 0}
\expandafter\gdef\csname R@an.cv.status.acdc\endcsname{16 of 16 runs finished}
\expandafter\gdef\csname R@an.cv.status.all\endcsname{48 of 48 runs finished}
\expandafter\gdef\csname R@an.cv.status.amos\endcsname{16 of 16 runs finished}
\expandafter\gdef\csname R@an.cv.status.failed\endcsname{no Addendum-P run has failed}
\expandafter\gdef\csname R@an.cv.status.kits\endcsname{16 of 16 runs finished}
\expandafter\gdef\csname R@an.cv.status.l1b\endcsname{12 of 12 runs finished}
\expandafter\gdef\csname R@an.cv.status.l1b.acdc\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.l1b.amos\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.l1b.failed\endcsname{no Addendum-X cross-validation run has failed}
\expandafter\gdef\csname R@an.cv.status.l1b.kits\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.l1b.n\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.l1b.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.l1b.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.n\endcsname{48}
\expandafter\gdef\csname R@an.cv.status.p3c\endcsname{12 of 12 runs finished}
\expandafter\gdef\csname R@an.cv.status.p3c.acdc\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.p3c.amos\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.p3c.failed\endcsname{no Addendum-W cross-validation run has failed}
\expandafter\gdef\csname R@an.cv.status.p3c.kits\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.p3c.n\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.p3c.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.p3c.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.p6\endcsname{P6 queued (12 runs)}
\expandafter\gdef\csname R@an.cv.status.p6.sentence\endcsname{the cross-validation of LeanDec was queued although Addendum P6 owed it none (Addendum AB); 12 of its 12 seed-0 runs have finished (and the 24 extension runs of Addendum AH2: 0 finished)}
\expandafter\gdef\csname R@an.cv.status.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.total\endcsname{48}
\expandafter\gdef\csname R@an.cv.status.v5b1\endcsname{12 of 12 runs finished}
\expandafter\gdef\csname R@an.cv.status.v5b1.acdc\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v5b1.amos\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v5b1.failed\endcsname{no cross-validation run of LeanAdd has failed}
\expandafter\gdef\csname R@an.cv.status.v5b1.kits\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v5b1.n\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v5b1.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.v5b1.sentence\endcsname{the cross-validation of LeanAdd (Addendum AM) has 12 of its 12 runs finished (AMOS22 4 of 4, KiTS23 4 of 4, ACDC 4 of 4)}
\expandafter\gdef\csname R@an.cv.status.v5b1.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v5b2\endcsname{12 of 12 runs finished}
\expandafter\gdef\csname R@an.cv.status.v5b2.acdc\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v5b2.amos\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v5b2.failed\endcsname{no cross-validation run of LeanAdd-NeXt has failed}
\expandafter\gdef\csname R@an.cv.status.v5b2.kits\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v5b2.n\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v5b2.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.v5b2.sentence\endcsname{the cross-validation of LeanAdd-NeXt (Addendum AM) has 12 of its 12 runs finished (AMOS22 4 of 4, KiTS23 4 of 4, ACDC 4 of 4)}
\expandafter\gdef\csname R@an.cv.status.v5b2.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v6a1r\endcsname{12 of 12 runs finished}
\expandafter\gdef\csname R@an.cv.status.v6a1r.acdc\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v6a1r.amos\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v6a1r.failed\endcsname{no cross-validation run of HyReX-k9 has failed}
\expandafter\gdef\csname R@an.cv.status.v6a1r.kits\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v6a1r.n\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v6a1r.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.v6a1r.sentence\endcsname{the cross-validation of HyReX-k9 (Addendum AO) has 12 of its 12 runs finished (AMOS22 4 of 4, KiTS23 4 of 4, ACDC 4 of 4)}
\expandafter\gdef\csname R@an.cv.status.v6a1r.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v7a1\endcsname{12 of 12 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7a1.acdc\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7a1.amos\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7a1.failed\endcsname{no cross-validation run of LeanDeepMid has failed}
\expandafter\gdef\csname R@an.cv.status.v7a1.kits\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7a1.n\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v7a1.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.v7a1.sentence\endcsname{the cross-validation of LeanDeepMid (Addendum AP) has 12 of its 12 runs finished (AMOS22 4 of 4, KiTS23 4 of 4, ACDC 4 of 4)}
\expandafter\gdef\csname R@an.cv.status.v7a1.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v7a2\endcsname{4 of 12 runs finished, 8 running}
\expandafter\gdef\csname R@an.cv.status.v7a2.acdc\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7a2.amos\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7a2.failed\endcsname{no cross-validation run of LeanDeepMid+FD has failed}
\expandafter\gdef\csname R@an.cv.status.v7a2.kits\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7a2.n\endcsname{4}
\expandafter\gdef\csname R@an.cv.status.v7a2.running\endcsname{8}
\expandafter\gdef\csname R@an.cv.status.v7a2.sentence\endcsname{the cross-validation of LeanDeepMid+FD (Addendum AW) has 4 of its 12 runs finished (AMOS22 0 of 4, KiTS23 4 of 4, ACDC 0 of 4)}
\expandafter\gdef\csname R@an.cv.status.v7a2.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v7b1\endcsname{0 of 12 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7b1.acdc\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7b1.amos\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7b1.failed\endcsname{no cross-validation run of LeanSep has failed}
\expandafter\gdef\csname R@an.cv.status.v7b1.kits\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7b1.n\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.v7b1.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.v7b1.sentence\endcsname{the cross-validation of LeanSep (Addendum AQ) has 0 of its 12 runs finished (AMOS22 0 of 4, KiTS23 0 of 4, ACDC 0 of 4)}
\expandafter\gdef\csname R@an.cv.status.v7b1.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v7b2\endcsname{0 of 12 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7b2.acdc\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7b2.amos\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7b2.failed\endcsname{no cross-validation run of LeanDil has failed}
\expandafter\gdef\csname R@an.cv.status.v7b2.kits\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7b2.n\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.v7b2.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.v7b2.sentence\endcsname{the cross-validation of LeanDil (Addendum AQ) has 0 of its 12 runs finished (AMOS22 0 of 4, KiTS23 0 of 4, ACDC 0 of 4)}
\expandafter\gdef\csname R@an.cv.status.v7b2.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v7c1\endcsname{12 of 12 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7c1.acdc\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7c1.amos\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7c1.failed\endcsname{no cross-validation run of LeanNeXt-s5 has failed}
\expandafter\gdef\csname R@an.cv.status.v7c1.kits\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v7c1.n\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v7c1.running\endcsname{0}
\expandafter\gdef\csname R@an.cv.status.v7c1.sentence\endcsname{the cross-validation of LeanNeXt-s5 (Addendum AP) has 12 of its 12 runs finished (AMOS22 4 of 4, KiTS23 4 of 4, ACDC 4 of 4)}
\expandafter\gdef\csname R@an.cv.status.v7c1.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.status.v8b2\endcsname{4 of 12 runs finished, 5 running}
\expandafter\gdef\csname R@an.cv.status.v8b2.acdc\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v8b2.amos\endcsname{0 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v8b2.failed\endcsname{no cross-validation run of Stem1 has failed}
\expandafter\gdef\csname R@an.cv.status.v8b2.kits\endcsname{4 of 4 runs finished}
\expandafter\gdef\csname R@an.cv.status.v8b2.n\endcsname{4}
\expandafter\gdef\csname R@an.cv.status.v8b2.running\endcsname{5}
\expandafter\gdef\csname R@an.cv.status.v8b2.sentence\endcsname{the cross-validation of Stem1 (Addendum AY) has 4 of its 12 runs finished (AMOS22 0 of 4, KiTS23 4 of 4, ACDC 0 of 4)}
\expandafter\gdef\csname R@an.cv.status.v8b2.total\endcsname{12}
\expandafter\gdef\csname R@an.cv.tta.acdc\endcsname{with}
\expandafter\gdef\csname R@an.cv.tta.amos\endcsname{without}
\expandafter\gdef\csname R@an.cv.tta.kits\endcsname{without}
\expandafter\gdef\csname R@an.cv.tta.note\endcsname{inference without test-time mirroring on AMOS22 and KiTS23 and with it on ACDC}
\expandafter\gdef\csname R@an.cv.vram.cap\endcsname{12}
\expandafter\gdef\csname R@an.cv.vram.capnote\endcsname{the registered 12\,GB training-memory cap, read from the profile entries of the cross-validation arms and not a measured peak}
\expandafter\gdef\csname R@an.cv.xarm.V5B1.file\endcsname{cand\_V5B1\_leanadd.py}
\expandafter\gdef\csname R@an.cv.xarm.V5B1.name\endcsname{LeanDec with additive skips}
\expandafter\gdef\csname R@an.cv.xarm.V5B1.parents\endcsname{LeanDec}
\expandafter\gdef\csname R@an.cv.xarm.V5B1.registration\endcsname{Addendum AM}
\expandafter\gdef\csname R@an.cv.xarm.V5B2.file\endcsname{cand\_V5B2\_leanaddnext.py}
\expandafter\gdef\csname R@an.cv.xarm.V5B2.name\endcsname{LeanAdd with coarse large kernels}
\expandafter\gdef\csname R@an.cv.xarm.V5B2.parents\endcsname{LeanAdd and HyReX}
\expandafter\gdef\csname R@an.cv.xarm.V5B2.registration\endcsname{Addendum AM}
\expandafter\gdef\csname R@an.cv.xarm.V6A1r.file\endcsname{cand\_V6A1r\_k9coarse.py}
\expandafter\gdef\csname R@an.cv.xarm.V6A1r.name\endcsname{HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.cv.xarm.V6A1r.parents\endcsname{HyReX}
\expandafter\gdef\csname R@an.cv.xarm.V6A1r.registration\endcsname{Addendum AO}
\expandafter\gdef\csname R@an.cv.xarm.V7A1.file\endcsname{cand\_V7A1\_deepmid.py}
\expandafter\gdef\csname R@an.cv.xarm.V7A1.name\endcsname{LeanAdd-NeXt with a deeper middle encoder}
\expandafter\gdef\csname R@an.cv.xarm.V7A1.parents\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.cv.xarm.V7A1.registration\endcsname{Addendum AP}
\expandafter\gdef\csname R@an.cv.xarm.V7A2.file\endcsname{cand\_V7A2\_finedec.py}
\expandafter\gdef\csname R@an.cv.xarm.V7A2.name\endcsname{LeanDeepMid with the finest decoder convolutions}
\expandafter\gdef\csname R@an.cv.xarm.V7A2.parents\endcsname{LeanDeepMid}
\expandafter\gdef\csname R@an.cv.xarm.V7A2.registration\endcsname{Addendum AW}
\expandafter\gdef\csname R@an.cv.xarm.V7B1.file\endcsname{cand\_V7B1\_leansep.py}
\expandafter\gdef\csname R@an.cv.xarm.V7B1.name\endcsname{LeanAdd-NeXt with separable coarse kernels}
\expandafter\gdef\csname R@an.cv.xarm.V7B1.parents\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.cv.xarm.V7B1.registration\endcsname{Addendum AQ}
\expandafter\gdef\csname R@an.cv.xarm.V7B2.file\endcsname{cand\_V7B2\_leandil.py}
\expandafter\gdef\csname R@an.cv.xarm.V7B2.name\endcsname{LeanAdd-NeXt with dilated coarse kernels}
\expandafter\gdef\csname R@an.cv.xarm.V7B2.parents\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.cv.xarm.V7B2.registration\endcsname{Addendum AQ}
\expandafter\gdef\csname R@an.cv.xarm.V7C1.file\endcsname{cand\_V7C1\_s5only.py}
\expandafter\gdef\csname R@an.cv.xarm.V7C1.name\endcsname{LeanAdd-NeXt with the coarse operator at stage 5 only}
\expandafter\gdef\csname R@an.cv.xarm.V7C1.parents\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.cv.xarm.V7C1.registration\endcsname{Addendum AP}
\expandafter\gdef\csname R@an.cv.xarm.V8B2.file\endcsname{cand\_V8B2\_stem1.py}
\expandafter\gdef\csname R@an.cv.xarm.V8B2.name\endcsname{LeanNeXt-s5 with one convolution at encoder stage 0}
\expandafter\gdef\csname R@an.cv.xarm.V8B2.parents\endcsname{none}
\expandafter\gdef\csname R@an.cv.xarm.V8B2.registration\endcsname{Addendum AY}
\expandafter\gdef\csname R@an.cv.xarms.n\endcsname{9}
\expandafter\gdef\csname R@an.cv.xarms.names\endcsname{LeanAdd, LeanAdd-NeXt, HyReX-k9, LeanDeepMid, LeanNeXt-s5, LeanSep, LeanDil, LeanDeepMid+FD and Stem1}
\expandafter\gdef\csname R@an.cv.xarms.tags\endcsname{V5B1, V5B2, V6A1r, V7A1, V7C1, V7B1, V7B2, V7A2, V8B2}
\expandafter\gdef\csname R@an.cv3.D2.acdc.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.D2.acdc.nrun\endcsname{4}
\expandafter\gdef\csname R@an.cv3.D2.amos.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.D2.amos.nrun\endcsname{4}
\expandafter\gdef\csname R@an.cv3.D2.kits.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.D2.kits.nrun\endcsname{4}
\expandafter\gdef\csname R@an.cv3.D2base.acdc.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.D2base.acdc.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv3.D2base.acdc.vs1\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.cv3.D2base.acdc.vs1.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv3.D2base.amos.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.D2base.amos.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv3.D2base.amos.vs1\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.cv3.D2base.amos.vs1.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv3.D2base.kits.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.D2base.kits.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv3.D2base.kits.vs1\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@an.cv3.D2base.kits.vs1.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv3.L1.acdc.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.L1.acdc.nrun\endcsname{4}
\expandafter\gdef\csname R@an.cv3.L1.amos.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.L1.amos.nrun\endcsname{4}
\expandafter\gdef\csname R@an.cv3.L1.kits.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.L1.kits.nrun\endcsname{4}
\expandafter\gdef\csname R@an.cv3.L1base.acdc.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.L1base.acdc.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv3.L1base.acdc.vs1\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cv3.L1base.acdc.vs1.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv3.L1base.amos.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.L1base.amos.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv3.L1base.amos.vs1\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv3.L1base.amos.vs1.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv3.L1base.kits.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.L1base.kits.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv3.L1base.kits.vs1\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.cv3.L1base.kits.vs1.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv3.L3.acdc.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.L3.acdc.nrun\endcsname{4}
\expandafter\gdef\csname R@an.cv3.L3.amos.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.L3.amos.nrun\endcsname{4}
\expandafter\gdef\csname R@an.cv3.L3.kits.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.L3.kits.nrun\endcsname{4}
\expandafter\gdef\csname R@an.cv3.L3L1.acdc.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.L3L1.acdc.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv3.L3L1.acdc.vs1\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.cv3.L3L1.acdc.vs1.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv3.L3L1.amos.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.L3L1.amos.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv3.L3L1.amos.vs1\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.cv3.L3L1.amos.vs1.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv3.L3L1.kits.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.L3L1.kits.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv3.L3L1.kits.vs1\endcsname{\ensuremath{-1.47}}
\expandafter\gdef\csname R@an.cv3.L3L1.kits.vs1.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv3.L3P3c.acdc.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.L3P3c.acdc.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv3.L3P3c.acdc.vs1\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cv3.L3P3c.acdc.vs1.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv3.L3P3c.amos.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.L3P3c.amos.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv3.L3P3c.amos.vs1\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv3.L3P3c.amos.vs1.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv3.L3P3c.kits.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.L3P3c.kits.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv3.L3P3c.kits.vs1\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv3.L3P3c.kits.vs1.word\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.cv3.L3base.acdc.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.L3base.acdc.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv3.L3base.acdc.vs1\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv3.L3base.acdc.vs1.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.cv3.L3base.amos.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.L3base.amos.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv3.L3base.amos.vs1\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv3.L3base.amos.vs1.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv3.L3base.kits.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.L3base.kits.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv3.L3base.kits.vs1\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.cv3.L3base.kits.vs1.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv3.P3c.acdc.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.P3c.acdc.nrun\endcsname{4}
\expandafter\gdef\csname R@an.cv3.P3c.amos.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.P3c.amos.nrun\endcsname{4}
\expandafter\gdef\csname R@an.cv3.P3c.kits.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.P3c.kits.nrun\endcsname{4}
\expandafter\gdef\csname R@an.cv3.P3cbase.acdc.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.P3cbase.acdc.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv3.P3cbase.acdc.vs1\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cv3.P3cbase.acdc.vs1.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv3.P3cbase.amos.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.P3cbase.amos.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv3.P3cbase.amos.vs1\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv3.P3cbase.amos.vs1.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.cv3.P3cbase.kits.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.P3cbase.kits.nfold.word\endcsname{none}
\expandafter\gdef\csname R@an.cv3.P3cbase.kits.vs1\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cv3.P3cbase.kits.vs1.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.cv3.base.acdc.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.base.acdc.nrun\endcsname{4}
\expandafter\gdef\csname R@an.cv3.base.amos.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.base.amos.nrun\endcsname{4}
\expandafter\gdef\csname R@an.cv3.base.kits.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.base.kits.nrun\endcsname{4}
\expandafter\gdef\csname R@an.cv3.boot.B\endcsname{20\,000}
\expandafter\gdef\csname R@an.cv3.boot.def\endcsname{a descriptive case-level companion to the interval over folds: the validation cases are resampled with replacement within each fold (the same draw for each arm of the contrast), the per-case Dice of each arm is its mean over the three seeds, the statistic is the mean over the four folds of the within-fold difference, and the interval is the percentile 95\,\% interval of 20\,000 resamples; it describes case sampling with the trained networks fixed and is never printed instead of the paired-$t$ interval over folds}
\expandafter\gdef\csname R@an.cv3.boot.seed\endcsname{20261009}
\expandafter\gdef\csname R@an.cv3.ci.df\endcsname{3}
\expandafter\gdef\csname R@an.cv3.ci.level\endcsname{95\,\%}
\expandafter\gdef\csname R@an.cv3.equiv.L3L1.acdc.margin\endcsname{0.50}
\expandafter\gdef\csname R@an.cv3.equiv.L3L1.acdc.sentence\endcsname{On ACDC the reading of HyReX minus ResEnc-M against the registered margin of \ensuremath{\pm}0.50\,pp (Addendum AK) is formed when all twelve runs of each arm have landed (none of the four folds has all three seeds of each arm)}
\expandafter\gdef\csname R@an.cv3.equiv.L3L1.acdc.state\endcsname{pending}
\expandafter\gdef\csname R@an.cv3.equiv.L3L1.amos.margin\endcsname{0.50}
\expandafter\gdef\csname R@an.cv3.equiv.L3L1.amos.sentence\endcsname{On AMOS22 the reading of HyReX minus ResEnc-M against the registered margin of \ensuremath{\pm}0.50\,pp (Addendum AK) is formed when all twelve runs of each arm have landed (none of the four folds has all three seeds of each arm)}
\expandafter\gdef\csname R@an.cv3.equiv.L3L1.amos.state\endcsname{pending}
\expandafter\gdef\csname R@an.cv3.equiv.L3L1.kits.margin\endcsname{0.50}
\expandafter\gdef\csname R@an.cv3.equiv.L3L1.kits.sentence\endcsname{On KiTS23 the reading of HyReX minus ResEnc-M against the registered margin of \ensuremath{\pm}0.50\,pp (Addendum AK) is formed when all twelve runs of each arm have landed (none of the four folds has all three seeds of each arm)}
\expandafter\gdef\csname R@an.cv3.equiv.L3L1.kits.state\endcsname{pending}
\expandafter\gdef\csname R@an.cv3.equiv.margin\endcsname{0.50}
\expandafter\gdef\csname R@an.cv3.equiv.params.acdc\endcsname{0.28}
\expandafter\gdef\csname R@an.cv3.equiv.params.amos\endcsname{0.29}
\expandafter\gdef\csname R@an.cv3.equiv.params.kits\endcsname{0.29}
\expandafter\gdef\csname R@an.cv3.equiv.summary\endcsname{At the registered margin of \ensuremath{\pm}0.50\,pp, the study's one-seed pair floor (Addendum AK), the 95\,\% interval of HyReX minus ResEnc-M over the three-seed cross-validation folds is read on each dataset and never pooled across datasets: it is formed on a dataset when all twelve runs of each arm have landed, and none of the three datasets has them yet; HyReX holds 0.29 times ResEnc-M's parameters on the AMOS22 plan, 0.29 times on the KiTS23 plan and 0.28 times on the ACDC plan}
\expandafter\gdef\csname R@an.cv3.nfolds\endcsname{4}
\expandafter\gdef\csname R@an.cv3.nfolds.word\endcsname{four}
\expandafter\gdef\csname R@an.cv3.nseeds\endcsname{3}
\expandafter\gdef\csname R@an.cv3.nseeds.new.word\endcsname{two}
\expandafter\gdef\csname R@an.cv3.nseeds.word\endcsname{three}
\expandafter\gdef\csname R@an.cv3.nval.acdc.f1\endcsname{40}
\expandafter\gdef\csname R@an.cv3.nval.acdc.f2\endcsname{40}
\expandafter\gdef\csname R@an.cv3.nval.acdc.f3\endcsname{40}
\expandafter\gdef\csname R@an.cv3.nval.acdc.f4\endcsname{40}
\expandafter\gdef\csname R@an.cv3.nval.amos.f1\endcsname{40}
\expandafter\gdef\csname R@an.cv3.nval.amos.f2\endcsname{40}
\expandafter\gdef\csname R@an.cv3.nval.amos.f3\endcsname{40}
\expandafter\gdef\csname R@an.cv3.nval.amos.f4\endcsname{40}
\expandafter\gdef\csname R@an.cv3.nval.kits.f1\endcsname{98}
\expandafter\gdef\csname R@an.cv3.nval.kits.f2\endcsname{98}
\expandafter\gdef\csname R@an.cv3.nval.kits.f3\endcsname{98}
\expandafter\gdef\csname R@an.cv3.nval.kits.f4\endcsname{97}
\expandafter\gdef\csname R@an.cv3.pooled.L3.acdc.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.pooled.L3.acdc.sentence\endcsname{Against the average of the default and the function-identical control on ACDC, the pooled-baseline contrast of HyReX, taking the default and its function-identical rebuild as two replicates of one network (Addendum AC: their difference is within seed noise at the resolution of the runs, which does not show that it is zero), is formed when all twelve runs of each of the three arms (HyReX, the default and the function-identical control) have landed (none of the four folds has all three seeds of each of them)}
\expandafter\gdef\csname R@an.cv3.pooled.L3.acdc.state\endcsname{pending}
\expandafter\gdef\csname R@an.cv3.pooled.L3.amos.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.pooled.L3.amos.sentence\endcsname{Against the average of the default and the function-identical control on AMOS22, the pooled-baseline contrast of HyReX, taking the default and its function-identical rebuild as two replicates of one network (Addendum AC: their difference is within seed noise at the resolution of the runs, which does not show that it is zero), is formed when all twelve runs of each of the three arms (HyReX, the default and the function-identical control) have landed (none of the four folds has all three seeds of each of them)}
\expandafter\gdef\csname R@an.cv3.pooled.L3.amos.state\endcsname{pending}
\expandafter\gdef\csname R@an.cv3.pooled.L3.kits.nfold\endcsname{0}
\expandafter\gdef\csname R@an.cv3.pooled.L3.kits.sentence\endcsname{Against the average of the default and the function-identical control on KiTS23, the pooled-baseline contrast of HyReX, taking the default and its function-identical rebuild as two replicates of one network (Addendum AC: their difference is within seed noise at the resolution of the runs, which does not show that it is zero), is formed when all twelve runs of each of the three arms (HyReX, the default and the function-identical control) have landed (none of the four folds has all three seeds of each of them)}
\expandafter\gdef\csname R@an.cv3.pooled.L3.kits.state\endcsname{pending}
\expandafter\gdef\csname R@an.cv3.pooled.assumption\endcsname{taking the default and its function-identical rebuild as two replicates of one network (Addendum AC: their difference is within seed noise at the resolution of the runs, which does not show that it is zero)}
\expandafter\gdef\csname R@an.cv3.se1.premise\endcsname{the standard error of a one-seed fold difference implied by the within-fold seed spread of the two arms, the square root of the sum of the two arms' within-fold seed variances, which assumes the seeds of the two arms are independent; the paired value is the same quantity measured on the per-seed differences themselves}
\expandafter\gdef\csname R@an.cv3.seedphrase\endcsname{three seeds per arm and fold}
\expandafter\gdef\csname R@an.cv3.sentence.D2base.acdc\endcsname{Against the default on ACDC, none of the four folds has all three seeds of each arm yet, and the contrast over three seeds per arm and fold is formed when all four do}
\expandafter\gdef\csname R@an.cv3.sentence.D2base.amos\endcsname{Against the default on AMOS22, none of the four folds has all three seeds of each arm yet, and the contrast over three seeds per arm and fold is formed when all four do}
\expandafter\gdef\csname R@an.cv3.sentence.D2base.kits\endcsname{Against the default on KiTS23, none of the four folds has all three seeds of each arm yet, and the contrast over three seeds per arm and fold is formed when all four do}
\expandafter\gdef\csname R@an.cv3.sentence.L1base.acdc\endcsname{Against the default on ACDC, none of the four folds has all three seeds of each arm yet, and the contrast over three seeds per arm and fold is formed when all four do}
\expandafter\gdef\csname R@an.cv3.sentence.L1base.amos\endcsname{Against the default on AMOS22, none of the four folds has all three seeds of each arm yet, and the contrast over three seeds per arm and fold is formed when all four do}
\expandafter\gdef\csname R@an.cv3.sentence.L1base.kits\endcsname{Against the default on KiTS23, none of the four folds has all three seeds of each arm yet, and the contrast over three seeds per arm and fold is formed when all four do}
\expandafter\gdef\csname R@an.cv3.sentence.L3L1.acdc\endcsname{Against ResEnc-M on ACDC, none of the four folds has all three seeds of each arm yet, and the contrast over three seeds per arm and fold is formed when all four do}
\expandafter\gdef\csname R@an.cv3.sentence.L3L1.amos\endcsname{Against ResEnc-M on AMOS22, none of the four folds has all three seeds of each arm yet, and the contrast over three seeds per arm and fold is formed when all four do}
\expandafter\gdef\csname R@an.cv3.sentence.L3L1.kits\endcsname{Against ResEnc-M on KiTS23, none of the four folds has all three seeds of each arm yet, and the contrast over three seeds per arm and fold is formed when all four do}
\expandafter\gdef\csname R@an.cv3.sentence.L3P3c.acdc\endcsname{Against the function-identical control on ACDC, none of the four folds has all three seeds of each arm yet, and the contrast over three seeds per arm and fold is formed when all four do}
\expandafter\gdef\csname R@an.cv3.sentence.L3P3c.amos\endcsname{Against the function-identical control on AMOS22, none of the four folds has all three seeds of each arm yet, and the contrast over three seeds per arm and fold is formed when all four do}
\expandafter\gdef\csname R@an.cv3.sentence.L3P3c.kits\endcsname{Against the function-identical control on KiTS23, none of the four folds has all three seeds of each arm yet, and the contrast over three seeds per arm and fold is formed when all four do}
\expandafter\gdef\csname R@an.cv3.sentence.L3base.acdc\endcsname{Against the default on ACDC, none of the four folds has all three seeds of each arm yet, and the contrast over three seeds per arm and fold is formed when all four do}
\expandafter\gdef\csname R@an.cv3.sentence.L3base.amos\endcsname{Against the default on AMOS22, none of the four folds has all three seeds of each arm yet, and the contrast over three seeds per arm and fold is formed when all four do}
\expandafter\gdef\csname R@an.cv3.sentence.L3base.kits\endcsname{Against the default on KiTS23, none of the four folds has all three seeds of each arm yet, and the contrast over three seeds per arm and fold is formed when all four do}
\expandafter\gdef\csname R@an.cv3.sentence.P3cbase.acdc\endcsname{Against the default on ACDC, none of the four folds has all three seeds of each arm yet, and the contrast over three seeds per arm and fold is formed when all four do}
\expandafter\gdef\csname R@an.cv3.sentence.P3cbase.amos\endcsname{Against the default on AMOS22, none of the four folds has all three seeds of each arm yet, and the contrast over three seeds per arm and fold is formed when all four do}
\expandafter\gdef\csname R@an.cv3.sentence.P3cbase.kits\endcsname{Against the default on KiTS23, none of the four folds has all three seeds of each arm yet, and the contrast over three seeds per arm and fold is formed when all four do}
\expandafter\gdef\csname R@an.cv3.status.acdc\endcsname{0 of 40 further runs finished}
\expandafter\gdef\csname R@an.cv3.status.all\endcsname{60 of 180 runs finished}
\expandafter\gdef\csname R@an.cv3.status.amos\endcsname{0 of 40 further runs finished}
\expandafter\gdef\csname R@an.cv3.status.cells\endcsname{0 of 18 contrast-dataset cells finished}
\expandafter\gdef\csname R@an.cv3.status.cells.n\endcsname{0}
\expandafter\gdef\csname R@an.cv3.status.cells.total\endcsname{18}
\expandafter\gdef\csname R@an.cv3.status.failed\endcsname{no Addendum-AH2 run has failed}
\expandafter\gdef\csname R@an.cv3.status.failed.n\endcsname{0}
\expandafter\gdef\csname R@an.cv3.status.kits\endcsname{0 of 40 further runs finished}
\expandafter\gdef\csname R@an.cv3.status.new\endcsname{0 of 120 further runs finished}
\expandafter\gdef\csname R@an.cv3.status.new.n\endcsname{0}
\expandafter\gdef\csname R@an.cv3.status.new.total\endcsname{120}
\expandafter\gdef\csname R@an.cv3.status.running\endcsname{0}
\expandafter\gdef\csname R@an.cv3.status.seed0\endcsname{60 of 60 seed-0 runs finished}
\expandafter\gdef\csname R@an.cv3.status.seed0.n\endcsname{60}
\expandafter\gdef\csname R@an.cv3.status.seed0.running\endcsname{0}
\expandafter\gdef\csname R@an.cv3.status.seed0.total\endcsname{60}
\expandafter\gdef\csname R@an.cv3.summary\endcsname{Addendum AH2 adds two further seeds to every arm of the cross-validation (120 runs): 0 of them have finished, and the contrast over three seeds per arm and fold is read for 0 of the 18 contrast-dataset cells; a cell is read when all four of its folds have all three seeds of each arm, and the single-seed contrast of Addendum P remains the estimand under which the earlier statements were made}
\expandafter\gdef\csname R@an.cvxx.acdc.caption\endcsname{Of the four cross-validation folds on ACDC, {\ifdefined\archL\archL\else XX-Net-L\fi} improves on nnU-Net in 0, {\ifdefined\archA\archA\else XX-Net-A\fi} in 2, ResEnc-M in 4 and the rebuilt nnU-Net in 1}
\expandafter\gdef\csname R@an.cvxx.acdc.noise\endcsname{0.28}
\expandafter\gdef\csname R@an.cvxx.acdc.reb.dcv\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.cvxx.acdc.reb.f1\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cvxx.acdc.reb.f2\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cvxx.acdc.reb.f3\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cvxx.acdc.reb.f4\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.cvxx.acdc.reb.hi\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.cvxx.acdc.reb.lo\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.cvxx.acdc.reb.name\endcsname{nnU-Net (rebuilt)}
\expandafter\gdef\csname R@an.cvxx.acdc.reb.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cvxx.acdc.reb.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.cvxx.acdc.reb.tag\endcsname{P3c}
\expandafter\gdef\csname R@an.cvxx.acdc.resm.dcv\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.cvxx.acdc.resm.f1\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.cvxx.acdc.resm.f2\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.cvxx.acdc.resm.f3\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.cvxx.acdc.resm.f4\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cvxx.acdc.resm.hi\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cvxx.acdc.resm.lo\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cvxx.acdc.resm.name\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.cvxx.acdc.resm.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cvxx.acdc.resm.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cvxx.acdc.resm.tag\endcsname{L1}
\expandafter\gdef\csname R@an.cvxx.acdc.xa.dcv\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cvxx.acdc.xa.f1\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cvxx.acdc.xa.f2\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.cvxx.acdc.xa.f3\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cvxx.acdc.xa.f4\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.cvxx.acdc.xa.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.cvxx.acdc.xa.lo\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.cvxx.acdc.xa.name\endcsname{{\ifdefined\archA\archA\else XX-Net-A\fi}}
\expandafter\gdef\csname R@an.cvxx.acdc.xa.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cvxx.acdc.xa.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cvxx.acdc.xa.tag\endcsname{V7A1}
\expandafter\gdef\csname R@an.cvxx.acdc.xl.dcv\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.cvxx.acdc.xl.f1\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cvxx.acdc.xl.f2\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.cvxx.acdc.xl.f3\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.cvxx.acdc.xl.f4\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cvxx.acdc.xl.hi\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.cvxx.acdc.xl.lo\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.cvxx.acdc.xl.name\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi}}
\expandafter\gdef\csname R@an.cvxx.acdc.xl.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cvxx.acdc.xl.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cvxx.acdc.xl.tag\endcsname{V7C1}
\expandafter\gdef\csname R@an.cvxx.amos.caption\endcsname{Of the four cross-validation folds on AMOS22, {\ifdefined\archL\archL\else XX-Net-L\fi} improves on nnU-Net in 0, {\ifdefined\archA\archA\else XX-Net-A\fi} in 2, ResEnc-M in 3 and the rebuilt nnU-Net in 2}
\expandafter\gdef\csname R@an.cvxx.amos.noise\endcsname{0.35}
\expandafter\gdef\csname R@an.cvxx.amos.reb.dcv\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cvxx.amos.reb.f1\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.cvxx.amos.reb.f2\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.cvxx.amos.reb.f3\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cvxx.amos.reb.f4\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cvxx.amos.reb.hi\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.cvxx.amos.reb.lo\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.cvxx.amos.reb.name\endcsname{nnU-Net (rebuilt)}
\expandafter\gdef\csname R@an.cvxx.amos.reb.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cvxx.amos.reb.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cvxx.amos.reb.tag\endcsname{P3c}
\expandafter\gdef\csname R@an.cvxx.amos.resm.dcv\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.cvxx.amos.resm.f1\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.cvxx.amos.resm.f2\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.cvxx.amos.resm.f3\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.cvxx.amos.resm.f4\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.cvxx.amos.resm.hi\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.cvxx.amos.resm.lo\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.cvxx.amos.resm.name\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.cvxx.amos.resm.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cvxx.amos.resm.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cvxx.amos.resm.tag\endcsname{L1}
\expandafter\gdef\csname R@an.cvxx.amos.xa.dcv\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cvxx.amos.xa.f1\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.cvxx.amos.xa.f2\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.cvxx.amos.xa.f3\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.cvxx.amos.xa.f4\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.cvxx.amos.xa.hi\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.cvxx.amos.xa.lo\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.cvxx.amos.xa.name\endcsname{{\ifdefined\archA\archA\else XX-Net-A\fi}}
\expandafter\gdef\csname R@an.cvxx.amos.xa.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cvxx.amos.xa.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.cvxx.amos.xa.tag\endcsname{V7A1}
\expandafter\gdef\csname R@an.cvxx.amos.xl.dcv\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.cvxx.amos.xl.f1\endcsname{\ensuremath{-0.58}}
\expandafter\gdef\csname R@an.cvxx.amos.xl.f2\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.cvxx.amos.xl.f3\endcsname{\ensuremath{-0.71}}
\expandafter\gdef\csname R@an.cvxx.amos.xl.f4\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cvxx.amos.xl.hi\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cvxx.amos.xl.lo\endcsname{\ensuremath{-0.81}}
\expandafter\gdef\csname R@an.cvxx.amos.xl.name\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi}}
\expandafter\gdef\csname R@an.cvxx.amos.xl.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cvxx.amos.xl.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.cvxx.amos.xl.tag\endcsname{V7C1}
\expandafter\gdef\csname R@an.cvxx.caption\endcsname{Of the four cross-validation folds, {\ifdefined\archL\archL\else XX-Net-L\fi} improves on nnU-Net in 3 on KiTS23, 0 on AMOS22 and 0 on ACDC, {\ifdefined\archA\archA\else XX-Net-A\fi} in 4, 2 and 2, ResEnc-M in 4, 3 and 4 and the rebuilt nnU-Net in 3, 2 and 1}
\expandafter\gdef\csname R@an.cvxx.fallback\endcsname{no}
\expandafter\gdef\csname R@an.cvxx.kits.caption\endcsname{Of the four cross-validation folds on KiTS23, {\ifdefined\archL\archL\else XX-Net-L\fi} improves on nnU-Net in 3, {\ifdefined\archA\archA\else XX-Net-A\fi} in 4, ResEnc-M in 4 and the rebuilt nnU-Net in 3}
\expandafter\gdef\csname R@an.cvxx.kits.noise\endcsname{2.25}
\expandafter\gdef\csname R@an.cvxx.kits.reb.dcv\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.cvxx.kits.reb.f1\endcsname{\ensuremath{+2.38}}
\expandafter\gdef\csname R@an.cvxx.kits.reb.f2\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cvxx.kits.reb.f3\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.cvxx.kits.reb.f4\endcsname{\ensuremath{-1.02}}
\expandafter\gdef\csname R@an.cvxx.kits.reb.hi\endcsname{\ensuremath{+2.82}}
\expandafter\gdef\csname R@an.cvxx.kits.reb.lo\endcsname{\ensuremath{-1.71}}
\expandafter\gdef\csname R@an.cvxx.kits.reb.name\endcsname{nnU-Net (rebuilt)}
\expandafter\gdef\csname R@an.cvxx.kits.reb.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cvxx.kits.reb.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cvxx.kits.reb.tag\endcsname{P3c}
\expandafter\gdef\csname R@an.cvxx.kits.resm.dcv\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.cvxx.kits.resm.f1\endcsname{\ensuremath{+2.58}}
\expandafter\gdef\csname R@an.cvxx.kits.resm.f2\endcsname{\ensuremath{+2.94}}
\expandafter\gdef\csname R@an.cvxx.kits.resm.f3\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.cvxx.kits.resm.f4\endcsname{\ensuremath{+1.71}}
\expandafter\gdef\csname R@an.cvxx.kits.resm.hi\endcsname{\ensuremath{+3.32}}
\expandafter\gdef\csname R@an.cvxx.kits.resm.lo\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.cvxx.kits.resm.name\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.cvxx.kits.resm.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cvxx.kits.resm.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cvxx.kits.resm.tag\endcsname{L1}
\expandafter\gdef\csname R@an.cvxx.kits.xa.dcv\endcsname{\ensuremath{+1.63}}
\expandafter\gdef\csname R@an.cvxx.kits.xa.f1\endcsname{\ensuremath{+2.03}}
\expandafter\gdef\csname R@an.cvxx.kits.xa.f2\endcsname{\ensuremath{+2.40}}
\expandafter\gdef\csname R@an.cvxx.kits.xa.f3\endcsname{\ensuremath{+1.98}}
\expandafter\gdef\csname R@an.cvxx.kits.xa.f4\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cvxx.kits.xa.hi\endcsname{\ensuremath{+3.27}}
\expandafter\gdef\csname R@an.cvxx.kits.xa.lo\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.cvxx.kits.xa.name\endcsname{{\ifdefined\archA\archA\else XX-Net-A\fi}}
\expandafter\gdef\csname R@an.cvxx.kits.xa.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cvxx.kits.xa.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.cvxx.kits.xa.tag\endcsname{V7A1}
\expandafter\gdef\csname R@an.cvxx.kits.xl.dcv\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.cvxx.kits.xl.f1\endcsname{\ensuremath{+2.14}}
\expandafter\gdef\csname R@an.cvxx.kits.xl.f2\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.cvxx.kits.xl.f3\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.cvxx.kits.xl.f4\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.cvxx.kits.xl.hi\endcsname{\ensuremath{+2.48}}
\expandafter\gdef\csname R@an.cvxx.kits.xl.lo\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@an.cvxx.kits.xl.name\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi}}
\expandafter\gdef\csname R@an.cvxx.kits.xl.nfold\endcsname{4}
\expandafter\gdef\csname R@an.cvxx.kits.xl.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.cvxx.kits.xl.tag\endcsname{V7C1}
\expandafter\gdef\csname R@an.cvxx.state\endcsname{12 of 12 contrasts with all 4 folds finished}
\expandafter\gdef\csname R@an.cvxx.tags\endcsname{xl = V7C1, xa = V7A1, resm = L1, reb = P3c}
\expandafter\gdef\csname R@an.design_space.acdc.basis\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.design_space.acdc.fresh.landed.arms\endcsname{HyReX, ResEnc-matched, ResEnc-M, fn.-identical control}
\expandafter\gdef\csname R@an.design_space.acdc.fresh.n_registered\endcsname{4}
\expandafter\gdef\csname R@an.design_space.acdc.fresh.registered.arms\endcsname{HyReX, ResEnc-M, ResEnc-matched, fn.-identical control}
\expandafter\gdef\csname R@an.design_space.acdc.hero.pp\endcsname{+0.616}
\expandafter\gdef\csname R@an.design_space.acdc.hero.rank\endcsname{1}
\expandafter\gdef\csname R@an.design_space.acdc.l1.pp\endcsname{+0.336}
\expandafter\gdef\csname R@an.design_space.acdc.l1.rank\endcsname{5}
\expandafter\gdef\csname R@an.design_space.acdc.n_eval\endcsname{12}
\expandafter\gdef\csname R@an.design_space.acdc.n_fresh_done\endcsname{4}
\expandafter\gdef\csname R@an.design_space.acdc.pool.n\endcsname{6}
\expandafter\gdef\csname R@an.design_space.acdc.pool.sd\endcsname{0.099}
\expandafter\gdef\csname R@an.design_space.acdc.role\endcsname{guard}
\expandafter\gdef\csname R@an.design_space.acdc.second.arm\endcsname{HyReX-k9}
\expandafter\gdef\csname R@an.design_space.acdc.second.pp\endcsname{+0.573}
\expandafter\gdef\csname R@an.design_space.acdc.second.variant\endcsname{a HyReX variant}
\expandafter\gdef\csname R@an.design_space.acdc.top.arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.design_space.acdc.top.pp\endcsname{+0.616}
\expandafter\gdef\csname R@an.design_space.acdc.top.vs_l1.pp\endcsname{+0.281}
\expandafter\gdef\csname R@an.design_space.alpha\endcsname{0.05}
\expandafter\gdef\csname R@an.design_space.amos.fresh.all.list\endcsname{ResEnc-M +0.465 pp, ResEnc+context +0.455 pp, ResEnc-matched +0.298 pp, ConvNeXt-k3 +0.194 pp, HyReX +0.132 pp}
\expandafter\gdef\csname R@an.design_space.amos.fresh.done.arms\endcsname{HyReX, ResEnc-M, ResEnc-matched, ConvNeXt-k3, ResEnc+context}
\expandafter\gdef\csname R@an.design_space.amos.fresh.done.rug.arms\endcsname{none}
\expandafter\gdef\csname R@an.design_space.amos.fresh.l1.arm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.design_space.amos.fresh.l1.pp\endcsname{+0.465}
\expandafter\gdef\csname R@an.design_space.amos.fresh.l1vsl3.clause\endcsname{ResEnc-M +0.465 pp against HyReX +0.132 pp (ahead by 0.332 pp)}
\expandafter\gdef\csname R@an.design_space.amos.fresh.l1vsl3.pp\endcsname{+0.332}
\expandafter\gdef\csname R@an.design_space.amos.fresh.l1vsl3.word\endcsname{ahead of}
\expandafter\gdef\csname R@an.design_space.amos.fresh.l3.pp\endcsname{+0.132}
\expandafter\gdef\csname R@an.design_space.amos.fresh.lead.pp\endcsname{+0.332}
\expandafter\gdef\csname R@an.design_space.amos.fresh.n\endcsname{5}
\expandafter\gdef\csname R@an.design_space.amos.fresh.n_all\endcsname{5}
\expandafter\gdef\csname R@an.design_space.amos.fresh.six.l3.rank\endcsname{5}
\expandafter\gdef\csname R@an.design_space.amos.fresh.six.lead.pp\endcsname{+0.332}
\expandafter\gdef\csname R@an.design_space.amos.fresh.six.n\endcsname{5}
\expandafter\gdef\csname R@an.design_space.amos.fresh.six.n_set\endcsname{6}
\expandafter\gdef\csname R@an.design_space.amos.fresh.six.top.arm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.design_space.amos.fresh.six.top.pp\endcsname{+0.465}
\expandafter\gdef\csname R@an.design_space.amos.fresh.top.arm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.design_space.amos.fresh.top.clause\endcsname{the highest of the 5 AMOS22 fresh means that have landed is ResEnc-M's +0.465 pp (reference design)}
\expandafter\gdef\csname R@an.design_space.amos.fresh.top.pp\endcsname{+0.465}
\expandafter\gdef\csname R@an.design_space.amos.fresh.top.role\endcsname{reference}
\expandafter\gdef\csname R@an.design_space.amos.rep.arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.design_space.amos.rep.fresh\endcsname{+0.132}
\expandafter\gdef\csname R@an.design_space.amos.rep.fresh.margin\endcsname{-0.218}
\expandafter\gdef\csname R@an.design_space.amos.rep.fresh.word\endcsname{does not reach}
\expandafter\gdef\csname R@an.design_space.amos.rep.m\endcsname{2}
\expandafter\gdef\csname R@an.design_space.amos.rep.ratio\endcsname{1.33}
\expandafter\gdef\csname R@an.design_space.amos.rep.resolved\endcsname{no}
\expandafter\gdef\csname R@an.design_space.amos.rep.s0\endcsname{+0.382}
\expandafter\gdef\csname R@an.design_space.amos.rep.s0.margin\endcsname{+0.032}
\expandafter\gdef\csname R@an.design_space.amos.rep.s0.word\endcsname{clears}
\expandafter\gdef\csname R@an.design_space.amos.rep.sd_obs\endcsname{0.209}
\expandafter\gdef\csname R@an.design_space.amos.rep.se\endcsname{0.100}
\expandafter\gdef\csname R@an.design_space.amos.rep.se_obs\endcsname{0.148}
\expandafter\gdef\csname R@an.design_space.amos.rep.seedhi\endcsname{+0.280}
\expandafter\gdef\csname R@an.design_space.amos.rep.seedlo\endcsname{-0.016}
\expandafter\gdef\csname R@an.design_space.amos.rep.sign\endcsname{positive}
\expandafter\gdef\csname R@an.design_space.amos.rep.spread\endcsname{0.296}
\expandafter\gdef\csname R@an.design_space.amos.rep.state\endcsname{not survived}
\expandafter\gdef\csname R@an.design_space.amos.sep.clause\endcsname{at two fresh seeds AMOS22 separates ResEnc-M's +0.465 pp, ResEnc+context's +0.455 pp and ResEnc-matched's +0.298 pp and does not separate ConvNeXt-k3's +0.194 pp or HyReX's +0.132 pp (registered SE 0.100 pp; separation threshold 0.196 pp)}
\expandafter\gdef\csname R@an.design_space.amos.sep.floor.pp\endcsname{0.196}
\expandafter\gdef\csname R@an.design_space.amos.sep.floor.t.df\endcsname{5}
\expandafter\gdef\csname R@an.design_space.amos.sep.floor.t.pp\endcsname{0.257}
\expandafter\gdef\csname R@an.design_space.amos.sep.l1.arm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.design_space.amos.sep.l1.pp\endcsname{+0.465}
\expandafter\gdef\csname R@an.design_space.amos.sep.l1.ratio_obs\endcsname{2.36}
\expandafter\gdef\csname R@an.design_space.amos.sep.l1.ratio_reg\endcsname{4.66}
\expandafter\gdef\csname R@an.design_space.amos.sep.l1.robust\endcsname{yes}
\expandafter\gdef\csname R@an.design_space.amos.sep.l1.se_obs\endcsname{0.197}
\expandafter\gdef\csname R@an.design_space.amos.sep.l1.se_reg\endcsname{0.100}
\expandafter\gdef\csname R@an.design_space.amos.sep.l1.word\endcsname{separates}
\expandafter\gdef\csname R@an.design_space.amos.sep.l1b.arm\endcsname{ResEnc-matched}
\expandafter\gdef\csname R@an.design_space.amos.sep.l1b.pp\endcsname{+0.298}
\expandafter\gdef\csname R@an.design_space.amos.sep.l1b.ratio_obs\endcsname{2.31}
\expandafter\gdef\csname R@an.design_space.amos.sep.l1b.ratio_reg\endcsname{2.98}
\expandafter\gdef\csname R@an.design_space.amos.sep.l1b.robust\endcsname{yes}
\expandafter\gdef\csname R@an.design_space.amos.sep.l1b.se_obs\endcsname{0.129}
\expandafter\gdef\csname R@an.design_space.amos.sep.l1b.se_reg\endcsname{0.100}
\expandafter\gdef\csname R@an.design_space.amos.sep.l1b.word\endcsname{separates}
\expandafter\gdef\csname R@an.design_space.amos.sep.l2.arm\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.design_space.amos.sep.l2.pp\endcsname{+0.194}
\expandafter\gdef\csname R@an.design_space.amos.sep.l2.ratio_obs\endcsname{3.21}
\expandafter\gdef\csname R@an.design_space.amos.sep.l2.ratio_reg\endcsname{1.95}
\expandafter\gdef\csname R@an.design_space.amos.sep.l2.robust\endcsname{yes}
\expandafter\gdef\csname R@an.design_space.amos.sep.l2.se_obs\endcsname{0.061}
\expandafter\gdef\csname R@an.design_space.amos.sep.l2.se_reg\endcsname{0.100}
\expandafter\gdef\csname R@an.design_space.amos.sep.l2.word\endcsname{does not separate}
\expandafter\gdef\csname R@an.design_space.amos.sep.l3.arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.design_space.amos.sep.l3.pp\endcsname{+0.132}
\expandafter\gdef\csname R@an.design_space.amos.sep.l3.ratio_obs\endcsname{0.90}
\expandafter\gdef\csname R@an.design_space.amos.sep.l3.ratio_reg\endcsname{1.33}
\expandafter\gdef\csname R@an.design_space.amos.sep.l3.robust\endcsname{yes}
\expandafter\gdef\csname R@an.design_space.amos.sep.l3.se_obs\endcsname{0.148}
\expandafter\gdef\csname R@an.design_space.amos.sep.l3.se_reg\endcsname{0.100}
\expandafter\gdef\csname R@an.design_space.amos.sep.l3.word\endcsname{does not separate}
\expandafter\gdef\csname R@an.design_space.amos.sep.l4.arm\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.design_space.amos.sep.l4.pp\endcsname{+0.455}
\expandafter\gdef\csname R@an.design_space.amos.sep.l4.ratio_obs\endcsname{4.44}
\expandafter\gdef\csname R@an.design_space.amos.sep.l4.ratio_reg\endcsname{4.56}
\expandafter\gdef\csname R@an.design_space.amos.sep.l4.robust\endcsname{yes}
\expandafter\gdef\csname R@an.design_space.amos.sep.l4.se_obs\endcsname{0.102}
\expandafter\gdef\csname R@an.design_space.amos.sep.l4.se_reg\endcsname{0.100}
\expandafter\gdef\csname R@an.design_space.amos.sep.l4.word\endcsname{separates}
\expandafter\gdef\csname R@an.design_space.amos.sep.n\endcsname{5}
\expandafter\gdef\csname R@an.design_space.amos.sep.n_basis_dependent\endcsname{0}
\expandafter\gdef\csname R@an.design_space.amos.sep.n_notsep\endcsname{2}
\expandafter\gdef\csname R@an.design_space.amos.sep.n_sep\endcsname{3}
\expandafter\gdef\csname R@an.design_space.amos.sep.notsep.arms\endcsname{ConvNeXt-k3, HyReX}
\expandafter\gdef\csname R@an.design_space.amos.sep.se_reg\endcsname{0.100}
\expandafter\gdef\csname R@an.design_space.amos.sep.sep.arms\endcsname{ResEnc-M, ResEnc+context, ResEnc-matched}
\expandafter\gdef\csname R@an.design_space.amos.sep.v7c1.arm\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.design_space.amos.sep.v7c1.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.design_space.amos.sep.v7c1.ratio_obs\endcsname{\pend}
\expandafter\gdef\csname R@an.design_space.amos.sep.v7c1.ratio_reg\endcsname{\pend}
\expandafter\gdef\csname R@an.design_space.amos.sep.v7c1.robust\endcsname{\pend}
\expandafter\gdef\csname R@an.design_space.amos.sep.v7c1.se_obs\endcsname{\pend}
\expandafter\gdef\csname R@an.design_space.amos.sep.v7c1.se_reg\endcsname{\pend}
\expandafter\gdef\csname R@an.design_space.amos.sep.v7c1.word\endcsname{\pend}
\expandafter\gdef\csname R@an.design_space.amos.sep.v8b2.arm\endcsname{Stem1}
\expandafter\gdef\csname R@an.design_space.amos.sep.v8b2.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.design_space.amos.sep.v8b2.ratio_obs\endcsname{\pend}
\expandafter\gdef\csname R@an.design_space.amos.sep.v8b2.ratio_reg\endcsname{\pend}
\expandafter\gdef\csname R@an.design_space.amos.sep.v8b2.robust\endcsname{\pend}
\expandafter\gdef\csname R@an.design_space.amos.sep.v8b2.se_obs\endcsname{\pend}
\expandafter\gdef\csname R@an.design_space.amos.sep.v8b2.se_reg\endcsname{\pend}
\expandafter\gdef\csname R@an.design_space.amos.sep.v8b2.word\endcsname{\pend}
\expandafter\gdef\csname R@an.design_space.atlas.agent.arms\endcsname{HyReX, ConvNeXt-k3, ResEnc+context, HyReX+context, HyReX, finer ConvNeXt, HyReX point-fuse, HyReX+dec. capacity, LeanDec, default+GN16, LeanAdd, LeanAdd-NeXt, HyReX-LeanDec, LeanTrunk, Stem1, CoarseStack, StackDec, LeanDeepMid+FD, LeanSep, LeanDil, LeanDeepMid, LeanNeXt-s5, HyReX-k9}
\expandafter\gdef\csname R@an.design_space.atlas.move.clause\endcsname{where the move is shorter than an arrowhead (ResEnc+context, HyReX, finer ConvNeXt, HyReX point-fuse, LeanDec, fn.-identical control, LeanAdd, LeanAdd-NeXt, HyReX-LeanDec, Stem1, CoarseStack, StackDec, LeanDeepMid+FD, LeanSep, LeanDeepMid, LeanNeXt-s5, HyReX-k9) the fresh mean is drawn inside its own seed-0 ring}
\expandafter\gdef\csname R@an.design_space.atlas.move.diag.arms\endcsname{ResEnc-M, ResEnc-matched, ConvNeXt-k3, HyReX, ResEnc+context}
\expandafter\gdef\csname R@an.design_space.atlas.move.n\endcsname{25}
\expandafter\gdef\csname R@an.design_space.atlas.move.n_arrow\endcsname{9}
\expandafter\gdef\csname R@an.design_space.atlas.move.n_diag\endcsname{5}
\expandafter\gdef\csname R@an.design_space.atlas.move.n_ring\endcsname{16}
\expandafter\gdef\csname R@an.design_space.atlas.move.ring.amos\endcsname{+0.000}
\expandafter\gdef\csname R@an.design_space.atlas.move.ring.arms\endcsname{ResEnc+context, HyReX, finer ConvNeXt, HyReX point-fuse, LeanDec, fn.-identical control, LeanAdd, LeanAdd-NeXt, HyReX-LeanDec, Stem1, CoarseStack, StackDec, LeanDeepMid+FD, LeanSep, LeanDeepMid, LeanNeXt-s5, HyReX-k9}
\expandafter\gdef\csname R@an.design_space.atlas.move.ring.kits\endcsname{-0.771}
\expandafter\gdef\csname R@an.design_space.atlas.pending.amos.arms\endcsname{LeanNeXt-s5, Stem1}
\expandafter\gdef\csname R@an.design_space.atlas.pending.clause\endcsname{2 registered AMOS22 fresh means have no value yet (LeanNeXt-s5, Stem1), drawn as a dotted ring at the left edge of the panel}
\expandafter\gdef\csname R@an.design_space.atlas.roles.clause\endcsname{22 agent designs, 6 attribution arms, 3 matched controls and 1 reference design}
\expandafter\gdef\csname R@an.design_space.atlas.unlabelled.arms\endcsname{HyReX w/o GRN, HyReX-k3, HyReX+pooled skip, LeanNeXt-k3, LeanFullDec, NarrowTrunk, ResEnc-matched, ResEnc+context, HyReX+context, branch control, HyReX, finer ConvNeXt, HyReX point-fuse, HyReX+dec. capacity, LeanDec, LeanAdd, LeanAdd-NeXt, HyReX-LeanDec, LeanDeepMid+FD, LeanSep, LeanDeepMid, LeanNeXt-s5, HyReX-k9}
\expandafter\gdef\csname R@an.design_space.atlas.unlabelled.clause\endcsname{22 arm names have no collision-free place on the plane and are left off (HyReX w/o GRN, HyReX-k3, HyReX+pooled skip, LeanNeXt-k3, LeanFullDec, NarrowTrunk, ResEnc-matched, ResEnc+context, HyReX+context, branch control, HyReX, finer ConvNeXt, HyReX point-fuse, HyReX+dec. capacity, LeanDec, LeanAdd, LeanAdd-NeXt, HyReX-LeanDec, LeanDeepMid+FD, LeanSep, LeanDeepMid, LeanNeXt-s5, HyReX-k9), each named in the factor map; the name of 1 registered reference line is left to the caption}
\expandafter\gdef\csname R@an.design_space.atlas.unlabelled.lines\endcsname{1}
\expandafter\gdef\csname R@an.design_space.atlas.unlabelled.n\endcsname{22}
\expandafter\gdef\csname R@an.design_space.bar.guard\endcsname{-0.15}
\expandafter\gdef\csname R@an.design_space.bar.nonempty\endcsname{+0.20}
\expandafter\gdef\csname R@an.design_space.bar.pairfloor\endcsname{0.50}
\expandafter\gdef\csname R@an.design_space.bar.primary\endcsname{+0.35}
\expandafter\gdef\csname R@an.design_space.conf.clause\endcsname{1 group of structural choices cannot be told apart by the arms that have a result; 1 (context module = dilation mixing) cannot be split by any registered arm}
\expandafter\gdef\csname R@an.design_space.conf.ctx.mark\endcsname{$^{\ddagger}$}
\expandafter\gdef\csname R@an.design_space.conf.ctx.n_cols\endcsname{2}
\expandafter\gdef\csname R@an.design_space.conf.ctx.names\endcsname{context module = dilation mixing}
\expandafter\gdef\csname R@an.design_space.conf.ctx.sep\endcsname{no registered arm}
\expandafter\gdef\csname R@an.design_space.conf.n_cols_perm\endcsname{2}
\expandafter\gdef\csname R@an.design_space.conf.n_cols_tmp\endcsname{0}
\expandafter\gdef\csname R@an.design_space.conf.n_perm\endcsname{1}
\expandafter\gdef\csname R@an.design_space.conf.n_rows\endcsname{1}
\expandafter\gdef\csname R@an.design_space.conf.n_tmp\endcsname{0}
\expandafter\gdef\csname R@an.design_space.conf.n_tmp_arms\endcsname{0}
\expandafter\gdef\csname R@an.design_space.conf.perm.names\endcsname{context module = dilation mixing}
\expandafter\gdef\csname R@an.design_space.conf.tmp.arms\endcsname{none}
\expandafter\gdef\csname R@an.design_space.conf.tmp.names\endcsname{none}
\expandafter\gdef\csname R@an.design_space.ellipse.amos\endcsname{0.264}
\expandafter\gdef\csname R@an.design_space.ellipse.both2sd.arms\endcsname{HyReX, ResEnc-M, ResEnc+context, branch control, HyReX w/o GRN, HyReX+pooled skip, HyReX+dec. capacity, LeanDec, default+GN16, LeanTrunk, NarrowTrunk, LeanDeepMid+FD, LeanDil, LeanNeXt-k3, HyReX-k9}
\expandafter\gdef\csname R@an.design_space.ellipse.kits\endcsname{1.836}
\expandafter\gdef\csname R@an.design_space.ellipse.n_both2sd\endcsname{15}
\expandafter\gdef\csname R@an.design_space.ellipse.n_both2sd.ctl\endcsname{2}
\expandafter\gdef\csname R@an.design_space.ellipse.n_inside\endcsname{3}
\expandafter\gdef\csname R@an.design_space.ellipse.n_outside\endcsname{29}
\expandafter\gdef\csname R@an.design_space.exact.max.n\endcsname{16}
\expandafter\gdef\csname R@an.design_space.exact.ties.max.n\endcsname{14}
\expandafter\gdef\csname R@an.design_space.feature.bigk.amos.diff\endcsname{-0.12}
\expandafter\gdef\csname R@an.design_space.feature.bigk.amos.m0\endcsname{+0.11}
\expandafter\gdef\csname R@an.design_space.feature.bigk.amos.m1\endcsname{-0.01}
\expandafter\gdef\csname R@an.design_space.feature.bigk.amos.n0\endcsname{16}
\expandafter\gdef\csname R@an.design_space.feature.bigk.amos.n0_abs\endcsname{13}
\expandafter\gdef\csname R@an.design_space.feature.bigk.amos.n0_ctl\endcsname{3}
\expandafter\gdef\csname R@an.design_space.feature.bigk.amos.n1\endcsname{22}
\expandafter\gdef\csname R@an.design_space.feature.bigk.amos.se\endcsname{0.04}
\expandafter\gdef\csname R@an.design_space.feature.bigk.def\endcsname{depthwise kernel $\ge 5$ (hollow: ConvNeXt with $3^3$ only)}
\expandafter\gdef\csname R@an.design_space.feature.bigk.kits.diff\endcsname{+1.03}
\expandafter\gdef\csname R@an.design_space.feature.bigk.kits.m0\endcsname{+1.12}
\expandafter\gdef\csname R@an.design_space.feature.bigk.kits.m1\endcsname{+2.15}
\expandafter\gdef\csname R@an.design_space.feature.bigk.kits.n0\endcsname{11}
\expandafter\gdef\csname R@an.design_space.feature.bigk.kits.n0_abs\endcsname{8}
\expandafter\gdef\csname R@an.design_space.feature.bigk.kits.n0_ctl\endcsname{3}
\expandafter\gdef\csname R@an.design_space.feature.bigk.kits.n1\endcsname{21}
\expandafter\gdef\csname R@an.design_space.feature.bigk.kits.se\endcsname{0.30}
\expandafter\gdef\csname R@an.design_space.feature.bigk.name\endcsname{depthwise $k\ge5$}
\expandafter\gdef\csname R@an.design_space.feature.coarsenext.amos.diff\endcsname{-0.09}
\expandafter\gdef\csname R@an.design_space.feature.coarsenext.amos.m0\endcsname{+0.11}
\expandafter\gdef\csname R@an.design_space.feature.coarsenext.amos.m1\endcsname{+0.01}
\expandafter\gdef\csname R@an.design_space.feature.coarsenext.amos.n0\endcsname{13}
\expandafter\gdef\csname R@an.design_space.feature.coarsenext.amos.n0_abs\endcsname{13}
\expandafter\gdef\csname R@an.design_space.feature.coarsenext.amos.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.coarsenext.amos.n1\endcsname{25}
\expandafter\gdef\csname R@an.design_space.feature.coarsenext.amos.se\endcsname{0.04}
\expandafter\gdef\csname R@an.design_space.feature.coarsenext.def\endcsname{ConvNeXt block at encoder stage 3--5}
\expandafter\gdef\csname R@an.design_space.feature.coarsenext.kits.diff\endcsname{+1.01}
\expandafter\gdef\csname R@an.design_space.feature.coarsenext.kits.m0\endcsname{+1.04}
\expandafter\gdef\csname R@an.design_space.feature.coarsenext.kits.m1\endcsname{+2.05}
\expandafter\gdef\csname R@an.design_space.feature.coarsenext.kits.n0\endcsname{8}
\expandafter\gdef\csname R@an.design_space.feature.coarsenext.kits.n0_abs\endcsname{8}
\expandafter\gdef\csname R@an.design_space.feature.coarsenext.kits.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.coarsenext.kits.n1\endcsname{24}
\expandafter\gdef\csname R@an.design_space.feature.coarsenext.kits.se\endcsname{0.32}
\expandafter\gdef\csname R@an.design_space.feature.coarsenext.name\endcsname{ConvNeXt, stages 3--5}
\expandafter\gdef\csname R@an.design_space.feature.coarsethin.def\endcsname{one convolution instead of the plan's two at a plain encoder stage 3--5}
\expandafter\gdef\csname R@an.design_space.feature.coarsethin.name\endcsname{1-conv encoder, stages 3--5}
\expandafter\gdef\csname R@an.design_space.feature.coarsewide.amos.diff\endcsname{+0.19}
\expandafter\gdef\csname R@an.design_space.feature.coarsewide.amos.m0\endcsname{-0.05}
\expandafter\gdef\csname R@an.design_space.feature.coarsewide.amos.m1\endcsname{+0.14}
\expandafter\gdef\csname R@an.design_space.feature.coarsewide.amos.n0\endcsname{19}
\expandafter\gdef\csname R@an.design_space.feature.coarsewide.amos.n0_abs\endcsname{13}
\expandafter\gdef\csname R@an.design_space.feature.coarsewide.amos.n0_ctl\endcsname{6}
\expandafter\gdef\csname R@an.design_space.feature.coarsewide.amos.n1\endcsname{19}
\expandafter\gdef\csname R@an.design_space.feature.coarsewide.amos.se\endcsname{0.04}
\expandafter\gdef\csname R@an.design_space.feature.coarsewide.def\endcsname{ConvNeXt block at two or more of the three coarse encoder stages 3--5 (hollow: at exactly one of them)}
\expandafter\gdef\csname R@an.design_space.feature.coarsewide.kits.diff\endcsname{+0.50}
\expandafter\gdef\csname R@an.design_space.feature.coarsewide.kits.m0\endcsname{+1.51}
\expandafter\gdef\csname R@an.design_space.feature.coarsewide.kits.m1\endcsname{+2.02}
\expandafter\gdef\csname R@an.design_space.feature.coarsewide.kits.n0\endcsname{14}
\expandafter\gdef\csname R@an.design_space.feature.coarsewide.kits.n0_abs\endcsname{8}
\expandafter\gdef\csname R@an.design_space.feature.coarsewide.kits.n0_ctl\endcsname{6}
\expandafter\gdef\csname R@an.design_space.feature.coarsewide.kits.n1\endcsname{18}
\expandafter\gdef\csname R@an.design_space.feature.coarsewide.kits.se\endcsname{0.28}
\expandafter\gdef\csname R@an.design_space.feature.coarsewide.name\endcsname{ConvNeXt, $\ge2$ coarse stages}
\expandafter\gdef\csname R@an.design_space.feature.ctx.amos.diff\endcsname{+0.19}
\expandafter\gdef\csname R@an.design_space.feature.ctx.amos.m0\endcsname{+0.03}
\expandafter\gdef\csname R@an.design_space.feature.ctx.amos.m1\endcsname{+0.22}
\expandafter\gdef\csname R@an.design_space.feature.ctx.amos.n0\endcsname{36}
\expandafter\gdef\csname R@an.design_space.feature.ctx.amos.n0_abs\endcsname{36}
\expandafter\gdef\csname R@an.design_space.feature.ctx.amos.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.ctx.amos.n1\endcsname{2}
\expandafter\gdef\csname R@an.design_space.feature.ctx.amos.se\endcsname{0.09}
\expandafter\gdef\csname R@an.design_space.feature.ctx.def\endcsname{context module (pyramid pooling / global context)}
\expandafter\gdef\csname R@an.design_space.feature.ctx.kits.diff\endcsname{+0.60}
\expandafter\gdef\csname R@an.design_space.feature.ctx.kits.m0\endcsname{+1.76}
\expandafter\gdef\csname R@an.design_space.feature.ctx.kits.m1\endcsname{+2.36}
\expandafter\gdef\csname R@an.design_space.feature.ctx.kits.n0\endcsname{30}
\expandafter\gdef\csname R@an.design_space.feature.ctx.kits.n0_abs\endcsname{30}
\expandafter\gdef\csname R@an.design_space.feature.ctx.kits.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.ctx.kits.n1\endcsname{2}
\expandafter\gdef\csname R@an.design_space.feature.ctx.kits.se\endcsname{0.58}
\expandafter\gdef\csname R@an.design_space.feature.ctx.name\endcsname{context module}
\expandafter\gdef\csname R@an.design_space.feature.deccap.def\endcsname{a decoder stage deeper than the plan}
\expandafter\gdef\csname R@an.design_space.feature.deccap.name\endcsname{deeper decoder}
\expandafter\gdef\csname R@an.design_space.feature.decnext.amos.diff\endcsname{+0.33}
\expandafter\gdef\csname R@an.design_space.feature.decnext.amos.m0\endcsname{-0.05}
\expandafter\gdef\csname R@an.design_space.feature.decnext.amos.m1\endcsname{+0.28}
\expandafter\gdef\csname R@an.design_space.feature.decnext.amos.n0\endcsname{27}
\expandafter\gdef\csname R@an.design_space.feature.decnext.amos.n0_abs\endcsname{27}
\expandafter\gdef\csname R@an.design_space.feature.decnext.amos.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.decnext.amos.n1\endcsname{11}
\expandafter\gdef\csname R@an.design_space.feature.decnext.amos.se\endcsname{0.04}
\expandafter\gdef\csname R@an.design_space.feature.decnext.def\endcsname{ConvNeXt block in the decoder}
\expandafter\gdef\csname R@an.design_space.feature.decnext.kits.diff\endcsname{+0.15}
\expandafter\gdef\csname R@an.design_space.feature.decnext.kits.m0\endcsname{+1.75}
\expandafter\gdef\csname R@an.design_space.feature.decnext.kits.m1\endcsname{+1.90}
\expandafter\gdef\csname R@an.design_space.feature.decnext.kits.n0\endcsname{22}
\expandafter\gdef\csname R@an.design_space.feature.decnext.kits.n0_abs\endcsname{22}
\expandafter\gdef\csname R@an.design_space.feature.decnext.kits.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.decnext.kits.n1\endcsname{10}
\expandafter\gdef\csname R@an.design_space.feature.decnext.kits.se\endcsname{0.30}
\expandafter\gdef\csname R@an.design_space.feature.decnext.name\endcsname{ConvNeXt decoder}
\expandafter\gdef\csname R@an.design_space.feature.decpoint.def\endcsname{point-wise ($1^3$) decoder fusion}
\expandafter\gdef\csname R@an.design_space.feature.decpoint.name\endcsname{point-wise fusion}
\expandafter\gdef\csname R@an.design_space.feature.decres.amos.diff\endcsname{+0.35}
\expandafter\gdef\csname R@an.design_space.feature.decres.amos.m0\endcsname{-0.05}
\expandafter\gdef\csname R@an.design_space.feature.decres.amos.m1\endcsname{+0.30}
\expandafter\gdef\csname R@an.design_space.feature.decres.amos.n0\endcsname{28}
\expandafter\gdef\csname R@an.design_space.feature.decres.amos.n0_abs\endcsname{28}
\expandafter\gdef\csname R@an.design_space.feature.decres.amos.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.decres.amos.n1\endcsname{10}
\expandafter\gdef\csname R@an.design_space.feature.decres.amos.se\endcsname{0.05}
\expandafter\gdef\csname R@an.design_space.feature.decres.def\endcsname{residual block in the decoder}
\expandafter\gdef\csname R@an.design_space.feature.decres.kits.diff\endcsname{+0.56}
\expandafter\gdef\csname R@an.design_space.feature.decres.kits.m0\endcsname{+1.62}
\expandafter\gdef\csname R@an.design_space.feature.decres.kits.m1\endcsname{+2.18}
\expandafter\gdef\csname R@an.design_space.feature.decres.kits.n0\endcsname{22}
\expandafter\gdef\csname R@an.design_space.feature.decres.kits.n0_abs\endcsname{22}
\expandafter\gdef\csname R@an.design_space.feature.decres.kits.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.decres.kits.n1\endcsname{10}
\expandafter\gdef\csname R@an.design_space.feature.decres.kits.se\endcsname{0.30}
\expandafter\gdef\csname R@an.design_space.feature.decres.name\endcsname{residual decoder}
\expandafter\gdef\csname R@an.design_space.feature.decthin.amos.diff\endcsname{-0.27}
\expandafter\gdef\csname R@an.design_space.feature.decthin.amos.m0\endcsname{+0.16}
\expandafter\gdef\csname R@an.design_space.feature.decthin.amos.m1\endcsname{-0.10}
\expandafter\gdef\csname R@an.design_space.feature.decthin.amos.n0\endcsname{21}
\expandafter\gdef\csname R@an.design_space.feature.decthin.amos.n0_abs\endcsname{21}
\expandafter\gdef\csname R@an.design_space.feature.decthin.amos.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.decthin.amos.n1\endcsname{17}
\expandafter\gdef\csname R@an.design_space.feature.decthin.amos.se\endcsname{0.04}
\expandafter\gdef\csname R@an.design_space.feature.decthin.def\endcsname{one convolution per decoder stage}
\expandafter\gdef\csname R@an.design_space.feature.decthin.kits.diff\endcsname{+0.74}
\expandafter\gdef\csname R@an.design_space.feature.decthin.kits.m0\endcsname{+1.43}
\expandafter\gdef\csname R@an.design_space.feature.decthin.kits.m1\endcsname{+2.17}
\expandafter\gdef\csname R@an.design_space.feature.decthin.kits.n0\endcsname{16}
\expandafter\gdef\csname R@an.design_space.feature.decthin.kits.n0_abs\endcsname{16}
\expandafter\gdef\csname R@an.design_space.feature.decthin.kits.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.decthin.kits.n1\endcsname{16}
\expandafter\gdef\csname R@an.design_space.feature.decthin.kits.se\endcsname{0.28}
\expandafter\gdef\csname R@an.design_space.feature.decthin.name\endcsname{1-conv decoder}
\expandafter\gdef\csname R@an.design_space.feature.dilmix.amos.diff\endcsname{+0.19}
\expandafter\gdef\csname R@an.design_space.feature.dilmix.amos.m0\endcsname{+0.03}
\expandafter\gdef\csname R@an.design_space.feature.dilmix.amos.m1\endcsname{+0.22}
\expandafter\gdef\csname R@an.design_space.feature.dilmix.amos.n0\endcsname{36}
\expandafter\gdef\csname R@an.design_space.feature.dilmix.amos.n0_abs\endcsname{36}
\expandafter\gdef\csname R@an.design_space.feature.dilmix.amos.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.dilmix.amos.n1\endcsname{2}
\expandafter\gdef\csname R@an.design_space.feature.dilmix.amos.se\endcsname{0.09}
\expandafter\gdef\csname R@an.design_space.feature.dilmix.def\endcsname{multi-dilation branch block}
\expandafter\gdef\csname R@an.design_space.feature.dilmix.kits.diff\endcsname{+0.60}
\expandafter\gdef\csname R@an.design_space.feature.dilmix.kits.m0\endcsname{+1.76}
\expandafter\gdef\csname R@an.design_space.feature.dilmix.kits.m1\endcsname{+2.36}
\expandafter\gdef\csname R@an.design_space.feature.dilmix.kits.n0\endcsname{30}
\expandafter\gdef\csname R@an.design_space.feature.dilmix.kits.n0_abs\endcsname{30}
\expandafter\gdef\csname R@an.design_space.feature.dilmix.kits.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.dilmix.kits.n1\endcsname{2}
\expandafter\gdef\csname R@an.design_space.feature.dilmix.kits.se\endcsname{0.58}
\expandafter\gdef\csname R@an.design_space.feature.dilmix.name\endcsname{dilation mixing}
\expandafter\gdef\csname R@an.design_space.feature.dwdil.def\endcsname{dilated depthwise operator, three taps per axis at dilation $(k{-}1)/2$ instead of one dense kernel (hollow: ConvNeXt with the dense kernel)}
\expandafter\gdef\csname R@an.design_space.feature.dwdil.name\endcsname{dilated depthwise}
\expandafter\gdef\csname R@an.design_space.feature.dwsep.def\endcsname{rank-1 separable depthwise operator, three 1-D passes in series instead of one dense kernel (hollow: ConvNeXt with the dense kernel)}
\expandafter\gdef\csname R@an.design_space.feature.dwsep.name\endcsname{separable depthwise}
\expandafter\gdef\csname R@an.design_space.feature.finenext.amos.diff\endcsname{+0.25}
\expandafter\gdef\csname R@an.design_space.feature.finenext.amos.m0\endcsname{+0.02}
\expandafter\gdef\csname R@an.design_space.feature.finenext.amos.m1\endcsname{+0.27}
\expandafter\gdef\csname R@an.design_space.feature.finenext.amos.n0\endcsname{35}
\expandafter\gdef\csname R@an.design_space.feature.finenext.amos.n0_abs\endcsname{35}
\expandafter\gdef\csname R@an.design_space.feature.finenext.amos.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.finenext.amos.n1\endcsname{3}
\expandafter\gdef\csname R@an.design_space.feature.finenext.amos.se\endcsname{0.07}
\expandafter\gdef\csname R@an.design_space.feature.finenext.def\endcsname{ConvNeXt block at encoder stage 0--2}
\expandafter\gdef\csname R@an.design_space.feature.finenext.kits.diff\endcsname{-0.85}
\expandafter\gdef\csname R@an.design_space.feature.finenext.kits.m0\endcsname{+1.85}
\expandafter\gdef\csname R@an.design_space.feature.finenext.kits.m1\endcsname{+1.00}
\expandafter\gdef\csname R@an.design_space.feature.finenext.kits.n0\endcsname{30}
\expandafter\gdef\csname R@an.design_space.feature.finenext.kits.n0_abs\endcsname{30}
\expandafter\gdef\csname R@an.design_space.feature.finenext.kits.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.finenext.kits.n1\endcsname{2}
\expandafter\gdef\csname R@an.design_space.feature.finenext.kits.se\endcsname{0.58}
\expandafter\gdef\csname R@an.design_space.feature.finenext.name\endcsname{ConvNeXt, stages 0--2}
\expandafter\gdef\csname R@an.design_space.feature.fineres.amos.diff\endcsname{+0.50}
\expandafter\gdef\csname R@an.design_space.feature.fineres.amos.m0\endcsname{-0.20}
\expandafter\gdef\csname R@an.design_space.feature.fineres.amos.m1\endcsname{+0.31}
\expandafter\gdef\csname R@an.design_space.feature.fineres.amos.n0\endcsname{20}
\expandafter\gdef\csname R@an.design_space.feature.fineres.amos.n0_abs\endcsname{20}
\expandafter\gdef\csname R@an.design_space.feature.fineres.amos.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.fineres.amos.n1\endcsname{18}
\expandafter\gdef\csname R@an.design_space.feature.fineres.amos.se\endcsname{0.04}
\expandafter\gdef\csname R@an.design_space.feature.fineres.def\endcsname{dense residual block at encoder stage 0--2}
\expandafter\gdef\csname R@an.design_space.feature.fineres.kits.diff\endcsname{+0.68}
\expandafter\gdef\csname R@an.design_space.feature.fineres.kits.m0\endcsname{+1.46}
\expandafter\gdef\csname R@an.design_space.feature.fineres.kits.m1\endcsname{+2.14}
\expandafter\gdef\csname R@an.design_space.feature.fineres.kits.n0\endcsname{16}
\expandafter\gdef\csname R@an.design_space.feature.fineres.kits.n0_abs\endcsname{16}
\expandafter\gdef\csname R@an.design_space.feature.fineres.kits.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.fineres.kits.n1\endcsname{16}
\expandafter\gdef\csname R@an.design_space.feature.fineres.kits.se\endcsname{0.28}
\expandafter\gdef\csname R@an.design_space.feature.fineres.name\endcsname{dense residual, stages 0--2}
\expandafter\gdef\csname R@an.design_space.feature.finethin.amos.diff\endcsname{-0.59}
\expandafter\gdef\csname R@an.design_space.feature.finethin.amos.m0\endcsname{+0.07}
\expandafter\gdef\csname R@an.design_space.feature.finethin.amos.m1\endcsname{-0.52}
\expandafter\gdef\csname R@an.design_space.feature.finethin.amos.n0\endcsname{36}
\expandafter\gdef\csname R@an.design_space.feature.finethin.amos.n0_abs\endcsname{36}
\expandafter\gdef\csname R@an.design_space.feature.finethin.amos.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.finethin.amos.n1\endcsname{2}
\expandafter\gdef\csname R@an.design_space.feature.finethin.amos.se\endcsname{0.09}
\expandafter\gdef\csname R@an.design_space.feature.finethin.def\endcsname{one convolution instead of the plan's two at a plain encoder stage 0--2 (Addendum AR: LeanDec's rule moved to the encoder)}
\expandafter\gdef\csname R@an.design_space.feature.finethin.kits.diff\endcsname{+0.51}
\expandafter\gdef\csname R@an.design_space.feature.finethin.kits.m0\endcsname{+1.76}
\expandafter\gdef\csname R@an.design_space.feature.finethin.kits.m1\endcsname{+2.28}
\expandafter\gdef\csname R@an.design_space.feature.finethin.kits.n0\endcsname{30}
\expandafter\gdef\csname R@an.design_space.feature.finethin.kits.n0_abs\endcsname{30}
\expandafter\gdef\csname R@an.design_space.feature.finethin.kits.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.finethin.kits.n1\endcsname{2}
\expandafter\gdef\csname R@an.design_space.feature.finethin.kits.se\endcsname{0.58}
\expandafter\gdef\csname R@an.design_space.feature.finethin.name\endcsname{1-conv encoder, stages 0--2}
\expandafter\gdef\csname R@an.design_space.feature.gn.def\endcsname{GroupNorm-16 instead of InstanceNorm}
\expandafter\gdef\csname R@an.design_space.feature.gn.name\endcsname{GroupNorm-16}
\expandafter\gdef\csname R@an.design_space.feature.grn.amos.diff\endcsname{-0.15}
\expandafter\gdef\csname R@an.design_space.feature.grn.amos.m0\endcsname{+0.13}
\expandafter\gdef\csname R@an.design_space.feature.grn.amos.m1\endcsname{-0.02}
\expandafter\gdef\csname R@an.design_space.feature.grn.amos.n0\endcsname{15}
\expandafter\gdef\csname R@an.design_space.feature.grn.amos.n0_abs\endcsname{13}
\expandafter\gdef\csname R@an.design_space.feature.grn.amos.n0_ctl\endcsname{2}
\expandafter\gdef\csname R@an.design_space.feature.grn.amos.n1\endcsname{23}
\expandafter\gdef\csname R@an.design_space.feature.grn.amos.se\endcsname{0.04}
\expandafter\gdef\csname R@an.design_space.feature.grn.def\endcsname{global response normalisation (hollow: ConvNeXt without GRN)}
\expandafter\gdef\csname R@an.design_space.feature.grn.kits.diff\endcsname{+0.94}
\expandafter\gdef\csname R@an.design_space.feature.grn.kits.m0\endcsname{+1.15}
\expandafter\gdef\csname R@an.design_space.feature.grn.kits.m1\endcsname{+2.09}
\expandafter\gdef\csname R@an.design_space.feature.grn.kits.n0\endcsname{10}
\expandafter\gdef\csname R@an.design_space.feature.grn.kits.n0_abs\endcsname{8}
\expandafter\gdef\csname R@an.design_space.feature.grn.kits.n0_ctl\endcsname{2}
\expandafter\gdef\csname R@an.design_space.feature.grn.kits.n1\endcsname{22}
\expandafter\gdef\csname R@an.design_space.feature.grn.kits.se\endcsname{0.30}
\expandafter\gdef\csname R@an.design_space.feature.grn.name\endcsname{GRN}
\expandafter\gdef\csname R@an.design_space.feature.k3full.def\endcsname{full-resolution kernel $3^3$ instead of the planned $1\times3\times3$}
\expandafter\gdef\csname R@an.design_space.feature.k3full.name\endcsname{full-res $3^3$}
\expandafter\gdef\csname R@an.design_space.feature.skipadd.amos.diff\endcsname{-0.45}
\expandafter\gdef\csname R@an.design_space.feature.skipadd.amos.m0\endcsname{+0.21}
\expandafter\gdef\csname R@an.design_space.feature.skipadd.amos.m1\endcsname{-0.24}
\expandafter\gdef\csname R@an.design_space.feature.skipadd.amos.n0\endcsname{24}
\expandafter\gdef\csname R@an.design_space.feature.skipadd.amos.n0_abs\endcsname{24}
\expandafter\gdef\csname R@an.design_space.feature.skipadd.amos.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.skipadd.amos.n1\endcsname{14}
\expandafter\gdef\csname R@an.design_space.feature.skipadd.amos.se\endcsname{0.04}
\expandafter\gdef\csname R@an.design_space.feature.skipadd.def\endcsname{the encoder skip is ADDED to the upsampled decoder feature, not concatenated (hollow: the same library with the concatenating default)}
\expandafter\gdef\csname R@an.design_space.feature.skipadd.kits.diff\endcsname{+0.47}
\expandafter\gdef\csname R@an.design_space.feature.skipadd.kits.m0\endcsname{+1.59}
\expandafter\gdef\csname R@an.design_space.feature.skipadd.kits.m1\endcsname{+2.06}
\expandafter\gdef\csname R@an.design_space.feature.skipadd.kits.n0\endcsname{18}
\expandafter\gdef\csname R@an.design_space.feature.skipadd.kits.n0_abs\endcsname{18}
\expandafter\gdef\csname R@an.design_space.feature.skipadd.kits.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.skipadd.kits.n1\endcsname{14}
\expandafter\gdef\csname R@an.design_space.feature.skipadd.kits.se\endcsname{0.28}
\expandafter\gdef\csname R@an.design_space.feature.skipadd.name\endcsname{additive skip fusion}
\expandafter\gdef\csname R@an.design_space.feature.skippool.amos.diff\endcsname{-0.18}
\expandafter\gdef\csname R@an.design_space.feature.skippool.amos.m0\endcsname{+0.14}
\expandafter\gdef\csname R@an.design_space.feature.skippool.amos.m1\endcsname{-0.04}
\expandafter\gdef\csname R@an.design_space.feature.skippool.amos.n0\endcsname{18}
\expandafter\gdef\csname R@an.design_space.feature.skippool.amos.n0_abs\endcsname{6}
\expandafter\gdef\csname R@an.design_space.feature.skippool.amos.n0_ctl\endcsname{12}
\expandafter\gdef\csname R@an.design_space.feature.skippool.amos.n1\endcsname{20}
\expandafter\gdef\csname R@an.design_space.feature.skippool.amos.se\endcsname{0.04}
\expandafter\gdef\csname R@an.design_space.feature.skippool.def\endcsname{pooled residual skip (hollow: strided)}
\expandafter\gdef\csname R@an.design_space.feature.skippool.kits.diff\endcsname{+0.60}
\expandafter\gdef\csname R@an.design_space.feature.skippool.kits.m0\endcsname{+1.50}
\expandafter\gdef\csname R@an.design_space.feature.skippool.kits.m1\endcsname{+2.10}
\expandafter\gdef\csname R@an.design_space.feature.skippool.kits.n0\endcsname{16}
\expandafter\gdef\csname R@an.design_space.feature.skippool.kits.n0_abs\endcsname{4}
\expandafter\gdef\csname R@an.design_space.feature.skippool.kits.n0_ctl\endcsname{12}
\expandafter\gdef\csname R@an.design_space.feature.skippool.kits.n1\endcsname{16}
\expandafter\gdef\csname R@an.design_space.feature.skippool.kits.se\endcsname{0.28}
\expandafter\gdef\csname R@an.design_space.feature.skippool.name\endcsname{pooled residual skip}
\expandafter\gdef\csname R@an.design_space.feature.stackdeep.amos.diff\endcsname{-0.48}
\expandafter\gdef\csname R@an.design_space.feature.stackdeep.amos.m0\endcsname{+0.07}
\expandafter\gdef\csname R@an.design_space.feature.stackdeep.amos.m1\endcsname{-0.41}
\expandafter\gdef\csname R@an.design_space.feature.stackdeep.amos.n0\endcsname{36}
\expandafter\gdef\csname R@an.design_space.feature.stackdeep.amos.n0_abs\endcsname{36}
\expandafter\gdef\csname R@an.design_space.feature.stackdeep.amos.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.stackdeep.amos.n1\endcsname{2}
\expandafter\gdef\csname R@an.design_space.feature.stackdeep.amos.se\endcsname{0.09}
\expandafter\gdef\csname R@an.design_space.feature.stackdeep.def\endcsname{more blocks at one encoder stage than any stage of the library residual preset holds (more than its deepest stage)}
\expandafter\gdef\csname R@an.design_space.feature.stackdeep.kits.diff\endcsname{-0.26}
\expandafter\gdef\csname R@an.design_space.feature.stackdeep.kits.m0\endcsname{+1.81}
\expandafter\gdef\csname R@an.design_space.feature.stackdeep.kits.m1\endcsname{+1.56}
\expandafter\gdef\csname R@an.design_space.feature.stackdeep.kits.n0\endcsname{30}
\expandafter\gdef\csname R@an.design_space.feature.stackdeep.kits.n0_abs\endcsname{30}
\expandafter\gdef\csname R@an.design_space.feature.stackdeep.kits.n0_ctl\endcsname{0}
\expandafter\gdef\csname R@an.design_space.feature.stackdeep.kits.n1\endcsname{2}
\expandafter\gdef\csname R@an.design_space.feature.stackdeep.kits.se\endcsname{0.58}
\expandafter\gdef\csname R@an.design_space.feature.stackdeep.name\endcsname{deep ConvNeXt stack}
\expandafter\gdef\csname R@an.design_space.feature.upalt.def\endcsname{learned-offset upsampling (hollow: trilinear control)}
\expandafter\gdef\csname R@an.design_space.feature.upalt.name\endcsname{offset upsampling}
\expandafter\gdef\csname R@an.design_space.feature.warp.def\endcsname{sub-voxel logit warp (hollow: function-identical control)}
\expandafter\gdef\csname R@an.design_space.feature.warp.name\endcsname{logit warp}
\expandafter\gdef\csname R@an.design_space.feature.widthvec.def\endcsname{channel counts that are not the plan's at some stage}
\expandafter\gdef\csname R@an.design_space.feature.widthvec.name\endcsname{channel widths}
\expandafter\gdef\csname R@an.design_space.feature.zdil.amos.diff\endcsname{+0.12}
\expandafter\gdef\csname R@an.design_space.feature.zdil.amos.m0\endcsname{+0.04}
\expandafter\gdef\csname R@an.design_space.feature.zdil.amos.m1\endcsname{+0.16}
\expandafter\gdef\csname R@an.design_space.feature.zdil.amos.n0\endcsname{36}
\expandafter\gdef\csname R@an.design_space.feature.zdil.amos.n0_abs\endcsname{35}
\expandafter\gdef\csname R@an.design_space.feature.zdil.amos.n0_ctl\endcsname{1}
\expandafter\gdef\csname R@an.design_space.feature.zdil.amos.n1\endcsname{2}
\expandafter\gdef\csname R@an.design_space.feature.zdil.amos.se\endcsname{0.09}
\expandafter\gdef\csname R@an.design_space.feature.zdil.def\endcsname{through-plane dilations (hollow: the same block at dilation 1)}
\expandafter\gdef\csname R@an.design_space.feature.zdil.name\endcsname{through-plane dilation}
\expandafter\gdef\csname R@an.design_space.feature.zgate.def\endcsname{per-sample anisotropy gate}
\expandafter\gdef\csname R@an.design_space.feature.zgate.name\endcsname{anisotropy gate}
\expandafter\gdef\csname R@an.design_space.features.n0_mixed\endcsname{9}
\expandafter\gdef\csname R@an.design_space.features.n_cells\endcsname{31}
\expandafter\gdef\csname R@an.design_space.features.se.clause\endcsname{the null the $\pm$ assumes (arm deltas are iid seed noise) is the null the AMOS22 range test rejects ($p=0.004$), so the $\pm$ is a floor on the spread and never a 95\% interval}
\expandafter\gdef\csname R@an.design_space.fresh.bar.amos.arms\endcsname{ResEnc-M, ResEnc+context}
\expandafter\gdef\csname R@an.design_space.fresh.bar.amos.n\endcsname{2}
\expandafter\gdef\csname R@an.design_space.fresh.bar.both.arms\endcsname{ResEnc-M, ResEnc+context}
\expandafter\gdef\csname R@an.design_space.fresh.bar.both.n\endcsname{2}
\expandafter\gdef\csname R@an.design_space.fresh.bar.clause\endcsname{Arms with a fresh mean at or above the +0.35 pp primary bar: ResEnc-M and ResEnc+context on AMOS22; ResEnc-M, LeanDeepMid, LeanNeXt-s5, HyReX+dec. capacity, LeanSep, ResEnc-matched, LeanDeepMid+FD, LeanAdd, ResEnc+context, HyReX-LeanDec, HyReX, LeanDec, StackDec, LeanDil, Stem1, HyReX-k9, HyReX+context, HyReX point-fuse, LeanAdd-NeXt, LeanTrunk, CoarseStack, fn.-identical control, branch control and HyReX, finer ConvNeXt on KiTS23; on both co-primaries ResEnc-M and ResEnc+context}
\expandafter\gdef\csname R@an.design_space.fresh.bar.kits.arms\endcsname{ResEnc-M, LeanDeepMid, LeanNeXt-s5, HyReX+dec. capacity, LeanSep, ResEnc-matched, LeanDeepMid+FD, LeanAdd, ResEnc+context, HyReX-LeanDec, HyReX, LeanDec, StackDec, LeanDil, Stem1, HyReX-k9, HyReX+context, HyReX point-fuse, LeanAdd-NeXt, LeanTrunk, CoarseStack, fn.-identical control, branch control, HyReX, finer ConvNeXt}
\expandafter\gdef\csname R@an.design_space.fresh.bar.kits.n\endcsname{24}
\expandafter\gdef\csname R@an.design_space.kits.ctl.arm\endcsname{branch control}
\expandafter\gdef\csname R@an.design_space.kits.ctl.fresh_n\endcsname{2}
\expandafter\gdef\csname R@an.design_space.kits.ctl.params\endcsname{31.21}
\expandafter\gdef\csname R@an.design_space.kits.ctl.params.amosplan\endcsname{31.14}
\expandafter\gdef\csname R@an.design_space.kits.ctl.params.base\endcsname{31.20}
\expandafter\gdef\csname R@an.design_space.kits.ctl.params.baseamosplan\endcsname{31.12}
\expandafter\gdef\csname R@an.design_space.kits.ctl.params.gap\endcsname{+0.01}
\expandafter\gdef\csname R@an.design_space.kits.ctl.plan\endcsname{KiTS23 plan}
\expandafter\gdef\csname R@an.design_space.kits.ctl.pp\endcsname{+2.636}
\expandafter\gdef\csname R@an.design_space.kits.ctl.seed\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.design_space.kits.ctl.vs_l3.m\endcsname{2}
\expandafter\gdef\csname R@an.design_space.kits.ctl.vs_l3.pp\endcsname{+0.542}
\expandafter\gdef\csname R@an.design_space.kits.ctl.vs_l3.ratio\endcsname{0.56}
\expandafter\gdef\csname R@an.design_space.kits.ctl.vs_l3.se\endcsname{0.974}
\expandafter\gdef\csname R@an.design_space.kits.ctl.vs_l3.word\endcsname{is not resolved}
\expandafter\gdef\csname R@an.design_space.kits.fresh.all.list\endcsname{ResEnc-M +3.475 pp, LeanDeepMid +2.662 pp, LeanNeXt-s5 +2.440 pp, HyReX+dec. capacity +2.401 pp, LeanSep +2.382 pp, ResEnc-matched +2.313 pp, LeanDeepMid+FD +2.289 pp, LeanAdd +2.285 pp, ResEnc+context +2.246 pp, HyReX-LeanDec +2.165 pp, HyReX +2.094 pp, LeanDec +1.892 pp, StackDec +1.877 pp, LeanDil +1.838 pp, Stem1 +1.731 pp, HyReX-k9 +1.704 pp, HyReX+context +1.591 pp, HyReX point-fuse +1.477 pp, LeanAdd-NeXt +1.448 pp, LeanTrunk +1.375 pp, CoarseStack +1.249 pp, fn.-identical control +1.176 pp, branch control +1.067 pp, HyReX, finer ConvNeXt +0.570 pp, ConvNeXt-k3 +0.110 pp}
\expandafter\gdef\csname R@an.design_space.kits.fresh.l1.arm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.design_space.kits.fresh.l1.pp\endcsname{+3.475}
\expandafter\gdef\csname R@an.design_space.kits.fresh.l1vsl3.clause\endcsname{ResEnc-M +3.475 pp against HyReX +2.094 pp (ahead by 1.382 pp)}
\expandafter\gdef\csname R@an.design_space.kits.fresh.l1vsl3.pp\endcsname{+1.382}
\expandafter\gdef\csname R@an.design_space.kits.fresh.l1vsl3.word\endcsname{ahead of}
\expandafter\gdef\csname R@an.design_space.kits.fresh.l3.pp\endcsname{+2.094}
\expandafter\gdef\csname R@an.design_space.kits.fresh.l3.rank\endcsname{11}
\expandafter\gdef\csname R@an.design_space.kits.fresh.l3.rank.clause\endcsname{11 of 25}
\expandafter\gdef\csname R@an.design_space.kits.fresh.lead.pp\endcsname{+1.382}
\expandafter\gdef\csname R@an.design_space.kits.fresh.n\endcsname{25}
\expandafter\gdef\csname R@an.design_space.kits.fresh.n_all\endcsname{25}
\expandafter\gdef\csname R@an.design_space.kits.fresh.n_ranked\endcsname{25}
\expandafter\gdef\csname R@an.design_space.kits.fresh.six.l3.rank\endcsname{4}
\expandafter\gdef\csname R@an.design_space.kits.fresh.six.lead.pp\endcsname{+1.382}
\expandafter\gdef\csname R@an.design_space.kits.fresh.six.n\endcsname{6}
\expandafter\gdef\csname R@an.design_space.kits.fresh.six.n_set\endcsname{6}
\expandafter\gdef\csname R@an.design_space.kits.fresh.six.top.arm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.design_space.kits.fresh.six.top.pp\endcsname{+3.475}
\expandafter\gdef\csname R@an.design_space.kits.fresh.top.arm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.design_space.kits.fresh.top.clause\endcsname{the highest of the 25 KiTS23 fresh means that have landed is ResEnc-M's +3.475 pp (reference design)}
\expandafter\gdef\csname R@an.design_space.kits.fresh.top.pp\endcsname{+3.475}
\expandafter\gdef\csname R@an.design_space.kits.fresh.top.role\endcsname{reference}
\expandafter\gdef\csname R@an.design_space.kits.fresh.verb\endcsname{reorder}
\expandafter\gdef\csname R@an.design_space.kits.move.max\endcsname{1.569}
\expandafter\gdef\csname R@an.design_space.kits.move.max.arm\endcsname{branch control}
\expandafter\gdef\csname R@an.design_space.kits.move.min\endcsname{0.048}
\expandafter\gdef\csname R@an.design_space.kits.move.min.arm\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.design_space.kits.move.n\endcsname{25}
\expandafter\gdef\csname R@an.design_space.kits.near.all.maxgap\endcsname{8.586}
\expandafter\gdef\csname R@an.design_space.kits.near.all.maxgap.arm\endcsname{default+GN16}
\expandafter\gdef\csname R@an.design_space.kits.near.all.n\endcsname{27}
\expandafter\gdef\csname R@an.design_space.kits.near.all.n_within_ctl\endcsname{23}
\expandafter\gdef\csname R@an.design_space.kits.near.arms\endcsname{ConvNeXt-k3, HyReX, HyReX+context, branch control, full-res addition, coarse-capacity ctl, logit warp, fn.-identical control, LeanDec, HyReX+pooled skip, default+GN16, HyReX, finer ConvNeXt, HyReX point-fuse, HyReX w/o GRN, HyReX-k3, HyReX-LeanDec, LeanAdd, LeanAdd-NeXt, HyReX-k9, LeanDeepMid, LeanDeepMid+FD, LeanFullDec, LeanSep, LeanDil, LeanNeXt-s5, LeanNeXt-k3, CoarseStack, StackDec, LeanTrunk, Stem1, NarrowTrunk}
\expandafter\gdef\csname R@an.design_space.kits.near.base.params\endcsname{31.20}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.d0\endcsname{\ensuremath{+2.636}}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.d0_vs_l3\endcsname{\ensuremath{+0.542}}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.d0_vs_l3.se\endcsname{0.974}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.d0_vs_l3.word\endcsname{is not resolved}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.dfresh\endcsname{\ensuremath{+1.067}}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.est\endcsname{\ensuremath{+1.067}}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.est.kind\endcsname{two-seed fresh mean}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.est.phrase\endcsname{\ensuremath{+1.067} pp on its two fresh seeds}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.fresh_n\endcsname{2}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.gap\endcsname{\ensuremath{-1.027}}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.gap.abs\endcsname{1.027}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.gap.kind\endcsname{two-seed fresh mean against HyReX's fresh mean}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.gap.reading\endcsname{more than one contrast standard error below HyReX}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.gap.se\endcsname{0.795}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.label\endcsname{the branch control}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.move\endcsname{\ensuremath{-1.569}}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.name\endcsname{branch control}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.params\endcsname{31.21}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.params.ratio\endcsname{1.00}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.ratio\endcsname{1.29}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.role\endcsname{matched control}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.role.label\endcsname{matched control (the z-dilation mixing network with every dilation set to 1)}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.role.source\endcsname{Addendum V1 and V3}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.se\endcsname{0.795}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.six.d0\endcsname{\ensuremath{+2.392}}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.six.dfresh\endcsname{\ensuremath{+0.823}}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.state\endcsname{survived}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.vs_l3\endcsname{\ensuremath{-1.027}}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.vs_l3.abs\endcsname{1.027}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.vs_l3.dir\endcsname{below}
\expandafter\gdef\csname R@an.design_space.kits.near.branch.word\endcsname{is not resolved}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.d0\endcsname{\ensuremath{+3.507}}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.d0_vs_l3\endcsname{\ensuremath{+1.414}}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.d0_vs_l3.se\endcsname{0.974}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.d0_vs_l3.word\endcsname{is not resolved}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.dfresh\endcsname{\ensuremath{+2.401}}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.est\endcsname{\ensuremath{+2.401}}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.est.kind\endcsname{two-seed fresh mean}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.est.phrase\endcsname{\ensuremath{+2.401} pp on its two fresh seeds}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.fresh_n\endcsname{2}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.gap\endcsname{\ensuremath{+0.307}}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.gap.abs\endcsname{0.307}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.gap.kind\endcsname{two-seed fresh mean against HyReX's fresh mean}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.gap.reading\endcsname{within one contrast standard error of HyReX}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.gap.se\endcsname{0.795}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.label\endcsname{C1 (HyReX with a dense-residual coarse decoder)}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.move\endcsname{\ensuremath{-1.106}}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.name\endcsname{HyReX+dec. capacity}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.params\endcsname{52.41}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.params.ratio\endcsname{1.68}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.ratio\endcsname{0.39}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.role\endcsname{agent design}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.role.label\endcsname{agent design}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.role.source\endcsname{the registration of the arm}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.se\endcsname{0.795}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.six.d0\endcsname{\ensuremath{+3.264}}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.six.dfresh\endcsname{\ensuremath{+2.157}}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.state\endcsname{survived}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.vs_l3\endcsname{\ensuremath{+0.307}}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.vs_l3.abs\endcsname{0.307}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.vs_l3.dir\endcsname{above}
\expandafter\gdef\csname R@an.design_space.kits.near.c1.word\endcsname{is not resolved}
\expandafter\gdef\csname R@an.design_space.kits.near.ctl.arms\endcsname{branch control, fn.-identical control, LeanDec}
\expandafter\gdef\csname R@an.design_space.kits.near.ctl.branch\endcsname{mixed}
\expandafter\gdef\csname R@an.design_space.kits.near.ctl.landed.arms\endcsname{branch control, fn.-identical control, LeanDec}
\expandafter\gdef\csname R@an.design_space.kits.near.ctl.maxgap\endcsname{1.028}
\expandafter\gdef\csname R@an.design_space.kits.near.ctl.maxgap.arm\endcsname{branch control}
\expandafter\gdef\csname R@an.design_space.kits.near.ctl.maxratio\endcsname{1.29}
\expandafter\gdef\csname R@an.design_space.kits.near.ctl.mingap\endcsname{0.202}
\expandafter\gdef\csname R@an.design_space.kits.near.ctl.mingap.arm\endcsname{LeanDec}
\expandafter\gdef\csname R@an.design_space.kits.near.ctl.n\endcsname{3}
\expandafter\gdef\csname R@an.design_space.kits.near.ctl.n_landed\endcsname{3}
\expandafter\gdef\csname R@an.design_space.kits.near.ctl.pending.arms\endcsname{none}
\expandafter\gdef\csname R@an.design_space.kits.near.ctl.reading.clause\endcsname{the landed controls do not agree: some read within one contrast standard error of HyReX and some beyond it}
\expandafter\gdef\csname R@an.design_space.kits.near.ctl.within.clause\endcsname{the KiTS23 gains of the branch control (\ensuremath{+1.067} pp on its two fresh seeds), the function-identical control (\ensuremath{+1.176} pp on its two fresh seeds) and LeanDec (\ensuremath{+1.892} pp on its two fresh seeds) lie within 1.028 pp of HyReX's \ensuremath{+2.094} pp fresh mean}
\expandafter\gdef\csname R@an.design_space.kits.near.dparams\endcsname{1.0}
\expandafter\gdef\csname R@an.design_space.kits.near.fresh_pending.arms\endcsname{none}
\expandafter\gdef\csname R@an.design_space.kits.near.hyrex.d0\endcsname{\ensuremath{+2.842}}
\expandafter\gdef\csname R@an.design_space.kits.near.hyrex.dfresh\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.design_space.kits.near.hyrex.est\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.design_space.kits.near.hyrex.est.kind\endcsname{two-seed fresh mean}
\expandafter\gdef\csname R@an.design_space.kits.near.hyrex.est.phrase\endcsname{\ensuremath{+2.094} pp on its two fresh seeds}
\expandafter\gdef\csname R@an.design_space.kits.near.hyrex.fresh_n\endcsname{2}
\expandafter\gdef\csname R@an.design_space.kits.near.hyrex.label\endcsname{HyReX}
\expandafter\gdef\csname R@an.design_space.kits.near.hyrex.move\endcsname{\ensuremath{-0.748}}
\expandafter\gdef\csname R@an.design_space.kits.near.hyrex.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.design_space.kits.near.hyrex.params\endcsname{29.66}
\expandafter\gdef\csname R@an.design_space.kits.near.hyrex.params.ratio\endcsname{0.95}
\expandafter\gdef\csname R@an.design_space.kits.near.hyrex.ref\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.design_space.kits.near.hyrex.role\endcsname{agent design}
\expandafter\gdef\csname R@an.design_space.kits.near.hyrex.role.label\endcsname{agent design}
\expandafter\gdef\csname R@an.design_space.kits.near.hyrex.role.source\endcsname{the registration of the arm}
\expandafter\gdef\csname R@an.design_space.kits.near.hyrex.six.d0\endcsname{\ensuremath{+2.598}}
\expandafter\gdef\csname R@an.design_space.kits.near.hyrex.six.dfresh\endcsname{\ensuremath{+1.850}}
\expandafter\gdef\csname R@an.design_space.kits.near.hyrex.state\endcsname{survived}
\expandafter\gdef\csname R@an.design_space.kits.near.landed.arms\endcsname{ConvNeXt-k3, HyReX, HyReX+context, branch control, fn.-identical control, LeanDec, HyReX+pooled skip, default+GN16, HyReX, finer ConvNeXt, HyReX point-fuse, HyReX w/o GRN, HyReX-k3, HyReX-LeanDec, LeanAdd, LeanAdd-NeXt, HyReX-k9, LeanDeepMid, LeanDeepMid+FD, LeanFullDec, LeanSep, LeanDil, LeanNeXt-s5, LeanNeXt-k3, CoarseStack, StackDec, LeanTrunk, Stem1, NarrowTrunk}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.d0\endcsname{\ensuremath{+2.355}}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.d0_vs_l3\endcsname{\ensuremath{+0.262}}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.d0_vs_l3.se\endcsname{0.974}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.d0_vs_l3.word\endcsname{is not resolved}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.dfresh\endcsname{\ensuremath{+1.892}}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.est\endcsname{\ensuremath{+1.892}}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.est.kind\endcsname{two-seed fresh mean}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.est.phrase\endcsname{\ensuremath{+1.892} pp on its two fresh seeds}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.fresh_n\endcsname{2}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.gap\endcsname{\ensuremath{-0.202}}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.gap.abs\endcsname{0.202}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.gap.kind\endcsname{two-seed fresh mean against HyReX's fresh mean}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.gap.reading\endcsname{within one contrast standard error of HyReX}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.gap.se\endcsname{0.795}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.label\endcsname{LeanDec}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.move\endcsname{\ensuremath{-0.464}}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.params\endcsname{26.08}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.params.ratio\endcsname{0.84}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.ratio\endcsname{0.25}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.role\endcsname{decoder-depth control}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.role.label\endcsname{decoder-depth control (the default topology with one convolution per decoder stage)}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.role.source\endcsname{CLAIM_FRAME 11 and Addendum O3}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.se\endcsname{0.795}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.six.d0\endcsname{\ensuremath{+2.112}}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.six.dfresh\endcsname{\ensuremath{+1.648}}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.state\endcsname{survived}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.vs_l3\endcsname{\ensuremath{-0.202}}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.vs_l3.abs\endcsname{0.202}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.vs_l3.dir\endcsname{below}
\expandafter\gdef\csname R@an.design_space.kits.near.lean.word\endcsname{is not resolved}
\expandafter\gdef\csname R@an.design_space.kits.near.n\endcsname{31}
\expandafter\gdef\csname R@an.design_space.kits.near.n_fresh\endcsname{21}
\expandafter\gdef\csname R@an.design_space.kits.near.n_fresh_pending\endcsname{0}
\expandafter\gdef\csname R@an.design_space.kits.near.n_landed\endcsname{28}
\expandafter\gdef\csname R@an.design_space.kits.near.n_pending\endcsname{3}
\expandafter\gdef\csname R@an.design_space.kits.near.n_unregistered\endcsname{5}
\expandafter\gdef\csname R@an.design_space.kits.near.others.arms\endcsname{ConvNeXt-k3, HyReX+context, HyReX+pooled skip, default+GN16, HyReX, finer ConvNeXt, HyReX point-fuse, HyReX w/o GRN, HyReX-k3, HyReX-LeanDec, LeanAdd, LeanAdd-NeXt, HyReX-k9, LeanDeepMid, LeanDeepMid+FD, LeanFullDec, LeanSep, LeanDil, LeanNeXt-s5, LeanNeXt-k3, CoarseStack, StackDec, LeanTrunk, Stem1, NarrowTrunk}
\expandafter\gdef\csname R@an.design_space.kits.near.others.clause\endcsname{the other default-sized or smaller designs with a KiTS23 result read LeanDeepMid \ensuremath{+2.662} pp on its two fresh seeds, HyReX w/o GRN \ensuremath{+2.561} pp at its one seed, NarrowTrunk \ensuremath{+2.535} pp at its one seed, LeanNeXt-s5 \ensuremath{+2.440} pp on its two fresh seeds, LeanSep \ensuremath{+2.382} pp on its two fresh seeds, LeanDeepMid+FD \ensuremath{+2.289} pp on its two fresh seeds, LeanAdd \ensuremath{+2.285} pp on its two fresh seeds, HyReX-LeanDec \ensuremath{+2.165} pp on its two fresh seeds, LeanNeXt-k3 \ensuremath{+2.000} pp at its one seed, HyReX+pooled skip \ensuremath{+1.893} pp at its one seed, StackDec \ensuremath{+1.877} pp on its two fresh seeds, LeanDil \ensuremath{+1.838} pp on its two fresh seeds, Stem1 \ensuremath{+1.731} pp on its two fresh seeds, HyReX-k9 \ensuremath{+1.704} pp on its two fresh seeds, HyReX+context \ensuremath{+1.591} pp on its two fresh seeds, HyReX point-fuse \ensuremath{+1.477} pp on its two fresh seeds, LeanAdd-NeXt \ensuremath{+1.448} pp on its two fresh seeds, LeanTrunk \ensuremath{+1.375} pp on its two fresh seeds, HyReX-k3 \ensuremath{+1.366} pp at its one seed, CoarseStack \ensuremath{+1.249} pp on its two fresh seeds, HyReX, finer ConvNeXt \ensuremath{+0.570} pp on its two fresh seeds, LeanFullDec \ensuremath{+0.542} pp at its one seed, ConvNeXt-k3 \ensuremath{+0.110} pp on its two fresh seeds and default+GN16 \ensuremath{-6.492} pp at its one seed}
\expandafter\gdef\csname R@an.design_space.kits.near.others.hi\endcsname{\ensuremath{+2.662}}
\expandafter\gdef\csname R@an.design_space.kits.near.others.hi.arm\endcsname{LeanDeepMid}
\expandafter\gdef\csname R@an.design_space.kits.near.others.lo\endcsname{\ensuremath{-6.492}}
\expandafter\gdef\csname R@an.design_space.kits.near.others.lo.arm\endcsname{default+GN16}
\expandafter\gdef\csname R@an.design_space.kits.near.others.n\endcsname{24}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.d0\endcsname{\ensuremath{+1.364}}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.d0_vs_l3\endcsname{\ensuremath{-0.729}}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.d0_vs_l3.se\endcsname{0.974}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.d0_vs_l3.word\endcsname{is not resolved}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.dfresh\endcsname{\ensuremath{+1.176}}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.est\endcsname{\ensuremath{+1.176}}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.est.kind\endcsname{two-seed fresh mean}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.est.phrase\endcsname{\ensuremath{+1.176} pp on its two fresh seeds}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.fresh_n\endcsname{2}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.gap\endcsname{\ensuremath{-0.918}}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.gap.abs\endcsname{0.918}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.gap.kind\endcsname{two-seed fresh mean against HyReX's fresh mean}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.gap.reading\endcsname{more than one contrast standard error below HyReX}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.gap.se\endcsname{0.795}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.label\endcsname{the function-identical control}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.move\endcsname{\ensuremath{-0.189}}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.name\endcsname{fn.-identical control}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.params\endcsname{31.20}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.params.ratio\endcsname{1.00}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.ratio\endcsname{1.15}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.role\endcsname{implementation control}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.role.label\endcsname{implementation control (the function-identical rebuild of the default network)}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.role.source\endcsname{Addendum T1, N4 and W1}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.se\endcsname{0.795}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.six.d0\endcsname{\ensuremath{+1.121}}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.six.dfresh\endcsname{\ensuremath{+0.932}}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.state\endcsname{survived}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.vs_l3\endcsname{\ensuremath{-0.918}}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.vs_l3.abs\endcsname{0.918}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.vs_l3.dir\endcsname{below}
\expandafter\gdef\csname R@an.design_space.kits.near.p3c.word\endcsname{is not resolved}
\expandafter\gdef\csname R@an.design_space.kits.near.pending.arms\endcsname{full-res addition, coarse-capacity ctl, logit warp}
\expandafter\gdef\csname R@an.design_space.kits.near.rule\endcsname{KiTS23-plan parameters at most 1.0 M above the default's}
\expandafter\gdef\csname R@an.design_space.kits.near.six.mean\endcsname{83.622}
\expandafter\gdef\csname R@an.design_space.kits.near.six.n\endcsname{6}
\expandafter\gdef\csname R@an.design_space.kits.near.six.shift\endcsname{\ensuremath{+0.244}}
\expandafter\gdef\csname R@an.design_space.kits.near.unregistered.arms\endcsname{z-dilation mixing, thickness-gated, trilinear control, offset upsampling, full-res 3$^3$}
\expandafter\gdef\csname R@an.design_space.kits.s0.top.arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.design_space.kits.s0.top.pp\endcsname{+2.842}
\expandafter\gdef\csname R@an.design_space.mdes.nsim\endcsname{8000000}
\expandafter\gdef\csname R@an.design_space.n_arms\endcsname{42}
\expandafter\gdef\csname R@an.design_space.n_atlas\endcsname{32}
\expandafter\gdef\csname R@an.design_space.n_atlas.agent\endcsname{22}
\expandafter\gdef\csname R@an.design_space.n_atlas.attribution\endcsname{6}
\expandafter\gdef\csname R@an.design_space.n_atlas.control\endcsname{3}
\expandafter\gdef\csname R@an.design_space.n_atlas.default\endcsname{0}
\expandafter\gdef\csname R@an.design_space.n_atlas.llm\endcsname{0}
\expandafter\gdef\csname R@an.design_space.n_atlas.notagent\endcsname{10}
\expandafter\gdef\csname R@an.design_space.n_atlas.other\endcsname{0}
\expandafter\gdef\csname R@an.design_space.n_atlas.reference\endcsname{1}
\expandafter\gdef\csname R@an.design_space.n_atlas.scaled\endcsname{0}
\expandafter\gdef\csname R@an.design_space.n_atlas.search\endcsname{0}
\expandafter\gdef\csname R@an.design_space.n_feature_confounded\endcsname{2}
\expandafter\gdef\csname R@an.design_space.n_feature_rows\endcsname{15}
\expandafter\gdef\csname R@an.design_space.n_feature_tested\endcsname{16}
\expandafter\gdef\csname R@an.design_space.n_feature_untested\endcsname{11}
\expandafter\gdef\csname R@an.design_space.n_features\endcsname{27}
\expandafter\gdef\csname R@an.design_space.n_fresh_done.amos\endcsname{5}
\expandafter\gdef\csname R@an.design_space.n_fresh_done.amos.rug\endcsname{0}
\expandafter\gdef\csname R@an.design_space.n_fresh_done.kits\endcsname{25}
\expandafter\gdef\csname R@an.design_space.n_fresh_pending.amos\endcsname{2}
\expandafter\gdef\csname R@an.design_space.n_fresh_pending.amos.rug\endcsname{0}
\expandafter\gdef\csname R@an.design_space.n_fresh_pending.kits\endcsname{0}
\expandafter\gdef\csname R@an.design_space.n_map_rows\endcsname{43}
\expandafter\gdef\csname R@an.design_space.n_onlyone\endcsname{21}
\expandafter\gdef\csname R@an.design_space.n_pending\endcsname{4}
\expandafter\gdef\csname R@an.design_space.n_rug_amos\endcsname{6}
\expandafter\gdef\csname R@an.design_space.n_rug_amos.kits_sched\endcsname{1}
\expandafter\gdef\csname R@an.design_space.n_rug_amos.kits_unreg\endcsname{5}
\expandafter\gdef\csname R@an.design_space.n_tri\endcsname{6}
\expandafter\gdef\csname R@an.design_space.n_tri.extra\endcsname{6}
\expandafter\gdef\csname R@an.design_space.nperm.big\endcsname{2000000}
\expandafter\gdef\csname R@an.design_space.onlyone.arms\endcsname{ResEnc-matched, HyReX+context, fn.-identical control, LeanDec, HyReX+pooled skip, HyReX point-fuse, HyReX w/o GRN, HyReX-LeanDec, LeanAdd, LeanAdd-NeXt, LeanDeepMid, LeanFullDec, LeanSep, LeanDil, LeanNeXt-s5, LeanNeXt-k3, CoarseStack, StackDec, LeanTrunk, Stem1, NarrowTrunk}
\expandafter\gdef\csname R@an.design_space.params.amos.base\endcsname{31.12}
\expandafter\gdef\csname R@an.design_space.params.amos.l1\endcsname{102.28}
\expandafter\gdef\csname R@an.design_space.params.amos.l3\endcsname{29.59}
\expandafter\gdef\csname R@an.design_space.params.amos.l3.fewer.pct\endcsname{4.9}
\expandafter\gdef\csname R@an.design_space.params.amos.l3.of_l1.pct\endcsname{29}
\expandafter\gdef\csname R@an.design_space.params.kits.base\endcsname{31.20}
\expandafter\gdef\csname R@an.design_space.params.kits.l1\endcsname{102.35}
\expandafter\gdef\csname R@an.design_space.params.kits.l3\endcsname{29.66}
\expandafter\gdef\csname R@an.design_space.params.kits.l3.fewer.pct\endcsname{4.9}
\expandafter\gdef\csname R@an.design_space.params.kits.l3.of_l1.pct\endcsname{29}
\expandafter\gdef\csname R@an.design_space.params.max\endcsname{102.8}
\expandafter\gdef\csname R@an.design_space.params.min\endcsname{18.2}
\expandafter\gdef\csname R@an.design_space.params.plan\endcsname{AMOS22 plan}
\expandafter\gdef\csname R@an.design_space.ranks.acdc.fresh.clause\endcsname{fresh ACDC seeds: 4 of 4 registered pairs landed - HyReX +0.450 pp, ResEnc-matched +0.319 pp, ResEnc-M +0.242 pp, fn.-identical control +0.117 pp}
\expandafter\gdef\csname R@an.design_space.ranks.acdc.top3.clause\endcsname{ACDC seed-0 $\Delta$Dice, highest three: HyReX +0.616 pp, HyReX+context +0.451 pp, ResEnc-M +0.336 pp; frozen pool SD 0.099 pp over 6 runs}
\expandafter\gdef\csname R@an.design_space.ranks.amos.fresh.clause\endcsname{fresh AMOS22 means: 5 of 6 landed (ResEnc-M, ResEnc+context, ResEnc-matched, ConvNeXt-k3, HyReX), not in this column's order: ResEnc-M +0.465 pp, ResEnc+context +0.455 pp, ResEnc-matched +0.298 pp, ConvNeXt-k3 +0.194 pp, HyReX +0.132 pp}
\expandafter\gdef\csname R@an.design_space.ranks.amos.fresh.order\endcsname{not in this column's order}
\expandafter\gdef\csname R@an.design_space.ranks.basis.clause\endcsname{Discovery-seed-0 ranks of the 6 arms run on all three datasets (ResEnc-M, ResEnc-matched, ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context)}
\expandafter\gdef\csname R@an.design_space.ranks.fresh_column.clause\endcsname{the third column ranks the same arms by their KiTS23 fresh means (the mean of fresh seeds one and two, the selection-free estimate); the gaps beside it carry the rank correlation and the resolution floor of that many arms and no p-value}
\expandafter\gdef\csname R@an.design_space.ranks.kits.fresh.clause\endcsname{the registered fresh KiTS23 seeds reorder this column: the largest fresh mean is ResEnc-M's +3.475 pp and HyReX's +2.094 pp is 4th of 6}
\expandafter\gdef\csname R@an.design_space.ranks.top.clause\endcsname{Rank 1 over rank 2 at seed 0: AMOS22 ResEnc-M +0.217 pp; KiTS23 HyReX +0.316 pp; ACDC HyReX +0.165 pp; registered one-seed pair floor 0.50 pp}
\expandafter\gdef\csname R@an.design_space.refs.acdc.alt\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.design_space.refs.acdc.n\endcsname{6}
\expandafter\gdef\csname R@an.design_space.refs.acdc.n_alt\endcsname{1}
\expandafter\gdef\csname R@an.design_space.refs.acdc.uncompiled.delta_shift\endcsname{-0.007}
\expandafter\gdef\csname R@an.design_space.refs.acdc.uncompiled.n\endcsname{3}
\expandafter\gdef\csname R@an.design_space.refs.acdc.uncompiled.ne_shift\endcsname{+0.007}
\expandafter\gdef\csname R@an.design_space.refs.acdc.uncompiled.shift\endcsname{+0.007}
\expandafter\gdef\csname R@an.design_space.refs.amos.alt\endcsname{uncompiled sub-pool, contemporaneous default runs}
\expandafter\gdef\csname R@an.design_space.refs.amos.contemporaneous.delta_shift\endcsname{-0.011}
\expandafter\gdef\csname R@an.design_space.refs.amos.contemporaneous.n\endcsname{3}
\expandafter\gdef\csname R@an.design_space.refs.amos.contemporaneous.shift\endcsname{+0.011}
\expandafter\gdef\csname R@an.design_space.refs.amos.n\endcsname{6}
\expandafter\gdef\csname R@an.design_space.refs.amos.n_alt\endcsname{2}
\expandafter\gdef\csname R@an.design_space.refs.amos.uncompiled.delta_shift\endcsname{-0.029}
\expandafter\gdef\csname R@an.design_space.refs.amos.uncompiled.n\endcsname{3}
\expandafter\gdef\csname R@an.design_space.refs.amos.uncompiled.ne_shift\endcsname{+0.077}
\expandafter\gdef\csname R@an.design_space.refs.amos.uncompiled.shift\endcsname{+0.029}
\expandafter\gdef\csname R@an.design_space.refs.kits.alt\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.design_space.refs.kits.contemporaneous.delta_shift\endcsname{-0.487}
\expandafter\gdef\csname R@an.design_space.refs.kits.contemporaneous.n\endcsname{3}
\expandafter\gdef\csname R@an.design_space.refs.kits.contemporaneous.shift\endcsname{+0.487}
\expandafter\gdef\csname R@an.design_space.refs.kits.n\endcsname{3}
\expandafter\gdef\csname R@an.design_space.refs.kits.n_alt\endcsname{1}
\expandafter\gdef\csname R@an.design_space.rep.amos.landed\endcsname{1}
\expandafter\gdef\csname R@an.design_space.rep.amos.landed.arms\endcsname{ResEnc-matched}
\expandafter\gdef\csname R@an.design_space.rep.amos.n_done\endcsname{4}
\expandafter\gdef\csname R@an.design_space.rep.amos.notsurvived\endcsname{2}
\expandafter\gdef\csname R@an.design_space.rep.amos.notsurvived.arms\endcsname{HyReX, ConvNeXt-k3}
\expandafter\gdef\csname R@an.design_space.rep.amos.pending\endcsname{2}
\expandafter\gdef\csname R@an.design_space.rep.amos.survived\endcsname{2}
\expandafter\gdef\csname R@an.design_space.rep.amos.survived.arms\endcsname{ResEnc-M, ResEnc+context}
\expandafter\gdef\csname R@an.design_space.rep.kits.landed\endcsname{0}
\expandafter\gdef\csname R@an.design_space.rep.kits.landed.arms\endcsname{none}
\expandafter\gdef\csname R@an.design_space.rep.kits.n_done\endcsname{25}
\expandafter\gdef\csname R@an.design_space.rep.kits.notsurvived\endcsname{1}
\expandafter\gdef\csname R@an.design_space.rep.kits.notsurvived.arms\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.design_space.rep.kits.pending\endcsname{0}
\expandafter\gdef\csname R@an.design_space.rep.kits.survived\endcsname{24}
\expandafter\gdef\csname R@an.design_space.rep.kits.survived.arms\endcsname{HyReX, ResEnc-M, ResEnc-matched, ResEnc+context, HyReX+context, branch control, HyReX, finer ConvNeXt, HyReX point-fuse, HyReX+dec. capacity, LeanDec, fn.-identical control, LeanAdd, LeanAdd-NeXt, HyReX-LeanDec, LeanTrunk, Stem1, CoarseStack, StackDec, LeanDeepMid+FD, LeanSep, LeanDil, LeanDeepMid, LeanNeXt-s5, HyReX-k9}
\expandafter\gdef\csname R@an.design_space.rho.amos_acdc\endcsname{+0.59}
\expandafter\gdef\csname R@an.design_space.rho.amos_acdc.atcrit\endcsname{yes}
\expandafter\gdef\csname R@an.design_space.rho.amos_acdc.clause\endcsname{$\rho=+0.59$ ($n=12$; exact permutation $p=0.049$; $p\le 0.05$ needs $|\rho|\ge 0.59$ at $n=12$)}
\expandafter\gdef\csname R@an.design_space.rho.amos_acdc.edge.sentence\endcsname{ This is exactly the smallest correlation that reaches the 5\,\% level at $n=12$ (exact $p=0.049$); the next smaller attainable correlation has $p=0.052$.}
\expandafter\gdef\csname R@an.design_space.rho.amos_acdc.floor.clause\endcsname{$p\le 0.05$ needs $|\rho|\ge 0.59$ at $n=12$}
\expandafter\gdef\csname R@an.design_space.rho.amos_acdc.mdes\endcsname{0.59}
\expandafter\gdef\csname R@an.design_space.rho.amos_acdc.mdes.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.amos_acdc.mdes.p\endcsname{0.049}
\expandafter\gdef\csname R@an.design_space.rho.amos_acdc.n\endcsname{12}
\expandafter\gdef\csname R@an.design_space.rho.amos_acdc.next.p\endcsname{0.052}
\expandafter\gdef\csname R@an.design_space.rho.amos_acdc.order\endcsname{with detectable agreement}
\expandafter\gdef\csname R@an.design_space.rho.amos_acdc.p\endcsname{0.049}
\expandafter\gdef\csname R@an.design_space.rho.amos_acdc.p.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.amos_acdc.p.eq\endcsname{$p=0.049$}
\expandafter\gdef\csname R@an.design_space.rho.amos_acdc.p.exact\endcsname{0.04888}
\expandafter\gdef\csname R@an.design_space.rho.amos_acdc.p.print\endcsname{0.049}
\expandafter\gdef\csname R@an.design_space.rho.amos_acdc.p.print.eq\endcsname{$p=0.049$}
\expandafter\gdef\csname R@an.design_space.rho.amos_acdc.verdict\endcsname{detectable agreement}
\expandafter\gdef\csname R@an.design_space.rho.amos_acdc.verdict.assoc\endcsname{a detectable positive association}
\expandafter\gdef\csname R@an.design_space.rho.amos_kits\endcsname{+0.12}
\expandafter\gdef\csname R@an.design_space.rho.amos_kits.atcrit\endcsname{n/a}
\expandafter\gdef\csname R@an.design_space.rho.amos_kits.clause\endcsname{$\rho=+0.12$ ($n=32$; Monte-Carlo permutation $p=0.5$; $p\le 0.05$ needs $|\rho|\ge 0.35$ at $n=32$)}
\expandafter\gdef\csname R@an.design_space.rho.amos_kits.edge.sentence\endcsname{{}}
\expandafter\gdef\csname R@an.design_space.rho.amos_kits.floor.clause\endcsname{$p\le 0.05$ needs $|\rho|\ge 0.35$ at $n=32$}
\expandafter\gdef\csname R@an.design_space.rho.amos_kits.mdes\endcsname{0.35}
\expandafter\gdef\csname R@an.design_space.rho.amos_kits.mdes.basis\endcsname{simulated}
\expandafter\gdef\csname R@an.design_space.rho.amos_kits.mdes.p\endcsname{0.050}
\expandafter\gdef\csname R@an.design_space.rho.amos_kits.n\endcsname{32}
\expandafter\gdef\csname R@an.design_space.rho.amos_kits.next.p\endcsname{n/a}
\expandafter\gdef\csname R@an.design_space.rho.amos_kits.order\endcsname{with no detectable agreement}
\expandafter\gdef\csname R@an.design_space.rho.amos_kits.p\endcsname{0.5}
\expandafter\gdef\csname R@an.design_space.rho.amos_kits.p.basis\endcsname{Monte-Carlo}
\expandafter\gdef\csname R@an.design_space.rho.amos_kits.p.eq\endcsname{$p=0.5$}
\expandafter\gdef\csname R@an.design_space.rho.amos_kits.p.exact\endcsname{n/a}
\expandafter\gdef\csname R@an.design_space.rho.amos_kits.p.print\endcsname{0.5}
\expandafter\gdef\csname R@an.design_space.rho.amos_kits.p.print.eq\endcsname{$p=0.5$}
\expandafter\gdef\csname R@an.design_space.rho.amos_kits.verdict\endcsname{no detectable agreement}
\expandafter\gdef\csname R@an.design_space.rho.amos_kits.verdict.assoc\endcsname{no detectable association}
\expandafter\gdef\csname R@an.design_space.rho.amos_s0_fresh\endcsname{+0.60}
\expandafter\gdef\csname R@an.design_space.rho.amos_s0_fresh.atcrit\endcsname{no}
\expandafter\gdef\csname R@an.design_space.rho.amos_s0_fresh.clause\endcsname{$\rho=+0.60$ ($n=5$; exact permutation $p=0.350$; $p\le 0.05$ needs $|\rho|\ge 1.00$ at $n=5$)}
\expandafter\gdef\csname R@an.design_space.rho.amos_s0_fresh.edge.sentence\endcsname{{}}
\expandafter\gdef\csname R@an.design_space.rho.amos_s0_fresh.floor.clause\endcsname{$p\le 0.05$ needs $|\rho|\ge 1.00$ at $n=5$}
\expandafter\gdef\csname R@an.design_space.rho.amos_s0_fresh.mdes\endcsname{1.00}
\expandafter\gdef\csname R@an.design_space.rho.amos_s0_fresh.mdes.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.amos_s0_fresh.mdes.p\endcsname{0.017}
\expandafter\gdef\csname R@an.design_space.rho.amos_s0_fresh.n\endcsname{5}
\expandafter\gdef\csname R@an.design_space.rho.amos_s0_fresh.next.p\endcsname{0.450}
\expandafter\gdef\csname R@an.design_space.rho.amos_s0_fresh.order\endcsname{with no detectable agreement}
\expandafter\gdef\csname R@an.design_space.rho.amos_s0_fresh.p\endcsname{0.350}
\expandafter\gdef\csname R@an.design_space.rho.amos_s0_fresh.p.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.amos_s0_fresh.p.eq\endcsname{$p=0.350$}
\expandafter\gdef\csname R@an.design_space.rho.amos_s0_fresh.p.exact\endcsname{0.35000}
\expandafter\gdef\csname R@an.design_space.rho.amos_s0_fresh.p.print\endcsname{0.350}
\expandafter\gdef\csname R@an.design_space.rho.amos_s0_fresh.p.print.eq\endcsname{$p=0.350$}
\expandafter\gdef\csname R@an.design_space.rho.amos_s0_fresh.verdict\endcsname{no detectable agreement}
\expandafter\gdef\csname R@an.design_space.rho.amos_s0_fresh.verdict.assoc\endcsname{no detectable association}
\expandafter\gdef\csname R@an.design_space.rho.coincidence.clause\endcsname{AMOS22 against KiTS23 at the discovery seed, AMOS22 against ACDC at the discovery seed, KiTS23 discovery seed against KiTS23 fresh mean and KiTS23 fresh mean against ACDC share one rank correlation ($\rho=+0.09$), a sum of squared rank differences of 32 over 6 arms: an arithmetic coincidence of these rankings, not a repeated entry}
\expandafter\gdef\csname R@an.design_space.rho.kits_acdc\endcsname{+0.48}
\expandafter\gdef\csname R@an.design_space.rho.kits_acdc.atcrit\endcsname{no}
\expandafter\gdef\csname R@an.design_space.rho.kits_acdc.clause\endcsname{$\rho=+0.48$ ($n=12$; exact permutation $p=0.121$; $p\le 0.05$ needs $|\rho|\ge 0.59$ at $n=12$)}
\expandafter\gdef\csname R@an.design_space.rho.kits_acdc.edge.sentence\endcsname{{}}
\expandafter\gdef\csname R@an.design_space.rho.kits_acdc.floor.clause\endcsname{$p\le 0.05$ needs $|\rho|\ge 0.59$ at $n=12$}
\expandafter\gdef\csname R@an.design_space.rho.kits_acdc.mdes\endcsname{0.59}
\expandafter\gdef\csname R@an.design_space.rho.kits_acdc.mdes.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.kits_acdc.mdes.p\endcsname{0.049}
\expandafter\gdef\csname R@an.design_space.rho.kits_acdc.n\endcsname{12}
\expandafter\gdef\csname R@an.design_space.rho.kits_acdc.next.p\endcsname{0.128}
\expandafter\gdef\csname R@an.design_space.rho.kits_acdc.order\endcsname{with no detectable agreement}
\expandafter\gdef\csname R@an.design_space.rho.kits_acdc.p\endcsname{0.121}
\expandafter\gdef\csname R@an.design_space.rho.kits_acdc.p.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.kits_acdc.p.eq\endcsname{$p=0.121$}
\expandafter\gdef\csname R@an.design_space.rho.kits_acdc.p.exact\endcsname{0.12147}
\expandafter\gdef\csname R@an.design_space.rho.kits_acdc.p.print\endcsname{0.121}
\expandafter\gdef\csname R@an.design_space.rho.kits_acdc.p.print.eq\endcsname{$p=0.121$}
\expandafter\gdef\csname R@an.design_space.rho.kits_acdc.verdict\endcsname{no detectable agreement}
\expandafter\gdef\csname R@an.design_space.rho.kits_acdc.verdict.assoc\endcsname{no detectable association}
\expandafter\gdef\csname R@an.design_space.rho.kits_fresh_acdc\endcsname{+0.09}
\expandafter\gdef\csname R@an.design_space.rho.kits_fresh_acdc.arms\endcsname{ResEnc-M, ResEnc-matched, ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context, fn.-identical control, LeanAdd-NeXt, LeanDeepMid+FD, LeanDeepMid, LeanNeXt-s5, HyReX-k9}
\expandafter\gdef\csname R@an.design_space.rho.kits_fresh_acdc.basis\endcsname{KiTS23 fresh mean (seeds 1--2) against ACDC discovery seed 0}
\expandafter\gdef\csname R@an.design_space.rho.kits_fresh_acdc.clause\endcsname{$\rho=+0.09$ ($n=12$ arms; $|\rho|\ge 0.59$ is the smallest agreement that $n=12$ arms resolve)}
\expandafter\gdef\csname R@an.design_space.rho.kits_fresh_acdc.dp3\endcsname{+0.091}
\expandafter\gdef\csname R@an.design_space.rho.kits_fresh_acdc.floor.clause\endcsname{$|\rho|\ge 0.59$ is the smallest agreement that $n=12$ arms resolve}
\expandafter\gdef\csname R@an.design_space.rho.kits_fresh_acdc.mdes\endcsname{0.59}
\expandafter\gdef\csname R@an.design_space.rho.kits_fresh_acdc.mdes.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.kits_fresh_acdc.n\endcsname{12}
\expandafter\gdef\csname R@an.design_space.rho.kits_fresh_acdc.order\endcsname{with $\rho=+0.09$}
\expandafter\gdef\csname R@an.design_space.rho.kits_fresh_acdc.s0\endcsname{+0.48}
\expandafter\gdef\csname R@an.design_space.rho.kits_fresh_acdc.s0.clause\endcsname{against $\rho=+0.48$ for the same arms at the KiTS23 discovery seed}
\expandafter\gdef\csname R@an.design_space.rho.kits_fresh_acdc.state\endcsname{not resolved}
\expandafter\gdef\csname R@an.design_space.rho.kits_fresh_acdc.verdict\endcsname{agreement below the resolution floor}
\expandafter\gdef\csname R@an.design_space.rho.kits_s0_fresh\endcsname{+0.43}
\expandafter\gdef\csname R@an.design_space.rho.kits_s0_fresh.atcrit\endcsname{n/a}
\expandafter\gdef\csname R@an.design_space.rho.kits_s0_fresh.clause\endcsname{$\rho=+0.43$ ($n=25$; Monte-Carlo permutation $p=0.033$; $p\le 0.05$ needs $|\rho|\ge 0.40$ at $n=25$)}
\expandafter\gdef\csname R@an.design_space.rho.kits_s0_fresh.edge.sentence\endcsname{{}}
\expandafter\gdef\csname R@an.design_space.rho.kits_s0_fresh.floor.clause\endcsname{$p\le 0.05$ needs $|\rho|\ge 0.40$ at $n=25$}
\expandafter\gdef\csname R@an.design_space.rho.kits_s0_fresh.mdes\endcsname{0.40}
\expandafter\gdef\csname R@an.design_space.rho.kits_s0_fresh.mdes.basis\endcsname{simulated}
\expandafter\gdef\csname R@an.design_space.rho.kits_s0_fresh.mdes.p\endcsname{0.050}
\expandafter\gdef\csname R@an.design_space.rho.kits_s0_fresh.n\endcsname{25}
\expandafter\gdef\csname R@an.design_space.rho.kits_s0_fresh.next.p\endcsname{n/a}
\expandafter\gdef\csname R@an.design_space.rho.kits_s0_fresh.order\endcsname{with detectable agreement}
\expandafter\gdef\csname R@an.design_space.rho.kits_s0_fresh.p\endcsname{0.033}
\expandafter\gdef\csname R@an.design_space.rho.kits_s0_fresh.p.basis\endcsname{Monte-Carlo}
\expandafter\gdef\csname R@an.design_space.rho.kits_s0_fresh.p.eq\endcsname{$p=0.033$}
\expandafter\gdef\csname R@an.design_space.rho.kits_s0_fresh.p.exact\endcsname{n/a}
\expandafter\gdef\csname R@an.design_space.rho.kits_s0_fresh.p.print\endcsname{0.033}
\expandafter\gdef\csname R@an.design_space.rho.kits_s0_fresh.p.print.eq\endcsname{$p=0.033$}
\expandafter\gdef\csname R@an.design_space.rho.kits_s0_fresh.verdict\endcsname{detectable agreement}
\expandafter\gdef\csname R@an.design_space.rho.kits_s0_fresh.verdict.assoc\endcsname{a detectable positive association}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n10\endcsname{0.65}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n10.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n10.p\endcsname{0.049}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n11\endcsname{0.62}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n11.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n11.p\endcsname{0.048}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n12\endcsname{0.59}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n12.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n12.p\endcsname{0.049}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n13\endcsname{0.56}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n13.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n13.p\endcsname{0.050}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n14\endcsname{0.54}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n14.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n14.p\endcsname{0.050}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n15\endcsname{0.52}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n15.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n15.p\endcsname{0.049}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n16\endcsname{0.50}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n16.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n16.p\endcsname{0.049}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n17\endcsname{0.49}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n17.basis\endcsname{simulated}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n17.p\endcsname{0.049}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n18\endcsname{0.47}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n18.basis\endcsname{simulated}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n18.p\endcsname{0.050}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n19\endcsname{0.46}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n19.basis\endcsname{simulated}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n19.p\endcsname{0.049}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n20\endcsname{0.45}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n20.basis\endcsname{simulated}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n20.p\endcsname{0.050}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n21\endcsname{0.44}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n21.basis\endcsname{simulated}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n21.p\endcsname{0.050}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n22\endcsname{0.43}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n22.basis\endcsname{simulated}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n22.p\endcsname{0.050}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n23\endcsname{0.42}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n23.basis\endcsname{simulated}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n23.p\endcsname{0.049}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n24\endcsname{0.41}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n24.basis\endcsname{simulated}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n24.p\endcsname{0.050}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n25\endcsname{0.40}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n25.basis\endcsname{simulated}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n25.p\endcsname{0.050}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n26\endcsname{0.39}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n26.basis\endcsname{simulated}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n26.p\endcsname{0.050}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n32\endcsname{0.35}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n32.basis\endcsname{simulated}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n32.p\endcsname{0.050}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n38\endcsname{0.32}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n38.basis\endcsname{simulated}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n38.p\endcsname{0.050}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n5\endcsname{1.00}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n5.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n5.p\endcsname{0.017}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n6\endcsname{0.89}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n6.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n6.p\endcsname{0.033}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n7\endcsname{0.79}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n7.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n7.p\endcsname{0.048}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n8\endcsname{0.74}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n8.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n8.p\endcsname{0.046}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n9\endcsname{0.70}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n9.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.mdes.n9.p\endcsname{0.043}
\expandafter\gdef\csname R@an.design_space.rho.params.amos\endcsname{+0.45}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.atcrit\endcsname{n/a}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.clause\endcsname{$\rho=+0.45$ ($n=38$; Monte-Carlo permutation $p=0.0048$; $p\le 0.05$ needs $|\rho|\ge 0.32$ at $n=38$)}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.edge.sentence\endcsname{{}}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.floor.clause\endcsname{$p\le 0.05$ needs $|\rho|\ge 0.32$ at $n=38$}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.max\endcsname{102.8}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.max.arm\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.mdes\endcsname{0.32}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.mdes.basis\endcsname{simulated}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.mdes.p\endcsname{0.050}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.min\endcsname{18.2}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.min.arm\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.n\endcsname{38}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.next.p\endcsname{n/a}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.order\endcsname{with detectable agreement}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.p\endcsname{0.0048}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.p.basis\endcsname{Monte-Carlo}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.p.eq\endcsname{$p=0.0048$}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.p.exact\endcsname{n/a}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.p.print\endcsname{0.0048}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.p.print.eq\endcsname{$p=0.0048$}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.range.clause\endcsname{from 18.2 M (LeanTrunk) to 102.8 M (ResEnc+context) across the 38 AMOS22 arms screened}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.verdict\endcsname{detectable agreement}
\expandafter\gdef\csname R@an.design_space.rho.params.amos.verdict.assoc\endcsname{a detectable positive association}
\expandafter\gdef\csname R@an.design_space.rho.params.kits\endcsname{+0.01}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.atcrit\endcsname{n/a}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.clause\endcsname{$\rho=+0.01$ ($n=32$; Monte-Carlo permutation $p=0.97$; $p\le 0.05$ needs $|\rho|\ge 0.35$ at $n=32$)}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.edge.sentence\endcsname{{}}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.floor.clause\endcsname{$p\le 0.05$ needs $|\rho|\ge 0.35$ at $n=32$}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.max\endcsname{102.8}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.max.arm\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.mdes\endcsname{0.35}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.mdes.basis\endcsname{simulated}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.mdes.p\endcsname{0.050}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.min\endcsname{18.2}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.min.arm\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.n\endcsname{32}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.next.p\endcsname{n/a}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.order\endcsname{with no detectable agreement}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.p\endcsname{0.97}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.p.basis\endcsname{Monte-Carlo}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.p.eq\endcsname{$p=0.97$}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.p.exact\endcsname{n/a}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.p.print\endcsname{0.97}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.p.print.eq\endcsname{$p=0.97$}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.range.clause\endcsname{from 18.2 M (LeanTrunk) to 102.8 M (ResEnc+context) across the 32 KiTS23 arms screened}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.verdict\endcsname{no detectable agreement}
\expandafter\gdef\csname R@an.design_space.rho.params.kits.verdict.assoc\endcsname{no detectable association}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_acdc\endcsname{+0.09}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_acdc.atcrit\endcsname{no}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_acdc.clause\endcsname{$\rho=+0.09$ ($n=6$; exact permutation $p=0.919$; $p\le 0.05$ needs $|\rho|\ge 0.89$ at $n=6$)}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_acdc.edge.sentence\endcsname{{}}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_acdc.floor.clause\endcsname{$p\le 0.05$ needs $|\rho|\ge 0.89$ at $n=6$}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_acdc.mdes\endcsname{0.89}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_acdc.mdes.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_acdc.mdes.p\endcsname{0.033}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_acdc.n\endcsname{6}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_acdc.next.p\endcsname{1.000}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_acdc.order\endcsname{with no detectable agreement}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_acdc.p\endcsname{0.919}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_acdc.p.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_acdc.p.eq\endcsname{$p=0.919$}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_acdc.p.exact\endcsname{0.91944}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_acdc.p.print\endcsname{0.919}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_acdc.p.print.eq\endcsname{$p=0.919$}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_acdc.verdict\endcsname{no detectable agreement}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_acdc.verdict.assoc\endcsname{no detectable association}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_kits\endcsname{+0.09}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_kits.atcrit\endcsname{no}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_kits.clause\endcsname{$\rho=+0.09$ ($n=6$; exact permutation $p=0.919$; $p\le 0.05$ needs $|\rho|\ge 0.89$ at $n=6$)}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_kits.edge.sentence\endcsname{{}}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_kits.floor.clause\endcsname{$p\le 0.05$ needs $|\rho|\ge 0.89$ at $n=6$}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_kits.mdes\endcsname{0.89}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_kits.mdes.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_kits.mdes.p\endcsname{0.033}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_kits.n\endcsname{6}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_kits.next.p\endcsname{1.000}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_kits.order\endcsname{with no detectable agreement}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_kits.p\endcsname{0.919}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_kits.p.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_kits.p.eq\endcsname{$p=0.919$}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_kits.p.exact\endcsname{0.91944}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_kits.p.print\endcsname{0.919}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_kits.p.print.eq\endcsname{$p=0.919$}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_kits.verdict\endcsname{no detectable agreement}
\expandafter\gdef\csname R@an.design_space.rho.tri.amos_kits.verdict.assoc\endcsname{no detectable association}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_acdc\endcsname{+1.00}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_acdc.atcrit\endcsname{no}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_acdc.clause\endcsname{$\rho=+1.00$ ($n=6$; exact permutation $p=0.003$; $p\le 0.05$ needs $|\rho|\ge 0.89$ at $n=6$)}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_acdc.edge.sentence\endcsname{{}}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_acdc.floor.clause\endcsname{$p\le 0.05$ needs $|\rho|\ge 0.89$ at $n=6$}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_acdc.mdes\endcsname{0.89}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_acdc.mdes.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_acdc.mdes.p\endcsname{0.033}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_acdc.n\endcsname{6}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_acdc.next.p\endcsname{0.017}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_acdc.order\endcsname{in exactly the same order}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_acdc.p\endcsname{0.003}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_acdc.p.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_acdc.p.eq\endcsname{$p=0.003$}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_acdc.p.exact\endcsname{0.00278}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_acdc.p.print\endcsname{0.003}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_acdc.p.print.eq\endcsname{$p=0.003$}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_acdc.verdict\endcsname{detectable agreement}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_acdc.verdict.assoc\endcsname{a detectable positive association}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_fresh_acdc\endcsname{+0.09}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_fresh_acdc.arms\endcsname{ResEnc-M, ResEnc-matched, ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_fresh_acdc.basis\endcsname{KiTS23 fresh mean (seeds 1--2) against ACDC discovery seed 0}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_fresh_acdc.clause\endcsname{$\rho=+0.09$ ($n=6$ arms; $|\rho|\ge 0.89$ is the smallest agreement that $n=6$ arms resolve)}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_fresh_acdc.dp3\endcsname{+0.086}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_fresh_acdc.floor.clause\endcsname{$|\rho|\ge 0.89$ is the smallest agreement that $n=6$ arms resolve}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_fresh_acdc.mdes\endcsname{0.89}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_fresh_acdc.mdes.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_fresh_acdc.n\endcsname{6}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_fresh_acdc.order\endcsname{with $\rho=+0.09$}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_fresh_acdc.s0\endcsname{+1.00}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_fresh_acdc.s0.clause\endcsname{against $\rho=+1.00$ for the same arms at the KiTS23 discovery seed}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_fresh_acdc.state\endcsname{not resolved}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_fresh_acdc.verdict\endcsname{agreement below the resolution floor}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_s0_fresh\endcsname{+0.09}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_s0_fresh.arms\endcsname{ResEnc-M, ResEnc-matched, ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_s0_fresh.basis\endcsname{KiTS23 discovery seed 0 against KiTS23 fresh mean (seeds 1--2)}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_s0_fresh.clause\endcsname{$\rho=+0.09$ ($n=6$ arms; $|\rho|\ge 0.89$ is the smallest agreement that $n=6$ arms resolve)}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_s0_fresh.dp3\endcsname{+0.086}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_s0_fresh.floor.clause\endcsname{$|\rho|\ge 0.89$ is the smallest agreement that $n=6$ arms resolve}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_s0_fresh.mdes\endcsname{0.89}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_s0_fresh.mdes.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_s0_fresh.n\endcsname{6}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_s0_fresh.order\endcsname{with $\rho=+0.09$}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_s0_fresh.s0\endcsname{n/a}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_s0_fresh.s0.clause\endcsname{the same arms have no complete KiTS23 discovery-seed order}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_s0_fresh.state\endcsname{not resolved}
\expandafter\gdef\csname R@an.design_space.rho.tri.kits_s0_fresh.verdict\endcsname{agreement below the resolution floor}
\expandafter\gdef\csname R@an.design_space.screen.cut\endcsname{0.05}
\expandafter\gdef\csname R@an.design_space.screen.flip.arm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.design_space.screen.flip.arms\endcsname{none}
\expandafter\gdef\csname R@an.design_space.screen.flip.clause\endcsname{it has not changed a decision: no arm sits in the flip-driven region}
\expandafter\gdef\csname R@an.design_space.screen.flip.max\endcsname{0.155}
\expandafter\gdef\csname R@an.design_space.screen.flip.pct\endcsname{44}
\expandafter\gdef\csname R@an.design_space.screen.move.cut\endcsname{0.10}
\expandafter\gdef\csname R@an.design_space.screen.n\endcsname{38}
\expandafter\gdef\csname R@an.design_space.screen.n_clear\endcsname{11}
\expandafter\gdef\csname R@an.design_space.screen.n_flat\endcsname{17}
\expandafter\gdef\csname R@an.design_space.screen.n_flipregion\endcsname{0}
\expandafter\gdef\csname R@an.design_space.screen.n_moved\endcsname{21}
\expandafter\gdef\csname R@an.design_space.screen.n_unlabelled\endcsname{22}
\expandafter\gdef\csname R@an.design_space.screen.nearest\endcsname{branch control}
\expandafter\gdef\csname R@an.design_space.screen.nearest.pp\endcsname{0.021}
\expandafter\gdef\csname R@an.design_space.screen.nearest.signed\endcsname{+0.021}
\expandafter\gdef\csname R@an.design_space.screen.nearest.verb\endcsname{clears}
\expandafter\gdef\csname R@an.design_space.screen.unlabelled.dropped.arms\endcsname{ResEnc+context, HyReX+dec. capacity, HyReX, finer ConvNeXt, HyReX w/o GRN, HyReX-k3, HyReX-k9, LeanDeepMid}
\expandafter\gdef\csname R@an.design_space.spread.acdc.n\endcsname{6}
\expandafter\gdef\csname R@an.design_space.spread.acdc.p\endcsname{$<$0.001}
\expandafter\gdef\csname R@an.design_space.spread.acdc.p.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.spread.acdc.p.eq\endcsname{$p<0.001$}
\expandafter\gdef\csname R@an.design_space.spread.acdc.p.print\endcsname{$<$0.001}
\expandafter\gdef\csname R@an.design_space.spread.acdc.p.print.eq\endcsname{$p<0.001$}
\expandafter\gdef\csname R@an.design_space.spread.acdc.range\endcsname{+0.63}
\expandafter\gdef\csname R@an.design_space.spread.acdc.sd\endcsname{0.099}
\expandafter\gdef\csname R@an.design_space.spread.acdc.second.arm\endcsname{HyReX+context}
\expandafter\gdef\csname R@an.design_space.spread.acdc.top.arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.design_space.spread.acdc.topmargin\endcsname{0.165}
\expandafter\gdef\csname R@an.design_space.spread.acdc.topmargin.resolved\endcsname{no}
\expandafter\gdef\csname R@an.design_space.spread.amos.n\endcsname{6}
\expandafter\gdef\csname R@an.design_space.spread.amos.p\endcsname{0.004}
\expandafter\gdef\csname R@an.design_space.spread.amos.p.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.spread.amos.p.eq\endcsname{$p=0.004$}
\expandafter\gdef\csname R@an.design_space.spread.amos.p.print\endcsname{0.004}
\expandafter\gdef\csname R@an.design_space.spread.amos.p.print.eq\endcsname{$p=0.004$}
\expandafter\gdef\csname R@an.design_space.spread.amos.range\endcsname{+0.63}
\expandafter\gdef\csname R@an.design_space.spread.amos.sd\endcsname{0.122}
\expandafter\gdef\csname R@an.design_space.spread.amos.second.arm\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.design_space.spread.amos.top.arm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.design_space.spread.amos.topmargin\endcsname{0.217}
\expandafter\gdef\csname R@an.design_space.spread.amos.topmargin.resolved\endcsname{no}
\expandafter\gdef\csname R@an.design_space.spread.amos.verdict\endcsname{rejects}
\expandafter\gdef\csname R@an.design_space.spread.kits.n\endcsname{6}
\expandafter\gdef\csname R@an.design_space.spread.kits.p\endcsname{0.379}
\expandafter\gdef\csname R@an.design_space.spread.kits.p.basis\endcsname{exact}
\expandafter\gdef\csname R@an.design_space.spread.kits.p.eq\endcsname{$p=0.379$}
\expandafter\gdef\csname R@an.design_space.spread.kits.p.print\endcsname{0.379}
\expandafter\gdef\csname R@an.design_space.spread.kits.p.print.eq\endcsname{$p=0.379$}
\expandafter\gdef\csname R@an.design_space.spread.kits.range\endcsname{+2.18}
\expandafter\gdef\csname R@an.design_space.spread.kits.sd\endcsname{0.795}
\expandafter\gdef\csname R@an.design_space.spread.kits.second.arm\endcsname{HyReX+context}
\expandafter\gdef\csname R@an.design_space.spread.kits.top.arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.design_space.spread.kits.topmargin\endcsname{0.316}
\expandafter\gdef\csname R@an.design_space.spread.kits.topmargin.resolved\endcsname{no}
\expandafter\gdef\csname R@an.design_space.spread.n_reject\endcsname{2}
\expandafter\gdef\csname R@an.design_space.spread.n_set\endcsname{6}
\expandafter\gdef\csname R@an.design_space.spread.n_topresolved\endcsname{0}
\expandafter\gdef\csname R@an.design_space.spread.notreject.ds\endcsname{KiTS23}
\expandafter\gdef\csname R@an.design_space.spread.reject.ds\endcsname{AMOS22 and ACDC}
\expandafter\gdef\csname R@an.design_space.spread.set\endcsname{ResEnc-M, ResEnc-matched, ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context}
\expandafter\gdef\csname R@an.design_space.status.acdc.blank\endcsname{30}
\expandafter\gdef\csname R@an.design_space.status.acdc.landed\endcsname{0}
\expandafter\gdef\csname R@an.design_space.status.acdc.met\endcsname{10}
\expandafter\gdef\csname R@an.design_space.status.acdc.notmet\endcsname{2}
\expandafter\gdef\csname R@an.design_space.status.acdc.pending\endcsname{0}
\expandafter\gdef\csname R@an.design_space.status.amos.blank\endcsname{0}
\expandafter\gdef\csname R@an.design_space.status.amos.landed\endcsname{0}
\expandafter\gdef\csname R@an.design_space.status.amos.met\endcsname{11}
\expandafter\gdef\csname R@an.design_space.status.amos.notmet\endcsname{27}
\expandafter\gdef\csname R@an.design_space.status.amos.pending\endcsname{4}
\expandafter\gdef\csname R@an.design_space.status.code.blank\endcsname{0}
\expandafter\gdef\csname R@an.design_space.status.code.landed\endcsname{0}
\expandafter\gdef\csname R@an.design_space.status.code.met\endcsname{10}
\expandafter\gdef\csname R@an.design_space.status.code.notmet\endcsname{14}
\expandafter\gdef\csname R@an.design_space.status.code.pending\endcsname{18}
\expandafter\gdef\csname R@an.design_space.status.kits.blank\endcsname{0}
\expandafter\gdef\csname R@an.design_space.status.kits.landed\endcsname{0}
\expandafter\gdef\csname R@an.design_space.status.kits.met\endcsname{31}
\expandafter\gdef\csname R@an.design_space.status.kits.notmet\endcsname{1}
\expandafter\gdef\csname R@an.design_space.status.kits.pending\endcsname{10}
\expandafter\gdef\csname R@an.design_space.status.rep_amos.blank\endcsname{35}
\expandafter\gdef\csname R@an.design_space.status.rep_amos.landed\endcsname{1}
\expandafter\gdef\csname R@an.design_space.status.rep_amos.met\endcsname{2}
\expandafter\gdef\csname R@an.design_space.status.rep_amos.notmet\endcsname{2}
\expandafter\gdef\csname R@an.design_space.status.rep_amos.pending\endcsname{2}
\expandafter\gdef\csname R@an.design_space.status.rep_kits.blank\endcsname{17}
\expandafter\gdef\csname R@an.design_space.status.rep_kits.landed\endcsname{0}
\expandafter\gdef\csname R@an.design_space.status.rep_kits.met\endcsname{24}
\expandafter\gdef\csname R@an.design_space.status.rep_kits.notmet\endcsname{1}
\expandafter\gdef\csname R@an.design_space.status.rep_kits.pending\endcsname{0}
\expandafter\gdef\csname R@an.design_space.tri.arms\endcsname{ResEnc-M, ResEnc-matched, ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context}
\expandafter\gdef\csname R@an.design_space.tri.extra.arms\endcsname{fn.-identical control, LeanAdd-NeXt, LeanDeepMid+FD, LeanDeepMid, LeanNeXt-s5, HyReX-k9}
\expandafter\gdef\csname R@an.design_space.wave.attribution.src\endcsname{ADDENDUM\_N\_enrichment\_20261005.md N3; Addendum Q1c (KiTS23)}
\expandafter\gdef\csname R@an.design_space.wave.laterregistrations.src\endcsname{ADDENDUM\_AD\_wave5\_screens\_20261008.md; REGISTRY.md; ADDENDUM\_AM\_wave5\_selection\_free\_runs\_20261009.md; ADDENDUM\_AO\_V6A1r\_selection\_free\_and\_acdc\_guards\_20261009.md; ADDENDUM\_AF\_wave6\_V6A1r\_20261008.md; ADDENDUM\_AN\_wave7\_20261009.md; ADDENDUM\_AP\_wave7\_followups\_20261010.md; ADDENDUM\_AT\_inference\_cost\_lean\_candidates\_20261010.md; ADDENDUM\_AU\_designation\_accuracy\_variant\_20261010.md; ADDENDUM\_AU2\_V7A2\_joins\_accuracy\_set\_20261010.md; ADDENDUM\_AW\_owed\_replications\_V7A2\_followups\_20261010.md; ADDENDUM\_AQ\_wave7\_B\_arms\_20261010.md; ADDENDUM\_AR\_wave8\_20261010.md; ADDENDUM\_AS\_headline\_designation\_20261010.md; ADDENDUM\_AZ\_precision\_seeds\_xxnet\_20261011.md; ADDENDUM\_BA\_ablation\_and\_cost\_controls\_20261011.md; ADDENDUM\_AY\_wave8\_readings\_20261010.md}
\expandafter\gdef\csname R@an.design_space.wave.nnunetdefault.src\endcsname{nnUNetPlans.json 3d\_fullres (the frozen plan)}
\expandafter\gdef\csname R@an.design_space.wave.wave1.src\endcsname{WAVE1\_REGISTRATION.md, table rows L1\_resenc--L6\_full}
\expandafter\gdef\csname R@an.design_space.wave.wave2.src\endcsname{WAVE2\_REGISTRATION.md, table rows W1c--W4; Addendum W2-B (W5)}
\expandafter\gdef\csname R@an.design_space.wave.wave3.src\endcsname{WAVE3\_REGISTRATION.md, Addendum W3-A sections 1--2}
\expandafter\gdef\csname R@an.design_space.wave.wave4.src\endcsname{ADDENDUM\_O\_wave4\_20261005.md, table O3}
\expandafter\gdef\csname R@an.design_space.withheld.all_three_datasets.sentence\endcsname{WITHHELD CLAIM all\_three\_datasets}
\expandafter\gdef\csname R@an.design_space.withheld.all_three_datasets.status\endcsname{not true}
\expandafter\gdef\csname R@an.design_space.withheld.amos_cannot_resolve.sentence\endcsname{WITHHELD CLAIM amos\_cannot\_resolve}
\expandafter\gdef\csname R@an.design_space.withheld.amos_cannot_resolve.status\endcsname{not true}
\expandafter\gdef\csname R@an.design_space.withheld.amos_gain_per_parameter.sentence\endcsname{WITHHELD CLAIM amos\_gain\_per\_parameter}
\expandafter\gdef\csname R@an.design_space.withheld.amos_gain_per_parameter.status\endcsname{not true}
\expandafter\gdef\csname R@an.design_space.withheld.n\endcsname{5}
\expandafter\gdef\csname R@an.design_space.withheld.n_not_true\endcsname{5}
\expandafter\gdef\csname R@an.design_space.withheld.only_survivor.sentence\endcsname{WITHHELD CLAIM only\_survivor}
\expandafter\gdef\csname R@an.design_space.withheld.only_survivor.status\endcsname{not true}
\expandafter\gdef\csname R@an.design_space.withheld.operator_causal.condition\endcsname{not met}
\expandafter\gdef\csname R@an.design_space.withheld.operator_causal.sentence\endcsname{WITHHELD CLAIM operator\_causal}
\expandafter\gdef\csname R@an.design_space.withheld.operator_causal.status\endcsname{not true}
\expandafter\gdef\csname R@an.designation.xa.cand.L3.cancelled.n\endcsname{0}
\expandafter\gdef\csname R@an.designation.xa.cand.L3.cancelled.what\endcsname{none}
\expandafter\gdef\csname R@an.designation.xa.cand.L3.outcome\endcsname{clears}
\expandafter\gdef\csname R@an.designation.xa.cand.L3.params\endcsname{29.37}
\expandafter\gdef\csname R@an.designation.xa.cand.L3.status\endcsname{member}
\expandafter\gdef\csname R@an.designation.xa.cand.L3.step\endcsname{1.52}
\expandafter\gdef\csname R@an.designation.xa.cand.V7A1.cancelled.n\endcsname{0}
\expandafter\gdef\csname R@an.designation.xa.cand.V7A1.cancelled.what\endcsname{none}
\expandafter\gdef\csname R@an.designation.xa.cand.V7A1.outcome\endcsname{clears}
\expandafter\gdef\csname R@an.designation.xa.cand.V7A1.params\endcsname{30.77}
\expandafter\gdef\csname R@an.designation.xa.cand.V7A1.status\endcsname{member}
\expandafter\gdef\csname R@an.designation.xa.cand.V7A1.step\endcsname{1.00}
\expandafter\gdef\csname R@an.designation.xa.cand.V7A2.cancelled.n\endcsname{8}
\expandafter\gdef\csname R@an.designation.xa.cand.V7A2.cancelled.what\endcsname{its AMOS22 and ACDC cross-validation was not run to completion}
\expandafter\gdef\csname R@an.designation.xa.cand.V7A2.outcome\endcsname{not completed}
\expandafter\gdef\csname R@an.designation.xa.cand.V7A2.params\endcsname{30.89}
\expandafter\gdef\csname R@an.designation.xa.cand.V7A2.status\endcsname{not completed}
\expandafter\gdef\csname R@an.designation.xa.cand.V7A2.step\endcsname{1.16}
\expandafter\gdef\csname R@an.designation.xa.cand.V8A1.cancelled.n\endcsname{0}
\expandafter\gdef\csname R@an.designation.xa.cand.V8A1.cancelled.what\endcsname{none}
\expandafter\gdef\csname R@an.designation.xa.cand.V8A1.outcome\endcsname{withdrawn}
\expandafter\gdef\csname R@an.designation.xa.cand.V8A1.params\endcsname{31.04}
\expandafter\gdef\csname R@an.designation.xa.cand.V8A1.status\endcsname{withdrawn}
\expandafter\gdef\csname R@an.designation.xa.cand.V8A1.step\endcsname{0.93}
\expandafter\gdef\csname R@an.designation.xa.cand.V8A2.cancelled.n\endcsname{0}
\expandafter\gdef\csname R@an.designation.xa.cand.V8A2.cancelled.what\endcsname{none}
\expandafter\gdef\csname R@an.designation.xa.cand.V8A2.outcome\endcsname{withdrawn}
\expandafter\gdef\csname R@an.designation.xa.cand.V8A2.params\endcsname{31.20}
\expandafter\gdef\csname R@an.designation.xa.cand.V8A2.status\endcsname{withdrawn}
\expandafter\gdef\csname R@an.designation.xa.cand.V8A2.step\endcsname{0.88}
\expandafter\gdef\csname R@an.designation.xa.clause\endcsname{{\ifdefined\archA\archA\else XX-Net-A\fi} (LeanDeepMid) clears all three gates (A-G1 \ensuremath{+2.66}\,pp, A-G2 \ensuremath{+0.26}\,pp, A-G3 \ensuremath{+0.08}\,pp); HyReX also clears them at a step ratio of 1.52 against 1.00; LeanDeepMid+FD was not completed (its AMOS22 and ACDC cross-validation was not run to completion); CoarseStack and StackDec were withdrawn}
\expandafter\gdef\csname R@an.designation.xa.complete.n\endcsname{2}
\expandafter\gdef\csname R@an.designation.xa.gates.L3.g1.line\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.designation.xa.gates.L3.g1.state\endcsname{pass}
\expandafter\gdef\csname R@an.designation.xa.gates.L3.g1.value\endcsname{\ensuremath{+2.09}}
\expandafter\gdef\csname R@an.designation.xa.gates.L3.g2.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.designation.xa.gates.L3.g2.line\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.designation.xa.gates.L3.g2.lo\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.designation.xa.gates.L3.g2.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.designation.xa.gates.L3.g2.state\endcsname{pass}
\expandafter\gdef\csname R@an.designation.xa.gates.L3.g2.value\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.designation.xa.gates.L3.g3.hi\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.designation.xa.gates.L3.g3.line\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.designation.xa.gates.L3.g3.lo\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.designation.xa.gates.L3.g3.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.designation.xa.gates.L3.g3.state\endcsname{pass}
\expandafter\gdef\csname R@an.designation.xa.gates.L3.g3.value\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A1.g1.line\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A1.g1.state\endcsname{pass}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A1.g1.value\endcsname{\ensuremath{+2.66}}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A1.g2.hi\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A1.g2.line\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A1.g2.lo\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A1.g2.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A1.g2.state\endcsname{pass}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A1.g2.value\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A1.g3.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A1.g3.line\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A1.g3.lo\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A1.g3.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A1.g3.state\endcsname{pass}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A1.g3.value\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A2.g1.line\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A2.g1.state\endcsname{pass}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A2.g1.value\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A2.g2.line\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A2.g2.state\endcsname{pending}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A2.g2.value\endcsname{\pend}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A2.g3.line\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A2.g3.state\endcsname{pending}
\expandafter\gdef\csname R@an.designation.xa.gates.V7A2.g3.value\endcsname{\pend}
\expandafter\gdef\csname R@an.designation.xa.members\endcsname{HyReX, LeanDeepMid, LeanDeepMid+FD}
\expandafter\gdef\csname R@an.designation.xa.missing\endcsname{none}
\expandafter\gdef\csname R@an.designation.xa.name\endcsname{LeanDeepMid}
\expandafter\gdef\csname R@an.designation.xa.nmissing\endcsname{0}
\expandafter\gdef\csname R@an.designation.xa.notcompleted\endcsname{LeanDeepMid+FD}
\expandafter\gdef\csname R@an.designation.xa.notcompleted.n\endcsname{1}
\expandafter\gdef\csname R@an.designation.xa.out\endcsname{CoarseStack (withdrawn, Addendum AY), StackDec (withdrawn, Addendum AY)}
\expandafter\gdef\csname R@an.designation.xa.rule.g1.line\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.designation.xa.rule.g2.line\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.designation.xa.rule.g3.line\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.designation.xa.rule.tie\endcsname{0.02}
\expandafter\gdef\csname R@an.designation.xa.state\endcsname{designated}
\expandafter\gdef\csname R@an.designation.xa.tag\endcsname{V7A1}
\expandafter\gdef\csname R@an.designation.xl.cand.V7C1.cancelled.n\endcsname{0}
\expandafter\gdef\csname R@an.designation.xl.cand.V7C1.cancelled.what\endcsname{none}
\expandafter\gdef\csname R@an.designation.xl.cand.V7C1.outcome\endcsname{clears}
\expandafter\gdef\csname R@an.designation.xl.cand.V7C1.params\endcsname{20.84}
\expandafter\gdef\csname R@an.designation.xl.cand.V7C1.status\endcsname{member}
\expandafter\gdef\csname R@an.designation.xl.cand.V7C1.step\endcsname{0.78}
\expandafter\gdef\csname R@an.designation.xl.cand.V8B1.cancelled.n\endcsname{0}
\expandafter\gdef\csname R@an.designation.xl.cand.V8B1.cancelled.what\endcsname{none}
\expandafter\gdef\csname R@an.designation.xl.cand.V8B1.outcome\endcsname{withdrawn}
\expandafter\gdef\csname R@an.designation.xl.cand.V8B1.params\endcsname{17.95}
\expandafter\gdef\csname R@an.designation.xl.cand.V8B1.status\endcsname{withdrawn}
\expandafter\gdef\csname R@an.designation.xl.cand.V8B1.step\endcsname{0.61}
\expandafter\gdef\csname R@an.designation.xl.cand.V8B2.cancelled.n\endcsname{4}
\expandafter\gdef\csname R@an.designation.xl.cand.V8B2.cancelled.what\endcsname{its AMOS22 cross-validation was not run to completion}
\expandafter\gdef\csname R@an.designation.xl.cand.V8B2.outcome\endcsname{not completed}
\expandafter\gdef\csname R@an.designation.xl.cand.V8B2.params\endcsname{20.82}
\expandafter\gdef\csname R@an.designation.xl.cand.V8B2.status\endcsname{not completed}
\expandafter\gdef\csname R@an.designation.xl.cand.V8B2.step\endcsname{0.66}
\expandafter\gdef\csname R@an.designation.xl.clause\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi} (LeanNeXt-s5) clears both gates (G1 \ensuremath{+2.44}\,pp, G2 \ensuremath{-0.46}\,pp) and is the only member with a complete selection-free set; Stem1 was not completed (its AMOS22 cross-validation was not run to completion); LeanTrunk was withdrawn}
\expandafter\gdef\csname R@an.designation.xl.complete.n\endcsname{1}
\expandafter\gdef\csname R@an.designation.xl.gates.V7C1.g1.line\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.designation.xl.gates.V7C1.g1.state\endcsname{pass}
\expandafter\gdef\csname R@an.designation.xl.gates.V7C1.g1.value\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@an.designation.xl.gates.V7C1.g2.hi\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.designation.xl.gates.V7C1.g2.line\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.designation.xl.gates.V7C1.g2.lo\endcsname{\ensuremath{-0.81}}
\expandafter\gdef\csname R@an.designation.xl.gates.V7C1.g2.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.designation.xl.gates.V7C1.g2.state\endcsname{pass}
\expandafter\gdef\csname R@an.designation.xl.gates.V7C1.g2.value\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.designation.xl.gates.V8B2.g1.line\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.designation.xl.gates.V8B2.g1.state\endcsname{pass}
\expandafter\gdef\csname R@an.designation.xl.gates.V8B2.g1.value\endcsname{\ensuremath{+1.73}}
\expandafter\gdef\csname R@an.designation.xl.gates.V8B2.g2.line\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.designation.xl.gates.V8B2.g2.state\endcsname{pending}
\expandafter\gdef\csname R@an.designation.xl.gates.V8B2.g2.value\endcsname{\pend}
\expandafter\gdef\csname R@an.designation.xl.members\endcsname{LeanNeXt-s5, Stem1}
\expandafter\gdef\csname R@an.designation.xl.missing\endcsname{none}
\expandafter\gdef\csname R@an.designation.xl.name\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.designation.xl.nmissing\endcsname{0}
\expandafter\gdef\csname R@an.designation.xl.notcompleted\endcsname{Stem1}
\expandafter\gdef\csname R@an.designation.xl.notcompleted.n\endcsname{1}
\expandafter\gdef\csname R@an.designation.xl.out\endcsname{LeanTrunk (withdrawn, Addendum AY)}
\expandafter\gdef\csname R@an.designation.xl.rule.g1.line\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.designation.xl.rule.g2.line\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.designation.xl.rule.tie\endcsname{0.02}
\expandafter\gdef\csname R@an.designation.xl.state\endcsname{designated}
\expandafter\gdef\csname R@an.designation.xl.tag\endcsname{V7C1}
\expandafter\gdef\csname R@an.error_anatomy.amos_a_sd_base\endcsname{0.107}
\expandafter\gdef\csname R@an.error_anatomy.amos_ai_arms\endcsname{L2, L3, L4, L6, W1, W2, W3}
\expandafter\gdef\csname R@an.error_anatomy.amos_ai_n\endcsname{7}
\expandafter\gdef\csname R@an.error_anatomy.amos_altref_contemporaneous_n\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_altref_contemporaneous_shift\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.error_anatomy.amos_altref_contemporaneous_short\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.error_anatomy.amos_altref_finished\endcsname{contemporaneous default runs, uncompiled sub-pool}
\expandafter\gdef\csname R@an.error_anatomy.amos_altref_n_finished\endcsname{2}
\expandafter\gdef\csname R@an.error_anatomy.amos_altref_n_pending\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_altref_pending\endcsname{none}
\expandafter\gdef\csname R@an.error_anatomy.amos_altref_uncompiled_n\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_altref_uncompiled_shift\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.error_anatomy.amos_altref_uncompiled_short\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.error_anatomy.amos_class15_absmax_arms\endcsname{0.088}
\expandafter\gdef\csname R@an.error_anatomy.amos_class15_absmax_arms_class\endcsname{left adrenal gland}
\expandafter\gdef\csname R@an.error_anatomy.amos_class15_absmax_arms_pct\endcsname{6.3}
\expandafter\gdef\csname R@an.error_anatomy.amos_class15_absmax_base\endcsname{0.082}
\expandafter\gdef\csname R@an.error_anatomy.amos_class15_absmax_base_class\endcsname{left adrenal gland}
\expandafter\gdef\csname R@an.error_anatomy.amos_class15_absmax_base_pct\endcsname{5.9}
\expandafter\gdef\csname R@an.error_anatomy.amos_dice_delta_L1\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.error_anatomy.amos_dice_delta_L1_contemporaneous\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.error_anatomy.amos_dice_delta_L1_uncompiled\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.error_anatomy.amos_dice_delta_L3\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.error_anatomy.amos_dice_delta_L3_contemporaneous\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.error_anatomy.amos_dice_delta_L3_uncompiled\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.error_anatomy.amos_duodenum_medlog2_L1\endcsname{\ensuremath{-0.018}}
\expandafter\gdef\csname R@an.error_anatomy.amos_duodenum_medlog2_L3\endcsname{\ensuremath{+0.006}}
\expandafter\gdef\csname R@an.error_anatomy.amos_duodenum_medlog2_base\endcsname{\ensuremath{-0.012}}
\expandafter\gdef\csname R@an.error_anatomy.amos_empty_pairs\endcsname{6}
\expandafter\gdef\csname R@an.error_anatomy.amos_esophagus_medlog2_L1\endcsname{\ensuremath{-0.004}}
\expandafter\gdef\csname R@an.error_anatomy.amos_esophagus_medlog2_L3\endcsname{\ensuremath{-0.014}}
\expandafter\gdef\csname R@an.error_anatomy.amos_esophagus_medlog2_base\endcsname{\ensuremath{-0.020}}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_nruns\endcsname{29}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_L1\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_L1_seeds\endcsname{4, 4, 6}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_L1b\endcsname{6}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_L1b_seeds\endcsname{6, 6, 6}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_L2\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_L2_seeds\endcsname{5, 5, 6}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_L3\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_L3_seeds\endcsname{5, 5, 6}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_L3vL1\endcsname{\ensuremath{+1}}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_L4\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_L4_seeds\endcsname{4, 5, 4}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_L6\endcsname{6}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_W1\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_W1c\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_W2\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_W3\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_W3c\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_W4\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_W5\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_ai_max\endcsname{6}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_ai_mean\endcsname{4.9}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_ai_min\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_all_mean\endcsname{4.8}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_all_n\endcsname{13}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_base\endcsname{5.0}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_base_max\endcsname{6}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_base_min\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_pairs_base_runs\endcsname{5, 6, 5, 5, 4, 5}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_rest_L1\endcsname{2\,143}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_rest_L3\endcsname{7\,669}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_rest_ai_above\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_rest_ai_below\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_rest_ai_within\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_rest_arms_above\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_rest_arms_below\endcsname{7}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_rest_arms_n\endcsname{13}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_rest_arms_within\endcsname{6}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_rest_base_max\endcsname{22\,507}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_rest_base_median\endcsname{11\,471}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_rest_base_min\endcsname{5\,789}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_toppair_case\endcsname{amos\_0115}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_toppair_organ\endcsname{spleen}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_toppair_share_L3\endcsname{85}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_toppair_share_base\endcsname{67}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_Head\endcsname{A stray-voxel total is not a design signature}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_L1\endcsname{6\,526}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_L1b\endcsname{27\,705}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_L2\endcsname{13\,862}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_L3\endcsname{51\,517}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_L3vL1\endcsname{\ensuremath{+44\,991}}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_L4\endcsname{13\,939}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_L6\endcsname{24\,451}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_W1\endcsname{23\,431}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_W1c\endcsname{13\,028}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_W2\endcsname{13\,005}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_W3\endcsname{17\,222}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_W3c\endcsname{72\,544}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_W4\endcsname{51\,107}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_W5\endcsname{4\,687}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_ai_above\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_ai_below\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_ai_max\endcsname{51\,517}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_ai_median\endcsname{17\,222}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_ai_min\endcsname{13\,005}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_ai_within\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_arms_above\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_arms_above_arms\endcsname{none}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_arms_below\endcsname{7}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_arms_max\endcsname{72\,544}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_arms_n\endcsname{13}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_arms_within\endcsname{6}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_base\endcsname{46\,076}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_base_fold\endcsname{4.2}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_base_max\endcsname{74\,863}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_base_median\endcsname{46\,954}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_base_min\endcsname{17\,918}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_base_sd\endcsname{24\,719}
\expandafter\gdef\csname R@an.error_anatomy.amos_fp_vox_head\endcsname{a stray-voxel total is not a design signature}
\expandafter\gdef\csname R@an.error_anatomy.amos_gall_bladder_medlog2_L1\endcsname{\ensuremath{-0.006}}
\expandafter\gdef\csname R@an.error_anatomy.amos_gall_bladder_medlog2_L3\endcsname{\ensuremath{-0.006}}
\expandafter\gdef\csname R@an.error_anatomy.amos_gall_bladder_medlog2_base\endcsname{\ensuremath{-0.004}}
\expandafter\gdef\csname R@an.error_anatomy.amos_left_adrenal_gland_medlog2_L1\endcsname{\ensuremath{-0.027}}
\expandafter\gdef\csname R@an.error_anatomy.amos_left_adrenal_gland_medlog2_L3\endcsname{\ensuremath{-0.088}}
\expandafter\gdef\csname R@an.error_anatomy.amos_left_adrenal_gland_medlog2_base\endcsname{\ensuremath{-0.023}}
\expandafter\gdef\csname R@an.error_anatomy.amos_nbase\endcsname{6}
\expandafter\gdef\csname R@an.error_anatomy.amos_ncases\endcsname{40}
\expandafter\gdef\csname R@an.error_anatomy.amos_outside_null\endcsname{29}
\expandafter\gdef\csname R@an.error_anatomy.amos_pairs_always\endcsname{2}
\expandafter\gdef\csname R@an.error_anatomy.amos_pairs_never\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_pairs_total\endcsname{600}
\expandafter\gdef\csname R@an.error_anatomy.amos_pairs_variable\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_absmax_arms\endcsname{0.088}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_absmax_arms_class\endcsname{left adrenal gland}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_absmax_arms_pct\endcsname{6.3}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_absmax_base\endcsname{0.082}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_absmax_base_class\endcsname{left adrenal gland}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_absmax_base_pct\endcsname{5.9}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_L1\endcsname{\ensuremath{-0.002}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_L1_hi\endcsname{\ensuremath{+0.010}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_L1_lo\endcsname{\ensuremath{-0.016}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_L1b\endcsname{\ensuremath{-0.006}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_L1b_hi\endcsname{\ensuremath{+0.014}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_L1b_lo\endcsname{\ensuremath{-0.023}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_L2\endcsname{\ensuremath{-0.005}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_L2_hi\endcsname{\ensuremath{+0.014}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_L2_lo\endcsname{\ensuremath{-0.014}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_L3\endcsname{\ensuremath{+0.004}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_L3_hi\endcsname{\ensuremath{+0.017}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_L3_lo\endcsname{\ensuremath{-0.013}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_L4\endcsname{\ensuremath{-0.011}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_L4_hi\endcsname{\ensuremath{+0.006}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_L4_lo\endcsname{\ensuremath{-0.029}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_L6\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_L6_hi\endcsname{\ensuremath{+0.028}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_L6_lo\endcsname{\ensuremath{+0.001}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W1\endcsname{\ensuremath{-0.004}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W1_hi\endcsname{\ensuremath{+0.009}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W1_lo\endcsname{\ensuremath{-0.026}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W1c\endcsname{\ensuremath{+0.006}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W1c_hi\endcsname{\ensuremath{+0.027}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W1c_lo\endcsname{\ensuremath{-0.012}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W2\endcsname{\ensuremath{-0.020}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W2_hi\endcsname{\ensuremath{-0.002}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W2_lo\endcsname{\ensuremath{-0.034}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W3\endcsname{\ensuremath{-0.004}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W3_hi\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W3_lo\endcsname{\ensuremath{-0.020}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W3c\endcsname{\ensuremath{+0.014}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W3c_hi\endcsname{\ensuremath{+0.028}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W3c_lo\endcsname{\ensuremath{-0.005}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W4\endcsname{\ensuremath{+0.017}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W4_hi\endcsname{\ensuremath{+0.035}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W4_lo\endcsname{\ensuremath{+0.004}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W5\endcsname{\ensuremath{-0.007}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W5_hi\endcsname{\ensuremath{+0.010}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_dmedlog2_W5_lo\endcsname{\ensuremath{-0.016}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_fn_L1\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_fn_L1b\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_fn_L2\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_fn_L3\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_fn_L4\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_fn_L6\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_fn_W1\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_fn_W1c\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_fn_W2\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_fn_W3\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_fn_W3c\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_fn_W4\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_fn_W5\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_fn_ai_total\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_fn_base_max\endcsname{2}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_fn_base_mean\endcsname{0.3}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_fn_base_min\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_fn_base_runs\endcsname{0, 2, 0, 0, 0, 0}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_fn_base_total\endcsname{2}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L1\endcsname{\ensuremath{-0.013}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L1_fresh\endcsname{\ensuremath{-0.017}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L1_hi\endcsname{\ensuremath{+0.001}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L1_lo\endcsname{\ensuremath{-0.035}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L1b\endcsname{\ensuremath{-0.017}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L1b_fresh\endcsname{\ensuremath{-0.008}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L1b_hi\endcsname{\ensuremath{+0.014}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L1b_lo\endcsname{\ensuremath{-0.050}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L2\endcsname{\ensuremath{-0.016}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L2_fresh\endcsname{\ensuremath{-0.003}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L2_hi\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L2_lo\endcsname{\ensuremath{-0.035}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L3\endcsname{\ensuremath{-0.008}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L3_fresh\endcsname{\ensuremath{-0.001}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L3_hi\endcsname{\ensuremath{+0.013}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L3_lo\endcsname{\ensuremath{-0.043}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L3vL1\endcsname{\ensuremath{+0.005}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L3vL1_hi\endcsname{\ensuremath{+0.023}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L3vL1_lo\endcsname{\ensuremath{-0.015}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L4\endcsname{\ensuremath{-0.022}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L4_fresh\endcsname{\ensuremath{-0.008}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L4_hi\endcsname{\ensuremath{-0.002}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L4_lo\endcsname{\ensuremath{-0.057}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L6\endcsname{0.000}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L6_hi\endcsname{\ensuremath{+0.024}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_L6_lo\endcsname{\ensuremath{-0.023}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W1\endcsname{\ensuremath{-0.015}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W1_hi\endcsname{\ensuremath{+0.004}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W1_lo\endcsname{\ensuremath{-0.046}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W1c\endcsname{\ensuremath{-0.005}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W1c_hi\endcsname{\ensuremath{+0.026}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W1c_lo\endcsname{\ensuremath{-0.037}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W2\endcsname{\ensuremath{-0.031}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W2_hi\endcsname{\ensuremath{-0.007}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W2_lo\endcsname{\ensuremath{-0.051}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W3\endcsname{\ensuremath{-0.015}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W3_hi\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W3_lo\endcsname{\ensuremath{-0.042}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W3c\endcsname{\ensuremath{+0.003}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W3c_hi\endcsname{\ensuremath{+0.030}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W3c_lo\endcsname{\ensuremath{-0.033}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W4\endcsname{\ensuremath{+0.006}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W4_hi\endcsname{\ensuremath{+0.035}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W4_lo\endcsname{\ensuremath{-0.022}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W5\endcsname{\ensuremath{-0.018}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W5_hi\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_W5_lo\endcsname{\ensuremath{-0.040}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_base\endcsname{\ensuremath{-0.011}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_base_hi\endcsname{\ensuremath{+0.008}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_base_lo\endcsname{\ensuremath{-0.037}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_base_max\endcsname{\ensuremath{-0.002}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medlog2_base_min\endcsname{\ensuremath{-0.025}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_L1\endcsname{0.991}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_L1_fresh\endcsname{0.988}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_L1b\endcsname{0.988}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_L1b_fresh\endcsname{0.995}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_L2\endcsname{0.989}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_L2_fresh\endcsname{0.998}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_L3\endcsname{0.995}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_L3_fresh\endcsname{0.999}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_L4\endcsname{0.985}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_L4_fresh\endcsname{0.994}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_L6\endcsname{1.000}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_W1\endcsname{0.990}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_W1c\endcsname{0.996}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_W2\endcsname{0.978}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_W3\endcsname{0.990}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_W3c\endcsname{1.002}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_W4\endcsname{1.004}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_W5\endcsname{0.988}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_ai_above\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_ai_below\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_ai_max\endcsname{1.000}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_ai_min\endcsname{0.978}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_ai_within\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_base\endcsname{0.992}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_base_max\endcsname{0.999}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_base_min\endcsname{0.983}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_fresh_ci_over_pool\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_fresh_margin\endcsname{\ensuremath{+0.002}}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_fresh_max\endcsname{0.999}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_fresh_max_arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_fresh_n\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_fresh_pending\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_fresh_runnerup\endcsname{0.998}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_fresh_runnerup_arm\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_main_above\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_main_above_arms\endcsname{HyReX+context}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_main_below\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_main_below_arms\endcsname{none}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_main_n\endcsname{6}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_medratio_main_within\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_names\endcsname{right adrenal gland, left adrenal gland, gall bladder, esophagus, duodenum}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_L1\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_L1b\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_L2\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_L3\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_L4\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_L6\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_W1\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_W1c\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_W2\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_W3\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_W3c\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_W4\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_W5\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_ai_max\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_ai_min\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_base_max\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_base_mean\endcsname{3.5}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_base_min\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_base_runs\endcsname{3, 5, 4, 3, 3, 3}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_nf_base_total\endcsname{21}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_pairs\endcsname{197}
\expandafter\gdef\csname R@an.error_anatomy.amos_panel_pairs_total\endcsname{200}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_L1\endcsname{0.59}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_L1b\endcsname{0.89}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_L2\endcsname{0.75}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_L3\endcsname{0.75}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_L4\endcsname{0.60}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_L6\endcsname{0.89}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_W1\endcsname{0.75}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_W1c\endcsname{0.60}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_W2\endcsname{0.60}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_W3\endcsname{0.75}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_W3c\endcsname{0.75}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_W4\endcsname{0.75}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_W5\endcsname{0.75}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_ai_max\endcsname{0.89}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_ai_min\endcsname{0.60}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_base\endcsname{0.75}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_base_max\endcsname{0.89}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_base_min\endcsname{0.60}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_d_L1\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_d_L1b\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_d_L2\endcsname{0.00}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_d_L3\endcsname{0.00}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_d_L4\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_d_L6\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_d_W1\endcsname{0.00}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_d_W1c\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_d_W2\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_d_W3\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_d_W3c\endcsname{0.00}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_d_W4\endcsname{0.00}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_d_W5\endcsname{0.00}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_sd_base\endcsname{0.093}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_slope\endcsname{0.15}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_span\endcsname{0.29}
\expandafter\gdef\csname R@an.error_anatomy.amos_penalty_span_share\endcsname{84}
\expandafter\gdef\csname R@an.error_anatomy.amos_primary_sd_base\endcsname{0.122}
\expandafter\gdef\csname R@an.error_anatomy.amos_ref_n\endcsname{6}
\expandafter\gdef\csname R@an.error_anatomy.amos_ref_short\endcsname{frozen pool}
\expandafter\gdef\csname R@an.error_anatomy.amos_refclause\endcsname{AMOS22 deltas are against the 6-run frozen pool and against its uncompiled sub-pool of 3 runs, the like-for-like reference (\ensuremath{+0.029}\,pp from the frozen mean; at seed 0 the deltas against it are \ensuremath{+0.35}\,pp for HyReX and \ensuremath{+0.62}\,pp for ResEnc-M) and against the 3 contemporaneous default runs (\ensuremath{+0.011}\,pp from the frozen mean; at seed 0 the deltas against it are \ensuremath{+0.37}\,pp for HyReX and \ensuremath{+0.64}\,pp for ResEnc-M)}
\expandafter\gdef\csname R@an.error_anatomy.amos_right_adrenal_gland_medlog2_L1\endcsname{\ensuremath{-0.019}}
\expandafter\gdef\csname R@an.error_anatomy.amos_right_adrenal_gland_medlog2_L3\endcsname{\ensuremath{-0.006}}
\expandafter\gdef\csname R@an.error_anatomy.amos_right_adrenal_gland_medlog2_base\endcsname{\ensuremath{-0.021}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_L1\endcsname{\ensuremath{-0.009}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_L1_hi\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_L1_lo\endcsname{\ensuremath{-0.021}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_L1b\endcsname{\ensuremath{-0.013}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_L1b_hi\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_L1b_lo\endcsname{\ensuremath{-0.030}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_L2\endcsname{0.000}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_L2_hi\endcsname{\ensuremath{+0.016}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_L2_lo\endcsname{\ensuremath{-0.017}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_L3\endcsname{\ensuremath{-0.013}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_L3_hi\endcsname{\ensuremath{+0.005}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_L3_lo\endcsname{\ensuremath{-0.035}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_L4\endcsname{\ensuremath{-0.012}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_L4_hi\endcsname{\ensuremath{+0.008}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_L4_lo\endcsname{\ensuremath{-0.030}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_L6\endcsname{0.000}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_L6_hi\endcsname{\ensuremath{+0.014}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_L6_lo\endcsname{\ensuremath{-0.016}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W1\endcsname{\ensuremath{-0.006}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W1_hi\endcsname{\ensuremath{+0.006}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W1_lo\endcsname{\ensuremath{-0.027}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W1c\endcsname{\ensuremath{-0.001}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W1c_hi\endcsname{\ensuremath{+0.021}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W1c_lo\endcsname{\ensuremath{-0.014}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W2\endcsname{\ensuremath{-0.023}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W2_hi\endcsname{\ensuremath{-0.004}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W2_lo\endcsname{\ensuremath{-0.036}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W3\endcsname{\ensuremath{-0.008}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W3_hi\endcsname{\ensuremath{+0.009}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W3_lo\endcsname{\ensuremath{-0.022}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W3c\endcsname{\ensuremath{+0.002}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W3c_hi\endcsname{\ensuremath{+0.020}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W3c_lo\endcsname{\ensuremath{-0.014}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W4\endcsname{\ensuremath{+0.005}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W4_hi\endcsname{\ensuremath{+0.024}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W4_lo\endcsname{\ensuremath{-0.010}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W5\endcsname{\ensuremath{+0.004}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W5_hi\endcsname{\ensuremath{+0.022}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_dmedlog2_W5_lo\endcsname{\ensuremath{-0.010}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_fn_L1\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_fn_L1b\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_fn_L2\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_fn_L3\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_fn_L4\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_fn_L6\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_fn_W1\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_fn_W1c\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_fn_W2\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_fn_W3\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_fn_W3c\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_fn_W4\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_fn_W5\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_fn_ai_total\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_fn_base_max\endcsname{2}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_fn_base_mean\endcsname{0.3}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_fn_base_min\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_fn_base_runs\endcsname{0, 2, 0, 0, 0, 0}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_fn_base_total\endcsname{2}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L1\endcsname{\ensuremath{-0.018}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L1_hi\endcsname{0.000}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L1_lo\endcsname{\ensuremath{-0.042}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L1b\endcsname{\ensuremath{-0.022}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L1b_hi\endcsname{\ensuremath{+0.006}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L1b_lo\endcsname{\ensuremath{-0.049}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L2\endcsname{\ensuremath{-0.008}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L2_hi\endcsname{\ensuremath{+0.013}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L2_lo\endcsname{\ensuremath{-0.035}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L3\endcsname{\ensuremath{-0.022}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L3_hi\endcsname{\ensuremath{+0.006}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L3_lo\endcsname{\ensuremath{-0.063}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L3vL1\endcsname{\ensuremath{-0.004}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L3vL1_hi\endcsname{\ensuremath{+0.016}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L3vL1_lo\endcsname{\ensuremath{-0.032}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L4\endcsname{\ensuremath{-0.021}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L4_hi\endcsname{\ensuremath{+0.002}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L4_lo\endcsname{\ensuremath{-0.051}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L6\endcsname{\ensuremath{-0.009}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L6_hi\endcsname{\ensuremath{+0.010}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_L6_lo\endcsname{\ensuremath{-0.031}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W1\endcsname{\ensuremath{-0.015}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W1_hi\endcsname{\ensuremath{+0.001}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W1_lo\endcsname{\ensuremath{-0.045}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W1c\endcsname{\ensuremath{-0.010}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W1c_hi\endcsname{\ensuremath{+0.023}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W1c_lo\endcsname{\ensuremath{-0.031}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W2\endcsname{\ensuremath{-0.032}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W2_hi\endcsname{\ensuremath{-0.006}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W2_lo\endcsname{\ensuremath{-0.050}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W3\endcsname{\ensuremath{-0.017}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W3_hi\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W3_lo\endcsname{\ensuremath{-0.041}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W3c\endcsname{\ensuremath{-0.006}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W3c_hi\endcsname{\ensuremath{+0.024}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W3c_lo\endcsname{\ensuremath{-0.046}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W4\endcsname{\ensuremath{-0.004}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W4_hi\endcsname{\ensuremath{+0.022}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W4_lo\endcsname{\ensuremath{-0.037}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W5\endcsname{\ensuremath{-0.004}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W5_hi\endcsname{\ensuremath{+0.015}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_W5_lo\endcsname{\ensuremath{-0.030}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_base\endcsname{\ensuremath{-0.009}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_base_hi\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_base_lo\endcsname{\ensuremath{-0.036}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_base_max\endcsname{\ensuremath{+0.002}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medlog2_base_min\endcsname{\ensuremath{-0.017}}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_L1\endcsname{0.988}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_L1b\endcsname{0.985}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_L2\endcsname{0.994}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_L3\endcsname{0.985}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_L4\endcsname{0.986}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_L6\endcsname{0.994}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_W1\endcsname{0.990}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_W1c\endcsname{0.993}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_W2\endcsname{0.978}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_W3\endcsname{0.988}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_W3c\endcsname{0.996}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_W4\endcsname{0.997}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_W5\endcsname{0.997}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_ai_above\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_ai_below\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_ai_max\endcsname{0.994}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_ai_min\endcsname{0.978}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_ai_within\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_base\endcsname{0.994}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_base_max\endcsname{1.002}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_medratio_base_min\endcsname{0.988}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_names\endcsname{right adrenal gland, left adrenal gland, esophagus, gall bladder, prostate/uterus}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_L1\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_L1b\endcsname{2}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_L2\endcsname{2}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_L3\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_L4\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_L6\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_W1\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_W1c\endcsname{2}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_W2\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_W3\endcsname{2}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_W3c\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_W4\endcsname{2}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_W5\endcsname{2}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_ai_max\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_ai_min\endcsname{2}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_base_max\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_base_mean\endcsname{2.5}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_base_min\endcsname{2}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_base_runs\endcsname{2, 4, 3, 2, 2, 2}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_nf_base_total\endcsname{15}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_overlap\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_pairs\endcsname{196}
\expandafter\gdef\csname R@an.error_anatomy.amos_s5_pairs_total\endcsname{200}
\expandafter\gdef\csname R@an.error_anatomy.amos_screen_threshold\endcsname{0.35}
\expandafter\gdef\csname R@an.error_anatomy.amos_seeds_L1\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_seeds_L1b\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_seeds_L2\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_seeds_L3\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.amos_seeds_L4\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_ai_arms\endcsname{L2, L3, L4, L6}
\expandafter\gdef\csname R@an.error_anatomy.kits_ai_n\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.kits_altref_contemporaneous_n\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_altref_contemporaneous_shift\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.error_anatomy.kits_altref_contemporaneous_short\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.error_anatomy.kits_altref_finished\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.error_anatomy.kits_altref_n_finished\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.kits_altref_n_pending\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_altref_pending\endcsname{none}
\expandafter\gdef\csname R@an.error_anatomy.kits_altref_union_n\endcsname{6}
\expandafter\gdef\csname R@an.error_anatomy.kits_altref_union_shift\endcsname{\ensuremath{+0.244}}
\expandafter\gdef\csname R@an.error_anatomy.kits_altref_union_short\endcsname{six-run reference}
\expandafter\gdef\csname R@an.error_anatomy.kits_dice_delta_L1\endcsname{\ensuremath{+2.33}}
\expandafter\gdef\csname R@an.error_anatomy.kits_dice_delta_L1_contemporaneous\endcsname{\ensuremath{+1.84}}
\expandafter\gdef\csname R@an.error_anatomy.kits_dice_delta_L1_union\endcsname{\ensuremath{+2.08}}
\expandafter\gdef\csname R@an.error_anatomy.kits_dice_delta_L3\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.error_anatomy.kits_dice_delta_L3_contemporaneous\endcsname{\ensuremath{+2.35}}
\expandafter\gdef\csname R@an.error_anatomy.kits_dice_delta_L3_union\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@an.error_anatomy.kits_fn_case_top\endcsname{case\_00463}
\expandafter\gdef\csname R@an.error_anatomy.kits_fn_case_top_nref\endcsname{2\,061}
\expandafter\gdef\csname R@an.error_anatomy.kits_fn_case_top_runs\endcsname{7}
\expandafter\gdef\csname R@an.error_anatomy.kits_fn_case_top_small\endcsname{smallest}
\expandafter\gdef\csname R@an.error_anatomy.kits_fn_cases_n\endcsname{2}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_fn_L1\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_fn_L1b\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_fn_L2\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_fn_L3\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_fn_L4\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_fn_L6\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_fn_W1c\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_fn_base_max\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_fn_base_mean\endcsname{0.0}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_fn_base_min\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_fn_base_runs\endcsname{0, 0, 0}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_fn_base_total\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medlog2_L1\endcsname{\ensuremath{+0.004}}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medlog2_L1b\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medlog2_L2\endcsname{\ensuremath{+0.012}}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medlog2_L3\endcsname{\ensuremath{+0.010}}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medlog2_L4\endcsname{\ensuremath{+0.003}}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medlog2_L6\endcsname{\ensuremath{+0.003}}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medlog2_W1c\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medlog2_base\endcsname{\ensuremath{+0.009}}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medlog2_base_max\endcsname{\ensuremath{+0.013}}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medlog2_base_min\endcsname{\ensuremath{+0.005}}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medratio_L1\endcsname{1.003}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medratio_L1b\endcsname{1.005}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medratio_L2\endcsname{1.008}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medratio_L3\endcsname{1.007}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medratio_L4\endcsname{1.002}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medratio_L6\endcsname{1.002}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medratio_W1c\endcsname{1.005}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medratio_base\endcsname{1.007}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medratio_base_max\endcsname{1.009}
\expandafter\gdef\csname R@an.error_anatomy.kits_kidney_medratio_base_min\endcsname{1.004}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_fn_L1\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_fn_L1b\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_fn_L2\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_fn_L3\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_fn_L4\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_fn_L6\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_fn_W1c\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_fn_base_max\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_fn_base_mean\endcsname{0.0}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_fn_base_min\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_fn_base_runs\endcsname{0, 0, 0}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_fn_base_total\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medlog2_L1\endcsname{\ensuremath{+0.047}}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medlog2_L1b\endcsname{\ensuremath{+0.064}}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medlog2_L2\endcsname{\ensuremath{+0.061}}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medlog2_L3\endcsname{\ensuremath{+0.091}}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medlog2_L4\endcsname{\ensuremath{+0.032}}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medlog2_L6\endcsname{\ensuremath{+0.073}}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medlog2_W1c\endcsname{\ensuremath{+0.053}}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medlog2_base\endcsname{\ensuremath{+0.074}}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medlog2_base_max\endcsname{\ensuremath{+0.080}}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medlog2_base_min\endcsname{\ensuremath{+0.062}}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medratio_L1\endcsname{1.033}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medratio_L1b\endcsname{1.045}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medratio_L2\endcsname{1.043}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medratio_L3\endcsname{1.065}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medratio_L4\endcsname{1.023}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medratio_L6\endcsname{1.052}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medratio_W1c\endcsname{1.038}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medratio_base\endcsname{1.052}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medratio_base_max\endcsname{1.057}
\expandafter\gdef\csname R@an.error_anatomy.kits_masses_medratio_base_min\endcsname{1.044}
\expandafter\gdef\csname R@an.error_anatomy.kits_nbase\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_ncases\endcsname{98}
\expandafter\gdef\csname R@an.error_anatomy.kits_outside_null\endcsname{50}
\expandafter\gdef\csname R@an.error_anatomy.kits_ref_n\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_ref_short\endcsname{frozen pool}
\expandafter\gdef\csname R@an.error_anatomy.kits_refclause\endcsname{KiTS23 deltas are against the 3-run frozen pool and against the six-run reference of the frozen and contemporaneous default runs (\ensuremath{+0.244}\,pp from the frozen mean; at seed 0 the deltas against it are \ensuremath{+2.60}\,pp for HyReX and \ensuremath{+2.08}\,pp for ResEnc-M)}
\expandafter\gdef\csname R@an.error_anatomy.kits_seeds_L1\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_seeds_L1b\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_seeds_L2\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_seeds_L3\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_seeds_L4\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_seeds_L6\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_seeds_W1c\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_contriblarge_L1\endcsname{\ensuremath{+0.84}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_contriblarge_L3\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_contribmid_L1\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_contribmid_L3\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_contribsmall_L1\endcsname{\ensuremath{+2.37}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_contribsmall_L3\endcsname{\ensuremath{+3.71}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dice_large_base\endcsname{83.1}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dice_large_base_max\endcsname{83.7}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dice_large_base_min\endcsname{82.3}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dice_mid_base\endcsname{82.9}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dice_mid_base_max\endcsname{85.2}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dice_mid_base_min\endcsname{81.3}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dice_small_base\endcsname{57.1}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dice_small_base_max\endcsname{58.5}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dice_small_base_min\endcsname{55.2}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dlarge_L1\endcsname{\ensuremath{+2.6}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dlarge_L1_hi\endcsname{\ensuremath{+5.5}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dlarge_L1_lo\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dlarge_L3\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dlarge_L3_hi\endcsname{\ensuremath{+4.3}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dlarge_L3_lo\endcsname{\ensuremath{-0.2}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dlarge_L3vL1\endcsname{\ensuremath{-0.8}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dlarge_L3vL1_hi\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dlarge_L3vL1_lo\endcsname{\ensuremath{-1.8}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dmid_L1\endcsname{\ensuremath{-0.9}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dmid_L1_hi\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dmid_L1_lo\endcsname{\ensuremath{-5.3}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dmid_L3\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dmid_L3_hi\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dmid_L3_lo\endcsname{\ensuremath{-4.5}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dmid_L3vL1\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dmid_L3vL1_hi\endcsname{\ensuremath{+3.0}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dmid_L3vL1_lo\endcsname{\ensuremath{-1.8}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dsmall_L1\endcsname{\ensuremath{+7.0}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dsmall_L1_hi\endcsname{\ensuremath{+12.9}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dsmall_L1_lo\endcsname{\ensuremath{+1.7}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dsmall_L3\endcsname{\ensuremath{+11.0}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dsmall_L3_hi\endcsname{\ensuremath{+17.4}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dsmall_L3_lo\endcsname{\ensuremath{+5.2}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dsmall_L3vL1\endcsname{\ensuremath{+4.0}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dsmall_L3vL1_hi\endcsname{\ensuremath{+10.5}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_dsmall_L3vL1_lo\endcsname{\ensuremath{-2.3}}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_n_large\endcsname{32}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_n_mid\endcsname{33}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_n_small\endcsname{33}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_nrefmax_large\endcsname{1\,489\,413}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_nrefmax_mid\endcsname{28\,542}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_nrefmax_small\endcsname{7\,619}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_nrefmin_large\endcsname{31\,056}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_nrefmin_mid\endcsname{8\,399}
\expandafter\gdef\csname R@an.error_anatomy.kits_size_nrefmin_small\endcsname{513}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dicegain_L1\endcsname{\ensuremath{+2.90}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dicegain_L3\endcsname{\ensuremath{+4.11}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_L1\endcsname{\ensuremath{-0.036}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_L1_hi\endcsname{\ensuremath{-0.006}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_L1_lo\endcsname{\ensuremath{-0.097}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_L1b\endcsname{\ensuremath{-0.001}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_L1b_hi\endcsname{\ensuremath{+0.026}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_L1b_lo\endcsname{\ensuremath{-0.069}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_L2\endcsname{\ensuremath{+0.010}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_L2_hi\endcsname{\ensuremath{+0.085}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_L2_lo\endcsname{\ensuremath{-0.052}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_L3\endcsname{0.000}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_L3_hi\endcsname{\ensuremath{+0.062}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_L3_lo\endcsname{\ensuremath{-0.040}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_L4\endcsname{\ensuremath{-0.037}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_L4_hi\endcsname{\ensuremath{+0.004}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_L4_lo\endcsname{\ensuremath{-0.101}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_L6\endcsname{\ensuremath{-0.026}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_L6_hi\endcsname{\ensuremath{+0.010}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_L6_lo\endcsname{\ensuremath{-0.084}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_W1c\endcsname{\ensuremath{-0.009}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_W1c_hi\endcsname{\ensuremath{+0.024}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dmedlog2_W1c_lo\endcsname{\ensuremath{-0.062}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dprec_L1\endcsname{\ensuremath{+5.0}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dprec_L1_hi\endcsname{\ensuremath{+8.0}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dprec_L1_lo\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dprec_L3\endcsname{\ensuremath{+4.3}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dprec_L3_hi\endcsname{\ensuremath{+7.6}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dprec_L3_lo\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dprec_ai_max\endcsname{\ensuremath{+5.3}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_dprec_ai_min\endcsname{\ensuremath{-0.2}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_drec_L1\endcsname{\ensuremath{-0.5}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_drec_L1_hi\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_drec_L1_lo\endcsname{\ensuremath{-1.8}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_drec_L3\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_drec_L3_hi\endcsname{\ensuremath{+3.5}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_drec_L3_lo\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_drec_ai_max\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_drec_ai_min\endcsname{0.0}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_L1\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_L1_seeds\endcsname{1, 0, 1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_L1b\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_L1b_seeds\endcsname{0, 0, 1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_L2\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_L2_seeds\endcsname{0, 0, 1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_L3\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_L3_seeds\endcsname{0, 0, 0}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_L3vL1\endcsname{\ensuremath{-1}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_L4\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_L4_seeds\endcsname{1, 0, 1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_L6\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_L6_seeds\endcsname{0, 0, 0}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_W1c\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_W1c_seeds\endcsname{0, 1, 0}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_ai_max\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_ai_total\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_base_max\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_base_mean\endcsname{0.3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_base_min\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_base_runs\endcsname{0, 1, 0}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_fn_base_total\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L1\endcsname{\ensuremath{+0.071}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L1_fresh\endcsname{\ensuremath{+0.072}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L1_hi\endcsname{\ensuremath{+0.147}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L1_lo\endcsname{\ensuremath{+0.027}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L1b\endcsname{\ensuremath{+0.106}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L1b_fresh\endcsname{\ensuremath{+0.096}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L1b_hi\endcsname{\ensuremath{+0.163}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L1b_lo\endcsname{\ensuremath{+0.036}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L2\endcsname{\ensuremath{+0.117}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L2_fresh\endcsname{\ensuremath{+0.124}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L2_hi\endcsname{\ensuremath{+0.227}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L2_lo\endcsname{\ensuremath{+0.057}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L3\endcsname{\ensuremath{+0.107}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L3_fresh\endcsname{\ensuremath{+0.135}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L3_hi\endcsname{\ensuremath{+0.206}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L3_lo\endcsname{\ensuremath{+0.068}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L3vL1\endcsname{\ensuremath{+0.037}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L3vL1_hi\endcsname{\ensuremath{+0.109}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L3vL1_lo\endcsname{\ensuremath{+0.002}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L4\endcsname{\ensuremath{+0.070}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L4_fresh\endcsname{\ensuremath{+0.081}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L4_hi\endcsname{\ensuremath{+0.135}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L4_lo\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L6\endcsname{\ensuremath{+0.081}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L6_fresh\endcsname{\ensuremath{+0.079}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L6_hi\endcsname{\ensuremath{+0.130}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_L6_lo\endcsname{\ensuremath{+0.037}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_W1c\endcsname{\ensuremath{+0.099}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_W1c_hi\endcsname{\ensuremath{+0.162}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_W1c_lo\endcsname{\ensuremath{+0.060}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_base\endcsname{\ensuremath{+0.107}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_base_hi\endcsname{\ensuremath{+0.198}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_base_lo\endcsname{\ensuremath{+0.070}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_base_max\endcsname{\ensuremath{+0.113}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medlog2_base_min\endcsname{\ensuremath{+0.101}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L1\endcsname{1.050}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L1_fresh\endcsname{1.051}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L1_seedmax\endcsname{1.052}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L1_seedmin\endcsname{1.050}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L1b\endcsname{1.076}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L1b_fresh\endcsname{1.068}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L1b_seedmax\endcsname{1.076}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L1b_seedmin\endcsname{1.064}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L2\endcsname{1.085}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L2_fresh\endcsname{1.089}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L2_seedmax\endcsname{1.092}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L2_seedmin\endcsname{1.085}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L3\endcsname{1.077}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L3_fresh\endcsname{1.098}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L3_fresh_dir\endcsname{above}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L3_fresh_dirclause\endcsname{is above the default pool's 1.077: the direction is the opposite of a network that gains by predicting less tumour}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L3_seedmax\endcsname{1.106}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L3_seedmin\endcsname{1.077}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L4\endcsname{1.050}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L4_fresh\endcsname{1.058}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L4_seedmax\endcsname{1.075}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L4_seedmin\endcsname{1.041}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L6\endcsname{1.058}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L6_fresh\endcsname{1.057}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L6_seedmax\endcsname{1.060}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_L6_seedmin\endcsname{1.053}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_W1c\endcsname{1.071}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_W1c_seedmax\endcsname{1.074}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_W1c_seedmin\endcsname{1.058}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_ai_above\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_ai_below\endcsname{2}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_ai_max\endcsname{1.085}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_ai_min\endcsname{1.050}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_ai_within\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_armspan\endcsname{0.035}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_armspan_n\endcsname{6}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_base\endcsname{1.077}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_base_max\endcsname{1.081}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_base_min\endcsname{1.073}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_fresh_ci_over_pool\endcsname{6}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_fresh_margin\endcsname{\ensuremath{+0.009}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_fresh_max\endcsname{1.098}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_fresh_max_arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_fresh_n\endcsname{6}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_fresh_order_caption\endcsname{The two highest KiTS23 fresh medians differ by \ensuremath{+0.009}, against a pool range of 0.009 and a widest within-arm seed span of 0.035, so the medians locate the arms and do not order them}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_fresh_order_clause\endcsname{the fresh-seed medians do not order the arms at the scale this measurement resolves: the two highest, HyReX at 1.098 and ConvNeXt-k3 at 1.089, differ by \ensuremath{+0.009}, while three runs of the default network alone span 0.009 and the widest within-arm seed-to-seed span is 0.035 (ResEnc+context)}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_fresh_overlap_Clause\endcsname{Every arm's volume-ratio interval overlaps the default pool's own range on KiTS23 (6 of 6 arms with a fresh mean)}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_fresh_overlap_clause\endcsname{every arm's volume-ratio interval overlaps the default pool's own range on KiTS23 (6 of 6 arms with a fresh mean)}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_fresh_pending\endcsname{0}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_fresh_poolrange\endcsname{0.009}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_fresh_resolved\endcsname{no}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_fresh_runnerup\endcsname{1.089}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_fresh_runnerup_arm\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_fresh_scale\endcsname{0.035}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_fresh_scale_what\endcsname{the widest within-arm seed-to-seed span}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_main_above\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_main_above_arms\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_main_below\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_main_below_arms\endcsname{ResEnc-M, ResEnc+context, HyReX+context}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_main_n\endcsname{6}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_main_within\endcsname{2}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_seedspan_arm\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_seedspan_max\endcsname{0.035}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_seedspan_n\endcsname{7}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_span_Clause\endcsname{The seed-to-seed spread of one arm is as wide as the spread between arms: the widest within-arm span is 0.99 times the 0.035 spread between the discovery seeds of the 6 drawn arms}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_span_clause\endcsname{the seed-to-seed spread of one arm is as wide as the spread between arms: the widest within-arm span is 0.99 times the 0.035 spread between the discovery seeds of the 6 drawn arms}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_span_rel\endcsname{as wide as}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_medratio_spanratio\endcsname{0.99}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_L1\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_L1_seeds\endcsname{5, 4, 3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_L1b\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_L1b_seeds\endcsname{5, 3, 4}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_L2\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_L2_seeds\endcsname{3, 4, 2}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_L3\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_L3_seeds\endcsname{1, 2, 3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_L4\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_L4_seeds\endcsname{3, 4, 4}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_L6\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_L6_seeds\endcsname{5, 3, 5}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_W1c\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_W1c_seeds\endcsname{3, 2, 4}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_ai_max\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_ai_min\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_base_max\endcsname{6}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_base_mean\endcsname{5.3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_base_min\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_base_runs\endcsname{5, 5, 6}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_base_total\endcsname{16}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_small_L1\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_small_L1b\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_small_L2\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_small_L3\endcsname{1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_small_L4\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_small_L6\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_small_W1c\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_small_base_max\endcsname{6}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_small_base_mean\endcsname{5.0}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_small_base_min\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_small_base_runs\endcsname{5, 4, 6}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_nf_small_base_total\endcsname{15}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_L1\endcsname{8}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_L1b\endcsname{14}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_L2\endcsname{12}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_L3\endcsname{12}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_L3vL1\endcsname{\ensuremath{+4}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_L4\endcsname{9}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_L6\endcsname{10}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_W1c\endcsname{6}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_ai_max\endcsname{12}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_ai_min\endcsname{9}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_base_max\endcsname{17}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_base_mean\endcsname{14.3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_base_min\endcsname{12}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_base_runs\endcsname{12, 14, 17}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_base_total\endcsname{43}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_small_L1\endcsname{5}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_small_L1b\endcsname{9}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_small_L2\endcsname{9}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_small_L3\endcsname{8}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_small_L4\endcsname{6}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_small_L6\endcsname{8}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_small_W1c\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_small_base_max\endcsname{12}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_small_base_mean\endcsname{10.7}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_small_base_min\endcsname{9}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_small_base_runs\endcsname{9, 11, 12}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_over_small_base_total\endcsname{32}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_L1\endcsname{76.9}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_L1_seedmax\endcsname{80.1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_L1_seedmin\endcsname{76.9}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_L1b_seedmax\endcsname{76.3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_L1b_seedmin\endcsname{75.3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_L2_seedmax\endcsname{72.8}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_L2_seedmin\endcsname{70.8}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_L3\endcsname{76.3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_L3_seedmax\endcsname{76.3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_L3_seedmin\endcsname{73.8}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_L3vL1\endcsname{\ensuremath{-0.7}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_L3vL1_hi\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_L3vL1_lo\endcsname{\ensuremath{-3.2}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_L4_seedmax\endcsname{78.1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_L4_seedmin\endcsname{76.6}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_L6_seedmax\endcsname{76.7}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_L6_seedmin\endcsname{74.1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_W1c_seedmax\endcsname{76.4}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_W1c_seedmin\endcsname{73.0}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_ai_max\endcsname{77.3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_ai_min\endcsname{71.8}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_base\endcsname{72.0}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_base_max\endcsname{73.1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_prec_base_min\endcsname{70.5}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_L1\endcsname{83.7}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_L1_seedmax\endcsname{84.7}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_L1_seedmin\endcsname{83.7}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_L1b_seedmax\endcsname{86.2}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_L1b_seedmin\endcsname{84.0}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_L2_seedmax\endcsname{86.1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_L2_seedmin\endcsname{84.5}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_L3\endcsname{86.3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_L3_seedmax\endcsname{86.3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_L3_seedmin\endcsname{85.3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_L3vL1\endcsname{\ensuremath{+2.6}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_L3vL1_hi\endcsname{\ensuremath{+4.9}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_L3vL1_lo\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_L4_seedmax\endcsname{84.2}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_L4_seedmin\endcsname{83.4}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_L6_seedmax\endcsname{85.0}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_L6_seedmin\endcsname{83.7}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_W1c_seedmax\endcsname{84.1}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_W1c_seedmin\endcsname{83.2}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_ai_max\endcsname{86.3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_ai_min\endcsname{84.2}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_base\endcsname{84.2}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_base_max\endcsname{84.7}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_rec_base_min\endcsname{83.6}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_under_L1\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_under_L1b\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_under_L2\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_under_L3\endcsname{2}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_under_L4\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_under_L6\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_under_W1c\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_under_base_max\endcsname{4}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_under_base_mean\endcsname{3.3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_under_base_min\endcsname{3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_under_base_runs\endcsname{3, 4, 3}
\expandafter\gdef\csname R@an.error_anatomy.kits_tumor_under_base_total\endcsname{10}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.allseedsgap.poolmax\endcsname{\ensuremath{+0.106}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.allseedsmax\endcsname{92.345}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.allseedsmin\endcsname{92.234}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.ci6.hi\endcsname{\ensuremath{+0.449}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.ci6.lo\endcsname{\ensuremath{+0.034}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.clearspairfloor\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.delta_s0\endcsname{\ensuremath{+0.336}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.delta_vscontemp\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.delta_vscontemp.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.delta_vsdefault\endcsname{\ensuremath{+0.242}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.delta_vsrebuild\endcsname{\ensuremath{+0.125}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.delta_vsrebuild.s1\endcsname{\ensuremath{+0.134}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.delta_vsrebuild.s2\endcsname{\ensuremath{+0.116}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.delta_vsrebuild.se\endcsname{0.019}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.delta_vsrebuild.spread\endcsname{0.018}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.delta_vsunion\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.delta_vsunion.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.discoveryseed0\endcsname{92.345}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.fresh_in_se_units\endcsname{3.00}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.fresh_vsL3\endcsname{\ensuremath{-0.208}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.fresh_vsL3.abs\endcsname{0.208}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.fresh_vsL3.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.fresh_vsL3.inscale\endcsname{2.11}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.fresh_vsL3.order\endcsname{every HyReX fresh run lies above every fresh run of this arm}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.fresh_vsL3.ordergap\endcsname{0.158}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.fresh_vsL3.relfloor\endcsname{0.42}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.fresh_vsL3.se\endcsname{0.038}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.freshbar\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.freshgap.poolmax\endcsname{\ensuremath{+0.106}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.freshmax\endcsname{92.268}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.freshmean\endcsname{92.251}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.freshmin\endcsname{92.234}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.freshminusbar\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.freshminuss0\endcsname{\ensuremath{-0.094}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.freshresolution\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.freshspread\endcsname{0.034}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.freshvsownse\endcsname{14.16}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.pairsd\endcsname{0.024}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.resolutionbinding\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.retained\endcsname{retained}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.s0_in_single_seed_sd\endcsname{3.14}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.s0minusbar\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.samedefault.fresh\endcsname{\ensuremath{+0.275}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.samedefault.s0\endcsname{\ensuremath{+0.248}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.samedefault.s1\endcsname{\ensuremath{+0.285}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.samedefault.s2\endcsname{\ensuremath{+0.266}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.sedelta\endcsname{0.081}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.seed1\endcsname{92.268}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.seed2\endcsname{92.234}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.sepair\endcsname{0.017}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.threeseeddelta\endcsname{\ensuremath{+0.273}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.threeseedmean\endcsname{92.282}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.vsL3.clause\endcsname{ResEnc-M's fresh mean, 92.251 Dice, is 0.208\,pp below HyReX's 92.460, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.038\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1.vsL3.sentence\endcsname{on ACDC fold 0, at 2 fresh seeds per arm, ResEnc-M reads 0.208\,pp below HyReX, 0.42 times the registered 0.50\,pp one-seed pair floor and 2.11 standard errors at the frozen ACDC pool seed SD of 0.099\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); every HyReX fresh run lies above every fresh run of ResEnc-M, the smallest gap 0.158\,pp}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.allseedsgap.poolmax\endcsname{\ensuremath{+0.164}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.allseedsmax\endcsname{92.361}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.allseedsmin\endcsname{92.293}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.ci6.hi\endcsname{\ensuremath{+0.526}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.ci6.lo\endcsname{\ensuremath{+0.112}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.clearspairfloor\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.delta_s0\endcsname{\ensuremath{+0.283}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.delta_vscontemp\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.delta_vscontemp.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.delta_vsdefault\endcsname{\ensuremath{+0.319}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.delta_vsrebuild\endcsname{\ensuremath{+0.202}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.delta_vsrebuild.s1\endcsname{\ensuremath{+0.161}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.delta_vsrebuild.s2\endcsname{\ensuremath{+0.243}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.delta_vsrebuild.se\endcsname{0.034}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.delta_vsrebuild.spread\endcsname{0.082}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.delta_vsunion\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.delta_vsunion.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.discoveryseed0\endcsname{92.293}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.fresh_in_se_units\endcsname{3.95}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.fresh_vsL1\endcsname{\ensuremath{+0.077}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.fresh_vsL1.dir\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.fresh_vsL1.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.fresh_vsL3\endcsname{\ensuremath{-0.131}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.fresh_vsL3.abs\endcsname{0.131}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.fresh_vsL3.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.fresh_vsL3.inscale\endcsname{1.33}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.fresh_vsL3.order\endcsname{every HyReX fresh run lies above every fresh run of this arm}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.fresh_vsL3.ordergap\endcsname{0.065}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.fresh_vsL3.relfloor\endcsname{0.26}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.fresh_vsL3.se\endcsname{0.047}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.freshbar\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.freshgap.poolmax\endcsname{\ensuremath{+0.167}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.freshmax\endcsname{92.361}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.freshmean\endcsname{92.328}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.freshmin\endcsname{92.296}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.freshminusbar\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.freshminuss0\endcsname{\ensuremath{+0.036}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.freshresolution\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.freshspread\endcsname{0.065}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.freshvsownse\endcsname{9.75}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.pairsd\endcsname{0.046}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.refminusfresh\endcsname{\ensuremath{-0.077}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.refminusfresh.inse\endcsname{2.09}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.refminusfresh.se\endcsname{0.037}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.resolutionbinding\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.retained\endcsname{retained}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.s0_in_single_seed_sd\endcsname{2.65}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.s0minusbar\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.samedefault.fresh\endcsname{\ensuremath{+0.352}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.samedefault.s0\endcsname{\ensuremath{+0.195}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.samedefault.s1\endcsname{\ensuremath{+0.312}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.samedefault.s2\endcsname{\ensuremath{+0.393}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.sedelta\endcsname{0.081}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.seed1\endcsname{92.296}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.seed2\endcsname{92.361}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.sepair\endcsname{0.033}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.threeseeddelta\endcsname{\ensuremath{+0.307}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.threeseedmean\endcsname{92.316}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.vsL3.clause\endcsname{ResEnc-matched's fresh mean, 92.328 Dice, is 0.131\,pp below HyReX's 92.460, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.047\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L1b.vsL3.sentence\endcsname{on ACDC fold 0, at 2 fresh seeds per arm, ResEnc-matched reads 0.131\,pp below HyReX, 0.26 times the registered 0.50\,pp one-seed pair floor and 1.33 standard errors at the frozen ACDC pool seed SD of 0.099\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); every HyReX fresh run lies above every fresh run of ResEnc-matched, the smallest gap 0.065\,pp}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.allseedsgap.poolmax\endcsname{\ensuremath{+0.298}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.allseedsmax\endcsname{92.626}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.allseedsmin\endcsname{92.426}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.ci6.hi\endcsname{\ensuremath{+0.658}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.ci6.lo\endcsname{\ensuremath{+0.243}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.clearspairfloor\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.delta_s0\endcsname{\ensuremath{+0.616}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.delta_vscontemp\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.delta_vscontemp.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.delta_vsdefault\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.delta_vsrebuild\endcsname{\ensuremath{+0.334}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.delta_vsrebuild.s1\endcsname{\ensuremath{+0.292}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.delta_vsrebuild.s2\endcsname{\ensuremath{+0.375}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.delta_vsrebuild.se\endcsname{0.034}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.delta_vsrebuild.spread\endcsname{0.083}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.delta_vsunion\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.delta_vsunion.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.discoveryseed0\endcsname{92.626}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.fresh_in_se_units\endcsname{5.58}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.fresh_vsL1\endcsname{\ensuremath{+0.208}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.fresh_vsL1.dir\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.fresh_vsL1.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.freshbar\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.freshgap.poolmax\endcsname{\ensuremath{+0.298}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.freshmax\endcsname{92.493}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.freshmean\endcsname{92.460}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.freshmin\endcsname{92.426}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.freshminusbar\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.freshminuss0\endcsname{\ensuremath{-0.166}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.freshresolution\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.freshspread\endcsname{0.067}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.freshvsownse\endcsname{13.45}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.pairsd\endcsname{0.047}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.refminusfresh\endcsname{\ensuremath{-0.208}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.refminusfresh.inse\endcsname{5.55}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.refminusfresh.se\endcsname{0.038}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.resolutionbinding\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.retained\endcsname{retained}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.s0_in_single_seed_sd\endcsname{5.77}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.s0minusbar\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.samedefault.fresh\endcsname{\ensuremath{+0.484}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.samedefault.s0\endcsname{\ensuremath{+0.528}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.samedefault.s1\endcsname{\ensuremath{+0.442}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.samedefault.s2\endcsname{\ensuremath{+0.525}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.sedelta\endcsname{0.081}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.seed1\endcsname{92.426}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.seed2\endcsname{92.493}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.sepair\endcsname{0.033}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.threeseeddelta\endcsname{\ensuremath{+0.506}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.threeseedmean\endcsname{92.515}
\expandafter\gdef\csname R@an.fresh_replication.acdc.L3.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.allseedsgap.poolmax\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.allseedsmax\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.allseedsmin\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.allseedsrange.vspool\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.ci6.hi\endcsname{\ensuremath{+0.324}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.ci6.lo\endcsname{\ensuremath{-0.091}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.clearspairfloor\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.delta_s0\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.delta_vscontemp\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.delta_vscontemp.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.delta_vsdefault\endcsname{\ensuremath{+0.117}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.delta_vsunion\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.delta_vsunion.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.discoveryseed0\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.discoveryseed0.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.fresh_in_se_units\endcsname{1.45}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.fresh_vsL1\endcsname{\ensuremath{-0.125}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.fresh_vsL1.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.fresh_vsL3\endcsname{\ensuremath{-0.334}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.fresh_vsL3.abs\endcsname{0.334}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.fresh_vsL3.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.fresh_vsL3.inscale\endcsname{3.37}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.fresh_vsL3.order\endcsname{every HyReX fresh run lies above every fresh run of this arm}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.fresh_vsL3.ordergap\endcsname{0.292}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.fresh_vsL3.relfloor\endcsname{0.67}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.fresh_vsL3.se\endcsname{0.034}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.freshbar\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.freshgap.poolmax\endcsname{\ensuremath{-0.011}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.freshmax\endcsname{92.134}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.freshmean\endcsname{92.126}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.freshmin\endcsname{92.118}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.freshminusbar\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.freshminuss0\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.freshrange.vspool\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.freshrange.vspool.phrase\endcsname{overlap}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.freshresolution\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.freshspread\endcsname{0.016}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.freshvsownse\endcsname{14.26}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.pairsd\endcsname{0.012}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.refminusfresh\endcsname{\ensuremath{+0.125}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.refminusfresh.inse\endcsname{6.61}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.refminusfresh.se\endcsname{0.019}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.resolutionbinding\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.retained\endcsname{retained}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.s0_in_single_seed_sd\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.s0_in_single_seed_sd.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.s0minusbar\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.samedefault.fresh\endcsname{\ensuremath{+0.150}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.samedefault.s0\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.samedefault.s1\endcsname{\ensuremath{+0.151}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.samedefault.s2\endcsname{\ensuremath{+0.150}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.sedelta\endcsname{0.081}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.seed1\endcsname{92.134}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.seed2\endcsname{92.118}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.sepair\endcsname{0.008}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.threeseeddelta\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.threeseedmean\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.threeseedmean.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.vsL3.clause\endcsname{the fn.-identical control's fresh mean, 92.126 Dice, is 0.334\,pp below HyReX's 92.460, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.034\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.acdc.P3c.vsL3.sentence\endcsname{on ACDC fold 0, at 2 fresh seeds per arm, the fn.-identical control reads 0.334\,pp below HyReX, 0.67 times the registered 0.50\,pp one-seed pair floor and 3.37 standard errors at the frozen ACDC pool seed SD of 0.099\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); every HyReX fresh run lies above every fresh run of the fn.-identical control, the smallest gap 0.292\,pp}
\expandafter\gdef\csname R@an.fresh_replication.acdc.ci6.half\endcsname{0.207}
\expandafter\gdef\csname R@an.fresh_replication.acdc.ci6.tq\endcsname{2.571}
\expandafter\gdef\csname R@an.fresh_replication.acdc.contemp.mean\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.contemp.shift\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.contemp.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.acdc.defaultadj\endcsname{six-run}
\expandafter\gdef\csname R@an.fresh_replication.acdc.defaultmean\endcsname{92.009}
\expandafter\gdef\csname R@an.fresh_replication.acdc.defaultn\endcsname{6}
\expandafter\gdef\csname R@an.fresh_replication.acdc.defaultsd\endcsname{0.099}
\expandafter\gdef\csname R@an.fresh_replication.acdc.deltaclause\endcsname{HyReX \ensuremath{+0.450}\,pp (\ensuremath{+0.243} to \ensuremath{+0.658}\,pp), ResEnc-matched \ensuremath{+0.319}\,pp (\ensuremath{+0.112} to \ensuremath{+0.526}\,pp), ResEnc-M \ensuremath{+0.242}\,pp (\ensuremath{+0.034} to \ensuremath{+0.449}\,pp) and the fn.-identical control \ensuremath{+0.117}\,pp (\ensuremath{-0.091} to \ensuremath{+0.324}\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.acdc.freshL3minusL1\endcsname{\ensuremath{+0.208}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.freshL3minusL1.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.freshabovelist.pool\endcsname{HyReX, ResEnc-M, ResEnc-matched}
\expandafter\gdef\csname R@an.fresh_replication.acdc.freshbelowbarlist\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.freshnotabovelist.pool\endcsname{fn.-identical control}
\expandafter\gdef\csname R@an.fresh_replication.acdc.freshresolvedlist\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.freshunresolvedlist\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.leaderclause\endcsname{the two highest fresh-seed deltas, HyReX \ensuremath{+0.450}\,pp and ResEnc-matched \ensuremath{+0.319}\,pp, are 0.131\,pp apart, a margin inside the registered 0.50\,pp one-seed pair floor; ACDC is the registered guard dataset}
\expandafter\gdef\csname R@an.fresh_replication.acdc.leaderclause.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.nbelowref\endcsname{1}
\expandafter\gdef\csname R@an.fresh_replication.acdc.ncases\endcsname{40}
\expandafter\gdef\csname R@an.fresh_replication.acdc.nfreshabove.pool\endcsname{3}
\expandafter\gdef\csname R@an.fresh_replication.acdc.nfreshbelowbar\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.nfreshclearsbar\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.nfreshnotabove.pool\endcsname{1}
\expandafter\gdef\csname R@an.fresh_replication.acdc.nfreshresolved\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.nfreshunresolved\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.nmoved\endcsname{3}
\expandafter\gdef\csname R@an.fresh_replication.acdc.nnotreproduced\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.nnotretained\endcsname{0}
\expandafter\gdef\csname R@an.fresh_replication.acdc.notreproducedlist\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.npending\endcsname{0}
\expandafter\gdef\csname R@an.fresh_replication.acdc.nregistered\endcsname{4}
\expandafter\gdef\csname R@an.fresh_replication.acdc.nreplicated\endcsname{4}
\expandafter\gdef\csname R@an.fresh_replication.acdc.nretained\endcsname{4}
\expandafter\gdef\csname R@an.fresh_replication.acdc.nshiftinside\endcsname{2}
\expandafter\gdef\csname R@an.fresh_replication.acdc.nshiftoutside\endcsname{1}
\expandafter\gdef\csname R@an.fresh_replication.acdc.nvshero\endcsname{3}
\expandafter\gdef\csname R@an.fresh_replication.acdc.nvsref\endcsname{3}
\expandafter\gdef\csname R@an.fresh_replication.acdc.nwithinhero\endcsname{3}
\expandafter\gdef\csname R@an.fresh_replication.acdc.pool.max\endcsname{92.128}
\expandafter\gdef\csname R@an.fresh_replication.acdc.pool.min\endcsname{91.853}
\expandafter\gdef\csname R@an.fresh_replication.acdc.poolspread\endcsname{0.275}
\expandafter\gdef\csname R@an.fresh_replication.acdc.referencearm\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.fresh_replication.acdc.replicated.clause\endcsname{all 4 registered arms have a complete fresh pair}
\expandafter\gdef\csname R@an.fresh_replication.acdc.retainedlist\endcsname{HyReX, ResEnc-M, ResEnc-matched, fn.-identical control}
\expandafter\gdef\csname R@an.fresh_replication.acdc.runnerupfresharm\endcsname{ResEnc-matched}
\expandafter\gdef\csname R@an.fresh_replication.acdc.runnerupfreshdelta\endcsname{\ensuremath{+0.319}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.samedefaultfreshmean\endcsname{91.976}
\expandafter\gdef\csname R@an.fresh_replication.acdc.samedefaultgap\endcsname{\ensuremath{+0.034}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.samedefaultgap.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.samedefaultn\endcsname{3}
\expandafter\gdef\csname R@an.fresh_replication.acdc.samedefaultsource\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.fresh_replication.acdc.sddf\endcsname{5}
\expandafter\gdef\csname R@an.fresh_replication.acdc.sdfresh\endcsname{0.081}
\expandafter\gdef\csname R@an.fresh_replication.acdc.sdfreshpair\endcsname{0.099}
\expandafter\gdef\csname R@an.fresh_replication.acdc.sdshift\endcsname{0.121}
\expandafter\gdef\csname R@an.fresh_replication.acdc.sdsingle\endcsname{0.107}
\expandafter\gdef\csname R@an.fresh_replication.acdc.shiftinsidelist\endcsname{ResEnc-M, ResEnc-matched}
\expandafter\gdef\csname R@an.fresh_replication.acdc.shiftoutsidelist\endcsname{HyReX}
\expandafter\gdef\csname R@an.fresh_replication.acdc.topfresh.licence\endcsname{an ordering, not a resolved superlative}
\expandafter\gdef\csname R@an.fresh_replication.acdc.topfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.acdc.topfresharm\endcsname{HyReX}
\expandafter\gdef\csname R@an.fresh_replication.acdc.topfreshdelta\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.fresh_replication.acdc.topfreshmargin\endcsname{0.131}
\expandafter\gdef\csname R@an.fresh_replication.acdc.topfreshmargin.binding\endcsname{the registered one-seed pair floor}
\expandafter\gdef\csname R@an.fresh_replication.acdc.topfreshmargin.inse\endcsname{2.80}
\expandafter\gdef\csname R@an.fresh_replication.acdc.topfreshmargin.se\endcsname{0.047}
\expandafter\gdef\csname R@an.fresh_replication.acdc.union.mean\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.union.n\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.acdc.withinhero.clause\endcsname{of the 3 other arms with a complete fresh pair, all lie inside the registered 0.50\,pp one-seed pair floor of HyReX's fresh mean: ResEnc-M, ResEnc-matched, fn.-identical control}
\expandafter\gdef\csname R@an.fresh_replication.acdc.withinherolist\endcsname{ResEnc-M, ResEnc-matched, fn.-identical control}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.allseedsgap.poolmax\endcsname{\ensuremath{+0.096}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.allseedsmax\endcsname{88.363}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.allseedsmin\endcsname{87.969}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.ci6.hi\endcsname{\ensuremath{+0.721}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.ci6.lo\endcsname{\ensuremath{+0.208}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.clearspairfloor\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.delta_s0\endcsname{\ensuremath{+0.647}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.delta_vscontemp\endcsname{\ensuremath{+0.454}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.delta_vsdefault\endcsname{\ensuremath{+0.465}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.delta_vsrebuild\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.delta_vsrebuild.s1\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.delta_vsrebuild.s2\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.delta_vsrebuild.se\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.delta_vsrebuild.spread\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.delta_vsrebuild.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.delta_vsunion\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.delta_vsunion.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.discoveryseed0\endcsname{88.348}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.fresh_in_se_units\endcsname{4.66}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.fresh_vsL3\endcsname{\ensuremath{+0.332}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.fresh_vsL3.abs\endcsname{0.332}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.fresh_vsL3.dir\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.fresh_vsL3.inscale\endcsname{2.72}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.fresh_vsL3.order\endcsname{the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.fresh_vsL3.relfloor\endcsname{0.66}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.fresh_vsL3.se\endcsname{0.246}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.freshgap.poolmax\endcsname{\ensuremath{+0.096}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.freshmax\endcsname{88.363}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.freshmean\endcsname{88.166}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.freshmin\endcsname{87.969}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.freshminusbar\endcsname{\ensuremath{+0.115}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.freshminuss0\endcsname{\ensuremath{-0.182}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.freshspread\endcsname{0.394}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.freshvsownse\endcsname{2.36}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.pairsd\endcsname{0.278}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.s0_in_single_seed_sd\endcsname{4.90}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.s0minusbar\endcsname{\ensuremath{+0.297}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.samedefault.fresh\endcsname{\ensuremath{+0.364}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.samedefault.s0\endcsname{\ensuremath{+0.762}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.samedefault.s1\endcsname{\ensuremath{+0.632}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.samedefault.s2\endcsname{\ensuremath{+0.096}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.sedelta\endcsname{0.100}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.seed1\endcsname{88.363}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.seed2\endcsname{87.969}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.sepair\endcsname{0.197}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.threeseeddelta\endcsname{\ensuremath{+0.525}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.threeseedmean\endcsname{88.226}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.vsL3.clause\endcsname{ResEnc-M's fresh mean, 88.166 Dice, is 0.332\,pp above HyReX's 87.833, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.246\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1.vsL3.sentence\endcsname{on AMOS22 fold 0, at 2 fresh seeds per arm, ResEnc-M reads 0.332\,pp above HyReX, 0.66 times the registered 0.50\,pp one-seed pair floor and 2.72 standard errors at the frozen AMOS22 pool seed SD of 0.122\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.allseedsgap.poolmax\endcsname{\ensuremath{-0.034}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.allseedsmax\endcsname{88.127}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.allseedsmin\endcsname{87.839}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.allseedsrange.vspool\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.ci6.hi\endcsname{\ensuremath{+0.554}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.ci6.lo\endcsname{\ensuremath{+0.041}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.clearspairfloor\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.delta_s0\endcsname{\ensuremath{+0.138}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.delta_vscontemp\endcsname{\ensuremath{+0.287}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.delta_vsdefault\endcsname{\ensuremath{+0.298}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.delta_vsrebuild\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.delta_vsrebuild.s1\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.delta_vsrebuild.s2\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.delta_vsrebuild.se\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.delta_vsrebuild.spread\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.delta_vsrebuild.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.delta_vsunion\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.delta_vsunion.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.discoveryseed0\endcsname{87.839}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.fresh_in_se_units\endcsname{2.98}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.fresh_vsL1\endcsname{\ensuremath{-0.167}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.fresh_vsL1.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.fresh_vsL3\endcsname{\ensuremath{+0.165}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.fresh_vsL3.abs\endcsname{0.165}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.fresh_vsL3.dir\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.fresh_vsL3.inscale\endcsname{1.35}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.fresh_vsL3.order\endcsname{the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.fresh_vsL3.relfloor\endcsname{0.33}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.fresh_vsL3.se\endcsname{0.196}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.freshbar\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.freshgap.poolmax\endcsname{\ensuremath{-0.003}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.freshmax\endcsname{88.127}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.freshmean\endcsname{87.999}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.freshmin\endcsname{87.870}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.freshminusbar\endcsname{\ensuremath{-0.052}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.freshminuss0\endcsname{\ensuremath{+0.160}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.freshrange.vspool\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.freshrange.vspool.phrase\endcsname{overlap}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.freshresolution\endcsname{not resolved}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.freshspread\endcsname{0.257}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.freshvsownse\endcsname{2.31}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.pairsd\endcsname{0.182}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.refminusfresh\endcsname{\ensuremath{+0.167}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.refminusfresh.inse\endcsname{0.71}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.refminusfresh.se\endcsname{0.235}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.resolutionbinding\endcsname{the registered primary bar}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.s0_in_single_seed_sd\endcsname{1.05}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.s0minusbar\endcsname{\ensuremath{-0.212}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.samedefault.fresh\endcsname{\ensuremath{+0.197}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.samedefault.s0\endcsname{\ensuremath{+0.253}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.samedefault.s1\endcsname{\ensuremath{+0.397}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.samedefault.s2\endcsname{\ensuremath{-0.003}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.sedelta\endcsname{0.100}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.seed1\endcsname{88.127}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.seed2\endcsname{87.870}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.sepair\endcsname{0.129}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.threeseeddelta\endcsname{\ensuremath{+0.244}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.threeseedmean\endcsname{87.945}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.vsL3.clause\endcsname{ResEnc-matched's fresh mean, 87.999 Dice, is 0.165\,pp above HyReX's 87.833, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.196\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.amos.L1b.vsL3.sentence\endcsname{on AMOS22 fold 0, at 2 fresh seeds per arm, ResEnc-matched reads 0.165\,pp above HyReX, 0.33 times the registered 0.50\,pp one-seed pair floor and 1.35 standard errors at the frozen AMOS22 pool seed SD of 0.122\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.allseedsgap.poolmax\endcsname{\ensuremath{-0.038}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.allseedsmax\endcsname{88.063}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.allseedsmin\endcsname{87.835}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.allseedsrange.vspool\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.ci6.hi\endcsname{\ensuremath{+0.451}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.ci6.lo\endcsname{\ensuremath{-0.062}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.clearspairfloor\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.delta_s0\endcsname{\ensuremath{+0.362}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.delta_vscontemp\endcsname{\ensuremath{+0.184}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.delta_vsdefault\endcsname{\ensuremath{+0.194}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.delta_vsrebuild\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.delta_vsrebuild.s1\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.delta_vsrebuild.s2\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.delta_vsrebuild.se\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.delta_vsrebuild.spread\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.delta_vsrebuild.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.delta_vsunion\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.delta_vsunion.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.discoveryseed0\endcsname{88.063}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.fresh_in_se_units\endcsname{1.95}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.fresh_vsL1\endcsname{\ensuremath{-0.270}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.fresh_vsL1.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.fresh_vsL3\endcsname{\ensuremath{+0.062}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.fresh_vsL3.abs\endcsname{0.062}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.fresh_vsL3.dir\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.fresh_vsL3.inscale\endcsname{0.51}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.fresh_vsL3.order\endcsname{the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.fresh_vsL3.relfloor\endcsname{0.12}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.fresh_vsL3.se\endcsname{0.160}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.freshbar\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.freshgap.poolmax\endcsname{\ensuremath{-0.038}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.freshmax\endcsname{87.956}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.freshmean\endcsname{87.895}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.freshmin\endcsname{87.835}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.freshminusbar\endcsname{\ensuremath{-0.156}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.freshminuss0\endcsname{\ensuremath{-0.168}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.freshrange.vspool\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.freshrange.vspool.phrase\endcsname{overlap}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.freshresolution\endcsname{not resolved}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.freshspread\endcsname{0.121}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.freshvsownse\endcsname{3.21}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.pairsd\endcsname{0.086}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.refminusfresh\endcsname{\ensuremath{+0.270}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.refminusfresh.inse\endcsname{1.31}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.refminusfresh.se\endcsname{0.206}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.resolutionbinding\endcsname{the registered primary bar}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.s0_in_single_seed_sd\endcsname{2.74}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.s0minusbar\endcsname{\ensuremath{+0.012}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.samedefault.fresh\endcsname{\ensuremath{+0.094}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.samedefault.s0\endcsname{\ensuremath{+0.477}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.samedefault.s1\endcsname{\ensuremath{+0.226}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.samedefault.s2\endcsname{\ensuremath{-0.038}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.sedelta\endcsname{0.100}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.seed1\endcsname{87.956}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.seed2\endcsname{87.835}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.sepair\endcsname{0.061}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.threeseeddelta\endcsname{\ensuremath{+0.250}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.threeseedmean\endcsname{87.951}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.vsL3.clause\endcsname{ConvNeXt-k3's fresh mean, 87.895 Dice, is 0.062\,pp above HyReX's 87.833, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.160\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.amos.L2.vsL3.sentence\endcsname{on AMOS22 fold 0, at 2 fresh seeds per arm, ConvNeXt-k3 reads 0.062\,pp above HyReX, 0.12 times the registered 0.50\,pp one-seed pair floor and 0.51 standard errors at the frozen AMOS22 pool seed SD of 0.122\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.allseedsgap.poolmax\endcsname{\ensuremath{-0.188}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.allseedsmax\endcsname{88.083}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.allseedsmin\endcsname{87.686}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.allseedsrange.vspool\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.ci6.hi\endcsname{\ensuremath{+0.389}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.ci6.lo\endcsname{\ensuremath{-0.124}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.clearsownse\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.clearspairfloor\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.delta_s0\endcsname{\ensuremath{+0.382}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.delta_vscontemp\endcsname{\ensuremath{+0.121}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.delta_vsdefault\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.delta_vsrebuild\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.delta_vsrebuild.s1\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.delta_vsrebuild.s2\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.delta_vsrebuild.se\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.delta_vsrebuild.spread\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.delta_vsrebuild.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.delta_vsunion\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.delta_vsunion.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.discoveryseed0\endcsname{88.083}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.fresh_in_se_units\endcsname{1.33}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.fresh_vsL1\endcsname{\ensuremath{-0.332}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.fresh_vsL1.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.freshbar\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.freshgap.poolmax\endcsname{\ensuremath{-0.188}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.freshmax\endcsname{87.981}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.freshmean\endcsname{87.833}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.freshmin\endcsname{87.686}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.freshminusbar\endcsname{\ensuremath{-0.218}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.freshminuss0\endcsname{\ensuremath{-0.249}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.freshrange.vspool\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.freshrange.vspool.phrase\endcsname{overlap}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.freshresolution\endcsname{not resolved}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.freshspread\endcsname{0.296}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.freshvsownse\endcsname{0.90}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.pairsd\endcsname{0.209}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.refminusfresh\endcsname{\ensuremath{+0.332}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.refminusfresh.inse\endcsname{1.35}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.refminusfresh.se\endcsname{0.246}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.resolutionbinding\endcsname{the registered primary bar}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.s0_in_single_seed_sd\endcsname{2.89}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.s0minusbar\endcsname{\ensuremath{+0.032}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.samedefault.fresh\endcsname{\ensuremath{+0.032}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.samedefault.s0\endcsname{\ensuremath{+0.496}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.samedefault.s1\endcsname{\ensuremath{+0.251}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.samedefault.s2\endcsname{\ensuremath{-0.188}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.sedelta\endcsname{0.100}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.seed1\endcsname{87.981}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.seed2\endcsname{87.686}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.sepair\endcsname{0.148}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.threeseeddelta\endcsname{\ensuremath{+0.215}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.threeseedmean\endcsname{87.916}
\expandafter\gdef\csname R@an.fresh_replication.amos.L3.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.allseedsgap.poolmax\endcsname{\ensuremath{+0.180}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.allseedsmax\endcsname{88.258}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.allseedsmin\endcsname{88.053}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.ci6.hi\endcsname{\ensuremath{+0.711}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.ci6.lo\endcsname{\ensuremath{+0.198}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.clearspairfloor\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.delta_s0\endcsname{\ensuremath{+0.430}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.delta_vscontemp\endcsname{\ensuremath{+0.444}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.delta_vsdefault\endcsname{\ensuremath{+0.455}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.delta_vsrebuild\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.delta_vsrebuild.s1\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.delta_vsrebuild.s2\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.delta_vsrebuild.se\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.delta_vsrebuild.spread\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.delta_vsrebuild.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.delta_vsunion\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.delta_vsunion.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.discoveryseed0\endcsname{88.131}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.fresh_in_se_units\endcsname{4.56}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.fresh_vsL1\endcsname{\ensuremath{-0.010}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.fresh_vsL1.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.fresh_vsL3\endcsname{\ensuremath{+0.322}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.fresh_vsL3.abs\endcsname{0.322}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.fresh_vsL3.dir\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.fresh_vsL3.inscale\endcsname{2.64}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.fresh_vsL3.order\endcsname{every fresh run of this arm lies above every HyReX fresh run}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.fresh_vsL3.ordergap\endcsname{0.072}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.fresh_vsL3.relfloor\endcsname{0.64}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.fresh_vsL3.se\endcsname{0.180}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.freshgap.poolmax\endcsname{\ensuremath{+0.180}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.freshmax\endcsname{88.258}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.freshmean\endcsname{88.156}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.freshmin\endcsname{88.053}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.freshminusbar\endcsname{\ensuremath{+0.105}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.freshminuss0\endcsname{\ensuremath{+0.025}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.freshspread\endcsname{0.205}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.freshvsownse\endcsname{4.44}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.pairsd\endcsname{0.145}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.refminusfresh\endcsname{\ensuremath{+0.010}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.refminusfresh.inse\endcsname{0.05}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.refminusfresh.se\endcsname{0.222}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.s0_in_single_seed_sd\endcsname{3.25}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.s0minusbar\endcsname{\ensuremath{+0.080}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.samedefault.fresh\endcsname{\ensuremath{+0.354}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.samedefault.s0\endcsname{\ensuremath{+0.544}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.samedefault.s1\endcsname{\ensuremath{+0.323}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.samedefault.s2\endcsname{\ensuremath{+0.385}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.sedelta\endcsname{0.100}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.seed1\endcsname{88.053}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.seed2\endcsname{88.258}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.sepair\endcsname{0.102}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.threeseeddelta\endcsname{\ensuremath{+0.446}}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.threeseedmean\endcsname{88.147}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.vsL3.clause\endcsname{ResEnc+context's fresh mean, 88.156 Dice, is 0.322\,pp above HyReX's 87.833, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.180\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.amos.L4.vsL3.sentence\endcsname{on AMOS22 fold 0, at 2 fresh seeds per arm, ResEnc+context reads 0.322\,pp above HyReX, 0.64 times the registered 0.50\,pp one-seed pair floor and 2.64 standard errors at the frozen AMOS22 pool seed SD of 0.122\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); every fresh run of ResEnc+context lies above every HyReX fresh run, the smallest gap 0.072\,pp}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.allseedsgap.poolmax\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.allseedsmax\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.allseedsmin\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.allseedsrange.vspool\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.ci6.hi\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.ci6.lo\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.clearsownse\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.clearspairfloor\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.delta_s0\endcsname{\ensuremath{-0.106}}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.delta_vscontemp\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.delta_vscontemp.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.delta_vsdefault\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.delta_vsdefault.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.delta_vsrebuild\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.delta_vsrebuild.s1\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.delta_vsrebuild.s2\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.delta_vsrebuild.se\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.delta_vsrebuild.spread\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.delta_vsrebuild.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.delta_vsunion\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.delta_vsunion.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.discoveryseed0\endcsname{87.595}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.fresh_in_se_units\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.fresh_in_se_units.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.fresh_vsL1\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.fresh_vsL1.dir\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.fresh_vsL1.floor\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.fresh_vsL3\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.fresh_vsL3.abs\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.fresh_vsL3.dir\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.fresh_vsL3.floor\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.fresh_vsL3.inscale\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.fresh_vsL3.order\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.fresh_vsL3.relfloor\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.fresh_vsL3.se\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.fresh_vsL3.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.freshbar\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.freshgap.poolmax\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.freshmax\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.freshmean.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.freshmin\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.freshminusbar\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.freshminuss0\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.freshrange.vspool\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.freshrange.vspool.phrase\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.freshresolution\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.freshspread\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.freshvsownse\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.pairsd\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.refminusfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.refminusfresh.inse\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.refminusfresh.se\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.refminusfresh.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.resolutionbinding\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.s0_in_single_seed_sd\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.s0_in_single_seed_sd.status\endcsname{withheld-pending-fresh}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.s0minusbar\endcsname{\ensuremath{-0.456}}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.samedefault.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.samedefault.s0\endcsname{\ensuremath{+0.009}}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.samedefault.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.samedefault.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.sedelta\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.seed1\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.seed1.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.seed2\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.seed2.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.sepair\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.sepair.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.threeseeddelta\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.threeseedmean\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.threeseedmean.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.vsL3.clause\endcsname{LeanNeXt-s5's fresh pair is pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V7C1.vsL3.sentence\endcsname{LeanNeXt-s5's fresh pair is pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.allseedsgap.poolmax\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.allseedsmax\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.allseedsmin\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.allseedsrange.vspool\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.ci6.hi\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.ci6.lo\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.clearsownse\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.clearspairfloor\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.delta_s0\endcsname{\ensuremath{-0.287}}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.delta_vscontemp\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.delta_vscontemp.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.delta_vsdefault\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.delta_vsdefault.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.delta_vsrebuild\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.delta_vsrebuild.s1\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.delta_vsrebuild.s2\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.delta_vsrebuild.se\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.delta_vsrebuild.spread\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.delta_vsrebuild.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.delta_vsunion\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.delta_vsunion.status\endcsname{not registered}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.discoveryseed0\endcsname{87.414}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.fresh_in_se_units\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.fresh_in_se_units.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.fresh_vsL1\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.fresh_vsL1.dir\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.fresh_vsL1.floor\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.fresh_vsL3\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.fresh_vsL3.abs\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.fresh_vsL3.dir\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.fresh_vsL3.floor\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.fresh_vsL3.inscale\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.fresh_vsL3.order\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.fresh_vsL3.relfloor\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.fresh_vsL3.se\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.fresh_vsL3.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.freshbar\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.freshgap.poolmax\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.freshmax\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.freshmean.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.freshmin\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.freshminusbar\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.freshminuss0\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.freshrange.vspool\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.freshrange.vspool.phrase\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.freshresolution\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.freshspread\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.freshvsownse\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.pairsd\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.refminusfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.refminusfresh.inse\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.refminusfresh.se\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.refminusfresh.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.resolutionbinding\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.s0_in_single_seed_sd\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.s0_in_single_seed_sd.status\endcsname{withheld-pending-fresh}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.s0minusbar\endcsname{\ensuremath{-0.637}}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.samedefault.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.samedefault.s0\endcsname{\ensuremath{-0.173}}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.samedefault.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.samedefault.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.sedelta\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.seed1\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.seed1.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.seed2\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.seed2.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.sepair\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.sepair.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.threeseeddelta\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.threeseedmean\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.threeseedmean.status\endcsname{pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.vsL3.clause\endcsname{Stem1's fresh pair is pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.V8B2.vsL3.sentence\endcsname{Stem1's fresh pair is pending}
\expandafter\gdef\csname R@an.fresh_replication.amos.ci6.half\endcsname{0.257}
\expandafter\gdef\csname R@an.fresh_replication.amos.ci6.tq\endcsname{2.571}
\expandafter\gdef\csname R@an.fresh_replication.amos.contemp.max\endcsname{87.795}
\expandafter\gdef\csname R@an.fresh_replication.amos.contemp.mean\endcsname{87.712}
\expandafter\gdef\csname R@an.fresh_replication.amos.contemp.min\endcsname{87.568}
\expandafter\gdef\csname R@an.fresh_replication.amos.contemp.n\endcsname{3}
\expandafter\gdef\csname R@an.fresh_replication.amos.contemp.nfinished\endcsname{3}
\expandafter\gdef\csname R@an.fresh_replication.amos.contemp.nregistered\endcsname{3}
\expandafter\gdef\csname R@an.fresh_replication.amos.contemp.sd\endcsname{0.125}
\expandafter\gdef\csname R@an.fresh_replication.amos.contemp.shift\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.fresh_replication.amos.contemp.shiftunc\endcsname{\ensuremath{-0.018}}
\expandafter\gdef\csname R@an.fresh_replication.amos.contemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.defaultadj\endcsname{six-run}
\expandafter\gdef\csname R@an.fresh_replication.amos.defaultmean\endcsname{87.701}
\expandafter\gdef\csname R@an.fresh_replication.amos.defaultn\endcsname{6}
\expandafter\gdef\csname R@an.fresh_replication.amos.defaultsd\endcsname{0.122}
\expandafter\gdef\csname R@an.fresh_replication.amos.deltaclause\endcsname{ResEnc-M \ensuremath{+0.465}\,pp (\ensuremath{+0.208} to \ensuremath{+0.721}\,pp), ResEnc+context \ensuremath{+0.455}\,pp (\ensuremath{+0.198} to \ensuremath{+0.711}\,pp), ResEnc-matched \ensuremath{+0.298}\,pp (\ensuremath{+0.041} to \ensuremath{+0.554}\,pp), ConvNeXt-k3 \ensuremath{+0.194}\,pp (\ensuremath{-0.062} to \ensuremath{+0.451}\,pp) and HyReX \ensuremath{+0.132}\,pp (\ensuremath{-0.124} to \ensuremath{+0.389}\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.amos.freshL3minusL1\endcsname{\ensuremath{-0.332}}
\expandafter\gdef\csname R@an.fresh_replication.amos.freshL3minusL1.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.freshabovelist.pool\endcsname{ResEnc-M, ResEnc+context}
\expandafter\gdef\csname R@an.fresh_replication.amos.freshbelowbarlist\endcsname{HyReX, ResEnc-matched, ConvNeXt-k3}
\expandafter\gdef\csname R@an.fresh_replication.amos.freshnotabovelist.pool\endcsname{HyReX, ResEnc-matched, ConvNeXt-k3}
\expandafter\gdef\csname R@an.fresh_replication.amos.freshresolvedlist\endcsname{ResEnc-M, ResEnc+context}
\expandafter\gdef\csname R@an.fresh_replication.amos.freshunresolvedlist\endcsname{HyReX, ResEnc-matched, ConvNeXt-k3}
\expandafter\gdef\csname R@an.fresh_replication.amos.leaderclause\endcsname{the two highest fresh-seed deltas, ResEnc-M \ensuremath{+0.465}\,pp and ResEnc+context \ensuremath{+0.455}\,pp, are 0.010\,pp apart, a margin inside the registered 0.50\,pp one-seed pair floor}
\expandafter\gdef\csname R@an.fresh_replication.amos.leaderclause.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.nbelowref\endcsname{4}
\expandafter\gdef\csname R@an.fresh_replication.amos.ncases\endcsname{40}
\expandafter\gdef\csname R@an.fresh_replication.amos.nfreshabove.pool\endcsname{2}
\expandafter\gdef\csname R@an.fresh_replication.amos.nfreshbelowbar\endcsname{3}
\expandafter\gdef\csname R@an.fresh_replication.amos.nfreshclearsbar\endcsname{2}
\expandafter\gdef\csname R@an.fresh_replication.amos.nfreshnotabove.pool\endcsname{3}
\expandafter\gdef\csname R@an.fresh_replication.amos.nfreshresolved\endcsname{2}
\expandafter\gdef\csname R@an.fresh_replication.amos.nfreshunresolved\endcsname{3}
\expandafter\gdef\csname R@an.fresh_replication.amos.nmoved\endcsname{5}
\expandafter\gdef\csname R@an.fresh_replication.amos.nnotreproduced\endcsname{2}
\expandafter\gdef\csname R@an.fresh_replication.amos.notreproducedlist\endcsname{HyReX, ConvNeXt-k3}
\expandafter\gdef\csname R@an.fresh_replication.amos.npending\endcsname{2}
\expandafter\gdef\csname R@an.fresh_replication.amos.nregistered\endcsname{7}
\expandafter\gdef\csname R@an.fresh_replication.amos.nreplicated\endcsname{5}
\expandafter\gdef\csname R@an.fresh_replication.amos.nshiftinside\endcsname{1}
\expandafter\gdef\csname R@an.fresh_replication.amos.nshiftoutside\endcsname{4}
\expandafter\gdef\csname R@an.fresh_replication.amos.nvshero\endcsname{4}
\expandafter\gdef\csname R@an.fresh_replication.amos.nvsref\endcsname{4}
\expandafter\gdef\csname R@an.fresh_replication.amos.nwithinhero\endcsname{4}
\expandafter\gdef\csname R@an.fresh_replication.amos.pool.max\endcsname{87.873}
\expandafter\gdef\csname R@an.fresh_replication.amos.pool.min\endcsname{87.552}
\expandafter\gdef\csname R@an.fresh_replication.amos.poolspread\endcsname{0.321}
\expandafter\gdef\csname R@an.fresh_replication.amos.referencearm\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.fresh_replication.amos.refrank.clause\endcsname{ResEnc-M has the highest fresh mean of the 5 arms with a complete fresh pair on AMOS22, 0.010\,pp above the next, ResEnc+context}
\expandafter\gdef\csname R@an.fresh_replication.amos.replicated.clause\endcsname{5 of the 7 registered arms have a complete fresh pair}
\expandafter\gdef\csname R@an.fresh_replication.amos.runnerupfresharm\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.fresh_replication.amos.runnerupfreshdelta\endcsname{\ensuremath{+0.455}}
\expandafter\gdef\csname R@an.fresh_replication.amos.samedefaultfreshmean\endcsname{87.802}
\expandafter\gdef\csname R@an.fresh_replication.amos.samedefaultgap\endcsname{\ensuremath{-0.101}}
\expandafter\gdef\csname R@an.fresh_replication.amos.samedefaultgap.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.samedefaultn\endcsname{3}
\expandafter\gdef\csname R@an.fresh_replication.amos.samedefaultsource\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.fresh_replication.amos.sddf\endcsname{5}
\expandafter\gdef\csname R@an.fresh_replication.amos.sdfresh\endcsname{0.100}
\expandafter\gdef\csname R@an.fresh_replication.amos.sdfreshpair\endcsname{0.122}
\expandafter\gdef\csname R@an.fresh_replication.amos.sdshift\endcsname{0.150}
\expandafter\gdef\csname R@an.fresh_replication.amos.sdsingle\endcsname{0.132}
\expandafter\gdef\csname R@an.fresh_replication.amos.shiftinsidelist\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.fresh_replication.amos.shiftoutsidelist\endcsname{HyReX, ResEnc-M, ResEnc-matched, ConvNeXt-k3}
\expandafter\gdef\csname R@an.fresh_replication.amos.topfresh.licence\endcsname{an ordering, not a resolved superlative}
\expandafter\gdef\csname R@an.fresh_replication.amos.topfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.amos.topfresharm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.fresh_replication.amos.topfreshdelta\endcsname{\ensuremath{+0.465}}
\expandafter\gdef\csname R@an.fresh_replication.amos.topfreshmargin\endcsname{0.010}
\expandafter\gdef\csname R@an.fresh_replication.amos.topfreshmargin.binding\endcsname{the registered one-seed pair floor}
\expandafter\gdef\csname R@an.fresh_replication.amos.topfreshmargin.inse\endcsname{0.05}
\expandafter\gdef\csname R@an.fresh_replication.amos.topfreshmargin.se\endcsname{0.222}
\expandafter\gdef\csname R@an.fresh_replication.amos.union.mean\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.union.n\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.amos.withinhero.clause\endcsname{of the 4 other arms with a complete fresh pair, all lie inside the registered 0.50\,pp one-seed pair floor of HyReX's fresh mean: ResEnc-M, ResEnc-matched, ConvNeXt-k3, ResEnc+context}
\expandafter\gdef\csname R@an.fresh_replication.amos.withinherolist\endcsname{ResEnc-M, ResEnc-matched, ConvNeXt-k3, ResEnc+context}
\expandafter\gdef\csname R@an.fresh_replication.freshunresolvedlist\endcsname{ConvNeXt-k3 (KiTS23), HyReX (AMOS22), ResEnc-matched (AMOS22), ConvNeXt-k3 (AMOS22)}
\expandafter\gdef\csname R@an.fresh_replication.guard.L1.delta\endcsname{\ensuremath{+0.336}}
\expandafter\gdef\csname R@an.fresh_replication.guard.L1.dice\endcsname{92.345}
\expandafter\gdef\csname R@an.fresh_replication.guard.L1.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.guard.L1b.delta\endcsname{\ensuremath{+0.283}}
\expandafter\gdef\csname R@an.fresh_replication.guard.L1b.dice\endcsname{92.293}
\expandafter\gdef\csname R@an.fresh_replication.guard.L1b.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.guard.L2.delta\endcsname{\ensuremath{-0.015}}
\expandafter\gdef\csname R@an.fresh_replication.guard.L2.dice\endcsname{91.995}
\expandafter\gdef\csname R@an.fresh_replication.guard.L2.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.guard.L3.delta\endcsname{\ensuremath{+0.616}}
\expandafter\gdef\csname R@an.fresh_replication.guard.L3.dice\endcsname{92.626}
\expandafter\gdef\csname R@an.fresh_replication.guard.L3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.guard.L4.delta\endcsname{\ensuremath{+0.315}}
\expandafter\gdef\csname R@an.fresh_replication.guard.L4.dice\endcsname{92.325}
\expandafter\gdef\csname R@an.fresh_replication.guard.L4.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.guard.L6.delta\endcsname{\ensuremath{+0.451}}
\expandafter\gdef\csname R@an.fresh_replication.guard.L6.dice\endcsname{92.461}
\expandafter\gdef\csname R@an.fresh_replication.guard.L6.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.guard.P3c.delta\endcsname{\ensuremath{-0.013}}
\expandafter\gdef\csname R@an.fresh_replication.guard.P3c.dice\endcsname{91.997}
\expandafter\gdef\csname R@an.fresh_replication.guard.P3c.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.guard.V5B2.delta\endcsname{\ensuremath{-0.181}}
\expandafter\gdef\csname R@an.fresh_replication.guard.V5B2.dice\endcsname{91.828}
\expandafter\gdef\csname R@an.fresh_replication.guard.V5B2.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.guard.V6A1r.delta\endcsname{\ensuremath{+0.573}}
\expandafter\gdef\csname R@an.fresh_replication.guard.V6A1r.dice\endcsname{92.582}
\expandafter\gdef\csname R@an.fresh_replication.guard.V6A1r.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.guard.V7A1.delta\endcsname{\ensuremath{+0.229}}
\expandafter\gdef\csname R@an.fresh_replication.guard.V7A1.dice\endcsname{92.238}
\expandafter\gdef\csname R@an.fresh_replication.guard.V7A1.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.guard.V7A2.delta\endcsname{\ensuremath{+0.362}}
\expandafter\gdef\csname R@an.fresh_replication.guard.V7A2.dice\endcsname{92.371}
\expandafter\gdef\csname R@an.fresh_replication.guard.V7A2.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.guard.V7C1.delta\endcsname{\ensuremath{-0.252}}
\expandafter\gdef\csname R@an.fresh_replication.guard.V7C1.dice\endcsname{91.757}
\expandafter\gdef\csname R@an.fresh_replication.guard.V7C1.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.guard.dataset\endcsname{ACDC}
\expandafter\gdef\csname R@an.fresh_replication.guard.estimand\endcsname{the discovery seed (seed 0) of each arm}
\expandafter\gdef\csname R@an.fresh_replication.guard.nabovethreshold\endcsname{10}
\expandafter\gdef\csname R@an.fresh_replication.guard.narms\endcsname{12}
\expandafter\gdef\csname R@an.fresh_replication.guard.nfreshdone\endcsname{2}
\expandafter\gdef\csname R@an.fresh_replication.guard.nfreshregistered\endcsname{2}
\expandafter\gdef\csname R@an.fresh_replication.guard.orderclause\endcsname{at the discovery seed (seed 0) of each arm, the two highest deltas, HyReX \ensuremath{+0.616}\,pp and HyReX-k9 \ensuremath{+0.573}\,pp, are 0.043\,pp apart, a one-seed pair difference inside the registered 0.50\,pp pair floor; 10 of the 12 arms clear the registered \ensuremath{-0.15}\,pp guard threshold}
\expandafter\gdef\csname R@an.fresh_replication.guard.pooldf\endcsname{5}
\expandafter\gdef\csname R@an.fresh_replication.guard.poolmean\endcsname{92.009}
\expandafter\gdef\csname R@an.fresh_replication.guard.pooln\endcsname{6}
\expandafter\gdef\csname R@an.fresh_replication.guard.poolsd\endcsname{0.099}
\expandafter\gdef\csname R@an.fresh_replication.guard.runneruparm\endcsname{HyReX-k9}
\expandafter\gdef\csname R@an.fresh_replication.guard.runnerupdelta\endcsname{\ensuremath{+0.573}}
\expandafter\gdef\csname R@an.fresh_replication.guard.threshold\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.fresh_replication.guard.toparm\endcsname{HyReX}
\expandafter\gdef\csname R@an.fresh_replication.guard.topdelta\endcsname{\ensuremath{+0.616}}
\expandafter\gdef\csname R@an.fresh_replication.guard.topfresh.licence\endcsname{an ordering, not a resolved superlative}
\expandafter\gdef\csname R@an.fresh_replication.guard.topmargin\endcsname{0.043}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.allseedsgap.poolmax\endcsname{\ensuremath{+1.234}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.allseedsmax\endcsname{86.885}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.allseedsmin\endcsname{85.506}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.ci3.hi\endcsname{\ensuremath{+5.523}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.ci3.lo\endcsname{\ensuremath{-0.721}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.ci6.hi\endcsname{\ensuremath{+3.673}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.ci6.lo\endcsname{\ensuremath{+0.641}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.delta_s0\endcsname{\ensuremath{+3.507}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.delta_s0_vsunion\endcsname{\ensuremath{+3.264}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.delta_vscontemp\endcsname{\ensuremath{+1.914}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.delta_vsdefault\endcsname{\ensuremath{+2.401}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.delta_vsrebuild\endcsname{\ensuremath{+1.225}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.delta_vsrebuild.s1\endcsname{\ensuremath{+0.977}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.delta_vsrebuild.s2\endcsname{\ensuremath{+1.473}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.delta_vsrebuild.se\endcsname{0.274}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.delta_vsrebuild.spread\endcsname{0.496}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.delta_vsunion\endcsname{\ensuremath{+2.157}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.discoveryseed0\endcsname{86.885}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.fresh_in_se_units\endcsname{3.31}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.fresh_in_se_units_union\endcsname{3.66}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.fresh_vsL1\endcsname{\ensuremath{-1.074}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.fresh_vsL3\endcsname{\ensuremath{+0.307}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.fresh_vsL3.abs\endcsname{0.307}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.fresh_vsL3.dir\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.fresh_vsL3.inscale\endcsname{0.39}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.fresh_vsL3.order\endcsname{the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.fresh_vsL3.relfloor\endcsname{0.61}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.fresh_vsL3.se\endcsname{0.403}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.freshgap.poolmax\endcsname{\ensuremath{+1.234}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.freshgap.unionmax\endcsname{\ensuremath{+0.886}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.freshmax\endcsname{86.052}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.freshmean\endcsname{85.779}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.freshmin\endcsname{85.506}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.freshminusbar\endcsname{\ensuremath{+2.051}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.freshminuss0\endcsname{\ensuremath{-1.106}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.freshrange.vsunion\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.freshspread\endcsname{0.546}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.freshvsownse\endcsname{8.79}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.pairsd\endcsname{0.386}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.refminusfresh\endcsname{\ensuremath{+1.074}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.refminusfresh.inse\endcsname{2.46}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.refminusfresh.se\endcsname{0.437}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.s0_in_single_seed_sd\endcsname{3.82}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.s0minusbar\endcsname{\ensuremath{+3.157}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.samedefault.fresh\endcsname{\ensuremath{+2.848}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.samedefault.s0\endcsname{\ensuremath{+2.614}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.samedefault.s1\endcsname{\ensuremath{+2.393}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.samedefault.s2\endcsname{\ensuremath{+3.303}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.seed1\endcsname{85.506}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.seed2\endcsname{86.052}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.sepair\endcsname{0.273}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.threeseeddelta\endcsname{\ensuremath{+2.770}}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.threeseedmean\endcsname{86.148}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.vsL3.clause\endcsname{HyReX+dec. capacity's fresh mean, 85.779 Dice, is 0.307\,pp above HyReX's 85.472, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.403\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.C1.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, HyReX+dec. capacity reads 0.307\,pp above HyReX, 0.61 times the registered 0.50\,pp one-seed pair floor and 0.39 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.allseedsgap.poolmax\endcsname{\ensuremath{+0.301}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.allseedsmax\endcsname{85.137}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.allseedsmin\endcsname{84.572}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.ci3.hi\endcsname{\ensuremath{+4.599}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.ci3.lo\endcsname{\ensuremath{-1.645}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.ci6.hi\endcsname{\ensuremath{+2.749}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.ci6.lo\endcsname{\ensuremath{-0.283}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.delta_s0\endcsname{\ensuremath{+1.607}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.delta_s0_vsunion\endcsname{\ensuremath{+1.363}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.delta_vscontemp\endcsname{\ensuremath{+0.989}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.delta_vsdefault\endcsname{\ensuremath{+1.477}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.delta_vsrebuild\endcsname{\ensuremath{+0.301}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.delta_vsrebuild.s1\endcsname{\ensuremath{+0.608}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.delta_vsrebuild.s2\endcsname{\ensuremath{-0.007}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.delta_vsrebuild.se\endcsname{0.284}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.delta_vsrebuild.spread\endcsname{0.615}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.delta_vsunion\endcsname{\ensuremath{+1.233}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.discoveryseed0\endcsname{84.985}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.fresh_in_se_units\endcsname{2.03}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.fresh_in_se_units_union\endcsname{2.09}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.fresh_vsL1\endcsname{\ensuremath{-1.999}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.fresh_vsL3\endcsname{\ensuremath{-0.617}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.fresh_vsL3.abs\endcsname{0.617}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.fresh_vsL3.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.fresh_vsL3.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.fresh_vsL3.inscale\endcsname{0.78}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.fresh_vsL3.order\endcsname{every HyReX fresh run lies above every fresh run of this arm}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.fresh_vsL3.ordergap\endcsname{0.038}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.fresh_vsL3.relfloor\endcsname{1.23}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.fresh_vsL3.se\endcsname{0.409}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.freshgap.poolmax\endcsname{\ensuremath{+0.301}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.freshgap.unionmax\endcsname{\ensuremath{-0.048}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.freshmax\endcsname{85.137}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.freshmean\endcsname{84.855}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.freshmin\endcsname{84.572}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.freshminusbar\endcsname{\ensuremath{+1.127}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.freshminuss0\endcsname{\ensuremath{-0.131}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.freshrange.vsunion\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.freshspread\endcsname{0.565}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.freshvsownse\endcsname{5.22}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.pairsd\endcsname{0.400}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.refminusfresh\endcsname{\ensuremath{+1.999}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.refminusfresh.inse\endcsname{4.51}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.refminusfresh.se\endcsname{0.443}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.s0_in_single_seed_sd\endcsname{1.75}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.s0minusbar\endcsname{\ensuremath{+1.257}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.samedefault.fresh\endcsname{\ensuremath{+1.923}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.samedefault.s0\endcsname{\ensuremath{+0.714}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.samedefault.s1\endcsname{\ensuremath{+2.024}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.samedefault.s2\endcsname{\ensuremath{+1.823}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.seed1\endcsname{85.137}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.seed2\endcsname{84.572}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.sepair\endcsname{0.283}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.threeseeddelta\endcsname{\ensuremath{+1.520}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.threeseedmean\endcsname{84.898}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.vsL3.clause\endcsname{HyReX point-fuse's fresh mean, 84.855 Dice, is 0.617\,pp below HyReX's 85.472, a difference beyond the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.409\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.D1.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, HyReX point-fuse reads 0.617\,pp below HyReX, 1.23 times the registered 0.50\,pp one-seed pair floor and 0.78 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); every HyReX fresh run lies above every fresh run of HyReX point-fuse, the smallest gap 0.038\,pp}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.allseedsgap.poolmax\endcsname{\ensuremath{+0.911}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.allseedsmax\endcsname{85.734}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.allseedsmin\endcsname{85.182}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.attrib.clause\endcsname{a default-topology network with a thinned decoder and no new operator reaches a KiTS23 fresh gain of \ensuremath{+1.892}\,pp (\ensuremath{+1.648}\,pp against the six-run reference), within 0.202\,pp of HyReX's \ensuremath{+2.094}\,pp (\ensuremath{+1.850}\,pp against the six-run reference), so the KiTS23 gain does not identify the operator assignment as its source}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.ci3.hi\endcsname{\ensuremath{+5.014}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.ci3.lo\endcsname{\ensuremath{-1.230}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.ci6.hi\endcsname{\ensuremath{+3.164}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.ci6.lo\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.delta_s0\endcsname{\ensuremath{+2.355}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.delta_s0_vsunion\endcsname{\ensuremath{+2.112}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.delta_vscontemp\endcsname{\ensuremath{+1.404}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.delta_vsdefault\endcsname{\ensuremath{+1.892}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.delta_vsrebuild\endcsname{\ensuremath{+0.716}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.delta_vsrebuild.s1\endcsname{\ensuremath{+0.828}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.delta_vsrebuild.s2\endcsname{\ensuremath{+0.603}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.delta_vsrebuild.se\endcsname{0.091}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.delta_vsrebuild.spread\endcsname{0.225}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.delta_vsunion\endcsname{\ensuremath{+1.648}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.discoveryseed0\endcsname{85.734}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.fresh_in_se_units\endcsname{2.61}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.fresh_in_se_units_union\endcsname{2.79}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.fresh_vsL1\endcsname{\ensuremath{-1.584}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.fresh_vsL3\endcsname{\ensuremath{-0.202}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.fresh_vsL3.abs\endcsname{0.202}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.fresh_vsL3.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.fresh_vsL3.inscale\endcsname{0.25}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.fresh_vsL3.order\endcsname{the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.fresh_vsL3.relfloor\endcsname{0.40}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.fresh_vsL3.se\endcsname{0.309}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.freshgap.poolmax\endcsname{\ensuremath{+0.911}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.freshgap.unionmax\endcsname{\ensuremath{+0.562}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.freshmax\endcsname{85.357}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.freshmean\endcsname{85.270}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.freshmin\endcsname{85.182}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.freshminusbar\endcsname{\ensuremath{+1.542}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.freshminuss0\endcsname{\ensuremath{-0.464}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.freshrange.vsunion\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.freshspread\endcsname{0.175}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.freshvsownse\endcsname{21.60}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.pairsd\endcsname{0.124}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.refminusfresh\endcsname{\ensuremath{+1.584}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.refminusfresh.inse\endcsname{4.49}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.refminusfresh.se\endcsname{0.353}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.s0_in_single_seed_sd\endcsname{2.57}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.s0minusbar\endcsname{\ensuremath{+2.005}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.samedefault.fresh\endcsname{\ensuremath{+2.338}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.samedefault.s0\endcsname{\ensuremath{+1.462}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.samedefault.s1\endcsname{\ensuremath{+2.244}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.samedefault.s2\endcsname{\ensuremath{+2.433}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.seed1\endcsname{85.357}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.seed2\endcsname{85.182}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.sepair\endcsname{0.088}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.threeseeddelta\endcsname{\ensuremath{+2.046}}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.threeseedmean\endcsname{85.424}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.vsL3.clause\endcsname{LeanDec's fresh mean, 85.270 Dice, is 0.202\,pp below HyReX's 85.472, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.309\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.D2.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, LeanDec reads 0.202\,pp below HyReX, 0.40 times the registered 0.50\,pp one-seed pair floor and 0.25 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.allseedsgap.poolmax\endcsname{\ensuremath{+1.433}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.allseedsmax\endcsname{87.195}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.allseedsmin\endcsname{85.704}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.ci3.hi\endcsname{\ensuremath{+6.597}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.ci3.lo\endcsname{\ensuremath{+0.353}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.ci6.hi\endcsname{\ensuremath{+4.747}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.ci6.lo\endcsname{\ensuremath{+1.716}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.delta_s0\endcsname{\ensuremath{+2.326}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.delta_s0_vsunion\endcsname{\ensuremath{+2.082}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.delta_vscontemp\endcsname{\ensuremath{+2.988}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.delta_vsdefault\endcsname{\ensuremath{+3.475}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.delta_vsrebuild\endcsname{\ensuremath{+2.300}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.delta_vsrebuild.s1\endcsname{\ensuremath{+1.983}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.delta_vsrebuild.s2\endcsname{\ensuremath{+2.616}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.delta_vsrebuild.se\endcsname{0.342}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.delta_vsrebuild.spread\endcsname{0.633}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.delta_vsunion\endcsname{\ensuremath{+3.232}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.discoveryseed0\endcsname{85.704}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.fresh_in_se_units\endcsname{4.79}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.fresh_in_se_units_union\endcsname{5.48}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.fresh_vsL3\endcsname{\ensuremath{+1.382}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.fresh_vsL3.abs\endcsname{1.382}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.fresh_vsL3.dir\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.fresh_vsL3.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.fresh_vsL3.inscale\endcsname{1.74}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.fresh_vsL3.order\endcsname{every fresh run of this arm lies above every HyReX fresh run}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.fresh_vsL3.ordergap\endcsname{0.744}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.fresh_vsL3.relfloor\endcsname{2.76}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.fresh_vsL3.se\endcsname{0.452}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.freshgap.poolmax\endcsname{\ensuremath{+2.240}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.freshgap.unionmax\endcsname{\ensuremath{+1.891}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.freshmax\endcsname{87.195}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.freshmean\endcsname{86.853}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.freshmin\endcsname{86.512}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.freshminusbar\endcsname{\ensuremath{+3.125}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.freshminuss0\endcsname{\ensuremath{+1.149}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.freshrange.vsunion\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.freshspread\endcsname{0.683}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.freshvsownse\endcsname{10.17}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.pairsd\endcsname{0.483}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.pubdeficit.fresh\endcsname{\ensuremath{-1.057}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.pubdeficit3\endcsname{\ensuremath{-1.440}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.pubmargin.fresh\endcsname{\ensuremath{+1.815}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.pubmargin.fresh.nse\endcsname{2.50}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.s0_in_single_seed_sd\endcsname{2.53}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.s0minusbar\endcsname{\ensuremath{+1.976}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.samedefault.fresh\endcsname{\ensuremath{+3.922}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.samedefault.s0\endcsname{\ensuremath{+1.433}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.samedefault.s1\endcsname{\ensuremath{+3.398}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.samedefault.s2\endcsname{\ensuremath{+4.446}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.seed1\endcsname{86.512}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.seed2\endcsname{87.195}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.sepair\endcsname{0.342}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.threeseeddelta\endcsname{\ensuremath{+3.092}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.threeseedmean\endcsname{86.470}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.vsL3.clause\endcsname{ResEnc-M's fresh mean, 86.853 Dice, is 1.382\,pp above HyReX's 85.472, a difference beyond the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.452\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, ResEnc-M reads 1.382\,pp above HyReX, 2.76 times the registered 0.50\,pp one-seed pair floor and 1.74 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); every fresh run of ResEnc-M lies above every HyReX fresh run, the smallest gap 0.744\,pp}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.allseedsgap.poolmax\endcsname{\ensuremath{+0.849}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.allseedsmax\endcsname{85.942}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.allseedsmin\endcsname{85.121}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.ci3.hi\endcsname{\ensuremath{+5.435}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.ci3.lo\endcsname{\ensuremath{-0.809}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.ci6.hi\endcsname{\ensuremath{+3.585}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.ci6.lo\endcsname{\ensuremath{+0.554}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.delta_s0\endcsname{\ensuremath{+1.743}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.delta_s0_vsunion\endcsname{\ensuremath{+1.499}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.delta_vscontemp\endcsname{\ensuremath{+1.826}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.delta_vsdefault\endcsname{\ensuremath{+2.313}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.delta_vsrebuild\endcsname{\ensuremath{+1.137}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.delta_vsrebuild.s1\endcsname{\ensuremath{+1.413}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.delta_vsrebuild.s2\endcsname{\ensuremath{+0.862}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.delta_vsrebuild.se\endcsname{0.252}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.delta_vsrebuild.spread\endcsname{0.551}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.delta_vsunion\endcsname{\ensuremath{+2.070}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.discoveryseed0\endcsname{85.121}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.fresh_in_se_units\endcsname{3.19}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.fresh_in_se_units_union\endcsname{3.51}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.fresh_vsL1\endcsname{\ensuremath{-1.162}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.fresh_vsL3\endcsname{\ensuremath{+0.220}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.fresh_vsL3.abs\endcsname{0.220}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.fresh_vsL3.dir\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.fresh_vsL3.inscale\endcsname{0.28}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.fresh_vsL3.order\endcsname{the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.fresh_vsL3.relfloor\endcsname{0.44}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.fresh_vsL3.se\endcsname{0.388}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.freshgap.poolmax\endcsname{\ensuremath{+1.169}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.freshgap.unionmax\endcsname{\ensuremath{+0.820}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.freshmax\endcsname{85.942}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.freshmean\endcsname{85.691}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.freshmin\endcsname{85.441}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.freshminusbar\endcsname{\ensuremath{+1.963}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.freshminuss0\endcsname{\ensuremath{+0.571}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.freshrange.vsunion\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.freshspread\endcsname{0.501}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.freshvsownse\endcsname{9.23}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.pairsd\endcsname{0.355}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.refminusfresh\endcsname{\ensuremath{+1.162}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.refminusfresh.inse\endcsname{2.74}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.refminusfresh.se\endcsname{0.424}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.s0_in_single_seed_sd\endcsname{1.90}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.s0minusbar\endcsname{\ensuremath{+1.393}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.samedefault.fresh\endcsname{\ensuremath{+2.760}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.samedefault.s0\endcsname{\ensuremath{+0.849}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.samedefault.s1\endcsname{\ensuremath{+2.829}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.samedefault.s2\endcsname{\ensuremath{+2.691}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.seed1\endcsname{85.942}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.seed2\endcsname{85.441}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.sepair\endcsname{0.251}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.threeseeddelta\endcsname{\ensuremath{+2.123}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.threeseedmean\endcsname{85.501}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.vsL3.clause\endcsname{ResEnc-matched's fresh mean, 85.691 Dice, is 0.220\,pp above HyReX's 85.472, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.388\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.L1b.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, ResEnc-matched reads 0.220\,pp above HyReX, 0.44 times the registered 0.50\,pp one-seed pair floor and 0.28 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.allseedsgap.poolmax\endcsname{\ensuremath{-1.699}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.allseedsmax\endcsname{84.404}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.allseedsmin\endcsname{82.573}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.allseedsrange.vspool\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.ci3.hi\endcsname{\ensuremath{+3.232}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.ci3.lo\endcsname{\ensuremath{-3.012}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.ci6.hi\endcsname{\ensuremath{+1.382}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.ci6.lo\endcsname{\ensuremath{-1.649}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.clearsownse\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.clearspairfloor\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.delta_s0\endcsname{\ensuremath{+0.664}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.delta_s0_vsunion\endcsname{\ensuremath{+0.420}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.delta_vscontemp\endcsname{\ensuremath{-0.377}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.delta_vsdefault\endcsname{\ensuremath{+0.110}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.delta_vsrebuild\endcsname{\ensuremath{-1.065}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.delta_vsrebuild.s1\endcsname{\ensuremath{-1.956}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.delta_vsrebuild.s2\endcsname{\ensuremath{-0.175}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.delta_vsrebuild.se\endcsname{0.916}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.delta_vsrebuild.spread\endcsname{1.781}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.delta_vsunion\endcsname{\ensuremath{-0.133}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.discoveryseed0\endcsname{84.042}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.fresh_in_se_units\endcsname{0.15}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.fresh_in_se_units_union\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.fresh_vsL1\endcsname{\ensuremath{-3.365}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.fresh_vsL3\endcsname{\ensuremath{-1.983}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.fresh_vsL3.abs\endcsname{1.983}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.fresh_vsL3.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.fresh_vsL3.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.fresh_vsL3.inscale\endcsname{2.50}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.fresh_vsL3.order\endcsname{every HyReX fresh run lies above every fresh run of this arm}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.fresh_vsL3.ordergap\endcsname{0.772}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.fresh_vsL3.relfloor\endcsname{3.97}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.fresh_vsL3.se\endcsname{0.962}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.freshbar\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.freshbar_vsunion\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.freshgap.poolmax\endcsname{\ensuremath{-1.699}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.freshgap.unionmax\endcsname{\ensuremath{-2.047}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.freshmax\endcsname{84.404}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.freshmean\endcsname{83.489}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.freshmin\endcsname{82.573}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.freshminusbar\endcsname{\ensuremath{-0.240}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.freshminuss0\endcsname{\ensuremath{-0.554}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.freshrange.vspool\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.freshrange.vspool.phrase\endcsname{overlap}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.freshrange.vsunion\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.freshresolution\endcsname{not resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.freshspread\endcsname{1.831}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.freshvsownse\endcsname{0.12}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.pairsd\endcsname{1.295}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.refminusfresh\endcsname{\ensuremath{+3.365}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.refminusfresh.inse\endcsname{3.44}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.refminusfresh.se\endcsname{0.977}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.resolutionbinding\endcsname{the registered primary bar}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.s0_in_single_seed_sd\endcsname{0.72}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.s0minusbar\endcsname{\ensuremath{+0.314}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.samedefault.fresh\endcsname{\ensuremath{+0.557}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.samedefault.s0\endcsname{\ensuremath{-0.230}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.samedefault.s1\endcsname{\ensuremath{-0.540}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.samedefault.s2\endcsname{\ensuremath{+1.654}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.seed1\endcsname{82.573}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.seed2\endcsname{84.404}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.sepair\endcsname{0.915}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.threeseeddelta\endcsname{\ensuremath{+0.295}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.threeseedmean\endcsname{83.673}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.vsL3.clause\endcsname{ConvNeXt-k3's fresh mean, 83.489 Dice, is 1.983\,pp below HyReX's 85.472, a difference beyond the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.962\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.L2.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, ConvNeXt-k3 reads 1.983\,pp below HyReX, 3.97 times the registered 0.50\,pp one-seed pair floor and 2.50 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); every HyReX fresh run lies above every fresh run of ConvNeXt-k3, the smallest gap 0.772\,pp}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.allseedsgap.poolmax\endcsname{\ensuremath{+0.904}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.allseedsmax\endcsname{86.220}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.allseedsmin\endcsname{85.176}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.ci3.hi\endcsname{\ensuremath{+5.216}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.ci3.lo\endcsname{\ensuremath{-1.028}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.ci6.hi\endcsname{\ensuremath{+3.366}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.ci6.lo\endcsname{\ensuremath{+0.334}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.delta_s0\endcsname{\ensuremath{+2.842}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.delta_s0_vsunion\endcsname{\ensuremath{+2.598}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.delta_vscontemp\endcsname{\ensuremath{+1.606}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.delta_vsdefault\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.delta_vsrebuild\endcsname{\ensuremath{+0.918}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.delta_vsrebuild.s1\endcsname{\ensuremath{+0.647}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.delta_vsrebuild.s2\endcsname{\ensuremath{+1.189}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.delta_vsrebuild.se\endcsname{0.297}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.delta_vsrebuild.spread\endcsname{0.542}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.delta_vsunion\endcsname{\ensuremath{+1.850}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.discoveryseed0\endcsname{86.220}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.fresh_in_se_units\endcsname{2.89}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.fresh_in_se_units_union\endcsname{3.14}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.fresh_vsL1\endcsname{\ensuremath{-1.382}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.freshgap.poolmax\endcsname{\ensuremath{+0.904}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.freshgap.unionmax\endcsname{\ensuremath{+0.555}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.freshmax\endcsname{85.768}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.freshmean\endcsname{85.472}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.freshmin\endcsname{85.176}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.freshminusbar\endcsname{\ensuremath{+1.744}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.freshminuss0\endcsname{\ensuremath{-0.748}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.freshrange.vsunion\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.freshspread\endcsname{0.592}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.freshvsownse\endcsname{7.07}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.pairsd\endcsname{0.419}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.refminusfresh\endcsname{\ensuremath{+1.382}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.refminusfresh.inse\endcsname{3.06}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.refminusfresh.se\endcsname{0.452}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.s0_in_single_seed_sd\endcsname{3.10}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.s0minusbar\endcsname{\ensuremath{+2.492}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.samedefault.fresh\endcsname{\ensuremath{+2.540}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.samedefault.s0\endcsname{\ensuremath{+1.948}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.samedefault.s1\endcsname{\ensuremath{+2.062}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.samedefault.s2\endcsname{\ensuremath{+3.018}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.seed1\endcsname{85.176}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.seed2\endcsname{85.768}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.sepair\endcsname{0.296}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.threeseeddelta\endcsname{\ensuremath{+2.343}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.threeseedmean\endcsname{85.721}
\expandafter\gdef\csname R@an.fresh_replication.kits.L3.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.allseedsgap.poolmax\endcsname{\ensuremath{+0.922}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.allseedsmax\endcsname{86.055}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.allseedsmin\endcsname{85.194}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.ci3.hi\endcsname{\ensuremath{+5.368}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.ci3.lo\endcsname{\ensuremath{-0.876}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.ci6.hi\endcsname{\ensuremath{+3.518}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.ci6.lo\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.delta_s0\endcsname{\ensuremath{+2.198}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.delta_s0_vsunion\endcsname{\ensuremath{+1.954}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.delta_vscontemp\endcsname{\ensuremath{+1.759}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.delta_vsdefault\endcsname{\ensuremath{+2.246}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.delta_vsrebuild\endcsname{\ensuremath{+1.071}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.delta_vsrebuild.s1\endcsname{\ensuremath{+1.526}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.delta_vsrebuild.s2\endcsname{\ensuremath{+0.615}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.delta_vsrebuild.se\endcsname{0.432}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.delta_vsrebuild.spread\endcsname{0.912}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.delta_vsunion\endcsname{\ensuremath{+2.003}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.discoveryseed0\endcsname{85.576}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.fresh_in_se_units\endcsname{3.10}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.fresh_in_se_units_union\endcsname{3.40}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.fresh_vsL1\endcsname{\ensuremath{-1.229}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.fresh_vsL3\endcsname{\ensuremath{+0.153}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.fresh_vsL3.abs\endcsname{0.153}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.fresh_vsL3.dir\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.fresh_vsL3.inscale\endcsname{0.19}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.fresh_vsL3.order\endcsname{the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.fresh_vsL3.relfloor\endcsname{0.31}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.fresh_vsL3.se\endcsname{0.523}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.freshgap.poolmax\endcsname{\ensuremath{+0.922}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.freshgap.unionmax\endcsname{\ensuremath{+0.573}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.freshmax\endcsname{86.055}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.freshmean\endcsname{85.625}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.freshmin\endcsname{85.194}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.freshminusbar\endcsname{\ensuremath{+1.896}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.freshminuss0\endcsname{\ensuremath{+0.048}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.freshrange.vsunion\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.freshspread\endcsname{0.862}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.freshvsownse\endcsname{5.21}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.pairsd\endcsname{0.609}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.refminusfresh\endcsname{\ensuremath{+1.229}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.refminusfresh.inse\endcsname{2.24}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.refminusfresh.se\endcsname{0.550}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.s0_in_single_seed_sd\endcsname{2.39}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.s0minusbar\endcsname{\ensuremath{+1.848}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.samedefault.fresh\endcsname{\ensuremath{+2.693}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.samedefault.s0\endcsname{\ensuremath{+1.305}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.samedefault.s1\endcsname{\ensuremath{+2.942}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.samedefault.s2\endcsname{\ensuremath{+2.444}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.seed1\endcsname{86.055}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.seed2\endcsname{85.194}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.sepair\endcsname{0.431}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.threeseeddelta\endcsname{\ensuremath{+2.230}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.threeseedmean\endcsname{85.608}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.vsL3.clause\endcsname{ResEnc+context's fresh mean, 85.625 Dice, is 0.153\,pp above HyReX's 85.472, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.523\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.L4.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, ResEnc+context reads 0.153\,pp above HyReX, 0.31 times the registered 0.50\,pp one-seed pair floor and 0.19 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.allseedsgap.poolmax\endcsname{\ensuremath{+0.305}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.allseedsmax\endcsname{85.904}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.allseedsmin\endcsname{84.577}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.ci3.hi\endcsname{\ensuremath{+4.713}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.ci3.lo\endcsname{\ensuremath{-1.531}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.ci6.hi\endcsname{\ensuremath{+2.864}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.ci6.lo\endcsname{\ensuremath{-0.168}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.delta_s0\endcsname{\ensuremath{+2.526}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.delta_s0_vsunion\endcsname{\ensuremath{+2.283}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.delta_vscontemp\endcsname{\ensuremath{+1.104}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.delta_vsdefault\endcsname{\ensuremath{+1.591}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.delta_vsrebuild\endcsname{\ensuremath{+0.416}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.delta_vsrebuild.s1\endcsname{\ensuremath{+0.048}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.delta_vsrebuild.s2\endcsname{\ensuremath{+0.784}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.delta_vsrebuild.se\endcsname{0.394}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.delta_vsrebuild.spread\endcsname{0.736}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.delta_vsunion\endcsname{\ensuremath{+1.348}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.discoveryseed0\endcsname{85.904}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.fresh_in_se_units\endcsname{2.19}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.fresh_in_se_units_union\endcsname{2.29}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.fresh_vsL1\endcsname{\ensuremath{-1.884}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.fresh_vsL3\endcsname{\ensuremath{-0.502}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.fresh_vsL3.abs\endcsname{0.502}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.fresh_vsL3.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.fresh_vsL3.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.fresh_vsL3.inscale\endcsname{0.63}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.fresh_vsL3.order\endcsname{the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.fresh_vsL3.relfloor\endcsname{1.00}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.fresh_vsL3.se\endcsname{0.492}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.freshgap.poolmax\endcsname{\ensuremath{+0.305}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.freshgap.unionmax\endcsname{\ensuremath{-0.044}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.freshmax\endcsname{85.363}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.freshmean\endcsname{84.970}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.freshmin\endcsname{84.577}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.freshminusbar\endcsname{\ensuremath{+1.241}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.freshminuss0\endcsname{\ensuremath{-0.935}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.freshrange.vsunion\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.freshspread\endcsname{0.786}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.freshvsownse\endcsname{4.05}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.pairsd\endcsname{0.556}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.refminusfresh\endcsname{\ensuremath{+1.884}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.refminusfresh.inse\endcsname{3.62}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.refminusfresh.se\endcsname{0.521}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.s0_in_single_seed_sd\endcsname{2.75}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.s0minusbar\endcsname{\ensuremath{+2.176}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.samedefault.fresh\endcsname{\ensuremath{+2.038}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.samedefault.s0\endcsname{\ensuremath{+1.633}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.samedefault.s1\endcsname{\ensuremath{+1.463}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.samedefault.s2\endcsname{\ensuremath{+2.613}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.seed1\endcsname{84.577}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.seed2\endcsname{85.363}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.sepair\endcsname{0.393}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.threeseeddelta\endcsname{\ensuremath{+1.903}}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.threeseedmean\endcsname{85.281}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.vsL3.clause\endcsname{HyReX+context's fresh mean, 84.970 Dice, is 0.502\,pp below HyReX's 85.472, a difference beyond the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.492\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.L6.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, HyReX+context reads 0.502\,pp below HyReX, 1.00 times the registered 0.50\,pp one-seed pair floor and 0.63 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.allseedsgap.poolmax\endcsname{\ensuremath{+0.257}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.allseedsmax\endcsname{84.743}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.allseedsmin\endcsname{84.529}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.ci3.hi\endcsname{\ensuremath{+4.298}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.ci3.lo\endcsname{\ensuremath{-1.946}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.ci6.hi\endcsname{\ensuremath{+2.448}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.ci6.lo\endcsname{\ensuremath{-0.584}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.delta_s0\endcsname{\ensuremath{+1.364}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.delta_s0_vsunion\endcsname{\ensuremath{+1.121}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.delta_vscontemp\endcsname{\ensuremath{+0.688}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.delta_vsdefault\endcsname{\ensuremath{+1.176}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.delta_vsunion\endcsname{\ensuremath{+0.932}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.discoveryseed0\endcsname{84.743}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.fresh_in_se_units\endcsname{1.62}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.fresh_in_se_units_union\endcsname{1.58}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.fresh_vsL1\endcsname{\ensuremath{-2.300}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.fresh_vsL3\endcsname{\ensuremath{-0.918}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.fresh_vsL3.abs\endcsname{0.918}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.fresh_vsL3.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.fresh_vsL3.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.fresh_vsL3.inscale\endcsname{1.15}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.fresh_vsL3.order\endcsname{every HyReX fresh run lies above every fresh run of this arm}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.fresh_vsL3.ordergap\endcsname{0.597}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.fresh_vsL3.relfloor\endcsname{1.84}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.fresh_vsL3.se\endcsname{0.297}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.freshgap.poolmax\endcsname{\ensuremath{+0.257}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.freshgap.unionmax\endcsname{\ensuremath{-0.091}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.freshmax\endcsname{84.579}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.freshmean\endcsname{84.554}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.freshmin\endcsname{84.529}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.freshminusbar\endcsname{\ensuremath{+0.826}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.freshminuss0\endcsname{\ensuremath{-0.189}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.freshrange.vsunion\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.freshspread\endcsname{0.050}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.freshvsownse\endcsname{47.12}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.pairsd\endcsname{0.035}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.refminusfresh\endcsname{\ensuremath{+2.300}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.refminusfresh.inse\endcsname{6.71}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.refminusfresh.se\endcsname{0.342}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.s0_in_single_seed_sd\endcsname{1.49}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.s0minusbar\endcsname{\ensuremath{+1.014}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.samedefault.fresh\endcsname{\ensuremath{+1.622}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.samedefault.s0\endcsname{\ensuremath{+0.471}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.samedefault.s1\endcsname{\ensuremath{+1.415}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.samedefault.s2\endcsname{\ensuremath{+1.829}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.seed1\endcsname{84.529}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.seed2\endcsname{84.579}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.sepair\endcsname{0.025}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.threeseeddelta\endcsname{\ensuremath{+1.239}}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.threeseedmean\endcsname{84.617}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.vsL3.clause\endcsname{the fn.-identical control's fresh mean, 84.554 Dice, is 0.918\,pp below HyReX's 85.472, a difference beyond the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.297\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.P3c.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, the fn.-identical control reads 0.918\,pp below HyReX, 1.84 times the registered 0.50\,pp one-seed pair floor and 1.15 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); every HyReX fresh run lies above every fresh run of the fn.-identical control, the smallest gap 0.597\,pp}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.allseedsgap.poolmax\endcsname{\ensuremath{-0.536}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.allseedsmax\endcsname{84.720}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.allseedsmin\endcsname{83.736}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.allseedsrange.vspool\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.ci3.hi\endcsname{\ensuremath{+3.692}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.ci3.lo\endcsname{\ensuremath{-2.552}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.ci6.hi\endcsname{\ensuremath{+1.842}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.ci6.lo\endcsname{\ensuremath{-1.189}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.delta_s0\endcsname{\ensuremath{+1.341}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.delta_s0_vsunion\endcsname{\ensuremath{+1.098}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.delta_vscontemp\endcsname{\ensuremath{+0.083}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.delta_vsdefault\endcsname{\ensuremath{+0.570}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.delta_vsrebuild\endcsname{\ensuremath{-0.606}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.delta_vsrebuild.s1\endcsname{\ensuremath{-0.368}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.delta_vsrebuild.s2\endcsname{\ensuremath{-0.843}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.delta_vsrebuild.se\endcsname{0.214}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.delta_vsrebuild.spread\endcsname{0.475}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.delta_vsunion\endcsname{\ensuremath{+0.326}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.discoveryseed0\endcsname{84.720}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.fresh_in_se_units\endcsname{0.79}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.fresh_in_se_units_union\endcsname{0.55}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.fresh_vsL1\endcsname{\ensuremath{-2.905}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.fresh_vsL3\endcsname{\ensuremath{-1.523}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.fresh_vsL3.abs\endcsname{1.523}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.fresh_vsL3.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.fresh_vsL3.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.fresh_vsL3.inscale\endcsname{1.92}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.fresh_vsL3.order\endcsname{every HyReX fresh run lies above every fresh run of this arm}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.fresh_vsL3.ordergap\endcsname{1.015}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.fresh_vsL3.relfloor\endcsname{3.05}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.fresh_vsL3.se\endcsname{0.364}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.freshbar_vsunion\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.freshgap.poolmax\endcsname{\ensuremath{-0.536}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.freshgap.unionmax\endcsname{\ensuremath{-0.885}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.freshmax\endcsname{84.161}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.freshmean\endcsname{83.948}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.freshmin\endcsname{83.736}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.freshminusbar\endcsname{\ensuremath{+0.220}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.freshminuss0\endcsname{\ensuremath{-0.771}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.freshrange.vspool\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.freshrange.vspool.phrase\endcsname{overlap}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.freshrange.vsunion\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.freshspread\endcsname{0.425}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.freshvsownse\endcsname{2.69}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.pairsd\endcsname{0.300}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.refminusfresh\endcsname{\ensuremath{+2.905}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.refminusfresh.inse\endcsname{7.22}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.refminusfresh.se\endcsname{0.402}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.s0_in_single_seed_sd\endcsname{1.46}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.s0minusbar\endcsname{\ensuremath{+0.991}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.samedefault.fresh\endcsname{\ensuremath{+1.017}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.samedefault.s0\endcsname{\ensuremath{+0.448}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.samedefault.s1\endcsname{\ensuremath{+1.047}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.samedefault.s2\endcsname{\ensuremath{+0.987}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.seed1\endcsname{84.161}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.seed2\endcsname{83.736}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.sepair\endcsname{0.212}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.threeseeddelta\endcsname{\ensuremath{+0.827}}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.threeseedmean\endcsname{84.205}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.vsL3.clause\endcsname{HyReX, finer ConvNeXt's fresh mean, 83.948 Dice, is 1.523\,pp below HyReX's 85.472, a difference beyond the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.364\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.S2.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, HyReX, finer ConvNeXt reads 1.523\,pp below HyReX, 3.05 times the registered 0.50\,pp one-seed pair floor and 1.92 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); every HyReX fresh run lies above every fresh run of HyReX, finer ConvNeXt, the smallest gap 1.015\,pp}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.allseedsgap.poolmax\endcsname{\ensuremath{+1.056}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.allseedsmax\endcsname{85.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.allseedsmin\endcsname{85.328}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.ci3.hi\endcsname{\ensuremath{+5.287}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.ci3.lo\endcsname{\ensuremath{-0.957}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.ci6.hi\endcsname{\ensuremath{+3.438}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.ci6.lo\endcsname{\ensuremath{+0.406}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.delta_s0\endcsname{\ensuremath{+1.949}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.delta_s0_vsunion\endcsname{\ensuremath{+1.706}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.delta_vscontemp\endcsname{\ensuremath{+1.678}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.delta_vsdefault\endcsname{\ensuremath{+2.165}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.delta_vsrebuild\endcsname{\ensuremath{+0.990}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.delta_vsrebuild.s1\endcsname{\ensuremath{+1.197}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.delta_vsrebuild.s2\endcsname{\ensuremath{+0.782}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.delta_vsrebuild.se\endcsname{0.184}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.delta_vsrebuild.spread\endcsname{0.415}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.delta_vsunion\endcsname{\ensuremath{+1.922}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.discoveryseed0\endcsname{85.328}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.fresh_in_se_units\endcsname{2.98}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.fresh_in_se_units_union\endcsname{3.26}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.fresh_vsL1\endcsname{\ensuremath{-1.310}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.fresh_vsL3\endcsname{\ensuremath{+0.072}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.fresh_vsL3.abs\endcsname{0.072}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.fresh_vsL3.dir\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.fresh_vsL3.inscale\endcsname{0.09}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.fresh_vsL3.order\endcsname{the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.fresh_vsL3.relfloor\endcsname{0.14}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.fresh_vsL3.se\endcsname{0.348}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.freshgap.poolmax\endcsname{\ensuremath{+1.089}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.freshgap.unionmax\endcsname{\ensuremath{+0.741}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.freshmax\endcsname{85.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.freshmean\endcsname{85.544}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.freshmin\endcsname{85.361}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.freshminusbar\endcsname{\ensuremath{+1.815}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.freshminuss0\endcsname{\ensuremath{+0.216}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.freshrange.vsunion\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.freshspread\endcsname{0.365}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.freshvsownse\endcsname{11.87}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.pairsd\endcsname{0.258}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.refminusfresh\endcsname{\ensuremath{+1.310}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.refminusfresh.inse\endcsname{3.38}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.refminusfresh.se\endcsname{0.387}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.s0_in_single_seed_sd\endcsname{2.12}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.s0minusbar\endcsname{\ensuremath{+1.599}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.samedefault.fresh\endcsname{\ensuremath{+2.612}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.samedefault.s0\endcsname{\ensuremath{+1.056}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.samedefault.s1\endcsname{\ensuremath{+2.612}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.samedefault.s2\endcsname{\ensuremath{+2.612}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.seed1\endcsname{85.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.seed2\endcsname{85.361}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.sepair\endcsname{0.182}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.threeseeddelta\endcsname{\ensuremath{+2.093}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.threeseedmean\endcsname{85.472}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.vsL3.clause\endcsname{HyReX-LeanDec's fresh mean, 85.544 Dice, is 0.072\,pp above HyReX's 85.472, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.348\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5A5.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, HyReX-LeanDec reads 0.072\,pp above HyReX, 0.14 times the registered 0.50\,pp one-seed pair floor and 0.09 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.allseedsgap.poolmax\endcsname{\ensuremath{+1.269}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.allseedsmax\endcsname{85.707}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.allseedsmin\endcsname{85.541}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.ci3.hi\endcsname{\ensuremath{+5.407}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.ci3.lo\endcsname{\ensuremath{-0.837}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.ci6.hi\endcsname{\ensuremath{+3.557}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.ci6.lo\endcsname{\ensuremath{+0.526}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.delta_s0\endcsname{\ensuremath{+2.162}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.delta_s0_vsunion\endcsname{\ensuremath{+1.919}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.delta_vscontemp\endcsname{\ensuremath{+1.798}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.delta_vsdefault\endcsname{\ensuremath{+2.285}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.delta_vsrebuild\endcsname{\ensuremath{+1.109}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.delta_vsrebuild.s1\endcsname{\ensuremath{+1.091}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.delta_vsrebuild.s2\endcsname{\ensuremath{+1.128}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.delta_vsrebuild.se\endcsname{0.050}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.delta_vsrebuild.spread\endcsname{0.037}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.delta_vsunion\endcsname{\ensuremath{+2.042}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.discoveryseed0\endcsname{85.541}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.fresh_in_se_units\endcsname{3.15}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.fresh_in_se_units_union\endcsname{3.46}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.fresh_vsL1\endcsname{\ensuremath{-1.190}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.fresh_vsL3\endcsname{\ensuremath{+0.192}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.fresh_vsL3.abs\endcsname{0.192}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.fresh_vsL3.dir\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.fresh_vsL3.inscale\endcsname{0.24}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.fresh_vsL3.order\endcsname{the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.fresh_vsL3.relfloor\endcsname{0.38}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.fresh_vsL3.se\endcsname{0.299}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.freshgap.poolmax\endcsname{\ensuremath{+1.348}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.freshgap.unionmax\endcsname{\ensuremath{+1.000}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.freshmax\endcsname{85.707}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.freshmean\endcsname{85.663}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.freshmin\endcsname{85.620}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.freshminusbar\endcsname{\ensuremath{+1.935}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.freshminuss0\endcsname{\ensuremath{+0.123}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.freshrange.vsunion\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.freshspread\endcsname{0.087}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.freshvsownse\endcsname{52.79}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.pairsd\endcsname{0.061}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.refminusfresh\endcsname{\ensuremath{+1.190}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.refminusfresh.inse\endcsname{3.46}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.refminusfresh.se\endcsname{0.344}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.s0_in_single_seed_sd\endcsname{2.36}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.s0minusbar\endcsname{\ensuremath{+1.812}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.samedefault.fresh\endcsname{\ensuremath{+2.732}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.samedefault.s0\endcsname{\ensuremath{+1.269}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.samedefault.s1\endcsname{\ensuremath{+2.507}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.samedefault.s2\endcsname{\ensuremath{+2.957}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.seed1\endcsname{85.620}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.seed2\endcsname{85.707}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.sepair\endcsname{0.043}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.threeseeddelta\endcsname{\ensuremath{+2.244}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.threeseedmean\endcsname{85.622}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.vsL3.clause\endcsname{LeanAdd's fresh mean, 85.663 Dice, is 0.192\,pp above HyReX's 85.472, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.299\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B1.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, LeanAdd reads 0.192\,pp above HyReX, 0.38 times the registered 0.50\,pp one-seed pair floor and 0.24 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.allseedsgap.poolmax\endcsname{\ensuremath{+0.371}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.allseedsmax\endcsname{84.876}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.allseedsmin\endcsname{84.643}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.ci3.hi\endcsname{\ensuremath{+4.570}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.ci3.lo\endcsname{\ensuremath{-1.674}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.ci6.hi\endcsname{\ensuremath{+2.720}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.ci6.lo\endcsname{\ensuremath{-0.311}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.delta_s0\endcsname{\ensuremath{+1.264}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.delta_s0_vsunion\endcsname{\ensuremath{+1.021}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.delta_vscontemp\endcsname{\ensuremath{+0.961}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.delta_vsdefault\endcsname{\ensuremath{+1.448}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.delta_vsrebuild\endcsname{\ensuremath{+0.272}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.delta_vsrebuild.s1\endcsname{\ensuremath{+0.347}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.delta_vsrebuild.s2\endcsname{\ensuremath{+0.198}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.delta_vsrebuild.se\endcsname{0.055}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.delta_vsrebuild.spread\endcsname{0.149}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.delta_vsunion\endcsname{\ensuremath{+1.205}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.discoveryseed0\endcsname{84.643}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.fresh_in_se_units\endcsname{2.00}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.fresh_in_se_units_union\endcsname{2.04}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.fresh_vsL1\endcsname{\ensuremath{-2.027}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.fresh_vsL3\endcsname{\ensuremath{-0.645}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.fresh_vsL3.abs\endcsname{0.645}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.fresh_vsL3.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.fresh_vsL3.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.fresh_vsL3.inscale\endcsname{0.81}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.fresh_vsL3.order\endcsname{every HyReX fresh run lies above every fresh run of this arm}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.fresh_vsL3.ordergap\endcsname{0.300}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.fresh_vsL3.relfloor\endcsname{1.29}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.fresh_vsL3.se\endcsname{0.300}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.freshgap.poolmax\endcsname{\ensuremath{+0.505}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.freshgap.unionmax\endcsname{\ensuremath{+0.157}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.freshmax\endcsname{84.876}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.freshmean\endcsname{84.826}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.freshmin\endcsname{84.777}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.freshminusbar\endcsname{\ensuremath{+1.098}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.freshminuss0\endcsname{\ensuremath{+0.184}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.freshrange.vsunion\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.freshspread\endcsname{0.099}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.freshvsownse\endcsname{29.30}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.pairsd\endcsname{0.070}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.refminusfresh\endcsname{\ensuremath{+2.027}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.refminusfresh.inse\endcsname{5.87}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.refminusfresh.se\endcsname{0.345}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.s0_in_single_seed_sd\endcsname{1.38}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.s0minusbar\endcsname{\ensuremath{+0.914}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.samedefault.fresh\endcsname{\ensuremath{+1.895}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.samedefault.s0\endcsname{\ensuremath{+0.371}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.samedefault.s1\endcsname{\ensuremath{+1.762}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.samedefault.s2\endcsname{\ensuremath{+2.028}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.seed1\endcsname{84.876}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.seed2\endcsname{84.777}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.sepair\endcsname{0.049}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.threeseeddelta\endcsname{\ensuremath{+1.387}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.threeseedmean\endcsname{84.765}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.vsL3.clause\endcsname{LeanAdd-NeXt's fresh mean, 84.826 Dice, is 0.645\,pp below HyReX's 85.472, a difference beyond the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.300\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V5B2.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, LeanAdd-NeXt reads 0.645\,pp below HyReX, 1.29 times the registered 0.50\,pp one-seed pair floor and 0.81 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); every HyReX fresh run lies above every fresh run of LeanAdd-NeXt, the smallest gap 0.300\,pp}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.allseedsgap.poolmax\endcsname{\ensuremath{+0.802}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.allseedsmax\endcsname{85.614}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.allseedsmin\endcsname{85.073}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.ci3.hi\endcsname{\ensuremath{+4.826}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.ci3.lo\endcsname{\ensuremath{-1.418}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.ci6.hi\endcsname{\ensuremath{+2.976}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.ci6.lo\endcsname{\ensuremath{-0.055}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.delta_s0\endcsname{\ensuremath{+2.236}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.delta_s0_vsunion\endcsname{\ensuremath{+1.992}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.delta_vscontemp\endcsname{\ensuremath{+1.217}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.delta_vsdefault\endcsname{\ensuremath{+1.704}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.delta_vsrebuild\endcsname{\ensuremath{+0.528}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.delta_vsrebuild.s1\endcsname{\ensuremath{+0.544}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.delta_vsrebuild.s2\endcsname{\ensuremath{+0.513}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.delta_vsrebuild.se\endcsname{0.027}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.delta_vsrebuild.spread\endcsname{0.032}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.delta_vsunion\endcsname{\ensuremath{+1.461}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.discoveryseed0\endcsname{85.614}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.fresh_in_se_units\endcsname{2.35}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.fresh_in_se_units_union\endcsname{2.48}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.fresh_vsL1\endcsname{\ensuremath{-1.771}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.fresh_vsL3\endcsname{\ensuremath{-0.389}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.fresh_vsL3.abs\endcsname{0.389}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.fresh_vsL3.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.fresh_vsL3.inscale\endcsname{0.49}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.fresh_vsL3.order\endcsname{every HyReX fresh run lies above every fresh run of this arm}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.fresh_vsL3.ordergap\endcsname{0.084}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.fresh_vsL3.relfloor\endcsname{0.78}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.fresh_vsL3.se\endcsname{0.296}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.freshgap.poolmax\endcsname{\ensuremath{+0.802}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.freshgap.unionmax\endcsname{\ensuremath{+0.453}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.freshmax\endcsname{85.091}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.freshmean\endcsname{85.082}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.freshmin\endcsname{85.073}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.freshminusbar\endcsname{\ensuremath{+1.354}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.freshminuss0\endcsname{\ensuremath{-0.532}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.freshrange.vsunion\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.freshspread\endcsname{0.018}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.freshvsownse\endcsname{188.28}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.pairsd\endcsname{0.013}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.refminusfresh\endcsname{\ensuremath{+1.771}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.refminusfresh.inse\endcsname{5.18}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.refminusfresh.se\endcsname{0.342}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.s0_in_single_seed_sd\endcsname{2.44}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.s0minusbar\endcsname{\ensuremath{+1.886}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.samedefault.fresh\endcsname{\ensuremath{+2.151}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.samedefault.s0\endcsname{\ensuremath{+1.343}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.samedefault.s1\endcsname{\ensuremath{+1.960}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.samedefault.s2\endcsname{\ensuremath{+2.342}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.seed1\endcsname{85.073}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.seed2\endcsname{85.091}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.sepair\endcsname{0.009}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.threeseeddelta\endcsname{\ensuremath{+1.881}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.threeseedmean\endcsname{85.260}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.vsL3.clause\endcsname{HyReX-k9's fresh mean, 85.082 Dice, is 0.389\,pp below HyReX's 85.472, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.296\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V6A1r.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, HyReX-k9 reads 0.389\,pp below HyReX, 0.78 times the registered 0.50\,pp one-seed pair floor and 0.49 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); every HyReX fresh run lies above every fresh run of HyReX-k9, the smallest gap 0.084\,pp}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.allseedsgap.poolmax\endcsname{\ensuremath{+1.433}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.allseedsmax\endcsname{86.375}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.allseedsmin\endcsname{85.705}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.ci3.hi\endcsname{\ensuremath{+5.784}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.ci3.lo\endcsname{\ensuremath{-0.460}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.ci6.hi\endcsname{\ensuremath{+3.934}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.ci6.lo\endcsname{\ensuremath{+0.902}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.delta_s0\endcsname{\ensuremath{+2.548}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.delta_s0_vsunion\endcsname{\ensuremath{+2.305}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.delta_vscontemp\endcsname{\ensuremath{+2.174}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.delta_vsdefault\endcsname{\ensuremath{+2.662}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.delta_vsrebuild\endcsname{\ensuremath{+1.486}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.delta_vsrebuild.s1\endcsname{\ensuremath{+1.176}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.delta_vsrebuild.s2\endcsname{\ensuremath{+1.796}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.delta_vsrebuild.se\endcsname{0.336}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.delta_vsrebuild.spread\endcsname{0.621}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.delta_vsunion\endcsname{\ensuremath{+2.418}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.discoveryseed0\endcsname{85.927}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.fresh_in_se_units\endcsname{3.67}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.fresh_in_se_units_union\endcsname{4.10}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.fresh_vsL1\endcsname{\ensuremath{-0.814}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.fresh_vsL3\endcsname{\ensuremath{+0.568}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.fresh_vsL3.abs\endcsname{0.568}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.fresh_vsL3.dir\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.fresh_vsL3.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.fresh_vsL3.inscale\endcsname{0.71}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.fresh_vsL3.order\endcsname{the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.fresh_vsL3.relfloor\endcsname{1.14}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.fresh_vsL3.se\endcsname{0.447}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.freshgap.poolmax\endcsname{\ensuremath{+1.433}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.freshgap.unionmax\endcsname{\ensuremath{+1.084}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.freshmax\endcsname{86.375}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.freshmean\endcsname{86.040}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.freshmin\endcsname{85.705}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.freshminusbar\endcsname{\ensuremath{+2.312}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.freshminuss0\endcsname{\ensuremath{+0.113}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.freshrange.vsunion\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.freshspread\endcsname{0.671}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.freshvsownse\endcsname{7.94}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.pairsd\endcsname{0.474}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.refminusfresh\endcsname{\ensuremath{+0.814}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.refminusfresh.inse\endcsname{1.70}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.refminusfresh.se\endcsname{0.479}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.s0_in_single_seed_sd\endcsname{2.78}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.s0minusbar\endcsname{\ensuremath{+2.198}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.samedefault.fresh\endcsname{\ensuremath{+3.108}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.samedefault.s0\endcsname{\ensuremath{+1.655}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.samedefault.s1\endcsname{\ensuremath{+2.591}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.samedefault.s2\endcsname{\ensuremath{+3.626}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.seed1\endcsname{85.705}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.seed2\endcsname{86.375}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.sepair\endcsname{0.335}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.threeseeddelta\endcsname{\ensuremath{+2.624}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.threeseedmean\endcsname{86.002}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.vsL3.clause\endcsname{LeanDeepMid's fresh mean, 86.040 Dice, is 0.568\,pp above HyReX's 85.472, a difference beyond the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.447\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A1.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, LeanDeepMid reads 0.568\,pp above HyReX, 1.14 times the registered 0.50\,pp one-seed pair floor and 0.71 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.allseedsgap.poolmax\endcsname{\ensuremath{+1.079}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.allseedsmax\endcsname{86.264}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.allseedsmin\endcsname{85.351}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.ci3.hi\endcsname{\ensuremath{+5.411}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.ci3.lo\endcsname{\ensuremath{-0.833}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.ci6.hi\endcsname{\ensuremath{+3.561}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.ci6.lo\endcsname{\ensuremath{+0.530}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.delta_s0\endcsname{\ensuremath{+2.886}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.delta_s0_vsunion\endcsname{\ensuremath{+2.642}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.delta_vscontemp\endcsname{\ensuremath{+1.802}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.delta_vsdefault\endcsname{\ensuremath{+2.289}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.delta_vsrebuild\endcsname{\ensuremath{+1.113}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.delta_vsrebuild.s1\endcsname{\ensuremath{+0.822}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.delta_vsrebuild.s2\endcsname{\ensuremath{+1.405}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.delta_vsrebuild.se\endcsname{0.317}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.delta_vsrebuild.spread\endcsname{0.583}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.delta_vsunion\endcsname{\ensuremath{+2.046}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.discoveryseed0\endcsname{86.264}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.fresh_in_se_units\endcsname{3.15}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.fresh_in_se_units_union\endcsname{3.47}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.fresh_vsL1\endcsname{\ensuremath{-1.186}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.fresh_vsL3\endcsname{\ensuremath{+0.196}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.fresh_vsL3.abs\endcsname{0.196}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.fresh_vsL3.dir\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.fresh_vsL3.inscale\endcsname{0.25}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.fresh_vsL3.order\endcsname{the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.fresh_vsL3.relfloor\endcsname{0.39}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.fresh_vsL3.se\endcsname{0.433}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.freshgap.poolmax\endcsname{\ensuremath{+1.079}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.freshgap.unionmax\endcsname{\ensuremath{+0.731}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.freshmax\endcsname{85.984}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.freshmean\endcsname{85.667}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.freshmin\endcsname{85.351}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.freshminusbar\endcsname{\ensuremath{+1.939}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.freshminuss0\endcsname{\ensuremath{-0.597}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.freshrange.vsunion\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.freshspread\endcsname{0.633}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.freshvsownse\endcsname{7.24}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.pairsd\endcsname{0.447}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.refminusfresh\endcsname{\ensuremath{+1.186}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.refminusfresh.inse\endcsname{2.55}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.refminusfresh.se\endcsname{0.466}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.s0_in_single_seed_sd\endcsname{3.14}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.s0minusbar\endcsname{\ensuremath{+2.536}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.samedefault.fresh\endcsname{\ensuremath{+2.736}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.samedefault.s0\endcsname{\ensuremath{+1.993}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.samedefault.s1\endcsname{\ensuremath{+2.238}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.samedefault.s2\endcsname{\ensuremath{+3.234}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.seed1\endcsname{85.351}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.seed2\endcsname{85.984}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.sepair\endcsname{0.316}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.threeseeddelta\endcsname{\ensuremath{+2.488}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.threeseedmean\endcsname{85.866}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.vsL3.clause\endcsname{LeanDeepMid+FD's fresh mean, 85.667 Dice, is 0.196\,pp above HyReX's 85.472, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.433\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7A2.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, LeanDeepMid+FD reads 0.196\,pp above HyReX, 0.39 times the registered 0.50\,pp one-seed pair floor and 0.25 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.allseedsgap.poolmax\endcsname{\ensuremath{+0.828}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.allseedsmax\endcsname{86.088}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.allseedsmin\endcsname{85.100}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.ci3.hi\endcsname{\ensuremath{+5.504}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.ci3.lo\endcsname{\ensuremath{-0.740}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.ci6.hi\endcsname{\ensuremath{+3.654}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.ci6.lo\endcsname{\ensuremath{+0.622}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.delta_s0\endcsname{\ensuremath{+1.721}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.delta_s0_vsunion\endcsname{\ensuremath{+1.478}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.delta_vscontemp\endcsname{\ensuremath{+1.894}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.delta_vsdefault\endcsname{\ensuremath{+2.382}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.delta_vsrebuild\endcsname{\ensuremath{+1.206}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.delta_vsrebuild.s1\endcsname{\ensuremath{+0.902}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.delta_vsrebuild.s2\endcsname{\ensuremath{+1.509}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.delta_vsrebuild.se\endcsname{0.329}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.delta_vsrebuild.spread\endcsname{0.607}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.delta_vsunion\endcsname{\ensuremath{+2.138}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.discoveryseed0\endcsname{85.100}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.fresh_in_se_units\endcsname{3.28}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.fresh_in_se_units_union\endcsname{3.63}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.fresh_vsL1\endcsname{\ensuremath{-1.094}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.fresh_vsL3\endcsname{\ensuremath{+0.288}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.fresh_vsL3.abs\endcsname{0.288}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.fresh_vsL3.dir\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.fresh_vsL3.inscale\endcsname{0.36}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.fresh_vsL3.order\endcsname{the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.fresh_vsL3.relfloor\endcsname{0.58}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.fresh_vsL3.se\endcsname{0.442}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.freshgap.poolmax\endcsname{\ensuremath{+1.160}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.freshgap.unionmax\endcsname{\ensuremath{+0.811}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.freshmax\endcsname{86.088}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.freshmean\endcsname{85.760}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.freshmin\endcsname{85.431}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.freshminusbar\endcsname{\ensuremath{+2.032}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.freshminuss0\endcsname{\ensuremath{+0.660}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.freshrange.vsunion\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.freshspread\endcsname{0.657}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.freshvsownse\endcsname{7.25}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.pairsd\endcsname{0.465}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.refminusfresh\endcsname{\ensuremath{+1.094}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.refminusfresh.inse\endcsname{2.31}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.refminusfresh.se\endcsname{0.474}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.s0_in_single_seed_sd\endcsname{1.88}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.s0minusbar\endcsname{\ensuremath{+1.371}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.samedefault.fresh\endcsname{\ensuremath{+2.828}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.samedefault.s0\endcsname{\ensuremath{+0.828}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.samedefault.s1\endcsname{\ensuremath{+2.318}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.samedefault.s2\endcsname{\ensuremath{+3.339}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.seed1\endcsname{85.431}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.seed2\endcsname{86.088}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.sepair\endcsname{0.329}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.threeseeddelta\endcsname{\ensuremath{+2.162}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.threeseedmean\endcsname{85.540}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.vsL3.clause\endcsname{LeanSep's fresh mean, 85.760 Dice, is 0.288\,pp above HyReX's 85.472, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.442\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B1.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, LeanSep reads 0.288\,pp above HyReX, 0.58 times the registered 0.50\,pp one-seed pair floor and 0.36 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.allseedsgap.poolmax\endcsname{\ensuremath{+0.388}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.allseedsmax\endcsname{86.203}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.allseedsmin\endcsname{84.660}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.ci3.hi\endcsname{\ensuremath{+4.960}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.ci3.lo\endcsname{\ensuremath{-1.284}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.ci6.hi\endcsname{\ensuremath{+3.111}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.ci6.lo\endcsname{\ensuremath{+0.079}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.delta_s0\endcsname{\ensuremath{+2.824}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.delta_s0_vsunion\endcsname{\ensuremath{+2.581}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.delta_vscontemp\endcsname{\ensuremath{+1.351}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.delta_vsdefault\endcsname{\ensuremath{+1.838}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.delta_vsrebuild\endcsname{\ensuremath{+0.663}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.delta_vsrebuild.s1\endcsname{\ensuremath{+1.244}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.delta_vsrebuild.s2\endcsname{\ensuremath{+0.081}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.delta_vsrebuild.se\endcsname{0.557}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.delta_vsrebuild.spread\endcsname{1.163}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.delta_vsunion\endcsname{\ensuremath{+1.595}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.discoveryseed0\endcsname{86.203}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.fresh_in_se_units\endcsname{2.53}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.fresh_in_se_units_union\endcsname{2.70}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.fresh_vsL1\endcsname{\ensuremath{-1.637}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.fresh_vsL3\endcsname{\ensuremath{-0.255}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.fresh_vsL3.abs\endcsname{0.255}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.fresh_vsL3.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.fresh_vsL3.inscale\endcsname{0.32}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.fresh_vsL3.order\endcsname{the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.fresh_vsL3.relfloor\endcsname{0.51}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.fresh_vsL3.se\endcsname{0.630}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.freshgap.poolmax\endcsname{\ensuremath{+0.388}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.freshgap.unionmax\endcsname{\ensuremath{+0.039}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.freshmax\endcsname{85.773}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.freshmean\endcsname{85.217}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.freshmin\endcsname{84.660}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.freshminusbar\endcsname{\ensuremath{+1.488}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.freshminuss0\endcsname{\ensuremath{-0.986}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.freshrange.vsunion\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.freshspread\endcsname{1.113}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.freshvsownse\endcsname{3.30}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.pairsd\endcsname{0.787}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.refminusfresh\endcsname{\ensuremath{+1.637}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.refminusfresh.inse\endcsname{2.51}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.refminusfresh.se\endcsname{0.653}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.s0_in_single_seed_sd\endcsname{3.08}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.s0minusbar\endcsname{\ensuremath{+2.474}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.samedefault.fresh\endcsname{\ensuremath{+2.285}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.samedefault.s0\endcsname{\ensuremath{+1.931}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.samedefault.s1\endcsname{\ensuremath{+2.660}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.samedefault.s2\endcsname{\ensuremath{+1.911}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.seed1\endcsname{85.773}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.seed2\endcsname{84.660}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.sepair\endcsname{0.557}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.threeseeddelta\endcsname{\ensuremath{+2.167}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.threeseedmean\endcsname{85.545}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.vsL3.clause\endcsname{LeanDil's fresh mean, 85.217 Dice, is 0.255\,pp below HyReX's 85.472, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.630\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7B2.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, LeanDil reads 0.255\,pp below HyReX, 0.51 times the registered 0.50\,pp one-seed pair floor and 0.32 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.allseedsgap.poolmax\endcsname{\ensuremath{+1.228}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.allseedsmax\endcsname{86.137}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.allseedsmin\endcsname{85.500}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.ci3.hi\endcsname{\ensuremath{+5.562}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.ci3.lo\endcsname{\ensuremath{-0.682}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.ci6.hi\endcsname{\ensuremath{+3.712}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.ci6.lo\endcsname{\ensuremath{+0.680}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.delta_s0\endcsname{\ensuremath{+2.707}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.delta_s0_vsunion\endcsname{\ensuremath{+2.463}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.delta_vscontemp\endcsname{\ensuremath{+1.953}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.delta_vsdefault\endcsname{\ensuremath{+2.440}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.delta_vsrebuild\endcsname{\ensuremath{+1.264}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.delta_vsrebuild.s1\endcsname{\ensuremath{+1.608}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.delta_vsrebuild.s2\endcsname{\ensuremath{+0.921}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.delta_vsrebuild.se\endcsname{0.319}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.delta_vsrebuild.spread\endcsname{0.687}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.delta_vsunion\endcsname{\ensuremath{+2.196}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.discoveryseed0\endcsname{86.085}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.fresh_in_se_units\endcsname{3.36}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.fresh_in_se_units_union\endcsname{3.72}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.fresh_vsL1\endcsname{\ensuremath{-1.035}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.fresh_vsL3\endcsname{\ensuremath{+0.346}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.fresh_vsL3.abs\endcsname{0.346}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.fresh_vsL3.dir\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.fresh_vsL3.inscale\endcsname{0.44}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.fresh_vsL3.order\endcsname{the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.fresh_vsL3.relfloor\endcsname{0.69}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.fresh_vsL3.se\endcsname{0.435}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.freshgap.poolmax\endcsname{\ensuremath{+1.228}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.freshgap.unionmax\endcsname{\ensuremath{+0.879}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.freshmax\endcsname{86.137}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.freshmean\endcsname{85.818}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.freshmin\endcsname{85.500}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.freshminusbar\endcsname{\ensuremath{+2.090}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.freshminuss0\endcsname{\ensuremath{-0.267}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.freshrange.vsunion\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.freshspread\endcsname{0.637}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.freshvsownse\endcsname{7.66}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.pairsd\endcsname{0.450}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.refminusfresh\endcsname{\ensuremath{+1.035}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.refminusfresh.inse\endcsname{2.22}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.refminusfresh.se\endcsname{0.467}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.s0_in_single_seed_sd\endcsname{2.95}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.s0minusbar\endcsname{\ensuremath{+2.357}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.samedefault.fresh\endcsname{\ensuremath{+2.887}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.samedefault.s0\endcsname{\ensuremath{+1.813}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.samedefault.s1\endcsname{\ensuremath{+3.023}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.samedefault.s2\endcsname{\ensuremath{+2.750}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.seed1\endcsname{86.137}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.seed2\endcsname{85.500}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.sepair\endcsname{0.318}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.threeseeddelta\endcsname{\ensuremath{+2.529}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.threeseedmean\endcsname{85.907}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.vsL3.clause\endcsname{LeanNeXt-s5's fresh mean, 85.818 Dice, is 0.346\,pp above HyReX's 85.472, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.435\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V7C1.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, LeanNeXt-s5 reads 0.346\,pp above HyReX, 0.69 times the registered 0.50\,pp one-seed pair floor and 0.44 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.allseedsgap.poolmax\endcsname{\ensuremath{+0.184}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.allseedsmax\endcsname{85.138}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.allseedsmin\endcsname{84.456}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.ci3.hi\endcsname{\ensuremath{+4.371}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.ci3.lo\endcsname{\ensuremath{-1.873}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.ci6.hi\endcsname{\ensuremath{+2.521}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.ci6.lo\endcsname{\ensuremath{-0.511}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.delta_s0\endcsname{\ensuremath{+1.760}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.delta_s0_vsunion\endcsname{\ensuremath{+1.516}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.delta_vscontemp\endcsname{\ensuremath{+0.762}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.delta_vsdefault\endcsname{\ensuremath{+1.249}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.delta_vsrebuild\endcsname{\ensuremath{+0.073}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.delta_vsrebuild.s1\endcsname{\ensuremath{-0.073}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.delta_vsrebuild.s2\endcsname{\ensuremath{+0.220}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.delta_vsrebuild.se\endcsname{0.173}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.delta_vsrebuild.spread\endcsname{0.293}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.delta_vsunion\endcsname{\ensuremath{+1.005}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.discoveryseed0\endcsname{85.138}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.fresh_in_se_units\endcsname{1.72}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.fresh_in_se_units_union\endcsname{1.70}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.fresh_vsL1\endcsname{\ensuremath{-2.226}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.fresh_vsL3\endcsname{\ensuremath{-0.845}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.fresh_vsL3.abs\endcsname{0.845}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.fresh_vsL3.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.fresh_vsL3.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.fresh_vsL3.inscale\endcsname{1.06}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.fresh_vsL3.order\endcsname{every HyReX fresh run lies above every fresh run of this arm}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.fresh_vsL3.ordergap\endcsname{0.377}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.fresh_vsL3.relfloor\endcsname{1.69}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.fresh_vsL3.se\endcsname{0.342}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.freshgap.poolmax\endcsname{\ensuremath{+0.184}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.freshgap.unionmax\endcsname{\ensuremath{-0.165}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.freshmax\endcsname{84.799}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.freshmean\endcsname{84.627}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.freshmin\endcsname{84.456}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.freshminusbar\endcsname{\ensuremath{+0.899}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.freshminuss0\endcsname{\ensuremath{-0.511}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.freshrange.vsunion\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.freshspread\endcsname{0.343}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.freshvsownse\endcsname{7.28}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.pairsd\endcsname{0.243}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.refminusfresh\endcsname{\ensuremath{+2.226}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.refminusfresh.inse\endcsname{5.82}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.refminusfresh.se\endcsname{0.382}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.s0_in_single_seed_sd\endcsname{1.92}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.s0minusbar\endcsname{\ensuremath{+1.410}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.samedefault.fresh\endcsname{\ensuremath{+1.696}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.samedefault.s0\endcsname{\ensuremath{+0.867}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.samedefault.s1\endcsname{\ensuremath{+1.342}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.samedefault.s2\endcsname{\ensuremath{+2.049}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.seed1\endcsname{84.456}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.seed2\endcsname{84.799}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.sepair\endcsname{0.172}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.threeseeddelta\endcsname{\ensuremath{+1.419}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.threeseedmean\endcsname{84.798}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.vsL3.clause\endcsname{CoarseStack's fresh mean, 84.627 Dice, is 0.845\,pp below HyReX's 85.472, a difference beyond the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.342\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A1.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, CoarseStack reads 0.845\,pp below HyReX, 1.69 times the registered 0.50\,pp one-seed pair floor and 1.06 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); every HyReX fresh run lies above every fresh run of CoarseStack, the smallest gap 0.377\,pp}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.allseedsgap.poolmax\endcsname{\ensuremath{+0.460}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.allseedsmax\endcsname{85.540}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.allseedsmin\endcsname{84.732}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.ci3.hi\endcsname{\ensuremath{+4.999}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.ci3.lo\endcsname{\ensuremath{-1.245}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.ci6.hi\endcsname{\ensuremath{+3.149}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.ci6.lo\endcsname{\ensuremath{+0.118}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.delta_s0\endcsname{\ensuremath{+1.353}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.delta_s0_vsunion\endcsname{\ensuremath{+1.110}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.delta_vscontemp\endcsname{\ensuremath{+1.390}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.delta_vsdefault\endcsname{\ensuremath{+1.877}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.delta_vsrebuild\endcsname{\ensuremath{+0.701}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.delta_vsrebuild.s1\endcsname{\ensuremath{+0.442}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.delta_vsrebuild.s2\endcsname{\ensuremath{+0.961}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.delta_vsrebuild.se\endcsname{0.285}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.delta_vsrebuild.spread\endcsname{0.519}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.delta_vsunion\endcsname{\ensuremath{+1.634}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.discoveryseed0\endcsname{84.732}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.fresh_in_se_units\endcsname{2.59}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.fresh_in_se_units_union\endcsname{2.77}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.fresh_vsL1\endcsname{\ensuremath{-1.598}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.fresh_vsL3\endcsname{\ensuremath{-0.216}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.fresh_vsL3.abs\endcsname{0.216}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.fresh_vsL3.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.fresh_vsL3.inscale\endcsname{0.27}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.fresh_vsL3.order\endcsname{the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.fresh_vsL3.relfloor\endcsname{0.43}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.fresh_vsL3.se\endcsname{0.410}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.freshgap.poolmax\endcsname{\ensuremath{+0.699}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.freshgap.unionmax\endcsname{\ensuremath{+0.351}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.freshmax\endcsname{85.540}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.freshmean\endcsname{85.255}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.freshmin\endcsname{84.971}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.freshminusbar\endcsname{\ensuremath{+1.527}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.freshminuss0\endcsname{\ensuremath{+0.524}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.freshrange.vsunion\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.freshspread\endcsname{0.569}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.freshvsownse\endcsname{6.60}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.pairsd\endcsname{0.402}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.refminusfresh\endcsname{\ensuremath{+1.598}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.refminusfresh.inse\endcsname{3.60}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.refminusfresh.se\endcsname{0.444}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.s0_in_single_seed_sd\endcsname{1.47}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.s0minusbar\endcsname{\ensuremath{+1.003}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.samedefault.fresh\endcsname{\ensuremath{+2.324}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.samedefault.s0\endcsname{\ensuremath{+0.460}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.samedefault.s1\endcsname{\ensuremath{+1.858}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.samedefault.s2\endcsname{\ensuremath{+2.790}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.seed1\endcsname{84.971}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.seed2\endcsname{85.540}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.sepair\endcsname{0.284}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.threeseeddelta\endcsname{\ensuremath{+1.703}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.threeseedmean\endcsname{85.081}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.vsL3.clause\endcsname{StackDec's fresh mean, 85.255 Dice, is 0.216\,pp below HyReX's 85.472, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.410\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8A2.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, StackDec reads 0.216\,pp below HyReX, 0.43 times the registered 0.50\,pp one-seed pair floor and 0.27 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.allseedsgap.poolmax\endcsname{\ensuremath{-0.223}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.allseedsmax\endcsname{86.289}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.allseedsmin\endcsname{84.049}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.allseedsrange.vspool\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.ci3.hi\endcsname{\ensuremath{+4.497}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.ci3.lo\endcsname{\ensuremath{-1.747}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.ci6.hi\endcsname{\ensuremath{+2.647}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.ci6.lo\endcsname{\ensuremath{-0.385}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.delta_s0\endcsname{\ensuremath{+2.911}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.delta_s0_vsunion\endcsname{\ensuremath{+2.667}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.delta_vscontemp\endcsname{\ensuremath{+0.887}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.delta_vsdefault\endcsname{\ensuremath{+1.375}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.delta_vsrebuild\endcsname{\ensuremath{+0.199}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.delta_vsrebuild.s1\endcsname{\ensuremath{+0.928}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.delta_vsrebuild.s2\endcsname{\ensuremath{-0.530}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.delta_vsrebuild.se\endcsname{0.705}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.delta_vsrebuild.spread\endcsname{1.459}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.delta_vsunion\endcsname{\ensuremath{+1.131}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.discoveryseed0\endcsname{86.289}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.fresh_in_se_units\endcsname{1.89}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.fresh_in_se_units_union\endcsname{1.92}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.fresh_vsL1\endcsname{\ensuremath{-2.101}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.fresh_vsL3\endcsname{\ensuremath{-0.719}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.fresh_vsL3.abs\endcsname{0.719}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.fresh_vsL3.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.fresh_vsL3.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.fresh_vsL3.inscale\endcsname{0.90}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.fresh_vsL3.order\endcsname{the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.fresh_vsL3.relfloor\endcsname{1.44}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.fresh_vsL3.se\endcsname{0.764}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.freshgap.poolmax\endcsname{\ensuremath{-0.223}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.freshgap.unionmax\endcsname{\ensuremath{-0.572}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.freshmax\endcsname{85.457}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.freshmean\endcsname{84.753}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.freshmin\endcsname{84.049}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.freshminusbar\endcsname{\ensuremath{+1.025}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.freshminuss0\endcsname{\ensuremath{-1.536}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.freshrange.vspool\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.freshrange.vspool.phrase\endcsname{overlap}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.freshrange.vsunion\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.freshspread\endcsname{1.409}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.freshvsownse\endcsname{1.95}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.pairsd\endcsname{0.996}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.refminusfresh\endcsname{\ensuremath{+2.101}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.refminusfresh.inse\endcsname{2.68}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.refminusfresh.se\endcsname{0.783}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.s0_in_single_seed_sd\endcsname{3.17}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.s0minusbar\endcsname{\ensuremath{+2.561}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.samedefault.fresh\endcsname{\ensuremath{+1.821}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.samedefault.s0\endcsname{\ensuremath{+2.017}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.samedefault.s1\endcsname{\ensuremath{+2.344}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.samedefault.s2\endcsname{\ensuremath{+1.299}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.seed1\endcsname{85.457}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.seed2\endcsname{84.049}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.sepair\endcsname{0.704}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.threeseeddelta\endcsname{\ensuremath{+1.887}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.threeseedmean\endcsname{85.265}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.vsL3.clause\endcsname{LeanTrunk's fresh mean, 84.753 Dice, is 0.719\,pp below HyReX's 85.472, a difference beyond the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.764\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B1.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, LeanTrunk reads 0.719\,pp below HyReX, 1.44 times the registered 0.50\,pp one-seed pair floor and 0.90 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.allseedsgap.poolmax\endcsname{\ensuremath{+0.677}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.allseedsmax\endcsname{85.270}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.allseedsmin\endcsname{84.949}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.allseedsrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.ci3.hi\endcsname{\ensuremath{+4.853}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.ci3.lo\endcsname{\ensuremath{-1.391}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.ci6.hi\endcsname{\ensuremath{+3.003}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.ci6.lo\endcsname{\ensuremath{-0.028}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.delta_s0\endcsname{\ensuremath{+1.646}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.delta_s0_vsunion\endcsname{\ensuremath{+1.402}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.delta_vscontemp\endcsname{\ensuremath{+1.244}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.delta_vsdefault\endcsname{\ensuremath{+1.731}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.delta_vsrebuild\endcsname{\ensuremath{+0.555}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.delta_vsrebuild.s1\endcsname{\ensuremath{+0.741}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.delta_vsrebuild.s2\endcsname{\ensuremath{+0.370}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.delta_vsrebuild.se\endcsname{0.163}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.delta_vsrebuild.spread\endcsname{0.371}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.delta_vsunion\endcsname{\ensuremath{+1.487}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.discoveryseed0\endcsname{85.024}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.fresh_in_se_units\endcsname{2.39}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.fresh_in_se_units_union\endcsname{2.52}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.fresh_vsL1\endcsname{\ensuremath{-1.744}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.fresh_vsL3\endcsname{\ensuremath{-0.362}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.fresh_vsL3.abs\endcsname{0.362}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.fresh_vsL3.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.fresh_vsL3.floor\endcsname{inside}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.fresh_vsL3.inscale\endcsname{0.46}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.fresh_vsL3.order\endcsname{the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.fresh_vsL3.ordergap\endcsname{\pend}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.fresh_vsL3.relfloor\endcsname{0.72}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.fresh_vsL3.se\endcsname{0.337}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.freshgap.poolmax\endcsname{\ensuremath{+0.677}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.freshgap.unionmax\endcsname{\ensuremath{+0.328}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.freshmax\endcsname{85.270}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.freshmean\endcsname{85.109}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.freshmin\endcsname{84.949}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.freshminusbar\endcsname{\ensuremath{+1.381}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.freshminuss0\endcsname{\ensuremath{+0.085}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.freshrange.vspool\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.freshrange.vspool.phrase\endcsname{lie above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.freshrange.vsunion\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.freshspread\endcsname{0.321}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.freshvsownse\endcsname{10.77}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.pairsd\endcsname{0.227}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.refminusfresh\endcsname{\ensuremath{+1.744}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.refminusfresh.inse\endcsname{4.62}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.refminusfresh.se\endcsname{0.377}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.s0_in_single_seed_sd\endcsname{1.79}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.s0minusbar\endcsname{\ensuremath{+1.296}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.samedefault.fresh\endcsname{\ensuremath{+2.178}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.samedefault.s0\endcsname{\ensuremath{+0.752}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.samedefault.s1\endcsname{\ensuremath{+2.156}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.samedefault.s2\endcsname{\ensuremath{+2.199}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.seed1\endcsname{85.270}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.seed2\endcsname{84.949}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.sepair\endcsname{0.161}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.threeseeddelta\endcsname{\ensuremath{+1.703}}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.threeseedmean\endcsname{85.081}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.vsL3.clause\endcsname{Stem1's fresh mean, 85.109 Dice, is 0.362\,pp below HyReX's 85.472, a difference inside the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.337\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.V8B2.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, Stem1 reads 0.362\,pp below HyReX, 0.72 times the registered 0.50\,pp one-seed pair floor and 0.46 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); the two arms' fresh runs interleave}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.allseedsgap.poolmax\endcsname{\ensuremath{-0.494}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.allseedsmax\endcsname{86.014}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.allseedsmin\endcsname{83.777}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.allseedsrange.vspool\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.ci3.hi\endcsname{\ensuremath{+4.189}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.ci3.lo\endcsname{\ensuremath{-2.055}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.ci6.hi\endcsname{\ensuremath{+2.339}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.ci6.lo\endcsname{\ensuremath{-0.693}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.clearsownse\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.clearspairfloor\endcsname{above}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.delta_s0\endcsname{\ensuremath{+2.636}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.delta_s0_vsunion\endcsname{\ensuremath{+2.392}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.delta_vscontemp\endcsname{\ensuremath{+0.579}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.delta_vscontemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.delta_vsdefault\endcsname{\ensuremath{+1.067}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.delta_vsdefault.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.delta_vsrebuild\endcsname{\ensuremath{-0.109}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.delta_vsrebuild.s1\endcsname{\ensuremath{+0.583}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.delta_vsrebuild.s2\endcsname{\ensuremath{-0.801}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.delta_vsrebuild.se\endcsname{0.668}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.delta_vsrebuild.spread\endcsname{1.384}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.delta_vsrebuild.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.delta_vsunion\endcsname{\ensuremath{+0.823}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.delta_vsunion.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.discoveryseed0\endcsname{86.014}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.discoveryseed0.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.fresh_in_se_units\endcsname{1.47}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.fresh_in_se_units.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.fresh_in_se_units_union\endcsname{1.40}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.fresh_vsL1\endcsname{\ensuremath{-2.409}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.fresh_vsL1.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.fresh_vsL1.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.fresh_vsL3\endcsname{\ensuremath{-1.027}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.fresh_vsL3.abs\endcsname{1.027}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.fresh_vsL3.dir\endcsname{below}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.fresh_vsL3.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.fresh_vsL3.inscale\endcsname{1.29}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.fresh_vsL3.order\endcsname{every HyReX fresh run lies above every fresh run of this arm}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.fresh_vsL3.ordergap\endcsname{0.064}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.fresh_vsL3.relfloor\endcsname{2.05}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.fresh_vsL3.se\endcsname{0.730}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.fresh_vsL3.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.freshbar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.freshgap.poolmax\endcsname{\ensuremath{-0.494}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.freshgap.unionmax\endcsname{\ensuremath{-0.843}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.freshmax\endcsname{85.112}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.freshmean\endcsname{84.445}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.freshmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.freshmin\endcsname{83.777}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.freshminusbar\endcsname{\ensuremath{+0.717}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.freshminuss0\endcsname{\ensuremath{-1.569}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.freshrange.vspool\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.freshrange.vspool.phrase\endcsname{overlap}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.freshrange.vsunion\endcsname{overlaps}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.freshresolution\endcsname{resolved}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.freshspread\endcsname{1.335}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.freshvsownse\endcsname{1.60}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.pairsd\endcsname{0.944}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.refminusfresh\endcsname{\ensuremath{+2.409}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.refminusfresh.inse\endcsname{3.21}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.refminusfresh.se\endcsname{0.750}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.refminusfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.resolutionbinding\endcsname{none (every leg of the rule holds)}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.s0_in_single_seed_sd\endcsname{2.87}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.s0_in_single_seed_sd.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.s0bar_vsunion\endcsname{clears}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.s0minusbar\endcsname{\ensuremath{+2.286}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.samedefault.fresh\endcsname{\ensuremath{+1.513}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.samedefault.s0\endcsname{\ensuremath{+1.742}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.samedefault.s1\endcsname{\ensuremath{+1.999}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.samedefault.s2\endcsname{\ensuremath{+1.028}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.sedelta\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.seed1\endcsname{85.112}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.seed1.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.seed2\endcsname{83.777}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.seed2.status\endcsname{verified}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.sepair\endcsname{0.667}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.sepair.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.threeseeddelta\endcsname{\ensuremath{+1.590}}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.threeseedmean\endcsname{84.968}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.threeseedmean.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.vsL3.clause\endcsname{the branch control's fresh mean, 84.445 Dice, is 1.027\,pp below HyReX's 85.472, a difference beyond the registered 0.50\,pp one-seed pair floor (empirical SE of the difference, from the two pairs' own spread: 0.730\,pp)}
\expandafter\gdef\csname R@an.fresh_replication.kits.W1c.vsL3.sentence\endcsname{on KiTS23 fold 0, at 2 fresh seeds per arm, the branch control reads 1.027\,pp below HyReX, 2.05 times the registered 0.50\,pp one-seed pair floor and 1.29 standard errors at the frozen KiTS23 pool seed SD of 0.795\,pp (a model-based SE of a two-versus-two difference, not the empirical SE of these two pairs); every HyReX fresh run lies above every fresh run of the branch control, the smallest gap 0.064\,pp}
\expandafter\gdef\csname R@an.fresh_replication.kits.barfliplist\endcsname{HyReX, finer ConvNeXt}
\expandafter\gdef\csname R@an.fresh_replication.kits.base.pubdeficit.contemp\endcsname{\ensuremath{-2.384}}
\expandafter\gdef\csname R@an.fresh_replication.kits.base.pubdeficit.frozen\endcsname{\ensuremath{-2.872}}
\expandafter\gdef\csname R@an.fresh_replication.kits.base.pubdeficit.union\endcsname{\ensuremath{-2.628}}
\expandafter\gdef\csname R@an.fresh_replication.kits.ci3.half\endcsname{3.122}
\expandafter\gdef\csname R@an.fresh_replication.kits.ci3.tq\endcsname{4.303}
\expandafter\gdef\csname R@an.fresh_replication.kits.ci6.half\endcsname{1.516}
\expandafter\gdef\csname R@an.fresh_replication.kits.ci6.tq\endcsname{2.571}
\expandafter\gdef\csname R@an.fresh_replication.kits.contemp.max\endcsname{84.621}
\expandafter\gdef\csname R@an.fresh_replication.kits.contemp.mean\endcsname{83.866}
\expandafter\gdef\csname R@an.fresh_replication.kits.contemp.min\endcsname{83.230}
\expandafter\gdef\csname R@an.fresh_replication.kits.contemp.n\endcsname{3}
\expandafter\gdef\csname R@an.fresh_replication.kits.contemp.nfinished\endcsname{3}
\expandafter\gdef\csname R@an.fresh_replication.kits.contemp.nregistered\endcsname{3}
\expandafter\gdef\csname R@an.fresh_replication.kits.contemp.sd\endcsname{0.703}
\expandafter\gdef\csname R@an.fresh_replication.kits.contemp.shift\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.fresh_replication.kits.contemp.shiftunc\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.kits.contemp.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.defaultadj\endcsname{three-run}
\expandafter\gdef\csname R@an.fresh_replication.kits.defaultmean\endcsname{83.378}
\expandafter\gdef\csname R@an.fresh_replication.kits.defaultn\endcsname{3}
\expandafter\gdef\csname R@an.fresh_replication.kits.defaultsd\endcsname{0.795}
\expandafter\gdef\csname R@an.fresh_replication.kits.deltaclause\endcsname{ResEnc-M \ensuremath{+3.475}\,pp (\ensuremath{+0.353} to \ensuremath{+6.597}\,pp; \ensuremath{+3.232}\,pp, \ensuremath{+1.716} to \ensuremath{+4.747}\,pp, against the six-run reference), LeanDeepMid \ensuremath{+2.662}\,pp (\ensuremath{-0.460} to \ensuremath{+5.784}\,pp; \ensuremath{+2.418}\,pp, \ensuremath{+0.902} to \ensuremath{+3.934}\,pp, against the six-run reference), LeanNeXt-s5 \ensuremath{+2.440}\,pp (\ensuremath{-0.682} to \ensuremath{+5.562}\,pp; \ensuremath{+2.196}\,pp, \ensuremath{+0.680} to \ensuremath{+3.712}\,pp, against the six-run reference), HyReX+dec. capacity \ensuremath{+2.401}\,pp (\ensuremath{-0.721} to \ensuremath{+5.523}\,pp; \ensuremath{+2.157}\,pp, \ensuremath{+0.641} to \ensuremath{+3.673}\,pp, against the six-run reference), LeanSep \ensuremath{+2.382}\,pp (\ensuremath{-0.740} to \ensuremath{+5.504}\,pp; \ensuremath{+2.138}\,pp, \ensuremath{+0.622} to \ensuremath{+3.654}\,pp, against the six-run reference), ResEnc-matched \ensuremath{+2.313}\,pp (\ensuremath{-0.809} to \ensuremath{+5.435}\,pp; \ensuremath{+2.070}\,pp, \ensuremath{+0.554} to \ensuremath{+3.585}\,pp, against the six-run reference), LeanDeepMid+FD \ensuremath{+2.289}\,pp (\ensuremath{-0.833} to \ensuremath{+5.411}\,pp; \ensuremath{+2.046}\,pp, \ensuremath{+0.530} to \ensuremath{+3.561}\,pp, against the six-run reference), LeanAdd \ensuremath{+2.285}\,pp (\ensuremath{-0.837} to \ensuremath{+5.407}\,pp; \ensuremath{+2.042}\,pp, \ensuremath{+0.526} to \ensuremath{+3.557}\,pp, against the six-run reference), ResEnc+context \ensuremath{+2.246}\,pp (\ensuremath{-0.876} to \ensuremath{+5.368}\,pp; \ensuremath{+2.003}\,pp, \ensuremath{+0.487} to \ensuremath{+3.518}\,pp, against the six-run reference), HyReX-LeanDec \ensuremath{+2.165}\,pp (\ensuremath{-0.957} to \ensuremath{+5.287}\,pp; \ensuremath{+1.922}\,pp, \ensuremath{+0.406} to \ensuremath{+3.438}\,pp, against the six-run reference), HyReX \ensuremath{+2.094}\,pp (\ensuremath{-1.028} to \ensuremath{+5.216}\,pp; \ensuremath{+1.850}\,pp, \ensuremath{+0.334} to \ensuremath{+3.366}\,pp, against the six-run reference), LeanDec \ensuremath{+1.892}\,pp (\ensuremath{-1.230} to \ensuremath{+5.014}\,pp; \ensuremath{+1.648}\,pp, \ensuremath{+0.132} to \ensuremath{+3.164}\,pp, against the six-run reference), StackDec \ensuremath{+1.877}\,pp (\ensuremath{-1.245} to \ensuremath{+4.999}\,pp; \ensuremath{+1.634}\,pp, \ensuremath{+0.118} to \ensuremath{+3.149}\,pp, against the six-run reference), LeanDil \ensuremath{+1.838}\,pp (\ensuremath{-1.284} to \ensuremath{+4.960}\,pp; \ensuremath{+1.595}\,pp, \ensuremath{+0.079} to \ensuremath{+3.111}\,pp, against the six-run reference), Stem1 \ensuremath{+1.731}\,pp (\ensuremath{-1.391} to \ensuremath{+4.853}\,pp; \ensuremath{+1.487}\,pp, \ensuremath{-0.028} to \ensuremath{+3.003}\,pp, against the six-run reference), HyReX-k9 \ensuremath{+1.704}\,pp (\ensuremath{-1.418} to \ensuremath{+4.826}\,pp; \ensuremath{+1.461}\,pp, \ensuremath{-0.055} to \ensuremath{+2.976}\,pp, against the six-run reference), HyReX+context \ensuremath{+1.591}\,pp (\ensuremath{-1.531} to \ensuremath{+4.713}\,pp; \ensuremath{+1.348}\,pp, \ensuremath{-0.168} to \ensuremath{+2.864}\,pp, against the six-run reference), HyReX point-fuse \ensuremath{+1.477}\,pp (\ensuremath{-1.645} to \ensuremath{+4.599}\,pp; \ensuremath{+1.233}\,pp, \ensuremath{-0.283} to \ensuremath{+2.749}\,pp, against the six-run reference), LeanAdd-NeXt \ensuremath{+1.448}\,pp (\ensuremath{-1.674} to \ensuremath{+4.570}\,pp; \ensuremath{+1.205}\,pp, \ensuremath{-0.311} to \ensuremath{+2.720}\,pp, against the six-run reference), LeanTrunk \ensuremath{+1.375}\,pp (\ensuremath{-1.747} to \ensuremath{+4.497}\,pp; \ensuremath{+1.131}\,pp, \ensuremath{-0.385} to \ensuremath{+2.647}\,pp, against the six-run reference), CoarseStack \ensuremath{+1.249}\,pp (\ensuremath{-1.873} to \ensuremath{+4.371}\,pp; \ensuremath{+1.005}\,pp, \ensuremath{-0.511} to \ensuremath{+2.521}\,pp, against the six-run reference), the fn.-identical control \ensuremath{+1.176}\,pp (\ensuremath{-1.946} to \ensuremath{+4.298}\,pp; \ensuremath{+0.932}\,pp, \ensuremath{-0.584} to \ensuremath{+2.448}\,pp, against the six-run reference), the branch control \ensuremath{+1.067}\,pp (\ensuremath{-2.055} to \ensuremath{+4.189}\,pp; \ensuremath{+0.823}\,pp, \ensuremath{-0.693} to \ensuremath{+2.339}\,pp, against the six-run reference), HyReX, finer ConvNeXt \ensuremath{+0.570}\,pp (\ensuremath{-2.552} to \ensuremath{+3.692}\,pp; \ensuremath{+0.326}\,pp, \ensuremath{-1.189} to \ensuremath{+1.842}\,pp, against the six-run reference) and ConvNeXt-k3 \ensuremath{+0.110}\,pp (\ensuremath{-3.012} to \ensuremath{+3.232}\,pp; \ensuremath{-0.133}\,pp, \ensuremath{-1.649} to \ensuremath{+1.382}\,pp, against the six-run reference)}
\expandafter\gdef\csname R@an.fresh_replication.kits.freshL3minusL1\endcsname{\ensuremath{-1.382}}
\expandafter\gdef\csname R@an.fresh_replication.kits.freshL3minusL1.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.freshabovelist.pool\endcsname{HyReX, ResEnc-M, ResEnc-matched, ResEnc+context, HyReX+context, HyReX point-fuse, HyReX+dec. capacity, LeanDec, fn.-identical control, LeanAdd, LeanAdd-NeXt, HyReX-LeanDec, Stem1, CoarseStack, StackDec, LeanDeepMid+FD, LeanSep, LeanDil, LeanDeepMid, LeanNeXt-s5, HyReX-k9}
\expandafter\gdef\csname R@an.fresh_replication.kits.freshabovelist.union\endcsname{HyReX, ResEnc-M, ResEnc-matched, ResEnc+context, HyReX+dec. capacity, LeanDec, LeanAdd, LeanAdd-NeXt, HyReX-LeanDec, Stem1, StackDec, LeanDeepMid+FD, LeanSep, LeanDil, LeanDeepMid, LeanNeXt-s5, HyReX-k9}
\expandafter\gdef\csname R@an.fresh_replication.kits.freshbelowbarlist\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.fresh_replication.kits.freshnotabovelist.pool\endcsname{ConvNeXt-k3, branch control, HyReX, finer ConvNeXt, LeanTrunk}
\expandafter\gdef\csname R@an.fresh_replication.kits.freshnotabovelist.union\endcsname{ConvNeXt-k3, HyReX+context, branch control, HyReX, finer ConvNeXt, HyReX point-fuse, fn.-identical control, LeanTrunk, CoarseStack}
\expandafter\gdef\csname R@an.fresh_replication.kits.freshresolvedlist\endcsname{HyReX, ResEnc-M, ResEnc-matched, ResEnc+context, HyReX+context, branch control, HyReX, finer ConvNeXt, HyReX point-fuse, HyReX+dec. capacity, LeanDec, fn.-identical control, LeanAdd, LeanAdd-NeXt, HyReX-LeanDec, LeanTrunk, Stem1, CoarseStack, StackDec, LeanDeepMid+FD, LeanSep, LeanDil, LeanDeepMid, LeanNeXt-s5, HyReX-k9}
\expandafter\gdef\csname R@an.fresh_replication.kits.freshunresolvedlist\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.fresh_replication.kits.leaderclause\endcsname{the two highest fresh-seed deltas, ResEnc-M \ensuremath{+3.475}\,pp (\ensuremath{+3.232}\,pp against the six-run reference) and LeanDeepMid \ensuremath{+2.662}\,pp (\ensuremath{+2.418}\,pp against the six-run reference), are 0.814\,pp apart, a margin above the registered 0.50\,pp one-seed pair floor}
\expandafter\gdef\csname R@an.fresh_replication.kits.leaderclause.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.nbarflip.fresh\endcsname{1}
\expandafter\gdef\csname R@an.fresh_replication.kits.nbarflip.phrase\endcsname{under the six-run reference 1 fresh-mean and 0 discovery-seed threshold readings change side of the registered 0.35\,pp bar (HyReX, finer ConvNeXt)}
\expandafter\gdef\csname R@an.fresh_replication.kits.nbarflip.s0\endcsname{0}
\expandafter\gdef\csname R@an.fresh_replication.kits.nbelowref\endcsname{24}
\expandafter\gdef\csname R@an.fresh_replication.kits.ncases\endcsname{98}
\expandafter\gdef\csname R@an.fresh_replication.kits.nfreshabove.pool\endcsname{21}
\expandafter\gdef\csname R@an.fresh_replication.kits.nfreshabove.union\endcsname{17}
\expandafter\gdef\csname R@an.fresh_replication.kits.nfreshbelowbar\endcsname{1}
\expandafter\gdef\csname R@an.fresh_replication.kits.nfreshclearsbar\endcsname{24}
\expandafter\gdef\csname R@an.fresh_replication.kits.nfreshnotabove.pool\endcsname{4}
\expandafter\gdef\csname R@an.fresh_replication.kits.nfreshnotabove.union\endcsname{8}
\expandafter\gdef\csname R@an.fresh_replication.kits.nfreshresolved\endcsname{24}
\expandafter\gdef\csname R@an.fresh_replication.kits.nfreshunresolved\endcsname{1}
\expandafter\gdef\csname R@an.fresh_replication.kits.nmoved\endcsname{25}
\expandafter\gdef\csname R@an.fresh_replication.kits.nnotreproduced\endcsname{1}
\expandafter\gdef\csname R@an.fresh_replication.kits.notreproducedlist\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.fresh_replication.kits.npending\endcsname{0}
\expandafter\gdef\csname R@an.fresh_replication.kits.nregistered\endcsname{25}
\expandafter\gdef\csname R@an.fresh_replication.kits.nreplicated\endcsname{25}
\expandafter\gdef\csname R@an.fresh_replication.kits.nshiftinside\endcsname{20}
\expandafter\gdef\csname R@an.fresh_replication.kits.nshiftoutside\endcsname{5}
\expandafter\gdef\csname R@an.fresh_replication.kits.nvshero\endcsname{24}
\expandafter\gdef\csname R@an.fresh_replication.kits.nvsref\endcsname{24}
\expandafter\gdef\csname R@an.fresh_replication.kits.nwithinhero\endcsname{13}
\expandafter\gdef\csname R@an.fresh_replication.kits.pool.max\endcsname{84.272}
\expandafter\gdef\csname R@an.fresh_replication.kits.pool.min\endcsname{82.749}
\expandafter\gdef\csname R@an.fresh_replication.kits.poolspread\endcsname{1.522}
\expandafter\gdef\csname R@an.fresh_replication.kits.pub.margin\endcsname{\ensuremath{+1.660}}
\expandafter\gdef\csname R@an.fresh_replication.kits.pubdeficit.clause\endcsname{the preset sits 1.432\,pp closer to its published level than the default pool does}
\expandafter\gdef\csname R@an.fresh_replication.kits.pubdeficit.presetcloser\endcsname{\ensuremath{+1.432}}
\expandafter\gdef\csname R@an.fresh_replication.kits.referencearm\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.fresh_replication.kits.refrank.clause\endcsname{ResEnc-M has the highest fresh mean of the 25 arms with a complete fresh pair on KiTS23, 0.814\,pp above the next, LeanDeepMid}
\expandafter\gdef\csname R@an.fresh_replication.kits.replicated.clause\endcsname{all 25 registered arms have a complete fresh pair}
\expandafter\gdef\csname R@an.fresh_replication.kits.runnerupfresharm\endcsname{LeanDeepMid}
\expandafter\gdef\csname R@an.fresh_replication.kits.runnerupfreshdelta\endcsname{\ensuremath{+2.662}}
\expandafter\gdef\csname R@an.fresh_replication.kits.samedefaultfreshmean\endcsname{82.932}
\expandafter\gdef\csname R@an.fresh_replication.kits.samedefaultgap\endcsname{\ensuremath{+0.447}}
\expandafter\gdef\csname R@an.fresh_replication.kits.samedefaultgap.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.samedefaultn\endcsname{3}
\expandafter\gdef\csname R@an.fresh_replication.kits.samedefaultsource\endcsname{frozen pool}
\expandafter\gdef\csname R@an.fresh_replication.kits.sddf\endcsname{2}
\expandafter\gdef\csname R@an.fresh_replication.kits.sdfresh\endcsname{0.726}
\expandafter\gdef\csname R@an.fresh_replication.kits.sdfreshpair\endcsname{0.795}
\expandafter\gdef\csname R@an.fresh_replication.kits.sdshift\endcsname{0.974}
\expandafter\gdef\csname R@an.fresh_replication.kits.sdsingle\endcsname{0.918}
\expandafter\gdef\csname R@an.fresh_replication.kits.shiftinsidelist\endcsname{HyReX, ResEnc-matched, ConvNeXt-k3, ResEnc+context, HyReX+context, HyReX, finer ConvNeXt, HyReX point-fuse, LeanDec, fn.-identical control, LeanAdd, LeanAdd-NeXt, HyReX-LeanDec, Stem1, CoarseStack, StackDec, LeanDeepMid+FD, LeanSep, LeanDeepMid, LeanNeXt-s5, HyReX-k9}
\expandafter\gdef\csname R@an.fresh_replication.kits.shiftoutsidelist\endcsname{ResEnc-M, branch control, HyReX+dec. capacity, LeanTrunk, LeanDil}
\expandafter\gdef\csname R@an.fresh_replication.kits.topfresh.licence\endcsname{a resolved superlative}
\expandafter\gdef\csname R@an.fresh_replication.kits.topfresh.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.topfresharm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.fresh_replication.kits.topfreshdelta\endcsname{\ensuremath{+3.475}}
\expandafter\gdef\csname R@an.fresh_replication.kits.topfreshmargin\endcsname{0.814}
\expandafter\gdef\csname R@an.fresh_replication.kits.topfreshmargin.binding\endcsname{the pool-derived no-effect scale of a fresh-minus-fresh difference (sdfreshpair)}
\expandafter\gdef\csname R@an.fresh_replication.kits.topfreshmargin.inse\endcsname{1.70}
\expandafter\gdef\csname R@an.fresh_replication.kits.topfreshmargin.se\endcsname{0.479}
\expandafter\gdef\csname R@an.fresh_replication.kits.union.adj\endcsname{six-run}
\expandafter\gdef\csname R@an.fresh_replication.kits.union.max\endcsname{84.621}
\expandafter\gdef\csname R@an.fresh_replication.kits.union.mean\endcsname{83.622}
\expandafter\gdef\csname R@an.fresh_replication.kits.union.min\endcsname{82.749}
\expandafter\gdef\csname R@an.fresh_replication.kits.union.n\endcsname{6}
\expandafter\gdef\csname R@an.fresh_replication.kits.union.sd\endcsname{0.722}
\expandafter\gdef\csname R@an.fresh_replication.kits.union.sddf\endcsname{5}
\expandafter\gdef\csname R@an.fresh_replication.kits.union.sdfresh\endcsname{0.590}
\expandafter\gdef\csname R@an.fresh_replication.kits.union.shift\endcsname{\ensuremath{+0.244}}
\expandafter\gdef\csname R@an.fresh_replication.kits.union.status\endcsname{complete}
\expandafter\gdef\csname R@an.fresh_replication.kits.withinhero.clause\endcsname{of the 24 other arms with a complete fresh pair, 13 lie inside the registered 0.50\,pp one-seed pair floor of HyReX's fresh mean: ResEnc-matched, ResEnc+context, HyReX+dec. capacity, LeanDec, LeanAdd, HyReX-LeanDec, Stem1, StackDec, LeanDeepMid+FD, LeanSep, LeanDil, LeanNeXt-s5, HyReX-k9}
\expandafter\gdef\csname R@an.fresh_replication.kits.withinherolist\endcsname{ResEnc-matched, ResEnc+context, HyReX+dec. capacity, LeanDec, LeanAdd, HyReX-LeanDec, Stem1, StackDec, LeanDeepMid+FD, LeanSep, LeanDil, LeanNeXt-s5, HyReX-k9}
\expandafter\gdef\csname R@an.fresh_replication.nfreshseeds\endcsname{2}
\expandafter\gdef\csname R@an.fresh_replication.nfreshseeds.word\endcsname{two}
\expandafter\gdef\csname R@an.fresh_replication.nfreshunresolved\endcsname{4}
\expandafter\gdef\csname R@an.fresh_replication.nnotreproduced\endcsname{3}
\expandafter\gdef\csname R@an.fresh_replication.notreproducedlist\endcsname{ConvNeXt-k3 (KiTS23), HyReX (AMOS22), ConvNeXt-k3 (AMOS22)}
\expandafter\gdef\csname R@an.fresh_replication.nreplicated\endcsname{34}
\expandafter\gdef\csname R@an.fresh_replication.nrows\endcsname{36}
\expandafter\gdef\csname R@an.fresh_replication.pairfloor\endcsname{0.50}
\expandafter\gdef\csname R@an.fresh_replication.thresh.primary\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.fresh_replication.withheld.acdclead\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.withheld.acdclead.status\endcsname{withheld}
\expandafter\gdef\csname R@an.fresh_replication.withheld.allthree\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.withheld.allthree.status\endcsname{withheld}
\expandafter\gdef\csname R@an.fresh_replication.withheld.amoscannot\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.withheld.amoscannot.status\endcsname{withheld}
\expandafter\gdef\csname R@an.fresh_replication.withheld.onlysurvivor.kits\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.withheld.onlysurvivor.kits.status\endcsname{withheld}
\expandafter\gdef\csname R@an.fresh_replication.withheld.opattrib.kits\endcsname{\textemdash}
\expandafter\gdef\csname R@an.fresh_replication.withheld.opattrib.kits.status\endcsname{withheld}
\expandafter\gdef\csname R@an.gpu_measures.assd.acdc.L3_L1.d\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.assd.acdc.L3_base.d\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.assd.amos.L3_L1.d\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.gpu_measures.assd.amos.L3_base.d\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.gpu_measures.assd.kits.L3_L1.d\endcsname{\ensuremath{+4.56}}
\expandafter\gdef\csname R@an.gpu_measures.assd.kits.L3_base.d\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.gpu_measures.assdpen.acdc.L3_L1.d\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.assdpen.acdc.L3_base.d\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.assdpen.amos.L3_L1.d\endcsname{\ensuremath{+1.19}}
\expandafter\gdef\csname R@an.gpu_measures.assdpen.amos.L3_base.d\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.gpu_measures.assdpen.kits.L3_L1.d\endcsname{\ensuremath{+3.87}}
\expandafter\gdef\csname R@an.gpu_measures.assdpen.kits.L3_base.d\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.gpu_measures.bd.ncomputable\endcsname{6}
\expandafter\gdef\csname R@an.gpu_measures.bd.nfilled\endcsname{6}
\expandafter\gdef\csname R@an.gpu_measures.bd.nrows\endcsname{6}
\expandafter\gdef\csname R@an.gpu_measures.bd.state\endcsname{6 of the 6 boundary contrasts are complete over folds 1 to 4 (HyReX minus the nnU-Net default, ResEnc-M minus the nnU-Net default and HyReX minus ResEnc-M on AMOS22 and HyReX minus the nnU-Net default, ResEnc-M minus the nnU-Net default and HyReX minus ResEnc-M on KiTS23)}
\expandafter\gdef\csname R@an.gpu_measures.ci.note\endcsname{the intervals are 95\,\% paired-$t$ intervals over folds 1 to 4 (df = 3) with one seed per fold: they describe fold-to-fold variation and not training-seed uncertainty}
\expandafter\gdef\csname R@an.gpu_measures.ckpt.armlist\endcsname{HyReX on AMOS22 (2 replication seeds, 4 cross-validation folds); ResEnc-M on AMOS22 (2 replication seeds, 4 cross-validation folds); HyReX on KiTS23 (4 cross-validation folds); ResEnc-M on KiTS23 (4 cross-validation folds); HyReX on ACDC (2 replication seeds, 4 cross-validation folds); ResEnc-M on ACDC (2 replication seeds, 4 cross-validation folds)}
\expandafter\gdef\csname R@an.gpu_measures.ckpt.arms\endcsname{32}
\expandafter\gdef\csname R@an.gpu_measures.ckpt.armsphrase\endcsname{32 of them design-arm runs}
\expandafter\gdef\csname R@an.gpu_measures.ckpt.default.acdc\endcsname{3 of 6}
\expandafter\gdef\csname R@an.gpu_measures.ckpt.default.amos\endcsname{3 of 6}
\expandafter\gdef\csname R@an.gpu_measures.ckpt.default.kits\endcsname{none}
\expandafter\gdef\csname R@an.gpu_measures.ckpt.kept\endcsname{56}
\expandafter\gdef\csname R@an.gpu_measures.ckpt.ntested\endcsname{75}
\expandafter\gdef\csname R@an.gpu_measures.ckpt.scope\endcsname{the runs the boundary-metrics contrasts draw on, kept / tested by group: fold-0 frozen-pool default runs (AMOS22 3 of 6, KiTS23 0 of 3, ACDC 3 of 6); contemporaneous default runs (seeds 3--5) (AMOS22 3 of 3, KiTS23 3 of 3); default cross-validation folds (AMOS22 4 of 4, KiTS23 4 of 4, ACDC 4 of 4); design-arm fold-0 runs (AMOS22 0 of 2, KiTS23 0 of 2, ACDC 0 of 2); design-arm replication seeds (AMOS22 4 of 4, KiTS23 0 of 4, ACDC 4 of 4); design-arm cross-validation folds (AMOS22 8 of 8, KiTS23 8 of 8, ACDC 8 of 8)}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.acdc.range_off\endcsname{0.033 to 0.040}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.acdc.range_on\endcsname{0.205 to 0.743}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.acdc.spread_off\endcsname{1.20}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.acdc.spread_on\endcsname{3.62}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.acdc.unstable\endcsname{yes}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.acdc.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.acdc.unstable_on\endcsname{yes}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.amos.range_off\endcsname{6.680 to 7.054}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.amos.range_on\endcsname{46.234 to 46.258}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.amos.spread_off\endcsname{1.06}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.amos.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.amos.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.amos.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.amos.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.kits.range_off\endcsname{3.572 to 5.229}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.kits.range_on\endcsname{27.411 to 27.465}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.kits.spread_off\endcsname{1.46}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.kits.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.kits.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.kits.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.D2.kits.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.acdc.range_off\endcsname{0.063 to 0.069}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.acdc.range_on\endcsname{0.379 to 0.386}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.acdc.spread_off\endcsname{1.10}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.acdc.spread_on\endcsname{1.02}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.acdc.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.acdc.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.acdc.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.amos.range_off\endcsname{11.527 to 11.554}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.amos.range_on\endcsname{85.141 to 85.187}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.amos.spread_off\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.amos.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.amos.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.amos.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.amos.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.kits.range_off\endcsname{5.919 to 5.965}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.kits.range_on\endcsname{46.358 to 46.473}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.kits.spread_off\endcsname{1.01}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.kits.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.kits.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.kits.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1.kits.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.acdc.range_off\endcsname{0.057 to 0.086}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.acdc.range_on\endcsname{0.371 to 0.387}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.acdc.spread_off\endcsname{1.51}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.acdc.spread_on\endcsname{1.04}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.acdc.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.acdc.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.acdc.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.amos.range_off\endcsname{11.380 to 11.418}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.amos.range_on\endcsname{84.069 to 84.090}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.amos.spread_off\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.amos.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.amos.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.amos.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.amos.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.kits.range_off\endcsname{5.732 to 5.786}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.kits.range_on\endcsname{44.786 to 44.812}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.kits.spread_off\endcsname{1.01}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.kits.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.kits.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.kits.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L1b.kits.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.acdc.range_off\endcsname{0.054 to 0.063}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.acdc.range_on\endcsname{0.355 to 0.361}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.acdc.spread_off\endcsname{1.17}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.acdc.spread_on\endcsname{1.02}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.acdc.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.acdc.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.acdc.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.amos.range_off\endcsname{11.196 to 11.242}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.amos.range_on\endcsname{82.592 to 82.625}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.amos.spread_off\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.amos.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.amos.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.amos.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.amos.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.kits.range_off\endcsname{5.877 to 5.908}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.kits.range_on\endcsname{45.959 to 45.968}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.kits.spread_off\endcsname{1.01}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.kits.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.kits.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.kits.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L2.kits.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.acdc.range_off\endcsname{0.056 to 0.056}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.acdc.range_on\endcsname{0.383 to 0.394}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.acdc.spread_off\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.acdc.spread_on\endcsname{1.03}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.acdc.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.acdc.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.acdc.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.amos.range_off\endcsname{11.870 to 11.904}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.amos.range_on\endcsname{87.585 to 89.347}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.amos.spread_off\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.amos.spread_on\endcsname{1.02}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.amos.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.amos.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.amos.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.kits.range_off\endcsname{6.180 to 6.198}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.kits.range_on\endcsname{48.325 to 48.598}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.kits.spread_off\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.kits.spread_on\endcsname{1.01}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.kits.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.kits.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L3.kits.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.acdc.range_off\endcsname{0.062 to 0.111}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.acdc.range_on\endcsname{0.400 to 0.413}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.acdc.spread_off\endcsname{1.81}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.acdc.spread_on\endcsname{1.03}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.acdc.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.acdc.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.acdc.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.amos.range_off\endcsname{12.027 to 12.362}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.amos.range_on\endcsname{89.222 to 89.516}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.amos.spread_off\endcsname{1.03}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.amos.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.amos.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.amos.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.amos.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.kits.range_off\endcsname{6.078 to 6.157}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.kits.range_on\endcsname{47.480 to 47.484}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.kits.spread_off\endcsname{1.01}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.kits.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.kits.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.kits.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L4.kits.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.acdc.range_off\endcsname{0.066 to 0.080}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.acdc.range_on\endcsname{0.451 to 0.458}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.acdc.spread_off\endcsname{1.22}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.acdc.spread_on\endcsname{1.02}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.acdc.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.acdc.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.acdc.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.amos.range_off\endcsname{13.483 to 13.497}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.amos.range_on\endcsname{100.842 to 100.847}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.amos.spread_off\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.amos.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.amos.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.amos.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.amos.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.kits.range_off\endcsname{6.890 to 6.909}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.kits.range_on\endcsname{53.928 to 53.961}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.kits.spread_off\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.kits.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.kits.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.kits.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.L6.kits.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.acdc.range_off\endcsname{0.046 to 0.082}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.acdc.range_on\endcsname{0.276 to 2.274}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.acdc.spread_off\endcsname{1.79}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.acdc.spread_on\endcsname{8.25}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.acdc.unstable\endcsname{yes}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.acdc.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.acdc.unstable_on\endcsname{yes}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.amos.range_off\endcsname{8.097 to 8.124}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.amos.range_on\endcsname{54.758 to 54.779}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.amos.spread_off\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.amos.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.amos.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.amos.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.amos.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.kits.range_off\endcsname{3.941 to 3.970}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.kits.range_on\endcsname{30.167 to 31.285}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.kits.spread_off\endcsname{1.01}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.kits.spread_on\endcsname{1.04}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.kits.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.kits.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7A1.kits.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.acdc.range_off\endcsname{0.035 to 0.037}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.acdc.range_on\endcsname{0.192 to 0.201}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.acdc.spread_off\endcsname{1.07}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.acdc.spread_on\endcsname{1.05}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.acdc.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.acdc.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.acdc.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.amos.range_off\endcsname{6.700 to 6.826}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.amos.range_on\endcsname{44.122 to 44.153}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.amos.spread_off\endcsname{1.02}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.amos.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.amos.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.amos.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.amos.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.kits.range_off\endcsname{3.397 to 3.428}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.kits.range_on\endcsname{25.806 to 25.849}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.kits.spread_off\endcsname{1.01}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.kits.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.kits.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.kits.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V7C1.kits.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.acdc.range_off\endcsname{0.038 to 0.046}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.acdc.range_on\endcsname{0.238 to 0.278}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.acdc.spread_off\endcsname{1.23}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.acdc.spread_on\endcsname{1.16}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.acdc.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.acdc.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.acdc.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.amos.range_off\endcsname{7.325 to 8.463}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.amos.range_on\endcsname{48.748 to 48.898}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.amos.spread_off\endcsname{1.16}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.amos.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.amos.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.amos.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.amos.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.kits.range_off\endcsname{3.744 to 3.764}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.kits.range_on\endcsname{28.642 to 28.671}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.kits.spread_off\endcsname{1.01}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.kits.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.kits.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.kits.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8A1.kits.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.acdc.range_off\endcsname{0.045 to 0.090}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.acdc.range_on\endcsname{0.154 to 0.184}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.acdc.spread_off\endcsname{1.99}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.acdc.spread_on\endcsname{1.19}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.acdc.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.acdc.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.acdc.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.amos.range_off\endcsname{5.310 to 5.386}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.amos.range_on\endcsname{33.343 to 33.434}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.amos.spread_off\endcsname{1.01}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.amos.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.amos.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.amos.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.amos.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.kits.range_off\endcsname{2.537 to 2.555}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.kits.range_on\endcsname{18.774 to 18.791}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.kits.spread_off\endcsname{1.01}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.kits.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.kits.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.kits.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B1.kits.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.acdc.range_off\endcsname{0.035 to 0.048}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.acdc.range_on\endcsname{0.167 to 0.176}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.acdc.spread_off\endcsname{1.37}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.acdc.spread_on\endcsname{1.06}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.acdc.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.acdc.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.acdc.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.amos.range_off\endcsname{5.786 to 5.901}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.amos.range_on\endcsname{36.898 to 37.199}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.amos.spread_off\endcsname{1.02}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.amos.spread_on\endcsname{1.01}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.amos.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.amos.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.amos.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.kits.range_off\endcsname{2.690 to 2.695}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.kits.range_on\endcsname{20.154 to 20.172}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.kits.spread_off\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.kits.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.kits.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.kits.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.V8B2.kits.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.acdc.range_off\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.acdc.range_on\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.acdc.spread_off\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.acdc.spread_on\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.acdc.unstable\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.acdc.unstable_off\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.acdc.unstable_on\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.amos.range_off\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.amos.range_on\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.amos.spread_off\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.amos.spread_on\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.amos.unstable\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.amos.unstable_off\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.amos.unstable_on\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.kits.range_off\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.kits.range_on\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.kits.spread_off\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.kits.spread_on\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.kits.unstable\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.kits.unstable_off\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.cost.W4.kits.unstable_on\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.cost.armlist\endcsname{nnU-Net default, HyReX, ResEnc-M, ResEnc-matched, LeanDec, ConvNeXt-k3, ResEnc+context, HyReX+context, LeanNeXt-s5, LeanDeepMid, LeanTrunk, Stem1 and CoarseStack}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.acdc.range_off\endcsname{0.057 to 0.080}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.acdc.range_on\endcsname{0.255 to 0.264}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.acdc.spread_off\endcsname{1.40}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.acdc.spread_on\endcsname{1.04}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.acdc.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.acdc.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.acdc.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.amos.range_off\endcsname{8.347 to 8.387}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.amos.range_on\endcsname{58.704 to 58.731}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.amos.spread_off\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.amos.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.amos.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.amos.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.amos.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.kits.range_off\endcsname{4.551 to 4.563}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.kits.range_on\endcsname{35.125 to 35.167}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.kits.spread_off\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.kits.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.kits.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.kits.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.base.kits.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.new.armlist\endcsname{LeanNeXt-s5, LeanDeepMid, LeanTrunk, Stem1 and CoarseStack}
\expandafter\gdef\csname R@an.gpu_measures.cost.new.nratio\endcsname{15}
\expandafter\gdef\csname R@an.gpu_measures.cost.new.nrec\endcsname{15}
\expandafter\gdef\csname R@an.gpu_measures.cost.new.nstable\endcsname{14}
\expandafter\gdef\csname R@an.gpu_measures.cost.new.nunstable\endcsname{1}
\expandafter\gdef\csname R@an.gpu_measures.cost.new.nwant\endcsname{15}
\expandafter\gdef\csname R@an.gpu_measures.cost.new.sentence\endcsname{against the same-batch default the added designs take LeanNeXt-s5 0.78 on AMOS22, 0.74 on KiTS23, 0.86 on ACDC; LeanDeepMid 0.94 on AMOS22, 0.86 on KiTS23; LeanTrunk 0.62 on AMOS22, 0.56 on KiTS23, 1.26 on ACDC; Stem1 0.68 on AMOS22, 0.59 on KiTS23, 0.89 on ACDC; CoarseStack 0.86 on AMOS22, 0.82 on KiTS23, 1.03 on ACDC of its seconds per volume with mirroring off; 1 of 15 measured cells had repeats spanning more than a factor of 2 and are not quoted; between its two records the default's own seconds per volume moved by -28.0\,\% on ACDC, more than its repeats within a batch show}
\expandafter\gdef\csname R@an.gpu_measures.cost.nextra\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.cost.nrec\endcsname{39}
\expandafter\gdef\csname R@an.gpu_measures.cost.nunstable\endcsname{2}
\expandafter\gdef\csname R@an.gpu_measures.cost.nwant\endcsname{39}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.acdc.range_off\endcsname{0.043 to 0.043}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.acdc.range_on\endcsname{0.259 to 0.268}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.acdc.spread_off\endcsname{1.01}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.acdc.spread_on\endcsname{1.03}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.acdc.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.acdc.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.acdc.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.amos.range_off\endcsname{8.551 to 9.886}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.amos.range_on\endcsname{59.072 to 59.147}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.amos.spread_off\endcsname{1.16}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.amos.spread_on\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.amos.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.amos.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.amos.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.kits.range_off\endcsname{4.571 to 4.583}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.kits.range_on\endcsname{35.143 to 35.326}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.kits.spread_off\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.kits.spread_on\endcsname{1.01}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.kits.unstable\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.kits.unstable_off\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.kits.unstable_on\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.nrec\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.nunstable\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.nwant\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.cost.ref.unstablelist\endcsname{none}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.acdc.ga\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.acdc.gb\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.acdc.gflops\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.acdc.params\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.acdc.patch_ms\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.acdc.s_vol\endcsname{\ensuremath{-28.0}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.acdc.s_vol_tta\endcsname{\ensuremath{+3.9}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.amos.ga\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.amos.gb\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.amos.gflops\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.amos.params\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.amos.patch_ms\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.amos.s_vol\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.amos.s_vol_tta\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.atlasdate\endcsname{2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.kits.ga\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.kits.gb\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.kits.gflops\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.kits.params\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.kits.patch_ms\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.kits.s_vol\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.kits.s_vol_tta\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.max\endcsname{28.0}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.ncells\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.nwant\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.refdate\endcsname{2026-10-10}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.sentence\endcsname{measured again in the batch of the 5 added designs, the nnU-Net default reads AMOS22 +2.7\,\%, KiTS23 +0.3\,\%, ACDC -28.0\,\% in seconds per volume against its record of 2026-10-07 (the largest of the three timings moved by 28.0\,\%); its parameters and arithmetic are identical}
\expandafter\gdef\csname R@an.gpu_measures.cost.refdrift.struct\endcsname{identical}
\expandafter\gdef\csname R@an.gpu_measures.cost.unstable.list\endcsname{LeanDec on ACDC and LeanDeepMid on ACDC}
\expandafter\gdef\csname R@an.gpu_measures.cost.unstable.note\endcsname{a dagger marks a cell whose repeats span more than a factor of 2: its median is printed with the range of its repeats and it is not quoted in the sentences}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_L1.d\endcsname{\ensuremath{+0.208}}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_L1.d0\endcsname{\ensuremath{+0.281}}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_L1.d0clause\endcsname{HyReX minus ResEnc-M at seed 0 of each arm is \ensuremath{+0.281} pp, which is inside the registered 0.5 pp one-seed pair floor: the difference is not resolved against the floor at one seed per arm, and no ordering is read from it}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_L1.d0est\endcsname{seed 0 of each arm}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_L1.d0flip\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_L1.d0se\endcsname{0.140}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_L1.dfresh\endcsname{\ensuremath{+0.208}}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_L1.dfreshest\endcsname{2 fresh seeds per arm}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_L1.est\endcsname{2 fresh seeds $-$ 2 fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_L1.estlong\endcsname{fresh mean, seeds 1--2 for HyReX against fresh mean, seeds 1--2 for ResEnc-M}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_L1.mixed\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_L1.repred\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_L1.se\endcsname{0.099}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_L1.sens\endcsname{\ensuremath{+0.208}}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_L1.z\endcsname{\ensuremath{+2.11}}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_base.d\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_base.d0\endcsname{\ensuremath{+0.616}}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_base.d0est\endcsname{seed 0 $-$ frozen pool}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_base.d0flip\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_base.dfresh\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_base.dfreshest\endcsname{2 fresh seeds $-$ frozen pool}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_base.est\endcsname{2 fresh seeds $-$ frozen pool}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_base.estlong\endcsname{fresh mean, seeds 1--2 for HyReX against frozen pool mean, 6 runs for nnU-Net default}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_base.mixed\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_base.repred\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_base.se\endcsname{0.081}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_base.sens\endcsname{\ensuremath{+0.443}}
\expandafter\gdef\csname R@an.gpu_measures.dice.acdc.L3_base.z\endcsname{\ensuremath{+5.58}}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_L1.d\endcsname{\ensuremath{-0.332}}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_L1.d0\endcsname{\ensuremath{-0.265}}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_L1.d0clause\endcsname{HyReX minus ResEnc-M at seed 0 of each arm is \ensuremath{-0.265} pp, which is inside the registered 0.5 pp one-seed pair floor and above the gap's own null SD of 0.173 pp: the difference is not resolved against the floor at one seed per arm, and no ordering is read from it}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_L1.d0est\endcsname{seed 0 of each arm}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_L1.d0flip\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_L1.d0se\endcsname{0.173}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_L1.dfresh\endcsname{\ensuremath{-0.332}}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_L1.dfreshest\endcsname{2 fresh seeds per arm}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_L1.est\endcsname{2 fresh seeds $-$ 2 fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_L1.estlong\endcsname{fresh mean, seeds 1--2 for HyReX against fresh mean, seeds 1--2 for ResEnc-M}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_L1.mixed\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_L1.repred\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_L1.se\endcsname{0.122}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_L1.sens\endcsname{\ensuremath{-0.332}}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_L1.z\endcsname{\ensuremath{-2.72}}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_base.d\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_base.d0\endcsname{\ensuremath{+0.382}}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_base.d0est\endcsname{seed 0 $-$ frozen pool}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_base.d0flip\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_base.dfresh\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_base.dfreshest\endcsname{2 fresh seeds $-$ frozen pool}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_base.est\endcsname{2 fresh seeds $-$ frozen pool}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_base.estlong\endcsname{fresh mean, seeds 1--2 for HyReX against frozen pool mean, 6 runs for nnU-Net default}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_base.mixed\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_base.repred\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_base.se\endcsname{0.100}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_base.sens\endcsname{\ensuremath{+0.104}}
\expandafter\gdef\csname R@an.gpu_measures.dice.amos.L3_base.z\endcsname{\ensuremath{+1.33}}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_L1.d\endcsname{\ensuremath{-1.382}}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_L1.d0\endcsname{\ensuremath{+0.516}}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_L1.d0clause\endcsname{HyReX minus ResEnc-M at seed 0 of each arm is \ensuremath{+0.516} pp, which is above the registered 0.5 pp one-seed pair floor and inside the gap's own null SD of 1.124 pp: the difference is not resolved against the gap's own null SD at one seed per arm, and no ordering is read from it; the registered contrast of the two arms (fresh mean, seeds 1--2 for each arm) has the opposite sign, \ensuremath{-1.382} pp}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_L1.d0est\endcsname{seed 0 of each arm}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_L1.d0flip\endcsname{yes}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_L1.d0se\endcsname{1.124}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_L1.dfresh\endcsname{\ensuremath{-1.382}}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_L1.dfreshest\endcsname{2 fresh seeds per arm}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_L1.est\endcsname{2 fresh seeds $-$ 2 fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_L1.estlong\endcsname{fresh mean, seeds 1--2 for HyReX against fresh mean, seeds 1--2 for ResEnc-M}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_L1.mixed\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_L1.repred\endcsname{\ensuremath{-1.47}}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_L1.se\endcsname{0.795}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_L1.sens\endcsname{\ensuremath{-1.382}}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_L1.z\endcsname{\ensuremath{-1.74}}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_base.d\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_base.d0\endcsname{\ensuremath{+2.842}}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_base.d0est\endcsname{seed 0 $-$ frozen pool}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_base.d0flip\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_base.dfresh\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_base.dfreshest\endcsname{2 fresh seeds $-$ frozen pool}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_base.est\endcsname{2 fresh seeds $-$ frozen pool}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_base.estlong\endcsname{fresh mean, seeds 1--2 for HyReX against frozen pool mean, 3 runs for nnU-Net default}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_base.mixed\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_base.repred\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_base.se\endcsname{0.726}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_base.sens\endcsname{\ensuremath{+1.606}}
\expandafter\gdef\csname R@an.gpu_measures.dice.kits.L3_base.z\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.L1.f1\endcsname{\ensuremath{+0.289}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.L1.f2\endcsname{\ensuremath{+0.626}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.L1.f3\endcsname{\ensuremath{+0.461}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.L1.f4\endcsname{\ensuremath{+0.565}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.L1.max\endcsname{\ensuremath{+0.626}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.L1.mean\endcsname{\ensuremath{+0.485}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.L1.min\endcsname{\ensuremath{+0.289}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.L1.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.L1.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.L3.f1\endcsname{\ensuremath{+0.315}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.L3.f2\endcsname{\ensuremath{+0.431}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.L3.f3\endcsname{\ensuremath{+0.325}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.L3.f4\endcsname{\ensuremath{+0.711}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.L3.max\endcsname{\ensuremath{+0.711}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.L3.mean\endcsname{\ensuremath{+0.446}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.L3.min\endcsname{\ensuremath{+0.315}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.L3.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.L3.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.P3c.f1\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.P3c.f2\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.P3c.f3\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.P3c.f4\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.P3c.max\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.P3c.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.P3c.min\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.P3c.n\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.P3c.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.base.f1\endcsname{\ensuremath{+0.342}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.base.f2\endcsname{\ensuremath{+0.817}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.base.f3\endcsname{\ensuremath{+0.094}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.base.f4\endcsname{\ensuremath{+0.669}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.base.max\endcsname{\ensuremath{+0.817}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.base.mean\endcsname{\ensuremath{+0.481}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.base.min\endcsname{\ensuremath{+0.094}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.base.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.base.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.clause\endcsname{on AMOS22 the mirroring increment over folds 1 to 4 (per-fold values in parentheses) reads: the nnU-Net default \ensuremath{+0.481}\,pp (\ensuremath{+0.342}, \ensuremath{+0.817}, \ensuremath{+0.094}, \ensuremath{+0.669}); ResEnc-M \ensuremath{+0.485}\,pp (\ensuremath{+0.289}, \ensuremath{+0.626}, \ensuremath{+0.461}, \ensuremath{+0.565}); HyReX \ensuremath{+0.446}\,pp (\ensuremath{+0.315}, \ensuremath{+0.431}, \ensuremath{+0.325}, \ensuremath{+0.711})}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L1base.f1\endcsname{\ensuremath{-0.053}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L1base.f2\endcsname{\ensuremath{-0.191}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L1base.f3\endcsname{\ensuremath{+0.366}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L1base.f4\endcsname{\ensuremath{-0.104}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L1base.mean\endcsname{\ensuremath{+0.005}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L3L1.f1\endcsname{\ensuremath{+0.026}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L3L1.f2\endcsname{\ensuremath{-0.194}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L3L1.f3\endcsname{\ensuremath{-0.135}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L3L1.f4\endcsname{\ensuremath{+0.146}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L3L1.mean\endcsname{\ensuremath{-0.039}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L3P3c.f1\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L3P3c.f2\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L3P3c.f3\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L3P3c.f4\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L3P3c.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L3base.f1\endcsname{\ensuremath{-0.026}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L3base.f2\endcsname{\ensuremath{-0.385}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L3base.f3\endcsname{\ensuremath{+0.231}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L3base.f4\endcsname{\ensuremath{+0.042}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.L3base.mean\endcsname{\ensuremath{-0.035}}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.P3cbase.f1\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.P3cbase.f2\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.P3cbase.f3\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.P3cbase.f4\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.d.P3cbase.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.list\endcsname{the nnU-Net default \ensuremath{+0.481}\,pp (\ensuremath{+0.342}, \ensuremath{+0.817}, \ensuremath{+0.094}, \ensuremath{+0.669}); ResEnc-M \ensuremath{+0.485}\,pp (\ensuremath{+0.289}, \ensuremath{+0.626}, \ensuremath{+0.461}, \ensuremath{+0.565}); HyReX \ensuremath{+0.446}\,pp (\ensuremath{+0.315}, \ensuremath{+0.431}, \ensuremath{+0.325}, \ensuremath{+0.711})}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.spread\endcsname{0.039}
\expandafter\gdef\csname R@an.gpu_measures.e1.amos.xclause\endcsname{on AMOS22 the mirroring increment of the function-identical control is not measured yet}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.L1.f1\endcsname{\ensuremath{+1.387}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.L1.f2\endcsname{\ensuremath{+0.502}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.L1.f3\endcsname{\ensuremath{+0.994}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.L1.f4\endcsname{\ensuremath{+0.579}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.L1.max\endcsname{\ensuremath{+1.387}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.L1.mean\endcsname{\ensuremath{+0.866}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.L1.min\endcsname{\ensuremath{+0.502}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.L1.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.L1.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.L3.f1\endcsname{\ensuremath{+1.209}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.L3.f2\endcsname{\ensuremath{+1.727}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.L3.f3\endcsname{\ensuremath{+1.551}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.L3.f4\endcsname{\ensuremath{+1.166}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.L3.max\endcsname{\ensuremath{+1.727}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.L3.mean\endcsname{\ensuremath{+1.413}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.L3.min\endcsname{\ensuremath{+1.166}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.L3.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.L3.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.P3c.f1\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.P3c.f2\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.P3c.f3\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.P3c.f4\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.P3c.max\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.P3c.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.P3c.min\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.P3c.n\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.P3c.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.base.f1\endcsname{\ensuremath{+2.394}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.base.f2\endcsname{\ensuremath{+1.441}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.base.f3\endcsname{\ensuremath{+1.118}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.base.f4\endcsname{\ensuremath{+1.129}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.base.max\endcsname{\ensuremath{+2.394}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.base.mean\endcsname{\ensuremath{+1.520}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.base.min\endcsname{\ensuremath{+1.118}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.base.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.base.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.clause\endcsname{on KiTS23 the mirroring increment over folds 1 to 4 (per-fold values in parentheses) reads: the nnU-Net default \ensuremath{+1.520}\,pp (\ensuremath{+2.394}, \ensuremath{+1.441}, \ensuremath{+1.118}, \ensuremath{+1.129}); ResEnc-M \ensuremath{+0.866}\,pp (\ensuremath{+1.387}, \ensuremath{+0.502}, \ensuremath{+0.994}, \ensuremath{+0.579}); HyReX \ensuremath{+1.413}\,pp (\ensuremath{+1.209}, \ensuremath{+1.727}, \ensuremath{+1.551}, \ensuremath{+1.166})}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L1base.f1\endcsname{\ensuremath{-1.007}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L1base.f2\endcsname{\ensuremath{-0.939}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L1base.f3\endcsname{\ensuremath{-0.123}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L1base.f4\endcsname{\ensuremath{-0.550}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L1base.mean\endcsname{\ensuremath{-0.655}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L3L1.f1\endcsname{\ensuremath{-0.179}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L3L1.f2\endcsname{\ensuremath{+1.225}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L3L1.f3\endcsname{\ensuremath{+0.557}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L3L1.f4\endcsname{\ensuremath{+0.587}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L3L1.mean\endcsname{\ensuremath{+0.548}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L3P3c.f1\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L3P3c.f2\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L3P3c.f3\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L3P3c.f4\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L3P3c.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L3base.f1\endcsname{\ensuremath{-1.186}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L3base.f2\endcsname{\ensuremath{+0.286}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L3base.f3\endcsname{\ensuremath{+0.433}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L3base.f4\endcsname{\ensuremath{+0.037}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.L3base.mean\endcsname{\ensuremath{-0.107}}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.P3cbase.f1\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.P3cbase.f2\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.P3cbase.f3\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.P3cbase.f4\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.d.P3cbase.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.list\endcsname{the nnU-Net default \ensuremath{+1.520}\,pp (\ensuremath{+2.394}, \ensuremath{+1.441}, \ensuremath{+1.118}, \ensuremath{+1.129}); ResEnc-M \ensuremath{+0.866}\,pp (\ensuremath{+1.387}, \ensuremath{+0.502}, \ensuremath{+0.994}, \ensuremath{+0.579}); HyReX \ensuremath{+1.413}\,pp (\ensuremath{+1.209}, \ensuremath{+1.727}, \ensuremath{+1.551}, \ensuremath{+1.166})}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.spread\endcsname{0.655}
\expandafter\gdef\csname R@an.gpu_measures.e1.kits.xclause\endcsname{on KiTS23 the mirroring increment of the function-identical control is not measured yet}
\expandafter\gdef\csname R@an.gpu_measures.e1.ncells\endcsname{24}
\expandafter\gdef\csname R@an.gpu_measures.e1.npos\endcsname{24}
\expandafter\gdef\csname R@an.gpu_measures.e1.nwant\endcsname{24}
\expandafter\gdef\csname R@an.gpu_measures.e1.spreadclause\endcsname{the mean mirroring increments of the three arms differ by at most 0.039\,pp on AMOS22 and 0.655\,pp on KiTS23}
\expandafter\gdef\csname R@an.gpu_measures.e1.status\endcsname{measured on all 24 arm $\times$ dataset $\times$ fold cells}
\expandafter\gdef\csname R@an.gpu_measures.e1.xncells\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e1.xnwant\endcsname{8}
\expandafter\gdef\csname R@an.gpu_measures.e1.xstatus\endcsname{the extension arm is not measured on any fold yet}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.changed\endcsname{yes}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.chg\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.name\endcsname{ResEnc-M minus the nnU-Net default}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.off.ci\endcsname{[\ensuremath{-0.27}, \ensuremath{+1.09}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.off.dcv\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.off.f1\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.off.f2\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.off.f3\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.off.f4\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.off.hi\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.off.lo\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.off.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.off.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.off.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.on.ci\endcsname{[\ensuremath{+0.09}, \ensuremath{+0.73}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.on.dcv\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.on.f1\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.on.f2\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.on.f3\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.on.f4\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.on.hi\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.on.lo\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.on.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.on.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.on.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L1base.wordchg\endcsname{the registered wording changes from "improves on average (3/4 folds)" to "improves in every fold"}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.changed\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.chg\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.chgrev\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.name\endcsname{HyReX minus ResEnc-M}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.off.ci\endcsname{[\ensuremath{-0.76}, \ensuremath{+0.40}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.off.cirev\endcsname{[\ensuremath{-0.40}, \ensuremath{+0.76}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.off.dcv\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.off.dcvrev\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.off.f1\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.off.f2\endcsname{\ensuremath{-0.41}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.off.f3\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.off.f4\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.off.hi\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.off.lo\endcsname{\ensuremath{-0.76}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.off.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.off.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.off.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.off.wordrev\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.on.ci\endcsname{[\ensuremath{-0.77}, \ensuremath{+0.34}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.on.cirev\endcsname{[\ensuremath{-0.34}, \ensuremath{+0.77}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.on.dcv\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.on.dcvrev\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.on.f1\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.on.f2\endcsname{\ensuremath{-0.60}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.on.f3\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.on.f4\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.on.hi\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.on.lo\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.on.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.on.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.on.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.on.wordrev\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.reversed\endcsname{yes}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3L1.wordchg\endcsname{the registered wording is "does not improve in cross-validation" in both readings}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.changed\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.chg\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.name\endcsname{HyReX minus the function-identical control}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.off.ci\endcsname{[\ensuremath{-0.03}, \ensuremath{+0.55}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.off.dcv\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.off.f1\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.off.f2\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.off.f3\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.off.f4\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.off.hi\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.off.lo\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.off.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.off.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.off.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.on.ci\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.on.dcv\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.on.f1\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.on.f2\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.on.f3\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.on.f4\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.on.hi\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.on.lo\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.on.n\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.on.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.on.word\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3P3c.wordchg\endcsname{the mirroring-on reading is pending}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.changed\endcsname{yes}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.chg\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.name\endcsname{HyReX minus the nnU-Net default}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.off.ci\endcsname{[\ensuremath{-0.08}, \ensuremath{+0.54}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.off.dcv\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.off.f1\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.off.f2\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.off.f3\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.off.f4\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.off.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.off.lo\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.off.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.off.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.off.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.on.ci\endcsname{[\ensuremath{-0.23}, \ensuremath{+0.62}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.on.dcv\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.on.f1\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.on.f2\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.on.f3\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.on.f4\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.on.hi\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.on.lo\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.on.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.on.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.on.word\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.L3base.wordchg\endcsname{the registered wording changes from "improves on average (3/4 folds)" to "improves on average (2/4 folds)"}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.changed\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.chg\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.name\endcsname{the function-identical control minus the nnU-Net default}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.off.ci\endcsname{[\ensuremath{-0.57}, \ensuremath{+0.51}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.off.dcv\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.off.f1\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.off.f2\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.off.f3\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.off.f4\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.off.hi\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.off.lo\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.off.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.off.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.off.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.on.ci\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.on.dcv\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.on.f1\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.on.f2\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.on.f3\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.on.f4\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.on.hi\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.on.lo\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.on.n\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.on.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.on.word\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.P3cbase.wordchg\endcsname{the mirroring-on reading is pending}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.clause\endcsname{on AMOS22, HyReX minus the nnU-Net default \ensuremath{+0.23}\,pp [\ensuremath{-0.08}, \ensuremath{+0.54}], improves on average (3/4 folds) with mirroring off and \ensuremath{+0.19}\,pp [\ensuremath{-0.23}, \ensuremath{+0.62}], improves on average (2/4 folds) with mirroring on (a change of \ensuremath{-0.03}\,pp); ResEnc-M minus the nnU-Net default \ensuremath{+0.41}\,pp [\ensuremath{-0.27}, \ensuremath{+1.09}], improves on average (3/4 folds) with mirroring off and \ensuremath{+0.41}\,pp [\ensuremath{+0.09}, \ensuremath{+0.73}], improves in every fold with mirroring on (a change of \ensuremath{0.00}\,pp); ResEnc-M minus HyReX \ensuremath{+0.18}\,pp [\ensuremath{-0.40}, \ensuremath{+0.76}], improves on average (3/4 folds) with mirroring off and \ensuremath{+0.22}\,pp [\ensuremath{-0.34}, \ensuremath{+0.77}], improves on average (3/4 folds) with mirroring on (a change of \ensuremath{+0.04}\,pp)}
\expandafter\gdef\csname R@an.gpu_measures.e2.amos.xclause\endcsname{on AMOS22, the function-identical control minus the nnU-Net default \ensuremath{-0.03}\,pp [\ensuremath{-0.57}, \ensuremath{+0.51}], does not improve in cross-validation with mirroring off; HyReX minus the function-identical control \ensuremath{+0.26}\,pp [\ensuremath{-0.03}, \ensuremath{+0.55}], improves in every fold with mirroring off; the mirroring-on reading of the function-identical control minus the nnU-Net default and HyReX minus the function-identical control is pending, with 0 of 4 folds of the function-identical control measured}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.changed\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.chg\endcsname{\ensuremath{-0.65}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.name\endcsname{ResEnc-M minus the nnU-Net default}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.off.ci\endcsname{[\ensuremath{+0.98}, \ensuremath{+3.32}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.off.dcv\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.off.f1\endcsname{\ensuremath{+2.58}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.off.f2\endcsname{\ensuremath{+2.94}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.off.f3\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.off.f4\endcsname{\ensuremath{+1.71}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.off.hi\endcsname{\ensuremath{+3.32}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.off.lo\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.off.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.off.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.off.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.on.ci\endcsname{[\ensuremath{+0.88}, \ensuremath{+2.10}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.on.dcv\endcsname{\ensuremath{+1.49}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.on.f1\endcsname{\ensuremath{+1.57}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.on.f2\endcsname{\ensuremath{+2.00}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.on.f3\endcsname{\ensuremath{+1.23}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.on.f4\endcsname{\ensuremath{+1.16}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.on.hi\endcsname{\ensuremath{+2.10}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.on.lo\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.on.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.on.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.on.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L1base.wordchg\endcsname{the registered wording is "improves in every fold" in both readings}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.changed\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.chg\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.chgrev\endcsname{\ensuremath{-0.55}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.name\endcsname{HyReX minus ResEnc-M}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.off.ci\endcsname{[\ensuremath{-3.17}, \ensuremath{+0.24}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.off.cirev\endcsname{[\ensuremath{-0.24}, \ensuremath{+3.17}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.off.dcv\endcsname{\ensuremath{-1.47}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.off.dcvrev\endcsname{\ensuremath{+1.47}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.off.f1\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.off.f2\endcsname{\ensuremath{-2.74}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.off.f3\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.off.f4\endcsname{\ensuremath{-1.87}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.off.hi\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.off.lo\endcsname{\ensuremath{-3.17}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.off.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.off.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.off.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.off.wordrev\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.on.ci\endcsname{[\ensuremath{-1.81}, \ensuremath{-0.02}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.on.cirev\endcsname{[\ensuremath{+0.02}, \ensuremath{+1.81}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.on.dcv\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.on.dcvrev\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.on.f1\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.on.f2\endcsname{\ensuremath{-1.52}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.on.f3\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.on.f4\endcsname{\ensuremath{-1.28}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.on.hi\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.on.lo\endcsname{\ensuremath{-1.81}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.on.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.on.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.on.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.on.wordrev\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.reversed\endcsname{yes}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3L1.wordchg\endcsname{the registered wording is "does not improve in cross-validation" in both readings}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.changed\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.chg\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.name\endcsname{HyReX minus the function-identical control}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.off.ci\endcsname{[\ensuremath{-0.73}, \ensuremath{+0.98}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.off.dcv\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.off.f1\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.off.f2\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.off.f3\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.off.f4\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.off.hi\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.off.lo\endcsname{\ensuremath{-0.73}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.off.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.off.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.off.word\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.on.ci\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.on.dcv\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.on.f1\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.on.f2\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.on.f3\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.on.f4\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.on.hi\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.on.lo\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.on.n\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.on.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.on.word\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3P3c.wordchg\endcsname{the mirroring-on reading is pending}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.changed\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.chg\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.name\endcsname{HyReX minus the nnU-Net default}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.off.ci\endcsname{[\ensuremath{-1.08}, \ensuremath{+2.44}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.off.dcv\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.off.f1\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.off.f2\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.off.f3\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.off.f4\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.off.hi\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.off.lo\endcsname{\ensuremath{-1.08}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.off.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.off.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.off.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.on.ci\endcsname{[\ensuremath{-0.27}, \ensuremath{+1.42}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.on.dcv\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.on.f1\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.on.f2\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.on.f3\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.on.f4\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.on.hi\endcsname{\ensuremath{+1.42}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.on.lo\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.on.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.on.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.on.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.L3base.wordchg\endcsname{the registered wording is "improves on average (3/4 folds)" in both readings}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.changed\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.chg\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.name\endcsname{the function-identical control minus the nnU-Net default}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.off.ci\endcsname{[\ensuremath{-1.71}, \ensuremath{+2.82}]}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.off.dcv\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.off.f1\endcsname{\ensuremath{+2.38}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.off.f2\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.off.f3\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.off.f4\endcsname{\ensuremath{-1.02}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.off.hi\endcsname{\ensuremath{+2.82}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.off.lo\endcsname{\ensuremath{-1.71}}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.off.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.off.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.off.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.on.ci\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.on.dcv\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.on.f1\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.on.f2\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.on.f3\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.on.f4\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.on.hi\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.on.lo\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.on.n\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.on.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.on.word\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.P3cbase.wordchg\endcsname{the mirroring-on reading is pending}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.clause\endcsname{on KiTS23, HyReX minus the nnU-Net default \ensuremath{+0.68}\,pp [\ensuremath{-1.08}, \ensuremath{+2.44}], improves on average (3/4 folds) with mirroring off and \ensuremath{+0.57}\,pp [\ensuremath{-0.27}, \ensuremath{+1.42}], improves on average (3/4 folds) with mirroring on (a change of \ensuremath{-0.11}\,pp); ResEnc-M minus the nnU-Net default \ensuremath{+2.15}\,pp [\ensuremath{+0.98}, \ensuremath{+3.32}], improves in every fold with mirroring off and \ensuremath{+1.49}\,pp [\ensuremath{+0.88}, \ensuremath{+2.10}], improves in every fold with mirroring on (a change of \ensuremath{-0.65}\,pp); ResEnc-M minus HyReX \ensuremath{+1.47}\,pp [\ensuremath{-0.24}, \ensuremath{+3.17}], improves in every fold with mirroring off and \ensuremath{+0.92}\,pp [\ensuremath{+0.02}, \ensuremath{+1.81}], improves in every fold with mirroring on (a change of \ensuremath{-0.55}\,pp)}
\expandafter\gdef\csname R@an.gpu_measures.e2.kits.xclause\endcsname{on KiTS23, the function-identical control minus the nnU-Net default \ensuremath{+0.56}\,pp [\ensuremath{-1.71}, \ensuremath{+2.82}], improves on average (3/4 folds) with mirroring off; HyReX minus the function-identical control \ensuremath{+0.12}\,pp [\ensuremath{-0.73}, \ensuremath{+0.98}], improves on average (2/4 folds) with mirroring off; the mirroring-on reading of the function-identical control minus the nnU-Net default and HyReX minus the function-identical control is pending, with 0 of 4 folds of the function-identical control measured}
\expandafter\gdef\csname R@an.gpu_measures.e2.nchanged\endcsname{2}
\expandafter\gdef\csname R@an.gpu_measures.e2.ncomp\endcsname{6}
\expandafter\gdef\csname R@an.gpu_measures.e2.nwant\endcsname{6}
\expandafter\gdef\csname R@an.gpu_measures.e2.status\endcsname{the mirroring-on reading is complete for 6 of 6 contrasts and changes the registered wording of 2}
\expandafter\gdef\csname R@an.gpu_measures.e2.xncomp\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e2.xnwant\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e2.xstatus\endcsname{the mirroring-on reading of the two parts is pending for all 4 (dataset, part) pairs}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.L1.gapoff\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.L1.gapon\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.L1.inc\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.L1.non\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.L1.on\endcsname{89.24}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.L1.pub\endcsname{88.77}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.L1.reg\endcsname{88.75}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.base.five\endcsname{88.22}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.base.fiveall\endcsname{88.22}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.base.fold0\endcsname{87.70}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.base.fold0all\endcsname{87.70}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.base.fold0alln\endcsname{9}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.base.gapfive\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.base.gapoff\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.base.gapon\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.base.inc\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.base.non\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.base.on\endcsname{88.83}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.base.pub\endcsname{88.64}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.base.reg\endcsname{88.35}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.base.sub\endcsname{\ensuremath{-0.65}}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.clause\endcsname{on AMOS22 the nnU-Net default reads 88.35 with mirroring off and 88.83 with mirroring on, a mirroring increment of \ensuremath{+0.48}\,pp over folds 1 to 4, against 88.64 in the published five-fold table: our level is 0.29\,pp below it at the registered reading and 0.19\,pp above it with mirroring on}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.devn\endcsname{200}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.fold0clause\endcsname{fold 0, which every decision of the study read, stands at 87.70 for the frozen pool of the default (6 runs) and at 87.70 with the contemporaneous default runs added (9 runs)}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.margin.off\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.margin.on\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.margin.pub\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.nval\endcsname{40}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.pubn\endcsname{360}
\expandafter\gdef\csname R@an.gpu_measures.e3.amos.sizes\endcsname{on AMOS22 the development set holds 200 cases here and 360 in the published table}
\expandafter\gdef\csname R@an.gpu_measures.e3.gapdef\endcsname{a gap is the published five-fold value minus ours, so a positive gap is a published value above ours}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.L1.gapoff\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.L1.gapon\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.L1.inc\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.L1.non\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.L1.on\endcsname{87.01}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.L1.pub\endcsname{86.79}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.L1.reg\endcsname{86.14}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.base.five\endcsname{83.87}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.base.fiveall\endcsname{83.92}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.base.fold0\endcsname{83.38}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.base.fold0all\endcsname{83.62}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.base.fold0alln\endcsname{6}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.base.gapfive\endcsname{\ensuremath{+2.17}}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.base.gapoff\endcsname{\ensuremath{+2.05}}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.base.gapon\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.base.inc\endcsname{\ensuremath{+1.52}}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.base.non\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.base.on\endcsname{85.51}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.base.pub\endcsname{86.04}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.base.reg\endcsname{83.99}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.base.sub\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.clause\endcsname{on KiTS23 the nnU-Net default reads 83.99 with mirroring off and 85.51 with mirroring on, a mirroring increment of \ensuremath{+1.52}\,pp over folds 1 to 4, against 86.04 in the published five-fold table: our level is 2.05\,pp below it at the registered reading and 0.53\,pp below it with mirroring on}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.devn\endcsname{489}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.fold0clause\endcsname{fold 0, which every decision of the study read, stands at 83.38 for the frozen pool of the default (3 runs) and at 83.62 with the contemporaneous default runs added (6 runs)}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.margin.off\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.margin.on\endcsname{\ensuremath{+1.49}}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.margin.pub\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.nval\endcsname{98}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.pubn\endcsname{489}
\expandafter\gdef\csname R@an.gpu_measures.e3.kits.sizes\endcsname{on KiTS23 the development set holds 489 cases here and 489 in the published table}
\expandafter\gdef\csname R@an.gpu_measures.e3.nocause\endcsname{The remaining gap is reported as a number; no cause is assigned to it.}
\expandafter\gdef\csname R@an.gpu_measures.e3.pipeline\endcsname{this study trains for the registered budget under a 12\,GB memory cap, validates by sliding window with mirroring switched on or off as stated, and reads folds 1 to 4 of development sets of 200 and 489 cases here against 360 and 489 in the published table (AMOS22 and KiTS23); only the maintainers' published table is read, and the pipeline that produced it is not reproduced here}
\expandafter\gdef\csname R@an.gpu_measures.e3.subset\endcsname{the published value is a mean over five folds of its own splits and the level measured here is a mean over folds 1 to 4 of the splits of this study, one seed per fold; fold 0, the fold every decision of the study read, is outside it and enters only as the fold-0 level of the default shown beside it}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assd.ci\endcsname{[\ensuremath{-0.27}, \ensuremath{0.00}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assd.dcv\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assd.f1\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assd.f2\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assd.f3\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assd.f4\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assd.hi\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assd.lo\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assd.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assd.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assd.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assdp.ci\endcsname{[\ensuremath{-4.82}, \ensuremath{+4.45}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assdp.dcv\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assdp.f1\endcsname{\ensuremath{-1.38}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assdp.f2\endcsname{\ensuremath{-3.00}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assdp.f3\endcsname{\ensuremath{+3.83}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assdp.f4\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assdp.hi\endcsname{\ensuremath{+4.45}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assdp.lo\endcsname{\ensuremath{-4.82}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assdp.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assdp.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.assdp.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.clause\endcsname{ResEnc-M minus the nnU-Net default on AMOS22 over folds 1 to 4, mirroring off: Dice \ensuremath{+0.41}\,pp [\ensuremath{-0.27}, \ensuremath{+1.09}]; NSD@1 mm \ensuremath{+0.71}\,pp [\ensuremath{+0.07}, \ensuremath{+1.36}]; NSD@2 mm \ensuremath{+0.64}\,pp [\ensuremath{-0.05}, \ensuremath{+1.33}]; HD95 \ensuremath{-1.01}\,mm [\ensuremath{-1.33}, \ensuremath{-0.70}]; ASSD \ensuremath{-0.14}\,mm [\ensuremath{-0.27}, \ensuremath{0.00}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.dice.ci\endcsname{[\ensuremath{-0.27}, \ensuremath{+1.09}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.dice.dcv\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.dice.f1\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.dice.f2\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.dice.f3\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.dice.f4\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.dice.hi\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.dice.lo\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.dice.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.dice.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.dice.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95.ci\endcsname{[\ensuremath{-1.33}, \ensuremath{-0.70}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95.dcv\endcsname{\ensuremath{-1.01}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95.f1\endcsname{\ensuremath{-1.21}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95.f2\endcsname{\ensuremath{-0.80}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95.f3\endcsname{\ensuremath{-0.90}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95.f4\endcsname{\ensuremath{-1.14}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95.hi\endcsname{\ensuremath{-0.70}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95.lo\endcsname{\ensuremath{-1.33}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95p.ci\endcsname{[\ensuremath{-5.56}, \ensuremath{+3.45}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95p.dcv\endcsname{\ensuremath{-1.05}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95p.f1\endcsname{\ensuremath{-2.45}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95p.f2\endcsname{\ensuremath{-3.56}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95p.f3\endcsname{\ensuremath{+2.92}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95p.f4\endcsname{\ensuremath{-1.13}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95p.hi\endcsname{\ensuremath{+3.45}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95p.lo\endcsname{\ensuremath{-5.56}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95p.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95p.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.hd95p.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd1.ci\endcsname{[\ensuremath{+0.07}, \ensuremath{+1.36}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd1.dcv\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd1.f1\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd1.f2\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd1.f3\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd1.f4\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd1.hi\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd1.lo\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd1.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd1.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd1.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd2.ci\endcsname{[\ensuremath{-0.05}, \ensuremath{+1.33}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd2.dcv\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd2.f1\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd2.f2\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd2.f3\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd2.f4\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd2.hi\endcsname{\ensuremath{+1.33}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd2.lo\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd2.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd2.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.nsd2.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.sepsummary\endcsname{three of the four separate ResEnc-M from the nnU-Net default with an interval clear of zero (NSD at 1\,mm, HD95 and ASSD) and NSD at 2\,mm has an interval spanning zero}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.sepsummary.n\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.sepsummary.nspan\endcsname{1}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.summary\endcsname{ResEnc-M minus the nnU-Net default improves in every fold on four of the four surface-distance measures (NSD at 1\,mm, NSD at 2\,mm, HD95 and ASSD); HD95 and ASSD are distances in mm, for which a lower value is the improvement}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.summary.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.summary.nevery\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.summary.nnamed\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L1base.summary.npend\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assd.ci\endcsname{[\ensuremath{-0.37}, \ensuremath{+0.22}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assd.dcv\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assd.f1\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assd.f2\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assd.f3\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assd.f4\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assd.hi\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assd.lo\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assd.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assd.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assd.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assdp.ci\endcsname{[\ensuremath{-1.55}, \ensuremath{+3.92}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assdp.dcv\endcsname{\ensuremath{+1.19}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assdp.f1\endcsname{\ensuremath{+2.57}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assdp.f2\endcsname{\ensuremath{+2.74}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assdp.f3\endcsname{\ensuremath{-0.55}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assdp.f4\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assdp.hi\endcsname{\ensuremath{+3.92}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assdp.lo\endcsname{\ensuremath{-1.55}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assdp.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assdp.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.assdp.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.clause\endcsname{HyReX minus ResEnc-M on AMOS22 over folds 1 to 4, mirroring off: Dice \ensuremath{-0.18}\,pp [\ensuremath{-0.76}, \ensuremath{+0.40}]; NSD@1 mm \ensuremath{-0.29}\,pp [\ensuremath{-0.94}, \ensuremath{+0.36}]; NSD@2 mm \ensuremath{-0.29}\,pp [\ensuremath{-0.92}, \ensuremath{+0.35}]; HD95 \ensuremath{+0.38}\,mm [\ensuremath{-0.84}, \ensuremath{+1.60}]; ASSD \ensuremath{-0.08}\,mm [\ensuremath{-0.37}, \ensuremath{+0.22}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.dice.ci\endcsname{[\ensuremath{-0.76}, \ensuremath{+0.40}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.dice.dcv\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.dice.f1\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.dice.f2\endcsname{\ensuremath{-0.41}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.dice.f3\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.dice.f4\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.dice.hi\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.dice.lo\endcsname{\ensuremath{-0.76}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.dice.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.dice.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.dice.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95.ci\endcsname{[\ensuremath{-0.84}, \ensuremath{+1.60}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95.dcv\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95.f1\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95.f2\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95.f3\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95.f4\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95.hi\endcsname{\ensuremath{+1.60}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95.lo\endcsname{\ensuremath{-0.84}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95p.ci\endcsname{[\ensuremath{-2.04}, \ensuremath{+5.27}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95p.dcv\endcsname{\ensuremath{+1.62}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95p.f1\endcsname{\ensuremath{+3.66}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95p.f2\endcsname{\ensuremath{+3.55}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95p.f3\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95p.f4\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95p.hi\endcsname{\ensuremath{+5.27}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95p.lo\endcsname{\ensuremath{-2.04}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95p.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95p.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.hd95p.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd1.ci\endcsname{[\ensuremath{-0.94}, \ensuremath{+0.36}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd1.dcv\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd1.f1\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd1.f2\endcsname{\ensuremath{-0.58}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd1.f3\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd1.f4\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd1.hi\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd1.lo\endcsname{\ensuremath{-0.94}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd1.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd1.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd1.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd2.ci\endcsname{[\ensuremath{-0.92}, \ensuremath{+0.35}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd2.dcv\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd2.f1\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd2.f2\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd2.f3\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd2.f4\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd2.hi\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd2.lo\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd2.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd2.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.nsd2.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.sepsummary\endcsname{none of the four separates HyReX from ResEnc-M: every interval spans zero (NSD at 1\,mm, NSD at 2\,mm, HD95 and ASSD)}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.sepsummary.n\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.sepsummary.nspan\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.summary\endcsname{HyReX minus ResEnc-M does not improve in cross-validation on three of the four surface-distance measures (NSD at 1\,mm, NSD at 2\,mm and HD95) and improves on average (3/4 folds) on ASSD; HD95 and ASSD are distances in mm, for which a lower value is the improvement}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.summary.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.summary.nevery\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.summary.nnamed\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3L1.summary.npend\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assd.ci\endcsname{[\ensuremath{-0.42}, \ensuremath{-0.01}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assd.dcv\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assd.f1\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assd.f2\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assd.f3\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assd.f4\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assd.hi\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assd.lo\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assd.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assd.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assd.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assdp.ci\endcsname{[\ensuremath{-1.63}, \ensuremath{+3.64}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assdp.dcv\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assdp.f1\endcsname{\ensuremath{+1.19}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assdp.f2\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assdp.f3\endcsname{\ensuremath{+3.28}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assdp.f4\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assdp.hi\endcsname{\ensuremath{+3.64}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assdp.lo\endcsname{\ensuremath{-1.63}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assdp.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assdp.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.assdp.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.clause\endcsname{HyReX minus the nnU-Net default on AMOS22 over folds 1 to 4, mirroring off: Dice \ensuremath{+0.23}\,pp [\ensuremath{-0.08}, \ensuremath{+0.54}]; NSD@1 mm \ensuremath{+0.42}\,pp [\ensuremath{+0.19}, \ensuremath{+0.66}]; NSD@2 mm \ensuremath{+0.36}\,pp [\ensuremath{+0.06}, \ensuremath{+0.66}]; HD95 \ensuremath{-0.63}\,mm [\ensuremath{-1.85}, \ensuremath{+0.59}]; ASSD \ensuremath{-0.21}\,mm [\ensuremath{-0.42}, \ensuremath{-0.01}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.dice.ci\endcsname{[\ensuremath{-0.08}, \ensuremath{+0.54}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.dice.dcv\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.dice.f1\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.dice.f2\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.dice.f3\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.dice.f4\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.dice.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.dice.lo\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.dice.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.dice.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.dice.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95.ci\endcsname{[\ensuremath{-1.85}, \ensuremath{+0.59}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95.dcv\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95.f1\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95.f2\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95.f3\endcsname{\ensuremath{-1.20}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95.f4\endcsname{\ensuremath{-1.38}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95.hi\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95.lo\endcsname{\ensuremath{-1.85}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95p.ci\endcsname{[\ensuremath{-2.01}, \ensuremath{+3.14}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95p.dcv\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95p.f1\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95p.f2\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95p.f3\endcsname{\ensuremath{+2.41}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95p.f4\endcsname{\ensuremath{-1.36}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95p.hi\endcsname{\ensuremath{+3.14}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95p.lo\endcsname{\ensuremath{-2.01}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95p.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95p.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.hd95p.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd1.ci\endcsname{[\ensuremath{+0.19}, \ensuremath{+0.66}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd1.dcv\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd1.f1\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd1.f2\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd1.f3\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd1.f4\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd1.hi\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd1.lo\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd1.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd1.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd1.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd2.ci\endcsname{[\ensuremath{+0.06}, \ensuremath{+0.66}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd2.dcv\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd2.f1\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd2.f2\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd2.f3\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd2.f4\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd2.hi\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd2.lo\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd2.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd2.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.nsd2.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.sepsummary\endcsname{three of the four separate HyReX from the nnU-Net default with an interval clear of zero (NSD at 1\,mm, NSD at 2\,mm and ASSD) and HD95 has an interval spanning zero}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.sepsummary.n\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.sepsummary.nspan\endcsname{1}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.summary\endcsname{HyReX minus the nnU-Net default improves in every fold on three of the four surface-distance measures (NSD at 1\,mm, NSD at 2\,mm and ASSD) and improves on average (3/4 folds) on HD95; HD95 and ASSD are distances in mm, for which a lower value is the improvement}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.summary.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.summary.nevery\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.summary.nnamed\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.amos.L3base.summary.npend\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assd.ci\endcsname{[\ensuremath{-7.10}, \ensuremath{-2.77}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assd.dcv\endcsname{\ensuremath{-4.94}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assd.f1\endcsname{\ensuremath{-5.82}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assd.f2\endcsname{\ensuremath{-6.32}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assd.f3\endcsname{\ensuremath{-3.43}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assd.f4\endcsname{\ensuremath{-4.17}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assd.hi\endcsname{\ensuremath{-2.77}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assd.lo\endcsname{\ensuremath{-7.10}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assd.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assd.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assd.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assdp.ci\endcsname{[\ensuremath{-6.85}, \ensuremath{-0.31}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assdp.dcv\endcsname{\ensuremath{-3.58}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assdp.f1\endcsname{\ensuremath{-5.82}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assdp.f2\endcsname{\ensuremath{-0.89}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assdp.f3\endcsname{\ensuremath{-3.43}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assdp.f4\endcsname{\ensuremath{-4.17}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assdp.hi\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assdp.lo\endcsname{\ensuremath{-6.85}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assdp.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assdp.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.assdp.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.clause\endcsname{ResEnc-M minus the nnU-Net default on KiTS23 over folds 1 to 4, mirroring off: Dice \ensuremath{+2.15}\,pp [\ensuremath{+0.98}, \ensuremath{+3.32}]; NSD@1 mm \ensuremath{+2.29}\,pp [\ensuremath{+1.55}, \ensuremath{+3.03}]; NSD@2 mm \ensuremath{+2.49}\,pp [\ensuremath{+1.78}, \ensuremath{+3.20}]; HD95 \ensuremath{-19.27}\,mm [\ensuremath{-28.73}, \ensuremath{-9.80}]; ASSD \ensuremath{-4.94}\,mm [\ensuremath{-7.10}, \ensuremath{-2.77}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.dice.ci\endcsname{[\ensuremath{+0.98}, \ensuremath{+3.32}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.dice.dcv\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.dice.f1\endcsname{\ensuremath{+2.58}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.dice.f2\endcsname{\ensuremath{+2.94}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.dice.f3\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.dice.f4\endcsname{\ensuremath{+1.71}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.dice.hi\endcsname{\ensuremath{+3.32}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.dice.lo\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.dice.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.dice.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.dice.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95.ci\endcsname{[\ensuremath{-28.73}, \ensuremath{-9.80}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95.dcv\endcsname{\ensuremath{-19.27}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95.f1\endcsname{\ensuremath{-27.37}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95.f2\endcsname{\ensuremath{-20.07}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95.f3\endcsname{\ensuremath{-15.06}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95.f4\endcsname{\ensuremath{-14.56}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95.hi\endcsname{\ensuremath{-9.80}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95.lo\endcsname{\ensuremath{-28.73}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95p.ci\endcsname{[\ensuremath{-27.95}, \ensuremath{-7.98}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95p.dcv\endcsname{\ensuremath{-17.96}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95p.f1\endcsname{\ensuremath{-27.37}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95p.f2\endcsname{\ensuremath{-14.86}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95p.f3\endcsname{\ensuremath{-15.06}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95p.f4\endcsname{\ensuremath{-14.56}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95p.hi\endcsname{\ensuremath{-7.98}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95p.lo\endcsname{\ensuremath{-27.95}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95p.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95p.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.hd95p.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd1.ci\endcsname{[\ensuremath{+1.55}, \ensuremath{+3.03}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd1.dcv\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd1.f1\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd1.f2\endcsname{\ensuremath{+2.86}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd1.f3\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd1.f4\endcsname{\ensuremath{+2.10}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd1.hi\endcsname{\ensuremath{+3.03}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd1.lo\endcsname{\ensuremath{+1.55}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd1.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd1.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd1.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd2.ci\endcsname{[\ensuremath{+1.78}, \ensuremath{+3.20}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd2.dcv\endcsname{\ensuremath{+2.49}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd2.f1\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd2.f2\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd2.f3\endcsname{\ensuremath{+1.98}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd2.f4\endcsname{\ensuremath{+2.26}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd2.hi\endcsname{\ensuremath{+3.20}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd2.lo\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd2.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd2.npos\endcsname{4/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.nsd2.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.sepsummary\endcsname{all four separate ResEnc-M from the nnU-Net default, every interval clear of zero (NSD at 1\,mm, NSD at 2\,mm, HD95 and ASSD)}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.sepsummary.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.sepsummary.nspan\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.summary\endcsname{ResEnc-M minus the nnU-Net default improves in every fold on four of the four surface-distance measures (NSD at 1\,mm, NSD at 2\,mm, HD95 and ASSD); HD95 and ASSD are distances in mm, for which a lower value is the improvement}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.summary.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.summary.nevery\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.summary.nnamed\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L1base.summary.npend\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assd.ci\endcsname{[\ensuremath{-0.30}, \ensuremath{+9.41}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assd.dcv\endcsname{\ensuremath{+4.56}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assd.f1\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assd.f2\endcsname{\ensuremath{+8.48}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assd.f3\endcsname{\ensuremath{+3.41}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assd.f4\endcsname{\ensuremath{+5.10}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assd.hi\endcsname{\ensuremath{+9.41}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assd.lo\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assd.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assd.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assd.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assdp.ci\endcsname{[\ensuremath{+0.69}, \ensuremath{+7.04}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assdp.dcv\endcsname{\ensuremath{+3.87}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assdp.f1\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assdp.f2\endcsname{\ensuremath{+5.71}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assdp.f3\endcsname{\ensuremath{+3.41}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assdp.f4\endcsname{\ensuremath{+5.10}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assdp.hi\endcsname{\ensuremath{+7.04}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assdp.lo\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assdp.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assdp.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.assdp.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.clause\endcsname{HyReX minus ResEnc-M on KiTS23 over folds 1 to 4, mirroring off: Dice \ensuremath{-1.47}\,pp [\ensuremath{-3.17}, \ensuremath{+0.24}]; NSD@1 mm \ensuremath{-1.42}\,pp [\ensuremath{-3.38}, \ensuremath{+0.54}]; NSD@2 mm \ensuremath{-1.66}\,pp [\ensuremath{-3.43}, \ensuremath{+0.12}]; HD95 \ensuremath{+14.91}\,mm [\ensuremath{+3.75}, \ensuremath{+26.06}]; ASSD \ensuremath{+4.56}\,mm [\ensuremath{-0.30}, \ensuremath{+9.41}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.dice.ci\endcsname{[\ensuremath{-3.17}, \ensuremath{+0.24}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.dice.dcv\endcsname{\ensuremath{-1.47}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.dice.f1\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.dice.f2\endcsname{\ensuremath{-2.74}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.dice.f3\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.dice.f4\endcsname{\ensuremath{-1.86}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.dice.hi\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.dice.lo\endcsname{\ensuremath{-3.17}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.dice.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.dice.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.dice.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95.ci\endcsname{[\ensuremath{+3.75}, \ensuremath{+26.06}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95.dcv\endcsname{\ensuremath{+14.91}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95.f1\endcsname{\ensuremath{+6.90}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95.f2\endcsname{\ensuremath{+23.95}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95.f3\endcsname{\ensuremath{+15.11}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95.f4\endcsname{\ensuremath{+13.66}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95.hi\endcsname{\ensuremath{+26.06}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95.lo\endcsname{\ensuremath{+3.75}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95p.ci\endcsname{[\ensuremath{+4.87}, \ensuremath{+23.58}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95p.dcv\endcsname{\ensuremath{+14.22}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95p.f1\endcsname{\ensuremath{+6.90}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95p.f2\endcsname{\ensuremath{+21.22}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95p.f3\endcsname{\ensuremath{+15.11}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95p.f4\endcsname{\ensuremath{+13.66}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95p.hi\endcsname{\ensuremath{+23.58}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95p.lo\endcsname{\ensuremath{+4.87}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95p.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95p.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.hd95p.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd1.ci\endcsname{[\ensuremath{-3.38}, \ensuremath{+0.54}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd1.dcv\endcsname{\ensuremath{-1.42}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd1.f1\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd1.f2\endcsname{\ensuremath{-2.97}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd1.f3\endcsname{\ensuremath{-1.29}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd1.f4\endcsname{\ensuremath{-1.46}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd1.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd1.lo\endcsname{\ensuremath{-3.38}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd1.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd1.npos\endcsname{1/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd1.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd2.ci\endcsname{[\ensuremath{-3.43}, \ensuremath{+0.12}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd2.dcv\endcsname{\ensuremath{-1.66}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd2.f1\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd2.f2\endcsname{\ensuremath{-3.02}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd2.f3\endcsname{\ensuremath{-1.52}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd2.f4\endcsname{\ensuremath{-1.79}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd2.hi\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd2.lo\endcsname{\ensuremath{-3.43}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd2.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd2.npos\endcsname{0/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.nsd2.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.sepsummary\endcsname{one of the four separates HyReX from ResEnc-M with an interval clear of zero (HD95) and NSD at 1\,mm, NSD at 2\,mm and ASSD have an interval spanning zero}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.sepsummary.n\endcsname{1}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.sepsummary.nspan\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.summary\endcsname{HyReX minus ResEnc-M does not improve in cross-validation on four of the four surface-distance measures (NSD at 1\,mm, NSD at 2\,mm, HD95 and ASSD); HD95 and ASSD are distances in mm, for which a lower value is the improvement}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.summary.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.summary.nevery\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.summary.nnamed\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3L1.summary.npend\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assd.ci\endcsname{[\ensuremath{-5.05}, \ensuremath{+4.29}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assd.dcv\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assd.f1\endcsname{\ensuremath{-4.58}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assd.f2\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assd.f3\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assd.f4\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assd.hi\endcsname{\ensuremath{+4.29}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assd.lo\endcsname{\ensuremath{-5.05}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assd.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assd.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assd.word\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assdp.ci\endcsname{[\ensuremath{-5.86}, \ensuremath{+6.43}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assdp.dcv\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assdp.f1\endcsname{\ensuremath{-4.58}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assdp.f2\endcsname{\ensuremath{+4.82}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assdp.f3\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assdp.f4\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assdp.hi\endcsname{\ensuremath{+6.43}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assdp.lo\endcsname{\ensuremath{-5.86}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assdp.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assdp.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.assdp.word\endcsname{does not improve in cross-validation}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.clause\endcsname{HyReX minus the nnU-Net default on KiTS23 over folds 1 to 4, mirroring off: Dice \ensuremath{+0.68}\,pp [\ensuremath{-1.08}, \ensuremath{+2.44}]; NSD@1 mm \ensuremath{+0.87}\,pp [\ensuremath{-0.89}, \ensuremath{+2.63}]; NSD@2 mm \ensuremath{+0.83}\,pp [\ensuremath{-1.03}, \ensuremath{+2.70}]; HD95 \ensuremath{-4.36}\,mm [\ensuremath{-21.76}, \ensuremath{+13.04}]; ASSD \ensuremath{-0.38}\,mm [\ensuremath{-5.05}, \ensuremath{+4.29}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.dice.ci\endcsname{[\ensuremath{-1.08}, \ensuremath{+2.44}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.dice.dcv\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.dice.f1\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.dice.f2\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.dice.f3\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.dice.f4\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.dice.hi\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.dice.lo\endcsname{\ensuremath{-1.08}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.dice.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.dice.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.dice.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95.ci\endcsname{[\ensuremath{-21.76}, \ensuremath{+13.04}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95.dcv\endcsname{\ensuremath{-4.36}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95.f1\endcsname{\ensuremath{-20.47}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95.f2\endcsname{\ensuremath{+3.88}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95.f3\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95.f4\endcsname{\ensuremath{-0.91}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95.hi\endcsname{\ensuremath{+13.04}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95.lo\endcsname{\ensuremath{-21.76}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95.word\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95p.ci\endcsname{[\ensuremath{-22.21}, \ensuremath{+14.73}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95p.dcv\endcsname{\ensuremath{-3.74}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95p.f1\endcsname{\ensuremath{-20.47}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95p.f2\endcsname{\ensuremath{+6.37}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95p.f3\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95p.f4\endcsname{\ensuremath{-0.91}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95p.hi\endcsname{\ensuremath{+14.73}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95p.lo\endcsname{\ensuremath{-22.21}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95p.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95p.npos\endcsname{2/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.hd95p.word\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd1.ci\endcsname{[\ensuremath{-0.89}, \ensuremath{+2.63}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd1.dcv\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd1.f1\endcsname{\ensuremath{+2.46}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd1.f2\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd1.f3\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd1.f4\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd1.hi\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd1.lo\endcsname{\ensuremath{-0.89}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd1.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd1.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd1.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd2.ci\endcsname{[\ensuremath{-1.03}, \ensuremath{+2.70}]}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd2.dcv\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd2.f1\endcsname{\ensuremath{+2.54}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd2.f2\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd2.f3\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd2.f4\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd2.hi\endcsname{\ensuremath{+2.70}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd2.lo\endcsname{\ensuremath{-1.03}}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd2.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd2.npos\endcsname{3/4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.nsd2.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.sepsummary\endcsname{none of the four separates HyReX from the nnU-Net default: every interval spans zero (NSD at 1\,mm, NSD at 2\,mm, HD95 and ASSD)}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.sepsummary.n\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.sepsummary.nspan\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.summary\endcsname{HyReX minus the nnU-Net default improves on average (3/4 folds) on two of the four surface-distance measures (NSD at 1\,mm and NSD at 2\,mm) and improves on average (2/4 folds) on two of them (HD95 and ASSD); HD95 and ASSD are distances in mm, for which a lower value is the improvement}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.summary.n\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.summary.nevery\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.summary.nnamed\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.e4.kits.L3base.summary.npend\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.e4.nfull\endcsname{42}
\expandafter\gdef\csname R@an.gpu_measures.e4.nread\endcsname{42}
\expandafter\gdef\csname R@an.gpu_measures.e4.orient\endcsname{differences are first arm minus second arm in the metric's own unit; Dice and NSD improve upward, HD95 and ASSD improve downward, and the registered wording counts the folds in which the first arm improves; the boundary figure draws HD95 and ASSD as minus the difference, so that a mark to the right means the first arm is better in every panel}
\expandafter\gdef\csname R@an.gpu_measures.e4.secondary\endcsname{the four surface-distance measures are secondary to Dice, read with mirroring off on the same predictions and described without correction across measures or datasets; none of the four is designated primary (Addendum U, E4)}
\expandafter\gdef\csname R@an.gpu_measures.e4.status\endcsname{42 of 42 boundary-metric contrasts are complete over folds 1 to 4}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.assd.f1\endcsname{1.17}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.assd.f2\endcsname{1.21}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.assd.f3\endcsname{1.64}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.assd.f4\endcsname{1.39}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.assd.mean\endcsname{1.35}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.assdp.f1\endcsname{3.78}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.assdp.f2\endcsname{5.01}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.assdp.f3\endcsname{7.00}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.assdp.f4\endcsname{6.55}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.assdp.mean\endcsname{5.58}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.dice.f1\endcsname{89.46}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.dice.f2\endcsname{89.25}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.dice.f3\endcsname{88.63}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.dice.f4\endcsname{87.68}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.dice.mean\endcsname{88.75}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.hd95.f1\endcsname{5.53}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.hd95.f2\endcsname{6.72}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.hd95.f3\endcsname{7.51}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.hd95.f4\endcsname{7.53}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.hd95.mean\endcsname{6.82}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.hd95p.f1\endcsname{8.13}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.hd95p.f2\endcsname{10.48}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.hd95p.f3\endcsname{12.84}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.hd95p.f4\endcsname{12.65}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.hd95p.mean\endcsname{11.03}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.nsd1.f1\endcsname{83.27}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.nsd1.f2\endcsname{83.24}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.nsd1.f3\endcsname{82.35}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.nsd1.f4\endcsname{80.17}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.nsd1.mean\endcsname{82.26}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.nsd2.f1\endcsname{91.00}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.nsd2.f2\endcsname{90.59}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.nsd2.f3\endcsname{90.11}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.nsd2.f4\endcsname{88.62}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L1.nsd2.mean\endcsname{90.08}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.assd.f1\endcsname{1.26}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.assd.f2\endcsname{1.18}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.assd.f3\endcsname{1.30}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.assd.f4\endcsname{1.36}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.assd.mean\endcsname{1.27}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.assdp.f1\endcsname{6.35}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.assdp.f2\endcsname{7.76}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.assdp.f3\endcsname{6.45}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.assdp.f4\endcsname{6.52}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.assdp.mean\endcsname{6.77}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.dice.f1\endcsname{89.09}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.dice.f2\endcsname{88.84}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.dice.f3\endcsname{88.99}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.dice.f4\endcsname{87.38}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.dice.mean\endcsname{88.58}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.hd95.f1\endcsname{6.74}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.hd95.f2\endcsname{7.58}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.hd95.f3\endcsname{7.21}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.hd95.f4\endcsname{7.30}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.hd95.mean\endcsname{7.21}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.hd95p.f1\endcsname{11.79}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.hd95p.f2\endcsname{14.04}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.hd95p.f3\endcsname{12.33}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.hd95p.f4\endcsname{12.42}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.hd95p.mean\endcsname{12.64}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.nsd1.f1\endcsname{82.82}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.nsd1.f2\endcsname{82.66}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.nsd1.f3\endcsname{82.67}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.nsd1.f4\endcsname{79.73}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.nsd1.mean\endcsname{81.97}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.nsd2.f1\endcsname{90.53}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.nsd2.f2\endcsname{89.99}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.nsd2.f3\endcsname{90.41}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.nsd2.f4\endcsname{88.25}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.L3.nsd2.mean\endcsname{89.79}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.assd.f1\endcsname{1.30}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.assd.f2\endcsname{1.43}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.assd.f3\endcsname{1.65}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.assd.f4\endcsname{1.56}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.assd.mean\endcsname{1.49}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.assdp.f1\endcsname{5.16}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.assdp.f2\endcsname{8.02}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.assdp.f3\endcsname{3.17}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.assdp.f4\endcsname{6.72}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.assdp.mean\endcsname{5.77}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.dice.f1\endcsname{89.12}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.dice.f2\endcsname{88.48}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.dice.f3\endcsname{88.80}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.dice.f4\endcsname{87.00}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.dice.mean\endcsname{88.35}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.hd95.f1\endcsname{6.75}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.hd95.f2\endcsname{7.52}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.hd95.f3\endcsname{8.41}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.hd95.f4\endcsname{8.68}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.hd95.mean\endcsname{7.84}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.hd95p.f1\endcsname{10.58}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.hd95p.f2\endcsname{14.04}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.hd95p.f3\endcsname{9.91}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.hd95p.f4\endcsname{13.78}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.hd95p.mean\endcsname{12.08}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.nsd1.f1\endcsname{82.62}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.nsd1.f2\endcsname{82.13}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.nsd1.f3\endcsname{82.18}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.nsd1.f4\endcsname{79.25}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.nsd1.mean\endcsname{81.54}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.nsd2.f1\endcsname{90.44}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.nsd2.f2\endcsname{89.52}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.nsd2.f3\endcsname{90.04}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.nsd2.f4\endcsname{87.75}
\expandafter\gdef\csname R@an.gpu_measures.e4a.amos.base.nsd2.mean\endcsname{89.44}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.assd.f1\endcsname{7.65}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.assd.f2\endcsname{6.13}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.assd.f3\endcsname{4.86}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.assd.f4\endcsname{6.79}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.assd.mean\endcsname{6.36}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.assdp.f1\endcsname{7.65}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.assdp.f2\endcsname{11.56}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.assdp.f3\endcsname{4.86}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.assdp.f4\endcsname{6.79}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.assdp.mean\endcsname{7.72}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.dice.f1\endcsname{85.44}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.dice.f2\endcsname{86.25}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.dice.f3\endcsname{88.27}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.dice.f4\endcsname{84.60}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.dice.mean\endcsname{86.14}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.hd95.f1\endcsname{33.38}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.hd95.f2\endcsname{31.40}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.hd95.f3\endcsname{27.11}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.hd95.f4\endcsname{33.60}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.hd95.mean\endcsname{31.37}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.hd95p.f1\endcsname{33.38}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.hd95p.f2\endcsname{36.61}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.hd95p.f3\endcsname{27.11}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.hd95p.f4\endcsname{33.60}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.hd95p.mean\endcsname{32.68}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.nsd1.f1\endcsname{72.39}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.nsd1.f2\endcsname{73.68}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.nsd1.f3\endcsname{73.26}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.nsd1.f4\endcsname{72.39}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.nsd1.mean\endcsname{72.93}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.nsd2.f1\endcsname{80.71}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.nsd2.f2\endcsname{80.88}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.nsd2.f3\endcsname{81.80}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.nsd2.f4\endcsname{79.98}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L1.nsd2.mean\endcsname{80.84}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.assd.f1\endcsname{8.90}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.assd.f2\endcsname{14.60}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.assd.f3\endcsname{8.26}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.assd.f4\endcsname{11.89}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.assd.mean\endcsname{10.91}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.assdp.f1\endcsname{8.90}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.assdp.f2\endcsname{17.27}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.assdp.f3\endcsname{8.26}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.assdp.f4\endcsname{11.89}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.assdp.mean\endcsname{11.58}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.dice.f1\endcsname{85.17}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.dice.f2\endcsname{83.51}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.dice.f3\endcsname{87.29}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.dice.f4\endcsname{82.74}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.dice.mean\endcsname{84.67}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.hd95.f1\endcsname{40.29}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.hd95.f2\endcsname{55.35}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.hd95.f3\endcsname{42.22}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.hd95.f4\endcsname{47.26}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.hd95.mean\endcsname{46.28}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.hd95p.f1\endcsname{40.29}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.hd95p.f2\endcsname{57.83}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.hd95p.f3\endcsname{42.22}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.hd95p.f4\endcsname{47.26}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.hd95p.mean\endcsname{46.90}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.nsd1.f1\endcsname{72.43}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.nsd1.f2\endcsname{70.72}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.nsd1.f3\endcsname{71.97}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.nsd1.f4\endcsname{70.92}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.nsd1.mean\endcsname{71.51}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.nsd2.f1\endcsname{80.41}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.nsd2.f2\endcsname{77.87}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.nsd2.f3\endcsname{80.28}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.nsd2.f4\endcsname{78.18}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.L3.nsd2.mean\endcsname{79.19}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.assd.f1\endcsname{13.48}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.assd.f2\endcsname{12.45}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.assd.f3\endcsname{8.28}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.assd.f4\endcsname{10.96}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.assd.mean\endcsname{11.29}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.assdp.f1\endcsname{13.48}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.assdp.f2\endcsname{12.45}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.assdp.f3\endcsname{8.28}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.assdp.f4\endcsname{10.96}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.assdp.mean\endcsname{11.29}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.dice.f1\endcsname{82.86}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.dice.f2\endcsname{83.31}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.dice.f3\endcsname{86.91}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.dice.f4\endcsname{82.89}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.dice.mean\endcsname{83.99}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.hd95.f1\endcsname{60.75}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.hd95.f2\endcsname{51.47}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.hd95.f3\endcsname{42.17}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.hd95.f4\endcsname{48.16}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.hd95.mean\endcsname{50.64}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.hd95p.f1\endcsname{60.75}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.hd95p.f2\endcsname{51.47}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.hd95p.f3\endcsname{42.17}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.hd95p.f4\endcsname{48.16}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.hd95p.mean\endcsname{50.64}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.nsd1.f1\endcsname{69.97}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.nsd1.f2\endcsname{70.82}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.nsd1.f3\endcsname{71.48}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.nsd1.f4\endcsname{70.29}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.nsd1.mean\endcsname{70.64}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.nsd2.f1\endcsname{77.87}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.nsd2.f2\endcsname{78.00}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.nsd2.f3\endcsname{79.82}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.nsd2.f4\endcsname{77.72}
\expandafter\gdef\csname R@an.gpu_measures.e4a.kits.base.nsd2.mean\endcsname{78.35}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q10.L1\endcsname{83.91}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q10.L3\endcsname{82.87}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q10.base\endcsname{83.78}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q10.case\endcsname{\texttt{amos\_0181}}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q10.dice\endcsname{83.78}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q10.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q10.rank\endcsname{5 of 40}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q50.L1\endcsname{90.51}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q50.L3\endcsname{90.77}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q50.base\endcsname{91.07}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q50.case\endcsname{\texttt{amos\_0116}}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q50.dice\endcsname{91.07}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q50.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q50.rank\endcsname{21 of 40}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q90.L1\endcsname{93.82}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q90.L3\endcsname{93.74}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q90.base\endcsname{93.51}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q90.case\endcsname{\texttt{amos\_0196}}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q90.dice\endcsname{93.51}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q90.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f1.q90.rank\endcsname{36 of 40}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q10.L1\endcsname{82.34}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q10.L3\endcsname{82.98}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q10.base\endcsname{82.23}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q10.case\endcsname{\texttt{amos\_0047}}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q10.dice\endcsname{82.23}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q10.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q10.rank\endcsname{5 of 40}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q50.L1\endcsname{89.47}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q50.L3\endcsname{89.74}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q50.base\endcsname{89.52}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q50.case\endcsname{\texttt{amos\_0024}}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q50.dice\endcsname{89.52}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q50.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q50.rank\endcsname{21 of 40}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q90.L1\endcsname{95.07}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q90.L3\endcsname{94.51}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q90.base\endcsname{94.76}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q90.case\endcsname{\texttt{amos\_0135}}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q90.dice\endcsname{94.76}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q90.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f2.q90.rank\endcsname{36 of 40}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q10.L1\endcsname{82.17}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q10.L3\endcsname{84.01}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q10.base\endcsname{81.17}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q10.case\endcsname{\texttt{amos\_0370}}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q10.dice\endcsname{81.17}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q10.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q10.rank\endcsname{5 of 40}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q50.L1\endcsname{90.66}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q50.L3\endcsname{90.90}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q50.base\endcsname{90.67}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q50.case\endcsname{\texttt{amos\_0406}}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q50.dice\endcsname{90.67}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q50.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q50.rank\endcsname{21 of 40}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q90.L1\endcsname{94.72}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q90.L3\endcsname{94.51}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q90.base\endcsname{94.00}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q90.case\endcsname{\texttt{amos\_0159}}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q90.dice\endcsname{94.00}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q90.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f3.q90.rank\endcsname{36 of 40}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q10.L1\endcsname{80.03}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q10.L3\endcsname{76.44}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q10.base\endcsname{79.08}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q10.case\endcsname{\texttt{amos\_0245}}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q10.dice\endcsname{79.08}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q10.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q10.rank\endcsname{5 of 40}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q50.L1\endcsname{89.76}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q50.L3\endcsname{89.70}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q50.base\endcsname{88.57}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q50.case\endcsname{\texttt{amos\_0154}}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q50.dice\endcsname{88.57}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q50.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q50.rank\endcsname{21 of 40}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q90.L1\endcsname{93.88}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q90.L3\endcsname{93.87}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q90.base\endcsname{93.83}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q90.case\endcsname{\texttt{amos\_0162}}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q90.dice\endcsname{93.83}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q90.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.amos.f4.q90.rank\endcsname{36 of 40}
\expandafter\gdef\csname R@an.gpu_measures.e5.galfold\endcsname{1}
\expandafter\gdef\csname R@an.gpu_measures.e5.illustration\endcsname{the cases are chosen on the default network's own scores, so per-case differences on them illustrate and do not estimate an arm's effect}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q10.L1\endcsname{40.71}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q10.L3\endcsname{90.22}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q10.base\endcsname{51.44}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q10.case\endcsname{\texttt{case\_00031}}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q10.dice\endcsname{51.44}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q10.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q10.rank\endcsname{11 of 98}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q50.L1\endcsname{89.00}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q50.L3\endcsname{88.09}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q50.base\endcsname{89.45}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q50.case\endcsname{\texttt{case\_00018}}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q50.dice\endcsname{89.45}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q50.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q50.rank\endcsname{50 of 98}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q90.L1\endcsname{92.41}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q90.L3\endcsname{92.78}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q90.base\endcsname{96.00}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q90.case\endcsname{\texttt{case\_00292}}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q90.dice\endcsname{96.00}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q90.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f1.q90.rank\endcsname{88 of 98}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q10.L1\endcsname{57.96}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q10.L3\endcsname{35.41}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q10.base\endcsname{57.95}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q10.case\endcsname{\texttt{case\_00502}}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q10.dice\endcsname{57.95}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q10.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q10.rank\endcsname{11 of 98}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q50.L1\endcsname{90.06}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q50.L3\endcsname{89.78}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q50.base\endcsname{89.62}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q50.case\endcsname{\texttt{case\_00057}}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q50.dice\endcsname{89.62}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q50.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q50.rank\endcsname{50 of 98}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q90.L1\endcsname{95.17}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q90.L3\endcsname{95.83}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q90.base\endcsname{95.95}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q90.case\endcsname{\texttt{case\_00044}}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q90.dice\endcsname{95.95}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q90.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f2.q90.rank\endcsname{88 of 98}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q10.L1\endcsname{78.24}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q10.L3\endcsname{81.03}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q10.base\endcsname{74.97}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q10.case\endcsname{\texttt{case\_00193}}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q10.dice\endcsname{74.97}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q10.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q10.rank\endcsname{11 of 98}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q50.L1\endcsname{91.65}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q50.L3\endcsname{90.76}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q50.base\endcsname{91.36}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q50.case\endcsname{\texttt{case\_00153}}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q50.dice\endcsname{91.36}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q50.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q50.rank\endcsname{50 of 98}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q90.L1\endcsname{96.55}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q90.L3\endcsname{95.62}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q90.base\endcsname{95.22}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q90.case\endcsname{\texttt{case\_00139}}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q90.dice\endcsname{95.22}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q90.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f3.q90.rank\endcsname{88 of 98}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q10.L1\endcsname{92.00}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q10.L3\endcsname{93.48}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q10.base\endcsname{60.58}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q10.case\endcsname{\texttt{case\_00409}}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q10.dice\endcsname{60.58}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q10.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q10.rank\endcsname{11 of 97}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q50.L1\endcsname{84.65}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q50.L3\endcsname{85.78}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q50.base\endcsname{89.01}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q50.case\endcsname{\texttt{case\_00005}}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q50.dice\endcsname{89.01}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q50.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q50.rank\endcsname{49 of 97}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q90.L1\endcsname{94.94}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q90.L3\endcsname{94.97}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q90.base\endcsname{95.22}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q90.case\endcsname{\texttt{case\_00489}}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q90.dice\endcsname{95.22}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q90.nexp\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.kits.f4.q90.rank\endcsname{87 of 97}
\expandafter\gdef\csname R@an.gpu_measures.e5.ncases\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.e5.ncases.word\endcsname{three}
\expandafter\gdef\csname R@an.gpu_measures.e5.nexp\endcsname{72}
\expandafter\gdef\csname R@an.gpu_measures.e5.nsel\endcsname{24}
\expandafter\gdef\csname R@an.gpu_measures.e5.nwant\endcsname{24}
\expandafter\gdef\csname R@an.gpu_measures.e5.pctlist\endcsname{10th, 50th and 90th}
\expandafter\gdef\csname R@an.gpu_measures.e5.rule\endcsname{those at the 10th, 50th and 90th percentile of the per-case Dice of the default network trained on the same fold (ascending by case Dice, ties by case id; rank $\lfloor q(n-1)+\tfrac12\rfloor$), the slice with the largest reference foreground area, fixed before any HyReX or ResEnc-M prediction exists}
\expandafter\gdef\csname R@an.gpu_measures.e5.status\endcsname{24 of 24 selected cases are fixed by the default runs that have finished; 72 of 72 slice exports (cases times arms) have landed}
\expandafter\gdef\csname R@an.gpu_measures.e5.tails\endcsname{the two other arms score above the default in 12 of 16 arm-by-case pairs on the 10th-percentile cases and below it in 7 of 16 arm-by-case pairs on the 90th-percentile cases}
\expandafter\gdef\csname R@an.gpu_measures.empty.acdc.both\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.empty.acdc.one\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.empty.acdc.pairs\endcsname{720}
\expandafter\gdef\csname R@an.gpu_measures.empty.acdc.pct\endcsname{0.00}
\expandafter\gdef\csname R@an.gpu_measures.empty.acdc.shape\endcsname{40 cases $\times$ 3 classes $\times$ 6 frozen-pool default runs}
\expandafter\gdef\csname R@an.gpu_measures.empty.acdc.undef\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.empty.amos.both\endcsname{6}
\expandafter\gdef\csname R@an.gpu_measures.empty.amos.one\endcsname{32}
\expandafter\gdef\csname R@an.gpu_measures.empty.amos.pairs\endcsname{3600}
\expandafter\gdef\csname R@an.gpu_measures.empty.amos.pct\endcsname{1.06}
\expandafter\gdef\csname R@an.gpu_measures.empty.amos.shape\endcsname{40 cases $\times$ 15 classes $\times$ 6 frozen-pool default runs}
\expandafter\gdef\csname R@an.gpu_measures.empty.amos.undef\endcsname{38}
\expandafter\gdef\csname R@an.gpu_measures.empty.kits.both\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.empty.kits.one\endcsname{1}
\expandafter\gdef\csname R@an.gpu_measures.empty.kits.pairs\endcsname{882}
\expandafter\gdef\csname R@an.gpu_measures.empty.kits.pct\endcsname{0.11}
\expandafter\gdef\csname R@an.gpu_measures.empty.kits.shape\endcsname{98 cases $\times$ 3 classes $\times$ 3 frozen-pool default runs}
\expandafter\gdef\csname R@an.gpu_measures.empty.kits.undef\endcsname{1}
\expandafter\gdef\csname R@an.gpu_measures.erf.L1init.acdc.r50xy\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L1init.acdc.r50z\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L1init.amos.r50xy\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L1init.amos.r50z\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L1init.kits.r50xy\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L1init.kits.r50z\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L1trained.acdc.r50xy\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L1trained.acdc.r50z\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L1trained.amos.r50xy\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L1trained.amos.r50z\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L1trained.kits.r50xy\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L1trained.kits.r50z\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L3init.acdc.r50xy\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L3init.acdc.r50z\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L3init.amos.r50xy\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L3init.amos.r50z\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L3init.kits.r50xy\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L3init.kits.r50z\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L3trained.acdc.r50xy\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L3trained.acdc.r50z\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L3trained.amos.r50xy\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L3trained.amos.r50z\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L3trained.kits.r50xy\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.L3trained.kits.r50z\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.baseinit.acdc.r50xy\endcsname{48.8}
\expandafter\gdef\csname R@an.gpu_measures.erf.baseinit.acdc.r50z\endcsname{22.5}
\expandafter\gdef\csname R@an.gpu_measures.erf.baseinit.amos.r50xy\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.baseinit.amos.r50z\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.baseinit.kits.r50xy\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.baseinit.kits.r50z\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.basetrained.acdc.r50xy\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.basetrained.acdc.r50z\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.basetrained.amos.r50xy\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.basetrained.amos.r50z\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.erf.basetrained.kits.r50xy\endcsname{10.5}
\expandafter\gdef\csname R@an.gpu_measures.erf.basetrained.kits.r50z\endcsname{13.5}
\expandafter\gdef\csname R@an.gpu_measures.erf.bound.acdc.axmax\endcsname{y}
\expandafter\gdef\csname R@an.gpu_measures.erf.bound.acdc.axmin\endcsname{z}
\expandafter\gdef\csname R@an.gpu_measures.erf.bound.acdc.riso\endcsname{50.0}
\expandafter\gdef\csname R@an.gpu_measures.erf.bound.acdc.rmax\endcsname{195.0}
\expandafter\gdef\csname R@an.gpu_measures.erf.bound.amos.axmax\endcsname{y}
\expandafter\gdef\csname R@an.gpu_measures.erf.bound.amos.axmin\endcsname{x}
\expandafter\gdef\csname R@an.gpu_measures.erf.bound.amos.riso\endcsname{54.8}
\expandafter\gdef\csname R@an.gpu_measures.erf.bound.amos.rmax\endcsname{65.7}
\expandafter\gdef\csname R@an.gpu_measures.erf.bound.kits.axmax\endcsname{z}
\expandafter\gdef\csname R@an.gpu_measures.erf.bound.kits.axmin\endcsname{y}
\expandafter\gdef\csname R@an.gpu_measures.erf.bound.kits.riso\endcsname{50.0}
\expandafter\gdef\csname R@an.gpu_measures.erf.bound.kits.rmax\endcsname{64.0}
\expandafter\gdef\csname R@an.gpu_measures.erf.cover.acdc.max\endcsname{111}
\expandafter\gdef\csname R@an.gpu_measures.erf.cover.acdc.min\endcsname{105}
\expandafter\gdef\csname R@an.gpu_measures.erf.cover.acdc.z\endcsname{111}
\expandafter\gdef\csname R@an.gpu_measures.erf.cover.amos.max\endcsname{33}
\expandafter\gdef\csname R@an.gpu_measures.erf.cover.amos.min\endcsname{27}
\expandafter\gdef\csname R@an.gpu_measures.erf.cover.amos.z\endcsname{27}
\expandafter\gdef\csname R@an.gpu_measures.erf.cover.kits.max\endcsname{31}
\expandafter\gdef\csname R@an.gpu_measures.erf.cover.kits.min\endcsname{25}
\expandafter\gdef\csname R@an.gpu_measures.erf.cover.kits.z\endcsname{31}
\expandafter\gdef\csname R@an.gpu_measures.erf.extent.acdc\endcsname{$100\times390\times341$ mm}
\expandafter\gdef\csname R@an.gpu_measures.erf.extent.amos\endcsname{$128\times131\times110$ mm}
\expandafter\gdef\csname R@an.gpu_measures.erf.extent.kits\endcsname{$128\times100\times100$ mm}
\expandafter\gdef\csname R@an.gpu_measures.erf.median.acdc\endcsname{$90\times360\times324$ mm}
\expandafter\gdef\csname R@an.gpu_measures.erf.median.amos\endcsname{$470\times400\times400$ mm}
\expandafter\gdef\csname R@an.gpu_measures.erf.median.kits\endcsname{$417\times400\times400$ mm}
\expandafter\gdef\csname R@an.gpu_measures.erf.patch.acdc\endcsname{$20\times256\times224$ voxels at $5.00\times1.52\times1.52$ mm}
\expandafter\gdef\csname R@an.gpu_measures.erf.patch.amos\endcsname{$64\times192\times160$ voxels at $2.00\times0.68\times0.68$ mm}
\expandafter\gdef\csname R@an.gpu_measures.erf.patch.kits\endcsname{$128\times128\times128$ voxels at $1.00\times0.78\times0.78$ mm}
\expandafter\gdef\csname R@an.gpu_measures.est.L1.acdc.kind\endcsname{fresh mean, seeds 1--2}
\expandafter\gdef\csname R@an.gpu_measures.est.L1.acdc.n\endcsname{2}
\expandafter\gdef\csname R@an.gpu_measures.est.L1.acdc.runs\endcsname{ai\_benchrepL1\_acdc\_f0\_e1000\_s1, ai\_benchrepL1\_acdc\_f0\_e1000\_s2}
\expandafter\gdef\csname R@an.gpu_measures.est.L1.acdc.short\endcsname{2 fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.est.L1.amos.kind\endcsname{fresh mean, seeds 1--2}
\expandafter\gdef\csname R@an.gpu_measures.est.L1.amos.n\endcsname{2}
\expandafter\gdef\csname R@an.gpu_measures.est.L1.amos.runs\endcsname{ai\_L1\_amos\_f0\_e1000\_s1, ai\_L1\_amos\_f0\_e1000\_s2}
\expandafter\gdef\csname R@an.gpu_measures.est.L1.amos.short\endcsname{2 fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.est.L1.kits.kind\endcsname{fresh mean, seeds 1--2}
\expandafter\gdef\csname R@an.gpu_measures.est.L1.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.gpu_measures.est.L1.kits.runs\endcsname{ai\_L1\_kits\_f0\_e1000\_s1, ai\_L1\_kits\_f0\_e1000\_s2}
\expandafter\gdef\csname R@an.gpu_measures.est.L1.kits.short\endcsname{2 fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.est.L3.acdc.kind\endcsname{fresh mean, seeds 1--2}
\expandafter\gdef\csname R@an.gpu_measures.est.L3.acdc.n\endcsname{2}
\expandafter\gdef\csname R@an.gpu_measures.est.L3.acdc.runs\endcsname{ai\_benchrepL3\_acdc\_f0\_e1000\_s1, ai\_benchrepL3\_acdc\_f0\_e1000\_s2}
\expandafter\gdef\csname R@an.gpu_measures.est.L3.acdc.short\endcsname{2 fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.est.L3.amos.kind\endcsname{fresh mean, seeds 1--2}
\expandafter\gdef\csname R@an.gpu_measures.est.L3.amos.n\endcsname{2}
\expandafter\gdef\csname R@an.gpu_measures.est.L3.amos.runs\endcsname{ai\_L3\_amos\_f0\_e1000\_s1, ai\_L3\_amos\_f0\_e1000\_s2}
\expandafter\gdef\csname R@an.gpu_measures.est.L3.amos.short\endcsname{2 fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.est.L3.kits.kind\endcsname{fresh mean, seeds 1--2}
\expandafter\gdef\csname R@an.gpu_measures.est.L3.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.gpu_measures.est.L3.kits.runs\endcsname{ai\_L3\_kits\_f0\_e1000\_s1, ai\_L3\_kits\_f0\_e1000\_s2}
\expandafter\gdef\csname R@an.gpu_measures.est.L3.kits.short\endcsname{2 fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.est.base.acdc.kind\endcsname{frozen pool mean, 6 runs}
\expandafter\gdef\csname R@an.gpu_measures.est.base.acdc.n\endcsname{6}
\expandafter\gdef\csname R@an.gpu_measures.est.base.acdc.runs\endcsname{calib\_d027\_base\_e1000\_s0\_r2, calib\_d027\_base\_e1000\_s1\_r1, calib\_d027\_base\_e1000\_s2, team\_static\_confirm\_v1\_baseline\_acdc\_f0\_e1000\_s0, team\_static\_confirm\_v1\_baseline\_acdc\_f0\_e1000\_s1, team\_static\_confirm\_v1\_baseline\_acdc\_f0\_e1000\_s2}
\expandafter\gdef\csname R@an.gpu_measures.est.base.acdc.short\endcsname{frozen pool}
\expandafter\gdef\csname R@an.gpu_measures.est.base.amos.kind\endcsname{frozen pool mean, 6 runs}
\expandafter\gdef\csname R@an.gpu_measures.est.base.amos.n\endcsname{6}
\expandafter\gdef\csname R@an.gpu_measures.est.base.amos.runs\endcsname{calib\_d218\_base\_e1000\_s0, calib\_d218\_base\_e1000\_s1, team\_baseline\_amos\_f0\_e1000\_s2, team\_static\_confirm\_v1\_baseline\_amos\_f0\_e1000\_s0, team\_static\_confirm\_v1\_baseline\_amos\_f0\_e1000\_s1, team\_static\_confirm\_v1\_baseline\_amos\_f0\_e1000\_s2}
\expandafter\gdef\csname R@an.gpu_measures.est.base.amos.short\endcsname{frozen pool}
\expandafter\gdef\csname R@an.gpu_measures.est.base.kits.kind\endcsname{frozen pool mean, 3 runs}
\expandafter\gdef\csname R@an.gpu_measures.est.base.kits.n\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.est.base.kits.runs\endcsname{ai\_base\_kits\_f0\_e1000\_s0, ai\_base\_kits\_f0\_e1000\_s1, ai\_base\_kits\_f0\_e1000\_s2}
\expandafter\gdef\csname R@an.gpu_measures.est.base.kits.short\endcsname{frozen pool}
\expandafter\gdef\csname R@an.gpu_measures.est.freshstate\endcsname{all 6 design-arm $\times$ dataset cells rest on a fresh pair}
\expandafter\gdef\csname R@an.gpu_measures.est.kinds\endcsname{nnU-Net default on AMOS22 rests on its frozen pool mean, 6 runs; HyReX on AMOS22 rests on its fresh mean, seeds 1--2; ResEnc-M on AMOS22 rests on its fresh mean, seeds 1--2; nnU-Net default on KiTS23 rests on its frozen pool mean, 3 runs; HyReX on KiTS23 rests on its fresh mean, seeds 1--2; ResEnc-M on KiTS23 rests on its fresh mean, seeds 1--2; nnU-Net default on ACDC rests on its frozen pool mean, 6 runs; HyReX on ACDC rests on its fresh mean, seeds 1--2; ResEnc-M on ACDC rests on its fresh mean, seeds 1--2}
\expandafter\gdef\csname R@an.gpu_measures.est.ladder\endcsname{the default is its frozen pool (registered, frozen by run id); a design arm is the mean of its registered fresh seeds (1, 2) once every one of them has finished, and its discovery seed 0 until then; a fresh seed is never averaged with the discovery seed and never stands alone}
\expandafter\gdef\csname R@an.gpu_measures.est.ncells\endcsname{6}
\expandafter\gdef\csname R@an.gpu_measures.est.nfresh\endcsname{6}
\expandafter\gdef\csname R@an.gpu_measures.floor.below\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.floor.belowrows\endcsname{none}
\expandafter\gdef\csname R@an.gpu_measures.floor.clause\endcsname{no contrast in this section rests on one seed per arm}
\expandafter\gdef\csname R@an.gpu_measures.floor.hollow\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.floor.mixedrows\endcsname{none}
\expandafter\gdef\csname R@an.gpu_measures.floor.nmixed\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.floor.nrows\endcsname{6}
\expandafter\gdef\csname R@an.gpu_measures.floor.oneseed\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.floor.oneseedrows\endcsname{none}
\expandafter\gdef\csname R@an.gpu_measures.floor.rule\endcsname{the 0.5 pp floor is the registered resolution floor of a difference at one seed per arm (the SE of such a difference is $\sqrt{2}\sigma$); a difference below it is a measured value that is not resolved, and it is reported without a direction.  The boundary figure draws it on a contrast only where each side is a single seed; the gap between two multi-run arms is read against it and against that gap's own null SD}
\expandafter\gdef\csname R@an.gpu_measures.floor.value\endcsname{0.5}
\expandafter\gdef\csname R@an.gpu_measures.hd95.acdc.L3_L1.d\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.hd95.acdc.L3_base.d\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.hd95.amos.L3_L1.d\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.gpu_measures.hd95.amos.L3_base.d\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.gpu_measures.hd95.kits.L3_L1.d\endcsname{\ensuremath{+14.91}}
\expandafter\gdef\csname R@an.gpu_measures.hd95.kits.L3_base.d\endcsname{\ensuremath{-4.36}}
\expandafter\gdef\csname R@an.gpu_measures.hd95pen.acdc.L3_L1.d\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.hd95pen.acdc.L3_base.d\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.hd95pen.amos.L3_L1.d\endcsname{\ensuremath{+1.62}}
\expandafter\gdef\csname R@an.gpu_measures.hd95pen.amos.L3_base.d\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.gpu_measures.hd95pen.kits.L3_L1.d\endcsname{\ensuremath{+14.22}}
\expandafter\gdef\csname R@an.gpu_measures.hd95pen.kits.L3_base.d\endcsname{\ensuremath{-3.74}}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.ga\endcsname{0.74}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.gb\endcsname{1.04}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.gflops\endcsname{492}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.params\endcsname{25.28}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.patch_ms\endcsname{11.7}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.ratio\endcsname{0.57}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.ratio_ga\endcsname{0.97}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.ratio_gb\endcsname{0.99}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.ratio_gflops\endcsname{0.78}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.ratio_params\endcsname{0.83}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.ratio_range\endcsname{0.56 to 0.67}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.ratio_tta\endcsname{0.81}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.ratio_tta_range\endcsname{0.80 to 2.90}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.ratiox\endcsname{0.57$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.s_vol\endcsname{0.03}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.s_vol_tta\endcsname{0.21}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.state\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.state_tta\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.acdc.tflops\endcsname{42.0}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.ga\endcsname{8.51}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.gb\endcsname{10.03}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.gflops\endcsname{821}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.params\endcsname{26.03}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.patch_ms\endcsname{19.1}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.ratio\endcsname{0.84}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.ratio_ga\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.ratio_gb\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.ratio_gflops\endcsname{0.78}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.ratio_params\endcsname{0.84}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.ratio_range\endcsname{0.80 to 0.84}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.ratio_tta\endcsname{0.79}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.ratio_tta_range\endcsname{0.79 to 0.79}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.ratiox\endcsname{0.84$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.s_vol\endcsname{7.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.s_vol_tta\endcsname{46.24}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.state\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.state_tta\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.amos.tflops\endcsname{43.0}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.ga\endcsname{1.96}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.gb\endcsname{2.35}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.gflops\endcsname{734}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.params\endcsname{26.08}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.patch_ms\endcsname{17.8}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.ratio\endcsname{0.79}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.ratio_ga\endcsname{0.99}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.ratio_gb\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.ratio_gflops\endcsname{0.77}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.ratio_params\endcsname{0.84}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.ratio_range\endcsname{0.78 to 1.15}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.ratio_tta\endcsname{0.78}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.ratio_tta_range\endcsname{0.78 to 0.78}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.ratiox\endcsname{0.79$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.s_vol\endcsname{3.58}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.s_vol_tta\endcsname{27.41}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.state\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.state_tta\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.D2.kits.tflops\endcsname{41.1}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.ga\endcsname{1.04}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.gb\endcsname{1.32}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.gflops\endcsname{1195}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.params\endcsname{101.53}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.patch_ms\endcsname{22.7}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.ratio\endcsname{1.07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.ratio_ga\endcsname{1.38}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.ratio_gb\endcsname{1.25}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.ratio_gflops\endcsname{1.90}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.ratio_params\endcsname{3.34}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.ratio_range\endcsname{1.06 to 1.16}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.ratio_tta\endcsname{1.50}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.ratio_tta_range\endcsname{1.48 to 1.51}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.ratiox\endcsname{1.07$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.s_vol\endcsname{0.06}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.s_vol_tta\endcsname{0.38}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.state\endcsname{not resolved from the default}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.state_tta\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.acdc.tflops\endcsname{52.6}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.ga\endcsname{8.82}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.gb\endcsname{10.26}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.gflops\endcsname{1953}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.params\endcsname{102.28}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.patch_ms\endcsname{35.7}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.ratio\endcsname{1.38}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.ratio_ga\endcsname{1.03}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.ratio_gb\endcsname{1.02}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.ratio_gflops\endcsname{1.86}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.ratio_params\endcsname{3.29}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.ratio_range\endcsname{1.38 to 1.38}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.ratio_tta\endcsname{1.45}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.ratio_tta_range\endcsname{1.45 to 1.45}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.ratiox\endcsname{1.38$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.s_vol\endcsname{11.55}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.s_vol_tta\endcsname{85.15}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.state\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.state_tta\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.amos.tflops\endcsname{54.8}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.ga\endcsname{2.27}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.gb\endcsname{2.93}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.gflops\endcsname{1435}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.params\endcsname{102.35}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.patch_ms\endcsname{30.2}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.ratio\endcsname{1.30}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.ratio_ga\endcsname{1.15}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.ratio_gb\endcsname{1.24}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.ratio_gflops\endcsname{1.50}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.ratio_params\endcsname{3.28}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.ratio_range\endcsname{1.30 to 1.31}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.ratio_tta\endcsname{1.32}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.ratio_tta_range\endcsname{1.32 to 1.32}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.ratiox\endcsname{1.30$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.s_vol\endcsname{5.92}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.s_vol_tta\endcsname{46.40}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.state\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.state_tta\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1.kits.tflops\endcsname{47.5}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.ga\endcsname{1.04}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.gb\endcsname{1.36}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.gflops\endcsname{1174}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.params\endcsname{101.63}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.patch_ms\endcsname{22.5}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.ratio\endcsname{1.03}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.ratio_ga\endcsname{1.38}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.ratio_gb\endcsname{1.29}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.ratio_gflops\endcsname{1.86}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.ratio_params\endcsname{3.35}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.ratio_range\endcsname{0.96 to 1.45}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.ratio_tta\endcsname{1.49}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.ratio_tta_range\endcsname{1.45 to 1.51}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.ratiox\endcsname{1.03$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.s_vol\endcsname{0.06}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.s_vol_tta\endcsname{0.38}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.state\endcsname{not resolved from the default}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.state_tta\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.acdc.tflops\endcsname{52.1}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.ga\endcsname{8.82}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.gb\endcsname{10.32}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.gflops\endcsname{1917}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.params\endcsname{102.37}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.patch_ms\endcsname{35.2}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.ratio\endcsname{1.36}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.ratio_ga\endcsname{1.03}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.ratio_gb\endcsname{1.03}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.ratio_gflops\endcsname{1.82}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.ratio_params\endcsname{3.29}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.ratio_range\endcsname{1.36 to 1.36}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.ratio_tta\endcsname{1.43}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.ratio_tta_range\endcsname{1.43 to 1.43}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.ratiox\endcsname{1.36$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.s_vol\endcsname{11.39}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.s_vol_tta\endcsname{84.07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.state\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.state_tta\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.amos.tflops\endcsname{54.4}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.ga\endcsname{2.26}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.gb\endcsname{2.69}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.gflops\endcsname{1319}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.params\endcsname{102.43}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.patch_ms\endcsname{29.1}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.ratio\endcsname{1.26}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.ratio_ga\endcsname{1.14}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.ratio_gb\endcsname{1.14}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.ratio_gflops\endcsname{1.38}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.ratio_params\endcsname{3.28}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.ratio_range\endcsname{1.26 to 1.27}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.ratio_tta\endcsname{1.28}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.ratio_tta_range\endcsname{1.28 to 1.28}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.ratiox\endcsname{1.26$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.s_vol\endcsname{5.75}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.s_vol_tta\endcsname{44.79}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.state\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.state_tta\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L1b.kits.tflops\endcsname{45.3}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.ga\endcsname{0.73}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.gb\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.gflops\endcsname{462}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.params\endcsname{23.68}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.patch_ms\endcsname{21.2}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.ratio\endcsname{0.96}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.ratio_ga\endcsname{0.96}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.ratio_gb\endcsname{0.95}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.ratio_gflops\endcsname{0.73}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.ratio_params\endcsname{0.78}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.ratio_range\endcsname{0.91 to 1.07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.ratio_tta\endcsname{1.41}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.ratio_tta_range\endcsname{1.39 to 1.41}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.ratiox\endcsname{0.96$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.s_vol\endcsname{0.06}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.s_vol_tta\endcsname{0.36}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.state\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.state_tta\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.acdc.tflops\endcsname{21.8}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.ga\endcsname{8.51}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.gb\endcsname{10.07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.gflops\endcsname{770}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.params\endcsname{24.43}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.patch_ms\endcsname{34.6}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.ratio\endcsname{1.34}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.ratio_ga\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.ratio_gb\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.ratio_gflops\endcsname{0.73}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.ratio_params\endcsname{0.78}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.ratio_range\endcsname{1.34 to 1.34}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.ratio_tta\endcsname{1.41}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.ratio_tta_range\endcsname{1.41 to 1.41}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.ratiox\endcsname{1.34$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.s_vol\endcsname{11.23}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.s_vol_tta\endcsname{82.61}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.state\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.state_tta\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.amos.tflops\endcsname{22.2}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.ga\endcsname{1.95}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.gb\endcsname{2.43}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.gflops\endcsname{804}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.params\endcsname{24.50}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.patch_ms\endcsname{29.9}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.ratio\endcsname{1.29}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.ratio_ga\endcsname{0.99}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.ratio_gb\endcsname{1.03}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.ratio_gflops\endcsname{0.84}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.ratio_params\endcsname{0.79}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.ratio_range\endcsname{1.29 to 1.30}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.ratio_tta\endcsname{1.31}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.ratio_tta_range\endcsname{1.31 to 1.31}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.ratiox\endcsname{1.29$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.s_vol\endcsname{5.90}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.s_vol_tta\endcsname{45.96}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.state\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.state_tta\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L2.kits.tflops\endcsname{26.8}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.ga\endcsname{0.75}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.gb\endcsname{0.94}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.gflops\endcsname{868}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.params\endcsname{28.85}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.patch_ms\endcsname{23.1}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.ratio\endcsname{0.94}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.ratio_ga\endcsname{0.99}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.ratio_gb\endcsname{0.89}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.ratio_gflops\endcsname{1.38}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.ratio_params\endcsname{0.95}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.ratio_range\endcsname{0.94 to 0.94}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.ratio_tta\endcsname{1.50}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.ratio_tta_range\endcsname{1.50 to 1.54}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.ratiox\endcsname{0.94$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.s_vol\endcsname{0.06}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.s_vol_tta\endcsname{0.38}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.state\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.state_tta\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.acdc.tflops\endcsname{37.6}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.ga\endcsname{8.53}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.gb\endcsname{9.84}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.gflops\endcsname{1463}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.params\endcsname{29.59}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.patch_ms\endcsname{36.7}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.ratio\endcsname{1.42}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.ratio_ga\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.ratio_gb\endcsname{0.98}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.ratio_gflops\endcsname{1.39}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.ratio_params\endcsname{0.95}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.ratio_range\endcsname{1.42 to 1.42}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.ratio_tta\endcsname{1.49}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.ratio_tta_range\endcsname{1.49 to 1.52}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.ratiox\endcsname{1.42$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.s_vol\endcsname{11.88}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.s_vol_tta\endcsname{87.59}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.state\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.state_tta\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.amos.tflops\endcsname{39.8}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.ga\endcsname{1.97}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.gb\endcsname{2.34}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.gflops\endcsname{1173}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.params\endcsname{29.66}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.patch_ms\endcsname{31.5}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.ratio\endcsname{1.36}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.ratio_ga\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.ratio_gb\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.ratio_gflops\endcsname{1.23}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.ratio_params\endcsname{0.95}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.ratio_range\endcsname{1.36 to 1.36}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.ratio_tta\endcsname{1.38}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.ratio_tta_range\endcsname{1.38 to 1.38}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.ratiox\endcsname{1.36$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.s_vol\endcsname{6.19}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.s_vol_tta\endcsname{48.34}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.state\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.state_tta\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L3.kits.tflops\endcsname{37.2}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.ga\endcsname{1.05}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.gb\endcsname{1.33}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.gflops\endcsname{1175}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.params\endcsname{102.02}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.patch_ms\endcsname{24.3}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.ratio\endcsname{1.59}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.ratio_ga\endcsname{1.39}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.ratio_gb\endcsname{1.26}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.ratio_gflops\endcsname{1.86}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.ratio_params\endcsname{3.36}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.ratio_range\endcsname{1.04 to 1.87}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.ratio_tta\endcsname{1.61}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.ratio_tta_range\endcsname{1.56 to 1.61}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.ratiox\endcsname{1.59$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.s_vol\endcsname{0.09}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.s_vol_tta\endcsname{0.41}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.state\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.state_tta\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.acdc.tflops\endcsname{48.3}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.ga\endcsname{8.83}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.gb\endcsname{10.34}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.gflops\endcsname{1917}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.params\endcsname{102.77}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.patch_ms\endcsname{37.4}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.ratio\endcsname{1.44}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.ratio_ga\endcsname{1.03}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.ratio_gb\endcsname{1.03}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.ratio_gflops\endcsname{1.82}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.ratio_params\endcsname{3.30}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.ratio_range\endcsname{1.44 to 1.48}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.ratio_tta\endcsname{1.52}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.ratio_tta_range\endcsname{1.52 to 1.52}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.ratiox\endcsname{1.44$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.s_vol\endcsname{12.09}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.s_vol_tta\endcsname{89.23}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.state\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.state_tta\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.amos.tflops\endcsname{51.3}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.ga\endcsname{2.27}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.gb\endcsname{2.70}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.gflops\endcsname{1319}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.params\endcsname{102.82}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.patch_ms\endcsname{30.9}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.ratio\endcsname{1.33}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.ratio_ga\endcsname{1.15}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.ratio_gb\endcsname{1.15}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.ratio_gflops\endcsname{1.38}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.ratio_params\endcsname{3.30}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.ratio_range\endcsname{1.33 to 1.35}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.ratio_tta\endcsname{1.35}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.ratio_tta_range\endcsname{1.35 to 1.35}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.ratiox\endcsname{1.33$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.s_vol\endcsname{6.08}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.s_vol_tta\endcsname{47.48}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.state\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.state_tta\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L4.kits.tflops\endcsname{42.6}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.ga\endcsname{0.77}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.gb\endcsname{1.03}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.gflops\endcsname{1058}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.params\endcsname{30.35}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.patch_ms\endcsname{27.0}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.ratio\endcsname{1.11}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.ratio_ga\endcsname{1.01}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.ratio_gb\endcsname{0.97}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.ratio_gflops\endcsname{1.68}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.ratio_params\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.ratio_range\endcsname{1.10 to 1.35}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.ratio_tta\endcsname{1.77}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.ratio_tta_range\endcsname{1.76 to 1.79}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.ratiox\endcsname{1.11$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.s_vol\endcsname{0.07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.s_vol_tta\endcsname{0.45}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.state\endcsname{not resolved from the default}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.state_tta\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.acdc.tflops\endcsname{39.2}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.ga\endcsname{8.54}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.gb\endcsname{9.99}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.gflops\endcsname{1789}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.params\endcsname{31.09}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.patch_ms\endcsname{42.4}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.ratio\endcsname{1.61}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.ratio_ga\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.ratio_gb\endcsname{0.99}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.ratio_gflops\endcsname{1.70}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.ratio_params\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.ratio_range\endcsname{1.61 to 1.61}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.ratio_tta\endcsname{1.72}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.ratio_tta_range\endcsname{1.72 to 1.72}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.ratiox\endcsname{1.61$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.s_vol\endcsname{13.50}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.s_vol_tta\endcsname{100.85}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.state\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.state_tta\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.amos.tflops\endcsname{42.2}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.ga\endcsname{1.99}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.gb\endcsname{2.36}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.gflops\endcsname{1347}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.params\endcsname{31.17}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.patch_ms\endcsname{35.1}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.ratio\endcsname{1.51}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.ratio_ga\endcsname{1.01}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.ratio_gb\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.ratio_gflops\endcsname{1.41}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.ratio_params\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.ratio_range\endcsname{1.51 to 1.52}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.ratio_tta\endcsname{1.54}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.ratio_tta_range\endcsname{1.54 to 1.54}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.ratiox\endcsname{1.51$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.s_vol\endcsname{6.89}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.s_vol_tta\endcsname{53.95}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.state\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.state_tta\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.L6.kits.tflops\endcsname{38.4}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.ga\endcsname{0.68}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.gb\endcsname{0.83}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.gflops\endcsname{609}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.params\endcsname{30.26}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.patch_ms\endcsname{14.7}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.ratio\endcsname{1.23}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.ratio_ga\endcsname{0.90}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.ratio_gb\endcsname{0.79}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.ratio_gflops\endcsname{0.97}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.ratio_params\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.ratio_range\endcsname{1.07 to 1.91}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.ratio_tta\endcsname{4.98}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.ratio_tta_range\endcsname{1.04 to 8.55}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.ratiox\endcsname{1.23$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.refbasis\endcsname{same-batch default (Addendum AT)}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.s_vol\endcsname{0.05}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.s_vol_tta\endcsname{1.32}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.state\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.state_tta\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.acdc.tflops\endcsname{41.4}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.ga\endcsname{8.53}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.gb\endcsname{9.93}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.gflops\endcsname{1026}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.params\endcsname{31.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.patch_ms\endcsname{22.7}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.ratio\endcsname{0.94}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.ratio_ga\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.ratio_gb\endcsname{0.99}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.ratio_gflops\endcsname{0.97}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.ratio_params\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.ratio_range\endcsname{0.94 to 0.94}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.ratio_tta\endcsname{0.93}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.ratio_tta_range\endcsname{0.93 to 0.93}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.ratiox\endcsname{0.94$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.refbasis\endcsname{same-batch default (Addendum AT)}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.s_vol\endcsname{8.12}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.s_vol_tta\endcsname{54.76}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.state\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.state_tta\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.amos.tflops\endcsname{45.3}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.ga\endcsname{1.85}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.gb\endcsname{2.48}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.gflops\endcsname{747}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.params\endcsname{31.04}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.patch_ms\endcsname{19.7}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.ratio\endcsname{0.86}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.ratio_ga\endcsname{0.93}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.ratio_gb\endcsname{1.05}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.ratio_gflops\endcsname{0.78}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.ratio_params\endcsname{0.99}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.ratio_range\endcsname{0.86 to 0.87}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.ratio_tta\endcsname{0.87}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.ratio_tta_range\endcsname{0.86 to 0.89}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.ratiox\endcsname{0.86$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.refbasis\endcsname{same-batch default (Addendum AT)}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.s_vol\endcsname{3.95}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.s_vol_tta\endcsname{30.76}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.state\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.state_tta\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7A1.kits.tflops\endcsname{37.9}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.ga\endcsname{0.64}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.gb\endcsname{0.95}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.gflops\endcsname{354}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.params\endcsname{20.33}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.patch_ms\endcsname{11.4}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.ratio\endcsname{0.86}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.ratio_ga\endcsname{0.85}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.ratio_gb\endcsname{0.90}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.ratio_gflops\endcsname{0.56}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.ratio_params\endcsname{0.67}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.ratio_range\endcsname{0.82 to 0.87}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.ratio_tta\endcsname{0.76}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.ratio_tta_range\endcsname{0.72 to 0.76}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.ratiox\endcsname{0.86$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.refbasis\endcsname{same-batch default (Addendum AT)}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.s_vol\endcsname{0.04}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.s_vol_tta\endcsname{0.20}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.state\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.state_tta\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.acdc.tflops\endcsname{31.0}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.ga\endcsname{8.49}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.gb\endcsname{9.63}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.gflops\endcsname{589}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.params\endcsname{21.08}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.patch_ms\endcsname{18.2}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.ratio\endcsname{0.78}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.ratio_ga\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.ratio_gb\endcsname{0.96}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.ratio_gflops\endcsname{0.56}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.ratio_params\endcsname{0.68}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.ratio_range\endcsname{0.78 to 0.79}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.ratio_tta\endcsname{0.75}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.ratio_tta_range\endcsname{0.75 to 0.75}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.ratiox\endcsname{0.78$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.refbasis\endcsname{same-batch default (Addendum AT)}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.s_vol\endcsname{6.71}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.s_vol_tta\endcsname{44.13}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.state\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.state_tta\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.amos.tflops\endcsname{32.4}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.ga\endcsname{1.80}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.gb\endcsname{2.42}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.gflops\endcsname{514}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.params\endcsname{21.11}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.patch_ms\endcsname{16.8}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.ratio\endcsname{0.74}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.ratio_ga\endcsname{0.91}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.ratio_gb\endcsname{1.03}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.ratio_gflops\endcsname{0.54}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.ratio_params\endcsname{0.68}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.ratio_range\endcsname{0.74 to 0.75}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.ratio_tta\endcsname{0.73}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.ratio_tta_range\endcsname{0.73 to 0.73}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.ratiox\endcsname{0.74$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.refbasis\endcsname{same-batch default (Addendum AT)}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.s_vol\endcsname{3.41}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.s_vol_tta\endcsname{25.81}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.state\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.state_tta\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V7C1.kits.tflops\endcsname{30.6}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.ga\endcsname{0.68}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.gb\endcsname{0.84}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.gflops\endcsname{360}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.params\endcsname{30.53}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.patch_ms\endcsname{16.0}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.ratio\endcsname{1.03}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.ratio_ga\endcsname{0.90}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.ratio_gb\endcsname{0.79}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.ratio_gflops\endcsname{0.57}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.ratio_params\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.ratio_range\endcsname{0.88 to 1.09}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.ratio_tta\endcsname{0.94}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.ratio_tta_range\endcsname{0.90 to 1.04}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.ratiox\endcsname{1.03$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.refbasis\endcsname{same-batch default (Addendum AT)}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.s_vol\endcsname{0.04}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.s_vol_tta\endcsname{0.25}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.state\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.state_tta\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.acdc.tflops\endcsname{22.5}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.ga\endcsname{8.53}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.gb\endcsname{9.84}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.gflops\endcsname{592}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.params\endcsname{31.27}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.patch_ms\endcsname{20.1}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.ratio\endcsname{0.86}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.ratio_ga\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.ratio_gb\endcsname{0.98}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.ratio_gflops\endcsname{0.56}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.ratio_params\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.ratio_range\endcsname{0.85 to 0.98}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.ratio_tta\endcsname{0.83}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.ratio_tta_range\endcsname{0.82 to 0.83}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.ratiox\endcsname{0.86$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.refbasis\endcsname{same-batch default (Addendum AT)}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.s_vol\endcsname{7.37}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.s_vol_tta\endcsname{48.81}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.state\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.state_tta\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.amos.tflops\endcsname{29.4}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.ga\endcsname{1.84}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.gb\endcsname{2.48}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.gflops\endcsname{515}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.params\endcsname{31.31}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.patch_ms\endcsname{18.7}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.ratio\endcsname{0.82}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.ratio_ga\endcsname{0.93}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.ratio_gb\endcsname{1.05}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.ratio_gflops\endcsname{0.54}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.ratio_params\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.ratio_range\endcsname{0.82 to 0.82}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.ratio_tta\endcsname{0.81}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.ratio_tta_range\endcsname{0.81 to 0.82}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.ratiox\endcsname{0.82$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.refbasis\endcsname{same-batch default (Addendum AT)}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.s_vol\endcsname{3.76}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.s_vol_tta\endcsname{28.65}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.state\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.state_tta\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8A1.kits.tflops\endcsname{27.6}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.ga\endcsname{0.63}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.gb\endcsname{0.82}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.gflops\endcsname{263}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.params\endcsname{17.44}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.patch_ms\endcsname{9.0}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.ratio\endcsname{1.26}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.ratio_ga\endcsname{0.83}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.ratio_gb\endcsname{0.78}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.ratio_gflops\endcsname{0.42}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.ratio_params\endcsname{0.57}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.ratio_range\endcsname{1.05 to 2.10}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.ratio_tta\endcsname{0.63}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.ratio_tta_range\endcsname{0.58 to 0.69}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.ratiox\endcsname{1.26$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.refbasis\endcsname{same-batch default (Addendum AT)}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.s_vol\endcsname{0.05}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.s_vol_tta\endcsname{0.17}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.state\endcsname{above the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.state_tta\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.acdc.tflops\endcsname{29.4}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.ga\endcsname{8.48}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.gb\endcsname{9.68}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.gflops\endcsname{439}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.params\endcsname{18.19}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.patch_ms\endcsname{13.5}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.ratio\endcsname{0.62}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.ratio_ga\endcsname{0.99}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.ratio_gb\endcsname{0.96}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.ratio_gflops\endcsname{0.42}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.ratio_params\endcsname{0.58}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.ratio_range\endcsname{0.62 to 0.63}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.ratio_tta\endcsname{0.56}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.ratio_tta_range\endcsname{0.56 to 0.57}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.ratiox\endcsname{0.62$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.refbasis\endcsname{same-batch default (Addendum AT)}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.s_vol\endcsname{5.35}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.s_vol_tta\endcsname{33.39}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.state\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.state_tta\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.amos.tflops\endcsname{32.5}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.ga\endcsname{1.79}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.gb\endcsname{2.44}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.gflops\endcsname{337}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.params\endcsname{18.21}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.patch_ms\endcsname{12.3}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.ratio\endcsname{0.56}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.ratio_ga\endcsname{0.91}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.ratio_gb\endcsname{1.04}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.ratio_gflops\endcsname{0.35}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.ratio_params\endcsname{0.58}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.ratio_range\endcsname{0.55 to 0.56}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.ratio_tta\endcsname{0.53}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.ratio_tta_range\endcsname{0.53 to 0.53}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.ratiox\endcsname{0.56$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.refbasis\endcsname{same-batch default (Addendum AT)}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.s_vol\endcsname{2.54}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.s_vol_tta\endcsname{18.79}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.state\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.state_tta\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B1.kits.tflops\endcsname{27.5}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.ga\endcsname{0.64}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.gb\endcsname{0.99}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.gflops\endcsname{333}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.params\endcsname{20.32}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.patch_ms\endcsname{9.6}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.ratio\endcsname{0.89}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.ratio_ga\endcsname{0.85}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.ratio_gb\endcsname{0.94}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.ratio_gflops\endcsname{0.53}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.ratio_params\endcsname{0.67}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.ratio_range\endcsname{0.82 to 1.12}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.ratio_tta\endcsname{0.65}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.ratio_tta_range\endcsname{0.63 to 0.66}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.ratiox\endcsname{0.89$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.refbasis\endcsname{same-batch default (Addendum AT)}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.s_vol\endcsname{0.04}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.s_vol_tta\endcsname{0.17}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.state\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.state_tta\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.acdc.tflops\endcsname{34.5}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.ga\endcsname{8.49}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.gb\endcsname{9.71}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.gflops\endcsname{553}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.params\endcsname{21.07}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.patch_ms\endcsname{15.2}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.ratio\endcsname{0.68}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.ratio_ga\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.ratio_gb\endcsname{0.97}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.ratio_gflops\endcsname{0.53}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.ratio_params\endcsname{0.68}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.ratio_range\endcsname{0.67 to 0.69}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.ratio_tta\endcsname{0.62}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.ratio_tta_range\endcsname{0.62 to 0.63}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.ratiox\endcsname{0.68$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.refbasis\endcsname{same-batch default (Addendum AT)}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.s_vol\endcsname{5.82}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.s_vol_tta\endcsname{36.90}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.state\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.state_tta\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.amos.tflops\endcsname{36.4}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.ga\endcsname{1.80}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.gb\endcsname{2.46}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.gflops\endcsname{398}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.params\endcsname{21.08}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.patch_ms\endcsname{13.2}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.ratio\endcsname{0.59}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.ratio_ga\endcsname{0.91}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.ratio_gb\endcsname{1.04}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.ratio_gflops\endcsname{0.42}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.ratio_params\endcsname{0.68}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.ratio_range\endcsname{0.59 to 0.59}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.ratio_tta\endcsname{0.57}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.ratio_tta_range\endcsname{0.57 to 0.57}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.ratiox\endcsname{0.59$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.refbasis\endcsname{same-batch default (Addendum AT)}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.s_vol\endcsname{2.69}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.s_vol_tta\endcsname{20.16}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.state\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.state_tta\endcsname{below the default's repeat range}
\expandafter\gdef\csname R@an.gpu_measures.infer.V8B2.kits.tflops\endcsname{30.1}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.fellback\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.ga\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.gb\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.gflops\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.params\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.patch_ms\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.ratio\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.ratio_ga\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.ratio_gb\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.ratio_gflops\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.ratio_params\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.ratio_range\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.ratio_tta\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.ratio_tta_range\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.ratiox\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.s_vol\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.s_vol_tta\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.state\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.state_tta\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.acdc.tflops\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.fellback\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.ga\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.gb\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.gflops\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.params\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.patch_ms\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.ratio\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.ratio_ga\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.ratio_gb\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.ratio_gflops\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.ratio_params\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.ratio_range\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.ratio_tta\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.ratio_tta_range\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.ratiox\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.s_vol\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.s_vol_tta\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.state\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.state_tta\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.amos.tflops\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.fellback\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.ga\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.gb\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.gflops\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.params\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.patch_ms\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.ratio\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.ratio_ga\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.ratio_gb\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.ratio_gflops\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.ratio_params\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.ratio_range\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.ratio_tta\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.ratio_tta_range\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.ratiox\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.s_vol\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.s_vol_tta\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.state\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.state_tta\endcsname{pending}
\expandafter\gdef\csname R@an.gpu_measures.infer.W4.kits.tflops\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.ga\endcsname{0.76}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.gb\endcsname{1.06}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.gflops\endcsname{630}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.params\endcsname{30.38}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.patch_ms\endcsname{15.0}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.ratio\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.ratio_ga\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.ratio_gb\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.ratio_gflops\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.ratio_params\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.ratio_range\endcsname{0.96 to 1.34}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.ratio_tta\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.ratio_tta_range\endcsname{1.00 to 1.03}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.ratiox\endcsname{1.00$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.s_vol\endcsname{0.06}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.s_vol_tta\endcsname{0.26}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.state\endcsname{not resolved from the default}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.state_tta\endcsname{not resolved from the default}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.acdc.tflops\endcsname{42.2}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.ga\endcsname{8.53}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.gb\endcsname{10.05}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.gflops\endcsname{1053}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.params\endcsname{31.12}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.patch_ms\endcsname{24.5}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.ratio\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.ratio_ga\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.ratio_gb\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.ratio_gflops\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.ratio_params\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.ratio_range\endcsname{1.00 to 1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.ratio_tta\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.ratio_tta_range\endcsname{1.00 to 1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.ratiox\endcsname{1.00$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.s_vol\endcsname{8.38}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.s_vol_tta\endcsname{58.72}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.state\endcsname{not resolved from the default}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.state_tta\endcsname{not resolved from the default}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.amos.tflops\endcsname{43.0}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.fellback\endcsname{no}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.ga\endcsname{1.98}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.gb\endcsname{2.35}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.gflops\endcsname{955}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.params\endcsname{31.20}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.patch_ms\endcsname{23.0}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.ratio\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.ratio_ga\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.ratio_gb\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.ratio_gflops\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.ratio_params\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.ratio_range\endcsname{1.00 to 1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.ratio_tta\endcsname{1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.ratio_tta_range\endcsname{1.00 to 1.00}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.ratiox\endcsname{1.00$\times$}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.refbasis\endcsname{atlas default of 2026-10-07}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.s_vol\endcsname{4.56}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.s_vol_tta\endcsname{35.13}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.state\endcsname{not resolved from the default}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.state_tta\endcsname{not resolved from the default}
\expandafter\gdef\csname R@an.gpu_measures.infer.base.kits.tflops\endcsname{41.6}
\expandafter\gdef\csname R@an.gpu_measures.lesion.L1.fp\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.lesion.L1.sens.large\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.lesion.L1.sens.mid\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.lesion.L1.sens.small\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.lesion.L3.fp\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.lesion.L3.sens.large\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.lesion.L3.sens.mid\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.lesion.L3.sens.small\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.lesion.base.fp\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.lesion.base.sens.large\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.lesion.base.sens.mid\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.lesion.base.sens.small\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.lesion.rule\endcsname{a reference lesion counts as detected when a predicted component overlaps it with Dice $\geq 0.1$; size bins are thirds of the reference lesion volume, fixed on the reference alone}
\expandafter\gdef\csname R@an.gpu_measures.meas.excl\endcsname{no registered cross-validation harness run has been excluded for its provenance}
\expandafter\gdef\csname R@an.gpu_measures.meas.ncells\endcsname{48}
\expandafter\gdef\csname R@an.gpu_measures.meas.nexcl\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.meas.nfailed\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.meas.nheld\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.meas.nother\endcsname{16}
\expandafter\gdef\csname R@an.gpu_measures.meas.npartial\endcsname{2}
\expandafter\gdef\csname R@an.gpu_measures.meas.nrec\endcsname{36}
\expandafter\gdef\csname R@an.gpu_measures.meas.ntrials\endcsname{24}
\expandafter\gdef\csname R@an.gpu_measures.meas.nunreg\endcsname{8}
\expandafter\gdef\csname R@an.gpu_measures.meas.status\endcsname{36 of 36 checkpoint-measurement records have landed (48 of 48 trial-by-setting cells, 24 of 24 trials in both mirroring settings)}
\expandafter\gdef\csname R@an.gpu_measures.meas.unreg\endcsname{8 measured cross-validation trials have no registered harness run (ai\_benchcvV7A1\_kits\_f1\_e1000\_s0, ai\_benchcvV7A1\_kits\_f2\_e1000\_s0, ai\_benchcvV7A1\_kits\_f3\_e1000\_s0 ...) and are held as pending records, outside every estimate}
\expandafter\gdef\csname R@an.gpu_measures.nsd1.acdc.L3_L1.d\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.nsd1.acdc.L3_base.d\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.nsd1.amos.L3_L1.d\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.gpu_measures.nsd1.amos.L3_base.d\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.gpu_measures.nsd1.kits.L3_L1.d\endcsname{\ensuremath{-1.42}}
\expandafter\gdef\csname R@an.gpu_measures.nsd1.kits.L3_base.d\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.gpu_measures.nsd2.acdc.L3_L1.d\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.nsd2.acdc.L3_base.d\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.nsd2.amos.L3_L1.d\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.gpu_measures.nsd2.amos.L3_base.d\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.gpu_measures.nsd2.kits.L3_L1.d\endcsname{\ensuremath{-1.66}}
\expandafter\gdef\csname R@an.gpu_measures.nsd2.kits.L3_base.d\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@an.gpu_measures.plan.acdc.batch\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.plan.amos.batch\endcsname{2}
\expandafter\gdef\csname R@an.gpu_measures.plan.kits.batch\endcsname{2}
\expandafter\gdef\csname R@an.gpu_measures.protocol.acdc\endcsname{TTA}
\expandafter\gdef\csname R@an.gpu_measures.protocol.amos\endcsname{no TTA}
\expandafter\gdef\csname R@an.gpu_measures.protocol.kits\endcsname{no TTA}
\expandafter\gdef\csname R@an.gpu_measures.qual.acdc.adv.case\endcsname{\texttt{patient085\_frame09}}
\expandafter\gdef\csname R@an.gpu_measures.qual.acdc.adv.delta\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.gpu_measures.qual.acdc.adv.dice\endcsname{91.99}
\expandafter\gdef\csname R@an.gpu_measures.qual.acdc.adv.rank\endcsname{1 of 40 by $\Delta$}
\expandafter\gdef\csname R@an.gpu_measures.qual.acdc.q10.case\endcsname{\texttt{patient046\_frame10}}
\expandafter\gdef\csname R@an.gpu_measures.qual.acdc.q10.dice\endcsname{88.61}
\expandafter\gdef\csname R@an.gpu_measures.qual.acdc.q10.rank\endcsname{5 of 40}
\expandafter\gdef\csname R@an.gpu_measures.qual.acdc.q50.case\endcsname{\texttt{patient070\_frame10}}
\expandafter\gdef\csname R@an.gpu_measures.qual.acdc.q50.dice\endcsname{92.68}
\expandafter\gdef\csname R@an.gpu_measures.qual.acdc.q50.rank\endcsname{21 of 40}
\expandafter\gdef\csname R@an.gpu_measures.qual.acdc.q90.case\endcsname{\texttt{patient080\_frame10}}
\expandafter\gdef\csname R@an.gpu_measures.qual.acdc.q90.dice\endcsname{94.72}
\expandafter\gdef\csname R@an.gpu_measures.qual.acdc.q90.rank\endcsname{36 of 40}
\expandafter\gdef\csname R@an.gpu_measures.qual.advrule\endcsname{the validation case with the most negative per-case HyReX (discovery seed 0) $-$ frozen default pool Dice: the one slot that reads the evaluated design's own scores, fixed on a finished seed before any re-prediction exists and chosen to be the worst case for HyReX}
\expandafter\gdef\csname R@an.gpu_measures.qual.amos.adv.case\endcsname{\texttt{amos\_0104}}
\expandafter\gdef\csname R@an.gpu_measures.qual.amos.adv.delta\endcsname{\ensuremath{-3.29}}
\expandafter\gdef\csname R@an.gpu_measures.qual.amos.adv.dice\endcsname{92.47}
\expandafter\gdef\csname R@an.gpu_measures.qual.amos.adv.rank\endcsname{1 of 40 by $\Delta$}
\expandafter\gdef\csname R@an.gpu_measures.qual.amos.anchor.case\endcsname{\texttt{amos\_0299}}
\expandafter\gdef\csname R@an.gpu_measures.qual.amos.anchor.dice\endcsname{89.87}
\expandafter\gdef\csname R@an.gpu_measures.qual.amos.anchor.rank\endcsname{5 of 10 in stratum}
\expandafter\gdef\csname R@an.gpu_measures.qual.amos.q10.case\endcsname{\texttt{amos\_0057}}
\expandafter\gdef\csname R@an.gpu_measures.qual.amos.q10.dice\endcsname{73.37}
\expandafter\gdef\csname R@an.gpu_measures.qual.amos.q10.rank\endcsname{5 of 40}
\expandafter\gdef\csname R@an.gpu_measures.qual.amos.q50.case\endcsname{\texttt{amos\_0358}}
\expandafter\gdef\csname R@an.gpu_measures.qual.amos.q50.dice\endcsname{90.22}
\expandafter\gdef\csname R@an.gpu_measures.qual.amos.q50.rank\endcsname{21 of 40}
\expandafter\gdef\csname R@an.gpu_measures.qual.amos.q90.case\endcsname{\texttt{amos\_0141}}
\expandafter\gdef\csname R@an.gpu_measures.qual.amos.q90.dice\endcsname{94.14}
\expandafter\gdef\csname R@an.gpu_measures.qual.amos.q90.rank\endcsname{36 of 40}
\expandafter\gdef\csname R@an.gpu_measures.qual.amos.stratum.n\endcsname{10}
\expandafter\gdef\csname R@an.gpu_measures.qual.amos.stratum.rule\endcsname{native through-plane spacing $\leq$ 2.5 mm}
\expandafter\gdef\csname R@an.gpu_measures.qual.kits.adv.case\endcsname{\texttt{case\_00110}}
\expandafter\gdef\csname R@an.gpu_measures.qual.kits.adv.delta\endcsname{\ensuremath{-30.90}}
\expandafter\gdef\csname R@an.gpu_measures.qual.kits.adv.dice\endcsname{79.41}
\expandafter\gdef\csname R@an.gpu_measures.qual.kits.adv.rank\endcsname{1 of 98 by $\Delta$}
\expandafter\gdef\csname R@an.gpu_measures.qual.kits.anchor.case\endcsname{\texttt{case\_00156}}
\expandafter\gdef\csname R@an.gpu_measures.qual.kits.anchor.dice\endcsname{75.95}
\expandafter\gdef\csname R@an.gpu_measures.qual.kits.anchor.rank\endcsname{17 of 33 in stratum}
\expandafter\gdef\csname R@an.gpu_measures.qual.kits.q10.case\endcsname{\texttt{case\_00048}}
\expandafter\gdef\csname R@an.gpu_measures.qual.kits.q10.dice\endcsname{61.11}
\expandafter\gdef\csname R@an.gpu_measures.qual.kits.q10.rank\endcsname{11 of 98}
\expandafter\gdef\csname R@an.gpu_measures.qual.kits.q50.case\endcsname{\texttt{case\_00255}}
\expandafter\gdef\csname R@an.gpu_measures.qual.kits.q50.dice\endcsname{89.92}
\expandafter\gdef\csname R@an.gpu_measures.qual.kits.q50.rank\endcsname{50 of 98}
\expandafter\gdef\csname R@an.gpu_measures.qual.kits.q90.case\endcsname{\texttt{case\_00148}}
\expandafter\gdef\csname R@an.gpu_measures.qual.kits.q90.dice\endcsname{95.64}
\expandafter\gdef\csname R@an.gpu_measures.qual.kits.q90.rank\endcsname{88 of 98}
\expandafter\gdef\csname R@an.gpu_measures.qual.kits.stratum.n\endcsname{33}
\expandafter\gdef\csname R@an.gpu_measures.qual.kits.stratum.rule\endcsname{smallest third of the GT tumour voxel count}
\expandafter\gdef\csname R@an.gpu_measures.qual.n.acdc\endcsname{40}
\expandafter\gdef\csname R@an.gpu_measures.qual.n.amos\endcsname{40}
\expandafter\gdef\csname R@an.gpu_measures.qual.n.kits\endcsname{98}
\expandafter\gdef\csname R@an.gpu_measures.qual.nadv\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.qual.nblind\endcsname{11}
\expandafter\gdef\csname R@an.gpu_measures.qual.npct\endcsname{9}
\expandafter\gdef\csname R@an.gpu_measures.qual.nsel\endcsname{14}
\expandafter\gdef\csname R@an.gpu_measures.qual.rule\endcsname{cases at the 10th, 50th, 90th percentile of the per-case Dice of the frozen default pool (ascending by pool Dice, ties by case id; rank $\lfloor q(n-1)+\tfrac12\rfloor$), plus one median-difficulty case inside a reference-defined stratum per co-primary}
\expandafter\gdef\csname R@an.gpu_measures.qual.sha\endcsname{8ecffa93dbb7}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.acdc.band\endcsname{0.16}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.acdc.d\endcsname{\ensuremath{+0.242}}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.acdc.d0\endcsname{\ensuremath{+0.336}}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.acdc.d0bar\endcsname{n/a (guard dataset, read descriptively)}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.acdc.dfresh\endcsname{\ensuremath{+0.242}}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.acdc.est\endcsname{fresh mean, seeds 1--2}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.acdc.freshbar\endcsname{n/a (guard dataset, read descriptively)}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.acdc.inband\endcsname{n/a (guard dataset, read descriptively)}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.acdc.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.acdc.reading\endcsname{the discovery seed is \ensuremath{+0.336} pp; the two fresh seeds average \ensuremath{+0.242} pp (standard error of the mean 0.017 pp between the two seeds)}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.acdc.resolved\endcsname{n/a (guard dataset, read descriptively)}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.acdc.sdpair\endcsname{0.024}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.acdc.sem\endcsname{0.017}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.acdc.senull\endcsname{0.081}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.acdc.sep\endcsname{n/a (guard dataset, read descriptively)}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.acdc.spread\endcsname{0.034}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.acdc.status\endcsname{the registered fresh pair (seeds 1--2) has landed and is the estimand}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.amos.band\endcsname{0.20}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.amos.d\endcsname{\ensuremath{+0.465}}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.amos.d0\endcsname{\ensuremath{+0.647}}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.amos.d0bar\endcsname{cleared}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.amos.dfresh\endcsname{\ensuremath{+0.465}}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.amos.est\endcsname{fresh mean, seeds 1--2}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.amos.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.amos.inband\endcsname{outside}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.amos.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.amos.reading\endcsname{the discovery seed is \ensuremath{+0.647} pp, which clears the +0.35 pp screening bar; the two fresh seeds average \ensuremath{+0.465} pp (standard error of the mean 0.197 pp between the two seeds), which sits outside its own $\pm$0.20 pp two-seed null band and above the screening bar: separated from the default at two fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.amos.resolved\endcsname{resolved at two fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.amos.sdpair\endcsname{0.278}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.amos.sem\endcsname{0.197}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.amos.senull\endcsname{0.100}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.amos.sep\endcsname{separated from the default at two fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.amos.spread\endcsname{0.394}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.amos.status\endcsname{the registered fresh pair (seeds 1--2) has landed and is the estimand}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.kits.band\endcsname{1.45}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.kits.d\endcsname{\ensuremath{+3.475}}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.kits.d0\endcsname{\ensuremath{+2.326}}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.kits.d0bar\endcsname{cleared}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.kits.dfresh\endcsname{\ensuremath{+3.475}}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.kits.est\endcsname{fresh mean, seeds 1--2}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.kits.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.kits.inband\endcsname{outside}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.kits.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.kits.reading\endcsname{the discovery seed is \ensuremath{+2.326} pp, which clears the +0.35 pp screening bar; the two fresh seeds average \ensuremath{+3.475} pp (standard error of the mean 0.342 pp between the two seeds), which sits outside its own $\pm$1.45 pp two-seed null band and above the screening bar: separated from the default at two fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.kits.resolved\endcsname{resolved at two fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.kits.sdpair\endcsname{0.483}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.kits.sem\endcsname{0.342}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.kits.senull\endcsname{0.726}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.kits.sep\endcsname{separated from the default at two fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.kits.spread\endcsname{0.683}
\expandafter\gdef\csname R@an.gpu_measures.rep.L1.kits.status\endcsname{the registered fresh pair (seeds 1--2) has landed and is the estimand}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.acdc.band\endcsname{0.16}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.acdc.d\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.acdc.d0\endcsname{\ensuremath{+0.616}}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.acdc.d0bar\endcsname{n/a (guard dataset, read descriptively)}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.acdc.dfresh\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.acdc.est\endcsname{fresh mean, seeds 1--2}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.acdc.freshbar\endcsname{n/a (guard dataset, read descriptively)}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.acdc.inband\endcsname{n/a (guard dataset, read descriptively)}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.acdc.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.acdc.reading\endcsname{the discovery seed is \ensuremath{+0.616} pp; the two fresh seeds average \ensuremath{+0.450} pp (standard error of the mean 0.033 pp between the two seeds)}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.acdc.resolved\endcsname{n/a (guard dataset, read descriptively)}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.acdc.sdpair\endcsname{0.047}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.acdc.sem\endcsname{0.033}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.acdc.senull\endcsname{0.081}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.acdc.sep\endcsname{n/a (guard dataset, read descriptively)}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.acdc.spread\endcsname{0.067}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.acdc.status\endcsname{the registered fresh pair (seeds 1--2) has landed and is the estimand}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.amos.band\endcsname{0.20}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.amos.d\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.amos.d0\endcsname{\ensuremath{+0.382}}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.amos.d0bar\endcsname{cleared}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.amos.dfresh\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.amos.est\endcsname{fresh mean, seeds 1--2}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.amos.freshbar\endcsname{does not clear}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.amos.inband\endcsname{inside}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.amos.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.amos.reading\endcsname{the discovery seed is \ensuremath{+0.382} pp, which clears the +0.35 pp screening bar; the two fresh seeds average \ensuremath{+0.132} pp (standard error of the mean 0.148 pp between the two seeds), which sits inside its own $\pm$0.20 pp two-seed null band and below the screening bar: not separated from the default at two fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.amos.resolved\endcsname{not resolved at two fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.amos.sdpair\endcsname{0.209}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.amos.sem\endcsname{0.148}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.amos.senull\endcsname{0.100}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.amos.sep\endcsname{not separated from the default at two fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.amos.spread\endcsname{0.296}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.amos.status\endcsname{the registered fresh pair (seeds 1--2) has landed and is the estimand}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.kits.band\endcsname{1.45}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.kits.d\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.kits.d0\endcsname{\ensuremath{+2.842}}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.kits.d0bar\endcsname{cleared}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.kits.dfresh\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.kits.est\endcsname{fresh mean, seeds 1--2}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.kits.freshbar\endcsname{clears}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.kits.inband\endcsname{outside}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.kits.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.kits.reading\endcsname{the discovery seed is \ensuremath{+2.842} pp, which clears the +0.35 pp screening bar; the two fresh seeds average \ensuremath{+2.094} pp (standard error of the mean 0.296 pp between the two seeds), which sits outside its own $\pm$1.45 pp two-seed null band and above the screening bar: separated from the default at two fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.kits.resolved\endcsname{resolved at two fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.kits.sdpair\endcsname{0.419}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.kits.sem\endcsname{0.296}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.kits.senull\endcsname{0.726}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.kits.sep\endcsname{separated from the default at two fresh seeds}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.kits.spread\endcsname{0.592}
\expandafter\gdef\csname R@an.gpu_measures.rep.L3.kits.status\endcsname{the registered fresh pair (seeds 1--2) has landed and is the estimand}
\expandafter\gdef\csname R@an.gpu_measures.repred.L1.acdc.est\endcsname{fresh mean, seeds 1--2}
\expandafter\gdef\csname R@an.gpu_measures.repred.L1.acdc.shift\endcsname{\ensuremath{+0.242}}
\expandafter\gdef\csname R@an.gpu_measures.repred.L1.amos.est\endcsname{fresh mean, seeds 1--2}
\expandafter\gdef\csname R@an.gpu_measures.repred.L1.amos.shift\endcsname{\ensuremath{+0.465}}
\expandafter\gdef\csname R@an.gpu_measures.repred.L1.kits.est\endcsname{no weights kept (fresh mean, seeds 1--2)}
\expandafter\gdef\csname R@an.gpu_measures.repred.L1.kits.shift\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.repred.L3.acdc.est\endcsname{fresh mean, seeds 1--2}
\expandafter\gdef\csname R@an.gpu_measures.repred.L3.acdc.shift\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.gpu_measures.repred.L3.amos.est\endcsname{fresh mean, seeds 1--2}
\expandafter\gdef\csname R@an.gpu_measures.repred.L3.amos.shift\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.gpu_measures.repred.L3.kits.est\endcsname{no weights kept (fresh mean, seeds 1--2)}
\expandafter\gdef\csname R@an.gpu_measures.repred.L3.kits.shift\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.repred.base.acdc.est\endcsname{uncompiled sub-pool, 3 of 6 pool runs}
\expandafter\gdef\csname R@an.gpu_measures.repred.base.acdc.rel\endcsname{exactly the registered uncompiled sub-pool}
\expandafter\gdef\csname R@an.gpu_measures.repred.base.acdc.shift\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.gpu_measures.repred.base.amos.est\endcsname{uncompiled sub-pool, 3 of 6 pool runs}
\expandafter\gdef\csname R@an.gpu_measures.repred.base.amos.rel\endcsname{exactly the registered uncompiled sub-pool}
\expandafter\gdef\csname R@an.gpu_measures.repred.base.amos.shift\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.gpu_measures.repred.base.kits.est\endcsname{no weights kept (frozen pool mean, 3 runs)}
\expandafter\gdef\csname R@an.gpu_measures.repred.base.kits.rel\endcsname{no frozen-pool run kept weights}
\expandafter\gdef\csname R@an.gpu_measures.repred.base.kits.shift\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.repred.paired\endcsname{AMOS22, ACDC}
\expandafter\gdef\csname R@an.gpu_measures.screen.bar\endcsname{+0.35}
\expandafter\gdef\csname R@an.gpu_measures.selfcheck.n\endcsname{52}
\expandafter\gdef\csname R@an.gpu_measures.selfcheck.tol\endcsname{$10^{-4}$}
\expandafter\gdef\csname R@an.gpu_measures.selfcheck.worst\endcsname{$2.9\times10^{-5}$}
\expandafter\gdef\csname R@an.gpu_measures.sens.acdc.n\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.sens.acdc.name\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.gpu_measures.sens.acdc.pending\endcsname{contemporaneous default runs (seeds 3--5)}
\expandafter\gdef\csname R@an.gpu_measures.sens.acdc.shift\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.gpu_measures.sens.acdc.status\endcsname{uncompiled sub-pool, 3 runs, \ensuremath{+0.007} pp from the frozen pool mean}
\expandafter\gdef\csname R@an.gpu_measures.sens.amos.n\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.sens.amos.name\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.gpu_measures.sens.amos.pending\endcsname{none}
\expandafter\gdef\csname R@an.gpu_measures.sens.amos.shift\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.gpu_measures.sens.amos.status\endcsname{uncompiled sub-pool, 3 runs, \ensuremath{+0.029} pp from the frozen pool mean}
\expandafter\gdef\csname R@an.gpu_measures.sens.kits.baseparams\endcsname{31.20}
\expandafter\gdef\csname R@an.gpu_measures.sens.kits.ctl\endcsname{\ensuremath{+1.067}}
\expandafter\gdef\csname R@an.gpu_measures.sens.kits.ctlbasis\endcsname{fresh mean, seeds 1--2}
\expandafter\gdef\csname R@an.gpu_measures.sens.kits.ctlest\endcsname{fresh mean, seeds 1--2}
\expandafter\gdef\csname R@an.gpu_measures.sens.kits.ctlgap\endcsname{\ensuremath{+1.027}}
\expandafter\gdef\csname R@an.gpu_measures.sens.kits.ctlhy\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.gpu_measures.sens.kits.ctlname\endcsname{branch control}
\expandafter\gdef\csname R@an.gpu_measures.sens.kits.ctlparams\endcsname{31.21}
\expandafter\gdef\csname R@an.gpu_measures.sens.kits.ctlphrase\endcsname{the branch control, at 31.21 M parameters against the default's 31.20 M on the KiTS23 plan, gains \ensuremath{+1.067} pp against the same pool on its fresh mean, seeds 1--2; on the same basis HyReX gains \ensuremath{+2.094} pp, so HyReX minus the control is \ensuremath{+1.027} pp, which is above the registered 0.5 pp one-seed pair floor and above the gap's own null SD of 0.795 pp}
\expandafter\gdef\csname R@an.gpu_measures.sens.kits.ctlrel\endcsname{the 1.027 pp between them is above the registered 0.5 pp one-seed pair floor and above the gap's own null SD of 0.795 pp}
\expandafter\gdef\csname R@an.gpu_measures.sens.kits.n\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.sens.kits.name\endcsname{contemporaneous default runs (seeds 3--5)}
\expandafter\gdef\csname R@an.gpu_measures.sens.kits.pending\endcsname{none}
\expandafter\gdef\csname R@an.gpu_measures.sens.kits.pooln\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.sens.kits.poolsd\endcsname{0.795}
\expandafter\gdef\csname R@an.gpu_measures.sens.kits.poolspread\endcsname{1.522}
\expandafter\gdef\csname R@an.gpu_measures.sens.kits.shift\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.gpu_measures.sens.kits.spreadbars\endcsname{4.3}
\expandafter\gdef\csname R@an.gpu_measures.sens.kits.status\endcsname{contemporaneous default runs (seeds 3--5), 3 runs, \ensuremath{+0.487} pp from the frozen pool mean}
\expandafter\gdef\csname R@an.gpu_measures.sep.acdc.band\endcsname{0.16}
\expandafter\gdef\csname R@an.gpu_measures.sep.acdc.form\endcsname{at two fresh seeds ACDC reads HyReX (\ensuremath{+0.450} pp) and ResEnc-M (\ensuremath{+0.242} pp) against the frozen default pool}
\expandafter\gdef\csname R@an.gpu_measures.sep.acdc.nnot\endcsname{n/a (guard dataset, read descriptively)}
\expandafter\gdef\csname R@an.gpu_measures.sep.acdc.nsep\endcsname{n/a (guard dataset, read descriptively)}
\expandafter\gdef\csname R@an.gpu_measures.sep.amos.band\endcsname{0.20}
\expandafter\gdef\csname R@an.gpu_measures.sep.amos.form\endcsname{at two fresh seeds AMOS22 separates ResEnc-M (\ensuremath{+0.465} pp) from the frozen default pool and does not separate HyReX (\ensuremath{+0.132} pp), against a two-seed null band of $\pm$0.20 pp}
\expandafter\gdef\csname R@an.gpu_measures.sep.amos.nnot\endcsname{1}
\expandafter\gdef\csname R@an.gpu_measures.sep.amos.nsep\endcsname{1}
\expandafter\gdef\csname R@an.gpu_measures.sep.kits.band\endcsname{1.45}
\expandafter\gdef\csname R@an.gpu_measures.sep.kits.form\endcsname{at two fresh seeds KiTS23 separates HyReX (\ensuremath{+2.094} pp) and ResEnc-M (\ensuremath{+3.475} pp) from the frozen default pool, against a two-seed null band of $\pm$1.45 pp}
\expandafter\gdef\csname R@an.gpu_measures.sep.kits.nnot\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.sep.kits.nsep\endcsname{2}
\expandafter\gdef\csname R@an.gpu_measures.status.ckpt\endcsname{54 checkpoint-measurement records}
\expandafter\gdef\csname R@an.gpu_measures.status.compile\endcsname{no compiled-inference arm exists in tools/measure\_cost.py, so the compiled vs uncompiled inference latency of the efficiency subsection cannot be filled; 0 records carry one}
\expandafter\gdef\csname R@an.gpu_measures.status.cost\endcsname{39 of 39 design$\times$dataset records}
\expandafter\gdef\csname R@an.gpu_measures.status.erf\endcsname{5 records}
\expandafter\gdef\csname R@an.gpu_measures.status.qual\endcsname{selection fixed (14 cases, hash 8ecffa93dbb7); 20 fold-0 slice files exported}
\expandafter\gdef\csname R@an.gpu_measures.surf.hd95rule\endcsname{HD95 is the maximum of the two directed 95th percentiles of the surface-to-surface distance and ASSD their mean, both on the native grid}
\expandafter\gdef\csname R@an.gpu_measures.surf.pooled\endcsname{the pooled (medpy) HD95 variant the enrichment plan also lists is not computed by tools/measure\_ckpt.py and is not reported here}
\expandafter\gdef\csname R@an.gpu_measures.take.tta\endcsname{the measured mirroring increments run from \ensuremath{+0.094} to \ensuremath{+2.394} pp over 24 of 24 arm-by-dataset-by-fold cells and are positive in 24 of them}
\expandafter\gdef\csname R@an.gpu_measures.tta.L1.acdc.inc\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.tta.L1.amos.inc\endcsname{\ensuremath{+0.485}}
\expandafter\gdef\csname R@an.gpu_measures.tta.L1.kits.inc\endcsname{\ensuremath{+0.866}}
\expandafter\gdef\csname R@an.gpu_measures.tta.L3.acdc.inc\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.tta.L3.amos.inc\endcsname{\ensuremath{+0.446}}
\expandafter\gdef\csname R@an.gpu_measures.tta.L3.kits.inc\endcsname{\ensuremath{+1.413}}
\expandafter\gdef\csname R@an.gpu_measures.tta.acdc.dd\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.tta.amos.dd\endcsname{\ensuremath{-0.035}}
\expandafter\gdef\csname R@an.gpu_measures.tta.base.acdc.inc\endcsname{\ensuremath{+0.335}}
\expandafter\gdef\csname R@an.gpu_measures.tta.base.amos.inc\endcsname{\ensuremath{+0.481}}
\expandafter\gdef\csname R@an.gpu_measures.tta.base.kits.inc\endcsname{\ensuremath{+1.520}}
\expandafter\gdef\csname R@an.gpu_measures.tta.kits.dd\endcsname{\ensuremath{-0.107}}
\expandafter\gdef\csname R@an.gpu_measures.tta.status\endcsname{measured on all 24 arm $\times$ dataset $\times$ fold cells}
\expandafter\gdef\csname R@an.gpu_measures.u.df\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.u.ds\endcsname{AMOS22 and KiTS23}
\expandafter\gdef\csname R@an.gpu_measures.u.folds\endcsname{folds 1 to 4}
\expandafter\gdef\csname R@an.gpu_measures.u.narms\endcsname{3}
\expandafter\gdef\csname R@an.gpu_measures.u.narms.word\endcsname{three}
\expandafter\gdef\csname R@an.gpu_measures.u.ncells\endcsname{48}
\expandafter\gdef\csname R@an.gpu_measures.u.nfolds\endcsname{4}
\expandafter\gdef\csname R@an.gpu_measures.u.nfolds.word\endcsname{four}
\expandafter\gdef\csname R@an.gpu_measures.u.njobs\endcsname{36}
\expandafter\gdef\csname R@an.gpu_measures.u.ntrials\endcsname{24}
\expandafter\gdef\csname R@an.gpu_measures.val.acdc.L1.cases\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.acdc.L1.inc\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.acdc.L1.n\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.val.acdc.L1.off\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.acdc.L1.on\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.acdc.L1.selfdiff\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.acdc.L3.cases\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.acdc.L3.inc\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.acdc.L3.n\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.val.acdc.L3.off\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.acdc.L3.on\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.acdc.L3.selfdiff\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.acdc.base.cases\endcsname{40}
\expandafter\gdef\csname R@an.gpu_measures.val.acdc.base.inc\endcsname{\ensuremath{+0.335}}
\expandafter\gdef\csname R@an.gpu_measures.val.acdc.base.n\endcsname{1}
\expandafter\gdef\csname R@an.gpu_measures.val.acdc.base.off\endcsname{91.763}
\expandafter\gdef\csname R@an.gpu_measures.val.acdc.base.on\endcsname{92.098}
\expandafter\gdef\csname R@an.gpu_measures.val.acdc.base.selfdiff\endcsname{$6.9\times10^{-6}$}
\expandafter\gdef\csname R@an.gpu_measures.val.amos.L1.cases\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.amos.L1.inc\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.amos.L1.n\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.val.amos.L1.off\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.amos.L1.on\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.amos.L1.selfdiff\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.amos.L3.cases\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.amos.L3.inc\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.amos.L3.n\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.val.amos.L3.off\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.amos.L3.on\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.amos.L3.selfdiff\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.amos.base.cases\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.amos.base.inc\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.amos.base.n\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.val.amos.base.off\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.amos.base.on\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.amos.base.selfdiff\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.kits.L1.cases\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.kits.L1.inc\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.kits.L1.n\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.val.kits.L1.off\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.kits.L1.on\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.kits.L1.selfdiff\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.kits.L3.cases\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.kits.L3.inc\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.kits.L3.n\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.val.kits.L3.off\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.kits.L3.on\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.kits.L3.selfdiff\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.kits.base.cases\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.kits.base.inc\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.kits.base.n\endcsname{0}
\expandafter\gdef\csname R@an.gpu_measures.val.kits.base.off\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.kits.base.on\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.kits.base.selfdiff\endcsname{\pend}
\expandafter\gdef\csname R@an.gpu_measures.val.nrec\endcsname{1}
\expandafter\gdef\csname R@an.gpu_measures.val.status\endcsname{outside the registered grid, one full-fold record has landed: the nnU-Net default on ACDC, fold 0 (40 cases), a mirroring increment of \ensuremath{+0.335}\,pp, the re-prediction reproducing the harness headline to $6.9\times10^{-6}$ Dice}
\expandafter\gdef\csname R@an.gpu_measures.vsref.acdc.d\endcsname{\ensuremath{+0.208}}
\expandafter\gdef\csname R@an.gpu_measures.vsref.acdc.da\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.gpu_measures.vsref.acdc.db\endcsname{\ensuremath{+0.242}}
\expandafter\gdef\csname R@an.gpu_measures.vsref.acdc.gap\endcsname{0.208}
\expandafter\gdef\csname R@an.gpu_measures.vsref.acdc.hi\endcsname{HyReX}
\expandafter\gdef\csname R@an.gpu_measures.vsref.acdc.lo\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.gpu_measures.vsref.acdc.matched\endcsname{yes}
\expandafter\gdef\csname R@an.gpu_measures.vsref.acdc.order\endcsname{neutral}
\expandafter\gdef\csname R@an.gpu_measures.vsref.acdc.phrase\endcsname{HyReX is \ensuremath{+0.450} pp and ResEnc-M \ensuremath{+0.242} pp against the frozen default pool on the same estimand (fresh mean, seeds 1--2); the 0.208 pp between them is inside the registered 0.5 pp one-seed pair floor: the difference is not resolved against the floor, and no ordering is read from it}
\expandafter\gdef\csname R@an.gpu_measures.vsref.acdc.res\endcsname{the 0.208 pp between them is inside the registered 0.5 pp one-seed pair floor: the difference is not resolved against the floor, and no ordering is read from it}
\expandafter\gdef\csname R@an.gpu_measures.vsref.acdc.se\endcsname{0.099}
\expandafter\gdef\csname R@an.gpu_measures.vsref.agree\endcsname{ResEnc-M is ahead of HyReX on AMOS22 and KiTS23}
\expandafter\gdef\csname R@an.gpu_measures.vsref.amos.d\endcsname{\ensuremath{-0.332}}
\expandafter\gdef\csname R@an.gpu_measures.vsref.amos.da\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.gpu_measures.vsref.amos.db\endcsname{\ensuremath{+0.465}}
\expandafter\gdef\csname R@an.gpu_measures.vsref.amos.gap\endcsname{0.332}
\expandafter\gdef\csname R@an.gpu_measures.vsref.amos.hi\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.gpu_measures.vsref.amos.lo\endcsname{HyReX}
\expandafter\gdef\csname R@an.gpu_measures.vsref.amos.matched\endcsname{yes}
\expandafter\gdef\csname R@an.gpu_measures.vsref.amos.order\endcsname{ordered}
\expandafter\gdef\csname R@an.gpu_measures.vsref.amos.phrase\endcsname{ResEnc-M reaches \ensuremath{+0.465} pp and HyReX \ensuremath{+0.132} pp against the frozen default pool on the same estimand (fresh mean, seeds 1--2): ResEnc-M is ahead, and the 0.332 pp between them is inside the registered 0.5 pp one-seed pair floor and above the gap's own null SD of 0.122 pp: the difference is not resolved against the floor, and no ordering is read from it}
\expandafter\gdef\csname R@an.gpu_measures.vsref.amos.res\endcsname{the 0.332 pp between them is inside the registered 0.5 pp one-seed pair floor and above the gap's own null SD of 0.122 pp: the difference is not resolved against the floor, and no ordering is read from it}
\expandafter\gdef\csname R@an.gpu_measures.vsref.amos.se\endcsname{0.122}
\expandafter\gdef\csname R@an.gpu_measures.vsref.kits.d\endcsname{\ensuremath{-1.382}}
\expandafter\gdef\csname R@an.gpu_measures.vsref.kits.da\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.gpu_measures.vsref.kits.db\endcsname{\ensuremath{+3.475}}
\expandafter\gdef\csname R@an.gpu_measures.vsref.kits.gap\endcsname{1.382}
\expandafter\gdef\csname R@an.gpu_measures.vsref.kits.hi\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.gpu_measures.vsref.kits.lo\endcsname{HyReX}
\expandafter\gdef\csname R@an.gpu_measures.vsref.kits.matched\endcsname{yes}
\expandafter\gdef\csname R@an.gpu_measures.vsref.kits.order\endcsname{ordered}
\expandafter\gdef\csname R@an.gpu_measures.vsref.kits.phrase\endcsname{ResEnc-M reaches \ensuremath{+3.475} pp and HyReX \ensuremath{+2.094} pp against the frozen default pool on the same estimand (fresh mean, seeds 1--2): ResEnc-M is ahead, and the 1.382 pp between them is above the registered 0.5 pp one-seed pair floor and above the gap's own null SD of 0.795 pp}
\expandafter\gdef\csname R@an.gpu_measures.vsref.kits.res\endcsname{the 1.382 pp between them is above the registered 0.5 pp one-seed pair floor and above the gap's own null SD of 0.795 pp}
\expandafter\gdef\csname R@an.gpu_measures.vsref.kits.se\endcsname{0.795}
\expandafter\gdef\csname R@an.gpu_measures.vsref.summary\endcsname{On AMOS22, ResEnc-M reaches \ensuremath{+0.465} pp and HyReX \ensuremath{+0.132} pp against the frozen default pool on the same estimand (fresh mean, seeds 1--2): ResEnc-M is ahead, and the 0.332 pp between them is inside the registered 0.5 pp one-seed pair floor and above the gap's own null SD of 0.122 pp: the difference is not resolved against the floor, and no ordering is read from it. On KiTS23, ResEnc-M reaches \ensuremath{+3.475} pp and HyReX \ensuremath{+2.094} pp against the frozen default pool on the same estimand (fresh mean, seeds 1--2): ResEnc-M is ahead, and the 1.382 pp between them is above the registered 0.5 pp one-seed pair floor and above the gap's own null SD of 0.795 pp. On ACDC, HyReX is \ensuremath{+0.450} pp and ResEnc-M \ensuremath{+0.242} pp against the frozen default pool on the same estimand (fresh mean, seeds 1--2); the 0.208 pp between them is inside the registered 0.5 pp one-seed pair floor: the difference is not resolved against the floor, and no ordering is read from it.}
\expandafter\gdef\csname R@an.heldout.L1.params.clause\endcsname{carries $3.28\times$, $3.32\times$ and $3.28\times$ the default's parameters on LiTS, BTCV and BraTS-MSD, respectively}
\expandafter\gdef\csname R@an.heldout.L3.params.clause\endcsname{carries $0.95\times$ the default's parameters}
\expandafter\gdef\csname R@an.heldout.band.def\endcsname{the $\pm2$ SD band of the difference of two three-seed means, with the seed SD of the dataset's own default runs}
\expandafter\gdef\csname R@an.heldout.band.k\endcsname{2}
\expandafter\gdef\csname R@an.heldout.band.phrase\endcsname{the band of seed noise of that dataset}
\expandafter\gdef\csname R@an.heldout.brats.L1.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L1.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L1.d0\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.heldout.brats.L1.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L1.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L1.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L1.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L1.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L1.n\endcsname{1}
\expandafter\gdef\csname R@an.heldout.brats.L1.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L1.params\endcsname{102.35}
\expandafter\gdef\csname R@an.heldout.brats.L1.params_vs_default\endcsname{3.28}
\expandafter\gdef\csname R@an.heldout.brats.L1.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.brats.L1.s0\endcsname{82.95}
\expandafter\gdef\csname R@an.heldout.brats.L1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L1.sd_default\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L1.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L1.state\endcsname{1 of 3 finished}
\expandafter\gdef\csname R@an.heldout.brats.L1.step_ms\endcsname{172.0}
\expandafter\gdef\csname R@an.heldout.brats.L1.step_vs_default\endcsname{1.32}
\expandafter\gdef\csname R@an.heldout.brats.L1.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.brats.L3.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L3.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L3.d0\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.heldout.brats.L3.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L3.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L3.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L3.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L3.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L3.n\endcsname{1}
\expandafter\gdef\csname R@an.heldout.brats.L3.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L3.params\endcsname{29.67}
\expandafter\gdef\csname R@an.heldout.brats.L3.params_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.heldout.brats.L3.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.brats.L3.s0\endcsname{83.05}
\expandafter\gdef\csname R@an.heldout.brats.L3.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L3.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L3.sd_default\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L3.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.L3.state\endcsname{1 of 3 finished}
\expandafter\gdef\csname R@an.heldout.brats.L3.step_ms\endcsname{181.7}
\expandafter\gdef\csname R@an.heldout.brats.L3.step_vs_default\endcsname{1.40}
\expandafter\gdef\csname R@an.heldout.brats.L3.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.n\endcsname{0}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.params\endcsname{31.04}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.params_vs_default\endcsname{0.99}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.s0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.sd_default\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.state\endcsname{0 of 3 finished, 1 running}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.step_ms\endcsname{121.9}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.step_vs_default\endcsname{0.94}
\expandafter\gdef\csname R@an.heldout.brats.V7A1.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.n\endcsname{0}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.params\endcsname{31.18}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.s0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.sd_default\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.state\endcsname{0 of 3 finished}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.step_ms\endcsname{143.1}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.step_vs_default\endcsname{1.10}
\expandafter\gdef\csname R@an.heldout.brats.V7A2.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.n\endcsname{0}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.params\endcsname{21.11}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.params_vs_default\endcsname{0.68}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.s0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.sd_default\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.state\endcsname{0 of 3 finished, 1 running}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.step_ms\endcsname{101.2}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.step_vs_default\endcsname{0.78}
\expandafter\gdef\csname R@an.heldout.brats.V7C1.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.n\endcsname{0}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.params\endcsname{31.31}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.s0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.sd_default\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.state\endcsname{0 of 3 finished}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.step_ms\endcsname{116.4}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.step_vs_default\endcsname{0.89}
\expandafter\gdef\csname R@an.heldout.brats.V8A1.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.n\endcsname{0}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.params\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.params_vs_default\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.s0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.sd_default\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.state\endcsname{0 of 3 finished}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.step_ms\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.step_vs_default\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8A2.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.n\endcsname{0}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.params\endcsname{18.21}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.params_vs_default\endcsname{0.58}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.s0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.sd_default\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.state\endcsname{0 of 3 finished}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.step_ms\endcsname{78.5}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.step_vs_default\endcsname{0.60}
\expandafter\gdef\csname R@an.heldout.brats.V8B1.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.n\endcsname{0}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.params\endcsname{21.09}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.params_vs_default\endcsname{0.68}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.s0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.sd_default\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.state\endcsname{0 of 3 finished}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.step_ms\endcsname{83.1}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.step_vs_default\endcsname{0.64}
\expandafter\gdef\csname R@an.heldout.brats.V8B2.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.brats.band\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.base.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.base.n\endcsname{1}
\expandafter\gdef\csname R@an.heldout.brats.base.params\endcsname{31.20}
\expandafter\gdef\csname R@an.heldout.brats.base.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.heldout.brats.base.s0\endcsname{82.98}
\expandafter\gdef\csname R@an.heldout.brats.base.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.base.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.base.sd_default\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.base.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.base.state\endcsname{1 of 3 finished}
\expandafter\gdef\csname R@an.heldout.brats.base.step_ms\endcsname{130.1}
\expandafter\gdef\csname R@an.heldout.brats.base.step_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.heldout.brats.batch\endcsname{2}
\expandafter\gdef\csname R@an.heldout.brats.complete\endcsname{no}
\expandafter\gdef\csname R@an.heldout.brats.mean_default\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.metric\endcsname{the mean Dice over the three scored regions (whole tumour, tumour core and enhancing tumour)}
\expandafter\gdef\csname R@an.heldout.brats.n.done\endcsname{3}
\expandafter\gdef\csname R@an.heldout.brats.n.total\endcsname{9}
\expandafter\gdef\csname R@an.heldout.brats.name\endcsname{BraTS-MSD}
\expandafter\gdef\csname R@an.heldout.brats.ncases\endcsname{484}
\expandafter\gdef\csname R@an.heldout.brats.nfg\endcsname{3}
\expandafter\gdef\csname R@an.heldout.brats.ntrain\endcsname{387}
\expandafter\gdef\csname R@an.heldout.brats.nval\endcsname{97}
\expandafter\gdef\csname R@an.heldout.brats.patch\endcsname{$128\times 128\times 128$}
\expandafter\gdef\csname R@an.heldout.brats.read\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.sd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.sd_default\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.sd_hi\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.sd_lo\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.brats.state\endcsname{3 of 9 finished}
\expandafter\gdef\csname R@an.heldout.btcv.L1.clause\endcsname{transfers (\ensuremath{+0.71}\,pp; above the band of seed noise of that dataset)}
\expandafter\gdef\csname R@an.heldout.btcv.L1.d\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.heldout.btcv.L1.d0\endcsname{\ensuremath{+1.67}}
\expandafter\gdef\csname R@an.heldout.btcv.L1.d1\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.heldout.btcv.L1.d2\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.heldout.btcv.L1.d3\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.heldout.btcv.L1.dsd\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.heldout.btcv.L1.mean\endcsname{78.52}
\expandafter\gdef\csname R@an.heldout.btcv.L1.n\endcsname{3}
\expandafter\gdef\csname R@an.heldout.btcv.L1.npos\endcsname{3}
\expandafter\gdef\csname R@an.heldout.btcv.L1.params\endcsname{101.87}
\expandafter\gdef\csname R@an.heldout.btcv.L1.params_vs_default\endcsname{3.32}
\expandafter\gdef\csname R@an.heldout.btcv.L1.place\endcsname{above}
\expandafter\gdef\csname R@an.heldout.btcv.L1.s0\endcsname{79.24}
\expandafter\gdef\csname R@an.heldout.btcv.L1.s1\endcsname{78.23}
\expandafter\gdef\csname R@an.heldout.btcv.L1.s2\endcsname{78.10}
\expandafter\gdef\csname R@an.heldout.btcv.L1.sd_default\endcsname{0.301}
\expandafter\gdef\csname R@an.heldout.btcv.L1.sd_own\endcsname{0.619}
\expandafter\gdef\csname R@an.heldout.btcv.L1.state\endcsname{3 of 3 finished}
\expandafter\gdef\csname R@an.heldout.btcv.L1.step_ms\endcsname{184.7}
\expandafter\gdef\csname R@an.heldout.btcv.L1.step_vs_default\endcsname{1.48}
\expandafter\gdef\csname R@an.heldout.btcv.L1.word\endcsname{transfers}
\expandafter\gdef\csname R@an.heldout.btcv.L3.clause\endcsname{transfers (\ensuremath{+0.71}\,pp; above the band of seed noise of that dataset)}
\expandafter\gdef\csname R@an.heldout.btcv.L3.d\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.heldout.btcv.L3.d0\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.heldout.btcv.L3.d1\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.heldout.btcv.L3.d2\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.heldout.btcv.L3.d3\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.heldout.btcv.L3.dsd\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.heldout.btcv.L3.mean\endcsname{78.53}
\expandafter\gdef\csname R@an.heldout.btcv.L3.n\endcsname{3}
\expandafter\gdef\csname R@an.heldout.btcv.L3.npos\endcsname{3}
\expandafter\gdef\csname R@an.heldout.btcv.L3.params\endcsname{29.18}
\expandafter\gdef\csname R@an.heldout.btcv.L3.params_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.heldout.btcv.L3.place\endcsname{above}
\expandafter\gdef\csname R@an.heldout.btcv.L3.s0\endcsname{77.85}
\expandafter\gdef\csname R@an.heldout.btcv.L3.s1\endcsname{79.74}
\expandafter\gdef\csname R@an.heldout.btcv.L3.s2\endcsname{78.00}
\expandafter\gdef\csname R@an.heldout.btcv.L3.sd_default\endcsname{0.301}
\expandafter\gdef\csname R@an.heldout.btcv.L3.sd_own\endcsname{1.052}
\expandafter\gdef\csname R@an.heldout.btcv.L3.state\endcsname{3 of 3 finished}
\expandafter\gdef\csname R@an.heldout.btcv.L3.step_ms\endcsname{196.1}
\expandafter\gdef\csname R@an.heldout.btcv.L3.step_vs_default\endcsname{1.57}
\expandafter\gdef\csname R@an.heldout.btcv.L3.word\endcsname{transfers}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.clause\endcsname{transfers (\ensuremath{+0.49}\,pp; inside the band of seed noise of that dataset)}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.d\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.d0\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.d1\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.d2\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.d3\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.dsd\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.mean\endcsname{78.30}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.n\endcsname{3}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.npos\endcsname{3}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.params\endcsname{30.59}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.place\endcsname{inside}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.s0\endcsname{78.43}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.s1\endcsname{78.26}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.s2\endcsname{78.22}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.sd_default\endcsname{0.301}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.sd_own\endcsname{0.112}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.state\endcsname{3 of 3 finished}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.step_ms\endcsname{126.1}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.step_vs_default\endcsname{1.01}
\expandafter\gdef\csname R@an.heldout.btcv.V7A1.word\endcsname{transfers}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.n\endcsname{0}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.params\endcsname{30.71}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.s0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.sd_default\endcsname{0.301}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.state\endcsname{0 of 3 finished}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.step_ms\endcsname{144.6}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.step_vs_default\endcsname{1.16}
\expandafter\gdef\csname R@an.heldout.btcv.V7A2.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.n\endcsname{0}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.params\endcsname{20.67}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.params_vs_default\endcsname{0.67}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.s0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.sd_default\endcsname{0.301}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.state\endcsname{0 of 3 finished, 3 running}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.step_ms\endcsname{100.1}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.step_vs_default\endcsname{0.80}
\expandafter\gdef\csname R@an.heldout.btcv.V7C1.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.n\endcsname{0}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.params\endcsname{30.86}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.s0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.sd_default\endcsname{0.301}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.state\endcsname{0 of 3 finished}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.step_ms\endcsname{119.3}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.step_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.heldout.btcv.V8A1.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.n\endcsname{0}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.params\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.params_vs_default\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.s0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.sd_default\endcsname{0.301}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.state\endcsname{0 of 3 finished}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.step_ms\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.step_vs_default\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8A2.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.n\endcsname{0}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.params\endcsname{17.78}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.params_vs_default\endcsname{0.58}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.s0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.sd_default\endcsname{0.301}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.state\endcsname{0 of 3 finished}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.step_ms\endcsname{79.4}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.step_vs_default\endcsname{0.64}
\expandafter\gdef\csname R@an.heldout.btcv.V8B1.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.n\endcsname{0}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.params\endcsname{20.66}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.params_vs_default\endcsname{0.67}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.s0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.sd_default\endcsname{0.301}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.state\endcsname{0 of 3 finished}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.step_ms\endcsname{87.4}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.step_vs_default\endcsname{0.70}
\expandafter\gdef\csname R@an.heldout.btcv.V8B2.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.btcv.band\endcsname{0.49}
\expandafter\gdef\csname R@an.heldout.btcv.base.mean\endcsname{77.82}
\expandafter\gdef\csname R@an.heldout.btcv.base.n\endcsname{3}
\expandafter\gdef\csname R@an.heldout.btcv.base.params\endcsname{30.71}
\expandafter\gdef\csname R@an.heldout.btcv.base.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.heldout.btcv.base.s0\endcsname{77.57}
\expandafter\gdef\csname R@an.heldout.btcv.base.s1\endcsname{78.15}
\expandafter\gdef\csname R@an.heldout.btcv.base.s2\endcsname{77.73}
\expandafter\gdef\csname R@an.heldout.btcv.base.sd_default\endcsname{0.301}
\expandafter\gdef\csname R@an.heldout.btcv.base.sd_own\endcsname{0.301}
\expandafter\gdef\csname R@an.heldout.btcv.base.state\endcsname{3 of 3 finished}
\expandafter\gdef\csname R@an.heldout.btcv.base.step_ms\endcsname{125.0}
\expandafter\gdef\csname R@an.heldout.btcv.base.step_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.heldout.btcv.batch\endcsname{2}
\expandafter\gdef\csname R@an.heldout.btcv.complete\endcsname{yes}
\expandafter\gdef\csname R@an.heldout.btcv.mean_default\endcsname{77.82}
\expandafter\gdef\csname R@an.heldout.btcv.metric\endcsname{the mean Dice over the 13 scored classes}
\expandafter\gdef\csname R@an.heldout.btcv.n.done\endcsname{9}
\expandafter\gdef\csname R@an.heldout.btcv.n.total\endcsname{9}
\expandafter\gdef\csname R@an.heldout.btcv.name\endcsname{BTCV}
\expandafter\gdef\csname R@an.heldout.btcv.ncases\endcsname{30}
\expandafter\gdef\csname R@an.heldout.btcv.nfg\endcsname{13}
\expandafter\gdef\csname R@an.heldout.btcv.ntrain\endcsname{24}
\expandafter\gdef\csname R@an.heldout.btcv.nval\endcsname{6}
\expandafter\gdef\csname R@an.heldout.btcv.patch\endcsname{$48\times 192\times 192$}
\expandafter\gdef\csname R@an.heldout.btcv.read\endcsname{HyReX transfers (\ensuremath{+0.71}\,pp; above the band of seed noise of that dataset), and ResEnc-M transfers (\ensuremath{+0.71}\,pp; above the band of seed noise of that dataset)}
\expandafter\gdef\csname R@an.heldout.btcv.sd\endcsname{0.301}
\expandafter\gdef\csname R@an.heldout.btcv.sd_default\endcsname{0.301}
\expandafter\gdef\csname R@an.heldout.btcv.sd_hi\endcsname{1.89}
\expandafter\gdef\csname R@an.heldout.btcv.sd_lo\endcsname{0.16}
\expandafter\gdef\csname R@an.heldout.btcv.state\endcsname{9 of 9 finished}
\expandafter\gdef\csname R@an.heldout.complete\endcsname{no}
\expandafter\gdef\csname R@an.heldout.dev.acdc.mean\endcsname{92.01}
\expandafter\gdef\csname R@an.heldout.dev.acdc.n\endcsname{6}
\expandafter\gdef\csname R@an.heldout.dev.acdc.name\endcsname{ACDC}
\expandafter\gdef\csname R@an.heldout.dev.acdc.ncomp\endcsname{3}
\expandafter\gdef\csname R@an.heldout.dev.acdc.nunc\endcsname{3}
\expandafter\gdef\csname R@an.heldout.dev.acdc.sd\endcsname{0.099}
\expandafter\gdef\csname R@an.heldout.dev.acdc.sd_hi\endcsname{0.24}
\expandafter\gdef\csname R@an.heldout.dev.acdc.sd_lo\endcsname{0.06}
\expandafter\gdef\csname R@an.heldout.dev.acdc.sdfac.hi\endcsname{2.45}
\expandafter\gdef\csname R@an.heldout.dev.acdc.sdfac.lo\endcsname{0.62}
\expandafter\gdef\csname R@an.heldout.dev.amos.mean\endcsname{87.70}
\expandafter\gdef\csname R@an.heldout.dev.amos.n\endcsname{6}
\expandafter\gdef\csname R@an.heldout.dev.amos.name\endcsname{AMOS22}
\expandafter\gdef\csname R@an.heldout.dev.amos.ncomp\endcsname{3}
\expandafter\gdef\csname R@an.heldout.dev.amos.nunc\endcsname{3}
\expandafter\gdef\csname R@an.heldout.dev.amos.sd\endcsname{0.122}
\expandafter\gdef\csname R@an.heldout.dev.amos.sd_hi\endcsname{0.30}
\expandafter\gdef\csname R@an.heldout.dev.amos.sd_lo\endcsname{0.08}
\expandafter\gdef\csname R@an.heldout.dev.amos.sdfac.hi\endcsname{2.45}
\expandafter\gdef\csname R@an.heldout.dev.amos.sdfac.lo\endcsname{0.62}
\expandafter\gdef\csname R@an.heldout.dev.kits.mean\endcsname{83.38}
\expandafter\gdef\csname R@an.heldout.dev.kits.n\endcsname{3}
\expandafter\gdef\csname R@an.heldout.dev.kits.name\endcsname{KiTS23}
\expandafter\gdef\csname R@an.heldout.dev.kits.ncomp\endcsname{0}
\expandafter\gdef\csname R@an.heldout.dev.kits.nunc\endcsname{3}
\expandafter\gdef\csname R@an.heldout.dev.kits.sd\endcsname{0.795}
\expandafter\gdef\csname R@an.heldout.dev.kits.sd_hi\endcsname{5.00}
\expandafter\gdef\csname R@an.heldout.dev.kits.sd_lo\endcsname{0.41}
\expandafter\gdef\csname R@an.heldout.dev.kits.sdfac.hi\endcsname{6.28}
\expandafter\gdef\csname R@an.heldout.dev.kits.sdfac.lo\endcsname{0.52}
\expandafter\gdef\csname R@an.heldout.epochs\endcsname{1000}
\expandafter\gdef\csname R@an.heldout.fold\endcsname{0}
\expandafter\gdef\csname R@an.heldout.lits.L1.clause\endcsname{transfers (\ensuremath{+1.13}\,pp; inside the band of seed noise of that dataset)}
\expandafter\gdef\csname R@an.heldout.lits.L1.d\endcsname{\ensuremath{+1.13}}
\expandafter\gdef\csname R@an.heldout.lits.L1.d0\endcsname{\ensuremath{+1.93}}
\expandafter\gdef\csname R@an.heldout.lits.L1.d1\endcsname{\ensuremath{+1.79}}
\expandafter\gdef\csname R@an.heldout.lits.L1.d2\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.heldout.lits.L1.d3\endcsname{\ensuremath{+1.13}}
\expandafter\gdef\csname R@an.heldout.lits.L1.dsd\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.heldout.lits.L1.mean\endcsname{81.93}
\expandafter\gdef\csname R@an.heldout.lits.L1.n\endcsname{3}
\expandafter\gdef\csname R@an.heldout.lits.L1.npos\endcsname{2}
\expandafter\gdef\csname R@an.heldout.lits.L1.params\endcsname{102.35}
\expandafter\gdef\csname R@an.heldout.lits.L1.params_vs_default\endcsname{3.28}
\expandafter\gdef\csname R@an.heldout.lits.L1.place\endcsname{inside}
\expandafter\gdef\csname R@an.heldout.lits.L1.s0\endcsname{81.80}
\expandafter\gdef\csname R@an.heldout.lits.L1.s1\endcsname{81.76}
\expandafter\gdef\csname R@an.heldout.lits.L1.s2\endcsname{82.22}
\expandafter\gdef\csname R@an.heldout.lits.L1.sd_default\endcsname{1.515}
\expandafter\gdef\csname R@an.heldout.lits.L1.sd_own\endcsname{0.252}
\expandafter\gdef\csname R@an.heldout.lits.L1.state\endcsname{3 of 3 finished}
\expandafter\gdef\csname R@an.heldout.lits.L1.step_ms\endcsname{162.2}
\expandafter\gdef\csname R@an.heldout.lits.L1.step_vs_default\endcsname{1.33}
\expandafter\gdef\csname R@an.heldout.lits.L1.word\endcsname{transfers}
\expandafter\gdef\csname R@an.heldout.lits.L3.clause\endcsname{transfers (\ensuremath{+0.50}\,pp; inside the band of seed noise of that dataset)}
\expandafter\gdef\csname R@an.heldout.lits.L3.d\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.heldout.lits.L3.d0\endcsname{\ensuremath{+0.94}}
\expandafter\gdef\csname R@an.heldout.lits.L3.d1\endcsname{\ensuremath{+2.20}}
\expandafter\gdef\csname R@an.heldout.lits.L3.d2\endcsname{\ensuremath{-1.64}}
\expandafter\gdef\csname R@an.heldout.lits.L3.d3\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.heldout.lits.L3.dsd\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.heldout.lits.L3.mean\endcsname{81.29}
\expandafter\gdef\csname R@an.heldout.lits.L3.n\endcsname{3}
\expandafter\gdef\csname R@an.heldout.lits.L3.npos\endcsname{2}
\expandafter\gdef\csname R@an.heldout.lits.L3.params\endcsname{29.66}
\expandafter\gdef\csname R@an.heldout.lits.L3.params_vs_default\endcsname{0.95}
\expandafter\gdef\csname R@an.heldout.lits.L3.place\endcsname{inside}
\expandafter\gdef\csname R@an.heldout.lits.L3.s0\endcsname{80.80}
\expandafter\gdef\csname R@an.heldout.lits.L3.s1\endcsname{82.17}
\expandafter\gdef\csname R@an.heldout.lits.L3.s2\endcsname{80.90}
\expandafter\gdef\csname R@an.heldout.lits.L3.sd_default\endcsname{1.515}
\expandafter\gdef\csname R@an.heldout.lits.L3.sd_own\endcsname{0.762}
\expandafter\gdef\csname R@an.heldout.lits.L3.state\endcsname{3 of 3 finished}
\expandafter\gdef\csname R@an.heldout.lits.L3.step_ms\endcsname{174.8}
\expandafter\gdef\csname R@an.heldout.lits.L3.step_vs_default\endcsname{1.44}
\expandafter\gdef\csname R@an.heldout.lits.L3.word\endcsname{transfers}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.clause\endcsname{transfers (\ensuremath{+1.65}\,pp; inside the band of seed noise of that dataset)}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.d\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.d0\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.d1\endcsname{\ensuremath{+4.18}}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.d2\endcsname{\ensuremath{-1.20}}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.d3\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.dsd\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.mean\endcsname{82.44}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.n\endcsname{3}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.npos\endcsname{2}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.params\endcsname{31.04}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.params_vs_default\endcsname{0.99}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.place\endcsname{inside}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.s0\endcsname{81.83}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.s1\endcsname{84.16}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.s2\endcsname{81.34}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.sd_default\endcsname{1.515}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.sd_own\endcsname{1.506}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.state\endcsname{3 of 3 finished}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.step_ms\endcsname{111.5}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.step_vs_default\endcsname{0.92}
\expandafter\gdef\csname R@an.heldout.lits.V7A1.word\endcsname{transfers}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.n\endcsname{0}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.params\endcsname{31.18}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.s0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.sd_default\endcsname{1.515}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.state\endcsname{0 of 3 finished}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.step_ms\endcsname{132.9}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.step_vs_default\endcsname{1.09}
\expandafter\gdef\csname R@an.heldout.lits.V7A2.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.clause\endcsname{transfers (\ensuremath{+0.85}\,pp; inside the band of seed noise of that dataset)}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.d\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.d0\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.d1\endcsname{\ensuremath{+2.78}}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.d2\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.d3\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.dsd\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.mean\endcsname{81.65}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.n\endcsname{3}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.npos\endcsname{2}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.params\endcsname{21.11}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.params_vs_default\endcsname{0.68}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.place\endcsname{inside}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.s0\endcsname{79.54}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.s1\endcsname{82.76}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.s2\endcsname{82.65}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.sd_default\endcsname{1.515}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.sd_own\endcsname{1.831}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.state\endcsname{3 of 3 finished}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.step_ms\endcsname{92.2}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.step_vs_default\endcsname{0.76}
\expandafter\gdef\csname R@an.heldout.lits.V7C1.word\endcsname{transfers}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.n\endcsname{0}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.params\endcsname{31.31}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.s0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.sd_default\endcsname{1.515}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.state\endcsname{0 of 3 finished}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.step_ms\endcsname{108.8}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.step_vs_default\endcsname{0.89}
\expandafter\gdef\csname R@an.heldout.lits.V8A1.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.n\endcsname{0}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.params\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.params_vs_default\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.s0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.sd_default\endcsname{1.515}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.state\endcsname{0 of 3 finished}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.step_ms\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.step_vs_default\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8A2.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.n\endcsname{0}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.params\endcsname{18.21}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.params_vs_default\endcsname{0.58}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.s0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.sd_default\endcsname{1.515}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.state\endcsname{0 of 3 finished}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.step_ms\endcsname{69.9}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.step_vs_default\endcsname{0.57}
\expandafter\gdef\csname R@an.heldout.lits.V8B1.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.clause\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.d\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.d1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.d2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.dsd\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.n\endcsname{0}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.npos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.params\endcsname{21.08}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.params_vs_default\endcsname{0.68}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.place\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.s0\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.sd_default\endcsname{1.515}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.sd_own\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.state\endcsname{0 of 3 finished}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.step_ms\endcsname{74.1}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.step_vs_default\endcsname{0.61}
\expandafter\gdef\csname R@an.heldout.lits.V8B2.word\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.lits.band\endcsname{2.47}
\expandafter\gdef\csname R@an.heldout.lits.base.mean\endcsname{80.79}
\expandafter\gdef\csname R@an.heldout.lits.base.n\endcsname{3}
\expandafter\gdef\csname R@an.heldout.lits.base.params\endcsname{31.20}
\expandafter\gdef\csname R@an.heldout.lits.base.params_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.heldout.lits.base.s0\endcsname{79.86}
\expandafter\gdef\csname R@an.heldout.lits.base.s1\endcsname{79.98}
\expandafter\gdef\csname R@an.heldout.lits.base.s2\endcsname{82.54}
\expandafter\gdef\csname R@an.heldout.lits.base.sd_default\endcsname{1.515}
\expandafter\gdef\csname R@an.heldout.lits.base.sd_own\endcsname{1.515}
\expandafter\gdef\csname R@an.heldout.lits.base.state\endcsname{3 of 3 finished}
\expandafter\gdef\csname R@an.heldout.lits.base.step_ms\endcsname{121.8}
\expandafter\gdef\csname R@an.heldout.lits.base.step_vs_default\endcsname{1.00}
\expandafter\gdef\csname R@an.heldout.lits.batch\endcsname{2}
\expandafter\gdef\csname R@an.heldout.lits.complete\endcsname{yes}
\expandafter\gdef\csname R@an.heldout.lits.mean_default\endcsname{80.79}
\expandafter\gdef\csname R@an.heldout.lits.metric\endcsname{the mean Dice over the two scored classes (liver and tumour)}
\expandafter\gdef\csname R@an.heldout.lits.n.done\endcsname{9}
\expandafter\gdef\csname R@an.heldout.lits.n.total\endcsname{9}
\expandafter\gdef\csname R@an.heldout.lits.name\endcsname{LiTS}
\expandafter\gdef\csname R@an.heldout.lits.ncases\endcsname{131}
\expandafter\gdef\csname R@an.heldout.lits.nfg\endcsname{2}
\expandafter\gdef\csname R@an.heldout.lits.ntrain\endcsname{104}
\expandafter\gdef\csname R@an.heldout.lits.nval\endcsname{27}
\expandafter\gdef\csname R@an.heldout.lits.patch\endcsname{$128\times 128\times 128$}
\expandafter\gdef\csname R@an.heldout.lits.read\endcsname{HyReX transfers (\ensuremath{+0.50}\,pp; inside the band of seed noise of that dataset), and ResEnc-M transfers (\ensuremath{+1.13}\,pp; inside the band of seed noise of that dataset)}
\expandafter\gdef\csname R@an.heldout.lits.sd\endcsname{1.515}
\expandafter\gdef\csname R@an.heldout.lits.sd_default\endcsname{1.515}
\expandafter\gdef\csname R@an.heldout.lits.sd_hi\endcsname{9.52}
\expandafter\gdef\csname R@an.heldout.lits.sd_lo\endcsname{0.79}
\expandafter\gdef\csname R@an.heldout.lits.state\endcsname{9 of 9 finished}
\expandafter\gdef\csname R@an.heldout.n.bad\endcsname{0}
\expandafter\gdef\csname R@an.heldout.n.done\endcsname{21}
\expandafter\gdef\csname R@an.heldout.n.failed\endcsname{0}
\expandafter\gdef\csname R@an.heldout.n.notstarted\endcsname{6}
\expandafter\gdef\csname R@an.heldout.n.registered\endcsname{27}
\expandafter\gdef\csname R@an.heldout.n.running\endcsname{0}
\expandafter\gdef\csname R@an.heldout.narms\endcsname{3}
\expandafter\gdef\csname R@an.heldout.ndatasets\endcsname{3}
\expandafter\gdef\csname R@an.heldout.ndatasets.word\endcsname{three}
\expandafter\gdef\csname R@an.heldout.nperds\endcsname{9}
\expandafter\gdef\csname R@an.heldout.nseeds\endcsname{3}
\expandafter\gdef\csname R@an.heldout.nseeds.word\endcsname{three}
\expandafter\gdef\csname R@an.heldout.rule\endcsname{transfers iff the three-seed mean difference to the default of the same dataset is positive; every dataset is read by itself and none is pooled}
\expandafter\gdef\csname R@an.heldout.sdfac.hi\endcsname{6.28}
\expandafter\gdef\csname R@an.heldout.sdfac.level\endcsname{95}
\expandafter\gdef\csname R@an.heldout.sdfac.lo\endcsname{0.52}
\expandafter\gdef\csname R@an.heldout.seeds.range\endcsname{0 to 2}
\expandafter\gdef\csname R@an.heldout.sets.complete\endcsname{2}
\expandafter\gdef\csname R@an.heldout.smallest.name\endcsname{BTCV}
\expandafter\gdef\csname R@an.heldout.smallest.nval\endcsname{6}
\expandafter\gdef\csname R@an.heldout.state\endcsname{21 of 27 finished}
\expandafter\gdef\csname R@an.heldout.target.T1.D2.arm\endcsname{LeanDec}
\expandafter\gdef\csname R@an.heldout.target.T1.D2.k\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.D2.kpos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.D2.m\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.D2.nlanded\endcsname{3}
\expandafter\gdef\csname R@an.heldout.target.T1.D2.outcome\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.target.T1.D2.paramline\endcsname{$0.836\times$ / $0.836\times$ / $0.832\times$ the default's profiled parameters on the AMOS22, KiTS23 and ACDC plans (pass line: at most $1.05\times$ on each; the largest is $0.836\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T1.D2.passline\endcsname{Addendum AA3 (T1)}
\expandafter\gdef\csname R@an.heldout.target.T1.D2.primary\endcsname{no}
\expandafter\gdef\csname R@an.heldout.target.T1.D2.sentence\endcsname{the registered claim target T1 for LeanDec has no outcome yet (Addendum AA3 (T1): the profiled parameters at most $1.05\times$ the default's on every development plan, the mean of the six benchmark contrasts above 0 and at least four of the six positive): three of the six benchmark contrasts have landed; LiTS, BTCV and BraTS-MSD are still to come. The six contrasts are AMOS22 \ensuremath{-0.44}\,pp, KiTS23 \ensuremath{+1.04}\,pp, ACDC \ensuremath{-0.05}\,pp, LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds). T1 is a registered claim target, not a transfer verdict; its mean and count over six benchmarks depart from the no-pooling clause of Addendum Q2-E, a departure Addendum AE registers, and every held-out dataset keeps its own reading beside it.}
\expandafter\gdef\csname R@an.heldout.target.T1.D2.short\endcsname{pending (three of six benchmarks landed)}
\expandafter\gdef\csname R@an.heldout.target.T1.D2.six\endcsname{AMOS22 \ensuremath{-0.44}\,pp, KiTS23 \ensuremath{+1.04}\,pp, ACDC \ensuremath{-0.05}\,pp, LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds)}
\expandafter\gdef\csname R@an.heldout.target.T1.D2.state\endcsname{three of the six benchmark contrasts have landed; LiTS, BTCV and BraTS-MSD are still to come}
\expandafter\gdef\csname R@an.heldout.target.T1.D2.stepline\endcsname{$0.812\times$ / $0.808\times$ / $0.806\times$ the default's profiled training step on the AMOS22, KiTS23 and ACDC plans; T1 does not read the training step}
\expandafter\gdef\csname R@an.heldout.target.T1.D2.title\endcsname{average accuracy at the default's size}
\expandafter\gdef\csname R@an.heldout.target.T1.L3.arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.heldout.target.T1.L3.k\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.L3.kpos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.L3.m\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.L3.nlanded\endcsname{5}
\expandafter\gdef\csname R@an.heldout.target.T1.L3.outcome\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.target.T1.L3.paramline\endcsname{$0.951\times$ / $0.951\times$ / $0.950\times$ the default's profiled parameters on the AMOS22, KiTS23 and ACDC plans (pass line: at most $1.05\times$ on each; the largest is $0.951\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T1.L3.passline\endcsname{Addendum AA3 (T1)}
\expandafter\gdef\csname R@an.heldout.target.T1.L3.primary\endcsname{yes}
\expandafter\gdef\csname R@an.heldout.target.T1.L3.sentence\endcsname{the registered claim target T1 for HyReX has no outcome yet (Addendum AA3 (T1): the profiled parameters at most $1.05\times$ the default's on every development plan, the mean of the six benchmark contrasts above 0 and at least four of the six positive): five of the six benchmark contrasts have landed; BraTS-MSD is still to come. The six contrasts are AMOS22 \ensuremath{+0.23}\,pp, KiTS23 \ensuremath{+0.68}\,pp, ACDC \ensuremath{+0.33}\,pp, LiTS \ensuremath{+0.50}\,pp, BTCV \ensuremath{+0.71}\,pp, BraTS-MSD pending (one of three seeds). T1 is a registered claim target, not a transfer verdict; its mean and count over six benchmarks depart from the no-pooling clause of Addendum Q2-E, a departure Addendum AE registers, and every held-out dataset keeps its own reading beside it.}
\expandafter\gdef\csname R@an.heldout.target.T1.L3.short\endcsname{pending (five of six benchmarks landed)}
\expandafter\gdef\csname R@an.heldout.target.T1.L3.six\endcsname{AMOS22 \ensuremath{+0.23}\,pp, KiTS23 \ensuremath{+0.68}\,pp, ACDC \ensuremath{+0.33}\,pp, LiTS \ensuremath{+0.50}\,pp, BTCV \ensuremath{+0.71}\,pp, BraTS-MSD pending (one of three seeds)}
\expandafter\gdef\csname R@an.heldout.target.T1.L3.state\endcsname{five of the six benchmark contrasts have landed; BraTS-MSD is still to come}
\expandafter\gdef\csname R@an.heldout.target.T1.L3.stepline\endcsname{$1.528\times$ / $1.401\times$ / $1.642\times$ the default's profiled training step on the AMOS22, KiTS23 and ACDC plans; T1 does not read the training step}
\expandafter\gdef\csname R@an.heldout.target.T1.L3.title\endcsname{average accuracy at the default's size}
\expandafter\gdef\csname R@an.heldout.target.T1.V5A5.arm\endcsname{HyReX-LeanDec}
\expandafter\gdef\csname R@an.heldout.target.T1.V5A5.k\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V5A5.kpos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V5A5.m\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V5A5.nlanded\endcsname{0}
\expandafter\gdef\csname R@an.heldout.target.T1.V5A5.outcome\endcsname{NOT MET}
\expandafter\gdef\csname R@an.heldout.target.T1.V5A5.paramline\endcsname{$0.947\times$ / $0.946\times$ / $0.946\times$ the default's profiled parameters on the AMOS22, KiTS23 and ACDC plans (pass line: at most $1.05\times$ on each; the largest is $0.947\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T1.V5A5.passline\endcsname{Addendum AA3 (T1)}
\expandafter\gdef\csname R@an.heldout.target.T1.V5A5.primary\endcsname{no}
\expandafter\gdef\csname R@an.heldout.target.T1.V5A5.sentence\endcsname{HyReX-LeanDec does not meet the registered claim target T1 (Addendum AA3 (T1): the profiled parameters at most $1.05\times$ the default's on every development plan, the mean of the six benchmark contrasts above 0 and at least four of the six positive): no ACDC cell: the ACDC plan does not fit the cap (allocated 11.74\,GB, the profiler's allocated bar refuses it; reserved 11.98\,GB against the 12\,GB cap), so the six benchmarks the pass line reads can never all exist. The six contrasts are AMOS22 pending (the cross-validation runs are not registered yet), KiTS23 pending (the cross-validation runs are not registered yet), ACDC no cell (the ACDC plan does not fit the cap (allocated 11.74\,GB, the profiler's allocated bar refuses it; reserved 11.98\,GB against the 12\,GB cap)), LiTS pending (the held-out runs are not registered yet), BTCV pending (the held-out runs are not registered yet), BraTS-MSD pending (the held-out runs are not registered yet). T1 is a registered claim target, not a transfer verdict; its mean and count over six benchmarks depart from the no-pooling clause of Addendum Q2-E, a departure Addendum AE registers, and every held-out dataset keeps its own reading beside it.}
\expandafter\gdef\csname R@an.heldout.target.T1.V5A5.short\endcsname{NOT MET (no ACDC cell: the plan does not fit the cap)}
\expandafter\gdef\csname R@an.heldout.target.T1.V5A5.six\endcsname{AMOS22 pending (the cross-validation runs are not registered yet), KiTS23 pending (the cross-validation runs are not registered yet), ACDC no cell (the ACDC plan does not fit the cap (allocated 11.74\,GB, the profiler's allocated bar refuses it; reserved 11.98\,GB against the 12\,GB cap)), LiTS pending (the held-out runs are not registered yet), BTCV pending (the held-out runs are not registered yet), BraTS-MSD pending (the held-out runs are not registered yet)}
\expandafter\gdef\csname R@an.heldout.target.T1.V5A5.state\endcsname{no ACDC cell: the ACDC plan does not fit the cap (allocated 11.74\,GB, the profiler's allocated bar refuses it; reserved 11.98\,GB against the 12\,GB cap), so the six benchmarks the pass line reads can never all exist}
\expandafter\gdef\csname R@an.heldout.target.T1.V5A5.stepline\endcsname{$1.393\times$ / $1.235\times$ / $1.494\times$ the default's profiled training step on the AMOS22, KiTS23 and ACDC plans; T1 does not read the training step}
\expandafter\gdef\csname R@an.heldout.target.T1.V5A5.title\endcsname{average accuracy at the default's size}
\expandafter\gdef\csname R@an.heldout.target.T1.V5B2.arm\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.heldout.target.T1.V5B2.k\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V5B2.kpos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V5B2.m\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V5B2.nlanded\endcsname{3}
\expandafter\gdef\csname R@an.heldout.target.T1.V5B2.outcome\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.target.T1.V5B2.paramline\endcsname{$0.682\times$ / $0.681\times$ / $0.674\times$ the default's profiled parameters on the AMOS22, KiTS23 and ACDC plans (pass line: at most $1.05\times$ on each; the largest is $0.682\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T1.V5B2.passline\endcsname{Addendum AA3 (T1)}
\expandafter\gdef\csname R@an.heldout.target.T1.V5B2.primary\endcsname{no}
\expandafter\gdef\csname R@an.heldout.target.T1.V5B2.sentence\endcsname{the registered claim target T1 for LeanAdd-NeXt has no outcome yet (Addendum AA3 (T1): the profiled parameters at most $1.05\times$ the default's on every development plan, the mean of the six benchmark contrasts above 0 and at least four of the six positive): three of the six benchmark contrasts have landed; LiTS, BTCV and BraTS-MSD are still to come. The six contrasts are AMOS22 \ensuremath{-0.25}\,pp, KiTS23 \ensuremath{-0.75}\,pp, ACDC \ensuremath{-0.11}\,pp, LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds). T1 is a registered claim target, not a transfer verdict; its mean and count over six benchmarks depart from the no-pooling clause of Addendum Q2-E, a departure Addendum AE registers, and every held-out dataset keeps its own reading beside it.}
\expandafter\gdef\csname R@an.heldout.target.T1.V5B2.short\endcsname{pending (three of six benchmarks landed)}
\expandafter\gdef\csname R@an.heldout.target.T1.V5B2.six\endcsname{AMOS22 \ensuremath{-0.25}\,pp, KiTS23 \ensuremath{-0.75}\,pp, ACDC \ensuremath{-0.11}\,pp, LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds)}
\expandafter\gdef\csname R@an.heldout.target.T1.V5B2.state\endcsname{three of the six benchmark contrasts have landed; LiTS, BTCV and BraTS-MSD are still to come}
\expandafter\gdef\csname R@an.heldout.target.T1.V5B2.stepline\endcsname{$0.853\times$ / $0.836\times$ / $0.915\times$ the default's profiled training step on the AMOS22, KiTS23 and ACDC plans; T1 does not read the training step}
\expandafter\gdef\csname R@an.heldout.target.T1.V5B2.title\endcsname{average accuracy at the default's size}
\expandafter\gdef\csname R@an.heldout.target.T1.V6A1r.arm\endcsname{HyReX-k9}
\expandafter\gdef\csname R@an.heldout.target.T1.V6A1r.k\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V6A1r.kpos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V6A1r.m\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V6A1r.nlanded\endcsname{3}
\expandafter\gdef\csname R@an.heldout.target.T1.V6A1r.outcome\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.target.T1.V6A1r.paramline\endcsname{$0.987\times$ / $0.987\times$ / $0.986\times$ the default's profiled parameters on the AMOS22, KiTS23 and ACDC plans (pass line: at most $1.05\times$ on each; the largest is $0.987\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T1.V6A1r.passline\endcsname{Addendum AA3 (T1)}
\expandafter\gdef\csname R@an.heldout.target.T1.V6A1r.primary\endcsname{no}
\expandafter\gdef\csname R@an.heldout.target.T1.V6A1r.sentence\endcsname{the registered claim target T1 for HyReX-k9 has no outcome yet (Addendum AA3 (T1): the profiled parameters at most $1.05\times$ the default's on every development plan, the mean of the six benchmark contrasts above 0 and at least four of the six positive): three of the six benchmark contrasts have landed; LiTS, BTCV and BraTS-MSD are still to come. The six contrasts are AMOS22 \ensuremath{+0.20}\,pp, KiTS23 \ensuremath{+0.28}\,pp, ACDC \ensuremath{+0.31}\,pp, LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds). T1 is a registered claim target, not a transfer verdict; its mean and count over six benchmarks depart from the no-pooling clause of Addendum Q2-E, a departure Addendum AE registers, and every held-out dataset keeps its own reading beside it.}
\expandafter\gdef\csname R@an.heldout.target.T1.V6A1r.short\endcsname{pending (three of six benchmarks landed)}
\expandafter\gdef\csname R@an.heldout.target.T1.V6A1r.six\endcsname{AMOS22 \ensuremath{+0.20}\,pp, KiTS23 \ensuremath{+0.28}\,pp, ACDC \ensuremath{+0.31}\,pp, LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds)}
\expandafter\gdef\csname R@an.heldout.target.T1.V6A1r.state\endcsname{three of the six benchmark contrasts have landed; LiTS, BTCV and BraTS-MSD are still to come}
\expandafter\gdef\csname R@an.heldout.target.T1.V6A1r.stepline\endcsname{$1.630\times$ / $1.490\times$ / $1.811\times$ the default's profiled training step on the AMOS22, KiTS23 and ACDC plans; T1 does not read the training step}
\expandafter\gdef\csname R@an.heldout.target.T1.V6A1r.title\endcsname{average accuracy at the default's size}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A1.arm\endcsname{LeanDeepMid}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A1.k\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A1.kpos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A1.m\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A1.nlanded\endcsname{5}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A1.outcome\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A1.paramline\endcsname{$0.996\times$ / $0.995\times$ / $0.996\times$ the default's profiled parameters on the AMOS22, KiTS23 and ACDC plans (pass line: at most $1.05\times$ on each; the largest is $0.996\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A1.passline\endcsname{Addendum AA3 (T1)}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A1.primary\endcsname{no}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A1.sentence\endcsname{the registered claim target T1 for LeanDeepMid has no outcome yet (Addendum AA3 (T1): the profiled parameters at most $1.05\times$ the default's on every development plan, the mean of the six benchmark contrasts above 0 and at least four of the six positive): five of the six benchmark contrasts have landed; BraTS-MSD is still to come. The six contrasts are AMOS22 \ensuremath{+0.26}\,pp, KiTS23 \ensuremath{+1.63}\,pp, ACDC \ensuremath{+0.08}\,pp, LiTS \ensuremath{+1.65}\,pp, BTCV \ensuremath{+0.49}\,pp, BraTS-MSD pending (0 of three seeds). T1 is a registered claim target, not a transfer verdict; its mean and count over six benchmarks depart from the no-pooling clause of Addendum Q2-E, a departure Addendum AE registers, and every held-out dataset keeps its own reading beside it.}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A1.short\endcsname{pending (five of six benchmarks landed)}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A1.six\endcsname{AMOS22 \ensuremath{+0.26}\,pp, KiTS23 \ensuremath{+1.63}\,pp, ACDC \ensuremath{+0.08}\,pp, LiTS \ensuremath{+1.65}\,pp, BTCV \ensuremath{+0.49}\,pp, BraTS-MSD pending (0 of three seeds)}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A1.state\endcsname{five of the six benchmark contrasts have landed; BraTS-MSD is still to come}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A1.stepline\endcsname{$0.999\times$ / $0.917\times$ / $1.069\times$ the default's profiled training step on the AMOS22, KiTS23 and ACDC plans; T1 does not read the training step}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A1.title\endcsname{average accuracy at the default's size}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A2.arm\endcsname{LeanDeepMid+FD}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A2.k\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A2.kpos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A2.m\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A2.nlanded\endcsname{1}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A2.outcome\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A2.paramline\endcsname{$1.000\times$ / $0.999\times$ / $1.000\times$ the default's profiled parameters on the AMOS22, KiTS23 and ACDC plans (pass line: at most $1.05\times$ on each; the largest is $1.000\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A2.passline\endcsname{Addendum AA3 (T1)}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A2.primary\endcsname{no}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A2.sentence\endcsname{the registered claim target T1 for LeanDeepMid+FD has no outcome yet (Addendum AA3 (T1): the profiled parameters at most $1.05\times$ the default's on every development plan, the mean of the six benchmark contrasts above 0 and at least four of the six positive): one of the six benchmark contrasts have landed; AMOS22, ACDC, LiTS, BTCV and BraTS-MSD are still to come. The six contrasts are AMOS22 pending (0 of four folds), KiTS23 \ensuremath{+0.91}\,pp, ACDC pending (0 of four folds), LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds). T1 is a registered claim target, not a transfer verdict; its mean and count over six benchmarks depart from the no-pooling clause of Addendum Q2-E, a departure Addendum AE registers, and every held-out dataset keeps its own reading beside it.}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A2.short\endcsname{pending (one of six benchmarks landed)}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A2.six\endcsname{AMOS22 pending (0 of four folds), KiTS23 \ensuremath{+0.91}\,pp, ACDC pending (0 of four folds), LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds)}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A2.state\endcsname{one of the six benchmark contrasts have landed; AMOS22, ACDC, LiTS, BTCV and BraTS-MSD are still to come}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A2.stepline\endcsname{$1.147\times$ / $1.092\times$ / $1.227\times$ the default's profiled training step on the AMOS22, KiTS23 and ACDC plans; T1 does not read the training step}
\expandafter\gdef\csname R@an.heldout.target.T1.V7A2.title\endcsname{average accuracy at the default's size}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A1.arm\endcsname{CoarseStack}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A1.k\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A1.kpos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A1.m\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A1.nlanded\endcsname{0}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A1.outcome\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A1.paramline\endcsname{$1.005\times$ / $1.004\times$ / $1.005\times$ the default's profiled parameters on the AMOS22, KiTS23 and ACDC plans (pass line: at most $1.05\times$ on each; the largest is $1.005\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A1.passline\endcsname{Addendum AA3 (T1)}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A1.primary\endcsname{no}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A1.sentence\endcsname{the registered claim target T1 for CoarseStack has no outcome yet (Addendum AA3 (T1): the profiled parameters at most $1.05\times$ the default's on every development plan, the mean of the six benchmark contrasts above 0 and at least four of the six positive): 0 of the six benchmark contrasts have landed; AMOS22, KiTS23, ACDC, LiTS, BTCV and BraTS-MSD are still to come. The six contrasts are AMOS22 pending (the cross-validation runs are not registered yet), KiTS23 pending (the cross-validation runs are not registered yet), ACDC pending (the cross-validation runs are not registered yet), LiTS pending (the held-out runs are not registered yet), BTCV pending (the held-out runs are not registered yet), BraTS-MSD pending (the held-out runs are not registered yet). T1 is a registered claim target, not a transfer verdict; its mean and count over six benchmarks depart from the no-pooling clause of Addendum Q2-E, a departure Addendum AE registers, and every held-out dataset keeps its own reading beside it.}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A1.short\endcsname{pending (0 of six benchmarks landed)}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A1.six\endcsname{AMOS22 pending (the cross-validation runs are not registered yet), KiTS23 pending (the cross-validation runs are not registered yet), ACDC pending (the cross-validation runs are not registered yet), LiTS pending (the held-out runs are not registered yet), BTCV pending (the held-out runs are not registered yet), BraTS-MSD pending (the held-out runs are not registered yet)}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A1.state\endcsname{0 of the six benchmark contrasts have landed; AMOS22, KiTS23, ACDC, LiTS, BTCV and BraTS-MSD are still to come}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A1.stepline\endcsname{$0.895\times$ / $0.912\times$ / $0.997\times$ the default's profiled training step on the AMOS22, KiTS23 and ACDC plans; T1 does not read the training step}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A1.title\endcsname{average accuracy at the default's size}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A2.arm\endcsname{StackDec}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A2.k\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A2.kpos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A2.m\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A2.nlanded\endcsname{0}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A2.outcome\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A2.paramline\endcsname{$1.010\times$ / $1.009\times$ / $1.010\times$ the default's profiled parameters on the AMOS22, KiTS23 and ACDC plans (pass line: at most $1.05\times$ on each; the largest is $1.010\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A2.passline\endcsname{Addendum AA3 (T1)}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A2.primary\endcsname{no}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A2.sentence\endcsname{the registered claim target T1 for StackDec has no outcome yet (Addendum AA3 (T1): the profiled parameters at most $1.05\times$ the default's on every development plan, the mean of the six benchmark contrasts above 0 and at least four of the six positive): 0 of the six benchmark contrasts have landed; AMOS22, KiTS23, ACDC, LiTS, BTCV and BraTS-MSD are still to come. The six contrasts are AMOS22 pending (the cross-validation runs are not registered yet), KiTS23 pending (the cross-validation runs are not registered yet), ACDC pending (the cross-validation runs are not registered yet), LiTS pending (the held-out runs are not registered yet), BTCV pending (the held-out runs are not registered yet), BraTS-MSD pending (the held-out runs are not registered yet). T1 is a registered claim target, not a transfer verdict; its mean and count over six benchmarks depart from the no-pooling clause of Addendum Q2-E, a departure Addendum AE registers, and every held-out dataset keeps its own reading beside it.}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A2.short\endcsname{pending (0 of six benchmarks landed)}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A2.six\endcsname{AMOS22 pending (the cross-validation runs are not registered yet), KiTS23 pending (the cross-validation runs are not registered yet), ACDC pending (the cross-validation runs are not registered yet), LiTS pending (the held-out runs are not registered yet), BTCV pending (the held-out runs are not registered yet), BraTS-MSD pending (the held-out runs are not registered yet)}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A2.state\endcsname{0 of the six benchmark contrasts have landed; AMOS22, KiTS23, ACDC, LiTS, BTCV and BraTS-MSD are still to come}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A2.stepline\endcsname{$0.858\times$ / $0.854\times$ / $0.920\times$ the default's profiled training step on the AMOS22, KiTS23 and ACDC plans; T1 does not read the training step}
\expandafter\gdef\csname R@an.heldout.target.T1.V8A2.title\endcsname{average accuracy at the default's size}
\expandafter\gdef\csname R@an.heldout.target.T2.D2.arm\endcsname{LeanDec}
\expandafter\gdef\csname R@an.heldout.target.T2.D2.k\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.D2.kpos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.D2.m\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.D2.nlanded\endcsname{3}
\expandafter\gdef\csname R@an.heldout.target.T2.D2.outcome\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.target.T2.D2.paramline\endcsname{$0.836\times$ / $0.836\times$ / $0.832\times$ the default's profiled parameters on the AMOS22, KiTS23 and ACDC plans (pass line: at most $0.85\times$ on each; the largest is $0.836\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T2.D2.passline\endcsname{Addendum AA3 (T2)}
\expandafter\gdef\csname R@an.heldout.target.T2.D2.primary\endcsname{yes}
\expandafter\gdef\csname R@an.heldout.target.T2.D2.sentence\endcsname{the registered claim target T2 for LeanDec has no outcome yet (Addendum AA3 (T2): the profiled parameters at most $0.85\times$ the default's on every development plan, the profiled training step at most $0.85\times$ the default's on every development plan, the mean of the six benchmark contrasts at least $-0.50$\,pp and at least four of the six at least $-0.50$\,pp): three of the six benchmark contrasts have landed; LiTS, BTCV and BraTS-MSD are still to come. The six contrasts are AMOS22 \ensuremath{-0.44}\,pp, KiTS23 \ensuremath{+1.04}\,pp, ACDC \ensuremath{-0.05}\,pp, LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds). T2 is a registered claim target, not a transfer verdict; its mean and count over six benchmarks depart from the no-pooling clause of Addendum Q2-E, a departure Addendum AE registers, and every held-out dataset keeps its own reading beside it.}
\expandafter\gdef\csname R@an.heldout.target.T2.D2.short\endcsname{pending (three of six benchmarks landed)}
\expandafter\gdef\csname R@an.heldout.target.T2.D2.six\endcsname{AMOS22 \ensuremath{-0.44}\,pp, KiTS23 \ensuremath{+1.04}\,pp, ACDC \ensuremath{-0.05}\,pp, LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds)}
\expandafter\gdef\csname R@an.heldout.target.T2.D2.state\endcsname{three of the six benchmark contrasts have landed; LiTS, BTCV and BraTS-MSD are still to come}
\expandafter\gdef\csname R@an.heldout.target.T2.D2.stepline\endcsname{$0.812\times$ / $0.808\times$ / $0.806\times$ the default's profiled training step on the AMOS22, KiTS23 and ACDC plans (pass line: at most $0.85\times$ on each; the largest is $0.812\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T2.D2.title\endcsname{smaller and faster, with accuracy not resolved as worse at the registered margin}
\expandafter\gdef\csname R@an.heldout.target.T2.L3.arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.heldout.target.T2.L3.k\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.L3.kpos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.L3.m\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.L3.nlanded\endcsname{5}
\expandafter\gdef\csname R@an.heldout.target.T2.L3.outcome\endcsname{NOT MET}
\expandafter\gdef\csname R@an.heldout.target.T2.L3.paramline\endcsname{$0.951\times$ / $0.951\times$ / $0.950\times$ the default's profiled parameters on the AMOS22, KiTS23 and ACDC plans (pass line: at most $0.85\times$ on each; the largest is $0.951\times$): NOT met}
\expandafter\gdef\csname R@an.heldout.target.T2.L3.passline\endcsname{Addendum AA3 (T2)}
\expandafter\gdef\csname R@an.heldout.target.T2.L3.primary\endcsname{no}
\expandafter\gdef\csname R@an.heldout.target.T2.L3.sentence\endcsname{HyReX does not meet the registered claim target T2 (Addendum AA3 (T2): the profiled parameters at most $0.85\times$ the default's on every development plan, the profiled training step at most $0.85\times$ the default's on every development plan, the mean of the six benchmark contrasts at least $-0.50$\,pp and at least four of the six at least $-0.50$\,pp): the cost line is not met (parameters $0.950$ to $0.951\times$ on all three plans and step $1.401$ to $1.642\times$ on all three plans). The six contrasts, as read so far, are AMOS22 \ensuremath{+0.23}\,pp, KiTS23 \ensuremath{+0.68}\,pp, ACDC \ensuremath{+0.33}\,pp, LiTS \ensuremath{+0.50}\,pp, BTCV \ensuremath{+0.71}\,pp, BraTS-MSD pending (one of three seeds); they are not needed for the outcome, which the cost line decides. T2 is a registered claim target, not a transfer verdict; its mean and count over six benchmarks depart from the no-pooling clause of Addendum Q2-E, a departure Addendum AE registers, and every held-out dataset keeps its own reading beside it.}
\expandafter\gdef\csname R@an.heldout.target.T2.L3.short\endcsname{NOT MET (cost line: parameters $0.950$ to $0.951\times$ on all three plans and step $1.401$ to $1.642\times$ on all three plans)}
\expandafter\gdef\csname R@an.heldout.target.T2.L3.six\endcsname{AMOS22 \ensuremath{+0.23}\,pp, KiTS23 \ensuremath{+0.68}\,pp, ACDC \ensuremath{+0.33}\,pp, LiTS \ensuremath{+0.50}\,pp, BTCV \ensuremath{+0.71}\,pp, BraTS-MSD pending (one of three seeds) (read so far, not needed for the outcome)}
\expandafter\gdef\csname R@an.heldout.target.T2.L3.state\endcsname{the cost line is not met (parameters $0.950$ to $0.951\times$ on all three plans and step $1.401$ to $1.642\times$ on all three plans)}
\expandafter\gdef\csname R@an.heldout.target.T2.L3.stepline\endcsname{$1.528\times$ / $1.401\times$ / $1.642\times$ the default's profiled training step on the AMOS22, KiTS23 and ACDC plans (pass line: at most $0.85\times$ on each; the largest is $1.642\times$): NOT met}
\expandafter\gdef\csname R@an.heldout.target.T2.L3.title\endcsname{smaller and faster, with accuracy not resolved as worse at the registered margin}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B1.arm\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B1.k\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B1.kpos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B1.m\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B1.nlanded\endcsname{3}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B1.outcome\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B1.paramline\endcsname{$0.673\times$ / $0.672\times$ / $0.664\times$ the default's profiled parameters on the AMOS22, KiTS23 and ACDC plans (pass line: at most $0.85\times$ on each; the largest is $0.673\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B1.passline\endcsname{Addendum AA3 (T2)}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B1.primary\endcsname{no}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B1.sentence\endcsname{the registered claim target T2 for LeanAdd has no outcome yet (Addendum AA3 (T2): the profiled parameters at most $0.85\times$ the default's on every development plan, the profiled training step at most $0.85\times$ the default's on every development plan, the mean of the six benchmark contrasts at least $-0.50$\,pp and at least four of the six at least $-0.50$\,pp): three of the six benchmark contrasts have landed; LiTS, BTCV and BraTS-MSD are still to come. The six contrasts are AMOS22 \ensuremath{-0.46}\,pp, KiTS23 \ensuremath{+0.99}\,pp, ACDC \ensuremath{-0.12}\,pp, LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds). T2 is a registered claim target, not a transfer verdict; its mean and count over six benchmarks depart from the no-pooling clause of Addendum Q2-E, a departure Addendum AE registers, and every held-out dataset keeps its own reading beside it.}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B1.short\endcsname{pending (three of six benchmarks landed)}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B1.six\endcsname{AMOS22 \ensuremath{-0.46}\,pp, KiTS23 \ensuremath{+0.99}\,pp, ACDC \ensuremath{-0.12}\,pp, LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds)}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B1.state\endcsname{three of the six benchmark contrasts have landed; LiTS, BTCV and BraTS-MSD are still to come}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B1.stepline\endcsname{$0.740\times$ / $0.727\times$ / $0.719\times$ the default's profiled training step on the AMOS22, KiTS23 and ACDC plans (pass line: at most $0.85\times$ on each; the largest is $0.740\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B1.title\endcsname{smaller and faster, with accuracy not resolved as worse at the registered margin}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B2.arm\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B2.k\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B2.kpos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B2.m\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B2.nlanded\endcsname{3}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B2.outcome\endcsname{NOT MET}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B2.paramline\endcsname{$0.682\times$ / $0.681\times$ / $0.674\times$ the default's profiled parameters on the AMOS22, KiTS23 and ACDC plans (pass line: at most $0.85\times$ on each; the largest is $0.682\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B2.passline\endcsname{Addendum AA3 (T2)}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B2.primary\endcsname{no}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B2.sentence\endcsname{LeanAdd-NeXt does not meet the registered claim target T2 (Addendum AA3 (T2): the profiled parameters at most $0.85\times$ the default's on every development plan, the profiled training step at most $0.85\times$ the default's on every development plan, the mean of the six benchmark contrasts at least $-0.50$\,pp and at least four of the six at least $-0.50$\,pp): the cost line is not met (step $0.853\times$ on AMOS22 and step $0.915\times$ on ACDC). The six contrasts, as read so far, are AMOS22 \ensuremath{-0.25}\,pp, KiTS23 \ensuremath{-0.75}\,pp, ACDC \ensuremath{-0.11}\,pp, LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds); they are not needed for the outcome, which the cost line decides. T2 is a registered claim target, not a transfer verdict; its mean and count over six benchmarks depart from the no-pooling clause of Addendum Q2-E, a departure Addendum AE registers, and every held-out dataset keeps its own reading beside it.}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B2.short\endcsname{NOT MET (cost line: step $0.853\times$ on AMOS22 and step $0.915\times$ on ACDC)}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B2.six\endcsname{AMOS22 \ensuremath{-0.25}\,pp, KiTS23 \ensuremath{-0.75}\,pp, ACDC \ensuremath{-0.11}\,pp, LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds) (read so far, not needed for the outcome)}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B2.state\endcsname{the cost line is not met (step $0.853\times$ on AMOS22 and step $0.915\times$ on ACDC)}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B2.stepline\endcsname{$0.853\times$ / $0.836\times$ / $0.915\times$ the default's profiled training step on the AMOS22, KiTS23 and ACDC plans (pass line: at most $0.85\times$ on each; the largest is $0.915\times$): NOT met}
\expandafter\gdef\csname R@an.heldout.target.T2.V5B2.title\endcsname{smaller and faster, with accuracy not resolved as worse at the registered margin}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B1.arm\endcsname{LeanSep}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B1.k\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B1.kpos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B1.m\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B1.nlanded\endcsname{0}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B1.outcome\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B1.paramline\endcsname{$0.656\times$ / $0.655\times$ / $0.647\times$ the default's profiled parameters on the AMOS22, KiTS23 and ACDC plans (pass line: at most $0.85\times$ on each; the largest is $0.656\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B1.passline\endcsname{Addendum AA3 (T2)}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B1.primary\endcsname{no}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B1.sentence\endcsname{the registered claim target T2 for LeanSep has no outcome yet (Addendum AA3 (T2): the profiled parameters at most $0.85\times$ the default's on every development plan, the profiled training step at most $0.85\times$ the default's on every development plan, the mean of the six benchmark contrasts at least $-0.50$\,pp and at least four of the six at least $-0.50$\,pp): 0 of the six benchmark contrasts have landed; AMOS22, KiTS23, ACDC, LiTS, BTCV and BraTS-MSD are still to come. The six contrasts are AMOS22 pending (0 of four folds), KiTS23 pending (0 of four folds), ACDC pending (0 of four folds), LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds). T2 is a registered claim target, not a transfer verdict; its mean and count over six benchmarks depart from the no-pooling clause of Addendum Q2-E, a departure Addendum AE registers, and every held-out dataset keeps its own reading beside it.}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B1.short\endcsname{pending (0 of six benchmarks landed)}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B1.six\endcsname{AMOS22 pending (0 of four folds), KiTS23 pending (0 of four folds), ACDC pending (0 of four folds), LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds)}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B1.state\endcsname{0 of the six benchmark contrasts have landed; AMOS22, KiTS23, ACDC, LiTS, BTCV and BraTS-MSD are still to come}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B1.stepline\endcsname{$0.779\times$ / $0.773\times$ / $0.785\times$ the default's profiled training step on the AMOS22, KiTS23 and ACDC plans (pass line: at most $0.85\times$ on each; the largest is $0.785\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B1.title\endcsname{smaller and faster, with accuracy not resolved as worse at the registered margin}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B2.arm\endcsname{LeanDil}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B2.k\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B2.kpos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B2.m\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B2.nlanded\endcsname{0}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B2.outcome\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B2.paramline\endcsname{$0.656\times$ / $0.655\times$ / $0.647\times$ the default's profiled parameters on the AMOS22, KiTS23 and ACDC plans (pass line: at most $0.85\times$ on each; the largest is $0.656\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B2.passline\endcsname{Addendum AA3 (T2)}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B2.primary\endcsname{no}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B2.sentence\endcsname{the registered claim target T2 for LeanDil has no outcome yet (Addendum AA3 (T2): the profiled parameters at most $0.85\times$ the default's on every development plan, the profiled training step at most $0.85\times$ the default's on every development plan, the mean of the six benchmark contrasts at least $-0.50$\,pp and at least four of the six at least $-0.50$\,pp): 0 of the six benchmark contrasts have landed; AMOS22, KiTS23, ACDC, LiTS, BTCV and BraTS-MSD are still to come. The six contrasts are AMOS22 pending (0 of four folds), KiTS23 pending (0 of four folds), ACDC pending (0 of four folds), LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds). T2 is a registered claim target, not a transfer verdict; its mean and count over six benchmarks depart from the no-pooling clause of Addendum Q2-E, a departure Addendum AE registers, and every held-out dataset keeps its own reading beside it.}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B2.short\endcsname{pending (0 of six benchmarks landed)}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B2.six\endcsname{AMOS22 pending (0 of four folds), KiTS23 pending (0 of four folds), ACDC pending (0 of four folds), LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds)}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B2.state\endcsname{0 of the six benchmark contrasts have landed; AMOS22, KiTS23, ACDC, LiTS, BTCV and BraTS-MSD are still to come}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B2.stepline\endcsname{$0.781\times$ / $0.762\times$ / $0.765\times$ the default's profiled training step on the AMOS22, KiTS23 and ACDC plans (pass line: at most $0.85\times$ on each; the largest is $0.781\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T2.V7B2.title\endcsname{smaller and faster, with accuracy not resolved as worse at the registered margin}
\expandafter\gdef\csname R@an.heldout.target.T2.V7C1.arm\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.heldout.target.T2.V7C1.k\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V7C1.kpos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V7C1.m\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V7C1.nlanded\endcsname{4}
\expandafter\gdef\csname R@an.heldout.target.T2.V7C1.outcome\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.target.T2.V7C1.paramline\endcsname{$0.677\times$ / $0.677\times$ / $0.669\times$ the default's profiled parameters on the AMOS22, KiTS23 and ACDC plans (pass line: at most $0.85\times$ on each; the largest is $0.677\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T2.V7C1.passline\endcsname{Addendum AA3 (T2)}
\expandafter\gdef\csname R@an.heldout.target.T2.V7C1.primary\endcsname{no}
\expandafter\gdef\csname R@an.heldout.target.T2.V7C1.sentence\endcsname{the registered claim target T2 for LeanNeXt-s5 has no outcome yet (Addendum AA3 (T2): the profiled parameters at most $0.85\times$ the default's on every development plan, the profiled training step at most $0.85\times$ the default's on every development plan, the mean of the six benchmark contrasts at least $-0.50$\,pp and at least four of the six at least $-0.50$\,pp): four of the six benchmark contrasts have landed; BTCV and BraTS-MSD are still to come. The six contrasts are AMOS22 \ensuremath{-0.46}\,pp, KiTS23 \ensuremath{+0.78}\,pp, ACDC \ensuremath{-0.19}\,pp, LiTS \ensuremath{+0.85}\,pp, BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds). T2 is a registered claim target, not a transfer verdict; its mean and count over six benchmarks depart from the no-pooling clause of Addendum Q2-E, a departure Addendum AE registers, and every held-out dataset keeps its own reading beside it.}
\expandafter\gdef\csname R@an.heldout.target.T2.V7C1.short\endcsname{pending (four of six benchmarks landed)}
\expandafter\gdef\csname R@an.heldout.target.T2.V7C1.six\endcsname{AMOS22 \ensuremath{-0.46}\,pp, KiTS23 \ensuremath{+0.78}\,pp, ACDC \ensuremath{-0.19}\,pp, LiTS \ensuremath{+0.85}\,pp, BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds)}
\expandafter\gdef\csname R@an.heldout.target.T2.V7C1.state\endcsname{four of the six benchmark contrasts have landed; BTCV and BraTS-MSD are still to come}
\expandafter\gdef\csname R@an.heldout.target.T2.V7C1.stepline\endcsname{$0.776\times$ / $0.771\times$ / $0.785\times$ the default's profiled training step on the AMOS22, KiTS23 and ACDC plans (pass line: at most $0.85\times$ on each; the largest is $0.785\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T2.V7C1.title\endcsname{smaller and faster, with accuracy not resolved as worse at the registered margin}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B1.arm\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B1.k\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B1.kpos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B1.m\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B1.nlanded\endcsname{0}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B1.outcome\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B1.paramline\endcsname{$0.585\times$ / $0.584\times$ / $0.574\times$ the default's profiled parameters on the AMOS22, KiTS23 and ACDC plans (pass line: at most $0.85\times$ on each; the largest is $0.585\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B1.passline\endcsname{Addendum AA3 (T2)}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B1.primary\endcsname{no}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B1.sentence\endcsname{the registered claim target T2 for LeanTrunk has no outcome yet (Addendum AA3 (T2): the profiled parameters at most $0.85\times$ the default's on every development plan, the profiled training step at most $0.85\times$ the default's on every development plan, the mean of the six benchmark contrasts at least $-0.50$\,pp and at least four of the six at least $-0.50$\,pp): 0 of the six benchmark contrasts have landed; AMOS22, KiTS23, ACDC, LiTS, BTCV and BraTS-MSD are still to come. The six contrasts are AMOS22 pending (the cross-validation runs are not registered yet), KiTS23 pending (the cross-validation runs are not registered yet), ACDC pending (the cross-validation runs are not registered yet), LiTS pending (the held-out runs are not registered yet), BTCV pending (the held-out runs are not registered yet), BraTS-MSD pending (the held-out runs are not registered yet). T2 is a registered claim target, not a transfer verdict; its mean and count over six benchmarks depart from the no-pooling clause of Addendum Q2-E, a departure Addendum AE registers, and every held-out dataset keeps its own reading beside it.}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B1.short\endcsname{pending (0 of six benchmarks landed)}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B1.six\endcsname{AMOS22 pending (the cross-validation runs are not registered yet), KiTS23 pending (the cross-validation runs are not registered yet), ACDC pending (the cross-validation runs are not registered yet), LiTS pending (the held-out runs are not registered yet), BTCV pending (the held-out runs are not registered yet), BraTS-MSD pending (the held-out runs are not registered yet)}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B1.state\endcsname{0 of the six benchmark contrasts have landed; AMOS22, KiTS23, ACDC, LiTS, BTCV and BraTS-MSD are still to come}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B1.stepline\endcsname{$0.615\times$ / $0.588\times$ / $0.624\times$ the default's profiled training step on the AMOS22, KiTS23 and ACDC plans (pass line: at most $0.85\times$ on each; the largest is $0.624\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B1.title\endcsname{smaller and faster, with accuracy not resolved as worse at the registered margin}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B2.arm\endcsname{Stem1}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B2.k\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B2.kpos\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B2.m\endcsname{\pend}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B2.nlanded\endcsname{1}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B2.outcome\endcsname{pending}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B2.paramline\endcsname{$0.677\times$ / $0.676\times$ / $0.669\times$ the default's profiled parameters on the AMOS22, KiTS23 and ACDC plans (pass line: at most $0.85\times$ on each; the largest is $0.677\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B2.passline\endcsname{Addendum AA3 (T2)}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B2.primary\endcsname{no}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B2.sentence\endcsname{the registered claim target T2 for Stem1 has no outcome yet (Addendum AA3 (T2): the profiled parameters at most $0.85\times$ the default's on every development plan, the profiled training step at most $0.85\times$ the default's on every development plan, the mean of the six benchmark contrasts at least $-0.50$\,pp and at least four of the six at least $-0.50$\,pp): one of the six benchmark contrasts have landed; AMOS22, ACDC, LiTS, BTCV and BraTS-MSD are still to come. The six contrasts are AMOS22 pending (0 of four folds), KiTS23 \ensuremath{-0.24}\,pp, ACDC pending (0 of four folds), LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds). T2 is a registered claim target, not a transfer verdict; its mean and count over six benchmarks depart from the no-pooling clause of Addendum Q2-E, a departure Addendum AE registers, and every held-out dataset keeps its own reading beside it.}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B2.short\endcsname{pending (one of six benchmarks landed)}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B2.six\endcsname{AMOS22 pending (0 of four folds), KiTS23 \ensuremath{-0.24}\,pp, ACDC pending (0 of four folds), LiTS pending (0 of three seeds), BTCV pending (0 of three seeds), BraTS-MSD pending (0 of three seeds)}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B2.state\endcsname{one of the six benchmark contrasts have landed; AMOS22, ACDC, LiTS, BTCV and BraTS-MSD are still to come}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B2.stepline\endcsname{$0.672\times$ / $0.629\times$ / $0.683\times$ the default's profiled training step on the AMOS22, KiTS23 and ACDC plans (pass line: at most $0.85\times$ on each; the largest is $0.683\times$): met}
\expandafter\gdef\csname R@an.heldout.target.T2.V8B2.title\endcsname{smaller and faster, with accuracy not resolved as worse at the registered margin}
\expandafter\gdef\csname R@an.heldout.target.asym.sentence\endcsname{The two target leads were designated after their fold-0 results were known: LeanDec after a seed-0 AMOS22 reading of \ensuremath{-0.36}\,pp that failed the clause of Addendum P6 (Addendum AB), and the T2 margin that admits it was fixed after that value was known. Later candidates must first read at or above the frozen default pool mean \ensuremath{-0.50}\,pp on both co-primaries at fold 0 (Addendum AD3), an admission gate neither lead faced, so the set of arms able to reach a met outcome is itself selected (Addendum AG3); LeanDec would pass that gate.}
\expandafter\gdef\csname R@an.heldout.target.chance.T1.familywise\endcsname{0.95}
\expandafter\gdef\csname R@an.heldout.target.chance.T1.n\endcsname{9}
\expandafter\gdef\csname R@an.heldout.target.chance.T1.q\endcsname{0.28}
\expandafter\gdef\csname R@an.heldout.target.chance.T1.q.exact\endcsname{0.344}
\expandafter\gdef\csname R@an.heldout.target.chance.T2.familywise\endcsname{0.999999999998}
\expandafter\gdef\csname R@an.heldout.target.chance.T2.n\endcsname{9}
\expandafter\gdef\csname R@an.heldout.target.chance.T2.q\endcsname{0.95}
\expandafter\gdef\csname R@an.heldout.target.chance.T2.q.loss03\endcsname{0.73}
\expandafter\gdef\csname R@an.heldout.target.defn.sentence\endcsname{Each target is a pass line fixed in advance for more than one candidate: nine candidates are registered for T1 (HyReX, LeanDec, LeanAdd-NeXt, HyReX-LeanDec, HyReX-k9, LeanDeepMid, LeanDeepMid+FD, CoarseStack and StackDec) and nine for T2 (HyReX, LeanDec, LeanAdd, LeanAdd-NeXt, LeanSep, LeanDil, LeanNeXt-s5, LeanTrunk and Stem1). By simulation with the study's own standard errors -- 2\,000\,000 draws of the six benchmark contrasts, independent and normal about zero on the scales this study measured (AMOS22 0.10, KiTS23 0.55, ACDC 0.07, LiTS 1.24, BTCV 0.25 and BraTS-MSD 1.00\,pp, of which BraTS-MSD is a labelled placeholder until its own runs land) -- an arm with no effect meets T1's accuracy clauses with probability 0.28, and at least one of the nine registered T1 candidates does so with probability $1-(1-0.28)^{9} = 0.95$. Its count clause alone is met with probability $22/64 = 0.344$ by any arm whose contrasts are independent and symmetric about zero, whatever those scales are, and adding the mean clause can only lower that. By the same simulation with the study's own standard errors, T2's two accuracy lines are met by an arm with no effect with probability 0.95, by an arm that truly loses 0.30\,pp on every benchmark with 0.73, and by at least one of its nine registered candidates with probability 0.999999999998. T2's accuracy margin, \ensuremath{-0.50}\,pp, equals this study's one-seed resolution floor and is not wider than it, so a met T2 reads: the cost lines are met and no benchmark-level point estimate shows a loss beyond that margin. It does not establish non-inferiority (Addendum AG2). A target outcome is therefore the reading of a pre-specified pass line and not by itself evidence of an effect; the evidence is the selection-free contrasts with their intervals.}
\expandafter\gdef\csname R@an.heldout.target.list\endcsname{T1 for HyReX, T2 for LeanDec, T2 for LeanAdd, T2 for LeanAdd-NeXt, T1 for HyReX-LeanDec, T1 for HyReX-k9, T1 for LeanDec, T2 for HyReX, T1 for LeanAdd-NeXt, T1 for LeanDeepMid, T1 for LeanDeepMid+FD, T2 for LeanSep, T2 for LeanDil, T2 for LeanNeXt-s5, T1 for CoarseStack, T1 for StackDec, T2 for LeanTrunk and T2 for Stem1}
\expandafter\gdef\csname R@an.heldout.target.n\endcsname{18}
\expandafter\gdef\csname R@an.heldout.target.nbench\endcsname{6}
\expandafter\gdef\csname R@an.heldout.target.nbench.word\endcsname{six}
\expandafter\gdef\csname R@an.heldout.word.no\endcsname{does not transfer}
\expandafter\gdef\csname R@an.heldout.word.yes\endcsname{transfers}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.clusterorder\endcsname{HyReX, ResEnc-M, ResEnc-matched, ConvNeXt-k3, ResEnc+context, HyReX+context}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L1.count\endcsname{56}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L1.denominator\endcsname{98}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L1.fraction\endcsname{57.1}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L1.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L1b.count\endcsname{53}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L1b.denominator\endcsname{98}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L1b.fraction\endcsname{54.1}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L1b.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L2.count\endcsname{38}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L2.denominator\endcsname{98}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L2.fraction\endcsname{38.8}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L2.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L3.count\endcsname{48}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L3.denominator\endcsname{98}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L3.fraction\endcsname{49.0}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L3.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L4.count\endcsname{54}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L4.denominator\endcsname{98}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L4.fraction\endcsname{55.1}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L4.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L6.count\endcsname{42}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L6.denominator\endcsname{98}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L6.fraction\endcsname{42.9}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.L6.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.count\endcsname{48}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.all.denominator\endcsname{98}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L1.count\endcsname{15}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L1.denominator\endcsname{32}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L1.fraction\endcsname{46.9}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L1.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L1b.count\endcsname{22}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L1b.denominator\endcsname{32}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L1b.fraction\endcsname{68.8}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L1b.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L2.count\endcsname{11}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L2.denominator\endcsname{32}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L2.fraction\endcsname{34.4}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L2.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L3.count\endcsname{16}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L3.denominator\endcsname{32}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L3.fraction\endcsname{50.0}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L3.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L4.count\endcsname{19}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L4.denominator\endcsname{32}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L4.fraction\endcsname{59.4}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L4.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L6.count\endcsname{10}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L6.denominator\endcsname{32}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L6.fraction\endcsname{31.2}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.L6.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.count\endcsname{16}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.large.denominator\endcsname{32}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L1.count\endcsname{22}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L1.denominator\endcsname{33}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L1.fraction\endcsname{66.7}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L1.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L1b.count\endcsname{18}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L1b.denominator\endcsname{33}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L1b.fraction\endcsname{54.5}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L1b.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L2.count\endcsname{13}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L2.denominator\endcsname{33}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L2.fraction\endcsname{39.4}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L2.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L3.count\endcsname{18}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L3.denominator\endcsname{33}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L3.fraction\endcsname{54.5}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L3.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L4.count\endcsname{19}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L4.denominator\endcsname{33}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L4.fraction\endcsname{57.6}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L4.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L6.count\endcsname{19}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L6.denominator\endcsname{33}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L6.fraction\endcsname{57.6}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.L6.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.count\endcsname{18}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.mid.denominator\endcsname{33}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L1.count\endcsname{19}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L1.denominator\endcsname{33}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L1.fraction\endcsname{57.6}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L1.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L1b.count\endcsname{13}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L1b.denominator\endcsname{33}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L1b.fraction\endcsname{39.4}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L1b.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L2.count\endcsname{14}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L2.denominator\endcsname{33}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L2.fraction\endcsname{42.4}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L2.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L3.count\endcsname{14}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L3.denominator\endcsname{33}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L3.fraction\endcsname{42.4}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L3.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L4.count\endcsname{16}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L4.denominator\endcsname{33}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L4.fraction\endcsname{48.5}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L4.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L6.count\endcsname{13}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L6.denominator\endcsname{33}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L6.fraction\endcsname{39.4}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.L6.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.count\endcsname{14}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.consistent_positive.small.denominator\endcsname{33}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.cut1.ml\endcsname{9.88}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.cut2.ml\endcsname{44.67}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.discovery.smallgain\endcsname{\ensuremath{+6.49}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.herorefunresolvedlist\endcsname{kidney region, large tumours}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.herorefworst\endcsname{\ensuremath{-6.42}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.herorefworst.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.herorefworstgroup\endcsname{small tumours}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.L1.freshminuss0\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.L1b.fresh_vsL1\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.L1b.freshminuss0\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.L1b.s0_vsL1\endcsname{\ensuremath{-0.86}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.L2.fresh_vsL1\endcsname{\ensuremath{-1.44}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.L2.freshminuss0\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.L2.s0_vsL1\endcsname{\ensuremath{-0.72}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.L3.fresh_vsL1\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.L3.freshminuss0\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.L3.s0_vsL1\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.L4.fresh_vsL1\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.L4.freshminuss0\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.L4.s0_vsL1\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.L6.fresh_vsL1\endcsname{\ensuremath{-0.55}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.L6.freshminuss0\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.L6.s0_vsL1\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.altshift\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.altshift.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.band1\endcsname{0.90}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.band2\endcsname{0.71}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.clearbandlist\endcsname{HyReX, ResEnc-M, ResEnc-matched, ResEnc+context}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.default\endcsname{96.02}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.n\endcsname{98}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.nclearband\endcsname{4}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.kidney.poolsd\endcsname{0.39}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.ksd\endcsname{2}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L1.freshminuss0\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L1b.fresh_vsL1\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L1b.freshminuss0\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L1b.s0_vsL1\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L1bfreshgain\endcsname{\ensuremath{+3.20}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L1bfreshgain.ci\endcsname{\ensuremath{[+0.97,\,+6.29]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L1bfreshgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L1bs0gain\endcsname{\ensuremath{+1.99}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L1bs0gain.ci\endcsname{\ensuremath{[+0.13,\,+4.24]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L1bs0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L1freshgain\endcsname{\ensuremath{+2.67}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L1freshgain.ci\endcsname{\ensuremath{[+0.25,\,+5.83]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L1freshgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L1s0gain\endcsname{\ensuremath{+2.16}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L1s0gain.ci\endcsname{\ensuremath{[-0.04,\,+5.17]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L1s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L2.fresh_vsL1\endcsname{\ensuremath{-2.35}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L2.freshminuss0\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L2.s0_vsL1\endcsname{\ensuremath{-2.69}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L2freshgain\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L2freshgain.ci\endcsname{\ensuremath{[-0.90,\,+1.58]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L2freshgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L2s0gain\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L2s0gain.ci\endcsname{\ensuremath{[-2.01,\,+0.96]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L2s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L3.fresh_vsL1\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L3.freshminuss0\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L3.s0_vsL1\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L3freshgain\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L3freshgain.ci\endcsname{\ensuremath{[+0.57,\,+5.25]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L3freshgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L3s0gain\endcsname{\ensuremath{+1.92}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L3s0gain.ci\endcsname{\ensuremath{[-0.11,\,+4.48]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L3s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L4.fresh_vsL1\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L4.freshminuss0\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L4.s0_vsL1\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L4freshgain\endcsname{\ensuremath{+3.23}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L4freshgain.ci\endcsname{\ensuremath{[+0.78,\,+6.31]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L4freshgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L4s0gain\endcsname{\ensuremath{+2.61}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L4s0gain.ci\endcsname{\ensuremath{[+0.39,\,+5.50]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L4s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L6.fresh_vsL1\endcsname{\ensuremath{-0.95}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L6.freshminuss0\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L6.s0_vsL1\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L6freshgain\endcsname{\ensuremath{+1.71}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L6freshgain.ci\endcsname{\ensuremath{[-0.13,\,+4.24]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L6freshgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L6s0gain\endcsname{\ensuremath{+2.13}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L6s0gain.ci\endcsname{\ensuremath{[+0.06,\,+4.96]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.L6s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.altshift\endcsname{\ensuremath{+0.95}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.altshift.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.band1\endcsname{0.80}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.band2\endcsname{0.63}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.clearbandlist\endcsname{HyReX, ResEnc-M, ResEnc-matched, ResEnc+context, HyReX+context}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.default\endcsname{82.15}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.n\endcsname{32}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.nclearband\endcsname{5}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.large.poolsd\endcsname{0.35}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.L1.freshminuss0\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.L1b.fresh_vsL1\endcsname{\ensuremath{-0.89}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.L1b.freshminuss0\endcsname{\ensuremath{+1.24}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.L1b.s0_vsL1\endcsname{\ensuremath{-1.01}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.L2.fresh_vsL1\endcsname{\ensuremath{-3.54}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.L2.freshminuss0\endcsname{\ensuremath{-0.79}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.L2.s0_vsL1\endcsname{\ensuremath{-1.64}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.L3.fresh_vsL1\endcsname{\ensuremath{-1.13}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.L3.freshminuss0\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.L3.s0_vsL1\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.L4.fresh_vsL1\endcsname{\ensuremath{-1.41}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.L4.freshminuss0\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.L4.s0_vsL1\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.L6.fresh_vsL1\endcsname{\ensuremath{-2.42}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.L6.freshminuss0\endcsname{\ensuremath{-1.00}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.L6.s0_vsL1\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.altshift\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.altshift.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.band1\endcsname{2.49}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.band2\endcsname{1.97}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.clearbandlist\endcsname{HyReX, ResEnc-M, ResEnc-matched, ResEnc+context}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.default\endcsname{79.84}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.n\endcsname{98}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.nclearband\endcsname{4}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.masses.poolsd\endcsname{1.08}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L1.freshminuss0\endcsname{\ensuremath{+1.41}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L1b.fresh_vsL1\endcsname{\ensuremath{-2.53}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L1b.freshminuss0\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L1b.s0_vsL1\endcsname{\ensuremath{-1.79}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L1bfreshgain\endcsname{\ensuremath{+2.30}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L1bfreshgain.ci\endcsname{\ensuremath{[-0.46,\,+5.58]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L1bfreshgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L1bs0gain\endcsname{\ensuremath{+1.62}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L1bs0gain.ci\endcsname{\ensuremath{[-1.75,\,+5.32]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L1bs0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L1freshgain\endcsname{\ensuremath{+4.83}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L1freshgain.ci\endcsname{\ensuremath{[+2.04,\,+8.48]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L1freshgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L1s0gain\endcsname{\ensuremath{+3.42}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L1s0gain.ci\endcsname{\ensuremath{[-1.55,\,+8.87]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L1s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L2.fresh_vsL1\endcsname{\ensuremath{-5.19}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L2.freshminuss0\endcsname{\ensuremath{-1.01}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L2.s0_vsL1\endcsname{\ensuremath{-2.77}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L2freshgain\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L2freshgain.ci\endcsname{\ensuremath{[-4.02,\,+3.12]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L2freshgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L2s0gain\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L2s0gain.ci\endcsname{\ensuremath{[-1.72,\,+2.93]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L2s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L3.fresh_vsL1\endcsname{\ensuremath{-1.71}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L3.freshminuss0\endcsname{\ensuremath{-0.72}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L3.s0_vsL1\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L3freshgain\endcsname{\ensuremath{+3.12}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L3freshgain.ci\endcsname{\ensuremath{[+0.08,\,+7.33]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L3freshgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L3s0gain\endcsname{\ensuremath{+3.84}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L3s0gain.ci\endcsname{\ensuremath{[-1.20,\,+9.92]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L3s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L4.fresh_vsL1\endcsname{\ensuremath{-1.58}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L4.freshminuss0\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L4.s0_vsL1\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L4freshgain\endcsname{\ensuremath{+3.25}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L4freshgain.ci\endcsname{\ensuremath{[+0.59,\,+6.28]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L4freshgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L4s0gain\endcsname{\ensuremath{+3.16}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L4s0gain.ci\endcsname{\ensuremath{[+1.75,\,+4.83]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L4s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L6.fresh_vsL1\endcsname{\ensuremath{-2.14}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L6.freshminuss0\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L6.s0_vsL1\endcsname{\ensuremath{-0.99}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L6freshgain\endcsname{\ensuremath{+2.68}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L6freshgain.ci\endcsname{\ensuremath{[-1.11,\,+6.81]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L6freshgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L6s0gain\endcsname{\ensuremath{+2.43}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L6s0gain.ci\endcsname{\ensuremath{[-1.99,\,+8.08]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.L6s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.altshift\endcsname{\ensuremath{+1.39}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.altshift.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.band1\endcsname{1.58}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.band2\endcsname{1.25}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.clearbandlist\endcsname{HyReX, ResEnc-M, ResEnc-matched, ResEnc+context, HyReX+context}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.default\endcsname{77.97}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.n\endcsname{33}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.nclearband\endcsname{5}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.mid.poolsd\endcsname{0.68}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.narms\endcsname{6}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.nboot\endcsname{10000}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.ngroups\endcsname{6}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.nheroaboveref\endcsname{0}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.nherobelowref\endcsname{6}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.nherogroups\endcsname{6}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.nherorefunresolved\endcsname{2}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.npending\endcsname{0}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.nreplicated\endcsname{6}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.nsmall\endcsname{33}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.ntotal\endcsname{98}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.pairfloor\endcsname{0.50}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.reference\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L1bgain\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L1bgain.ci\endcsname{\ensuremath{[+0.37,\,+1.57]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L1bgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L1bs0gain\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L1bs0gain.ci\endcsname{\ensuremath{[-0.65,\,+0.93]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L1bs0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L1gain\endcsname{\ensuremath{+1.19}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L1gain.ci\endcsname{\ensuremath{[+0.64,\,+1.84]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L1gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L1s0gain\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L1s0gain.ci\endcsname{\ensuremath{[+0.34,\,+1.92]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L1s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L2gain\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L2gain.ci\endcsname{\ensuremath{[-0.96,\,+0.38]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L2gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L2s0gain\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L2s0gain.ci\endcsname{\ensuremath{[-0.14,\,+1.03]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L2s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L3gain\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L3gain.ci\endcsname{\ensuremath{[+0.41,\,+1.57]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L3gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L3s0gain\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L3s0gain.ci\endcsname{\ensuremath{[+0.24,\,+1.82]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L3s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L4gain\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L4gain.ci\endcsname{\ensuremath{[+0.45,\,+1.41]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L4gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L4s0gain\endcsname{\ensuremath{+0.67}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L4s0gain.ci\endcsname{\ensuremath{[+0.15,\,+1.33]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L4s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L6gain\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L6gain.ci\endcsname{\ensuremath{[+0.16,\,+1.23]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L6gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L6s0gain\endcsname{\ensuremath{+0.95}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L6s0gain.ci\endcsname{\ensuremath{[+0.33,\,+1.73]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.kidney.L6s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L1bgain\endcsname{\ensuremath{+3.26}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L1bgain.ci\endcsname{\ensuremath{[+1.43,\,+5.35]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L1bgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L1bs0gain\endcsname{\ensuremath{+2.01}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L1bs0gain.ci\endcsname{\ensuremath{[+0.45,\,+3.70]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L1bs0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L1gain\endcsname{\ensuremath{+4.15}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L1gain.ci\endcsname{\ensuremath{[+2.23,\,+6.37]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L1gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L1s0gain\endcsname{\ensuremath{+3.03}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L1s0gain.ci\endcsname{\ensuremath{[+0.81,\,+5.49]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L1s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L2gain\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L2gain.ci\endcsname{\ensuremath{[-1.41,\,+2.68]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L2gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L2s0gain\endcsname{\ensuremath{+1.39}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L2s0gain.ci\endcsname{\ensuremath{[-1.06,\,+3.91]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L2s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L3gain\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L3gain.ci\endcsname{\ensuremath{[+1.22,\,+4.95]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L3gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L3s0gain\endcsname{\ensuremath{+3.49}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L3s0gain.ci\endcsname{\ensuremath{[+1.15,\,+6.02]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L3s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L4gain\endcsname{\ensuremath{+2.73}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L4gain.ci\endcsname{\ensuremath{[+1.20,\,+4.49]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L4gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L4s0gain\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L4s0gain.ci\endcsname{\ensuremath{[+1.13,\,+3.88]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L4s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L6gain\endcsname{\ensuremath{+1.72}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L6gain.ci\endcsname{\ensuremath{[-0.21,\,+3.67]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L6gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L6s0gain\endcsname{\ensuremath{+2.73}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L6s0gain.ci\endcsname{\ensuremath{[+0.71,\,+4.93]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.masses.L6s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L1bgain\endcsname{\ensuremath{+2.80}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L1bgain.ci\endcsname{\ensuremath{[+0.88,\,+4.75]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L1bgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L1bs0gain\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L1bs0gain.ci\endcsname{\ensuremath{[+1.05,\,+5.14]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L1bs0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L1gain\endcsname{\ensuremath{+5.09}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L1gain.ci\endcsname{\ensuremath{[+3.17,\,+7.23]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L1gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L1s0gain\endcsname{\ensuremath{+2.90}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L1s0gain.ci\endcsname{\ensuremath{[+0.41,\,+5.46]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L1s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L2gain\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L2gain.ci\endcsname{\ensuremath{[-2.20,\,+2.13]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L2gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L2s0gain\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L2s0gain.ci\endcsname{\ensuremath{[-1.90,\,+2.21]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L2s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L3gain\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L3gain.ci\endcsname{\ensuremath{[+0.17,\,+4.56]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L3gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L3s0gain\endcsname{\ensuremath{+4.11}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L3s0gain.ci\endcsname{\ensuremath{[+1.69,\,+6.88]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L3s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L4gain\endcsname{\ensuremath{+3.14}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L4gain.ci\endcsname{\ensuremath{[+1.09,\,+5.17]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L4gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L4s0gain\endcsname{\ensuremath{+3.50}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L4s0gain.ci\endcsname{\ensuremath{[+2.06,\,+5.02]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L4s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L6gain\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L6gain.ci\endcsname{\ensuremath{[+0.47,\,+4.37]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L6gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L6s0gain\endcsname{\ensuremath{+3.90}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L6s0gain.ci\endcsname{\ensuremath{[+1.58,\,+6.50]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.region.tumour.L6s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.resolved.L1.ngroups\endcsname{6}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.resolved.L1.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.resolved.L1b.ngroups\endcsname{5}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.resolved.L1b.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.resolved.L2.ngroups\endcsname{0}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.resolved.L2.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.resolved.L3.ngroups\endcsname{5}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.resolved.L3.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.resolved.L4.ngroups\endcsname{5}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.resolved.L4.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.resolved.L6.ngroups\endcsname{3}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.resolved.L6.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.resolved.nowhere.count\endcsname{1}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.resolved.nowhere.list\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L1.freshminuss0\endcsname{\ensuremath{+4.61}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L1b.fresh_vsL1\endcsname{\ensuremath{-4.79}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L1b.freshminuss0\endcsname{\ensuremath{-2.50}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L1b.s0_vsL1\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L1bfreshgain\endcsname{\ensuremath{+2.92}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L1bfreshgain.ci\endcsname{\ensuremath{[-1.27,\,+6.90]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L1bfreshgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L1bs0gain\endcsname{\ensuremath{+5.42}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L1bs0gain.ci\endcsname{\ensuremath{[+1.09,\,+10.15]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L1bs0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L1freshgain\endcsname{\ensuremath{+7.71}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L1freshgain.ci\endcsname{\ensuremath{[+3.71,\,+11.83]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L1freshgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L1s0gain\endcsname{\ensuremath{+3.10}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L1s0gain.ci\endcsname{\ensuremath{[-1.67,\,+7.94]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L1s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L2.fresh_vsL1\endcsname{\ensuremath{-7.72}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L2.freshminuss0\endcsname{\ensuremath{-0.67}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L2.s0_vsL1\endcsname{\ensuremath{-2.44}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L2freshgain\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L2freshgain.ci\endcsname{\ensuremath{[-5.20,\,+5.08]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L2freshgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L2s0gain\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L2s0gain.ci\endcsname{\ensuremath{[-5.04,\,+5.44]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L2s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L3.fresh_vsL1\endcsname{\ensuremath{-6.42}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L3.freshminuss0\endcsname{\ensuremath{-5.20}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L3.s0_vsL1\endcsname{\ensuremath{+3.39}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L3freshgain\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L3freshgain.ci\endcsname{\ensuremath{[-3.77,\,+5.98]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L3freshgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L3s0gain\endcsname{\ensuremath{+6.49}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L3s0gain.ci\endcsname{\ensuremath{[+1.93,\,+11.46]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L3s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L4.fresh_vsL1\endcsname{\ensuremath{-4.76}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L4.freshminuss0\endcsname{\ensuremath{-1.75}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L4.s0_vsL1\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L4freshgain\endcsname{\ensuremath{+2.95}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L4freshgain.ci\endcsname{\ensuremath{[-1.79,\,+7.61]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L4freshgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L4s0gain\endcsname{\ensuremath{+4.70}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L4s0gain.ci\endcsname{\ensuremath{[+1.51,\,+8.02]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L4s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L6.fresh_vsL1\endcsname{\ensuremath{-4.88}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L6.freshminuss0\endcsname{\ensuremath{-4.25}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L6.s0_vsL1\endcsname{\ensuremath{+3.98}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L6freshgain\endcsname{\ensuremath{+2.83}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L6freshgain.ci\endcsname{\ensuremath{[-0.90,\,+6.49]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L6freshgain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L6s0gain\endcsname{\ensuremath{+7.08}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L6s0gain.ci\endcsname{\ensuremath{[+2.96,\,+11.78]}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.L6s0gain.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.altshift\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.altshift.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.band1\endcsname{5.65}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.band2\endcsname{4.47}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.clearbandlist\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.default\endcsname{62.94}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.n\endcsname{33}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.nclearband\endcsname{1}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.small.poolsd\endcsname{2.45}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.smallL3minusL1\endcsname{\ensuremath{-6.42}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.L1.freshminuss0\endcsname{\ensuremath{+2.19}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.L1b.fresh_vsL1\endcsname{\ensuremath{-2.29}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.L1b.freshminuss0\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.L1b.s0_vsL1\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.L2.fresh_vsL1\endcsname{\ensuremath{-5.11}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.L2.freshminuss0\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.L2.s0_vsL1\endcsname{\ensuremath{-2.63}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.L3.fresh_vsL1\endcsname{\ensuremath{-2.76}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.L3.freshminuss0\endcsname{\ensuremath{-1.77}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.L3.s0_vsL1\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.L4.fresh_vsL1\endcsname{\ensuremath{-1.95}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.L4.freshminuss0\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.L4.s0_vsL1\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.L6.fresh_vsL1\endcsname{\ensuremath{-2.68}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.L6.freshminuss0\endcsname{\ensuremath{-1.48}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.L6.s0_vsL1\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.altshift\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.altshift.status\endcsname{complete}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.band1\endcsname{2.46}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.band2\endcsname{1.94}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.clearbandlist\endcsname{HyReX, ResEnc-M, ResEnc-matched, ResEnc+context, HyReX+context}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.default\endcsname{74.27}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.n\endcsname{98}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.nclearband\endcsname{5}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.tumour.poolsd\endcsname{1.06}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.widestband.group\endcsname{small tumours}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.widestband.margin\endcsname{3.16}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.widestband.runnerup\endcsname{masses}
\expandafter\gdef\csname R@an.kits_fresh_anatomy.widestband.value\endcsname{5.65}
\expandafter\gdef\csname R@an.l4_replication.kits.L1b.delta_vsdefault\endcsname{+2.313}
\expandafter\gdef\csname R@an.l4_replication.kits.L1b.freshmean\endcsname{85.691}
\expandafter\gdef\csname R@an.l4_replication.kits.L1b.seed1\endcsname{85.942}
\expandafter\gdef\csname R@an.l4_replication.kits.L1b.seed2\endcsname{85.441}
\expandafter\gdef\csname R@an.l4_replication.kits.L4.delta_vsdefault\endcsname{+2.246}
\expandafter\gdef\csname R@an.l4_replication.kits.L4.freshmean\endcsname{85.625}
\expandafter\gdef\csname R@an.l4_replication.kits.L4.seed1\endcsname{86.055}
\expandafter\gdef\csname R@an.l4_replication.kits.L4.seed2\endcsname{85.194}
\expandafter\gdef\csname R@an.l4_replication.kits.defaultmean\endcsname{83.378}
\expandafter\gdef\csname R@an.l4_replication.kits.freshL4minusL1b\endcsname{-0.067}
\expandafter\gdef\csname R@an.l4_replication.kits.paired.seed1\endcsname{+0.113}
\expandafter\gdef\csname R@an.l4_replication.kits.paired.seed2\endcsname{-0.247}
\expandafter\gdef\csname R@an.l4_replication.verdict\endcsname{PENDING}
\expandafter\gdef\csname R@an.lineage.agent.n\endcsname{28}
\expandafter\gdef\csname R@an.lineage.arm.C1.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.C1.delta.amos\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.lineage.arm.C1.delta.kits\endcsname{\ensuremath{+2.40}}
\expandafter\gdef\csname R@an.lineage.arm.C1.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.C1.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.C1.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.C1.name\endcsname{HyReX + decoder capacity}
\expandafter\gdef\csname R@an.lineage.arm.C1.params.acdc\endcsname{1.698}
\expandafter\gdef\csname R@an.lineage.arm.C1.params.amos\endcsname{1.682}
\expandafter\gdef\csname R@an.lineage.arm.C1.params.kits\endcsname{1.680}
\expandafter\gdef\csname R@an.lineage.arm.C1.parent\endcsname{L3}
\expandafter\gdef\csname R@an.lineage.arm.C1.parent_short\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.arm.C1.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.C1.short\endcsname{HyReX+dec. capacity}
\expandafter\gdef\csname R@an.lineage.arm.C1.state\endcsname{replicated}
\expandafter\gdef\csname R@an.lineage.arm.C1.step.acdc\endcsname{1.804}
\expandafter\gdef\csname R@an.lineage.arm.C1.step.amos\endcsname{1.693}
\expandafter\gdef\csname R@an.lineage.arm.C1.step.kits\endcsname{1.580}
\expandafter\gdef\csname R@an.lineage.arm.C1.tag\endcsname{C1\_deccap}
\expandafter\gdef\csname R@an.lineage.arm.C1.wave\endcsname{4}
\expandafter\gdef\csname R@an.lineage.arm.D1.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.D1.delta.amos\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.lineage.arm.D1.delta.kits\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.lineage.arm.D1.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.D1.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.D1.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.D1.name\endcsname{HyReX point-fuse decoder}
\expandafter\gdef\csname R@an.lineage.arm.D1.params.acdc\endcsname{0.662}
\expandafter\gdef\csname R@an.lineage.arm.D1.params.amos\endcsname{0.670}
\expandafter\gdef\csname R@an.lineage.arm.D1.params.kits\endcsname{0.671}
\expandafter\gdef\csname R@an.lineage.arm.D1.parent\endcsname{L3}
\expandafter\gdef\csname R@an.lineage.arm.D1.parent_short\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.arm.D1.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.D1.short\endcsname{HyReX point-fuse}
\expandafter\gdef\csname R@an.lineage.arm.D1.state\endcsname{replicated}
\expandafter\gdef\csname R@an.lineage.arm.D1.step.acdc\endcsname{1.634}
\expandafter\gdef\csname R@an.lineage.arm.D1.step.amos\endcsname{1.520}
\expandafter\gdef\csname R@an.lineage.arm.D1.step.kits\endcsname{1.401}
\expandafter\gdef\csname R@an.lineage.arm.D1.tag\endcsname{D1\_pointfuse}
\expandafter\gdef\csname R@an.lineage.arm.D1.wave\endcsname{4}
\expandafter\gdef\csname R@an.lineage.arm.D2.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.D2.delta.amos\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.lineage.arm.D2.delta.kits\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.lineage.arm.D2.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.D2.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.D2.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.D2.name\endcsname{LeanDec (default with one conv per decoder stage)}
\expandafter\gdef\csname R@an.lineage.arm.D2.params.acdc\endcsname{0.832}
\expandafter\gdef\csname R@an.lineage.arm.D2.params.amos\endcsname{0.836}
\expandafter\gdef\csname R@an.lineage.arm.D2.params.kits\endcsname{0.836}
\expandafter\gdef\csname R@an.lineage.arm.D2.parent\endcsname{base}
\expandafter\gdef\csname R@an.lineage.arm.D2.parent_short\endcsname{default}
\expandafter\gdef\csname R@an.lineage.arm.D2.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.D2.short\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.arm.D2.state\endcsname{cross-validated}
\expandafter\gdef\csname R@an.lineage.arm.D2.step.acdc\endcsname{0.806}
\expandafter\gdef\csname R@an.lineage.arm.D2.step.amos\endcsname{0.812}
\expandafter\gdef\csname R@an.lineage.arm.D2.step.kits\endcsname{0.808}
\expandafter\gdef\csname R@an.lineage.arm.D2.tag\endcsname{D2\_dec1}
\expandafter\gdef\csname R@an.lineage.arm.D2.wave\endcsname{4}
\expandafter\gdef\csname R@an.lineage.arm.I1.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.I1.delta.amos\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.lineage.arm.I1.delta.kits\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.lineage.arm.I1.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.I1.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.I1.delta_sf.kits\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.I1.name\endcsname{HyReX + pooled skip}
\expandafter\gdef\csname R@an.lineage.arm.I1.params.acdc\endcsname{0.950}
\expandafter\gdef\csname R@an.lineage.arm.I1.params.amos\endcsname{0.951}
\expandafter\gdef\csname R@an.lineage.arm.I1.params.kits\endcsname{0.951}
\expandafter\gdef\csname R@an.lineage.arm.I1.parent\endcsname{L3}
\expandafter\gdef\csname R@an.lineage.arm.I1.parent_short\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.arm.I1.role\endcsname{attribution}
\expandafter\gdef\csname R@an.lineage.arm.I1.short\endcsname{HyReX+pooled skip}
\expandafter\gdef\csname R@an.lineage.arm.I1.state\endcsname{screened}
\expandafter\gdef\csname R@an.lineage.arm.I1.step.acdc\endcsname{1.643}
\expandafter\gdef\csname R@an.lineage.arm.I1.step.amos\endcsname{1.535}
\expandafter\gdef\csname R@an.lineage.arm.I1.step.kits\endcsname{1.407}
\expandafter\gdef\csname R@an.lineage.arm.I1.tag\endcsname{I1\_L3pool}
\expandafter\gdef\csname R@an.lineage.arm.I1.wave\endcsname{4}
\expandafter\gdef\csname R@an.lineage.arm.L1.delta.acdc\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.lineage.arm.L1.delta.amos\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.lineage.arm.L1.delta.kits\endcsname{\ensuremath{+3.48}}
\expandafter\gdef\csname R@an.lineage.arm.L1.delta_sf.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.L1.delta_sf.amos\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.L1.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.L1.name\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.lineage.arm.L1.params.acdc\endcsname{3.342}
\expandafter\gdef\csname R@an.lineage.arm.L1.params.amos\endcsname{3.287}
\expandafter\gdef\csname R@an.lineage.arm.L1.params.kits\endcsname{3.280}
\expandafter\gdef\csname R@an.lineage.arm.L1.parent\endcsname{base}
\expandafter\gdef\csname R@an.lineage.arm.L1.parent_short\endcsname{default}
\expandafter\gdef\csname R@an.lineage.arm.L1.role\endcsname{reference}
\expandafter\gdef\csname R@an.lineage.arm.L1.short\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.lineage.arm.L1.state\endcsname{held-out}
\expandafter\gdef\csname R@an.lineage.arm.L1.step.acdc\endcsname{1.508}
\expandafter\gdef\csname R@an.lineage.arm.L1.step.amos\endcsname{1.462}
\expandafter\gdef\csname R@an.lineage.arm.L1.step.kits\endcsname{1.335}
\expandafter\gdef\csname R@an.lineage.arm.L1.tag\endcsname{L1}
\expandafter\gdef\csname R@an.lineage.arm.L1.wave\endcsname{1}
\expandafter\gdef\csname R@an.lineage.arm.L1b.delta.acdc\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.lineage.arm.L1b.delta.amos\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.lineage.arm.L1b.delta.kits\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.lineage.arm.L1b.delta_sf.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.L1b.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.L1b.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.L1b.name\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.lineage.arm.L1b.params.acdc\endcsname{3.345}
\expandafter\gdef\csname R@an.lineage.arm.L1b.params.amos\endcsname{3.290}
\expandafter\gdef\csname R@an.lineage.arm.L1b.params.kits\endcsname{3.283}
\expandafter\gdef\csname R@an.lineage.arm.L1b.parent\endcsname{L1}
\expandafter\gdef\csname R@an.lineage.arm.L1b.parent_short\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.lineage.arm.L1b.role\endcsname{control}
\expandafter\gdef\csname R@an.lineage.arm.L1b.short\endcsname{ResEnc-matched}
\expandafter\gdef\csname R@an.lineage.arm.L1b.state\endcsname{cross-validated}
\expandafter\gdef\csname R@an.lineage.arm.L1b.step.acdc\endcsname{1.409}
\expandafter\gdef\csname R@an.lineage.arm.L1b.step.amos\endcsname{1.380}
\expandafter\gdef\csname R@an.lineage.arm.L1b.step.kits\endcsname{1.227}
\expandafter\gdef\csname R@an.lineage.arm.L1b.tag\endcsname{L1b}
\expandafter\gdef\csname R@an.lineage.arm.L1b.wave\endcsname{1}
\expandafter\gdef\csname R@an.lineage.arm.L2.delta.acdc\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.lineage.arm.L2.delta.amos\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.lineage.arm.L2.delta.kits\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.lineage.arm.L2.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.L2.delta_sf.amos\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.L2.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.L2.name\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.lineage.arm.L2.params.acdc\endcsname{0.779}
\expandafter\gdef\csname R@an.lineage.arm.L2.params.amos\endcsname{0.785}
\expandafter\gdef\csname R@an.lineage.arm.L2.params.kits\endcsname{0.785}
\expandafter\gdef\csname R@an.lineage.arm.L2.parent\endcsname{base}
\expandafter\gdef\csname R@an.lineage.arm.L2.parent_short\endcsname{default}
\expandafter\gdef\csname R@an.lineage.arm.L2.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.L2.short\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.lineage.arm.L2.state\endcsname{replicated}
\expandafter\gdef\csname R@an.lineage.arm.L2.step.acdc\endcsname{1.502}
\expandafter\gdef\csname R@an.lineage.arm.L2.step.amos\endcsname{1.463}
\expandafter\gdef\csname R@an.lineage.arm.L2.step.kits\endcsname{1.330}
\expandafter\gdef\csname R@an.lineage.arm.L2.tag\endcsname{L2}
\expandafter\gdef\csname R@an.lineage.arm.L2.wave\endcsname{1}
\expandafter\gdef\csname R@an.lineage.arm.L3.delta.acdc\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.lineage.arm.L3.delta.amos\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.lineage.arm.L3.delta.kits\endcsname{\ensuremath{+2.09}}
\expandafter\gdef\csname R@an.lineage.arm.L3.delta_sf.acdc\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.L3.delta_sf.amos\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.L3.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.L3.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.arm.L3.params.acdc\endcsname{0.950}
\expandafter\gdef\csname R@an.lineage.arm.L3.params.amos\endcsname{0.951}
\expandafter\gdef\csname R@an.lineage.arm.L3.params.kits\endcsname{0.951}
\expandafter\gdef\csname R@an.lineage.arm.L3.parent\endcsname{base}
\expandafter\gdef\csname R@an.lineage.arm.L3.parent_short\endcsname{default}
\expandafter\gdef\csname R@an.lineage.arm.L3.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.L3.short\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.arm.L3.state\endcsname{held-out}
\expandafter\gdef\csname R@an.lineage.arm.L3.step.acdc\endcsname{1.642}
\expandafter\gdef\csname R@an.lineage.arm.L3.step.amos\endcsname{1.528}
\expandafter\gdef\csname R@an.lineage.arm.L3.step.kits\endcsname{1.401}
\expandafter\gdef\csname R@an.lineage.arm.L3.tag\endcsname{L3}
\expandafter\gdef\csname R@an.lineage.arm.L3.wave\endcsname{1}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.delta.amos\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.delta.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.delta_sf.kits\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.name\endcsname{HyReX-k3}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.params.acdc\endcsname{0.916}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.params.amos\endcsname{0.918}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.params.kits\endcsname{0.918}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.parent\endcsname{L3}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.parent_short\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.role\endcsname{attribution}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.short\endcsname{HyReX-k3}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.state\endcsname{screened}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.step.acdc\endcsname{1.384}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.step.amos\endcsname{1.346}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.step.kits\endcsname{1.273}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.tag\endcsname{L3k3}
\expandafter\gdef\csname R@an.lineage.arm.L3k3.wave\endcsname{3}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.delta.amos\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.delta.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.delta_sf.kits\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.name\endcsname{HyReX w/o GRN}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.params.acdc\endcsname{0.949}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.params.amos\endcsname{0.950}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.params.kits\endcsname{0.950}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.parent\endcsname{L3}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.parent_short\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.role\endcsname{attribution}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.short\endcsname{HyReX w/o GRN}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.state\endcsname{screened}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.step.acdc\endcsname{1.590}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.step.amos\endcsname{1.491}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.step.kits\endcsname{1.376}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.tag\endcsname{L3ng}
\expandafter\gdef\csname R@an.lineage.arm.L3ng.wave\endcsname{3}
\expandafter\gdef\csname R@an.lineage.arm.L4.delta.acdc\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.lineage.arm.L4.delta.amos\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.lineage.arm.L4.delta.kits\endcsname{\ensuremath{+2.25}}
\expandafter\gdef\csname R@an.lineage.arm.L4.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.L4.delta_sf.amos\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.L4.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.L4.name\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.lineage.arm.L4.params.acdc\endcsname{3.358}
\expandafter\gdef\csname R@an.lineage.arm.L4.params.amos\endcsname{3.302}
\expandafter\gdef\csname R@an.lineage.arm.L4.params.kits\endcsname{3.296}
\expandafter\gdef\csname R@an.lineage.arm.L4.parent\endcsname{L1b}
\expandafter\gdef\csname R@an.lineage.arm.L4.parent_short\endcsname{ResEnc-matched}
\expandafter\gdef\csname R@an.lineage.arm.L4.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.L4.short\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.lineage.arm.L4.state\endcsname{replicated}
\expandafter\gdef\csname R@an.lineage.arm.L4.step.acdc\endcsname{1.519}
\expandafter\gdef\csname R@an.lineage.arm.L4.step.amos\endcsname{1.459}
\expandafter\gdef\csname R@an.lineage.arm.L4.step.kits\endcsname{1.298}
\expandafter\gdef\csname R@an.lineage.arm.L4.tag\endcsname{L4}
\expandafter\gdef\csname R@an.lineage.arm.L4.wave\endcsname{1}
\expandafter\gdef\csname R@an.lineage.arm.L6.delta.acdc\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.lineage.arm.L6.delta.amos\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.lineage.arm.L6.delta.kits\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.lineage.arm.L6.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.L6.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.L6.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.L6.name\endcsname{HyReX+context}
\expandafter\gdef\csname R@an.lineage.arm.L6.params.acdc\endcsname{0.999}
\expandafter\gdef\csname R@an.lineage.arm.L6.params.amos\endcsname{0.999}
\expandafter\gdef\csname R@an.lineage.arm.L6.params.kits\endcsname{0.999}
\expandafter\gdef\csname R@an.lineage.arm.L6.parent\endcsname{L3}
\expandafter\gdef\csname R@an.lineage.arm.L6.parent_short\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.arm.L6.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.L6.short\endcsname{HyReX+context}
\expandafter\gdef\csname R@an.lineage.arm.L6.state\endcsname{replicated}
\expandafter\gdef\csname R@an.lineage.arm.L6.step.acdc\endcsname{2.031}
\expandafter\gdef\csname R@an.lineage.arm.L6.step.amos\endcsname{1.877}
\expandafter\gdef\csname R@an.lineage.arm.L6.step.kits\endcsname{1.634}
\expandafter\gdef\csname R@an.lineage.arm.L6.tag\endcsname{L6}
\expandafter\gdef\csname R@an.lineage.arm.L6.wave\endcsname{1}
\expandafter\gdef\csname R@an.lineage.arm.N1.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.N1.delta.amos\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@an.lineage.arm.N1.delta.kits\endcsname{\ensuremath{-6.49}}
\expandafter\gdef\csname R@an.lineage.arm.N1.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.N1.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.N1.delta_sf.kits\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.N1.name\endcsname{default + GroupNorm16}
\expandafter\gdef\csname R@an.lineage.arm.N1.params.acdc\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.arm.N1.params.amos\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.arm.N1.params.kits\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.arm.N1.parent\endcsname{base}
\expandafter\gdef\csname R@an.lineage.arm.N1.parent_short\endcsname{default}
\expandafter\gdef\csname R@an.lineage.arm.N1.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.N1.short\endcsname{default+GN16}
\expandafter\gdef\csname R@an.lineage.arm.N1.state\endcsname{screened}
\expandafter\gdef\csname R@an.lineage.arm.N1.step.acdc\endcsname{1.601}
\expandafter\gdef\csname R@an.lineage.arm.N1.step.amos\endcsname{2.059}
\expandafter\gdef\csname R@an.lineage.arm.N1.step.kits\endcsname{2.142}
\expandafter\gdef\csname R@an.lineage.arm.N1.tag\endcsname{N1\_gnw16}
\expandafter\gdef\csname R@an.lineage.arm.N1.wave\endcsname{4}
\expandafter\gdef\csname R@an.lineage.arm.P1.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.P1.delta.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.P1.delta.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.P1.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.P1.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.P1.delta_sf.kits\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.P1.name\endcsname{full-res addition}
\expandafter\gdef\csname R@an.lineage.arm.P1.params.acdc\endcsname{1.002}
\expandafter\gdef\csname R@an.lineage.arm.P1.params.amos\endcsname{1.003}
\expandafter\gdef\csname R@an.lineage.arm.P1.params.kits\endcsname{1.007}
\expandafter\gdef\csname R@an.lineage.arm.P1.parent\endcsname{base}
\expandafter\gdef\csname R@an.lineage.arm.P1.parent_short\endcsname{default}
\expandafter\gdef\csname R@an.lineage.arm.P1.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.P1.short\endcsname{full-res addition}
\expandafter\gdef\csname R@an.lineage.arm.P1.state\endcsname{registered}
\expandafter\gdef\csname R@an.lineage.arm.P1.step.acdc\endcsname{2.146}
\expandafter\gdef\csname R@an.lineage.arm.P1.step.amos\endcsname{2.145}
\expandafter\gdef\csname R@an.lineage.arm.P1.step.kits\endcsname{2.647}
\expandafter\gdef\csname R@an.lineage.arm.P1.tag\endcsname{P1\_frcap32}
\expandafter\gdef\csname R@an.lineage.arm.P1.wave\endcsname{3}
\expandafter\gdef\csname R@an.lineage.arm.P1b.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.P1b.delta.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.P1b.delta.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.P1b.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.P1b.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.P1b.delta_sf.kits\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.P1b.name\endcsname{full-res kernel $3^3$}
\expandafter\gdef\csname R@an.lineage.arm.P1b.params.acdc\endcsname{1.002}
\expandafter\gdef\csname R@an.lineage.arm.P1b.params.amos\endcsname{1.003}
\expandafter\gdef\csname R@an.lineage.arm.P1b.params.kits\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.arm.P1b.parent\endcsname{base}
\expandafter\gdef\csname R@an.lineage.arm.P1b.parent_short\endcsname{default}
\expandafter\gdef\csname R@an.lineage.arm.P1b.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.P1b.short\endcsname{full-res 3$^3$}
\expandafter\gdef\csname R@an.lineage.arm.P1b.state\endcsname{registered}
\expandafter\gdef\csname R@an.lineage.arm.P1b.step.acdc\endcsname{1.088}
\expandafter\gdef\csname R@an.lineage.arm.P1b.step.amos\endcsname{1.074}
\expandafter\gdef\csname R@an.lineage.arm.P1b.step.kits\endcsname{1.008}
\expandafter\gdef\csname R@an.lineage.arm.P1b.tag\endcsname{P1b\_kernel}
\expandafter\gdef\csname R@an.lineage.arm.P1b.wave\endcsname{3}
\expandafter\gdef\csname R@an.lineage.arm.P1c.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.P1c.delta.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.P1c.delta.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.P1c.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.P1c.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.P1c.delta_sf.kits\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.P1c.name\endcsname{coarse-capacity control (parameter-matched)}
\expandafter\gdef\csname R@an.lineage.arm.P1c.params.acdc\endcsname{1.014}
\expandafter\gdef\csname R@an.lineage.arm.P1c.params.amos\endcsname{1.014}
\expandafter\gdef\csname R@an.lineage.arm.P1c.params.kits\endcsname{1.014}
\expandafter\gdef\csname R@an.lineage.arm.P1c.parent\endcsname{base}
\expandafter\gdef\csname R@an.lineage.arm.P1c.parent_short\endcsname{default}
\expandafter\gdef\csname R@an.lineage.arm.P1c.role\endcsname{control}
\expandafter\gdef\csname R@an.lineage.arm.P1c.short\endcsname{coarse-capacity ctl}
\expandafter\gdef\csname R@an.lineage.arm.P1c.state\endcsname{registered}
\expandafter\gdef\csname R@an.lineage.arm.P1c.step.acdc\endcsname{1.019}
\expandafter\gdef\csname R@an.lineage.arm.P1c.step.amos\endcsname{1.018}
\expandafter\gdef\csname R@an.lineage.arm.P1c.step.kits\endcsname{1.007}
\expandafter\gdef\csname R@an.lineage.arm.P1c.tag\endcsname{P1c\_coarsecap}
\expandafter\gdef\csname R@an.lineage.arm.P1c.wave\endcsname{3}
\expandafter\gdef\csname R@an.lineage.arm.P3c.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.P3c.delta.amos\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.lineage.arm.P3c.delta.kits\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.lineage.arm.P3c.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.P3c.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.P3c.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.P3c.name\endcsname{function-identical control}
\expandafter\gdef\csname R@an.lineage.arm.P3c.params.acdc\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.arm.P3c.params.amos\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.arm.P3c.params.kits\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.arm.P3c.parent\endcsname{base}
\expandafter\gdef\csname R@an.lineage.arm.P3c.parent_short\endcsname{default}
\expandafter\gdef\csname R@an.lineage.arm.P3c.role\endcsname{control}
\expandafter\gdef\csname R@an.lineage.arm.P3c.short\endcsname{fn.-identical control}
\expandafter\gdef\csname R@an.lineage.arm.P3c.state\endcsname{cross-validated}
\expandafter\gdef\csname R@an.lineage.arm.P3c.step.acdc\endcsname{1.036}
\expandafter\gdef\csname R@an.lineage.arm.P3c.step.amos\endcsname{1.046}
\expandafter\gdef\csname R@an.lineage.arm.P3c.step.kits\endcsname{1.034}
\expandafter\gdef\csname R@an.lineage.arm.P3c.tag\endcsname{P3c}
\expandafter\gdef\csname R@an.lineage.arm.P3c.wave\endcsname{3}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.delta.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.delta.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.delta_sf.kits\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.name\endcsname{logit warp (head 0)}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.params.acdc\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.params.amos\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.params.kits\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.parent\endcsname{base}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.parent_short\endcsname{default}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.short\endcsname{logit warp}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.state\endcsname{registered}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.step.acdc\endcsname{1.029}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.step.amos\endcsname{1.048}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.step.kits\endcsname{1.032}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.tag\endcsname{P3lite}
\expandafter\gdef\csname R@an.lineage.arm.P3lite.wave\endcsname{3}
\expandafter\gdef\csname R@an.lineage.arm.S2.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.S2.delta.amos\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.lineage.arm.S2.delta.kits\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.lineage.arm.S2.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.S2.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.S2.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.S2.name\endcsname{HyReX, ConvNeXt one stage finer}
\expandafter\gdef\csname R@an.lineage.arm.S2.params.acdc\endcsname{0.888}
\expandafter\gdef\csname R@an.lineage.arm.S2.params.amos\endcsname{0.891}
\expandafter\gdef\csname R@an.lineage.arm.S2.params.kits\endcsname{0.891}
\expandafter\gdef\csname R@an.lineage.arm.S2.parent\endcsname{L3}
\expandafter\gdef\csname R@an.lineage.arm.S2.parent_short\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.arm.S2.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.S2.short\endcsname{HyReX, finer ConvNeXt}
\expandafter\gdef\csname R@an.lineage.arm.S2.state\endcsname{replicated}
\expandafter\gdef\csname R@an.lineage.arm.S2.step.acdc\endcsname{2.111}
\expandafter\gdef\csname R@an.lineage.arm.S2.step.amos\endcsname{1.961}
\expandafter\gdef\csname R@an.lineage.arm.S2.step.kits\endcsname{1.677}
\expandafter\gdef\csname R@an.lineage.arm.S2.tag\endcsname{S2\_s2next}
\expandafter\gdef\csname R@an.lineage.arm.S2.wave\endcsname{4}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.delta.amos\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.delta.kits\endcsname{\ensuremath{+2.17}}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.name\endcsname{HyReX with LeanDec fine decoder stages}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.params.acdc\endcsname{0.946}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.params.amos\endcsname{0.947}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.params.kits\endcsname{0.946}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.parent\endcsname{L3}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.parent_short\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.short\endcsname{HyReX-LeanDec}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.state\endcsname{replicated}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.step.acdc\endcsname{1.494}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.step.amos\endcsname{1.393}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.step.kits\endcsname{1.235}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.tag\endcsname{V5A5}
\expandafter\gdef\csname R@an.lineage.arm.V5A5.wave\endcsname{5}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.delta.amos\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.delta.kits\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.name\endcsname{LeanDec with additive skips (LeanAdd)}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.params.acdc\endcsname{0.664}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.params.amos\endcsname{0.673}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.params.kits\endcsname{0.672}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.parent\endcsname{D2\_dec1}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.parent_short\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.short\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.state\endcsname{cross-validated}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.step.acdc\endcsname{0.719}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.step.amos\endcsname{0.740}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.step.kits\endcsname{0.727}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.tag\endcsname{V5B1}
\expandafter\gdef\csname R@an.lineage.arm.V5B1.wave\endcsname{5}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.delta.acdc\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.delta.amos\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.delta.kits\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.name\endcsname{LeanAdd with coarse large kernels (LeanAdd-NeXt)}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.params.acdc\endcsname{0.674}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.params.amos\endcsname{0.682}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.params.kits\endcsname{0.681}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.parent\endcsname{V5B1}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.parent_short\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.short\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.state\endcsname{cross-validated}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.step.acdc\endcsname{0.915}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.step.amos\endcsname{0.853}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.step.kits\endcsname{0.836}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.tag\endcsname{V5B2}
\expandafter\gdef\csname R@an.lineage.arm.V5B2.wave\endcsname{5}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.delta.acdc\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.delta.amos\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.delta.kits\endcsname{\ensuremath{+1.70}}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.name\endcsname{HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.params.acdc\endcsname{0.986}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.params.amos\endcsname{0.987}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.params.kits\endcsname{0.987}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.parent\endcsname{L3}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.parent_short\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.short\endcsname{HyReX-k9}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.state\endcsname{cross-validated}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.step.acdc\endcsname{1.811}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.step.amos\endcsname{1.630}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.step.kits\endcsname{1.490}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.tag\endcsname{V6A1r}
\expandafter\gdef\csname R@an.lineage.arm.V6A1r.wave\endcsname{6}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.delta.acdc\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.delta.amos\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.delta.kits\endcsname{\ensuremath{+2.66}}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.name\endcsname{LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid)}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.params.acdc\endcsname{0.996}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.params.amos\endcsname{0.996}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.params.kits\endcsname{0.995}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.parent\endcsname{V5B2}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.parent_short\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.short\endcsname{LeanDeepMid}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.state\endcsname{held-out}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.step.acdc\endcsname{1.069}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.step.amos\endcsname{0.999}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.step.kits\endcsname{0.917}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.tag\endcsname{V7A1}
\expandafter\gdef\csname R@an.lineage.arm.V7A1.wave\endcsname{7}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.delta.acdc\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.delta.amos\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.delta.kits\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.name\endcsname{LeanDeepMid with the two finest decoder convolutions restored}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.params.acdc\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.params.amos\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.params.kits\endcsname{0.999}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.parent\endcsname{V7A1}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.parent_short\endcsname{LeanDeepMid}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.short\endcsname{LeanDeepMid+FD}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.state\endcsname{cross-validated}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.step.acdc\endcsname{1.227}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.step.amos\endcsname{1.147}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.step.kits\endcsname{1.092}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.tag\endcsname{V7A2}
\expandafter\gdef\csname R@an.lineage.arm.V7A2.wave\endcsname{7}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.delta.amos\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.delta.kits\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.delta_sf.kits\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.name\endcsname{LeanAdd-NeXt with every decoder second convolution restored}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.params.acdc\endcsname{0.842}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.params.amos\endcsname{0.846}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.params.kits\endcsname{0.846}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.parent\endcsname{V5B2}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.parent_short\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.role\endcsname{attribution}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.short\endcsname{LeanFullDec}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.state\endcsname{screened}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.step.acdc\endcsname{1.102}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.step.amos\endcsname{1.033}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.step.kits\endcsname{1.018}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.tag\endcsname{V7A3}
\expandafter\gdef\csname R@an.lineage.arm.V7A3.wave\endcsname{7}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.delta.amos\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.delta.kits\endcsname{\ensuremath{+2.38}}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.name\endcsname{LeanAdd-NeXt with separable coarse kernels (LeanSep)}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.params.acdc\endcsname{0.647}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.params.amos\endcsname{0.656}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.params.kits\endcsname{0.655}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.parent\endcsname{V5B2}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.parent_short\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.short\endcsname{LeanSep}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.state\endcsname{replicated}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.step.acdc\endcsname{0.785}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.step.amos\endcsname{0.779}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.step.kits\endcsname{0.773}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.tag\endcsname{V7B1}
\expandafter\gdef\csname R@an.lineage.arm.V7B1.wave\endcsname{7}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.delta.amos\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.delta.kits\endcsname{\ensuremath{+1.84}}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.name\endcsname{LeanAdd-NeXt with dilated coarse kernels (LeanDil)}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.params.acdc\endcsname{0.647}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.params.amos\endcsname{0.656}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.params.kits\endcsname{0.655}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.parent\endcsname{V5B2}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.parent_short\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.short\endcsname{LeanDil}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.state\endcsname{replicated}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.step.acdc\endcsname{0.765}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.step.amos\endcsname{0.781}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.step.kits\endcsname{0.762}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.tag\endcsname{V7B2}
\expandafter\gdef\csname R@an.lineage.arm.V7B2.wave\endcsname{7}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.delta.acdc\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.delta.amos\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.delta.kits\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.name\endcsname{LeanAdd-NeXt with the coarse operator at stage 5 only}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.params.acdc\endcsname{0.669}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.params.amos\endcsname{0.677}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.params.kits\endcsname{0.677}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.parent\endcsname{V5B2}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.parent_short\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.short\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.state\endcsname{held-out}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.step.acdc\endcsname{0.785}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.step.amos\endcsname{0.776}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.step.kits\endcsname{0.771}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.tag\endcsname{V7C1}
\expandafter\gdef\csname R@an.lineage.arm.V7C1.wave\endcsname{7}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.delta.amos\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.delta.kits\endcsname{\ensuremath{+2.00}}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.delta_sf.kits\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.name\endcsname{LeanAdd-NeXt with 3-tap coarse kernels (extent control)}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.params.acdc\endcsname{0.647}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.params.amos\endcsname{0.656}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.params.kits\endcsname{0.655}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.parent\endcsname{V5B2}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.parent_short\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.role\endcsname{attribution}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.short\endcsname{LeanNeXt-k3}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.state\endcsname{screened}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.step.acdc\endcsname{0.775}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.step.amos\endcsname{0.772}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.step.kits\endcsname{0.764}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.tag\endcsname{V7C2}
\expandafter\gdef\csname R@an.lineage.arm.V7C2.wave\endcsname{7}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.delta.amos\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.delta.kits\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.name\endcsname{LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack)}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.params.acdc\endcsname{1.005}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.params.amos\endcsname{1.005}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.params.kits\endcsname{1.004}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.parent\endcsname{V7C1}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.parent_short\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.short\endcsname{CoarseStack}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.state\endcsname{replicated}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.step.acdc\endcsname{0.997}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.step.amos\endcsname{0.895}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.step.kits\endcsname{0.912}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.tag\endcsname{V8A1}
\expandafter\gdef\csname R@an.lineage.arm.V8A1.wave\endcsname{8}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.delta.amos\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.delta.kits\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.name\endcsname{LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec)}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.params.acdc\endcsname{1.010}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.params.amos\endcsname{1.010}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.params.kits\endcsname{1.009}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.parent\endcsname{V7C1}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.parent_short\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.short\endcsname{StackDec}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.state\endcsname{replicated}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.step.acdc\endcsname{0.920}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.step.amos\endcsname{0.858}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.step.kits\endcsname{0.854}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.tag\endcsname{V8A2}
\expandafter\gdef\csname R@an.lineage.arm.V8A2.wave\endcsname{8}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.delta.amos\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.delta.kits\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.name\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk)}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.params.acdc\endcsname{0.574}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.params.amos\endcsname{0.585}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.params.kits\endcsname{0.584}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.parent\endcsname{V7C1}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.parent_short\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.short\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.state\endcsname{replicated}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.step.acdc\endcsname{0.624}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.step.amos\endcsname{0.615}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.step.kits\endcsname{0.588}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.tag\endcsname{V8B1}
\expandafter\gdef\csname R@an.lineage.arm.V8B1.wave\endcsname{8}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.delta.amos\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.delta.kits\endcsname{\ensuremath{+1.73}}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.name\endcsname{LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1)}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.params.acdc\endcsname{0.669}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.params.amos\endcsname{0.677}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.params.kits\endcsname{0.676}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.parent\endcsname{V7C1}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.parent_short\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.short\endcsname{Stem1}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.state\endcsname{cross-validated}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.step.acdc\endcsname{0.683}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.step.amos\endcsname{0.672}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.step.kits\endcsname{0.629}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.tag\endcsname{V8B2}
\expandafter\gdef\csname R@an.lineage.arm.V8B2.wave\endcsname{8}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.delta.amos\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.delta.kits\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.delta_sf.kits\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.name\endcsname{LeanNeXt-s5 narrowed to the parameter count of LeanTrunk (parameter control)}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.params.acdc\endcsname{0.579}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.params.amos\endcsname{0.585}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.params.kits\endcsname{0.585}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.parent\endcsname{V7C1}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.parent_short\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.role\endcsname{attribution}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.short\endcsname{NarrowTrunk}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.state\endcsname{screened}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.step.acdc\endcsname{0.777}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.step.amos\endcsname{0.774}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.step.kits\endcsname{0.767}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.tag\endcsname{V8X1}
\expandafter\gdef\csname R@an.lineage.arm.V8X1.wave\endcsname{8}
\expandafter\gdef\csname R@an.lineage.arm.W1.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.W1.delta.amos\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.lineage.arm.W1.delta.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.W1.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W1.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W1.delta_sf.kits\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W1.name\endcsname{$z$-dilation mixing}
\expandafter\gdef\csname R@an.lineage.arm.W1.params.acdc\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.arm.W1.params.amos\endcsname{1.001}
\expandafter\gdef\csname R@an.lineage.arm.W1.params.kits\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.arm.W1.parent\endcsname{W1c}
\expandafter\gdef\csname R@an.lineage.arm.W1.parent_short\endcsname{branch control}
\expandafter\gdef\csname R@an.lineage.arm.W1.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.W1.short\endcsname{z-dilation mixing}
\expandafter\gdef\csname R@an.lineage.arm.W1.state\endcsname{screened}
\expandafter\gdef\csname R@an.lineage.arm.W1.step.acdc\endcsname{1.149}
\expandafter\gdef\csname R@an.lineage.arm.W1.step.amos\endcsname{1.142}
\expandafter\gdef\csname R@an.lineage.arm.W1.step.kits\endcsname{1.124}
\expandafter\gdef\csname R@an.lineage.arm.W1.tag\endcsname{W1}
\expandafter\gdef\csname R@an.lineage.arm.W1.wave\endcsname{2}
\expandafter\gdef\csname R@an.lineage.arm.W1c.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.W1c.delta.amos\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.lineage.arm.W1c.delta.kits\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.lineage.arm.W1c.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W1c.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W1c.delta_sf.kits\endcsname{yes}
\expandafter\gdef\csname R@an.lineage.arm.W1c.name\endcsname{branch control}
\expandafter\gdef\csname R@an.lineage.arm.W1c.params.acdc\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.arm.W1c.params.amos\endcsname{1.001}
\expandafter\gdef\csname R@an.lineage.arm.W1c.params.kits\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.arm.W1c.parent\endcsname{base}
\expandafter\gdef\csname R@an.lineage.arm.W1c.parent_short\endcsname{default}
\expandafter\gdef\csname R@an.lineage.arm.W1c.role\endcsname{control}
\expandafter\gdef\csname R@an.lineage.arm.W1c.short\endcsname{branch control}
\expandafter\gdef\csname R@an.lineage.arm.W1c.state\endcsname{replicated}
\expandafter\gdef\csname R@an.lineage.arm.W1c.step.acdc\endcsname{1.154}
\expandafter\gdef\csname R@an.lineage.arm.W1c.step.amos\endcsname{1.145}
\expandafter\gdef\csname R@an.lineage.arm.W1c.step.kits\endcsname{1.131}
\expandafter\gdef\csname R@an.lineage.arm.W1c.tag\endcsname{W1c}
\expandafter\gdef\csname R@an.lineage.arm.W1c.wave\endcsname{2}
\expandafter\gdef\csname R@an.lineage.arm.W2.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.W2.delta.amos\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.lineage.arm.W2.delta.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.W2.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W2.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W2.delta_sf.kits\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W2.name\endcsname{thickness-gated mixing}
\expandafter\gdef\csname R@an.lineage.arm.W2.params.acdc\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.arm.W2.params.amos\endcsname{1.001}
\expandafter\gdef\csname R@an.lineage.arm.W2.params.kits\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.arm.W2.parent\endcsname{W1}
\expandafter\gdef\csname R@an.lineage.arm.W2.parent_short\endcsname{z-dilation mixing}
\expandafter\gdef\csname R@an.lineage.arm.W2.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.W2.short\endcsname{thickness-gated}
\expandafter\gdef\csname R@an.lineage.arm.W2.state\endcsname{screened}
\expandafter\gdef\csname R@an.lineage.arm.W2.step.acdc\endcsname{1.163}
\expandafter\gdef\csname R@an.lineage.arm.W2.step.amos\endcsname{1.151}
\expandafter\gdef\csname R@an.lineage.arm.W2.step.kits\endcsname{1.132}
\expandafter\gdef\csname R@an.lineage.arm.W2.tag\endcsname{W2}
\expandafter\gdef\csname R@an.lineage.arm.W2.wave\endcsname{2}
\expandafter\gdef\csname R@an.lineage.arm.W3.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.W3.delta.amos\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.lineage.arm.W3.delta.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.W3.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W3.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W3.delta_sf.kits\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W3.name\endcsname{offset upsampling}
\expandafter\gdef\csname R@an.lineage.arm.W3.params.acdc\endcsname{0.973}
\expandafter\gdef\csname R@an.lineage.arm.W3.params.amos\endcsname{0.950}
\expandafter\gdef\csname R@an.lineage.arm.W3.params.kits\endcsname{0.950}
\expandafter\gdef\csname R@an.lineage.arm.W3.parent\endcsname{W3c}
\expandafter\gdef\csname R@an.lineage.arm.W3.parent_short\endcsname{trilinear control}
\expandafter\gdef\csname R@an.lineage.arm.W3.role\endcsname{agent}
\expandafter\gdef\csname R@an.lineage.arm.W3.short\endcsname{offset upsampling}
\expandafter\gdef\csname R@an.lineage.arm.W3.state\endcsname{screened}
\expandafter\gdef\csname R@an.lineage.arm.W3.step.acdc\endcsname{1.097}
\expandafter\gdef\csname R@an.lineage.arm.W3.step.amos\endcsname{1.083}
\expandafter\gdef\csname R@an.lineage.arm.W3.step.kits\endcsname{1.084}
\expandafter\gdef\csname R@an.lineage.arm.W3.tag\endcsname{W3}
\expandafter\gdef\csname R@an.lineage.arm.W3.wave\endcsname{2}
\expandafter\gdef\csname R@an.lineage.arm.W3c.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.W3c.delta.amos\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.lineage.arm.W3c.delta.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.W3c.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W3c.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W3c.delta_sf.kits\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W3c.name\endcsname{trilinear-decoder control}
\expandafter\gdef\csname R@an.lineage.arm.W3c.params.acdc\endcsname{0.972}
\expandafter\gdef\csname R@an.lineage.arm.W3c.params.amos\endcsname{0.949}
\expandafter\gdef\csname R@an.lineage.arm.W3c.params.kits\endcsname{0.949}
\expandafter\gdef\csname R@an.lineage.arm.W3c.parent\endcsname{base}
\expandafter\gdef\csname R@an.lineage.arm.W3c.parent_short\endcsname{default}
\expandafter\gdef\csname R@an.lineage.arm.W3c.role\endcsname{control}
\expandafter\gdef\csname R@an.lineage.arm.W3c.short\endcsname{trilinear control}
\expandafter\gdef\csname R@an.lineage.arm.W3c.state\endcsname{screened}
\expandafter\gdef\csname R@an.lineage.arm.W3c.step.acdc\endcsname{1.094}
\expandafter\gdef\csname R@an.lineage.arm.W3c.step.amos\endcsname{1.070}
\expandafter\gdef\csname R@an.lineage.arm.W3c.step.kits\endcsname{1.059}
\expandafter\gdef\csname R@an.lineage.arm.W3c.tag\endcsname{W3c}
\expandafter\gdef\csname R@an.lineage.arm.W3c.wave\endcsname{2}
\expandafter\gdef\csname R@an.lineage.arm.W4.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.W4.delta.amos\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.lineage.arm.W4.delta.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.W4.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W4.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W4.delta_sf.kits\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W4.name\endcsname{ConvNeXt-4$\times$-GRN (MedNeXt-like reference)}
\expandafter\gdef\csname R@an.lineage.arm.W4.params.acdc\endcsname{1.102}
\expandafter\gdef\csname R@an.lineage.arm.W4.params.amos\endcsname{1.100}
\expandafter\gdef\csname R@an.lineage.arm.W4.params.kits\endcsname{1.099}
\expandafter\gdef\csname R@an.lineage.arm.W4.parent\endcsname{base}
\expandafter\gdef\csname R@an.lineage.arm.W4.parent_short\endcsname{default}
\expandafter\gdef\csname R@an.lineage.arm.W4.role\endcsname{reference}
\expandafter\gdef\csname R@an.lineage.arm.W4.short\endcsname{MedNeXt-like}
\expandafter\gdef\csname R@an.lineage.arm.W4.state\endcsname{screened}
\expandafter\gdef\csname R@an.lineage.arm.W4.step.acdc\endcsname{3.837}
\expandafter\gdef\csname R@an.lineage.arm.W4.step.amos\endcsname{3.513}
\expandafter\gdef\csname R@an.lineage.arm.W4.step.kits\endcsname{2.624}
\expandafter\gdef\csname R@an.lineage.arm.W4.tag\endcsname{W4}
\expandafter\gdef\csname R@an.lineage.arm.W4.wave\endcsname{2}
\expandafter\gdef\csname R@an.lineage.arm.W5.delta.acdc\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.W5.delta.amos\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.lineage.arm.W5.delta.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.arm.W5.delta_sf.acdc\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W5.delta_sf.amos\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W5.delta_sf.kits\endcsname{no}
\expandafter\gdef\csname R@an.lineage.arm.W5.name\endcsname{pooled-skip control}
\expandafter\gdef\csname R@an.lineage.arm.W5.params.acdc\endcsname{3.345}
\expandafter\gdef\csname R@an.lineage.arm.W5.params.amos\endcsname{3.290}
\expandafter\gdef\csname R@an.lineage.arm.W5.params.kits\endcsname{3.283}
\expandafter\gdef\csname R@an.lineage.arm.W5.parent\endcsname{L1b}
\expandafter\gdef\csname R@an.lineage.arm.W5.parent_short\endcsname{ResEnc-matched}
\expandafter\gdef\csname R@an.lineage.arm.W5.role\endcsname{control}
\expandafter\gdef\csname R@an.lineage.arm.W5.short\endcsname{pooled-skip control}
\expandafter\gdef\csname R@an.lineage.arm.W5.state\endcsname{screened}
\expandafter\gdef\csname R@an.lineage.arm.W5.step.acdc\endcsname{1.411}
\expandafter\gdef\csname R@an.lineage.arm.W5.step.amos\endcsname{1.373}
\expandafter\gdef\csname R@an.lineage.arm.W5.step.kits\endcsname{1.223}
\expandafter\gdef\csname R@an.lineage.arm.W5.tag\endcsname{W5}
\expandafter\gdef\csname R@an.lineage.arm.W5.wave\endcsname{2}
\expandafter\gdef\csname R@an.lineage.chain\endcsname{default $\to$ LeanDec $\to$ LeanAdd $\to$ LeanAdd-NeXt $\to$ LeanNeXt-s5 $\to$ NarrowTrunk}
\expandafter\gdef\csname R@an.lineage.chain.n\endcsname{6}
\expandafter\gdef\csname R@an.lineage.children.max\endcsname{13}
\expandafter\gdef\csname R@an.lineage.depth.arm\endcsname{V8X1}
\expandafter\gdef\csname R@an.lineage.depth.max\endcsname{5}
\expandafter\gdef\csname R@an.lineage.derived\endcsname{29}
\expandafter\gdef\csname R@an.lineage.derived.agent\endcsname{21}
\expandafter\gdef\csname R@an.lineage.derived.from_agent\endcsname{24}
\expandafter\gdef\csname R@an.lineage.derived.from_other\endcsname{5}
\expandafter\gdef\csname R@an.lineage.docs.n\endcsname{52}
\expandafter\gdef\csname R@an.lineage.edges\endcsname{42}
\expandafter\gdef\csname R@an.lineage.from_prev_wave\endcsname{7}
\expandafter\gdef\csname R@an.lineage.front.any.par.w1.amos\endcsname{88.083}
\expandafter\gdef\csname R@an.lineage.front.any.par.w1.best.at085\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w1.best.at085.name\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.lineage.front.any.par.w1.best.at1\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w1.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.front.any.par.w1.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.front.any.par.w1.kits\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w1.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.any.par.w1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.front.any.par.w1.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.any.par.w1.par\endcsname{0.951}
\expandafter\gdef\csname R@an.lineage.front.any.par.w1.step\endcsname{1.401}
\expandafter\gdef\csname R@an.lineage.front.any.par.w1.tag\endcsname{L3}
\expandafter\gdef\csname R@an.lineage.front.any.par.w1.tags\endcsname{HyReX, ConvNeXt-k3}
\expandafter\gdef\csname R@an.lineage.front.any.par.w2.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w2.best.at085\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w2.best.at085.name\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.lineage.front.any.par.w2.best.at1\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w2.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.front.any.par.w2.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w2.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w2.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.any.par.w2.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w2.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.front.any.par.w2.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w2.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w2.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w2.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w3.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w3.best.at085\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w3.best.at085.name\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.lineage.front.any.par.w3.best.at1\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w3.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.front.any.par.w3.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w3.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w3.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.any.par.w3.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w3.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.front.any.par.w3.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w3.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w3.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w3.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w4.amos\endcsname{88.091}
\expandafter\gdef\csname R@an.lineage.front.any.par.w4.best.at085\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w4.best.at085.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.front.any.par.w4.best.at1\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w4.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.front.any.par.w4.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.front.any.par.w4.kits\endcsname{\ensuremath{+3.51}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w4.n\endcsname{4}
\expandafter\gdef\csname R@an.lineage.front.any.par.w4.name\endcsname{HyReX+dec. capacity}
\expandafter\gdef\csname R@an.lineage.front.any.par.w4.new\endcsname{3}
\expandafter\gdef\csname R@an.lineage.front.any.par.w4.par\endcsname{1.680}
\expandafter\gdef\csname R@an.lineage.front.any.par.w4.step\endcsname{1.580}
\expandafter\gdef\csname R@an.lineage.front.any.par.w4.tag\endcsname{C1\_deccap}
\expandafter\gdef\csname R@an.lineage.front.any.par.w4.tags\endcsname{HyReX+dec. capacity, LeanDec, HyReX point-fuse}
\expandafter\gdef\csname R@an.lineage.front.any.par.w5.amos\endcsname{87.440}
\expandafter\gdef\csname R@an.lineage.front.any.par.w5.best.at085\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w5.best.at085.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.front.any.par.w5.best.at1\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w5.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.front.any.par.w5.guard\endcsname{not met}
\expandafter\gdef\csname R@an.lineage.front.any.par.w5.kits\endcsname{\ensuremath{+2.16}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w5.n\endcsname{5}
\expandafter\gdef\csname R@an.lineage.front.any.par.w5.name\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.lineage.front.any.par.w5.new\endcsname{1}
\expandafter\gdef\csname R@an.lineage.front.any.par.w5.par\endcsname{0.672}
\expandafter\gdef\csname R@an.lineage.front.any.par.w5.step\endcsname{0.727}
\expandafter\gdef\csname R@an.lineage.front.any.par.w5.tag\endcsname{V5B1}
\expandafter\gdef\csname R@an.lineage.front.any.par.w5.tags\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.lineage.front.any.par.w6.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w6.best.at085\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w6.best.at085.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.front.any.par.w6.best.at1\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w6.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.front.any.par.w6.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w6.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w6.n\endcsname{5}
\expandafter\gdef\csname R@an.lineage.front.any.par.w6.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w6.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.front.any.par.w6.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w6.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w6.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w6.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.par.w7.amos\endcsname{88.060}
\expandafter\gdef\csname R@an.lineage.front.any.par.w7.best.at085\endcsname{\ensuremath{+2.82}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w7.best.at085.name\endcsname{LeanDil}
\expandafter\gdef\csname R@an.lineage.front.any.par.w7.best.at1\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w7.best.at1.name\endcsname{LeanDeepMid+FD}
\expandafter\gdef\csname R@an.lineage.front.any.par.w7.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.front.any.par.w7.kits\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w7.n\endcsname{5}
\expandafter\gdef\csname R@an.lineage.front.any.par.w7.name\endcsname{LeanDeepMid+FD}
\expandafter\gdef\csname R@an.lineage.front.any.par.w7.new\endcsname{3}
\expandafter\gdef\csname R@an.lineage.front.any.par.w7.par\endcsname{0.999}
\expandafter\gdef\csname R@an.lineage.front.any.par.w7.step\endcsname{1.092}
\expandafter\gdef\csname R@an.lineage.front.any.par.w7.tag\endcsname{V7A2}
\expandafter\gdef\csname R@an.lineage.front.any.par.w7.tags\endcsname{LeanDeepMid+FD, LeanDil, LeanSep}
\expandafter\gdef\csname R@an.lineage.front.any.par.w8.amos\endcsname{86.950}
\expandafter\gdef\csname R@an.lineage.front.any.par.w8.best.at085\endcsname{\ensuremath{+2.91}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w8.best.at085.name\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.lineage.front.any.par.w8.best.at1\endcsname{\ensuremath{+2.91}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w8.best.at1.name\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.lineage.front.any.par.w8.guard\endcsname{not met}
\expandafter\gdef\csname R@an.lineage.front.any.par.w8.kits\endcsname{\ensuremath{+2.91}}
\expandafter\gdef\csname R@an.lineage.front.any.par.w8.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.any.par.w8.name\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.lineage.front.any.par.w8.new\endcsname{1}
\expandafter\gdef\csname R@an.lineage.front.any.par.w8.par\endcsname{0.584}
\expandafter\gdef\csname R@an.lineage.front.any.par.w8.step\endcsname{0.588}
\expandafter\gdef\csname R@an.lineage.front.any.par.w8.tag\endcsname{V8B1}
\expandafter\gdef\csname R@an.lineage.front.any.par.w8.tags\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.lineage.front.any.w1.amos\endcsname{88.083}
\expandafter\gdef\csname R@an.lineage.front.any.w1.best.at085\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w1.best.at085.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w1.best.at1\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w1.best.at1.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w1.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.front.any.w1.kits\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.lineage.front.any.w1.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.any.w1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.front.any.w1.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.any.w1.par\endcsname{0.951}
\expandafter\gdef\csname R@an.lineage.front.any.w1.step\endcsname{1.401}
\expandafter\gdef\csname R@an.lineage.front.any.w1.tag\endcsname{L3}
\expandafter\gdef\csname R@an.lineage.front.any.w1.tags\endcsname{HyReX, ResEnc+context}
\expandafter\gdef\csname R@an.lineage.front.any.w2.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w2.best.at085\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w2.best.at085.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w2.best.at1\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w2.best.at1.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w2.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w2.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w2.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.any.w2.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w2.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.front.any.w2.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w2.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w2.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w2.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w3.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w3.best.at085\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w3.best.at085.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w3.best.at1\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w3.best.at1.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w3.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w3.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w3.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.any.w3.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w3.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.front.any.w3.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w3.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w3.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w3.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w4.amos\endcsname{88.091}
\expandafter\gdef\csname R@an.lineage.front.any.w4.best.at085\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.lineage.front.any.w4.best.at085.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.front.any.w4.best.at1\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.lineage.front.any.w4.best.at1.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.front.any.w4.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.front.any.w4.kits\endcsname{\ensuremath{+3.51}}
\expandafter\gdef\csname R@an.lineage.front.any.w4.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.front.any.w4.name\endcsname{HyReX+dec. capacity}
\expandafter\gdef\csname R@an.lineage.front.any.w4.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.any.w4.par\endcsname{1.680}
\expandafter\gdef\csname R@an.lineage.front.any.w4.step\endcsname{1.580}
\expandafter\gdef\csname R@an.lineage.front.any.w4.tag\endcsname{C1\_deccap}
\expandafter\gdef\csname R@an.lineage.front.any.w4.tags\endcsname{HyReX+dec. capacity, LeanDec}
\expandafter\gdef\csname R@an.lineage.front.any.w5.amos\endcsname{87.440}
\expandafter\gdef\csname R@an.lineage.front.any.w5.best.at085\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.lineage.front.any.w5.best.at085.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.front.any.w5.best.at1\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.lineage.front.any.w5.best.at1.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.front.any.w5.guard\endcsname{not met}
\expandafter\gdef\csname R@an.lineage.front.any.w5.kits\endcsname{\ensuremath{+2.16}}
\expandafter\gdef\csname R@an.lineage.front.any.w5.n\endcsname{4}
\expandafter\gdef\csname R@an.lineage.front.any.w5.name\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.lineage.front.any.w5.new\endcsname{1}
\expandafter\gdef\csname R@an.lineage.front.any.w5.par\endcsname{0.672}
\expandafter\gdef\csname R@an.lineage.front.any.w5.step\endcsname{0.727}
\expandafter\gdef\csname R@an.lineage.front.any.w5.tag\endcsname{V5B1}
\expandafter\gdef\csname R@an.lineage.front.any.w5.tags\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.lineage.front.any.w6.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w6.best.at085\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.lineage.front.any.w6.best.at085.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.front.any.w6.best.at1\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.lineage.front.any.w6.best.at1.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.front.any.w6.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w6.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w6.n\endcsname{4}
\expandafter\gdef\csname R@an.lineage.front.any.w6.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w6.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.front.any.w6.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w6.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w6.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w6.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.any.w7.amos\endcsname{88.060}
\expandafter\gdef\csname R@an.lineage.front.any.w7.best.at085\endcsname{\ensuremath{+2.82}}
\expandafter\gdef\csname R@an.lineage.front.any.w7.best.at085.name\endcsname{LeanDil}
\expandafter\gdef\csname R@an.lineage.front.any.w7.best.at1\endcsname{\ensuremath{+2.82}}
\expandafter\gdef\csname R@an.lineage.front.any.w7.best.at1.name\endcsname{LeanDil}
\expandafter\gdef\csname R@an.lineage.front.any.w7.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.front.any.w7.kits\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.lineage.front.any.w7.n\endcsname{4}
\expandafter\gdef\csname R@an.lineage.front.any.w7.name\endcsname{LeanDeepMid+FD}
\expandafter\gdef\csname R@an.lineage.front.any.w7.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.any.w7.par\endcsname{0.999}
\expandafter\gdef\csname R@an.lineage.front.any.w7.step\endcsname{1.092}
\expandafter\gdef\csname R@an.lineage.front.any.w7.tag\endcsname{V7A2}
\expandafter\gdef\csname R@an.lineage.front.any.w7.tags\endcsname{LeanDeepMid+FD, LeanDil}
\expandafter\gdef\csname R@an.lineage.front.any.w8.amos\endcsname{86.950}
\expandafter\gdef\csname R@an.lineage.front.any.w8.best.at085\endcsname{\ensuremath{+2.91}}
\expandafter\gdef\csname R@an.lineage.front.any.w8.best.at085.name\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.lineage.front.any.w8.best.at1\endcsname{\ensuremath{+2.91}}
\expandafter\gdef\csname R@an.lineage.front.any.w8.best.at1.name\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.lineage.front.any.w8.guard\endcsname{not met}
\expandafter\gdef\csname R@an.lineage.front.any.w8.kits\endcsname{\ensuremath{+2.91}}
\expandafter\gdef\csname R@an.lineage.front.any.w8.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.any.w8.name\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.lineage.front.any.w8.new\endcsname{1}
\expandafter\gdef\csname R@an.lineage.front.any.w8.par\endcsname{0.584}
\expandafter\gdef\csname R@an.lineage.front.any.w8.step\endcsname{0.588}
\expandafter\gdef\csname R@an.lineage.front.any.w8.tag\endcsname{V8B1}
\expandafter\gdef\csname R@an.lineage.front.any.w8.tags\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.lineage.front.foot\endcsname{A cross on a grey point marks a design whose AMOS22 seed-0 Dice is below 87.551 (the frozen pool mean minus 0.15 points): LeanDec, default+GN16, LeanAdd, LeanFullDec, LeanSep, LeanDil, LeanNeXt-k3, CoarseStack, StackDec, LeanTrunk, Stem1, NarrowTrunk.}
\expandafter\gdef\csname R@an.lineage.front.guard.breach.names\endcsname{LeanDec, default+GN16, LeanAdd, LeanSep, LeanDil, CoarseStack, StackDec, LeanTrunk, Stem1}
\expandafter\gdef\csname R@an.lineage.front.guard.breach.tags\endcsname{D2\_dec1, N1\_gnw16, V5B1, V7B1, V7B2, V8A1, V8A2, V8B1, V8B2}
\expandafter\gdef\csname R@an.lineage.front.guard.line\endcsname{87.551}
\expandafter\gdef\csname R@an.lineage.front.guard.n_breach\endcsname{9}
\expandafter\gdef\csname R@an.lineage.front.guard.n_met\endcsname{13}
\expandafter\gdef\csname R@an.lineage.front.guard.n_pending\endcsname{0}
\expandafter\gdef\csname R@an.lineage.front.guard.pp\endcsname{-0.15}
\expandafter\gdef\csname R@an.lineage.front.off\endcsname{Off the scale of the parameter panel, above 1.8$\times$ the default's parameters: ResEnc-M (3.28$\times$, arrow), ResEnc+context (3.30$\times$), ResEnc-matched (3.28$\times$).}
\expandafter\gdef\csname R@an.lineage.front.off.limit\endcsname{1.8}
\expandafter\gdef\csname R@an.lineage.front.off.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.front.par.w1.amos\endcsname{88.083}
\expandafter\gdef\csname R@an.lineage.front.par.w1.best.at085\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.lineage.front.par.w1.best.at085.name\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.lineage.front.par.w1.best.at1\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.lineage.front.par.w1.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.front.par.w1.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.front.par.w1.kits\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.lineage.front.par.w1.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.par.w1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.front.par.w1.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.par.w1.par\endcsname{0.951}
\expandafter\gdef\csname R@an.lineage.front.par.w1.step\endcsname{1.401}
\expandafter\gdef\csname R@an.lineage.front.par.w1.tag\endcsname{L3}
\expandafter\gdef\csname R@an.lineage.front.par.w1.tags\endcsname{HyReX, ConvNeXt-k3}
\expandafter\gdef\csname R@an.lineage.front.par.w2.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w2.best.at085\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.lineage.front.par.w2.best.at085.name\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.lineage.front.par.w2.best.at1\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.lineage.front.par.w2.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.front.par.w2.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w2.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w2.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.par.w2.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w2.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.front.par.w2.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w2.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w2.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w2.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w3.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w3.best.at085\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.lineage.front.par.w3.best.at085.name\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.lineage.front.par.w3.best.at1\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.lineage.front.par.w3.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.front.par.w3.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w3.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w3.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.par.w3.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w3.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.front.par.w3.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w3.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w3.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w3.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w4.amos\endcsname{88.091}
\expandafter\gdef\csname R@an.lineage.front.par.w4.best.at085\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.lineage.front.par.w4.best.at085.name\endcsname{HyReX point-fuse}
\expandafter\gdef\csname R@an.lineage.front.par.w4.best.at1\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.lineage.front.par.w4.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.front.par.w4.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.front.par.w4.kits\endcsname{\ensuremath{+3.51}}
\expandafter\gdef\csname R@an.lineage.front.par.w4.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.front.par.w4.name\endcsname{HyReX+dec. capacity}
\expandafter\gdef\csname R@an.lineage.front.par.w4.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.par.w4.par\endcsname{1.680}
\expandafter\gdef\csname R@an.lineage.front.par.w4.step\endcsname{1.580}
\expandafter\gdef\csname R@an.lineage.front.par.w4.tag\endcsname{C1\_deccap}
\expandafter\gdef\csname R@an.lineage.front.par.w4.tags\endcsname{HyReX+dec. capacity, HyReX point-fuse}
\expandafter\gdef\csname R@an.lineage.front.par.w5.amos\endcsname{87.742}
\expandafter\gdef\csname R@an.lineage.front.par.w5.best.at085\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.lineage.front.par.w5.best.at085.name\endcsname{HyReX point-fuse}
\expandafter\gdef\csname R@an.lineage.front.par.w5.best.at1\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.lineage.front.par.w5.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.front.par.w5.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.front.par.w5.kits\endcsname{\ensuremath{+1.95}}
\expandafter\gdef\csname R@an.lineage.front.par.w5.n\endcsname{4}
\expandafter\gdef\csname R@an.lineage.front.par.w5.name\endcsname{HyReX-LeanDec}
\expandafter\gdef\csname R@an.lineage.front.par.w5.new\endcsname{1}
\expandafter\gdef\csname R@an.lineage.front.par.w5.par\endcsname{0.946}
\expandafter\gdef\csname R@an.lineage.front.par.w5.step\endcsname{1.235}
\expandafter\gdef\csname R@an.lineage.front.par.w5.tag\endcsname{V5A5}
\expandafter\gdef\csname R@an.lineage.front.par.w5.tags\endcsname{HyReX-LeanDec}
\expandafter\gdef\csname R@an.lineage.front.par.w6.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w6.best.at085\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.lineage.front.par.w6.best.at085.name\endcsname{HyReX point-fuse}
\expandafter\gdef\csname R@an.lineage.front.par.w6.best.at1\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.lineage.front.par.w6.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.front.par.w6.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w6.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w6.n\endcsname{4}
\expandafter\gdef\csname R@an.lineage.front.par.w6.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w6.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.front.par.w6.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w6.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w6.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w6.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w7.amos\endcsname{88.060}
\expandafter\gdef\csname R@an.lineage.front.par.w7.best.at085\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.lineage.front.par.w7.best.at085.name\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.front.par.w7.best.at1\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.lineage.front.par.w7.best.at1.name\endcsname{LeanDeepMid+FD}
\expandafter\gdef\csname R@an.lineage.front.par.w7.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.front.par.w7.kits\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.lineage.front.par.w7.n\endcsname{5}
\expandafter\gdef\csname R@an.lineage.front.par.w7.name\endcsname{LeanDeepMid+FD}
\expandafter\gdef\csname R@an.lineage.front.par.w7.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.par.w7.par\endcsname{0.999}
\expandafter\gdef\csname R@an.lineage.front.par.w7.step\endcsname{1.092}
\expandafter\gdef\csname R@an.lineage.front.par.w7.tag\endcsname{V7A2}
\expandafter\gdef\csname R@an.lineage.front.par.w7.tags\endcsname{LeanDeepMid+FD, LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.front.par.w8.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w8.best.at085\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.lineage.front.par.w8.best.at085.name\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.front.par.w8.best.at1\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.lineage.front.par.w8.best.at1.name\endcsname{LeanDeepMid+FD}
\expandafter\gdef\csname R@an.lineage.front.par.w8.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w8.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w8.n\endcsname{5}
\expandafter\gdef\csname R@an.lineage.front.par.w8.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w8.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.front.par.w8.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w8.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w8.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.par.w8.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w1.amos\endcsname{88.083}
\expandafter\gdef\csname R@an.lineage.front.w1.best.at085\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w1.best.at085.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w1.best.at1\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w1.best.at1.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w1.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.front.w1.kits\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.lineage.front.w1.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.w1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.front.w1.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.w1.par\endcsname{0.951}
\expandafter\gdef\csname R@an.lineage.front.w1.step\endcsname{1.401}
\expandafter\gdef\csname R@an.lineage.front.w1.tag\endcsname{L3}
\expandafter\gdef\csname R@an.lineage.front.w1.tags\endcsname{HyReX, ResEnc+context}
\expandafter\gdef\csname R@an.lineage.front.w2.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w2.best.at085\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w2.best.at085.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w2.best.at1\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w2.best.at1.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w2.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w2.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w2.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.w2.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w2.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.front.w2.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w2.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w2.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w2.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w3.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w3.best.at085\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w3.best.at085.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w3.best.at1\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w3.best.at1.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w3.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w3.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w3.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.w3.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w3.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.front.w3.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w3.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w3.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w3.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w4.amos\endcsname{88.091}
\expandafter\gdef\csname R@an.lineage.front.w4.best.at085\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w4.best.at085.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w4.best.at1\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w4.best.at1.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w4.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.front.w4.kits\endcsname{\ensuremath{+3.51}}
\expandafter\gdef\csname R@an.lineage.front.w4.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.front.w4.name\endcsname{HyReX+dec. capacity}
\expandafter\gdef\csname R@an.lineage.front.w4.new\endcsname{1}
\expandafter\gdef\csname R@an.lineage.front.w4.par\endcsname{1.680}
\expandafter\gdef\csname R@an.lineage.front.w4.step\endcsname{1.580}
\expandafter\gdef\csname R@an.lineage.front.w4.tag\endcsname{C1\_deccap}
\expandafter\gdef\csname R@an.lineage.front.w4.tags\endcsname{HyReX+dec. capacity}
\expandafter\gdef\csname R@an.lineage.front.w5.amos\endcsname{87.742}
\expandafter\gdef\csname R@an.lineage.front.w5.best.at085\endcsname{\ensuremath{+1.26}}
\expandafter\gdef\csname R@an.lineage.front.w5.best.at085.name\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.front.w5.best.at1\endcsname{\ensuremath{+1.26}}
\expandafter\gdef\csname R@an.lineage.front.w5.best.at1.name\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.front.w5.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.front.w5.kits\endcsname{\ensuremath{+1.95}}
\expandafter\gdef\csname R@an.lineage.front.w5.n\endcsname{5}
\expandafter\gdef\csname R@an.lineage.front.w5.name\endcsname{HyReX-LeanDec}
\expandafter\gdef\csname R@an.lineage.front.w5.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.w5.par\endcsname{0.946}
\expandafter\gdef\csname R@an.lineage.front.w5.step\endcsname{1.235}
\expandafter\gdef\csname R@an.lineage.front.w5.tag\endcsname{V5A5}
\expandafter\gdef\csname R@an.lineage.front.w5.tags\endcsname{HyReX-LeanDec, LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.front.w6.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w6.best.at085\endcsname{\ensuremath{+1.26}}
\expandafter\gdef\csname R@an.lineage.front.w6.best.at085.name\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.front.w6.best.at1\endcsname{\ensuremath{+1.26}}
\expandafter\gdef\csname R@an.lineage.front.w6.best.at1.name\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.front.w6.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w6.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w6.n\endcsname{5}
\expandafter\gdef\csname R@an.lineage.front.w6.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w6.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.front.w6.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w6.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w6.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w6.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w7.amos\endcsname{88.060}
\expandafter\gdef\csname R@an.lineage.front.w7.best.at085\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.lineage.front.w7.best.at085.name\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.front.w7.best.at1\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.lineage.front.w7.best.at1.name\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.front.w7.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.front.w7.kits\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.lineage.front.w7.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.front.w7.name\endcsname{LeanDeepMid+FD}
\expandafter\gdef\csname R@an.lineage.front.w7.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.front.w7.par\endcsname{0.999}
\expandafter\gdef\csname R@an.lineage.front.w7.step\endcsname{1.092}
\expandafter\gdef\csname R@an.lineage.front.w7.tag\endcsname{V7A2}
\expandafter\gdef\csname R@an.lineage.front.w7.tags\endcsname{LeanDeepMid+FD, LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.front.w8.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w8.best.at085\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.lineage.front.w8.best.at085.name\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.front.w8.best.at1\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.lineage.front.w8.best.at1.name\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.front.w8.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w8.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w8.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.front.w8.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w8.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.front.w8.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w8.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w8.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.front.w8.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.lvl\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.lvl_w1\endcsname{2.031}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.lvl_w8\endcsname{1.811}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.move\endcsname{0.000}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.move_guard\endcsname{0.000}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.move_guard_x\endcsname{1.00}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.move_x\endcsname{1.00}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.sf_share\endcsname{17}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w1.minstep\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w1.minstep_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w1.minstep_guard\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w1.minstep_guard_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w1.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w2.minstep\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w2.minstep_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w2.minstep_guard\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w2.minstep_guard_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w2.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w3.minstep\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w3.minstep_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w3.minstep_guard\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w3.minstep_guard_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w3.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w4.minstep\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w4.minstep_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w4.minstep_guard\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w4.minstep_guard_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w4.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w5.minstep\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w5.minstep_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w5.minstep_guard\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w5.minstep_guard_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w5.n\endcsname{4}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w6.minstep\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w6.minstep_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w6.minstep_guard\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w6.minstep_guard_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w6.n\endcsname{4}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w7.minstep\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w7.minstep_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w7.minstep_guard\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w7.minstep_guard_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w7.n\endcsname{6}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w8.minstep\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w8.minstep_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w8.minstep_guard\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w8.minstep_guard_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.acdc.w8.n\endcsname{6}
\expandafter\gdef\csname R@an.lineage.frontier.amos.lvl\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.lineage.frontier.amos.lvl_w1\endcsname{1.459}
\expandafter\gdef\csname R@an.lineage.frontier.amos.lvl_w8\endcsname{1.459}
\expandafter\gdef\csname R@an.lineage.frontier.amos.move\endcsname{-0.147}
\expandafter\gdef\csname R@an.lineage.frontier.amos.move_guard\endcsname{-0.224}
\expandafter\gdef\csname R@an.lineage.frontier.amos.move_guard_x\endcsname{0.78}
\expandafter\gdef\csname R@an.lineage.frontier.amos.move_x\endcsname{0.85}
\expandafter\gdef\csname R@an.lineage.frontier.amos.sf_share\endcsname{11}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w1.minstep\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w1.minstep_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w1.minstep_guard\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w1.minstep_guard_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w1.n\endcsname{1}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w2.minstep\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w2.minstep_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w2.minstep_guard\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w2.minstep_guard_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w2.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w3.minstep\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w3.minstep_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w3.minstep_guard\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w3.minstep_guard_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w3.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w4.minstep\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w4.minstep_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w4.minstep_guard\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w4.minstep_guard_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w4.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w5.minstep\endcsname{0.853}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w5.minstep_arm\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w5.minstep_guard\endcsname{0.853}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w5.minstep_guard_arm\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w5.n\endcsname{4}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w6.minstep\endcsname{0.853}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w6.minstep_arm\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w6.minstep_guard\endcsname{0.853}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w6.minstep_guard_arm\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w6.n\endcsname{5}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w7.minstep\endcsname{0.853}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w7.minstep_arm\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w7.minstep_guard\endcsname{0.776}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w7.minstep_guard_arm\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w7.n\endcsname{7}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w8.minstep\endcsname{0.853}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w8.minstep_arm\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w8.minstep_guard\endcsname{0.776}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w8.minstep_guard_arm\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.frontier.amos.w8.n\endcsname{9}
\expandafter\gdef\csname R@an.lineage.frontier.kits.lvl\endcsname{\ensuremath{+2.25}}
\expandafter\gdef\csname R@an.lineage.frontier.kits.lvl_w1\endcsname{1.298}
\expandafter\gdef\csname R@an.lineage.frontier.kits.lvl_w8\endcsname{0.727}
\expandafter\gdef\csname R@an.lineage.frontier.kits.move\endcsname{-0.412}
\expandafter\gdef\csname R@an.lineage.frontier.kits.move_ag\endcsname{-0.229}
\expandafter\gdef\csname R@an.lineage.frontier.kits.move_guard\endcsname{-0.412}
\expandafter\gdef\csname R@an.lineage.frontier.kits.move_guard_x\endcsname{0.59}
\expandafter\gdef\csname R@an.lineage.frontier.kits.move_x\endcsname{0.59}
\expandafter\gdef\csname R@an.lineage.frontier.kits.sf_share\endcsname{100}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w1.minstep\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w1.minstep_ag\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w1.minstep_ag_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w1.minstep_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w1.minstep_guard\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w1.minstep_guard_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w1.n\endcsname{1}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w2.minstep\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w2.minstep_ag\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w2.minstep_ag_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w2.minstep_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w2.minstep_guard\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w2.minstep_guard_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w2.n\endcsname{1}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w3.minstep\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w3.minstep_ag\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w3.minstep_ag_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w3.minstep_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w3.minstep_guard\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w3.minstep_guard_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w3.n\endcsname{1}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w4.minstep\endcsname{0.808}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w4.minstep_ag\endcsname{1.000}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w4.minstep_ag_arm\endcsname{default}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w4.minstep_arm\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w4.minstep_guard\endcsname{0.808}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w4.minstep_guard_arm\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w4.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w5.minstep\endcsname{0.727}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w5.minstep_ag\endcsname{0.836}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w5.minstep_ag_arm\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w5.minstep_arm\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w5.minstep_guard\endcsname{0.727}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w5.minstep_guard_arm\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w5.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w6.minstep\endcsname{0.727}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w6.minstep_ag\endcsname{0.836}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w6.minstep_ag_arm\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w6.minstep_arm\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w6.minstep_guard\endcsname{0.727}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w6.minstep_guard_arm\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w6.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w7.minstep\endcsname{0.727}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w7.minstep_ag\endcsname{0.771}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w7.minstep_ag_arm\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w7.minstep_arm\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w7.minstep_guard\endcsname{0.727}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w7.minstep_guard_arm\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w7.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w8.minstep\endcsname{0.588}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w8.minstep_ag\endcsname{0.771}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w8.minstep_ag_arm\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w8.minstep_arm\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w8.minstep_guard\endcsname{0.588}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w8.minstep_guard_arm\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.lineage.frontier.kits.w8.n\endcsname{5}
\expandafter\gdef\csname R@an.lineage.guard.pp\endcsname{-0.15}
\expandafter\gdef\csname R@an.lineage.pred.n\endcsname{15}
\expandafter\gdef\csname R@an.lineage.pred.rows\endcsname{45}
\expandafter\gdef\csname R@an.lineage.pred.w1.n\endcsname{0}
\expandafter\gdef\csname R@an.lineage.pred.w2.n\endcsname{0}
\expandafter\gdef\csname R@an.lineage.pred.w3.n\endcsname{0}
\expandafter\gdef\csname R@an.lineage.pred.w4.n\endcsname{0}
\expandafter\gdef\csname R@an.lineage.pred.w5.bias\endcsname{\ensuremath{-11.7}}
\expandafter\gdef\csname R@an.lineage.pred.w5.max_abs\endcsname{25.7}
\expandafter\gdef\csname R@an.lineage.pred.w5.mean_abs\endcsname{12.6}
\expandafter\gdef\csname R@an.lineage.pred.w5.min_abs\endcsname{0.2}
\expandafter\gdef\csname R@an.lineage.pred.w5.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.pred.w5.n_cons\endcsname{2}
\expandafter\gdef\csname R@an.lineage.pred.w5.n_saving\endcsname{6}
\expandafter\gdef\csname R@an.lineage.pred.w5.rows\endcsname{9}
\expandafter\gdef\csname R@an.lineage.pred.w5.saving\endcsname{1.71}
\expandafter\gdef\csname R@an.lineage.pred.w6.n\endcsname{0}
\expandafter\gdef\csname R@an.lineage.pred.w7.bias\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.lineage.pred.w7.max_abs\endcsname{5.9}
\expandafter\gdef\csname R@an.lineage.pred.w7.mean_abs\endcsname{2.0}
\expandafter\gdef\csname R@an.lineage.pred.w7.min_abs\endcsname{0.3}
\expandafter\gdef\csname R@an.lineage.pred.w7.n\endcsname{7}
\expandafter\gdef\csname R@an.lineage.pred.w7.n_cons\endcsname{14}
\expandafter\gdef\csname R@an.lineage.pred.w7.n_saving\endcsname{14}
\expandafter\gdef\csname R@an.lineage.pred.w7.rows\endcsname{21}
\expandafter\gdef\csname R@an.lineage.pred.w7.saving\endcsname{0.94}
\expandafter\gdef\csname R@an.lineage.pred.w8.bias\endcsname{\ensuremath{+2.3}}
\expandafter\gdef\csname R@an.lineage.pred.w8.max_abs\endcsname{5.6}
\expandafter\gdef\csname R@an.lineage.pred.w8.mean_abs\endcsname{2.8}
\expandafter\gdef\csname R@an.lineage.pred.w8.min_abs\endcsname{0.5}
\expandafter\gdef\csname R@an.lineage.pred.w8.n\endcsname{5}
\expandafter\gdef\csname R@an.lineage.pred.w8.n_cons\endcsname{12}
\expandafter\gdef\csname R@an.lineage.pred.w8.n_saving\endcsname{14}
\expandafter\gdef\csname R@an.lineage.pred.w8.rows\endcsname{15}
\expandafter\gdef\csname R@an.lineage.pred.w8.saving\endcsname{0.94}
\expandafter\gdef\csname R@an.lineage.registry.generated\endcsname{2026-10-12 11:27:36}
\expandafter\gdef\csname R@an.lineage.roots\endcsname{13}
\expandafter\gdef\csname R@an.lineage.same_wave\endcsname{8}
\expandafter\gdef\csname R@an.lineage.sent.front\endcsname{On KiTS23, among the agent-designed networks with AMOS22 seed 0 inside the registered $-$0.15 pp guard and a step time at or below the default's, the best seed-0 (discovery) Dice difference is \ensuremath{+1.26} pp (LeanAdd-NeXt) from wave 5, then \ensuremath{+2.71} pp (LeanNeXt-s5) from wave 7, and no design qualifies before wave 5; the same designs hold at 0.85$\times$ the default's step time.}
\expandafter\gdef\csname R@an.lineage.sent.front.any\endcsname{On KiTS23, among the agent-designed networks with a step time at or below the default's, the best seed-0 (discovery) Dice difference is \ensuremath{+2.36} pp (LeanDec) from wave 4, then \ensuremath{+2.82} pp (LeanDil) from wave 7, then \ensuremath{+2.91} pp (LeanTrunk) from wave 8, and no design qualifies before wave 4; the same designs hold at 0.85$\times$ the default's step time.}
\expandafter\gdef\csname R@an.lineage.sent.front.plain\endcsname{On KiTS23, among the agent-designed networks whose AMOS22 Dice stays within 0.15 points of nnU-Net's at seed 0 and whose step time is at or below the default's, the best seed-0 (discovery) Dice difference is \ensuremath{+1.26} pp (LeanAdd-NeXt) from wave 5, then \ensuremath{+2.71} pp (LeanNeXt-s5) from wave 7, and no design qualifies before wave 5; the same designs hold at 0.85$\times$ the default's step time.}
\expandafter\gdef\csname R@an.lineage.sent.front.plain.cond\endcsname{whose AMOS22 Dice stays within 0.15 points of nnU-Net's at seed 0}
\expandafter\gdef\csname R@an.lineage.sent.frontier\endcsname{Smallest profiled step time as a multiple of the default's, among designs with a Dice difference of at least 0 on the named dataset (the default counts; KiTS23 designs also need AMOS22 seed 0 inside the registered $-$0.15 pp guard): KiTS23 1.00$\times$ after wave 1 and 0.77$\times$ after wave 8 (LeanNeXt-s5, fresh-seed mean); AMOS22 1.00$\times$ after wave 1 and 0.85$\times$ after wave 8 (LeanAdd-NeXt, seed-0 discovery value); ACDC 1.00$\times$ after wave 1 and 1.00$\times$ after wave 8 (the default).}
\expandafter\gdef\csname R@an.lineage.sent.frontier.any\endcsname{Smallest profiled step time as a multiple of the default's, among designs with a Dice difference of at least 0 (the default counts; no AMOS22 condition): KiTS23 1.00$\times$ after wave 1 and 0.59$\times$ after wave 8 (LeanTrunk, fresh-seed mean); AMOS22 1.00$\times$ after wave 1 and 0.85$\times$ after wave 8 (LeanAdd-NeXt, seed-0 discovery value); ACDC 1.00$\times$ after wave 1 and 1.00$\times$ after wave 8 (the default). Among designs not below the registered $-$0.15 pp guard on the named dataset: KiTS23 1.00$\times$ after wave 1 and 0.59$\times$ after wave 8 (LeanTrunk, fresh-seed mean); AMOS22 1.00$\times$ after wave 1 and 0.78$\times$ after wave 8 (LeanNeXt-s5, seed-0 discovery value); ACDC 1.00$\times$ after wave 1 and 1.00$\times$ after wave 8 (the default).}
\expandafter\gdef\csname R@an.lineage.sent.genealogy\endcsname{The team registered 42 designs over 8 waves; 29 descend from another registered arm and 13 from the nnU-Net default. The longest line has 5 steps (6 networks including the default: default $\to$ LeanDec $\to$ LeanAdd $\to$ LeanAdd-NeXt $\to$ LeanNeXt-s5 $\to$ NarrowTrunk). 38 designs have a seed-0 screen, 25 a fresh-seed pair, 12 at least one cross-validation run and 4 at least one held-out run.}
\expandafter\gdef\csname R@an.lineage.sent.loop.amos\endcsname{On AMOS22 fresh seeds exist for the designs of wave 1 only (4 designs): their fresh-seed mean differs from the seed-0 value by \ensuremath{-0.14} pp on average (range \ensuremath{-0.25} to \ensuremath{+0.03}), and all 4 of them lie inside the band of $\pm$0.30 pp that the seed noise of the frozen pool allows if a design has no effect}
\expandafter\gdef\csname R@an.lineage.sent.shrink\endcsname{Of the 32 arm-dataset pairs with a seed-0 value and a fresh-seed mean, 15 of 25 on KiTS23, 3 of 4 on AMOS22, 2 of 3 on ACDC are lower. Mean change from seed 0 to the fresh mean: \ensuremath{-0.29} pp on KiTS23 (25 pairs, range \ensuremath{-1.57} to \ensuremath{+1.15}); \ensuremath{-0.14} pp on AMOS22 (4 pairs, range \ensuremath{-0.25} to \ensuremath{+0.03}); \ensuremath{-0.07} pp on ACDC (3 pairs, range \ensuremath{-0.17} to \ensuremath{+0.04}).}
\expandafter\gdef\csname R@an.lineage.sent.stagecost.sentence\endcsname{The profile records locate the default's cost. Removing the second convolution of the two finest decoder stages cuts the profiled step time by 18.9, 21.0, 20.4 ms (13.5, 14.8, 16.5 \% of the default's) and 0.12, 0.12, 0.13 M parameters (0.39, 0.39, 0.42 \%) on the AMOS22, ACDC and KiTS23 plans; removing the second convolution at encoder stage 0 alone cuts 14.6, 14.5, 17.5 ms (10.4, 10.2, 14.2 \%) and 0.01, 0.01, 0.03 M parameters. On the AMOS22 operator bench one dense 3$\times$3$\times$3 convolution at each of encoder stages 3 and 4 holds 4\,534\,272 weights (14.6 \% of the default's parameters) and costs 1.70 ms (1.2 \% of its step).}
\expandafter\gdef\csname R@an.lineage.sent.stagecost.short\endcsname{The second convolution of the two finest decoder stages holds 0.4 \% of the default's parameters and 13.5 to 16.5 \% of its step time}
\expandafter\gdef\csname R@an.lineage.sent.steperr.sentence\endcsname{The ideators' step-time predictions differ from the profile records by a mean of 12.6 \% in wave 5 (3 designs, 9 cells, from 0.2 to 25.7 \%; 2 of the 9 cells predicted at or above the profiled step; the savings of the designs predicted below the default's step were over-predicted 1.7-fold (median)); 2.0 \% in wave 7 (7 designs, 21 cells, from 0.3 to 5.9 \%; 14 of the 21 cells predicted at or above the profiled step); 2.8 \% in wave 8 (5 designs, 15 cells, from 0.5 to 5.6 \%; 12 of the 15 cells predicted at or above the profiled step).}
\expandafter\gdef\csname R@an.lineage.sent.steperr.short\endcsname{Predicted step times differed from the profile by 12.6 \% (wave 5), 2.0 \% (wave 7) and 2.8 \% (wave 8) on average}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.hi\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.lo\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.mean\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.n_down\endcsname{2}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.w1.mean\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.w1.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.w2.mean\endcsname{none}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.w2.n\endcsname{0}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.w3.mean\endcsname{none}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.w3.n\endcsname{0}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.w4.mean\endcsname{none}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.w4.n\endcsname{0}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.w5.mean\endcsname{none}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.w5.n\endcsname{0}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.w6.mean\endcsname{none}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.w6.n\endcsname{0}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.w7.mean\endcsname{none}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.w7.n\endcsname{0}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.w8.mean\endcsname{none}
\expandafter\gdef\csname R@an.lineage.shrink.acdc.w8.n\endcsname{0}
\expandafter\gdef\csname R@an.lineage.shrink.amos.hi\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.lineage.shrink.amos.lo\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.lineage.shrink.amos.mean\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.lineage.shrink.amos.n\endcsname{4}
\expandafter\gdef\csname R@an.lineage.shrink.amos.n_down\endcsname{3}
\expandafter\gdef\csname R@an.lineage.shrink.amos.nwaves\endcsname{1}
\expandafter\gdef\csname R@an.lineage.shrink.amos.w1.mean\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.lineage.shrink.amos.w1.n\endcsname{4}
\expandafter\gdef\csname R@an.lineage.shrink.amos.w2.mean\endcsname{none}
\expandafter\gdef\csname R@an.lineage.shrink.amos.w2.n\endcsname{0}
\expandafter\gdef\csname R@an.lineage.shrink.amos.w3.mean\endcsname{none}
\expandafter\gdef\csname R@an.lineage.shrink.amos.w3.n\endcsname{0}
\expandafter\gdef\csname R@an.lineage.shrink.amos.w4.mean\endcsname{none}
\expandafter\gdef\csname R@an.lineage.shrink.amos.w4.n\endcsname{0}
\expandafter\gdef\csname R@an.lineage.shrink.amos.w5.mean\endcsname{none}
\expandafter\gdef\csname R@an.lineage.shrink.amos.w5.n\endcsname{0}
\expandafter\gdef\csname R@an.lineage.shrink.amos.w6.mean\endcsname{none}
\expandafter\gdef\csname R@an.lineage.shrink.amos.w6.n\endcsname{0}
\expandafter\gdef\csname R@an.lineage.shrink.amos.w7.mean\endcsname{none}
\expandafter\gdef\csname R@an.lineage.shrink.amos.w7.n\endcsname{0}
\expandafter\gdef\csname R@an.lineage.shrink.amos.w8.mean\endcsname{none}
\expandafter\gdef\csname R@an.lineage.shrink.amos.w8.n\endcsname{0}
\expandafter\gdef\csname R@an.lineage.shrink.amos.waves\endcsname{1}
\expandafter\gdef\csname R@an.lineage.shrink.kits.hi\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.lineage.shrink.kits.lo\endcsname{\ensuremath{-1.57}}
\expandafter\gdef\csname R@an.lineage.shrink.kits.mean\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.lineage.shrink.kits.n\endcsname{25}
\expandafter\gdef\csname R@an.lineage.shrink.kits.n_down\endcsname{15}
\expandafter\gdef\csname R@an.lineage.shrink.kits.w1.mean\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.lineage.shrink.kits.w1.n\endcsname{6}
\expandafter\gdef\csname R@an.lineage.shrink.kits.w2.mean\endcsname{\ensuremath{-1.57}}
\expandafter\gdef\csname R@an.lineage.shrink.kits.w2.n\endcsname{1}
\expandafter\gdef\csname R@an.lineage.shrink.kits.w3.mean\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.lineage.shrink.kits.w3.n\endcsname{1}
\expandafter\gdef\csname R@an.lineage.shrink.kits.w4.mean\endcsname{\ensuremath{-0.62}}
\expandafter\gdef\csname R@an.lineage.shrink.kits.w4.n\endcsname{4}
\expandafter\gdef\csname R@an.lineage.shrink.kits.w5.mean\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.lineage.shrink.kits.w5.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.shrink.kits.w6.mean\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.lineage.shrink.kits.w6.n\endcsname{1}
\expandafter\gdef\csname R@an.lineage.shrink.kits.w7.mean\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.lineage.shrink.kits.w7.n\endcsname{5}
\expandafter\gdef\csname R@an.lineage.shrink.kits.w8.mean\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.lineage.shrink.kits.w8.n\endcsname{4}
\expandafter\gdef\csname R@an.lineage.stagecost.coarse.ms\endcsname{1.70}
\expandafter\gdef\csname R@an.lineage.stagecost.coarse.mshare\endcsname{1.2}
\expandafter\gdef\csname R@an.lineage.stagecost.coarse.s3.c\endcsname{256}
\expandafter\gdef\csname R@an.lineage.stagecost.coarse.s3.ms\endcsname{1.07}
\expandafter\gdef\csname R@an.lineage.stagecost.coarse.s3.weights\endcsname{1\,769\,472}
\expandafter\gdef\csname R@an.lineage.stagecost.coarse.s4.c\endcsname{320}
\expandafter\gdef\csname R@an.lineage.stagecost.coarse.s4.ms\endcsname{0.63}
\expandafter\gdef\csname R@an.lineage.stagecost.coarse.s4.weights\endcsname{2\,764\,800}
\expandafter\gdef\csname R@an.lineage.stagecost.coarse.weights\endcsname{4\,534\,272}
\expandafter\gdef\csname R@an.lineage.stagecost.coarse.wshare\endcsname{14.6}
\expandafter\gdef\csname R@an.lineage.stagecost.dec_fine.ms.acdc\endcsname{21.0}
\expandafter\gdef\csname R@an.lineage.stagecost.dec_fine.ms.amos\endcsname{18.9}
\expandafter\gdef\csname R@an.lineage.stagecost.dec_fine.ms.kits\endcsname{20.4}
\expandafter\gdef\csname R@an.lineage.stagecost.dec_fine.params.acdc\endcsname{0.12}
\expandafter\gdef\csname R@an.lineage.stagecost.dec_fine.params.amos\endcsname{0.12}
\expandafter\gdef\csname R@an.lineage.stagecost.dec_fine.params.kits\endcsname{0.13}
\expandafter\gdef\csname R@an.lineage.stagecost.dec_fine.pshare.acdc\endcsname{0.39}
\expandafter\gdef\csname R@an.lineage.stagecost.dec_fine.pshare.amos\endcsname{0.39}
\expandafter\gdef\csname R@an.lineage.stagecost.dec_fine.pshare.kits\endcsname{0.42}
\expandafter\gdef\csname R@an.lineage.stagecost.dec_fine.pshare.max\endcsname{0.42}
\expandafter\gdef\csname R@an.lineage.stagecost.dec_fine.share.acdc\endcsname{14.8}
\expandafter\gdef\csname R@an.lineage.stagecost.dec_fine.share.amos\endcsname{13.5}
\expandafter\gdef\csname R@an.lineage.stagecost.dec_fine.share.kits\endcsname{16.5}
\expandafter\gdef\csname R@an.lineage.stagecost.dec_fine.share.max\endcsname{16.5}
\expandafter\gdef\csname R@an.lineage.stagecost.dec_fine.share.min\endcsname{13.5}
\expandafter\gdef\csname R@an.lineage.stagecost.enc0.ms.acdc\endcsname{14.5}
\expandafter\gdef\csname R@an.lineage.stagecost.enc0.ms.amos\endcsname{14.6}
\expandafter\gdef\csname R@an.lineage.stagecost.enc0.ms.kits\endcsname{17.5}
\expandafter\gdef\csname R@an.lineage.stagecost.enc0.params.acdc\endcsname{0.01}
\expandafter\gdef\csname R@an.lineage.stagecost.enc0.params.amos\endcsname{0.01}
\expandafter\gdef\csname R@an.lineage.stagecost.enc0.params.kits\endcsname{0.03}
\expandafter\gdef\csname R@an.lineage.stagecost.enc0.pshare.acdc\endcsname{0.03}
\expandafter\gdef\csname R@an.lineage.stagecost.enc0.pshare.amos\endcsname{0.03}
\expandafter\gdef\csname R@an.lineage.stagecost.enc0.pshare.kits\endcsname{0.10}
\expandafter\gdef\csname R@an.lineage.stagecost.enc0.pshare.max\endcsname{0.10}
\expandafter\gdef\csname R@an.lineage.stagecost.enc0.share.acdc\endcsname{10.2}
\expandafter\gdef\csname R@an.lineage.stagecost.enc0.share.amos\endcsname{10.4}
\expandafter\gdef\csname R@an.lineage.stagecost.enc0.share.kits\endcsname{14.2}
\expandafter\gdef\csname R@an.lineage.stagecost.enc0.share.max\endcsname{14.2}
\expandafter\gdef\csname R@an.lineage.stagecost.enc0.share.min\endcsname{10.2}
\expandafter\gdef\csname R@an.lineage.stagecost.enc014.ms.acdc\endcsname{22.9}
\expandafter\gdef\csname R@an.lineage.stagecost.enc014.ms.amos\endcsname{22.5}
\expandafter\gdef\csname R@an.lineage.stagecost.enc014.ms.kits\endcsname{22.6}
\expandafter\gdef\csname R@an.lineage.stagecost.enc014.params.acdc\endcsname{2.89}
\expandafter\gdef\csname R@an.lineage.stagecost.enc014.params.amos\endcsname{2.89}
\expandafter\gdef\csname R@an.lineage.stagecost.enc014.params.kits\endcsname{2.90}
\expandafter\gdef\csname R@an.lineage.stagecost.enc014.pshare.acdc\endcsname{9.51}
\expandafter\gdef\csname R@an.lineage.stagecost.enc014.pshare.amos\endcsname{9.29}
\expandafter\gdef\csname R@an.lineage.stagecost.enc014.pshare.kits\endcsname{9.29}
\expandafter\gdef\csname R@an.lineage.stagecost.enc014.pshare.max\endcsname{9.51}
\expandafter\gdef\csname R@an.lineage.stagecost.enc014.share.acdc\endcsname{16.1}
\expandafter\gdef\csname R@an.lineage.stagecost.enc014.share.amos\endcsname{16.0}
\expandafter\gdef\csname R@an.lineage.stagecost.enc014.share.kits\endcsname{18.3}
\expandafter\gdef\csname R@an.lineage.stagecost.enc014.share.max\endcsname{18.3}
\expandafter\gdef\csname R@an.lineage.stagecost.enc014.share.min\endcsname{16.0}
\expandafter\gdef\csname R@an.lineage.stagecost.sentence\endcsname{The profile records locate the default's cost. Removing the second convolution of the two finest decoder stages cuts the profiled step time by 18.9, 21.0, 20.4 ms (13.5, 14.8, 16.5 \% of the default's) and 0.12, 0.12, 0.13 M parameters (0.39, 0.39, 0.42 \%) on the AMOS22, ACDC and KiTS23 plans; removing the second convolution at encoder stage 0 alone cuts 14.6, 14.5, 17.5 ms (10.4, 10.2, 14.2 \%) and 0.01, 0.01, 0.03 M parameters. On the AMOS22 operator bench one dense 3$\times$3$\times$3 convolution at each of encoder stages 3 and 4 holds 4\,534\,272 weights (14.6 \% of the default's parameters) and costs 1.70 ms (1.2 \% of its step).}
\expandafter\gdef\csname R@an.lineage.stagecost.short\endcsname{The second convolution of the two finest decoder stages holds 0.4 \% of the default's parameters and 13.5 to 16.5 \% of its step time}
\expandafter\gdef\csname R@an.lineage.state.cross_validated\endcsname{12}
\expandafter\gdef\csname R@an.lineage.state.held_out\endcsname{4}
\expandafter\gdef\csname R@an.lineage.state.registered\endcsname{42}
\expandafter\gdef\csname R@an.lineage.state.replicated\endcsname{25}
\expandafter\gdef\csname R@an.lineage.state.screened\endcsname{38}
\expandafter\gdef\csname R@an.lineage.state_only.cross_validated\endcsname{8}
\expandafter\gdef\csname R@an.lineage.state_only.held_out\endcsname{4}
\expandafter\gdef\csname R@an.lineage.state_only.registered\endcsname{4}
\expandafter\gdef\csname R@an.lineage.state_only.replicated\endcsname{13}
\expandafter\gdef\csname R@an.lineage.state_only.screened\endcsname{13}
\expandafter\gdef\csname R@an.lineage.steperr.sentence\endcsname{The ideators' step-time predictions differ from the profile records by a mean of 12.6 \% in wave 5 (3 designs, 9 cells, from 0.2 to 25.7 \%; 2 of the 9 cells predicted at or above the profiled step; the savings of the designs predicted below the default's step were over-predicted 1.7-fold (median)); 2.0 \% in wave 7 (7 designs, 21 cells, from 0.3 to 5.9 \%; 14 of the 21 cells predicted at or above the profiled step); 2.8 \% in wave 8 (5 designs, 15 cells, from 0.5 to 5.6 \%; 12 of the 15 cells predicted at or above the profiled step).}
\expandafter\gdef\csname R@an.lineage.steperr.short\endcsname{Predicted step times differed from the profile by 12.6 \% (wave 5), 2.0 \% (wave 7) and 2.8 \% (wave 8) on average}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w1.amos\endcsname{88.083}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w1.best.at085\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w1.best.at085.name\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w1.best.at1\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w1.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w1.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w1.kits\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w1.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w1.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w1.par\endcsname{0.951}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w1.step\endcsname{1.401}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w1.tag\endcsname{L3}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w1.tags\endcsname{HyReX, ConvNeXt-k3}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w2.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w2.best.at085\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w2.best.at085.name\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w2.best.at1\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w2.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w2.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w2.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w2.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w2.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w2.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w2.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w2.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w2.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w2.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w3.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w3.best.at085\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w3.best.at085.name\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w3.best.at1\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w3.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w3.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w3.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w3.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w3.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w3.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w3.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w3.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w3.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w3.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w4.amos\endcsname{88.091}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w4.best.at085\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w4.best.at085.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w4.best.at1\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w4.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w4.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w4.kits\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w4.n\endcsname{4}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w4.name\endcsname{HyReX+dec. capacity}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w4.new\endcsname{3}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w4.par\endcsname{1.680}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w4.step\endcsname{1.580}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w4.tag\endcsname{C1\_deccap}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w4.tags\endcsname{HyReX+dec. capacity, LeanDec, HyReX point-fuse}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w5.amos\endcsname{87.440}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w5.best.at085\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w5.best.at085.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w5.best.at1\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w5.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w5.guard\endcsname{not met}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w5.kits\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w5.n\endcsname{5}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w5.name\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w5.new\endcsname{1}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w5.par\endcsname{0.672}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w5.step\endcsname{0.727}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w5.tag\endcsname{V5B1}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w5.tags\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w6.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w6.best.at085\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w6.best.at085.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w6.best.at1\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w6.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w6.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w6.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w6.n\endcsname{5}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w6.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w6.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w6.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w6.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w6.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w6.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w7.amos\endcsname{88.060}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w7.best.at085\endcsname{\ensuremath{+1.95}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w7.best.at085.name\endcsname{LeanDil}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w7.best.at1\endcsname{\ensuremath{+2.01}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w7.best.at1.name\endcsname{LeanDeepMid+FD}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w7.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w7.kits\endcsname{\ensuremath{+2.01}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w7.n\endcsname{5}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w7.name\endcsname{LeanDeepMid+FD}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w7.new\endcsname{3}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w7.par\endcsname{0.999}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w7.step\endcsname{1.092}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w7.tag\endcsname{V7A2}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w7.tags\endcsname{LeanDeepMid+FD, LeanDil, LeanSep}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w8.amos\endcsname{86.950}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w8.best.at085\endcsname{\ensuremath{+2.03}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w8.best.at085.name\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w8.best.at1\endcsname{\ensuremath{+2.03}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w8.best.at1.name\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w8.guard\endcsname{not met}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w8.kits\endcsname{\ensuremath{+2.03}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w8.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w8.name\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w8.new\endcsname{1}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w8.par\endcsname{0.584}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w8.step\endcsname{0.588}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w8.tag\endcsname{V8B1}
\expandafter\gdef\csname R@an.lineage.stk.front.any.par.w8.tags\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w1.amos\endcsname{88.083}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w1.best.at085\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w1.best.at085.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w1.best.at1\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w1.best.at1.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w1.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w1.kits\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w1.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w1.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w1.par\endcsname{0.951}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w1.step\endcsname{1.401}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w1.tag\endcsname{L3}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w1.tags\endcsname{HyReX, ResEnc+context}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w2.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w2.best.at085\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w2.best.at085.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w2.best.at1\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w2.best.at1.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w2.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w2.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w2.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w2.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w2.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w2.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w2.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w2.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w2.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w3.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w3.best.at085\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w3.best.at085.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w3.best.at1\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w3.best.at1.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w3.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w3.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w3.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w3.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w3.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w3.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w3.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w3.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w3.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w4.amos\endcsname{88.091}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w4.best.at085\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w4.best.at085.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w4.best.at1\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w4.best.at1.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w4.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w4.kits\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w4.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w4.name\endcsname{HyReX+dec. capacity}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w4.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w4.par\endcsname{1.680}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w4.step\endcsname{1.580}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w4.tag\endcsname{C1\_deccap}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w4.tags\endcsname{HyReX+dec. capacity, LeanDec}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w5.amos\endcsname{87.440}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w5.best.at085\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w5.best.at085.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w5.best.at1\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w5.best.at1.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w5.guard\endcsname{not met}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w5.kits\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w5.n\endcsname{4}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w5.name\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w5.new\endcsname{1}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w5.par\endcsname{0.672}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w5.step\endcsname{0.727}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w5.tag\endcsname{V5B1}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w5.tags\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w6.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w6.best.at085\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w6.best.at085.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w6.best.at1\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w6.best.at1.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w6.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w6.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w6.n\endcsname{4}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w6.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w6.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w6.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w6.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w6.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w6.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w7.amos\endcsname{88.060}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w7.best.at085\endcsname{\ensuremath{+1.95}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w7.best.at085.name\endcsname{LeanDil}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w7.best.at1\endcsname{\ensuremath{+1.95}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w7.best.at1.name\endcsname{LeanDil}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w7.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w7.kits\endcsname{\ensuremath{+2.01}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w7.n\endcsname{4}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w7.name\endcsname{LeanDeepMid+FD}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w7.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w7.par\endcsname{0.999}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w7.step\endcsname{1.092}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w7.tag\endcsname{V7A2}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w7.tags\endcsname{LeanDeepMid+FD, LeanDil}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w8.amos\endcsname{86.950}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w8.best.at085\endcsname{\ensuremath{+2.03}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w8.best.at085.name\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w8.best.at1\endcsname{\ensuremath{+2.03}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w8.best.at1.name\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w8.guard\endcsname{not met}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w8.kits\endcsname{\ensuremath{+2.03}}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w8.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w8.name\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w8.new\endcsname{1}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w8.par\endcsname{0.584}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w8.step\endcsname{0.588}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w8.tag\endcsname{V8B1}
\expandafter\gdef\csname R@an.lineage.stk.front.any.w8.tags\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.lineage.stk.front.foot\endcsname{A cross on a grey point marks a design whose AMOS22 seed-0 Dice is below 87.551 (the frozen pool mean minus 0.15 points): LeanDec, default+GN16, LeanAdd, LeanFullDec, LeanSep, LeanDil, LeanNeXt-k3, CoarseStack, StackDec, LeanTrunk, Stem1, NarrowTrunk.}
\expandafter\gdef\csname R@an.lineage.stk.front.guard.breach.names\endcsname{LeanDec, default+GN16, LeanAdd, LeanSep, LeanDil, CoarseStack, StackDec, LeanTrunk, Stem1}
\expandafter\gdef\csname R@an.lineage.stk.front.guard.breach.tags\endcsname{D2\_dec1, N1\_gnw16, V5B1, V7B1, V7B2, V8A1, V8A2, V8B1, V8B2}
\expandafter\gdef\csname R@an.lineage.stk.front.guard.line\endcsname{87.551}
\expandafter\gdef\csname R@an.lineage.stk.front.guard.n_breach\endcsname{9}
\expandafter\gdef\csname R@an.lineage.stk.front.guard.n_met\endcsname{13}
\expandafter\gdef\csname R@an.lineage.stk.front.guard.n_pending\endcsname{0}
\expandafter\gdef\csname R@an.lineage.stk.front.guard.pp\endcsname{-0.15}
\expandafter\gdef\csname R@an.lineage.stk.front.off\endcsname{Off the scale of the parameter panel, above 1.8$\times$ the default's parameters: ResEnc-M (3.28$\times$, arrow), ResEnc+context (3.30$\times$), ResEnc-matched (3.28$\times$).}
\expandafter\gdef\csname R@an.lineage.stk.front.off.limit\endcsname{1.8}
\expandafter\gdef\csname R@an.lineage.stk.front.off.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w1.amos\endcsname{88.083}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w1.best.at085\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w1.best.at085.name\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w1.best.at1\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w1.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w1.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w1.kits\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w1.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w1.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w1.par\endcsname{0.951}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w1.step\endcsname{1.401}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w1.tag\endcsname{L3}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w1.tags\endcsname{HyReX, ConvNeXt-k3}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w2.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w2.best.at085\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w2.best.at085.name\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w2.best.at1\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w2.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w2.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w2.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w2.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w2.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w2.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w2.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w2.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w2.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w2.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w3.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w3.best.at085\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w3.best.at085.name\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w3.best.at1\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w3.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w3.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w3.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w3.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w3.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w3.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w3.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w3.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w3.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w3.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w4.amos\endcsname{88.091}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w4.best.at085\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w4.best.at085.name\endcsname{HyReX point-fuse}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w4.best.at1\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w4.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w4.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w4.kits\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w4.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w4.name\endcsname{HyReX+dec. capacity}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w4.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w4.par\endcsname{1.680}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w4.step\endcsname{1.580}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w4.tag\endcsname{C1\_deccap}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w4.tags\endcsname{HyReX+dec. capacity, HyReX point-fuse}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w5.amos\endcsname{87.742}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w5.best.at085\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w5.best.at085.name\endcsname{HyReX point-fuse}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w5.best.at1\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w5.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w5.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w5.kits\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w5.n\endcsname{4}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w5.name\endcsname{HyReX-LeanDec}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w5.new\endcsname{1}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w5.par\endcsname{0.946}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w5.step\endcsname{1.235}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w5.tag\endcsname{V5A5}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w5.tags\endcsname{HyReX-LeanDec}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w6.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w6.best.at085\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w6.best.at085.name\endcsname{HyReX point-fuse}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w6.best.at1\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w6.best.at1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w6.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w6.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w6.n\endcsname{4}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w6.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w6.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w6.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w6.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w6.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w6.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w7.amos\endcsname{88.060}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w7.best.at085\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w7.best.at085.name\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w7.best.at1\endcsname{\ensuremath{+2.01}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w7.best.at1.name\endcsname{LeanDeepMid+FD}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w7.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w7.kits\endcsname{\ensuremath{+2.01}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w7.n\endcsname{5}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w7.name\endcsname{LeanDeepMid+FD}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w7.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w7.par\endcsname{0.999}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w7.step\endcsname{1.092}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w7.tag\endcsname{V7A2}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w7.tags\endcsname{LeanDeepMid+FD, LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w8.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w8.best.at085\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w8.best.at085.name\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w8.best.at1\endcsname{\ensuremath{+2.01}}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w8.best.at1.name\endcsname{LeanDeepMid+FD}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w8.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w8.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w8.n\endcsname{5}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w8.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w8.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w8.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w8.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w8.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.par.w8.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w1.amos\endcsname{88.083}
\expandafter\gdef\csname R@an.lineage.stk.front.w1.best.at085\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w1.best.at085.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w1.best.at1\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w1.best.at1.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w1.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.stk.front.w1.kits\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.lineage.stk.front.w1.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.w1.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.lineage.stk.front.w1.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.w1.par\endcsname{0.951}
\expandafter\gdef\csname R@an.lineage.stk.front.w1.step\endcsname{1.401}
\expandafter\gdef\csname R@an.lineage.stk.front.w1.tag\endcsname{L3}
\expandafter\gdef\csname R@an.lineage.stk.front.w1.tags\endcsname{HyReX, ResEnc+context}
\expandafter\gdef\csname R@an.lineage.stk.front.w2.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w2.best.at085\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w2.best.at085.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w2.best.at1\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w2.best.at1.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w2.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w2.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w2.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.w2.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w2.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.stk.front.w2.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w2.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w2.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w2.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w3.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w3.best.at085\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w3.best.at085.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w3.best.at1\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w3.best.at1.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w3.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w3.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w3.n\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.w3.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w3.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.stk.front.w3.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w3.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w3.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w3.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w4.amos\endcsname{88.091}
\expandafter\gdef\csname R@an.lineage.stk.front.w4.best.at085\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w4.best.at085.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w4.best.at1\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w4.best.at1.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w4.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.stk.front.w4.kits\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@an.lineage.stk.front.w4.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.stk.front.w4.name\endcsname{HyReX+dec. capacity}
\expandafter\gdef\csname R@an.lineage.stk.front.w4.new\endcsname{1}
\expandafter\gdef\csname R@an.lineage.stk.front.w4.par\endcsname{1.680}
\expandafter\gdef\csname R@an.lineage.stk.front.w4.step\endcsname{1.580}
\expandafter\gdef\csname R@an.lineage.stk.front.w4.tag\endcsname{C1\_deccap}
\expandafter\gdef\csname R@an.lineage.stk.front.w4.tags\endcsname{HyReX+dec. capacity}
\expandafter\gdef\csname R@an.lineage.stk.front.w5.amos\endcsname{87.742}
\expandafter\gdef\csname R@an.lineage.stk.front.w5.best.at085\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.lineage.stk.front.w5.best.at085.name\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.stk.front.w5.best.at1\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.lineage.stk.front.w5.best.at1.name\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.stk.front.w5.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.stk.front.w5.kits\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.lineage.stk.front.w5.n\endcsname{5}
\expandafter\gdef\csname R@an.lineage.stk.front.w5.name\endcsname{HyReX-LeanDec}
\expandafter\gdef\csname R@an.lineage.stk.front.w5.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.w5.par\endcsname{0.946}
\expandafter\gdef\csname R@an.lineage.stk.front.w5.step\endcsname{1.235}
\expandafter\gdef\csname R@an.lineage.stk.front.w5.tag\endcsname{V5A5}
\expandafter\gdef\csname R@an.lineage.stk.front.w5.tags\endcsname{HyReX-LeanDec, LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.stk.front.w6.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w6.best.at085\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.lineage.stk.front.w6.best.at085.name\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.stk.front.w6.best.at1\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.lineage.stk.front.w6.best.at1.name\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.lineage.stk.front.w6.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w6.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w6.n\endcsname{5}
\expandafter\gdef\csname R@an.lineage.stk.front.w6.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w6.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.stk.front.w6.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w6.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w6.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w6.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w7.amos\endcsname{88.060}
\expandafter\gdef\csname R@an.lineage.stk.front.w7.best.at085\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@an.lineage.stk.front.w7.best.at085.name\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.stk.front.w7.best.at1\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@an.lineage.stk.front.w7.best.at1.name\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.stk.front.w7.guard\endcsname{met}
\expandafter\gdef\csname R@an.lineage.stk.front.w7.kits\endcsname{\ensuremath{+2.01}}
\expandafter\gdef\csname R@an.lineage.stk.front.w7.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.stk.front.w7.name\endcsname{LeanDeepMid+FD}
\expandafter\gdef\csname R@an.lineage.stk.front.w7.new\endcsname{2}
\expandafter\gdef\csname R@an.lineage.stk.front.w7.par\endcsname{0.999}
\expandafter\gdef\csname R@an.lineage.stk.front.w7.step\endcsname{1.092}
\expandafter\gdef\csname R@an.lineage.stk.front.w7.tag\endcsname{V7A2}
\expandafter\gdef\csname R@an.lineage.stk.front.w7.tags\endcsname{LeanDeepMid+FD, LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.stk.front.w8.amos\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w8.best.at085\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@an.lineage.stk.front.w8.best.at085.name\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.stk.front.w8.best.at1\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@an.lineage.stk.front.w8.best.at1.name\endcsname{LeanNeXt-s5}
\expandafter\gdef\csname R@an.lineage.stk.front.w8.guard\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w8.kits\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w8.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.stk.front.w8.name\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w8.new\endcsname{0}
\expandafter\gdef\csname R@an.lineage.stk.front.w8.par\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w8.step\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w8.tag\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.front.w8.tags\endcsname{none}
\expandafter\gdef\csname R@an.lineage.stk.ref.amos.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.stk.ref.amos.shift\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.lineage.stk.ref.mean\endcsname{84.26}
\expandafter\gdef\csname R@an.lineage.stk.ref.n\endcsname{9}
\expandafter\gdef\csname R@an.lineage.stk.ref.pool\endcsname{83.38}
\expandafter\gdef\csname R@an.lineage.stk.ref.pool.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.stk.ref.sd\endcsname{0.63}
\expandafter\gdef\csname R@an.lineage.stk.ref.se_mark\endcsname{0.45}
\expandafter\gdef\csname R@an.lineage.stk.ref.seeds\endcsname{3--11}
\expandafter\gdef\csname R@an.lineage.stk.ref.sentence\endcsname{every KiTS23 Dice difference is read against the mean of nnU-Net's nine stock runs of the same pipeline (seeds 3--11; 84.26 Dice, SD 0.63), which lies 0.88 points above the frozen pool of three runs (83.38), so each equals the difference against the pool minus 0.88; the bars on the fresh-seed means are one standard error of a mean of two runs, the SD of the stock runs divided by the square root of two (0.45 points)}
\expandafter\gdef\csname R@an.lineage.stk.ref.shift\endcsname{0.88}
\expandafter\gdef\csname R@an.lineage.stk.ref.word\endcsname{nine}
\expandafter\gdef\csname R@an.lineage.stk.ref.ylabel\endcsname{Dice difference to nnU-Net (nine stock runs)}
\expandafter\gdef\csname R@an.lineage.stk.sent.front\endcsname{On KiTS23, among the agent-designed networks with AMOS22 seed 0 inside the registered $-$0.15 pp guard and a step time at or below the default's, the best seed-0 (discovery) Dice difference to nnU-Net (the mean of its nine stock runs) is \ensuremath{+0.39} pp (LeanAdd-NeXt) from wave 5, then \ensuremath{+1.83} pp (LeanNeXt-s5) from wave 7, and no design qualifies before wave 5; the same designs hold at 0.85$\times$ the default's step time.}
\expandafter\gdef\csname R@an.lineage.stk.sent.front.any\endcsname{On KiTS23, among the agent-designed networks with a step time at or below the default's, the best seed-0 (discovery) Dice difference to nnU-Net (the mean of its nine stock runs) is \ensuremath{+1.48} pp (LeanDec) from wave 4, then \ensuremath{+1.95} pp (LeanDil) from wave 7, then \ensuremath{+2.03} pp (LeanTrunk) from wave 8, and no design qualifies before wave 4; the same designs hold at 0.85$\times$ the default's step time.}
\expandafter\gdef\csname R@an.lineage.stk.sent.front.plain\endcsname{On KiTS23, among the agent-designed networks whose AMOS22 Dice stays within 0.15 points of nnU-Net's at seed 0 and whose step time is at or below the default's, the best seed-0 (discovery) Dice difference to nnU-Net (the mean of its nine stock runs) is \ensuremath{+0.39} pp (LeanAdd-NeXt) from wave 5, then \ensuremath{+1.83} pp (LeanNeXt-s5) from wave 7, and no design qualifies before wave 5; the same designs hold at 0.85$\times$ the default's step time.}
\expandafter\gdef\csname R@an.lineage.stk.sent.front.plain.cond\endcsname{whose AMOS22 Dice stays within 0.15 points of nnU-Net's at seed 0}
\expandafter\gdef\csname R@an.lineage.w7.extent.V7B2.name\endcsname{LeanDil}
\expandafter\gdef\csname R@an.lineage.w7.extent.V7B2.value\endcsname{87.435}
\expandafter\gdef\csname R@an.lineage.w7.extent.V7C2.name\endcsname{LeanNeXt-k3}
\expandafter\gdef\csname R@an.lineage.w7.extent.V7C2.value\endcsname{87.339}
\expandafter\gdef\csname R@an.lineage.w7.extent.diff\endcsname{\ensuremath{+0.095}}
\expandafter\gdef\csname R@an.lineage.w7.extent.floor\endcsname{0.50}
\expandafter\gdef\csname R@an.lineage.w7.extent.sentence\endcsname{On AMOS22 the seed-0 difference LeanDil minus LeanNeXt-k3 is \ensuremath{+0.095} pp (87.435 against 87.339) against the registered 0.50 pp claim line (Addendum AN4, confirmed in AR0): the line is not met, so neither arm is described as showing that extent matters.}
\expandafter\gdef\csname R@an.lineage.w7.extent.state\endcsname{not met}
\expandafter\gdef\csname R@an.lineage.w7.mech.V7B1.dist\endcsname{0.174}
\expandafter\gdef\csname R@an.lineage.w7.mech.V7B1.margin\endcsname{\ensuremath{-0.174}}
\expandafter\gdef\csname R@an.lineage.w7.mech.V7B1.name\endcsname{LeanSep}
\expandafter\gdef\csname R@an.lineage.w7.mech.V7B1.state\endcsname{reported dead}
\expandafter\gdef\csname R@an.lineage.w7.mech.V7B1.value\endcsname{87.266}
\expandafter\gdef\csname R@an.lineage.w7.mech.V7B2.dist\endcsname{0.005}
\expandafter\gdef\csname R@an.lineage.w7.mech.V7B2.margin\endcsname{\ensuremath{-0.005}}
\expandafter\gdef\csname R@an.lineage.w7.mech.V7B2.name\endcsname{LeanDil}
\expandafter\gdef\csname R@an.lineage.w7.mech.V7B2.state\endcsname{reported dead}
\expandafter\gdef\csname R@an.lineage.w7.mech.V7B2.value\endcsname{87.435}
\expandafter\gdef\csname R@an.lineage.w7.mech.line\endcsname{87.440}
\expandafter\gdef\csname R@an.lineage.w7.mech.se\endcsname{0.13}
\expandafter\gdef\csname R@an.lineage.w7.mech.sentence\endcsname{Addendum AN4 registered that the AMOS22 movement of LeanAdd-NeXt over LeanAdd is reported dead if a cheaper operator's AMOS22 seed-0 value is at or below LeanAdd's 87.440. LeanSep reads 87.266 (at or below the line by 0.174 pp) and LeanDil reads 87.435 (at or below the line by 0.005 pp), so both are reported dead by the registered rule: one seed, standard error 0.13 pp, a decision rule, not an estimate.}
\expandafter\gdef\csname R@an.lineage.w7.mech.state\endcsname{reported dead}
\expandafter\gdef\csname R@an.lineage.w7.sent.extent\endcsname{On AMOS22 the seed-0 difference LeanDil minus LeanNeXt-k3 is \ensuremath{+0.095} pp (87.435 against 87.339) against the registered 0.50 pp claim line (Addendum AN4, confirmed in AR0): the line is not met, so neither arm is described as showing that extent matters.}
\expandafter\gdef\csname R@an.lineage.w7.sent.mech\endcsname{Addendum AN4 registered that the AMOS22 movement of LeanAdd-NeXt over LeanAdd is reported dead if a cheaper operator's AMOS22 seed-0 value is at or below LeanAdd's 87.440. LeanSep reads 87.266 (at or below the line by 0.174 pp) and LeanDil reads 87.435 (at or below the line by 0.005 pp), so both are reported dead by the registered rule: one seed, standard error 0.13 pp, a decision rule, not an estimate.}
\expandafter\gdef\csname R@an.lineage.wave.1.agent\endcsname{4}
\expandafter\gdef\csname R@an.lineage.wave.1.at_cross_validated\endcsname{1}
\expandafter\gdef\csname R@an.lineage.wave.1.at_held_out\endcsname{2}
\expandafter\gdef\csname R@an.lineage.wave.1.at_registered\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.1.at_replicated\endcsname{3}
\expandafter\gdef\csname R@an.lineage.wave.1.at_screened\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.1.attribution\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.1.control\endcsname{1}
\expandafter\gdef\csname R@an.lineage.wave.1.n\endcsname{6}
\expandafter\gdef\csname R@an.lineage.wave.1.reference\endcsname{1}
\expandafter\gdef\csname R@an.lineage.wave.2.agent\endcsname{3}
\expandafter\gdef\csname R@an.lineage.wave.2.at_cross_validated\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.2.at_held_out\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.2.at_registered\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.2.at_replicated\endcsname{1}
\expandafter\gdef\csname R@an.lineage.wave.2.at_screened\endcsname{6}
\expandafter\gdef\csname R@an.lineage.wave.2.attribution\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.2.control\endcsname{3}
\expandafter\gdef\csname R@an.lineage.wave.2.n\endcsname{7}
\expandafter\gdef\csname R@an.lineage.wave.2.reference\endcsname{1}
\expandafter\gdef\csname R@an.lineage.wave.3.agent\endcsname{3}
\expandafter\gdef\csname R@an.lineage.wave.3.at_cross_validated\endcsname{1}
\expandafter\gdef\csname R@an.lineage.wave.3.at_held_out\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.3.at_registered\endcsname{4}
\expandafter\gdef\csname R@an.lineage.wave.3.at_replicated\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.3.at_screened\endcsname{2}
\expandafter\gdef\csname R@an.lineage.wave.3.attribution\endcsname{2}
\expandafter\gdef\csname R@an.lineage.wave.3.control\endcsname{2}
\expandafter\gdef\csname R@an.lineage.wave.3.n\endcsname{7}
\expandafter\gdef\csname R@an.lineage.wave.3.reference\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.4.agent\endcsname{5}
\expandafter\gdef\csname R@an.lineage.wave.4.at_cross_validated\endcsname{1}
\expandafter\gdef\csname R@an.lineage.wave.4.at_held_out\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.4.at_registered\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.4.at_replicated\endcsname{3}
\expandafter\gdef\csname R@an.lineage.wave.4.at_screened\endcsname{2}
\expandafter\gdef\csname R@an.lineage.wave.4.attribution\endcsname{1}
\expandafter\gdef\csname R@an.lineage.wave.4.control\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.4.n\endcsname{6}
\expandafter\gdef\csname R@an.lineage.wave.4.reference\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.5.agent\endcsname{3}
\expandafter\gdef\csname R@an.lineage.wave.5.at_cross_validated\endcsname{2}
\expandafter\gdef\csname R@an.lineage.wave.5.at_held_out\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.5.at_registered\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.5.at_replicated\endcsname{1}
\expandafter\gdef\csname R@an.lineage.wave.5.at_screened\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.5.attribution\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.5.control\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.5.n\endcsname{3}
\expandafter\gdef\csname R@an.lineage.wave.5.reference\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.6.agent\endcsname{1}
\expandafter\gdef\csname R@an.lineage.wave.6.at_cross_validated\endcsname{1}
\expandafter\gdef\csname R@an.lineage.wave.6.at_held_out\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.6.at_registered\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.6.at_replicated\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.6.at_screened\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.6.attribution\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.6.control\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.6.n\endcsname{1}
\expandafter\gdef\csname R@an.lineage.wave.6.reference\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.7.agent\endcsname{5}
\expandafter\gdef\csname R@an.lineage.wave.7.at_cross_validated\endcsname{1}
\expandafter\gdef\csname R@an.lineage.wave.7.at_held_out\endcsname{2}
\expandafter\gdef\csname R@an.lineage.wave.7.at_registered\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.7.at_replicated\endcsname{2}
\expandafter\gdef\csname R@an.lineage.wave.7.at_screened\endcsname{2}
\expandafter\gdef\csname R@an.lineage.wave.7.attribution\endcsname{2}
\expandafter\gdef\csname R@an.lineage.wave.7.control\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.7.n\endcsname{7}
\expandafter\gdef\csname R@an.lineage.wave.7.reference\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.8.agent\endcsname{4}
\expandafter\gdef\csname R@an.lineage.wave.8.at_cross_validated\endcsname{1}
\expandafter\gdef\csname R@an.lineage.wave.8.at_held_out\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.8.at_registered\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.8.at_replicated\endcsname{3}
\expandafter\gdef\csname R@an.lineage.wave.8.at_screened\endcsname{1}
\expandafter\gdef\csname R@an.lineage.wave.8.attribution\endcsname{1}
\expandafter\gdef\csname R@an.lineage.wave.8.control\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave.8.n\endcsname{5}
\expandafter\gdef\csname R@an.lineage.wave.8.reference\endcsname{0}
\expandafter\gdef\csname R@an.lineage.wave_table_n\endcsname{42}
\expandafter\gdef\csname R@an.lineage.waves\endcsname{8}
\expandafter\gdef\csname R@an.lineage.waves.docs\endcsname{1,2,3,4,5,6,7,8}
\expandafter\gdef\csname R@an.master_table.C1.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.C1.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.params\endcsname{51.59}
\expandafter\gdef\csname R@an.master_table.C1.acdc.peak\endcsname{10.26}
\expandafter\gdef\csname R@an.master_table.C1.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.acdc.step\endcsname{1.80}
\expandafter\gdef\csname R@an.master_table.C1.amos.d0\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.master_table.C1.amos.d0_3\endcsname{\ensuremath{+0.390}}
\expandafter\gdef\csname R@an.master_table.C1.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.C1.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.amos.ne0\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.master_table.C1.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.amos.params\endcsname{52.34}
\expandafter\gdef\csname R@an.master_table.C1.amos.peak\endcsname{11.14}
\expandafter\gdef\csname R@an.master_table.C1.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.amos.step\endcsname{1.69}
\expandafter\gdef\csname R@an.master_table.C1.kits.d0\endcsname{\ensuremath{+3.51}}
\expandafter\gdef\csname R@an.master_table.C1.kits.d0_3\endcsname{\ensuremath{+3.507}}
\expandafter\gdef\csname R@an.master_table.C1.kits.d3\endcsname{\ensuremath{+2.770}}
\expandafter\gdef\csname R@an.master_table.C1.kits.d3_df\endcsname{3.9}
\expandafter\gdef\csname R@an.master_table.C1.kits.d3_hi\endcsname{\ensuremath{+4.474}}
\expandafter\gdef\csname R@an.master_table.C1.kits.d3_lo\endcsname{\ensuremath{+1.066}}
\expandafter\gdef\csname R@an.master_table.C1.kits.d3_span\endcsname{lies above the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.C1.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.C1.kits.dfresh\endcsname{\ensuremath{+2.401}}
\expandafter\gdef\csname R@an.master_table.C1.kits.fresh_max\endcsname{\ensuremath{+2.674}}
\expandafter\gdef\csname R@an.master_table.C1.kits.fresh_min\endcsname{\ensuremath{+2.128}}
\expandafter\gdef\csname R@an.master_table.C1.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.C1.kits.fresh_phrase\endcsname{\ensuremath{+2.401} pp over its two fresh seeds (seed deltas \ensuremath{+2.128} and \ensuremath{+2.674})}
\expandafter\gdef\csname R@an.master_table.C1.kits.fresh_se\endcsname{0.273}
\expandafter\gdef\csname R@an.master_table.C1.kits.fresh_vs_L3\endcsname{\ensuremath{+0.307}}
\expandafter\gdef\csname R@an.master_table.C1.kits.fresh_vs_L3_abs\endcsname{0.307}
\expandafter\gdef\csname R@an.master_table.C1.kits.fresh_vs_L3_dir\endcsname{above}
\expandafter\gdef\csname R@an.master_table.C1.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.C1.kits.ne0\endcsname{\ensuremath{+3.51}}
\expandafter\gdef\csname R@an.master_table.C1.kits.nefresh\endcsname{\ensuremath{+2.401}}
\expandafter\gdef\csname R@an.master_table.C1.kits.nefresh_margin\endcsname{\ensuremath{+2.201}}
\expandafter\gdef\csname R@an.master_table.C1.kits.params\endcsname{52.41}
\expandafter\gdef\csname R@an.master_table.C1.kits.peak\endcsname{9.08}
\expandafter\gdef\csname R@an.master_table.C1.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 2.051 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 2.201 pp}
\expandafter\gdef\csname R@an.master_table.C1.kits.step\endcsname{1.58}
\expandafter\gdef\csname R@an.master_table.C1.params\endcsname{52.34}
\expandafter\gdef\csname R@an.master_table.C1.params_pct_vs_default\endcsname{\ensuremath{+68.2}}
\expandafter\gdef\csname R@an.master_table.C1.peak\endcsname{11.14}
\expandafter\gdef\csname R@an.master_table.C1.step\endcsname{1.69}
\expandafter\gdef\csname R@an.master_table.D1.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.D1.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.params\endcsname{20.11}
\expandafter\gdef\csname R@an.master_table.D1.acdc.peak\endcsname{10.37}
\expandafter\gdef\csname R@an.master_table.D1.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.acdc.step\endcsname{1.63}
\expandafter\gdef\csname R@an.master_table.D1.amos.d0\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.master_table.D1.amos.d0_3\endcsname{\ensuremath{+0.278}}
\expandafter\gdef\csname R@an.master_table.D1.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.D1.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.amos.ne0\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.master_table.D1.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.amos.params\endcsname{20.86}
\expandafter\gdef\csname R@an.master_table.D1.amos.peak\endcsname{10.69}
\expandafter\gdef\csname R@an.master_table.D1.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.amos.step\endcsname{1.52}
\expandafter\gdef\csname R@an.master_table.D1.kits.d0\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.master_table.D1.kits.d0_3\endcsname{\ensuremath{+1.607}}
\expandafter\gdef\csname R@an.master_table.D1.kits.d3\endcsname{\ensuremath{+1.520}}
\expandafter\gdef\csname R@an.master_table.D1.kits.d3_df\endcsname{2.5}
\expandafter\gdef\csname R@an.master_table.D1.kits.d3_hi\endcsname{\ensuremath{+3.252}}
\expandafter\gdef\csname R@an.master_table.D1.kits.d3_lo\endcsname{\ensuremath{-0.212}}
\expandafter\gdef\csname R@an.master_table.D1.kits.d3_span\endcsname{spans both zero and the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.D1.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D1.kits.dfresh\endcsname{\ensuremath{+1.477}}
\expandafter\gdef\csname R@an.master_table.D1.kits.fresh_max\endcsname{\ensuremath{+1.759}}
\expandafter\gdef\csname R@an.master_table.D1.kits.fresh_min\endcsname{\ensuremath{+1.194}}
\expandafter\gdef\csname R@an.master_table.D1.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.D1.kits.fresh_phrase\endcsname{\ensuremath{+1.477} pp over its two fresh seeds (seed deltas \ensuremath{+1.194} and \ensuremath{+1.759})}
\expandafter\gdef\csname R@an.master_table.D1.kits.fresh_se\endcsname{0.283}
\expandafter\gdef\csname R@an.master_table.D1.kits.fresh_vs_L3\endcsname{\ensuremath{-0.617}}
\expandafter\gdef\csname R@an.master_table.D1.kits.fresh_vs_L3_abs\endcsname{0.617}
\expandafter\gdef\csname R@an.master_table.D1.kits.fresh_vs_L3_dir\endcsname{below}
\expandafter\gdef\csname R@an.master_table.D1.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.D1.kits.ne0\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.master_table.D1.kits.nefresh\endcsname{\ensuremath{+1.477}}
\expandafter\gdef\csname R@an.master_table.D1.kits.nefresh_margin\endcsname{\ensuremath{+1.277}}
\expandafter\gdef\csname R@an.master_table.D1.kits.params\endcsname{20.93}
\expandafter\gdef\csname R@an.master_table.D1.kits.peak\endcsname{9.51}
\expandafter\gdef\csname R@an.master_table.D1.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 1.127 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 1.277 pp}
\expandafter\gdef\csname R@an.master_table.D1.kits.step\endcsname{1.40}
\expandafter\gdef\csname R@an.master_table.D1.params\endcsname{20.86}
\expandafter\gdef\csname R@an.master_table.D1.params_pct_vs_default\endcsname{\ensuremath{-33.0}}
\expandafter\gdef\csname R@an.master_table.D1.peak\endcsname{10.69}
\expandafter\gdef\csname R@an.master_table.D1.step\endcsname{1.52}
\expandafter\gdef\csname R@an.master_table.D2.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.D2.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.params\endcsname{25.28}
\expandafter\gdef\csname R@an.master_table.D2.acdc.peak\endcsname{9.45}
\expandafter\gdef\csname R@an.master_table.D2.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.acdc.step\endcsname{0.81}
\expandafter\gdef\csname R@an.master_table.D2.amos.d0\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.master_table.D2.amos.d0_3\endcsname{\ensuremath{-0.362}}
\expandafter\gdef\csname R@an.master_table.D2.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.D2.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.amos.ne0\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.master_table.D2.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.amos.params\endcsname{26.03}
\expandafter\gdef\csname R@an.master_table.D2.amos.peak\endcsname{8.14}
\expandafter\gdef\csname R@an.master_table.D2.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.amos.step\endcsname{0.81}
\expandafter\gdef\csname R@an.master_table.D2.kits.d0\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.master_table.D2.kits.d0_3\endcsname{\ensuremath{+2.355}}
\expandafter\gdef\csname R@an.master_table.D2.kits.d3\endcsname{\ensuremath{+2.046}}
\expandafter\gdef\csname R@an.master_table.D2.kits.d3_df\endcsname{2.5}
\expandafter\gdef\csname R@an.master_table.D2.kits.d3_hi\endcsname{\ensuremath{+3.789}}
\expandafter\gdef\csname R@an.master_table.D2.kits.d3_lo\endcsname{\ensuremath{+0.303}}
\expandafter\gdef\csname R@an.master_table.D2.kits.d3_span\endcsname{lies above zero and contains the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.D2.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.D2.kits.dfresh\endcsname{\ensuremath{+1.892}}
\expandafter\gdef\csname R@an.master_table.D2.kits.fresh_max\endcsname{\ensuremath{+1.979}}
\expandafter\gdef\csname R@an.master_table.D2.kits.fresh_min\endcsname{\ensuremath{+1.804}}
\expandafter\gdef\csname R@an.master_table.D2.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.D2.kits.fresh_phrase\endcsname{\ensuremath{+1.892} pp over its two fresh seeds (seed deltas \ensuremath{+1.804} and \ensuremath{+1.979})}
\expandafter\gdef\csname R@an.master_table.D2.kits.fresh_se\endcsname{0.088}
\expandafter\gdef\csname R@an.master_table.D2.kits.fresh_vs_L3\endcsname{\ensuremath{-0.202}}
\expandafter\gdef\csname R@an.master_table.D2.kits.fresh_vs_L3_abs\endcsname{0.202}
\expandafter\gdef\csname R@an.master_table.D2.kits.fresh_vs_L3_dir\endcsname{below}
\expandafter\gdef\csname R@an.master_table.D2.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.D2.kits.ne0\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.master_table.D2.kits.nefresh\endcsname{\ensuremath{+1.892}}
\expandafter\gdef\csname R@an.master_table.D2.kits.nefresh_margin\endcsname{\ensuremath{+1.692}}
\expandafter\gdef\csname R@an.master_table.D2.kits.params\endcsname{26.08}
\expandafter\gdef\csname R@an.master_table.D2.kits.peak\endcsname{7.76}
\expandafter\gdef\csname R@an.master_table.D2.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 1.542 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 1.692 pp}
\expandafter\gdef\csname R@an.master_table.D2.kits.step\endcsname{0.81}
\expandafter\gdef\csname R@an.master_table.D2.params\endcsname{26.03}
\expandafter\gdef\csname R@an.master_table.D2.params_pct_vs_default\endcsname{\ensuremath{-16.4}}
\expandafter\gdef\csname R@an.master_table.D2.peak\endcsname{8.14}
\expandafter\gdef\csname R@an.master_table.D2.step\endcsname{0.81}
\expandafter\gdef\csname R@an.master_table.I1.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.I1.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.params\endcsname{28.85}
\expandafter\gdef\csname R@an.master_table.I1.acdc.peak\endcsname{10.52}
\expandafter\gdef\csname R@an.master_table.I1.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.acdc.step\endcsname{1.64}
\expandafter\gdef\csname R@an.master_table.I1.amos.d0\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.master_table.I1.amos.d0_3\endcsname{\ensuremath{+0.294}}
\expandafter\gdef\csname R@an.master_table.I1.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.I1.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.amos.ne0\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.master_table.I1.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.amos.params\endcsname{29.59}
\expandafter\gdef\csname R@an.master_table.I1.amos.peak\endcsname{10.83}
\expandafter\gdef\csname R@an.master_table.I1.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.amos.step\endcsname{1.53}
\expandafter\gdef\csname R@an.master_table.I1.kits.d0\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.master_table.I1.kits.d0_3\endcsname{\ensuremath{+1.893}}
\expandafter\gdef\csname R@an.master_table.I1.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.I1.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.kits.ne0\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.master_table.I1.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.kits.params\endcsname{29.66}
\expandafter\gdef\csname R@an.master_table.I1.kits.peak\endcsname{9.61}
\expandafter\gdef\csname R@an.master_table.I1.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.I1.kits.step\endcsname{1.41}
\expandafter\gdef\csname R@an.master_table.I1.params\endcsname{29.59}
\expandafter\gdef\csname R@an.master_table.I1.params_pct_vs_default\endcsname{\ensuremath{-4.9}}
\expandafter\gdef\csname R@an.master_table.I1.peak\endcsname{10.83}
\expandafter\gdef\csname R@an.master_table.I1.step\endcsname{1.53}
\expandafter\gdef\csname R@an.master_table.L1.acdc.d0\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.master_table.L1.acdc.d0_3\endcsname{\ensuremath{+0.336}}
\expandafter\gdef\csname R@an.master_table.L1.acdc.d3\endcsname{\ensuremath{+0.273}}
\expandafter\gdef\csname R@an.master_table.L1.acdc.d3_df\endcsname{6.6}
\expandafter\gdef\csname R@an.master_table.L1.acdc.d3_hi\endcsname{\ensuremath{+0.398}}
\expandafter\gdef\csname R@an.master_table.L1.acdc.d3_lo\endcsname{\ensuremath{+0.149}}
\expandafter\gdef\csname R@an.master_table.L1.acdc.d3_span\endcsname{lies above zero and contains the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.L1.acdc.d3_unc\endcsname{\ensuremath{+0.266}}
\expandafter\gdef\csname R@an.master_table.L1.acdc.dfresh\endcsname{\ensuremath{+0.242}}
\expandafter\gdef\csname R@an.master_table.L1.acdc.fresh_max\endcsname{\ensuremath{+0.259}}
\expandafter\gdef\csname R@an.master_table.L1.acdc.fresh_min\endcsname{\ensuremath{+0.225}}
\expandafter\gdef\csname R@an.master_table.L1.acdc.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.L1.acdc.fresh_phrase\endcsname{\ensuremath{+0.242} pp over its two fresh seeds (seed deltas \ensuremath{+0.225} and \ensuremath{+0.259})}
\expandafter\gdef\csname R@an.master_table.L1.acdc.fresh_se\endcsname{0.017}
\expandafter\gdef\csname R@an.master_table.L1.acdc.fresh_vs_L3\endcsname{\ensuremath{-0.208}}
\expandafter\gdef\csname R@an.master_table.L1.acdc.fresh_vs_L3_abs\endcsname{0.208}
\expandafter\gdef\csname R@an.master_table.L1.acdc.fresh_vs_L3_dir\endcsname{below}
\expandafter\gdef\csname R@an.master_table.L1.acdc.fresh_vs_L3_se\endcsname{0.099}
\expandafter\gdef\csname R@an.master_table.L1.acdc.ne0\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.master_table.L1.acdc.nefresh\endcsname{\ensuremath{+0.242}}
\expandafter\gdef\csname R@an.master_table.L1.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L1.acdc.params\endcsname{101.53}
\expandafter\gdef\csname R@an.master_table.L1.acdc.peak\endcsname{10.46}
\expandafter\gdef\csname R@an.master_table.L1.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L1.acdc.step\endcsname{1.51}
\expandafter\gdef\csname R@an.master_table.L1.amos.d0\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.master_table.L1.amos.d0_3\endcsname{\ensuremath{+0.647}}
\expandafter\gdef\csname R@an.master_table.L1.amos.d3\endcsname{\ensuremath{+0.525}}
\expandafter\gdef\csname R@an.master_table.L1.amos.d3_df\endcsname{2.6}
\expandafter\gdef\csname R@an.master_table.L1.amos.d3_hi\endcsname{\ensuremath{+1.003}}
\expandafter\gdef\csname R@an.master_table.L1.amos.d3_lo\endcsname{\ensuremath{+0.047}}
\expandafter\gdef\csname R@an.master_table.L1.amos.d3_span\endcsname{lies above zero and contains the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.L1.amos.d3_unc\endcsname{\ensuremath{+0.497}}
\expandafter\gdef\csname R@an.master_table.L1.amos.dfresh\endcsname{\ensuremath{+0.465}}
\expandafter\gdef\csname R@an.master_table.L1.amos.fresh_max\endcsname{\ensuremath{+0.662}}
\expandafter\gdef\csname R@an.master_table.L1.amos.fresh_min\endcsname{\ensuremath{+0.268}}
\expandafter\gdef\csname R@an.master_table.L1.amos.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.L1.amos.fresh_phrase\endcsname{\ensuremath{+0.465} pp over its two fresh seeds (seed deltas \ensuremath{+0.268} and \ensuremath{+0.662})}
\expandafter\gdef\csname R@an.master_table.L1.amos.fresh_se\endcsname{0.197}
\expandafter\gdef\csname R@an.master_table.L1.amos.fresh_vs_L3\endcsname{\ensuremath{+0.332}}
\expandafter\gdef\csname R@an.master_table.L1.amos.fresh_vs_L3_abs\endcsname{0.332}
\expandafter\gdef\csname R@an.master_table.L1.amos.fresh_vs_L3_dir\endcsname{above}
\expandafter\gdef\csname R@an.master_table.L1.amos.fresh_vs_L3_se\endcsname{0.122}
\expandafter\gdef\csname R@an.master_table.L1.amos.ne0\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.master_table.L1.amos.nefresh\endcsname{\ensuremath{+0.469}}
\expandafter\gdef\csname R@an.master_table.L1.amos.nefresh_margin\endcsname{\ensuremath{+0.269}}
\expandafter\gdef\csname R@an.master_table.L1.amos.params\endcsname{102.28}
\expandafter\gdef\csname R@an.master_table.L1.amos.peak\endcsname{10.93}
\expandafter\gdef\csname R@an.master_table.L1.amos.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 0.115 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 0.269 pp}
\expandafter\gdef\csname R@an.master_table.L1.amos.step\endcsname{1.46}
\expandafter\gdef\csname R@an.master_table.L1.kits.d0\endcsname{\ensuremath{+2.33}}
\expandafter\gdef\csname R@an.master_table.L1.kits.d0_3\endcsname{\ensuremath{+2.326}}
\expandafter\gdef\csname R@an.master_table.L1.kits.d3\endcsname{\ensuremath{+3.092}}
\expandafter\gdef\csname R@an.master_table.L1.kits.d3_df\endcsname{4.0}
\expandafter\gdef\csname R@an.master_table.L1.kits.d3_hi\endcsname{\ensuremath{+4.843}}
\expandafter\gdef\csname R@an.master_table.L1.kits.d3_lo\endcsname{\ensuremath{+1.342}}
\expandafter\gdef\csname R@an.master_table.L1.kits.d3_span\endcsname{lies above the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.L1.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L1.kits.dfresh\endcsname{\ensuremath{+3.475}}
\expandafter\gdef\csname R@an.master_table.L1.kits.fresh_max\endcsname{\ensuremath{+3.817}}
\expandafter\gdef\csname R@an.master_table.L1.kits.fresh_min\endcsname{\ensuremath{+3.134}}
\expandafter\gdef\csname R@an.master_table.L1.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.L1.kits.fresh_phrase\endcsname{\ensuremath{+3.475} pp over its two fresh seeds (seed deltas \ensuremath{+3.134} and \ensuremath{+3.817})}
\expandafter\gdef\csname R@an.master_table.L1.kits.fresh_se\endcsname{0.342}
\expandafter\gdef\csname R@an.master_table.L1.kits.fresh_vs_L3\endcsname{\ensuremath{+1.382}}
\expandafter\gdef\csname R@an.master_table.L1.kits.fresh_vs_L3_abs\endcsname{1.382}
\expandafter\gdef\csname R@an.master_table.L1.kits.fresh_vs_L3_dir\endcsname{above}
\expandafter\gdef\csname R@an.master_table.L1.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.L1.kits.ne0\endcsname{\ensuremath{+2.33}}
\expandafter\gdef\csname R@an.master_table.L1.kits.nefresh\endcsname{\ensuremath{+3.475}}
\expandafter\gdef\csname R@an.master_table.L1.kits.nefresh_margin\endcsname{\ensuremath{+3.275}}
\expandafter\gdef\csname R@an.master_table.L1.kits.params\endcsname{102.35}
\expandafter\gdef\csname R@an.master_table.L1.kits.peak\endcsname{9.73}
\expandafter\gdef\csname R@an.master_table.L1.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 3.125 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 3.275 pp}
\expandafter\gdef\csname R@an.master_table.L1.kits.step\endcsname{1.33}
\expandafter\gdef\csname R@an.master_table.L1.params\endcsname{102.28}
\expandafter\gdef\csname R@an.master_table.L1.params_pct_vs_default\endcsname{\ensuremath{+228.7}}
\expandafter\gdef\csname R@an.master_table.L1.peak\endcsname{10.93}
\expandafter\gdef\csname R@an.master_table.L1.step\endcsname{1.46}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.d0\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.d0_3\endcsname{\ensuremath{+0.283}}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.d3\endcsname{\ensuremath{+0.307}}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.d3_df\endcsname{6.9}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.d3_hi\endcsname{\ensuremath{+0.416}}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.d3_lo\endcsname{\ensuremath{+0.198}}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.d3_span\endcsname{lies above zero and contains the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.d3_unc\endcsname{\ensuremath{+0.300}}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.dfresh\endcsname{\ensuremath{+0.319}}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.fresh_max\endcsname{\ensuremath{+0.352}}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.fresh_min\endcsname{\ensuremath{+0.286}}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.fresh_phrase\endcsname{\ensuremath{+0.319} pp over its two fresh seeds (seed deltas \ensuremath{+0.286} and \ensuremath{+0.352})}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.fresh_se\endcsname{0.033}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.fresh_vs_L3\endcsname{\ensuremath{-0.131}}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.fresh_vs_L3_abs\endcsname{0.131}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.fresh_vs_L3_dir\endcsname{below}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.fresh_vs_L3_se\endcsname{0.099}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.ne0\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.nefresh\endcsname{\ensuremath{+0.319}}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.params\endcsname{101.63}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.peak\endcsname{10.56}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L1b.acdc.step\endcsname{1.41}
\expandafter\gdef\csname R@an.master_table.L1b.amos.d0\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.master_table.L1b.amos.d0_3\endcsname{\ensuremath{+0.138}}
\expandafter\gdef\csname R@an.master_table.L1b.amos.d3\endcsname{\ensuremath{+0.244}}
\expandafter\gdef\csname R@an.master_table.L1b.amos.d3_df\endcsname{3.3}
\expandafter\gdef\csname R@an.master_table.L1b.amos.d3_hi\endcsname{\ensuremath{+0.561}}
\expandafter\gdef\csname R@an.master_table.L1b.amos.d3_lo\endcsname{\ensuremath{-0.073}}
\expandafter\gdef\csname R@an.master_table.L1b.amos.d3_span\endcsname{spans both zero and the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.L1b.amos.d3_unc\endcsname{\ensuremath{+0.216}}
\expandafter\gdef\csname R@an.master_table.L1b.amos.dfresh\endcsname{\ensuremath{+0.298}}
\expandafter\gdef\csname R@an.master_table.L1b.amos.fresh_max\endcsname{\ensuremath{+0.426}}
\expandafter\gdef\csname R@an.master_table.L1b.amos.fresh_min\endcsname{\ensuremath{+0.169}}
\expandafter\gdef\csname R@an.master_table.L1b.amos.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.L1b.amos.fresh_phrase\endcsname{\ensuremath{+0.298} pp over its two fresh seeds (seed deltas \ensuremath{+0.169} and \ensuremath{+0.426})}
\expandafter\gdef\csname R@an.master_table.L1b.amos.fresh_se\endcsname{0.129}
\expandafter\gdef\csname R@an.master_table.L1b.amos.fresh_vs_L3\endcsname{\ensuremath{+0.165}}
\expandafter\gdef\csname R@an.master_table.L1b.amos.fresh_vs_L3_abs\endcsname{0.165}
\expandafter\gdef\csname R@an.master_table.L1b.amos.fresh_vs_L3_dir\endcsname{above}
\expandafter\gdef\csname R@an.master_table.L1b.amos.fresh_vs_L3_se\endcsname{0.122}
\expandafter\gdef\csname R@an.master_table.L1b.amos.ne0\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.master_table.L1b.amos.nefresh\endcsname{\ensuremath{+0.445}}
\expandafter\gdef\csname R@an.master_table.L1b.amos.nefresh_margin\endcsname{\ensuremath{+0.245}}
\expandafter\gdef\csname R@an.master_table.L1b.amos.params\endcsname{102.37}
\expandafter\gdef\csname R@an.master_table.L1b.amos.peak\endcsname{10.60}
\expandafter\gdef\csname R@an.master_table.L1b.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L1b.amos.step\endcsname{1.38}
\expandafter\gdef\csname R@an.master_table.L1b.kits.d0\endcsname{\ensuremath{+1.74}}
\expandafter\gdef\csname R@an.master_table.L1b.kits.d0_3\endcsname{\ensuremath{+1.743}}
\expandafter\gdef\csname R@an.master_table.L1b.kits.d3\endcsname{\ensuremath{+2.123}}
\expandafter\gdef\csname R@an.master_table.L1b.kits.d3_df\endcsname{3.0}
\expandafter\gdef\csname R@an.master_table.L1b.kits.d3_hi\endcsname{\ensuremath{+3.766}}
\expandafter\gdef\csname R@an.master_table.L1b.kits.d3_lo\endcsname{\ensuremath{+0.480}}
\expandafter\gdef\csname R@an.master_table.L1b.kits.d3_span\endcsname{lies above the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.L1b.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L1b.kits.dfresh\endcsname{\ensuremath{+2.313}}
\expandafter\gdef\csname R@an.master_table.L1b.kits.fresh_max\endcsname{\ensuremath{+2.564}}
\expandafter\gdef\csname R@an.master_table.L1b.kits.fresh_min\endcsname{\ensuremath{+2.062}}
\expandafter\gdef\csname R@an.master_table.L1b.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.L1b.kits.fresh_phrase\endcsname{\ensuremath{+2.313} pp over its two fresh seeds (seed deltas \ensuremath{+2.062} and \ensuremath{+2.564})}
\expandafter\gdef\csname R@an.master_table.L1b.kits.fresh_se\endcsname{0.251}
\expandafter\gdef\csname R@an.master_table.L1b.kits.fresh_vs_L3\endcsname{\ensuremath{+0.220}}
\expandafter\gdef\csname R@an.master_table.L1b.kits.fresh_vs_L3_abs\endcsname{0.220}
\expandafter\gdef\csname R@an.master_table.L1b.kits.fresh_vs_L3_dir\endcsname{above}
\expandafter\gdef\csname R@an.master_table.L1b.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.L1b.kits.ne0\endcsname{\ensuremath{+1.74}}
\expandafter\gdef\csname R@an.master_table.L1b.kits.nefresh\endcsname{\ensuremath{+2.313}}
\expandafter\gdef\csname R@an.master_table.L1b.kits.nefresh_margin\endcsname{\ensuremath{+2.113}}
\expandafter\gdef\csname R@an.master_table.L1b.kits.params\endcsname{102.43}
\expandafter\gdef\csname R@an.master_table.L1b.kits.peak\endcsname{9.43}
\expandafter\gdef\csname R@an.master_table.L1b.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 1.963 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 2.113 pp}
\expandafter\gdef\csname R@an.master_table.L1b.kits.step\endcsname{1.23}
\expandafter\gdef\csname R@an.master_table.L1b.params\endcsname{102.37}
\expandafter\gdef\csname R@an.master_table.L1b.params_pct_vs_default\endcsname{\ensuremath{+229.0}}
\expandafter\gdef\csname R@an.master_table.L1b.peak\endcsname{10.60}
\expandafter\gdef\csname R@an.master_table.L1b.step\endcsname{1.38}
\expandafter\gdef\csname R@an.master_table.L2.acdc.d0\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.master_table.L2.acdc.d0_3\endcsname{\ensuremath{-0.015}}
\expandafter\gdef\csname R@an.master_table.L2.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L2.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L2.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L2.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L2.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L2.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L2.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L2.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L2.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L2.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L2.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.L2.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L2.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L2.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L2.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L2.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L2.acdc.ne0\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.master_table.L2.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L2.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L2.acdc.params\endcsname{23.68}
\expandafter\gdef\csname R@an.master_table.L2.acdc.peak\endcsname{11.42}
\expandafter\gdef\csname R@an.master_table.L2.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L2.acdc.step\endcsname{1.50}
\expandafter\gdef\csname R@an.master_table.L2.amos.d0\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.master_table.L2.amos.d0_3\endcsname{\ensuremath{+0.362}}
\expandafter\gdef\csname R@an.master_table.L2.amos.d3\endcsname{\ensuremath{+0.250}}
\expandafter\gdef\csname R@an.master_table.L2.amos.d3_df\endcsname{4.4}
\expandafter\gdef\csname R@an.master_table.L2.amos.d3_hi\endcsname{\ensuremath{+0.472}}
\expandafter\gdef\csname R@an.master_table.L2.amos.d3_lo\endcsname{\ensuremath{+0.028}}
\expandafter\gdef\csname R@an.master_table.L2.amos.d3_span\endcsname{lies above zero and contains the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.L2.amos.d3_unc\endcsname{\ensuremath{+0.221}}
\expandafter\gdef\csname R@an.master_table.L2.amos.dfresh\endcsname{\ensuremath{+0.194}}
\expandafter\gdef\csname R@an.master_table.L2.amos.fresh_max\endcsname{\ensuremath{+0.255}}
\expandafter\gdef\csname R@an.master_table.L2.amos.fresh_min\endcsname{\ensuremath{+0.134}}
\expandafter\gdef\csname R@an.master_table.L2.amos.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.L2.amos.fresh_phrase\endcsname{\ensuremath{+0.194} pp over its two fresh seeds (seed deltas \ensuremath{+0.134} and \ensuremath{+0.255})}
\expandafter\gdef\csname R@an.master_table.L2.amos.fresh_se\endcsname{0.061}
\expandafter\gdef\csname R@an.master_table.L2.amos.fresh_vs_L3\endcsname{\ensuremath{+0.062}}
\expandafter\gdef\csname R@an.master_table.L2.amos.fresh_vs_L3_abs\endcsname{0.062}
\expandafter\gdef\csname R@an.master_table.L2.amos.fresh_vs_L3_dir\endcsname{above}
\expandafter\gdef\csname R@an.master_table.L2.amos.fresh_vs_L3_se\endcsname{0.122}
\expandafter\gdef\csname R@an.master_table.L2.amos.ne0\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.master_table.L2.amos.nefresh\endcsname{\ensuremath{+0.266}}
\expandafter\gdef\csname R@an.master_table.L2.amos.nefresh_margin\endcsname{\ensuremath{+0.066}}
\expandafter\gdef\csname R@an.master_table.L2.amos.params\endcsname{24.43}
\expandafter\gdef\csname R@an.master_table.L2.amos.peak\endcsname{9.93}
\expandafter\gdef\csname R@an.master_table.L2.amos.rule_phrase\endcsname{the fresh mean falls short of the \ensuremath{+0.35} pp primary bar by 0.156 pp while the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 0.066 pp, so the registered rule is decided by the primary leg alone}
\expandafter\gdef\csname R@an.master_table.L2.amos.step\endcsname{1.46}
\expandafter\gdef\csname R@an.master_table.L2.kits.d0\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.master_table.L2.kits.d0_3\endcsname{\ensuremath{+0.664}}
\expandafter\gdef\csname R@an.master_table.L2.kits.d3\endcsname{\ensuremath{+0.295}}
\expandafter\gdef\csname R@an.master_table.L2.kits.d3_df\endcsname{3.9}
\expandafter\gdef\csname R@an.master_table.L2.kits.d3_hi\endcsname{\ensuremath{+2.335}}
\expandafter\gdef\csname R@an.master_table.L2.kits.d3_lo\endcsname{\ensuremath{-1.746}}
\expandafter\gdef\csname R@an.master_table.L2.kits.d3_span\endcsname{spans both zero and the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.L2.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L2.kits.dfresh\endcsname{\ensuremath{+0.110}}
\expandafter\gdef\csname R@an.master_table.L2.kits.fresh_max\endcsname{\ensuremath{+1.026}}
\expandafter\gdef\csname R@an.master_table.L2.kits.fresh_min\endcsname{\ensuremath{-0.805}}
\expandafter\gdef\csname R@an.master_table.L2.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.L2.kits.fresh_phrase\endcsname{\ensuremath{+0.110} pp over its two fresh seeds (seed deltas \ensuremath{-0.805} and \ensuremath{+1.026})}
\expandafter\gdef\csname R@an.master_table.L2.kits.fresh_se\endcsname{0.915}
\expandafter\gdef\csname R@an.master_table.L2.kits.fresh_vs_L3\endcsname{\ensuremath{-1.983}}
\expandafter\gdef\csname R@an.master_table.L2.kits.fresh_vs_L3_abs\endcsname{1.983}
\expandafter\gdef\csname R@an.master_table.L2.kits.fresh_vs_L3_dir\endcsname{below}
\expandafter\gdef\csname R@an.master_table.L2.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.L2.kits.ne0\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.master_table.L2.kits.nefresh\endcsname{\ensuremath{+0.110}}
\expandafter\gdef\csname R@an.master_table.L2.kits.nefresh_margin\endcsname{\ensuremath{-0.090}}
\expandafter\gdef\csname R@an.master_table.L2.kits.params\endcsname{24.50}
\expandafter\gdef\csname R@an.master_table.L2.kits.peak\endcsname{9.12}
\expandafter\gdef\csname R@an.master_table.L2.kits.rule_phrase\endcsname{both legs of the registered rule fall short: the fresh mean falls short of the \ensuremath{+0.35} pp primary bar by 0.240 pp and the non-empty-reference fresh mean falls short of the \ensuremath{+0.20} pp secondary bar by 0.090 pp}
\expandafter\gdef\csname R@an.master_table.L2.kits.step\endcsname{1.33}
\expandafter\gdef\csname R@an.master_table.L2.params\endcsname{24.43}
\expandafter\gdef\csname R@an.master_table.L2.params_pct_vs_default\endcsname{\ensuremath{-21.5}}
\expandafter\gdef\csname R@an.master_table.L2.peak\endcsname{9.93}
\expandafter\gdef\csname R@an.master_table.L2.step\endcsname{1.46}
\expandafter\gdef\csname R@an.master_table.L3.acdc.d0\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.master_table.L3.acdc.d0_3\endcsname{\ensuremath{+0.616}}
\expandafter\gdef\csname R@an.master_table.L3.acdc.d3\endcsname{\ensuremath{+0.506}}
\expandafter\gdef\csname R@an.master_table.L3.acdc.d3_df\endcsname{4.0}
\expandafter\gdef\csname R@an.master_table.L3.acdc.d3_hi\endcsname{\ensuremath{+0.703}}
\expandafter\gdef\csname R@an.master_table.L3.acdc.d3_lo\endcsname{\ensuremath{+0.308}}
\expandafter\gdef\csname R@an.master_table.L3.acdc.d3_span\endcsname{lies above zero and contains the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.L3.acdc.d3_unc\endcsname{\ensuremath{+0.499}}
\expandafter\gdef\csname R@an.master_table.L3.acdc.dfresh\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.master_table.L3.acdc.fresh_max\endcsname{\ensuremath{+0.484}}
\expandafter\gdef\csname R@an.master_table.L3.acdc.fresh_min\endcsname{\ensuremath{+0.417}}
\expandafter\gdef\csname R@an.master_table.L3.acdc.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.L3.acdc.fresh_phrase\endcsname{\ensuremath{+0.450} pp over its two fresh seeds (seed deltas \ensuremath{+0.417} and \ensuremath{+0.484})}
\expandafter\gdef\csname R@an.master_table.L3.acdc.fresh_se\endcsname{0.033}
\expandafter\gdef\csname R@an.master_table.L3.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3.acdc.ne0\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.master_table.L3.acdc.nefresh\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.master_table.L3.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3.acdc.params\endcsname{28.85}
\expandafter\gdef\csname R@an.master_table.L3.acdc.peak\endcsname{10.43}
\expandafter\gdef\csname R@an.master_table.L3.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3.acdc.step\endcsname{1.64}
\expandafter\gdef\csname R@an.master_table.L3.amos.d0\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.master_table.L3.amos.d0_3\endcsname{\ensuremath{+0.382}}
\expandafter\gdef\csname R@an.master_table.L3.amos.d3\endcsname{\ensuremath{+0.215}}
\expandafter\gdef\csname R@an.master_table.L3.amos.d3_df\endcsname{2.7}
\expandafter\gdef\csname R@an.master_table.L3.amos.d3_hi\endcsname{\ensuremath{+0.650}}
\expandafter\gdef\csname R@an.master_table.L3.amos.d3_lo\endcsname{\ensuremath{-0.220}}
\expandafter\gdef\csname R@an.master_table.L3.amos.d3_span\endcsname{spans both zero and the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.L3.amos.d3_unc\endcsname{\ensuremath{+0.187}}
\expandafter\gdef\csname R@an.master_table.L3.amos.dfresh\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.master_table.L3.amos.fresh_max\endcsname{\ensuremath{+0.280}}
\expandafter\gdef\csname R@an.master_table.L3.amos.fresh_min\endcsname{\ensuremath{-0.016}}
\expandafter\gdef\csname R@an.master_table.L3.amos.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.L3.amos.fresh_phrase\endcsname{\ensuremath{+0.132} pp over its two fresh seeds (seed deltas \ensuremath{-0.016} and \ensuremath{+0.280})}
\expandafter\gdef\csname R@an.master_table.L3.amos.fresh_se\endcsname{0.148}
\expandafter\gdef\csname R@an.master_table.L3.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3.amos.ne0\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.master_table.L3.amos.nefresh\endcsname{\ensuremath{+0.204}}
\expandafter\gdef\csname R@an.master_table.L3.amos.nefresh_margin\endcsname{\ensuremath{+0.004}}
\expandafter\gdef\csname R@an.master_table.L3.amos.params\endcsname{29.59}
\expandafter\gdef\csname R@an.master_table.L3.amos.peak\endcsname{10.74}
\expandafter\gdef\csname R@an.master_table.L3.amos.rule_phrase\endcsname{the fresh mean falls short of the \ensuremath{+0.35} pp primary bar by 0.218 pp while the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 0.004 pp, so the registered rule is decided by the primary leg alone}
\expandafter\gdef\csname R@an.master_table.L3.amos.step\endcsname{1.53}
\expandafter\gdef\csname R@an.master_table.L3.kits.d0\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.master_table.L3.kits.d0_3\endcsname{\ensuremath{+2.842}}
\expandafter\gdef\csname R@an.master_table.L3.kits.d3\endcsname{\ensuremath{+2.343}}
\expandafter\gdef\csname R@an.master_table.L3.kits.d3_df\endcsname{3.5}
\expandafter\gdef\csname R@an.master_table.L3.kits.d3_hi\endcsname{\ensuremath{+3.967}}
\expandafter\gdef\csname R@an.master_table.L3.kits.d3_lo\endcsname{\ensuremath{+0.719}}
\expandafter\gdef\csname R@an.master_table.L3.kits.d3_span\endcsname{lies above the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.L3.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3.kits.dfresh\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.master_table.L3.kits.fresh_max\endcsname{\ensuremath{+2.390}}
\expandafter\gdef\csname R@an.master_table.L3.kits.fresh_min\endcsname{\ensuremath{+1.798}}
\expandafter\gdef\csname R@an.master_table.L3.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.L3.kits.fresh_phrase\endcsname{\ensuremath{+2.094} pp over its two fresh seeds (seed deltas \ensuremath{+1.798} and \ensuremath{+2.390})}
\expandafter\gdef\csname R@an.master_table.L3.kits.fresh_se\endcsname{0.296}
\expandafter\gdef\csname R@an.master_table.L3.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3.kits.ne0\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.master_table.L3.kits.nefresh\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.master_table.L3.kits.nefresh_margin\endcsname{\ensuremath{+1.894}}
\expandafter\gdef\csname R@an.master_table.L3.kits.params\endcsname{29.66}
\expandafter\gdef\csname R@an.master_table.L3.kits.peak\endcsname{9.56}
\expandafter\gdef\csname R@an.master_table.L3.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 1.744 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 1.894 pp}
\expandafter\gdef\csname R@an.master_table.L3.kits.step\endcsname{1.40}
\expandafter\gdef\csname R@an.master_table.L3.params\endcsname{29.59}
\expandafter\gdef\csname R@an.master_table.L3.params_pct_vs_default\endcsname{\ensuremath{-4.9}}
\expandafter\gdef\csname R@an.master_table.L3.peak\endcsname{10.74}
\expandafter\gdef\csname R@an.master_table.L3.step\endcsname{1.53}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.params\endcsname{27.83}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.peak\endcsname{10.42}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.acdc.step\endcsname{1.38}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.d0\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.d0_3\endcsname{\ensuremath{+0.459}}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.ne0\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.params\endcsname{28.58}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.peak\endcsname{10.74}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.amos.step\endcsname{1.35}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.d0\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.d0_3\endcsname{\ensuremath{+1.366}}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.ne0\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.params\endcsname{28.65}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.peak\endcsname{9.56}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3k3.kits.step\endcsname{1.27}
\expandafter\gdef\csname R@an.master_table.L3k3.params\endcsname{28.58}
\expandafter\gdef\csname R@an.master_table.L3k3.params_pct_vs_default\endcsname{\ensuremath{-8.2}}
\expandafter\gdef\csname R@an.master_table.L3k3.peak\endcsname{10.74}
\expandafter\gdef\csname R@an.master_table.L3k3.step\endcsname{1.35}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.params\endcsname{28.82}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.peak\endcsname{11.70}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.acdc.step\endcsname{1.59}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.d0\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.d0_3\endcsname{\ensuremath{+0.268}}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.ne0\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.params\endcsname{29.57}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.peak\endcsname{10.51}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.amos.step\endcsname{1.49}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.d0\endcsname{\ensuremath{+2.56}}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.d0_3\endcsname{\ensuremath{+2.561}}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.ne0\endcsname{\ensuremath{+2.56}}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.params\endcsname{29.64}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.peak\endcsname{9.44}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3ng.kits.step\endcsname{1.38}
\expandafter\gdef\csname R@an.master_table.L3ng.params\endcsname{29.57}
\expandafter\gdef\csname R@an.master_table.L3ng.params_pct_vs_default\endcsname{\ensuremath{-5.0}}
\expandafter\gdef\csname R@an.master_table.L3ng.peak\endcsname{10.51}
\expandafter\gdef\csname R@an.master_table.L3ng.step\endcsname{1.49}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.params\endcsname{96.82}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.peak\endcsname{11.72}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.acdc.step\endcsname{2.11}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.ne0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.params\endcsname{99.79}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.peak\endcsname{11.30}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.amos.step\endcsname{1.87}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.ne0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.params\endcsname{99.85}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.peak\endcsname{10.33}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_L.kits.step\endcsname{1.66}
\expandafter\gdef\csname R@an.master_table.L3w_L.params\endcsname{99.79}
\expandafter\gdef\csname R@an.master_table.L3w_L.params_pct_vs_default\endcsname{\ensuremath{+220.7}}
\expandafter\gdef\csname R@an.master_table.L3w_L.peak\endcsname{11.30}
\expandafter\gdef\csname R@an.master_table.L3w_L.step\endcsname{1.87}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.params\endcsname{57.36}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.peak\endcsname{11.06}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.acdc.step\endcsname{1.88}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.ne0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.params\endcsname{59.03}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.peak\endcsname{11.24}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.amos.step\endcsname{1.70}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.ne0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.params\endcsname{59.10}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.peak\endcsname{9.91}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L3w_M.kits.step\endcsname{1.54}
\expandafter\gdef\csname R@an.master_table.L3w_M.params\endcsname{59.03}
\expandafter\gdef\csname R@an.master_table.L3w_M.params_pct_vs_default\endcsname{\ensuremath{+89.7}}
\expandafter\gdef\csname R@an.master_table.L3w_M.peak\endcsname{11.24}
\expandafter\gdef\csname R@an.master_table.L3w_M.step\endcsname{1.70}
\expandafter\gdef\csname R@an.master_table.L4.acdc.d0\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.master_table.L4.acdc.d0_3\endcsname{\ensuremath{+0.315}}
\expandafter\gdef\csname R@an.master_table.L4.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L4.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L4.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L4.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L4.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L4.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L4.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L4.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L4.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L4.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L4.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.L4.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L4.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L4.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L4.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L4.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L4.acdc.ne0\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.master_table.L4.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L4.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L4.acdc.params\endcsname{102.02}
\expandafter\gdef\csname R@an.master_table.L4.acdc.peak\endcsname{10.27}
\expandafter\gdef\csname R@an.master_table.L4.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L4.acdc.step\endcsname{1.52}
\expandafter\gdef\csname R@an.master_table.L4.amos.d0\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.master_table.L4.amos.d0_3\endcsname{\ensuremath{+0.430}}
\expandafter\gdef\csname R@an.master_table.L4.amos.d3\endcsname{\ensuremath{+0.446}}
\expandafter\gdef\csname R@an.master_table.L4.amos.d3_df\endcsname{4.8}
\expandafter\gdef\csname R@an.master_table.L4.amos.d3_hi\endcsname{\ensuremath{+0.648}}
\expandafter\gdef\csname R@an.master_table.L4.amos.d3_lo\endcsname{\ensuremath{+0.244}}
\expandafter\gdef\csname R@an.master_table.L4.amos.d3_span\endcsname{lies above zero and contains the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.L4.amos.d3_unc\endcsname{\ensuremath{+0.417}}
\expandafter\gdef\csname R@an.master_table.L4.amos.dfresh\endcsname{\ensuremath{+0.455}}
\expandafter\gdef\csname R@an.master_table.L4.amos.fresh_max\endcsname{\ensuremath{+0.557}}
\expandafter\gdef\csname R@an.master_table.L4.amos.fresh_min\endcsname{\ensuremath{+0.352}}
\expandafter\gdef\csname R@an.master_table.L4.amos.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.L4.amos.fresh_phrase\endcsname{\ensuremath{+0.455} pp over its two fresh seeds (seed deltas \ensuremath{+0.352} and \ensuremath{+0.557})}
\expandafter\gdef\csname R@an.master_table.L4.amos.fresh_se\endcsname{0.102}
\expandafter\gdef\csname R@an.master_table.L4.amos.fresh_vs_L3\endcsname{\ensuremath{+0.322}}
\expandafter\gdef\csname R@an.master_table.L4.amos.fresh_vs_L3_abs\endcsname{0.322}
\expandafter\gdef\csname R@an.master_table.L4.amos.fresh_vs_L3_dir\endcsname{above}
\expandafter\gdef\csname R@an.master_table.L4.amos.fresh_vs_L3_se\endcsname{0.122}
\expandafter\gdef\csname R@an.master_table.L4.amos.ne0\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.master_table.L4.amos.nefresh\endcsname{\ensuremath{+0.379}}
\expandafter\gdef\csname R@an.master_table.L4.amos.nefresh_margin\endcsname{\ensuremath{+0.179}}
\expandafter\gdef\csname R@an.master_table.L4.amos.params\endcsname{102.77}
\expandafter\gdef\csname R@an.master_table.L4.amos.peak\endcsname{10.75}
\expandafter\gdef\csname R@an.master_table.L4.amos.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 0.105 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 0.179 pp}
\expandafter\gdef\csname R@an.master_table.L4.amos.step\endcsname{1.46}
\expandafter\gdef\csname R@an.master_table.L4.kits.d0\endcsname{\ensuremath{+2.20}}
\expandafter\gdef\csname R@an.master_table.L4.kits.d0_3\endcsname{\ensuremath{+2.198}}
\expandafter\gdef\csname R@an.master_table.L4.kits.d3\endcsname{\ensuremath{+2.230}}
\expandafter\gdef\csname R@an.master_table.L4.kits.d3_df\endcsname{3.1}
\expandafter\gdef\csname R@an.master_table.L4.kits.d3_hi\endcsname{\ensuremath{+3.866}}
\expandafter\gdef\csname R@an.master_table.L4.kits.d3_lo\endcsname{\ensuremath{+0.594}}
\expandafter\gdef\csname R@an.master_table.L4.kits.d3_span\endcsname{lies above the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.L4.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L4.kits.dfresh\endcsname{\ensuremath{+2.246}}
\expandafter\gdef\csname R@an.master_table.L4.kits.fresh_max\endcsname{\ensuremath{+2.677}}
\expandafter\gdef\csname R@an.master_table.L4.kits.fresh_min\endcsname{\ensuremath{+1.815}}
\expandafter\gdef\csname R@an.master_table.L4.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.L4.kits.fresh_phrase\endcsname{\ensuremath{+2.246} pp over its two fresh seeds (seed deltas \ensuremath{+1.815} and \ensuremath{+2.677})}
\expandafter\gdef\csname R@an.master_table.L4.kits.fresh_se\endcsname{0.431}
\expandafter\gdef\csname R@an.master_table.L4.kits.fresh_vs_L3\endcsname{\ensuremath{+0.153}}
\expandafter\gdef\csname R@an.master_table.L4.kits.fresh_vs_L3_abs\endcsname{0.153}
\expandafter\gdef\csname R@an.master_table.L4.kits.fresh_vs_L3_dir\endcsname{above}
\expandafter\gdef\csname R@an.master_table.L4.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.L4.kits.ne0\endcsname{\ensuremath{+2.20}}
\expandafter\gdef\csname R@an.master_table.L4.kits.nefresh\endcsname{\ensuremath{+2.246}}
\expandafter\gdef\csname R@an.master_table.L4.kits.nefresh_margin\endcsname{\ensuremath{+2.046}}
\expandafter\gdef\csname R@an.master_table.L4.kits.params\endcsname{102.82}
\expandafter\gdef\csname R@an.master_table.L4.kits.peak\endcsname{9.52}
\expandafter\gdef\csname R@an.master_table.L4.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 1.896 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 2.046 pp}
\expandafter\gdef\csname R@an.master_table.L4.kits.step\endcsname{1.30}
\expandafter\gdef\csname R@an.master_table.L4.params\endcsname{102.77}
\expandafter\gdef\csname R@an.master_table.L4.params_pct_vs_default\endcsname{\ensuremath{+230.2}}
\expandafter\gdef\csname R@an.master_table.L4.peak\endcsname{10.75}
\expandafter\gdef\csname R@an.master_table.L4.step\endcsname{1.46}
\expandafter\gdef\csname R@an.master_table.L6.acdc.d0\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.master_table.L6.acdc.d0_3\endcsname{\ensuremath{+0.451}}
\expandafter\gdef\csname R@an.master_table.L6.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.L6.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.acdc.ne0\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.master_table.L6.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.acdc.params\endcsname{30.35}
\expandafter\gdef\csname R@an.master_table.L6.acdc.peak\endcsname{11.49}
\expandafter\gdef\csname R@an.master_table.L6.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.acdc.step\endcsname{2.03}
\expandafter\gdef\csname R@an.master_table.L6.amos.d0\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.master_table.L6.amos.d0_3\endcsname{\ensuremath{+0.016}}
\expandafter\gdef\csname R@an.master_table.L6.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.L6.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.amos.ne0\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.master_table.L6.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.amos.params\endcsname{31.09}
\expandafter\gdef\csname R@an.master_table.L6.amos.peak\endcsname{10.27}
\expandafter\gdef\csname R@an.master_table.L6.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.amos.step\endcsname{1.88}
\expandafter\gdef\csname R@an.master_table.L6.kits.d0\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.master_table.L6.kits.d0_3\endcsname{\ensuremath{+2.526}}
\expandafter\gdef\csname R@an.master_table.L6.kits.d3\endcsname{\ensuremath{+1.903}}
\expandafter\gdef\csname R@an.master_table.L6.kits.d3_df\endcsname{3.9}
\expandafter\gdef\csname R@an.master_table.L6.kits.d3_hi\endcsname{\ensuremath{+3.587}}
\expandafter\gdef\csname R@an.master_table.L6.kits.d3_lo\endcsname{\ensuremath{+0.219}}
\expandafter\gdef\csname R@an.master_table.L6.kits.d3_span\endcsname{lies above zero and contains the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.L6.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.L6.kits.dfresh\endcsname{\ensuremath{+1.591}}
\expandafter\gdef\csname R@an.master_table.L6.kits.fresh_max\endcsname{\ensuremath{+1.984}}
\expandafter\gdef\csname R@an.master_table.L6.kits.fresh_min\endcsname{\ensuremath{+1.198}}
\expandafter\gdef\csname R@an.master_table.L6.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.L6.kits.fresh_phrase\endcsname{\ensuremath{+1.591} pp over its two fresh seeds (seed deltas \ensuremath{+1.198} and \ensuremath{+1.984})}
\expandafter\gdef\csname R@an.master_table.L6.kits.fresh_se\endcsname{0.393}
\expandafter\gdef\csname R@an.master_table.L6.kits.fresh_vs_L3\endcsname{\ensuremath{-0.502}}
\expandafter\gdef\csname R@an.master_table.L6.kits.fresh_vs_L3_abs\endcsname{0.502}
\expandafter\gdef\csname R@an.master_table.L6.kits.fresh_vs_L3_dir\endcsname{below}
\expandafter\gdef\csname R@an.master_table.L6.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.L6.kits.ne0\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.master_table.L6.kits.nefresh\endcsname{\ensuremath{+1.591}}
\expandafter\gdef\csname R@an.master_table.L6.kits.nefresh_margin\endcsname{\ensuremath{+1.391}}
\expandafter\gdef\csname R@an.master_table.L6.kits.params\endcsname{31.17}
\expandafter\gdef\csname R@an.master_table.L6.kits.peak\endcsname{9.33}
\expandafter\gdef\csname R@an.master_table.L6.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 1.241 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 1.391 pp}
\expandafter\gdef\csname R@an.master_table.L6.kits.step\endcsname{1.63}
\expandafter\gdef\csname R@an.master_table.L6.params\endcsname{31.09}
\expandafter\gdef\csname R@an.master_table.L6.params_pct_vs_default\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.master_table.L6.peak\endcsname{10.27}
\expandafter\gdef\csname R@an.master_table.L6.step\endcsname{1.88}
\expandafter\gdef\csname R@an.master_table.N1.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.N1.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.params\endcsname{30.38}
\expandafter\gdef\csname R@an.master_table.N1.acdc.peak\endcsname{10.27}
\expandafter\gdef\csname R@an.master_table.N1.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.acdc.step\endcsname{1.60}
\expandafter\gdef\csname R@an.master_table.N1.amos.d0\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@an.master_table.N1.amos.d0_3\endcsname{\ensuremath{-0.923}}
\expandafter\gdef\csname R@an.master_table.N1.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.N1.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.amos.ne0\endcsname{\ensuremath{-0.80}}
\expandafter\gdef\csname R@an.master_table.N1.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.amos.params\endcsname{31.12}
\expandafter\gdef\csname R@an.master_table.N1.amos.peak\endcsname{9.01}
\expandafter\gdef\csname R@an.master_table.N1.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.amos.step\endcsname{2.06}
\expandafter\gdef\csname R@an.master_table.N1.kits.d0\endcsname{\ensuremath{-6.49}}
\expandafter\gdef\csname R@an.master_table.N1.kits.d0_3\endcsname{\ensuremath{-6.492}}
\expandafter\gdef\csname R@an.master_table.N1.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.N1.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.kits.ne0\endcsname{\ensuremath{-6.49}}
\expandafter\gdef\csname R@an.master_table.N1.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.kits.params\endcsname{31.20}
\expandafter\gdef\csname R@an.master_table.N1.kits.peak\endcsname{8.51}
\expandafter\gdef\csname R@an.master_table.N1.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.N1.kits.step\endcsname{2.14}
\expandafter\gdef\csname R@an.master_table.N1.params\endcsname{31.12}
\expandafter\gdef\csname R@an.master_table.N1.params_pct_vs_default\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.master_table.N1.peak\endcsname{9.01}
\expandafter\gdef\csname R@an.master_table.N1.step\endcsname{2.06}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.params\endcsname{30.45}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.peak\endcsname{11.05}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.acdc.step\endcsname{2.15}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.ne0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.params\endcsname{31.20}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.peak\endcsname{10.94}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.amos.step\endcsname{2.15}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.ne0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.params\endcsname{31.42}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.peak\endcsname{9.59}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.kits.step\endcsname{2.65}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.params\endcsname{31.20}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.params_pct_vs_default\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.peak\endcsname{10.94}
\expandafter\gdef\csname R@an.master_table.P1_frcap32.step\endcsname{2.15}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.params\endcsname{30.45}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.peak\endcsname{10.27}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.acdc.step\endcsname{1.09}
\expandafter\gdef\csname R@an.master_table.P1b.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P1b.amos.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P1b.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.P1b.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.amos.ne0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P1b.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.amos.params\endcsname{31.20}
\expandafter\gdef\csname R@an.master_table.P1b.amos.peak\endcsname{9.01}
\expandafter\gdef\csname R@an.master_table.P1b.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.amos.step\endcsname{1.07}
\expandafter\gdef\csname R@an.master_table.P1b.kits.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.P1b.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.params\endcsname{31.20}
\expandafter\gdef\csname R@an.master_table.P1b.kits.peak\endcsname{8.51}
\expandafter\gdef\csname R@an.master_table.P1b.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1b.kits.step\endcsname{1.01}
\expandafter\gdef\csname R@an.master_table.P1b.params\endcsname{31.20}
\expandafter\gdef\csname R@an.master_table.P1b.params_pct_vs_default\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.master_table.P1b.peak\endcsname{9.01}
\expandafter\gdef\csname R@an.master_table.P1b.step\endcsname{1.07}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.params\endcsname{30.82}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.peak\endcsname{10.35}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.acdc.step\endcsname{1.02}
\expandafter\gdef\csname R@an.master_table.P1c.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P1c.amos.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P1c.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.P1c.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.amos.ne0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P1c.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.amos.params\endcsname{31.57}
\expandafter\gdef\csname R@an.master_table.P1c.amos.peak\endcsname{9.07}
\expandafter\gdef\csname R@an.master_table.P1c.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.amos.step\endcsname{1.02}
\expandafter\gdef\csname R@an.master_table.P1c.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P1c.kits.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P1c.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.P1c.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.kits.ne0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P1c.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.kits.params\endcsname{31.64}
\expandafter\gdef\csname R@an.master_table.P1c.kits.peak\endcsname{8.54}
\expandafter\gdef\csname R@an.master_table.P1c.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P1c.kits.step\endcsname{1.01}
\expandafter\gdef\csname R@an.master_table.P1c.params\endcsname{31.57}
\expandafter\gdef\csname R@an.master_table.P1c.params_pct_vs_default\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.master_table.P1c.peak\endcsname{9.07}
\expandafter\gdef\csname R@an.master_table.P1c.step\endcsname{1.02}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.d0\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.d0_3\endcsname{\ensuremath{-0.013}}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.d3\endcsname{\ensuremath{+0.074}}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.d3_df\endcsname{5.4}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.d3_hi\endcsname{\ensuremath{+0.223}}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.d3_lo\endcsname{\ensuremath{-0.076}}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.d3_span\endcsname{contains zero and lies below the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.d3_unc\endcsname{\ensuremath{+0.067}}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.dfresh\endcsname{\ensuremath{+0.117}}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.fresh_max\endcsname{\ensuremath{+0.125}}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.fresh_min\endcsname{\ensuremath{+0.109}}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.fresh_phrase\endcsname{\ensuremath{+0.117} pp over its two fresh seeds (seed deltas \ensuremath{+0.109} and \ensuremath{+0.125})}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.fresh_se\endcsname{0.008}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.fresh_vs_L3\endcsname{\ensuremath{-0.334}}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.fresh_vs_L3_abs\endcsname{0.334}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.fresh_vs_L3_dir\endcsname{below}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.fresh_vs_L3_se\endcsname{0.099}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.ne0\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.nefresh\endcsname{\ensuremath{+0.117}}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.params\endcsname{30.38}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.peak\endcsname{10.29}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.acdc.step\endcsname{1.04}
\expandafter\gdef\csname R@an.master_table.P3c.amos.d0\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.master_table.P3c.amos.d0_3\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.master_table.P3c.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.P3c.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.amos.ne0\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.master_table.P3c.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.amos.params\endcsname{31.12}
\expandafter\gdef\csname R@an.master_table.P3c.amos.peak\endcsname{9.01}
\expandafter\gdef\csname R@an.master_table.P3c.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.amos.step\endcsname{1.05}
\expandafter\gdef\csname R@an.master_table.P3c.kits.d0\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.master_table.P3c.kits.d0_3\endcsname{\ensuremath{+1.364}}
\expandafter\gdef\csname R@an.master_table.P3c.kits.d3\endcsname{\ensuremath{+1.239}}
\expandafter\gdef\csname R@an.master_table.P3c.kits.d3_df\endcsname{2.1}
\expandafter\gdef\csname R@an.master_table.P3c.kits.d3_hi\endcsname{\ensuremath{+3.162}}
\expandafter\gdef\csname R@an.master_table.P3c.kits.d3_lo\endcsname{\ensuremath{-0.684}}
\expandafter\gdef\csname R@an.master_table.P3c.kits.d3_span\endcsname{spans both zero and the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.P3c.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3c.kits.dfresh\endcsname{\ensuremath{+1.176}}
\expandafter\gdef\csname R@an.master_table.P3c.kits.fresh_max\endcsname{\ensuremath{+1.201}}
\expandafter\gdef\csname R@an.master_table.P3c.kits.fresh_min\endcsname{\ensuremath{+1.151}}
\expandafter\gdef\csname R@an.master_table.P3c.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.P3c.kits.fresh_phrase\endcsname{\ensuremath{+1.176} pp over its two fresh seeds (seed deltas \ensuremath{+1.151} and \ensuremath{+1.201})}
\expandafter\gdef\csname R@an.master_table.P3c.kits.fresh_se\endcsname{0.025}
\expandafter\gdef\csname R@an.master_table.P3c.kits.fresh_vs_L3\endcsname{\ensuremath{-0.918}}
\expandafter\gdef\csname R@an.master_table.P3c.kits.fresh_vs_L3_abs\endcsname{0.918}
\expandafter\gdef\csname R@an.master_table.P3c.kits.fresh_vs_L3_dir\endcsname{below}
\expandafter\gdef\csname R@an.master_table.P3c.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.P3c.kits.ne0\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.master_table.P3c.kits.nefresh\endcsname{\ensuremath{+1.176}}
\expandafter\gdef\csname R@an.master_table.P3c.kits.nefresh_margin\endcsname{\ensuremath{+0.976}}
\expandafter\gdef\csname R@an.master_table.P3c.kits.params\endcsname{31.20}
\expandafter\gdef\csname R@an.master_table.P3c.kits.peak\endcsname{8.52}
\expandafter\gdef\csname R@an.master_table.P3c.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 0.826 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 0.976 pp}
\expandafter\gdef\csname R@an.master_table.P3c.kits.step\endcsname{1.03}
\expandafter\gdef\csname R@an.master_table.P3c.params\endcsname{31.12}
\expandafter\gdef\csname R@an.master_table.P3c.params_pct_vs_default\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.master_table.P3c.peak\endcsname{9.01}
\expandafter\gdef\csname R@an.master_table.P3c.role.label\endcsname{implementation control (the function-identical rebuild of the default network)}
\expandafter\gdef\csname R@an.master_table.P3c.role.short\endcsname{impl.\ control}
\expandafter\gdef\csname R@an.master_table.P3c.role.source\endcsname{Addendum T1 (with N4 and W1)}
\expandafter\gdef\csname R@an.master_table.P3c.step\endcsname{1.05}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.params\endcsname{30.38}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.peak\endcsname{10.29}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.acdc.step\endcsname{1.03}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.ne0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.params\endcsname{31.12}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.peak\endcsname{9.01}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.amos.step\endcsname{1.05}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.ne0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.params\endcsname{31.20}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.peak\endcsname{8.52}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.P3lite.kits.step\endcsname{1.03}
\expandafter\gdef\csname R@an.master_table.P3lite.params\endcsname{31.12}
\expandafter\gdef\csname R@an.master_table.P3lite.params_pct_vs_default\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.master_table.P3lite.peak\endcsname{9.01}
\expandafter\gdef\csname R@an.master_table.P3lite.step\endcsname{1.05}
\expandafter\gdef\csname R@an.master_table.S2.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.S2.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.params\endcsname{26.97}
\expandafter\gdef\csname R@an.master_table.S2.acdc.peak\endcsname{11.72}
\expandafter\gdef\csname R@an.master_table.S2.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.acdc.step\endcsname{2.11}
\expandafter\gdef\csname R@an.master_table.S2.amos.d0\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.master_table.S2.amos.d0_3\endcsname{\ensuremath{+0.378}}
\expandafter\gdef\csname R@an.master_table.S2.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.S2.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.amos.ne0\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.master_table.S2.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.amos.params\endcsname{27.72}
\expandafter\gdef\csname R@an.master_table.S2.amos.peak\endcsname{10.48}
\expandafter\gdef\csname R@an.master_table.S2.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.amos.step\endcsname{1.96}
\expandafter\gdef\csname R@an.master_table.S2.kits.d0\endcsname{\ensuremath{+1.34}}
\expandafter\gdef\csname R@an.master_table.S2.kits.d0_3\endcsname{\ensuremath{+1.341}}
\expandafter\gdef\csname R@an.master_table.S2.kits.d3\endcsname{\ensuremath{+0.827}}
\expandafter\gdef\csname R@an.master_table.S2.kits.d3_df\endcsname{3.3}
\expandafter\gdef\csname R@an.master_table.S2.kits.d3_hi\endcsname{\ensuremath{+2.451}}
\expandafter\gdef\csname R@an.master_table.S2.kits.d3_lo\endcsname{\ensuremath{-0.796}}
\expandafter\gdef\csname R@an.master_table.S2.kits.d3_span\endcsname{spans both zero and the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.S2.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.S2.kits.dfresh\endcsname{\ensuremath{+0.570}}
\expandafter\gdef\csname R@an.master_table.S2.kits.fresh_max\endcsname{\ensuremath{+0.782}}
\expandafter\gdef\csname R@an.master_table.S2.kits.fresh_min\endcsname{\ensuremath{+0.358}}
\expandafter\gdef\csname R@an.master_table.S2.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.S2.kits.fresh_phrase\endcsname{\ensuremath{+0.570} pp over its two fresh seeds (seed deltas \ensuremath{+0.358} and \ensuremath{+0.782})}
\expandafter\gdef\csname R@an.master_table.S2.kits.fresh_se\endcsname{0.212}
\expandafter\gdef\csname R@an.master_table.S2.kits.fresh_vs_L3\endcsname{\ensuremath{-1.523}}
\expandafter\gdef\csname R@an.master_table.S2.kits.fresh_vs_L3_abs\endcsname{1.523}
\expandafter\gdef\csname R@an.master_table.S2.kits.fresh_vs_L3_dir\endcsname{below}
\expandafter\gdef\csname R@an.master_table.S2.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.S2.kits.ne0\endcsname{\ensuremath{+1.34}}
\expandafter\gdef\csname R@an.master_table.S2.kits.nefresh\endcsname{\ensuremath{+0.570}}
\expandafter\gdef\csname R@an.master_table.S2.kits.nefresh_margin\endcsname{\ensuremath{+0.370}}
\expandafter\gdef\csname R@an.master_table.S2.kits.params\endcsname{27.79}
\expandafter\gdef\csname R@an.master_table.S2.kits.peak\endcsname{9.42}
\expandafter\gdef\csname R@an.master_table.S2.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 0.220 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 0.370 pp}
\expandafter\gdef\csname R@an.master_table.S2.kits.step\endcsname{1.68}
\expandafter\gdef\csname R@an.master_table.S2.params\endcsname{27.72}
\expandafter\gdef\csname R@an.master_table.S2.params_pct_vs_default\endcsname{\ensuremath{-10.9}}
\expandafter\gdef\csname R@an.master_table.S2.peak\endcsname{10.48}
\expandafter\gdef\csname R@an.master_table.S2.step\endcsname{1.96}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.params\endcsname{107.11}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.peak\endcsname{10.37}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.acdc.step\endcsname{1.97}
\expandafter\gdef\csname R@an.master_table.SP1.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.SP1.amos.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.SP1.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.SP1.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.amos.ne0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.SP1.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.amos.params\endcsname{107.85}
\expandafter\gdef\csname R@an.master_table.SP1.amos.peak\endcsname{9.98}
\expandafter\gdef\csname R@an.master_table.SP1.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.amos.step\endcsname{1.91}
\expandafter\gdef\csname R@an.master_table.SP1.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.SP1.kits.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.SP1.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.SP1.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.kits.ne0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.SP1.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.kits.params\endcsname{107.93}
\expandafter\gdef\csname R@an.master_table.SP1.kits.peak\endcsname{9.82}
\expandafter\gdef\csname R@an.master_table.SP1.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP1.kits.step\endcsname{1.69}
\expandafter\gdef\csname R@an.master_table.SP1.params\endcsname{107.85}
\expandafter\gdef\csname R@an.master_table.SP1.params_pct_vs_default\endcsname{\ensuremath{+246.6}}
\expandafter\gdef\csname R@an.master_table.SP1.peak\endcsname{9.98}
\expandafter\gdef\csname R@an.master_table.SP1.step\endcsname{1.91}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.params\endcsname{107.11}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.peak\endcsname{10.57}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.acdc.step\endcsname{2.15}
\expandafter\gdef\csname R@an.master_table.SP2.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.SP2.amos.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.SP2.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.SP2.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.amos.ne0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.SP2.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.amos.params\endcsname{107.86}
\expandafter\gdef\csname R@an.master_table.SP2.amos.peak\endcsname{9.25}
\expandafter\gdef\csname R@an.master_table.SP2.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.amos.step\endcsname{2.07}
\expandafter\gdef\csname R@an.master_table.SP2.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.SP2.kits.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.SP2.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.SP2.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.kits.ne0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.SP2.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.kits.params\endcsname{107.95}
\expandafter\gdef\csname R@an.master_table.SP2.kits.peak\endcsname{8.13}
\expandafter\gdef\csname R@an.master_table.SP2.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.SP2.kits.step\endcsname{1.91}
\expandafter\gdef\csname R@an.master_table.SP2.params\endcsname{107.86}
\expandafter\gdef\csname R@an.master_table.SP2.params_pct_vs_default\endcsname{\ensuremath{+246.6}}
\expandafter\gdef\csname R@an.master_table.SP2.peak\endcsname{9.25}
\expandafter\gdef\csname R@an.master_table.SP2.step\endcsname{2.07}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.params\endcsname{28.73}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.peak\endcsname{11.74}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.acdc.step\endcsname{1.49}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.d0\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.d0_3\endcsname{\ensuremath{+0.041}}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.ne0\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.params\endcsname{29.47}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.peak\endcsname{9.99}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.amos.step\endcsname{1.39}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.d0\endcsname{\ensuremath{+1.95}}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.d0_3\endcsname{\ensuremath{+1.949}}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.d3\endcsname{\ensuremath{+2.093}}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.d3_df\endcsname{2.3}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.d3_hi\endcsname{\ensuremath{+3.902}}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.d3_lo\endcsname{\ensuremath{+0.285}}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.d3_span\endcsname{lies above zero and contains the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.dfresh\endcsname{\ensuremath{+2.165}}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.fresh_max\endcsname{\ensuremath{+2.348}}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.fresh_min\endcsname{\ensuremath{+1.983}}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.fresh_phrase\endcsname{\ensuremath{+2.165} pp over its two fresh seeds (seed deltas \ensuremath{+1.983} and \ensuremath{+2.348})}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.fresh_se\endcsname{0.182}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.fresh_vs_L3\endcsname{\ensuremath{+0.072}}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.fresh_vs_L3_abs\endcsname{0.072}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.fresh_vs_L3_dir\endcsname{above}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.ne0\endcsname{\ensuremath{+1.95}}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.nefresh\endcsname{\ensuremath{+2.165}}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.nefresh_margin\endcsname{\ensuremath{+1.965}}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.params\endcsname{29.53}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.peak\endcsname{8.89}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 1.815 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 1.965 pp}
\expandafter\gdef\csname R@an.master_table.V5A5.kits.step\endcsname{1.24}
\expandafter\gdef\csname R@an.master_table.V5A5.params\endcsname{29.47}
\expandafter\gdef\csname R@an.master_table.V5A5.params_pct_vs_default\endcsname{\ensuremath{-5.3}}
\expandafter\gdef\csname R@an.master_table.V5A5.peak\endcsname{9.99}
\expandafter\gdef\csname R@an.master_table.V5A5.step\endcsname{1.39}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.params\endcsname{20.18}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.peak\endcsname{9.03}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.acdc.step\endcsname{0.72}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.d0\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.d0_3\endcsname{\ensuremath{-0.261}}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.ne0\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.params\endcsname{20.93}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.peak\endcsname{7.94}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.amos.step\endcsname{0.74}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.d0\endcsname{\ensuremath{+2.16}}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.d0_3\endcsname{\ensuremath{+2.162}}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.d3\endcsname{\ensuremath{+2.244}}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.d3_df\endcsname{2.0}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.d3_hi\endcsname{\ensuremath{+4.189}}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.d3_lo\endcsname{\ensuremath{+0.299}}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.d3_span\endcsname{lies above zero and contains the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.dfresh\endcsname{\ensuremath{+2.285}}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.fresh_max\endcsname{\ensuremath{+2.328}}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.fresh_min\endcsname{\ensuremath{+2.242}}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.fresh_phrase\endcsname{\ensuremath{+2.285} pp over its two fresh seeds (seed deltas \ensuremath{+2.242} and \ensuremath{+2.328})}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.fresh_se\endcsname{0.043}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.fresh_vs_L3\endcsname{\ensuremath{+0.192}}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.fresh_vs_L3_abs\endcsname{0.192}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.fresh_vs_L3_dir\endcsname{above}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.ne0\endcsname{\ensuremath{+2.16}}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.nefresh\endcsname{\ensuremath{+2.285}}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.nefresh_margin\endcsname{\ensuremath{+2.085}}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.params\endcsname{20.96}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.peak\endcsname{7.64}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 1.935 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 2.085 pp}
\expandafter\gdef\csname R@an.master_table.V5B1.kits.step\endcsname{0.73}
\expandafter\gdef\csname R@an.master_table.V5B1.params\endcsname{20.93}
\expandafter\gdef\csname R@an.master_table.V5B1.params_pct_vs_default\endcsname{\ensuremath{-32.7}}
\expandafter\gdef\csname R@an.master_table.V5B1.peak\endcsname{7.94}
\expandafter\gdef\csname R@an.master_table.V5B1.step\endcsname{0.74}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.d0\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.d0_3\endcsname{\ensuremath{-0.181}}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.ne0\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.params\endcsname{20.48}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.peak\endcsname{9.25}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.acdc.step\endcsname{0.92}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.d0\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.d0_3\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.ne0\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.params\endcsname{21.22}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.peak\endcsname{8.02}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.amos.step\endcsname{0.85}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.d0\endcsname{\ensuremath{+1.26}}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.d0_3\endcsname{\ensuremath{+1.264}}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.d3\endcsname{\ensuremath{+1.387}}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.d3_df\endcsname{2.1}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.d3_hi\endcsname{\ensuremath{+3.305}}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.d3_lo\endcsname{\ensuremath{-0.531}}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.d3_span\endcsname{spans both zero and the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.dfresh\endcsname{\ensuremath{+1.448}}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.fresh_max\endcsname{\ensuremath{+1.498}}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.fresh_min\endcsname{\ensuremath{+1.399}}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.fresh_phrase\endcsname{\ensuremath{+1.448} pp over its two fresh seeds (seed deltas \ensuremath{+1.399} and \ensuremath{+1.498})}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.fresh_se\endcsname{0.049}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.fresh_vs_L3\endcsname{\ensuremath{-0.645}}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.fresh_vs_L3_abs\endcsname{0.645}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.fresh_vs_L3_dir\endcsname{below}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.ne0\endcsname{\ensuremath{+1.26}}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.nefresh\endcsname{\ensuremath{+1.448}}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.nefresh_margin\endcsname{\ensuremath{+1.248}}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.params\endcsname{21.26}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.peak\endcsname{7.68}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 1.098 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 1.248 pp}
\expandafter\gdef\csname R@an.master_table.V5B2.kits.step\endcsname{0.84}
\expandafter\gdef\csname R@an.master_table.V5B2.params\endcsname{21.22}
\expandafter\gdef\csname R@an.master_table.V5B2.params_pct_vs_default\endcsname{\ensuremath{-31.8}}
\expandafter\gdef\csname R@an.master_table.V5B2.peak\endcsname{8.02}
\expandafter\gdef\csname R@an.master_table.V5B2.step\endcsname{0.85}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.d0\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.d0_3\endcsname{\ensuremath{+0.573}}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.ne0\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.params\endcsname{29.96}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.peak\endcsname{10.43}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.acdc.step\endcsname{1.81}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.d0\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.d0_3\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.ne0\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.params\endcsname{30.70}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.peak\endcsname{10.75}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.amos.step\endcsname{1.63}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.d0\endcsname{\ensuremath{+2.24}}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.d0_3\endcsname{\ensuremath{+2.236}}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.d3\endcsname{\ensuremath{+1.881}}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.d3_df\endcsname{2.6}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.d3_hi\endcsname{\ensuremath{+3.600}}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.d3_lo\endcsname{\ensuremath{+0.163}}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.d3_span\endcsname{lies above zero and contains the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.dfresh\endcsname{\ensuremath{+1.704}}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.fresh_max\endcsname{\ensuremath{+1.713}}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.fresh_min\endcsname{\ensuremath{+1.695}}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.fresh_phrase\endcsname{\ensuremath{+1.704} pp over its two fresh seeds (seed deltas \ensuremath{+1.695} and \ensuremath{+1.713})}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.fresh_se\endcsname{0.009}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.fresh_vs_L3\endcsname{\ensuremath{-0.389}}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.fresh_vs_L3_abs\endcsname{0.389}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.fresh_vs_L3_dir\endcsname{below}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.ne0\endcsname{\ensuremath{+2.24}}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.nefresh\endcsname{\ensuremath{+1.704}}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.nefresh_margin\endcsname{\ensuremath{+1.504}}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.params\endcsname{30.78}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.peak\endcsname{9.57}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 1.354 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 1.504 pp}
\expandafter\gdef\csname R@an.master_table.V6A1r.kits.step\endcsname{1.49}
\expandafter\gdef\csname R@an.master_table.V6A1r.params\endcsname{30.70}
\expandafter\gdef\csname R@an.master_table.V6A1r.params_pct_vs_default\endcsname{\ensuremath{-1.3}}
\expandafter\gdef\csname R@an.master_table.V6A1r.peak\endcsname{10.75}
\expandafter\gdef\csname R@an.master_table.V6A1r.step\endcsname{1.63}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.d0\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.d0_3\endcsname{\ensuremath{+0.229}}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.ne0\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.params\endcsname{30.26}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.peak\endcsname{9.89}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.acdc.step\endcsname{1.07}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.d0\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.d0_3\endcsname{\ensuremath{-0.045}}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.ne0\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.params\endcsname{31.00}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.peak\endcsname{8.59}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.amos.step\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.d0\endcsname{\ensuremath{+2.55}}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.d0_3\endcsname{\ensuremath{+2.548}}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.d3\endcsname{\ensuremath{+2.624}}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.d3_df\endcsname{2.7}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.d3_hi\endcsname{\ensuremath{+4.312}}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.d3_lo\endcsname{\ensuremath{+0.935}}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.d3_span\endcsname{lies above the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.dfresh\endcsname{\ensuremath{+2.662}}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.fresh_max\endcsname{\ensuremath{+2.997}}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.fresh_min\endcsname{\ensuremath{+2.326}}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.fresh_phrase\endcsname{\ensuremath{+2.662} pp over its two fresh seeds (seed deltas \ensuremath{+2.326} and \ensuremath{+2.997})}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.fresh_se\endcsname{0.335}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.fresh_vs_L3\endcsname{\ensuremath{+0.568}}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.fresh_vs_L3_abs\endcsname{0.568}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.fresh_vs_L3_dir\endcsname{above}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.ne0\endcsname{\ensuremath{+2.55}}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.nefresh\endcsname{\ensuremath{+2.662}}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.nefresh_margin\endcsname{\ensuremath{+2.462}}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.params\endcsname{31.04}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.peak\endcsname{8.02}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 2.312 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 2.462 pp}
\expandafter\gdef\csname R@an.master_table.V7A1.kits.step\endcsname{0.92}
\expandafter\gdef\csname R@an.master_table.V7A1.params\endcsname{31.00}
\expandafter\gdef\csname R@an.master_table.V7A1.params_pct_vs_default\endcsname{\ensuremath{-0.4}}
\expandafter\gdef\csname R@an.master_table.V7A1.peak\endcsname{8.59}
\expandafter\gdef\csname R@an.master_table.V7A1.step\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.d0\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.d0_3\endcsname{\ensuremath{+0.362}}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.ne0\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.params\endcsname{30.38}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.peak\endcsname{10.78}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.acdc.step\endcsname{1.23}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.d0\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.d0_3\endcsname{\ensuremath{+0.359}}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.ne0\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.params\endcsname{31.12}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.peak\endcsname{9.34}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.amos.step\endcsname{1.15}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.d0\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.d0_3\endcsname{\ensuremath{+2.886}}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.d3\endcsname{\ensuremath{+2.488}}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.d3_df\endcsname{3.2}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.d3_hi\endcsname{\ensuremath{+4.115}}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.d3_lo\endcsname{\ensuremath{+0.862}}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.d3_span\endcsname{lies above the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.dfresh\endcsname{\ensuremath{+2.289}}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.fresh_max\endcsname{\ensuremath{+2.606}}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.fresh_min\endcsname{\ensuremath{+1.973}}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.fresh_phrase\endcsname{\ensuremath{+2.289} pp over its two fresh seeds (seed deltas \ensuremath{+1.973} and \ensuremath{+2.606})}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.fresh_se\endcsname{0.316}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.fresh_vs_L3\endcsname{\ensuremath{+0.196}}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.fresh_vs_L3_abs\endcsname{0.196}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.fresh_vs_L3_dir\endcsname{above}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.ne0\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.nefresh\endcsname{\ensuremath{+2.289}}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.nefresh_margin\endcsname{\ensuremath{+2.089}}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.params\endcsname{31.18}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.peak\endcsname{8.69}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 1.939 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 2.089 pp}
\expandafter\gdef\csname R@an.master_table.V7A2.kits.step\endcsname{1.09}
\expandafter\gdef\csname R@an.master_table.V7A2.params\endcsname{31.12}
\expandafter\gdef\csname R@an.master_table.V7A2.params_pct_vs_default\endcsname{\ensuremath{0.0}}
\expandafter\gdef\csname R@an.master_table.V7A2.peak\endcsname{9.34}
\expandafter\gdef\csname R@an.master_table.V7A2.step\endcsname{1.15}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.params\endcsname{25.58}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.peak\endcsname{10.26}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.acdc.step\endcsname{1.10}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.d0\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.d0_3\endcsname{\ensuremath{-0.216}}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.ne0\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.params\endcsname{26.32}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.peak\endcsname{8.89}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.amos.step\endcsname{1.03}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.d0\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.d0_3\endcsname{\ensuremath{+0.542}}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.ne0\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.params\endcsname{26.38}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.peak\endcsname{8.43}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7A3.kits.step\endcsname{1.02}
\expandafter\gdef\csname R@an.master_table.V7A3.params\endcsname{26.32}
\expandafter\gdef\csname R@an.master_table.V7A3.params_pct_vs_default\endcsname{\ensuremath{-15.4}}
\expandafter\gdef\csname R@an.master_table.V7A3.peak\endcsname{8.89}
\expandafter\gdef\csname R@an.master_table.V7A3.step\endcsname{1.03}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.params\endcsname{19.65}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.peak\endcsname{9.28}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.acdc.step\endcsname{0.79}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.d0\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.d0_3\endcsname{\ensuremath{-0.436}}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.ne0\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.params\endcsname{20.40}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.peak\endcsname{8.03}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.amos.step\endcsname{0.78}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.d0\endcsname{\ensuremath{+1.72}}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.d0_3\endcsname{\ensuremath{+1.721}}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.d3\endcsname{\ensuremath{+2.162}}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.d3_df\endcsname{3.4}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.d3_hi\endcsname{\ensuremath{+3.785}}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.d3_lo\endcsname{\ensuremath{+0.538}}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.d3_span\endcsname{lies above the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.dfresh\endcsname{\ensuremath{+2.382}}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.fresh_max\endcsname{\ensuremath{+2.710}}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.fresh_min\endcsname{\ensuremath{+2.053}}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.fresh_phrase\endcsname{\ensuremath{+2.382} pp over its two fresh seeds (seed deltas \ensuremath{+2.053} and \ensuremath{+2.710})}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.fresh_se\endcsname{0.329}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.fresh_vs_L3\endcsname{\ensuremath{+0.288}}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.fresh_vs_L3_abs\endcsname{0.288}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.fresh_vs_L3_dir\endcsname{above}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.ne0\endcsname{\ensuremath{+1.72}}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.nefresh\endcsname{\ensuremath{+2.382}}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.nefresh_margin\endcsname{\ensuremath{+2.182}}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.params\endcsname{20.43}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.peak\endcsname{7.69}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 2.032 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 2.182 pp}
\expandafter\gdef\csname R@an.master_table.V7B1.kits.step\endcsname{0.77}
\expandafter\gdef\csname R@an.master_table.V7B1.params\endcsname{20.40}
\expandafter\gdef\csname R@an.master_table.V7B1.params_pct_vs_default\endcsname{\ensuremath{-34.4}}
\expandafter\gdef\csname R@an.master_table.V7B1.peak\endcsname{8.03}
\expandafter\gdef\csname R@an.master_table.V7B1.step\endcsname{0.78}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.params\endcsname{19.67}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.peak\endcsname{9.25}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.acdc.step\endcsname{0.76}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.d0\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.d0_3\endcsname{\ensuremath{-0.267}}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.ne0\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.params\endcsname{20.42}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.peak\endcsname{8.02}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.amos.step\endcsname{0.78}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.d0\endcsname{\ensuremath{+2.82}}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.d0_3\endcsname{\ensuremath{+2.824}}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.d3\endcsname{\ensuremath{+2.167}}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.d3_df\endcsname{4.0}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.d3_hi\endcsname{\ensuremath{+3.970}}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.d3_lo\endcsname{\ensuremath{+0.364}}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.d3_span\endcsname{lies above the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.dfresh\endcsname{\ensuremath{+1.838}}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.fresh_max\endcsname{\ensuremath{+2.395}}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.fresh_min\endcsname{\ensuremath{+1.282}}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.fresh_phrase\endcsname{\ensuremath{+1.838} pp over its two fresh seeds (seed deltas \ensuremath{+1.282} and \ensuremath{+2.395})}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.fresh_se\endcsname{0.557}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.fresh_vs_L3\endcsname{\ensuremath{-0.255}}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.fresh_vs_L3_abs\endcsname{0.255}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.fresh_vs_L3_dir\endcsname{below}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.ne0\endcsname{\ensuremath{+2.82}}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.nefresh\endcsname{\ensuremath{+1.838}}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.nefresh_margin\endcsname{\ensuremath{+1.638}}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.params\endcsname{20.45}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.peak\endcsname{7.68}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 1.488 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 1.638 pp}
\expandafter\gdef\csname R@an.master_table.V7B2.kits.step\endcsname{0.76}
\expandafter\gdef\csname R@an.master_table.V7B2.params\endcsname{20.42}
\expandafter\gdef\csname R@an.master_table.V7B2.params_pct_vs_default\endcsname{\ensuremath{-34.4}}
\expandafter\gdef\csname R@an.master_table.V7B2.peak\endcsname{8.02}
\expandafter\gdef\csname R@an.master_table.V7B2.step\endcsname{0.78}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.d0\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.d0_3\endcsname{\ensuremath{-0.252}}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.ne0\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.params\endcsname{20.33}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.peak\endcsname{9.08}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.acdc.step\endcsname{0.79}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.d0\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.d0_3\endcsname{\ensuremath{-0.106}}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.d3_df\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.d3_hi\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.d3_lo\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.d3_span\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.d3_unc\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.fresh_max\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.fresh_min\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.fresh_partial\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.fresh_phrase\endcsname{its registered fresh pair (seeds 1 and 2) has not finished}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.fresh_se\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.fresh_vs_L3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.fresh_vs_L3_abs\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.fresh_vs_L3_dir\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.fresh_vs_L3_se\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.ne0\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.nefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.nefresh_margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.params\endcsname{21.08}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.peak\endcsname{7.95}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.amos.step\endcsname{0.78}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.d0\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.d0_3\endcsname{\ensuremath{+2.707}}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.d3\endcsname{\ensuremath{+2.529}}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.d3_df\endcsname{2.8}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.d3_hi\endcsname{\ensuremath{+4.208}}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.d3_lo\endcsname{\ensuremath{+0.850}}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.d3_span\endcsname{lies above the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.dfresh\endcsname{\ensuremath{+2.440}}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.fresh_max\endcsname{\ensuremath{+2.758}}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.fresh_min\endcsname{\ensuremath{+2.121}}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.fresh_phrase\endcsname{\ensuremath{+2.440} pp over its two fresh seeds (seed deltas \ensuremath{+2.121} and \ensuremath{+2.758})}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.fresh_se\endcsname{0.318}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.fresh_vs_L3\endcsname{\ensuremath{+0.346}}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.fresh_vs_L3_abs\endcsname{0.346}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.fresh_vs_L3_dir\endcsname{above}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.ne0\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.nefresh\endcsname{\ensuremath{+2.440}}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.nefresh_margin\endcsname{\ensuremath{+2.240}}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.params\endcsname{21.11}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.peak\endcsname{7.65}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 2.090 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 2.240 pp}
\expandafter\gdef\csname R@an.master_table.V7C1.kits.step\endcsname{0.77}
\expandafter\gdef\csname R@an.master_table.V7C1.params\endcsname{21.08}
\expandafter\gdef\csname R@an.master_table.V7C1.params_pct_vs_default\endcsname{\ensuremath{-32.3}}
\expandafter\gdef\csname R@an.master_table.V7C1.peak\endcsname{7.95}
\expandafter\gdef\csname R@an.master_table.V7C1.step\endcsname{0.78}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.params\endcsname{19.67}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.peak\endcsname{9.25}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.acdc.step\endcsname{0.77}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.d0\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.d0_3\endcsname{\ensuremath{-0.362}}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.ne0\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.params\endcsname{20.42}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.peak\endcsname{8.02}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.amos.step\endcsname{0.77}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.d0\endcsname{\ensuremath{+2.00}}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.d0_3\endcsname{\ensuremath{+2.000}}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.ne0\endcsname{\ensuremath{+2.00}}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.params\endcsname{20.45}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.peak\endcsname{7.68}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V7C2.kits.step\endcsname{0.76}
\expandafter\gdef\csname R@an.master_table.V7C2.params\endcsname{20.42}
\expandafter\gdef\csname R@an.master_table.V7C2.params_pct_vs_default\endcsname{\ensuremath{-34.4}}
\expandafter\gdef\csname R@an.master_table.V7C2.peak\endcsname{8.02}
\expandafter\gdef\csname R@an.master_table.V7C2.step\endcsname{0.77}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.params\endcsname{30.53}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.peak\endcsname{9.29}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.acdc.step\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.d0\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.d0_3\endcsname{\ensuremath{-0.505}}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.ne0\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.params\endcsname{31.27}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.peak\endcsname{8.04}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.amos.step\endcsname{0.90}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.d0\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.d0_3\endcsname{\ensuremath{+1.760}}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.d3\endcsname{\ensuremath{+1.419}}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.d3_df\endcsname{2.7}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.d3_hi\endcsname{\ensuremath{+3.108}}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.d3_lo\endcsname{\ensuremath{-0.269}}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.d3_span\endcsname{spans both zero and the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.dfresh\endcsname{\ensuremath{+1.249}}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.fresh_max\endcsname{\ensuremath{+1.421}}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.fresh_min\endcsname{\ensuremath{+1.077}}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.fresh_phrase\endcsname{\ensuremath{+1.249} pp over its two fresh seeds (seed deltas \ensuremath{+1.077} and \ensuremath{+1.421})}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.fresh_se\endcsname{0.172}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.fresh_vs_L3\endcsname{\ensuremath{-0.845}}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.fresh_vs_L3_abs\endcsname{0.845}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.fresh_vs_L3_dir\endcsname{below}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.ne0\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.nefresh\endcsname{\ensuremath{+1.249}}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.nefresh_margin\endcsname{\ensuremath{+1.049}}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.params\endcsname{31.31}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.peak\endcsname{7.72}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 0.899 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 1.049 pp}
\expandafter\gdef\csname R@an.master_table.V8A1.kits.step\endcsname{0.91}
\expandafter\gdef\csname R@an.master_table.V8A1.params\endcsname{31.27}
\expandafter\gdef\csname R@an.master_table.V8A1.params_pct_vs_default\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.master_table.V8A1.peak\endcsname{8.04}
\expandafter\gdef\csname R@an.master_table.V8A1.step\endcsname{0.90}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.params\endcsname{30.69}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.peak\endcsname{9.25}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.acdc.step\endcsname{0.92}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.d0\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.d0_3\endcsname{\ensuremath{-0.312}}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.ne0\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.params\endcsname{31.44}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.peak\endcsname{8.05}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.amos.step\endcsname{0.86}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.d0\endcsname{\ensuremath{+1.35}}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.d0_3\endcsname{\ensuremath{+1.353}}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.d3\endcsname{\ensuremath{+1.703}}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.d3_df\endcsname{3.0}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.d3_hi\endcsname{\ensuremath{+3.345}}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.d3_lo\endcsname{\ensuremath{+0.060}}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.d3_span\endcsname{lies above zero and contains the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.dfresh\endcsname{\ensuremath{+1.877}}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.fresh_max\endcsname{\ensuremath{+2.162}}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.fresh_min\endcsname{\ensuremath{+1.593}}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.fresh_phrase\endcsname{\ensuremath{+1.877} pp over its two fresh seeds (seed deltas \ensuremath{+1.593} and \ensuremath{+2.162})}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.fresh_se\endcsname{0.284}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.fresh_vs_L3\endcsname{\ensuremath{-0.216}}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.fresh_vs_L3_abs\endcsname{0.216}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.fresh_vs_L3_dir\endcsname{below}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.ne0\endcsname{\ensuremath{+1.35}}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.nefresh\endcsname{\ensuremath{+1.877}}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.nefresh_margin\endcsname{\ensuremath{+1.677}}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.params\endcsname{31.47}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.peak\endcsname{7.73}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 1.527 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 1.677 pp}
\expandafter\gdef\csname R@an.master_table.V8A2.kits.step\endcsname{0.85}
\expandafter\gdef\csname R@an.master_table.V8A2.params\endcsname{31.44}
\expandafter\gdef\csname R@an.master_table.V8A2.params_pct_vs_default\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.master_table.V8A2.peak\endcsname{8.05}
\expandafter\gdef\csname R@an.master_table.V8A2.step\endcsname{0.86}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.params\endcsname{17.44}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.peak\endcsname{8.17}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.acdc.step\endcsname{0.62}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.d0\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.d0_3\endcsname{\ensuremath{-0.751}}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.ne0\endcsname{\ensuremath{-0.62}}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.params\endcsname{18.19}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.peak\endcsname{7.17}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.amos.step\endcsname{0.62}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.d0\endcsname{\ensuremath{+2.91}}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.d0_3\endcsname{\ensuremath{+2.911}}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.d3\endcsname{\ensuremath{+1.887}}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.d3_df\endcsname{3.6}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.d3_hi\endcsname{\ensuremath{+4.210}}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.d3_lo\endcsname{\ensuremath{-0.436}}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.d3_span\endcsname{spans both zero and the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.dfresh\endcsname{\ensuremath{+1.375}}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.fresh_max\endcsname{\ensuremath{+2.079}}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.fresh_min\endcsname{\ensuremath{+0.670}}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.fresh_phrase\endcsname{\ensuremath{+1.375} pp over its two fresh seeds (seed deltas \ensuremath{+0.670} and \ensuremath{+2.079})}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.fresh_se\endcsname{0.704}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.fresh_vs_L3\endcsname{\ensuremath{-0.719}}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.fresh_vs_L3_abs\endcsname{0.719}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.fresh_vs_L3_dir\endcsname{below}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.ne0\endcsname{\ensuremath{+2.91}}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.nefresh\endcsname{\ensuremath{+1.375}}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.nefresh_margin\endcsname{\ensuremath{+1.175}}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.params\endcsname{18.21}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.peak\endcsname{6.96}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 1.025 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 1.175 pp}
\expandafter\gdef\csname R@an.master_table.V8B1.kits.step\endcsname{0.59}
\expandafter\gdef\csname R@an.master_table.V8B1.params\endcsname{18.19}
\expandafter\gdef\csname R@an.master_table.V8B1.params_pct_vs_default\endcsname{\ensuremath{-41.5}}
\expandafter\gdef\csname R@an.master_table.V8B1.peak\endcsname{7.17}
\expandafter\gdef\csname R@an.master_table.V8B1.step\endcsname{0.62}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.params\endcsname{20.32}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.peak\endcsname{8.49}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.acdc.step\endcsname{0.68}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.d0\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.d0_3\endcsname{\ensuremath{-0.287}}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.d3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.d3_df\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.d3_hi\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.d3_lo\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.d3_span\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.d3_unc\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.fresh_max\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.fresh_min\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.fresh_partial\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.fresh_phrase\endcsname{its registered fresh pair (seeds 1 and 2) has not finished}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.fresh_se\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.fresh_vs_L3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.fresh_vs_L3_abs\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.fresh_vs_L3_dir\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.fresh_vs_L3_se\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.ne0\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.nefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.nefresh_margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.params\endcsname{21.07}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.peak\endcsname{7.45}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.amos.step\endcsname{0.67}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.d0\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.d0_3\endcsname{\ensuremath{+1.646}}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.d3\endcsname{\ensuremath{+1.703}}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.d3_df\endcsname{2.2}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.d3_hi\endcsname{\ensuremath{+3.570}}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.d3_lo\endcsname{\ensuremath{-0.165}}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.d3_span\endcsname{spans both zero and the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.dfresh\endcsname{\ensuremath{+1.731}}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.fresh_max\endcsname{\ensuremath{+1.892}}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.fresh_min\endcsname{\ensuremath{+1.570}}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.fresh_phrase\endcsname{\ensuremath{+1.731} pp over its two fresh seeds (seed deltas \ensuremath{+1.570} and \ensuremath{+1.892})}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.fresh_se\endcsname{0.161}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.fresh_vs_L3\endcsname{\ensuremath{-0.362}}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.fresh_vs_L3_abs\endcsname{0.362}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.fresh_vs_L3_dir\endcsname{below}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.ne0\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.nefresh\endcsname{\ensuremath{+1.731}}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.nefresh_margin\endcsname{\ensuremath{+1.531}}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.params\endcsname{21.08}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.peak\endcsname{7.11}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 1.381 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 1.531 pp}
\expandafter\gdef\csname R@an.master_table.V8B2.kits.step\endcsname{0.63}
\expandafter\gdef\csname R@an.master_table.V8B2.params\endcsname{21.07}
\expandafter\gdef\csname R@an.master_table.V8B2.params_pct_vs_default\endcsname{\ensuremath{-32.3}}
\expandafter\gdef\csname R@an.master_table.V8B2.peak\endcsname{7.45}
\expandafter\gdef\csname R@an.master_table.V8B2.step\endcsname{0.67}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.params\endcsname{17.58}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.peak\endcsname{9.05}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.acdc.step\endcsname{0.78}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.d0\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.d0_3\endcsname{\ensuremath{-0.361}}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.ne0\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.params\endcsname{18.21}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.peak\endcsname{7.93}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.amos.step\endcsname{0.77}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.d0\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.d0_3\endcsname{\ensuremath{+2.535}}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.ne0\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.params\endcsname{18.25}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.peak\endcsname{7.63}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.V8X1.kits.step\endcsname{0.77}
\expandafter\gdef\csname R@an.master_table.V8X1.params\endcsname{18.21}
\expandafter\gdef\csname R@an.master_table.V8X1.params_pct_vs_default\endcsname{\ensuremath{-41.5}}
\expandafter\gdef\csname R@an.master_table.V8X1.peak\endcsname{7.93}
\expandafter\gdef\csname R@an.master_table.V8X1.step\endcsname{0.77}
\expandafter\gdef\csname R@an.master_table.W1.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W1.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.params\endcsname{30.39}
\expandafter\gdef\csname R@an.master_table.W1.acdc.peak\endcsname{10.73}
\expandafter\gdef\csname R@an.master_table.W1.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.acdc.step\endcsname{1.15}
\expandafter\gdef\csname R@an.master_table.W1.amos.d0\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.master_table.W1.amos.d0_3\endcsname{\ensuremath{+0.099}}
\expandafter\gdef\csname R@an.master_table.W1.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W1.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.amos.ne0\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.master_table.W1.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.amos.params\endcsname{31.14}
\expandafter\gdef\csname R@an.master_table.W1.amos.peak\endcsname{9.40}
\expandafter\gdef\csname R@an.master_table.W1.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.amos.step\endcsname{1.14}
\expandafter\gdef\csname R@an.master_table.W1.kits.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W1.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.params\endcsname{31.21}
\expandafter\gdef\csname R@an.master_table.W1.kits.peak\endcsname{8.72}
\expandafter\gdef\csname R@an.master_table.W1.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1.kits.step\endcsname{1.12}
\expandafter\gdef\csname R@an.master_table.W1.params\endcsname{31.14}
\expandafter\gdef\csname R@an.master_table.W1.params_pct_vs_default\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.master_table.W1.peak\endcsname{9.40}
\expandafter\gdef\csname R@an.master_table.W1.step\endcsname{1.14}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.params\endcsname{30.39}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.peak\endcsname{10.73}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.acdc.step\endcsname{1.15}
\expandafter\gdef\csname R@an.master_table.W1c.amos.d0\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.master_table.W1c.amos.d0_3\endcsname{\ensuremath{+0.363}}
\expandafter\gdef\csname R@an.master_table.W1c.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W1c.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.amos.ne0\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.master_table.W1c.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.amos.params\endcsname{31.14}
\expandafter\gdef\csname R@an.master_table.W1c.amos.peak\endcsname{9.40}
\expandafter\gdef\csname R@an.master_table.W1c.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.amos.step\endcsname{1.15}
\expandafter\gdef\csname R@an.master_table.W1c.kits.d0\endcsname{\ensuremath{+2.64}}
\expandafter\gdef\csname R@an.master_table.W1c.kits.d0_3\endcsname{\ensuremath{+2.636}}
\expandafter\gdef\csname R@an.master_table.W1c.kits.d3\endcsname{\ensuremath{+1.590}}
\expandafter\gdef\csname R@an.master_table.W1c.kits.d3_df\endcsname{3.6}
\expandafter\gdef\csname R@an.master_table.W1c.kits.d3_hi\endcsname{\ensuremath{+3.898}}
\expandafter\gdef\csname R@an.master_table.W1c.kits.d3_lo\endcsname{\ensuremath{-0.719}}
\expandafter\gdef\csname R@an.master_table.W1c.kits.d3_span\endcsname{spans both zero and the registered \ensuremath{+0.35} pp bar}
\expandafter\gdef\csname R@an.master_table.W1c.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W1c.kits.dfresh\endcsname{\ensuremath{+1.067}}
\expandafter\gdef\csname R@an.master_table.W1c.kits.fresh_max\endcsname{\ensuremath{+1.734}}
\expandafter\gdef\csname R@an.master_table.W1c.kits.fresh_min\endcsname{\ensuremath{+0.399}}
\expandafter\gdef\csname R@an.master_table.W1c.kits.fresh_partial\endcsname{seeds 1 and 2 are both finished}
\expandafter\gdef\csname R@an.master_table.W1c.kits.fresh_phrase\endcsname{\ensuremath{+1.067} pp over its two fresh seeds (seed deltas \ensuremath{+0.399} and \ensuremath{+1.734})}
\expandafter\gdef\csname R@an.master_table.W1c.kits.fresh_se\endcsname{0.667}
\expandafter\gdef\csname R@an.master_table.W1c.kits.fresh_vs_L3\endcsname{\ensuremath{-1.027}}
\expandafter\gdef\csname R@an.master_table.W1c.kits.fresh_vs_L3_abs\endcsname{1.027}
\expandafter\gdef\csname R@an.master_table.W1c.kits.fresh_vs_L3_dir\endcsname{below}
\expandafter\gdef\csname R@an.master_table.W1c.kits.fresh_vs_L3_se\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.W1c.kits.ne0\endcsname{\ensuremath{+2.64}}
\expandafter\gdef\csname R@an.master_table.W1c.kits.nefresh\endcsname{\ensuremath{+1.067}}
\expandafter\gdef\csname R@an.master_table.W1c.kits.nefresh_margin\endcsname{\ensuremath{+0.867}}
\expandafter\gdef\csname R@an.master_table.W1c.kits.params\endcsname{31.21}
\expandafter\gdef\csname R@an.master_table.W1c.kits.peak\endcsname{8.72}
\expandafter\gdef\csname R@an.master_table.W1c.kits.rule_phrase\endcsname{both legs of the registered rule are met: the fresh mean clears the \ensuremath{+0.35} pp primary bar by 0.717 pp and the non-empty-reference fresh mean clears the \ensuremath{+0.20} pp secondary bar by 0.867 pp}
\expandafter\gdef\csname R@an.master_table.W1c.kits.step\endcsname{1.13}
\expandafter\gdef\csname R@an.master_table.W1c.params\endcsname{31.14}
\expandafter\gdef\csname R@an.master_table.W1c.params_pct_vs_default\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.master_table.W1c.peak\endcsname{9.40}
\expandafter\gdef\csname R@an.master_table.W1c.step\endcsname{1.15}
\expandafter\gdef\csname R@an.master_table.W2.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W2.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.params\endcsname{30.39}
\expandafter\gdef\csname R@an.master_table.W2.acdc.peak\endcsname{10.74}
\expandafter\gdef\csname R@an.master_table.W2.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.acdc.step\endcsname{1.16}
\expandafter\gdef\csname R@an.master_table.W2.amos.d0\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.master_table.W2.amos.d0_3\endcsname{\ensuremath{+0.211}}
\expandafter\gdef\csname R@an.master_table.W2.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W2.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.amos.ne0\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.master_table.W2.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.amos.params\endcsname{31.14}
\expandafter\gdef\csname R@an.master_table.W2.amos.peak\endcsname{9.41}
\expandafter\gdef\csname R@an.master_table.W2.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.amos.step\endcsname{1.15}
\expandafter\gdef\csname R@an.master_table.W2.kits.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W2.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.params\endcsname{31.21}
\expandafter\gdef\csname R@an.master_table.W2.kits.peak\endcsname{8.73}
\expandafter\gdef\csname R@an.master_table.W2.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W2.kits.step\endcsname{1.13}
\expandafter\gdef\csname R@an.master_table.W2.params\endcsname{31.14}
\expandafter\gdef\csname R@an.master_table.W2.params_pct_vs_default\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.master_table.W2.peak\endcsname{9.41}
\expandafter\gdef\csname R@an.master_table.W2.step\endcsname{1.15}
\expandafter\gdef\csname R@an.master_table.W3.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W3.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.params\endcsname{29.55}
\expandafter\gdef\csname R@an.master_table.W3.acdc.peak\endcsname{10.61}
\expandafter\gdef\csname R@an.master_table.W3.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.acdc.step\endcsname{1.10}
\expandafter\gdef\csname R@an.master_table.W3.amos.d0\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.master_table.W3.amos.d0_3\endcsname{\ensuremath{+0.270}}
\expandafter\gdef\csname R@an.master_table.W3.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W3.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.amos.ne0\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.master_table.W3.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.amos.params\endcsname{29.57}
\expandafter\gdef\csname R@an.master_table.W3.amos.peak\endcsname{9.29}
\expandafter\gdef\csname R@an.master_table.W3.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.amos.step\endcsname{1.08}
\expandafter\gdef\csname R@an.master_table.W3.kits.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W3.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.params\endcsname{29.63}
\expandafter\gdef\csname R@an.master_table.W3.kits.peak\endcsname{8.70}
\expandafter\gdef\csname R@an.master_table.W3.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3.kits.step\endcsname{1.08}
\expandafter\gdef\csname R@an.master_table.W3.params\endcsname{29.57}
\expandafter\gdef\csname R@an.master_table.W3.params_pct_vs_default\endcsname{\ensuremath{-5.0}}
\expandafter\gdef\csname R@an.master_table.W3.peak\endcsname{9.29}
\expandafter\gdef\csname R@an.master_table.W3.step\endcsname{1.08}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.params\endcsname{29.53}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.peak\endcsname{11.04}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.acdc.step\endcsname{1.09}
\expandafter\gdef\csname R@an.master_table.W3c.amos.d0\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.master_table.W3c.amos.d0_3\endcsname{\ensuremath{+0.162}}
\expandafter\gdef\csname R@an.master_table.W3c.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W3c.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.amos.ne0\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.master_table.W3c.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.amos.params\endcsname{29.54}
\expandafter\gdef\csname R@an.master_table.W3c.amos.peak\endcsname{9.50}
\expandafter\gdef\csname R@an.master_table.W3c.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.amos.step\endcsname{1.07}
\expandafter\gdef\csname R@an.master_table.W3c.kits.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W3c.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.params\endcsname{29.61}
\expandafter\gdef\csname R@an.master_table.W3c.kits.peak\endcsname{8.50}
\expandafter\gdef\csname R@an.master_table.W3c.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W3c.kits.step\endcsname{1.06}
\expandafter\gdef\csname R@an.master_table.W3c.params\endcsname{29.54}
\expandafter\gdef\csname R@an.master_table.W3c.params_pct_vs_default\endcsname{\ensuremath{-5.1}}
\expandafter\gdef\csname R@an.master_table.W3c.peak\endcsname{9.50}
\expandafter\gdef\csname R@an.master_table.W3c.step\endcsname{1.07}
\expandafter\gdef\csname R@an.master_table.W4.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W4.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.params\endcsname{33.48}
\expandafter\gdef\csname R@an.master_table.W4.acdc.peak\endcsname{10.76}
\expandafter\gdef\csname R@an.master_table.W4.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.acdc.step\endcsname{3.84}
\expandafter\gdef\csname R@an.master_table.W4.amos.d0\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.master_table.W4.amos.d0_3\endcsname{\ensuremath{+0.076}}
\expandafter\gdef\csname R@an.master_table.W4.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W4.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.amos.ne0\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.master_table.W4.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.amos.params\endcsname{34.23}
\expandafter\gdef\csname R@an.master_table.W4.amos.peak\endcsname{10.51}
\expandafter\gdef\csname R@an.master_table.W4.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.amos.step\endcsname{3.51}
\expandafter\gdef\csname R@an.master_table.W4.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.W4.kits.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.W4.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W4.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.kits.ne0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.W4.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.kits.params\endcsname{34.30}
\expandafter\gdef\csname R@an.master_table.W4.kits.peak\endcsname{9.45}
\expandafter\gdef\csname R@an.master_table.W4.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W4.kits.step\endcsname{2.62}
\expandafter\gdef\csname R@an.master_table.W4.params\endcsname{34.23}
\expandafter\gdef\csname R@an.master_table.W4.params_pct_vs_default\endcsname{\ensuremath{+10.0}}
\expandafter\gdef\csname R@an.master_table.W4.peak\endcsname{10.51}
\expandafter\gdef\csname R@an.master_table.W4.step\endcsname{3.51}
\expandafter\gdef\csname R@an.master_table.W5.acdc.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W5.acdc.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.params\endcsname{101.63}
\expandafter\gdef\csname R@an.master_table.W5.acdc.peak\endcsname{10.66}
\expandafter\gdef\csname R@an.master_table.W5.acdc.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.acdc.step\endcsname{1.41}
\expandafter\gdef\csname R@an.master_table.W5.amos.d0\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.master_table.W5.amos.d0_3\endcsname{\ensuremath{+0.591}}
\expandafter\gdef\csname R@an.master_table.W5.amos.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.amos.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.amos.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.amos.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.amos.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.amos.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.amos.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.amos.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.amos.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.amos.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.amos.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W5.amos.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.amos.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.amos.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.amos.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.amos.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.amos.ne0\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.master_table.W5.amos.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.amos.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.amos.params\endcsname{102.37}
\expandafter\gdef\csname R@an.master_table.W5.amos.peak\endcsname{10.69}
\expandafter\gdef\csname R@an.master_table.W5.amos.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.amos.step\endcsname{1.37}
\expandafter\gdef\csname R@an.master_table.W5.kits.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.d0_3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.d3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.d3_df\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.d3_hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.d3_lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.d3_span\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.d3_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.dfresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.fresh_max\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.fresh_min\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.fresh_partial\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.fresh_phrase\endcsname{no fresh pair is registered for it}
\expandafter\gdef\csname R@an.master_table.W5.kits.fresh_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.fresh_vs_L3\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.fresh_vs_L3_abs\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.fresh_vs_L3_dir\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.fresh_vs_L3_se\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.ne0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.nefresh\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.nefresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.params\endcsname{102.43}
\expandafter\gdef\csname R@an.master_table.W5.kits.peak\endcsname{9.47}
\expandafter\gdef\csname R@an.master_table.W5.kits.rule_phrase\endcsname{--}
\expandafter\gdef\csname R@an.master_table.W5.kits.step\endcsname{1.22}
\expandafter\gdef\csname R@an.master_table.W5.params\endcsname{102.37}
\expandafter\gdef\csname R@an.master_table.W5.params_pct_vs_default\endcsname{\ensuremath{+229.0}}
\expandafter\gdef\csname R@an.master_table.W5.peak\endcsname{10.69}
\expandafter\gdef\csname R@an.master_table.W5.step\endcsname{1.37}
\expandafter\gdef\csname R@an.master_table.acdcfresh.above.clause\endcsname{7 of the 8 ACDC fresh runs of HyReX, ResEnc-M, ResEnc-matched and fn.-identical control lie above the highest of the 6 frozen default runs (92.128)}
\expandafter\gdef\csname R@an.master_table.acdcfresh.arms\endcsname{HyReX, ResEnc-M, ResEnc-matched and fn.-identical control}
\expandafter\gdef\csname R@an.master_table.acdcfresh.diff\endcsname{\ensuremath{+0.208}}
\expandafter\gdef\csname R@an.master_table.acdcfresh.diff.abs\endcsname{0.208}
\expandafter\gdef\csname R@an.master_table.acdcfresh.diff.clause\endcsname{HyReX minus ResEnc-M on the same two fresh seeds is \ensuremath{+0.208} pp (\ensuremath{+0.158} and \ensuremath{+0.259} pp seed by seed), inside the registered 0.50 pp one-seed pair floor}
\expandafter\gdef\csname R@an.master_table.acdcfresh.diff.floor\endcsname{0.50}
\expandafter\gdef\csname R@an.master_table.acdcfresh.diff.s1\endcsname{\ensuremath{+0.158}}
\expandafter\gdef\csname R@an.master_table.acdcfresh.diff.s2\endcsname{\ensuremath{+0.259}}
\expandafter\gdef\csname R@an.master_table.acdcfresh.diff.where\endcsname{inside}
\expandafter\gdef\csname R@an.master_table.acdcfresh.hero.dfresh\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.master_table.acdcfresh.hero.sd_frac\endcsname{4.55}
\expandafter\gdef\csname R@an.master_table.acdcfresh.leader.licensed\endcsname{no}
\expandafter\gdef\csname R@an.master_table.acdcfresh.n\endcsname{4}
\expandafter\gdef\csname R@an.master_table.acdcfresh.n_above\endcsname{7}
\expandafter\gdef\csname R@an.master_table.acdcfresh.n_runs\endcsname{8}
\expandafter\gdef\csname R@an.master_table.acdcfresh.poolmax\endcsname{92.128}
\expandafter\gdef\csname R@an.master_table.acdcfresh.poolmax_d\endcsname{\ensuremath{+0.119}}
\expandafter\gdef\csname R@an.master_table.acdcfresh.ref.dfresh\endcsname{\ensuremath{+0.242}}
\expandafter\gdef\csname R@an.master_table.base.acdc.params\endcsname{30.38}
\expandafter\gdef\csname R@an.master_table.base.acdc.peak\endcsname{10.27}
\expandafter\gdef\csname R@an.master_table.base.acdc.step\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.base.amos.params\endcsname{31.12}
\expandafter\gdef\csname R@an.master_table.base.amos.peak\endcsname{9.01}
\expandafter\gdef\csname R@an.master_table.base.amos.step\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.base.kits.params\endcsname{31.20}
\expandafter\gdef\csname R@an.master_table.base.kits.peak\endcsname{8.51}
\expandafter\gdef\csname R@an.master_table.base.kits.step\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.base.params\endcsname{31.12}
\expandafter\gdef\csname R@an.master_table.base.peak\endcsname{9.01}
\expandafter\gdef\csname R@an.master_table.base.step\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.bothbars.acdc_list\endcsname{HyReX and HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.master_table.bothbars.exclusive\endcsname{no}
\expandafter\gdef\csname R@an.master_table.bothbars.kits_list\endcsname{HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented), ResEnc+context, HyReX+context, function-identical control, LeanAdd with coarse large kernels, LeanDeepMid with the finest decoder convolutions, LeanAdd-NeXt with a deeper middle encoder, LeanAdd-NeXt with the coarse operator at stage 5 only and HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.master_table.bothbars.list\endcsname{HyReX and HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.master_table.bothbars.n\endcsname{12}
\expandafter\gdef\csname R@an.master_table.bothbars.n_acdc\endcsname{2}
\expandafter\gdef\csname R@an.master_table.bothbars.n_both\endcsname{2}
\expandafter\gdef\csname R@an.master_table.bothbars.n_kits\endcsname{11}
\expandafter\gdef\csname R@an.master_table.bothbars.phrase\endcsname{11 of the 12 arms with a KiTS23 fresh-seed pair and an ACDC run clear the registered KiTS23 fresh-seed bar (\ensuremath{+0.35} pp) and 2 clear the registered 0.50 pp one-seed pair floor on the ACDC guard; HyReX is in both sets, together with HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.master_table.bothbars.universe_list\endcsname{HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented), ConvNeXt-k3, ResEnc+context, HyReX+context, function-identical control, LeanAdd with coarse large kernels, LeanDeepMid with the finest decoder convolutions, LeanAdd-NeXt with a deeper middle encoder, LeanAdd-NeXt with the coarse operator at stage 5 only and HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.master_table.capctl.amos.diff\endcsname{\ensuremath{+0.157}}
\expandafter\gdef\csname R@an.master_table.capctl.amos.phrase\endcsname{ResEnc+context minus ResEnc-matched is \ensuremath{+0.157} pp on AMOS22 fresh seeds (\ensuremath{+1.28} of the 0.122 pp null scale of one fresh mean minus another)}
\expandafter\gdef\csname R@an.master_table.capctl.amos.sd_frac\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.master_table.capctl.kits.diff\endcsname{\ensuremath{-0.067}}
\expandafter\gdef\csname R@an.master_table.capctl.kits.phrase\endcsname{ResEnc+context minus ResEnc-matched is \ensuremath{-0.067} pp on KiTS23 fresh seeds (\ensuremath{-0.08} of the 0.795 pp null scale of one fresh mean minus another)}
\expandafter\gdef\csname R@an.master_table.capctl.kits.sd_frac\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.master_table.count.adjudicated_acdc\endcsname{0}
\expandafter\gdef\csname R@an.master_table.count.adjudicated_amos\endcsname{4}
\expandafter\gdef\csname R@an.master_table.count.adjudicated_kits\endcsname{25}
\expandafter\gdef\csname R@an.master_table.count.agent\endcsname{30}
\expandafter\gdef\csname R@an.master_table.count.amos_rep_phrase\endcsname{2 of the 4 arms with a finished AMOS22 fresh-seed pair and a registered verdict cleared the registered bar on that pair; 1 complete pair of an arm whose screen did not fire carries no registered verdict}
\expandafter\gdef\csname R@an.master_table.count.amos_survivor_phrase\endcsname{ResEnc-M (library preset) and ResEnc+context}
\expandafter\gdef\csname R@an.master_table.count.attribution\endcsname{6}
\expandafter\gdef\csname R@an.master_table.count.cells_done\endcsname{82}
\expandafter\gdef\csname R@an.master_table.count.control\endcsname{6}
\expandafter\gdef\csname R@an.master_table.count.fired_amos\endcsname{11}
\expandafter\gdef\csname R@an.master_table.count.fired_kits\endcsname{29}
\expandafter\gdef\csname R@an.master_table.count.kits_rep_phrase\endcsname{24 of the 25 arms with a finished KiTS23 fresh-seed pair and a registered verdict cleared the registered bar on that pair}
\expandafter\gdef\csname R@an.master_table.count.kits_survivor_phrase\endcsname{HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented), ResEnc+context, HyReX+context, branch control, HyReX, ConvNeXt one stage finer, HyReX point-fuse decoder, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), function-identical control, LeanDec with additive skips, LeanAdd with coarse large kernels, HyReX with LeanDec fine decoder, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4, LeanNeXt-s5 with one convolution at encoder stage 0, LeanNeXt-s5 with eighteen coarse blocks, LeanNeXt-s5 with twelve coarse blocks and the coarse decoder convolutions, LeanDeepMid with the finest decoder convolutions, LeanAdd-NeXt with separable coarse kernels, LeanAdd-NeXt with dilated coarse kernels, LeanAdd-NeXt with a deeper middle encoder, LeanAdd-NeXt with the coarse operator at stage 5 only and HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.master_table.count.lag_acdc\endcsname{0}
\expandafter\gdef\csname R@an.master_table.count.lag_amos\endcsname{0}
\expandafter\gdef\csname R@an.master_table.count.lag_kits\endcsname{0}
\expandafter\gdef\csname R@an.master_table.count.llm\endcsname{2}
\expandafter\gdef\csname R@an.master_table.count.norule_acdc\endcsname{4}
\expandafter\gdef\csname R@an.master_table.count.norule_amos\endcsname{1}
\expandafter\gdef\csname R@an.master_table.count.norule_kits\endcsname{0}
\expandafter\gdef\csname R@an.master_table.count.pass\endcsname{9}
\expandafter\gdef\csname R@an.master_table.count.pass_agent\endcsname{7}
\expandafter\gdef\csname R@an.master_table.count.pend_macros\endcsname{196}
\expandafter\gdef\csname R@an.master_table.count.pending_runs\endcsname{20}
\expandafter\gdef\csname R@an.master_table.count.reference\endcsname{2}
\expandafter\gdef\csname R@an.master_table.count.registered\endcsname{42}
\expandafter\gdef\csname R@an.master_table.count.rep_done_acdc\endcsname{4}
\expandafter\gdef\csname R@an.master_table.count.rep_done_amos\endcsname{5}
\expandafter\gdef\csname R@an.master_table.count.rep_done_kits\endcsname{25}
\expandafter\gdef\csname R@an.master_table.count.rows\endcsname{46}
\expandafter\gdef\csname R@an.master_table.count.scaled\endcsname{2}
\expandafter\gdef\csname R@an.master_table.count.survived_amos\endcsname{2}
\expandafter\gdef\csname R@an.master_table.count.survived_kits\endcsname{24}
\expandafter\gdef\csname R@an.master_table.count.unadjudicated\endcsname{4}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1L3.dcv\endcsname{\ensuremath{+0.037}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1L3.f1\endcsname{\ensuremath{-0.056}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1L3.f2\endcsname{\ensuremath{-0.149}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1L3.f3\endcsname{\ensuremath{+0.244}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1L3.f4\endcsname{\ensuremath{+0.109}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1L3.hi\endcsname{\ensuremath{+0.314}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1L3.interval\endcsname{\ensuremath{[-0.24,\,+0.31]}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1L3.lo\endcsname{\ensuremath{-0.240}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1L3.n_done\endcsname{4}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1L3.npos\endcsname{2}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1L3.status\endcsname{complete}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1L3.word\endcsname{improves on average (2/4 folds)}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1base.dcv\endcsname{\ensuremath{+0.370}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1base.f1\endcsname{\ensuremath{+0.283}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1base.f2\endcsname{\ensuremath{+0.358}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1base.f3\endcsname{\ensuremath{+0.397}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1base.f4\endcsname{\ensuremath{+0.440}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1base.hi\endcsname{\ensuremath{+0.476}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1base.interval\endcsname{\ensuremath{[+0.26,\,+0.48]}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1base.lo\endcsname{\ensuremath{+0.263}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1base.n_done\endcsname{4}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1base.npos\endcsname{4}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1base.status\endcsname{complete}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L1base.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L3base.dcv\endcsname{\ensuremath{+0.333}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L3base.f1\endcsname{\ensuremath{+0.339}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L3base.f2\endcsname{\ensuremath{+0.508}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L3base.f3\endcsname{\ensuremath{+0.153}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L3base.f4\endcsname{\ensuremath{+0.331}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L3base.hi\endcsname{\ensuremath{+0.563}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L3base.interval\endcsname{\ensuremath{[+0.10,\,+0.56]}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L3base.lo\endcsname{\ensuremath{+0.102}}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L3base.n_done\endcsname{4}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L3base.npos\endcsname{4}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L3base.status\endcsname{complete}
\expandafter\gdef\csname R@an.master_table.cv.acdc.L3base.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.master_table.cv.acdc.complete\endcsname{yes}
\expandafter\gdef\csname R@an.master_table.cv.acdc.n_runs\endcsname{12}
\expandafter\gdef\csname R@an.master_table.cv.acdc.n_runs_done\endcsname{12}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1L3.dcv\endcsname{\ensuremath{+0.178}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1L3.f1\endcsname{\ensuremath{+0.371}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1L3.f2\endcsname{\ensuremath{+0.405}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1L3.f3\endcsname{\ensuremath{-0.365}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1L3.f4\endcsname{\ensuremath{+0.299}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1L3.hi\endcsname{\ensuremath{+0.758}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1L3.interval\endcsname{\ensuremath{[-0.40,\,+0.76]}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1L3.lo\endcsname{\ensuremath{-0.402}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1L3.n_done\endcsname{4}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1L3.npos\endcsname{3}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1L3.status\endcsname{complete}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1L3.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1base.dcv\endcsname{\ensuremath{+0.406}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1base.f1\endcsname{\ensuremath{+0.341}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1base.f2\endcsname{\ensuremath{+0.770}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1base.f3\endcsname{\ensuremath{-0.171}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1base.f4\endcsname{\ensuremath{+0.685}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1base.hi\endcsname{\ensuremath{+1.086}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1base.interval\endcsname{\ensuremath{[-0.27,\,+1.09]}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1base.lo\endcsname{\ensuremath{-0.274}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1base.n_done\endcsname{4}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1base.npos\endcsname{3}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1base.status\endcsname{complete}
\expandafter\gdef\csname R@an.master_table.cv.amos.L1base.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.master_table.cv.amos.L3base.dcv\endcsname{\ensuremath{+0.228}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L3base.f1\endcsname{\ensuremath{-0.030}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L3base.f2\endcsname{\ensuremath{+0.365}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L3base.f3\endcsname{\ensuremath{+0.194}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L3base.f4\endcsname{\ensuremath{+0.385}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L3base.hi\endcsname{\ensuremath{+0.535}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L3base.interval\endcsname{\ensuremath{[-0.08,\,+0.54]}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L3base.lo\endcsname{\ensuremath{-0.078}}
\expandafter\gdef\csname R@an.master_table.cv.amos.L3base.n_done\endcsname{4}
\expandafter\gdef\csname R@an.master_table.cv.amos.L3base.npos\endcsname{3}
\expandafter\gdef\csname R@an.master_table.cv.amos.L3base.status\endcsname{complete}
\expandafter\gdef\csname R@an.master_table.cv.amos.L3base.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.master_table.cv.amos.complete\endcsname{yes}
\expandafter\gdef\csname R@an.master_table.cv.amos.n_runs\endcsname{12}
\expandafter\gdef\csname R@an.master_table.cv.amos.n_runs_done\endcsname{12}
\expandafter\gdef\csname R@an.master_table.cv.complete.ds\endcsname{AMOS22, KiTS23 and ACDC}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1L3.dcv\endcsname{\ensuremath{+1.465}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1L3.f1\endcsname{\ensuremath{+0.274}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1L3.f2\endcsname{\ensuremath{+2.742}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1L3.f3\endcsname{\ensuremath{+0.981}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1L3.f4\endcsname{\ensuremath{+1.865}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1L3.hi\endcsname{\ensuremath{+3.170}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1L3.interval\endcsname{\ensuremath{[-0.24,\,+3.17]}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1L3.lo\endcsname{\ensuremath{-0.239}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1L3.n_done\endcsname{4}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1L3.npos\endcsname{4}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1L3.status\endcsname{complete}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1L3.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1base.dcv\endcsname{\ensuremath{+2.147}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1base.f1\endcsname{\ensuremath{+2.581}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1base.f2\endcsname{\ensuremath{+2.937}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1base.f3\endcsname{\ensuremath{+1.357}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1base.f4\endcsname{\ensuremath{+1.713}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1base.hi\endcsname{\ensuremath{+3.319}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1base.interval\endcsname{\ensuremath{[+0.98,\,+3.32]}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1base.lo\endcsname{\ensuremath{+0.976}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1base.n_done\endcsname{4}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1base.npos\endcsname{4}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1base.status\endcsname{complete}
\expandafter\gdef\csname R@an.master_table.cv.kits.L1base.word\endcsname{improves in every fold}
\expandafter\gdef\csname R@an.master_table.cv.kits.L3base.dcv\endcsname{\ensuremath{+0.682}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L3base.f1\endcsname{\ensuremath{+2.308}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L3base.f2\endcsname{\ensuremath{+0.196}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L3base.f3\endcsname{\ensuremath{+0.375}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L3base.f4\endcsname{\ensuremath{-0.152}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L3base.hi\endcsname{\ensuremath{+2.441}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L3base.interval\endcsname{\ensuremath{[-1.08,\,+2.44]}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L3base.lo\endcsname{\ensuremath{-1.078}}
\expandafter\gdef\csname R@an.master_table.cv.kits.L3base.n_done\endcsname{4}
\expandafter\gdef\csname R@an.master_table.cv.kits.L3base.npos\endcsname{3}
\expandafter\gdef\csname R@an.master_table.cv.kits.L3base.status\endcsname{complete}
\expandafter\gdef\csname R@an.master_table.cv.kits.L3base.word\endcsname{improves on average (3/4 folds)}
\expandafter\gdef\csname R@an.master_table.cv.kits.complete\endcsname{yes}
\expandafter\gdef\csname R@an.master_table.cv.kits.n_runs\endcsname{12}
\expandafter\gdef\csname R@an.master_table.cv.kits.n_runs_done\endcsname{12}
\expandafter\gdef\csname R@an.master_table.cv.n_done\endcsname{36}
\expandafter\gdef\csname R@an.master_table.cv.n_runs\endcsname{36}
\expandafter\gdef\csname R@an.master_table.cv.pending.ds\endcsname{no dataset}
\expandafter\gdef\csname R@an.master_table.cv.phrase\endcsname{the cross-validation is complete on AMOS22, KiTS23 and ACDC}
\expandafter\gdef\csname R@an.master_table.fig.refstrip.n_amos\endcsname{38}
\expandafter\gdef\csname R@an.master_table.fig.refstrip.n_kits\endcsname{32}
\expandafter\gdef\csname R@an.master_table.freshtop.acdc.leader\endcsname{HyReX}
\expandafter\gdef\csname R@an.master_table.freshtop.acdc.leader_d\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.master_table.freshtop.acdc.margin\endcsname{\ensuremath{+0.131}}
\expandafter\gdef\csname R@an.master_table.freshtop.acdc.margin_sd_frac\endcsname{1.33}
\expandafter\gdef\csname R@an.master_table.freshtop.acdc.n_pairs\endcsname{4}
\expandafter\gdef\csname R@an.master_table.freshtop.acdc.order\endcsname{HyReX \ensuremath{+0.450}, ResEnc-matched (re-implemented) \ensuremath{+0.319}, ResEnc-M (library preset) \ensuremath{+0.242}, function-identical control \ensuremath{+0.117}}
\expandafter\gdef\csname R@an.master_table.freshtop.acdc.phrase\endcsname{of the 4 ACDC arms with a complete registered fresh pair, HyReX is highest at \ensuremath{+0.450} pp and ResEnc-matched (re-implemented) next at \ensuremath{+0.319} pp, 0.131 pp apart (1.33 times the 0.099 pp null scale of one fresh mean minus another)}
\expandafter\gdef\csname R@an.master_table.freshtop.acdc.runner_up\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.master_table.freshtop.acdc.runner_up_d\endcsname{\ensuremath{+0.319}}
\expandafter\gdef\csname R@an.master_table.freshtop.amos.leader\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.master_table.freshtop.amos.leader_d\endcsname{\ensuremath{+0.465}}
\expandafter\gdef\csname R@an.master_table.freshtop.amos.margin\endcsname{\ensuremath{+0.010}}
\expandafter\gdef\csname R@an.master_table.freshtop.amos.margin_sd_frac\endcsname{0.08}
\expandafter\gdef\csname R@an.master_table.freshtop.amos.n_pairs\endcsname{5}
\expandafter\gdef\csname R@an.master_table.freshtop.amos.order\endcsname{ResEnc-M (library preset) \ensuremath{+0.465}, ResEnc+context \ensuremath{+0.455}, ResEnc-matched (re-implemented) \ensuremath{+0.298}, ConvNeXt-k3 \ensuremath{+0.194}, HyReX \ensuremath{+0.132}}
\expandafter\gdef\csname R@an.master_table.freshtop.amos.phrase\endcsname{of the 5 AMOS22 arms with a complete registered fresh pair, ResEnc-M (library preset) is highest at \ensuremath{+0.465} pp and ResEnc+context next at \ensuremath{+0.455} pp, 0.010 pp apart (inside the 0.122 pp null scale of one fresh mean minus another)}
\expandafter\gdef\csname R@an.master_table.freshtop.amos.runner_up\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.master_table.freshtop.amos.runner_up_d\endcsname{\ensuremath{+0.455}}
\expandafter\gdef\csname R@an.master_table.freshtop.kits.leader\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.master_table.freshtop.kits.leader_d\endcsname{\ensuremath{+3.475}}
\expandafter\gdef\csname R@an.master_table.freshtop.kits.margin\endcsname{\ensuremath{+0.814}}
\expandafter\gdef\csname R@an.master_table.freshtop.kits.margin_sd_frac\endcsname{1.02}
\expandafter\gdef\csname R@an.master_table.freshtop.kits.n_pairs\endcsname{25}
\expandafter\gdef\csname R@an.master_table.freshtop.kits.order\endcsname{ResEnc-M (library preset) \ensuremath{+3.475}, LeanAdd-NeXt with a deeper middle encoder \ensuremath{+2.662}, LeanAdd-NeXt with the coarse operator at stage 5 only \ensuremath{+2.440}, HyReX + decoder capacity \ensuremath{+2.401}, LeanAdd-NeXt with separable coarse kernels \ensuremath{+2.382}, ResEnc-matched (re-implemented) \ensuremath{+2.313}, LeanDeepMid with the finest decoder convolutions \ensuremath{+2.289}, LeanDec with additive skips \ensuremath{+2.285}, ResEnc+context \ensuremath{+2.246}, HyReX with LeanDec fine decoder \ensuremath{+2.165}, HyReX \ensuremath{+2.094}, LeanDec (default with one conv per decoder stage) \ensuremath{+1.892}, LeanNeXt-s5 with twelve coarse blocks and the coarse decoder convolutions \ensuremath{+1.877}, LeanAdd-NeXt with dilated coarse kernels \ensuremath{+1.838}, LeanNeXt-s5 with one convolution at encoder stage 0 \ensuremath{+1.731}, HyReX with 9-kernel coarse stages \ensuremath{+1.704}, HyReX+context \ensuremath{+1.591}, HyReX point-fuse decoder \ensuremath{+1.477}, LeanAdd with coarse large kernels \ensuremath{+1.448}, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 \ensuremath{+1.375}, LeanNeXt-s5 with eighteen coarse blocks \ensuremath{+1.249}, function-identical control \ensuremath{+1.176}, branch control \ensuremath{+1.067}, HyReX, ConvNeXt one stage finer \ensuremath{+0.570}, ConvNeXt-k3 \ensuremath{+0.110}}
\expandafter\gdef\csname R@an.master_table.freshtop.kits.phrase\endcsname{of the 25 KiTS23 arms with a complete registered fresh pair, ResEnc-M (library preset) is highest at \ensuremath{+3.475} pp and LeanAdd-NeXt with a deeper middle encoder next at \ensuremath{+2.662} pp, 0.814 pp apart (1.02 times the 0.795 pp null scale of one fresh mean minus another)}
\expandafter\gdef\csname R@an.master_table.freshtop.kits.runner_up\endcsname{LeanAdd-NeXt with a deeper middle encoder}
\expandafter\gdef\csname R@an.master_table.freshtop.kits.runner_up_d\endcsname{\ensuremath{+2.662}}
\expandafter\gdef\csname R@an.master_table.glyphkey\endcsname{the two co-primary screens in the order AMOS22, KiTS23 (\cmark{} fires, \ensuremath{\circ} no evidence, \ensuremath{\cdots} scheduled, -- not scheduled); then \textsf{R} and the two replication states in the same order (\cmark{} survived, \xmark{} not survived, \ensuremath{\cdots} scheduled, \ensuremath{\cdot} none registered); then \textsf{G} and the ACDC guard (\cmark{} at or above the registered guard, \xmark{} below it, -- not scheduled); and \textbf{PASS} where the registered code is PASS}
\expandafter\gdef\csname R@an.master_table.guard.floor_list\endcsname{HyReX and HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.master_table.guard.floor_phrase\endcsname{two of the 12 arms with a finished ACDC run reach the registered 0.50 pp one-seed pair floor on their discovery-seed gain (HyReX and HyReX with 9-kernel coarse stages)}
\expandafter\gdef\csname R@an.master_table.guard.hero.place\endcsname{the largest discovery-seed gain of the 12 arms with a finished ACDC run}
\expandafter\gdef\csname R@an.master_table.guard.hero.rank\endcsname{1}
\expandafter\gdef\csname R@an.master_table.guard.leader\endcsname{HyReX}
\expandafter\gdef\csname R@an.master_table.guard.leader_d\endcsname{\ensuremath{+0.616}}
\expandafter\gdef\csname R@an.master_table.guard.n_arms\endcsname{12}
\expandafter\gdef\csname R@an.master_table.guard.n_floor\endcsname{2}
\expandafter\gdef\csname R@an.master_table.guard.order\endcsname{HyReX \ensuremath{+0.616}, HyReX with 9-kernel coarse stages \ensuremath{+0.573}, HyReX+context \ensuremath{+0.451}, LeanDeepMid with the finest decoder convolutions \ensuremath{+0.362}, ResEnc-M (library preset) \ensuremath{+0.336}, ResEnc+context \ensuremath{+0.315}, ResEnc-matched (re-implemented) \ensuremath{+0.283}, LeanAdd-NeXt with a deeper middle encoder \ensuremath{+0.229}, function-identical control \ensuremath{-0.013}, ConvNeXt-k3 \ensuremath{-0.015}, LeanAdd with coarse large kernels \ensuremath{-0.181}, LeanAdd-NeXt with the coarse operator at stage 5 only \ensuremath{-0.252}}
\expandafter\gdef\csname R@an.master_table.guard.others.n\endcsname{11}
\expandafter\gdef\csname R@an.master_table.guard.others.top\endcsname{HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.master_table.guard.others.top_d\endcsname{\ensuremath{+0.573}}
\expandafter\gdef\csname R@an.master_table.guard.phrase\endcsname{HyReX records the largest discovery-seed gain of the 12 arms with a finished ACDC run, \ensuremath{+0.616} pp over the frozen default pool}
\expandafter\gdef\csname R@an.master_table.guard.runner_up\endcsname{HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.master_table.guard.runner_up_d\endcsname{\ensuremath{+0.573}}
\expandafter\gdef\csname R@an.master_table.heldout.brats.L1.delta\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.heldout.brats.L1.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.heldout.brats.L1.n\endcsname{1}
\expandafter\gdef\csname R@an.master_table.heldout.brats.L1.s0\endcsname{82.955}
\expandafter\gdef\csname R@an.master_table.heldout.brats.L1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.heldout.brats.L1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.heldout.brats.L1.sd\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.heldout.brats.L3.delta\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.heldout.brats.L3.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.heldout.brats.L3.n\endcsname{1}
\expandafter\gdef\csname R@an.master_table.heldout.brats.L3.s0\endcsname{83.046}
\expandafter\gdef\csname R@an.master_table.heldout.brats.L3.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.heldout.brats.L3.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.heldout.brats.L3.sd\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.heldout.brats.base.delta\endcsname{--}
\expandafter\gdef\csname R@an.master_table.heldout.brats.base.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.heldout.brats.base.n\endcsname{1}
\expandafter\gdef\csname R@an.master_table.heldout.brats.base.s0\endcsname{82.977}
\expandafter\gdef\csname R@an.master_table.heldout.brats.base.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.heldout.brats.base.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.heldout.brats.base.sd\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.heldout.brats.n_done\endcsname{3}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.L1.delta\endcsname{\ensuremath{+0.708}}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.L1.mean\endcsname{78.525}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.L1.n\endcsname{3}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.L1.s0\endcsname{79.236}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.L1.s1\endcsname{78.235}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.L1.s2\endcsname{78.104}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.L1.sd\endcsname{0.619}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.L3.delta\endcsname{\ensuremath{+0.711}}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.L3.mean\endcsname{78.528}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.L3.n\endcsname{3}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.L3.s0\endcsname{77.848}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.L3.s1\endcsname{79.739}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.L3.s2\endcsname{77.996}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.L3.sd\endcsname{1.052}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.base.delta\endcsname{--}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.base.mean\endcsname{77.817}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.base.n\endcsname{3}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.base.s0\endcsname{77.567}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.base.s1\endcsname{78.150}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.base.s2\endcsname{77.733}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.base.sd\endcsname{0.301}
\expandafter\gdef\csname R@an.master_table.heldout.btcv.n_done\endcsname{9}
\expandafter\gdef\csname R@an.master_table.heldout.lits.L1.delta\endcsname{\ensuremath{+1.132}}
\expandafter\gdef\csname R@an.master_table.heldout.lits.L1.mean\endcsname{81.927}
\expandafter\gdef\csname R@an.master_table.heldout.lits.L1.n\endcsname{3}
\expandafter\gdef\csname R@an.master_table.heldout.lits.L1.s0\endcsname{81.799}
\expandafter\gdef\csname R@an.master_table.heldout.lits.L1.s1\endcsname{81.763}
\expandafter\gdef\csname R@an.master_table.heldout.lits.L1.s2\endcsname{82.217}
\expandafter\gdef\csname R@an.master_table.heldout.lits.L1.sd\endcsname{0.252}
\expandafter\gdef\csname R@an.master_table.heldout.lits.L3.delta\endcsname{\ensuremath{+0.499}}
\expandafter\gdef\csname R@an.master_table.heldout.lits.L3.mean\endcsname{81.294}
\expandafter\gdef\csname R@an.master_table.heldout.lits.L3.n\endcsname{3}
\expandafter\gdef\csname R@an.master_table.heldout.lits.L3.s0\endcsname{80.804}
\expandafter\gdef\csname R@an.master_table.heldout.lits.L3.s1\endcsname{82.172}
\expandafter\gdef\csname R@an.master_table.heldout.lits.L3.s2\endcsname{80.905}
\expandafter\gdef\csname R@an.master_table.heldout.lits.L3.sd\endcsname{0.762}
\expandafter\gdef\csname R@an.master_table.heldout.lits.base.delta\endcsname{--}
\expandafter\gdef\csname R@an.master_table.heldout.lits.base.mean\endcsname{80.795}
\expandafter\gdef\csname R@an.master_table.heldout.lits.base.n\endcsname{3}
\expandafter\gdef\csname R@an.master_table.heldout.lits.base.s0\endcsname{79.865}
\expandafter\gdef\csname R@an.master_table.heldout.lits.base.s1\endcsname{79.977}
\expandafter\gdef\csname R@an.master_table.heldout.lits.base.s2\endcsname{82.543}
\expandafter\gdef\csname R@an.master_table.heldout.lits.base.sd\endcsname{1.515}
\expandafter\gdef\csname R@an.master_table.heldout.lits.n_done\endcsname{9}
\expandafter\gdef\csname R@an.master_table.heldout.n_done\endcsname{21}
\expandafter\gdef\csname R@an.master_table.heldout.n_pending\endcsname{6}
\expandafter\gdef\csname R@an.master_table.heldout.n_registered\endcsname{27}
\expandafter\gdef\csname R@an.master_table.heldout.phrase\endcsname{21 of the 27 registered held-out runs (3 datasets, 3 frozen arms, 3 seeds each) have finished}
\expandafter\gdef\csname R@an.master_table.implctl.phrase\endcsname{the implementation control, the function-identical rebuild of the default network, reads \ensuremath{+1.364} pp on KiTS23 and \ensuremath{+0.007} pp on AMOS22 at its first seed, and \ensuremath{+1.176} pp on its KiTS23 fresh seeds 1 and 2}
\expandafter\gdef\csname R@an.master_table.more.2.groups\endcsname{Design wave 7, Design wave 8 and Other registered arms}
\expandafter\gdef\csname R@an.master_table.more.2.idx\endcsname{2}
\expandafter\gdef\csname R@an.master_table.more.2.n_arms\endcsname{12}
\expandafter\gdef\csname R@an.master_table.more.groups\endcsname{Design wave 7, Design wave 8 and Other registered arms}
\expandafter\gdef\csname R@an.master_table.more.n_arms\endcsname{12}
\expandafter\gdef\csname R@an.master_table.more.n_floats\endcsname{1}
\expandafter\gdef\csname R@an.master_table.more.n_total\endcsname{2}
\expandafter\gdef\csname R@an.master_table.pool.acdc.hi\endcsname{92.128}
\expandafter\gdef\csname R@an.master_table.pool.acdc.lo\endcsname{91.853}
\expandafter\gdef\csname R@an.master_table.pool.acdc.mean\endcsname{92.009}
\expandafter\gdef\csname R@an.master_table.pool.acdc.n\endcsname{6}
\expandafter\gdef\csname R@an.master_table.pool.acdc.sd\endcsname{0.099}
\expandafter\gdef\csname R@an.master_table.pool.acdc.spread\endcsname{0.275}
\expandafter\gdef\csname R@an.master_table.pool.acdc.spread_bars\endcsname{0.79}
\expandafter\gdef\csname R@an.master_table.pool.amos.hi\endcsname{87.873}
\expandafter\gdef\csname R@an.master_table.pool.amos.lo\endcsname{87.552}
\expandafter\gdef\csname R@an.master_table.pool.amos.mean\endcsname{87.701}
\expandafter\gdef\csname R@an.master_table.pool.amos.n\endcsname{6}
\expandafter\gdef\csname R@an.master_table.pool.amos.sd\endcsname{0.122}
\expandafter\gdef\csname R@an.master_table.pool.amos.spread\endcsname{0.321}
\expandafter\gdef\csname R@an.master_table.pool.amos.spread_bars\endcsname{0.92}
\expandafter\gdef\csname R@an.master_table.pool.kits.hi\endcsname{84.272}
\expandafter\gdef\csname R@an.master_table.pool.kits.lo\endcsname{82.749}
\expandafter\gdef\csname R@an.master_table.pool.kits.mean\endcsname{83.378}
\expandafter\gdef\csname R@an.master_table.pool.kits.n\endcsname{3}
\expandafter\gdef\csname R@an.master_table.pool.kits.sd\endcsname{0.795}
\expandafter\gdef\csname R@an.master_table.pool.kits.spread\endcsname{1.522}
\expandafter\gdef\csname R@an.master_table.pool.kits.spread_bars\endcsname{4.35}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.D2.gpp\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.D2.hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.D2.lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.D2.params_frac\endcsname{0.25}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.D2.params_x\endcsname{4.02}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.D2.peak_frac\endcsname{0.90}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.D2.pneg\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.D2.ppm\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.D2.ppm_ref\endcsname{0.0024}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.D2.ratio\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.D2.step_frac\endcsname{0.53}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.D2.vs_ref\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L1b.gpp\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L1b.hi\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L1b.lo\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L1b.params_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L1b.params_x\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L1b.peak_frac\endcsname{1.01}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L1b.pneg\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L1b.ppm\endcsname{0.0031}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L1b.ppm_ref\endcsname{0.0024}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L1b.ratio\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L1b.step_frac\endcsname{0.93}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L1b.vs_ref\endcsname{\ensuremath{+0.077}}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L2.gpp\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L2.hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L2.lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L2.params_frac\endcsname{0.23}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L2.params_x\endcsname{4.29}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L2.peak_frac\endcsname{1.09}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L2.pneg\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L2.ppm\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L2.ppm_ref\endcsname{0.0024}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L2.ratio\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L2.step_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L2.vs_ref\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L3.gpp\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L3.hi\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L3.lo\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L3.params_frac\endcsname{0.28}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L3.params_x\endcsname{3.52}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L3.peak_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L3.pneg\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L3.ppm\endcsname{0.0156}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L3.ppm_ref\endcsname{0.0024}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L3.ratio\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L3.step_frac\endcsname{1.09}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L3.vs_ref\endcsname{\ensuremath{+0.208}}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L4.gpp\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L4.hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L4.lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L4.params_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L4.params_x\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L4.peak_frac\endcsname{0.98}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L4.pneg\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L4.ppm\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L4.ppm_ref\endcsname{0.0024}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L4.ratio\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L4.step_frac\endcsname{1.01}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L4.vs_ref\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L6.gpp\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L6.hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L6.lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L6.params_frac\endcsname{0.30}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L6.params_x\endcsname{3.35}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L6.peak_frac\endcsname{1.10}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L6.pneg\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L6.ppm\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L6.ppm_ref\endcsname{0.0024}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L6.ratio\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L6.step_frac\endcsname{1.35}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.L6.vs_ref\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.refgain\endcsname{\ensuremath{+0.242}}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.fresh.status\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.D2.gpp\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.D2.hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.D2.lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.D2.params_frac\endcsname{0.25}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.D2.params_x\endcsname{4.02}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.D2.peak_frac\endcsname{0.90}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.D2.pneg\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.D2.ppm\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.D2.ppm_ref\endcsname{0.0033}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.D2.ratio\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.D2.step_frac\endcsname{0.53}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.D2.vs_ref\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L1b.gpp\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L1b.hi\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L1b.lo\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L1b.params_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L1b.params_x\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L1b.peak_frac\endcsname{1.01}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L1b.pneg\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L1b.ppm\endcsname{0.0028}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L1b.ppm_ref\endcsname{0.0033}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L1b.ratio\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L1b.step_frac\endcsname{0.93}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L1b.vs_ref\endcsname{\ensuremath{-0.052}}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L2.gpp\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L2.hi\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L2.lo\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L2.params_frac\endcsname{0.23}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L2.params_x\endcsname{4.29}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L2.peak_frac\endcsname{1.09}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L2.pneg\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L2.ppm\endcsname{-0.0006}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L2.ppm_ref\endcsname{0.0033}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L2.ratio\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L2.step_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L2.vs_ref\endcsname{\ensuremath{-0.350}}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L3.gpp\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L3.hi\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L3.lo\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L3.params_frac\endcsname{0.28}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L3.params_x\endcsname{3.52}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L3.peak_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L3.pneg\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L3.ppm\endcsname{0.0214}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L3.ppm_ref\endcsname{0.0033}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L3.ratio\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L3.step_frac\endcsname{1.09}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L3.vs_ref\endcsname{\ensuremath{+0.281}}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L4.gpp\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L4.hi\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L4.lo\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L4.params_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L4.params_x\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L4.peak_frac\endcsname{0.98}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L4.pneg\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L4.ppm\endcsname{0.0031}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L4.ppm_ref\endcsname{0.0033}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L4.ratio\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L4.step_frac\endcsname{1.01}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L4.vs_ref\endcsname{\ensuremath{-0.020}}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L6.gpp\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L6.hi\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L6.lo\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L6.params_frac\endcsname{0.30}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L6.params_x\endcsname{3.35}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L6.peak_frac\endcsname{1.10}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L6.pneg\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L6.ppm\endcsname{0.0149}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L6.ppm_ref\endcsname{0.0033}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L6.ratio\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L6.step_frac\endcsname{1.35}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.L6.vs_ref\endcsname{\ensuremath{+0.116}}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.refgain\endcsname{\ensuremath{+0.336}}
\expandafter\gdef\csname R@an.master_table.recovery.acdc.s0.status\endcsname{withheld}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.D2.gpp\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.D2.hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.D2.lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.D2.params_frac\endcsname{0.25}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.D2.params_x\endcsname{3.93}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.D2.peak_frac\endcsname{0.74}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.D2.pneg\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.D2.ppm\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.D2.ppm_ref\endcsname{0.0045}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.D2.ratio\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.D2.step_frac\endcsname{0.56}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.D2.vs_ref\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L1b.gpp\endcsname{0.64}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L1b.hi\endcsname{1.21}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L1b.lo\endcsname{0.23}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L1b.params_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L1b.params_x\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L1b.peak_frac\endcsname{0.97}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L1b.pneg\endcsname{0.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L1b.ppm\endcsname{0.0029}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L1b.ppm_ref\endcsname{0.0045}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L1b.ratio\endcsname{0.64}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L1b.step_frac\endcsname{0.94}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L1b.vs_ref\endcsname{\ensuremath{-0.167}}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L2.gpp\endcsname{1.75}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L2.hi\endcsname{0.91}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L2.lo\endcsname{0.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L2.params_frac\endcsname{0.24}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L2.params_x\endcsname{4.19}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L2.peak_frac\endcsname{0.91}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L2.pneg\endcsname{0.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L2.ppm\endcsname{0.0080}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L2.ppm_ref\endcsname{0.0045}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L2.ratio\endcsname{0.42}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L2.step_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L2.vs_ref\endcsname{\ensuremath{-0.270}}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L3.gpp\endcsname{0.98}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L3.hi\endcsname{0.74}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L3.lo\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L3.params_frac\endcsname{0.29}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L3.params_x\endcsname{3.46}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L3.peak_frac\endcsname{0.98}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L3.pneg\endcsname{0.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L3.ppm\endcsname{0.0045}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L3.ppm_ref\endcsname{0.0045}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L3.ratio\endcsname{0.28}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L3.step_frac\endcsname{1.04}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L3.vs_ref\endcsname{\ensuremath{-0.332}}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L4.gpp\endcsname{0.97}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L4.hi\endcsname{1.72}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L4.lo\endcsname{0.55}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L4.params_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L4.params_x\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L4.peak_frac\endcsname{0.98}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L4.pneg\endcsname{0.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L4.ppm\endcsname{0.0044}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L4.ppm_ref\endcsname{0.0045}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L4.ratio\endcsname{0.98}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L4.step_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L4.vs_ref\endcsname{\ensuremath{-0.010}}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L6.gpp\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L6.hi\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L6.lo\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L6.params_frac\endcsname{0.30}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L6.params_x\endcsname{3.29}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L6.peak_frac\endcsname{0.94}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L6.pneg\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L6.ppm\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L6.ppm_ref\endcsname{0.0045}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L6.ratio\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L6.step_frac\endcsname{1.28}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.L6.vs_ref\endcsname{--}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.refgain\endcsname{\ensuremath{+0.465}}
\expandafter\gdef\csname R@an.master_table.recovery.amos.fresh.status\endcsname{published}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.D2.gpp\endcsname{-2.20}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.D2.hi\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.D2.lo\endcsname{\ensuremath{-1.24}}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.D2.params_frac\endcsname{0.25}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.D2.params_x\endcsname{3.93}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.D2.peak_frac\endcsname{0.74}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.D2.pneg\endcsname{0.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.D2.ppm\endcsname{-0.0139}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.D2.ppm_ref\endcsname{0.0063}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.D2.ratio\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.D2.step_frac\endcsname{0.56}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.D2.vs_ref\endcsname{\ensuremath{-1.009}}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L1b.gpp\endcsname{0.21}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L1b.hi\endcsname{0.65}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L1b.lo\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L1b.params_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L1b.params_x\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L1b.peak_frac\endcsname{0.97}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L1b.pneg\endcsname{0.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L1b.ppm\endcsname{0.0013}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L1b.ppm_ref\endcsname{0.0063}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L1b.ratio\endcsname{0.21}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L1b.step_frac\endcsname{0.94}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L1b.vs_ref\endcsname{\ensuremath{-0.509}}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L2.gpp\endcsname{2.34}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L2.hi\endcsname{1.11}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L2.lo\endcsname{0.16}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L2.params_frac\endcsname{0.24}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L2.params_x\endcsname{4.19}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L2.peak_frac\endcsname{0.91}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L2.pneg\endcsname{0.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L2.ppm\endcsname{0.0148}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L2.ppm_ref\endcsname{0.0063}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L2.ratio\endcsname{0.56}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L2.step_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L2.vs_ref\endcsname{\ensuremath{-0.285}}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L3.gpp\endcsname{2.04}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L3.hi\endcsname{1.16}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L3.lo\endcsname{0.19}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L3.params_frac\endcsname{0.29}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L3.params_x\endcsname{3.46}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L3.peak_frac\endcsname{0.98}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L3.pneg\endcsname{0.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L3.ppm\endcsname{0.0129}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L3.ppm_ref\endcsname{0.0063}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L3.ratio\endcsname{0.59}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L3.step_frac\endcsname{1.04}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L3.vs_ref\endcsname{\ensuremath{-0.265}}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L4.gpp\endcsname{0.66}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L4.hi\endcsname{1.26}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L4.lo\endcsname{0.26}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L4.params_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L4.params_x\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L4.peak_frac\endcsname{0.98}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L4.pneg\endcsname{0.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L4.ppm\endcsname{0.0042}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L4.ppm_ref\endcsname{0.0063}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L4.ratio\endcsname{0.66}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L4.step_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L4.vs_ref\endcsname{\ensuremath{-0.217}}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L6.gpp\endcsname{0.08}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L6.hi\endcsname{0.43}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L6.lo\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L6.params_frac\endcsname{0.30}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L6.params_x\endcsname{3.29}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L6.peak_frac\endcsname{0.94}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L6.pneg\endcsname{0.00}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L6.ppm\endcsname{0.0005}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L6.ppm_ref\endcsname{0.0063}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L6.ratio\endcsname{0.02}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L6.step_frac\endcsname{1.28}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.L6.vs_ref\endcsname{\ensuremath{-0.631}}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.refgain\endcsname{\ensuremath{+0.647}}
\expandafter\gdef\csname R@an.master_table.recovery.amos.s0.status\endcsname{published}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.D2.gpp\endcsname{2.14}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.D2.hi\endcsname{0.99}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.D2.lo\endcsname{0.15}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.D2.params_frac\endcsname{0.25}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.D2.params_x\endcsname{3.92}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.D2.peak_frac\endcsname{0.80}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.D2.pneg\endcsname{0.00}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.D2.ppm\endcsname{0.0725}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.D2.ppm_ref\endcsname{0.0340}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.D2.ratio\endcsname{0.54}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.D2.step_frac\endcsname{0.61}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.D2.vs_ref\endcsname{\ensuremath{-1.584}}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L1b.gpp\endcsname{0.67}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L1b.hi\endcsname{1.15}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L1b.lo\endcsname{0.29}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L1b.params_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L1b.params_x\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L1b.peak_frac\endcsname{0.97}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L1b.pneg\endcsname{0.00}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L1b.ppm\endcsname{0.0226}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L1b.ppm_ref\endcsname{0.0340}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L1b.ratio\endcsname{0.67}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L1b.step_frac\endcsname{0.92}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L1b.vs_ref\endcsname{\ensuremath{-1.162}}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L2.gpp\endcsname{0.13}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L2.hi\endcsname{0.41}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L2.lo\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L2.params_frac\endcsname{0.24}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L2.params_x\endcsname{4.18}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L2.peak_frac\endcsname{0.94}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L2.pneg\endcsname{0.00}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L2.ppm\endcsname{0.0045}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L2.ppm_ref\endcsname{0.0340}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L2.ratio\endcsname{0.03}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L2.step_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L2.vs_ref\endcsname{\ensuremath{-3.365}}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L3.gpp\endcsname{2.08}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L3.hi\endcsname{1.07}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L3.lo\endcsname{0.22}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L3.params_frac\endcsname{0.29}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L3.params_x\endcsname{3.45}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L3.peak_frac\endcsname{0.98}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L3.pneg\endcsname{0.00}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L3.ppm\endcsname{0.0706}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L3.ppm_ref\endcsname{0.0340}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L3.ratio\endcsname{0.60}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L3.step_frac\endcsname{1.05}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L3.vs_ref\endcsname{\ensuremath{-1.382}}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L4.gpp\endcsname{0.64}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L4.hi\endcsname{1.13}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L4.lo\endcsname{0.27}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L4.params_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L4.params_x\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L4.peak_frac\endcsname{0.98}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L4.pneg\endcsname{0.00}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L4.ppm\endcsname{0.0218}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L4.ppm_ref\endcsname{0.0340}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L4.ratio\endcsname{0.65}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L4.step_frac\endcsname{0.97}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L4.vs_ref\endcsname{\ensuremath{-1.229}}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L6.gpp\endcsname{1.50}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L6.hi\endcsname{0.88}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L6.lo\endcsname{0.05}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L6.params_frac\endcsname{0.30}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L6.params_x\endcsname{3.28}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L6.peak_frac\endcsname{0.96}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L6.pneg\endcsname{0.00}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L6.ppm\endcsname{0.0511}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L6.ppm_ref\endcsname{0.0340}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L6.ratio\endcsname{0.46}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L6.step_frac\endcsname{1.22}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.L6.vs_ref\endcsname{\ensuremath{-1.884}}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.refgain\endcsname{\ensuremath{+3.475}}
\expandafter\gdef\csname R@an.master_table.recovery.kits.fresh.status\endcsname{published}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.D2.gpp\endcsname{3.97}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.D2.hi\endcsname{3.51}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.D2.lo\endcsname{0.21}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.D2.params_frac\endcsname{0.25}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.D2.params_x\endcsname{3.92}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.D2.peak_frac\endcsname{0.80}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.D2.pneg\endcsname{0.60}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.D2.ppm\endcsname{0.0903}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.D2.ppm_ref\endcsname{0.0227}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.D2.ratio\endcsname{1.01}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.D2.step_frac\endcsname{0.61}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.D2.vs_ref\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L1b.gpp\endcsname{0.75}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L1b.hi\endcsname{2.65}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L1b.lo\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L1b.params_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L1b.params_x\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L1b.peak_frac\endcsname{0.97}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L1b.pneg\endcsname{0.60}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L1b.ppm\endcsname{0.0170}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L1b.ppm_ref\endcsname{0.0227}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L1b.ratio\endcsname{0.75}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L1b.step_frac\endcsname{0.92}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L1b.vs_ref\endcsname{\ensuremath{-0.583}}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L2.gpp\endcsname{1.19}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L2.hi\endcsname{1.42}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L2.lo\endcsname{\ensuremath{-0.86}}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L2.params_frac\endcsname{0.24}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L2.params_x\endcsname{4.18}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L2.peak_frac\endcsname{0.94}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L2.pneg\endcsname{0.60}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L2.ppm\endcsname{0.0271}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L2.ppm_ref\endcsname{0.0227}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L2.ratio\endcsname{0.29}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L2.step_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L2.vs_ref\endcsname{\ensuremath{-1.662}}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L3.gpp\endcsname{4.22}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L3.hi\endcsname{4.19}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L3.lo\endcsname{0.41}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L3.params_frac\endcsname{0.29}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L3.params_x\endcsname{3.45}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L3.peak_frac\endcsname{0.98}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L3.pneg\endcsname{0.60}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L3.ppm\endcsname{0.0958}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L3.ppm_ref\endcsname{0.0227}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L3.ratio\endcsname{1.22}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L3.step_frac\endcsname{1.05}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L3.vs_ref\endcsname{\ensuremath{+0.516}}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L4.gpp\endcsname{0.94}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L4.hi\endcsname{3.27}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L4.lo\endcsname{0.14}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L4.params_frac\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L4.params_x\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L4.peak_frac\endcsname{0.98}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L4.pneg\endcsname{0.60}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L4.ppm\endcsname{0.0214}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L4.ppm_ref\endcsname{0.0227}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L4.ratio\endcsname{0.94}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L4.step_frac\endcsname{0.97}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L4.vs_ref\endcsname{\ensuremath{-0.128}}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L6.gpp\endcsname{3.57}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L6.hi\endcsname{3.76}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L6.lo\endcsname{0.29}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L6.params_frac\endcsname{0.30}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L6.params_x\endcsname{3.28}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L6.peak_frac\endcsname{0.96}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L6.pneg\endcsname{0.60}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L6.ppm\endcsname{0.0810}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L6.ppm_ref\endcsname{0.0227}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L6.ratio\endcsname{1.09}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L6.step_frac\endcsname{1.22}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.L6.vs_ref\endcsname{\ensuremath{+0.200}}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.refgain\endcsname{\ensuremath{+2.326}}
\expandafter\gdef\csname R@an.master_table.recovery.kits.s0.status\endcsname{published}
\expandafter\gdef\csname R@an.master_table.recovery.n_ratios\endcsname{22}
\expandafter\gdef\csname R@an.master_table.recovery.n_unbounded\endcsname{6}
\expandafter\gdef\csname R@an.master_table.recovery.n_withheld\endcsname{7}
\expandafter\gdef\csname R@an.master_table.refsens.amos.C1.d_con\endcsname{\ensuremath{+0.379}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.C1.d_unc\endcsname{\ensuremath{+0.361}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.C1.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.C1.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.C1.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.C1.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.C1.margin\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.C1.margin_con\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.C1.margin_sd_frac\endcsname{0.083}
\expandafter\gdef\csname R@an.master_table.refsens.amos.C1.vs_p3c\endcsname{\ensuremath{+0.383}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D1.d_con\endcsname{\ensuremath{+0.267}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D1.d_unc\endcsname{\ensuremath{+0.249}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D1.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D1.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D1.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D1.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D1.margin\endcsname{\ensuremath{-0.101}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D1.margin_con\endcsname{\ensuremath{-0.083}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D1.margin_sd_frac\endcsname{-0.763}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D1.vs_p3c\endcsname{\ensuremath{+0.271}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D2.d_con\endcsname{\ensuremath{-0.373}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D2.d_unc\endcsname{\ensuremath{-0.391}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D2.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D2.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D2.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D2.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D2.margin\endcsname{\ensuremath{-0.741}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D2.margin_con\endcsname{\ensuremath{-0.723}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D2.margin_sd_frac\endcsname{-5.614}
\expandafter\gdef\csname R@an.master_table.refsens.amos.D2.vs_p3c\endcsname{\ensuremath{-0.369}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.I1.d_con\endcsname{\ensuremath{+0.283}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.I1.d_unc\endcsname{\ensuremath{+0.266}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.I1.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.I1.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.I1.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.I1.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.I1.margin\endcsname{\ensuremath{-0.084}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.I1.margin_con\endcsname{\ensuremath{-0.067}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.I1.margin_sd_frac\endcsname{-0.640}
\expandafter\gdef\csname R@an.master_table.refsens.amos.I1.vs_p3c\endcsname{\ensuremath{+0.288}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1.d_con\endcsname{\ensuremath{+0.636}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1.d_unc\endcsname{\ensuremath{+0.618}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1.dfresh_con\endcsname{\ensuremath{+0.454}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1.dfresh_margin\endcsname{\ensuremath{+0.086}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1.dfresh_margin_con\endcsname{\ensuremath{+0.104}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1.dfresh_unc\endcsname{\ensuremath{+0.436}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1.margin\endcsname{\ensuremath{+0.268}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1.margin_con\endcsname{\ensuremath{+0.286}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1.margin_sd_frac\endcsname{2.030}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1.vs_p3c\endcsname{\ensuremath{+0.640}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1b.d_con\endcsname{\ensuremath{+0.127}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1b.d_unc\endcsname{\ensuremath{+0.109}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1b.dfresh_con\endcsname{\ensuremath{+0.287}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1b.dfresh_margin\endcsname{\ensuremath{-0.081}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1b.dfresh_margin_con\endcsname{\ensuremath{-0.063}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1b.dfresh_unc\endcsname{\ensuremath{+0.269}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1b.margin\endcsname{\ensuremath{-0.241}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1b.margin_con\endcsname{\ensuremath{-0.223}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1b.margin_sd_frac\endcsname{-1.824}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L1b.vs_p3c\endcsname{\ensuremath{+0.131}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L2.d_con\endcsname{\ensuremath{+0.351}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L2.d_unc\endcsname{\ensuremath{+0.333}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L2.dfresh_con\endcsname{\ensuremath{+0.184}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L2.dfresh_margin\endcsname{\ensuremath{-0.184}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L2.dfresh_margin_con\endcsname{\ensuremath{-0.166}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L2.dfresh_unc\endcsname{\ensuremath{+0.166}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L2.margin\endcsname{\ensuremath{-0.017}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L2.margin_con\endcsname{\ensuremath{+0.001}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L2.margin_sd_frac\endcsname{-0.127}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L2.vs_p3c\endcsname{\ensuremath{+0.355}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3.d_con\endcsname{\ensuremath{+0.371}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3.d_unc\endcsname{\ensuremath{+0.353}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3.dfresh_con\endcsname{\ensuremath{+0.121}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3.dfresh_margin\endcsname{\ensuremath{-0.246}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3.dfresh_margin_con\endcsname{\ensuremath{-0.229}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3.dfresh_unc\endcsname{\ensuremath{+0.104}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3.margin\endcsname{\ensuremath{+0.003}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3.margin_con\endcsname{\ensuremath{+0.021}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3.margin_sd_frac\endcsname{0.021}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3.vs_p3c\endcsname{\ensuremath{+0.375}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3k3.d_con\endcsname{\ensuremath{+0.448}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3k3.d_unc\endcsname{\ensuremath{+0.430}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3k3.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3k3.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3k3.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3k3.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3k3.margin\endcsname{\ensuremath{+0.080}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3k3.margin_con\endcsname{\ensuremath{+0.098}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3k3.margin_sd_frac\endcsname{0.610}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3k3.vs_p3c\endcsname{\ensuremath{+0.453}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3ng.d_con\endcsname{\ensuremath{+0.257}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3ng.d_unc\endcsname{\ensuremath{+0.239}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3ng.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3ng.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3ng.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3ng.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3ng.margin\endcsname{\ensuremath{-0.111}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3ng.margin_con\endcsname{\ensuremath{-0.093}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3ng.margin_sd_frac\endcsname{-0.842}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3ng.vs_p3c\endcsname{\ensuremath{+0.261}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_L.d_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_L.d_unc\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_L.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_L.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_L.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_L.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_L.margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_L.margin_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_L.margin_sd_frac\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_L.vs_p3c\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_M.d_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_M.d_unc\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_M.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_M.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_M.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_M.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_M.margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_M.margin_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_M.margin_sd_frac\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L3w_M.vs_p3c\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L4.d_con\endcsname{\ensuremath{+0.419}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L4.d_unc\endcsname{\ensuremath{+0.401}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L4.dfresh_con\endcsname{\ensuremath{+0.444}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L4.dfresh_margin\endcsname{\ensuremath{+0.076}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L4.dfresh_margin_con\endcsname{\ensuremath{+0.094}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L4.dfresh_unc\endcsname{\ensuremath{+0.426}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L4.margin\endcsname{\ensuremath{+0.051}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L4.margin_con\endcsname{\ensuremath{+0.069}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L4.margin_sd_frac\endcsname{0.385}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L4.vs_p3c\endcsname{\ensuremath{+0.423}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L6.d_con\endcsname{\ensuremath{+0.005}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L6.d_unc\endcsname{\ensuremath{-0.013}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L6.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L6.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L6.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L6.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L6.margin\endcsname{\ensuremath{-0.363}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L6.margin_con\endcsname{\ensuremath{-0.345}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L6.margin_sd_frac\endcsname{-2.751}
\expandafter\gdef\csname R@an.master_table.refsens.amos.L6.vs_p3c\endcsname{\ensuremath{+0.009}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.N1.d_con\endcsname{\ensuremath{-0.934}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.N1.d_unc\endcsname{\ensuremath{-0.952}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.N1.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.N1.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.N1.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.N1.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.N1.margin\endcsname{\ensuremath{-1.302}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.N1.margin_con\endcsname{\ensuremath{-1.284}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.N1.margin_sd_frac\endcsname{-9.865}
\expandafter\gdef\csname R@an.master_table.refsens.amos.N1.vs_p3c\endcsname{\ensuremath{-0.930}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1_frcap32.d_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1_frcap32.d_unc\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1_frcap32.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1_frcap32.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1_frcap32.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1_frcap32.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1_frcap32.margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1_frcap32.margin_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1_frcap32.margin_sd_frac\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1_frcap32.vs_p3c\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1b.d_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1b.d_unc\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1b.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1b.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1b.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1b.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1b.margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1b.margin_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1b.margin_sd_frac\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1b.vs_p3c\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1c.d_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1c.d_unc\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1c.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1c.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1c.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1c.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1c.margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1c.margin_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1c.margin_sd_frac\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P1c.vs_p3c\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3c.d_con\endcsname{\ensuremath{-0.004}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3c.d_unc\endcsname{\ensuremath{-0.022}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3c.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3c.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3c.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3c.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3c.margin\endcsname{\ensuremath{-0.372}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3c.margin_con\endcsname{\ensuremath{-0.354}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3c.margin_sd_frac\endcsname{-2.819}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3c.vs_p3c\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3lite.d_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3lite.d_unc\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3lite.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3lite.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3lite.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3lite.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3lite.margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3lite.margin_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3lite.margin_sd_frac\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.P3lite.vs_p3c\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.S2.d_con\endcsname{\ensuremath{+0.367}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.S2.d_unc\endcsname{\ensuremath{+0.349}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.S2.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.S2.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.S2.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.S2.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.S2.margin\endcsname{\ensuremath{-0.001}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.S2.margin_con\endcsname{\ensuremath{+0.017}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.S2.margin_sd_frac\endcsname{-0.006}
\expandafter\gdef\csname R@an.master_table.refsens.amos.S2.vs_p3c\endcsname{\ensuremath{+0.371}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP1.d_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP1.d_unc\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP1.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP1.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP1.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP1.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP1.margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP1.margin_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP1.margin_sd_frac\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP1.vs_p3c\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP2.d_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP2.d_unc\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP2.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP2.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP2.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP2.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP2.margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP2.margin_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP2.margin_sd_frac\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.SP2.vs_p3c\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5A5.d_con\endcsname{\ensuremath{+0.030}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5A5.d_unc\endcsname{\ensuremath{+0.012}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5A5.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5A5.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5A5.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5A5.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5A5.margin\endcsname{\ensuremath{-0.338}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5A5.margin_con\endcsname{\ensuremath{-0.320}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5A5.margin_sd_frac\endcsname{-2.562}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5A5.vs_p3c\endcsname{\ensuremath{+0.034}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B1.d_con\endcsname{\ensuremath{-0.272}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B1.d_unc\endcsname{\ensuremath{-0.290}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B1.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B1.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B1.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B1.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B1.margin\endcsname{\ensuremath{-0.640}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B1.margin_con\endcsname{\ensuremath{-0.622}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B1.margin_sd_frac\endcsname{-4.849}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B1.vs_p3c\endcsname{\ensuremath{-0.268}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B2.d_con\endcsname{\ensuremath{+0.121}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B2.d_unc\endcsname{\ensuremath{+0.103}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B2.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B2.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B2.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B2.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B2.margin\endcsname{\ensuremath{-0.247}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B2.margin_con\endcsname{\ensuremath{-0.229}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B2.margin_sd_frac\endcsname{-1.868}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V5B2.vs_p3c\endcsname{\ensuremath{+0.126}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V6A1r.d_con\endcsname{\ensuremath{+0.476}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V6A1r.d_unc\endcsname{\ensuremath{+0.458}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V6A1r.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V6A1r.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V6A1r.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V6A1r.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V6A1r.margin\endcsname{\ensuremath{+0.108}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V6A1r.margin_con\endcsname{\ensuremath{+0.126}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V6A1r.margin_sd_frac\endcsname{0.819}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V6A1r.vs_p3c\endcsname{\ensuremath{+0.480}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A1.d_con\endcsname{\ensuremath{-0.055}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A1.d_unc\endcsname{\ensuremath{-0.073}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A1.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A1.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A1.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A1.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A1.margin\endcsname{\ensuremath{-0.423}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A1.margin_con\endcsname{\ensuremath{-0.405}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A1.margin_sd_frac\endcsname{-3.207}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A1.vs_p3c\endcsname{\ensuremath{-0.051}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A2.d_con\endcsname{\ensuremath{+0.349}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A2.d_unc\endcsname{\ensuremath{+0.331}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A2.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A2.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A2.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A2.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A2.margin\endcsname{\ensuremath{-0.019}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A2.margin_con\endcsname{\ensuremath{-0.001}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A2.margin_sd_frac\endcsname{-0.147}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A2.vs_p3c\endcsname{\ensuremath{+0.353}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A3.d_con\endcsname{\ensuremath{-0.226}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A3.d_unc\endcsname{\ensuremath{-0.244}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A3.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A3.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A3.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A3.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A3.margin\endcsname{\ensuremath{-0.594}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A3.margin_con\endcsname{\ensuremath{-0.576}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A3.margin_sd_frac\endcsname{-4.503}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7A3.vs_p3c\endcsname{\ensuremath{-0.222}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B1.d_con\endcsname{\ensuremath{-0.446}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B1.d_unc\endcsname{\ensuremath{-0.464}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B1.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B1.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B1.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B1.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B1.margin\endcsname{\ensuremath{-0.814}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B1.margin_con\endcsname{\ensuremath{-0.796}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B1.margin_sd_frac\endcsname{-6.169}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B1.vs_p3c\endcsname{\ensuremath{-0.442}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B2.d_con\endcsname{\ensuremath{-0.277}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B2.d_unc\endcsname{\ensuremath{-0.295}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B2.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B2.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B2.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B2.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B2.margin\endcsname{\ensuremath{-0.645}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B2.margin_con\endcsname{\ensuremath{-0.627}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B2.margin_sd_frac\endcsname{-4.889}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7B2.vs_p3c\endcsname{\ensuremath{-0.273}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C1.d_con\endcsname{\ensuremath{-0.117}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C1.d_unc\endcsname{\ensuremath{-0.135}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C1.dfresh_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C1.dfresh_margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C1.dfresh_margin_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C1.dfresh_unc\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C1.margin\endcsname{\ensuremath{-0.485}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C1.margin_con\endcsname{\ensuremath{-0.467}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C1.margin_sd_frac\endcsname{-3.672}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C1.vs_p3c\endcsname{\ensuremath{-0.113}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C2.d_con\endcsname{\ensuremath{-0.372}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C2.d_unc\endcsname{\ensuremath{-0.390}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C2.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C2.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C2.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C2.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C2.margin\endcsname{\ensuremath{-0.740}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C2.margin_con\endcsname{\ensuremath{-0.722}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C2.margin_sd_frac\endcsname{-5.609}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V7C2.vs_p3c\endcsname{\ensuremath{-0.368}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A1.d_con\endcsname{\ensuremath{-0.516}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A1.d_unc\endcsname{\ensuremath{-0.534}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A1.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A1.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A1.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A1.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A1.margin\endcsname{\ensuremath{-0.884}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A1.margin_con\endcsname{\ensuremath{-0.866}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A1.margin_sd_frac\endcsname{-6.694}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A1.vs_p3c\endcsname{\ensuremath{-0.511}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A2.d_con\endcsname{\ensuremath{-0.323}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A2.d_unc\endcsname{\ensuremath{-0.341}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A2.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A2.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A2.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A2.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A2.margin\endcsname{\ensuremath{-0.691}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A2.margin_con\endcsname{\ensuremath{-0.673}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A2.margin_sd_frac\endcsname{-5.235}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8A2.vs_p3c\endcsname{\ensuremath{-0.319}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B1.d_con\endcsname{\ensuremath{-0.761}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B1.d_unc\endcsname{\ensuremath{-0.779}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B1.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B1.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B1.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B1.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B1.margin\endcsname{\ensuremath{-1.129}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B1.margin_con\endcsname{\ensuremath{-1.111}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B1.margin_sd_frac\endcsname{-8.555}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B1.vs_p3c\endcsname{\ensuremath{-0.757}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B2.d_con\endcsname{\ensuremath{-0.298}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B2.d_unc\endcsname{\ensuremath{-0.316}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B2.dfresh_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B2.dfresh_margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B2.dfresh_margin_con\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B2.dfresh_unc\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B2.margin\endcsname{\ensuremath{-0.666}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B2.margin_con\endcsname{\ensuremath{-0.648}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B2.margin_sd_frac\endcsname{-5.047}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8B2.vs_p3c\endcsname{\ensuremath{-0.294}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8X1.d_con\endcsname{\ensuremath{-0.372}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8X1.d_unc\endcsname{\ensuremath{-0.390}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8X1.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8X1.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8X1.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8X1.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8X1.margin\endcsname{\ensuremath{-0.740}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8X1.margin_con\endcsname{\ensuremath{-0.722}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8X1.margin_sd_frac\endcsname{-5.605}
\expandafter\gdef\csname R@an.master_table.refsens.amos.V8X1.vs_p3c\endcsname{\ensuremath{-0.368}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1.d_con\endcsname{\ensuremath{+0.089}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1.d_unc\endcsname{\ensuremath{+0.071}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1.margin\endcsname{\ensuremath{-0.279}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1.margin_con\endcsname{\ensuremath{-0.261}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1.margin_sd_frac\endcsname{-2.116}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1.vs_p3c\endcsname{\ensuremath{+0.093}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1c.d_con\endcsname{\ensuremath{+0.352}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1c.d_unc\endcsname{\ensuremath{+0.334}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1c.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1c.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1c.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1c.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1c.margin\endcsname{\ensuremath{-0.016}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1c.margin_con\endcsname{\ensuremath{+0.002}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1c.margin_sd_frac\endcsname{-0.119}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W1c.vs_p3c\endcsname{\ensuremath{+0.356}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W2.d_con\endcsname{\ensuremath{+0.200}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W2.d_unc\endcsname{\ensuremath{+0.182}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W2.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W2.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W2.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W2.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W2.margin\endcsname{\ensuremath{-0.168}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W2.margin_con\endcsname{\ensuremath{-0.150}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W2.margin_sd_frac\endcsname{-1.270}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W2.vs_p3c\endcsname{\ensuremath{+0.204}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3.d_con\endcsname{\ensuremath{+0.259}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3.d_unc\endcsname{\ensuremath{+0.241}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3.margin\endcsname{\ensuremath{-0.109}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3.margin_con\endcsname{\ensuremath{-0.091}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3.margin_sd_frac\endcsname{-0.827}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3.vs_p3c\endcsname{\ensuremath{+0.263}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3c.d_con\endcsname{\ensuremath{+0.151}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3c.d_unc\endcsname{\ensuremath{+0.133}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3c.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3c.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3c.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3c.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3c.margin\endcsname{\ensuremath{-0.217}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3c.margin_con\endcsname{\ensuremath{-0.199}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3c.margin_sd_frac\endcsname{-1.642}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W3c.vs_p3c\endcsname{\ensuremath{+0.155}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W4.d_con\endcsname{\ensuremath{+0.065}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W4.d_unc\endcsname{\ensuremath{+0.047}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W4.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W4.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W4.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W4.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W4.margin\endcsname{\ensuremath{-0.303}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W4.margin_con\endcsname{\ensuremath{-0.285}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W4.margin_sd_frac\endcsname{-2.294}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W4.vs_p3c\endcsname{\ensuremath{+0.069}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W5.d_con\endcsname{\ensuremath{+0.580}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W5.d_unc\endcsname{\ensuremath{+0.562}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W5.dfresh_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W5.dfresh_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W5.dfresh_margin_con\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W5.dfresh_unc\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W5.margin\endcsname{\ensuremath{+0.212}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W5.margin_con\endcsname{\ensuremath{+0.230}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W5.margin_sd_frac\endcsname{1.610}
\expandafter\gdef\csname R@an.master_table.refsens.amos.W5.vs_p3c\endcsname{\ensuremath{+0.585}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.cluster_se\endcsname{0.066}
\expandafter\gdef\csname R@an.master_table.refsens.amos.contemp.mean\endcsname{87.712}
\expandafter\gdef\csname R@an.master_table.refsens.amos.contemp.n\endcsname{3}
\expandafter\gdef\csname R@an.master_table.refsens.amos.contemp.sd\endcsname{0.125}
\expandafter\gdef\csname R@an.master_table.refsens.amos.contemp.shift\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.flip_phrase\endcsname{changes the \ensuremath{+0.35} screen status of 4 of the 38 AMOS22 arms it can be applied to}
\expandafter\gdef\csname R@an.master_table.refsens.amos.flip_phrase_con\endcsname{changes the \ensuremath{+0.35} screen status of 1 of the 38 AMOS22 arms it can be applied to}
\expandafter\gdef\csname R@an.master_table.refsens.amos.n_arms\endcsname{38}
\expandafter\gdef\csname R@an.master_table.refsens.amos.n_ref\endcsname{38}
\expandafter\gdef\csname R@an.master_table.refsens.amos.n_sensitive\endcsname{4}
\expandafter\gdef\csname R@an.master_table.refsens.amos.n_sensitive_con\endcsname{1}
\expandafter\gdef\csname R@an.master_table.refsens.amos.p3c\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.unc_mean\endcsname{87.730}
\expandafter\gdef\csname R@an.master_table.refsens.amos.unc_shift\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.master_table.refsens.amos.unc_shift_sd_frac\endcsname{0.22}
\expandafter\gdef\csname R@an.master_table.refsens.kits.C1.d6\endcsname{\ensuremath{+3.264}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.C1.dfresh6\endcsname{\ensuremath{+2.157}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.C1.dfresh6_margin\endcsname{\ensuremath{+1.807}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.C1.margin\endcsname{\ensuremath{+2.914}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.C1.margin_sd_frac\endcsname{3.174}
\expandafter\gdef\csname R@an.master_table.refsens.kits.D1.d6\endcsname{\ensuremath{+1.363}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.D1.dfresh6\endcsname{\ensuremath{+1.233}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.D1.dfresh6_margin\endcsname{\ensuremath{+0.883}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.D1.margin\endcsname{\ensuremath{+1.013}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.D1.margin_sd_frac\endcsname{1.104}
\expandafter\gdef\csname R@an.master_table.refsens.kits.D2.d6\endcsname{\ensuremath{+2.112}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.D2.dfresh6\endcsname{\ensuremath{+1.648}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.D2.dfresh6_margin\endcsname{\ensuremath{+1.298}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.D2.margin\endcsname{\ensuremath{+1.762}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.D2.margin_sd_frac\endcsname{1.919}
\expandafter\gdef\csname R@an.master_table.refsens.kits.I1.d6\endcsname{\ensuremath{+1.649}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.I1.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.I1.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.I1.margin\endcsname{\ensuremath{+1.299}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.I1.margin_sd_frac\endcsname{1.416}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L1.d6\endcsname{\ensuremath{+2.082}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L1.dfresh6\endcsname{\ensuremath{+3.232}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L1.dfresh6_margin\endcsname{\ensuremath{+2.882}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L1.margin\endcsname{\ensuremath{+1.732}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L1.margin_sd_frac\endcsname{1.887}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L1b.d6\endcsname{\ensuremath{+1.499}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L1b.dfresh6\endcsname{\ensuremath{+2.070}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L1b.dfresh6_margin\endcsname{\ensuremath{+1.720}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L1b.margin\endcsname{\ensuremath{+1.149}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L1b.margin_sd_frac\endcsname{1.252}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L2.d6\endcsname{\ensuremath{+0.420}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L2.dfresh6\endcsname{\ensuremath{-0.133}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L2.dfresh6_margin\endcsname{\ensuremath{-0.483}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L2.margin\endcsname{\ensuremath{+0.070}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L2.margin_sd_frac\endcsname{0.076}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3.d6\endcsname{\ensuremath{+2.598}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3.dfresh6\endcsname{\ensuremath{+1.850}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3.dfresh6_margin\endcsname{\ensuremath{+1.500}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3.margin\endcsname{\ensuremath{+2.248}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3.margin_sd_frac\endcsname{2.449}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3k3.d6\endcsname{\ensuremath{+1.123}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3k3.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3k3.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3k3.margin\endcsname{\ensuremath{+0.773}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3k3.margin_sd_frac\endcsname{0.842}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3ng.d6\endcsname{\ensuremath{+2.317}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3ng.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3ng.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3ng.margin\endcsname{\ensuremath{+1.967}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3ng.margin_sd_frac\endcsname{2.144}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3w_L.d6\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3w_L.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3w_L.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3w_L.margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3w_L.margin_sd_frac\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3w_M.d6\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3w_M.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3w_M.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3w_M.margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L3w_M.margin_sd_frac\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L4.d6\endcsname{\ensuremath{+1.954}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L4.dfresh6\endcsname{\ensuremath{+2.003}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L4.dfresh6_margin\endcsname{\ensuremath{+1.653}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L4.margin\endcsname{\ensuremath{+1.604}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L4.margin_sd_frac\endcsname{1.748}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L6.d6\endcsname{\ensuremath{+2.283}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L6.dfresh6\endcsname{\ensuremath{+1.348}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L6.dfresh6_margin\endcsname{\ensuremath{+0.998}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L6.margin\endcsname{\ensuremath{+1.933}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.L6.margin_sd_frac\endcsname{2.106}
\expandafter\gdef\csname R@an.master_table.refsens.kits.N1.d6\endcsname{\ensuremath{-6.736}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.N1.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.N1.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.N1.margin\endcsname{\ensuremath{-7.086}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.N1.margin_sd_frac\endcsname{-7.720}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P1_frcap32.d6\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P1_frcap32.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P1_frcap32.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P1_frcap32.margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P1_frcap32.margin_sd_frac\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P1b.d6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P1b.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P1b.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P1b.margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P1b.margin_sd_frac\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P1c.d6\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P1c.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P1c.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P1c.margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P1c.margin_sd_frac\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P3c.d6\endcsname{\ensuremath{+1.121}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P3c.dfresh6\endcsname{\ensuremath{+0.932}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P3c.dfresh6_margin\endcsname{\ensuremath{+0.582}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P3c.margin\endcsname{\ensuremath{+0.771}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P3c.margin_sd_frac\endcsname{0.840}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P3lite.d6\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P3lite.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P3lite.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P3lite.margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.P3lite.margin_sd_frac\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.S2.d6\endcsname{\ensuremath{+1.098}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.S2.dfresh6\endcsname{\ensuremath{+0.326}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.S2.dfresh6_margin\endcsname{\ensuremath{-0.024}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.S2.margin\endcsname{\ensuremath{+0.748}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.S2.margin_sd_frac\endcsname{0.815}
\expandafter\gdef\csname R@an.master_table.refsens.kits.SP1.d6\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.SP1.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.SP1.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.SP1.margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.SP1.margin_sd_frac\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.SP2.d6\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.SP2.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.SP2.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.SP2.margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.SP2.margin_sd_frac\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V5A5.d6\endcsname{\ensuremath{+1.706}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V5A5.dfresh6\endcsname{\ensuremath{+1.922}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V5A5.dfresh6_margin\endcsname{\ensuremath{+1.572}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V5A5.margin\endcsname{\ensuremath{+1.356}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V5A5.margin_sd_frac\endcsname{1.477}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V5B1.d6\endcsname{\ensuremath{+1.919}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V5B1.dfresh6\endcsname{\ensuremath{+2.042}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V5B1.dfresh6_margin\endcsname{\ensuremath{+1.692}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V5B1.margin\endcsname{\ensuremath{+1.569}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V5B1.margin_sd_frac\endcsname{1.709}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V5B2.d6\endcsname{\ensuremath{+1.021}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V5B2.dfresh6\endcsname{\ensuremath{+1.205}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V5B2.dfresh6_margin\endcsname{\ensuremath{+0.855}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V5B2.margin\endcsname{\ensuremath{+0.671}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V5B2.margin_sd_frac\endcsname{0.731}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V6A1r.d6\endcsname{\ensuremath{+1.992}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V6A1r.dfresh6\endcsname{\ensuremath{+1.461}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V6A1r.dfresh6_margin\endcsname{\ensuremath{+1.111}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V6A1r.margin\endcsname{\ensuremath{+1.642}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V6A1r.margin_sd_frac\endcsname{1.789}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7A1.d6\endcsname{\ensuremath{+2.305}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7A1.dfresh6\endcsname{\ensuremath{+2.418}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7A1.dfresh6_margin\endcsname{\ensuremath{+2.068}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7A1.margin\endcsname{\ensuremath{+1.955}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7A1.margin_sd_frac\endcsname{2.130}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7A2.d6\endcsname{\ensuremath{+2.642}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7A2.dfresh6\endcsname{\ensuremath{+2.046}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7A2.dfresh6_margin\endcsname{\ensuremath{+1.696}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7A2.margin\endcsname{\ensuremath{+2.292}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7A2.margin_sd_frac\endcsname{2.498}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7A3.d6\endcsname{\ensuremath{+0.298}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7A3.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7A3.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7A3.margin\endcsname{\ensuremath{-0.052}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7A3.margin_sd_frac\endcsname{-0.057}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7B1.d6\endcsname{\ensuremath{+1.478}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7B1.dfresh6\endcsname{\ensuremath{+2.138}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7B1.dfresh6_margin\endcsname{\ensuremath{+1.788}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7B1.margin\endcsname{\ensuremath{+1.128}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7B1.margin_sd_frac\endcsname{1.229}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7B2.d6\endcsname{\ensuremath{+2.581}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7B2.dfresh6\endcsname{\ensuremath{+1.595}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7B2.dfresh6_margin\endcsname{\ensuremath{+1.245}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7B2.margin\endcsname{\ensuremath{+2.231}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7B2.margin_sd_frac\endcsname{2.431}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7C1.d6\endcsname{\ensuremath{+2.463}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7C1.dfresh6\endcsname{\ensuremath{+2.196}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7C1.dfresh6_margin\endcsname{\ensuremath{+1.846}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7C1.margin\endcsname{\ensuremath{+2.113}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7C1.margin_sd_frac\endcsname{2.302}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7C2.d6\endcsname{\ensuremath{+1.757}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7C2.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7C2.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7C2.margin\endcsname{\ensuremath{+1.407}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V7C2.margin_sd_frac\endcsname{1.533}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8A1.d6\endcsname{\ensuremath{+1.516}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8A1.dfresh6\endcsname{\ensuremath{+1.005}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8A1.dfresh6_margin\endcsname{\ensuremath{+0.655}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8A1.margin\endcsname{\ensuremath{+1.166}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8A1.margin_sd_frac\endcsname{1.271}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8A2.d6\endcsname{\ensuremath{+1.110}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8A2.dfresh6\endcsname{\ensuremath{+1.634}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8A2.dfresh6_margin\endcsname{\ensuremath{+1.284}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8A2.margin\endcsname{\ensuremath{+0.760}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8A2.margin_sd_frac\endcsname{0.828}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8B1.d6\endcsname{\ensuremath{+2.667}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8B1.dfresh6\endcsname{\ensuremath{+1.131}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8B1.dfresh6_margin\endcsname{\ensuremath{+0.781}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8B1.margin\endcsname{\ensuremath{+2.317}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8B1.margin_sd_frac\endcsname{2.525}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8B2.d6\endcsname{\ensuremath{+1.402}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8B2.dfresh6\endcsname{\ensuremath{+1.487}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8B2.dfresh6_margin\endcsname{\ensuremath{+1.137}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8B2.margin\endcsname{\ensuremath{+1.052}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8B2.margin_sd_frac\endcsname{1.146}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8X1.d6\endcsname{\ensuremath{+2.291}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8X1.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8X1.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8X1.margin\endcsname{\ensuremath{+1.941}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.V8X1.margin_sd_frac\endcsname{2.115}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W1.d6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W1.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W1.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W1.margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W1.margin_sd_frac\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W1c.d6\endcsname{\ensuremath{+2.392}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W1c.dfresh6\endcsname{\ensuremath{+0.823}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W1c.dfresh6_margin\endcsname{\ensuremath{+0.473}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W1c.margin\endcsname{\ensuremath{+2.042}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W1c.margin_sd_frac\endcsname{2.225}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W2.d6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W2.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W2.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W2.margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W2.margin_sd_frac\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W3.d6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W3.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W3.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W3.margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W3.margin_sd_frac\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W3c.d6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W3c.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W3c.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W3c.margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W3c.margin_sd_frac\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W4.d6\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W4.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W4.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W4.margin\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W4.margin_sd_frac\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W5.d6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W5.dfresh6\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W5.dfresh6_margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W5.margin\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.W5.margin_sd_frac\endcsname{--}
\expandafter\gdef\csname R@an.master_table.refsens.kits.flip_phrase\endcsname{changes the \ensuremath{+0.35} screen status of 1 of the 32 KiTS23 arms it can be applied to}
\expandafter\gdef\csname R@an.master_table.refsens.kits.mean6\endcsname{83.622}
\expandafter\gdef\csname R@an.master_table.refsens.kits.n_arms\endcsname{32}
\expandafter\gdef\csname R@an.master_table.refsens.kits.n_ref\endcsname{32}
\expandafter\gdef\csname R@an.master_table.refsens.kits.n_sensitive\endcsname{1}
\expandafter\gdef\csname R@an.master_table.refsens.kits.p3c\endcsname{\ensuremath{+1.364}}
\expandafter\gdef\csname R@an.master_table.refsens.kits.sd6\endcsname{0.722}
\expandafter\gdef\csname R@an.master_table.refsens.kits.sd6_hi\endcsname{1.771}
\expandafter\gdef\csname R@an.master_table.refsens.kits.sd6_lo\endcsname{0.451}
\expandafter\gdef\csname R@an.master_table.refsens.kits.shift6\endcsname{\ensuremath{+0.244}}
\expandafter\gdef\csname R@an.master_table.screen.bar\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.master_table.screen.guard\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.master_table.screen.nonempty\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.master_table.screen.pair_floor\endcsname{0.50}
\expandafter\gdef\csname R@an.master_table.search.RS01.amos.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.search.RS01.amos.status\endcsname{not scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS01.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS01.kits.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS02.amos.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.search.RS02.amos.status\endcsname{not scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS02.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS02.kits.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS05.amos.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.search.RS05.amos.status\endcsname{not scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS05.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS05.kits.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS07.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS07.amos.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS07.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS07.kits.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS08.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS08.amos.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS08.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS08.kits.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS09.amos.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.search.RS09.amos.status\endcsname{not scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS09.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS09.kits.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS11.amos.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.search.RS11.amos.status\endcsname{not scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS11.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS11.kits.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS12.amos.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.search.RS12.amos.status\endcsname{not scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS12.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS12.kits.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS13.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS13.amos.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS13.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS13.kits.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS15.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS15.amos.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS15.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS15.kits.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS19.amos.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.search.RS19.amos.status\endcsname{not scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS19.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS19.kits.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS20.amos.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.search.RS20.amos.status\endcsname{not scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS20.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS20.kits.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS22.amos.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.search.RS22.amos.status\endcsname{not scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS22.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS22.kits.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS23.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS23.amos.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS23.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS23.kits.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS24.amos.d0\endcsname{--}
\expandafter\gdef\csname R@an.master_table.search.RS24.amos.status\endcsname{not scheduled}
\expandafter\gdef\csname R@an.master_table.search.RS24.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.master_table.search.RS24.kits.status\endcsname{scheduled}
\expandafter\gdef\csname R@an.master_table.search.amos.n_done\endcsname{0}
\expandafter\gdef\csname R@an.master_table.search.amos.n_runs\endcsname{5}
\expandafter\gdef\csname R@an.master_table.search.kits.n_done\endcsname{0}
\expandafter\gdef\csname R@an.master_table.search.kits.n_runs\endcsname{15}
\expandafter\gdef\csname R@an.master_table.search.n_designs\endcsname{15}
\expandafter\gdef\csname R@an.master_table.search.n_done\endcsname{0}
\expandafter\gdef\csname R@an.master_table.search.n_pending\endcsname{20}
\expandafter\gdef\csname R@an.master_table.search.n_runs\endcsname{20}
\expandafter\gdef\csname R@an.master_table.search.phrase\endcsname{0 of the 20 registered random-search runs (15 designs: 5 on AMOS22, 15 on KiTS23) have finished}
\expandafter\gdef\csname R@an.master_table.sep.amos.n_nosep\endcsname{3}
\expandafter\gdef\csname R@an.master_table.sep.amos.n_pairs\endcsname{5}
\expandafter\gdef\csname R@an.master_table.sep.amos.n_sep\endcsname{2}
\expandafter\gdef\csname R@an.master_table.sep.amos.nosep_hi\endcsname{\ensuremath{+0.298}}
\expandafter\gdef\csname R@an.master_table.sep.amos.nosep_list\endcsname{HyReX, ResEnc-matched (re-implemented) and ConvNeXt-k3}
\expandafter\gdef\csname R@an.master_table.sep.amos.nosep_lo\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.master_table.sep.amos.phrase\endcsname{AMOS22 separates \ensuremath{+0.455} to \ensuremath{+0.465} pp (ResEnc-M, ResEnc+context) and does not separate \ensuremath{+0.132} to \ensuremath{+0.298} pp (ResEnc-matched, ConvNeXt-k3, HyReX) at two fresh seeds}
\expandafter\gdef\csname R@an.master_table.sep.amos.sep_hi\endcsname{\ensuremath{+0.465}}
\expandafter\gdef\csname R@an.master_table.sep.amos.sep_list\endcsname{ResEnc-M (library preset) and ResEnc+context}
\expandafter\gdef\csname R@an.master_table.sep.amos.sep_lo\endcsname{\ensuremath{+0.455}}
\expandafter\gdef\csname R@an.master_table.sep.kits.n_nosep\endcsname{1}
\expandafter\gdef\csname R@an.master_table.sep.kits.n_pairs\endcsname{25}
\expandafter\gdef\csname R@an.master_table.sep.kits.n_sep\endcsname{24}
\expandafter\gdef\csname R@an.master_table.sep.kits.nosep_hi\endcsname{\ensuremath{+0.110}}
\expandafter\gdef\csname R@an.master_table.sep.kits.nosep_list\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.master_table.sep.kits.nosep_lo\endcsname{\ensuremath{+0.110}}
\expandafter\gdef\csname R@an.master_table.sep.kits.phrase\endcsname{KiTS23 separates \ensuremath{+0.570} to \ensuremath{+3.475} pp (ResEnc-M, LeanDeepMid, LeanNeXt-s5, HyReX+dec. capacity, LeanSep, ResEnc-matched, LeanDeepMid+FD, LeanAdd, ResEnc+context, HyReX-LeanDec, HyReX, LeanDec, StackDec, LeanDil, Stem1, HyReX-k9, HyReX+context, HyReX point-fuse, LeanAdd-NeXt, LeanTrunk, CoarseStack, fn.-identical control, branch control, HyReX, finer ConvNeXt) and does not separate \ensuremath{+0.110} pp (ConvNeXt-k3) at two fresh seeds}
\expandafter\gdef\csname R@an.master_table.sep.kits.sep_hi\endcsname{\ensuremath{+3.475}}
\expandafter\gdef\csname R@an.master_table.sep.kits.sep_list\endcsname{HyReX, ResEnc-M (library preset), ResEnc-matched (re-implemented), ResEnc+context, HyReX+context, branch control, HyReX, ConvNeXt one stage finer, HyReX point-fuse decoder, HyReX + decoder capacity, LeanDec (default with one conv per decoder stage), function-identical control, LeanDec with additive skips, LeanAdd with coarse large kernels, HyReX with LeanDec fine decoder, LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4, LeanNeXt-s5 with one convolution at encoder stage 0, LeanNeXt-s5 with eighteen coarse blocks, LeanNeXt-s5 with twelve coarse blocks and the coarse decoder convolutions, LeanDeepMid with the finest decoder convolutions, LeanAdd-NeXt with separable coarse kernels, LeanAdd-NeXt with dilated coarse kernels, LeanAdd-NeXt with a deeper middle encoder, LeanAdd-NeXt with the coarse operator at stage 5 only and HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.master_table.sep.kits.sep_lo\endcsname{\ensuremath{+0.570}}
\expandafter\gdef\csname R@an.master_table.stepbelow.acdc.list\endcsname{LeanDec, LeanAdd, LeanAdd-NeXt, LeanTrunk, Stem1, CoarseStack, StackDec, NarrowTrunk, LeanSep, LeanDil, LeanNeXt-k3 and LeanNeXt-s5}
\expandafter\gdef\csname R@an.master_table.stepbelow.acdc.max\endcsname{3.84}
\expandafter\gdef\csname R@an.master_table.stepbelow.acdc.max_arm\endcsname{MedNeXt-like}
\expandafter\gdef\csname R@an.master_table.stepbelow.acdc.n\endcsname{12}
\expandafter\gdef\csname R@an.master_table.stepbelow.acdc.n_rows\endcsname{46}
\expandafter\gdef\csname R@an.master_table.stepbelow.acdc.next\endcsname{1.02}
\expandafter\gdef\csname R@an.master_table.stepbelow.acdc.next_arm\endcsname{coarse-capacity ctl}
\expandafter\gdef\csname R@an.master_table.stepbelow.amos.list\endcsname{LeanDec, LeanAdd, LeanAdd-NeXt, LeanTrunk, Stem1, CoarseStack, StackDec, NarrowTrunk, LeanSep, LeanDil, LeanNeXt-k3, LeanDeepMid and LeanNeXt-s5}
\expandafter\gdef\csname R@an.master_table.stepbelow.amos.max\endcsname{3.51}
\expandafter\gdef\csname R@an.master_table.stepbelow.amos.max_arm\endcsname{MedNeXt-like}
\expandafter\gdef\csname R@an.master_table.stepbelow.amos.n\endcsname{13}
\expandafter\gdef\csname R@an.master_table.stepbelow.amos.n_rows\endcsname{46}
\expandafter\gdef\csname R@an.master_table.stepbelow.amos.next\endcsname{1.02}
\expandafter\gdef\csname R@an.master_table.stepbelow.amos.next_arm\endcsname{coarse-capacity ctl}
\expandafter\gdef\csname R@an.master_table.stepbelow.kits.list\endcsname{LeanDec, LeanAdd, LeanAdd-NeXt, LeanTrunk, Stem1, CoarseStack, StackDec, NarrowTrunk, LeanSep, LeanDil, LeanNeXt-k3, LeanDeepMid and LeanNeXt-s5}
\expandafter\gdef\csname R@an.master_table.stepbelow.kits.max\endcsname{2.65}
\expandafter\gdef\csname R@an.master_table.stepbelow.kits.max_arm\endcsname{full-res addition}
\expandafter\gdef\csname R@an.master_table.stepbelow.kits.n\endcsname{13}
\expandafter\gdef\csname R@an.master_table.stepbelow.kits.n_rows\endcsname{46}
\expandafter\gdef\csname R@an.master_table.stepbelow.kits.next\endcsname{1.01}
\expandafter\gdef\csname R@an.master_table.stepbelow.kits.next_arm\endcsname{coarse-capacity ctl}
\expandafter\gdef\csname R@an.master_table.stepbelow.n\endcsname{12}
\expandafter\gdef\csname R@an.master_table.stepbelow.n.word\endcsname{12}
\expandafter\gdef\csname R@an.master_table.stepbelow.n_other\endcsname{34}
\expandafter\gdef\csname R@an.master_table.stepbelow.names\endcsname{LeanDec, LeanAdd, LeanAdd-NeXt, LeanTrunk, Stem1, CoarseStack, StackDec, NarrowTrunk, LeanSep, LeanDil, LeanNeXt-k3 and LeanNeXt-s5}
\expandafter\gdef\csname R@an.master_table.stepbelow.other_max\endcsname{3.51}
\expandafter\gdef\csname R@an.master_table.stepbelow.other_min\endcsname{1.00}
\expandafter\gdef\csname R@an.master_table.stepbelow.partial\endcsname{LeanDeepMid}
\expandafter\gdef\csname R@an.master_table.stepbelow.phrase\endcsname{12 of the 46 non-default rows of the master table have a profiled training step below the default's on each of the AMOS22, KiTS23 and ACDC plans: LeanDec (0.81\ensuremath{\times}), LeanAdd (0.72 to 0.74\ensuremath{\times}), LeanAdd-NeXt (0.84 to 0.92\ensuremath{\times}), LeanTrunk (0.59 to 0.62\ensuremath{\times}), Stem1 (0.63 to 0.68\ensuremath{\times}), CoarseStack (0.90 to 1.00\ensuremath{\times}), StackDec (0.85 to 0.92\ensuremath{\times}), NarrowTrunk (0.77 to 0.78\ensuremath{\times}), LeanSep (0.77 to 0.79\ensuremath{\times}), LeanDil (0.76 to 0.78\ensuremath{\times}), LeanNeXt-k3 (0.76 to 0.77\ensuremath{\times}) and LeanNeXt-s5 (0.77 to 0.79\ensuremath{\times}); LeanDeepMid is below it on some of those plans and not on others (AMOS22: LeanDec, LeanAdd, LeanAdd-NeXt, LeanTrunk, Stem1, CoarseStack, StackDec, NarrowTrunk, LeanSep, LeanDil, LeanNeXt-k3, LeanDeepMid and LeanNeXt-s5; KiTS23: LeanDec, LeanAdd, LeanAdd-NeXt, LeanTrunk, Stem1, CoarseStack, StackDec, NarrowTrunk, LeanSep, LeanDil, LeanNeXt-k3, LeanDeepMid and LeanNeXt-s5; ACDC: LeanDec, LeanAdd, LeanAdd-NeXt, LeanTrunk, Stem1, CoarseStack, StackDec, NarrowTrunk, LeanSep, LeanDil, LeanNeXt-k3 and LeanNeXt-s5); the other 34 rows run 1.00\ensuremath{\times} to 3.51\ensuremath{\times} the default's step on the AMOS22 plan}
\expandafter\gdef\csname R@an.master_table.withheld.acdc_leader.sentence\endcsname{WITHHELD CLAIM acdc\_leader}
\expandafter\gdef\csname R@an.master_table.withheld.acdc_leader.status\endcsname{not true}
\expandafter\gdef\csname R@an.master_table.withheld.n\endcsname{2}
\expandafter\gdef\csname R@an.master_table.withheld.resencm_parity.sentence\endcsname{WITHHELD CLAIM resencm\_parity}
\expandafter\gdef\csname R@an.master_table.withheld.resencm_parity.status\endcsname{not true}
\expandafter\gdef\csname R@an.matched.acdc.cost.rel\endcsname{0.91}
\expandafter\gdef\csname R@an.matched.acdc.e1500.mean\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.e1500.n\endcsname{0}
\expandafter\gdef\csname R@an.matched.acdc.e1500.nfail\endcsname{0}
\expandafter\gdef\csname R@an.matched.acdc.e1500.nreg\endcsname{3}
\expandafter\gdef\csname R@an.matched.acdc.e1500.nviol\endcsname{0}
\expandafter\gdef\csname R@an.matched.acdc.e1500.s0\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.e1500.s1\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.e1500.s2\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.e1500.sd\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.e1500.state\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.label\endcsname{ACDC}
\expandafter\gdef\csname R@an.matched.acdc.pool.mean\endcsname{92.009}
\expandafter\gdef\csname R@an.matched.acdc.pool.n\endcsname{6}
\expandafter\gdef\csname R@an.matched.acdc.pool.sd\endcsname{0.099}
\expandafter\gdef\csname R@an.matched.acdc.r1.alt.label\endcsname{the uncompiled sub-pool of the frozen pool (three runs, CORRECTIONS C30)}
\expandafter\gdef\csname R@an.matched.acdc.r1.alt.n\endcsname{3}
\expandafter\gdef\csname R@an.matched.acdc.r1.alt.nreg\endcsname{3}
\expandafter\gdef\csname R@an.matched.acdc.r1.alt.se\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.r1.alt.state\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.r1.alt.value\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.r1.n\endcsname{0}
\expandafter\gdef\csname R@an.matched.acdc.r1.se\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.r1.state\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.r1.value\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.r1.word\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.r2.d1\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.r2.d2\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.r2.default.mean\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.r2.hyrex.mean\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.r2.n\endcsname{0}
\expandafter\gdef\csname R@an.matched.acdc.r2.npos\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.r2.nreg\endcsname{2}
\expandafter\gdef\csname R@an.matched.acdc.r2.signs\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.r2.state\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.r2.value\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.r2.word\endcsname{pending}
\expandafter\gdef\csname R@an.matched.acdc.step.ratio\endcsname{1.64}
\expandafter\gdef\csname R@an.matched.amos.cost.rel\endcsname{0.98}
\expandafter\gdef\csname R@an.matched.amos.e1500.mean\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.e1500.n\endcsname{0}
\expandafter\gdef\csname R@an.matched.amos.e1500.nfail\endcsname{0}
\expandafter\gdef\csname R@an.matched.amos.e1500.nreg\endcsname{3}
\expandafter\gdef\csname R@an.matched.amos.e1500.nviol\endcsname{0}
\expandafter\gdef\csname R@an.matched.amos.e1500.s0\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.e1500.s1\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.e1500.s2\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.e1500.sd\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.e1500.state\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.label\endcsname{AMOS22}
\expandafter\gdef\csname R@an.matched.amos.pool.mean\endcsname{87.701}
\expandafter\gdef\csname R@an.matched.amos.pool.n\endcsname{6}
\expandafter\gdef\csname R@an.matched.amos.pool.sd\endcsname{0.122}
\expandafter\gdef\csname R@an.matched.amos.r1.alt.label\endcsname{the three contemporaneous default runs of Addendum Q1d}
\expandafter\gdef\csname R@an.matched.amos.r1.alt.n\endcsname{3}
\expandafter\gdef\csname R@an.matched.amos.r1.alt.nreg\endcsname{3}
\expandafter\gdef\csname R@an.matched.amos.r1.alt.se\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.r1.alt.state\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.r1.alt.value\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.r1.n\endcsname{0}
\expandafter\gdef\csname R@an.matched.amos.r1.se\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.r1.state\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.r1.value\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.r1.word\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.r2.d1\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.r2.d2\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.r2.default.mean\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.r2.hyrex.mean\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.r2.n\endcsname{0}
\expandafter\gdef\csname R@an.matched.amos.r2.npos\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.r2.nreg\endcsname{2}
\expandafter\gdef\csname R@an.matched.amos.r2.signs\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.r2.state\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.r2.value\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.r2.word\endcsname{pending}
\expandafter\gdef\csname R@an.matched.amos.step.ratio\endcsname{1.53}
\expandafter\gdef\csname R@an.matched.epochs.base\endcsname{1000}
\expandafter\gdef\csname R@an.matched.epochs.n\endcsname{1500}
\expandafter\gdef\csname R@an.matched.epochs.ratio\endcsname{1.5}
\expandafter\gdef\csname R@an.matched.excluded.n\endcsname{0}
\expandafter\gdef\csname R@an.matched.failed.n\endcsname{0}
\expandafter\gdef\csname R@an.matched.floor\endcsname{0.50}
\expandafter\gdef\csname R@an.matched.kits.cost.rel\endcsname{1.07}
\expandafter\gdef\csname R@an.matched.kits.e1500.mean\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.e1500.n\endcsname{0}
\expandafter\gdef\csname R@an.matched.kits.e1500.nfail\endcsname{0}
\expandafter\gdef\csname R@an.matched.kits.e1500.nreg\endcsname{3}
\expandafter\gdef\csname R@an.matched.kits.e1500.nviol\endcsname{0}
\expandafter\gdef\csname R@an.matched.kits.e1500.s0\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.e1500.s1\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.e1500.s2\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.e1500.sd\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.e1500.state\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.label\endcsname{KiTS23}
\expandafter\gdef\csname R@an.matched.kits.pool.mean\endcsname{83.378}
\expandafter\gdef\csname R@an.matched.kits.pool.n\endcsname{3}
\expandafter\gdef\csname R@an.matched.kits.pool.sd\endcsname{0.795}
\expandafter\gdef\csname R@an.matched.kits.r1.alt.label\endcsname{all twelve default runs of this study's conditions}
\expandafter\gdef\csname R@an.matched.kits.r1.alt.n\endcsname{12}
\expandafter\gdef\csname R@an.matched.kits.r1.alt.nreg\endcsname{12}
\expandafter\gdef\csname R@an.matched.kits.r1.alt.se\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.r1.alt.state\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.r1.alt.value\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.r1.n\endcsname{0}
\expandafter\gdef\csname R@an.matched.kits.r1.se\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.r1.state\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.r1.value\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.r1.vs12\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.r1.vs12.n\endcsname{12}
\expandafter\gdef\csname R@an.matched.kits.r1.vs12.nreg\endcsname{12}
\expandafter\gdef\csname R@an.matched.kits.r1.vs12.se\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.r1.vs12.state\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.r1.word\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.r2.d1\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.r2.d2\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.r2.default.mean\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.r2.hyrex.mean\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.r2.n\endcsname{0}
\expandafter\gdef\csname R@an.matched.kits.r2.npos\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.r2.nreg\endcsname{2}
\expandafter\gdef\csname R@an.matched.kits.r2.signs\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.r2.state\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.r2.value\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.r2.word\endcsname{pending}
\expandafter\gdef\csname R@an.matched.kits.step.ratio\endcsname{1.40}
\expandafter\gdef\csname R@an.matched.landed.n\endcsname{0}
\expandafter\gdef\csname R@an.matched.landed.word\endcsname{none}
\expandafter\gdef\csname R@an.matched.match.note\endcsname{The match is approximate: 1500 epochs is the harness maximum and 1.5 times the schedule of the 1000-epoch default, whereas HyReX's profiled step is 1.53 (AMOS22), 1.40 (KiTS23) and 1.64 (ACDC) times the default's; in profiled training steps the default trained for 1500 epochs therefore costs 0.98 (AMOS22), 1.07 (KiTS23) and 0.91 (ACDC) times what HyReX costs.}
\expandafter\gdef\csname R@an.matched.nds\endcsname{3}
\expandafter\gdef\csname R@an.matched.nds.word\endcsname{three}
\expandafter\gdef\csname R@an.matched.nruns\endcsname{9}
\expandafter\gdef\csname R@an.matched.nruns.word\endcsname{nine}
\expandafter\gdef\csname R@an.matched.nseeds\endcsname{3}
\expandafter\gdef\csname R@an.matched.nseeds.word\endcsname{three}
\expandafter\gdef\csname R@an.matched.r1.complete.n\endcsname{0}
\expandafter\gdef\csname R@an.matched.r2.complete.n\endcsname{0}
\expandafter\gdef\csname R@an.matched.sentence.r1.acdc\endcsname{The compute-matched default is pending on ACDC: 0 of 3 registered runs of the default trained for 1500 epochs have landed, and the registered reading, their mean against the frozen 1000-epoch pool, is formed once all of them have.}
\expandafter\gdef\csname R@an.matched.sentence.r1.amos\endcsname{The compute-matched default is pending on AMOS22: 0 of 3 registered runs of the default trained for 1500 epochs have landed, and the registered reading, their mean against the frozen 1000-epoch pool, is formed once all of them have.}
\expandafter\gdef\csname R@an.matched.sentence.r1.kits\endcsname{The compute-matched default is pending on KiTS23: 0 of 3 registered runs of the default trained for 1500 epochs have landed, and the registered reading, their mean against the frozen 1000-epoch pool, is formed once all of them have.}
\expandafter\gdef\csname R@an.matched.sentence.r2.acdc\endcsname{HyReX's compute-matched margin is pending on ACDC: 0 of 2 registered paired seeds have landed in each arm, and the margin is formed once all of them have.}
\expandafter\gdef\csname R@an.matched.sentence.r2.amos\endcsname{HyReX's compute-matched margin is pending on AMOS22: 0 of 2 registered paired seeds have landed in each arm, and the margin is formed once all of them have.}
\expandafter\gdef\csname R@an.matched.sentence.r2.kits\endcsname{HyReX's compute-matched margin is pending on KiTS23: 0 of 2 registered paired seeds have landed in each arm, and the margin is formed once all of them have.}
\expandafter\gdef\csname R@an.matched.summary\endcsname{The compute-matched default of Addendum AH1 (the default trained for 1500 epochs, three seeds on each of three datasets) is pending: 0 of 9 registered runs have landed, and each reading is formed once the registered runs of its dataset have all landed.}
\expandafter\gdef\csname R@an.p3d.acdc.d0\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.d1\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.d2\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.label\endcsname{ACDC}
\expandafter\gdef\csname R@an.p3d.acdc.n\endcsname{3}
\expandafter\gdef\csname R@an.p3d.acdc.nfail\endcsname{0}
\expandafter\gdef\csname R@an.p3d.acdc.nlanded\endcsname{0}
\expandafter\gdef\csname R@an.p3d.acdc.nviol\endcsname{0}
\expandafter\gdef\csname R@an.p3d.acdc.r1.alt.label\endcsname{the uncompiled sub-pool of the frozen pool (CORRECTIONS C30)}
\expandafter\gdef\csname R@an.p3d.acdc.r1.alt.n\endcsname{0}
\expandafter\gdef\csname R@an.p3d.acdc.r1.alt.se\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r1.alt.state\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r1.alt.value\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r1.df\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r1.n\endcsname{0}
\expandafter\gdef\csname R@an.p3d.acdc.r1.se\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r1.state\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r1.value\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r1.word\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r2.df\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r2.df1\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r2.df2\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r2.factor\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r2.hi\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r2.interval\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r2.lo\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r2.ratio\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r2.scale\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r2.sd_diff\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r2.sd_seed\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r2.state\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.r2.word\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.s0\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.s1\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.s2\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.state\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.acdc.stock.mean\endcsname{92.009}
\expandafter\gdef\csname R@an.p3d.acdc.stock.n\endcsname{6}
\expandafter\gdef\csname R@an.p3d.acdc.stock.nlanded\endcsname{6}
\expandafter\gdef\csname R@an.p3d.acdc.stock.s0\endcsname{92.113}
\expandafter\gdef\csname R@an.p3d.acdc.stock.s1\endcsname{91.919}
\expandafter\gdef\csname R@an.p3d.acdc.stock.s2\endcsname{91.997}
\expandafter\gdef\csname R@an.p3d.acdc.stock.sd\endcsname{0.099}
\expandafter\gdef\csname R@an.p3d.amos.d0\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.d1\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.d2\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.label\endcsname{AMOS22}
\expandafter\gdef\csname R@an.p3d.amos.n\endcsname{3}
\expandafter\gdef\csname R@an.p3d.amos.nfail\endcsname{0}
\expandafter\gdef\csname R@an.p3d.amos.nlanded\endcsname{0}
\expandafter\gdef\csname R@an.p3d.amos.nviol\endcsname{0}
\expandafter\gdef\csname R@an.p3d.amos.r1.alt.label\endcsname{the uncompiled sub-pool of the frozen pool (CORRECTIONS C30)}
\expandafter\gdef\csname R@an.p3d.amos.r1.alt.n\endcsname{0}
\expandafter\gdef\csname R@an.p3d.amos.r1.alt.se\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r1.alt.state\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r1.alt.value\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r1.df\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r1.n\endcsname{0}
\expandafter\gdef\csname R@an.p3d.amos.r1.se\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r1.state\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r1.value\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r1.word\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r2.df\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r2.df1\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r2.df2\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r2.factor\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r2.hi\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r2.interval\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r2.lo\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r2.ratio\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r2.scale\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r2.sd_diff\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r2.sd_seed\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r2.state\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.r2.word\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.s0\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.s1\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.s2\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.state\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.amos.stock.mean\endcsname{87.701}
\expandafter\gdef\csname R@an.p3d.amos.stock.n\endcsname{6}
\expandafter\gdef\csname R@an.p3d.amos.stock.nlanded\endcsname{6}
\expandafter\gdef\csname R@an.p3d.amos.stock.s0\endcsname{87.630}
\expandafter\gdef\csname R@an.p3d.amos.stock.s1\endcsname{87.641}
\expandafter\gdef\csname R@an.p3d.amos.stock.s2\endcsname{87.832}
\expandafter\gdef\csname R@an.p3d.amos.stock.sd\endcsname{0.122}
\expandafter\gdef\csname R@an.p3d.excluded.n\endcsname{0}
\expandafter\gdef\csname R@an.p3d.failed.n\endcsname{0}
\expandafter\gdef\csname R@an.p3d.floor\endcsname{0.50}
\expandafter\gdef\csname R@an.p3d.interval.conf\endcsname{95\%}
\expandafter\gdef\csname R@an.p3d.interval.dfmin\endcsname{5}
\expandafter\gdef\csname R@an.p3d.kits.d0\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.d1\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.d10\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.d11\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.d2\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.d3\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.d4\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.d5\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.d6\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.d7\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.d8\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.d9\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.label\endcsname{KiTS23}
\expandafter\gdef\csname R@an.p3d.kits.n\endcsname{12}
\expandafter\gdef\csname R@an.p3d.kits.nfail\endcsname{0}
\expandafter\gdef\csname R@an.p3d.kits.nlanded\endcsname{0}
\expandafter\gdef\csname R@an.p3d.kits.nviol\endcsname{0}
\expandafter\gdef\csname R@an.p3d.kits.r1.df\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.r1.n\endcsname{0}
\expandafter\gdef\csname R@an.p3d.kits.r1.se\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.r1.state\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.r1.value\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.r1.word\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.r2.df\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.r2.df1\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.r2.df2\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.r2.factor\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.r2.hi\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.r2.interval\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.r2.lo\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.r2.ratio\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.r2.scale\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.r2.sd_diff\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.r2.sd_seed\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.r2.state\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.r2.word\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.s0\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.s1\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.s10\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.s11\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.s2\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.s3\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.s4\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.s5\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.s6\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.s7\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.s8\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.s9\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.state\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.kits.stock.mean\endcsname{84.038}
\expandafter\gdef\csname R@an.p3d.kits.stock.n\endcsname{12}
\expandafter\gdef\csname R@an.p3d.kits.stock.nlanded\endcsname{12}
\expandafter\gdef\csname R@an.p3d.kits.stock.s0\endcsname{84.272}
\expandafter\gdef\csname R@an.p3d.kits.stock.s1\endcsname{83.114}
\expandafter\gdef\csname R@an.p3d.kits.stock.s10\endcsname{85.105}
\expandafter\gdef\csname R@an.p3d.kits.stock.s11\endcsname{84.803}
\expandafter\gdef\csname R@an.p3d.kits.stock.s2\endcsname{82.749}
\expandafter\gdef\csname R@an.p3d.kits.stock.s3\endcsname{83.746}
\expandafter\gdef\csname R@an.p3d.kits.stock.s4\endcsname{84.621}
\expandafter\gdef\csname R@an.p3d.kits.stock.s5\endcsname{83.230}
\expandafter\gdef\csname R@an.p3d.kits.stock.s6\endcsname{84.793}
\expandafter\gdef\csname R@an.p3d.kits.stock.s7\endcsname{83.926}
\expandafter\gdef\csname R@an.p3d.kits.stock.s8\endcsname{84.396}
\expandafter\gdef\csname R@an.p3d.kits.stock.s9\endcsname{83.697}
\expandafter\gdef\csname R@an.p3d.kits.stock.sd\endcsname{0.751}
\expandafter\gdef\csname R@an.p3d.landed.n\endcsname{0}
\expandafter\gdef\csname R@an.p3d.landed.word\endcsname{none}
\expandafter\gdef\csname R@an.p3d.nds\endcsname{3}
\expandafter\gdef\csname R@an.p3d.nds.word\endcsname{three}
\expandafter\gdef\csname R@an.p3d.nruns\endcsname{18}
\expandafter\gdef\csname R@an.p3d.nruns.word\endcsname{eighteen}
\expandafter\gdef\csname R@an.p3d.p3c.ac.hi\endcsname{+0.97}
\expandafter\gdef\csname R@an.p3d.p3c.ac.lo\endcsname{\ensuremath{-}0.18}
\expandafter\gdef\csname R@an.p3d.p3c.ac.np3c\endcsname{8}
\expandafter\gdef\csname R@an.p3d.p3c.ac.nstock\endcsname{9}
\expandafter\gdef\csname R@an.p3d.p3c.ac.sd.p3c\endcsname{0.55}
\expandafter\gdef\csname R@an.p3d.p3c.ac.sd.stock\endcsname{0.63}
\expandafter\gdef\csname R@an.p3d.p3c.ac.sdratio\endcsname{0.87}
\expandafter\gdef\csname R@an.p3d.p3c.ac.se\endcsname{0.29}
\expandafter\gdef\csname R@an.p3d.p3c.ac.state\endcsname{complete}
\expandafter\gdef\csname R@an.p3d.p3c.ac.val\endcsname{+0.39}
\expandafter\gdef\csname R@an.p3d.p3c.ac.word\endcsname{within the reference's seed noise}
\expandafter\gdef\csname R@an.p3d.p3c.acdc.w.status\endcsname{complete}
\expandafter\gdef\csname R@an.p3d.p3c.acdc.w.vspool\endcsname{\ensuremath{+0.117}}
\expandafter\gdef\csname R@an.p3d.p3c.acdc.w.vssix\endcsname{\textemdash}
\expandafter\gdef\csname R@an.p3d.p3c.amos.w.status\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.p3c.amos.w.vspool\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.p3c.amos.w.vssix\endcsname{pending}
\expandafter\gdef\csname R@an.p3d.p3c.kits.w.status\endcsname{complete}
\expandafter\gdef\csname R@an.p3d.p3c.kits.w.vspool\endcsname{\ensuremath{+1.176}}
\expandafter\gdef\csname R@an.p3d.p3c.kits.w.vssix\endcsname{\ensuremath{+0.932}}
\expandafter\gdef\csname R@an.p3d.r1.complete.n\endcsname{0}
\expandafter\gdef\csname R@an.p3d.r2.complete.n\endcsname{0}
\expandafter\gdef\csname R@an.p3d.sentence.r1.acdc\endcsname{The P3d replicate (the stock default's own initial weights, Addendum AI) is pending on ACDC: 0 of 3 registered runs have landed, and its mean difference from the stock default of the same nominal seeds is formed once all of them have.}
\expandafter\gdef\csname R@an.p3d.sentence.r1.amos\endcsname{The P3d replicate (the stock default's own initial weights, Addendum AI) is pending on AMOS22: 0 of 3 registered runs have landed, and its mean difference from the stock default of the same nominal seeds is formed once all of them have.}
\expandafter\gdef\csname R@an.p3d.sentence.r1.kits\endcsname{The P3d replicate (the stock default's own initial weights, Addendum AI) is pending on KiTS23: 0 of 12 registered runs have landed, and its mean difference from the stock default of the same nominal seeds is formed once all of them have.}
\expandafter\gdef\csname R@an.p3d.sentence.r2.acdc\endcsname{The spread of the P3d same-seed differences is pending on ACDC: 0 of 3 registered runs have landed, and the ratio of that spread to the spread of a pair of independent stock runs is formed once all of them have.}
\expandafter\gdef\csname R@an.p3d.sentence.r2.amos\endcsname{The spread of the P3d same-seed differences is pending on AMOS22: 0 of 3 registered runs have landed, and the ratio of that spread to the spread of a pair of independent stock runs is formed once all of them have.}
\expandafter\gdef\csname R@an.p3d.sentence.r2.kits\endcsname{The spread of the P3d same-seed differences is pending on KiTS23: 0 of 12 registered runs have landed, and the ratio of that spread to the spread of a pair of independent stock runs is formed once all of them have.}
\expandafter\gdef\csname R@an.p3d.sentence.r3.acdc\endcsname{Beside it, the function-identical rebuild P3c (its own initial weights, plan-aware build) reads \ensuremath{+0.117} pp from the frozen ACDC pool at fresh seeds 1 and 2 (Addendum W).}
\expandafter\gdef\csname R@an.p3d.sentence.r3.amos\endcsname{The fresh-seed reading of the function-identical rebuild P3c (Addendum W) is pending on AMOS22.}
\expandafter\gdef\csname R@an.p3d.sentence.r3.kits\endcsname{Beside it, the function-identical rebuild P3c (its own initial weights, plan-aware build) reads \ensuremath{+1.176} pp from the frozen KiTS23 pool at fresh seeds 1 and 2 (Addendum W); against the 9 stock runs of this study's conditions its offset reads +0.39 pp (interval \ensuremath{-}0.18 to +0.97, within the reference's seed noise; Addendum AC).}
\expandafter\gdef\csname R@an.p3d.summary\endcsname{The identity-initialised replicate P3d of Addendum AI (eighteen runs on three datasets) is pending: 0 of 18 registered runs have landed, and each reading is formed once the registered runs of its dataset have all landed.}
\expandafter\gdef\csname R@an.p3d.trainer.sha\endcsname{fc0f94fefbf3488b}
\expandafter\gdef\csname R@an.p3d.what_it_controls\endcsname{The identity-initialised replicate P3d is the function-identical rebuild of the stock default started from the stock default's own initial weights: at a given nominal seed its real parameter tensors and the torch random stream after initialisation are the stock run's (a CPU check of every parameter tensor), and its extra parameters receive exactly zero gradient. It does not control the data order or the numpy augmentation, which the harness seeds from the operating system's entropy in the dataloader workers (the case order differs even between stock runs of the same nominal seed), nor the GPU kernels (cudnn benchmark is on). Its same-seed difference from the stock run therefore measures the part of the seed-to-seed spread that is not initial weights.}
\expandafter\gdef\csname R@an.paired_cases.B\endcsname{10000}
\expandafter\gdef\csname R@an.paired_cases.amos.L1_L1b.ci_hi\endcsname{\ensuremath{+1.08}}
\expandafter\gdef\csname R@an.paired_cases.amos.L1_L1b.ci_lo\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.paired_cases.amos.L1_L1b.frac_improved\endcsname{52.5}
\expandafter\gdef\csname R@an.paired_cases.amos.L1_L1b.mean\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.paired_cases.amos.L1_L1b.mean_wo5\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.paired_cases.amos.L1_L1b.n_improved\endcsname{21}
\expandafter\gdef\csname R@an.paired_cases.amos.L1_L1b.se_case\endcsname{0.281}
\expandafter\gdef\csname R@an.paired_cases.amos.L1_L1b.top5_share\endcsname{105}
\expandafter\gdef\csname R@an.paired_cases.amos.L1_L1b.trim\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.paired_cases.amos.L1_L1b.wilcoxon_p\endcsname{0.295}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_L1.ci_hi\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_L1.ci_lo\endcsname{\ensuremath{-0.62}}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_L1.frac_improved\endcsname{47.5}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_L1.mean\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_L1.mean_wo5\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_L1.n_improved\endcsname{19}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_L1.se_case\endcsname{0.187}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_L1.top5_share\endcsname{131}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_L1.trim\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_L1.wilcoxon_p\endcsname{0.277}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_default.ci_hi\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_default.ci_lo\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_default.frac_improved\endcsname{67.5}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_default.mean\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_default.mean.contemporaneous\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_default.mean.uncompiled\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_default.mean_wo5\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_default.n_improved\endcsname{27}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_default.se_case\endcsname{0.171}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_default.top5_share\endcsname{68}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_default.trim\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.paired_cases.amos.L3_default.wilcoxon_p\endcsname{0.002}
\expandafter\gdef\csname R@an.paired_cases.amos.altref.contemporaneous.estimand\endcsname{per-case mean over the 40 validation cases}
\expandafter\gdef\csname R@an.paired_cases.amos.altref.contemporaneous.head\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.paired_cases.amos.altref.contemporaneous.n\endcsname{3}
\expandafter\gdef\csname R@an.paired_cases.amos.altref.contemporaneous.ratio\endcsname{88}
\expandafter\gdef\csname R@an.paired_cases.amos.altref.contemporaneous.shift\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.paired_cases.amos.altref.contemporaneous.short\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.paired_cases.amos.altref.contemporaneous.vs\endcsname{the arms' own deltas against the same reference}
\expandafter\gdef\csname R@an.paired_cases.amos.altref.n_drawn\endcsname{2}
\expandafter\gdef\csname R@an.paired_cases.amos.altref.n_pending\endcsname{0}
\expandafter\gdef\csname R@an.paired_cases.amos.altref.pending\endcsname{none}
\expandafter\gdef\csname R@an.paired_cases.amos.altref.uncompiled.estimand\endcsname{per-case mean over the 40 validation cases}
\expandafter\gdef\csname R@an.paired_cases.amos.altref.uncompiled.head\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.paired_cases.amos.altref.uncompiled.n\endcsname{3}
\expandafter\gdef\csname R@an.paired_cases.amos.altref.uncompiled.ratio\endcsname{25}
\expandafter\gdef\csname R@an.paired_cases.amos.altref.uncompiled.shift\endcsname{\ensuremath{+0.024}}
\expandafter\gdef\csname R@an.paired_cases.amos.altref.uncompiled.short\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.paired_cases.amos.altref.uncompiled.vs\endcsname{the arms' own deltas against the same reference}
\expandafter\gdef\csname R@an.paired_cases.amos.armspread\endcsname{0.614}
\expandafter\gdef\csname R@an.paired_cases.amos.armspread.n\endcsname{6}
\expandafter\gdef\csname R@an.paired_cases.amos.fresh.L1\endcsname{88.166}
\expandafter\gdef\csname R@an.paired_cases.amos.fresh.L3\endcsname{87.833}
\expandafter\gdef\csname R@an.paired_cases.amos.fresh.L3_L1\endcsname{\ensuremath{-0.332}}
\expandafter\gdef\csname R@an.paired_cases.amos.fresh.behind\endcsname{HyReX}
\expandafter\gdef\csname R@an.paired_cases.amos.fresh.gap_abs\endcsname{0.332}
\expandafter\gdef\csname R@an.paired_cases.amos.fresh.leader\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.paired_cases.amos.n\endcsname{40}
\expandafter\gdef\csname R@an.paired_cases.amos.n_empty_pairs\endcsname{6}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L1_L1b.ci_hi\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L1_L1b.ci_lo\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L1_L1b.frac_improved\endcsname{50.0}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L1_L1b.mean\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L1_L1b.mean_wo5\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L1_L1b.n_improved\endcsname{20}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L1_L1b.se_case\endcsname{0.207}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L1_L1b.top5_share\endcsname{163}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L1_L1b.trim\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L1_L1b.wilcoxon_p\endcsname{0.563}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_L1.ci_hi\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_L1.ci_lo\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_L1.frac_improved\endcsname{50.0}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_L1.mean\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_L1.mean_wo5\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_L1.n_improved\endcsname{20}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_L1.se_case\endcsname{0.179}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_L1.top5_share\endcsname{246}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_L1.trim\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_L1.wilcoxon_p\endcsname{0.572}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_default.ci_hi\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_default.ci_lo\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_default.frac_improved\endcsname{70.0}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_default.mean\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_default.mean_wo5\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_default.n_improved\endcsname{28}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_default.se_case\endcsname{0.085}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_default.top5_share\endcsname{43}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_default.trim\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.L3_default.wilcoxon_p\endcsname{\ensuremath{<}0.001}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.null.n\endcsname{6}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.null.n_ci_excl0\endcsname{1}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.null.n_p05\endcsname{1}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.rank.L1.p_first\endcsname{56.5}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.rank.L3.p_above_L1\endcsname{28.7}
\expandafter\gdef\csname R@an.paired_cases.amos.ne.rank.L3.p_first\endcsname{12.5}
\expandafter\gdef\csname R@an.paired_cases.amos.null.n\endcsname{6}
\expandafter\gdef\csname R@an.paired_cases.amos.null.n_ci_excl0\endcsname{0}
\expandafter\gdef\csname R@an.paired_cases.amos.null.n_p05\endcsname{0}
\expandafter\gdef\csname R@an.paired_cases.amos.rank.L1.p_first\endcsname{67.7}
\expandafter\gdef\csname R@an.paired_cases.amos.rank.L3.p_above_L1\endcsname{9.4}
\expandafter\gdef\csname R@an.paired_cases.amos.rank.L3.p_first\endcsname{3.2}
\expandafter\gdef\csname R@an.paired_cases.amos.ref.n\endcsname{6}
\expandafter\gdef\csname R@an.paired_cases.amos.ref.short\endcsname{frozen pool}
\expandafter\gdef\csname R@an.paired_cases.amos.sd_delta\endcsname{0.132}
\expandafter\gdef\csname R@an.paired_cases.kits.L1_L1b.ci_hi\endcsname{\ensuremath{+2.54}}
\expandafter\gdef\csname R@an.paired_cases.kits.L1_L1b.ci_lo\endcsname{\ensuremath{-1.17}}
\expandafter\gdef\csname R@an.paired_cases.kits.L1_L1b.frac_improved\endcsname{51.0}
\expandafter\gdef\csname R@an.paired_cases.kits.L1_L1b.mean\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.paired_cases.kits.L1_L1b.mean_wo5\endcsname{\ensuremath{-0.90}}
\expandafter\gdef\csname R@an.paired_cases.kits.L1_L1b.n_improved\endcsname{50}
\expandafter\gdef\csname R@an.paired_cases.kits.L1_L1b.se_case\endcsname{0.933}
\expandafter\gdef\csname R@an.paired_cases.kits.L1_L1b.top5_share\endcsname{246}
\expandafter\gdef\csname R@an.paired_cases.kits.L1_L1b.trim\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.paired_cases.kits.L1_L1b.wilcoxon_p\endcsname{0.740}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_L1.ci_hi\endcsname{\ensuremath{+1.86}}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_L1.ci_lo\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_L1.frac_improved\endcsname{40.8}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_L1.mean\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_L1.mean_wo5\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_L1.n_improved\endcsname{40}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_L1.se_case\endcsname{0.619}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_L1.top5_share\endcsname{197}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_L1.trim\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_L1.wilcoxon_p\endcsname{0.350}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_default.ci_hi\endcsname{\ensuremath{+4.74}}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_default.ci_lo\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_default.frac_improved\endcsname{71.4}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_default.mean\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_default.mean.contemporaneous\endcsname{\ensuremath{+2.35}}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_default.mean_wo5\endcsname{\ensuremath{+1.20}}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_default.n_improved\endcsname{70}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_default.se_case\endcsname{0.918}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_default.top5_share\endcsname{60}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_default.trim\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.paired_cases.kits.L3_default.wilcoxon_p\endcsname{\ensuremath{<}0.001}
\expandafter\gdef\csname R@an.paired_cases.kits.altref.contemporaneous.estimand\endcsname{per-case mean over the 98 validation cases}
\expandafter\gdef\csname R@an.paired_cases.kits.altref.contemporaneous.head\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.paired_cases.kits.altref.contemporaneous.n\endcsname{3}
\expandafter\gdef\csname R@an.paired_cases.kits.altref.contemporaneous.ratio\endcsname{4}
\expandafter\gdef\csname R@an.paired_cases.kits.altref.contemporaneous.shift\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.paired_cases.kits.altref.contemporaneous.short\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.paired_cases.kits.altref.contemporaneous.vs\endcsname{the arms' own deltas against the same reference}
\expandafter\gdef\csname R@an.paired_cases.kits.altref.n_drawn\endcsname{1}
\expandafter\gdef\csname R@an.paired_cases.kits.altref.n_pending\endcsname{0}
\expandafter\gdef\csname R@an.paired_cases.kits.altref.pending\endcsname{none}
\expandafter\gdef\csname R@an.paired_cases.kits.armspread\endcsname{2.178}
\expandafter\gdef\csname R@an.paired_cases.kits.armspread.n\endcsname{6}
\expandafter\gdef\csname R@an.paired_cases.kits.fresh.L1\endcsname{86.853}
\expandafter\gdef\csname R@an.paired_cases.kits.fresh.L3\endcsname{85.472}
\expandafter\gdef\csname R@an.paired_cases.kits.fresh.L3_L1\endcsname{\ensuremath{-1.382}}
\expandafter\gdef\csname R@an.paired_cases.kits.fresh.behind\endcsname{HyReX}
\expandafter\gdef\csname R@an.paired_cases.kits.fresh.gap_abs\endcsname{1.382}
\expandafter\gdef\csname R@an.paired_cases.kits.fresh.leader\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.paired_cases.kits.n\endcsname{98}
\expandafter\gdef\csname R@an.paired_cases.kits.n_empty_pairs\endcsname{0}
\expandafter\gdef\csname R@an.paired_cases.kits.null.n\endcsname{3}
\expandafter\gdef\csname R@an.paired_cases.kits.null.n_ci_excl0\endcsname{1}
\expandafter\gdef\csname R@an.paired_cases.kits.null.n_p05\endcsname{0}
\expandafter\gdef\csname R@an.paired_cases.kits.rank.L1.p_first\endcsname{9.5}
\expandafter\gdef\csname R@an.paired_cases.kits.rank.L3.p_above_L1\endcsname{79.8}
\expandafter\gdef\csname R@an.paired_cases.kits.rank.L3.p_first\endcsname{48.0}
\expandafter\gdef\csname R@an.paired_cases.kits.ref.n\endcsname{3}
\expandafter\gdef\csname R@an.paired_cases.kits.ref.short\endcsname{frozen pool}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L1_L1b_rep.ci_hi\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L1_L1b_rep.ci_lo\endcsname{\ensuremath{-1.13}}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L1_L1b_rep.frac_improved\endcsname{54.1}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L1_L1b_rep.mean\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L1_L1b_rep.wilcoxon_p\endcsname{0.675}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L1b_rep_default.ci_hi\endcsname{\ensuremath{+3.75}}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L1b_rep_default.ci_lo\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L1b_rep_default.frac_improved\endcsname{70.4}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L1b_rep_default.mean\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L1b_rep_default.wilcoxon_p\endcsname{\ensuremath{<}0.001}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L3_L1b_rep.ci_hi\endcsname{\ensuremath{+2.14}}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L3_L1b_rep.ci_lo\endcsname{\ensuremath{-0.81}}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L3_L1b_rep.frac_improved\endcsname{45.9}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L3_L1b_rep.mean\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L3_L1b_rep.wilcoxon_p\endcsname{0.302}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L4_L1b_rep.ci_hi\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L4_L1b_rep.ci_lo\endcsname{\ensuremath{-1.48}}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L4_L1b_rep.frac_improved\endcsname{56.1}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L4_L1b_rep.mean\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.paired_cases.kits.rep.L4_L1b_rep.wilcoxon_p\endcsname{0.240}
\expandafter\gdef\csname R@an.paired_cases.kits.sd_delta\endcsname{0.918}
\expandafter\gdef\csname R@an.paired_cases.seed\endcsname{20261005}
\expandafter\gdef\csname R@an.paired_cases.seed.label\endcsname{discovery seed~0}
\expandafter\gdef\csname R@an.paired_cases.topk\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c1.gap\endcsname{\ensuremath{-1.97}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c1.pp\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c1.ppalt\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c1.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c1.z\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c10.gap\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c10.pp\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c10.ppalt\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c10.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c10.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c11.gap\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c11.pp\endcsname{\ensuremath{+0.79}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c11.ppalt\endcsname{\ensuremath{+0.79}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c11.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c11.z\endcsname{\ensuremath{+4.8}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c12.gap\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c12.pp\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c12.ppalt\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c12.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c12.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c13.gap\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c13.pp\endcsname{\ensuremath{+1.26}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c13.ppalt\endcsname{\ensuremath{+1.32}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c13.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c13.z\endcsname{\ensuremath{+3.2}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c14.gap\endcsname{\ensuremath{-1.63}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c14.pp\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c14.ppalt\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c14.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c14.z\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c15.gap\endcsname{\ensuremath{-2.62}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c15.pp\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c15.ppalt\endcsname{\ensuremath{+1.20}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c15.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c15.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c2.gap\endcsname{\ensuremath{-0.72}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c2.pp\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c2.ppalt\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c2.rank\endcsname{26}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c2.z\endcsname{\ensuremath{-0.2}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c3.gap\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c3.pp\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c3.ppalt\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c3.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c3.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c4.gap\endcsname{\ensuremath{-6.54}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c4.pp\endcsname{\ensuremath{-1.88}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c4.ppalt\endcsname{\ensuremath{-2.49}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c4.rank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c4.z\endcsname{\ensuremath{-1.4}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c5.gap\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c5.pp\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c5.ppalt\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c5.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c5.z\endcsname{\ensuremath{+2.6}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c6.gap\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c6.pp\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c6.ppalt\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c6.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c6.z\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c7.gap\endcsname{\ensuremath{-0.69}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c7.pp\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c7.ppalt\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c7.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c7.z\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c8.gap\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c8.pp\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c8.ppalt\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c8.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c8.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c9.gap\endcsname{\ensuremath{-0.41}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c9.pp\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c9.ppalt\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c9.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.c9.z\endcsname{\ensuremath{+2.9}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.head_pp\endcsname{\ensuremath{+0.390}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.head_ppalt\endcsname{\ensuremath{+0.361}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.maxz\endcsname{\ensuremath{+4.8}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.maxz_class\endcsname{right adrenal gland}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.maxz_pp\endcsname{\ensuremath{+0.79}}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.npos2\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.npos2alt\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.pos2list\endcsname{right adrenal gland, duodenum, postcava, liver, esophagus, spleen}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.C1.amos.sumpos_pp\endcsname{\ensuremath{+4.28}}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.c123.gap\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.c123.pp\endcsname{\ensuremath{+0.97}}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.c123.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.c123.z\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.c2.gap\endcsname{\ensuremath{-2.28}}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.c2.pp\endcsname{\ensuremath{+2.81}}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.c2.ppalt\endcsname{\ensuremath{+2.52}}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.c2.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.c2.z\endcsname{\ensuremath{+2.9}}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.c23.gap\endcsname{\ensuremath{-0.73}}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.c23.pp\endcsname{\ensuremath{+3.42}}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.c23.ppalt\endcsname{\ensuremath{+3.10}}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.c23.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.c23.z\endcsname{\ensuremath{+3.5}}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.head_pp\endcsname{\ensuremath{+2.401}}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.head_ppalt\endcsname{\ensuremath{+2.157}}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.maxz\endcsname{\ensuremath{+3.5}}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.maxz_pp\endcsname{\ensuremath{+3.42}}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.pos2list\endcsname{masses, tumour, kidney}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.C1.fresh.kits.sumpos_pp\endcsname{\ensuremath{+7.20}}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.c123.gap\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.c123.pp\endcsname{\ensuremath{+1.22}}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.c123.ppalt\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.c123.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.c123.z\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.c2.gap\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.c2.pp\endcsname{\ensuremath{+4.98}}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.c2.ppalt\endcsname{\ensuremath{+4.69}}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.c2.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.c2.z\endcsname{\ensuremath{+4.1}}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.c23.gap\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.c23.pp\endcsname{\ensuremath{+4.32}}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.c23.ppalt\endcsname{\ensuremath{+3.99}}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.c23.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.c23.z\endcsname{\ensuremath{+3.5}}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.head_pp\endcsname{\ensuremath{+3.507}}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.head_ppalt\endcsname{\ensuremath{+3.264}}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.maxz\endcsname{\ensuremath{+4.1}}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.maxz_pp\endcsname{\ensuremath{+4.98}}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.pos2list\endcsname{tumour, masses, kidney}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.C1.kits.sumpos_pp\endcsname{\ensuremath{+10.52}}
\expandafter\gdef\csname R@an.perclass_all.C1.params\endcsname{52.3}
\expandafter\gdef\csname R@an.perclass_all.C1.params.acdc\endcsname{51.6}
\expandafter\gdef\csname R@an.perclass_all.C1.params.amos\endcsname{52.3}
\expandafter\gdef\csname R@an.perclass_all.C1.params.kits\endcsname{52.4}
\expandafter\gdef\csname R@an.perclass_all.C1.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c1.gap\endcsname{\ensuremath{-2.12}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c1.pp\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c1.ppalt\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c1.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c1.z\endcsname{\ensuremath{+1.7}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c10.gap\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c10.pp\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c10.ppalt\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c10.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c10.z\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c11.gap\endcsname{\ensuremath{-0.64}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c11.pp\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c11.ppalt\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c11.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c11.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c12.gap\endcsname{\ensuremath{-1.06}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c12.pp\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c12.ppalt\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c12.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c12.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c13.gap\endcsname{\ensuremath{-1.68}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c13.pp\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c13.ppalt\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c13.rank\endcsname{26}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c13.z\endcsname{\ensuremath{-0.7}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c14.gap\endcsname{\ensuremath{-2.57}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c14.pp\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c14.ppalt\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c14.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c14.z\endcsname{\ensuremath{-1.8}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c15.gap\endcsname{\ensuremath{-3.39}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c15.pp\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c15.ppalt\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c15.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c15.z\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c2.gap\endcsname{\ensuremath{-0.73}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c2.pp\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c2.ppalt\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c2.rank\endcsname{27}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c2.z\endcsname{\ensuremath{-0.2}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c3.gap\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c3.pp\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c3.ppalt\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c3.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c3.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c4.gap\endcsname{\ensuremath{-3.24}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c4.pp\endcsname{\ensuremath{+1.43}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c4.ppalt\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c4.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c4.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c5.gap\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c5.pp\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c5.ppalt\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c5.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c5.z\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c6.gap\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c6.pp\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c6.ppalt\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c6.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c6.z\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c7.gap\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c7.pp\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c7.ppalt\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c7.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c7.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c8.gap\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c8.pp\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c8.ppalt\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c8.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c8.z\endcsname{\ensuremath{-0.7}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c9.gap\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c9.pp\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c9.ppalt\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c9.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.c9.z\endcsname{\ensuremath{+1.7}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.head_pp\endcsname{\ensuremath{+0.278}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.head_ppalt\endcsname{\ensuremath{+0.249}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.maxz\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.maxz_class\endcsname{stomach}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.maxz_pp\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D1.amos.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.altflip\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.c123.gap\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.c123.pp\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.c123.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.c123.z\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.c2.gap\endcsname{\ensuremath{-3.51}}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.c2.pp\endcsname{\ensuremath{+1.58}}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.c2.ppalt\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.c2.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.c2.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.c23.gap\endcsname{\ensuremath{-2.07}}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.c23.pp\endcsname{\ensuremath{+2.07}}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.c23.ppalt\endcsname{\ensuremath{+1.75}}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.c23.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.c23.z\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.head_pp\endcsname{\ensuremath{+1.477}}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.head_ppalt\endcsname{\ensuremath{+1.233}}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.maxz\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.maxz_class\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.maxz_pp\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.npos2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.pos2list\endcsname{kidney, masses}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.D1.fresh.kits.sumpos_pp\endcsname{\ensuremath{+2.85}}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.c123.gap\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.c123.pp\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.c123.ppalt\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.c123.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.c123.z\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.c2.gap\endcsname{\ensuremath{-4.18}}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.c2.pp\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.c2.ppalt\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.c2.rank\endcsname{29}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.c2.z\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.c23.gap\endcsname{\ensuremath{-1.39}}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.c23.pp\endcsname{\ensuremath{+2.92}}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.c23.ppalt\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.c23.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.c23.z\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.head_pp\endcsname{\ensuremath{+1.607}}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.head_ppalt\endcsname{\ensuremath{+1.363}}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.maxz\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.maxz_class\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.maxz_pp\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.npos2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.npos2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.pos2list\endcsname{kidney, masses}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D1.kits.sumpos_pp\endcsname{\ensuremath{+4.02}}
\expandafter\gdef\csname R@an.perclass_all.D1.params\endcsname{20.9}
\expandafter\gdef\csname R@an.perclass_all.D1.params.acdc\endcsname{20.1}
\expandafter\gdef\csname R@an.perclass_all.D1.params.amos\endcsname{20.9}
\expandafter\gdef\csname R@an.perclass_all.D1.params.kits\endcsname{20.9}
\expandafter\gdef\csname R@an.perclass_all.D1.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c1.gap\endcsname{\ensuremath{-2.81}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c1.pp\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c1.ppalt\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c1.rank\endcsname{28}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c1.z\endcsname{\ensuremath{-0.7}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c10.gap\endcsname{\ensuremath{-0.65}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c10.pp\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c10.ppalt\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c10.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c10.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c11.gap\endcsname{\ensuremath{-1.56}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c11.pp\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c11.ppalt\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c11.rank\endcsname{30}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c11.z\endcsname{\ensuremath{-3.8}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c12.gap\endcsname{\ensuremath{-2.80}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c12.pp\endcsname{\ensuremath{-0.99}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c12.ppalt\endcsname{\ensuremath{-0.73}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c12.rank\endcsname{35}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c12.z\endcsname{\ensuremath{-1.1}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c13.gap\endcsname{\ensuremath{-1.73}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c13.pp\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c13.ppalt\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c13.rank\endcsname{29}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c13.z\endcsname{\ensuremath{-0.9}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c14.gap\endcsname{\ensuremath{-3.72}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c14.pp\endcsname{\ensuremath{-1.62}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c14.ppalt\endcsname{\ensuremath{-1.64}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c14.rank\endcsname{36}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c14.z\endcsname{\ensuremath{-6.3}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c15.gap\endcsname{\ensuremath{-4.12}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c15.pp\endcsname{\ensuremath{-0.64}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c15.ppalt\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c15.rank\endcsname{34}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c15.z\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c2.gap\endcsname{\ensuremath{-0.55}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c2.pp\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c2.ppalt\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c2.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c2.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c3.gap\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c3.pp\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c3.ppalt\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c3.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c3.z\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c4.gap\endcsname{\ensuremath{-5.28}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c4.pp\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c4.ppalt\endcsname{\ensuremath{-1.22}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c4.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c4.z\endcsname{\ensuremath{-0.5}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c5.gap\endcsname{\ensuremath{-1.09}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c5.pp\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c5.ppalt\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c5.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c5.z\endcsname{\ensuremath{-0.9}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c6.gap\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c6.pp\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c6.ppalt\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c6.rank\endcsname{30}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c6.z\endcsname{\ensuremath{-1.3}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c7.gap\endcsname{\ensuremath{-1.07}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c7.pp\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c7.ppalt\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c7.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c7.z\endcsname{\ensuremath{-0.4}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c8.gap\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c8.pp\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c8.ppalt\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c8.rank\endcsname{36}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c8.z\endcsname{\ensuremath{-3.2}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c9.gap\endcsname{\ensuremath{-0.87}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c9.pp\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c9.ppalt\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c9.rank\endcsname{30}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.c9.z\endcsname{\ensuremath{-0.7}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.head_pp\endcsname{\ensuremath{-0.362}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.head_ppalt\endcsname{\ensuremath{-0.391}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.maxz\endcsname{\ensuremath{-6.3}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.maxz_class\endcsname{bladder}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.maxz_pp\endcsname{\ensuremath{-1.62}}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.nneg2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.nneg2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D2.amos.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.c123.gap\endcsname{\ensuremath{-0.41}}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.c123.pp\endcsname{\ensuremath{+0.84}}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.72}}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.c123.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.c123.z\endcsname{\ensuremath{+2.3}}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.c2.gap\endcsname{\ensuremath{-2.57}}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.c2.pp\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.c2.ppalt\endcsname{\ensuremath{+2.24}}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.c2.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.c2.z\endcsname{\ensuremath{+2.6}}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.c23.gap\endcsname{\ensuremath{-1.83}}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.c23.pp\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.c23.ppalt\endcsname{\ensuremath{+1.99}}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.c23.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.c23.z\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.head_pp\endcsname{\ensuremath{+1.892}}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.head_ppalt\endcsname{\ensuremath{+1.648}}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.maxz\endcsname{\ensuremath{+2.6}}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.maxz_pp\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.pos2list\endcsname{tumour, masses, kidney}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.D2.fresh.kits.sumpos_pp\endcsname{\ensuremath{+5.67}}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.c123.gap\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.c123.pp\endcsname{\ensuremath{+0.72}}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.c123.ppalt\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.c123.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.c123.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.c2.gap\endcsname{\ensuremath{-1.26}}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.c2.pp\endcsname{\ensuremath{+3.72}}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.c2.ppalt\endcsname{\ensuremath{+3.43}}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.c2.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.c2.z\endcsname{\ensuremath{+3.0}}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.c23.gap\endcsname{\ensuremath{-1.69}}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.c23.pp\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.c23.ppalt\endcsname{\ensuremath{+2.30}}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.c23.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.c23.z\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.head_pp\endcsname{\ensuremath{+2.355}}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.head_ppalt\endcsname{\ensuremath{+2.112}}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.maxz\endcsname{\ensuremath{+3.0}}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.maxz_pp\endcsname{\ensuremath{+3.72}}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.npos2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.pos2list\endcsname{tumour, masses}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.D2.kits.sumpos_pp\endcsname{\ensuremath{+6.35}}
\expandafter\gdef\csname R@an.perclass_all.D2.params\endcsname{26.0}
\expandafter\gdef\csname R@an.perclass_all.D2.params.acdc\endcsname{25.3}
\expandafter\gdef\csname R@an.perclass_all.D2.params.amos\endcsname{26.0}
\expandafter\gdef\csname R@an.perclass_all.D2.params.kits\endcsname{26.1}
\expandafter\gdef\csname R@an.perclass_all.D2.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c1.gap\endcsname{\ensuremath{-2.38}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c1.pp\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c1.ppalt\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c1.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c1.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c10.gap\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c10.pp\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c10.ppalt\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c10.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c10.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c11.gap\endcsname{\ensuremath{-0.90}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c11.pp\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c11.ppalt\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c11.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c11.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c12.gap\endcsname{\ensuremath{-1.68}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c12.pp\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c12.ppalt\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c12.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c12.z\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c13.gap\endcsname{\ensuremath{-1.13}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c13.pp\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c13.ppalt\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c13.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c13.z\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c14.gap\endcsname{\ensuremath{-1.62}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c14.pp\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c14.ppalt\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c14.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c14.z\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c15.gap\endcsname{\ensuremath{-2.48}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c15.pp\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c15.ppalt\endcsname{\ensuremath{+1.33}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c15.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c15.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c2.gap\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c2.pp\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c2.ppalt\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c2.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c2.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c3.gap\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c3.pp\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c3.ppalt\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c3.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c3.z\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c4.gap\endcsname{\ensuremath{-3.60}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c4.pp\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c4.ppalt\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c4.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c4.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c5.gap\endcsname{\ensuremath{-1.17}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c5.pp\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c5.ppalt\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c5.rank\endcsname{26}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c5.z\endcsname{\ensuremath{-1.2}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c6.gap\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c6.pp\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c6.ppalt\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c6.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c6.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c7.gap\endcsname{\ensuremath{-0.81}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c7.pp\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c7.ppalt\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c7.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c7.z\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c8.gap\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c8.pp\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c8.ppalt\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c8.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c8.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c9.gap\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c9.pp\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c9.ppalt\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c9.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.c9.z\endcsname{\ensuremath{+1.7}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.head_pp\endcsname{\ensuremath{+0.294}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.head_ppalt\endcsname{\ensuremath{+0.266}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.maxz\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.maxz_class\endcsname{bladder}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.maxz_pp\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.I1.amos.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.c123.gap\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.c123.pp\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.c123.ppalt\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.c123.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.c123.z\endcsname{\ensuremath{+1.7}}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.c2.gap\endcsname{\ensuremath{-2.35}}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.c2.pp\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.c2.ppalt\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.c2.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.c2.z\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.c23.gap\endcsname{\ensuremath{-2.03}}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.c23.pp\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.c23.ppalt\endcsname{\ensuremath{+1.97}}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.c23.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.c23.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.head_pp\endcsname{\ensuremath{+1.893}}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.head_ppalt\endcsname{\ensuremath{+1.649}}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.maxz\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.maxz_pp\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.pos2list\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.I1.kits.sumpos_pp\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@an.perclass_all.I1.params\endcsname{29.6}
\expandafter\gdef\csname R@an.perclass_all.I1.params.acdc\endcsname{28.9}
\expandafter\gdef\csname R@an.perclass_all.I1.params.amos\endcsname{29.6}
\expandafter\gdef\csname R@an.perclass_all.I1.params.kits\endcsname{29.7}
\expandafter\gdef\csname R@an.perclass_all.I1.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.c1.gap\endcsname{\ensuremath{-0.62}}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.c1.pp\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.c1.ppalt\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.c1.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.c1.z\endcsname{\ensuremath{+4.3}}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.c2.gap\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.c2.pp\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.c2.ppalt\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.c2.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.c2.z\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.c3.gap\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.c3.pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.c3.ppalt\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.c3.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.c3.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.head_pp\endcsname{\ensuremath{+0.336}}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.head_ppalt\endcsname{\ensuremath{+0.329}}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.maxz\endcsname{\ensuremath{+4.3}}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.maxz_class\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.maxz_pp\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.npos2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.nrank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.pos2list\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.acdc.sumpos_pp\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c1.gap\endcsname{\ensuremath{+1.97}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c1.pp\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c1.ppalt\endcsname{\ensuremath{+2.55}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c1.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c1.z\endcsname{\ensuremath{+9.0}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c10.gap\endcsname{\ensuremath{-0.96}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c10.pp\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c10.ppalt\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c10.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c10.z\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c11.gap\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c11.pp\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c11.ppalt\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c11.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c11.z\endcsname{\ensuremath{+5.6}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c12.gap\endcsname{\ensuremath{-1.36}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c12.pp\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c12.ppalt\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c12.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c12.z\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c13.gap\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c13.pp\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c13.ppalt\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c13.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c13.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c14.gap\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c14.pp\endcsname{\ensuremath{+1.60}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c14.ppalt\endcsname{\ensuremath{+1.58}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c14.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c14.z\endcsname{\ensuremath{+6.3}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c15.gap\endcsname{\ensuremath{-3.12}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c15.pp\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c15.ppalt\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c15.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c15.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c2.gap\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c2.pp\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c2.ppalt\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c2.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c2.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c3.gap\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c3.pp\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c3.ppalt\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c3.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c3.z\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c4.gap\endcsname{\ensuremath{-4.20}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c4.pp\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c4.ppalt\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c4.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c4.z\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c5.gap\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c5.pp\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c5.ppalt\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c5.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c5.z\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c6.gap\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c6.pp\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c6.ppalt\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c6.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c6.z\endcsname{\ensuremath{-0.4}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c7.gap\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c7.pp\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c7.ppalt\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c7.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c7.z\endcsname{\ensuremath{+2.3}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c8.gap\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c8.pp\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c8.ppalt\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c8.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c8.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c9.gap\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c9.pp\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c9.ppalt\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c9.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.c9.z\endcsname{\ensuremath{+6.2}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.head_pp\endcsname{\ensuremath{+0.647}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.head_ppalt\endcsname{\ensuremath{+0.618}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.maxz\endcsname{\ensuremath{+9.0}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.maxz_class\endcsname{spleen}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.maxz_pp\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.npos2\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.npos2alt\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.pos2list\endcsname{spleen, bladder, postcava, right adrenal gland, stomach}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.amos.sumpos_pp\endcsname{\ensuremath{+6.58}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.c1.gap\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.c1.pp\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.c1.ppalt\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.c1.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.c1.z\endcsname{\ensuremath{+4.7}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.c2.gap\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.c2.pp\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.c2.ppalt\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.c2.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.c2.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.c3.gap\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.c3.pp\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.c3.ppalt\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.c3.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.c3.z\endcsname{\ensuremath{-1.0}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.head_pp\endcsname{\ensuremath{+0.242}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.head_ppalt\endcsname{\ensuremath{+0.235}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.maxz\endcsname{\ensuremath{+4.7}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.maxz_class\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.maxz_pp\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.nrank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.pos2list\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.acdc.sumpos_pp\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c1.gap\endcsname{\ensuremath{-1.22}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c1.pp\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c1.ppalt\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c1.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c1.z\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c10.gap\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c10.pp\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c10.ppalt\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c10.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c10.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c11.gap\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c11.pp\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c11.ppalt\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c11.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c11.z\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c12.gap\endcsname{\ensuremath{-1.22}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c12.pp\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c12.ppalt\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c12.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c12.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c13.gap\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c13.pp\endcsname{\ensuremath{+1.31}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c13.ppalt\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c13.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c13.z\endcsname{\ensuremath{+4.4}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c14.gap\endcsname{\ensuremath{-1.50}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c14.pp\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c14.ppalt\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c14.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c14.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c15.gap\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c15.pp\endcsname{\ensuremath{+1.93}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c15.ppalt\endcsname{\ensuremath{+2.27}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c15.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c15.z\endcsname{\ensuremath{+2.3}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c2.gap\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c2.pp\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c2.ppalt\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c2.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c2.z\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c3.gap\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c3.pp\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c3.ppalt\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c3.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c3.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c4.gap\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c4.pp\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c4.ppalt\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c4.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c4.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c5.gap\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c5.pp\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c5.ppalt\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c5.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c5.z\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c6.gap\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c6.pp\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c6.ppalt\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c6.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c6.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c7.gap\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c7.pp\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c7.ppalt\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c7.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c7.z\endcsname{\ensuremath{+3.9}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c8.gap\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c8.pp\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c8.ppalt\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c8.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c8.z\endcsname{\ensuremath{-1.1}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c9.gap\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c9.pp\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c9.ppalt\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c9.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.c9.z\endcsname{\ensuremath{+2.0}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.head_pp\endcsname{\ensuremath{+0.465}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.head_ppalt\endcsname{\ensuremath{+0.436}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.maxz\endcsname{\ensuremath{+4.4}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.maxz_class\endcsname{duodenum}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.maxz_pp\endcsname{\ensuremath{+1.31}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.nrank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.pos2list\endcsname{duodenum, stomach, prostate/uterus}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.amos.sumpos_pp\endcsname{\ensuremath{+4.07}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.c123.gap\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.c123.pp\endcsname{\ensuremath{+1.19}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.c123.ppalt\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.c123.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.c123.z\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.c2.gap\endcsname{\ensuremath{+1.70}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.c2.pp\endcsname{\ensuremath{+5.09}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.c2.ppalt\endcsname{\ensuremath{+4.80}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.c2.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.c2.z\endcsname{\ensuremath{+5.2}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.c23.gap\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.c23.pp\endcsname{\ensuremath{+4.15}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.c23.ppalt\endcsname{\ensuremath{+3.82}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.c23.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.c23.z\endcsname{\ensuremath{+4.2}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.head_pp\endcsname{\ensuremath{+3.475}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.head_ppalt\endcsname{\ensuremath{+3.232}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.maxz\endcsname{\ensuremath{+5.2}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.maxz_pp\endcsname{\ensuremath{+5.09}}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.pos2list\endcsname{tumour, masses, kidney}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.L1.fresh.kits.sumpos_pp\endcsname{\ensuremath{+10.43}}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.c123.gap\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.c123.pp\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.c123.ppalt\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.c123.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.c123.z\endcsname{\ensuremath{+2.3}}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.c2.gap\endcsname{\ensuremath{-2.08}}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.c2.pp\endcsname{\ensuremath{+2.90}}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.c2.ppalt\endcsname{\ensuremath{+2.61}}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.c2.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.c2.z\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.c23.gap\endcsname{\ensuremath{-1.29}}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.c23.pp\endcsname{\ensuremath{+3.03}}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.c23.ppalt\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.c23.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.c23.z\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.head_pp\endcsname{\ensuremath{+2.326}}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.head_ppalt\endcsname{\ensuremath{+2.082}}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.maxz\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.maxz_pp\endcsname{\ensuremath{+3.03}}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.pos2list\endcsname{masses, tumour, kidney}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1.kits.sumpos_pp\endcsname{\ensuremath{+6.98}}
\expandafter\gdef\csname R@an.perclass_all.L1.params\endcsname{102}
\expandafter\gdef\csname R@an.perclass_all.L1.params.acdc\endcsname{102}
\expandafter\gdef\csname R@an.perclass_all.L1.params.amos\endcsname{102}
\expandafter\gdef\csname R@an.perclass_all.L1.params.kits\endcsname{102}
\expandafter\gdef\csname R@an.perclass_all.L1.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.c1.gap\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.c1.pp\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.c1.ppalt\endcsname{\ensuremath{+0.97}}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.c1.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.c1.z\endcsname{\ensuremath{+5.4}}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.c2.gap\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.c2.pp\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.c2.ppalt\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.c2.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.c2.z\endcsname{\ensuremath{-0.3}}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.c3.gap\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.c3.pp\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.c3.ppalt\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.c3.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.c3.z\endcsname{\ensuremath{-0.9}}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.head_pp\endcsname{\ensuremath{+0.283}}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.head_ppalt\endcsname{\ensuremath{+0.276}}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.maxz\endcsname{\ensuremath{+5.4}}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.maxz_class\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.maxz_pp\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.nrank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.pos2list\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1b.acdc.sumpos_pp\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c1.gap\endcsname{\ensuremath{-2.45}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c1.pp\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c1.ppalt\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c1.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c1.z\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c10.gap\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c10.pp\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c10.ppalt\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c10.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c10.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c11.gap\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c11.pp\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c11.ppalt\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c11.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c11.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c12.gap\endcsname{\ensuremath{-0.94}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c12.pp\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c12.ppalt\endcsname{\ensuremath{+1.13}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c12.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c12.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c13.gap\endcsname{\ensuremath{-1.05}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c13.pp\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c13.ppalt\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c13.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c13.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c14.gap\endcsname{\ensuremath{-1.94}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c14.pp\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c14.ppalt\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c14.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c14.z\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c15.gap\endcsname{\ensuremath{-3.33}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c15.pp\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c15.ppalt\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c15.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c15.z\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c2.gap\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c2.pp\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c2.ppalt\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c2.rank\endcsname{28}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c2.z\endcsname{\ensuremath{-0.2}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c3.gap\endcsname{\ensuremath{-1.14}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c3.pp\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c3.ppalt\endcsname{\ensuremath{-0.64}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c3.rank\endcsname{36}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c3.z\endcsname{\ensuremath{-1.3}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c4.gap\endcsname{\ensuremath{-5.36}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c4.pp\endcsname{\ensuremath{-0.69}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c4.ppalt\endcsname{\ensuremath{-1.30}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c4.rank\endcsname{26}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c4.z\endcsname{\ensuremath{-0.5}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c5.gap\endcsname{\ensuremath{-0.65}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c5.pp\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c5.ppalt\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c5.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c5.z\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c6.gap\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c6.pp\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c6.ppalt\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c6.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c6.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c7.gap\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c7.pp\endcsname{\ensuremath{+0.97}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c7.ppalt\endcsname{\ensuremath{+1.06}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c7.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c7.z\endcsname{\ensuremath{+3.4}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c8.gap\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c8.pp\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c8.ppalt\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c8.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c8.z\endcsname{\ensuremath{-1.1}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c9.gap\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c9.pp\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c9.ppalt\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c9.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.c9.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.head_pp\endcsname{\ensuremath{+0.138}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.head_ppalt\endcsname{\ensuremath{+0.109}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.maxz\endcsname{\ensuremath{+3.4}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.maxz_class\endcsname{stomach}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.maxz_pp\endcsname{\ensuremath{+0.97}}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.pos2list\endcsname{stomach}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1b.amos.sumpos_pp\endcsname{\ensuremath{+0.97}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.c1.gap\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.c1.pp\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.c1.ppalt\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.c1.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.c1.z\endcsname{\ensuremath{+8.1}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.c2.gap\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.c2.pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.c2.ppalt\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.c2.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.c2.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.c3.gap\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.c3.pp\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.c3.ppalt\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.c3.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.c3.z\endcsname{\ensuremath{-2.0}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.head_pp\endcsname{\ensuremath{+0.319}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.head_ppalt\endcsname{\ensuremath{+0.312}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.maxz\endcsname{\ensuremath{+8.1}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.maxz_class\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.maxz_pp\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.nneg2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.nrank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.pos2list\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.acdc.sumpos_pp\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c1.gap\endcsname{\ensuremath{-1.33}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c1.pp\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c1.ppalt\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c1.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c1.z\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c10.gap\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c10.pp\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c10.ppalt\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c10.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c10.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c11.gap\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c11.pp\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c11.ppalt\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c11.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c11.z\endcsname{\ensuremath{+4.6}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c12.gap\endcsname{\ensuremath{-1.34}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c12.pp\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c12.ppalt\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c12.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c12.z\endcsname{\ensuremath{-0.3}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c13.gap\endcsname{\ensuremath{-0.91}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c13.pp\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c13.ppalt\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c13.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c13.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c14.gap\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c14.pp\endcsname{\ensuremath{+1.81}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c14.ppalt\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c14.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c14.z\endcsname{\ensuremath{+9.4}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c15.gap\endcsname{\ensuremath{-1.25}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c15.pp\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c15.ppalt\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c15.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c15.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c2.gap\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c2.pp\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c2.ppalt\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c2.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c2.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c3.gap\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c3.pp\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c3.ppalt\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c3.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c3.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c4.gap\endcsname{\ensuremath{-1.72}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c4.pp\endcsname{\ensuremath{-0.86}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c4.ppalt\endcsname{\ensuremath{-1.47}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c4.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c4.z\endcsname{\ensuremath{-0.9}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c5.gap\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c5.pp\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c5.ppalt\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c5.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c5.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c6.gap\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c6.pp\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c6.ppalt\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c6.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c6.z\endcsname{\ensuremath{+2.5}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c7.gap\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c7.pp\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c7.ppalt\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c7.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c7.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c8.gap\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c8.pp\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c8.ppalt\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c8.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c8.z\endcsname{\ensuremath{-0.4}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c9.gap\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c9.pp\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c9.ppalt\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c9.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.c9.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.head_pp\endcsname{\ensuremath{+0.298}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.head_ppalt\endcsname{\ensuremath{+0.269}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.maxz\endcsname{\ensuremath{+9.4}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.maxz_class\endcsname{bladder}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.maxz_pp\endcsname{\ensuremath{+1.81}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.npos2alt\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.nrank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.pos2list\endcsname{bladder, right adrenal gland, liver}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.amos.sumpos_pp\endcsname{\ensuremath{+2.67}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.c123.gap\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.c123.pp\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.c123.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.c123.z\endcsname{\ensuremath{+2.5}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.c2.gap\endcsname{\ensuremath{-2.29}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.c2.pp\endcsname{\ensuremath{+2.80}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.c2.ppalt\endcsname{\ensuremath{+2.51}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.c2.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.c2.z\endcsname{\ensuremath{+2.9}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.c23.gap\endcsname{\ensuremath{-0.89}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.c23.pp\endcsname{\ensuremath{+3.26}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.c23.ppalt\endcsname{\ensuremath{+2.93}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.c23.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.c23.z\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.head_pp\endcsname{\ensuremath{+2.313}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.head_ppalt\endcsname{\ensuremath{+2.070}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.maxz\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.maxz_pp\endcsname{\ensuremath{+3.26}}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.pos2list\endcsname{masses, tumour, kidney}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.L1b.fresh.kits.sumpos_pp\endcsname{\ensuremath{+6.94}}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.c123.gap\endcsname{\ensuremath{-1.03}}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.c123.pp\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.c123.ppalt\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.c123.rank\endcsname{30}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.c123.z\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.c2.gap\endcsname{\ensuremath{-1.96}}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.c2.pp\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.c2.ppalt\endcsname{\ensuremath{+2.73}}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.c2.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.c2.z\endcsname{\ensuremath{+2.5}}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.c23.gap\endcsname{\ensuremath{-2.30}}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.c23.pp\endcsname{\ensuremath{+2.01}}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.c23.ppalt\endcsname{\ensuremath{+1.69}}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.c23.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.c23.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.head_pp\endcsname{\ensuremath{+1.743}}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.head_ppalt\endcsname{\ensuremath{+1.499}}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.maxz\endcsname{\ensuremath{+2.5}}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.maxz_pp\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.pos2list\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L1b.kits.sumpos_pp\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@an.perclass_all.L1b.params\endcsname{102}
\expandafter\gdef\csname R@an.perclass_all.L1b.params.acdc\endcsname{102}
\expandafter\gdef\csname R@an.perclass_all.L1b.params.amos\endcsname{102}
\expandafter\gdef\csname R@an.perclass_all.L1b.params.kits\endcsname{102}
\expandafter\gdef\csname R@an.perclass_all.L1b.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.c1.gap\endcsname{\ensuremath{-1.17}}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.c1.pp\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.c1.ppalt\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.c1.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.c1.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.c2.gap\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.c2.pp\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.c2.ppalt\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.c2.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.c2.z\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.c3.gap\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.c3.pp\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.c3.ppalt\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.c3.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.c3.z\endcsname{\ensuremath{-1.9}}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.head_pp\endcsname{\ensuremath{-0.015}}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.head_ppalt\endcsname{\ensuremath{-0.022}}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.maxz\endcsname{\ensuremath{-1.9}}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.maxz_class\endcsname{LVC}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.maxz_pp\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.nneg2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.nrank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L2.acdc.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c1.gap\endcsname{\ensuremath{-2.25}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c1.pp\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c1.ppalt\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c1.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c1.z\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c10.gap\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c10.pp\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c10.ppalt\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c10.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c10.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c11.gap\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c11.pp\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c11.ppalt\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c11.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c11.z\endcsname{\ensuremath{+4.0}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c12.gap\endcsname{\ensuremath{-0.60}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c12.pp\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c12.ppalt\endcsname{\ensuremath{+1.47}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c12.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c12.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c13.gap\endcsname{\ensuremath{-0.94}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c13.pp\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c13.ppalt\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c13.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c13.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c14.gap\endcsname{\ensuremath{-1.95}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c14.pp\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c14.ppalt\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c14.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c14.z\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c15.gap\endcsname{\ensuremath{-3.44}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c15.pp\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c15.ppalt\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c15.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c15.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c2.gap\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c2.pp\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c2.ppalt\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c2.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c2.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c3.gap\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c3.pp\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c3.ppalt\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c3.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c3.z\endcsname{\ensuremath{+1.5}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c4.gap\endcsname{\ensuremath{-3.56}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c4.pp\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c4.ppalt\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c4.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c4.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c5.gap\endcsname{\ensuremath{-0.91}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c5.pp\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c5.ppalt\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c5.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c5.z\endcsname{\ensuremath{-0.3}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c6.gap\endcsname{\ensuremath{-0.62}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c6.pp\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c6.ppalt\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c6.rank\endcsname{29}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c6.z\endcsname{\ensuremath{-1.3}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c7.gap\endcsname{\ensuremath{-0.62}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c7.pp\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c7.ppalt\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c7.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c7.z\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c8.gap\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c8.pp\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c8.ppalt\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c8.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c8.z\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c9.gap\endcsname{\ensuremath{-0.89}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c9.pp\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c9.ppalt\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c9.rank\endcsname{31}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.c9.z\endcsname{\ensuremath{-0.9}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.head_pp\endcsname{\ensuremath{+0.362}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.head_ppalt\endcsname{\ensuremath{+0.333}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.maxz\endcsname{\ensuremath{+4.0}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.maxz_class\endcsname{right adrenal gland}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.maxz_pp\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.pos2list\endcsname{right adrenal gland}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L2.amos.sumpos_pp\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c1.gap\endcsname{\ensuremath{-1.38}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c1.pp\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c1.ppalt\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c1.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c1.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c10.gap\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c10.pp\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c10.ppalt\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c10.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c10.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c11.gap\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c11.pp\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c11.ppalt\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c11.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c11.z\endcsname{\ensuremath{+3.7}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c12.gap\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c12.pp\endcsname{\ensuremath{+1.16}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c12.ppalt\endcsname{\ensuremath{+1.42}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c12.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c12.z\endcsname{\ensuremath{+1.7}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c13.gap\endcsname{\ensuremath{-0.99}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c13.pp\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c13.ppalt\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c13.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c13.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c14.gap\endcsname{\ensuremath{-0.83}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c14.pp\endcsname{\ensuremath{+0.97}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c14.ppalt\endcsname{\ensuremath{+0.95}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c14.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c14.z\endcsname{\ensuremath{+5.0}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c15.gap\endcsname{\ensuremath{-2.60}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c15.pp\endcsname{\ensuremath{-0.67}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c15.ppalt\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c15.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c15.z\endcsname{\ensuremath{-0.8}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c2.gap\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c2.pp\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c2.ppalt\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c2.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c2.z\endcsname{\ensuremath{+1.5}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c3.gap\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c3.pp\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c3.ppalt\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c3.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c3.z\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c4.gap\endcsname{\ensuremath{-0.85}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c4.pp\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c4.ppalt\endcsname{\ensuremath{-0.60}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c4.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c4.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c5.gap\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c5.pp\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c5.ppalt\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c5.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c5.z\endcsname{\ensuremath{-0.5}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c6.gap\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c6.pp\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c6.ppalt\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c6.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c6.z\endcsname{\ensuremath{-0.5}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c7.gap\endcsname{\ensuremath{-0.95}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c7.pp\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c7.ppalt\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c7.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c7.z\endcsname{\ensuremath{-0.5}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c8.gap\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c8.pp\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c8.ppalt\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c8.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c8.z\endcsname{\ensuremath{-3.2}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c9.gap\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c9.pp\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c9.ppalt\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c9.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.c9.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.head_pp\endcsname{\ensuremath{+0.194}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.head_ppalt\endcsname{\ensuremath{+0.166}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.maxz\endcsname{\ensuremath{+5.0}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.maxz_class\endcsname{bladder}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.maxz_pp\endcsname{\ensuremath{+0.97}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.nneg2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.nneg2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.npos2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.nrank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.pos2list\endcsname{bladder, right adrenal gland}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.amos.sumpos_pp\endcsname{\ensuremath{+1.44}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.c123.gap\endcsname{\ensuremath{-1.50}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.c123.pp\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.c123.ppalt\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.c123.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.c123.z\endcsname{\ensuremath{-0.7}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.c2.gap\endcsname{\ensuremath{-5.11}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.c2.pp\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.c2.ppalt\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.c2.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.c2.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.c23.gap\endcsname{\ensuremath{-3.54}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.c23.pp\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.c23.ppalt\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.c23.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.c23.z\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.head_pp\endcsname{\ensuremath{+0.110}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.head_ppalt\endcsname{\ensuremath{-0.133}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.maxz\endcsname{\ensuremath{-0.7}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.maxz_class\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.maxz_pp\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.L2.fresh.kits.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.c123.gap\endcsname{\ensuremath{-0.89}}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.c123.pp\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.c123.ppalt\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.c123.rank\endcsname{29}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.c123.z\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.c2.gap\endcsname{\ensuremath{-4.71}}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.c2.pp\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.c2.ppalt\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.c2.rank\endcsname{31}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.c2.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.c23.gap\endcsname{\ensuremath{-2.93}}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.c23.pp\endcsname{\ensuremath{+1.39}}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.c23.ppalt\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.c23.rank\endcsname{30}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.c23.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.head_pp\endcsname{\ensuremath{+0.664}}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.head_ppalt\endcsname{\ensuremath{+0.420}}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.maxz\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.maxz_pp\endcsname{\ensuremath{+1.39}}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L2.kits.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.L2.params\endcsname{24.4}
\expandafter\gdef\csname R@an.perclass_all.L2.params.acdc\endcsname{23.7}
\expandafter\gdef\csname R@an.perclass_all.L2.params.amos\endcsname{24.4}
\expandafter\gdef\csname R@an.perclass_all.L2.params.kits\endcsname{24.5}
\expandafter\gdef\csname R@an.perclass_all.L2.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.c1.gap\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.c1.pp\endcsname{\ensuremath{+1.27}}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.c1.ppalt\endcsname{\ensuremath{+1.26}}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.c1.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.c1.z\endcsname{\ensuremath{+7.0}}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.c2.gap\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.c2.pp\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.c2.ppalt\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.c2.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.c2.z\endcsname{\ensuremath{+3.0}}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.c3.gap\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.c3.pp\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.c3.ppalt\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.c3.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.c3.z\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.head_pp\endcsname{\ensuremath{+0.616}}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.head_ppalt\endcsname{\ensuremath{+0.609}}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.maxz\endcsname{\ensuremath{+7.0}}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.maxz_class\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.maxz_pp\endcsname{\ensuremath{+1.27}}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.npos2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.nrank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.pos2list\endcsname{RV, MLV, LVC}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3.acdc.sumpos_pp\endcsname{\ensuremath{+1.85}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c1.gap\endcsname{\ensuremath{-2.39}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c1.pp\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c1.ppalt\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c1.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c1.z\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c10.gap\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c10.pp\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c10.ppalt\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c10.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c10.z\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c11.gap\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c11.pp\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c11.ppalt\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c11.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c11.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c12.gap\endcsname{\ensuremath{-1.49}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c12.pp\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c12.ppalt\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c12.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c12.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c13.gap\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c13.pp\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c13.ppalt\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c13.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c13.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c14.gap\endcsname{\ensuremath{-2.46}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c14.pp\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c14.ppalt\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c14.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c14.z\endcsname{\ensuremath{-1.4}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c15.gap\endcsname{\ensuremath{-2.46}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c15.pp\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c15.ppalt\endcsname{\ensuremath{+1.35}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c15.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c15.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c2.gap\endcsname{\ensuremath{-0.67}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c2.pp\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c2.ppalt\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c2.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c2.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c3.gap\endcsname{\ensuremath{-1.02}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c3.pp\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c3.ppalt\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c3.rank\endcsname{33}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c3.z\endcsname{\ensuremath{-1.0}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c4.gap\endcsname{\ensuremath{-2.94}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c4.pp\endcsname{\ensuremath{+1.73}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c4.ppalt\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c4.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c4.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c5.gap\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c5.pp\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c5.ppalt\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c5.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c5.z\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c6.gap\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c6.pp\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c6.ppalt\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c6.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c6.z\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c7.gap\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c7.pp\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c7.ppalt\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c7.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c7.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c8.gap\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c8.pp\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c8.ppalt\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c8.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c8.z\endcsname{\ensuremath{-0.3}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c9.gap\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c9.pp\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c9.ppalt\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c9.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.c9.z\endcsname{\ensuremath{+3.9}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.head_pp\endcsname{\ensuremath{+0.382}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.head_ppalt\endcsname{\ensuremath{+0.353}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.maxz\endcsname{\ensuremath{+3.9}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.maxz_class\endcsname{postcava}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.maxz_pp\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.nearest\endcsname{branch control}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.nearest.sentence\endcsname{Organ profiles on AMOS22 do not sort by role: HyReX's nearest profile is the branch control ($r$~=~\ensuremath{+0.75}), a never-selected control, ahead of the nearest agent-designed arm, HyReX with LeanDec fine decoder stages ($r$~=~\ensuremath{+0.68}), by 0.07}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.nearest.state\endcsname{other}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.nearest2\endcsname{HyReX with LeanDec fine decoder stages}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.nearest2_r\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.nearest_agent\endcsname{HyReX with LeanDec fine decoder stages}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.nearest_agent_r\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.nearest_agentmade\endcsname{no}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.nearest_margin\endcsname{0.07}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.nearest_other\endcsname{branch control}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.nearest_other_r\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.nearest_other_tag\endcsname{W1c}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.nearest_r\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.nearest_role\endcsname{control}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.nearest_tag\endcsname{W1c}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.npos2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.pos2list\endcsname{postcava, liver, pancreas}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.C1\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.D1\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.D2\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.I1\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.L1\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.L1b\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.L2\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.L3k3\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.L3ng\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.L4\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.L6\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.N1\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.P3c\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.S2\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.V5A5\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.V5B1\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.V5B2\endcsname{\ensuremath{-0.58}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.V6A1r\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.V7A1\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.V7A2\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.V7A3\endcsname{\ensuremath{-0.41}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.V7B1\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.V7B2\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.V7C1\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.V7C2\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.V8A1\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.V8A2\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.V8B1\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.V8B2\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.V8X1\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.W1\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.W1c\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.W2\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.W3\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.W3c\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.W4\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.r.W5\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.C1\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.D1\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.D2\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.I1\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.L1\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.L1b\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.L2\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.L3k3\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.L3ng\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.L4\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.L6\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.N1\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.P3c\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.S2\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.V5A5\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.V5B1\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.V5B2\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.V6A1r\endcsname{\ensuremath{+0.84}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.V7A1\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.V7A2\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.V7A3\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.V7B1\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.V7B2\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.V7C1\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.V7C2\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.V8A1\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.V8A2\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.V8B1\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.V8B2\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.V8X1\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.W1\endcsname{\ensuremath{+0.79}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.W1c\endcsname{\ensuremath{+0.91}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.W2\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.W3\endcsname{\ensuremath{+0.79}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.W3c\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.W4\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rhi.W5\endcsname{\ensuremath{+0.72}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.C1\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.D1\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.D2\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.I1\endcsname{\ensuremath{-0.54}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.L1\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.L1b\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.L2\endcsname{\ensuremath{-0.68}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.L3k3\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.L3ng\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.L4\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.L6\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.N1\endcsname{\ensuremath{-0.81}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.P3c\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.S2\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.V5A5\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.V5B1\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.V5B2\endcsname{\ensuremath{-0.84}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.V6A1r\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.V7A1\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.V7A2\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.V7A3\endcsname{\ensuremath{-0.76}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.V7B1\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.V7B2\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.V7C1\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.V7C2\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.V8A1\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.V8A2\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.V8B1\endcsname{\ensuremath{-0.81}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.V8B2\endcsname{\ensuremath{-0.62}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.V8X1\endcsname{\ensuremath{-0.55}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.W1\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.W1c\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.W2\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.W3\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.W3c\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.W4\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.rlo.W5\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3.amos.sumpos_pp\endcsname{\ensuremath{+1.71}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.c1.gap\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.c1.pp\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.c1.ppalt\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.c1.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.c1.z\endcsname{\ensuremath{+8.0}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.c2.gap\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.c2.pp\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.c2.ppalt\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.c2.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.c2.z\endcsname{\ensuremath{+3.5}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.c3.gap\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.c3.pp\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.c3.ppalt\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.c3.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.c3.z\endcsname{\ensuremath{-0.9}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.head_pp\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.head_ppalt\endcsname{\ensuremath{+0.443}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.maxz\endcsname{\ensuremath{+8.0}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.maxz_class\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.maxz_pp\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.npos2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.npos2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.nrank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.pos2list\endcsname{RV, MLV}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.acdc.sumpos_pp\endcsname{\ensuremath{+1.42}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c1.gap\endcsname{\ensuremath{-1.43}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c1.pp\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c1.ppalt\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c1.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c1.z\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c10.gap\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c10.pp\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c10.ppalt\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c10.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c10.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c11.gap\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c11.pp\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c11.ppalt\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c11.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c11.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c12.gap\endcsname{\ensuremath{-0.94}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c12.pp\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c12.ppalt\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c12.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c12.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c13.gap\endcsname{\ensuremath{-0.94}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c13.pp\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c13.ppalt\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c13.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c13.z\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c14.gap\endcsname{\ensuremath{-2.13}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c14.pp\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c14.ppalt\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c14.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c14.z\endcsname{\ensuremath{-1.7}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c15.gap\endcsname{\ensuremath{-1.95}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c15.pp\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c15.ppalt\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c15.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c15.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c2.gap\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c2.pp\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c2.ppalt\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c2.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c2.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c3.gap\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c3.pp\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c3.ppalt\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c3.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c3.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c4.gap\endcsname{\ensuremath{-1.37}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c4.pp\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c4.ppalt\endcsname{\ensuremath{-1.12}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c4.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c4.z\endcsname{\ensuremath{-0.5}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c5.gap\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c5.pp\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c5.ppalt\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c5.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c5.z\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c6.gap\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c6.pp\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c6.ppalt\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c6.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c6.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c7.gap\endcsname{\ensuremath{-0.65}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c7.pp\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c7.ppalt\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c7.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c7.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c8.gap\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c8.pp\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c8.ppalt\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c8.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c8.z\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c9.gap\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c9.pp\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c9.ppalt\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c9.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.c9.z\endcsname{\ensuremath{+4.1}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.head_pp\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.head_ppalt\endcsname{\ensuremath{+0.104}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.maxz\endcsname{\ensuremath{+4.1}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.maxz_class\endcsname{postcava}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.maxz_pp\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.nrank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.pos2list\endcsname{postcava}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.amos.sumpos_pp\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.c123.gap\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.c123.pp\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.c123.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.c123.z\endcsname{\ensuremath{+2.6}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.c2.gap\endcsname{\ensuremath{-2.76}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.c2.pp\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.c2.ppalt\endcsname{\ensuremath{+2.04}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.c2.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.c2.z\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.c23.gap\endcsname{\ensuremath{-1.13}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.c23.pp\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.c23.ppalt\endcsname{\ensuremath{+2.70}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.c23.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.c23.z\endcsname{\ensuremath{+3.1}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.head_pp\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.head_ppalt\endcsname{\ensuremath{+1.850}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.maxz\endcsname{\ensuremath{+3.1}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.maxz_pp\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.pos2list\endcsname{masses, kidney, tumour}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.L3.fresh.kits.sumpos_pp\endcsname{\ensuremath{+6.28}}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.c123.gap\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.c123.pp\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.c123.ppalt\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.c123.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.c123.z\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.c2.gap\endcsname{\ensuremath{-0.87}}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.c2.pp\endcsname{\ensuremath{+4.11}}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.c2.ppalt\endcsname{\ensuremath{+3.82}}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.c2.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.c2.z\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.c23.gap\endcsname{\ensuremath{-0.83}}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.c23.pp\endcsname{\ensuremath{+3.49}}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.c23.ppalt\endcsname{\ensuremath{+3.17}}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.c23.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.c23.z\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.head_pp\endcsname{\ensuremath{+2.842}}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.head_ppalt\endcsname{\ensuremath{+2.598}}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.maxz\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.maxz_pp\endcsname{\ensuremath{+4.11}}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.npos2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.pos2list\endcsname{tumour, masses, kidney}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3.kits.sumpos_pp\endcsname{\ensuremath{+8.53}}
\expandafter\gdef\csname R@an.perclass_all.L3.params\endcsname{29.6}
\expandafter\gdef\csname R@an.perclass_all.L3.params.acdc\endcsname{28.8}
\expandafter\gdef\csname R@an.perclass_all.L3.params.amos\endcsname{29.6}
\expandafter\gdef\csname R@an.perclass_all.L3.params.kits\endcsname{29.7}
\expandafter\gdef\csname R@an.perclass_all.L3.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c1.gap\endcsname{\ensuremath{-2.21}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c1.pp\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c1.ppalt\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c1.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c1.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c10.gap\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c10.pp\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c10.ppalt\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c10.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c10.z\endcsname{\ensuremath{+2.5}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c11.gap\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c11.pp\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c11.ppalt\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c11.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c11.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c12.gap\endcsname{\ensuremath{-0.79}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c12.pp\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c12.ppalt\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c12.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c12.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c13.gap\endcsname{\ensuremath{-1.16}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c13.pp\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c13.ppalt\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c13.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c13.z\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c14.gap\endcsname{\ensuremath{-2.68}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c14.pp\endcsname{\ensuremath{-0.58}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c14.ppalt\endcsname{\ensuremath{-0.60}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c14.rank\endcsname{27}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c14.z\endcsname{\ensuremath{-2.3}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c15.gap\endcsname{\ensuremath{-4.32}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c15.pp\endcsname{\ensuremath{-0.85}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c15.ppalt\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c15.rank\endcsname{36}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c15.z\endcsname{\ensuremath{-0.8}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c2.gap\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c2.pp\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c2.ppalt\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c2.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c2.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c3.gap\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c3.pp\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c3.ppalt\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c3.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c3.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c4.gap\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c4.pp\endcsname{\ensuremath{+4.67}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c4.ppalt\endcsname{\ensuremath{+4.06}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c4.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c4.z\endcsname{\ensuremath{+3.5}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c5.gap\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c5.pp\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c5.ppalt\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c5.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c5.z\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c6.gap\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c6.pp\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c6.ppalt\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c6.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c6.z\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c7.gap\endcsname{\ensuremath{-1.24}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c7.pp\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c7.ppalt\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c7.rank\endcsname{30}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c7.z\endcsname{\ensuremath{-1.0}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c8.gap\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c8.pp\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c8.ppalt\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c8.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c8.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c9.gap\endcsname{\ensuremath{-0.68}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c9.pp\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c9.ppalt\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c9.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.c9.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.head_pp\endcsname{\ensuremath{+0.459}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.head_ppalt\endcsname{\ensuremath{+0.430}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.maxz\endcsname{\ensuremath{+3.5}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.maxz_class\endcsname{gall bladder}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.maxz_pp\endcsname{\ensuremath{+4.67}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.nneg2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.nneg2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.npos2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.pos2list\endcsname{gall bladder, pancreas}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3k3.amos.sumpos_pp\endcsname{\ensuremath{+5.69}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.c123.gap\endcsname{\ensuremath{-0.72}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.c123.pp\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.c123.ppalt\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.c123.rank\endcsname{28}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.c123.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.c2.gap\endcsname{\ensuremath{-3.14}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.c2.pp\endcsname{\ensuremath{+1.84}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.c2.ppalt\endcsname{\ensuremath{+1.55}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.c2.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.c2.z\endcsname{\ensuremath{+1.5}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.c23.gap\endcsname{\ensuremath{-2.56}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.c23.pp\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.c23.ppalt\endcsname{\ensuremath{+1.43}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.c23.rank\endcsname{27}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.c23.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.head_pp\endcsname{\ensuremath{+1.366}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.head_ppalt\endcsname{\ensuremath{+1.123}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.maxz\endcsname{\ensuremath{+1.5}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.maxz_pp\endcsname{\ensuremath{+1.84}}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3k3.kits.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.L3k3.params\endcsname{28.6}
\expandafter\gdef\csname R@an.perclass_all.L3k3.params.acdc\endcsname{27.8}
\expandafter\gdef\csname R@an.perclass_all.L3k3.params.amos\endcsname{28.6}
\expandafter\gdef\csname R@an.perclass_all.L3k3.params.kits\endcsname{28.7}
\expandafter\gdef\csname R@an.perclass_all.L3k3.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c1.gap\endcsname{\ensuremath{-2.34}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c1.pp\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c1.ppalt\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c1.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c1.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c10.gap\endcsname{\ensuremath{-0.78}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c10.pp\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c10.ppalt\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c10.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c10.z\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c11.gap\endcsname{\ensuremath{-1.17}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c11.pp\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c11.ppalt\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c11.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c11.z\endcsname{\ensuremath{-1.4}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c12.gap\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c12.pp\endcsname{\ensuremath{+1.35}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c12.ppalt\endcsname{\ensuremath{+1.60}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c12.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c12.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c13.gap\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c13.pp\endcsname{\ensuremath{+0.89}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c13.ppalt\endcsname{\ensuremath{+0.95}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c13.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c13.z\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c14.gap\endcsname{\ensuremath{-2.54}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c14.pp\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c14.ppalt\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c14.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c14.z\endcsname{\ensuremath{-1.7}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c15.gap\endcsname{\ensuremath{-4.43}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c15.pp\endcsname{\ensuremath{-0.95}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c15.ppalt\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c15.rank\endcsname{37}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c15.z\endcsname{\ensuremath{-0.9}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c2.gap\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c2.pp\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c2.ppalt\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c2.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c2.z\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c3.gap\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c3.pp\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c3.ppalt\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c3.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c3.z\endcsname{\ensuremath{+1.5}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c4.gap\endcsname{\ensuremath{-2.40}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c4.pp\endcsname{\ensuremath{+2.27}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c4.ppalt\endcsname{\ensuremath{+1.66}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c4.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c4.z\endcsname{\ensuremath{+1.7}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c5.gap\endcsname{\ensuremath{-1.03}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c5.pp\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c5.ppalt\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c5.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c5.z\endcsname{\ensuremath{-0.7}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c6.gap\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c6.pp\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c6.ppalt\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c6.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c6.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c7.gap\endcsname{\ensuremath{-0.69}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c7.pp\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c7.ppalt\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c7.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c7.z\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c8.gap\endcsname{\ensuremath{-0.41}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c8.pp\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c8.ppalt\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c8.rank\endcsname{29}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c8.z\endcsname{\ensuremath{-2.2}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c9.gap\endcsname{\ensuremath{-1.00}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c9.pp\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c9.ppalt\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c9.rank\endcsname{35}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.c9.z\endcsname{\ensuremath{-1.8}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.head_pp\endcsname{\ensuremath{+0.268}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.head_ppalt\endcsname{\ensuremath{+0.239}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.maxz\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.maxz_class\endcsname{duodenum}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.maxz_pp\endcsname{\ensuremath{+0.89}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.nneg2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.nneg2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.pos2list\endcsname{duodenum}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3ng.amos.sumpos_pp\endcsname{\ensuremath{+0.89}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.c123.gap\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.c123.pp\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.c123.ppalt\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.c123.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.c123.z\endcsname{\ensuremath{+2.5}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.c2.gap\endcsname{\ensuremath{-1.86}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.c2.pp\endcsname{\ensuremath{+3.12}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.c2.ppalt\endcsname{\ensuremath{+2.83}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.c2.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.c2.z\endcsname{\ensuremath{+2.5}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.c23.gap\endcsname{\ensuremath{-0.90}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.c23.pp\endcsname{\ensuremath{+3.42}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.c23.ppalt\endcsname{\ensuremath{+3.10}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.c23.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.c23.z\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.head_pp\endcsname{\ensuremath{+2.561}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.head_ppalt\endcsname{\ensuremath{+2.317}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.maxz\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.maxz_pp\endcsname{\ensuremath{+3.42}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.pos2list\endcsname{masses, tumour, kidney}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L3ng.kits.sumpos_pp\endcsname{\ensuremath{+7.68}}
\expandafter\gdef\csname R@an.perclass_all.L3ng.params\endcsname{29.6}
\expandafter\gdef\csname R@an.perclass_all.L3ng.params.acdc\endcsname{28.8}
\expandafter\gdef\csname R@an.perclass_all.L3ng.params.amos\endcsname{29.6}
\expandafter\gdef\csname R@an.perclass_all.L3ng.params.kits\endcsname{29.6}
\expandafter\gdef\csname R@an.perclass_all.L3ng.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.altflip\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c1.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c1.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c1.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c1.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c1.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c10.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c10.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c10.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c10.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c10.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c11.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c11.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c11.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c11.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c11.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c12.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c12.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c12.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c12.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c12.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c13.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c13.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c13.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c13.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c13.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c14.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c14.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c14.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c14.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c14.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c15.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c15.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c15.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c15.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c15.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c2.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c2.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c2.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c2.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c2.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c3.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c3.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c3.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c3.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c3.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c4.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c4.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c4.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c4.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c4.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c5.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c5.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c5.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c5.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c5.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c6.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c6.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c6.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c6.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c6.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c7.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c7.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c7.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c7.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c7.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c8.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c8.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c8.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c8.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c8.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c9.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c9.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c9.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c9.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.c9.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.head_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.head_ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.maxz\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.maxz_class\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.maxz_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.nneg2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.nneg2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.npos2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.npos2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.nrank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.nseed\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.pos2list\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.regstate\endcsname{queued}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.seedlist\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.amos.sumpos_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.altflip\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.c123.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.c123.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.c123.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.c123.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.c123.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.c2.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.c2.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.c2.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.c2.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.c2.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.c23.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.c23.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.c23.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.c23.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.c23.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.head_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.head_ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.maxz\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.maxz_class\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.maxz_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.nneg2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.nneg2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.npos2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.npos2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.nrank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.nseed\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.pos2list\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.regstate\endcsname{queued}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.seedlist\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.kits.sumpos_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.params\endcsname{99.8}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.params.acdc\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.params.amos\endcsname{99.8}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.params.kits\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_L.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.altflip\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c1.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c1.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c1.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c1.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c1.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c10.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c10.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c10.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c10.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c10.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c11.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c11.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c11.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c11.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c11.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c12.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c12.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c12.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c12.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c12.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c13.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c13.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c13.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c13.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c13.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c14.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c14.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c14.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c14.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c14.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c15.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c15.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c15.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c15.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c15.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c2.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c2.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c2.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c2.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c2.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c3.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c3.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c3.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c3.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c3.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c4.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c4.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c4.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c4.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c4.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c5.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c5.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c5.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c5.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c5.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c6.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c6.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c6.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c6.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c6.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c7.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c7.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c7.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c7.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c7.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c8.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c8.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c8.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c8.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c8.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c9.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c9.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c9.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c9.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.c9.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.head_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.head_ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.maxz\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.maxz_class\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.maxz_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.nneg2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.nneg2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.npos2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.npos2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.nrank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.nseed\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.pos2list\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.regstate\endcsname{queued}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.seedlist\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.amos.sumpos_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.altflip\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.c123.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.c123.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.c123.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.c123.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.c123.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.c2.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.c2.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.c2.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.c2.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.c2.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.c23.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.c23.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.c23.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.c23.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.c23.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.head_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.head_ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.maxz\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.maxz_class\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.maxz_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.nneg2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.nneg2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.npos2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.npos2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.nrank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.nseed\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.pos2list\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.regstate\endcsname{queued}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.seedlist\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.kits.sumpos_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.params\endcsname{59.0}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.params.acdc\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.params.amos\endcsname{59.0}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.params.kits\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.L3w_M.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.c1.gap\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.c1.pp\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.c1.ppalt\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.c1.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.c1.z\endcsname{\ensuremath{+4.2}}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.c2.gap\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.c2.pp\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.c2.ppalt\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.c2.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.c2.z\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.c3.gap\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.c3.pp\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.c3.ppalt\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.c3.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.c3.z\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.head_pp\endcsname{\ensuremath{+0.315}}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.head_ppalt\endcsname{\ensuremath{+0.308}}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.maxz\endcsname{\ensuremath{+4.2}}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.maxz_class\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.maxz_pp\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.nrank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.pos2list\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L4.acdc.sumpos_pp\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c1.gap\endcsname{\ensuremath{-2.31}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c1.pp\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c1.ppalt\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c1.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c1.z\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c10.gap\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c10.pp\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c10.ppalt\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c10.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c10.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c11.gap\endcsname{\ensuremath{-0.68}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c11.pp\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c11.ppalt\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c11.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c11.z\endcsname{\ensuremath{+1.5}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c12.gap\endcsname{\ensuremath{-1.43}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c12.pp\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c12.ppalt\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c12.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c12.z\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c13.gap\endcsname{\ensuremath{-0.88}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c13.pp\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c13.ppalt\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c13.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c13.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c14.gap\endcsname{\ensuremath{-1.52}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c14.pp\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c14.ppalt\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c14.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c14.z\endcsname{\ensuremath{+2.3}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c15.gap\endcsname{\ensuremath{-1.11}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c15.pp\endcsname{\ensuremath{+2.37}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c15.ppalt\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c15.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c15.z\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c2.gap\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c2.pp\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c2.ppalt\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c2.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c2.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c3.gap\endcsname{\ensuremath{-0.72}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c3.pp\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c3.ppalt\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c3.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c3.z\endcsname{\ensuremath{-0.2}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c4.gap\endcsname{\ensuremath{-4.38}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c4.pp\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c4.ppalt\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c4.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c4.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c5.gap\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c5.pp\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c5.ppalt\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c5.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c5.z\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c6.gap\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c6.pp\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c6.ppalt\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c6.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c6.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c7.gap\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c7.pp\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c7.ppalt\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c7.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c7.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c8.gap\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c8.pp\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c8.ppalt\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c8.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c8.z\endcsname{\ensuremath{-0.8}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c9.gap\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c9.pp\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c9.ppalt\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c9.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.c9.z\endcsname{\ensuremath{+3.4}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.head_pp\endcsname{\ensuremath{+0.430}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.head_ppalt\endcsname{\ensuremath{+0.401}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.maxz\endcsname{\ensuremath{+3.4}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.maxz_class\endcsname{postcava}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.maxz_pp\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.npos2\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.npos2alt\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.pos2list\endcsname{postcava, bladder, prostate/uterus, esophagus}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L4.amos.sumpos_pp\endcsname{\ensuremath{+4.04}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.altflip\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c1.gap\endcsname{\ensuremath{+1.22}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c1.pp\endcsname{\ensuremath{+1.44}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c1.ppalt\endcsname{\ensuremath{+1.38}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c1.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c1.z\endcsname{\ensuremath{+6.6}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c10.gap\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c10.pp\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c10.ppalt\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c10.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c10.z\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c11.gap\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c11.pp\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c11.ppalt\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c11.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c11.z\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c12.gap\endcsname{\ensuremath{-0.58}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c12.pp\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c12.ppalt\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c12.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c12.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c13.gap\endcsname{\ensuremath{-0.73}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c13.pp\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c13.ppalt\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c13.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c13.z\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c14.gap\endcsname{\ensuremath{-1.48}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c14.pp\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c14.ppalt\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c14.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c14.z\endcsname{\ensuremath{+1.7}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c15.gap\endcsname{\ensuremath{-0.96}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c15.pp\endcsname{\ensuremath{+0.97}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c15.ppalt\endcsname{\ensuremath{+1.31}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c15.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c15.z\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c2.gap\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c2.pp\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c2.ppalt\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c2.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c2.z\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c3.gap\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c3.pp\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c3.ppalt\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c3.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c3.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c4.gap\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c4.pp\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c4.ppalt\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c4.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c4.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c5.gap\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c5.pp\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c5.ppalt\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c5.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c5.z\endcsname{\ensuremath{+1.5}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c6.gap\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c6.pp\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c6.ppalt\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c6.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c6.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c7.gap\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c7.pp\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c7.ppalt\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c7.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c7.z\endcsname{\ensuremath{+2.3}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c8.gap\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c8.pp\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c8.ppalt\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c8.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c8.z\endcsname{\ensuremath{-0.7}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c9.gap\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c9.pp\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c9.ppalt\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c9.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.c9.z\endcsname{\ensuremath{+2.6}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.head_pp\endcsname{\ensuremath{+0.455}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.head_ppalt\endcsname{\ensuremath{+0.426}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.maxz\endcsname{\ensuremath{+6.6}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.maxz_class\endcsname{spleen}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.maxz_pp\endcsname{\ensuremath{+1.44}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.npos2\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.npos2alt\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.nrank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.pos2list\endcsname{spleen, postcava, stomach, right adrenal gland}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.amos.sumpos_pp\endcsname{\ensuremath{+2.46}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.c123.gap\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.c123.pp\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.c123.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.c123.z\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.c2.gap\endcsname{\ensuremath{-1.95}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.c2.pp\endcsname{\ensuremath{+3.14}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.c2.ppalt\endcsname{\ensuremath{+2.85}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.c2.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.c2.z\endcsname{\ensuremath{+3.2}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.c23.gap\endcsname{\ensuremath{-1.41}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.c23.pp\endcsname{\ensuremath{+2.73}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.c23.ppalt\endcsname{\ensuremath{+2.41}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.c23.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.c23.z\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.head_pp\endcsname{\ensuremath{+2.246}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.head_ppalt\endcsname{\ensuremath{+2.003}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.maxz\endcsname{\ensuremath{+3.2}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.maxz_pp\endcsname{\ensuremath{+3.14}}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.pos2list\endcsname{tumour, masses, kidney}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.L4.fresh.kits.sumpos_pp\endcsname{\ensuremath{+6.74}}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.c123.gap\endcsname{\ensuremath{-0.55}}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.c123.pp\endcsname{\ensuremath{+0.67}}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.c123.ppalt\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.c123.rank\endcsname{26}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.c123.z\endcsname{\ensuremath{+1.5}}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.c2.gap\endcsname{\ensuremath{-1.48}}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.c2.pp\endcsname{\ensuremath{+3.50}}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.c2.ppalt\endcsname{\ensuremath{+3.21}}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.c2.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.c2.z\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.c23.gap\endcsname{\ensuremath{-1.90}}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.c23.pp\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.c23.ppalt\endcsname{\ensuremath{+2.10}}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.c23.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.c23.z\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.head_pp\endcsname{\ensuremath{+2.198}}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.head_ppalt\endcsname{\ensuremath{+1.954}}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.maxz\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.maxz_pp\endcsname{\ensuremath{+3.50}}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.pos2list\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L4.kits.sumpos_pp\endcsname{\ensuremath{+3.50}}
\expandafter\gdef\csname R@an.perclass_all.L4.params\endcsname{103}
\expandafter\gdef\csname R@an.perclass_all.L4.params.acdc\endcsname{102}
\expandafter\gdef\csname R@an.perclass_all.L4.params.amos\endcsname{103}
\expandafter\gdef\csname R@an.perclass_all.L4.params.kits\endcsname{103}
\expandafter\gdef\csname R@an.perclass_all.L4.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.c1.gap\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.c1.pp\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.c1.ppalt\endcsname{\ensuremath{+1.13}}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.c1.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.c1.z\endcsname{\ensuremath{+6.3}}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.c2.gap\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.c2.pp\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.c2.ppalt\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.c2.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.c2.z\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.c3.gap\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.c3.pp\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.c3.ppalt\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.c3.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.c3.z\endcsname{\ensuremath{-0.4}}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.head_pp\endcsname{\ensuremath{+0.451}}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.head_ppalt\endcsname{\ensuremath{+0.444}}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.maxz\endcsname{\ensuremath{+6.3}}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.maxz_class\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.maxz_pp\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.npos2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.npos2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.nrank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.pos2list\endcsname{RV, MLV}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L6.acdc.sumpos_pp\endcsname{\ensuremath{+1.39}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.altflip\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c1.gap\endcsname{\ensuremath{-2.37}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c1.pp\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c1.ppalt\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c1.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c1.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c10.gap\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c10.pp\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c10.ppalt\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c10.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c10.z\endcsname{\ensuremath{+2.0}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c11.gap\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c11.pp\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c11.ppalt\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c11.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c11.z\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c12.gap\endcsname{\ensuremath{-1.07}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c12.pp\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c12.ppalt\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c12.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c12.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c13.gap\endcsname{\ensuremath{-0.95}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c13.pp\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c13.ppalt\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c13.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c13.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c14.gap\endcsname{\ensuremath{-3.00}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c14.pp\endcsname{\ensuremath{-0.89}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c14.ppalt\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c14.rank\endcsname{30}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c14.z\endcsname{\ensuremath{-3.5}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c15.gap\endcsname{\ensuremath{-4.19}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c15.pp\endcsname{\ensuremath{-0.71}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c15.ppalt\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c15.rank\endcsname{35}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c15.z\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c2.gap\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c2.pp\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c2.ppalt\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c2.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c2.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c3.gap\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c3.pp\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c3.ppalt\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c3.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c3.z\endcsname{\ensuremath{+1.7}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c4.gap\endcsname{\ensuremath{-6.91}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c4.pp\endcsname{\ensuremath{-2.25}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c4.ppalt\endcsname{\ensuremath{-2.86}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c4.rank\endcsname{34}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c4.z\endcsname{\ensuremath{-1.7}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c5.gap\endcsname{\ensuremath{-0.83}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c5.pp\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c5.ppalt\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c5.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c5.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c6.gap\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c6.pp\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c6.ppalt\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c6.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c6.z\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c7.gap\endcsname{\ensuremath{-1.26}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c7.pp\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c7.ppalt\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c7.rank\endcsname{31}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c7.z\endcsname{\ensuremath{-1.0}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c8.gap\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c8.pp\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c8.ppalt\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c8.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c8.z\endcsname{\ensuremath{-0.4}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c9.gap\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c9.pp\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c9.ppalt\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c9.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.c9.z\endcsname{\ensuremath{+3.4}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.head_pp\endcsname{\ensuremath{+0.016}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.head_ppalt\endcsname{\ensuremath{-0.013}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.maxz\endcsname{\ensuremath{-3.5}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.maxz_class\endcsname{bladder}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.maxz_pp\endcsname{\ensuremath{-0.89}}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.nneg2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.nneg2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.npos2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.pos2list\endcsname{postcava, right adrenal gland, pancreas}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L6.amos.sumpos_pp\endcsname{\ensuremath{+1.60}}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.c123.gap\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.c123.pp\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.c123.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.c123.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.c2.gap\endcsname{\ensuremath{-2.68}}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.c2.pp\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.c2.ppalt\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.c2.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.c2.z\endcsname{\ensuremath{+2.5}}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.c23.gap\endcsname{\ensuremath{-2.42}}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.c23.pp\endcsname{\ensuremath{+1.72}}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.c23.ppalt\endcsname{\ensuremath{+1.40}}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.c23.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.c23.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.head_pp\endcsname{\ensuremath{+1.591}}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.head_ppalt\endcsname{\ensuremath{+1.348}}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.maxz\endcsname{\ensuremath{+2.5}}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.maxz_pp\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.pos2list\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.L6.fresh.kits.sumpos_pp\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.altflip\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.c123.gap\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.c123.pp\endcsname{\ensuremath{+0.95}}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.c123.ppalt\endcsname{\ensuremath{+0.84}}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.c123.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.c123.z\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.c2.gap\endcsname{\ensuremath{-1.08}}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.c2.pp\endcsname{\ensuremath{+3.90}}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.c2.ppalt\endcsname{\ensuremath{+3.61}}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.c2.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.c2.z\endcsname{\ensuremath{+3.2}}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.c23.gap\endcsname{\ensuremath{-1.59}}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.c23.pp\endcsname{\ensuremath{+2.73}}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.c23.ppalt\endcsname{\ensuremath{+2.41}}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.c23.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.c23.z\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.head_pp\endcsname{\ensuremath{+2.526}}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.head_ppalt\endcsname{\ensuremath{+2.283}}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.maxz\endcsname{\ensuremath{+3.2}}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.maxz_pp\endcsname{\ensuremath{+3.90}}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.pos2list\endcsname{tumour, masses, kidney}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.L6.kits.sumpos_pp\endcsname{\ensuremath{+7.58}}
\expandafter\gdef\csname R@an.perclass_all.L6.params\endcsname{31.1}
\expandafter\gdef\csname R@an.perclass_all.L6.params.acdc\endcsname{30.3}
\expandafter\gdef\csname R@an.perclass_all.L6.params.amos\endcsname{31.1}
\expandafter\gdef\csname R@an.perclass_all.L6.params.kits\endcsname{31.2}
\expandafter\gdef\csname R@an.perclass_all.L6.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c1.gap\endcsname{\ensuremath{-3.18}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c1.pp\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c1.ppalt\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c1.rank\endcsname{31}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c1.z\endcsname{\ensuremath{-2.0}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c10.gap\endcsname{\ensuremath{-1.96}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c10.pp\endcsname{\ensuremath{-0.93}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c10.ppalt\endcsname{\ensuremath{-1.17}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c10.rank\endcsname{37}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c10.z\endcsname{\ensuremath{-2.3}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c11.gap\endcsname{\ensuremath{-1.90}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c11.pp\endcsname{\ensuremath{-0.97}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c11.ppalt\endcsname{\ensuremath{-0.97}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c11.rank\endcsname{35}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c11.z\endcsname{\ensuremath{-5.8}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c12.gap\endcsname{\ensuremath{-2.61}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c12.pp\endcsname{\ensuremath{-0.81}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c12.ppalt\endcsname{\ensuremath{-0.55}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c12.rank\endcsname{34}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c12.z\endcsname{\ensuremath{-0.9}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c13.gap\endcsname{\ensuremath{-2.73}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c13.pp\endcsname{\ensuremath{-1.34}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c13.ppalt\endcsname{\ensuremath{-1.28}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c13.rank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c13.z\endcsname{\ensuremath{-3.4}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c14.gap\endcsname{\ensuremath{-1.14}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c14.pp\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c14.ppalt\endcsname{\ensuremath{+0.94}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c14.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c14.z\endcsname{\ensuremath{+3.8}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c15.gap\endcsname{\ensuremath{-4.77}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c15.pp\endcsname{\ensuremath{-1.30}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c15.ppalt\endcsname{\ensuremath{-0.96}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c15.rank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c15.z\endcsname{\ensuremath{-1.2}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c2.gap\endcsname{\ensuremath{-2.13}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c2.pp\endcsname{\ensuremath{-1.48}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c2.ppalt\endcsname{\ensuremath{-1.72}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c2.rank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c2.z\endcsname{\ensuremath{-3.3}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c3.gap\endcsname{\ensuremath{-1.10}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c3.pp\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c3.ppalt\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c3.rank\endcsname{35}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c3.z\endcsname{\ensuremath{-1.2}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c4.gap\endcsname{\ensuremath{-8.77}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c4.pp\endcsname{\ensuremath{-4.11}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c4.ppalt\endcsname{\ensuremath{-4.71}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c4.rank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c4.z\endcsname{\ensuremath{-3.1}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c5.gap\endcsname{\ensuremath{-2.13}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c5.pp\endcsname{\ensuremath{-1.32}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c5.ppalt\endcsname{\ensuremath{-1.06}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c5.rank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c5.z\endcsname{\ensuremath{-4.2}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c6.gap\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c6.pp\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c6.ppalt\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c6.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c6.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c7.gap\endcsname{\ensuremath{-1.53}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c7.pp\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c7.ppalt\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c7.rank\endcsname{37}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c7.z\endcsname{\ensuremath{-2.0}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c8.gap\endcsname{\ensuremath{-0.54}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c8.pp\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c8.ppalt\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c8.rank\endcsname{37}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c8.z\endcsname{\ensuremath{-3.2}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c9.gap\endcsname{\ensuremath{-1.42}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c9.pp\endcsname{\ensuremath{-0.64}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c9.ppalt\endcsname{\ensuremath{-0.71}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c9.rank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.c9.z\endcsname{\ensuremath{-5.1}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.head_pp\endcsname{\ensuremath{-0.923}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.head_ppalt\endcsname{\ensuremath{-0.952}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.maxz\endcsname{\ensuremath{-5.8}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.maxz_class\endcsname{right adrenal gland}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.maxz_pp\endcsname{\ensuremath{-0.97}}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.nneg2\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.nneg2alt\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.pos2list\endcsname{bladder}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.N1.amos.sumpos_pp\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.c123.gap\endcsname{\ensuremath{-5.54}}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.c123.pp\endcsname{\ensuremath{-4.31}}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.c123.ppalt\endcsname{\ensuremath{-4.43}}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.c123.rank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.c123.z\endcsname{\ensuremath{-9.6}}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.c2.gap\endcsname{\ensuremath{-13.58}}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.c2.pp\endcsname{\ensuremath{-8.59}}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.c2.ppalt\endcsname{\ensuremath{-8.89}}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.c2.rank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.c2.z\endcsname{\ensuremath{-7.0}}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.c23.gap\endcsname{\ensuremath{-10.89}}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.c23.pp\endcsname{\ensuremath{-6.57}}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.c23.ppalt\endcsname{\ensuremath{-6.89}}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.c23.rank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.c23.z\endcsname{\ensuremath{-5.3}}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.head_pp\endcsname{\ensuremath{-6.492}}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.head_ppalt\endcsname{\ensuremath{-6.736}}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.maxz\endcsname{\ensuremath{-9.6}}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.maxz_class\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.maxz_pp\endcsname{\ensuremath{-4.31}}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.nneg2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.nneg2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.N1.kits.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.N1.params\endcsname{31.1}
\expandafter\gdef\csname R@an.perclass_all.N1.params.acdc\endcsname{30.4}
\expandafter\gdef\csname R@an.perclass_all.N1.params.amos\endcsname{31.1}
\expandafter\gdef\csname R@an.perclass_all.N1.params.kits\endcsname{31.2}
\expandafter\gdef\csname R@an.perclass_all.N1.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.altflip\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c1.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c1.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c1.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c1.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c1.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c10.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c10.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c10.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c10.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c10.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c11.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c11.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c11.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c11.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c11.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c12.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c12.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c12.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c12.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c12.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c13.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c13.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c13.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c13.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c13.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c14.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c14.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c14.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c14.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c14.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c15.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c15.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c15.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c15.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c15.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c2.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c2.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c2.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c2.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c2.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c3.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c3.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c3.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c3.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c3.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c4.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c4.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c4.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c4.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c4.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c5.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c5.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c5.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c5.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c5.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c6.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c6.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c6.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c6.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c6.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c7.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c7.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c7.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c7.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c7.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c8.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c8.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c8.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c8.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c8.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c9.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c9.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c9.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c9.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.c9.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.head_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.head_ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.maxz\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.maxz_class\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.maxz_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.nneg2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.nneg2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.npos2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.npos2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.nrank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.nseed\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.pos2list\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.regstate\endcsname{queued}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.seedlist\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.amos.sumpos_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.altflip\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.c123.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.c123.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.c123.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.c123.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.c123.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.c2.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.c2.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.c2.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.c2.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.c2.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.c23.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.c23.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.c23.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.c23.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.c23.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.head_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.head_ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.maxz\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.maxz_class\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.maxz_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.nneg2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.nneg2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.npos2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.npos2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.nrank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.nseed\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.pos2list\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.regstate\endcsname{queued}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.seedlist\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.kits.sumpos_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.params\endcsname{31.2}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.params.acdc\endcsname{30.4}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.params.amos\endcsname{31.2}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.params.kits\endcsname{31.4}
\expandafter\gdef\csname R@an.perclass_all.P1_frcap32.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.altflip\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c1.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c1.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c1.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c1.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c1.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c10.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c10.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c10.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c10.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c10.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c11.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c11.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c11.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c11.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c11.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c12.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c12.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c12.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c12.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c12.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c13.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c13.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c13.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c13.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c13.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c14.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c14.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c14.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c14.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c14.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c15.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c15.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c15.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c15.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c15.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c2.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c2.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c2.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c2.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c2.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c3.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c3.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c3.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c3.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c3.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c4.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c4.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c4.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c4.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c4.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c5.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c5.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c5.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c5.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c5.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c6.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c6.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c6.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c6.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c6.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c7.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c7.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c7.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c7.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c7.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c8.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c8.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c8.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c8.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c8.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c9.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c9.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c9.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c9.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.c9.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.head_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.head_ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.maxz\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.maxz_class\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.maxz_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.nneg2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.nneg2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.npos2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.npos2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.nrank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.nseed\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.pos2list\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.regstate\endcsname{queued}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.seedlist\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.amos.sumpos_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1b.params\endcsname{31.2}
\expandafter\gdef\csname R@an.perclass_all.P1b.params.acdc\endcsname{30.4}
\expandafter\gdef\csname R@an.perclass_all.P1b.params.amos\endcsname{31.2}
\expandafter\gdef\csname R@an.perclass_all.P1b.params.kits\endcsname{31.2}
\expandafter\gdef\csname R@an.perclass_all.P1b.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.altflip\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c1.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c1.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c1.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c1.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c1.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c10.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c10.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c10.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c10.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c10.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c11.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c11.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c11.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c11.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c11.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c12.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c12.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c12.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c12.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c12.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c13.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c13.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c13.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c13.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c13.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c14.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c14.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c14.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c14.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c14.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c15.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c15.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c15.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c15.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c15.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c2.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c2.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c2.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c2.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c2.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c3.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c3.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c3.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c3.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c3.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c4.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c4.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c4.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c4.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c4.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c5.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c5.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c5.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c5.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c5.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c6.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c6.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c6.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c6.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c6.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c7.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c7.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c7.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c7.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c7.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c8.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c8.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c8.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c8.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c8.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c9.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c9.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c9.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c9.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.c9.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.head_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.head_ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.maxz\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.maxz_class\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.maxz_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.nneg2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.nneg2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.npos2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.npos2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.nrank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.nseed\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.pos2list\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.regstate\endcsname{queued}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.seedlist\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.amos.sumpos_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.altflip\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.c123.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.c123.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.c123.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.c123.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.c123.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.c2.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.c2.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.c2.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.c2.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.c2.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.c23.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.c23.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.c23.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.c23.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.c23.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.head_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.head_ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.maxz\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.maxz_class\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.maxz_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.nneg2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.nneg2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.npos2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.npos2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.nrank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.nseed\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.pos2list\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.regstate\endcsname{queued}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.seedlist\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.kits.sumpos_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P1c.params\endcsname{31.6}
\expandafter\gdef\csname R@an.perclass_all.P1c.params.acdc\endcsname{30.8}
\expandafter\gdef\csname R@an.perclass_all.P1c.params.amos\endcsname{31.6}
\expandafter\gdef\csname R@an.perclass_all.P1c.params.kits\endcsname{31.6}
\expandafter\gdef\csname R@an.perclass_all.P1c.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.c1.gap\endcsname{\ensuremath{-1.25}}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.c1.pp\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.c1.ppalt\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.c1.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.c1.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.c2.gap\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.c2.pp\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.c2.ppalt\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.c2.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.c2.z\endcsname{\ensuremath{-1.1}}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.c3.gap\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.c3.pp\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.c3.ppalt\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.c3.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.c3.z\endcsname{\ensuremath{-0.5}}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.head_pp\endcsname{\ensuremath{-0.013}}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.head_ppalt\endcsname{\ensuremath{-0.020}}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.maxz\endcsname{\ensuremath{-1.1}}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.maxz_class\endcsname{MLV}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.maxz_pp\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.nrank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.acdc.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c1.gap\endcsname{\ensuremath{-2.50}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c1.pp\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c1.ppalt\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c1.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c1.z\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c10.gap\endcsname{\ensuremath{-0.81}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c10.pp\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c10.ppalt\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c10.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c10.z\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c11.gap\endcsname{\ensuremath{-1.08}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c11.pp\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c11.ppalt\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c11.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c11.z\endcsname{\ensuremath{-0.9}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c12.gap\endcsname{\ensuremath{-1.79}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c12.pp\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c12.ppalt\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c12.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c12.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c13.gap\endcsname{\ensuremath{-1.51}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c13.pp\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c13.ppalt\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c13.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c13.z\endcsname{\ensuremath{-0.3}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c14.gap\endcsname{\ensuremath{-2.69}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c14.pp\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c14.ppalt\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c14.rank\endcsname{28}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c14.z\endcsname{\ensuremath{-2.3}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c15.gap\endcsname{\ensuremath{-0.95}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c15.pp\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c15.ppalt\endcsname{\ensuremath{+2.87}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c15.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c15.z\endcsname{\ensuremath{+2.3}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c2.gap\endcsname{\ensuremath{-0.91}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c2.pp\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c2.ppalt\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c2.rank\endcsname{29}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c2.z\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c3.gap\endcsname{\ensuremath{-1.04}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c3.pp\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c3.ppalt\endcsname{\ensuremath{-0.54}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c3.rank\endcsname{34}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c3.z\endcsname{\ensuremath{-1.1}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c4.gap\endcsname{\ensuremath{-5.25}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c4.pp\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c4.ppalt\endcsname{\ensuremath{-1.19}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c4.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c4.z\endcsname{\ensuremath{-0.4}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c5.gap\endcsname{\ensuremath{-0.64}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c5.pp\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c5.ppalt\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c5.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c5.z\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c6.gap\endcsname{\ensuremath{-0.87}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c6.pp\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c6.ppalt\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c6.rank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c6.z\endcsname{\ensuremath{-2.9}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c7.gap\endcsname{\ensuremath{-1.63}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c7.pp\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c7.ppalt\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c7.rank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c7.z\endcsname{\ensuremath{-2.3}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c8.gap\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c8.pp\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c8.ppalt\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c8.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c8.z\endcsname{\ensuremath{-1.6}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c9.gap\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c9.pp\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c9.ppalt\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c9.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.c9.z\endcsname{\ensuremath{+3.6}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.head_pp\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.head_ppalt\endcsname{\ensuremath{-0.022}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.maxz\endcsname{\ensuremath{+3.6}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.maxz_class\endcsname{postcava}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.maxz_pp\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.nneg2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.nneg2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.npos2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.npos2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.pos2list\endcsname{postcava, prostate/uterus}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.amos.sumpos_pp\endcsname{\ensuremath{+2.98}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.c1.gap\endcsname{\ensuremath{-0.85}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.c1.pp\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.c1.ppalt\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.c1.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.c1.z\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.c2.gap\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.c2.pp\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.c2.ppalt\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.c2.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.c2.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.c3.gap\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.c3.pp\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.c3.ppalt\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.c3.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.c3.z\endcsname{\ensuremath{-0.2}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.head_pp\endcsname{\ensuremath{+0.117}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.head_ppalt\endcsname{\ensuremath{+0.110}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.maxz\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.maxz_class\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.maxz_pp\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.nrank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.acdc.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.c123.gap\endcsname{\ensuremath{-0.70}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.c123.pp\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.c123.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.c123.z\endcsname{\ensuremath{+1.5}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.c2.gap\endcsname{\ensuremath{-3.65}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.c2.pp\endcsname{\ensuremath{+1.44}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.c2.ppalt\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.c2.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.c2.z\endcsname{\ensuremath{+1.5}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.c23.gap\endcsname{\ensuremath{-2.61}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.c23.pp\endcsname{\ensuremath{+1.54}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.c23.ppalt\endcsname{\ensuremath{+1.22}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.c23.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.c23.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.head_pp\endcsname{\ensuremath{+1.176}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.head_ppalt\endcsname{\ensuremath{+0.932}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.maxz\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.maxz_pp\endcsname{\ensuremath{+1.54}}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.P3c.fresh.kits.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.c123.gap\endcsname{\ensuremath{-0.64}}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.c123.pp\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.c123.ppalt\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.c123.rank\endcsname{27}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.c123.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.c2.gap\endcsname{\ensuremath{-3.22}}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.c2.pp\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.c2.ppalt\endcsname{\ensuremath{+1.47}}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.c2.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.c2.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.c23.gap\endcsname{\ensuremath{-2.57}}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.c23.pp\endcsname{\ensuremath{+1.75}}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.c23.ppalt\endcsname{\ensuremath{+1.43}}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.c23.rank\endcsname{28}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.c23.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.head_pp\endcsname{\ensuremath{+1.364}}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.head_ppalt\endcsname{\ensuremath{+1.121}}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.maxz\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.maxz_pp\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.P3c.kits.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.P3c.params\endcsname{31.1}
\expandafter\gdef\csname R@an.perclass_all.P3c.params.acdc\endcsname{30.4}
\expandafter\gdef\csname R@an.perclass_all.P3c.params.amos\endcsname{31.1}
\expandafter\gdef\csname R@an.perclass_all.P3c.params.kits\endcsname{31.2}
\expandafter\gdef\csname R@an.perclass_all.P3c.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.altflip\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c1.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c1.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c1.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c1.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c1.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c10.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c10.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c10.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c10.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c10.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c11.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c11.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c11.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c11.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c11.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c12.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c12.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c12.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c12.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c12.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c13.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c13.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c13.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c13.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c13.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c14.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c14.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c14.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c14.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c14.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c15.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c15.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c15.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c15.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c15.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c2.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c2.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c2.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c2.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c2.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c3.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c3.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c3.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c3.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c3.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c4.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c4.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c4.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c4.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c4.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c5.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c5.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c5.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c5.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c5.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c6.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c6.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c6.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c6.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c6.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c7.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c7.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c7.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c7.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c7.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c8.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c8.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c8.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c8.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c8.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c9.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c9.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c9.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c9.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.c9.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.head_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.head_ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.maxz\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.maxz_class\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.maxz_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.nneg2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.nneg2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.npos2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.npos2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.nrank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.nseed\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.pos2list\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.regstate\endcsname{queued}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.seedlist\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.amos.sumpos_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.altflip\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.c123.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.c123.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.c123.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.c123.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.c123.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.c2.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.c2.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.c2.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.c2.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.c2.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.c23.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.c23.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.c23.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.c23.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.c23.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.head_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.head_ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.maxz\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.maxz_class\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.maxz_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.nneg2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.nneg2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.npos2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.npos2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.nrank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.nseed\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.pos2list\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.regstate\endcsname{queued}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.seedlist\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.kits.sumpos_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.P3lite.params\endcsname{31.1}
\expandafter\gdef\csname R@an.perclass_all.P3lite.params.acdc\endcsname{30.4}
\expandafter\gdef\csname R@an.perclass_all.P3lite.params.amos\endcsname{31.1}
\expandafter\gdef\csname R@an.perclass_all.P3lite.params.kits\endcsname{31.2}
\expandafter\gdef\csname R@an.perclass_all.P3lite.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c1.gap\endcsname{\ensuremath{-2.40}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c1.pp\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c1.ppalt\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c1.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c1.z\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c10.gap\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c10.pp\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c10.ppalt\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c10.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c10.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c11.gap\endcsname{\ensuremath{-0.90}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c11.pp\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c11.ppalt\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c11.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c11.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c12.gap\endcsname{\ensuremath{-1.17}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c12.pp\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c12.ppalt\endcsname{\ensuremath{+0.90}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c12.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c12.z\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c13.gap\endcsname{\ensuremath{-0.55}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c13.pp\endcsname{\ensuremath{+0.84}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c13.ppalt\endcsname{\ensuremath{+0.89}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c13.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c13.z\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c14.gap\endcsname{\ensuremath{-2.93}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c14.pp\endcsname{\ensuremath{-0.82}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c14.ppalt\endcsname{\ensuremath{-0.85}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c14.rank\endcsname{29}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c14.z\endcsname{\ensuremath{-3.2}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c15.gap\endcsname{\ensuremath{-3.25}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c15.pp\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c15.ppalt\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c15.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c15.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c2.gap\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c2.pp\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c2.ppalt\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c2.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c2.z\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c3.gap\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c3.pp\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c3.ppalt\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c3.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c3.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c4.gap\endcsname{\ensuremath{-1.76}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c4.pp\endcsname{\ensuremath{+2.91}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c4.ppalt\endcsname{\ensuremath{+2.30}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c4.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c4.z\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c5.gap\endcsname{\ensuremath{-0.54}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c5.pp\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c5.ppalt\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c5.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c5.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c6.gap\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c6.pp\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c6.ppalt\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c6.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c6.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c7.gap\endcsname{\ensuremath{-0.72}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c7.pp\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c7.ppalt\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c7.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c7.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c8.gap\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c8.pp\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c8.ppalt\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c8.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c8.z\endcsname{\ensuremath{-0.2}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c9.gap\endcsname{\ensuremath{-0.71}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c9.pp\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c9.ppalt\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c9.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.c9.z\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.head_pp\endcsname{\ensuremath{+0.378}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.head_ppalt\endcsname{\ensuremath{+0.349}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.maxz\endcsname{\ensuremath{-3.2}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.maxz_class\endcsname{bladder}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.maxz_pp\endcsname{\ensuremath{-0.82}}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.nneg2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.nneg2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.npos2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.pos2list\endcsname{gall bladder, duodenum}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.S2.amos.sumpos_pp\endcsname{\ensuremath{+3.75}}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.c123.gap\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.c123.pp\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.c123.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.c123.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.c2.gap\endcsname{\ensuremath{-4.99}}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.c2.pp\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.c2.ppalt\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.c2.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.c2.z\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.c23.gap\endcsname{\ensuremath{-3.02}}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.c23.pp\endcsname{\ensuremath{+1.13}}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.c23.ppalt\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.c23.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.c23.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.head_pp\endcsname{\ensuremath{+0.570}}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.head_ppalt\endcsname{\ensuremath{+0.326}}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.maxz\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.maxz_class\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.maxz_pp\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.S2.fresh.kits.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.c123.gap\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.c123.pp\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.c123.ppalt\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.c123.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.c123.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.c2.gap\endcsname{\ensuremath{-3.69}}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.c2.pp\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.c2.ppalt\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.c2.rank\endcsname{28}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.c2.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.c23.gap\endcsname{\ensuremath{-2.38}}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.c23.pp\endcsname{\ensuremath{+1.93}}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.c23.ppalt\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.c23.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.c23.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.head_pp\endcsname{\ensuremath{+1.341}}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.head_ppalt\endcsname{\ensuremath{+1.098}}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.maxz\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.maxz_class\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.maxz_pp\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.S2.kits.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.S2.params\endcsname{27.7}
\expandafter\gdef\csname R@an.perclass_all.S2.params.acdc\endcsname{27.0}
\expandafter\gdef\csname R@an.perclass_all.S2.params.amos\endcsname{27.7}
\expandafter\gdef\csname R@an.perclass_all.S2.params.kits\endcsname{27.8}
\expandafter\gdef\csname R@an.perclass_all.S2.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.altflip\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c1.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c1.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c1.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c1.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c1.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c10.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c10.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c10.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c10.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c10.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c11.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c11.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c11.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c11.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c11.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c12.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c12.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c12.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c12.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c12.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c13.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c13.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c13.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c13.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c13.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c14.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c14.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c14.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c14.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c14.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c15.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c15.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c15.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c15.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c15.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c2.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c2.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c2.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c2.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c2.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c3.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c3.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c3.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c3.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c3.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c4.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c4.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c4.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c4.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c4.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c5.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c5.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c5.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c5.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c5.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c6.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c6.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c6.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c6.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c6.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c7.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c7.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c7.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c7.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c7.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c8.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c8.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c8.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c8.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c8.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c9.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c9.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c9.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c9.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.c9.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.head_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.head_ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.maxz\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.maxz_class\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.maxz_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.nneg2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.nneg2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.npos2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.npos2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.nrank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.nseed\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.pos2list\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.regstate\endcsname{queued}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.seedlist\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.amos.sumpos_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.altflip\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.c123.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.c123.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.c123.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.c123.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.c123.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.c2.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.c2.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.c2.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.c2.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.c2.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.c23.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.c23.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.c23.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.c23.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.c23.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.head_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.head_ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.maxz\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.maxz_class\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.maxz_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.nneg2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.nneg2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.npos2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.npos2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.nrank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.nseed\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.pos2list\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.regstate\endcsname{running}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.seedlist\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.kits.sumpos_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.params\endcsname{108}
\expandafter\gdef\csname R@an.perclass_all.SP1.params.acdc\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.params.amos\endcsname{108}
\expandafter\gdef\csname R@an.perclass_all.SP1.params.kits\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP1.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.altflip\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c1.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c1.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c1.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c1.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c1.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c10.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c10.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c10.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c10.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c10.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c11.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c11.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c11.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c11.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c11.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c12.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c12.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c12.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c12.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c12.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c13.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c13.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c13.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c13.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c13.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c14.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c14.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c14.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c14.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c14.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c15.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c15.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c15.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c15.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c15.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c2.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c2.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c2.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c2.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c2.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c3.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c3.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c3.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c3.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c3.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c4.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c4.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c4.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c4.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c4.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c5.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c5.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c5.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c5.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c5.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c6.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c6.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c6.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c6.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c6.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c7.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c7.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c7.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c7.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c7.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c8.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c8.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c8.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c8.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c8.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c9.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c9.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c9.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c9.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.c9.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.head_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.head_ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.maxz\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.maxz_class\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.maxz_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.nneg2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.nneg2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.npos2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.npos2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.nrank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.nseed\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.pos2list\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.regstate\endcsname{queued}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.seedlist\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.amos.sumpos_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.altflip\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.c123.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.c123.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.c123.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.c123.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.c123.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.c2.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.c2.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.c2.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.c2.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.c2.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.c23.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.c23.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.c23.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.c23.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.c23.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.head_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.head_ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.maxz\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.maxz_class\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.maxz_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.nneg2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.nneg2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.npos2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.npos2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.nrank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.nseed\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.pos2list\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.regstate\endcsname{running}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.seedlist\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.kits.sumpos_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.params\endcsname{108}
\expandafter\gdef\csname R@an.perclass_all.SP2.params.acdc\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.params.amos\endcsname{108}
\expandafter\gdef\csname R@an.perclass_all.SP2.params.kits\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.SP2.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.altflip\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c1.gap\endcsname{\ensuremath{-2.61}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c1.pp\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c1.ppalt\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c1.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c1.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c10.gap\endcsname{\ensuremath{-1.29}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c10.pp\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c10.ppalt\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c10.rank\endcsname{29}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c10.z\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c11.gap\endcsname{\ensuremath{-0.88}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c11.pp\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c11.ppalt\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c11.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c11.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c12.gap\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c12.pp\endcsname{\ensuremath{+1.43}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c12.ppalt\endcsname{\ensuremath{+1.68}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c12.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c12.z\endcsname{\ensuremath{+1.5}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c13.gap\endcsname{\ensuremath{-0.99}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c13.pp\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c13.ppalt\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c13.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c13.z\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c14.gap\endcsname{\ensuremath{-3.07}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c14.pp\endcsname{\ensuremath{-0.96}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c14.ppalt\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c14.rank\endcsname{31}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c14.z\endcsname{\ensuremath{-3.8}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c15.gap\endcsname{\ensuremath{-3.61}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c15.pp\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c15.ppalt\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c15.rank\endcsname{28}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c15.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c2.gap\endcsname{\ensuremath{-1.37}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c2.pp\endcsname{\ensuremath{-0.73}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c2.ppalt\endcsname{\ensuremath{-0.96}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c2.rank\endcsname{31}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c2.z\endcsname{\ensuremath{-1.6}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c3.gap\endcsname{\ensuremath{-0.80}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c3.pp\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c3.ppalt\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c3.rank\endcsname{30}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c3.z\endcsname{\ensuremath{-0.4}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c4.gap\endcsname{\ensuremath{-3.60}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c4.pp\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c4.ppalt\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c4.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c4.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c5.gap\endcsname{\ensuremath{-0.78}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c5.pp\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c5.ppalt\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c5.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c5.z\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c6.gap\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c6.pp\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c6.ppalt\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c6.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c6.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c7.gap\endcsname{\ensuremath{-1.45}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c7.pp\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c7.ppalt\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c7.rank\endcsname{36}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c7.z\endcsname{\ensuremath{-1.7}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c8.gap\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c8.pp\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c8.ppalt\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c8.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c8.z\endcsname{\ensuremath{-0.8}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c9.gap\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c9.pp\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c9.ppalt\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c9.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.c9.z\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.head_pp\endcsname{\ensuremath{+0.041}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.head_ppalt\endcsname{\ensuremath{+0.012}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.maxz\endcsname{\ensuremath{-3.8}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.maxz_class\endcsname{bladder}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.maxz_pp\endcsname{\ensuremath{-0.96}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.nneg2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.nneg2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.pos2list\endcsname{postcava}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5A5.amos.sumpos_pp\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.c123.gap\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.c123.pp\endcsname{\ensuremath{+0.72}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.c123.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.c123.z\endcsname{\ensuremath{+2.0}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.c2.gap\endcsname{\ensuremath{-1.91}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.c2.pp\endcsname{\ensuremath{+3.19}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.c2.ppalt\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.c2.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.c2.z\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.c23.gap\endcsname{\ensuremath{-1.55}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.c23.pp\endcsname{\ensuremath{+2.59}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.c23.ppalt\endcsname{\ensuremath{+2.27}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.c23.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.c23.z\endcsname{\ensuremath{+2.6}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.head_pp\endcsname{\ensuremath{+2.165}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.head_ppalt\endcsname{\ensuremath{+1.922}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.maxz\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.maxz_pp\endcsname{\ensuremath{+3.19}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.npos2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.pos2list\endcsname{tumour, masses, kidney}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.V5A5.fresh.kits.sumpos_pp\endcsname{\ensuremath{+6.50}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.altflip\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.c123.gap\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.c123.pp\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.c123.ppalt\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.c123.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.c123.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.c2.gap\endcsname{\ensuremath{-2.51}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.c2.pp\endcsname{\ensuremath{+2.47}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.c2.ppalt\endcsname{\ensuremath{+2.18}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.c2.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.c2.z\endcsname{\ensuremath{+2.0}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.c23.gap\endcsname{\ensuremath{-1.75}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.c23.pp\endcsname{\ensuremath{+2.57}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.c23.ppalt\endcsname{\ensuremath{+2.24}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.c23.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.c23.z\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.head_pp\endcsname{\ensuremath{+1.949}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.head_ppalt\endcsname{\ensuremath{+1.706}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.maxz\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.maxz_pp\endcsname{\ensuremath{+2.57}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.npos2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.pos2list\endcsname{masses, tumour}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5A5.kits.sumpos_pp\endcsname{\ensuremath{+5.04}}
\expandafter\gdef\csname R@an.perclass_all.V5A5.params\endcsname{29.5}
\expandafter\gdef\csname R@an.perclass_all.V5A5.params.acdc\endcsname{28.7}
\expandafter\gdef\csname R@an.perclass_all.V5A5.params.amos\endcsname{29.5}
\expandafter\gdef\csname R@an.perclass_all.V5A5.params.kits\endcsname{29.5}
\expandafter\gdef\csname R@an.perclass_all.V5A5.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c1.gap\endcsname{\ensuremath{-2.53}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c1.pp\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c1.ppalt\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c1.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c1.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c10.gap\endcsname{\ensuremath{-1.05}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c10.pp\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c10.ppalt\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c10.rank\endcsname{26}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c10.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c11.gap\endcsname{\ensuremath{-1.49}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c11.pp\endcsname{\ensuremath{-0.55}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c11.ppalt\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c11.rank\endcsname{29}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c11.z\endcsname{\ensuremath{-3.4}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c12.gap\endcsname{\ensuremath{-1.51}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c12.pp\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c12.ppalt\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c12.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c12.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c13.gap\endcsname{\ensuremath{-2.53}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c13.pp\endcsname{\ensuremath{-1.14}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c13.ppalt\endcsname{\ensuremath{-1.08}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c13.rank\endcsname{34}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c13.z\endcsname{\ensuremath{-2.9}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c14.gap\endcsname{\ensuremath{-3.83}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c14.pp\endcsname{\ensuremath{-1.72}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c14.ppalt\endcsname{\ensuremath{-1.75}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c14.rank\endcsname{37}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c14.z\endcsname{\ensuremath{-6.8}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c15.gap\endcsname{\ensuremath{-3.12}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c15.pp\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c15.ppalt\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c15.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c15.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c2.gap\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c2.pp\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c2.ppalt\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c2.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c2.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c3.gap\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c3.pp\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c3.ppalt\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c3.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c3.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c4.gap\endcsname{\ensuremath{-5.70}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c4.pp\endcsname{\ensuremath{-1.04}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c4.ppalt\endcsname{\ensuremath{-1.64}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c4.rank\endcsname{28}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c4.z\endcsname{\ensuremath{-0.8}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c5.gap\endcsname{\ensuremath{-1.30}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c5.pp\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c5.ppalt\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c5.rank\endcsname{28}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c5.z\endcsname{\ensuremath{-1.6}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c6.gap\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c6.pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c6.ppalt\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c6.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c6.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c7.gap\endcsname{\ensuremath{-0.95}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c7.pp\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c7.ppalt\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c7.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c7.z\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c8.gap\endcsname{\ensuremath{-0.55}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c8.pp\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c8.ppalt\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c8.rank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c8.z\endcsname{\ensuremath{-3.4}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c9.gap\endcsname{\ensuremath{-0.72}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c9.pp\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c9.ppalt\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c9.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.c9.z\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.head_pp\endcsname{\ensuremath{-0.261}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.head_ppalt\endcsname{\ensuremath{-0.290}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.maxz\endcsname{\ensuremath{-6.8}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.maxz_class\endcsname{bladder}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.maxz_pp\endcsname{\ensuremath{-1.72}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.nneg2\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.nneg2alt\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B1.amos.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.c123.gap\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.c123.pp\endcsname{\ensuremath{+0.94}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.c123.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.c123.z\endcsname{\ensuremath{+2.6}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.c2.gap\endcsname{\ensuremath{-2.38}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.c2.pp\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.c2.ppalt\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.c2.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.c2.z\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.c23.gap\endcsname{\ensuremath{-0.94}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.c23.pp\endcsname{\ensuremath{+3.21}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.c23.ppalt\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.c23.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.c23.z\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.head_pp\endcsname{\ensuremath{+2.285}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.head_ppalt\endcsname{\ensuremath{+2.042}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.maxz\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.maxz_pp\endcsname{\ensuremath{+3.21}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.pos2list\endcsname{masses, tumour, kidney}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.V5B1.fresh.kits.sumpos_pp\endcsname{\ensuremath{+6.86}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.c123.gap\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.c123.pp\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.c123.ppalt\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.c123.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.c123.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.c2.gap\endcsname{\ensuremath{-1.69}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.c2.pp\endcsname{\ensuremath{+3.29}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.c2.ppalt\endcsname{\ensuremath{+3.00}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.c2.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.c2.z\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.c23.gap\endcsname{\ensuremath{-1.83}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.c23.pp\endcsname{\ensuremath{+2.49}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.c23.ppalt\endcsname{\ensuremath{+2.17}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.c23.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.c23.z\endcsname{\ensuremath{+2.0}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.head_pp\endcsname{\ensuremath{+2.162}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.head_ppalt\endcsname{\ensuremath{+1.919}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.maxz\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.maxz_pp\endcsname{\ensuremath{+3.29}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.npos2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.pos2list\endcsname{tumour, masses}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B1.kits.sumpos_pp\endcsname{\ensuremath{+5.78}}
\expandafter\gdef\csname R@an.perclass_all.V5B1.params\endcsname{20.9}
\expandafter\gdef\csname R@an.perclass_all.V5B1.params.acdc\endcsname{20.2}
\expandafter\gdef\csname R@an.perclass_all.V5B1.params.amos\endcsname{20.9}
\expandafter\gdef\csname R@an.perclass_all.V5B1.params.kits\endcsname{21.0}
\expandafter\gdef\csname R@an.perclass_all.V5B1.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.c1.gap\endcsname{\ensuremath{-1.63}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.c1.pp\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.c1.ppalt\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.c1.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.c1.z\endcsname{\ensuremath{-1.3}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.c2.gap\endcsname{\ensuremath{-0.60}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.c2.pp\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.c2.ppalt\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.c2.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.c2.z\endcsname{\ensuremath{-2.0}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.c3.gap\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.c3.pp\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.c3.ppalt\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.c3.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.c3.z\endcsname{\ensuremath{-0.7}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.head_pp\endcsname{\ensuremath{-0.181}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.head_ppalt\endcsname{\ensuremath{-0.188}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.maxz\endcsname{\ensuremath{-2.0}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.maxz_class\endcsname{MLV}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.maxz_pp\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.nneg2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.nrank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.acdc.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c1.gap\endcsname{\ensuremath{-2.46}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c1.pp\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c1.ppalt\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c1.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c1.z\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c10.gap\endcsname{\ensuremath{-2.38}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c10.pp\endcsname{\ensuremath{-1.35}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c10.ppalt\endcsname{\ensuremath{-1.59}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c10.rank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c10.z\endcsname{\ensuremath{-3.3}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c11.gap\endcsname{\ensuremath{-1.23}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c11.pp\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c11.ppalt\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c11.rank\endcsname{26}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c11.z\endcsname{\ensuremath{-1.8}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c12.gap\endcsname{\ensuremath{-2.08}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c12.pp\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c12.ppalt\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c12.rank\endcsname{29}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c12.z\endcsname{\ensuremath{-0.3}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c13.gap\endcsname{\ensuremath{-1.82}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c13.pp\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c13.ppalt\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c13.rank\endcsname{30}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c13.z\endcsname{\ensuremath{-1.1}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c14.gap\endcsname{\ensuremath{-1.83}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c14.pp\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c14.ppalt\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c14.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c14.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c15.gap\endcsname{\ensuremath{-1.70}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c15.pp\endcsname{\ensuremath{+1.77}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c15.ppalt\endcsname{\ensuremath{+2.11}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c15.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c15.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c2.gap\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c2.pp\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c2.ppalt\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c2.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c2.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c3.gap\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c3.pp\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c3.ppalt\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c3.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c3.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c4.gap\endcsname{\ensuremath{-2.87}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c4.pp\endcsname{\ensuremath{+1.80}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c4.ppalt\endcsname{\ensuremath{+1.19}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c4.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c4.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c5.gap\endcsname{\ensuremath{-1.39}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c5.pp\endcsname{\ensuremath{-0.58}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c5.ppalt\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c5.rank\endcsname{31}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c5.z\endcsname{\ensuremath{-1.9}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c6.gap\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c6.pp\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c6.ppalt\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c6.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c6.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c7.gap\endcsname{\ensuremath{-0.82}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c7.pp\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c7.ppalt\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c7.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c7.z\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c8.gap\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c8.pp\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c8.ppalt\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c8.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c8.z\endcsname{\ensuremath{-0.8}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c9.gap\endcsname{\ensuremath{-1.08}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c9.pp\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c9.ppalt\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c9.rank\endcsname{36}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.c9.z\endcsname{\ensuremath{-2.4}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.head_pp\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.head_ppalt\endcsname{\ensuremath{+0.103}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.maxz\endcsname{\ensuremath{-3.3}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.maxz_class\endcsname{pancreas}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.maxz_pp\endcsname{\ensuremath{-1.35}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.nneg2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.nneg2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.amos.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.c123.gap\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.c123.pp\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.c123.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.c123.z\endcsname{\ensuremath{+2.6}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.c2.gap\endcsname{\ensuremath{-3.50}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.c2.pp\endcsname{\ensuremath{+1.60}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.c2.ppalt\endcsname{\ensuremath{+1.31}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.c2.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.c2.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.c23.gap\endcsname{\ensuremath{-2.32}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.c23.pp\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.c23.ppalt\endcsname{\ensuremath{+1.51}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.c23.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.c23.z\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.head_pp\endcsname{\ensuremath{+1.448}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.head_ppalt\endcsname{\ensuremath{+1.205}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.maxz\endcsname{\ensuremath{+2.6}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.maxz_class\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.maxz_pp\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.pos2list\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.V5B2.fresh.kits.sumpos_pp\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.c123.gap\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.c123.pp\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.c123.ppalt\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.c123.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.c123.z\endcsname{\ensuremath{+1.5}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.c2.gap\endcsname{\ensuremath{-3.66}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.c2.pp\endcsname{\ensuremath{+1.32}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.c2.ppalt\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.c2.rank\endcsname{27}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.c2.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.c23.gap\endcsname{\ensuremath{-2.55}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.c23.pp\endcsname{\ensuremath{+1.77}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.c23.ppalt\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.c23.rank\endcsname{26}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.c23.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.head_pp\endcsname{\ensuremath{+1.264}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.head_ppalt\endcsname{\ensuremath{+1.021}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.maxz\endcsname{\ensuremath{+1.5}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.maxz_class\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.maxz_pp\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V5B2.kits.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V5B2.params\endcsname{21.2}
\expandafter\gdef\csname R@an.perclass_all.V5B2.params.acdc\endcsname{20.5}
\expandafter\gdef\csname R@an.perclass_all.V5B2.params.amos\endcsname{21.2}
\expandafter\gdef\csname R@an.perclass_all.V5B2.params.kits\endcsname{21.3}
\expandafter\gdef\csname R@an.perclass_all.V5B2.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.c1.gap\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.c1.pp\endcsname{\ensuremath{+1.40}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.c1.ppalt\endcsname{\ensuremath{+1.39}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.c1.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.c1.z\endcsname{\ensuremath{+7.7}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.c2.gap\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.c2.pp\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.c2.ppalt\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.c2.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.c2.z\endcsname{\ensuremath{+2.6}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.c3.gap\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.c3.pp\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.c3.ppalt\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.c3.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.c3.z\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.head_pp\endcsname{\ensuremath{+0.573}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.head_ppalt\endcsname{\ensuremath{+0.566}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.maxz\endcsname{\ensuremath{+7.7}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.maxz_class\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.maxz_pp\endcsname{\ensuremath{+1.40}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.npos2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.npos2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.nrank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.pos2list\endcsname{RV, MLV}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.acdc.sumpos_pp\endcsname{\ensuremath{+1.70}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c1.gap\endcsname{\ensuremath{-2.35}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c1.pp\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c1.ppalt\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c1.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c1.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c10.gap\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c10.pp\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c10.ppalt\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c10.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c10.z\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c11.gap\endcsname{\ensuremath{-0.89}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c11.pp\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c11.ppalt\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c11.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c11.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c12.gap\endcsname{\ensuremath{-0.71}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c12.pp\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c12.ppalt\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c12.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c12.z\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c13.gap\endcsname{\ensuremath{-1.32}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c13.pp\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c13.ppalt\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c13.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c13.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c14.gap\endcsname{\ensuremath{-2.00}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c14.pp\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c14.ppalt\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c14.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c14.z\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c15.gap\endcsname{\ensuremath{-3.50}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c15.pp\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c15.ppalt\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c15.rank\endcsname{27}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c15.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c2.gap\endcsname{\ensuremath{-0.64}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c2.pp\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c2.ppalt\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c2.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c2.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c3.gap\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c3.pp\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c3.ppalt\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c3.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c3.z\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c4.gap\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c4.pp\endcsname{\ensuremath{+3.91}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c4.ppalt\endcsname{\ensuremath{+3.31}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c4.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c4.z\endcsname{\ensuremath{+2.9}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c5.gap\endcsname{\ensuremath{-0.62}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c5.pp\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c5.ppalt\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c5.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c5.z\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c6.gap\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c6.pp\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c6.ppalt\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c6.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c6.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c7.gap\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c7.pp\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c7.ppalt\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c7.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c7.z\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c8.gap\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c8.pp\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c8.ppalt\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c8.rank\endcsname{27}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c8.z\endcsname{\ensuremath{-2.0}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c9.gap\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c9.pp\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c9.ppalt\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c9.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.c9.z\endcsname{\ensuremath{+4.0}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.head_pp\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.head_ppalt\endcsname{\ensuremath{+0.458}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.maxz\endcsname{\ensuremath{+4.0}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.maxz_class\endcsname{postcava}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.maxz_pp\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.nneg2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.nneg2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.npos2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.pos2list\endcsname{postcava, gall bladder}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.amos.sumpos_pp\endcsname{\ensuremath{+4.42}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.altflip\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.c123.gap\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.c123.pp\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.c123.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.c123.z\endcsname{\ensuremath{+2.3}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.c2.gap\endcsname{\ensuremath{-3.11}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.c2.pp\endcsname{\ensuremath{+1.98}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.c2.ppalt\endcsname{\ensuremath{+1.69}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.c2.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.c2.z\endcsname{\ensuremath{+2.0}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.c23.gap\endcsname{\ensuremath{-1.82}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.c23.pp\endcsname{\ensuremath{+2.32}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.c23.ppalt\endcsname{\ensuremath{+2.00}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.c23.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.c23.z\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.head_pp\endcsname{\ensuremath{+1.704}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.head_ppalt\endcsname{\ensuremath{+1.461}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.maxz\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.maxz_pp\endcsname{\ensuremath{+2.32}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.pos2list\endcsname{masses, kidney, tumour}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.fresh.kits.sumpos_pp\endcsname{\ensuremath{+5.11}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.c123.gap\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.c123.pp\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.c123.ppalt\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.c123.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.c123.z\endcsname{\ensuremath{+2.0}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.c2.gap\endcsname{\ensuremath{-2.68}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.c2.pp\endcsname{\ensuremath{+2.30}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.c2.ppalt\endcsname{\ensuremath{+2.01}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.c2.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.c2.z\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.c23.gap\endcsname{\ensuremath{-0.83}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.c23.pp\endcsname{\ensuremath{+3.49}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.c23.ppalt\endcsname{\ensuremath{+3.17}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.c23.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.c23.z\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.head_pp\endcsname{\ensuremath{+2.236}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.head_ppalt\endcsname{\ensuremath{+1.992}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.maxz\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.maxz_pp\endcsname{\ensuremath{+3.49}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.npos2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.pos2list\endcsname{masses, kidney}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.kits.sumpos_pp\endcsname{\ensuremath{+4.41}}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.params\endcsname{30.7}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.params.acdc\endcsname{30.0}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.params.amos\endcsname{30.7}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.params.kits\endcsname{30.8}
\expandafter\gdef\csname R@an.perclass_all.V6A1r.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.c1.gap\endcsname{\ensuremath{-0.84}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.c1.pp\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.c1.ppalt\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.c1.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.c1.z\endcsname{\ensuremath{+3.0}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.c2.gap\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.c2.pp\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.c2.ppalt\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.c2.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.c2.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.c3.gap\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.c3.pp\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.c3.ppalt\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.c3.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.c3.z\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.head_pp\endcsname{\ensuremath{+0.229}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.head_ppalt\endcsname{\ensuremath{+0.222}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.maxz\endcsname{\ensuremath{+3.0}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.maxz_class\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.maxz_pp\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.nrank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.pos2list\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A1.acdc.sumpos_pp\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c1.gap\endcsname{\ensuremath{-2.91}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c1.pp\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c1.ppalt\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c1.rank\endcsname{29}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c1.z\endcsname{\ensuremath{-1.1}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c10.gap\endcsname{\ensuremath{-0.72}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c10.pp\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c10.ppalt\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c10.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c10.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c11.gap\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c11.pp\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c11.ppalt\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c11.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c11.z\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c12.gap\endcsname{\ensuremath{-1.57}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c12.pp\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c12.ppalt\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c12.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c12.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c13.gap\endcsname{\ensuremath{-1.05}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c13.pp\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c13.ppalt\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c13.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c13.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c14.gap\endcsname{\ensuremath{-3.09}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c14.pp\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c14.ppalt\endcsname{\ensuremath{-1.00}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c14.rank\endcsname{33}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c14.z\endcsname{\ensuremath{-3.9}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c15.gap\endcsname{\ensuremath{-3.85}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c15.pp\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c15.ppalt\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c15.rank\endcsname{31}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c15.z\endcsname{\ensuremath{-0.3}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c2.gap\endcsname{\ensuremath{-0.71}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c2.pp\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c2.ppalt\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c2.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c2.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c3.gap\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c3.pp\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c3.ppalt\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c3.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c3.z\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c4.gap\endcsname{\ensuremath{-6.29}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c4.pp\endcsname{\ensuremath{-1.62}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c4.ppalt\endcsname{\ensuremath{-2.23}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c4.rank\endcsname{31}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c4.z\endcsname{\ensuremath{-1.2}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c5.gap\endcsname{\ensuremath{-0.81}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c5.pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c5.ppalt\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c5.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c5.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c6.gap\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c6.pp\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c6.ppalt\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c6.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c6.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c7.gap\endcsname{\ensuremath{-0.54}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c7.pp\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c7.ppalt\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c7.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c7.z\endcsname{\ensuremath{+1.5}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c8.gap\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c8.pp\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c8.ppalt\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c8.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c8.z\endcsname{\ensuremath{-0.2}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c9.gap\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c9.pp\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c9.ppalt\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c9.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.c9.z\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.head_pp\endcsname{\ensuremath{-0.045}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.head_ppalt\endcsname{\ensuremath{-0.073}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.maxz\endcsname{\ensuremath{-3.9}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.maxz_class\endcsname{bladder}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.maxz_pp\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.nneg2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.nneg2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.npos2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.pos2list\endcsname{right adrenal gland, postcava}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A1.amos.sumpos_pp\endcsname{\ensuremath{+0.67}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.c123.gap\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.c123.pp\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.c123.ppalt\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.c123.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.c123.z\endcsname{\ensuremath{+3.2}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.c2.gap\endcsname{\ensuremath{-1.70}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.c2.pp\endcsname{\ensuremath{+3.40}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.c2.ppalt\endcsname{\ensuremath{+3.10}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.c2.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.c2.z\endcsname{\ensuremath{+3.5}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.c23.gap\endcsname{\ensuremath{-0.71}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.c23.pp\endcsname{\ensuremath{+3.44}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.c23.ppalt\endcsname{\ensuremath{+3.12}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.c23.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.c23.z\endcsname{\ensuremath{+3.5}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.head_pp\endcsname{\ensuremath{+2.662}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.head_ppalt\endcsname{\ensuremath{+2.418}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.maxz\endcsname{\ensuremath{+3.5}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.maxz_pp\endcsname{\ensuremath{+3.44}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.pos2list\endcsname{masses, tumour, kidney}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.V7A1.fresh.kits.sumpos_pp\endcsname{\ensuremath{+7.99}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.c123.gap\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.c123.pp\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.c123.ppalt\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.c123.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.c123.z\endcsname{\ensuremath{+2.3}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.c2.gap\endcsname{\ensuremath{-1.70}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.c2.pp\endcsname{\ensuremath{+3.28}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.c2.ppalt\endcsname{\ensuremath{+2.99}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.c2.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.c2.z\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.c23.gap\endcsname{\ensuremath{-1.00}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.c23.pp\endcsname{\ensuremath{+3.32}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.c23.ppalt\endcsname{\ensuremath{+2.99}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.c23.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.c23.z\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.head_pp\endcsname{\ensuremath{+2.548}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.head_ppalt\endcsname{\ensuremath{+2.305}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.maxz\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.maxz_pp\endcsname{\ensuremath{+3.28}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.pos2list\endcsname{tumour, masses, kidney}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A1.kits.sumpos_pp\endcsname{\ensuremath{+7.65}}
\expandafter\gdef\csname R@an.perclass_all.V7A1.params\endcsname{31.0}
\expandafter\gdef\csname R@an.perclass_all.V7A1.params.acdc\endcsname{30.3}
\expandafter\gdef\csname R@an.perclass_all.V7A1.params.amos\endcsname{31.0}
\expandafter\gdef\csname R@an.perclass_all.V7A1.params.kits\endcsname{31.0}
\expandafter\gdef\csname R@an.perclass_all.V7A1.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.c1.gap\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.c1.pp\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.c1.ppalt\endcsname{\ensuremath{+1.06}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.c1.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.c1.z\endcsname{\ensuremath{+5.9}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.c2.gap\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.c2.pp\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.c2.ppalt\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.c2.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.c2.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.c3.gap\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.c3.pp\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.c3.ppalt\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.c3.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.c3.z\endcsname{\ensuremath{-0.8}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.head_pp\endcsname{\ensuremath{+0.362}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.head_ppalt\endcsname{\ensuremath{+0.355}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.maxz\endcsname{\ensuremath{+5.9}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.maxz_class\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.maxz_pp\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.nrank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.pos2list\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A2.acdc.sumpos_pp\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c1.gap\endcsname{\ensuremath{-4.04}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c1.pp\endcsname{\ensuremath{-1.44}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c1.ppalt\endcsname{\ensuremath{-1.49}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c1.rank\endcsname{36}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c1.z\endcsname{\ensuremath{-5.0}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c10.gap\endcsname{\ensuremath{-0.91}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c10.pp\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c10.ppalt\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c10.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c10.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c11.gap\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c11.pp\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c11.ppalt\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c11.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c11.z\endcsname{\ensuremath{+5.2}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c12.gap\endcsname{\ensuremath{-1.17}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c12.pp\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c12.ppalt\endcsname{\ensuremath{+0.90}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c12.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c12.z\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c13.gap\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c13.pp\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c13.ppalt\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c13.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c13.z\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c14.gap\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c14.pp\endcsname{\ensuremath{+2.10}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c14.ppalt\endcsname{\ensuremath{+2.08}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c14.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c14.z\endcsname{\ensuremath{+8.3}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c15.gap\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c15.pp\endcsname{\ensuremath{+3.48}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c15.ppalt\endcsname{\ensuremath{+3.82}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c15.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c15.z\endcsname{\ensuremath{+3.2}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c2.gap\endcsname{\ensuremath{-0.65}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c2.pp\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c2.ppalt\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c2.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c2.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c3.gap\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c3.pp\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c3.ppalt\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c3.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c3.z\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c4.gap\endcsname{\ensuremath{-6.55}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c4.pp\endcsname{\ensuremath{-1.88}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c4.ppalt\endcsname{\ensuremath{-2.49}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c4.rank\endcsname{33}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c4.z\endcsname{\ensuremath{-1.4}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c5.gap\endcsname{\ensuremath{-0.80}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c5.pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c5.ppalt\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c5.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c5.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c6.gap\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c6.pp\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c6.ppalt\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c6.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c6.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c7.gap\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c7.pp\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c7.ppalt\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c7.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c7.z\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c8.gap\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c8.pp\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c8.ppalt\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c8.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c8.z\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c9.gap\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c9.pp\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c9.ppalt\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c9.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.c9.z\endcsname{\ensuremath{+3.4}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.head_pp\endcsname{\ensuremath{+0.359}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.head_ppalt\endcsname{\ensuremath{+0.331}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.maxz\endcsname{\ensuremath{+8.3}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.maxz_class\endcsname{bladder}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.maxz_pp\endcsname{\ensuremath{+2.10}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.nneg2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.nneg2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.npos2\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.npos2alt\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.pos2list\endcsname{bladder, right adrenal gland, postcava, prostate/uterus}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A2.amos.sumpos_pp\endcsname{\ensuremath{+6.87}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.c123.gap\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.c123.pp\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.94}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.c123.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.c123.z\endcsname{\ensuremath{+3.0}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.c2.gap\endcsname{\ensuremath{-1.92}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.c2.pp\endcsname{\ensuremath{+3.17}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.c2.ppalt\endcsname{\ensuremath{+2.88}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.c2.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.c2.z\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.c23.gap\endcsname{\ensuremath{-1.51}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.c23.pp\endcsname{\ensuremath{+2.64}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.c23.ppalt\endcsname{\ensuremath{+2.32}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.c23.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.c23.z\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.head_pp\endcsname{\ensuremath{+2.289}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.head_ppalt\endcsname{\ensuremath{+2.046}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.maxz\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.maxz_pp\endcsname{\ensuremath{+3.17}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.pos2list\endcsname{tumour, kidney, masses}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.V7A2.fresh.kits.sumpos_pp\endcsname{\ensuremath{+6.87}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.c123.gap\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.c123.pp\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.c123.ppalt\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.c123.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.c123.z\endcsname{\ensuremath{+2.5}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.c2.gap\endcsname{\ensuremath{-1.39}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.c2.pp\endcsname{\ensuremath{+3.59}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.c2.ppalt\endcsname{\ensuremath{+3.30}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.c2.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.c2.z\endcsname{\ensuremath{+2.9}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.c23.gap\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.c23.pp\endcsname{\ensuremath{+3.95}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.c23.ppalt\endcsname{\ensuremath{+3.63}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.c23.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.c23.z\endcsname{\ensuremath{+3.2}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.head_pp\endcsname{\ensuremath{+2.886}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.head_ppalt\endcsname{\ensuremath{+2.642}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.maxz\endcsname{\ensuremath{+3.2}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.maxz_pp\endcsname{\ensuremath{+3.95}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.pos2list\endcsname{masses, tumour, kidney}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A2.kits.sumpos_pp\endcsname{\ensuremath{+8.66}}
\expandafter\gdef\csname R@an.perclass_all.V7A2.params\endcsname{31.1}
\expandafter\gdef\csname R@an.perclass_all.V7A2.params.acdc\endcsname{30.4}
\expandafter\gdef\csname R@an.perclass_all.V7A2.params.amos\endcsname{31.1}
\expandafter\gdef\csname R@an.perclass_all.V7A2.params.kits\endcsname{31.2}
\expandafter\gdef\csname R@an.perclass_all.V7A2.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c1.gap\endcsname{\ensuremath{-2.77}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c1.pp\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c1.ppalt\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c1.rank\endcsname{26}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c1.z\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c10.gap\endcsname{\ensuremath{-1.41}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c10.pp\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c10.ppalt\endcsname{\ensuremath{-0.62}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c10.rank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c10.z\endcsname{\ensuremath{-0.9}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c11.gap\endcsname{\ensuremath{-0.84}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c11.pp\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c11.ppalt\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c11.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c11.z\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c12.gap\endcsname{\ensuremath{-2.04}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c12.pp\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c12.ppalt\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c12.rank\endcsname{28}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c12.z\endcsname{\ensuremath{-0.2}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c13.gap\endcsname{\ensuremath{-1.71}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c13.pp\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c13.ppalt\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c13.rank\endcsname{27}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c13.z\endcsname{\ensuremath{-0.8}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c14.gap\endcsname{\ensuremath{-2.00}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c14.pp\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c14.ppalt\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c14.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c14.z\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c15.gap\endcsname{\ensuremath{-3.00}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c15.pp\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c15.ppalt\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c15.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c15.z\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c2.gap\endcsname{\ensuremath{-0.71}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c2.pp\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c2.ppalt\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c2.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c2.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c3.gap\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c3.pp\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c3.ppalt\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c3.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c3.z\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c4.gap\endcsname{\ensuremath{-7.59}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c4.pp\endcsname{\ensuremath{-2.92}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c4.ppalt\endcsname{\ensuremath{-3.53}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c4.rank\endcsname{37}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c4.z\endcsname{\ensuremath{-2.2}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c5.gap\endcsname{\ensuremath{-0.80}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c5.pp\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c5.ppalt\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c5.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c5.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c6.gap\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c6.pp\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c6.ppalt\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c6.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c6.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c7.gap\endcsname{\ensuremath{-0.90}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c7.pp\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c7.ppalt\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c7.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c7.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c8.gap\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c8.pp\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c8.ppalt\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c8.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c8.z\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c9.gap\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c9.pp\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c9.ppalt\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c9.rank\endcsname{33}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.c9.z\endcsname{\ensuremath{-1.1}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.head_pp\endcsname{\ensuremath{-0.216}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.head_ppalt\endcsname{\ensuremath{-0.244}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.maxz\endcsname{\ensuremath{-2.2}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.maxz_class\endcsname{gall bladder}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.maxz_pp\endcsname{\ensuremath{-2.92}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.nneg2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.nneg2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A3.amos.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.c123.gap\endcsname{\ensuremath{-1.18}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.c123.pp\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.c123.ppalt\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.c123.rank\endcsname{31}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.c123.z\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.c2.gap\endcsname{\ensuremath{-4.34}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.c2.pp\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.c2.ppalt\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.c2.rank\endcsname{30}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.c2.z\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.c23.gap\endcsname{\ensuremath{-3.37}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.c23.pp\endcsname{\ensuremath{+0.94}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.c23.ppalt\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.c23.rank\endcsname{31}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.c23.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.head_pp\endcsname{\ensuremath{+0.542}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.head_ppalt\endcsname{\ensuremath{+0.298}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.maxz\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.maxz_pp\endcsname{\ensuremath{+0.94}}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7A3.kits.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V7A3.params\endcsname{26.3}
\expandafter\gdef\csname R@an.perclass_all.V7A3.params.acdc\endcsname{25.6}
\expandafter\gdef\csname R@an.perclass_all.V7A3.params.amos\endcsname{26.3}
\expandafter\gdef\csname R@an.perclass_all.V7A3.params.kits\endcsname{26.4}
\expandafter\gdef\csname R@an.perclass_all.V7A3.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.altflip\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c1.gap\endcsname{\ensuremath{-3.02}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c1.pp\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c1.ppalt\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c1.rank\endcsname{30}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c1.z\endcsname{\ensuremath{-1.4}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c10.gap\endcsname{\ensuremath{-1.03}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c10.pp\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c10.ppalt\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c10.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c10.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c11.gap\endcsname{\ensuremath{-1.60}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c11.pp\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c11.ppalt\endcsname{\ensuremath{-0.67}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c11.rank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c11.z\endcsname{\ensuremath{-4.0}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c12.gap\endcsname{\ensuremath{-2.51}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c12.pp\endcsname{\ensuremath{-0.70}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c12.ppalt\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c12.rank\endcsname{33}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c12.z\endcsname{\ensuremath{-0.8}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c13.gap\endcsname{\ensuremath{-1.63}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c13.pp\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c13.ppalt\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c13.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c13.z\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c14.gap\endcsname{\ensuremath{-2.26}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c14.pp\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c14.ppalt\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c14.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c14.z\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c15.gap\endcsname{\ensuremath{-3.08}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c15.pp\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c15.ppalt\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c15.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c15.z\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c2.gap\endcsname{\ensuremath{-1.18}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c2.pp\endcsname{\ensuremath{-0.54}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c2.ppalt\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c2.rank\endcsname{30}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c2.z\endcsname{\ensuremath{-1.2}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c3.gap\endcsname{\ensuremath{-0.62}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c3.pp\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c3.ppalt\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c3.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c3.z\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c4.gap\endcsname{\ensuremath{-7.24}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c4.pp\endcsname{\ensuremath{-2.57}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c4.ppalt\endcsname{\ensuremath{-3.18}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c4.rank\endcsname{35}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c4.z\endcsname{\ensuremath{-1.9}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c5.gap\endcsname{\ensuremath{-1.85}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c5.pp\endcsname{\ensuremath{-1.04}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c5.ppalt\endcsname{\ensuremath{-0.78}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c5.rank\endcsname{37}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c5.z\endcsname{\ensuremath{-3.3}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c6.gap\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c6.pp\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c6.ppalt\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c6.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c6.z\endcsname{\ensuremath{-0.4}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c7.gap\endcsname{\ensuremath{-1.10}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c7.pp\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c7.ppalt\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c7.rank\endcsname{26}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c7.z\endcsname{\ensuremath{-0.5}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c8.gap\endcsname{\ensuremath{-0.41}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c8.pp\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c8.ppalt\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c8.rank\endcsname{28}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c8.z\endcsname{\ensuremath{-2.1}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c9.gap\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c9.pp\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c9.ppalt\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c9.rank\endcsname{34}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.c9.z\endcsname{\ensuremath{-1.6}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.head_pp\endcsname{\ensuremath{-0.436}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.head_ppalt\endcsname{\ensuremath{-0.464}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.maxz\endcsname{\ensuremath{-4.0}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.maxz_class\endcsname{right adrenal gland}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.maxz_pp\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.nneg2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.nneg2alt\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B1.amos.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.c123.gap\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.c123.pp\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.c123.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.c123.z\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.c2.gap\endcsname{\ensuremath{-2.17}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.c2.pp\endcsname{\ensuremath{+2.93}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.c2.ppalt\endcsname{\ensuremath{+2.64}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.c2.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.c2.z\endcsname{\ensuremath{+3.0}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.c23.gap\endcsname{\ensuremath{-0.93}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.c23.pp\endcsname{\ensuremath{+3.22}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.c23.ppalt\endcsname{\ensuremath{+2.90}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.c23.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.c23.z\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.head_pp\endcsname{\ensuremath{+2.382}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.head_ppalt\endcsname{\ensuremath{+2.138}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.maxz\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.maxz_pp\endcsname{\ensuremath{+3.22}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.pos2list\endcsname{masses, tumour, kidney}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.V7B1.fresh.kits.sumpos_pp\endcsname{\ensuremath{+7.14}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.c123.gap\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.c123.pp\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.c123.ppalt\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.c123.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.c123.z\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.c2.gap\endcsname{\ensuremath{-2.77}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.c2.pp\endcsname{\ensuremath{+2.21}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.c2.ppalt\endcsname{\ensuremath{+1.92}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.c2.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.c2.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.c23.gap\endcsname{\ensuremath{-2.21}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.c23.pp\endcsname{\ensuremath{+2.10}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.c23.ppalt\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.c23.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.c23.z\endcsname{\ensuremath{+1.7}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.head_pp\endcsname{\ensuremath{+1.721}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.head_ppalt\endcsname{\ensuremath{+1.478}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.maxz\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.maxz_class\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.maxz_pp\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B1.kits.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V7B1.params\endcsname{20.4}
\expandafter\gdef\csname R@an.perclass_all.V7B1.params.acdc\endcsname{19.6}
\expandafter\gdef\csname R@an.perclass_all.V7B1.params.amos\endcsname{20.4}
\expandafter\gdef\csname R@an.perclass_all.V7B1.params.kits\endcsname{20.4}
\expandafter\gdef\csname R@an.perclass_all.V7B1.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c1.gap\endcsname{\ensuremath{-4.11}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c1.pp\endcsname{\ensuremath{-1.50}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c1.ppalt\endcsname{\ensuremath{-1.56}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c1.rank\endcsname{37}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c1.z\endcsname{\ensuremath{-5.2}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c10.gap\endcsname{\ensuremath{-1.38}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c10.pp\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c10.ppalt\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c10.rank\endcsname{31}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c10.z\endcsname{\ensuremath{-0.9}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c11.gap\endcsname{\ensuremath{-1.26}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c11.pp\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c11.ppalt\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c11.rank\endcsname{27}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c11.z\endcsname{\ensuremath{-2.0}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c12.gap\endcsname{\ensuremath{-2.03}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c12.pp\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c12.ppalt\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c12.rank\endcsname{26}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c12.z\endcsname{\ensuremath{-0.2}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c13.gap\endcsname{\ensuremath{-1.67}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c13.pp\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c13.ppalt\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c13.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c13.z\endcsname{\ensuremath{-0.7}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c14.gap\endcsname{\ensuremath{-2.56}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c14.pp\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c14.ppalt\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c14.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c14.z\endcsname{\ensuremath{-1.8}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c15.gap\endcsname{\ensuremath{-2.91}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c15.pp\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c15.ppalt\endcsname{\ensuremath{+0.91}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c15.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c15.z\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c2.gap\endcsname{\ensuremath{-0.68}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c2.pp\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c2.ppalt\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c2.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c2.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c3.gap\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c3.pp\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c3.ppalt\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c3.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c3.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c4.gap\endcsname{\ensuremath{-4.45}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c4.pp\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c4.ppalt\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c4.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c4.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c5.gap\endcsname{\ensuremath{-1.33}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c5.pp\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c5.ppalt\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c5.rank\endcsname{30}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c5.z\endcsname{\ensuremath{-1.6}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c6.gap\endcsname{\ensuremath{-0.80}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c6.pp\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c6.ppalt\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c6.rank\endcsname{37}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c6.z\endcsname{\ensuremath{-2.5}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c7.gap\endcsname{\ensuremath{-1.28}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c7.pp\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c7.ppalt\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c7.rank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c7.z\endcsname{\ensuremath{-1.1}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c8.gap\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c8.pp\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c8.ppalt\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c8.rank\endcsname{35}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c8.z\endcsname{\ensuremath{-2.9}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c9.gap\endcsname{\ensuremath{-0.84}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c9.pp\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c9.ppalt\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c9.rank\endcsname{28}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.c9.z\endcsname{\ensuremath{-0.5}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.head_pp\endcsname{\ensuremath{-0.267}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.head_ppalt\endcsname{\ensuremath{-0.295}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.maxz\endcsname{\ensuremath{-5.2}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.maxz_class\endcsname{spleen}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.maxz_pp\endcsname{\ensuremath{-1.50}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.nneg2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.nneg2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B2.amos.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.altflip\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.c123.gap\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.c123.pp\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.c123.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.c123.z\endcsname{\ensuremath{+2.3}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.c2.gap\endcsname{\ensuremath{-2.50}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.c2.pp\endcsname{\ensuremath{+2.59}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.c2.ppalt\endcsname{\ensuremath{+2.30}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.c2.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.c2.z\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.c23.gap\endcsname{\ensuremath{-2.04}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.c23.pp\endcsname{\ensuremath{+2.11}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.c23.ppalt\endcsname{\ensuremath{+1.79}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.c23.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.c23.z\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.head_pp\endcsname{\ensuremath{+1.838}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.head_ppalt\endcsname{\ensuremath{+1.595}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.maxz\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.maxz_pp\endcsname{\ensuremath{+2.59}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.pos2list\endcsname{tumour, kidney, masses}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.V7B2.fresh.kits.sumpos_pp\endcsname{\ensuremath{+5.51}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.c123.gap\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.c123.pp\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.c123.ppalt\endcsname{\ensuremath{+0.91}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.c123.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.c123.z\endcsname{\ensuremath{+2.3}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.c2.gap\endcsname{\ensuremath{-1.13}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.c2.pp\endcsname{\ensuremath{+3.85}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.c2.ppalt\endcsname{\ensuremath{+3.56}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.c2.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.c2.z\endcsname{\ensuremath{+3.1}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.c23.gap\endcsname{\ensuremath{-0.73}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.c23.pp\endcsname{\ensuremath{+3.59}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.c23.ppalt\endcsname{\ensuremath{+3.27}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.c23.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.c23.z\endcsname{\ensuremath{+2.9}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.head_pp\endcsname{\ensuremath{+2.824}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.head_ppalt\endcsname{\ensuremath{+2.581}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.maxz\endcsname{\ensuremath{+3.1}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.maxz_pp\endcsname{\ensuremath{+3.85}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.pos2list\endcsname{tumour, masses, kidney}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7B2.kits.sumpos_pp\endcsname{\ensuremath{+8.47}}
\expandafter\gdef\csname R@an.perclass_all.V7B2.params\endcsname{20.4}
\expandafter\gdef\csname R@an.perclass_all.V7B2.params.acdc\endcsname{19.7}
\expandafter\gdef\csname R@an.perclass_all.V7B2.params.amos\endcsname{20.4}
\expandafter\gdef\csname R@an.perclass_all.V7B2.params.kits\endcsname{20.5}
\expandafter\gdef\csname R@an.perclass_all.V7B2.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.c1.gap\endcsname{\ensuremath{-1.77}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.c1.pp\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.c1.ppalt\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.c1.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.c1.z\endcsname{\ensuremath{-2.1}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.c2.gap\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.c2.pp\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.c2.ppalt\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.c2.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.c2.z\endcsname{\ensuremath{-2.5}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.c3.gap\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.c3.pp\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.c3.ppalt\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.c3.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.c3.z\endcsname{\ensuremath{-0.8}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.head_pp\endcsname{\ensuremath{-0.252}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.head_ppalt\endcsname{\ensuremath{-0.259}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.maxz\endcsname{\ensuremath{-2.5}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.maxz_class\endcsname{MLV}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.maxz_pp\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.nneg2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.nneg2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.nrank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C1.acdc.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c1.gap\endcsname{\ensuremath{-2.53}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c1.pp\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c1.ppalt\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c1.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c1.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c10.gap\endcsname{\ensuremath{-1.62}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c10.pp\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c10.ppalt\endcsname{\ensuremath{-0.83}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c10.rank\endcsname{35}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c10.z\endcsname{\ensuremath{-1.5}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c11.gap\endcsname{\ensuremath{-1.64}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c11.pp\endcsname{\ensuremath{-0.71}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c11.ppalt\endcsname{\ensuremath{-0.72}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c11.rank\endcsname{33}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c11.z\endcsname{\ensuremath{-4.3}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c12.gap\endcsname{\ensuremath{-1.26}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c12.pp\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c12.ppalt\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c12.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c12.z\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c13.gap\endcsname{\ensuremath{-1.73}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c13.pp\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c13.ppalt\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c13.rank\endcsname{28}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c13.z\endcsname{\ensuremath{-0.8}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c14.gap\endcsname{\ensuremath{-1.64}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c14.pp\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c14.ppalt\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c14.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c14.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c15.gap\endcsname{\ensuremath{-3.02}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c15.pp\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c15.ppalt\endcsname{\ensuremath{+0.79}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c15.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c15.z\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c2.gap\endcsname{\ensuremath{-1.57}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c2.pp\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c2.ppalt\endcsname{\ensuremath{-1.15}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c2.rank\endcsname{33}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c2.z\endcsname{\ensuremath{-2.0}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c3.gap\endcsname{\ensuremath{-0.68}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c3.pp\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c3.ppalt\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c3.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c3.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c4.gap\endcsname{\ensuremath{-4.34}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c4.pp\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c4.ppalt\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c4.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c4.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c5.gap\endcsname{\ensuremath{-1.40}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c5.pp\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c5.ppalt\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c5.rank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c5.z\endcsname{\ensuremath{-1.9}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c6.gap\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c6.pp\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c6.ppalt\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c6.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c6.z\endcsname{\ensuremath{-0.3}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c7.gap\endcsname{\ensuremath{-1.01}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c7.pp\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c7.ppalt\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c7.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c7.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c8.gap\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c8.pp\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c8.ppalt\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c8.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c8.z\endcsname{\ensuremath{-1.2}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c9.gap\endcsname{\ensuremath{-0.82}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c9.pp\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c9.ppalt\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c9.rank\endcsname{27}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.c9.z\endcsname{\ensuremath{-0.4}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.head_pp\endcsname{\ensuremath{-0.106}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.head_ppalt\endcsname{\ensuremath{-0.135}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.maxz\endcsname{\ensuremath{-4.3}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.maxz_class\endcsname{right adrenal gland}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.maxz_pp\endcsname{\ensuremath{-0.71}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.nneg2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.nneg2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C1.amos.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.altflip\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c1.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c1.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c1.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c1.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c1.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c10.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c10.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c10.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c10.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c10.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c11.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c11.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c11.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c11.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c11.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c12.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c12.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c12.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c12.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c12.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c13.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c13.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c13.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c13.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c13.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c14.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c14.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c14.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c14.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c14.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c15.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c15.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c15.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c15.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c15.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c2.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c2.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c2.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c2.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c2.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c3.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c3.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c3.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c3.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c3.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c4.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c4.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c4.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c4.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c4.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c5.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c5.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c5.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c5.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c5.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c6.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c6.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c6.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c6.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c6.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c7.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c7.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c7.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c7.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c7.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c8.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c8.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c8.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c8.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c8.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c9.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c9.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c9.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c9.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.c9.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.head_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.head_ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.maxz\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.maxz_class\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.maxz_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.nneg2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.nneg2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.npos2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.npos2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.nrank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.nseed\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.pos2list\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.regstate\endcsname{queued}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.seedlist\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.amos.sumpos_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.c123.gap\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.c123.pp\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.c123.ppalt\endcsname{\ensuremath{+1.13}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.c123.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.c123.z\endcsname{\ensuremath{+3.5}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.c2.gap\endcsname{\ensuremath{-2.04}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.c2.pp\endcsname{\ensuremath{+3.06}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.c2.ppalt\endcsname{\ensuremath{+2.77}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.c2.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.c2.z\endcsname{\ensuremath{+3.1}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.c23.gap\endcsname{\ensuremath{-1.13}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.c23.pp\endcsname{\ensuremath{+3.01}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.c23.ppalt\endcsname{\ensuremath{+2.69}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.c23.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.c23.z\endcsname{\ensuremath{+3.1}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.head_pp\endcsname{\ensuremath{+2.440}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.head_ppalt\endcsname{\ensuremath{+2.196}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.maxz\endcsname{\ensuremath{+3.5}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.maxz_class\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.maxz_pp\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.pos2list\endcsname{kidney, tumour, masses}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.V7C1.fresh.kits.sumpos_pp\endcsname{\ensuremath{+7.32}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.c123.gap\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.c123.pp\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.c123.ppalt\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.c123.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.c123.z\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.c2.gap\endcsname{\ensuremath{-1.59}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.c2.pp\endcsname{\ensuremath{+3.39}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.c2.ppalt\endcsname{\ensuremath{+3.09}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.c2.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.c2.z\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.c23.gap\endcsname{\ensuremath{-0.67}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.c23.pp\endcsname{\ensuremath{+3.64}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.c23.ppalt\endcsname{\ensuremath{+3.32}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.c23.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.c23.z\endcsname{\ensuremath{+2.9}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.head_pp\endcsname{\ensuremath{+2.707}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.head_ppalt\endcsname{\ensuremath{+2.463}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.maxz\endcsname{\ensuremath{+2.9}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.maxz_pp\endcsname{\ensuremath{+3.64}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.pos2list\endcsname{masses, tumour, kidney}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C1.kits.sumpos_pp\endcsname{\ensuremath{+8.12}}
\expandafter\gdef\csname R@an.perclass_all.V7C1.params\endcsname{21.1}
\expandafter\gdef\csname R@an.perclass_all.V7C1.params.acdc\endcsname{20.3}
\expandafter\gdef\csname R@an.perclass_all.V7C1.params.amos\endcsname{21.1}
\expandafter\gdef\csname R@an.perclass_all.V7C1.params.kits\endcsname{21.1}
\expandafter\gdef\csname R@an.perclass_all.V7C1.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c1.gap\endcsname{\ensuremath{-3.21}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c1.pp\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c1.ppalt\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c1.rank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c1.z\endcsname{\ensuremath{-2.1}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c10.gap\endcsname{\ensuremath{-1.22}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c10.pp\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c10.ppalt\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c10.rank\endcsname{28}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c10.z\endcsname{\ensuremath{-0.5}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c11.gap\endcsname{\ensuremath{-2.10}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c11.pp\endcsname{\ensuremath{-1.17}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c11.ppalt\endcsname{\ensuremath{-1.17}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c11.rank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c11.z\endcsname{\ensuremath{-7.0}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c12.gap\endcsname{\ensuremath{-2.82}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c12.pp\endcsname{\ensuremath{-1.01}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c12.ppalt\endcsname{\ensuremath{-0.76}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c12.rank\endcsname{36}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c12.z\endcsname{\ensuremath{-1.1}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c13.gap\endcsname{\ensuremath{-2.48}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c13.pp\endcsname{\ensuremath{-1.09}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c13.ppalt\endcsname{\ensuremath{-1.03}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c13.rank\endcsname{33}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c13.z\endcsname{\ensuremath{-2.7}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c14.gap\endcsname{\ensuremath{-2.29}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c14.pp\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c14.ppalt\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c14.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c14.z\endcsname{\ensuremath{-0.7}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c15.gap\endcsname{\ensuremath{-3.18}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c15.pp\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c15.ppalt\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c15.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c15.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c2.gap\endcsname{\ensuremath{-1.61}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c2.pp\endcsname{\ensuremath{-0.96}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c2.ppalt\endcsname{\ensuremath{-1.20}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c2.rank\endcsname{34}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c2.z\endcsname{\ensuremath{-2.2}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c3.gap\endcsname{\ensuremath{-0.83}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c3.pp\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c3.ppalt\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c3.rank\endcsname{31}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c3.z\endcsname{\ensuremath{-0.5}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c4.gap\endcsname{\ensuremath{-3.42}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c4.pp\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c4.ppalt\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c4.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c4.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c5.gap\endcsname{\ensuremath{-1.32}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c5.pp\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c5.ppalt\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c5.rank\endcsname{29}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c5.z\endcsname{\ensuremath{-1.6}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c6.gap\endcsname{\ensuremath{-0.74}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c6.pp\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c6.ppalt\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c6.rank\endcsname{35}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c6.z\endcsname{\ensuremath{-2.1}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c7.gap\endcsname{\ensuremath{-1.37}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c7.pp\endcsname{\ensuremath{-0.41}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c7.ppalt\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c7.rank\endcsname{33}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c7.z\endcsname{\ensuremath{-1.4}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c8.gap\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c8.pp\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c8.ppalt\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c8.rank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c8.z\endcsname{\ensuremath{-2.3}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c9.gap\endcsname{\ensuremath{-0.84}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c9.pp\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c9.ppalt\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c9.rank\endcsname{29}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.c9.z\endcsname{\ensuremath{-0.5}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.head_pp\endcsname{\ensuremath{-0.362}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.head_ppalt\endcsname{\ensuremath{-0.390}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.maxz\endcsname{\ensuremath{-7.0}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.maxz_class\endcsname{right adrenal gland}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.maxz_pp\endcsname{\ensuremath{-1.17}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.nneg2\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.nneg2alt\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C2.amos.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.c123.gap\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.c123.pp\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.c123.ppalt\endcsname{\ensuremath{+0.95}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.c123.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.c123.z\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.c2.gap\endcsname{\ensuremath{-2.54}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.c2.pp\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.c2.ppalt\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.c2.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.c2.z\endcsname{\ensuremath{+2.0}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.c23.gap\endcsname{\ensuremath{-1.83}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.c23.pp\endcsname{\ensuremath{+2.49}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.c23.ppalt\endcsname{\ensuremath{+2.17}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.c23.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.c23.z\endcsname{\ensuremath{+2.0}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.head_pp\endcsname{\ensuremath{+2.000}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.head_ppalt\endcsname{\ensuremath{+1.757}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.maxz\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.maxz_class\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.maxz_pp\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.npos2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.pos2list\endcsname{kidney, masses}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V7C2.kits.sumpos_pp\endcsname{\ensuremath{+3.56}}
\expandafter\gdef\csname R@an.perclass_all.V7C2.params\endcsname{20.4}
\expandafter\gdef\csname R@an.perclass_all.V7C2.params.acdc\endcsname{19.7}
\expandafter\gdef\csname R@an.perclass_all.V7C2.params.amos\endcsname{20.4}
\expandafter\gdef\csname R@an.perclass_all.V7C2.params.kits\endcsname{20.5}
\expandafter\gdef\csname R@an.perclass_all.V7C2.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c1.gap\endcsname{\ensuremath{-4.20}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c1.pp\endcsname{\ensuremath{-1.60}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c1.ppalt\endcsname{\ensuremath{-1.66}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c1.rank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c1.z\endcsname{\ensuremath{-5.5}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c10.gap\endcsname{\ensuremath{-1.59}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c10.pp\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c10.ppalt\endcsname{\ensuremath{-0.81}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c10.rank\endcsname{34}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c10.z\endcsname{\ensuremath{-1.4}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c11.gap\endcsname{\ensuremath{-1.96}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c11.pp\endcsname{\ensuremath{-1.03}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c11.ppalt\endcsname{\ensuremath{-1.03}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c11.rank\endcsname{36}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c11.z\endcsname{\ensuremath{-6.2}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c12.gap\endcsname{\ensuremath{-2.43}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c12.pp\endcsname{\ensuremath{-0.62}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c12.ppalt\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c12.rank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c12.z\endcsname{\ensuremath{-0.7}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c13.gap\endcsname{\ensuremath{-2.65}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c13.pp\endcsname{\ensuremath{-1.26}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c13.ppalt\endcsname{\ensuremath{-1.20}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c13.rank\endcsname{37}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c13.z\endcsname{\ensuremath{-3.2}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c14.gap\endcsname{\ensuremath{-2.42}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c14.pp\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c14.ppalt\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c14.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c14.z\endcsname{\ensuremath{-1.2}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c15.gap\endcsname{\ensuremath{-1.69}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c15.pp\endcsname{\ensuremath{+1.79}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c15.ppalt\endcsname{\ensuremath{+2.13}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c15.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c15.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c2.gap\endcsname{\ensuremath{-1.95}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c2.pp\endcsname{\ensuremath{-1.30}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c2.ppalt\endcsname{\ensuremath{-1.53}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c2.rank\endcsname{37}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c2.z\endcsname{\ensuremath{-2.9}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c3.gap\endcsname{\ensuremath{-2.30}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c3.pp\endcsname{\ensuremath{-1.65}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c3.ppalt\endcsname{\ensuremath{-1.81}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c3.rank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c3.z\endcsname{\ensuremath{-4.6}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c4.gap\endcsname{\ensuremath{-4.15}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c4.pp\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c4.ppalt\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c4.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c4.z\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c5.gap\endcsname{\ensuremath{-1.79}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c5.pp\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c5.ppalt\endcsname{\ensuremath{-0.72}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c5.rank\endcsname{36}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c5.z\endcsname{\ensuremath{-3.1}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c6.gap\endcsname{\ensuremath{-0.65}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c6.pp\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c6.ppalt\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c6.rank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c6.z\endcsname{\ensuremath{-1.5}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c7.gap\endcsname{\ensuremath{-0.90}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c7.pp\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c7.ppalt\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c7.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c7.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c8.gap\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c8.pp\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c8.ppalt\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c8.rank\endcsname{33}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c8.z\endcsname{\ensuremath{-2.4}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c9.gap\endcsname{\ensuremath{-0.90}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c9.pp\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c9.ppalt\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c9.rank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.c9.z\endcsname{\ensuremath{-0.9}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.head_pp\endcsname{\ensuremath{-0.505}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.head_ppalt\endcsname{\ensuremath{-0.534}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.maxz\endcsname{\ensuremath{-6.2}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.maxz_class\endcsname{right adrenal gland}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.maxz_pp\endcsname{\ensuremath{-1.03}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.nneg2\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.nneg2alt\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A1.amos.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.c123.gap\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.c123.pp\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.c123.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.c123.z\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.c2.gap\endcsname{\ensuremath{-3.99}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.c2.pp\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.c2.ppalt\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.c2.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.c2.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.c23.gap\endcsname{\ensuremath{-2.26}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.c23.pp\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.c23.ppalt\endcsname{\ensuremath{+1.56}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.c23.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.c23.z\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.head_pp\endcsname{\ensuremath{+1.249}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.head_ppalt\endcsname{\ensuremath{+1.005}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.maxz\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.maxz_class\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.maxz_pp\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.pos2list\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.V8A1.fresh.kits.sumpos_pp\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.c123.gap\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.c123.pp\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.c123.ppalt\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.c123.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.c123.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.c2.gap\endcsname{\ensuremath{-3.02}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.c2.pp\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.c2.ppalt\endcsname{\ensuremath{+1.66}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.c2.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.c2.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.c23.gap\endcsname{\ensuremath{-1.73}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.c23.pp\endcsname{\ensuremath{+2.59}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.c23.ppalt\endcsname{\ensuremath{+2.27}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.c23.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.c23.z\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.head_pp\endcsname{\ensuremath{+1.760}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.head_ppalt\endcsname{\ensuremath{+1.516}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.maxz\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.maxz_pp\endcsname{\ensuremath{+2.59}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.pos2list\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A1.kits.sumpos_pp\endcsname{\ensuremath{+2.59}}
\expandafter\gdef\csname R@an.perclass_all.V8A1.params\endcsname{31.3}
\expandafter\gdef\csname R@an.perclass_all.V8A1.params.acdc\endcsname{30.5}
\expandafter\gdef\csname R@an.perclass_all.V8A1.params.amos\endcsname{31.3}
\expandafter\gdef\csname R@an.perclass_all.V8A1.params.kits\endcsname{31.3}
\expandafter\gdef\csname R@an.perclass_all.V8A1.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.altflip\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c1.gap\endcsname{\ensuremath{-2.63}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c1.pp\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c1.ppalt\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c1.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c1.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c10.gap\endcsname{\ensuremath{-0.83}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c10.pp\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c10.ppalt\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c10.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c10.z\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c11.gap\endcsname{\ensuremath{-1.36}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c11.pp\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c11.ppalt\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c11.rank\endcsname{28}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c11.z\endcsname{\ensuremath{-2.6}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c12.gap\endcsname{\ensuremath{-2.00}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c12.pp\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c12.ppalt\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c12.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c12.z\endcsname{\ensuremath{-0.2}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c13.gap\endcsname{\ensuremath{-1.91}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c13.pp\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c13.ppalt\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c13.rank\endcsname{31}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c13.z\endcsname{\ensuremath{-1.3}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c14.gap\endcsname{\ensuremath{-1.70}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c14.pp\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c14.ppalt\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c14.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c14.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c15.gap\endcsname{\ensuremath{-3.71}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c15.pp\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c15.ppalt\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c15.rank\endcsname{29}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c15.z\endcsname{\ensuremath{-0.2}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c2.gap\endcsname{\ensuremath{-1.68}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c2.pp\endcsname{\ensuremath{-1.03}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c2.ppalt\endcsname{\ensuremath{-1.27}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c2.rank\endcsname{35}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c2.z\endcsname{\ensuremath{-2.3}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c3.gap\endcsname{\ensuremath{-1.18}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c3.pp\endcsname{\ensuremath{-0.54}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c3.ppalt\endcsname{\ensuremath{-0.69}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c3.rank\endcsname{37}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c3.z\endcsname{\ensuremath{-1.5}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c4.gap\endcsname{\ensuremath{-5.76}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c4.pp\endcsname{\ensuremath{-1.09}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c4.ppalt\endcsname{\ensuremath{-1.70}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c4.rank\endcsname{30}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c4.z\endcsname{\ensuremath{-0.8}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c5.gap\endcsname{\ensuremath{-1.61}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c5.pp\endcsname{\ensuremath{-0.80}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c5.ppalt\endcsname{\ensuremath{-0.54}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c5.rank\endcsname{34}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c5.z\endcsname{\ensuremath{-2.6}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c6.gap\endcsname{\ensuremath{-0.58}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c6.pp\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c6.ppalt\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c6.rank\endcsname{28}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c6.z\endcsname{\ensuremath{-1.0}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c7.gap\endcsname{\ensuremath{-1.18}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c7.pp\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c7.ppalt\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c7.rank\endcsname{28}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c7.z\endcsname{\ensuremath{-0.7}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c8.gap\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c8.pp\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c8.ppalt\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c8.rank\endcsname{26}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c8.z\endcsname{\ensuremath{-1.9}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c9.gap\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c9.pp\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c9.ppalt\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c9.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.c9.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.head_pp\endcsname{\ensuremath{-0.312}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.head_ppalt\endcsname{\ensuremath{-0.341}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.maxz\endcsname{\ensuremath{-2.6}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.maxz_class\endcsname{right adrenal gland}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.maxz_pp\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.nneg2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.nneg2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A2.amos.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.c123.gap\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.c123.pp\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.c123.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.c123.z\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.c2.gap\endcsname{\ensuremath{-3.00}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.c2.pp\endcsname{\ensuremath{+2.09}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.c2.ppalt\endcsname{\ensuremath{+1.80}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.c2.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.c2.z\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.c23.gap\endcsname{\ensuremath{-1.46}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.c23.pp\endcsname{\ensuremath{+2.68}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.c23.ppalt\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.c23.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.c23.z\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.head_pp\endcsname{\ensuremath{+1.877}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.head_ppalt\endcsname{\ensuremath{+1.634}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.maxz\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.maxz_pp\endcsname{\ensuremath{+2.68}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.npos2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.pos2list\endcsname{masses, kidney, tumour}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.V8A2.fresh.kits.sumpos_pp\endcsname{\ensuremath{+5.63}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.c123.gap\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.c123.pp\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.c123.ppalt\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.c123.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.c123.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.c2.gap\endcsname{\ensuremath{-3.41}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.c2.pp\endcsname{\ensuremath{+1.57}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.c2.ppalt\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.c2.rank\endcsname{26}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.c2.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.c23.gap\endcsname{\ensuremath{-2.63}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.c23.pp\endcsname{\ensuremath{+1.69}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.c23.ppalt\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.c23.rank\endcsname{29}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.c23.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.head_pp\endcsname{\ensuremath{+1.353}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.head_ppalt\endcsname{\ensuremath{+1.110}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.maxz\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.maxz_class\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.maxz_pp\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8A2.kits.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V8A2.params\endcsname{31.4}
\expandafter\gdef\csname R@an.perclass_all.V8A2.params.acdc\endcsname{30.7}
\expandafter\gdef\csname R@an.perclass_all.V8A2.params.amos\endcsname{31.4}
\expandafter\gdef\csname R@an.perclass_all.V8A2.params.kits\endcsname{31.5}
\expandafter\gdef\csname R@an.perclass_all.V8A2.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c1.gap\endcsname{\ensuremath{-3.72}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c1.pp\endcsname{\ensuremath{-1.12}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c1.ppalt\endcsname{\ensuremath{-1.17}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c1.rank\endcsname{34}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c1.z\endcsname{\ensuremath{-3.9}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c10.gap\endcsname{\ensuremath{-1.92}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c10.pp\endcsname{\ensuremath{-0.90}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c10.ppalt\endcsname{\ensuremath{-1.14}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c10.rank\endcsname{36}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c10.z\endcsname{\ensuremath{-2.2}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c11.gap\endcsname{\ensuremath{-1.96}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c11.pp\endcsname{\ensuremath{-1.03}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c11.ppalt\endcsname{\ensuremath{-1.03}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c11.rank\endcsname{37}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c11.z\endcsname{\ensuremath{-6.2}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c12.gap\endcsname{\ensuremath{-3.21}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c12.pp\endcsname{\ensuremath{-1.40}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c12.ppalt\endcsname{\ensuremath{-1.15}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c12.rank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c12.z\endcsname{\ensuremath{-1.5}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c13.gap\endcsname{\ensuremath{-2.64}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c13.pp\endcsname{\ensuremath{-1.25}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c13.ppalt\endcsname{\ensuremath{-1.20}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c13.rank\endcsname{36}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c13.z\endcsname{\ensuremath{-3.2}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c14.gap\endcsname{\ensuremath{-1.50}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c14.pp\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c14.ppalt\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c14.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c14.z\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c15.gap\endcsname{\ensuremath{-3.73}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c15.pp\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c15.ppalt\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c15.rank\endcsname{30}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c15.z\endcsname{\ensuremath{-0.2}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c2.gap\endcsname{\ensuremath{-1.51}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c2.pp\endcsname{\ensuremath{-0.86}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c2.ppalt\endcsname{\ensuremath{-1.10}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c2.rank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c2.z\endcsname{\ensuremath{-1.9}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c3.gap\endcsname{\ensuremath{-0.73}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c3.pp\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c3.ppalt\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c3.rank\endcsname{27}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c3.z\endcsname{\ensuremath{-0.2}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c4.gap\endcsname{\ensuremath{-7.44}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c4.pp\endcsname{\ensuremath{-2.78}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c4.ppalt\endcsname{\ensuremath{-3.39}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c4.rank\endcsname{36}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c4.z\endcsname{\ensuremath{-2.1}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c5.gap\endcsname{\ensuremath{-1.73}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c5.pp\endcsname{\ensuremath{-0.93}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c5.ppalt\endcsname{\ensuremath{-0.67}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c5.rank\endcsname{35}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c5.z\endcsname{\ensuremath{-2.9}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c6.gap\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c6.pp\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c6.ppalt\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c6.rank\endcsname{31}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c6.z\endcsname{\ensuremath{-1.4}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c7.gap\endcsname{\ensuremath{-1.44}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c7.pp\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c7.ppalt\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c7.rank\endcsname{35}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c7.z\endcsname{\ensuremath{-1.7}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c8.gap\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c8.pp\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c8.ppalt\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c8.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c8.z\endcsname{\ensuremath{-1.7}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c9.gap\endcsname{\ensuremath{-1.16}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c9.pp\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c9.ppalt\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c9.rank\endcsname{37}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.c9.z\endcsname{\ensuremath{-3.0}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.head_pp\endcsname{\ensuremath{-0.751}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.head_ppalt\endcsname{\ensuremath{-0.779}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.maxz\endcsname{\ensuremath{-6.2}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.maxz_class\endcsname{right adrenal gland}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.maxz_pp\endcsname{\ensuremath{-1.03}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.nneg2\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.nneg2alt\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.pos2list\endcsname{bladder}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8B1.amos.sumpos_pp\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.c123.gap\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.c123.pp\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.c123.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.c123.z\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.c2.gap\endcsname{\ensuremath{-3.58}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.c2.pp\endcsname{\ensuremath{+1.51}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.c2.ppalt\endcsname{\ensuremath{+1.22}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.c2.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.c2.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.c23.gap\endcsname{\ensuremath{-2.30}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.c23.pp\endcsname{\ensuremath{+1.84}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.c23.ppalt\endcsname{\ensuremath{+1.52}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.c23.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.c23.z\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.head_pp\endcsname{\ensuremath{+1.375}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.head_ppalt\endcsname{\ensuremath{+1.131}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.maxz\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.maxz_class\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.maxz_pp\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.pos2list\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.V8B1.fresh.kits.sumpos_pp\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.c123.gap\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.c123.pp\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.c123.ppalt\endcsname{\ensuremath{+1.06}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.c123.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.c123.z\endcsname{\ensuremath{+2.6}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.c2.gap\endcsname{\ensuremath{-0.97}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.c2.pp\endcsname{\ensuremath{+4.01}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.c2.ppalt\endcsname{\ensuremath{+3.72}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.c2.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.c2.z\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.c23.gap\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.c23.pp\endcsname{\ensuremath{+3.55}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.c23.ppalt\endcsname{\ensuremath{+3.22}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.c23.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.c23.z\endcsname{\ensuremath{+2.9}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.head_pp\endcsname{\ensuremath{+2.911}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.head_ppalt\endcsname{\ensuremath{+2.667}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.maxz\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.maxz_pp\endcsname{\ensuremath{+4.01}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.pos2list\endcsname{tumour, masses, kidney}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8B1.kits.sumpos_pp\endcsname{\ensuremath{+8.73}}
\expandafter\gdef\csname R@an.perclass_all.V8B1.params\endcsname{18.2}
\expandafter\gdef\csname R@an.perclass_all.V8B1.params.acdc\endcsname{17.4}
\expandafter\gdef\csname R@an.perclass_all.V8B1.params.amos\endcsname{18.2}
\expandafter\gdef\csname R@an.perclass_all.V8B1.params.kits\endcsname{18.2}
\expandafter\gdef\csname R@an.perclass_all.V8B1.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c1.gap\endcsname{\ensuremath{-2.79}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c1.pp\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c1.ppalt\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c1.rank\endcsname{27}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c1.z\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c10.gap\endcsname{\ensuremath{-1.42}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c10.pp\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c10.ppalt\endcsname{\ensuremath{-0.64}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c10.rank\endcsname{33}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c10.z\endcsname{\ensuremath{-1.0}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c11.gap\endcsname{\ensuremath{-1.58}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c11.pp\endcsname{\ensuremath{-0.65}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c11.ppalt\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c11.rank\endcsname{31}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c11.z\endcsname{\ensuremath{-3.9}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c12.gap\endcsname{\ensuremath{-2.37}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c12.pp\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c12.ppalt\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c12.rank\endcsname{31}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c12.z\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c13.gap\endcsname{\ensuremath{-2.04}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c13.pp\endcsname{\ensuremath{-0.65}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c13.ppalt\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c13.rank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c13.z\endcsname{\ensuremath{-1.6}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c14.gap\endcsname{\ensuremath{-1.86}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c14.pp\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c14.ppalt\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c14.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c14.z\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c15.gap\endcsname{\ensuremath{-3.91}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c15.pp\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c15.ppalt\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c15.rank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c15.z\endcsname{\ensuremath{-0.4}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c2.gap\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c2.pp\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c2.ppalt\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c2.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c2.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c3.gap\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c3.pp\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c3.ppalt\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c3.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c3.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c4.gap\endcsname{\ensuremath{-5.66}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c4.pp\endcsname{\ensuremath{-0.99}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c4.ppalt\endcsname{\ensuremath{-1.60}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c4.rank\endcsname{27}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c4.z\endcsname{\ensuremath{-0.7}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c5.gap\endcsname{\ensuremath{-1.29}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c5.pp\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c5.ppalt\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c5.rank\endcsname{27}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c5.z\endcsname{\ensuremath{-1.5}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c6.gap\endcsname{\ensuremath{-0.76}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c6.pp\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c6.ppalt\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c6.rank\endcsname{36}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c6.z\endcsname{\ensuremath{-2.2}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c7.gap\endcsname{\ensuremath{-1.18}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c7.pp\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c7.ppalt\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c7.rank\endcsname{29}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c7.z\endcsname{\ensuremath{-0.8}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c8.gap\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c8.pp\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c8.ppalt\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c8.rank\endcsname{31}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c8.z\endcsname{\ensuremath{-2.3}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c9.gap\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c9.pp\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c9.ppalt\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c9.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.c9.z\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.head_pp\endcsname{\ensuremath{-0.287}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.head_ppalt\endcsname{\ensuremath{-0.316}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.maxz\endcsname{\ensuremath{-3.9}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.maxz_class\endcsname{right adrenal gland}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.maxz_pp\endcsname{\ensuremath{-0.65}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.nneg2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.nneg2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8B2.amos.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.altflip\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c1.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c1.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c1.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c1.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c1.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c10.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c10.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c10.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c10.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c10.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c11.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c11.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c11.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c11.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c11.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c12.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c12.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c12.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c12.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c12.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c13.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c13.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c13.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c13.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c13.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c14.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c14.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c14.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c14.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c14.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c15.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c15.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c15.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c15.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c15.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c2.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c2.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c2.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c2.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c2.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c3.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c3.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c3.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c3.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c3.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c4.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c4.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c4.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c4.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c4.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c5.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c5.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c5.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c5.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c5.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c6.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c6.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c6.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c6.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c6.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c7.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c7.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c7.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c7.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c7.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c8.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c8.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c8.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c8.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c8.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c9.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c9.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c9.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c9.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.c9.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.head_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.head_ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.maxz\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.maxz_class\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.maxz_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.nneg2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.nneg2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.npos2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.npos2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.nrank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.nseed\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.pos2list\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.regstate\endcsname{queued}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.seedlist\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.amos.sumpos_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.altflip\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.c123.gap\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.c123.pp\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.c123.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.c123.z\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.c2.gap\endcsname{\ensuremath{-2.72}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.c2.pp\endcsname{\ensuremath{+2.37}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.c2.ppalt\endcsname{\ensuremath{+2.08}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.c2.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.c2.z\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.c23.gap\endcsname{\ensuremath{-2.08}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.c23.pp\endcsname{\ensuremath{+2.07}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.c23.ppalt\endcsname{\ensuremath{+1.75}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.c23.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.c23.z\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.head_pp\endcsname{\ensuremath{+1.731}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.head_ppalt\endcsname{\ensuremath{+1.487}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.maxz\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.maxz_pp\endcsname{\ensuremath{+2.37}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.pos2list\endcsname{tumour, kidney, masses}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.V8B2.fresh.kits.sumpos_pp\endcsname{\ensuremath{+5.19}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.c123.gap\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.c123.pp\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.c123.ppalt\endcsname{\ensuremath{+0.91}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.c123.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.c123.z\endcsname{\ensuremath{+2.3}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.c2.gap\endcsname{\ensuremath{-3.05}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.c2.pp\endcsname{\ensuremath{+1.93}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.c2.ppalt\endcsname{\ensuremath{+1.64}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.c2.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.c2.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.c23.gap\endcsname{\ensuremath{-2.34}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.c23.pp\endcsname{\ensuremath{+1.98}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.c23.ppalt\endcsname{\ensuremath{+1.66}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.c23.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.c23.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.head_pp\endcsname{\ensuremath{+1.646}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.head_ppalt\endcsname{\ensuremath{+1.402}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.maxz\endcsname{\ensuremath{+2.3}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.maxz_class\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.maxz_pp\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.pos2list\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8B2.kits.sumpos_pp\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.perclass_all.V8B2.params\endcsname{21.1}
\expandafter\gdef\csname R@an.perclass_all.V8B2.params.acdc\endcsname{20.3}
\expandafter\gdef\csname R@an.perclass_all.V8B2.params.amos\endcsname{21.1}
\expandafter\gdef\csname R@an.perclass_all.V8B2.params.kits\endcsname{21.1}
\expandafter\gdef\csname R@an.perclass_all.V8B2.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.altflip\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c1.gap\endcsname{\ensuremath{-3.96}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c1.pp\endcsname{\ensuremath{-1.35}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c1.ppalt\endcsname{\ensuremath{-1.41}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c1.rank\endcsname{35}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c1.z\endcsname{\ensuremath{-4.7}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c10.gap\endcsname{\ensuremath{-1.35}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c10.pp\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c10.ppalt\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c10.rank\endcsname{30}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c10.z\endcsname{\ensuremath{-0.8}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c11.gap\endcsname{\ensuremath{-1.89}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c11.pp\endcsname{\ensuremath{-0.95}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c11.ppalt\endcsname{\ensuremath{-0.96}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c11.rank\endcsname{34}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c11.z\endcsname{\ensuremath{-5.8}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c12.gap\endcsname{\ensuremath{-2.08}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c12.pp\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c12.ppalt\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c12.rank\endcsname{30}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c12.z\endcsname{\ensuremath{-0.3}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c13.gap\endcsname{\ensuremath{-2.55}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c13.pp\endcsname{\ensuremath{-1.15}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c13.ppalt\endcsname{\ensuremath{-1.10}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c13.rank\endcsname{35}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c13.z\endcsname{\ensuremath{-2.9}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c14.gap\endcsname{\ensuremath{-1.78}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c14.pp\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c14.ppalt\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c14.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c14.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c15.gap\endcsname{\ensuremath{-3.49}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c15.pp\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c15.ppalt\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c15.rank\endcsname{26}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c15.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c2.gap\endcsname{\ensuremath{-1.87}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c2.pp\endcsname{\ensuremath{-1.22}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c2.ppalt\endcsname{\ensuremath{-1.45}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c2.rank\endcsname{36}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c2.z\endcsname{\ensuremath{-2.7}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c3.gap\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c3.pp\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c3.ppalt\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c3.rank\endcsname{29}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c3.z\endcsname{\ensuremath{-0.3}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c4.gap\endcsname{\ensuremath{-3.30}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c4.pp\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c4.ppalt\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c4.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c4.z\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c5.gap\endcsname{\ensuremath{-1.50}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c5.pp\endcsname{\ensuremath{-0.70}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c5.ppalt\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c5.rank\endcsname{33}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c5.z\endcsname{\ensuremath{-2.2}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c6.gap\endcsname{\ensuremath{-0.72}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c6.pp\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c6.ppalt\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c6.rank\endcsname{33}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c6.z\endcsname{\ensuremath{-2.0}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c7.gap\endcsname{\ensuremath{-1.40}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c7.pp\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c7.ppalt\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c7.rank\endcsname{34}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c7.z\endcsname{\ensuremath{-1.5}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c8.gap\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c8.pp\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c8.ppalt\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c8.rank\endcsname{34}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c8.z\endcsname{\ensuremath{-2.4}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c9.gap\endcsname{\ensuremath{-0.76}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c9.pp\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c9.ppalt\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c9.rank\endcsname{26}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.c9.z\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.head_pp\endcsname{\ensuremath{-0.361}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.head_ppalt\endcsname{\ensuremath{-0.390}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.maxz\endcsname{\ensuremath{-5.8}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.maxz_class\endcsname{right adrenal gland}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.maxz_pp\endcsname{\ensuremath{-0.95}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.nneg2\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.nneg2alt\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8X1.amos.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.c123.gap\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.c123.pp\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.c123.ppalt\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.c123.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.c123.z\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.c2.gap\endcsname{\ensuremath{-1.77}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.c2.pp\endcsname{\ensuremath{+3.21}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.c2.ppalt\endcsname{\ensuremath{+2.92}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.c2.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.c2.z\endcsname{\ensuremath{+2.6}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.c23.gap\endcsname{\ensuremath{-0.91}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.c23.pp\endcsname{\ensuremath{+3.41}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.c23.ppalt\endcsname{\ensuremath{+3.09}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.c23.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.c23.z\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.head_pp\endcsname{\ensuremath{+2.535}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.head_ppalt\endcsname{\ensuremath{+2.291}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.maxz\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.maxz_pp\endcsname{\ensuremath{+3.41}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.npos2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.pos2list\endcsname{masses, tumour, kidney}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.V8X1.kits.sumpos_pp\endcsname{\ensuremath{+7.60}}
\expandafter\gdef\csname R@an.perclass_all.V8X1.params\endcsname{18.2}
\expandafter\gdef\csname R@an.perclass_all.V8X1.params.acdc\endcsname{17.6}
\expandafter\gdef\csname R@an.perclass_all.V8X1.params.amos\endcsname{18.2}
\expandafter\gdef\csname R@an.perclass_all.V8X1.params.kits\endcsname{18.2}
\expandafter\gdef\csname R@an.perclass_all.V8X1.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c1.gap\endcsname{\ensuremath{-2.54}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c1.pp\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c1.ppalt\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c1.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c1.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c10.gap\endcsname{\ensuremath{-0.78}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c10.pp\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c10.ppalt\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c10.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c10.z\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c11.gap\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c11.pp\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c11.ppalt\endcsname{\ensuremath{+0.72}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c11.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c11.z\endcsname{\ensuremath{+4.4}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c12.gap\endcsname{\ensuremath{-1.40}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c12.pp\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c12.ppalt\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c12.rank\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c12.z\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c13.gap\endcsname{\ensuremath{-1.51}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c13.pp\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c13.ppalt\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c13.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c13.z\endcsname{\ensuremath{-0.3}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c14.gap\endcsname{\ensuremath{-3.42}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c14.pp\endcsname{\ensuremath{-1.32}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c14.ppalt\endcsname{\ensuremath{-1.34}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c14.rank\endcsname{35}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c14.z\endcsname{\ensuremath{-5.2}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c15.gap\endcsname{\ensuremath{-3.49}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c15.pp\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c15.ppalt\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c15.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c15.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c2.gap\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c2.pp\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c2.ppalt\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c2.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c2.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c3.gap\endcsname{\ensuremath{-0.88}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c3.pp\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c3.ppalt\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c3.rank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c3.z\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c4.gap\endcsname{\ensuremath{-3.49}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c4.pp\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c4.ppalt\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c4.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c4.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c5.gap\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c5.pp\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c5.ppalt\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c5.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c5.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c6.gap\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c6.pp\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c6.ppalt\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c6.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c6.z\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c7.gap\endcsname{\ensuremath{-0.82}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c7.pp\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c7.ppalt\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c7.rank\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c7.z\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c8.gap\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c8.pp\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c8.ppalt\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c8.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c8.z\endcsname{\ensuremath{-0.3}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c9.gap\endcsname{\ensuremath{-0.67}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c9.pp\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c9.ppalt\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c9.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.c9.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.head_pp\endcsname{\ensuremath{+0.099}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.head_ppalt\endcsname{\ensuremath{+0.071}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.maxz\endcsname{\ensuremath{-5.2}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.maxz_class\endcsname{bladder}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.maxz_pp\endcsname{\ensuremath{-1.32}}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.nneg2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.nneg2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.pos2list\endcsname{right adrenal gland}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W1.amos.sumpos_pp\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.perclass_all.W1.params\endcsname{31.1}
\expandafter\gdef\csname R@an.perclass_all.W1.params.acdc\endcsname{30.4}
\expandafter\gdef\csname R@an.perclass_all.W1.params.amos\endcsname{31.1}
\expandafter\gdef\csname R@an.perclass_all.W1.params.kits\endcsname{31.2}
\expandafter\gdef\csname R@an.perclass_all.W1.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c1.gap\endcsname{\ensuremath{-2.65}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c1.pp\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c1.ppalt\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c1.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c1.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c10.gap\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c10.pp\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c10.ppalt\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c10.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c10.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c11.gap\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c11.pp\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c11.ppalt\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c11.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c11.z\endcsname{\ensuremath{-0.3}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c12.gap\endcsname{\ensuremath{-1.71}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c12.pp\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c12.ppalt\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c12.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c12.z\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c13.gap\endcsname{\ensuremath{-1.34}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c13.pp\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c13.ppalt\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c13.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c13.z\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c14.gap\endcsname{\ensuremath{-3.07}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c14.pp\endcsname{\ensuremath{-0.97}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c14.ppalt\endcsname{\ensuremath{-0.99}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c14.rank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c14.z\endcsname{\ensuremath{-3.8}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c15.gap\endcsname{\ensuremath{-1.10}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c15.pp\endcsname{\ensuremath{+2.38}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c15.ppalt\endcsname{\ensuremath{+2.72}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c15.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c15.z\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c2.gap\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c2.pp\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c2.ppalt\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c2.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c2.z\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c3.gap\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c3.pp\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c3.ppalt\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c3.rank\endcsname{28}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c3.z\endcsname{\ensuremath{-0.3}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c4.gap\endcsname{\ensuremath{-2.75}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c4.pp\endcsname{\ensuremath{+1.92}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c4.ppalt\endcsname{\ensuremath{+1.31}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c4.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c4.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c5.gap\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c5.pp\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c5.ppalt\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c5.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c5.z\endcsname{\ensuremath{-0.4}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c6.gap\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c6.pp\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c6.ppalt\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c6.rank\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c6.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c7.gap\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c7.pp\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c7.ppalt\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c7.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c7.z\endcsname{\ensuremath{+2.3}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c8.gap\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c8.pp\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c8.ppalt\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c8.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c8.z\endcsname{\ensuremath{-0.3}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c9.gap\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c9.pp\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c9.ppalt\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c9.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.c9.z\endcsname{\ensuremath{+4.9}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.head_pp\endcsname{\ensuremath{+0.363}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.head_ppalt\endcsname{\ensuremath{+0.334}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.maxz\endcsname{\ensuremath{+4.9}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.maxz_class\endcsname{postcava}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.maxz_pp\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.nneg2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.nneg2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.pos2list\endcsname{postcava, stomach, prostate/uterus}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W1c.amos.sumpos_pp\endcsname{\ensuremath{+3.63}}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.c123.gap\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.c123.pp\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.c123.ppalt\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.c123.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.c123.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.c2.gap\endcsname{\ensuremath{-3.70}}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.c2.pp\endcsname{\ensuremath{+1.39}}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.c2.ppalt\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.c2.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.c2.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.c23.gap\endcsname{\ensuremath{-2.61}}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.c23.pp\endcsname{\ensuremath{+1.54}}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.c23.ppalt\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.c23.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.c23.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.estimand\endcsname{fresh mean of seeds 1--2}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.head_pp\endcsname{\ensuremath{+1.067}}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.head_ppalt\endcsname{\ensuremath{+0.823}}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.maxz\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.maxz_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.maxz_pp\endcsname{\ensuremath{+1.54}}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.nrank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.nseed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.seedlist\endcsname{1, 2}
\expandafter\gdef\csname R@an.perclass_all.W1c.fresh.kits.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.c123.gap\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.c123.pp\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.c123.ppalt\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.c123.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.c123.z\endcsname{\ensuremath{+2.5}}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.c2.gap\endcsname{\ensuremath{-1.49}}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.c2.pp\endcsname{\ensuremath{+3.49}}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.c2.ppalt\endcsname{\ensuremath{+3.20}}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.c2.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.c2.z\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.c23.gap\endcsname{\ensuremath{-1.02}}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.c23.pp\endcsname{\ensuremath{+3.30}}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.c23.ppalt\endcsname{\ensuremath{+2.98}}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.c23.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.c23.z\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.head_pp\endcsname{\ensuremath{+2.636}}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.head_ppalt\endcsname{\ensuremath{+2.392}}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.maxz\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.maxz_pp\endcsname{\ensuremath{+3.49}}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.nrank\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.pos2list\endcsname{tumour, masses, kidney}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W1c.kits.sumpos_pp\endcsname{\ensuremath{+7.91}}
\expandafter\gdef\csname R@an.perclass_all.W1c.params\endcsname{31.1}
\expandafter\gdef\csname R@an.perclass_all.W1c.params.acdc\endcsname{30.4}
\expandafter\gdef\csname R@an.perclass_all.W1c.params.amos\endcsname{31.1}
\expandafter\gdef\csname R@an.perclass_all.W1c.params.kits\endcsname{31.2}
\expandafter\gdef\csname R@an.perclass_all.W1c.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c1.gap\endcsname{\ensuremath{-3.22}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c1.pp\endcsname{\ensuremath{-0.62}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c1.ppalt\endcsname{\ensuremath{-0.67}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c1.rank\endcsname{33}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c1.z\endcsname{\ensuremath{-2.1}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c10.gap\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c10.pp\endcsname{\ensuremath{+0.79}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c10.ppalt\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c10.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c10.z\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c11.gap\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c11.pp\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c11.ppalt\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c11.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c11.z\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c12.gap\endcsname{\ensuremath{-2.91}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c12.pp\endcsname{\ensuremath{-1.10}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c12.ppalt\endcsname{\ensuremath{-0.84}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c12.rank\endcsname{37}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c12.z\endcsname{\ensuremath{-1.2}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c13.gap\endcsname{\ensuremath{-1.63}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c13.pp\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c13.ppalt\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c13.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c13.z\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c14.gap\endcsname{\ensuremath{-1.95}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c14.pp\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c14.ppalt\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c14.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c14.z\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c15.gap\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c15.pp\endcsname{\ensuremath{+2.96}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c15.ppalt\endcsname{\ensuremath{+3.30}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c15.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c15.z\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c2.gap\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c2.pp\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c2.ppalt\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c2.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c2.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c3.gap\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c3.pp\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c3.ppalt\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c3.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c3.z\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c4.gap\endcsname{\ensuremath{-4.33}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c4.pp\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c4.ppalt\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c4.rank\endcsname{19}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c4.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c5.gap\endcsname{\ensuremath{-0.54}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c5.pp\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c5.ppalt\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c5.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c5.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c6.gap\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c6.pp\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c6.ppalt\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c6.rank\endcsname{26}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c6.z\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c7.gap\endcsname{\ensuremath{-1.08}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c7.pp\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c7.ppalt\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c7.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c7.z\endcsname{\ensuremath{-0.4}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c8.gap\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c8.pp\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c8.ppalt\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c8.rank\endcsname{30}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c8.z\endcsname{\ensuremath{-2.2}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c9.gap\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c9.pp\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c9.ppalt\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c9.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.c9.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.head_pp\endcsname{\ensuremath{+0.211}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.head_ppalt\endcsname{\ensuremath{+0.182}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.maxz\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.maxz_class\endcsname{right adrenal gland}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.maxz_pp\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.nneg2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.nneg2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.npos2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.npos2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.pos2list\endcsname{right adrenal gland, prostate/uterus}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W2.amos.sumpos_pp\endcsname{\ensuremath{+3.50}}
\expandafter\gdef\csname R@an.perclass_all.W2.params\endcsname{31.1}
\expandafter\gdef\csname R@an.perclass_all.W2.params.acdc\endcsname{30.4}
\expandafter\gdef\csname R@an.perclass_all.W2.params.amos\endcsname{31.1}
\expandafter\gdef\csname R@an.perclass_all.W2.params.kits\endcsname{31.2}
\expandafter\gdef\csname R@an.perclass_all.W2.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.altflip\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c1.gap\endcsname{\ensuremath{-2.22}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c1.pp\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c1.ppalt\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c1.rank\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c1.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c10.gap\endcsname{\ensuremath{-0.60}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c10.pp\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c10.ppalt\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c10.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c10.z\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c11.gap\endcsname{\ensuremath{-1.13}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c11.pp\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c11.ppalt\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c11.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c11.z\endcsname{\ensuremath{-1.2}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c12.gap\endcsname{\ensuremath{-2.03}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c12.pp\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c12.ppalt\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c12.rank\endcsname{27}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c12.z\endcsname{\ensuremath{-0.2}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c13.gap\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c13.pp\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c13.ppalt\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c13.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c13.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c14.gap\endcsname{\ensuremath{-3.16}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c14.pp\endcsname{\ensuremath{-1.06}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c14.ppalt\endcsname{\ensuremath{-1.08}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c14.rank\endcsname{34}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c14.z\endcsname{\ensuremath{-4.1}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c15.gap\endcsname{\ensuremath{-2.13}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c15.pp\endcsname{\ensuremath{+1.35}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c15.ppalt\endcsname{\ensuremath{+1.68}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c15.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c15.z\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c2.gap\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c2.pp\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c2.ppalt\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c2.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c2.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c3.gap\endcsname{\ensuremath{-0.73}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c3.pp\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c3.ppalt\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c3.rank\endcsname{26}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c3.z\endcsname{\ensuremath{-0.2}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c4.gap\endcsname{\ensuremath{-2.09}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c4.pp\endcsname{\ensuremath{+2.58}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c4.ppalt\endcsname{\ensuremath{+1.97}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c4.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c4.z\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c5.gap\endcsname{\ensuremath{-1.04}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c5.pp\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c5.ppalt\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c5.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c5.z\endcsname{\ensuremath{-0.7}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c6.gap\endcsname{\ensuremath{-0.73}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c6.pp\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c6.ppalt\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c6.rank\endcsname{34}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c6.z\endcsname{\ensuremath{-2.0}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c7.gap\endcsname{\ensuremath{-1.13}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c7.pp\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c7.ppalt\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c7.rank\endcsname{27}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c7.z\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c8.gap\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c8.pp\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c8.ppalt\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c8.rank\endcsname{13}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c8.z\endcsname{\ensuremath{-0.4}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c9.gap\endcsname{\ensuremath{-0.54}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c9.pp\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c9.ppalt\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c9.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.c9.z\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.head_pp\endcsname{\ensuremath{+0.270}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.head_ppalt\endcsname{\ensuremath{+0.241}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.maxz\endcsname{\ensuremath{-4.1}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.maxz_class\endcsname{bladder}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.maxz_pp\endcsname{\ensuremath{-1.06}}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.nneg2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.nneg2alt\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.npos2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.pos2list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W3.amos.sumpos_pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.W3.params\endcsname{29.6}
\expandafter\gdef\csname R@an.perclass_all.W3.params.acdc\endcsname{29.6}
\expandafter\gdef\csname R@an.perclass_all.W3.params.amos\endcsname{29.6}
\expandafter\gdef\csname R@an.perclass_all.W3.params.kits\endcsname{29.6}
\expandafter\gdef\csname R@an.perclass_all.W3.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c1.gap\endcsname{\ensuremath{-2.54}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c1.pp\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c1.ppalt\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c1.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c1.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c10.gap\endcsname{\ensuremath{-1.07}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c10.pp\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c10.ppalt\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c10.rank\endcsname{27}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c10.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c11.gap\endcsname{\ensuremath{-1.07}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c11.pp\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c11.ppalt\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c11.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c11.z\endcsname{\ensuremath{-0.8}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c12.gap\endcsname{\ensuremath{-1.79}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c12.pp\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c12.ppalt\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c12.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c12.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c13.gap\endcsname{\ensuremath{-1.09}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c13.pp\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c13.ppalt\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c13.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c13.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c14.gap\endcsname{\ensuremath{-2.59}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c14.pp\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c14.ppalt\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c14.rank\endcsname{26}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c14.z\endcsname{\ensuremath{-1.9}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c15.gap\endcsname{\ensuremath{-3.18}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c15.pp\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c15.ppalt\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c15.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c15.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c2.gap\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c2.pp\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c2.ppalt\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c2.rank\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c2.z\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c3.gap\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c3.pp\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c3.ppalt\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c3.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c3.z\endcsname{0.0}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c4.gap\endcsname{\ensuremath{-2.94}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c4.pp\endcsname{\ensuremath{+1.73}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c4.ppalt\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c4.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c4.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c5.gap\endcsname{\ensuremath{-0.88}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c5.pp\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c5.ppalt\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c5.rank\endcsname{20}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c5.z\endcsname{\ensuremath{-0.2}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c6.gap\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c6.pp\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c6.ppalt\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c6.rank\endcsname{27}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c6.z\endcsname{\ensuremath{-1.0}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c7.gap\endcsname{\ensuremath{-1.00}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c7.pp\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c7.ppalt\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c7.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c7.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c8.gap\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c8.pp\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c8.ppalt\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c8.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c8.z\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c9.gap\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c9.pp\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c9.ppalt\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c9.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.c9.z\endcsname{\ensuremath{+4.0}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.head_pp\endcsname{\ensuremath{+0.162}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.head_ppalt\endcsname{\ensuremath{+0.133}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.maxz\endcsname{\ensuremath{+4.0}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.maxz_class\endcsname{postcava}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.maxz_pp\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.pos2list\endcsname{postcava}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W3c.amos.sumpos_pp\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.perclass_all.W3c.params\endcsname{29.5}
\expandafter\gdef\csname R@an.perclass_all.W3c.params.acdc\endcsname{29.5}
\expandafter\gdef\csname R@an.perclass_all.W3c.params.amos\endcsname{29.5}
\expandafter\gdef\csname R@an.perclass_all.W3c.params.kits\endcsname{29.6}
\expandafter\gdef\csname R@an.perclass_all.W3c.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.altflip\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c1.gap\endcsname{\ensuremath{-2.30}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c1.pp\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c1.ppalt\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c1.rank\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c1.z\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c10.gap\endcsname{\ensuremath{-0.69}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c10.pp\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c10.ppalt\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c10.rank\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c10.z\endcsname{\ensuremath{+0.8}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c11.gap\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c11.pp\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c11.ppalt\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c11.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c11.z\endcsname{\ensuremath{+4.0}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c12.gap\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c12.pp\endcsname{\ensuremath{+1.33}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c12.ppalt\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c12.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c12.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c13.gap\endcsname{\ensuremath{-1.29}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c13.pp\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c13.ppalt\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c13.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c13.z\endcsname{\ensuremath{+0.2}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c14.gap\endcsname{\ensuremath{-4.92}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c14.pp\endcsname{\ensuremath{-2.81}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c14.ppalt\endcsname{\ensuremath{-2.84}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c14.rank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c14.z\endcsname{\ensuremath{-11.0}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c15.gap\endcsname{\ensuremath{-3.97}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c15.pp\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c15.ppalt\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c15.rank\endcsname{33}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c15.z\endcsname{\ensuremath{-0.4}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c2.gap\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c2.pp\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c2.ppalt\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c2.rank\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c2.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c3.gap\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c3.pp\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c3.ppalt\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c3.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c3.z\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c4.gap\endcsname{\ensuremath{-4.52}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c4.pp\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c4.ppalt\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c4.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c4.z\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c5.gap\endcsname{\ensuremath{-0.65}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c5.pp\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c5.ppalt\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c5.rank\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c5.z\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c6.gap\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c6.pp\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c6.ppalt\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c6.rank\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c6.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c7.gap\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c7.pp\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c7.ppalt\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c7.rank\endcsname{7}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c7.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c8.gap\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c8.pp\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c8.ppalt\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c8.rank\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c8.z\endcsname{\ensuremath{-1.7}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c9.gap\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c9.pp\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c9.ppalt\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c9.rank\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.c9.z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.head_pp\endcsname{\ensuremath{+0.076}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.head_ppalt\endcsname{\ensuremath{+0.047}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.maxz\endcsname{\ensuremath{-11.0}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.maxz_class\endcsname{bladder}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.maxz_pp\endcsname{\ensuremath{-2.81}}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.nneg2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.nneg2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.pos2list\endcsname{right adrenal gland}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W4.amos.sumpos_pp\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.altflip\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.c123.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.c123.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.c123.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.c123.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.c123.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.c2.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.c2.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.c2.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.c2.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.c2.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.c23.gap\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.c23.pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.c23.ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.c23.rank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.c23.z\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.head_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.head_ppalt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.maxz\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.maxz_class\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.maxz_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.nneg2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.nneg2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.npos2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.npos2alt\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.nrank\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.nseed\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.pos2list\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.regstate\endcsname{queued}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.seedlist\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.kits.sumpos_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.W4.params\endcsname{34.2}
\expandafter\gdef\csname R@an.perclass_all.W4.params.acdc\endcsname{33.5}
\expandafter\gdef\csname R@an.perclass_all.W4.params.amos\endcsname{34.2}
\expandafter\gdef\csname R@an.perclass_all.W4.params.kits\endcsname{34.3}
\expandafter\gdef\csname R@an.perclass_all.W4.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.altflip\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c1.gap\endcsname{\ensuremath{-2.10}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c1.pp\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c1.ppalt\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c1.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c1.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c10.gap\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c10.pp\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c10.ppalt\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c10.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c10.z\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c11.gap\endcsname{\ensuremath{-0.64}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c11.pp\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c11.ppalt\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c11.rank\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c11.z\endcsname{\ensuremath{+1.8}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c12.gap\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c12.pp\endcsname{\ensuremath{+1.81}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c12.ppalt\endcsname{\ensuremath{+2.06}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c12.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c12.z\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c13.gap\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c13.pp\endcsname{\ensuremath{+1.39}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c13.ppalt\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c13.rank\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c13.z\endcsname{\ensuremath{+3.5}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c14.gap\endcsname{\ensuremath{-0.93}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c14.pp\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c14.ppalt\endcsname{\ensuremath{+1.16}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c14.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c14.z\endcsname{\ensuremath{+4.6}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c15.gap\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c15.pp\endcsname{\ensuremath{+3.12}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c15.ppalt\endcsname{\ensuremath{+3.46}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c15.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c15.z\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c2.gap\endcsname{\ensuremath{-0.68}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c2.pp\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c2.ppalt\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c2.rank\endcsname{22}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c2.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c3.gap\endcsname{\ensuremath{-0.70}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c3.pp\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c3.ppalt\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c3.rank\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c3.z\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c4.gap\endcsname{\ensuremath{-5.75}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c4.pp\endcsname{\ensuremath{-1.09}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c4.ppalt\endcsname{\ensuremath{-1.69}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c4.rank\endcsname{29}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c4.z\endcsname{\ensuremath{-0.8}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c5.gap\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c5.pp\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c5.ppalt\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c5.rank\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c5.z\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c6.gap\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c6.pp\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c6.ppalt\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c6.rank\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c6.z\endcsname{\ensuremath{+1.6}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c7.gap\endcsname{\ensuremath{-0.79}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c7.pp\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c7.ppalt\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c7.rank\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c7.z\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c8.gap\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c8.pp\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c8.ppalt\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c8.rank\endcsname{23}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c8.z\endcsname{\ensuremath{-1.7}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c9.gap\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c9.pp\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c9.ppalt\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c9.rank\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.c9.z\endcsname{\ensuremath{+5.1}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.estimand\endcsname{discovery seed 0}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.head_pp\endcsname{\ensuremath{+0.591}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.head_ppalt\endcsname{\ensuremath{+0.562}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.maxz\endcsname{\ensuremath{+5.1}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.maxz_class\endcsname{postcava}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.maxz_pp\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.nneg2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.nneg2alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.npos2\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.npos2alt\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.nrank\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.nseed\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.pos2list\endcsname{postcava, bladder, duodenum, prostate/uterus}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.regstate\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.seedlist\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.W5.amos.sumpos_pp\endcsname{\ensuremath{+6.33}}
\expandafter\gdef\csname R@an.perclass_all.W5.params\endcsname{102}
\expandafter\gdef\csname R@an.perclass_all.W5.params.acdc\endcsname{102}
\expandafter\gdef\csname R@an.perclass_all.W5.params.amos\endcsname{102}
\expandafter\gdef\csname R@an.perclass_all.W5.params.kits\endcsname{102}
\expandafter\gdef\csname R@an.perclass_all.W5.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.altref.acdc.label\endcsname{uncompiled sub-pool of the frozen pool (like-for-like, 3 runs)}
\expandafter\gdef\csname R@an.perclass_all.altref.acdc.maxpp\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.altref.acdc.maxpp2\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.perclass_all.altref.acdc.maxpp2_class\endcsname{MLV}
\expandafter\gdef\csname R@an.perclass_all.altref.acdc.maxpp_class\endcsname{LVC}
\expandafter\gdef\csname R@an.perclass_all.altref.acdc.maxz\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.altref.acdc.maxz2\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.perclass_all.altref.acdc.maxz_class\endcsname{LVC}
\expandafter\gdef\csname R@an.perclass_all.altref.acdc.maxz_pp\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.altref.acdc.n\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.altref.acdc.ncell\endcsname{48}
\expandafter\gdef\csname R@an.perclass_all.altref.acdc.nfinished\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.altref.acdc.nflip\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.altref.acdc.shift\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.perclass_all.altref.acdc.short\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.perclass_all.altref.acdc.source\endcsname{Correction C30, lines 358-363}
\expandafter\gdef\csname R@an.perclass_all.altref.acdc.state\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.altref.amos.label\endcsname{uncompiled sub-pool of the frozen pool (like-for-like, 3 runs)}
\expandafter\gdef\csname R@an.perclass_all.altref.amos.maxpp\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.perclass_all.altref.amos.maxpp2\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.perclass_all.altref.amos.maxpp2_class\endcsname{prostate/uterus}
\expandafter\gdef\csname R@an.perclass_all.altref.amos.maxpp_class\endcsname{gall bladder}
\expandafter\gdef\csname R@an.perclass_all.altref.amos.maxz\endcsname{\ensuremath{-0.83}}
\expandafter\gdef\csname R@an.perclass_all.altref.amos.maxz2\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.perclass_all.altref.amos.maxz_class\endcsname{esophagus}
\expandafter\gdef\csname R@an.perclass_all.altref.amos.maxz_pp\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.altref.amos.n\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.altref.amos.ncell\endcsname{645}
\expandafter\gdef\csname R@an.perclass_all.altref.amos.nfinished\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.altref.amos.nflip\endcsname{29}
\expandafter\gdef\csname R@an.perclass_all.altref.amos.shift\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.perclass_all.altref.amos.short\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.perclass_all.altref.amos.source\endcsname{Correction C30, lines 358-363}
\expandafter\gdef\csname R@an.perclass_all.altref.amos.state\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.altref.kits.label\endcsname{six-run default pool (the frozen 3 runs plus 3 contemporaneous runs, Addendum N2)}
\expandafter\gdef\csname R@an.perclass_all.altref.kits.maxpp\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.perclass_all.altref.kits.maxpp2\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.perclass_all.altref.kits.maxpp2_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.altref.kits.maxpp_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.altref.kits.maxz\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.perclass_all.altref.kits.maxz2\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.perclass_all.altref.kits.maxz_class\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.altref.kits.maxz_pp\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.perclass_all.altref.kits.n\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.altref.kits.ncell\endcsname{171}
\expandafter\gdef\csname R@an.perclass_all.altref.kits.nfinished\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.altref.kits.nflip\endcsname{24}
\expandafter\gdef\csname R@an.perclass_all.altref.kits.shift\endcsname{\ensuremath{+0.244}}
\expandafter\gdef\csname R@an.perclass_all.altref.kits.short\endcsname{six-run default pool}
\expandafter\gdef\csname R@an.perclass_all.altref.kits.source\endcsname{Addendum N2, lines 23-28 and 58-61}
\expandafter\gdef\csname R@an.perclass_all.altref.kits.state\endcsname{finished}
\expandafter\gdef\csname R@an.perclass_all.arms.acdc.frac2\endcsname{41.7}
\expandafter\gdef\csname R@an.perclass_all.arms.acdc.n2\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.arms.acdc.ncell\endcsname{36}
\expandafter\gdef\csname R@an.perclass_all.arms.acdc.ncol\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.arms.amos.frac2\endcsname{22.5}
\expandafter\gdef\csname R@an.perclass_all.arms.amos.n2\endcsname{128}
\expandafter\gdef\csname R@an.perclass_all.arms.amos.ncell\endcsname{570}
\expandafter\gdef\csname R@an.perclass_all.arms.amos.ncol\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.arms.kits.frac2\endcsname{58.3}
\expandafter\gdef\csname R@an.perclass_all.arms.kits.n2\endcsname{56}
\expandafter\gdef\csname R@an.perclass_all.arms.kits.ncell\endcsname{96}
\expandafter\gdef\csname R@an.perclass_all.arms.kits.ncol\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.armsf.acdc.frac2\endcsname{33.3}
\expandafter\gdef\csname R@an.perclass_all.armsf.acdc.n2\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.armsf.acdc.ncell\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.armsf.acdc.ncol\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.armsf.amos.frac2\endcsname{18.7}
\expandafter\gdef\csname R@an.perclass_all.armsf.amos.n2\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.armsf.amos.ncell\endcsname{75}
\expandafter\gdef\csname R@an.perclass_all.armsf.amos.ncol\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.armsf.kits.frac2\endcsname{72.0}
\expandafter\gdef\csname R@an.perclass_all.armsf.kits.n2\endcsname{54}
\expandafter\gdef\csname R@an.perclass_all.armsf.kits.ncell\endcsname{75}
\expandafter\gdef\csname R@an.perclass_all.armsf.kits.ncol\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.calib.amos.dir\endcsname{above}
\expandafter\gdef\csname R@an.perclass_all.calib.amos.mag\endcsname{10.3}
\expandafter\gdef\csname R@an.perclass_all.calib.amos.margin\endcsname{\ensuremath{+10.3}}
\expandafter\gdef\csname R@an.perclass_all.contemp.amos.maxpp\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.perclass_all.contemp.amos.maxpp_class\endcsname{prostate/uterus}
\expandafter\gdef\csname R@an.perclass_all.contemp.amos.n\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.contemp.amos.ncell\endcsname{645}
\expandafter\gdef\csname R@an.perclass_all.contemp.amos.nfinished\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.contemp.amos.nflip\endcsname{91}
\expandafter\gdef\csname R@an.perclass_all.contemp.amos.shift\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.perclass_all.contemp.kits.maxpp\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.perclass_all.contemp.kits.maxpp_class\endcsname{masses}
\expandafter\gdef\csname R@an.perclass_all.contemp.kits.n\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.contemp.kits.ncell\endcsname{171}
\expandafter\gdef\csname R@an.perclass_all.contemp.kits.nfinished\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.contemp.kits.nflip\endcsname{50}
\expandafter\gdef\csname R@an.perclass_all.contemp.kits.shift\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.perclass_all.cophenetic\endcsname{0.75}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.list\endcsname{function-identical control; ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.maxz\endcsname{\ensuremath{+5.4}}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.maxz_class\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.maxz_pp\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.n\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.nall\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.nall_alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.params\endcsname{102}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.top\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.top_fresh\endcsname{landed}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.top_fresh_clause\endcsname{has a landed fresh pair}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.top_fresh_npos2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.top_fresh_pp\endcsname{\ensuremath{+0.319}}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.top_margin\endcsname{4.24}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.top_npos2alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.top_ppalt\endcsname{\ensuremath{+0.97}}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.top_tag\endcsname{L1b}
\expandafter\gdef\csname R@an.perclass_all.ctl.acdc.top_zalt\endcsname{\ensuremath{+5.3}}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.list\endcsname{trilinear-decoder control; branch control; function-identical control; ResEnc-matched (re-implemented); pooled-skip control}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.maxz\endcsname{\ensuremath{+5.1}}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.maxz_class\endcsname{postcava}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.maxz_pp\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.n\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.nall\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.nall_alt\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.npos2\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.params\endcsname{102}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.top\endcsname{pooled-skip control}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.top_fresh\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.top_fresh_clause\endcsname{has no registered fresh pair}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.top_fresh_npos2\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.top_fresh_pp\endcsname{\pend}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.top_margin\endcsname{0.19}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.top_npos2alt\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.top_ppalt\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.top_tag\endcsname{W5}
\expandafter\gdef\csname R@an.perclass_all.ctl.amos.top_zalt\endcsname{\ensuremath{+4.5}}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.list\endcsname{branch control; function-identical control; ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.maxz\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.maxz_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.maxz_pp\endcsname{\ensuremath{+3.49}}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.n\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.nall\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.nall_alt\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.npos2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.params\endcsname{31.1}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.params_ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.top\endcsname{branch control}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.top_fresh\endcsname{landed}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.top_fresh_clause\endcsname{has a landed fresh pair}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.top_fresh_npos2\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.top_fresh_pp\endcsname{\ensuremath{+1.067}}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.top_margin\endcsname{0.39}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.top_npos2alt\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.top_ppalt\endcsname{\ensuremath{+3.20}}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.top_tag\endcsname{W1c}
\expandafter\gdef\csname R@an.perclass_all.ctl.kits.top_zalt\endcsname{\ensuremath{+2.6}}
\expandafter\gdef\csname R@an.perclass_all.d0f.C1.kits.c123.pp\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.perclass_all.d0f.C1.kits.c123.rel\endcsname{0.53}
\expandafter\gdef\csname R@an.perclass_all.d0f.C1.kits.c2.pp\endcsname{\ensuremath{-2.17}}
\expandafter\gdef\csname R@an.perclass_all.d0f.C1.kits.c2.rel\endcsname{1.66}
\expandafter\gdef\csname R@an.perclass_all.d0f.C1.kits.c23.pp\endcsname{\ensuremath{-0.90}}
\expandafter\gdef\csname R@an.perclass_all.d0f.C1.kits.c23.rel\endcsname{0.68}
\expandafter\gdef\csname R@an.perclass_all.d0f.D1.kits.c123.pp\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.d0f.D1.kits.c123.rel\endcsname{0.67}
\expandafter\gdef\csname R@an.perclass_all.d0f.D1.kits.c2.pp\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.perclass_all.d0f.D1.kits.c2.rel\endcsname{0.60}
\expandafter\gdef\csname R@an.perclass_all.d0f.D1.kits.c23.pp\endcsname{\ensuremath{-0.85}}
\expandafter\gdef\csname R@an.perclass_all.d0f.D1.kits.c23.rel\endcsname{0.64}
\expandafter\gdef\csname R@an.perclass_all.d0f.D2.kits.c123.pp\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.perclass_all.d0f.D2.kits.c123.rel\endcsname{0.25}
\expandafter\gdef\csname R@an.perclass_all.d0f.D2.kits.c2.pp\endcsname{\ensuremath{-1.19}}
\expandafter\gdef\csname R@an.perclass_all.d0f.D2.kits.c2.rel\endcsname{0.92}
\expandafter\gdef\csname R@an.perclass_all.d0f.D2.kits.c23.pp\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.perclass_all.d0f.D2.kits.c23.rel\endcsname{0.24}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.acdc.c1.pp\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.acdc.c1.rel\endcsname{0.62}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.acdc.c2.pp\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.acdc.c2.rel\endcsname{0.53}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.acdc.c3.pp\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.acdc.c3.rel\endcsname{0.68}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c1.pp\endcsname{\ensuremath{-2.39}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c1.rel\endcsname{7.27}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c10.pp\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c10.rel\endcsname{1.06}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c11.pp\endcsname{\ensuremath{-0.84}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c11.rel\endcsname{4.48}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c12.pp\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c12.rel\endcsname{0.47}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c13.pp\endcsname{\ensuremath{+0.67}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c13.rel\endcsname{1.49}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c14.pp\endcsname{\ensuremath{-1.30}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c14.rel\endcsname{4.49}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c15.pp\endcsname{\ensuremath{+1.58}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c15.rel\endcsname{1.27}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c2.pp\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c2.rel\endcsname{0.70}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c3.pp\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c3.rel\endcsname{0.17}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c4.pp\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c4.rel\endcsname{0.26}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c5.pp\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c5.rel\endcsname{0.15}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c6.pp\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c6.rel\endcsname{1.24}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c7.pp\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c7.rel\endcsname{0.53}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c8.pp\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c8.rel\endcsname{1.98}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c9.pp\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.amos.c9.rel\endcsname{4.12}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.kits.c123.pp\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.kits.c123.rel\endcsname{0.28}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.kits.c2.pp\endcsname{\ensuremath{+2.19}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.kits.c2.rel\endcsname{1.68}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.kits.c23.pp\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1.kits.c23.rel\endcsname{0.85}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.acdc.c1.pp\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.acdc.c1.rel\endcsname{0.68}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.acdc.c2.pp\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.acdc.c2.rel\endcsname{0.19}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.acdc.c3.pp\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.acdc.c3.rel\endcsname{0.49}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c1.pp\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c1.rel\endcsname{0.12}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c10.pp\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c10.rel\endcsname{0.00}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c11.pp\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c11.rel\endcsname{2.10}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c12.pp\endcsname{\ensuremath{-1.05}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c12.rel\endcsname{0.99}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c13.pp\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c13.rel\endcsname{0.13}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c14.pp\endcsname{\ensuremath{+1.64}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c14.rel\endcsname{5.67}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c15.pp\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c15.rel\endcsname{0.43}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c2.pp\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c2.rel\endcsname{1.06}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c3.pp\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c3.rel\endcsname{1.72}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c4.pp\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c4.rel\endcsname{0.11}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c5.pp\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c5.rel\endcsname{0.21}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c6.pp\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c6.rel\endcsname{1.45}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c7.pp\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c7.rel\endcsname{1.97}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c8.pp\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c8.rel\endcsname{0.72}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c9.pp\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.amos.c9.rel\endcsname{0.88}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.kits.c123.pp\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.kits.c123.rel\endcsname{1.44}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.kits.c2.pp\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.kits.c2.rel\endcsname{0.17}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.kits.c23.pp\endcsname{\ensuremath{+1.24}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L1b.kits.c23.rel\endcsname{0.94}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c1.pp\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c1.rel\endcsname{0.89}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c10.pp\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c10.rel\endcsname{0.52}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c11.pp\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c11.rel\endcsname{1.01}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c12.pp\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c12.rel\endcsname{0.05}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c13.pp\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c13.rel\endcsname{0.28}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c14.pp\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c14.rel\endcsname{2.83}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c15.pp\endcsname{\ensuremath{-0.71}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c15.rel\endcsname{0.57}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c2.pp\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c2.rel\endcsname{0.07}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c3.pp\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c3.rel\endcsname{0.54}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c4.pp\endcsname{\ensuremath{-1.10}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c4.rel\endcsname{0.73}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c5.pp\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c5.rel\endcsname{0.06}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c6.pp\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c6.rel\endcsname{0.86}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c7.pp\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c7.rel\endcsname{1.46}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c8.pp\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c8.rel\endcsname{1.56}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c9.pp\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.amos.c9.rel\endcsname{0.77}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.kits.c123.pp\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.kits.c123.rel\endcsname{1.23}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.kits.c2.pp\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.kits.c2.rel\endcsname{0.22}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.kits.c23.pp\endcsname{\ensuremath{-0.79}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L2.kits.c23.rel\endcsname{0.60}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.acdc.c1.pp\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.acdc.c1.rel\endcsname{0.78}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.acdc.c2.pp\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.acdc.c2.rel\endcsname{0.29}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.acdc.c3.pp\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.acdc.c3.rel\endcsname{2.46}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c1.pp\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c1.rel\endcsname{0.61}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c10.pp\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c10.rel\endcsname{0.70}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c11.pp\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c11.rel\endcsname{0.38}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c12.pp\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c12.rel\endcsname{0.09}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c13.pp\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c13.rel\endcsname{0.61}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c14.pp\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c14.rel\endcsname{0.11}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c15.pp\endcsname{\ensuremath{-1.03}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c15.rel\endcsname{0.83}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c2.pp\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c2.rel\endcsname{0.95}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c3.pp\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c3.rel\endcsname{1.40}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c4.pp\endcsname{\ensuremath{-2.24}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c4.rel\endcsname{1.49}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c5.pp\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c5.rel\endcsname{0.51}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c6.pp\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c6.rel\endcsname{1.06}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c7.pp\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c7.rel\endcsname{0.62}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c8.pp\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c8.rel\endcsname{0.62}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c9.pp\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.amos.c9.rel\endcsname{0.73}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.kits.c123.pp\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.kits.c123.rel\endcsname{0.01}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.kits.c2.pp\endcsname{\ensuremath{-1.77}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.kits.c2.rel\endcsname{1.36}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.kits.c23.pp\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L3.kits.c23.rel\endcsname{0.35}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c1.pp\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c1.rel\endcsname{3.49}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c10.pp\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c10.rel\endcsname{0.49}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c11.pp\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c11.rel\endcsname{0.13}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c12.pp\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c12.rel\endcsname{0.18}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c13.pp\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c13.rel\endcsname{0.16}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c14.pp\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c14.rel\endcsname{0.90}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c15.pp\endcsname{\ensuremath{-1.40}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c15.rel\endcsname{1.12}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c2.pp\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c2.rel\endcsname{0.41}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c3.pp\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c3.rel\endcsname{0.34}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c4.pp\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c4.rel\endcsname{0.31}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c5.pp\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c5.rel\endcsname{0.87}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c6.pp\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c6.rel\endcsname{0.26}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c7.pp\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c7.rel\endcsname{1.57}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c8.pp\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c8.rel\endcsname{0.25}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c9.pp\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.amos.c9.rel\endcsname{1.29}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.kits.c123.pp\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.kits.c123.rel\endcsname{0.39}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.kits.c2.pp\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.kits.c2.rel\endcsname{0.27}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.kits.c23.pp\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L4.kits.c23.rel\endcsname{0.24}
\expandafter\gdef\csname R@an.perclass_all.d0f.L6.kits.c123.pp\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L6.kits.c123.rel\endcsname{0.67}
\expandafter\gdef\csname R@an.perclass_all.d0f.L6.kits.c2.pp\endcsname{\ensuremath{-1.48}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L6.kits.c2.rel\endcsname{1.14}
\expandafter\gdef\csname R@an.perclass_all.d0f.L6.kits.c23.pp\endcsname{\ensuremath{-1.00}}
\expandafter\gdef\csname R@an.perclass_all.d0f.L6.kits.c23.rel\endcsname{0.76}
\expandafter\gdef\csname R@an.perclass_all.d0f.P3c.acdc.c1.pp\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.perclass_all.d0f.P3c.acdc.c1.rel\endcsname{0.58}
\expandafter\gdef\csname R@an.perclass_all.d0f.P3c.acdc.c2.pp\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.perclass_all.d0f.P3c.acdc.c2.rel\endcsname{1.72}
\expandafter\gdef\csname R@an.perclass_all.d0f.P3c.acdc.c3.pp\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.perclass_all.d0f.P3c.acdc.c3.rel\endcsname{0.31}
\expandafter\gdef\csname R@an.perclass_all.d0f.P3c.kits.c123.pp\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.perclass_all.d0f.P3c.kits.c123.rel\endcsname{0.08}
\expandafter\gdef\csname R@an.perclass_all.d0f.P3c.kits.c2.pp\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.d0f.P3c.kits.c2.rel\endcsname{0.24}
\expandafter\gdef\csname R@an.perclass_all.d0f.P3c.kits.c23.pp\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.perclass_all.d0f.P3c.kits.c23.rel\endcsname{0.16}
\expandafter\gdef\csname R@an.perclass_all.d0f.S2.kits.c123.pp\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.d0f.S2.kits.c123.rel\endcsname{0.67}
\expandafter\gdef\csname R@an.perclass_all.d0f.S2.kits.c2.pp\endcsname{\ensuremath{-1.19}}
\expandafter\gdef\csname R@an.perclass_all.d0f.S2.kits.c2.rel\endcsname{0.91}
\expandafter\gdef\csname R@an.perclass_all.d0f.S2.kits.c23.pp\endcsname{\ensuremath{-0.81}}
\expandafter\gdef\csname R@an.perclass_all.d0f.S2.kits.c23.rel\endcsname{0.61}
\expandafter\gdef\csname R@an.perclass_all.d0f.V5A5.kits.c123.pp\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V5A5.kits.c123.rel\endcsname{0.19}
\expandafter\gdef\csname R@an.perclass_all.d0f.V5A5.kits.c2.pp\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V5A5.kits.c2.rel\endcsname{0.55}
\expandafter\gdef\csname R@an.perclass_all.d0f.V5A5.kits.c23.pp\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V5A5.kits.c23.rel\endcsname{0.02}
\expandafter\gdef\csname R@an.perclass_all.d0f.V5B1.kits.c123.pp\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V5B1.kits.c123.rel\endcsname{0.47}
\expandafter\gdef\csname R@an.perclass_all.d0f.V5B1.kits.c2.pp\endcsname{\ensuremath{-0.58}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V5B1.kits.c2.rel\endcsname{0.44}
\expandafter\gdef\csname R@an.perclass_all.d0f.V5B1.kits.c23.pp\endcsname{\ensuremath{+0.72}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V5B1.kits.c23.rel\endcsname{0.55}
\expandafter\gdef\csname R@an.perclass_all.d0f.V5B2.kits.c123.pp\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V5B2.kits.c123.rel\endcsname{0.46}
\expandafter\gdef\csname R@an.perclass_all.d0f.V5B2.kits.c2.pp\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V5B2.kits.c2.rel\endcsname{0.21}
\expandafter\gdef\csname R@an.perclass_all.d0f.V5B2.kits.c23.pp\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V5B2.kits.c23.rel\endcsname{0.05}
\expandafter\gdef\csname R@an.perclass_all.d0f.V6A1r.kits.c123.pp\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V6A1r.kits.c123.rel\endcsname{0.23}
\expandafter\gdef\csname R@an.perclass_all.d0f.V6A1r.kits.c2.pp\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V6A1r.kits.c2.rel\endcsname{0.25}
\expandafter\gdef\csname R@an.perclass_all.d0f.V6A1r.kits.c23.pp\endcsname{\ensuremath{-1.17}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V6A1r.kits.c23.rel\endcsname{0.89}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7A1.kits.c123.pp\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7A1.kits.c123.rel\endcsname{0.21}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7A1.kits.c2.pp\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7A1.kits.c2.rel\endcsname{0.09}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7A1.kits.c23.pp\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7A1.kits.c23.rel\endcsname{0.09}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7A2.kits.c123.pp\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7A2.kits.c123.rel\endcsname{0.12}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7A2.kits.c2.pp\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7A2.kits.c2.rel\endcsname{0.32}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7A2.kits.c23.pp\endcsname{\ensuremath{-1.31}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7A2.kits.c23.rel\endcsname{1.00}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7B1.kits.c123.pp\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7B1.kits.c123.rel\endcsname{0.32}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7B1.kits.c2.pp\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7B1.kits.c2.rel\endcsname{0.55}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7B1.kits.c23.pp\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7B1.kits.c23.rel\endcsname{0.85}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7B2.kits.c123.pp\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7B2.kits.c123.rel\endcsname{0.46}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7B2.kits.c2.pp\endcsname{\ensuremath{-1.26}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7B2.kits.c2.rel\endcsname{0.97}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7B2.kits.c23.pp\endcsname{\ensuremath{-1.48}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7B2.kits.c23.rel\endcsname{1.12}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7C1.kits.c123.pp\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7C1.kits.c123.rel\endcsname{0.32}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7C1.kits.c2.pp\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7C1.kits.c2.rel\endcsname{0.25}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7C1.kits.c23.pp\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V7C1.kits.c23.rel\endcsname{0.48}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8A1.kits.c123.pp\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8A1.kits.c123.rel\endcsname{0.05}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8A1.kits.c2.pp\endcsname{\ensuremath{-0.85}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8A1.kits.c2.rel\endcsname{0.65}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8A1.kits.c23.pp\endcsname{\ensuremath{-0.70}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8A1.kits.c23.rel\endcsname{0.53}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8A2.kits.c123.pp\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8A2.kits.c123.rel\endcsname{0.11}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8A2.kits.c2.pp\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8A2.kits.c2.rel\endcsname{0.40}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8A2.kits.c23.pp\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8A2.kits.c23.rel\endcsname{0.76}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8B1.kits.c123.pp\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8B1.kits.c123.rel\endcsname{0.84}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8B1.kits.c2.pp\endcsname{\ensuremath{-2.50}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8B1.kits.c2.rel\endcsname{1.92}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8B1.kits.c23.pp\endcsname{\ensuremath{-1.70}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8B1.kits.c23.rel\endcsname{1.29}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8B2.kits.c123.pp\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8B2.kits.c123.rel\endcsname{0.58}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8B2.kits.c2.pp\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8B2.kits.c2.rel\endcsname{0.34}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8B2.kits.c23.pp\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.perclass_all.d0f.V8B2.kits.c23.rel\endcsname{0.07}
\expandafter\gdef\csname R@an.perclass_all.d0f.W1c.kits.c123.pp\endcsname{\ensuremath{-0.84}}
\expandafter\gdef\csname R@an.perclass_all.d0f.W1c.kits.c123.rel\endcsname{1.76}
\expandafter\gdef\csname R@an.perclass_all.d0f.W1c.kits.c2.pp\endcsname{\ensuremath{-2.10}}
\expandafter\gdef\csname R@an.perclass_all.d0f.W1c.kits.c2.rel\endcsname{1.61}
\expandafter\gdef\csname R@an.perclass_all.d0f.W1c.kits.c23.pp\endcsname{\ensuremath{-1.76}}
\expandafter\gdef\csname R@an.perclass_all.d0f.W1c.kits.c23.rel\endcsname{1.34}
\expandafter\gdef\csname R@an.perclass_all.ex.acdc.nonum_arm\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.perclass_all.ex.acdc.nonum_class\endcsname{RV}
\expandafter\gdef\csname R@an.perclass_all.ex.acdc.nonum_pp\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.perclass_all.ex.acdc.nonum_z\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.perclass_all.ex.acdc.num_arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.perclass_all.ex.acdc.num_class\endcsname{LVC}
\expandafter\gdef\csname R@an.perclass_all.ex.acdc.num_pp\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.perclass_all.ex.acdc.num_z\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.perclass_all.ex.amos.nonum_arm\endcsname{offset upsampling}
\expandafter\gdef\csname R@an.perclass_all.ex.amos.nonum_class\endcsname{gall bladder}
\expandafter\gdef\csname R@an.perclass_all.ex.amos.nonum_pp\endcsname{\ensuremath{+2.58}}
\expandafter\gdef\csname R@an.perclass_all.ex.amos.nonum_z\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.perclass_all.ex.amos.num_arm\endcsname{HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.perclass_all.ex.amos.num_class\endcsname{aorta}
\expandafter\gdef\csname R@an.perclass_all.ex.amos.num_pp\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.perclass_all.ex.amos.num_z\endcsname{\ensuremath{-2.0}}
\expandafter\gdef\csname R@an.perclass_all.ex.kits.nonum_arm\endcsname{LeanAdd-NeXt with 3-tap coarse kernels (extent control)}
\expandafter\gdef\csname R@an.perclass_all.ex.kits.nonum_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.ex.kits.nonum_pp\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@an.perclass_all.ex.kits.nonum_z\endcsname{\ensuremath{+2.0}}
\expandafter\gdef\csname R@an.perclass_all.ex.kits.num_arm\endcsname{HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.perclass_all.ex.kits.num_class\endcsname{kidney}
\expandafter\gdef\csname R@an.perclass_all.ex.kits.num_pp\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.perclass_all.ex.kits.num_z\endcsname{\ensuremath{+2.0}}
\expandafter\gdef\csname R@an.perclass_all.failedcols\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.hero.acdc.gaps.fresh\endcsname{\ensuremath{-0.01}, \ensuremath{+0.16} and \ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.hero.acdc.gaps.s0\endcsname{\ensuremath{-0.13}, \ensuremath{+0.05} and \ensuremath{+0.12}}
\expandafter\gdef\csname R@an.perclass_all.hero.acdc.names\endcsname{RV, MLV and LVC}
\expandafter\gdef\csname R@an.perclass_all.hero.acdc.nfirst.fresh\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.hero.acdc.nfirst.s0\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.hero.acdc.ninside.fresh\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.hero.acdc.ninside.s0\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.hero.acdc.nneg.fresh\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.hero.acdc.nneg.s0\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.hero.acdc.nrank.fresh\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.hero.acdc.nrank.s0\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.hero.acdc.pps.fresh\endcsname{\ensuremath{+1.11}, \ensuremath{+0.32} and \ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.hero.acdc.pps.s0\endcsname{\ensuremath{+1.27}, \ensuremath{+0.36} and \ensuremath{+0.22}}
\expandafter\gdef\csname R@an.perclass_all.hero.acdc.ranks.fresh\endcsname{2 of 4, 1 of 4 and 2 of 4}
\expandafter\gdef\csname R@an.perclass_all.hero.acdc.ranks.s0\endcsname{2 of 12, 1 of 12 and 1 of 12}
\expandafter\gdef\csname R@an.perclass_all.mix.acdc.drawn\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.mix.acdc.fresh\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.mix.acdc.freshlist\endcsname{HyReX; function-identical control; ResEnc-matched (re-implemented); ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.perclass_all.mix.acdc.none\endcsname{49}
\expandafter\gdef\csname R@an.perclass_all.mix.acdc.pend\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.mix.acdc.pending_failed\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.mix.acdc.pending_queued\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.mix.acdc.pending_registered\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.mix.acdc.pending_running\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.mix.acdc.s0\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.mix.amos.drawn\endcsname{43}
\expandafter\gdef\csname R@an.perclass_all.mix.amos.fresh\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.mix.amos.freshlist\endcsname{HyReX; ResEnc-matched (re-implemented); ConvNeXt-k3; ResEnc+context; ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.perclass_all.mix.amos.none\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.mix.amos.pend\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.mix.amos.pending_failed\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.mix.amos.pending_queued\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.mix.amos.pending_registered\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.mix.amos.pending_running\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.mix.amos.s0\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.mix.kits.drawn\endcsname{57}
\expandafter\gdef\csname R@an.perclass_all.mix.kits.fresh\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.mix.kits.freshlist\endcsname{HyReX with 9-kernel coarse stages; HyReX, ConvNeXt one stage finer; HyReX with LeanDec fine decoder stages; HyReX; HyReX+context; LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid); HyReX point-fuse decoder; LeanDec with additive skips (LeanAdd); LeanDec (default with one conv per decoder stage); branch control; function-identical control; LeanAdd with coarse large kernels (LeanAdd-NeXt); LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack); LeanAdd-NeXt with the coarse operator at stage 5 only; LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk); LeanAdd-NeXt with separable coarse kernels (LeanSep); LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec); LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1); LeanAdd-NeXt with dilated coarse kernels (LeanDil); ResEnc-matched (re-implemented); ConvNeXt-k3; LeanDeepMid with the two finest decoder convolutions restored; ResEnc+context; HyReX + decoder capacity; ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.perclass_all.mix.kits.none\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.mix.kits.pend\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.mix.kits.pending_failed\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.mix.kits.pending_queued\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.mix.kits.pending_registered\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.mix.kits.pending_running\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.mix.kits.s0\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.narm\endcsname{46}
\expandafter\gdef\csname R@an.perclass_all.narmline\endcsname{71}
\expandafter\gdef\csname R@an.perclass_all.nclass.acdc\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.nclass.amos\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.nclass.kits\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.ncol\endcsname{71}
\expandafter\gdef\csname R@an.perclass_all.ncoldrawn\endcsname{79}
\expandafter\gdef\csname R@an.perclass_all.neverqueued.list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.neverqueued.n\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.nfailedcol\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.nfresh\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.nnullcol\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.nnullrow\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.notstarted.list\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.notstarted.n\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.npair.acdc\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.npair.amos\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.npair.kits\endcsname{25}
\expandafter\gdef\csname R@an.perclass_all.npendcol\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.npendcol.acdc\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.npendcol.amos\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.npendcol.kits\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.npenddrawn\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.nqueuedcol\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.nrowclass\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.nrowdrawn\endcsname{79}
\expandafter\gdef\csname R@an.perclass_all.null.acdc.expclass\endcsname{0.3}
\expandafter\gdef\csname R@an.perclass_all.null.acdc.frac2\endcsname{11.1}
\expandafter\gdef\csname R@an.perclass_all.null.acdc.n2\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.null.acdc.ncell\endcsname{18}
\expandafter\gdef\csname R@an.perclass_all.null.acdc.nmember\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.null.all.frac2\endcsname{13.7}
\expandafter\gdef\csname R@an.perclass_all.null.all.n2\endcsname{16}
\expandafter\gdef\csname R@an.perclass_all.null.all.ncell\endcsname{117}
\expandafter\gdef\csname R@an.perclass_all.null.amos.expclass\endcsname{1.8}
\expandafter\gdef\csname R@an.perclass_all.null.amos.frac2\endcsname{12.2}
\expandafter\gdef\csname R@an.perclass_all.null.amos.n2\endcsname{11}
\expandafter\gdef\csname R@an.perclass_all.null.amos.ncell\endcsname{90}
\expandafter\gdef\csname R@an.perclass_all.null.amos.nmember\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.null.kits.expclass\endcsname{1.0}
\expandafter\gdef\csname R@an.perclass_all.null.kits.frac2\endcsname{33.3}
\expandafter\gdef\csname R@an.perclass_all.null.kits.n2\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.null.kits.ncell\endcsname{9}
\expandafter\gdef\csname R@an.perclass_all.null.kits.nmember\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.nundrawn\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.pairfloor\endcsname{0.50}
\expandafter\gdef\csname R@an.perclass_all.pairlist.acdc\endcsname{HyReX; function-identical control; ResEnc-matched (re-implemented); ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.perclass_all.pairlist.amos\endcsname{HyReX; ResEnc-matched (re-implemented); ConvNeXt-k3; ResEnc+context; ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.perclass_all.pairlist.kits\endcsname{HyReX with 9-kernel coarse stages; HyReX, ConvNeXt one stage finer; HyReX with LeanDec fine decoder stages; HyReX; HyReX+context; LeanAdd-NeXt with a deeper middle encoder (LeanDeepMid); HyReX point-fuse decoder; LeanDec with additive skips (LeanAdd); LeanDec (default with one conv per decoder stage); branch control; function-identical control; LeanAdd with coarse large kernels (LeanAdd-NeXt); LeanNeXt-s5 with eighteen coarse blocks at the bottleneck (CoarseStack); LeanAdd-NeXt with the coarse operator at stage 5 only; LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk); LeanAdd-NeXt with separable coarse kernels (LeanSep); LeanNeXt-s5 with twelve coarse blocks and the two coarse decoder second convolutions (StackDec); LeanNeXt-s5 with one convolution at encoder stage 0 (Stem1); LeanAdd-NeXt with dilated coarse kernels (LeanDil); ResEnc-matched (re-implemented); ConvNeXt-k3; LeanDeepMid with the two finest decoder convolutions restored; ResEnc+context; HyReX + decoder capacity; ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.perclass_all.params.ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.perclass_all.params.nmissing\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.params.spread\endcsname{0.97}
\expandafter\gdef\csname R@an.perclass_all.parts.1.first\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.parts.1.idx\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.parts.1.last\endcsname{32}
\expandafter\gdef\csname R@an.perclass_all.parts.2.first\endcsname{33}
\expandafter\gdef\csname R@an.perclass_all.parts.2.idx\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.parts.2.last\endcsname{63}
\expandafter\gdef\csname R@an.perclass_all.parts.lines\endcsname{63}
\expandafter\gdef\csname R@an.perclass_all.parts.n\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.parts.word\endcsname{two}
\expandafter\gdef\csname R@an.perclass_all.pendcols\endcsname{single-prompt LLM design 1; single-prompt LLM design 2}
\expandafter\gdef\csname R@an.perclass_all.pool.acdc.mean\endcsname{92.009}
\expandafter\gdef\csname R@an.perclass_all.pool.acdc.n\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.pool.acdc.sd\endcsname{0.099}
\expandafter\gdef\csname R@an.perclass_all.pool.acdc.spread\endcsname{0.275}
\expandafter\gdef\csname R@an.perclass_all.pool.amos.mean\endcsname{87.701}
\expandafter\gdef\csname R@an.perclass_all.pool.amos.n\endcsname{6}
\expandafter\gdef\csname R@an.perclass_all.pool.amos.sd\endcsname{0.122}
\expandafter\gdef\csname R@an.perclass_all.pool.amos.spread\endcsname{0.321}
\expandafter\gdef\csname R@an.perclass_all.pool.kits.mean\endcsname{83.378}
\expandafter\gdef\csname R@an.perclass_all.pool.kits.n\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.pool.kits.sd\endcsname{0.795}
\expandafter\gdef\csname R@an.perclass_all.pool.kits.spread\endcsname{1.522}
\expandafter\gdef\csname R@an.perclass_all.prof.amos.narm\endcsname{38}
\expandafter\gdef\csname R@an.perclass_all.prof.amos.npair\endcsname{703}
\expandafter\gdef\csname R@an.perclass_all.prof.amos.nsim\endcsname{4000}
\expandafter\gdef\csname R@an.perclass_all.prof.amos.rbar\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.perclass_all.prof.amos.rbar_an\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.perclass_all.prof.amos.rbar_p\endcsname{0.79}
\expandafter\gdef\csname R@an.perclass_all.prof.amos.rbar_sh\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.perclass_all.prof.amos.rbar_sh_hi\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.perclass_all.prof.amos.rbar_sh_lo\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.perclass_all.prof.amos.rmax\endcsname{\ensuremath{+0.89}}
\expandafter\gdef\csname R@an.perclass_all.prof.amos.rmin\endcsname{\ensuremath{-0.88}}
\expandafter\gdef\csname R@an.perclass_all.queuedcols\endcsname{HyReX, width-scaled (M); HyReX, width-scaled (L); full-res addition; full-res kernel $3^3$; coarse-capacity control (parameter-matched); logit warp (head 0)}
\expandafter\gdef\csname R@an.perclass_all.refgap.acdc.ahead\endcsname{HyReX}
\expandafter\gdef\csname R@an.perclass_all.refgap.acdc.clause\endcsname{the two discovery-seed gains differ by 0.281 pp, inside the 0.50 pp one-seed pair floor}
\expandafter\gdef\csname R@an.perclass_all.refgap.acdc.floor\endcsname{inside}
\expandafter\gdef\csname R@an.perclass_all.refgap.acdc.fresh.ahead\endcsname{HyReX}
\expandafter\gdef\csname R@an.perclass_all.refgap.acdc.fresh.clause\endcsname{the two fresh-seed gains differ by 0.208 pp, inside the 0.50 pp one-seed pair floor}
\expandafter\gdef\csname R@an.perclass_all.refgap.acdc.fresh.floor\endcsname{inside}
\expandafter\gdef\csname R@an.perclass_all.refgap.acdc.fresh.mag\endcsname{0.208}
\expandafter\gdef\csname R@an.perclass_all.refgap.acdc.fresh.pp\endcsname{\ensuremath{-0.208}}
\expandafter\gdef\csname R@an.perclass_all.refgap.acdc.fresh.ref\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.perclass_all.refgap.acdc.mag\endcsname{0.281}
\expandafter\gdef\csname R@an.perclass_all.refgap.acdc.pp\endcsname{\ensuremath{-0.281}}
\expandafter\gdef\csname R@an.perclass_all.refgap.acdc.ref\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.perclass_all.refgap.amos.ahead\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.perclass_all.refgap.amos.clause\endcsname{the two discovery-seed gains differ by 0.265 pp, inside the 0.50 pp one-seed pair floor}
\expandafter\gdef\csname R@an.perclass_all.refgap.amos.floor\endcsname{inside}
\expandafter\gdef\csname R@an.perclass_all.refgap.amos.fresh.ahead\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.perclass_all.refgap.amos.fresh.clause\endcsname{the two fresh-seed gains differ by 0.332 pp, inside the 0.50 pp one-seed pair floor}
\expandafter\gdef\csname R@an.perclass_all.refgap.amos.fresh.floor\endcsname{inside}
\expandafter\gdef\csname R@an.perclass_all.refgap.amos.fresh.mag\endcsname{0.332}
\expandafter\gdef\csname R@an.perclass_all.refgap.amos.fresh.pp\endcsname{\ensuremath{+0.332}}
\expandafter\gdef\csname R@an.perclass_all.refgap.amos.fresh.ref\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.perclass_all.refgap.amos.mag\endcsname{0.265}
\expandafter\gdef\csname R@an.perclass_all.refgap.amos.pp\endcsname{\ensuremath{+0.265}}
\expandafter\gdef\csname R@an.perclass_all.refgap.amos.ref\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.perclass_all.refgap.kits.ahead\endcsname{HyReX}
\expandafter\gdef\csname R@an.perclass_all.refgap.kits.clause\endcsname{HyReX is ahead of ResEnc-M (library preset) by 0.516 pp on the discovery-seed gains, beyond the 0.50 pp one-seed pair floor}
\expandafter\gdef\csname R@an.perclass_all.refgap.kits.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.perclass_all.refgap.kits.fresh.ahead\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.perclass_all.refgap.kits.fresh.clause\endcsname{ResEnc-M (library preset) is ahead of HyReX by 1.382 pp on the fresh-seed gains, beyond the 0.50 pp one-seed pair floor}
\expandafter\gdef\csname R@an.perclass_all.refgap.kits.fresh.floor\endcsname{beyond}
\expandafter\gdef\csname R@an.perclass_all.refgap.kits.fresh.mag\endcsname{1.382}
\expandafter\gdef\csname R@an.perclass_all.refgap.kits.fresh.pp\endcsname{\ensuremath{+1.382}}
\expandafter\gdef\csname R@an.perclass_all.refgap.kits.fresh.ref\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.perclass_all.refgap.kits.mag\endcsname{0.516}
\expandafter\gdef\csname R@an.perclass_all.refgap.kits.pp\endcsname{\ensuremath{-0.516}}
\expandafter\gdef\csname R@an.perclass_all.refgap.kits.ref\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.perclass_all.rep.acdc.arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.perclass_all.rep.acdc.change\endcsname{\ensuremath{-0.166}}
\expandafter\gdef\csname R@an.perclass_all.rep.acdc.d0\endcsname{\ensuremath{+0.616}}
\expandafter\gdef\csname R@an.perclass_all.rep.acdc.df2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.rep.acdc.dfresh\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.perclass_all.rep.acdc.npos0\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.rep.acdc.nposf\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.rep.acdc.nseedf\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.rep.acdc.ratio\endcsname{above 1}
\expandafter\gdef\csname R@an.perclass_all.rep.acdc.sd2\endcsname{0.047}
\expandafter\gdef\csname R@an.perclass_all.rep.acdc.se2\endcsname{0.033}
\expandafter\gdef\csname R@an.perclass_all.rep.acdc.seed_hi\endcsname{\ensuremath{+0.484}}
\expandafter\gdef\csname R@an.perclass_all.rep.acdc.seed_lo\endcsname{\ensuremath{+0.417}}
\expandafter\gdef\csname R@an.perclass_all.rep.acdc.senull\endcsname{0.081}
\expandafter\gdef\csname R@an.perclass_all.rep.acdc.spread2\endcsname{0.067}
\expandafter\gdef\csname R@an.perclass_all.rep.amos.arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.perclass_all.rep.amos.change\endcsname{\ensuremath{-0.249}}
\expandafter\gdef\csname R@an.perclass_all.rep.amos.d0\endcsname{\ensuremath{+0.382}}
\expandafter\gdef\csname R@an.perclass_all.rep.amos.d0_vs_bar\endcsname{\ensuremath{+0.032}}
\expandafter\gdef\csname R@an.perclass_all.rep.amos.df2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.rep.amos.dfresh\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.perclass_all.rep.amos.dfresh_vs_bar\endcsname{\ensuremath{-0.218}}
\expandafter\gdef\csname R@an.perclass_all.rep.amos.npos0\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.rep.amos.nposf\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.rep.amos.nseedf\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.rep.amos.ratio\endcsname{0.90}
\expandafter\gdef\csname R@an.perclass_all.rep.amos.sd2\endcsname{0.209}
\expandafter\gdef\csname R@an.perclass_all.rep.amos.se2\endcsname{0.148}
\expandafter\gdef\csname R@an.perclass_all.rep.amos.seed_hi\endcsname{\ensuremath{+0.280}}
\expandafter\gdef\csname R@an.perclass_all.rep.amos.seed_lo\endcsname{\ensuremath{-0.016}}
\expandafter\gdef\csname R@an.perclass_all.rep.amos.senull\endcsname{0.100}
\expandafter\gdef\csname R@an.perclass_all.rep.amos.spread2\endcsname{0.296}
\expandafter\gdef\csname R@an.perclass_all.rep.kits.arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.perclass_all.rep.kits.change\endcsname{\ensuremath{-0.748}}
\expandafter\gdef\csname R@an.perclass_all.rep.kits.d0\endcsname{\ensuremath{+2.842}}
\expandafter\gdef\csname R@an.perclass_all.rep.kits.d0_vs_bar\endcsname{\ensuremath{+2.492}}
\expandafter\gdef\csname R@an.perclass_all.rep.kits.df2\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.rep.kits.dfresh\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.perclass_all.rep.kits.dfresh_vs_bar\endcsname{\ensuremath{+1.744}}
\expandafter\gdef\csname R@an.perclass_all.rep.kits.npos0\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.rep.kits.nposf\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.rep.kits.nseedf\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.rep.kits.ratio\endcsname{above 1}
\expandafter\gdef\csname R@an.perclass_all.rep.kits.sd2\endcsname{0.419}
\expandafter\gdef\csname R@an.perclass_all.rep.kits.se2\endcsname{0.296}
\expandafter\gdef\csname R@an.perclass_all.rep.kits.seed_hi\endcsname{\ensuremath{+2.390}}
\expandafter\gdef\csname R@an.perclass_all.rep.kits.seed_lo\endcsname{\ensuremath{+1.798}}
\expandafter\gdef\csname R@an.perclass_all.rep.kits.senull\endcsname{0.726}
\expandafter\gdef\csname R@an.perclass_all.rep.kits.spread2\endcsname{0.592}
\expandafter\gdef\csname R@an.perclass_all.rep.ncopri\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.rep.ncopri_landed\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.rep.ncopri_over_bar\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.rep.nds\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.rep.nfresh_landed\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.rep.nfresh_over_bar\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.rowlabels.cut\endcsname{HyReX, finer ConvNeXt to HyReX, finer…}
\expandafter\gdef\csname R@an.perclass_all.scope.hero.landed\endcsname{AMOS22, KiTS23 and ACDC}
\expandafter\gdef\csname R@an.perclass_all.scope.hero.nlanded\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.scope.hero.none\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.scope.hero.npending\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.scope.hero.pending\endcsname{none}
\expandafter\gdef\csname R@an.perclass_all.screen.bar\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.perclass_all.sd.acdc.c1\endcsname{0.17}
\expandafter\gdef\csname R@an.perclass_all.sd.acdc.c2\endcsname{0.11}
\expandafter\gdef\csname R@an.perclass_all.sd.acdc.c3\endcsname{0.10}
\expandafter\gdef\csname R@an.perclass_all.sd.acdc.max\endcsname{0.17}
\expandafter\gdef\csname R@an.perclass_all.sd.acdc.min\endcsname{0.10}
\expandafter\gdef\csname R@an.perclass_all.sd.acdc.ratio\endcsname{1.7}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.c1\endcsname{0.27}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.c10\endcsname{0.38}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.c11\endcsname{0.15}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.c12\endcsname{0.86}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.c13\endcsname{0.37}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.c14\endcsname{0.24}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.c15\endcsname{1.02}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.c2\endcsname{0.41}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.c3\endcsname{0.34}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.c4\endcsname{1.23}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.c5\endcsname{0.29}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.c6\endcsname{0.14}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.c7\endcsname{0.26}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.c8\endcsname{0.11}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.c9\endcsname{0.12}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.max\endcsname{1.229}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.min\endcsname{0.107}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.ratio\endcsname{11.5}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.rho\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@an.perclass_all.sd.amos.rho_p\endcsname{0.071}
\expandafter\gdef\csname R@an.perclass_all.sd.kits.c123\endcsname{0.39}
\expandafter\gdef\csname R@an.perclass_all.sd.kits.c2\endcsname{1.06}
\expandafter\gdef\csname R@an.perclass_all.sd.kits.c23\endcsname{1.08}
\expandafter\gdef\csname R@an.perclass_all.sd.kits.max\endcsname{1.08}
\expandafter\gdef\csname R@an.perclass_all.sd.kits.min\endcsname{0.39}
\expandafter\gdef\csname R@an.perclass_all.sd.kits.ratio\endcsname{2.8}
\expandafter\gdef\csname R@an.perclass_all.sdpair.acdc.c1\endcsname{0.21}
\expandafter\gdef\csname R@an.perclass_all.sdpair.acdc.c2\endcsname{0.13}
\expandafter\gdef\csname R@an.perclass_all.sdpair.acdc.c3\endcsname{0.12}
\expandafter\gdef\csname R@an.perclass_all.sdpair.amos.c1\endcsname{0.33}
\expandafter\gdef\csname R@an.perclass_all.sdpair.amos.c10\endcsname{0.46}
\expandafter\gdef\csname R@an.perclass_all.sdpair.amos.c11\endcsname{0.19}
\expandafter\gdef\csname R@an.perclass_all.sdpair.amos.c12\endcsname{1.05}
\expandafter\gdef\csname R@an.perclass_all.sdpair.amos.c13\endcsname{0.45}
\expandafter\gdef\csname R@an.perclass_all.sdpair.amos.c14\endcsname{0.29}
\expandafter\gdef\csname R@an.perclass_all.sdpair.amos.c15\endcsname{1.25}
\expandafter\gdef\csname R@an.perclass_all.sdpair.amos.c2\endcsname{0.51}
\expandafter\gdef\csname R@an.perclass_all.sdpair.amos.c3\endcsname{0.41}
\expandafter\gdef\csname R@an.perclass_all.sdpair.amos.c4\endcsname{1.51}
\expandafter\gdef\csname R@an.perclass_all.sdpair.amos.c5\endcsname{0.36}
\expandafter\gdef\csname R@an.perclass_all.sdpair.amos.c6\endcsname{0.18}
\expandafter\gdef\csname R@an.perclass_all.sdpair.amos.c7\endcsname{0.32}
\expandafter\gdef\csname R@an.perclass_all.sdpair.amos.c8\endcsname{0.13}
\expandafter\gdef\csname R@an.perclass_all.sdpair.amos.c9\endcsname{0.14}
\expandafter\gdef\csname R@an.perclass_all.sdpair.kits.c123\endcsname{0.48}
\expandafter\gdef\csname R@an.perclass_all.sdpair.kits.c2\endcsname{1.30}
\expandafter\gdef\csname R@an.perclass_all.sdpair.kits.c23\endcsname{1.32}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.armclause\endcsname{2 of the 4 arms move by more than a structure's own seed SD on at least one structure (the single-arm movement farthest from zero is \ensuremath{-0.30} pp on LVC, 3.01 times that structure's seed SD)}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.armmax_arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.armmax_class\endcsname{LVC}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.armmax_pp\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.armmax_rel\endcsname{3.01}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.c1.mean\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.c1.ndown\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.c1.rel\endcsname{0.04}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.c2.mean\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.c2.ndown\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.c2.rel\endcsname{0.33}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.c3.mean\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.c3.ndown\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.c3.rel\endcsname{1.02}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.dirword\endcsname{in both directions}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.maxclass\endcsname{LVC}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.maxclass_agent_mean\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.maxclass_agent_n\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.maxclass_base_mean\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.maxclass_base_n\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.maxclass_ndown\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.maxclass_nup\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.maxdir\endcsname{down}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.maxmean\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.maxrel\endcsname{1.02}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.meanclause\endcsname{beyond one seed SD of its own structure on 1 of the 3 structures}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.narm_over1\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.ncell\endcsname{12}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.ncell_over1\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.nclass\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.ndownclass\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.shrink.acdc.nover1\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.armclause\endcsname{every one of the 5 arms moves by more than an organ's own seed SD on at least one organ (the single-arm movement farthest from zero is \ensuremath{-2.39} pp on spleen, 8.90 times that organ's seed SD)}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.armmax_arm\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.armmax_class\endcsname{spleen}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.armmax_pp\endcsname{\ensuremath{-2.39}}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.armmax_rel\endcsname{8.90}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c1.mean\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c1.ndown\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c1.rel\endcsname{1.32}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c10.mean\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c10.ndown\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c10.rel\endcsname{0.16}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c11.mean\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c11.ndown\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c11.rel\endcsname{0.89}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c12.mean\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c12.ndown\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c12.rel\endcsname{0.35}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c13.mean\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c13.ndown\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c13.rel\endcsname{0.22}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c14.mean\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c14.ndown\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c14.rel\endcsname{0.79}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c15.mean\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c15.ndown\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c15.rel\endcsname{0.20}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c2.mean\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c2.ndown\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c2.rel\endcsname{0.44}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c3.mean\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c3.ndown\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c3.rel\endcsname{0.67}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c4.mean\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c4.ndown\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c4.rel\endcsname{0.43}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c5.mean\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c5.ndown\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c5.rel\endcsname{0.37}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c6.mean\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c6.ndown\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c6.rel\endcsname{0.54}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c7.mean\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c7.ndown\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c7.rel\endcsname{0.48}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c8.mean\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c8.ndown\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c8.rel\endcsname{0.48}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c9.mean\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c9.ndown\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.c9.rel\endcsname{1.10}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.dirword\endcsname{in both directions}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.maxclass\endcsname{spleen}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.maxclass_agent_mean\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.maxclass_agent_n\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.maxclass_base_mean\endcsname{\ensuremath{-1.21}}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.maxclass_base_n\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.maxclass_ndown\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.maxclass_nup\endcsname{1}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.maxdir\endcsname{down}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.maxmean\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.maxrel\endcsname{1.32}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.meanclause\endcsname{beyond one seed SD of its own organ on 2 of the 15 organs}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.narm_over1\endcsname{5}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.ncell\endcsname{75}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.ncell_over1\endcsname{34}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.nclass\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.ndownclass\endcsname{10}
\expandafter\gdef\csname R@an.perclass_all.shrink.amos.nover1\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.armclause\endcsname{14 of the 25 arms move by more than a region's own seed SD on at least one region (the single-arm movement farthest from zero is \ensuremath{-2.50} pp on tumour, 2.35 times that region's seed SD)}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.armmax_arm\endcsname{LeanNeXt-s5 with one convolution at encoder stages 0, 1 and 4 (LeanTrunk)}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.armmax_class\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.armmax_pp\endcsname{\ensuremath{-2.50}}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.armmax_rel\endcsname{2.35}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.c123.mean\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.c123.ndown\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.c123.rel\endcsname{0.18}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.c2.mean\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.c2.ndown\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.c2.rel\endcsname{0.44}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.c23.mean\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.c23.ndown\endcsname{15}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.c23.rel\endcsname{0.31}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.dirword\endcsname{in both directions}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.maxclass\endcsname{tumour}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.maxclass_agent_mean\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.maxclass_agent_n\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.maxclass_base_mean\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.maxclass_base_n\endcsname{4}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.maxclass_ndown\endcsname{17}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.maxclass_nup\endcsname{8}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.maxdir\endcsname{down}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.maxmean\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.maxrel\endcsname{0.44}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.meanclause\endcsname{inside one seed SD of its own region on every region}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.narm_over1\endcsname{14}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.ncell\endcsname{75}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.ncell_over1\endcsname{21}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.nclass\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.ndownclass\endcsname{3}
\expandafter\gdef\csname R@an.perclass_all.shrink.kits.nover1\endcsname{0}
\expandafter\gdef\csname R@an.perclass_all.undrawncols\endcsname{HyReX, width-scaled (M); HyReX, width-scaled (L); full-res addition; full-res kernel $3^3$; coarse-capacity control (parameter-matched); logit warp (head 0)}
\expandafter\gdef\csname R@an.perclass_all.wc.acdc_resolved.sentence\endcsname{HyReX has a resolved lead over every other arm on every ACDC structure}
\expandafter\gdef\csname R@an.perclass_all.wc.all3.sentence\endcsname{HyReX improves on the nnU-Net default on every one of the three datasets}
\expandafter\gdef\csname R@an.perclass_all.wc.parity.sentence\endcsname{HyReX and the ResEnc-M preset are level on KiTS23}
\expandafter\gdef\csname R@an.perclass_all.zbig\endcsname{2}
\expandafter\gdef\csname R@an.perclass_all.zbig.word\endcsname{two}
\expandafter\gdef\csname R@an.perclass_stock.all.delta\endcsname{\ensuremath{+1.56}}
\expandafter\gdef\csname R@an.perclass_stock.all.delta_xa\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.perclass_stock.all.name\endcsname{Mean of the three regions}
\expandafter\gdef\csname R@an.perclass_stock.all.pool\endcsname{83.38}
\expandafter\gdef\csname R@an.perclass_stock.all.se\endcsname{0.49}
\expandafter\gdef\csname R@an.perclass_stock.all.se_xa\endcsname{0.49}
\expandafter\gdef\csname R@an.perclass_stock.all.stock\endcsname{84.26}
\expandafter\gdef\csname R@an.perclass_stock.all.stock.sd\endcsname{0.63}
\expandafter\gdef\csname R@an.perclass_stock.all.vspool\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.perclass_stock.all.xa\endcsname{86.04}
\expandafter\gdef\csname R@an.perclass_stock.all.xl\endcsname{85.82}
\expandafter\gdef\csname R@an.perclass_stock.c123.delta\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.perclass_stock.c123.delta_xa\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@an.perclass_stock.c123.name\endcsname{Kidney region}
\expandafter\gdef\csname R@an.perclass_stock.c123.pool\endcsname{96.02}
\expandafter\gdef\csname R@an.perclass_stock.c123.se\endcsname{0.26}
\expandafter\gdef\csname R@an.perclass_stock.c123.se_xa\endcsname{0.26}
\expandafter\gdef\csname R@an.perclass_stock.c123.stock\endcsname{96.34}
\expandafter\gdef\csname R@an.perclass_stock.c123.stock.sd\endcsname{0.33}
\expandafter\gdef\csname R@an.perclass_stock.c123.vspool\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.perclass_stock.c123.xa\endcsname{97.17}
\expandafter\gdef\csname R@an.perclass_stock.c123.xl\endcsname{97.27}
\expandafter\gdef\csname R@an.perclass_stock.c2.delta\endcsname{\ensuremath{+1.87}}
\expandafter\gdef\csname R@an.perclass_stock.c2.delta_xa\endcsname{\ensuremath{+2.21}}
\expandafter\gdef\csname R@an.perclass_stock.c2.name\endcsname{Tumour}
\expandafter\gdef\csname R@an.perclass_stock.c2.pool\endcsname{74.27}
\expandafter\gdef\csname R@an.perclass_stock.c2.se\endcsname{0.74}
\expandafter\gdef\csname R@an.perclass_stock.c2.se_xa\endcsname{0.74}
\expandafter\gdef\csname R@an.perclass_stock.c2.stock\endcsname{75.46}
\expandafter\gdef\csname R@an.perclass_stock.c2.stock.sd\endcsname{0.95}
\expandafter\gdef\csname R@an.perclass_stock.c2.vspool\endcsname{\ensuremath{+1.19}}
\expandafter\gdef\csname R@an.perclass_stock.c2.xa\endcsname{77.67}
\expandafter\gdef\csname R@an.perclass_stock.c2.xl\endcsname{77.33}
\expandafter\gdef\csname R@an.perclass_stock.c23.delta\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@an.perclass_stock.c23.delta_xa\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.perclass_stock.c23.name\endcsname{Masses}
\expandafter\gdef\csname R@an.perclass_stock.c23.pool\endcsname{79.84}
\expandafter\gdef\csname R@an.perclass_stock.c23.se\endcsname{0.71}
\expandafter\gdef\csname R@an.perclass_stock.c23.se_xa\endcsname{0.71}
\expandafter\gdef\csname R@an.perclass_stock.c23.stock\endcsname{80.97}
\expandafter\gdef\csname R@an.perclass_stock.c23.stock.sd\endcsname{0.90}
\expandafter\gdef\csname R@an.perclass_stock.c23.vspool\endcsname{\ensuremath{+1.13}}
\expandafter\gdef\csname R@an.perclass_stock.c23.xa\endcsname{83.28}
\expandafter\gdef\csname R@an.perclass_stock.c23.xl\endcsname{82.85}
\expandafter\gdef\csname R@an.perclass_stock.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.perclass_stock.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.perclass_stock.rule\endcsname{the standard error is the Welch standard error of a difference of two means: the square root of s squared over the number of arm runs plus s squared over the number of stock runs, with s the SD of the stock runs in that region for both terms (an arm's own SD of two runs is not a run-level SD); it describes how far a mean of two runs can differ from a mean of the stock runs through run-to-run variation of the recipe alone, and states no inference}
\expandafter\gdef\csname R@an.perclass_stock.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of {\ifdefined\archL\archL\else XX-Net-L\fi} differs from the mean of nnU-Net's nine stock runs by \ensuremath{+0.93}\,pp on the kidney region (SE 0.26), \ensuremath{+1.88}\,pp on the masses (SE 0.71) and \ensuremath{+1.87}\,pp on the tumour (SE 0.74), and that of {\ifdefined\archA\archA\else XX-Net-A\fi} by \ensuremath{+0.83}\,pp on the kidney region (SE 0.26), \ensuremath{+2.31}\,pp on the masses (SE 0.71) and \ensuremath{+2.21}\,pp on the tumour (SE 0.74)}
\expandafter\gdef\csname R@an.perclass_stock.state\endcsname{9 stock runs, XX-Net-L fresh pair complete, XX-Net-A fresh pair complete}
\expandafter\gdef\csname R@an.perclass_stock.stock.seeds\endcsname{3--11}
\expandafter\gdef\csname R@an.perclass_stock.xa.tag\endcsname{V7A1}
\expandafter\gdef\csname R@an.perclass_stock.xl.tag\endcsname{V7C1}
\expandafter\gdef\csname R@an.power_design.EK_acdc_gf\endcsname{1.31}
\expandafter\gdef\csname R@an.power_design.EK_acdc_pf\endcsname{0.03}
\expandafter\gdef\csname R@an.power_design.EK_amos\endcsname{0.29}
\expandafter\gdef\csname R@an.power_design.EK_kits\endcsname{2.59}
\expandafter\gdef\csname R@an.power_design.acdc_F_p\endcsname{0.10}
\expandafter\gdef\csname R@an.power_design.acdc_between\endcsname{0.088}
\expandafter\gdef\csname R@an.power_design.acdc_cls_indep\endcsname{1.75}
\expandafter\gdef\csname R@an.power_design.acdc_cls_max_name\endcsname{RV}
\expandafter\gdef\csname R@an.power_design.acdc_cls_max_sd\endcsname{0.17}
\expandafter\gdef\csname R@an.power_design.acdc_cls_min_name\endcsname{LVC}
\expandafter\gdef\csname R@an.power_design.acdc_cls_min_sd\endcsname{0.10}
\expandafter\gdef\csname R@an.power_design.acdc_comp_diff\endcsname{\ensuremath{-0.014}}
\expandafter\gdef\csname R@an.power_design.acdc_comp_mean_c\endcsname{92.002}
\expandafter\gdef\csname R@an.power_design.acdc_comp_mean_u\endcsname{92.016}
\expandafter\gdef\csname R@an.power_design.acdc_comp_z\endcsname{0.17}
\expandafter\gdef\csname R@an.power_design.acdc_icc\endcsname{0.69}
\expandafter\gdef\csname R@an.power_design.acdc_mean\endcsname{92.009}
\expandafter\gdef\csname R@an.power_design.acdc_n\endcsname{6}
\expandafter\gdef\csname R@an.power_design.acdc_nseed\endcsname{3}
\expandafter\gdef\csname R@an.power_design.acdc_pub_vs_rung\endcsname{above the one-seed rung}
\expandafter\gdef\csname R@an.power_design.acdc_pub_vs_rung_both\endcsname{above the one-seed rung on the seed scale and below the floor on the total-variance scale}
\expandafter\gdef\csname R@an.power_design.acdc_pub_vs_rung_total\endcsname{below the floor}
\expandafter\gdef\csname R@an.power_design.acdc_sd\endcsname{0.099}
\expandafter\gdef\csname R@an.power_design.acdc_sd_delta_cl\endcsname{0.114}
\expandafter\gdef\csname R@an.power_design.acdc_sd_fhi\endcsname{2.45}
\expandafter\gdef\csname R@an.power_design.acdc_sd_flo\endcsname{0.62}
\expandafter\gdef\csname R@an.power_design.acdc_sd_hi\endcsname{0.24}
\expandafter\gdef\csname R@an.power_design.acdc_sd_lo\endcsname{0.06}
\expandafter\gdef\csname R@an.power_design.acdc_se_cl\endcsname{0.056}
\expandafter\gdef\csname R@an.power_design.acdc_se_naive\endcsname{0.040}
\expandafter\gdef\csname R@an.power_design.acdc_se_under\endcsname{40}
\expandafter\gdef\csname R@an.power_design.acdc_trip_cl2\endcsname{15.92}
\expandafter\gdef\csname R@an.power_design.acdc_trip_cl5\endcsname{12.24}
\expandafter\gdef\csname R@an.power_design.acdc_within\endcsname{0.059}
\expandafter\gdef\csname R@an.power_design.amos_F_p\endcsname{0.17}
\expandafter\gdef\csname R@an.power_design.amos_between\endcsname{0.095}
\expandafter\gdef\csname R@an.power_design.amos_cls_indep\endcsname{0.80}
\expandafter\gdef\csname R@an.power_design.amos_cls_max_name\endcsname{gall bladder}
\expandafter\gdef\csname R@an.power_design.amos_cls_max_sd\endcsname{1.23}
\expandafter\gdef\csname R@an.power_design.amos_cls_min_name\endcsname{aorta}
\expandafter\gdef\csname R@an.power_design.amos_cls_min_sd\endcsname{0.11}
\expandafter\gdef\csname R@an.power_design.amos_cls_top3_names\endcsname{gall bladder, prostate/uterus, left adrenal gland}
\expandafter\gdef\csname R@an.power_design.amos_cls_top3_share\endcsname{78}
\expandafter\gdef\csname R@an.power_design.amos_comp_diff\endcsname{\ensuremath{-0.058}}
\expandafter\gdef\csname R@an.power_design.amos_comp_mean_c\endcsname{87.672}
\expandafter\gdef\csname R@an.power_design.amos_comp_mean_u\endcsname{87.730}
\expandafter\gdef\csname R@an.power_design.amos_comp_z\endcsname{0.58}
\expandafter\gdef\csname R@an.power_design.amos_icc\endcsname{0.54}
\expandafter\gdef\csname R@an.power_design.amos_mean\endcsname{87.701}
\expandafter\gdef\csname R@an.power_design.amos_n\endcsname{6}
\expandafter\gdef\csname R@an.power_design.amos_nseed\endcsname{3}
\expandafter\gdef\csname R@an.power_design.amos_sd\endcsname{0.122}
\expandafter\gdef\csname R@an.power_design.amos_sd_delta_cl\endcsname{0.139}
\expandafter\gdef\csname R@an.power_design.amos_sd_fhi\endcsname{2.45}
\expandafter\gdef\csname R@an.power_design.amos_sd_flo\endcsname{0.62}
\expandafter\gdef\csname R@an.power_design.amos_sd_hi\endcsname{0.30}
\expandafter\gdef\csname R@an.power_design.amos_sd_lo\endcsname{0.08}
\expandafter\gdef\csname R@an.power_design.amos_se_cl\endcsname{0.066}
\expandafter\gdef\csname R@an.power_design.amos_se_naive\endcsname{0.050}
\expandafter\gdef\csname R@an.power_design.amos_se_under\endcsname{32}
\expandafter\gdef\csname R@an.power_design.amos_trip_cl2\endcsname{6.38}
\expandafter\gdef\csname R@an.power_design.amos_trip_cl5\endcsname{2.65}
\expandafter\gdef\csname R@an.power_design.amos_within\endcsname{0.088}
\expandafter\gdef\csname R@an.power_design.amosu_EK\endcsname{1.10}
\expandafter\gdef\csname R@an.power_design.amosu_best_m11\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.power_design.amosu_best_m11_ub\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.power_design.amosu_d_l1\endcsname{\ensuremath{+0.618}}
\expandafter\gdef\csname R@an.power_design.amosu_d_l2\endcsname{\ensuremath{+0.333}}
\expandafter\gdef\csname R@an.power_design.amosu_d_l3\endcsname{\ensuremath{+0.353}}
\expandafter\gdef\csname R@an.power_design.amosu_d_l4\endcsname{\ensuremath{+0.401}}
\expandafter\gdef\csname R@an.power_design.amosu_floor\endcsname{0.47}
\expandafter\gdef\csname R@an.power_design.amosu_floorp\endcsname{0.23}
\expandafter\gdef\csname R@an.power_design.amosu_mde_n1\endcsname{0.94}
\expandafter\gdef\csname R@an.power_design.amosu_mde_n3\endcsname{0.66}
\expandafter\gdef\csname R@an.power_design.amosu_mde_n6\endcsname{0.57}
\expandafter\gdef\csname R@an.power_design.amosu_mdep_n1\endcsname{0.94}
\expandafter\gdef\csname R@an.power_design.amosu_mdep_n3\endcsname{0.44}
\expandafter\gdef\csname R@an.power_design.amosu_mdep_n6\endcsname{0.33}
\expandafter\gdef\csname R@an.power_design.amosu_mean\endcsname{87.730}
\expandafter\gdef\csname R@an.power_design.amosu_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.amosu_nclear\endcsname{4}
\expandafter\gdef\csname R@an.power_design.amosu_obs_arm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.power_design.amosu_obs_best\endcsname{\ensuremath{+0.618}}
\expandafter\gdef\csname R@an.power_design.amosu_pK\endcsname{11}
\expandafter\gdef\csname R@an.power_design.amosu_pK_indep\endcsname{2.0}
\expandafter\gdef\csname R@an.power_design.amosu_pclear_m11\endcsname{36}
\expandafter\gdef\csname R@an.power_design.amosu_pclear_m11_ub\endcsname{62}
\expandafter\gdef\csname R@an.power_design.amosu_pglobal\endcsname{16}
\expandafter\gdef\csname R@an.power_design.amosu_pglobal_ub\endcsname{35}
\expandafter\gdef\csname R@an.power_design.amosu_sd\endcsname{0.143}
\expandafter\gdef\csname R@an.power_design.amosu_sd_hi\endcsname{0.90}
\expandafter\gdef\csname R@an.power_design.amosu_sd_lo\endcsname{0.07}
\expandafter\gdef\csname R@an.power_design.amosu_seeds_l1_l1b\endcsname{6}
\expandafter\gdef\csname R@an.power_design.amosu_seeds_l3_default\endcsname{$\infty$}
\expandafter\gdef\csname R@an.power_design.amosu_seeds_l3_l1\endcsname{19}
\expandafter\gdef\csname R@an.power_design.amosu_seeds_thr\endcsname{$\infty$}
\expandafter\gdef\csname R@an.power_design.amosu_seedsp_l1_l1b\endcsname{3}
\expandafter\gdef\csname R@an.power_design.amosu_seedsp_l3_default\endcsname{5}
\expandafter\gdef\csname R@an.power_design.amosu_seedsp_l3_l1\endcsname{6}
\expandafter\gdef\csname R@an.power_design.amosu_seedsp_thr\endcsname{6}
\expandafter\gdef\csname R@an.power_design.bar\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.power_design.best_acdc_m12\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.power_design.best_acdc_m12_lb\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.power_design.best_acdc_m12_lb_sdhi\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.power_design.best_acdc_m12_lb_sdlo\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.power_design.best_acdc_m12_q95\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.power_design.best_acdc_m12_scl2\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.power_design.best_acdc_m12_scl5\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.power_design.best_acdc_m12_ub\endcsname{\ensuremath{+0.230}}
\expandafter\gdef\csname R@an.power_design.best_acdc_m_at_gf\endcsname{7}
\expandafter\gdef\csname R@an.power_design.best_acdc_m_at_pf\endcsname{$>$30}
\expandafter\gdef\csname R@an.power_design.best_acdc_mrun\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.power_design.best_acdc_mrun_lb\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.power_design.best_acdc_mrun_lb_sdhi\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.power_design.best_acdc_mrun_lb_sdlo\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.power_design.best_acdc_mrun_q95\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.power_design.best_acdc_mrun_scl2\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.power_design.best_acdc_mrun_scl5\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.power_design.best_acdc_mrun_ub\endcsname{\ensuremath{+0.230}}
\expandafter\gdef\csname R@an.power_design.best_amos_m11\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.power_design.best_amos_m11_lb\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.power_design.best_amos_m11_lb_sdhi\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.power_design.best_amos_m11_lb_sdlo\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.power_design.best_amos_m11_q95\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.power_design.best_amos_m11_scl2\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.power_design.best_amos_m11_scl5\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.power_design.best_amos_m11_ub\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.power_design.best_amos_m12\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.power_design.best_amos_m12_lb\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.power_design.best_amos_m12_lb_sdhi\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.power_design.best_amos_m12_lb_sdlo\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.power_design.best_amos_m12_q95\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.power_design.best_amos_m12_ub\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.power_design.best_amos_m13\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.power_design.best_amos_m13_lb\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.power_design.best_amos_m13_lb_sdhi\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.power_design.best_amos_m13_lb_sdlo\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.power_design.best_amos_m13_q95\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.power_design.best_amos_m13_ub\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.power_design.best_amos_m_at_bar\endcsname{$>$30}
\expandafter\gdef\csname R@an.power_design.best_amos_mrun\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.power_design.best_amos_mrun_lb\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.power_design.best_amos_mrun_lb_sdhi\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.power_design.best_amos_mrun_lb_sdlo\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.power_design.best_amos_mrun_q95\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.power_design.best_amos_mrun_ub\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.power_design.best_kits_m11\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.power_design.best_kits_m11_lb\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.power_design.best_kits_m11_lb_sdhi\endcsname{\ensuremath{+7.9}}
\expandafter\gdef\csname R@an.power_design.best_kits_m11_lb_sdlo\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.power_design.best_kits_m11_q95\endcsname{\ensuremath{+6.2}}
\expandafter\gdef\csname R@an.power_design.best_kits_m11_ub\endcsname{\ensuremath{+3.6}}
\expandafter\gdef\csname R@an.power_design.best_kits_m12\endcsname{\ensuremath{+2.3}}
\expandafter\gdef\csname R@an.power_design.best_kits_m12_lb\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.power_design.best_kits_m12_lb_sdhi\endcsname{\ensuremath{+8.1}}
\expandafter\gdef\csname R@an.power_design.best_kits_m12_lb_sdlo\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.power_design.best_kits_m12_q95\endcsname{\ensuremath{+6.3}}
\expandafter\gdef\csname R@an.power_design.best_kits_m12_ub\endcsname{\ensuremath{+3.8}}
\expandafter\gdef\csname R@an.power_design.best_kits_m7\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.power_design.best_kits_m7_lb\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.power_design.best_kits_m7_lb_sdhi\endcsname{\ensuremath{+6.8}}
\expandafter\gdef\csname R@an.power_design.best_kits_m7_lb_sdlo\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.power_design.best_kits_m7_q95\endcsname{\ensuremath{+5.5}}
\expandafter\gdef\csname R@an.power_design.best_kits_m7_ub\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.power_design.best_kits_m_at_bar\endcsname{2}
\expandafter\gdef\csname R@an.power_design.best_kits_mrun\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.power_design.best_kits_mrun_lb\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.power_design.best_kits_mrun_lb_sdhi\endcsname{\ensuremath{+6.8}}
\expandafter\gdef\csname R@an.power_design.best_kits_mrun_lb_sdlo\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.power_design.best_kits_mrun_q95\endcsname{\ensuremath{+5.5}}
\expandafter\gdef\csname R@an.power_design.best_kits_mrun_ub\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.power_design.cluster_s2_under\endcsname{20}
\expandafter\gdef\csname R@an.power_design.cluster_s2_weight\endcsname{0.8}
\expandafter\gdef\csname R@an.power_design.curse_nsim\endcsname{200000}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L1base_dcv\endcsname{\ensuremath{+0.370}}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L1base_hi\endcsname{\ensuremath{+0.476}}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L1base_lo\endcsname{\ensuremath{+0.263}}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L1base_minres\endcsname{0.106}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L1base_minres_hi\endcsname{0.4}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L1base_minres_lo\endcsname{0.06}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L1base_nfold\endcsname{4}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L1base_ratio\endcsname{3.5}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L1base_rung\endcsname{0.142}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L1base_sd\endcsname{0.067}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L1base_se\endcsname{0.033}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3L1_dcv\endcsname{\ensuremath{-0.037}}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3L1_hi\endcsname{\ensuremath{+0.240}}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3L1_lo\endcsname{\ensuremath{-0.314}}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3L1_minres\endcsname{0.277}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3L1_minres_hi\endcsname{1.0}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3L1_minres_lo\endcsname{0.16}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3L1_nfold\endcsname{4}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3L1_ratio\endcsname{0.13}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3L1_rung\endcsname{0.371}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3L1_sd\endcsname{0.174}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3L1_se\endcsname{0.087}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3base_dcv\endcsname{\ensuremath{+0.333}}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3base_hi\endcsname{\ensuremath{+0.563}}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3base_lo\endcsname{\ensuremath{+0.102}}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3base_minres\endcsname{0.230}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3base_minres_hi\endcsname{0.9}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3base_minres_lo\endcsname{0.13}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3base_nfold\endcsname{4}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3base_ratio\endcsname{1.4}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3base_rung\endcsname{0.308}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3base_sd\endcsname{0.145}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_L3base_se\endcsname{0.072}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_dcv\endcsname{\ensuremath{+0.333}}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_minres\endcsname{0.230}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_nfold\endcsname{4}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_rung\endcsname{0.308}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_sd\endcsname{0.145}
\expandafter\gdef\csname R@an.power_design.cvres_acdc_sentence\endcsname{On ACDC the four fold differences of HyReX minus the default network have an SD of 0.145\,pp, so a four-fold mean must exceed 0.230\,pp for its paired-$t$ interval (3.18 times the standard error, on 3 degrees of freedom) to exclude zero; the observed mean is \ensuremath{+0.333}\,pp}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L1base_dcv\endcsname{\ensuremath{+0.406}}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L1base_hi\endcsname{\ensuremath{+1.086}}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L1base_lo\endcsname{\ensuremath{-0.274}}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L1base_minres\endcsname{0.680}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L1base_minres_hi\endcsname{2.5}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L1base_minres_lo\endcsname{0.39}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L1base_nfold\endcsname{4}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L1base_ratio\endcsname{0.60}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L1base_rung\endcsname{0.909}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L1base_sd\endcsname{0.427}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L1base_se\endcsname{0.214}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3L1_dcv\endcsname{\ensuremath{-0.178}}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3L1_hi\endcsname{\ensuremath{+0.402}}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3L1_lo\endcsname{\ensuremath{-0.758}}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3L1_minres\endcsname{0.580}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3L1_minres_hi\endcsname{2.2}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3L1_minres_lo\endcsname{0.33}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3L1_nfold\endcsname{4}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3L1_ratio\endcsname{0.31}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3L1_rung\endcsname{0.776}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3L1_sd\endcsname{0.364}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3L1_se\endcsname{0.182}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3base_dcv\endcsname{\ensuremath{+0.228}}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3base_hi\endcsname{\ensuremath{+0.535}}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3base_lo\endcsname{\ensuremath{-0.078}}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3base_minres\endcsname{0.307}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3base_minres_hi\endcsname{1.1}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3base_minres_lo\endcsname{0.17}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3base_nfold\endcsname{4}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3base_ratio\endcsname{0.74}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3base_rung\endcsname{0.410}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3base_sd\endcsname{0.193}
\expandafter\gdef\csname R@an.power_design.cvres_amos_L3base_se\endcsname{0.096}
\expandafter\gdef\csname R@an.power_design.cvres_amos_dcv\endcsname{\ensuremath{+0.228}}
\expandafter\gdef\csname R@an.power_design.cvres_amos_minres\endcsname{0.307}
\expandafter\gdef\csname R@an.power_design.cvres_amos_nfold\endcsname{4}
\expandafter\gdef\csname R@an.power_design.cvres_amos_rung\endcsname{0.410}
\expandafter\gdef\csname R@an.power_design.cvres_amos_sd\endcsname{0.193}
\expandafter\gdef\csname R@an.power_design.cvres_amos_sentence\endcsname{On AMOS22 the four fold differences of HyReX minus the default network have an SD of 0.193\,pp, so a four-fold mean must exceed 0.307\,pp for its paired-$t$ interval (3.18 times the standard error, on 3 degrees of freedom) to exclude zero; the observed mean is \ensuremath{+0.228}\,pp}
\expandafter\gdef\csname R@an.power_design.cvres_df\endcsname{3}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L1base_dcv\endcsname{\ensuremath{+2.147}}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L1base_hi\endcsname{\ensuremath{+3.319}}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L1base_lo\endcsname{\ensuremath{+0.976}}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L1base_minres\endcsname{1.171}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L1base_minres_hi\endcsname{4.4}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L1base_minres_lo\endcsname{0.66}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L1base_nfold\endcsname{4}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L1base_ratio\endcsname{1.8}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L1base_rung\endcsname{1.567}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L1base_sd\endcsname{0.736}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L1base_se\endcsname{0.368}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3L1_dcv\endcsname{\ensuremath{-1.465}}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3L1_hi\endcsname{\ensuremath{+0.239}}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3L1_lo\endcsname{\ensuremath{-3.170}}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3L1_minres\endcsname{1.705}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3L1_minres_hi\endcsname{6.4}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3L1_minres_lo\endcsname{0.97}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3L1_nfold\endcsname{4}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3L1_ratio\endcsname{0.86}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3L1_rung\endcsname{2.280}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3L1_sd\endcsname{1.071}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3L1_se\endcsname{0.536}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3base_dcv\endcsname{\ensuremath{+0.682}}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3base_hi\endcsname{\ensuremath{+2.441}}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3base_lo\endcsname{\ensuremath{-1.078}}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3base_minres\endcsname{1.760}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3base_minres_hi\endcsname{6.6}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3base_minres_lo\endcsname{1.00}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3base_nfold\endcsname{4}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3base_ratio\endcsname{0.39}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3base_rung\endcsname{2.353}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3base_sd\endcsname{1.106}
\expandafter\gdef\csname R@an.power_design.cvres_kits_L3base_se\endcsname{0.553}
\expandafter\gdef\csname R@an.power_design.cvres_kits_dcv\endcsname{\ensuremath{+0.682}}
\expandafter\gdef\csname R@an.power_design.cvres_kits_minres\endcsname{1.760}
\expandafter\gdef\csname R@an.power_design.cvres_kits_nfold\endcsname{4}
\expandafter\gdef\csname R@an.power_design.cvres_kits_rung\endcsname{2.353}
\expandafter\gdef\csname R@an.power_design.cvres_kits_sd\endcsname{1.106}
\expandafter\gdef\csname R@an.power_design.cvres_kits_sentence\endcsname{On KiTS23 the four fold differences of HyReX minus the default network have an SD of 1.106\,pp, so a four-fold mean must exceed 1.760\,pp for its paired-$t$ interval (3.18 times the standard error, on 3 degrees of freedom) to exclude zero; the observed mean is \ensuremath{+0.682}\,pp}
\expandafter\gdef\csname R@an.power_design.cvres_label\endcsname{descriptive: computed from the observed SD of four fold differences, an estimate on three degrees of freedom, with one seed per fold; not a power calculation, not a test and not a statement about another set of folds}
\expandafter\gdef\csname R@an.power_design.cvres_nfolds\endcsname{4}
\expandafter\gdef\csname R@an.power_design.cvres_sdhi_factor\endcsname{3.7}
\expandafter\gdef\csname R@an.power_design.cvres_sdlo_factor\endcsname{0.57}
\expandafter\gdef\csname R@an.power_design.cvres_sdsentence\endcsname{The four-fold threshold is itself an SD on three degrees of freedom: it spans 0.57 to 3.7 times its value (descriptive: computed from the observed SD of four fold differences, an estimate on three degrees of freedom, with one seed per fold; not a power calculation, not a test and not a statement about another set of folds)}
\expandafter\gdef\csname R@an.power_design.cvres_tcrit\endcsname{3.18}
\expandafter\gdef\csname R@an.power_design.d_l1_l1b_acdc\endcsname{0.052}
\expandafter\gdef\csname R@an.power_design.d_l1_l1b_amos\endcsname{\ensuremath{+0.509}}
\expandafter\gdef\csname R@an.power_design.d_l1_l1b_kits\endcsname{\ensuremath{+0.583}}
\expandafter\gdef\csname R@an.power_design.d_l3_default_acdc\endcsname{\ensuremath{+0.616}}
\expandafter\gdef\csname R@an.power_design.d_l3_default_acdc_uncompiled\endcsname{\ensuremath{+0.609}}
\expandafter\gdef\csname R@an.power_design.d_l3_default_amos\endcsname{\ensuremath{+0.382}}
\expandafter\gdef\csname R@an.power_design.d_l3_default_amos_contemporaneous\endcsname{\ensuremath{+0.371}}
\expandafter\gdef\csname R@an.power_design.d_l3_default_amos_uncompiled\endcsname{\ensuremath{+0.353}}
\expandafter\gdef\csname R@an.power_design.d_l3_default_kits\endcsname{\ensuremath{+2.842}}
\expandafter\gdef\csname R@an.power_design.d_l3_default_kits_contemporaneous\endcsname{\ensuremath{+2.355}}
\expandafter\gdef\csname R@an.power_design.d_l3_l1_acdc\endcsname{0.281}
\expandafter\gdef\csname R@an.power_design.d_l3_l1_amos\endcsname{\ensuremath{-0.265}}
\expandafter\gdef\csname R@an.power_design.d_l3_l1_kits\endcsname{\ensuremath{+0.516}}
\expandafter\gdef\csname R@an.power_design.fig_acdc_h\endcsname{3.14}
\expandafter\gdef\csname R@an.power_design.fig_acdc_w\endcsname{6.86}
\expandafter\gdef\csname R@an.power_design.fig_curse_h\endcsname{3.01}
\expandafter\gdef\csname R@an.power_design.fig_curse_w\endcsname{6.84}
\expandafter\gdef\csname R@an.power_design.fig_mde_h\endcsname{3.09}
\expandafter\gdef\csname R@an.power_design.fig_mde_w\endcsname{6.80}
\expandafter\gdef\csname R@an.power_design.fig_resolve_h\endcsname{8.91}
\expandafter\gdef\csname R@an.power_design.fig_resolve_w\endcsname{6.74}
\expandafter\gdef\csname R@an.power_design.fig_total_h\endcsname{2.63}
\expandafter\gdef\csname R@an.power_design.fig_total_w\endcsname{6.86}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_altclause\endcsname{Against the uncompiled sub-pool (\ensuremath{+0.007}\,pp from the frozen pool) the same fresh means read HyReX \ensuremath{+0.443}\,pp, ResEnc-matched \ensuremath{+0.312}\,pp, ResEnc-M \ensuremath{+0.235}\,pp and fn.-identical control \ensuremath{+0.110}\,pp; 0 of 4 change side of the unchanged 0.16\,pp edge}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_altname\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_altshift\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_clause\endcsname{At two fresh seeds, against the frozen 6-run pool (two-seed null SD 0.081\,pp, edge 0.16\,pp, rung 0.28\,pp), ResEnc-M's \ensuremath{+0.242}\,pp lies between the null edge and the two-seed rung, HyReX's \ensuremath{+0.450}\,pp lies at or above the two-seed rung, ResEnc-matched's \ensuremath{+0.319}\,pp lies at or above the two-seed rung and fn.-identical control's \ensuremath{+0.117}\,pp lies inside the null edge}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_diff_l3_l1\endcsname{0.208}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_diff_sentence\endcsname{The fresh means of HyReX and ResEnc-M differ by 0.208\,pp, a magnitude with no direction}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_edge\endcsname{0.16}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_flipnames\endcsname{none}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l1_dalt\endcsname{\ensuremath{+0.235}}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l1_delta\endcsname{\ensuremath{+0.242}}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l1_pair\endcsname{\ensuremath{+0.242}\,pp}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l1_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l1_seed1\endcsname{\ensuremath{+0.259}}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l1_seed2\endcsname{\ensuremath{+0.225}}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l1_z\endcsname{3.00}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l1b_dalt\endcsname{\ensuremath{+0.312}}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l1b_delta\endcsname{\ensuremath{+0.319}}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l1b_pair\endcsname{\ensuremath{+0.319}\,pp}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l1b_pos\endcsname{at or above the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l1b_seed1\endcsname{\ensuremath{+0.286}}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l1b_seed2\endcsname{\ensuremath{+0.352}}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l1b_z\endcsname{3.95}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l3_dalt\endcsname{\ensuremath{+0.443}}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l3_delta\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l3_pair\endcsname{\ensuremath{+0.450}\,pp}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l3_pos\endcsname{at or above the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l3_seed1\endcsname{\ensuremath{+0.417}}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l3_seed2\endcsname{\ensuremath{+0.484}}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_l3_z\endcsname{5.58}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_maxarm\endcsname{HyReX}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_maxdalt\endcsname{\ensuremath{+0.443}}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_maxdelta\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_maxrel\endcsname{1.59}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_n\endcsname{4}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_nabove\endcsname{2}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_nbetween\endcsname{1}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_nflip\endcsname{0}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_ninside\endcsname{1}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_npool\endcsname{6}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_nu\endcsname{5}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_nullsd\endcsname{0.081}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_p3c_dalt\endcsname{\ensuremath{+0.110}}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_p3c_delta\endcsname{\ensuremath{+0.117}}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_p3c_pair\endcsname{\ensuremath{+0.117}\,pp}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_p3c_pos\endcsname{inside the null edge}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_p3c_seed1\endcsname{\ensuremath{+0.125}}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_p3c_seed2\endcsname{\ensuremath{+0.109}}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_p3c_z\endcsname{1.45}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_rung\endcsname{0.28}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_rungx\endcsname{1.79}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_tcrit\endcsname{2.57}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_tedge\endcsname{0.21}
\expandafter\gdef\csname R@an.power_design.fr2_acdc_zedge\endcsname{1.96}
\expandafter\gdef\csname R@an.power_design.fr2_amos_alt2clause\endcsname{Against the contemporaneous default runs (\ensuremath{+0.011}\,pp from the frozen pool, three runs) the same fresh means read ResEnc-M \ensuremath{+0.454}\,pp, ResEnc+context \ensuremath{+0.444}\,pp, ResEnc-matched \ensuremath{+0.287}\,pp, ConvNeXt-k3 \ensuremath{+0.184}\,pp and HyReX \ensuremath{+0.121}\,pp; 0 of 5 change side of the unchanged 0.20\,pp edge}
\expandafter\gdef\csname R@an.power_design.fr2_amos_alt2name\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.power_design.fr2_amos_alt2shift\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_altclause\endcsname{Against the uncompiled sub-pool (\ensuremath{+0.029}\,pp from the frozen pool) the same fresh means read ResEnc-M \ensuremath{+0.436}\,pp, ResEnc+context \ensuremath{+0.426}\,pp, ResEnc-matched \ensuremath{+0.269}\,pp, ConvNeXt-k3 \ensuremath{+0.166}\,pp and HyReX \ensuremath{+0.104}\,pp; 0 of 5 change side of the unchanged 0.20\,pp edge}
\expandafter\gdef\csname R@an.power_design.fr2_amos_altname\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.power_design.fr2_amos_altshift\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_anchor\endcsname{At two fresh seeds, against the frozen 6-run pool (two-seed null SD 0.100\,pp; edge 0.20\,pp on the normal scale, 0.26\,pp on the $t$ scale of the pool's five degrees of freedom), AMOS22 separates ResEnc-M's \ensuremath{+0.465}\,pp and does not separate HyReX's \ensuremath{+0.132}\,pp; the ladder's 80\,\%-power rung at two seeds is 0.351\,pp}
\expandafter\gdef\csname R@an.power_design.fr2_amos_bracket\endcsname{At two fresh seeds AMOS22 separates fresh means beyond the 0.20\,pp edge of its two-seed null (1.96 null SDs of 0.100\,pp): the smallest it separates among the arms with a finished pair is 0.298\,pp (ResEnc-matched) and the largest it does not separate is 0.194\,pp (ConvNeXt-k3); the ladder's rung at two seeds is 0.351\,pp}
\expandafter\gdef\csname R@an.power_design.fr2_amos_clause\endcsname{At two fresh seeds, against the frozen 6-run pool (two-seed null SD 0.100\,pp; edge 0.20\,pp on the normal scale, 0.26\,pp on the $t$ scale of the pool's five degrees of freedom), AMOS22 separates ResEnc-M's \ensuremath{+0.465}\,pp, ResEnc+context's \ensuremath{+0.455}\,pp and ResEnc-matched's \ensuremath{+0.298}\,pp; it does not separate ConvNeXt-k3's \ensuremath{+0.194}\,pp and HyReX's \ensuremath{+0.132}\,pp}
\expandafter\gdef\csname R@an.power_design.fr2_amos_diff_l3_l1\endcsname{0.332}
\expandafter\gdef\csname R@an.power_design.fr2_amos_diff_sentence\endcsname{The fresh means of HyReX and ResEnc-M differ by 0.332\,pp, a magnitude with no direction}
\expandafter\gdef\csname R@an.power_design.fr2_amos_edge\endcsname{0.20}
\expandafter\gdef\csname R@an.power_design.fr2_amos_flipnames\endcsname{none}
\expandafter\gdef\csname R@an.power_design.fr2_amos_flipnames2\endcsname{none}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l1_dalt\endcsname{\ensuremath{+0.436}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l1_dalt2\endcsname{\ensuremath{+0.454}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l1_delta\endcsname{\ensuremath{+0.465}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l1_pair\endcsname{\ensuremath{+0.465}\,pp}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l1_pos\endcsname{at or above the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l1_seed1\endcsname{\ensuremath{+0.662}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l1_seed2\endcsname{\ensuremath{+0.268}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l1_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l1_z\endcsname{4.66}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l1b_dalt\endcsname{\ensuremath{+0.269}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l1b_dalt2\endcsname{\ensuremath{+0.287}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l1b_delta\endcsname{\ensuremath{+0.298}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l1b_pair\endcsname{\ensuremath{+0.298}\,pp}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l1b_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l1b_seed1\endcsname{\ensuremath{+0.426}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l1b_seed2\endcsname{\ensuremath{+0.169}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l1b_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l1b_z\endcsname{2.98}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l2_dalt\endcsname{\ensuremath{+0.166}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l2_dalt2\endcsname{\ensuremath{+0.184}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l2_delta\endcsname{\ensuremath{+0.194}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l2_pair\endcsname{\ensuremath{+0.194}\,pp}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l2_pos\endcsname{inside the null edge}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l2_seed1\endcsname{\ensuremath{+0.255}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l2_seed2\endcsname{\ensuremath{+0.134}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l2_word\endcsname{does not separate}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l2_z\endcsname{1.95}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l3_dalt\endcsname{\ensuremath{+0.104}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l3_dalt2\endcsname{\ensuremath{+0.121}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l3_delta\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l3_pair\endcsname{\ensuremath{+0.132}\,pp}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l3_pos\endcsname{inside the null edge}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l3_seed1\endcsname{\ensuremath{+0.280}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l3_seed2\endcsname{\ensuremath{-0.016}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l3_word\endcsname{does not separate}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l3_z\endcsname{1.33}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l4_dalt\endcsname{\ensuremath{+0.426}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l4_dalt2\endcsname{\ensuremath{+0.444}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l4_delta\endcsname{\ensuremath{+0.455}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l4_pair\endcsname{\ensuremath{+0.455}\,pp}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l4_pos\endcsname{at or above the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l4_seed1\endcsname{\ensuremath{+0.352}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l4_seed2\endcsname{\ensuremath{+0.557}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l4_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_amos_l4_z\endcsname{4.56}
\expandafter\gdef\csname R@an.power_design.fr2_amos_largestnot\endcsname{0.194}
\expandafter\gdef\csname R@an.power_design.fr2_amos_largestnot_arm\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.power_design.fr2_amos_largestnot_dalt\endcsname{\ensuremath{+0.166}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_maxarm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.power_design.fr2_amos_maxdalt\endcsname{\ensuremath{+0.436}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_maxdelta\endcsname{\ensuremath{+0.465}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_maxrel\endcsname{1.33}
\expandafter\gdef\csname R@an.power_design.fr2_amos_n\endcsname{5}
\expandafter\gdef\csname R@an.power_design.fr2_amos_nabove\endcsname{2}
\expandafter\gdef\csname R@an.power_design.fr2_amos_nbetween\endcsname{1}
\expandafter\gdef\csname R@an.power_design.fr2_amos_nflip\endcsname{0}
\expandafter\gdef\csname R@an.power_design.fr2_amos_nflip2\endcsname{0}
\expandafter\gdef\csname R@an.power_design.fr2_amos_ninside\endcsname{2}
\expandafter\gdef\csname R@an.power_design.fr2_amos_nnot\endcsname{2}
\expandafter\gdef\csname R@an.power_design.fr2_amos_npool\endcsname{6}
\expandafter\gdef\csname R@an.power_design.fr2_amos_nsep\endcsname{3}
\expandafter\gdef\csname R@an.power_design.fr2_amos_ntsep\endcsname{3}
\expandafter\gdef\csname R@an.power_design.fr2_amos_nu\endcsname{5}
\expandafter\gdef\csname R@an.power_design.fr2_amos_nullsd\endcsname{0.100}
\expandafter\gdef\csname R@an.power_design.fr2_amos_rung\endcsname{0.351}
\expandafter\gdef\csname R@an.power_design.fr2_amos_rungsentence\endcsname{The largest fresh mean, \ensuremath{+0.465}\,pp (ResEnc-M), is 1.33 times the two-seed rung of 0.351\,pp}
\expandafter\gdef\csname R@an.power_design.fr2_amos_rungx\endcsname{1.79}
\expandafter\gdef\csname R@an.power_design.fr2_amos_smallest\endcsname{0.298}
\expandafter\gdef\csname R@an.power_design.fr2_amos_smallest_arm\endcsname{ResEnc-matched}
\expandafter\gdef\csname R@an.power_design.fr2_amos_smallest_dalt\endcsname{\ensuremath{+0.269}}
\expandafter\gdef\csname R@an.power_design.fr2_amos_tcrit\endcsname{2.57}
\expandafter\gdef\csname R@an.power_design.fr2_amos_tedge\endcsname{0.26}
\expandafter\gdef\csname R@an.power_design.fr2_amos_zedge\endcsname{1.96}
\expandafter\gdef\csname R@an.power_design.fr2_def\endcsname{A fresh mean of two fresh seeds (seeds 1 and 2, the discovery seed excluded) separates from the frozen pool when it lies more than 1.96 null SDs from the pool mean, the null SD of a two-seed mean being the pool SD times $\sqrt{1/2+1/n_p}$; the edge is a location on the normal scale and not a test, the $t$ quantile of the pool on its own degrees of freedom is stated beside it wherever the verb is used, and the ladder's rung is the 80\,\%-power size at the same number of seeds}
\expandafter\gdef\csname R@an.power_design.fr2_kits_altclause\endcsname{Against the six-run reference (\ensuremath{+0.244}\,pp from the frozen pool) the same fresh means read ResEnc-M \ensuremath{+3.232}\,pp, LeanDeepMid \ensuremath{+2.418}\,pp, LeanNeXt-s5 \ensuremath{+2.196}\,pp, HyReX+dec. capacity \ensuremath{+2.157}\,pp, LeanSep \ensuremath{+2.138}\,pp, ResEnc-matched \ensuremath{+2.070}\,pp, LeanDeepMid+FD \ensuremath{+2.046}\,pp, LeanAdd \ensuremath{+2.042}\,pp, ResEnc+context \ensuremath{+2.003}\,pp, HyReX-LeanDec \ensuremath{+1.922}\,pp, HyReX \ensuremath{+1.850}\,pp, LeanDec \ensuremath{+1.648}\,pp, StackDec \ensuremath{+1.634}\,pp, LeanDil \ensuremath{+1.595}\,pp, Stem1 \ensuremath{+1.487}\,pp, HyReX-k9 \ensuremath{+1.461}\,pp, HyReX+context \ensuremath{+1.348}\,pp, HyReX point-fuse \ensuremath{+1.233}\,pp, LeanAdd-NeXt \ensuremath{+1.205}\,pp, LeanTrunk \ensuremath{+1.131}\,pp, CoarseStack \ensuremath{+1.005}\,pp, fn.-identical control \ensuremath{+0.932}\,pp, branch control \ensuremath{+0.823}\,pp, HyReX, finer ConvNeXt \ensuremath{+0.326}\,pp and ConvNeXt-k3 \ensuremath{-0.133}\,pp; 3 of 25 change side of the unchanged 1.42\,pp edge}
\expandafter\gdef\csname R@an.power_design.fr2_kits_altname\endcsname{six-run reference}
\expandafter\gdef\csname R@an.power_design.fr2_kits_altshift\endcsname{\ensuremath{+0.244}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_anchor\endcsname{At two fresh seeds, against the frozen 3-run pool (two-seed null SD 0.726\,pp; edge 1.42\,pp on the normal scale, 3.12\,pp on the $t$ scale of the pool's two degrees of freedom), KiTS23 separates ResEnc-M's \ensuremath{+3.475}\,pp (\ensuremath{+3.232}\,pp against the six-run reference) and HyReX's \ensuremath{+2.094}\,pp (\ensuremath{+1.850}\,pp against the six-run reference); the ladder's 80\,\%-power rung at two seeds is 4.1\,pp}
\expandafter\gdef\csname R@an.power_design.fr2_kits_bracket\endcsname{At two fresh seeds KiTS23 separates fresh means beyond the 1.42\,pp edge of its two-seed null (1.96 null SDs of 0.726\,pp): the smallest it separates among the arms with a finished pair is 1.448\,pp (LeanAdd-NeXt; \ensuremath{+1.205}\,pp against the six-run reference) and the largest it does not separate is 1.375\,pp (LeanTrunk; \ensuremath{+1.131}\,pp against the six-run reference); the ladder's rung at two seeds is 4.1\,pp}
\expandafter\gdef\csname R@an.power_design.fr2_kits_c1_dalt\endcsname{\ensuremath{+2.157}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_c1_delta\endcsname{\ensuremath{+2.401}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_c1_pair\endcsname{\ensuremath{+2.401}\,pp (\ensuremath{+2.157}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_c1_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_kits_c1_seed1\endcsname{\ensuremath{+2.128}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_c1_seed2\endcsname{\ensuremath{+2.674}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_c1_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_kits_c1_z\endcsname{3.31}
\expandafter\gdef\csname R@an.power_design.fr2_kits_clause\endcsname{At two fresh seeds, against the frozen 3-run pool (two-seed null SD 0.726\,pp; edge 1.42\,pp on the normal scale, 3.12\,pp on the $t$ scale of the pool's two degrees of freedom), KiTS23 separates ResEnc-M's \ensuremath{+3.475}\,pp (\ensuremath{+3.232}\,pp against the six-run reference), LeanDeepMid's \ensuremath{+2.662}\,pp (\ensuremath{+2.418}\,pp against the six-run reference), LeanNeXt-s5's \ensuremath{+2.440}\,pp (\ensuremath{+2.196}\,pp against the six-run reference), HyReX+dec. capacity's \ensuremath{+2.401}\,pp (\ensuremath{+2.157}\,pp against the six-run reference), LeanSep's \ensuremath{+2.382}\,pp (\ensuremath{+2.138}\,pp against the six-run reference), ResEnc-matched's \ensuremath{+2.313}\,pp (\ensuremath{+2.070}\,pp against the six-run reference), LeanDeepMid+FD's \ensuremath{+2.289}\,pp (\ensuremath{+2.046}\,pp against the six-run reference), LeanAdd's \ensuremath{+2.285}\,pp (\ensuremath{+2.042}\,pp against the six-run reference), ResEnc+context's \ensuremath{+2.246}\,pp (\ensuremath{+2.003}\,pp against the six-run reference), HyReX-LeanDec's \ensuremath{+2.165}\,pp (\ensuremath{+1.922}\,pp against the six-run reference), HyReX's \ensuremath{+2.094}\,pp (\ensuremath{+1.850}\,pp against the six-run reference), LeanDec's \ensuremath{+1.892}\,pp (\ensuremath{+1.648}\,pp against the six-run reference), StackDec's \ensuremath{+1.877}\,pp (\ensuremath{+1.634}\,pp against the six-run reference), LeanDil's \ensuremath{+1.838}\,pp (\ensuremath{+1.595}\,pp against the six-run reference), Stem1's \ensuremath{+1.731}\,pp (\ensuremath{+1.487}\,pp against the six-run reference), HyReX-k9's \ensuremath{+1.704}\,pp (\ensuremath{+1.461}\,pp against the six-run reference), HyReX+context's \ensuremath{+1.591}\,pp (\ensuremath{+1.348}\,pp against the six-run reference), HyReX point-fuse's \ensuremath{+1.477}\,pp (\ensuremath{+1.233}\,pp against the six-run reference) and LeanAdd-NeXt's \ensuremath{+1.448}\,pp (\ensuremath{+1.205}\,pp against the six-run reference); it does not separate LeanTrunk's \ensuremath{+1.375}\,pp (\ensuremath{+1.131}\,pp against the six-run reference), CoarseStack's \ensuremath{+1.249}\,pp (\ensuremath{+1.005}\,pp against the six-run reference), fn.-identical control's \ensuremath{+1.176}\,pp (\ensuremath{+0.932}\,pp against the six-run reference), branch control's \ensuremath{+1.067}\,pp (\ensuremath{+0.823}\,pp against the six-run reference), HyReX, finer ConvNeXt's \ensuremath{+0.570}\,pp (\ensuremath{+0.326}\,pp against the six-run reference) and ConvNeXt-k3's \ensuremath{+0.110}\,pp (\ensuremath{-0.133}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_d1_dalt\endcsname{\ensuremath{+1.233}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_d1_delta\endcsname{\ensuremath{+1.477}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_d1_pair\endcsname{\ensuremath{+1.477}\,pp (\ensuremath{+1.233}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_d1_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_kits_d1_seed1\endcsname{\ensuremath{+1.759}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_d1_seed2\endcsname{\ensuremath{+1.194}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_d1_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_kits_d1_z\endcsname{2.03}
\expandafter\gdef\csname R@an.power_design.fr2_kits_d2_dalt\endcsname{\ensuremath{+1.648}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_d2_delta\endcsname{\ensuremath{+1.892}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_d2_pair\endcsname{\ensuremath{+1.892}\,pp (\ensuremath{+1.648}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_d2_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_kits_d2_seed1\endcsname{\ensuremath{+1.979}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_d2_seed2\endcsname{\ensuremath{+1.804}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_d2_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_kits_d2_z\endcsname{2.61}
\expandafter\gdef\csname R@an.power_design.fr2_kits_diff_l3_l1\endcsname{1.382}
\expandafter\gdef\csname R@an.power_design.fr2_kits_diff_sentence\endcsname{The fresh means of HyReX and ResEnc-M differ by 1.382\,pp, a magnitude with no direction}
\expandafter\gdef\csname R@an.power_design.fr2_kits_edge\endcsname{1.42}
\expandafter\gdef\csname R@an.power_design.fr2_kits_flipnames\endcsname{HyReX+context, HyReX point-fuse and LeanAdd-NeXt}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l1_dalt\endcsname{\ensuremath{+3.232}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l1_delta\endcsname{\ensuremath{+3.475}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l1_pair\endcsname{\ensuremath{+3.475}\,pp (\ensuremath{+3.232}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l1_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l1_seed1\endcsname{\ensuremath{+3.134}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l1_seed2\endcsname{\ensuremath{+3.817}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l1_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l1_z\endcsname{4.79}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l1b_dalt\endcsname{\ensuremath{+2.070}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l1b_delta\endcsname{\ensuremath{+2.313}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l1b_pair\endcsname{\ensuremath{+2.313}\,pp (\ensuremath{+2.070}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l1b_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l1b_seed1\endcsname{\ensuremath{+2.564}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l1b_seed2\endcsname{\ensuremath{+2.062}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l1b_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l1b_z\endcsname{3.19}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l2_dalt\endcsname{\ensuremath{-0.133}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l2_delta\endcsname{\ensuremath{+0.110}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l2_pair\endcsname{\ensuremath{+0.110}\,pp (\ensuremath{-0.133}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l2_pos\endcsname{inside the null edge}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l2_seed1\endcsname{\ensuremath{-0.805}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l2_seed2\endcsname{\ensuremath{+1.026}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l2_word\endcsname{does not separate}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l2_z\endcsname{0.15}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l3_dalt\endcsname{\ensuremath{+1.850}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l3_delta\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l3_pair\endcsname{\ensuremath{+2.094}\,pp (\ensuremath{+1.850}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l3_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l3_seed1\endcsname{\ensuremath{+1.798}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l3_seed2\endcsname{\ensuremath{+2.390}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l3_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l3_z\endcsname{2.89}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l4_dalt\endcsname{\ensuremath{+2.003}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l4_delta\endcsname{\ensuremath{+2.246}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l4_pair\endcsname{\ensuremath{+2.246}\,pp (\ensuremath{+2.003}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l4_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l4_seed1\endcsname{\ensuremath{+2.677}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l4_seed2\endcsname{\ensuremath{+1.815}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l4_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l4_z\endcsname{3.10}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l6_dalt\endcsname{\ensuremath{+1.348}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l6_delta\endcsname{\ensuremath{+1.591}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l6_pair\endcsname{\ensuremath{+1.591}\,pp (\ensuremath{+1.348}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l6_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l6_seed1\endcsname{\ensuremath{+1.198}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l6_seed2\endcsname{\ensuremath{+1.984}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l6_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_kits_l6_z\endcsname{2.19}
\expandafter\gdef\csname R@an.power_design.fr2_kits_largestnot\endcsname{1.375}
\expandafter\gdef\csname R@an.power_design.fr2_kits_largestnot_arm\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.power_design.fr2_kits_largestnot_dalt\endcsname{\ensuremath{+1.131}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_maxarm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.power_design.fr2_kits_maxdalt\endcsname{\ensuremath{+3.232}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_maxdelta\endcsname{\ensuremath{+3.475}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_maxrel\endcsname{0.85}
\expandafter\gdef\csname R@an.power_design.fr2_kits_n\endcsname{25}
\expandafter\gdef\csname R@an.power_design.fr2_kits_nabove\endcsname{0}
\expandafter\gdef\csname R@an.power_design.fr2_kits_nbetween\endcsname{19}
\expandafter\gdef\csname R@an.power_design.fr2_kits_nflip\endcsname{3}
\expandafter\gdef\csname R@an.power_design.fr2_kits_ninside\endcsname{6}
\expandafter\gdef\csname R@an.power_design.fr2_kits_nnot\endcsname{6}
\expandafter\gdef\csname R@an.power_design.fr2_kits_npool\endcsname{3}
\expandafter\gdef\csname R@an.power_design.fr2_kits_nsep\endcsname{19}
\expandafter\gdef\csname R@an.power_design.fr2_kits_ntsep\endcsname{1}
\expandafter\gdef\csname R@an.power_design.fr2_kits_nu\endcsname{2}
\expandafter\gdef\csname R@an.power_design.fr2_kits_nullsd\endcsname{0.726}
\expandafter\gdef\csname R@an.power_design.fr2_kits_p3c_dalt\endcsname{\ensuremath{+0.932}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_p3c_delta\endcsname{\ensuremath{+1.176}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_p3c_pair\endcsname{\ensuremath{+1.176}\,pp (\ensuremath{+0.932}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_p3c_pos\endcsname{inside the null edge}
\expandafter\gdef\csname R@an.power_design.fr2_kits_p3c_seed1\endcsname{\ensuremath{+1.151}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_p3c_seed2\endcsname{\ensuremath{+1.201}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_p3c_word\endcsname{does not separate}
\expandafter\gdef\csname R@an.power_design.fr2_kits_p3c_z\endcsname{1.62}
\expandafter\gdef\csname R@an.power_design.fr2_kits_rung\endcsname{4.1}
\expandafter\gdef\csname R@an.power_design.fr2_kits_rungsentence\endcsname{The two-seed rung, 4.1\,pp, lies above the largest fresh mean, \ensuremath{+3.475}\,pp (ResEnc-M; \ensuremath{+3.232}\,pp against the six-run reference), which is 0.85 of it}
\expandafter\gdef\csname R@an.power_design.fr2_kits_rungx\endcsname{2.88}
\expandafter\gdef\csname R@an.power_design.fr2_kits_s2_dalt\endcsname{\ensuremath{+0.326}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_s2_delta\endcsname{\ensuremath{+0.570}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_s2_pair\endcsname{\ensuremath{+0.570}\,pp (\ensuremath{+0.326}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_s2_pos\endcsname{inside the null edge}
\expandafter\gdef\csname R@an.power_design.fr2_kits_s2_seed1\endcsname{\ensuremath{+0.782}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_s2_seed2\endcsname{\ensuremath{+0.358}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_s2_word\endcsname{does not separate}
\expandafter\gdef\csname R@an.power_design.fr2_kits_s2_z\endcsname{0.79}
\expandafter\gdef\csname R@an.power_design.fr2_kits_smallest\endcsname{1.448}
\expandafter\gdef\csname R@an.power_design.fr2_kits_smallest_arm\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.power_design.fr2_kits_smallest_dalt\endcsname{\ensuremath{+1.205}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_tcrit\endcsname{4.30}
\expandafter\gdef\csname R@an.power_design.fr2_kits_tedge\endcsname{3.12}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5a5_dalt\endcsname{\ensuremath{+1.922}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5a5_delta\endcsname{\ensuremath{+2.165}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5a5_pair\endcsname{\ensuremath{+2.165}\,pp (\ensuremath{+1.922}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5a5_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5a5_seed1\endcsname{\ensuremath{+2.348}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5a5_seed2\endcsname{\ensuremath{+1.983}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5a5_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5a5_z\endcsname{2.98}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5b1_dalt\endcsname{\ensuremath{+2.042}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5b1_delta\endcsname{\ensuremath{+2.285}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5b1_pair\endcsname{\ensuremath{+2.285}\,pp (\ensuremath{+2.042}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5b1_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5b1_seed1\endcsname{\ensuremath{+2.242}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5b1_seed2\endcsname{\ensuremath{+2.328}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5b1_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5b1_z\endcsname{3.15}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5b2_dalt\endcsname{\ensuremath{+1.205}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5b2_delta\endcsname{\ensuremath{+1.448}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5b2_pair\endcsname{\ensuremath{+1.448}\,pp (\ensuremath{+1.205}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5b2_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5b2_seed1\endcsname{\ensuremath{+1.498}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5b2_seed2\endcsname{\ensuremath{+1.399}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5b2_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v5b2_z\endcsname{2.00}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v6a1r_dalt\endcsname{\ensuremath{+1.461}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v6a1r_delta\endcsname{\ensuremath{+1.704}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v6a1r_pair\endcsname{\ensuremath{+1.704}\,pp (\ensuremath{+1.461}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v6a1r_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v6a1r_seed1\endcsname{\ensuremath{+1.695}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v6a1r_seed2\endcsname{\ensuremath{+1.713}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v6a1r_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v6a1r_z\endcsname{2.35}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7a1_dalt\endcsname{\ensuremath{+2.418}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7a1_delta\endcsname{\ensuremath{+2.662}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7a1_pair\endcsname{\ensuremath{+2.662}\,pp (\ensuremath{+2.418}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7a1_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7a1_seed1\endcsname{\ensuremath{+2.326}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7a1_seed2\endcsname{\ensuremath{+2.997}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7a1_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7a1_z\endcsname{3.67}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7a2_dalt\endcsname{\ensuremath{+2.046}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7a2_delta\endcsname{\ensuremath{+2.289}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7a2_pair\endcsname{\ensuremath{+2.289}\,pp (\ensuremath{+2.046}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7a2_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7a2_seed1\endcsname{\ensuremath{+1.973}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7a2_seed2\endcsname{\ensuremath{+2.606}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7a2_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7a2_z\endcsname{3.15}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7b1_dalt\endcsname{\ensuremath{+2.138}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7b1_delta\endcsname{\ensuremath{+2.382}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7b1_pair\endcsname{\ensuremath{+2.382}\,pp (\ensuremath{+2.138}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7b1_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7b1_seed1\endcsname{\ensuremath{+2.053}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7b1_seed2\endcsname{\ensuremath{+2.710}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7b1_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7b1_z\endcsname{3.28}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7b2_dalt\endcsname{\ensuremath{+1.595}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7b2_delta\endcsname{\ensuremath{+1.838}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7b2_pair\endcsname{\ensuremath{+1.838}\,pp (\ensuremath{+1.595}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7b2_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7b2_seed1\endcsname{\ensuremath{+2.395}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7b2_seed2\endcsname{\ensuremath{+1.282}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7b2_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7b2_z\endcsname{2.53}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7c1_dalt\endcsname{\ensuremath{+2.196}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7c1_delta\endcsname{\ensuremath{+2.440}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7c1_pair\endcsname{\ensuremath{+2.440}\,pp (\ensuremath{+2.196}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7c1_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7c1_seed1\endcsname{\ensuremath{+2.758}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7c1_seed2\endcsname{\ensuremath{+2.121}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7c1_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v7c1_z\endcsname{3.36}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8a1_dalt\endcsname{\ensuremath{+1.005}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8a1_delta\endcsname{\ensuremath{+1.249}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8a1_pair\endcsname{\ensuremath{+1.249}\,pp (\ensuremath{+1.005}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8a1_pos\endcsname{inside the null edge}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8a1_seed1\endcsname{\ensuremath{+1.077}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8a1_seed2\endcsname{\ensuremath{+1.421}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8a1_word\endcsname{does not separate}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8a1_z\endcsname{1.72}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8a2_dalt\endcsname{\ensuremath{+1.634}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8a2_delta\endcsname{\ensuremath{+1.877}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8a2_pair\endcsname{\ensuremath{+1.877}\,pp (\ensuremath{+1.634}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8a2_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8a2_seed1\endcsname{\ensuremath{+1.593}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8a2_seed2\endcsname{\ensuremath{+2.162}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8a2_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8a2_z\endcsname{2.59}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8b1_dalt\endcsname{\ensuremath{+1.131}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8b1_delta\endcsname{\ensuremath{+1.375}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8b1_pair\endcsname{\ensuremath{+1.375}\,pp (\ensuremath{+1.131}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8b1_pos\endcsname{inside the null edge}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8b1_seed1\endcsname{\ensuremath{+2.079}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8b1_seed2\endcsname{\ensuremath{+0.670}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8b1_word\endcsname{does not separate}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8b1_z\endcsname{1.89}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8b2_dalt\endcsname{\ensuremath{+1.487}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8b2_delta\endcsname{\ensuremath{+1.731}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8b2_pair\endcsname{\ensuremath{+1.731}\,pp (\ensuremath{+1.487}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8b2_pos\endcsname{between the null edge and the two-seed rung}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8b2_seed1\endcsname{\ensuremath{+1.892}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8b2_seed2\endcsname{\ensuremath{+1.570}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8b2_word\endcsname{separates}
\expandafter\gdef\csname R@an.power_design.fr2_kits_v8b2_z\endcsname{2.39}
\expandafter\gdef\csname R@an.power_design.fr2_kits_w1c_dalt\endcsname{\ensuremath{+0.823}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_w1c_delta\endcsname{\ensuremath{+1.067}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_w1c_pair\endcsname{\ensuremath{+1.067}\,pp (\ensuremath{+0.823}\,pp against the six-run reference)}
\expandafter\gdef\csname R@an.power_design.fr2_kits_w1c_pos\endcsname{inside the null edge}
\expandafter\gdef\csname R@an.power_design.fr2_kits_w1c_seed1\endcsname{\ensuremath{+1.734}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_w1c_seed2\endcsname{\ensuremath{+0.399}}
\expandafter\gdef\csname R@an.power_design.fr2_kits_w1c_word\endcsname{does not separate}
\expandafter\gdef\csname R@an.power_design.fr2_kits_w1c_z\endcsname{1.47}
\expandafter\gdef\csname R@an.power_design.fr2_kits_zedge\endcsname{1.96}
\expandafter\gdef\csname R@an.power_design.fr2_nseeds\endcsname{2}
\expandafter\gdef\csname R@an.power_design.fr2_power\endcsname{80}
\expandafter\gdef\csname R@an.power_design.fr2_seedlist\endcsname{1 and 2}
\expandafter\gdef\csname R@an.power_design.fr2_zedge\endcsname{1.96}
\expandafter\gdef\csname R@an.power_design.gate_cvres_acdc\endcsname{open}
\expandafter\gdef\csname R@an.power_design.gate_cvres_amos\endcsname{open}
\expandafter\gdef\csname R@an.power_design.gate_cvres_kits\endcsname{open}
\expandafter\gdef\csname R@an.power_design.gate_fr2_acdc\endcsname{open}
\expandafter\gdef\csname R@an.power_design.gate_fr2_amos\endcsname{open}
\expandafter\gdef\csname R@an.power_design.gate_fr2_kits\endcsname{open}
\expandafter\gdef\csname R@an.power_design.guardbar\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.power_design.h7_agent_below\endcsname{31}
\expandafter\gdef\csname R@an.power_design.h7_agent_clause\endcsname{more than the screening-seed gain of any agent-designed arm (the largest, HyReX-k9, reads \ensuremath{+0.487}\,pp, and the largest candidate arm, ResEnc+context, \ensuremath{+0.430}\,pp)}
\expandafter\gdef\csname R@an.power_design.h7_agent_gains\endcsname{The AMOS22 implementation gap, 0.509\,pp, is larger than the AMOS22 gain of every one of the 31 agent-designed arms with a finished run (candidates, width-scaled variants, attribution arms and HyReX's children); the largest is 0.487\,pp (HyReX-k9)}
\expandafter\gdef\csname R@an.power_design.h7_agent_max\endcsname{\ensuremath{+0.430}}
\expandafter\gdef\csname R@an.power_design.h7_agent_max_arm\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.power_design.h7_agent_n\endcsname{7}
\expandafter\gdef\csname R@an.power_design.h7_agent_nabove\endcsname{0}
\expandafter\gdef\csname R@an.power_design.h7_agent_names_above\endcsname{none}
\expandafter\gdef\csname R@an.power_design.h7_design_max\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.power_design.h7_design_max_arm\endcsname{HyReX-k9}
\expandafter\gdef\csname R@an.power_design.h7_design_n\endcsname{31}
\expandafter\gdef\csname R@an.power_design.h7_iso_max\endcsname{0.923}
\expandafter\gdef\csname R@an.power_design.h7_iso_max_name\endcsname{default+GN16 $-$ default}
\expandafter\gdef\csname R@an.power_design.h7_iso_n\endcsname{14}
\expandafter\gdef\csname R@an.power_design.h7_iso_nabove\endcsname{1}
\expandafter\gdef\csname R@an.power_design.h7_iso_names_above\endcsname{default+GN16 $-$ default}
\expandafter\gdef\csname R@an.power_design.h7_iso_nreg\endcsname{16}
\expandafter\gdef\csname R@an.power_design.kits6_mde_dir\endcsname{falls}
\expandafter\gdef\csname R@an.power_design.kits6_mean\endcsname{83.622}
\expandafter\gdef\csname R@an.power_design.kits6_n\endcsname{6}
\expandafter\gdef\csname R@an.power_design.kits6_sd\endcsname{0.722}
\expandafter\gdef\csname R@an.power_design.kits6_shift\endcsname{\ensuremath{+0.244}}
\expandafter\gdef\csname R@an.power_design.kits_cls_indep\endcsname{2.33}
\expandafter\gdef\csname R@an.power_design.kits_cls_max_name\endcsname{masses}
\expandafter\gdef\csname R@an.power_design.kits_cls_max_sd\endcsname{1.08}
\expandafter\gdef\csname R@an.power_design.kits_cls_min_name\endcsname{kidney}
\expandafter\gdef\csname R@an.power_design.kits_cls_min_sd\endcsname{0.39}
\expandafter\gdef\csname R@an.power_design.kits_l1b_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.kits_l1b_sd\endcsname{0.414}
\expandafter\gdef\csname R@an.power_design.kits_l1b_sdratio_hi\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.kits_l1b_vratio\endcsname{0.27}
\expandafter\gdef\csname R@an.power_design.kits_l1b_vratio_hi\endcsname{39}
\expandafter\gdef\csname R@an.power_design.kits_l1b_vratio_lo\endcsname{0.026}
\expandafter\gdef\csname R@an.power_design.kits_mean\endcsname{83.378}
\expandafter\gdef\csname R@an.power_design.kits_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.kits_nseed\endcsname{3}
\expandafter\gdef\csname R@an.power_design.kits_pub_offset\endcsname{\ensuremath{-2.87}}
\expandafter\gdef\csname R@an.power_design.kits_sd\endcsname{0.795}
\expandafter\gdef\csname R@an.power_design.kits_sd_fhi\endcsname{6.28}
\expandafter\gdef\csname R@an.power_design.kits_sd_flo\endcsname{0.52}
\expandafter\gdef\csname R@an.power_design.kits_sd_hi\endcsname{5.00}
\expandafter\gdef\csname R@an.power_design.kits_sd_lo\endcsname{0.41}
\expandafter\gdef\csname R@an.power_design.kits_sd_pooled2\endcsname{0.634}
\expandafter\gdef\csname R@an.power_design.kits_sd_pooled2_hi\endcsname{1.82}
\expandafter\gdef\csname R@an.power_design.kits_sd_pooled2_lo\endcsname{0.38}
\expandafter\gdef\csname R@an.power_design.m_study\endcsname{13}
\expandafter\gdef\csname R@an.power_design.mde_acdc_floor\endcsname{0.14}
\expandafter\gdef\csname R@an.power_design.mde_acdc_n1\endcsname{0.38}
\expandafter\gdef\csname R@an.power_design.mde_acdc_n1_sdhi\endcsname{0.92}
\expandafter\gdef\csname R@an.power_design.mde_acdc_n1_sdlo\endcsname{0.23}
\expandafter\gdef\csname R@an.power_design.mde_acdc_n2\endcsname{0.28}
\expandafter\gdef\csname R@an.power_design.mde_acdc_n2_sdhi\endcsname{0.70}
\expandafter\gdef\csname R@an.power_design.mde_acdc_n2_sdlo\endcsname{0.18}
\expandafter\gdef\csname R@an.power_design.mde_acdc_n3\endcsname{0.25}
\expandafter\gdef\csname R@an.power_design.mde_acdc_n4\endcsname{0.22}
\expandafter\gdef\csname R@an.power_design.mde_acdc_n5\endcsname{0.21}
\expandafter\gdef\csname R@an.power_design.mde_acdc_n6\endcsname{0.20}
\expandafter\gdef\csname R@an.power_design.mde_acdc_n7\endcsname{0.19}
\expandafter\gdef\csname R@an.power_design.mde_acdc_n8\endcsname{0.19}
\expandafter\gdef\csname R@an.power_design.mde_acdc_pair_n1\endcsname{0.49}
\expandafter\gdef\csname R@an.power_design.mde_acdc_pair_n2\endcsname{0.35}
\expandafter\gdef\csname R@an.power_design.mde_acdc_pair_n3\endcsname{0.284}
\expandafter\gdef\csname R@an.power_design.mde_acdc_pair_n4\endcsname{0.25}
\expandafter\gdef\csname R@an.power_design.mde_acdc_pair_n5\endcsname{0.22}
\expandafter\gdef\csname R@an.power_design.mde_acdc_pair_n6\endcsname{0.20}
\expandafter\gdef\csname R@an.power_design.mde_acdc_pair_n7\endcsname{0.19}
\expandafter\gdef\csname R@an.power_design.mde_acdc_pair_n8\endcsname{0.17}
\expandafter\gdef\csname R@an.power_design.mde_amos_floor\endcsname{0.18}
\expandafter\gdef\csname R@an.power_design.mde_amos_n1\endcsname{0.46}
\expandafter\gdef\csname R@an.power_design.mde_amos_n1_sdhi\endcsname{1.14}
\expandafter\gdef\csname R@an.power_design.mde_amos_n1_sdlo\endcsname{0.29}
\expandafter\gdef\csname R@an.power_design.mde_amos_n2\endcsname{0.351}
\expandafter\gdef\csname R@an.power_design.mde_amos_n3\endcsname{0.30}
\expandafter\gdef\csname R@an.power_design.mde_amos_n6\endcsname{0.25}
\expandafter\gdef\csname R@an.power_design.mde_amos_pair_n1\endcsname{0.61}
\expandafter\gdef\csname R@an.power_design.mde_cross_acdc\endcsname{6}
\expandafter\gdef\csname R@an.power_design.mde_cross_amos\endcsname{6}
\expandafter\gdef\csname R@an.power_design.mde_cross_kits\endcsname{3}
\expandafter\gdef\csname R@an.power_design.mde_kits_floor\endcsname{2.6}
\expandafter\gdef\csname R@an.power_design.mde_kits_n1\endcsname{5.2}
\expandafter\gdef\csname R@an.power_design.mde_kits_n1_pool6ct\endcsname{2.7}
\expandafter\gdef\csname R@an.power_design.mde_kits_n1_sdhi\endcsname{32.6}
\expandafter\gdef\csname R@an.power_design.mde_kits_n1_sdlo\endcsname{2.7}
\expandafter\gdef\csname R@an.power_design.mde_kits_n2\endcsname{4.1}
\expandafter\gdef\csname R@an.power_design.mde_kits_n3\endcsname{3.7}
\expandafter\gdef\csname R@an.power_design.mde_kits_n3_pool6\endcsname{2.0}
\expandafter\gdef\csname R@an.power_design.mde_kits_n3_pool6ct\endcsname{1.8}
\expandafter\gdef\csname R@an.power_design.mde_kits_n6\endcsname{3.2}
\expandafter\gdef\csname R@an.power_design.mde_kits_n6_pool6ct\endcsname{1.5}
\expandafter\gdef\csname R@an.power_design.mde_kits_pair_n1\endcsname{6.4}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_casesd\endcsname{0.98}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_casesd_hi\endcsname{1.05}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_casesd_lo\endcsname{0.89}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_casese\endcsname{0.154}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_casese_ub\endcsname{0.171}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_dominant\endcsname{validation cases}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_domshare\endcsname{68}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_floor\endcsname{0.56}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_floor_hi\endcsname{0.60}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_floor_lo\endcsname{0.51}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_floor_range\endcsname{0.51 to 0.60}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_floor_ub\endcsname{0.618}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_n1\endcsname{0.66}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_n1_hi\endcsname{0.70}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_n1_lo\endcsname{0.620}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_n1_ub\endcsname{0.71}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_n2\endcsname{0.61}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_n2_ub\endcsname{0.67}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_n3\endcsname{0.59}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_n3_ub\endcsname{0.65}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_n6\endcsname{0.58}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_n6_ub\endcsname{0.63}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_narms\endcsname{12}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_nval\endcsname{40}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_seedse1\endcsname{0.107}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_sentence\endcsname{Counting the sampling of the 40 validation cases as well as the training seeds (architecture-by-case SD 0.98 pp, standard error 0.154 pp), one seed resolves 0.66 pp on ACDC instead of 0.38 pp and no number of design seeds goes below 0.56 pp instead of 0.14 pp (0.51 to 0.60 pp with the architecture-by-case variance one across-arm standard error either way); the validation cases supply the larger share (68\,\%) of the one-seed variance}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_share_n1\endcsname{68}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_sig2_max\endcsname{\ensuremath{+1.82}}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_sig2_min\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_sig2_se\endcsname{0.160}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_wider_floor\endcsname{295}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_wider_n1\endcsname{76}
\expandafter\gdef\csname R@an.power_design.mde_total_acdc_wider_n1_ub\endcsname{89}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_casesd\endcsname{0.48}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_casesd_hi\endcsname{0.58}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_casesd_lo\endcsname{0.36}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_casese\endcsname{0.076}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_casese_ub\endcsname{0.140}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_dominant\endcsname{training seeds}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_domshare\endcsname{75}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_floor\endcsname{0.32}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_floor_hi\endcsname{0.37}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_floor_lo\endcsname{0.27}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_floor_range\endcsname{0.27 to 0.37}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_floor_ub\endcsname{0.52}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_n1\endcsname{0.54}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_n1_hi\endcsname{0.56}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_n1_lo\endcsname{0.51}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_n1_ub\endcsname{0.67}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_n2\endcsname{0.44}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_n2_ub\endcsname{0.60}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_n3\endcsname{0.41}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_n3_ub\endcsname{0.58}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_n6\endcsname{0.37}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_n6_ub\endcsname{0.55}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_narms\endcsname{13}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_nval\endcsname{40}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_seedse1\endcsname{0.132}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_sentence\endcsname{Counting the sampling of the 40 validation cases as well as the training seeds (architecture-by-case SD 0.48 pp, standard error 0.076 pp), one seed resolves 0.54 pp on AMOS22 instead of 0.46 pp and no number of design seeds goes below 0.32 pp instead of 0.18 pp (0.27 to 0.37 pp with the architecture-by-case variance one across-arm standard error either way); the training seeds supply the larger share (75\,\%) of the one-seed variance}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_share_n1\endcsname{25}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_sig2_max\endcsname{\ensuremath{+0.94}}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_sig2_min\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_sig2_se\endcsname{0.103}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_wider_floor\endcsname{83}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_wider_n1\endcsname{16}
\expandafter\gdef\csname R@an.power_design.mde_total_amos_wider_n1_ub\endcsname{46}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_casesd\endcsname{0.62}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_casesd_hi\endcsname{0.70}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_casesd_lo\endcsname{0.53}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_casese\endcsname{0.099}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_casese_ub\endcsname{0.145}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_dominant\endcsname{training seeds}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_domshare\endcsname{74}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_floor\endcsname{0.73}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_floor_hi\endcsname{0.78}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_floor_lo\endcsname{0.67}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_floor_range\endcsname{0.67 to 0.78}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_floor_ub\endcsname{0.95}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_n1\endcsname{1.09}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_n1_hi\endcsname{1.13}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_n1_lo\endcsname{1.05}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_n1_ub\endcsname{1.25}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_n2\endcsname{0.93}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_n2_ub\endcsname{1.11}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_n3\endcsname{0.87}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_n3_ub\endcsname{1.06}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_n6\endcsname{0.80}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_n6_ub\endcsname{1.00}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_narms\endcsname{13}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_nval\endcsname{40}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_seedse1\endcsname{0.166}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_sentence\endcsname{Counting the sampling of the 40 validation cases as well as the training seeds (architecture-by-case SD 0.62 pp, standard error 0.099 pp), one seed resolves 1.09 pp on AMOS22 against the like-for-like uncompiled sub-pool instead of 0.94 pp and no number of design seeds goes below 0.73 pp instead of 0.47 pp (0.67 to 0.78 pp with the architecture-by-case variance one across-arm standard error either way); the training seeds supply the larger share (74\,\%) of the one-seed variance}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_share_n1\endcsname{26}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_sig2_max\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_sig2_min\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_sig2_se\endcsname{0.107}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_wider_floor\endcsname{55}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_wider_n1\endcsname{16}
\expandafter\gdef\csname R@an.power_design.mde_total_amosu_wider_n1_ub\endcsname{33}
\expandafter\gdef\csname R@an.power_design.mde_total_def\endcsname{The total-variance scale adds the variance from sampling the validation cases to the training-seed variance of the ladder: a design arm of $n$ seeds against a pool of $n_p$ runs with seed SD $s$ has the standard error $\sqrt{s^2(1/n+1/n_p)+\sigma_c^2/N}$, where $\sigma_c$ is the standard deviation across the $N$ validation cases of the architecture-by-case difference between a design and the default network, with the case-level seed noise removed, and its minimum detectable effect is the same noncentral-$t$ multiple of that standard error as on the seed scale}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_casesd\endcsname{4.58}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_casesd_hi\endcsname{5.37}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_casesd_lo\endcsname{3.61}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_casese\endcsname{0.462}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_casese_ub\endcsname{0.778}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_dominant\endcsname{training seeds}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_domshare\endcsname{80}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_floor\endcsname{3.7}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_floor_hi\endcsname{4.0}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_floor_lo\endcsname{3.3}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_floor_range\endcsname{3.3 to 4.0}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_floor_ub\endcsname{5.1}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_n1\endcsname{5.8}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_n1_hi\endcsname{6.0}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_n1_lo\endcsname{5.6}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_n1_ub\endcsname{6.8}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_n2\endcsname{4.9}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_n2_ub\endcsname{6.0}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_n3\endcsname{4.5}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_n3_ub\endcsname{5.7}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_n6\endcsname{4.1}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_n6_ub\endcsname{5.4}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_narms\endcsname{7}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_nval\endcsname{98}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_seedse1\endcsname{0.918}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_sentence\endcsname{Counting the sampling of the 98 validation cases as well as the training seeds (architecture-by-case SD 4.58 pp, standard error 0.462 pp), one seed resolves 5.8 pp on KiTS23 instead of 5.2 pp and no number of design seeds goes below 3.7 pp instead of 2.6 pp (3.3 to 4.0 pp with the architecture-by-case variance one across-arm standard error either way); the training seeds supply the larger share (80\,\%) of the one-seed variance}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_share_n1\endcsname{20}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_sig2_max\endcsname{\ensuremath{+45.54}}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_sig2_min\endcsname{\ensuremath{-14.30}}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_sig2_se\endcsname{7.882}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_wider_floor\endcsname{42}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_wider_n1\endcsname{12}
\expandafter\gdef\csname R@an.power_design.mde_total_kits_wider_n1_ub\endcsname{31}
\expandafter\gdef\csname R@an.power_design.mde_total_scatter_def\endcsname{The range moves the architecture-by-case variance one across-arm standard error either way; the arms differ in their own architecture-by-case variance, so the range describes the scatter among the arms run and is not a confidence interval}
\expandafter\gdef\csname R@an.power_design.mde_total_sent_finding\endcsname{Sampling the validation cases lifts the one-seed rung by 16, 12 and 76\,\% on AMOS22, KiTS23 and ACDC, and the floor that no number of design seeds lowers by 83, 42 and 295\,\%}
\expandafter\gdef\csname R@an.power_design.mde_total_sent_floor\endcsname{The case term does not shrink with seeds: the floor at any number of design seeds rises from 0.18 to 0.32\,pp on AMOS22 (0.27 to 0.37\,pp one across-arm standard error either way), from 2.6 to 3.7\,pp on KiTS23 (3.3 to 4.0\,pp) and from 0.14 to 0.56\,pp on ACDC (0.51 to 0.60\,pp)}
\expandafter\gdef\csname R@an.power_design.mde_total_sent_onseed\endcsname{Counting the sampling of the validation cases as well as the training seeds, one seed resolves 0.54 to 1.09\,pp on AMOS22 (0.46 to 0.94\,pp at a fixed validation fold) and 5.8\,pp on KiTS23 (5.2\,pp)}
\expandafter\gdef\csname R@an.power_design.mde_total_sent_wider\endcsname{Sampling the validation cases widens the one-seed rung by 16\,\% on AMOS22, 12\,\% on KiTS23 and 76\,\% on ACDC; counting the case-level seed noise a second time gives the upper bounds of 46, 31 and 89\,\%}
\expandafter\gdef\csname R@an.power_design.mde_total_ub_clause\endcsname{the upper bound keeps the case-level seed noise inside the case term, so it counts that noise a second time and is the larger of the two}
\expandafter\gdef\csname R@an.power_design.mde_total_ub_def\endcsname{The upper bound keeps the case-level seed noise inside the case term, so it counts that noise a second time and is the larger of the two}
\expandafter\gdef\csname R@an.power_design.mdec5_acdc_floor\endcsname{0.20}
\expandafter\gdef\csname R@an.power_design.mdec5_acdc_n1\endcsname{0.40}
\expandafter\gdef\csname R@an.power_design.mdec5_acdc_n2\endcsname{0.32}
\expandafter\gdef\csname R@an.power_design.mdec5_acdc_n3\endcsname{0.28}
\expandafter\gdef\csname R@an.power_design.mdec5_acdc_n4\endcsname{0.26}
\expandafter\gdef\csname R@an.power_design.mdec5_acdc_n5\endcsname{0.25}
\expandafter\gdef\csname R@an.power_design.mdec5_acdc_n6\endcsname{0.24}
\expandafter\gdef\csname R@an.power_design.mdec5_acdc_n7\endcsname{0.24}
\expandafter\gdef\csname R@an.power_design.mdec5_acdc_n8\endcsname{0.23}
\expandafter\gdef\csname R@an.power_design.mdec5_amos_n1\endcsname{0.49}
\expandafter\gdef\csname R@an.power_design.mdec5_amos_n3\endcsname{0.34}
\expandafter\gdef\csname R@an.power_design.mdec5_amos_n6\endcsname{0.29}
\expandafter\gdef\csname R@an.power_design.mdecl_acdc_floor\endcsname{0.32}
\expandafter\gdef\csname R@an.power_design.mdecl_acdc_n1\endcsname{0.64}
\expandafter\gdef\csname R@an.power_design.mdecl_acdc_n2\endcsname{0.51}
\expandafter\gdef\csname R@an.power_design.mdecl_acdc_n3\endcsname{0.45}
\expandafter\gdef\csname R@an.power_design.mdecl_acdc_n4\endcsname{0.42}
\expandafter\gdef\csname R@an.power_design.mdecl_acdc_n5\endcsname{0.41}
\expandafter\gdef\csname R@an.power_design.mdecl_acdc_n6\endcsname{0.39}
\expandafter\gdef\csname R@an.power_design.mdecl_acdc_n7\endcsname{0.38}
\expandafter\gdef\csname R@an.power_design.mdecl_acdc_n8\endcsname{0.38}
\expandafter\gdef\csname R@an.power_design.mdecl_amos_floor\endcsname{0.37}
\expandafter\gdef\csname R@an.power_design.mdecl_amos_n1\endcsname{0.78}
\expandafter\gdef\csname R@an.power_design.mdecl_amos_n3\endcsname{0.54}
\expandafter\gdef\csname R@an.power_design.mdecl_amos_n6\endcsname{0.47}
\expandafter\gdef\csname R@an.power_design.mdep_acdc_floor\endcsname{0.11}
\expandafter\gdef\csname R@an.power_design.mdep_acdc_n1\endcsname{0.38}
\expandafter\gdef\csname R@an.power_design.mdep_acdc_n2\endcsname{0.27}
\expandafter\gdef\csname R@an.power_design.mdep_acdc_n3\endcsname{0.23}
\expandafter\gdef\csname R@an.power_design.mdep_acdc_n4\endcsname{0.20}
\expandafter\gdef\csname R@an.power_design.mdep_acdc_n5\endcsname{0.19}
\expandafter\gdef\csname R@an.power_design.mdep_acdc_n6\endcsname{0.18}
\expandafter\gdef\csname R@an.power_design.mdep_acdc_n7\endcsname{0.17}
\expandafter\gdef\csname R@an.power_design.mdep_acdc_n8\endcsname{0.16}
\expandafter\gdef\csname R@an.power_design.mdep_acdc_pair_n1\endcsname{0.49}
\expandafter\gdef\csname R@an.power_design.mdep_acdc_pair_n2\endcsname{0.32}
\expandafter\gdef\csname R@an.power_design.mdep_acdc_pair_n3\endcsname{0.25}
\expandafter\gdef\csname R@an.power_design.mdep_acdc_pair_n4\endcsname{0.22}
\expandafter\gdef\csname R@an.power_design.mdep_acdc_pair_n5\endcsname{0.19}
\expandafter\gdef\csname R@an.power_design.mdep_acdc_pair_n6\endcsname{0.17}
\expandafter\gdef\csname R@an.power_design.mdep_acdc_pair_n7\endcsname{0.16}
\expandafter\gdef\csname R@an.power_design.mdep_acdc_pair_n8\endcsname{0.15}
\expandafter\gdef\csname R@an.power_design.mdep_amos_floor\endcsname{0.14}
\expandafter\gdef\csname R@an.power_design.mdep_amos_n1\endcsname{0.46}
\expandafter\gdef\csname R@an.power_design.mdep_amos_n3\endcsname{0.28}
\expandafter\gdef\csname R@an.power_design.mdep_amos_n6\endcsname{0.22}
\expandafter\gdef\csname R@an.power_design.mdep_kits_floor\endcsname{1.3}
\expandafter\gdef\csname R@an.power_design.mdep_kits_n1\endcsname{5.2}
\expandafter\gdef\csname R@an.power_design.mdep_kits_n3\endcsname{2.4}
\expandafter\gdef\csname R@an.power_design.mdep_kits_n6\endcsname{1.8}
\expandafter\gdef\csname R@an.power_design.mdepair_ratio_acdc_n1\endcsname{1.31}
\expandafter\gdef\csname R@an.power_design.mdepair_ratio_acdc_n2\endcsname{1.22}
\expandafter\gdef\csname R@an.power_design.mdepair_ratio_acdc_n3\endcsname{1.15}
\expandafter\gdef\csname R@an.power_design.mdepair_ratio_amos_n1\endcsname{1.31}
\expandafter\gdef\csname R@an.power_design.mdepair_ratio_amos_n2\endcsname{1.22}
\expandafter\gdef\csname R@an.power_design.mdepair_ratio_amos_n3\endcsname{1.15}
\expandafter\gdef\csname R@an.power_design.mdepair_ratio_kits_n1\endcsname{1.22}
\expandafter\gdef\csname R@an.power_design.mdepair_ratio_kits_n2\endcsname{1.10}
\expandafter\gdef\csname R@an.power_design.mdepair_ratio_kits_n3\endcsname{1.00}
\expandafter\gdef\csname R@an.power_design.mrun_acdc\endcsname{12}
\expandafter\gdef\csname R@an.power_design.mrun_amos\endcsname{13}
\expandafter\gdef\csname R@an.power_design.mrun_amos_collector\endcsname{13}
\expandafter\gdef\csname R@an.power_design.mrun_amos_q2\endcsname{0}
\expandafter\gdef\csname R@an.power_design.mrun_def\endcsname{the arms with a finished discovery-seed run on that dataset among the registered wave arms of the collector and the Addendum Q2 screens (random-search, scaled-HyReX, single-prompt and reference runs, counted as they finish): 13 on AMOS22 (13 + 0), 7 on KiTS23 (7 + 0)}
\expandafter\gdef\csname R@an.power_design.mrun_kits\endcsname{7}
\expandafter\gdef\csname R@an.power_design.mrun_kits_collector\endcsname{7}
\expandafter\gdef\csname R@an.power_design.mrun_kits_q2\endcsname{0}
\expandafter\gdef\csname R@an.power_design.multiseed_full\endcsname{3}
\expandafter\gdef\csname R@an.power_design.multiseed_fullword\endcsname{three}
\expandafter\gdef\csname R@an.power_design.n_multiseed_acdc\endcsname{3}
\expandafter\gdef\csname R@an.power_design.n_multiseed_acdc_arms\endcsname{ResEnc-M, ResEnc-matched, HyReX}
\expandafter\gdef\csname R@an.power_design.n_multiseed_acdc_seeds\endcsname{3}
\expandafter\gdef\csname R@an.power_design.n_multiseed_acdc_seedsmax\endcsname{3}
\expandafter\gdef\csname R@an.power_design.n_multiseed_amos\endcsname{5}
\expandafter\gdef\csname R@an.power_design.n_multiseed_amos_arms\endcsname{ResEnc-M, ResEnc-matched, ConvNeXt-k3, HyReX, ResEnc+context}
\expandafter\gdef\csname R@an.power_design.n_multiseed_amos_seeds\endcsname{3}
\expandafter\gdef\csname R@an.power_design.n_multiseed_amos_seedsmax\endcsname{3}
\expandafter\gdef\csname R@an.power_design.n_multiseed_kits\endcsname{25}
\expandafter\gdef\csname R@an.power_design.n_multiseed_kits_arms\endcsname{ResEnc-M, ResEnc-matched, ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context, branch control, LeanDec, HyReX+dec. capacity, fn.-identical control, HyReX point-fuse, HyReX, finer ConvNeXt, HyReX-LeanDec, LeanAdd, LeanAdd-NeXt, HyReX-k9, LeanDeepMid, LeanDeepMid+FD, LeanSep, LeanDil, LeanNeXt-s5, CoarseStack, StackDec, LeanTrunk, Stem1}
\expandafter\gdef\csname R@an.power_design.n_multiseed_kits_seeds\endcsname{3}
\expandafter\gdef\csname R@an.power_design.n_multiseed_kits_seedsmax\endcsname{3}
\expandafter\gdef\csname R@an.power_design.n_partialseed_acdc\endcsname{1}
\expandafter\gdef\csname R@an.power_design.n_partialseed_acdc_arms\endcsname{fn.-identical control}
\expandafter\gdef\csname R@an.power_design.n_partialseed_amos\endcsname{0}
\expandafter\gdef\csname R@an.power_design.n_partialseed_amos_arms\endcsname{none}
\expandafter\gdef\csname R@an.power_design.n_partialseed_kits\endcsname{0}
\expandafter\gdef\csname R@an.power_design.n_partialseed_kits_arms\endcsname{none}
\expandafter\gdef\csname R@an.power_design.n_varrows\endcsname{40}
\expandafter\gdef\csname R@an.power_design.nabove_acdc_gf\endcsname{8}
\expandafter\gdef\csname R@an.power_design.nabove_acdc_gf_of\endcsname{12}
\expandafter\gdef\csname R@an.power_design.nabove_acdc_pf\endcsname{2}
\expandafter\gdef\csname R@an.power_design.nabove_acdc_pf_of\endcsname{12}
\expandafter\gdef\csname R@an.power_design.nclear_acdc_gf\endcsname{8}
\expandafter\gdef\csname R@an.power_design.nclear_acdc_gf_of\endcsname{12}
\expandafter\gdef\csname R@an.power_design.nclear_acdc_pf\endcsname{2}
\expandafter\gdef\csname R@an.power_design.nclear_acdc_pf_of\endcsname{12}
\expandafter\gdef\csname R@an.power_design.nclear_amos\endcsname{6}
\expandafter\gdef\csname R@an.power_design.nclear_amos_of\endcsname{13}
\expandafter\gdef\csname R@an.power_design.nclear_amos_phrase\endcsname{6 of 13 AMOS22 arms clear the \ensuremath{+0.35}\,pp bar}
\expandafter\gdef\csname R@an.power_design.nclear_kits\endcsname{7}
\expandafter\gdef\csname R@an.power_design.nclear_kits_of\endcsname{7}
\expandafter\gdef\csname R@an.power_design.nclear_kits_phrase\endcsname{All 7 of 7 KiTS23 arms clear the \ensuremath{+0.35}\,pp bar}
\expandafter\gdef\csname R@an.power_design.ncp_df2\endcsname{5.65}
\expandafter\gdef\csname R@an.power_design.ncp_df5\endcsname{3.51}
\expandafter\gdef\csname R@an.power_design.ncp_dfinf\endcsname{2.80}
\expandafter\gdef\csname R@an.power_design.obs_arm_acdc\endcsname{HyReX}
\expandafter\gdef\csname R@an.power_design.obs_arm_amos\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.power_design.obs_arm_cand_acdc\endcsname{HyReX}
\expandafter\gdef\csname R@an.power_design.obs_arm_cand_amos\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.power_design.obs_arm_cand_kits\endcsname{HyReX}
\expandafter\gdef\csname R@an.power_design.obs_arm_kits\endcsname{HyReX}
\expandafter\gdef\csname R@an.power_design.obs_arm_other_acdc\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.power_design.obs_arm_other_amos\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.power_design.obs_arm_other_kits\endcsname{branch control}
\expandafter\gdef\csname R@an.power_design.obs_best_acdc\endcsname{\ensuremath{+0.616}}
\expandafter\gdef\csname R@an.power_design.obs_best_acdc_uncompiled\endcsname{\ensuremath{+0.609}}
\expandafter\gdef\csname R@an.power_design.obs_best_amos\endcsname{\ensuremath{+0.647}}
\expandafter\gdef\csname R@an.power_design.obs_best_amos_contemporaneous\endcsname{\ensuremath{+0.636}}
\expandafter\gdef\csname R@an.power_design.obs_best_amos_sd\endcsname{4.90}
\expandafter\gdef\csname R@an.power_design.obs_best_amos_uncompiled\endcsname{\ensuremath{+0.618}}
\expandafter\gdef\csname R@an.power_design.obs_best_cand_acdc\endcsname{\ensuremath{+0.616}}
\expandafter\gdef\csname R@an.power_design.obs_best_cand_amos\endcsname{\ensuremath{+0.430}}
\expandafter\gdef\csname R@an.power_design.obs_best_cand_kits\endcsname{\ensuremath{+2.842}}
\expandafter\gdef\csname R@an.power_design.obs_best_kits\endcsname{\ensuremath{+2.842}}
\expandafter\gdef\csname R@an.power_design.obs_best_kits_contemporaneous\endcsname{\ensuremath{+2.355}}
\expandafter\gdef\csname R@an.power_design.obs_best_kits_sd\endcsname{3.10}
\expandafter\gdef\csname R@an.power_design.obs_best_other_acdc\endcsname{\ensuremath{+0.336}}
\expandafter\gdef\csname R@an.power_design.obs_best_other_amos\endcsname{\ensuremath{+0.647}}
\expandafter\gdef\csname R@an.power_design.obs_best_other_amos_sd\endcsname{4.90}
\expandafter\gdef\csname R@an.power_design.obs_best_other_kits\endcsname{\ensuremath{+2.636}}
\expandafter\gdef\csname R@an.power_design.obs_best_other_kits_sd\endcsname{2.87}
\expandafter\gdef\csname R@an.power_design.obs_m_acdc\endcsname{12}
\expandafter\gdef\csname R@an.power_design.obs_m_amos\endcsname{13}
\expandafter\gdef\csname R@an.power_design.obs_m_cand_acdc\endcsname{9}
\expandafter\gdef\csname R@an.power_design.obs_m_cand_amos\endcsname{7}
\expandafter\gdef\csname R@an.power_design.obs_m_cand_kits\endcsname{4}
\expandafter\gdef\csname R@an.power_design.obs_m_kits\endcsname{7}
\expandafter\gdef\csname R@an.power_design.obs_m_other_acdc\endcsname{3}
\expandafter\gdef\csname R@an.power_design.obs_m_other_amos\endcsname{6}
\expandafter\gdef\csname R@an.power_design.obs_m_other_kits\endcsname{3}
\expandafter\gdef\csname R@an.power_design.pK_acdc_gf\endcsname{0.5}
\expandafter\gdef\csname R@an.power_design.pK_acdc_gf_indep\endcsname{$<$0.1}
\expandafter\gdef\csname R@an.power_design.pK_acdc_gf_scl2\endcsname{3.6}
\expandafter\gdef\csname R@an.power_design.pK_acdc_gf_scl5\endcsname{1.5}
\expandafter\gdef\csname R@an.power_design.pK_acdc_pf\endcsname{0.6}
\expandafter\gdef\csname R@an.power_design.pK_acdc_pf_indep\endcsname{$<$0.1}
\expandafter\gdef\csname R@an.power_design.pK_acdc_pf_scl2\endcsname{6.4}
\expandafter\gdef\csname R@an.power_design.pK_acdc_pf_scl5\endcsname{0.9}
\expandafter\gdef\csname R@an.power_design.pK_amos\endcsname{0.3}
\expandafter\gdef\csname R@an.power_design.pK_amos_indep\endcsname{$<$0.1}
\expandafter\gdef\csname R@an.power_design.pK_amos_scl2\endcsname{3.6}
\expandafter\gdef\csname R@an.power_design.pK_amos_scl5\endcsname{0.6}
\expandafter\gdef\csname R@an.power_design.pK_kits\endcsname{2.0}
\expandafter\gdef\csname R@an.power_design.pK_kits_indep\endcsname{0.1}
\expandafter\gdef\csname R@an.power_design.pairfloor\endcsname{0.50}
\expandafter\gdef\csname R@an.power_design.pclear_acdc_gf_m12\endcsname{58}
\expandafter\gdef\csname R@an.power_design.pclear_acdc_gf_m12_scl2\endcsname{61}
\expandafter\gdef\csname R@an.power_design.pclear_acdc_gf_m12_scl5\endcsname{58}
\expandafter\gdef\csname R@an.power_design.pclear_acdc_gf_m12_ub\endcsname{75}
\expandafter\gdef\csname R@an.power_design.pclear_acdc_gf_mrun\endcsname{58}
\expandafter\gdef\csname R@an.power_design.pclear_acdc_gf_mrun_scl2\endcsname{61}
\expandafter\gdef\csname R@an.power_design.pclear_acdc_gf_mrun_scl5\endcsname{58}
\expandafter\gdef\csname R@an.power_design.pclear_acdc_gf_mrun_ub\endcsname{75}
\expandafter\gdef\csname R@an.power_design.pclear_acdc_pf_m12\endcsname{2.2}
\expandafter\gdef\csname R@an.power_design.pclear_acdc_pf_m12_scl2\endcsname{12}
\expandafter\gdef\csname R@an.power_design.pclear_acdc_pf_m12_scl5\endcsname{2.7}
\expandafter\gdef\csname R@an.power_design.pclear_acdc_pf_m12_ub\endcsname{3.2}
\expandafter\gdef\csname R@an.power_design.pclear_acdc_pf_mrun\endcsname{2.2}
\expandafter\gdef\csname R@an.power_design.pclear_acdc_pf_mrun_scl2\endcsname{12}
\expandafter\gdef\csname R@an.power_design.pclear_acdc_pf_mrun_scl5\endcsname{2.7}
\expandafter\gdef\csname R@an.power_design.pclear_acdc_pf_mrun_ub\endcsname{3.2}
\expandafter\gdef\csname R@an.power_design.pclear_amos_m11\endcsname{16}
\expandafter\gdef\csname R@an.power_design.pclear_amos_m11_lb\endcsname{4.2}
\expandafter\gdef\csname R@an.power_design.pclear_amos_m11_scl2\endcsname{28}
\expandafter\gdef\csname R@an.power_design.pclear_amos_m11_scl5\endcsname{17}
\expandafter\gdef\csname R@an.power_design.pclear_amos_m11_ub\endcsname{22}
\expandafter\gdef\csname R@an.power_design.pclear_amos_m12\endcsname{16}
\expandafter\gdef\csname R@an.power_design.pclear_amos_m12_lb\endcsname{4.5}
\expandafter\gdef\csname R@an.power_design.pclear_amos_m12_ub\endcsname{24}
\expandafter\gdef\csname R@an.power_design.pclear_amos_m13\endcsname{17}
\expandafter\gdef\csname R@an.power_design.pclear_amos_m13_lb\endcsname{4.9}
\expandafter\gdef\csname R@an.power_design.pclear_amos_m13_ub\endcsname{26}
\expandafter\gdef\csname R@an.power_design.pclear_amos_mrun\endcsname{17}
\expandafter\gdef\csname R@an.power_design.pclear_amos_mrun_lb\endcsname{4.9}
\expandafter\gdef\csname R@an.power_design.pclear_amos_mrun_ub\endcsname{26}
\expandafter\gdef\csname R@an.power_design.pclear_kits_m11\endcsname{93}
\expandafter\gdef\csname R@an.power_design.pclear_kits_m11_lb\endcsname{92}
\expandafter\gdef\csname R@an.power_design.pclear_kits_m11_ub\endcsname{99}
\expandafter\gdef\csname R@an.power_design.pclear_kits_m12\endcsname{94}
\expandafter\gdef\csname R@an.power_design.pclear_kits_m12_lb\endcsname{93}
\expandafter\gdef\csname R@an.power_design.pclear_kits_m12_ub\endcsname{100}
\expandafter\gdef\csname R@an.power_design.pclear_kits_m7\endcsname{87}
\expandafter\gdef\csname R@an.power_design.pclear_kits_m7_lb\endcsname{86}
\expandafter\gdef\csname R@an.power_design.pclear_kits_m7_ub\endcsname{96}
\expandafter\gdef\csname R@an.power_design.pclear_kits_mrun\endcsname{87}
\expandafter\gdef\csname R@an.power_design.pclear_kits_mrun_lb\endcsname{86}
\expandafter\gdef\csname R@an.power_design.pclear_kits_mrun_ub\endcsname{96}
\expandafter\gdef\csname R@an.power_design.pglobal_acdc\endcsname{0.9}
\expandafter\gdef\csname R@an.power_design.pglobal_acdc_scl2\endcsname{7.9}
\expandafter\gdef\csname R@an.power_design.pglobal_acdc_scl5\endcsname{1.1}
\expandafter\gdef\csname R@an.power_design.pglobal_acdc_ub\endcsname{1.3}
\expandafter\gdef\csname R@an.power_design.pglobal_amos\endcsname{1.9}
\expandafter\gdef\csname R@an.power_design.pglobal_amos_scl2\endcsname{11}
\expandafter\gdef\csname R@an.power_design.pglobal_amos_scl5\endcsname{2.3}
\expandafter\gdef\csname R@an.power_design.pglobal_amos_ub\endcsname{2.9}
\expandafter\gdef\csname R@an.power_design.pglobal_cand_acdc\endcsname{0.7}
\expandafter\gdef\csname R@an.power_design.pglobal_cand_acdc_ub\endcsname{1.0}
\expandafter\gdef\csname R@an.power_design.pglobal_cand_amos\endcsname{5.9}
\expandafter\gdef\csname R@an.power_design.pglobal_cand_amos_ub\endcsname{7.7}
\expandafter\gdef\csname R@an.power_design.pglobal_cand_kits\endcsname{12}
\expandafter\gdef\csname R@an.power_design.pglobal_cand_kits_ub\endcsname{17}
\expandafter\gdef\csname R@an.power_design.pglobal_kits\endcsname{16}
\expandafter\gdef\csname R@an.power_design.pglobal_kits_ub\endcsname{28}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l1_ci_hi\endcsname{3.6}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l1_ci_lo\endcsname{0.20}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l1_crit\endcsname{2.9}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l1_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l1_ratio\endcsname{0.57}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l1_sd\endcsname{0.057}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l1_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l1_up80\endcsname{6.0}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l1b_ci_hi\endcsname{2.5}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l1b_ci_lo\endcsname{0.13}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l1b_crit\endcsname{2.9}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l1b_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l1b_ratio\endcsname{0.39}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l1b_sd\endcsname{0.039}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l1b_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l1b_up80\endcsname{6.0}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l3_ci_hi\endcsname{6.4}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l3_ci_lo\endcsname{0.35}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l3_crit\endcsname{2.9}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l3_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l3_ratio\endcsname{1.03}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l3_sd\endcsname{0.102}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l3_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_acdc_l3_up80\endcsname{6.0}
\expandafter\gdef\csname R@an.power_design.prem_acdc_p3c_ci_hi\endcsname{3.6}
\expandafter\gdef\csname R@an.power_design.prem_acdc_p3c_ci_lo\endcsname{0.04}
\expandafter\gdef\csname R@an.power_design.prem_acdc_p3c_crit\endcsname{3.2}
\expandafter\gdef\csname R@an.power_design.prem_acdc_p3c_n\endcsname{2}
\expandafter\gdef\csname R@an.power_design.prem_acdc_p3c_ratio\endcsname{0.12}
\expandafter\gdef\csname R@an.power_design.prem_acdc_p3c_sd\endcsname{0.012}
\expandafter\gdef\csname R@an.power_design.prem_acdc_p3c_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_acdc_p3c_up80\endcsname{11.7}
\expandafter\gdef\csname R@an.power_design.prem_amos_l1_ci_hi\endcsname{11.5}
\expandafter\gdef\csname R@an.power_design.prem_amos_l1_ci_lo\endcsname{0.63}
\expandafter\gdef\csname R@an.power_design.prem_amos_l1_crit\endcsname{2.9}
\expandafter\gdef\csname R@an.power_design.prem_amos_l1_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_amos_l1_ratio\endcsname{1.83}
\expandafter\gdef\csname R@an.power_design.prem_amos_l1_sd\endcsname{0.223}
\expandafter\gdef\csname R@an.power_design.prem_amos_l1_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_amos_l1_up80\endcsname{6.0}
\expandafter\gdef\csname R@an.power_design.prem_amos_l1b_ci_hi\endcsname{8.1}
\expandafter\gdef\csname R@an.power_design.prem_amos_l1b_ci_lo\endcsname{0.45}
\expandafter\gdef\csname R@an.power_design.prem_amos_l1b_crit\endcsname{2.9}
\expandafter\gdef\csname R@an.power_design.prem_amos_l1b_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_amos_l1b_ratio\endcsname{1.29}
\expandafter\gdef\csname R@an.power_design.prem_amos_l1b_sd\endcsname{0.158}
\expandafter\gdef\csname R@an.power_design.prem_amos_l1b_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_amos_l1b_up80\endcsname{6.0}
\expandafter\gdef\csname R@an.power_design.prem_amos_l2_ci_hi\endcsname{5.9}
\expandafter\gdef\csname R@an.power_design.prem_amos_l2_ci_lo\endcsname{0.32}
\expandafter\gdef\csname R@an.power_design.prem_amos_l2_crit\endcsname{2.9}
\expandafter\gdef\csname R@an.power_design.prem_amos_l2_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_amos_l2_ratio\endcsname{0.93}
\expandafter\gdef\csname R@an.power_design.prem_amos_l2_sd\endcsname{0.114}
\expandafter\gdef\csname R@an.power_design.prem_amos_l2_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_amos_l2_up80\endcsname{6.0}
\expandafter\gdef\csname R@an.power_design.prem_amos_l3_ci_hi\endcsname{10.6}
\expandafter\gdef\csname R@an.power_design.prem_amos_l3_ci_lo\endcsname{0.58}
\expandafter\gdef\csname R@an.power_design.prem_amos_l3_crit\endcsname{2.9}
\expandafter\gdef\csname R@an.power_design.prem_amos_l3_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_amos_l3_ratio\endcsname{1.69}
\expandafter\gdef\csname R@an.power_design.prem_amos_l3_sd\endcsname{0.206}
\expandafter\gdef\csname R@an.power_design.prem_amos_l3_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_amos_l3_up80\endcsname{6.0}
\expandafter\gdef\csname R@an.power_design.prem_amos_l4_ci_hi\endcsname{5.3}
\expandafter\gdef\csname R@an.power_design.prem_amos_l4_ci_lo\endcsname{0.29}
\expandafter\gdef\csname R@an.power_design.prem_amos_l4_crit\endcsname{2.9}
\expandafter\gdef\csname R@an.power_design.prem_amos_l4_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_amos_l4_ratio\endcsname{0.85}
\expandafter\gdef\csname R@an.power_design.prem_amos_l4_sd\endcsname{0.103}
\expandafter\gdef\csname R@an.power_design.prem_amos_l4_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_amos_l4_up80\endcsname{6.0}
\expandafter\gdef\csname R@an.power_design.prem_kits_c1_ci_hi\endcsname{5.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_c1_ci_lo\endcsname{0.14}
\expandafter\gdef\csname R@an.power_design.prem_kits_c1_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_c1_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_c1_ratio\endcsname{0.87}
\expandafter\gdef\csname R@an.power_design.prem_kits_c1_sd\endcsname{0.695}
\expandafter\gdef\csname R@an.power_design.prem_kits_c1_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_c1_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_d1_ci_hi\endcsname{2.3}
\expandafter\gdef\csname R@an.power_design.prem_kits_d1_ci_lo\endcsname{0.06}
\expandafter\gdef\csname R@an.power_design.prem_kits_d1_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_d1_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_d1_ratio\endcsname{0.37}
\expandafter\gdef\csname R@an.power_design.prem_kits_d1_sd\endcsname{0.292}
\expandafter\gdef\csname R@an.power_design.prem_kits_d1_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_d1_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_d2_ci_hi\endcsname{2.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_d2_ci_lo\endcsname{0.06}
\expandafter\gdef\csname R@an.power_design.prem_kits_d2_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_d2_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_d2_ratio\endcsname{0.35}
\expandafter\gdef\csname R@an.power_design.prem_kits_d2_sd\endcsname{0.282}
\expandafter\gdef\csname R@an.power_design.prem_kits_d2_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_d2_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_l1_ci_hi\endcsname{5.9}
\expandafter\gdef\csname R@an.power_design.prem_kits_l1_ci_lo\endcsname{0.15}
\expandafter\gdef\csname R@an.power_design.prem_kits_l1_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_l1_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_l1_ratio\endcsname{0.94}
\expandafter\gdef\csname R@an.power_design.prem_kits_l1_sd\endcsname{0.746}
\expandafter\gdef\csname R@an.power_design.prem_kits_l1_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_l1_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_l1b_ci_hi\endcsname{3.3}
\expandafter\gdef\csname R@an.power_design.prem_kits_l1b_ci_lo\endcsname{0.08}
\expandafter\gdef\csname R@an.power_design.prem_kits_l1b_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_l1b_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_l1b_ratio\endcsname{0.52}
\expandafter\gdef\csname R@an.power_design.prem_kits_l1b_sd\endcsname{0.414}
\expandafter\gdef\csname R@an.power_design.prem_kits_l1b_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_l1b_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_l2_ci_hi\endcsname{7.6}
\expandafter\gdef\csname R@an.power_design.prem_kits_l2_ci_lo\endcsname{0.20}
\expandafter\gdef\csname R@an.power_design.prem_kits_l2_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_l2_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_l2_ratio\endcsname{1.22}
\expandafter\gdef\csname R@an.power_design.prem_kits_l2_sd\endcsname{0.970}
\expandafter\gdef\csname R@an.power_design.prem_kits_l2_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_l2_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_l3_ci_hi\endcsname{4.1}
\expandafter\gdef\csname R@an.power_design.prem_kits_l3_ci_lo\endcsname{0.11}
\expandafter\gdef\csname R@an.power_design.prem_kits_l3_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_l3_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_l3_ratio\endcsname{0.66}
\expandafter\gdef\csname R@an.power_design.prem_kits_l3_sd\endcsname{0.524}
\expandafter\gdef\csname R@an.power_design.prem_kits_l3_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_l3_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_l4_ci_hi\endcsname{3.4}
\expandafter\gdef\csname R@an.power_design.prem_kits_l4_ci_lo\endcsname{0.09}
\expandafter\gdef\csname R@an.power_design.prem_kits_l4_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_l4_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_l4_ratio\endcsname{0.54}
\expandafter\gdef\csname R@an.power_design.prem_kits_l4_sd\endcsname{0.432}
\expandafter\gdef\csname R@an.power_design.prem_kits_l4_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_l4_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_l6_ci_hi\endcsname{5.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_l6_ci_lo\endcsname{0.13}
\expandafter\gdef\csname R@an.power_design.prem_kits_l6_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_l6_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_l6_ratio\endcsname{0.84}
\expandafter\gdef\csname R@an.power_design.prem_kits_l6_sd\endcsname{0.668}
\expandafter\gdef\csname R@an.power_design.prem_kits_l6_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_l6_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_p3c_ci_hi\endcsname{0.9}
\expandafter\gdef\csname R@an.power_design.prem_kits_p3c_ci_lo\endcsname{0.02}
\expandafter\gdef\csname R@an.power_design.prem_kits_p3c_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_p3c_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_p3c_ratio\endcsname{0.14}
\expandafter\gdef\csname R@an.power_design.prem_kits_p3c_sd\endcsname{0.112}
\expandafter\gdef\csname R@an.power_design.prem_kits_p3c_status\endcsname{FAIL}
\expandafter\gdef\csname R@an.power_design.prem_kits_p3c_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_s2_ci_hi\endcsname{3.9}
\expandafter\gdef\csname R@an.power_design.prem_kits_s2_ci_lo\endcsname{0.10}
\expandafter\gdef\csname R@an.power_design.prem_kits_s2_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_s2_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_s2_ratio\endcsname{0.62}
\expandafter\gdef\csname R@an.power_design.prem_kits_s2_sd\endcsname{0.493}
\expandafter\gdef\csname R@an.power_design.prem_kits_s2_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_s2_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5a5_ci_hi\endcsname{1.7}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5a5_ci_lo\endcsname{0.04}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5a5_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5a5_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5a5_ratio\endcsname{0.28}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5a5_sd\endcsname{0.221}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5a5_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5a5_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5b1_ci_hi\endcsname{0.7}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5b1_ci_lo\endcsname{0.02}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5b1_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5b1_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5b1_ratio\endcsname{0.10}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5b1_sd\endcsname{0.083}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5b1_status\endcsname{FAIL}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5b1_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5b2_ci_hi\endcsname{0.9}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5b2_ci_lo\endcsname{0.02}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5b2_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5b2_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5b2_ratio\endcsname{0.15}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5b2_sd\endcsname{0.117}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5b2_status\endcsname{FAIL}
\expandafter\gdef\csname R@an.power_design.prem_kits_v5b2_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_v6a1r_ci_hi\endcsname{2.4}
\expandafter\gdef\csname R@an.power_design.prem_kits_v6a1r_ci_lo\endcsname{0.06}
\expandafter\gdef\csname R@an.power_design.prem_kits_v6a1r_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_v6a1r_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_v6a1r_ratio\endcsname{0.39}
\expandafter\gdef\csname R@an.power_design.prem_kits_v6a1r_sd\endcsname{0.307}
\expandafter\gdef\csname R@an.power_design.prem_kits_v6a1r_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_v6a1r_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7a1_ci_hi\endcsname{2.7}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7a1_ci_lo\endcsname{0.07}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7a1_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7a1_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7a1_ratio\endcsname{0.43}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7a1_sd\endcsname{0.342}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7a1_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7a1_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7a2_ci_hi\endcsname{3.7}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7a2_ci_lo\endcsname{0.09}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7a2_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7a2_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7a2_ratio\endcsname{0.59}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7a2_sd\endcsname{0.468}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7a2_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7a2_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7b1_ci_hi\endcsname{4.0}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7b1_ci_lo\endcsname{0.10}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7b1_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7b1_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7b1_ratio\endcsname{0.63}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7b1_sd\endcsname{0.503}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7b1_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7b1_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7b2_ci_hi\endcsname{6.3}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7b2_ci_lo\endcsname{0.16}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7b2_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7b2_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7b2_ratio\endcsname{1.00}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7b2_sd\endcsname{0.796}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7b2_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7b2_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7c1_ci_hi\endcsname{2.8}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7c1_ci_lo\endcsname{0.07}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7c1_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7c1_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7c1_ratio\endcsname{0.45}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7c1_sd\endcsname{0.354}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7c1_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_v7c1_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8a1_ci_hi\endcsname{2.7}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8a1_ci_lo\endcsname{0.07}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8a1_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8a1_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8a1_ratio\endcsname{0.43}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8a1_sd\endcsname{0.341}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8a1_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8a1_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8a2_ci_hi\endcsname{3.3}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8a2_ci_lo\endcsname{0.08}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8a2_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8a2_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8a2_ratio\endcsname{0.52}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8a2_sd\endcsname{0.415}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8a2_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8a2_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8b1_ci_hi\endcsname{8.9}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8b1_ci_lo\endcsname{0.23}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8b1_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8b1_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8b1_ratio\endcsname{1.42}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8b1_sd\endcsname{1.133}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8b1_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8b1_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8b2_ci_hi\endcsname{1.3}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8b2_ci_lo\endcsname{0.03}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8b2_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8b2_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8b2_ratio\endcsname{0.21}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8b2_sd\endcsname{0.168}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8b2_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_v8b2_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_kits_w1c_ci_hi\endcsname{8.8}
\expandafter\gdef\csname R@an.power_design.prem_kits_w1c_ci_lo\endcsname{0.23}
\expandafter\gdef\csname R@an.power_design.prem_kits_w1c_crit\endcsname{6.2}
\expandafter\gdef\csname R@an.power_design.prem_kits_w1c_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.prem_kits_w1c_ratio\endcsname{1.42}
\expandafter\gdef\csname R@an.power_design.prem_kits_w1c_sd\endcsname{1.125}
\expandafter\gdef\csname R@an.power_design.prem_kits_w1c_status\endcsname{SKIP}
\expandafter\gdef\csname R@an.power_design.prem_kits_w1c_up80\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_offset_mde3_amos\endcsname{0.54}
\expandafter\gdef\csname R@an.power_design.prem_offset_mde3_kits\endcsname{3.67}
\expandafter\gdef\csname R@an.power_design.prem_runs_per_side\endcsname{19}
\expandafter\gdef\csname R@an.power_design.prem_tol\endcsname{2}
\expandafter\gdef\csname R@an.power_design.prem_up80_amos_3v6\endcsname{6.0}
\expandafter\gdef\csname R@an.power_design.prem_up80_amos_6v6\endcsname{4.0}
\expandafter\gdef\csname R@an.power_design.prem_up80_amos_inf_v6\endcsname{3.0}
\expandafter\gdef\csname R@an.power_design.prem_up80_kits_3v3\endcsname{12.5}
\expandafter\gdef\csname R@an.power_design.prem_up80_kits_inf_v3\endcsname{8.0}
\expandafter\gdef\csname R@an.power_design.premise.direction\endcsname{Of the rejected, 3 groups have less seed scatter than the pool, so every pool-SD resolution figure in this paper is CONSERVATIVE for those arms; nothing is shown either way for the 31 groups the test leaves untested.}
\expandafter\gdef\csname R@an.power_design.premise.n\endcsname{34}
\expandafter\gdef\csname R@an.power_design.premise.n_rejected\endcsname{3}
\expandafter\gdef\csname R@an.power_design.premise.n_supported\endcsname{0}
\expandafter\gdef\csname R@an.power_design.premise.n_untested\endcsname{31}
\expandafter\gdef\csname R@an.power_design.premise.rejected_arms\endcsname{KiTS23 fn.-identical control, KiTS23 LeanAdd, KiTS23 LeanAdd-NeXt}
\expandafter\gdef\csname R@an.power_design.premise.sentence\endcsname{The premise behind every resolution figure here -- that a design arm has the seed SD of its dataset's frozen default pool (charter 2b) -- is tested group by group with an $F$ test: of the 34 multi-seed groups the test rejects it for 3 (KiTS23 fn.-identical control over 3 seeds, SD 0.112\,pp on 2 df against the pool's 0.795 on 2 df, ratio 0.14, 95\,\% CI 0.02 to 0.88; KiTS23 LeanAdd over 3 seeds, SD 0.083\,pp on 2 df against the pool's 0.795 on 2 df, ratio 0.10, 95\,\% CI 0.02 to 0.65; KiTS23 LeanAdd-NeXt over 3 seeds, SD 0.117\,pp on 2 df against the pool's 0.795 on 2 df, ratio 0.15, 95\,\% CI 0.02 to 0.92) and leaves 31 untested, neither rejected nor supported, because it cannot see an SD ratio of 2, which would double every minimum detectable effect on this scale. Of the rejected, 3 groups have less seed scatter than the pool, so every pool-SD resolution figure in this paper is CONSERVATIVE for those arms; nothing is shown either way for the 31 groups the test leaves untested.}
\expandafter\gdef\csname R@an.power_design.premise.short\endcsname{the charter-2b seed-SD premise is rejected for 3 of the 34 multi-seed groups (KiTS23 fn.-identical control, KiTS23 LeanAdd, KiTS23 LeanAdd-NeXt; less seed scatter than the pool, so the pool-SD figures are conservative there) and untested for 31}
\expandafter\gdef\csname R@an.power_design.premise.status\endcsname{rejected for 3 of 34 groups}
\expandafter\gdef\csname R@an.power_design.ratio_l1l1b_pub_amos\endcsname{3.9}
\expandafter\gdef\csname R@an.power_design.ref_acdc_mean\endcsname{92.009}
\expandafter\gdef\csname R@an.power_design.ref_acdc_n\endcsname{6}
\expandafter\gdef\csname R@an.power_design.ref_amos_mean\endcsname{87.701}
\expandafter\gdef\csname R@an.power_design.ref_amos_n\endcsname{6}
\expandafter\gdef\csname R@an.power_design.ref_kits_mean\endcsname{83.378}
\expandafter\gdef\csname R@an.power_design.ref_kits_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.refalt_acdc\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.power_design.refalt_acdc_uncompiled_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.refalt_acdc_uncompiled_shift\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.power_design.refalt_amos\endcsname{contemporaneous default runs; uncompiled sub-pool}
\expandafter\gdef\csname R@an.power_design.refalt_amos_contemporaneous_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.refalt_amos_contemporaneous_shift\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.power_design.refalt_amos_pending\endcsname{none}
\expandafter\gdef\csname R@an.power_design.refalt_amos_uncompiled_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.refalt_amos_uncompiled_shift\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.power_design.refalt_kits\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.power_design.refalt_kits_contemporaneous_n\endcsname{3}
\expandafter\gdef\csname R@an.power_design.refalt_kits_contemporaneous_shift\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.power_design.refalt_kits_pending\endcsname{none}
\expandafter\gdef\csname R@an.power_design.rs_exp_amos\endcsname{0.11}
\expandafter\gdef\csname R@an.power_design.rs_exp_kits\endcsname{5.55}
\expandafter\gdef\csname R@an.power_design.rs_n_amos\endcsname{5}
\expandafter\gdef\csname R@an.power_design.rs_n_kits\endcsname{15}
\expandafter\gdef\csname R@an.power_design.seeds_gf_acdc\endcsname{51}
\expandafter\gdef\csname R@an.power_design.seeds_l1_l1b_acdc\endcsname{88}
\expandafter\gdef\csname R@an.power_design.seeds_l1_l1b_acdc_sdhi\endcsname{529}
\expandafter\gdef\csname R@an.power_design.seeds_l1_l1b_acdc_sdlo\endcsname{35}
\expandafter\gdef\csname R@an.power_design.seeds_l1_l1b_amos\endcsname{2}
\expandafter\gdef\csname R@an.power_design.seeds_l1_l1b_amos_sdhi\endcsname{9}
\expandafter\gdef\csname R@an.power_design.seeds_l1_l1b_amos_sdlo\endcsname{1}
\expandafter\gdef\csname R@an.power_design.seeds_l1_l1b_kits\endcsname{119}
\expandafter\gdef\csname R@an.power_design.seeds_l1_l1b_kits_sdhi\endcsname{4686}
\expandafter\gdef\csname R@an.power_design.seeds_l1_l1b_kits_sdlo\endcsname{33}
\expandafter\gdef\csname R@an.power_design.seeds_l3_default_acdc\endcsname{1}
\expandafter\gdef\csname R@an.power_design.seeds_l3_default_acdc_sdhi\endcsname{3}
\expandafter\gdef\csname R@an.power_design.seeds_l3_default_acdc_sdlo\endcsname{1}
\expandafter\gdef\csname R@an.power_design.seeds_l3_default_amos\endcsname{2}
\expandafter\gdef\csname R@an.power_design.seeds_l3_default_amos_sdhi\endcsname{$\infty$}
\expandafter\gdef\csname R@an.power_design.seeds_l3_default_amos_sdlo\endcsname{1}
\expandafter\gdef\csname R@an.power_design.seeds_l3_default_kits\endcsname{16}
\expandafter\gdef\csname R@an.power_design.seeds_l3_default_kits_sdhi\endcsname{$\infty$}
\expandafter\gdef\csname R@an.power_design.seeds_l3_default_kits_sdlo\endcsname{1}
\expandafter\gdef\csname R@an.power_design.seeds_l3_l1_acdc\endcsname{4}
\expandafter\gdef\csname R@an.power_design.seeds_l3_l1_acdc_sdhi\endcsname{19}
\expandafter\gdef\csname R@an.power_design.seeds_l3_l1_acdc_sdlo\endcsname{2}
\expandafter\gdef\csname R@an.power_design.seeds_l3_l1_amos\endcsname{6}
\expandafter\gdef\csname R@an.power_design.seeds_l3_l1_amos_sdhi\endcsname{32}
\expandafter\gdef\csname R@an.power_design.seeds_l3_l1_amos_sdlo\endcsname{3}
\expandafter\gdef\csname R@an.power_design.seeds_l3_l1_kits\endcsname{152}
\expandafter\gdef\csname R@an.power_design.seeds_l3_l1_kits_sdhi\endcsname{$>$5000}
\expandafter\gdef\csname R@an.power_design.seeds_l3_l1_kits_sdlo\endcsname{42}
\expandafter\gdef\csname R@an.power_design.seeds_pf_acdc\endcsname{1}
\expandafter\gdef\csname R@an.power_design.seeds_thr_amos\endcsname{3}
\expandafter\gdef\csname R@an.power_design.seeds_thr_kits\endcsname{$\infty$}
\expandafter\gdef\csname R@an.power_design.seedsc5_gf_acdc\endcsname{$\infty$}
\expandafter\gdef\csname R@an.power_design.seedsc5_pf_acdc\endcsname{1}
\expandafter\gdef\csname R@an.power_design.seedscl_gf_acdc\endcsname{$\infty$}
\expandafter\gdef\csname R@an.power_design.seedscl_pf_acdc\endcsname{3}
\expandafter\gdef\csname R@an.power_design.seedscl_thr_amos\endcsname{$\infty$}
\expandafter\gdef\csname R@an.power_design.seedsp_gf_acdc\endcsname{12}
\expandafter\gdef\csname R@an.power_design.seedsp_l1_l1b_acdc\endcsname{57}
\expandafter\gdef\csname R@an.power_design.seedsp_l1_l1b_amos\endcsname{2}
\expandafter\gdef\csname R@an.power_design.seedsp_l1_l1b_kits\endcsname{31}
\expandafter\gdef\csname R@an.power_design.seedsp_l3_default_acdc\endcsname{1}
\expandafter\gdef\csname R@an.power_design.seedsp_l3_default_amos\endcsname{2}
\expandafter\gdef\csname R@an.power_design.seedsp_l3_default_kits\endcsname{3}
\expandafter\gdef\csname R@an.power_design.seedsp_l3_l1_acdc\endcsname{3}
\expandafter\gdef\csname R@an.power_design.seedsp_l3_l1_amos\endcsname{5}
\expandafter\gdef\csname R@an.power_design.seedsp_l3_l1_kits\endcsname{39}
\expandafter\gdef\csname R@an.power_design.seedsp_pf_acdc\endcsname{1}
\expandafter\gdef\csname R@an.power_design.seedsp_thr_amos\endcsname{2}
\expandafter\gdef\csname R@an.power_design.seedsp_thr_kits\endcsname{$\infty$}
\expandafter\gdef\csname R@an.power_design.seedspair_gf_acdc\endcsname{11}
\expandafter\gdef\csname R@an.power_design.seedspair_pf_acdc\endcsname{1}
\expandafter\gdef\csname R@an.power_design.sens.acdc.arms\endcsname{ResEnc-matched, HyReX}
\expandafter\gdef\csname R@an.power_design.sens.acdc.df\endcsname{4}
\expandafter\gdef\csname R@an.power_design.sens.acdc.floor\endcsname{0.11}
\expandafter\gdef\csname R@an.power_design.sens.acdc.mde_n1\endcsname{0.29}
\expandafter\gdef\csname R@an.power_design.sens.acdc.mde_n2\endcsname{0.22}
\expandafter\gdef\csname R@an.power_design.sens.acdc.mde_n3\endcsname{0.19}
\expandafter\gdef\csname R@an.power_design.sens.acdc.mde_n6\endcsname{0.16}
\expandafter\gdef\csname R@an.power_design.sens.acdc.mdereg_n1\endcsname{0.38}
\expandafter\gdef\csname R@an.power_design.sens.acdc.mdereg_n2\endcsname{0.28}
\expandafter\gdef\csname R@an.power_design.sens.acdc.mdereg_n3\endcsname{0.25}
\expandafter\gdef\csname R@an.power_design.sens.acdc.mdereg_n6\endcsname{0.20}
\expandafter\gdef\csname R@an.power_design.sens.acdc.n\endcsname{2}
\expandafter\gdef\csname R@an.power_design.sens.acdc.pair_n1\endcsname{0.38}
\expandafter\gdef\csname R@an.power_design.sens.acdc.poolsd\endcsname{0.099}
\expandafter\gdef\csname R@an.power_design.sens.acdc.ratio\endcsname{0.78}
\expandafter\gdef\csname R@an.power_design.sens.acdc.sd\endcsname{0.077}
\expandafter\gdef\csname R@an.power_design.sens.acdc.sdmax\endcsname{0.102}
\expandafter\gdef\csname R@an.power_design.sens.acdc.sdmin\endcsname{0.039}
\expandafter\gdef\csname R@an.power_design.sens.acdc.sentence\endcsname{SENSITIVITY, beside the registered ACDC ladder and not replacing it: pooling the seed SD of the 2 plan-aware arms that hold 3 seeds each on ACDC (ResEnc-matched, HyReX) gives 0.077\,pp on 4 df, 0.78 times the frozen pool's 0.099\,pp, and the one-seed rung of 0.38\,pp becomes 0.29\,pp (three seeds 0.19 against 0.25). The 2 arms scatter from 0.039 to 0.102\,pp, so this is a statement about the SPREAD of design-arm seed noise and neither a test of the charter-2b premise nor a yardstick.}
\expandafter\gdef\csname R@an.power_design.sens.acdc.state\endcsname{computed}
\expandafter\gdef\csname R@an.power_design.sens.acdc.stock\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.power_design.sens.amos.arms\endcsname{ResEnc-matched, ConvNeXt-k3, HyReX, ResEnc+context}
\expandafter\gdef\csname R@an.power_design.sens.amos.df\endcsname{8}
\expandafter\gdef\csname R@an.power_design.sens.amos.floor\endcsname{0.22}
\expandafter\gdef\csname R@an.power_design.sens.amos.mde_n1\endcsname{0.57}
\expandafter\gdef\csname R@an.power_design.sens.amos.mde_n2\endcsname{0.43}
\expandafter\gdef\csname R@an.power_design.sens.amos.mde_n3\endcsname{0.375}
\expandafter\gdef\csname R@an.power_design.sens.amos.mde_n6\endcsname{0.31}
\expandafter\gdef\csname R@an.power_design.sens.amos.mdereg_n1\endcsname{0.46}
\expandafter\gdef\csname R@an.power_design.sens.amos.mdereg_n2\endcsname{0.351}
\expandafter\gdef\csname R@an.power_design.sens.amos.mdereg_n3\endcsname{0.30}
\expandafter\gdef\csname R@an.power_design.sens.amos.mdereg_n6\endcsname{0.25}
\expandafter\gdef\csname R@an.power_design.sens.amos.n\endcsname{4}
\expandafter\gdef\csname R@an.power_design.sens.amos.pair_n1\endcsname{0.75}
\expandafter\gdef\csname R@an.power_design.sens.amos.poolsd\endcsname{0.122}
\expandafter\gdef\csname R@an.power_design.sens.amos.ratio\endcsname{1.24}
\expandafter\gdef\csname R@an.power_design.sens.amos.sd\endcsname{0.151}
\expandafter\gdef\csname R@an.power_design.sens.amos.sdmax\endcsname{0.206}
\expandafter\gdef\csname R@an.power_design.sens.amos.sdmin\endcsname{0.103}
\expandafter\gdef\csname R@an.power_design.sens.amos.sentence\endcsname{SENSITIVITY, beside the registered AMOS22 ladder and not replacing it: pooling the seed SD of the 4 plan-aware arms that hold 3 seeds each on AMOS22 (ResEnc-matched, ConvNeXt-k3, HyReX, ResEnc+context) gives 0.151\,pp on 8 df, 1.24 times the frozen pool's 0.122\,pp, and the one-seed rung of 0.46\,pp becomes 0.57\,pp (three seeds 0.375 against 0.30). The 4 arms scatter from 0.103 to 0.206\,pp, so this is a statement about the SPREAD of design-arm seed noise and neither a test of the charter-2b premise nor a yardstick.}
\expandafter\gdef\csname R@an.power_design.sens.amos.state\endcsname{computed}
\expandafter\gdef\csname R@an.power_design.sens.amos.stock\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.power_design.sens.kits.arms\endcsname{HyReX+dec. capacity, HyReX point-fuse, LeanDec, ResEnc-matched, ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context, fn.-identical control, HyReX, finer ConvNeXt, HyReX-LeanDec, LeanAdd, LeanAdd-NeXt, HyReX-k9, LeanDeepMid, LeanDeepMid+FD, LeanSep, LeanDil, LeanNeXt-s5, CoarseStack, StackDec, LeanTrunk, Stem1, branch control}
\expandafter\gdef\csname R@an.power_design.sens.kits.df\endcsname{48}
\expandafter\gdef\csname R@an.power_design.sens.kits.floor\endcsname{1.8}
\expandafter\gdef\csname R@an.power_design.sens.kits.mde_n1\endcsname{3.6}
\expandafter\gdef\csname R@an.power_design.sens.kits.mde_n2\endcsname{2.85}
\expandafter\gdef\csname R@an.power_design.sens.kits.mde_n3\endcsname{2.5}
\expandafter\gdef\csname R@an.power_design.sens.kits.mde_n6\endcsname{2.2}
\expandafter\gdef\csname R@an.power_design.sens.kits.mdereg_n1\endcsname{5.2}
\expandafter\gdef\csname R@an.power_design.sens.kits.mdereg_n2\endcsname{4.1}
\expandafter\gdef\csname R@an.power_design.sens.kits.mdereg_n3\endcsname{3.7}
\expandafter\gdef\csname R@an.power_design.sens.kits.mdereg_n6\endcsname{3.2}
\expandafter\gdef\csname R@an.power_design.sens.kits.n\endcsname{24}
\expandafter\gdef\csname R@an.power_design.sens.kits.pair_n1\endcsname{4.4}
\expandafter\gdef\csname R@an.power_design.sens.kits.poolsd\endcsname{0.795}
\expandafter\gdef\csname R@an.power_design.sens.kits.ratio\endcsname{0.69}
\expandafter\gdef\csname R@an.power_design.sens.kits.sd\endcsname{0.551}
\expandafter\gdef\csname R@an.power_design.sens.kits.sdmax\endcsname{1.133}
\expandafter\gdef\csname R@an.power_design.sens.kits.sdmin\endcsname{0.083}
\expandafter\gdef\csname R@an.power_design.sens.kits.sentence\endcsname{SENSITIVITY, beside the registered KiTS23 ladder and not replacing it: pooling the seed SD of the 24 plan-aware arms that hold 3 seeds each on KiTS23 (HyReX+dec. capacity, HyReX point-fuse, LeanDec, ResEnc-matched, ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context, fn.-identical control, HyReX, finer ConvNeXt, HyReX-LeanDec, LeanAdd, LeanAdd-NeXt, HyReX-k9, LeanDeepMid, LeanDeepMid+FD, LeanSep, LeanDil, LeanNeXt-s5, CoarseStack, StackDec, LeanTrunk, Stem1, branch control) gives 0.551\,pp on 48 df, 0.69 times the frozen pool's 0.795\,pp, and the one-seed rung of 5.2\,pp becomes 3.6\,pp (three seeds 2.5 against 3.7). The 24 arms scatter from 0.083 to 1.133\,pp, so this is a statement about the SPREAD of design-arm seed noise and neither a test of the charter-2b premise nor a yardstick.}
\expandafter\gdef\csname R@an.power_design.sens.kits.state\endcsname{computed}
\expandafter\gdef\csname R@an.power_design.sens.kits.stock\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.power_design.sens12.kits.cvminres\endcsname{1.760}
\expandafter\gdef\csname R@an.power_design.sens12.kits.cvrung\endcsname{2.353}
\expandafter\gdef\csname R@an.power_design.sens12.kits.df\endcsname{11}
\expandafter\gdef\csname R@an.power_design.sens12.kits.floor\endcsname{0.7}
\expandafter\gdef\csname R@an.power_design.sens12.kits.floorp\endcsname{0.6}
\expandafter\gdef\csname R@an.power_design.sens12.kits.floorpreg\endcsname{1.3}
\expandafter\gdef\csname R@an.power_design.sens12.kits.floorreg\endcsname{2.6}
\expandafter\gdef\csname R@an.power_design.sens12.kits.label\endcsname{SENSITIVITY, beside the registered KiTS23 ladder and not replacing it}
\expandafter\gdef\csname R@an.power_design.sens12.kits.mde_n1\endcsname{2.4}
\expandafter\gdef\csname R@an.power_design.sens12.kits.mde_n2\endcsname{1.8}
\expandafter\gdef\csname R@an.power_design.sens12.kits.mde_n3\endcsname{1.5}
\expandafter\gdef\csname R@an.power_design.sens12.kits.mde_n6\endcsname{1.2}
\expandafter\gdef\csname R@an.power_design.sens12.kits.mdep_n1\endcsname{2.4}
\expandafter\gdef\csname R@an.power_design.sens12.kits.mdep_n3\endcsname{1.5}
\expandafter\gdef\csname R@an.power_design.sens12.kits.mdep_n6\endcsname{1.1}
\expandafter\gdef\csname R@an.power_design.sens12.kits.mdepreg_n1\endcsname{5.2}
\expandafter\gdef\csname R@an.power_design.sens12.kits.mdepreg_n3\endcsname{2.4}
\expandafter\gdef\csname R@an.power_design.sens12.kits.mdepreg_n6\endcsname{1.8}
\expandafter\gdef\csname R@an.power_design.sens12.kits.mdereg_n1\endcsname{5.2}
\expandafter\gdef\csname R@an.power_design.sens12.kits.mdereg_n2\endcsname{4.1}
\expandafter\gdef\csname R@an.power_design.sens12.kits.mdereg_n3\endcsname{3.7}
\expandafter\gdef\csname R@an.power_design.sens12.kits.mdereg_n6\endcsname{3.2}
\expandafter\gdef\csname R@an.power_design.sens12.kits.mean\endcsname{84.038}
\expandafter\gdef\csname R@an.power_design.sens12.kits.n\endcsname{12}
\expandafter\gdef\csname R@an.power_design.sens12.kits.nfailed\endcsname{0}
\expandafter\gdef\csname R@an.power_design.sens12.kits.nopen\endcsname{0}
\expandafter\gdef\csname R@an.power_design.sens12.kits.nreg\endcsname{12}
\expandafter\gdef\csname R@an.power_design.sens12.kits.pair_n1\endcsname{3.3}
\expandafter\gdef\csname R@an.power_design.sens12.kits.pairreg_n1\endcsname{6.4}
\expandafter\gdef\csname R@an.power_design.sens12.kits.sd\endcsname{0.751}
\expandafter\gdef\csname R@an.power_design.sens12.kits.sentence\endcsname{With the twelve stock runs as the reference (mean 84.038, SD 0.751, 11 degrees of freedom), one seed resolves 2.4\,pp and two seeds 1.8\,pp on KiTS23, against 5.2 and 4.1\,pp from the registered three-run pool; the registered screens and verdicts keep the frozen pool (Addendum F)}
\expandafter\gdef\csname R@an.power_design.sens12.kits.state\endcsname{computed}
\expandafter\gdef\csname R@an.power_design.trip1_acdc_chihi\endcsname{30}
\expandafter\gdef\csname R@an.power_design.trip1_acdc_chilo\endcsname{3.7}
\expandafter\gdef\csname R@an.power_design.trip1_acdc_gf\endcsname{11}
\expandafter\gdef\csname R@an.power_design.trip1_acdc_gf_chihi\endcsname{30}
\expandafter\gdef\csname R@an.power_design.trip1_acdc_gf_chilo\endcsname{3.7}
\expandafter\gdef\csname R@an.power_design.trip1_acdc_gf_hi\endcsname{16}
\expandafter\gdef\csname R@an.power_design.trip1_acdc_gf_lo\endcsname{11}
\expandafter\gdef\csname R@an.power_design.trip1_acdc_hi\endcsname{16}
\expandafter\gdef\csname R@an.power_design.trip1_acdc_lo\endcsname{11}
\expandafter\gdef\csname R@an.power_design.trip1_acdc_pf\endcsname{0.3}
\expandafter\gdef\csname R@an.power_design.trip1_acdc_pf_chihi\endcsname{5.7}
\expandafter\gdef\csname R@an.power_design.trip1_acdc_pf_chilo\endcsname{$<$0.1}
\expandafter\gdef\csname R@an.power_design.trip1_acdc_pf_hi\endcsname{2.4}
\expandafter\gdef\csname R@an.power_design.trip1_acdc_pf_lo\endcsname{0.3}
\expandafter\gdef\csname R@an.power_design.trip1_acdc_scr\endcsname{11}
\expandafter\gdef\csname R@an.power_design.trip1_amos\endcsname{2.3}
\expandafter\gdef\csname R@an.power_design.trip1_amos_chihi\endcsname{16}
\expandafter\gdef\csname R@an.power_design.trip1_amos_chilo\endcsname{0.4}
\expandafter\gdef\csname R@an.power_design.trip1_amos_hi\endcsname{6.4}
\expandafter\gdef\csname R@an.power_design.trip1_amos_lo\endcsname{2.3}
\expandafter\gdef\csname R@an.power_design.trip1_amos_scr\endcsname{2.3}
\expandafter\gdef\csname R@an.power_design.trip1_kits\endcsname{37}
\expandafter\gdef\csname R@an.power_design.trip1_kits_chihi\endcsname{48}
\expandafter\gdef\csname R@an.power_design.trip1_kits_chilo\endcsname{27}
\expandafter\gdef\csname R@an.power_design.trip1_kits_hi\endcsname{48}
\expandafter\gdef\csname R@an.power_design.trip1_kits_lo\endcsname{27}
\expandafter\gdef\csname R@an.power_design.trip1_kits_scr\endcsname{37}
\expandafter\gdef\csname R@an.power_design.tripm_acdc\endcsname{58}
\expandafter\gdef\csname R@an.power_design.tripm_acdc_gf\endcsname{58}
\expandafter\gdef\csname R@an.power_design.tripm_acdc_gf_of\endcsname{12}
\expandafter\gdef\csname R@an.power_design.tripm_acdc_of\endcsname{12}
\expandafter\gdef\csname R@an.power_design.tripm_acdc_pf\endcsname{2.2}
\expandafter\gdef\csname R@an.power_design.tripm_acdc_pf_of\endcsname{12}
\expandafter\gdef\csname R@an.power_design.tripm_amos\endcsname{17}
\expandafter\gdef\csname R@an.power_design.tripm_amos_of\endcsname{13}
\expandafter\gdef\csname R@an.power_design.tripm_kits\endcsname{87}
\expandafter\gdef\csname R@an.power_design.tripm_kits_of\endcsname{7}
\expandafter\gdef\csname R@an.process.cap.capped\endcsname{351}
\expandafter\gdef\csname R@an.process.cap.claim\endcsname{all 351 finished full-budget runs trained to completion inside the 12 GB cap}
\expandafter\gdef\csname R@an.process.cap.max_reserved_gb\endcsname{11.98}
\expandafter\gdef\csname R@an.process.cap.n\endcsname{351}
\expandafter\gdef\csname R@an.process.cap.nlogged\endcsname{338}
\expandafter\gdef\csname R@an.process.chain.anchor.after\endcsname{472}
\expandafter\gdef\csname R@an.process.chain.anchor.after_clause\endcsname{the 472 lines written after that anchor are not yet anchored}
\expandafter\gdef\csname R@an.process.chain.anchor.claim\endcsname{the first 224 lines of the amendment ledger were anchored by a second role, the reviewer, in a directory the lead does not write}
\expandafter\gdef\csname R@an.process.chain.anchor.first_lines\endcsname{10}
\expandafter\gdef\csname R@an.process.chain.anchor.lines\endcsname{224}
\expandafter\gdef\csname R@an.process.chain.anchor.n\endcsname{3}
\expandafter\gdef\csname R@an.process.chain.anchor.role\endcsname{reviewer}
\expandafter\gdef\csname R@an.process.chain.anchor.verified\endcsname{3}
\expandafter\gdef\csname R@an.process.chain.chained\endcsname{688}
\expandafter\gdef\csname R@an.process.chain.lines\endcsname{696}
\expandafter\gdef\csname R@an.process.chain.ok\endcsname{verified}
\expandafter\gdef\csname R@an.process.chain.snapshots\endcsname{6}
\expandafter\gdef\csname R@an.process.chain.unchained\endcsname{8}
\expandafter\gdef\csname R@an.process.chain.verdict\endcsname{verifies with no break}
\expandafter\gdef\csname R@an.process.chain.witness_carried\endcsname{1}
\expandafter\gdef\csname R@an.process.chain.witness_explained\endcsname{1}
\expandafter\gdef\csname R@an.process.chain.witness_explained.sentence\endcsname{ledger record 355 read 65 design trials with a result (5 started) against 72 in the records around it, during an open-file storm; it is carried forward, and the ledger tool no longer swallows read errors (CORRECTIONS C54)}
\expandafter\gdef\csname R@an.process.chain.witness_max\endcsname{137}
\expandafter\gdef\csname R@an.process.enforce.archonly\endcsname{351}
\expandafter\gdef\csname R@an.process.enforce.claim\endcsname{351 of 351 finished full-budget runs carry the architecture-only flag, the cap and the full iteration count}
\expandafter\gdef\csname R@an.process.enforce.n\endcsname{351}
\expandafter\gdef\csname R@an.process.forecast.cost_decided\endcsname{9}
\expandafter\gdef\csname R@an.process.forecast.cost_n\endcsname{9}
\expandafter\gdef\csname R@an.process.forecast.cost_ratio_median\endcsname{1.08}
\expandafter\gdef\csname R@an.process.forecast.cost_ratio_n\endcsname{9}
\expandafter\gdef\csname R@an.process.forecast.cost_ratio_second\endcsname{1.23}
\expandafter\gdef\csname R@an.process.forecast.cost_within_second\endcsname{8}
\expandafter\gdef\csname R@an.process.forecast.decided\endcsname{21}
\expandafter\gdef\csname R@an.process.forecast.decided_cost\endcsname{9}
\expandafter\gdef\csname R@an.process.forecast.decided_dated\endcsname{17}
\expandafter\gdef\csname R@an.process.forecast.decided_effect\endcsname{9}
\expandafter\gdef\csname R@an.process.forecast.decided_noise\endcsname{3}
\expandafter\gdef\csname R@an.process.forecast.fp_amos\endcsname{1.3}
\expandafter\gdef\csname R@an.process.forecast.fp_base\endcsname{0.19}
\expandafter\gdef\csname R@an.process.forecast.fp_conv_amos\endcsname{14.9}
\expandafter\gdef\csname R@an.process.forecast.fp_conv_kits\endcsname{1.2}
\expandafter\gdef\csname R@an.process.forecast.fp_df_amos\endcsname{5}
\expandafter\gdef\csname R@an.process.forecast.fp_df_kits\endcsname{2}
\expandafter\gdef\csname R@an.process.forecast.fp_disp_amos\endcsname{0.45}
\expandafter\gdef\csname R@an.process.forecast.fp_disp_kits\endcsname{119}
\expandafter\gdef\csname R@an.process.forecast.fp_kits\endcsname{26.7}
\expandafter\gdef\csname R@an.process.forecast.fp_ratio_amos\endcsname{6.5}
\expandafter\gdef\csname R@an.process.forecast.fp_ratio_kits\endcsname{133}
\expandafter\gdef\csname R@an.process.forecast.fp_registered\endcsname{0.2}
\expandafter\gdef\csname R@an.process.forecast.fp_sd_cand\endcsname{0.10}
\expandafter\gdef\csname R@an.process.forecast.hit\endcsname{7}
\expandafter\gdef\csname R@an.process.forecast.hit_cost\endcsname{4}
\expandafter\gdef\csname R@an.process.forecast.hit_dated\endcsname{6}
\expandafter\gdef\csname R@an.process.forecast.hit_effect\endcsname{3}
\expandafter\gdef\csname R@an.process.forecast.hit_noise\endcsname{0}
\expandafter\gdef\csname R@an.process.forecast.hitrate\endcsname{33}
\expandafter\gdef\csname R@an.process.forecast.in_chain\endcsname{18}
\expandafter\gdef\csname R@an.process.forecast.max_cost_ratio\endcsname{3.94}
\expandafter\gdef\csname R@an.process.forecast.miss\endcsname{14}
\expandafter\gdef\csname R@an.process.forecast.miss_cost\endcsname{5}
\expandafter\gdef\csname R@an.process.forecast.miss_effect\endcsname{6}
\expandafter\gdef\csname R@an.process.forecast.miss_noise\endcsname{3}
\expandafter\gdef\csname R@an.process.forecast.n\endcsname{21}
\expandafter\gdef\csname R@an.process.forecast.noise_clause\endcsname{The 3 decided benchmark-noise forecasts span 4.98$\times$ to 133$\times$ of the measurement, 0 landed, and 3 are re-derivations under the exact-$t$ convention this study adopted later}
\expandafter\gdef\csname R@an.process.forecast.noise_ratio_max\endcsname{133}
\expandafter\gdef\csname R@an.process.forecast.noise_ratio_min\endcsname{4.98}
\expandafter\gdef\csname R@an.process.forecast.noise_ratio_n\endcsname{3}
\expandafter\gdef\csname R@an.process.forecast.noise_rederived\endcsname{3}
\expandafter\gdef\csname R@an.process.forecast.not_in_chain\endcsname{3}
\expandafter\gdef\csname R@an.process.forecast.pending\endcsname{0}
\expandafter\gdef\csname R@an.process.forecast.pending_cost\endcsname{0}
\expandafter\gdef\csname R@an.process.forecast.pending_effect\endcsname{0}
\expandafter\gdef\csname R@an.process.forecast.pending_noise\endcsname{0}
\expandafter\gdef\csname R@an.process.forecast.pre_registered\endcsname{4}
\expandafter\gdef\csname R@an.process.forecast.restates\endcsname{4}
\expandafter\gdef\csname R@an.process.forecast.untimed\endcsname{5}
\expandafter\gdef\csname R@an.process.forecast.w1w2_below_floor\endcsname{11}
\expandafter\gdef\csname R@an.process.forecast.w1w2_classes\endcsname{15}
\expandafter\gdef\csname R@an.process.forecast.w1w2_p\endcsname{0.42}
\expandafter\gdef\csname R@an.process.forecast.w1w2_rho\endcsname{-0.225}
\expandafter\gdef\csname R@an.process.funnel.adj_amos\endcsname{4}
\expandafter\gdef\csname R@an.process.funnel.adj_kits\endcsname{25}
\expandafter\gdef\csname R@an.process.funnel.amos_awaiting\endcsname{0}
\expandafter\gdef\csname R@an.process.funnel.amos_awaiting_arms\endcsname{none}
\expandafter\gdef\csname R@an.process.funnel.amos_controls_read\endcsname{1}
\expandafter\gdef\csname R@an.process.funnel.amos_controls_read_arms\endcsname{ResEnc-matched}
\expandafter\gdef\csname R@an.process.funnel.amos_rep_cell\endcsname{5 of 7 fresh pairs complete, 4 adjudicated (1 control read), 2 survived (ResEnc-M, ResEnc+context)}
\expandafter\gdef\csname R@an.process.funnel.amos_rep_state\endcsname{5 of the 7 registered arms have a complete fresh pair, 4 adjudicated (ResEnc-matched, whose AMOS22 screen did not fire, carries no verdict to record), and 2 survived (ResEnc-M, ResEnc+context)}
\expandafter\gdef\csname R@an.process.funnel.amos_verdict_lag\endcsname{0}
\expandafter\gdef\csname R@an.process.funnel.cut.deferred\endcsname{11}
\expandafter\gdef\csname R@an.process.funnel.cut.diagnostic_only\endcsname{2}
\expandafter\gdef\csname R@an.process.funnel.cut.dominated\endcsname{18}
\expandafter\gdef\csname R@an.process.funnel.cut.duplicate\endcsname{2}
\expandafter\gdef\csname R@an.process.funnel.cut.held\endcsname{4}
\expandafter\gdef\csname R@an.process.funnel.cut.infeasible\endcsname{2}
\expandafter\gdef\csname R@an.process.funnel.cut.infeasible_memory\endcsname{5}
\expandafter\gdef\csname R@an.process.funnel.cut.novelty\endcsname{3}
\expandafter\gdef\csname R@an.process.funnel.cut.premise\endcsname{12}
\expandafter\gdef\csname R@an.process.funnel.cut.total\endcsname{59}
\expandafter\gdef\csname R@an.process.funnel.cv_done\endcsname{36}
\expandafter\gdef\csname R@an.process.funnel.cv_of\endcsname{36}
\expandafter\gdef\csname R@an.process.funnel.cv_state\endcsname{complete}
\expandafter\gdef\csname R@an.process.funnel.epochs\endcsname{1000}
\expandafter\gdef\csname R@an.process.funnel.fired\endcsname{31}
\expandafter\gdef\csname R@an.process.funnel.fired.agent\endcsname{21}
\expandafter\gdef\csname R@an.process.funnel.fired.ctl\endcsname{10}
\expandafter\gdef\csname R@an.process.funnel.fit_acdc.agent\endcsname{26}
\expandafter\gdef\csname R@an.process.funnel.fit_acdc.ctl\endcsname{19}
\expandafter\gdef\csname R@an.process.funnel.fit_all3\endcsname{45}
\expandafter\gdef\csname R@an.process.funnel.fit_all3.agent\endcsname{26}
\expandafter\gdef\csname R@an.process.funnel.fit_all3.ctl\endcsname{19}
\expandafter\gdef\csname R@an.process.funnel.fit_amos.agent\endcsname{29}
\expandafter\gdef\csname R@an.process.funnel.fit_amos.ctl\endcsname{22}
\expandafter\gdef\csname R@an.process.funnel.fit_both.agent\endcsname{29}
\expandafter\gdef\csname R@an.process.funnel.fit_both.ctl\endcsname{22}
\expandafter\gdef\csname R@an.process.funnel.fit_kits.agent\endcsname{29}
\expandafter\gdef\csname R@an.process.funnel.fit_kits.ctl\endcsname{22}
\expandafter\gdef\csname R@an.process.funnel.fresh_amos_arms\endcsname{7}
\expandafter\gdef\csname R@an.process.funnel.fresh_amos_arms_done\endcsname{5}
\expandafter\gdef\csname R@an.process.funnel.fresh_amos_done\endcsname{10}
\expandafter\gdef\csname R@an.process.funnel.fresh_amos_flight\endcsname{4}
\expandafter\gdef\csname R@an.process.funnel.fresh_amos_queued\endcsname{4}
\expandafter\gdef\csname R@an.process.funnel.fresh_amos_running\endcsname{0}
\expandafter\gdef\csname R@an.process.funnel.fresh_amos_status\endcsname{10 of 14 finished (5 complete pairs), 0 running and 4 queued}
\expandafter\gdef\csname R@an.process.funnel.fresh_amos_total\endcsname{14}
\expandafter\gdef\csname R@an.process.funnel.fresh_kits_arms\endcsname{25}
\expandafter\gdef\csname R@an.process.funnel.fresh_kits_done\endcsname{55}
\expandafter\gdef\csname R@an.process.funnel.fresh_kits_queued\endcsname{0}
\expandafter\gdef\csname R@an.process.funnel.fresh_kits_running\endcsname{0}
\expandafter\gdef\csname R@an.process.funnel.fresh_kits_status\endcsname{all 55 finished (25 complete pairs)}
\expandafter\gdef\csname R@an.process.funnel.fresh_kits_total\endcsname{55}
\expandafter\gdef\csname R@an.process.funnel.funded\endcsname{26}
\expandafter\gdef\csname R@an.process.funnel.funded.agent\endcsname{15}
\expandafter\gdef\csname R@an.process.funnel.funded.arms_by_both\endcsname{2}
\expandafter\gdef\csname R@an.process.funnel.funded.arms_by_brief\endcsname{20}
\expandafter\gdef\csname R@an.process.funnel.funded.arms_by_ideator\endcsname{8}
\expandafter\gdef\csname R@an.process.funnel.funded.by_brief\endcsname{20}
\expandafter\gdef\csname R@an.process.funnel.funded.by_ideator\endcsname{8}
\expandafter\gdef\csname R@an.process.funnel.funded.ctl\endcsname{11}
\expandafter\gdef\csname R@an.process.funnel.idea_lenses\endcsname{7}
\expandafter\gdef\csname R@an.process.funnel.idea_rounds\endcsname{2}
\expandafter\gdef\csname R@an.process.funnel.ideas\endcsname{87}
\expandafter\gdef\csname R@an.process.funnel.ideas.brief\endcsname{24}
\expandafter\gdef\csname R@an.process.funnel.ideas.ideator\endcsname{63}
\expandafter\gdef\csname R@an.process.funnel.ideas_distinct\endcsname{85}
\expandafter\gdef\csname R@an.process.funnel.ideas_funded\endcsname{28}
\expandafter\gdef\csname R@an.process.funnel.impl_no_ledger_row\endcsname{22}
\expandafter\gdef\csname R@an.process.funnel.impl_not_funded\endcsname{26}
\expandafter\gdef\csname R@an.process.funnel.impl_not_funded_arms\endcsname{25}
\expandafter\gdef\csname R@an.process.funnel.implemented\endcsname{52}
\expandafter\gdef\csname R@an.process.funnel.implemented.agent\endcsname{30}
\expandafter\gdef\csname R@an.process.funnel.implemented.ctl\endcsname{22}
\expandafter\gdef\csname R@an.process.funnel.kits_awaiting\endcsname{0}
\expandafter\gdef\csname R@an.process.funnel.kits_awaiting_arms\endcsname{none}
\expandafter\gdef\csname R@an.process.funnel.kits_controls_read\endcsname{0}
\expandafter\gdef\csname R@an.process.funnel.kits_ref_label\endcsname{frozen pool}
\expandafter\gdef\csname R@an.process.funnel.kits_ref_n\endcsname{3}
\expandafter\gdef\csname R@an.process.funnel.kits_ref_sd\endcsname{0.795}
\expandafter\gdef\csname R@an.process.funnel.kits_rep_state\endcsname{25 of the 25 registered arms have a complete fresh pair, 25 adjudicated, and 24 survived (HyReX, ResEnc-M, ResEnc-matched, ResEnc+context, HyReX+context, branch control, HyReX, finer ConvNeXt, HyReX point-fuse, HyReX+dec. capacity, LeanDec, fn.-identical control, LeanAdd, LeanAdd-NeXt, HyReX-LeanDec, LeanTrunk, Stem1, CoarseStack, StackDec, LeanDeepMid+FD, LeanSep, LeanDil, LeanDeepMid, LeanNeXt-s5, HyReX-k9)}
\expandafter\gdef\csname R@an.process.funnel.kits_sens_phrase\endcsname{the registered contemporaneous default runs sit +0.487 pp from it}
\expandafter\gdef\csname R@an.process.funnel.kits_sens_state\endcsname{+0.487 pp}
\expandafter\gdef\csname R@an.process.funnel.kits_six_mean\endcsname{83.622}
\expandafter\gdef\csname R@an.process.funnel.kits_six_n\endcsname{6}
\expandafter\gdef\csname R@an.process.funnel.kits_six_shift\endcsname{+0.244}
\expandafter\gdef\csname R@an.process.funnel.kits_unfinished_arms\endcsname{none}
\expandafter\gdef\csname R@an.process.funnel.nest_claim\endcsname{every arm that survived KiTS23 replication also passed the ACDC guard}
\expandafter\gdef\csname R@an.process.funnel.pass\endcsname{9}
\expandafter\gdef\csname R@an.process.funnel.pass.agent\endcsname{7}
\expandafter\gdef\csname R@an.process.funnel.pass.ctl\endcsname{2}
\expandafter\gdef\csname R@an.process.funnel.pass.nosurv\endcsname{1}
\expandafter\gdef\csname R@an.process.funnel.pass.nosurv_arms\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.process.funnel.pass_agent\endcsname{7}
\expandafter\gdef\csname R@an.process.funnel.proposed\endcsname{87}
\expandafter\gdef\csname R@an.process.funnel.randsearch\endcsname{24}
\expandafter\gdef\csname R@an.process.funnel.rep_amos\endcsname{5}
\expandafter\gdef\csname R@an.process.funnel.rep_amos_arms\endcsname{HyReX, ResEnc-M, ResEnc-matched, ConvNeXt-k3, ResEnc+context}
\expandafter\gdef\csname R@an.process.funnel.rep_kits\endcsname{25}
\expandafter\gdef\csname R@an.process.funnel.rep_kits_arms\endcsname{HyReX, ResEnc-M, ResEnc-matched, ConvNeXt-k3, ResEnc+context, HyReX+context, branch control, HyReX, finer ConvNeXt, HyReX point-fuse, HyReX+dec. capacity, LeanDec, fn.-identical control, LeanAdd, LeanAdd-NeXt, HyReX-LeanDec, LeanTrunk, Stem1, CoarseStack, StackDec, LeanDeepMid+FD, LeanSep, LeanDil, LeanDeepMid, LeanNeXt-s5, HyReX-k9}
\expandafter\gdef\csname R@an.process.funnel.rs.adm_amos\endcsname{5}
\expandafter\gdef\csname R@an.process.funnel.rs.adm_both\endcsname{5}
\expandafter\gdef\csname R@an.process.funnel.rs.adm_kits\endcsname{15}
\expandafter\gdef\csname R@an.process.funnel.rs.done\endcsname{0}
\expandafter\gdef\csname R@an.process.funnel.rs.draws\endcsname{38}
\expandafter\gdef\csname R@an.process.funnel.rs.fit_acdc\endcsname{10}
\expandafter\gdef\csname R@an.process.funnel.rs.fit_all3\endcsname{8}
\expandafter\gdef\csname R@an.process.funnel.rs.fit_amos\endcsname{10}
\expandafter\gdef\csname R@an.process.funnel.rs.fit_both\endcsname{10}
\expandafter\gdef\csname R@an.process.funnel.rs.fit_kits\endcsname{21}
\expandafter\gdef\csname R@an.process.funnel.rs.fresh_done\endcsname{0}
\expandafter\gdef\csname R@an.process.funnel.rs.fresh_runs\endcsname{0}
\expandafter\gdef\csname R@an.process.funnel.rs.iters\endcsname{250000}
\expandafter\gdef\csname R@an.process.funnel.rs.limit_amos\endcsname{40}
\expandafter\gdef\csname R@an.process.funnel.rs.limit_kits\endcsname{50}
\expandafter\gdef\csname R@an.process.funnel.rs.overhead\endcsname{1.10}
\expandafter\gdef\csname R@an.process.funnel.rs.plans_mem\endcsname{three}
\expandafter\gdef\csname R@an.process.funnel.rs.plans_wall\endcsname{two}
\expandafter\gdef\csname R@an.process.funnel.rs.queued\endcsname{3}
\expandafter\gdef\csname R@an.process.funnel.rs.rejected\endcsname{14}
\expandafter\gdef\csname R@an.process.funnel.rs.running\endcsname{17}
\expandafter\gdef\csname R@an.process.funnel.rs.runs\endcsname{20}
\expandafter\gdef\csname R@an.process.funnel.rs.runs_amos\endcsname{5}
\expandafter\gdef\csname R@an.process.funnel.rs.runs_kits\endcsname{15}
\expandafter\gdef\csname R@an.process.funnel.rs.sampled\endcsname{24}
\expandafter\gdef\csname R@an.process.funnel.rs.status\endcsname{0 of 20 finished, 17 running and 3 queued}
\expandafter\gdef\csname R@an.process.funnel.rs.window_below\endcsname{0}
\expandafter\gdef\csname R@an.process.funnel.rs.window_clause\endcsname{all 14 rejected draws lay above the AMOS22 parameter window}
\expandafter\gdef\csname R@an.process.funnel.rs.window_other\endcsname{0}
\expandafter\gdef\csname R@an.process.funnel.rs.window_reject\endcsname{14}
\expandafter\gdef\csname R@an.process.funnel.screen_decided\endcsname{32}
\expandafter\gdef\csname R@an.process.funnel.screen_decided.agent\endcsname{22}
\expandafter\gdef\csname R@an.process.funnel.screen_decided.ctl\endcsname{10}
\expandafter\gdef\csname R@an.process.funnel.search_confirmed\endcsname{50}
\expandafter\gdef\csname R@an.process.funnel.search_n\endcsname{191}
\expandafter\gdef\csname R@an.process.funnel.search_retested\endcsname{12}
\expandafter\gdef\csname R@an.process.funnel.search_retested_pairs\endcsname{19}
\expandafter\gdef\csname R@an.process.funnel.smoke\endcsname{52}
\expandafter\gdef\csname R@an.process.funnel.smoke.agent\endcsname{30}
\expandafter\gdef\csname R@an.process.funnel.smoke.ctl\endcsname{22}
\expandafter\gdef\csname R@an.process.funnel.source_arms\endcsname{51}
\expandafter\gdef\csname R@an.process.funnel.sources\endcsname{52}
\expandafter\gdef\csname R@an.process.funnel.survived\endcsname{24}
\expandafter\gdef\csname R@an.process.funnel.survived.agent\endcsname{20}
\expandafter\gdef\csname R@an.process.funnel.survived.ctl\endcsname{4}
\expandafter\gdef\csname R@an.process.funnel.survived.guard\endcsname{8}
\expandafter\gdef\csname R@an.process.funnel.survived.guard_clause\endcsname{8 of the 24 survivors also passed the ACDC guard, and LeanAdd-NeXt and LeanNeXt-s5 ran the guard and sit under its line and branch control, HyReX, finer ConvNeXt, HyReX point-fuse, HyReX+dec. capacity, LeanDec, fn.-identical control, LeanAdd, HyReX-LeanDec, LeanTrunk, Stem1, CoarseStack, StackDec, LeanSep, and LeanDil were replicated without an ACDC run}
\expandafter\gdef\csname R@an.process.funnel.survived.guard_failed\endcsname{2}
\expandafter\gdef\csname R@an.process.funnel.survived.noacdc\endcsname{14}
\expandafter\gdef\csname R@an.process.funnel.survived.noacdc_arms\endcsname{branch control, HyReX, finer ConvNeXt, HyReX point-fuse, HyReX+dec. capacity, LeanDec, fn.-identical control, LeanAdd, HyReX-LeanDec, LeanTrunk, Stem1, CoarseStack, StackDec, LeanSep, LeanDil}
\expandafter\gdef\csname R@an.process.funnel.survived_amos\endcsname{2}
\expandafter\gdef\csname R@an.process.funnel.survived_amos.agent\endcsname{1}
\expandafter\gdef\csname R@an.process.funnel.survived_amos.ctl\endcsname{1}
\expandafter\gdef\csname R@an.process.funnel.survived_amos_arms\endcsname{ResEnc-M, ResEnc+context}
\expandafter\gdef\csname R@an.process.funnel.survived_arms\endcsname{HyReX, ResEnc-M, ResEnc-matched, ResEnc+context, HyReX+context, branch control, HyReX, finer ConvNeXt, HyReX point-fuse, HyReX+dec. capacity, LeanDec, fn.-identical control, LeanAdd, LeanAdd-NeXt, HyReX-LeanDec, LeanTrunk, Stem1, CoarseStack, StackDec, LeanDeepMid+FD, LeanSep, LeanDil, LeanDeepMid, LeanNeXt-s5, HyReX-k9}
\expandafter\gdef\csname R@an.process.funnel.survived_ds\endcsname{KiTS23}
\expandafter\gdef\csname R@an.process.funnel.survived_lead\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.process.funnel.survived_lead_delta\endcsname{+3.475}
\expandafter\gdef\csname R@an.process.funnel.survived_lead_delta_six\endcsname{+3.232}
\expandafter\gdef\csname R@an.process.funnel.survived_order\endcsname{ResEnc-M (+3.475), LeanDeepMid (+2.662), LeanNeXt-s5 (+2.440), HyReX+dec. capacity (+2.401), LeanSep (+2.382), ResEnc-matched (+2.313), LeanDeepMid+FD (+2.289), LeanAdd (+2.285), ResEnc+context (+2.246), HyReX-LeanDec (+2.165), HyReX (+2.094), LeanDec (+1.892), StackDec (+1.877), LeanDil (+1.838), Stem1 (+1.731), HyReX-k9 (+1.704), HyReX+context (+1.591), HyReX point-fuse (+1.477), LeanAdd-NeXt (+1.448), LeanTrunk (+1.375), CoarseStack (+1.249), fn.-identical control (+1.176), branch control (+1.067), HyReX, finer ConvNeXt (+0.570)}
\expandafter\gdef\csname R@an.process.funnel.survived_order_clause\endcsname{On the fresh KiTS23 seeds, against the frozen 3-run default pool, the survivors order as ResEnc-M (+3.475), LeanDeepMid (+2.662), LeanNeXt-s5 (+2.440), HyReX+dec. capacity (+2.401), LeanSep (+2.382), ResEnc-matched (+2.313), LeanDeepMid+FD (+2.289), LeanAdd (+2.285), ResEnc+context (+2.246), HyReX-LeanDec (+2.165), HyReX (+2.094), LeanDec (+1.892), StackDec (+1.877), LeanDil (+1.838), Stem1 (+1.731), HyReX-k9 (+1.704), HyReX+context (+1.591), HyReX point-fuse (+1.477), LeanAdd-NeXt (+1.448), LeanTrunk (+1.375), CoarseStack (+1.249), fn.-identical control (+1.176), branch control (+1.067), HyReX, finer ConvNeXt (+0.570), ResEnc-M first; against the six-run sensitivity reference (the frozen pool plus the 3 contemporaneous default runs, +0.244 pp from the frozen pool's mean) the same arms read ResEnc-M (+3.232), LeanDeepMid (+2.418), LeanNeXt-s5 (+2.196), HyReX+dec. capacity (+2.157), LeanSep (+2.138), ResEnc-matched (+2.070), LeanDeepMid+FD (+2.046), LeanAdd (+2.042), ResEnc+context (+2.003), HyReX-LeanDec (+1.922), HyReX (+1.850), LeanDec (+1.648), StackDec (+1.634), LeanDil (+1.595), Stem1 (+1.487), HyReX-k9 (+1.461), HyReX+context (+1.348), HyReX point-fuse (+1.233), LeanAdd-NeXt (+1.205), LeanTrunk (+1.131), CoarseStack (+1.005), fn.-identical control (+0.932), branch control (+0.823), HyReX, finer ConvNeXt (+0.326).}
\expandafter\gdef\csname R@an.process.funnel.survived_order_six\endcsname{ResEnc-M (+3.232), LeanDeepMid (+2.418), LeanNeXt-s5 (+2.196), HyReX+dec. capacity (+2.157), LeanSep (+2.138), ResEnc-matched (+2.070), LeanDeepMid+FD (+2.046), LeanAdd (+2.042), ResEnc+context (+2.003), HyReX-LeanDec (+1.922), HyReX (+1.850), LeanDec (+1.648), StackDec (+1.634), LeanDil (+1.595), Stem1 (+1.487), HyReX-k9 (+1.461), HyReX+context (+1.348), HyReX point-fuse (+1.233), LeanAdd-NeXt (+1.205), LeanTrunk (+1.131), CoarseStack (+1.005), fn.-identical control (+0.932), branch control (+0.823), HyReX, finer ConvNeXt (+0.326)}
\expandafter\gdef\csname R@an.process.funnel.trained\endcsname{38}
\expandafter\gdef\csname R@an.process.funnel.trained.agent\endcsname{25}
\expandafter\gdef\csname R@an.process.funnel.trained.ctl\endcsname{13}
\expandafter\gdef\csname R@an.process.funnel.unknown_tag_names\endcsname{P2a\_aps, P2c\_fixed}
\expandafter\gdef\csname R@an.process.funnel.unknown_tags\endcsname{2}
\expandafter\gdef\csname R@an.process.funnel.wave_briefs\endcsname{4}
\expandafter\gdef\csname R@an.process.gpuh.acdc_guard\endcsname{314}
\expandafter\gdef\csname R@an.process.gpuh.acdc_guard.n\endcsname{11}
\expandafter\gdef\csname R@an.process.gpuh.acdc_guard.proj\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.acdc_guard.used\endcsname{157}
\expandafter\gdef\csname R@an.process.gpuh.attribution\endcsname{165}
\expandafter\gdef\csname R@an.process.gpuh.attribution.n\endcsname{6}
\expandafter\gdef\csname R@an.process.gpuh.attribution.proj\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.attribution.used\endcsname{80}
\expandafter\gdef\csname R@an.process.gpuh.base_sens\endcsname{247}
\expandafter\gdef\csname R@an.process.gpuh.base_sens.n\endcsname{21}
\expandafter\gdef\csname R@an.process.gpuh.base_sens.proj\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.base_sens.used\endcsname{120}
\expandafter\gdef\csname R@an.process.gpuh.basis_epochs\endcsname{1000}
\expandafter\gdef\csname R@an.process.gpuh.basis_gpus\endcsname{2}
\expandafter\gdef\csname R@an.process.gpuh.basis_n\endcsname{351}
\expandafter\gdef\csname R@an.process.gpuh.control\endcsname{388}
\expandafter\gdef\csname R@an.process.gpuh.control.n\endcsname{72}
\expandafter\gdef\csname R@an.process.gpuh.control.proj\endcsname{1115}
\expandafter\gdef\csname R@an.process.gpuh.control.used\endcsname{188}
\expandafter\gdef\csname R@an.process.gpuh.cv\endcsname{3378}
\expandafter\gdef\csname R@an.process.gpuh.cv.n\endcsname{332}
\expandafter\gdef\csname R@an.process.gpuh.cv.proj\endcsname{3993}
\expandafter\gdef\csname R@an.process.gpuh.cv.used\endcsname{1657}
\expandafter\gdef\csname R@an.process.gpuh.days_per_survived\endcsname{7.5}
\expandafter\gdef\csname R@an.process.gpuh.days_per_survived_agent\endcsname{9.0}
\expandafter\gdef\csname R@an.process.gpuh.earlier\endcsname{349}
\expandafter\gdef\csname R@an.process.gpuh.earlier.n\endcsname{54}
\expandafter\gdef\csname R@an.process.gpuh.earlier.proj\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.earlier.used\endcsname{339}
\expandafter\gdef\csname R@an.process.gpuh.efficiency\endcsname{52}
\expandafter\gdef\csname R@an.process.gpuh.fresh\endcsname{1693}
\expandafter\gdef\csname R@an.process.gpuh.fresh.n\endcsname{78}
\expandafter\gdef\csname R@an.process.gpuh.fresh.proj\endcsname{107}
\expandafter\gdef\csname R@an.process.gpuh.fresh.used\endcsname{825}
\expandafter\gdef\csname R@an.process.gpuh.heldout\endcsname{647}
\expandafter\gdef\csname R@an.process.gpuh.heldout.n\endcsname{117}
\expandafter\gdef\csname R@an.process.gpuh.heldout.proj\endcsname{1941}
\expandafter\gdef\csname R@an.process.gpuh.heldout.used\endcsname{322}
\expandafter\gdef\csname R@an.process.gpuh.inherited\endcsname{566}
\expandafter\gdef\csname R@an.process.gpuh.inherited_efficiency\endcsname{98}
\expandafter\gdef\csname R@an.process.gpuh.inherited_used\endcsname{553}
\expandafter\gdef\csname R@an.process.gpuh.judging\endcsname{4338}
\expandafter\gdef\csname R@an.process.gpuh.judging_cats\endcsname{discovery screens, ACDC guard runs, fresh-seed replication, matched controls, reference designs, attribution arms, the frozen KiTS23 default pool, and default-baseline sensitivity runs}
\expandafter\gdef\csname R@an.process.gpuh.judging_efficiency\endcsname{49}
\expandafter\gdef\csname R@an.process.gpuh.judging_failed\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.judging_runs\endcsname{181}
\expandafter\gdef\csname R@an.process.gpuh.judging_used\endcsname{2115}
\expandafter\gdef\csname R@an.process.gpuh.kits_pool\endcsname{55}
\expandafter\gdef\csname R@an.process.gpuh.kits_pool.n\endcsname{3}
\expandafter\gdef\csname R@an.process.gpuh.kits_pool.proj\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.kits_pool.used\endcsname{27}
\expandafter\gdef\csname R@an.process.gpuh.measurement\endcsname{61}
\expandafter\gdef\csname R@an.process.gpuh.measurement.ckpt.done\endcsname{54}
\expandafter\gdef\csname R@an.process.gpuh.measurement.ckpt.failed\endcsname{1}
\expandafter\gdef\csname R@an.process.gpuh.measurement.ckpt.hours\endcsname{59}
\expandafter\gdef\csname R@an.process.gpuh.measurement.ckpt.n\endcsname{55}
\expandafter\gdef\csname R@an.process.gpuh.measurement.ckpt.queued\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.ckpt.running\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.ckpt.unqueued\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.cost.done\endcsname{28}
\expandafter\gdef\csname R@an.process.gpuh.measurement.cost.failed\endcsname{4}
\expandafter\gdef\csname R@an.process.gpuh.measurement.cost.hours\endcsname{2.0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.cost.n\endcsname{32}
\expandafter\gdef\csname R@an.process.gpuh.measurement.cost.queued\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.cost.running\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.cost.unqueued\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.done\endcsname{91}
\expandafter\gdef\csname R@an.process.gpuh.measurement.early.done\endcsname{3}
\expandafter\gdef\csname R@an.process.gpuh.measurement.early.failed\endcsname{1}
\expandafter\gdef\csname R@an.process.gpuh.measurement.early.hours\endcsname{0.19}
\expandafter\gdef\csname R@an.process.gpuh.measurement.early.n\endcsname{4}
\expandafter\gdef\csname R@an.process.gpuh.measurement.early.queued\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.early.running\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.early.unqueued\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.failed\endcsname{5}
\expandafter\gdef\csname R@an.process.gpuh.measurement.n\endcsname{96}
\expandafter\gdef\csname R@an.process.gpuh.measurement.other.done\endcsname{9}
\expandafter\gdef\csname R@an.process.gpuh.measurement.other.failed\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.other.hours\endcsname{0.25}
\expandafter\gdef\csname R@an.process.gpuh.measurement.other.n\endcsname{9}
\expandafter\gdef\csname R@an.process.gpuh.measurement.other.queued\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.other.running\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.other.unqueued\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.plan_gpus\endcsname{1}
\expandafter\gdef\csname R@an.process.gpuh.measurement.plan_hours\endcsname{36}
\expandafter\gdef\csname R@an.process.gpuh.measurement.plan_jobs\endcsname{36}
\expandafter\gdef\csname R@an.process.gpuh.measurement.prog.done\endcsname{51}
\expandafter\gdef\csname R@an.process.gpuh.measurement.prog.failed\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.prog.hours\endcsname{59}
\expandafter\gdef\csname R@an.process.gpuh.measurement.prog.n\endcsname{51}
\expandafter\gdef\csname R@an.process.gpuh.measurement.prog.queued\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.prog.running\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.prog.unqueued\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.prog_clause\endcsname{51 checkpoint-measurement jobs have been submitted, 15 more than the plan lists (51 finished, 0 running, and 0 queued)}
\expandafter\gdef\csname R@an.process.gpuh.measurement.proj\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.queued\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.running\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.unqueued\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.measurement.used\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.other_budget.budgets\endcsname{1500 epochs on 2 GPUs}
\expandafter\gdef\csname R@an.process.gpuh.other_budget.clause\endcsname{9 queued runs are at another budget (1500 epochs on 2 GPUs), where no run has finished, and carry no projection}
\expandafter\gdef\csname R@an.process.gpuh.other_budget.runs\endcsname{9}
\expandafter\gdef\csname R@an.process.gpuh.other_finished\endcsname{4088}
\expandafter\gdef\csname R@an.process.gpuh.ours\endcsname{8426}
\expandafter\gdef\csname R@an.process.gpuh.ours_efficiency\endcsname{49}
\expandafter\gdef\csname R@an.process.gpuh.ours_used\endcsname{4094}
\expandafter\gdef\csname R@an.process.gpuh.pending_by_all\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.pending_by_ds\endcsname{333}
\expandafter\gdef\csname R@an.process.gpuh.pending_by_other\endcsname{9}
\expandafter\gdef\csname R@an.process.gpuh.pending_proj\endcsname{7517}
\expandafter\gdef\csname R@an.process.gpuh.pending_runs\endcsname{333}
\expandafter\gdef\csname R@an.process.gpuh.pending_used_proj\endcsname{3698}
\expandafter\gdef\csname R@an.process.gpuh.per_arm_trained\endcsname{114}
\expandafter\gdef\csname R@an.process.gpuh.per_decided_screen\endcsname{136}
\expandafter\gdef\csname R@an.process.gpuh.per_decided_screen_used\endcsname{66}
\expandafter\gdef\csname R@an.process.gpuh.per_survived\endcsname{181}
\expandafter\gdef\csname R@an.process.gpuh.profiling\endcsname{1.4}
\expandafter\gdef\csname R@an.process.gpuh.profiling.n\endcsname{135}
\expandafter\gdef\csname R@an.process.gpuh.profiling.proj\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.profiling.used\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.randsearch\endcsname{pending}
\expandafter\gdef\csname R@an.process.gpuh.randsearch.n\endcsname{20}
\expandafter\gdef\csname R@an.process.gpuh.randsearch.proj\endcsname{80}
\expandafter\gdef\csname R@an.process.gpuh.randsearch.used\endcsname{pending}
\expandafter\gdef\csname R@an.process.gpuh.reference\endcsname{128}
\expandafter\gdef\csname R@an.process.gpuh.reference.n\endcsname{4}
\expandafter\gdef\csname R@an.process.gpuh.reference.proj\endcsname{19}
\expandafter\gdef\csname R@an.process.gpuh.reference.used\endcsname{63}
\expandafter\gdef\csname R@an.process.gpuh.reused_pool\endcsname{217}
\expandafter\gdef\csname R@an.process.gpuh.reused_pool.n\endcsname{12}
\expandafter\gdef\csname R@an.process.gpuh.reused_pool.proj\endcsname{0}
\expandafter\gdef\csname R@an.process.gpuh.reused_pool.used\endcsname{214}
\expandafter\gdef\csname R@an.process.gpuh.running_alloc\endcsname{147}
\expandafter\gdef\csname R@an.process.gpuh.running_runs\endcsname{24}
\expandafter\gdef\csname R@an.process.gpuh.running_used\endcsname{72}
\expandafter\gdef\csname R@an.process.gpuh.scaled_llm\endcsname{pending}
\expandafter\gdef\csname R@an.process.gpuh.scaled_llm.n\endcsname{8}
\expandafter\gdef\csname R@an.process.gpuh.scaled_llm.proj\endcsname{144}
\expandafter\gdef\csname R@an.process.gpuh.scaled_llm.used\endcsname{pending}
\expandafter\gdef\csname R@an.process.gpuh.screen\endcsname{1350}
\expandafter\gdef\csname R@an.process.gpuh.screen.n\endcsname{58}
\expandafter\gdef\csname R@an.process.gpuh.screen.proj\endcsname{117}
\expandafter\gdef\csname R@an.process.gpuh.screen.used\endcsname{656}
\expandafter\gdef\csname R@an.process.gpuh.total_alloc\endcsname{8992}
\expandafter\gdef\csname R@an.process.gpuh.total_used\endcsname{4647}
\expandafter\gdef\csname R@an.process.queue.dir.done\endcsname{656}
\expandafter\gdef\csname R@an.process.queue.dir.pending\endcsname{342}
\expandafter\gdef\csname R@an.process.queue.dir.running\endcsname{24}
\expandafter\gdef\csname R@an.process.queue.failed\endcsname{18}
\expandafter\gdef\csname R@an.process.queue.queued.acdc_guard\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.queued.attribution\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.queued.base_sens\endcsname{9}
\expandafter\gdef\csname R@an.process.queue.queued.control\endcsname{53}
\expandafter\gdef\csname R@an.process.queue.queued.cv\endcsname{179}
\expandafter\gdef\csname R@an.process.queue.queued.earlier\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.queued.fresh\endcsname{4}
\expandafter\gdef\csname R@an.process.queue.queued.heldout\endcsname{82}
\expandafter\gdef\csname R@an.process.queue.queued.kits_pool\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.queued.measurement\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.queued.profiling\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.queued.randsearch\endcsname{3}
\expandafter\gdef\csname R@an.process.queue.queued.reference\endcsname{1}
\expandafter\gdef\csname R@an.process.queue.queued.reused_pool\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.queued.scaled_llm\endcsname{6}
\expandafter\gdef\csname R@an.process.queue.queued.screen\endcsname{5}
\expandafter\gdef\csname R@an.process.queue.running.acdc_guard\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.running.attribution\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.running.base_sens\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.running.control\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.running.cv\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.running.earlier\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.running.fresh\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.running.heldout\endcsname{5}
\expandafter\gdef\csname R@an.process.queue.running.kits_pool\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.running.measurement\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.running.profiling\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.running.randsearch\endcsname{17}
\expandafter\gdef\csname R@an.process.queue.running.reference\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.running.reused_pool\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.running.scaled_llm\endcsname{2}
\expandafter\gdef\csname R@an.process.queue.running.screen\endcsname{0}
\expandafter\gdef\csname R@an.process.queue.submitted\endcsname{961}
\expandafter\gdef\csname R@an.process.queue.unqueued\endcsname{3}
\expandafter\gdef\csname R@an.process.queue.withdrawn\endcsname{6}
\expandafter\gdef\csname R@an.process.reg.addendumo.of\endcsname{65}
\expandafter\gdef\csname R@an.process.reg.addendumo.prior_results\endcsname{0}
\expandafter\gdef\csname R@an.process.reg.addendump.of\endcsname{332}
\expandafter\gdef\csname R@an.process.reg.addendump.prior_results\endcsname{0}
\expandafter\gdef\csname R@an.process.reg.docs\endcsname{52}
\expandafter\gdef\csname R@an.process.reg.docs_clause\endcsname{are byte-identical to their last ledger entry}
\expandafter\gdef\csname R@an.process.reg.drift\endcsname{0}
\expandafter\gdef\csname R@an.process.reg.drift_names\endcsname{none}
\expandafter\gdef\csname R@an.process.reg.files\endcsname{4}
\expandafter\gdef\csname R@an.process.reg.files_names\endcsname{Wave 2, Wave 3, Addendum O, and Addendum P}
\expandafter\gdef\csname R@an.process.reg.identical\endcsname{52}
\expandafter\gdef\csname R@an.process.reg.identical_claim\endcsname{the 52 registration documents on disk are byte-identical to their last ledger entry}
\expandafter\gdef\csname R@an.process.reg.prior_results_total\endcsname{0}
\expandafter\gdef\csname R@an.process.reg.runs\endcsname{463}
\expandafter\gdef\csname R@an.process.reg.uncovered\endcsname{0}
\expandafter\gdef\csname R@an.process.reg.uncovered_names\endcsname{none}
\expandafter\gdef\csname R@an.process.reg.unledgered\endcsname{0}
\expandafter\gdef\csname R@an.process.reg.unledgered_names\endcsname{none}
\expandafter\gdef\csname R@an.process.reg.wave1.records\endcsname{11}
\expandafter\gdef\csname R@an.process.reg.wave1.snapshot_line\endcsname{2}
\expandafter\gdef\csname R@an.process.reg.wave1.started\endcsname{13}
\expandafter\gdef\csname R@an.process.reg.wave1.witness\endcsname{0}
\expandafter\gdef\csname R@an.process.reg.wave2.of\endcsname{11}
\expandafter\gdef\csname R@an.process.reg.wave2.prior_results\endcsname{0}
\expandafter\gdef\csname R@an.process.reg.wave3.of\endcsname{55}
\expandafter\gdef\csname R@an.process.reg.wave3.prior_results\endcsname{0}
\expandafter\gdef\csname R@an.process.runs.done\endcsname{363}
\expandafter\gdef\csname R@an.process.runs.full_budget\endcsname{742}
\expandafter\gdef\csname R@an.process.runs.pending\endcsname{342}
\expandafter\gdef\csname R@an.process.runs.profiling\endcsname{135}
\expandafter\gdef\csname R@an.process.runs.running\endcsname{24}
\expandafter\gdef\csname R@an.process.runs.withdrawn\endcsname{6}
\expandafter\gdef\csname R@an.process.safeguards.blocker\endcsname{6}
\expandafter\gdef\csname R@an.process.safeguards.by.build_check\endcsname{7}
\expandafter\gdef\csname R@an.process.safeguards.by.ideator\endcsname{2}
\expandafter\gdef\csname R@an.process.safeguards.by.independent_verifier\endcsname{5}
\expandafter\gdef\csname R@an.process.safeguards.by.other\endcsname{0}
\expandafter\gdef\csname R@an.process.safeguards.by.reviewer\endcsname{41}
\expandafter\gdef\csname R@an.process.safeguards.by.self_re_read\endcsname{30}
\expandafter\gdef\csname R@an.process.safeguards.by.writer\endcsname{8}
\expandafter\gdef\csname R@an.process.safeguards.caught_by_agent\endcsname{56}
\expandafter\gdef\csname R@an.process.safeguards.caught_by_check\endcsname{7}
\expandafter\gdef\csname R@an.process.safeguards.caught_by_other\endcsname{63}
\expandafter\gdef\csname R@an.process.safeguards.claim_wording_comparator.n\endcsname{17}
\expandafter\gdef\csname R@an.process.safeguards.code_correctness.n\endcsname{15}
\expandafter\gdef\csname R@an.process.safeguards.dispersion_across_regimes.n\endcsname{8}
\expandafter\gdef\csname R@an.process.safeguards.dispersion_rank\endcsname{6}
\expandafter\gdef\csname R@an.process.safeguards.dispersion_tied\endcsname{1}
\expandafter\gdef\csname R@an.process.safeguards.fail_open_guard.n\endcsname{6}
\expandafter\gdef\csname R@an.process.safeguards.items\endcsname{99}
\expandafter\gdef\csname R@an.process.safeguards.kappa.category\endcsname{pending}
\expandafter\gdef\csname R@an.process.safeguards.kappa.clause\endcsname{inter-coder agreement is reported once a second coder has coded all 99 items}
\expandafter\gdef\csname R@an.process.safeguards.kappa.detector\endcsname{pending}
\expandafter\gdef\csname R@an.process.safeguards.kappa.floor\endcsname{0.60}
\expandafter\gdef\csname R@an.process.safeguards.kappa.n\endcsname{0}
\expandafter\gdef\csname R@an.process.safeguards.kappa.of\endcsname{99}
\expandafter\gdef\csname R@an.process.safeguards.kappa.stage\endcsname{pending}
\expandafter\gdef\csname R@an.process.safeguards.kappa.state\endcsname{no second coder yet}
\expandafter\gdef\csname R@an.process.safeguards.manual_clauses\endcsname{33}
\expandafter\gdef\csname R@an.process.safeguards.manual_echoes\endcsname{6}
\expandafter\gdef\csname R@an.process.safeguards.n\endcsname{93}
\expandafter\gdef\csname R@an.process.safeguards.premise_refuted.n\endcsname{10}
\expandafter\gdef\csname R@an.process.safeguards.protocol_near_miss.n\endcsname{13}
\expandafter\gdef\csname R@an.process.safeguards.provenance_clock.n\endcsname{15}
\expandafter\gdef\csname R@an.process.safeguards.reached_pdf\endcsname{4}
\expandafter\gdef\csname R@an.process.safeguards.reached_pdf_clause\endcsname{4 reached a built PDF, 2 of them before the author's own re-read caught them and 2 before someone other than the author did}
\expandafter\gdef\csname R@an.process.safeguards.reached_pdf_detector\endcsname{reviewer, self re-read}
\expandafter\gdef\csname R@an.process.safeguards.reached_pdf_self\endcsname{2}
\expandafter\gdef\csname R@an.process.safeguards.run_condition_confound.n\endcsname{3}
\expandafter\gdef\csname R@an.process.safeguards.scope\endcsname{corrections C1-C66 and review-log rows 1-34}
\expandafter\gdef\csname R@an.process.safeguards.silent_tool_failure.n\endcsname{6}
\expandafter\gdef\csname R@an.process.safeguards.src.corrections\endcsname{65}
\expandafter\gdef\csname R@an.process.safeguards.src.review_log\endcsname{34}
\expandafter\gdef\csname R@an.process.safeguards.stage.macro\endcsname{10}
\expandafter\gdef\csname R@an.process.safeguards.stage.pdf\endcsname{4}
\expandafter\gdef\csname R@an.process.safeguards.stage.upstream\endcsname{79}
\expandafter\gdef\csname R@an.process.safeguards.top_category\endcsname{claim wording or comparator}
\expandafter\gdef\csname R@an.process.safeguards.top_category.n\endcsname{17}
\expandafter\gdef\csname R@an.process.safeguards.top_category_key\endcsname{claim_wording_comparator}
\expandafter\gdef\csname R@an.process.safeguards.top_margin\endcsname{2}
\expandafter\gdef\csname R@an.process.safeguards.top_runner_up\endcsname{code correctness}
\expandafter\gdef\csname R@an.process.safeguards.uncoded\endcsname{1}
\expandafter\gdef\csname R@an.process.safeguards.verifications\endcsname{6}
\expandafter\gdef\csname R@an.process.safeguards.would_reach_pdf\endcsname{55}
\expandafter\gdef\csname R@an.process.screen_vs_rep.arm\endcsname{HyReX}
\expandafter\gdef\csname R@an.process.screen_vs_rep.arms_adjudicable\endcsname{4}
\expandafter\gdef\csname R@an.process.screen_vs_rep.arms_below_bar\endcsname{2}
\expandafter\gdef\csname R@an.process.screen_vs_rep.arms_fired\endcsname{11}
\expandafter\gdef\csname R@an.process.screen_vs_rep.bar\endcsname{+0.35}
\expandafter\gdef\csname R@an.process.screen_vs_rep.below_phrase\endcsname{2 of those 4 sit below the bar their discovery seed cleared}
\expandafter\gdef\csname R@an.process.screen_vs_rep.controls\endcsname{1}
\expandafter\gdef\csname R@an.process.screen_vs_rep.controls_arms\endcsname{ResEnc-matched}
\expandafter\gdef\csname R@an.process.screen_vs_rep.d0\endcsname{+0.382}
\expandafter\gdef\csname R@an.process.screen_vs_rep.dfresh\endcsname{+0.132}
\expandafter\gdef\csname R@an.process.screen_vs_rep.dfresh_unc\endcsname{+0.104}
\expandafter\gdef\csname R@an.process.screen_vs_rep.ds\endcsname{AMOS22}
\expandafter\gdef\csname R@an.process.screen_vs_rep.fresh_n\endcsname{2}
\expandafter\gdef\csname R@an.process.screen_vs_rep.lead_arm\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.process.screen_vs_rep.lead_dfresh\endcsname{+0.465}
\expandafter\gdef\csname R@an.process.screen_vs_rep.margin0\endcsname{0.032}
\expandafter\gdef\csname R@an.process.screen_vs_rep.pair_sd\endcsname{0.209}
\expandafter\gdef\csname R@an.process.screen_vs_rep.se_mean\endcsname{0.148}
\expandafter\gdef\csname R@an.process.screen_vs_rep.sep_clause\endcsname{among the screen-fired arms, AMOS22 separates +0.465 pp (ResEnc-M) and +0.455 pp (ResEnc+context) from the frozen pool and does not separate +0.194 pp (ConvNeXt-k3) or +0.132 pp (HyReX)}
\expandafter\gdef\csname R@an.process.screen_vs_rep.sep_list\endcsname{+0.465 pp (ResEnc-M) and +0.455 pp (ResEnc+context)}
\expandafter\gdef\csname R@an.process.screen_vs_rep.sep_min\endcsname{+0.455}
\expandafter\gdef\csname R@an.process.screen_vs_rep.sep_min_arm\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.process.screen_vs_rep.sep_n\endcsname{2}
\expandafter\gdef\csname R@an.process.screen_vs_rep.shortfall\endcsname{0.218}
\expandafter\gdef\csname R@an.process.screen_vs_rep.spread\endcsname{0.296}
\expandafter\gdef\csname R@an.process.screen_vs_rep.state\endcsname{does not reproduce the margin it was selected on and is not separated from the frozen pool at 2 fresh seeds}
\expandafter\gdef\csname R@an.process.screen_vs_rep.unc_label\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.process.screen_vs_rep.unc_n\endcsname{3}
\expandafter\gdef\csname R@an.process.screen_vs_rep.unsep_list\endcsname{+0.194 pp (ConvNeXt-k3) and +0.132 pp (HyReX)}
\expandafter\gdef\csname R@an.process.screen_vs_rep.unsep_n\endcsname{2}
\expandafter\gdef\csname R@an.process.screen_vs_rep.wait_list\endcsname{none}
\expandafter\gdef\csname R@an.process.screen_vs_rep.wait_n\endcsname{0}
\expandafter\gdef\csname R@an.process.searchcost.controls.gpudays\endcsname{20.3}
\expandafter\gdef\csname R@an.process.searchcost.controls.gpuh\endcsname{488}
\expandafter\gdef\csname R@an.process.searchcost.controls.gpuh.used\endcsname{238}
\expandafter\gdef\csname R@an.process.searchcost.controls.n\endcsname{17}
\expandafter\gdef\csname R@an.process.searchcost.efficiency\endcsname{49}
\expandafter\gdef\csname R@an.process.searchcost.gpudays\endcsname{140}
\expandafter\gdef\csname R@an.process.searchcost.gpudays.used\endcsname{68}
\expandafter\gdef\csname R@an.process.searchcost.gpuh\endcsname{3357}
\expandafter\gdef\csname R@an.process.searchcost.gpuh.used\endcsname{1638}
\expandafter\gdef\csname R@an.process.searchcost.ndesigns\endcsname{28}
\expandafter\gdef\csname R@an.process.searchcost.nruns\endcsname{138}
\expandafter\gdef\csname R@an.process.searchcost.nwaves\endcsname{8}
\expandafter\gdef\csname R@an.process.searchcost.profile.gpudays\endcsname{0.0}
\expandafter\gdef\csname R@an.process.searchcost.profile.gpuh\endcsname{0.5}
\expandafter\gdef\csname R@an.process.searchcost.profile.gpuh.used\endcsname{0}
\expandafter\gdef\csname R@an.process.searchcost.profile.n\endcsname{48}
\expandafter\gdef\csname R@an.process.searchcost.ref.c2fnas.gpudays\endcsname{333}
\expandafter\gdef\csname R@an.process.searchcost.ref.c2fnas.name\endcsname{C2FNAS}
\expandafter\gdef\csname R@an.process.searchcost.ref.dints.gpudays\endcsname{5.8}
\expandafter\gdef\csname R@an.process.searchcost.ref.dints.name\endcsname{DiNTS}
\expandafter\gdef\csname R@an.process.searchcost.replication.gpudays\endcsname{70.5}
\expandafter\gdef\csname R@an.process.searchcost.replication.gpuh\endcsname{1693}
\expandafter\gdef\csname R@an.process.searchcost.replication.gpuh.used\endcsname{825}
\expandafter\gdef\csname R@an.process.searchcost.replication.n\endcsname{74}
\expandafter\gdef\csname R@an.process.searchcost.running.gpuh\endcsname{0}
\expandafter\gdef\csname R@an.process.searchcost.running.n\endcsname{0}
\expandafter\gdef\csname R@an.process.searchcost.screen.gpudays\endcsname{69.3}
\expandafter\gdef\csname R@an.process.searchcost.screen.gpuh\endcsname{1663}
\expandafter\gdef\csname R@an.process.searchcost.screen.gpuh.used\endcsname{813}
\expandafter\gdef\csname R@an.process.searchcost.screen.n\endcsname{64}
\expandafter\gdef\csname R@an.process.searchcost.sentence\endcsname{the agents' design loop trained 28 designs over 8 waves (138 finished training runs: discovery screens, ACDC guard runs and fresh-seed replications, plus the profiling jobs) for 140 GPU-days as allocated by the cluster, 68 GPU-days of training on the one device the network uses; DiNTS reports 5.8 GPU-days for its search and 333 GPU-days for C2FNAS}
\expandafter\gdef\csname R@an.process.searchcost.wave0.gpudays\endcsname{0.0}
\expandafter\gdef\csname R@an.process.searchcost.wave0.gpuh\endcsname{0}
\expandafter\gdef\csname R@an.process.searchcost.wave0.gpuh.used\endcsname{0}
\expandafter\gdef\csname R@an.process.searchcost.wave0.ndesigns\endcsname{0}
\expandafter\gdef\csname R@an.process.searchcost.wave0.nruns\endcsname{0}
\expandafter\gdef\csname R@an.process.searchcost.wave1.gpudays\endcsname{51.1}
\expandafter\gdef\csname R@an.process.searchcost.wave1.gpuh\endcsname{1227}
\expandafter\gdef\csname R@an.process.searchcost.wave1.gpuh.used\endcsname{602}
\expandafter\gdef\csname R@an.process.searchcost.wave1.ndesigns\endcsname{4}
\expandafter\gdef\csname R@an.process.searchcost.wave1.nruns\endcsname{42}
\expandafter\gdef\csname R@an.process.searchcost.wave2.gpudays\endcsname{4.8}
\expandafter\gdef\csname R@an.process.searchcost.wave2.gpuh\endcsname{116}
\expandafter\gdef\csname R@an.process.searchcost.wave2.gpuh.used\endcsname{57}
\expandafter\gdef\csname R@an.process.searchcost.wave2.ndesigns\endcsname{3}
\expandafter\gdef\csname R@an.process.searchcost.wave2.nruns\endcsname{5}
\expandafter\gdef\csname R@an.process.searchcost.wave3.gpudays\endcsname{8.1}
\expandafter\gdef\csname R@an.process.searchcost.wave3.gpuh\endcsname{195}
\expandafter\gdef\csname R@an.process.searchcost.wave3.gpuh.used\endcsname{95}
\expandafter\gdef\csname R@an.process.searchcost.wave3.ndesigns\endcsname{0}
\expandafter\gdef\csname R@an.process.searchcost.wave3.nruns\endcsname{10}
\expandafter\gdef\csname R@an.process.searchcost.wave4.gpudays\endcsname{21.8}
\expandafter\gdef\csname R@an.process.searchcost.wave4.gpuh\endcsname{524}
\expandafter\gdef\csname R@an.process.searchcost.wave4.gpuh.used\endcsname{254}
\expandafter\gdef\csname R@an.process.searchcost.wave4.ndesigns\endcsname{5}
\expandafter\gdef\csname R@an.process.searchcost.wave4.nruns\endcsname{18}
\expandafter\gdef\csname R@an.process.searchcost.wave5.gpudays\endcsname{11.0}
\expandafter\gdef\csname R@an.process.searchcost.wave5.gpuh\endcsname{263}
\expandafter\gdef\csname R@an.process.searchcost.wave5.gpuh.used\endcsname{128}
\expandafter\gdef\csname R@an.process.searchcost.wave5.ndesigns\endcsname{3}
\expandafter\gdef\csname R@an.process.searchcost.wave5.nruns\endcsname{13}
\expandafter\gdef\csname R@an.process.searchcost.wave6.gpudays\endcsname{6.3}
\expandafter\gdef\csname R@an.process.searchcost.wave6.gpuh\endcsname{152}
\expandafter\gdef\csname R@an.process.searchcost.wave6.gpuh.used\endcsname{74}
\expandafter\gdef\csname R@an.process.searchcost.wave6.ndesigns\endcsname{1}
\expandafter\gdef\csname R@an.process.searchcost.wave6.nruns\endcsname{5}
\expandafter\gdef\csname R@an.process.searchcost.wave7.gpudays\endcsname{22.5}
\expandafter\gdef\csname R@an.process.searchcost.wave7.gpuh\endcsname{539}
\expandafter\gdef\csname R@an.process.searchcost.wave7.gpuh.used\endcsname{263}
\expandafter\gdef\csname R@an.process.searchcost.wave7.ndesigns\endcsname{7}
\expandafter\gdef\csname R@an.process.searchcost.wave7.nruns\endcsname{27}
\expandafter\gdef\csname R@an.process.searchcost.wave8.gpudays\endcsname{14.2}
\expandafter\gdef\csname R@an.process.searchcost.wave8.gpuh\endcsname{340}
\expandafter\gdef\csname R@an.process.searchcost.wave8.gpuh.used\endcsname{165}
\expandafter\gdef\csname R@an.process.searchcost.wave8.ndesigns\endcsname{5}
\expandafter\gdef\csname R@an.process.searchcost.wave8.nruns\endcsname{18}
\expandafter\gdef\csname R@an.process.searchcost.withcontrols.gpudays\endcsname{160}
\expandafter\gdef\csname R@an.process.searchcost.withcontrols.gpuh\endcsname{3845}
\expandafter\gdef\csname R@an.process.stage.cap_gb\endcsname{12}
\expandafter\gdef\csname R@an.process.stage.guard_pass\endcsname{89}
\expandafter\gdef\csname R@an.process.stage.n_registered\endcsname{75}
\expandafter\gdef\csname R@an.process.stage.pair_pass_amos\endcsname{3}
\expandafter\gdef\csname R@an.process.stage.pair_pass_kits\endcsname{70}
\expandafter\gdef\csname R@an.process.timeline.campaign_days\endcsname{9.8}
\expandafter\gdef\csname R@an.process.timeline.campaign_hours\endcsname{234}
\expandafter\gdef\csname R@an.process.timeline.campaign_runs\endcsname{451}
\expandafter\gdef\csname R@an.process.timeline.pool_gpuh\endcsname{272}
\expandafter\gdef\csname R@an.process.timeline.pool_runs\endcsname{15}
\expandafter\gdef\csname R@an.process.timeline.pools_before_break\endcsname{3}
\expandafter\gdef\csname R@an.process.timeline.pools_in_campaign\endcsname{12}
\expandafter\gdef\csname R@an.process.timeline.record_hours\endcsname{369}
\expandafter\gdef\csname R@an.provenance.D2.cites\endcsname{nnU-Net Revisited; MedNeXt}
\expandafter\gdef\csname R@an.provenance.D2.cites.n\endcsname{2}
\expandafter\gdef\csname R@an.provenance.D2.cites.written\endcsname{nnU-Net Revisited; MedNeXt}
\expandafter\gdef\csname R@an.provenance.D2.fact\endcsname{no REVIEW\_*.md note covers it (reviews/ holds the check scripts rev\_v3\_decoder\_head\_check.py and chk8\_v3\_decoder\_head.py for the round-3 decoder lens)}
\expandafter\gdef\csname R@an.provenance.D2.idea\endcsname{D2\_dec1 --- Dec1: the missing cell of the ResEnc factorisation, and the only arm in the study that is cheaper than the default (IDEAS\_v3\_decoder\_head.md, line 184)}
\expandafter\gdef\csname R@an.provenance.D2.idea.file\endcsname{IDEAS\_v3\_decoder\_head.md}
\expandafter\gdef\csname R@an.provenance.D2.idea.id\endcsname{D2\_dec1}
\expandafter\gdef\csname R@an.provenance.D2.idea.line\endcsname{184}
\expandafter\gdef\csname R@an.provenance.D2.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.provenance.D2.premise\endcsname{``The nnU-Net default really does use two convolutions per decoder stage while the ResEnc presets use one, so ``decoder depth'' is an un-ablated factor inside the preset comparison this study's baselines are built on --- if both used the same decoder depth, D2 would only be an arbitrary shrink.'' (IDEAS\_v3\_decoder\_head.md, line 250)}
\expandafter\gdef\csname R@an.provenance.D2.premise.file\endcsname{IDEAS\_v3\_decoder\_head.md}
\expandafter\gdef\csname R@an.provenance.D2.premise.line\endcsname{250}
\expandafter\gdef\csname R@an.provenance.D2.premise.settled\endcsname{Premise holds. \ldots{}}
\expandafter\gdef\csname R@an.provenance.D2.premise.settled.line\endcsname{260}
\expandafter\gdef\csname R@an.provenance.D2.premise.text\endcsname{The nnU-Net default really does use two convolutions per decoder stage while the ResEnc presets use one, so ``decoder depth'' is an un-ablated factor inside the preset comparison this study's baselines are built on --- if both used the same decoder depth, D2 would only be an arbitrary shrink.}
\expandafter\gdef\csname R@an.provenance.D2.premise.verdict\endcsname{holds}
\expandafter\gdef\csname R@an.provenance.D2.reason\endcsname{The decoder holds most of nnU-Net's parameters, and almost all of them sit at two stages that see 0.4 \% of the voxels.}
\expandafter\gdef\csname R@an.provenance.D2.reason.cell\endcsname{The decoder holds most of nnU-Net's parameters, and almost all of them sit at two stages that see 0.4 \% \ldots{}}
\expandafter\gdef\csname R@an.provenance.D2.reason.file\endcsname{IDEAS\_v3\_decoder\_head.md}
\expandafter\gdef\csname R@an.provenance.D2.reason.kind\endcsname{sentence}
\expandafter\gdef\csname R@an.provenance.D2.reason.line\endcsname{17}
\expandafter\gdef\csname R@an.provenance.D2.reason.number\endcsname{yes}
\expandafter\gdef\csname R@an.provenance.D2.state\endcsname{found}
\expandafter\gdef\csname R@an.provenance.D2.wave\endcsname{4}
\expandafter\gdef\csname R@an.provenance.L3.cites\endcsname{MedNeXt; ConvNeXt (IDEAS\_v1.md, line 24: ``ConvNeXt micro-architecture is covered by wave-1 L2/L3'', the MedNeXt row)}
\expandafter\gdef\csname R@an.provenance.L3.cites.n\endcsname{2}
\expandafter\gdef\csname R@an.provenance.L3.fact\endcsname{no REVIEW\_*.md note rules on it: it is an arm the ideators were given, not an ideator proposal}
\expandafter\gdef\csname R@an.provenance.L3.idea\endcsname{none: HyReX (L3) is an arm the ideators were given, not a proposal of an ideator document (the phrase ``wave-1 L3'' of IDEAS\_v3\_decoder\_head.md, line 87)}
\expandafter\gdef\csname R@an.provenance.L3.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.provenance.L3.premise\endcsname{none stated: not an ideator proposal}
\expandafter\gdef\csname R@an.provenance.L3.reason\endcsname{none stated: not an ideator proposal}
\expandafter\gdef\csname R@an.provenance.L3.state\endcsname{found}
\expandafter\gdef\csname R@an.provenance.L3.wave\endcsname{1}
\expandafter\gdef\csname R@an.provenance.V5B1.cites\endcsname{LinkNet; nnU-Net Revisited}
\expandafter\gdef\csname R@an.provenance.V5B1.cites.n\endcsname{2}
\expandafter\gdef\csname R@an.provenance.V5B1.cites.written\endcsname{S7 (LinkNet); S6}
\expandafter\gdef\csname R@an.provenance.V5B1.fact\endcsname{the reviewer's note REVIEW\_wave5\_20261008.md rules ACCEPT (line 220) and did not change it}
\expandafter\gdef\csname R@an.provenance.V5B1.fact.verdict\endcsname{ACCEPT}
\expandafter\gdef\csname R@an.provenance.V5B1.idea\endcsname{B1 --- LeanAdd: additive skip fusion at every decoder stage, on top of LeanDec (IDEAS\_v4\_wave5.md, line 227)}
\expandafter\gdef\csname R@an.provenance.V5B1.idea.file\endcsname{IDEAS\_v4\_wave5.md}
\expandafter\gdef\csname R@an.provenance.V5B1.idea.id\endcsname{B1}
\expandafter\gdef\csname R@an.provenance.V5B1.idea.line\endcsname{227}
\expandafter\gdef\csname R@an.provenance.V5B1.name\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.provenance.V5B1.premise\endcsname{``The upsampled tensor and the skip do not have the same number of channels, so they cannot be added.'' (IDEAS\_v4\_wave5.md, line 265)}
\expandafter\gdef\csname R@an.provenance.V5B1.premise.file\endcsname{IDEAS\_v4\_wave5.md}
\expandafter\gdef\csname R@an.provenance.V5B1.premise.line\endcsname{265}
\expandafter\gdef\csname R@an.provenance.V5B1.premise.settled\endcsname{Settled by \texttt{lib\_v2.py::PlanNet.\_\_init\_\_}: \texttt{ups.append(nn.ConvTranspose3d(widths[below], widths[skip], strides[below], strides[below], ...))} \ldots{}}
\expandafter\gdef\csname R@an.provenance.V5B1.premise.settled.line\endcsname{266}
\expandafter\gdef\csname R@an.provenance.V5B1.premise.text\endcsname{The upsampled tensor and the skip do not have the same number of channels, so they cannot be added.}
\expandafter\gdef\csname R@an.provenance.V5B1.premise.verdict\endcsname{found false}
\expandafter\gdef\csname R@an.provenance.V5B1.reason\endcsname{The whole point is margin: D2 passes T2 by 5 ms per plan, and a target met by 5 ms on a two-point profile is not a result anyone should want to defend.}
\expandafter\gdef\csname R@an.provenance.V5B1.reason.cell\endcsname{The whole point is margin: D2 passes T2 by 5 ms per plan, and a target met by 5 ms on a two-point profile \ldots{}}
\expandafter\gdef\csname R@an.provenance.V5B1.reason.file\endcsname{IDEAS\_v4\_wave5.md}
\expandafter\gdef\csname R@an.provenance.V5B1.reason.kind\endcsname{sentence}
\expandafter\gdef\csname R@an.provenance.V5B1.reason.line\endcsname{235}
\expandafter\gdef\csname R@an.provenance.V5B1.reason.number\endcsname{yes}
\expandafter\gdef\csname R@an.provenance.V5B1.state\endcsname{found}
\expandafter\gdef\csname R@an.provenance.V5B1.wave\endcsname{5}
\expandafter\gdef\csname R@an.provenance.V5B2.cites\endcsname{Scaling Up Your Kernels to 31x31; UniRepLKNet; MedNeXt; nnU-Net Revisited; LinkNet}
\expandafter\gdef\csname R@an.provenance.V5B2.cites.n\endcsname{5}
\expandafter\gdef\csname R@an.provenance.V5B2.cites.written\endcsname{S1; S2 (large depthwise kernels, see wide without going deep); S3 (MedNeXt: a fully ConvNeXt 3D encoder--decoder with residual ConvNeXt down-sampling blocks, in this domain); S6 (ConvNeXt variants are named in the state-of-the-art recipe); S7}
\expandafter\gdef\csname R@an.provenance.V5B2.fact\endcsname{the reviewer's note REVIEW\_wave5\_20261008.md rules ACCEPT (line 239) and did not change it}
\expandafter\gdef\csname R@an.provenance.V5B2.fact.verdict\endcsname{ACCEPT}
\expandafter\gdef\csname R@an.provenance.V5B2.idea\endcsname{B2 --- LeanAdd-NeXt: LeanAdd, with HyReX's coarse operator transplanted into the freed budget (IDEAS\_v4\_wave5.md, line 270)}
\expandafter\gdef\csname R@an.provenance.V5B2.idea.file\endcsname{IDEAS\_v4\_wave5.md}
\expandafter\gdef\csname R@an.provenance.V5B2.idea.id\endcsname{B2}
\expandafter\gdef\csname R@an.provenance.V5B2.idea.line\endcsname{270}
\expandafter\gdef\csname R@an.provenance.V5B2.name\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.provenance.V5B2.premise\endcsname{``A \texttt{next} stage cannot replace a strided plain stage, because \texttt{make\_stage} does not build a down-sampler for it.'' (IDEAS\_v4\_wave5.md, line 301)}
\expandafter\gdef\csname R@an.provenance.V5B2.premise.file\endcsname{IDEAS\_v4\_wave5.md}
\expandafter\gdef\csname R@an.provenance.V5B2.premise.line\endcsname{301}
\expandafter\gdef\csname R@an.provenance.V5B2.premise.settled\endcsname{Settled by \texttt{lib\_v2.py::make\_stage}, \texttt{next} branch: \texttt{if cin != cout or any(v != 1 for v in s): layers.append(CNA(ctx, cin, cout, kf, s))} --- the dense strided convolution is built first and the ConvNeXt \ldots{}}
\expandafter\gdef\csname R@an.provenance.V5B2.premise.settled.line\endcsname{302}
\expandafter\gdef\csname R@an.provenance.V5B2.premise.text\endcsname{A \texttt{next} stage cannot replace a strided plain stage, because \texttt{make\_stage} does not build a down-sampler for it.}
\expandafter\gdef\csname R@an.provenance.V5B2.premise.verdict\endcsname{found false}
\expandafter\gdef\csname R@an.provenance.V5B2.reason\endcsname{So the lean network gets the large-kernel coarse context that the study measured at 1.48 pp (\S{}0(a)) and keeps nearly all of the efficiency.}
\expandafter\gdef\csname R@an.provenance.V5B2.reason.cell\endcsname{So the lean network gets the large-kernel coarse context that the study measured at 1.48 pp (\S{}0(a)) and keeps \ldots{}}
\expandafter\gdef\csname R@an.provenance.V5B2.reason.file\endcsname{IDEAS\_v4\_wave5.md}
\expandafter\gdef\csname R@an.provenance.V5B2.reason.kind\endcsname{sentence}
\expandafter\gdef\csname R@an.provenance.V5B2.reason.line\endcsname{274}
\expandafter\gdef\csname R@an.provenance.V5B2.reason.number\endcsname{yes}
\expandafter\gdef\csname R@an.provenance.V5B2.state\endcsname{found}
\expandafter\gdef\csname R@an.provenance.V5B2.wave\endcsname{5}
\expandafter\gdef\csname R@an.provenance.V7A3.cites\endcsname{nnU-Net Revisited}
\expandafter\gdef\csname R@an.provenance.V7A3.cites.n\endcsname{1}
\expandafter\gdef\csname R@an.provenance.V7A3.cites.written\endcsname{S6}
\expandafter\gdef\csname R@an.provenance.V7A3.fact\endcsname{the reviewer's note REVIEW\_wave7\_20261009.md rules ACCEPT (line 396) and did not change it}
\expandafter\gdef\csname R@an.provenance.V7A3.fact.verdict\endcsname{ACCEPT}
\expandafter\gdef\csname R@an.provenance.V7A3.idea\endcsname{A3 --- V7A3 ``LeanAdd-NeXt-FullDec'': the exact inverse of the LeanDec factor, in the additive family (IDEAS\_v5\_wave7.md, line 195)}
\expandafter\gdef\csname R@an.provenance.V7A3.idea.file\endcsname{IDEAS\_v5\_wave7.md}
\expandafter\gdef\csname R@an.provenance.V7A3.idea.id\endcsname{A3}
\expandafter\gdef\csname R@an.provenance.V7A3.idea.line\endcsname{195}
\expandafter\gdef\csname R@an.provenance.V7A3.name\endcsname{FullDec}
\expandafter\gdef\csname R@an.provenance.V7A3.premise\endcsname{``Under \texttt{skipfuse='add'} the decoder's second convolution is not the same layer as in the default, so the measured default - D2 delta does not transfer.'' (IDEAS\_v5\_wave7.md, line 214)}
\expandafter\gdef\csname R@an.provenance.V7A3.premise.file\endcsname{IDEAS\_v5\_wave7.md}
\expandafter\gdef\csname R@an.provenance.V7A3.premise.line\endcsname{214}
\expandafter\gdef\csname R@an.provenance.V7A3.premise.settled\endcsname{Settled by \texttt{lib\_v2.py::make\_stage}, \texttt{plain} branch: \texttt{add(CNA(ctx, cin if i == 0 else cout, cout, k, stride if i == 0 else 1))} --- only the first convolution of a stage sees \texttt{cin}, so the second is \texttt{cout $\rightarrow$ cout} \ldots{}}
\expandafter\gdef\csname R@an.provenance.V7A3.premise.settled.line\endcsname{215}
\expandafter\gdef\csname R@an.provenance.V7A3.premise.text\endcsname{Under \texttt{skipfuse='add'} the decoder's second convolution is not the same layer as in the default, so the measured default - D2 delta does not transfer.}
\expandafter\gdef\csname R@an.provenance.V7A3.premise.verdict\endcsname{found false}
\expandafter\gdef\csname R@an.provenance.V7A3.reason\endcsname{It is the one-factor inverse of the D2 change, re-run in the additive family, and it lands at 0.845/0.842/0.845$\times$ the default's parameters with $\approx$ 1.03--1.11$\times$ its step.}
\expandafter\gdef\csname R@an.provenance.V7A3.reason.cell\endcsname{It is the one-factor inverse of the D2 change, re-run in the additive family, and it lands \ldots{}}
\expandafter\gdef\csname R@an.provenance.V7A3.reason.file\endcsname{IDEAS\_v5\_wave7.md}
\expandafter\gdef\csname R@an.provenance.V7A3.reason.kind\endcsname{sentence}
\expandafter\gdef\csname R@an.provenance.V7A3.reason.line\endcsname{198}
\expandafter\gdef\csname R@an.provenance.V7A3.reason.number\endcsname{no}
\expandafter\gdef\csname R@an.provenance.V7A3.state\endcsname{found}
\expandafter\gdef\csname R@an.provenance.V7A3.wave\endcsname{7}
\expandafter\gdef\csname R@an.provenance.V7B1.cites\endcsname{InceptionNeXt; More ConvNets in the 2020s; Scaling Up Your Kernels to 31x31}
\expandafter\gdef\csname R@an.provenance.V7B1.cites.n\endcsname{3}
\expandafter\gdef\csname R@an.provenance.V7B1.cites.written\endcsname{S2 (InceptionNeXt, CVPR 2024); S3 (SLaK); S1}
\expandafter\gdef\csname R@an.provenance.V7B1.fact\endcsname{the reviewer's note REVIEW\_wave7\_20261009.md rules ACCEPT WITH CHANGES (major); demote below B2/C2 (line 395) and changed it: (1) Correct \S{}0(c)(ii) and B1's premise: bench/op\_bench.py::Axial is a parallel cross-shaped 19-tap sum, not a separable rank-1 kernel; B1's ...}
\expandafter\gdef\csname R@an.provenance.V7B1.fact.verdict\endcsname{ACCEPT WITH CHANGES (major); demote below B2/C2}
\expandafter\gdef\csname R@an.provenance.V7B1.idea\endcsname{B1 --- V7B1 ``LeanSep'': the same receptive field, rank-1 (IDEAS\_v5\_wave7.md, line 263)}
\expandafter\gdef\csname R@an.provenance.V7B1.idea.file\endcsname{IDEAS\_v5\_wave7.md}
\expandafter\gdef\csname R@an.provenance.V7B1.idea.id\endcsname{B1}
\expandafter\gdef\csname R@an.provenance.V7B1.idea.line\endcsname{263}
\expandafter\gdef\csname R@an.provenance.V7B1.name\endcsname{LeanSep}
\expandafter\gdef\csname R@an.provenance.V7B1.premise\endcsname{``The depthwise convolution is not where the coarse operator's step time goes, so a cheaper depthwise buys nothing.'' (IDEAS\_v5\_wave7.md, line 301)}
\expandafter\gdef\csname R@an.provenance.V7B1.premise.file\endcsname{IDEAS\_v5\_wave7.md}
\expandafter\gdef\csname R@an.provenance.V7B1.premise.line\endcsname{301}
\expandafter\gdef\csname R@an.provenance.V7B1.premise.settled\endcsname{Settled without running anything from two files already on disk: \texttt{candidates/ai\_arch\_20261004/bench/op\_bench\_result.json}, rows \texttt{stage=s4, c=320, spatial=[8,12,10], fmt=cf} \ldots{}}
\expandafter\gdef\csname R@an.provenance.V7B1.premise.settled.line\endcsname{302}
\expandafter\gdef\csname R@an.provenance.V7B1.premise.text\endcsname{The depthwise convolution is not where the coarse operator's step time goes, so a cheaper depthwise buys nothing.}
\expandafter\gdef\csname R@an.provenance.V7B1.premise.verdict\endcsname{found false}
\expandafter\gdef\csname R@an.provenance.V7B1.reason\endcsname{The receptive field is identical --- every voxel within $\pm$3 on each axis still reaches the output --- and the only thing lost is the kernel's rank: 21 weights instead of 343, i.e. the operator can express exactly the outer-product (separable) part of what V5B2 learns.}
\expandafter\gdef\csname R@an.provenance.V7B1.reason.cell\endcsname{The receptive field is identical --- every voxel within $\pm$3 on each axis still reaches the output --- and the only \ldots{}}
\expandafter\gdef\csname R@an.provenance.V7B1.reason.file\endcsname{IDEAS\_v5\_wave7.md}
\expandafter\gdef\csname R@an.provenance.V7B1.reason.kind\endcsname{sentence}
\expandafter\gdef\csname R@an.provenance.V7B1.reason.line\endcsname{266}
\expandafter\gdef\csname R@an.provenance.V7B1.reason.number\endcsname{yes}
\expandafter\gdef\csname R@an.provenance.V7B1.state\endcsname{found}
\expandafter\gdef\csname R@an.provenance.V7B1.wave\endcsname{7}
\expandafter\gdef\csname R@an.provenance.V7B2.cites\endcsname{Visual attention network; Multi-Scale Context Aggregation by Dilated Convolutions}
\expandafter\gdef\csname R@an.provenance.V7B2.cites.n\endcsname{2}
\expandafter\gdef\csname R@an.provenance.V7B2.cites.written\endcsname{S4 (VAN, CVM 9(4):733--752); S5 (Yu and Koltun, ICLR 2016)}
\expandafter\gdef\csname R@an.provenance.V7B2.fact\endcsname{the reviewer's note REVIEW\_wave7\_20261009.md rules ACCEPT WITH CHANGES (line 393) and changed it: (1) Print VAN Table 3 ``w/o DW-Conv 74.9'' (vs VAN-B0 75.4) --- the row that describes B2 --- beside the ``w/o DW-D-Conv 74.1'' row. ...}
\expandafter\gdef\csname R@an.provenance.V7B2.fact.verdict\endcsname{ACCEPT WITH CHANGES}
\expandafter\gdef\csname R@an.provenance.V7B2.idea\endcsname{B2 --- V7B2 ``LeanDil'': the same receptive field, 27 taps, sampled (IDEAS\_v5\_wave7.md, line 312)}
\expandafter\gdef\csname R@an.provenance.V7B2.idea.file\endcsname{IDEAS\_v5\_wave7.md}
\expandafter\gdef\csname R@an.provenance.V7B2.idea.id\endcsname{B2}
\expandafter\gdef\csname R@an.provenance.V7B2.idea.line\endcsname{312}
\expandafter\gdef\csname R@an.provenance.V7B2.name\endcsname{LeanDil}
\expandafter\gdef\csname R@an.provenance.V7B2.premise\endcsname{``A depthwise convolution with dilation 3 and 3 taps does not reach a 7-voxel extent on these feature maps, because the padding clips it.'' (IDEAS\_v5\_wave7.md, line 346)}
\expandafter\gdef\csname R@an.provenance.V7B2.premise.file\endcsname{IDEAS\_v5\_wave7.md}
\expandafter\gdef\csname R@an.provenance.V7B2.premise.line\endcsname{346}
\expandafter\gdef\csname R@an.provenance.V7B2.premise.settled\endcsname{Settled by \texttt{lib\_v2.py::CNA}'s own dilation arithmetic (\texttt{dil = \_dil(k, dilation)}, \texttt{pad = tuple(d (kk // 2) for kk, d in zip(k, dil))}) --- padding scales with the dilation, so the output shape is preserved \ldots{}}
\expandafter\gdef\csname R@an.provenance.V7B2.premise.settled.line\endcsname{347}
\expandafter\gdef\csname R@an.provenance.V7B2.premise.text\endcsname{A depthwise convolution with dilation 3 and 3 taps does not reach a 7-voxel extent on these feature maps, because the padding clips it.}
\expandafter\gdef\csname R@an.provenance.V7B2.premise.verdict\endcsname{found false}
\expandafter\gdef\csname R@an.provenance.V7B2.reason\endcsname{Replace the \texttt{7$^3$} depthwise by a 3-tap-per-axis depthwise at dilation 3: the same extent (1 + 2$\cdot$3 = 7), the same 27 weights per channel as a plain \texttt{3$^3$}, and 8.6$\times$ cheaper than \texttt{dw7} at \texttt{s4} by measurement.}
\expandafter\gdef\csname R@an.provenance.V7B2.reason.cell\endcsname{Replace the \texttt{7$^3$} depthwise by a 3-tap-per-axis depthwise at dilation 3: the same extent (1 + 2$\cdot$3 = 7), the same \ldots{}}
\expandafter\gdef\csname R@an.provenance.V7B2.reason.file\endcsname{IDEAS\_v5\_wave7.md}
\expandafter\gdef\csname R@an.provenance.V7B2.reason.kind\endcsname{sentence}
\expandafter\gdef\csname R@an.provenance.V7B2.reason.line\endcsname{314}
\expandafter\gdef\csname R@an.provenance.V7B2.reason.number\endcsname{yes}
\expandafter\gdef\csname R@an.provenance.V7B2.state\endcsname{found}
\expandafter\gdef\csname R@an.provenance.V7B2.wave\endcsname{7}
\expandafter\gdef\csname R@an.provenance.V7C1.cites\endcsname{none stated}
\expandafter\gdef\csname R@an.provenance.V7C1.cites.n\endcsname{0}
\expandafter\gdef\csname R@an.provenance.V7C1.cites.written\endcsname{none stated}
\expandafter\gdef\csname R@an.provenance.V7C1.fact\endcsname{the reviewer's note REVIEW\_wave7\_20261009.md rules ACCEPT WITH CHANGES (line 391) and changed it: Add: the two stage terms are differences of single seeds whose sum is pinned to the measured +0.393 / -0.898, so neither term can be called ...}
\expandafter\gdef\csname R@an.provenance.V7C1.fact.verdict\endcsname{ACCEPT WITH CHANGES}
\expandafter\gdef\csname R@an.provenance.V7C1.idea\endcsname{C1 --- V7C1 ``LeanNeXt-s5'': which of the two encoder stages carries V5B2's change (IDEAS\_v5\_wave7.md, line 393)}
\expandafter\gdef\csname R@an.provenance.V7C1.idea.file\endcsname{IDEAS\_v5\_wave7.md}
\expandafter\gdef\csname R@an.provenance.V7C1.idea.id\endcsname{C1}
\expandafter\gdef\csname R@an.provenance.V7C1.idea.line\endcsname{393}
\expandafter\gdef\csname R@an.provenance.V7C1.name\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi}}
\expandafter\gdef\csname R@an.provenance.V7C1.premise\endcsname{``V5B2's two coarse stages cannot be separated in the spec.'' (IDEAS\_v5\_wave7.md, line 410)}
\expandafter\gdef\csname R@an.provenance.V7C1.premise.file\endcsname{IDEAS\_v5\_wave7.md}
\expandafter\gdef\csname R@an.provenance.V7C1.premise.line\endcsname{410}
\expandafter\gdef\csname R@an.provenance.V7C1.premise.settled\endcsname{Settled by \texttt{candidates/ai\_arch\_20261004/cand\_V5B2\_leanaddnext.py::Candidate.spec\_for}: \texttt{enc=[(``plain'', 2, \{\})] 4 + [g(4, 7), g(4, 7)]} --- the two entries are independent list elements and \texttt{PlanNet.\_\_init\_\_} \ldots{}}
\expandafter\gdef\csname R@an.provenance.V7C1.premise.settled.line\endcsname{410}
\expandafter\gdef\csname R@an.provenance.V7C1.premise.text\endcsname{V5B2's two coarse stages cannot be separated in the spec.}
\expandafter\gdef\csname R@an.provenance.V7C1.premise.verdict\endcsname{found false}
\expandafter\gdef\csname R@an.provenance.V7C1.reason\endcsname{which of the two encoder stages carries V5B2's change}
\expandafter\gdef\csname R@an.provenance.V7C1.reason.cell\endcsname{which of the two encoder stages carries V5B2's change}
\expandafter\gdef\csname R@an.provenance.V7C1.reason.file\endcsname{IDEAS\_v5\_wave7.md}
\expandafter\gdef\csname R@an.provenance.V7C1.reason.kind\endcsname{heading}
\expandafter\gdef\csname R@an.provenance.V7C1.reason.line\endcsname{393}
\expandafter\gdef\csname R@an.provenance.V7C1.reason.number\endcsname{no}
\expandafter\gdef\csname R@an.provenance.V7C1.state\endcsname{found}
\expandafter\gdef\csname R@an.provenance.V7C1.wave\endcsname{7}
\expandafter\gdef\csname R@an.provenance.V7C2.cites\endcsname{none stated}
\expandafter\gdef\csname R@an.provenance.V7C2.cites.n\endcsname{0}
\expandafter\gdef\csname R@an.provenance.V7C2.cites.written\endcsname{none stated}
\expandafter\gdef\csname R@an.provenance.V7C2.fact\endcsname{the reviewer's note REVIEW\_wave7\_20261009.md rules ACCEPT (line 390) and did not change it}
\expandafter\gdef\csname R@an.provenance.V7C2.fact.verdict\endcsname{ACCEPT}
\expandafter\gdef\csname R@an.provenance.V7C2.idea\endcsname{C2 --- V7C2 ``LeanNeXt-k3'': extent, at matched parameters and matched arithmetic (IDEAS\_v5\_wave7.md, line 415)}
\expandafter\gdef\csname R@an.provenance.V7C2.idea.file\endcsname{IDEAS\_v5\_wave7.md}
\expandafter\gdef\csname R@an.provenance.V7C2.idea.id\endcsname{C2}
\expandafter\gdef\csname R@an.provenance.V7C2.idea.line\endcsname{415}
\expandafter\gdef\csname R@an.provenance.V7C2.name\endcsname{LeanNeXt-k3}
\expandafter\gdef\csname R@an.provenance.V7C2.premise\endcsname{``\texttt{dwk} does not reach the depthwise kernels of a \texttt{next} stage, so setting it to 3 changes nothing.'' (IDEAS\_v5\_wave7.md, line 427)}
\expandafter\gdef\csname R@an.provenance.V7C2.premise.file\endcsname{IDEAS\_v5\_wave7.md}
\expandafter\gdef\csname R@an.provenance.V7C2.premise.line\endcsname{427}
\expandafter\gdef\csname R@an.provenance.V7C2.premise.settled\endcsname{Settled by \texttt{lib\_v2.py::make\_stage}, \texttt{next} branch (\texttt{dw = tuple(o.get('dwk', 3) if kk > 1 else 1 for kk in k)}) and \texttt{lib\_v2.py::NeXt.\_\_init\_\_} \ldots{}}
\expandafter\gdef\csname R@an.provenance.V7C2.premise.settled.line\endcsname{428}
\expandafter\gdef\csname R@an.provenance.V7C2.premise.text\endcsname{\texttt{dwk} does not reach the depthwise kernels of a \texttt{next} stage, so setting it to 3 changes nothing.}
\expandafter\gdef\csname R@an.provenance.V7C2.premise.verdict\endcsname{found false}
\expandafter\gdef\csname R@an.provenance.V7C2.reason\endcsname{\texttt{L3k3} (the same reduction inside HyReX) is the study's only resolvable within-design ablation (-1.475 pp against HyReX's seed 0, -0.727 against its fresh-seed mean, below the parent's three-seed span, CLAIM\_FRAME 21).}
\expandafter\gdef\csname R@an.provenance.V7C2.reason.cell\endcsname{\texttt{L3k3} (the same reduction inside HyReX) is the study's only resolvable within-design ablation \ldots{}}
\expandafter\gdef\csname R@an.provenance.V7C2.reason.file\endcsname{IDEAS\_v5\_wave7.md}
\expandafter\gdef\csname R@an.provenance.V7C2.reason.kind\endcsname{sentence}
\expandafter\gdef\csname R@an.provenance.V7C2.reason.line\endcsname{420}
\expandafter\gdef\csname R@an.provenance.V7C2.reason.number\endcsname{no}
\expandafter\gdef\csname R@an.provenance.V7C2.state\endcsname{found}
\expandafter\gdef\csname R@an.provenance.V7C2.wave\endcsname{7}
\expandafter\gdef\csname R@an.provenance.V8A1.cites\endcsname{nnU-Net Revisited; MedNeXt}
\expandafter\gdef\csname R@an.provenance.V8A1.cites.n\endcsname{2}
\expandafter\gdef\csname R@an.provenance.V8A1.cites.written\endcsname{S1 (nnU-Net Revisited; Isensee, Wald, Ulrich, Baumgartner, Roy, Maier-Hein, Jaeger; MICCAI 2024; arXiv:2404.09556); S4 (MedNeXt; Roy, Koehler, Ulrich, Baumgartner, Petersen, Isensee, Jager, Maier-Hein; MICCAI 2023; arXiv:2303.09975)}
\expandafter\gdef\csname R@an.provenance.V8A1.fact\endcsname{the reviewer's note REVIEW\_wave8\_20261010.md rules ACCEPT WITH CHANGES (line 380) and changed it: (1) Delete ``four points already measured and paid for (0, 4 at enc5, 4+4, and A1's 18)'' and rewrite the motivation ...}
\expandafter\gdef\csname R@an.provenance.V8A1.fact.verdict\endcsname{ACCEPT WITH CHANGES}
\expandafter\gdef\csname R@an.provenance.V8A1.idea\endcsname{A1 --- V8A1 ``CoarseStack'': the dose-response of the one factor that moved AMOS22 (IDEAS\_v6\_wave8.md, line 147)}
\expandafter\gdef\csname R@an.provenance.V8A1.idea.file\endcsname{IDEAS\_v6\_wave8.md}
\expandafter\gdef\csname R@an.provenance.V8A1.idea.id\endcsname{A1}
\expandafter\gdef\csname R@an.provenance.V8A1.idea.line\endcsname{147}
\expandafter\gdef\csname R@an.provenance.V8A1.name\endcsname{CoarseStack}
\expandafter\gdef\csname R@an.provenance.V8A1.premise\endcsname{``A \texttt{next} stage's block count is taken from the plan, not from the spec, so the stack cannot be deepened and A1 is V7C1.'' (IDEAS\_v6\_wave8.md, line 191)}
\expandafter\gdef\csname R@an.provenance.V8A1.premise.file\endcsname{IDEAS\_v6\_wave8.md}
\expandafter\gdef\csname R@an.provenance.V8A1.premise.line\endcsname{191}
\expandafter\gdef\csname R@an.provenance.V8A1.premise.settled\endcsname{Settled without running anything by \texttt{candidates/ai\_arch\_20261004/lib\_v2.py::PlanNet.\_\_init\_\_} (\texttt{kind, n, o = spec['enc'][s]}) and \texttt{lib\_v2.py::make\_stage}, \texttt{next} branch \ldots{}}
\expandafter\gdef\csname R@an.provenance.V8A1.premise.settled.line\endcsname{192}
\expandafter\gdef\csname R@an.provenance.V8A1.premise.text\endcsname{A \texttt{next} stage's block count is taken from the plan, not from the spec, so the stack cannot be deepened and A1 is V7C1.}
\expandafter\gdef\csname R@an.provenance.V8A1.premise.verdict\endcsname{found false}
\expandafter\gdef\csname R@an.provenance.V8A1.reason\endcsname{Four blocks bought +0.155 pp over no blocks; eighteen is a 4.5$\times$ dose at the same site.}
\expandafter\gdef\csname R@an.provenance.V8A1.reason.cell\endcsname{Four blocks bought +0.155 pp over no blocks; eighteen is a 4.5$\times$ dose at the same site.}
\expandafter\gdef\csname R@an.provenance.V8A1.reason.file\endcsname{IDEAS\_v6\_wave8.md}
\expandafter\gdef\csname R@an.provenance.V8A1.reason.kind\endcsname{sentence}
\expandafter\gdef\csname R@an.provenance.V8A1.reason.line\endcsname{198}
\expandafter\gdef\csname R@an.provenance.V8A1.reason.number\endcsname{yes}
\expandafter\gdef\csname R@an.provenance.V8A1.state\endcsname{found}
\expandafter\gdef\csname R@an.provenance.V8A1.wave\endcsname{8}
\expandafter\gdef\csname R@an.provenance.V8B1.cites\endcsname{InceptionNeXt; nnU-Net Revisited}
\expandafter\gdef\csname R@an.provenance.V8B1.cites.n\endcsname{2}
\expandafter\gdef\csname R@an.provenance.V8B1.cites.written\endcsname{S2 (InceptionNeXt; Yu, Zhou, Yan, Wang; CVPR 2024 pp. 5672--5683; arXiv:2303.16900); S1}
\expandafter\gdef\csname R@an.provenance.V8B1.fact\endcsname{the reviewer's note REVIEW\_wave8\_20261010.md rules ACCEPT WITH CHANGES (line 378) and changed it: (1) State that the stage-0/stage-1 split of the 18.9/21.0/20.4 ms anchor is not independently measured and that the default - D2 cross-check ...}
\expandafter\gdef\csname R@an.provenance.V8B1.fact.verdict\endcsname{ACCEPT WITH CHANGES}
\expandafter\gdef\csname R@an.provenance.V8B1.idea\endcsname{B1 --- V8B1 ``LeanTrunk'': one convolution at encoder stages 0, 1 and 4 (IDEAS\_v6\_wave8.md, line 293)}
\expandafter\gdef\csname R@an.provenance.V8B1.idea.file\endcsname{IDEAS\_v6\_wave8.md}
\expandafter\gdef\csname R@an.provenance.V8B1.idea.id\endcsname{B1}
\expandafter\gdef\csname R@an.provenance.V8B1.idea.line\endcsname{293}
\expandafter\gdef\csname R@an.provenance.V8B1.name\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.provenance.V8B1.premise\endcsname{``The full-resolution encoder convolution is not where the step time is, so removing it buys nothing.'' (IDEAS\_v6\_wave8.md, line 337)}
\expandafter\gdef\csname R@an.provenance.V8B1.premise.file\endcsname{IDEAS\_v6\_wave8.md}
\expandafter\gdef\csname R@an.provenance.V8B1.premise.line\endcsname{337}
\expandafter\gdef\csname R@an.provenance.V8B1.premise.settled\endcsname{Settled without running anything, from two files on disk: \texttt{experiments/profile/03e1e8d35596283f.json} minus \texttt{experiments/profile/553df5e890cb1ded.json} \ldots{}}
\expandafter\gdef\csname R@an.provenance.V8B1.premise.settled.line\endcsname{338}
\expandafter\gdef\csname R@an.provenance.V8B1.premise.text\endcsname{The full-resolution encoder convolution is not where the step time is, so removing it buys nothing.}
\expandafter\gdef\csname R@an.provenance.V8B1.premise.verdict\endcsname{found false}
\expandafter\gdef\csname R@an.provenance.V8B1.reason\endcsname{Remove the second convolution of the two stages that cost the most time (0 and 1: 18.9 / 21.0 / 20.4 ms for 119,808 parameters) and of the stage that costs the most parameters per millisecond (4: 2,764,800 parameters for 0.63 / 1.47 / 0.34 ms).}
\expandafter\gdef\csname R@an.provenance.V8B1.reason.cell\endcsname{Remove the second convolution of the two stages that cost the most time \ldots{}}
\expandafter\gdef\csname R@an.provenance.V8B1.reason.file\endcsname{IDEAS\_v6\_wave8.md}
\expandafter\gdef\csname R@an.provenance.V8B1.reason.kind\endcsname{sentence}
\expandafter\gdef\csname R@an.provenance.V8B1.reason.line\endcsname{295}
\expandafter\gdef\csname R@an.provenance.V8B1.reason.number\endcsname{no}
\expandafter\gdef\csname R@an.provenance.V8B1.state\endcsname{found}
\expandafter\gdef\csname R@an.provenance.V8B1.wave\endcsname{8}
\expandafter\gdef\csname R@an.provenance.V8B2.cites\endcsname{InceptionNeXt}
\expandafter\gdef\csname R@an.provenance.V8B2.cites.n\endcsname{1}
\expandafter\gdef\csname R@an.provenance.V8B2.cites.written\endcsname{S2}
\expandafter\gdef\csname R@an.provenance.V8B2.fact\endcsname{the reviewer's note REVIEW\_wave8\_20261010.md rules ACCEPT WITH CHANGES (line 379) and changed it: Only: say that ``misses the 0.70$\times$ aim by $\approx$ 1 \%'' is inside its own error bar (D3 gives 0.687--0.728$\times$ on AMOS22), because that sentence ...}
\expandafter\gdef\csname R@an.provenance.V8B2.fact.verdict\endcsname{ACCEPT WITH CHANGES}
\expandafter\gdef\csname R@an.provenance.V8B2.idea\endcsname{B2 --- V8B2 ``Stem1'': one convolution at encoder stage 0, and nothing else (IDEAS\_v6\_wave8.md, line 357)}
\expandafter\gdef\csname R@an.provenance.V8B2.idea.file\endcsname{IDEAS\_v6\_wave8.md}
\expandafter\gdef\csname R@an.provenance.V8B2.idea.id\endcsname{B2}
\expandafter\gdef\csname R@an.provenance.V8B2.idea.line\endcsname{357}
\expandafter\gdef\csname R@an.provenance.V8B2.name\endcsname{Stem1}
\expandafter\gdef\csname R@an.provenance.V8B2.premise\endcsname{``An encoder stage with \texttt{n = 1} and a stride cannot be built, so B2 does not exist.'' (IDEAS\_v6\_wave8.md, line 381)}
\expandafter\gdef\csname R@an.provenance.V8B2.premise.file\endcsname{IDEAS\_v6\_wave8.md}
\expandafter\gdef\csname R@an.provenance.V8B2.premise.line\endcsname{381}
\expandafter\gdef\csname R@an.provenance.V8B2.premise.settled\endcsname{Settled by \texttt{lib\_v2.py::make\_stage}, \texttt{plain} branch (\texttt{for i in range(n): add(CNA(ctx, cin if i == 0 else cout, cout, k, stride if i == 0 else 1))}, which is well defined at n = 1) \ldots{}}
\expandafter\gdef\csname R@an.provenance.V8B2.premise.settled.line\endcsname{381}
\expandafter\gdef\csname R@an.provenance.V8B2.premise.text\endcsname{An encoder stage with \texttt{n = 1} and a stride cannot be built, so B2 does not exist.}
\expandafter\gdef\csname R@an.provenance.V8B2.premise.verdict\endcsname{found false}
\expandafter\gdef\csname R@an.provenance.V8B2.reason\endcsname{The single most expensive convolution in the network by time-per-parameter: 9,216 parameters (27,648 on KiTS23) for $\approx$ 9.5 / 10.0 / 15.4 ms, i.e. 6.8 / 7.0 / 12.5 \% of the default's entire step.}
\expandafter\gdef\csname R@an.provenance.V8B2.reason.cell\endcsname{The single most expensive convolution in the network by time-per-parameter: 9,216 parameters \ldots{}}
\expandafter\gdef\csname R@an.provenance.V8B2.reason.file\endcsname{IDEAS\_v6\_wave8.md}
\expandafter\gdef\csname R@an.provenance.V8B2.reason.kind\endcsname{sentence}
\expandafter\gdef\csname R@an.provenance.V8B2.reason.line\endcsname{359}
\expandafter\gdef\csname R@an.provenance.V8B2.reason.number\endcsname{yes}
\expandafter\gdef\csname R@an.provenance.V8B2.state\endcsname{found}
\expandafter\gdef\csname R@an.provenance.V8B2.wave\endcsname{8}
\expandafter\gdef\csname R@an.provenance.corpus.convnext.count\endcsname{16}
\expandafter\gdef\csname R@an.provenance.corpus.convnext.files\endcsname{IDEAS\_v1.md, IDEAS\_v2.md, IDEAS\_v3\_cheap\_axis.md, IDEAS\_v3\_decoder\_head.md, IDEAS\_v3\_frontier\_lit.md, IDEAS\_v3\_impl\_aware.md, IDEAS\_v3\_norm\_reg.md, IDEAS\_v3\_speed.md, IDEAS\_v3\_tumour\_small.md, IDEAS\_v3\_SLATE.md, IDEAS\_v4\_wave5.md, IDEAS\_v4\_wave5\_sources.md, IDEAS\_v5\_wave7.md, IDEAS\_v5\_wave7\_sources.md, IDEAS\_v6\_wave8.md, IDEAS\_v6\_wave8\_sources.md}
\expandafter\gdef\csname R@an.provenance.corpus.effidec.count\endcsname{0}
\expandafter\gdef\csname R@an.provenance.corpus.effidec.files\endcsname{none}
\expandafter\gdef\csname R@an.provenance.corpus.files\endcsname{IDEAS\_v1.md, IDEAS\_v2.md, IDEAS\_v3\_cheap\_axis.md, IDEAS\_v3\_decoder\_head.md, IDEAS\_v3\_frontier\_lit.md, IDEAS\_v3\_impl\_aware.md, IDEAS\_v3\_norm\_reg.md, IDEAS\_v3\_speed.md, IDEAS\_v3\_tumour\_small.md, IDEAS\_v3\_SLATE.md, IDEAS\_v4\_wave5.md, IDEAS\_v4\_wave5\_sources.md, IDEAS\_v5\_wave7.md, IDEAS\_v5\_wave7\_sources.md, IDEAS\_v6\_wave8.md, IDEAS\_v6\_wave8\_sources.md}
\expandafter\gdef\csname R@an.provenance.corpus.mednext.count\endcsname{13}
\expandafter\gdef\csname R@an.provenance.corpus.mednext.files\endcsname{IDEAS\_v1.md, IDEAS\_v3\_cheap\_axis.md, IDEAS\_v3\_decoder\_head.md, IDEAS\_v3\_frontier\_lit.md, IDEAS\_v3\_speed.md, IDEAS\_v3\_tumour\_small.md, IDEAS\_v3\_SLATE.md, IDEAS\_v4\_wave5.md, IDEAS\_v4\_wave5\_sources.md, IDEAS\_v5\_wave7.md, IDEAS\_v5\_wave7\_sources.md, IDEAS\_v6\_wave8.md, IDEAS\_v6\_wave8\_sources.md}
\expandafter\gdef\csname R@an.provenance.corpus.nfiles.count\endcsname{16}
\expandafter\gdef\csname R@an.provenance.corpus.uxnet.count\endcsname{2}
\expandafter\gdef\csname R@an.provenance.corpus.uxnet.files\endcsname{IDEAS\_v3\_frontier\_lit.md, IDEAS\_v3\_speed.md}
\expandafter\gdef\csname R@an.provenance.main.caption\endcsname{The reason the agents gave for each change of the XX-Net family, in their own words, with the wave that proposed it; the decoder rule, additive skips and the large-kernel block each came with a measured reason}
\expandafter\gdef\csname R@an.provenance.main.claim\endcsname{yes}
\expandafter\gdef\csname R@an.provenance.main.cut\endcsname{110}
\expandafter\gdef\csname R@an.provenance.main.n\endcsname{5}
\expandafter\gdef\csname R@an.provenance.main.nfound\endcsname{5}
\expandafter\gdef\csname R@an.provenance.main.premise.caption\endcsname{The premise sentence the agents named for each change of the XX-Net family before ranking it, with the wave that proposed it; a dagger marks a sentence that would have made the change pointless if it were true and that the proposal reports settled as false by reading the repository}
\expandafter\gdef\csname R@an.provenance.main.premise.state\endcsname{complete}
\expandafter\gdef\csname R@an.provenance.main.state\endcsname{complete}
\expandafter\gdef\csname R@an.provenance.n\endcsname{12}
\expandafter\gdef\csname R@an.provenance.premise.dagger\endcsname{a dagger marks a sentence that would have made the change pointless if it were true and that the proposal reports settled as false by reading the repository}
\expandafter\gdef\csname R@an.provenance.premise.kind\endcsname{the sentence a proposal names, before the change is ranked, as the premise to be checked against the repository (Charter 2b): for the decoder rule it is a premise the change rests on, which holds, and for the changes of waves 5 to 8 listed it is the sentence that would have made the change pointless if it were true, which the proposal reports settled as false}
\expandafter\gdef\csname R@an.provenance.premise.nfalse\endcsname{10}
\expandafter\gdef\csname R@an.provenance.premise.nholds\endcsname{1}
\expandafter\gdef\csname R@an.provenance.sent.decoder\endcsname{The decoder rule was proposed in wave 4 from the agents' own parameter and step-time measurements; none of the 16 ideator documents cites EffiDec3D}
\expandafter\gdef\csname R@an.provenance.sent.decoder.state\endcsname{supported}
\expandafter\gdef\csname R@an.provenance.sent.decoder.why\endcsname{the record supports the sentence}
\expandafter\gdef\csname R@an.provenance.tags\endcsname{L3, D2, V5B1, V5B2, V7C1, V8B2, V7C2, V7B1, V7B2, V7A3, V8B1, V8A1}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.C1.amos.logged\endcsname{62.4}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.C1.amos.pred\endcsname{63.4}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.C1.amos.ratio\endcsname{0.985}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.C1.kits.logged\endcsname{49.8}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.C1.kits.pred\endcsname{51.9}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.C1.kits.ratio\endcsname{0.958}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.D1.amos.logged\endcsname{56.3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.D1.amos.pred\endcsname{56.9}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.D1.amos.ratio\endcsname{0.989}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.D1.kits.logged\endcsname{44.7}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.D1.kits.pred\endcsname{46.1}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.D1.kits.ratio\endcsname{0.969}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.D2.amos.logged\endcsname{45.8}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.D2.amos.pred\endcsname{30.4}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.D2.amos.ratio\endcsname{1.506}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.D2.kits.logged\endcsname{26.5}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.D2.kits.pred\endcsname{26.6}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.D2.kits.ratio\endcsname{0.999}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.I1.amos.logged\endcsname{56.0}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.I1.amos.pred\endcsname{57.5}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.I1.amos.ratio\endcsname{0.974}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.I1.kits.logged\endcsname{44.3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.I1.kits.pred\endcsname{46.3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.I1.kits.ratio\endcsname{0.958}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L1.acdc.logged\endcsname{56.0}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L1.acdc.pred\endcsname{57.1}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L1.acdc.ratio\endcsname{0.981}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L1.amos.logged\endcsname{54.3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L1.amos.pred\endcsname{54.7}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L1.amos.ratio\endcsname{0.992}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L1.kits.logged\endcsname{42.2}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L1.kits.pred\endcsname{43.9}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L1.kits.ratio\endcsname{0.961}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L1b.acdc.logged\endcsname{52.2}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L1b.acdc.pred\endcsname{53.4}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L1b.acdc.ratio\endcsname{0.978}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L1b.amos.logged\endcsname{51.0}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L1b.amos.pred\endcsname{51.7}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L1b.amos.ratio\endcsname{0.987}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L1b.kits.logged\endcsname{38.9}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L1b.kits.pred\endcsname{40.3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L1b.kits.ratio\endcsname{0.963}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L2.acdc.logged\endcsname{55.2}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L2.acdc.pred\endcsname{56.9}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L2.acdc.ratio\endcsname{0.970}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L2.amos.logged\endcsname{54.1}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L2.amos.pred\endcsname{54.8}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L2.amos.ratio\endcsname{0.988}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L2.kits.logged\endcsname{41.9}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L2.kits.pred\endcsname{43.7}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L2.kits.ratio\endcsname{0.959}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L3.acdc.logged\endcsname{60.5}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L3.acdc.pred\endcsname{62.2}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L3.acdc.ratio\endcsname{0.974}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L3.amos.logged\endcsname{56.6}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L3.amos.pred\endcsname{57.2}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L3.amos.ratio\endcsname{0.990}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L3.kits.logged\endcsname{44.3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L3.kits.match\endcsname{0.7}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L3.kits.pred\endcsname{46.1}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L3.kits.ratio\endcsname{0.962}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L3.kits.x\endcsname{1.39}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L3k3.amos.logged\endcsname{49.8}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L3k3.amos.pred\endcsname{50.4}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L3k3.amos.ratio\endcsname{0.987}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L3ng.amos.logged\endcsname{54.8}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L3ng.amos.pred\endcsname{55.8}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L3ng.amos.ratio\endcsname{0.980}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L4.acdc.logged\endcsname{55.8}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L4.acdc.pred\endcsname{57.5}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L4.acdc.ratio\endcsname{0.969}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L4.amos.logged\endcsname{54.5}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L4.amos.pred\endcsname{54.6}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L4.amos.ratio\endcsname{0.997}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L4.kits.logged\endcsname{41.3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L4.kits.pred\endcsname{42.7}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L4.kits.ratio\endcsname{0.967}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L6.acdc.logged\endcsname{74.8}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L6.acdc.pred\endcsname{76.9}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L6.acdc.ratio\endcsname{0.973}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L6.amos.logged\endcsname{69.3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L6.amos.pred\endcsname{70.3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L6.amos.ratio\endcsname{0.986}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L6.kits.logged\endcsname{52.2}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L6.kits.pred\endcsname{53.7}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.L6.kits.ratio\endcsname{0.972}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.N1.amos.logged\endcsname{80.7}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.N1.amos.pred\endcsname{77.1}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.N1.amos.ratio\endcsname{1.046}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.N1.kits.logged\endcsname{73.6}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.N1.kits.pred\endcsname{70.4}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.N1.kits.ratio\endcsname{1.045}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.P3c.amos.logged\endcsname{43.4}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.P3c.amos.pred\endcsname{39.2}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.P3c.amos.ratio\endcsname{1.108}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.P3c.kits.logged\endcsname{33.0}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.P3c.kits.pred\endcsname{34.0}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.P3c.kits.ratio\endcsname{0.969}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.S2.amos.logged\endcsname{71.2}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.S2.amos.pred\endcsname{73.4}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.S2.amos.ratio\endcsname{0.970}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.S2.kits.logged\endcsname{53.2}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.S2.kits.pred\endcsname{55.1}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.S2.kits.ratio\endcsname{0.965}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W1.amos.logged\endcsname{43.7}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W1.amos.pred\endcsname{42.7}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W1.amos.ratio\endcsname{1.023}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W1c.amos.logged\endcsname{44.8}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W1c.amos.pred\endcsname{42.9}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W1c.amos.ratio\endcsname{1.045}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W1c.kits.logged\endcsname{35.2}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W1c.kits.pred\endcsname{37.2}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W1c.kits.ratio\endcsname{0.946}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W2.amos.logged\endcsname{45.1}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W2.amos.pred\endcsname{43.1}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W2.amos.ratio\endcsname{1.047}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W3.amos.logged\endcsname{43.3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W3.amos.pred\endcsname{40.6}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W3.amos.ratio\endcsname{1.067}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W3c.amos.logged\endcsname{44.7}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W3c.amos.pred\endcsname{40.1}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W3c.amos.ratio\endcsname{1.115}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W4.amos.logged\endcsname{128.4}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W4.amos.pred\endcsname{131.5}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W4.amos.ratio\endcsname{0.976}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W5.amos.logged\endcsname{50.4}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W5.amos.pred\endcsname{51.4}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.W5.amos.ratio\endcsname{0.981}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.acdc.max\endcsname{0.981}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.acdc.min\endcsname{0.968}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.acdc.n\endcsname{12}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.amos.max\endcsname{1.506}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.amos.min\endcsname{0.970}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.amos.n\endcsname{32}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.band\endcsname{10}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.excluded.acdc.max\endcsname{0.78}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.excluded.acdc.min\endcsname{0.76}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.excluded.acdc.n\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.excluded.acdc.why\endcsname{compiled runs (C30)}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.excluded.amos.max\endcsname{2.67}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.excluded.amos.min\endcsname{1.71}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.excluded.amos.n\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.excluded.amos.why\endcsname{contended allocation (C24)}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.excluded.max\endcsname{2.67}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.excluded.min\endcsname{0.76}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.excluded.n\endcsname{6}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.kits.max\endcsname{1.054}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.kits.min\endcsname{0.946}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.kits.n\endcsname{41}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.max\endcsname{1.506}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.maxdev\endcsname{50.6}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.median\endcsname{0.974}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.min\endcsname{0.946}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.n\endcsname{85}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.n_fresh\endcsname{42}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.n_s0\endcsname{43}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.narms_s0\endcsname{42}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.ndatasets\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.noprofile.acdc.n\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.noprofile.amos.n\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.noprofile.n\endcsname{6}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.noutside\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.noutside.above\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.noutside.below\endcsname{0}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.nwithin10\endcsname{82}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.outside.list\endcsname{LeanDec on AMOS22 (seed 0) at 1.506, trilinear control on AMOS22 (seed 0) at 1.115 and fn.-identical control on AMOS22 (seed 0) at 1.108}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.outside.nlisted\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.pool.acdc.nlogged\endcsname{6}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.pool.acdc.npred\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.pool.amos.nlogged\endcsname{6}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.pool.amos.npred\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.pool.kits.nlogged\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.pool.kits.npred\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.relation\endcsname{Across 85 comparable runs the logged epoch time is a median 0.974 of the time predicted from the profiled step; 82 lie within 10\,\% of it and the three others are LeanDec on AMOS22 (seed 0) at 1.506, trilinear control on AMOS22 (seed 0) at 1.115 and fn.-identical control on AMOS22 (seed 0) at 1.108}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.seedspread.argmax\endcsname{LeanDec on KiTS23}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.seedspread.beyond.list\endcsname{none}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.seedspread.max\endcsname{5.3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.seedspread.n\endcsname{21}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.seedspread.nbeyond\endcsname{0}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.seedspread.nseeds\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.eptime.typical\endcsname{yes}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.acdc.clause\endcsname{HyReX's fresh-seed mean delta (\ensuremath{+0.450}\,pp) and ResEnc-M's (\ensuremath{+0.242}\,pp) are 0.208\,pp apart, a margin inside the registered 0.50\,pp one-seed pair floor}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.acdc.hero.delta\endcsname{+0.45}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.acdc.hero.istop\endcsname{yes}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.acdc.hero.rank\endcsname{1}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.acdc.landed\endcsname{HyReX, ResEnc-M}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.acdc.margin12\endcsname{0.208}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.acdc.margin12.vsfloor\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.acdc.ndone\endcsname{2}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.acdc.nregistered\endcsname{2}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.acdc.runnerup\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.acdc.state\endcsname{complete}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.acdc.top\endcsname{HyReX}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.acdc.top.vshero\endcsname{0.00}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.amos.clause\endcsname{ResEnc-M's fresh-seed mean delta (\ensuremath{+0.465}\,pp) and HyReX's (\ensuremath{+0.132}\,pp) are 0.332\,pp apart, a margin inside the registered 0.50\,pp one-seed pair floor}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.amos.hero.delta\endcsname{+0.13}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.amos.hero.istop\endcsname{no}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.amos.hero.rank\endcsname{5}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.amos.landed\endcsname{ResEnc-M, ResEnc+context, ResEnc-matched, ConvNeXt-k3, HyReX}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.amos.margin12\endcsname{0.010}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.amos.margin12.vsfloor\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.amos.ndone\endcsname{5}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.amos.nregistered\endcsname{5}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.amos.runnerup\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.amos.state\endcsname{complete}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.amos.top\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.amos.top.vshero\endcsname{0.33}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.kits.clause\endcsname{ResEnc-M's fresh-seed mean delta (\ensuremath{+3.475}\,pp) is 1.382\,pp above HyReX's (\ensuremath{+2.094}\,pp), a margin beyond the registered 0.50\,pp one-seed pair floor}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.kits.hero.delta\endcsname{+2.09}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.kits.hero.istop\endcsname{no}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.kits.hero.rank\endcsname{4}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.kits.landed\endcsname{ResEnc-M, ResEnc-matched, ResEnc+context, HyReX, HyReX+context, ConvNeXt-k3}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.kits.margin12\endcsname{1.162}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.kits.margin12.vsfloor\endcsname{beyond}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.kits.ndone\endcsname{6}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.kits.nregistered\endcsname{6}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.kits.runnerup\endcsname{ResEnc-matched}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.kits.state\endcsname{complete}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.kits.top\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.proxy_dynamics.fresh.kits.top.vshero\endcsname{1.38}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.C1.amos\endcsname{+0.0347}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.C1.amos.pos\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.C1.kits\endcsname{+0.0187}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.C1.kits.pos\endcsname{below}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.D1.amos\endcsname{+0.0355}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.D1.amos.pos\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.D1.kits\endcsname{+0.0158}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.D1.kits.pos\endcsname{below}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.D2.amos\endcsname{+0.0373}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.D2.amos.pos\endcsname{above}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.D2.kits\endcsname{+0.0281}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.D2.kits.pos\endcsname{above}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.I1.amos\endcsname{+0.0389}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.I1.amos.pos\endcsname{above}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.I1.kits\endcsname{+0.0170}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.I1.kits.pos\endcsname{below}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L1.acdc\endcsname{+0.0845}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L1.acdc.pos\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L1.amos\endcsname{+0.0380}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L1.amos.pos\endcsname{above}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L1.kits\endcsname{+0.0327}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L1.kits.pos\endcsname{above}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L1b.acdc\endcsname{+0.0841}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L1b.acdc.pos\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L1b.amos\endcsname{+0.0299}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L1b.amos.pos\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L1b.kits\endcsname{+0.0186}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L1b.kits.pos\endcsname{below}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L2.acdc\endcsname{+0.0809}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L2.acdc.pos\endcsname{below}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L2.amos\endcsname{+0.0347}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L2.amos.pos\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L2.kits\endcsname{+0.0204}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L2.kits.pos\endcsname{below}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L3.acdc\endcsname{+0.0783}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L3.acdc.pos\endcsname{below}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L3.acdc.rank\endcsname{6}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L3.acdc.vsnext\endcsname{-0.00257}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L3.acdc.vspoolmax\endcsname{-0.0073}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L3.amos\endcsname{+0.0380}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L3.amos.pos\endcsname{above}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L3.amos.rank\endcsname{2}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L3.amos.vsnext\endcsname{-0.00082}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L3.amos.vspoolmax\endcsname{+0.0015}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L3.kits\endcsname{+0.0254}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L3.kits.pos\endcsname{above}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L3.kits.rank\endcsname{7}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L3.kits.vsnext\endcsname{-0.00044}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L3.kits.vspoolmax\endcsname{+0.0029}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L3k3.amos\endcsname{+0.0361}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L3k3.amos.pos\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L3ng.amos\endcsname{+0.0337}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L3ng.amos.pos\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L4.acdc\endcsname{+0.0826}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L4.acdc.pos\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L4.amos\endcsname{+0.0365}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L4.amos.pos\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L4.kits\endcsname{+0.0276}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L4.kits.pos\endcsname{above}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L6.acdc\endcsname{+0.0840}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L6.acdc.pos\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L6.amos\endcsname{+0.0363}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L6.amos.pos\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L6.kits\endcsname{+0.0258}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.L6.kits.pos\endcsname{above}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.N1.amos\endcsname{+0.0321}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.N1.amos.pos\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.N1.kits\endcsname{+0.0077}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.N1.kits.pos\endcsname{below}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.P3c.amos\endcsname{+0.0376}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.P3c.amos.pos\endcsname{above}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.P3c.kits\endcsname{+0.0302}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.P3c.kits.pos\endcsname{above}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.S2.amos\endcsname{+0.0372}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.S2.amos.pos\endcsname{above}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.S2.kits\endcsname{+0.0198}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.S2.kits.pos\endcsname{below}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.W1.amos\endcsname{+0.0346}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.W1.amos.pos\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.W1c.amos\endcsname{+0.0374}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.W1c.amos.pos\endcsname{above}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.W1c.kits\endcsname{+0.0285}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.W1c.kits.pos\endcsname{above}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.W2.amos\endcsname{+0.0379}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.W2.amos.pos\endcsname{above}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.W3.amos\endcsname{+0.0330}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.W3.amos.pos\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.W3c.amos\endcsname{+0.0286}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.W3c.amos.pos\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.W4.amos\endcsname{+0.0328}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.W4.amos.pos\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.W5.amos\endcsname{+0.0308}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.W5.amos.pos\endcsname{inside}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.acdc.argmax\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.acdc.max\endcsname{+0.0845}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.acdc.mean\endcsname{+0.0824}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.acdc.min\endcsname{+0.0783}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.acdc.n\endcsname{6}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.acdc.nabovepool\endcsname{0}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.acdc.nbelowpool\endcsname{2}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.acdc.ninpool\endcsname{4}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.acdc.nwithinvsnext\endcsname{2}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.acdc.toporder\endcsname{not resolved}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.acdc.toporder.clause\endcsname{its margin over the adjacent arm, -0.00257, is below that pool's own seed-to-seed spread of 0.0041 on the same quantity, so the order around it is not resolved}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.acdc.vsnext.rel\endcsname{below}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.amos.abovepool.spread\endcsname{0.0017}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.amos.argmax\endcsname{HyReX+pooled skip}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.amos.max\endcsname{+0.0389}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.amos.mean\endcsname{+0.0351}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.amos.min\endcsname{+0.0286}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.amos.n\endcsname{22}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.amos.nabovepool\endcsname{8}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.amos.nbelowpool\endcsname{0}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.amos.ninpool\endcsname{14}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.amos.nwithinvsnext\endcsname{7}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.amos.toporder\endcsname{not resolved}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.amos.toporder.clause\endcsname{its margin over the adjacent arm, -0.00082, is below that pool's own seed-to-seed spread of 0.0080 on the same quantity, so the order around it is not resolved}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.amos.vsnext.rel\endcsname{below}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.base.acdc.max\endcsname{+0.0856}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.base.acdc.min\endcsname{+0.0815}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.base.acdc.n\endcsname{6}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.base.acdc.width\endcsname{0.0041}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.base.amos.max\endcsname{+0.0366}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.base.amos.min\endcsname{+0.0286}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.base.amos.n\endcsname{6}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.base.amos.width\endcsname{0.0080}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.base.kits.max\endcsname{+0.0225}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.base.kits.min\endcsname{+0.0212}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.base.kits.n\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.base.kits.width\endcsname{0.0013}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.kits.abovepool.spread\endcsname{0.0074}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.kits.argmax\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.kits.max\endcsname{+0.0327}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.kits.mean\endcsname{+0.0226}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.kits.min\endcsname{+0.0077}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.kits.n\endcsname{14}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.kits.nabovepool\endcsname{7}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.kits.nbelowpool\endcsname{7}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.kits.ninpool\endcsname{0}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.kits.nwithinvsnext\endcsname{2}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.kits.toporder\endcsname{not resolved}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.kits.toporder.clause\endcsname{its margin over the adjacent arm, -0.00044, is below that pool's own seed-to-seed spread of 0.0013 on the same quantity, so the order around it is not resolved}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.kits.vsnext.rel\endcsname{below}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.max\endcsname{+0.0845}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.min\endcsname{+0.0077}
\expandafter\gdef\csname R@an.proxy_dynamics.gap.n\endcsname{42}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.acdc.collapse\endcsname{0.22}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.acdc.mean_full\endcsname{+0.05}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.acdc.mean_full_frozen\endcsname{+0.05}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.acdc.mean_short\endcsname{+0.27}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.acdc.n\endcsname{12}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.acdc.narch\endcsname{1}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.acdc.npos_full\endcsname{9}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.acdc.npos_full_frozen\endcsname{9}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.acdc.npos_short\endcsname{12}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.acdc.nrecipe\endcsname{11}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.acdc.refshift\endcsname{0.000}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.amos.collapse\endcsname{1.24}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.amos.mean_full\endcsname{-0.13}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.amos.mean_full_frozen\endcsname{-0.16}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.amos.mean_short\endcsname{+1.11}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.amos.n\endcsname{7}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.amos.narch\endcsname{1}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.amos.npos_full\endcsname{2}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.amos.npos_full_frozen\endcsname{2}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.amos.npos_short\endcsname{7}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.amos.nrecipe\endcsname{6}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.amos.refshift\endcsname{-0.029}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.bar\endcsname{+0.35}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.best_full\endcsname{+0.17}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.keep_frac\endcsname{58}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.mean_full\endcsname{-0.01}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.mean_short\endcsname{+0.58}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.n\endcsname{19}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.nabove_bar\endcsname{0}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.narch\endcsname{2}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.npos_full\endcsname{11}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.npos_short\endcsname{19}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.nrecipe\endcsname{17}
\expandafter\gdef\csname R@an.proxy_dynamics.pairs.rho\endcsname{-0.46}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.acdc.best100\endcsname{ResEnc-matched}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.acdc.best100.rankfinal_s0\endcsname{5}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.acdc.hero.rank100_s0\endcsname{4}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.acdc.hero.rankfinal_s0\endcsname{1}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.acdc.range100\endcsname{0.66}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.acdc.rangefinal\endcsname{0.63}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.acdc.scale100\endcsname{1.1}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.acdc.sd100\endcsname{0.22}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.acdc.sdfinal\endcsname{0.21}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.amos.best100\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.amos.best100.rankfinal_s0\endcsname{1}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.amos.hero.rank100_s0\endcsname{6}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.amos.hero.rankfinal_s0\endcsname{6}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.amos.range100\endcsname{35.21}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.amos.rangefinal\endcsname{1.57}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.amos.scale100\endcsname{21.5}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.amos.sd100\endcsname{7.17}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.amos.sdfinal\endcsname{0.33}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.kits.best100\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.kits.best100.rankfinal_s0\endcsname{6}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.kits.hero.rank100_s0\endcsname{10}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.kits.hero.rankfinal_s0\endcsname{2}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.kits.range100\endcsname{13.86}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.kits.rangefinal\endcsname{10.00}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.kits.scale100\endcsname{1.4}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.kits.sd100\endcsname{3.26}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.kits.sdfinal\endcsname{2.40}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.scale.comparable.list\endcsname{KiTS23 and ACDC}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.scale.ncomparable\endcsname{2}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.scale.nout\endcsname{1}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.scale.out.list\endcsname{AMOS22}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.scale.sentence\endcsname{At epoch 100 the across-arm spread of the proxy is 21.5\,\ensuremath{\times} the spread of the final deltas on AMOS22, 1.4\,\ensuremath{\times} on KiTS23 and 1.1\,\ensuremath{\times} on ACDC; that is out of scale (a factor of more than 2 either way) on AMOS22 and on a comparable scale (within a factor of 2) on KiTS23 and ACDC}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.scale.threshold\endcsname{2}
\expandafter\gdef\csname R@an.proxy_dynamics.proxy.scatter_epoch\endcsname{100}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.acdc.frozen.n\endcsname{6}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.acdc.frozen.sd\endcsname{0.099}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.acdc.frozen.sd1\endcsname{0.107}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.acdc.nalt\endcsname{1}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.acdc.uncompiled.n\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.acdc.uncompiled.shift\endcsname{+0.0070}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.amos.contemporaneous.n\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.amos.contemporaneous.shift\endcsname{+0.0108}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.amos.frozen.n\endcsname{6}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.amos.frozen.sd\endcsname{0.122}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.amos.frozen.sd1\endcsname{0.132}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.amos.nalt\endcsname{2}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.amos.uncompiled.n\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.amos.uncompiled.shift\endcsname{+0.0288}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.kits.contemporaneous.n\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.kits.contemporaneous.shift\endcsname{+0.4873}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.kits.frozen.n\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.kits.frozen.sd\endcsname{0.795}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.kits.frozen.sd1\endcsname{0.918}
\expandafter\gdef\csname R@an.proxy_dynamics.ref.kits.nalt\endcsname{1}
\expandafter\gdef\csname R@an.proxy_dynamics.runs.inflight\endcsname{0}
\expandafter\gdef\csname R@an.proxy_dynamics.runs.pending\endcsname{42}
\expandafter\gdef\csname R@an.proxy_dynamics.runs.read\endcsname{97}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.acdc.d0\endcsname{+0.616}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.acdc.dfresh\endcsname{+0.450}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.acdc.move\endcsname{+0.166}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.acdc.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.acdc.semove\endcsname{0.121}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.acdc.senull\endcsname{0.081}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.acdc.sepair\endcsname{0.033}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.acdc.spread\endcsname{0.067}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.acdc.state\endcsname{complete}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.acdc.verdict\endcsname{not resolved}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.amos.d0\endcsname{+0.382}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.amos.dfresh\endcsname{+0.132}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.amos.move\endcsname{+0.249}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.amos.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.amos.semove\endcsname{0.150}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.amos.senull\endcsname{0.100}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.amos.sepair\endcsname{0.148}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.amos.spread\endcsname{0.296}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.amos.state\endcsname{complete}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.amos.verdict\endcsname{not resolved}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.bar\endcsname{+0.35}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.floor\endcsname{0.50}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.kits.d0\endcsname{+2.842}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.kits.dfresh\endcsname{+2.094}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.kits.move\endcsname{+0.748}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.kits.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.kits.semove\endcsname{0.974}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.kits.senull\endcsname{0.726}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.kits.sepair\endcsname{0.296}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.kits.spread\endcsname{0.592}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.kits.state\endcsname{complete}
\expandafter\gdef\csname R@an.proxy_dynamics.screen.kits.verdict\endcsname{reproduces}
\expandafter\gdef\csname R@an.proxy_dynamics.sd.acdc.e100\endcsname{0.09}
\expandafter\gdef\csname R@an.proxy_dynamics.sd.acdc.e100.n\endcsname{5}
\expandafter\gdef\csname R@an.proxy_dynamics.sd.acdc.e1000\endcsname{0.10}
\expandafter\gdef\csname R@an.proxy_dynamics.sd.acdc.e1000.n\endcsname{6}
\expandafter\gdef\csname R@an.proxy_dynamics.sd.acdc.pairfull\endcsname{0.10}
\expandafter\gdef\csname R@an.proxy_dynamics.sd.acdc.pairshort\endcsname{0.08}
\expandafter\gdef\csname R@an.proxy_dynamics.sd.amos.e100\endcsname{0.71}
\expandafter\gdef\csname R@an.proxy_dynamics.sd.amos.e100.n\endcsname{5}
\expandafter\gdef\csname R@an.proxy_dynamics.sd.amos.e1000\endcsname{0.12}
\expandafter\gdef\csname R@an.proxy_dynamics.sd.amos.e1000.n\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.sd.amos.pairfull\endcsname{0.12}
\expandafter\gdef\csname R@an.proxy_dynamics.sd.amos.pairshort\endcsname{0.64}
\expandafter\gdef\csname R@an.proxy_dynamics.sdratio.acdc\endcsname{0.9}
\expandafter\gdef\csname R@an.proxy_dynamics.sdratio.acdc.frozen\endcsname{0.9}
\expandafter\gdef\csname R@an.proxy_dynamics.sdratio.acdc.pair\endcsname{0.8}
\expandafter\gdef\csname R@an.proxy_dynamics.sdratio.amos\endcsname{5.9}
\expandafter\gdef\csname R@an.proxy_dynamics.sdratio.amos.frozen\endcsname{5.8}
\expandafter\gdef\csname R@an.proxy_dynamics.sdratio.amos.pair\endcsname{5.3}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.acdc.d1000\endcsname{-0.03}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.acdc.d1000.n\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.acdc.d1000.nside\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.acdc.d1000.sd\endcsname{0.11}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.acdc.d1000.sd_default\endcsname{0.14}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.acdc.d1000.sd_design\endcsname{0.03}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.acdc.d1000.sd_paired\endcsname{0.11}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.acdc.d1000.state\endcsname{done}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.acdc.d250\endcsname{+0.06}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.acdc.d250.n\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.acdc.d250.nside\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.acdc.d250.sd\endcsname{0.11}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.acdc.d250.sd_default\endcsname{0.05}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.acdc.d250.sd_design\endcsname{0.10}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.acdc.d250.sd_paired\endcsname{0.11}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.acdc.d250.state\endcsname{done}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.amos.d1000\endcsname{+0.01}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.amos.d1000.n\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.amos.d1000.nside\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.amos.d1000.sd\endcsname{0.36}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.amos.d1000.sd_default\endcsname{0.12}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.amos.d1000.sd_design\endcsname{0.24}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.amos.d1000.sd_paired\endcsname{0.36}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.amos.d1000.state\endcsname{done}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.amos.d250\endcsname{+0.70}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.amos.d250.n\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.amos.d250.nside\endcsname{3}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.amos.d250.sd\endcsname{0.28}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.amos.d250.sd_default\endcsname{0.19}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.amos.d250.sd_design\endcsname{0.32}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.amos.d250.sd_paired\endcsname{0.28}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.amos.d250.state\endcsname{done}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.npending\endcsname{0}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.nsets\endcsname{4}
\expandafter\gdef\csname R@an.proxy_dynamics.spd.sd.def\endcsname{the sample SD (divisor $n-1$) of the three seed-matched design-minus-default differences}
\expandafter\gdef\csname R@an.proxy_dynamics.step.L3.acdc.x\endcsname{1.64}
\expandafter\gdef\csname R@an.proxy_dynamics.step.L3.amos.x\endcsname{1.53}
\expandafter\gdef\csname R@an.proxy_dynamics.step.L3.kits.x\endcsname{1.40}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.band_hi\endcsname{0.87}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.band_hi3\endcsname{0.867}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.e100\endcsname{-0.20}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.e1000\endcsname{+0.47}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.e250\endcsname{+0.20}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.e50\endcsname{+0.33}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.e500\endcsname{+0.60}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.e750\endcsname{+0.20}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.loo.arm\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.loo.maxabs\endcsname{0.80}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.loo.nout\endcsname{0}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.maxabs\endcsname{0.60}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.n\endcsname{6}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.n_registered\endcsname{28}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.nnull\endcsname{16}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.nout\endcsname{0}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.null\endcsname{exact}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.pe100\endcsname{0.719}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.pe1000\endcsname{0.272}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.pe250\endcsname{0.719}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.pe50\endcsname{0.469}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.pe500\endcsname{0.136}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.pe750\endcsname{0.719}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.reach\endcsname{no}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.resolve_n\endcsname{47}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.acdc.resolve_state\endcsname{found}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.band_hi\endcsname{0.31}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.band_hi3\endcsname{0.307}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.e100\endcsname{+0.43}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.e1000\endcsname{+0.35}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.e250\endcsname{+0.24}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.e50\endcsname{+0.33}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.e500\endcsname{+0.21}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.e750\endcsname{+0.37}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.loo.arm\endcsname{default+GN16}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.loo.maxabs\endcsname{0.37}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.loo.nout\endcsname{1}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.maxabs\endcsname{0.43}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.n\endcsname{22}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.n_registered\endcsname{28}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.nnull\endcsname{232}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.nout\endcsname{4}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.null\endcsname{exact}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.pe100\endcsname{0.005}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.pe1000\endcsname{0.023}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.pe250\endcsname{0.129}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.pe50\endcsname{0.031}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.pe500\endcsname{0.178}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.pe750\endcsname{0.017}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.reach\endcsname{yes}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.resolve_n\endcsname{22}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.amos.resolve_state\endcsname{found}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.edge.n12\endcsname{0.455}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.edge.n16\endcsname{0.383}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.edge.n20\endcsname{0.326}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.edge.n24\endcsname{0.290}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.edge.n28\endcsname{0.265}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.inband.sentence\endcsname{5 of the 18 (dataset, epoch) agreements leave the exact chance band of their arm count (AMOS22 at epochs 50 (\ensuremath{+0.33}), 100 (\ensuremath{+0.43}), 750 (\ensuremath{+0.37}) and 1000 (\ensuremath{+0.35}); KiTS23 at epoch 100 (\ensuremath{+0.47}); all positive); each cell is read at the 5\,\% level and the 18 cells are not corrected for one another; the largest $|\tau|$ is AMOS22 0.43, KiTS23 0.47, ACDC 0.60; leaving out, in each dataset, the one arm with the most extreme epoch-100 proxy (AMOS22 default+GN16, KiTS23 default+GN16, ACDC ConvNeXt-k3) leaves 1 of the 18 agreements outside their band}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.band_hi\endcsname{0.41}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.band_hi3\endcsname{0.407}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.e100\endcsname{+0.47}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.e1000\endcsname{+0.34}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.e250\endcsname{+0.32}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.e50\endcsname{+0.01}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.e500\endcsname{+0.19}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.e750\endcsname{+0.36}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.loo.arm\endcsname{default+GN16}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.loo.maxabs\endcsname{0.38}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.loo.nout\endcsname{0}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.maxabs\endcsname{0.47}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.n\endcsname{14}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.n_registered\endcsname{28}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.nnull\endcsname{92}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.nout\endcsname{1}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.null\endcsname{exact}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.pe100\endcsname{0.019}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.pe1000\endcsname{0.101}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.pe250\endcsname{0.127}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.pe50\endcsname{1.000}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.pe500\endcsname{0.388}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.pe750\endcsname{0.079}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.reach\endcsname{yes}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.resolve_n\endcsname{14}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.kits.resolve_state\endcsname{found}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.ncells\endcsname{18}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.nout.total\endcsname{5}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.out.list\endcsname{AMOS22 at epochs 50 (\ensuremath{+0.33}), 100 (\ensuremath{+0.43}), 750 (\ensuremath{+0.37}) and 1000 (\ensuremath{+0.35}); KiTS23 at epoch 100 (\ensuremath{+0.47})}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.out.sign\endcsname{positive}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.reach.list\endcsname{AMOS22, KiTS23}
\expandafter\gdef\csname R@an.proxy_dynamics.tau.reach.n\endcsname{2}
\expandafter\gdef\csname R@an.published.anchor.resm.ours\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.published.anchor.resm.ours.basis\endcsname{over folds 1-4, one seed per fold}
\expandafter\gdef\csname R@an.published.anchor.resm.pub\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.published.cap.gb\endcsname{12}
\expandafter\gdef\csname R@an.published.cap.maxgain\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.published.cap.maxname\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.published.cap.n\endcsname{6}
\expandafter\gdef\csname R@an.published.caption\endcsname{Gain over each pipeline's own nnU-Net: {\ifdefined\archL\archL\else XX-Net-L\fi}, {\ifdefined\archA\archA\else XX-Net-A\fi} and ResEnc-M trained in our pipeline beside the published networks of nnU-Net Revisited. Gains in pp; our block: over our nnU-Net default (KiTS23 frozen fold-0 pool 83.38), AMOS22 and ACDC as the mean over folds 1-4 of the difference to the default; published block: nnU-Net Revisited, Table~1 (five-fold means against its nnU-Net, KiTS23 86.04); unmarked: mean over folds 1-4 of (network $-$ default), one seed per fold; memory: ours the allocator peak of the profiled training step (KiTS23 plan), published the nvidia-smi reading during training; GPU-h: ours the measured KiTS23 training wall-clock (fold 0, mean over seeds), published the paper's A100 run time.}
\expandafter\gdef\csname R@an.published.figcaption\endcsname{KiTS23 gain over each pipeline's own nnU-Net against training GPU memory: filled, trained in our pipeline (gain over our nnU-Net default; {\ifdefined\archL\archL\else XX-Net-L\fi} over folds 1-4, one seed per fold); hollow, nnU-Net Revisited (gain over its nnU-Net, five-fold means); dashed, the 12\,GB cap of this study}
\expandafter\gdef\csname R@an.published.legend\endcsname{gains in pp; our block: over our nnU-Net default (KiTS23 frozen fold-0 pool 83.38), AMOS22 and ACDC as the mean over folds 1-4 of the difference to the default; published block: nnU-Net Revisited, Table~1 (five-fold means against its nnU-Net, KiTS23 86.04); unmarked: mean over folds 1-4 of (network $-$ default), one seed per fold; memory: ours the allocator peak of the profiled training step (KiTS23 plan), published the nvidia-smi reading during training; GPU-h: ours the measured KiTS23 training wall-clock (fold 0, mean over seeds), published the paper's A100 run time}
\expandafter\gdef\csname R@an.published.level.kits.ours\endcsname{83.38}
\expandafter\gdef\csname R@an.published.level.kits.pub\endcsname{86.04}
\expandafter\gdef\csname R@an.published.ours.def.basis.acdc\endcsname{reference}
\expandafter\gdef\csname R@an.published.ours.def.basis.amos\endcsname{reference}
\expandafter\gdef\csname R@an.published.ours.def.basis.kits\endcsname{reference}
\expandafter\gdef\csname R@an.published.ours.def.cell.acdc\endcsname{ref.}
\expandafter\gdef\csname R@an.published.ours.def.cell.amos\endcsname{ref.}
\expandafter\gdef\csname R@an.published.ours.def.cell.kits\endcsname{ref.}
\expandafter\gdef\csname R@an.published.ours.def.gain.acdc\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.published.ours.def.gain.amos\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.published.ours.def.gain.kits\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.published.ours.def.gpuh\endcsname{8.9}
\expandafter\gdef\csname R@an.published.ours.def.mem\endcsname{8.51}
\expandafter\gdef\csname R@an.published.ours.def.name\endcsname{nnU-Net}
\expandafter\gdef\csname R@an.published.ours.def.tag\endcsname{base}
\expandafter\gdef\csname R@an.published.ours.def.timex\endcsname{1.00}
\expandafter\gdef\csname R@an.published.ours.resm.basis.acdc\endcsname{over folds 1-4, one seed per fold}
\expandafter\gdef\csname R@an.published.ours.resm.basis.amos\endcsname{over folds 1-4, one seed per fold}
\expandafter\gdef\csname R@an.published.ours.resm.basis.kits\endcsname{over folds 1-4, one seed per fold}
\expandafter\gdef\csname R@an.published.ours.resm.cell.acdc\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.published.ours.resm.cell.amos\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.published.ours.resm.cell.kits\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.published.ours.resm.cv.acdc\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.published.ours.resm.cv.amos\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.published.ours.resm.cv.kits\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.published.ours.resm.fresh.kits\endcsname{\ensuremath{+3.48}}
\expandafter\gdef\csname R@an.published.ours.resm.gain.acdc\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.published.ours.resm.gain.amos\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.published.ours.resm.gain.kits\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.published.ours.resm.gpuh\endcsname{11.8}
\expandafter\gdef\csname R@an.published.ours.resm.mem\endcsname{9.73}
\expandafter\gdef\csname R@an.published.ours.resm.name\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.published.ours.resm.nfold.acdc\endcsname{4}
\expandafter\gdef\csname R@an.published.ours.resm.nfold.amos\endcsname{4}
\expandafter\gdef\csname R@an.published.ours.resm.nfold.kits\endcsname{4}
\expandafter\gdef\csname R@an.published.ours.resm.s0.acdc\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.published.ours.resm.s0.amos\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.published.ours.resm.s0.kits\endcsname{\ensuremath{+2.33}}
\expandafter\gdef\csname R@an.published.ours.resm.tag\endcsname{L1}
\expandafter\gdef\csname R@an.published.ours.resm.timex\endcsname{1.33}
\expandafter\gdef\csname R@an.published.ours.xa.basis.acdc\endcsname{over folds 1-4, one seed per fold}
\expandafter\gdef\csname R@an.published.ours.xa.basis.amos\endcsname{over folds 1-4, one seed per fold}
\expandafter\gdef\csname R@an.published.ours.xa.basis.kits\endcsname{over folds 1-4, one seed per fold}
\expandafter\gdef\csname R@an.published.ours.xa.cell.acdc\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.published.ours.xa.cell.amos\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.published.ours.xa.cell.kits\endcsname{\ensuremath{+1.63}}
\expandafter\gdef\csname R@an.published.ours.xa.cv.acdc\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.published.ours.xa.cv.amos\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.published.ours.xa.cv.kits\endcsname{\ensuremath{+1.63}}
\expandafter\gdef\csname R@an.published.ours.xa.fresh.kits\endcsname{\ensuremath{+2.66}}
\expandafter\gdef\csname R@an.published.ours.xa.gain.acdc\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.published.ours.xa.gain.amos\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.published.ours.xa.gain.kits\endcsname{\ensuremath{+1.63}}
\expandafter\gdef\csname R@an.published.ours.xa.gpuh\endcsname{8.5}
\expandafter\gdef\csname R@an.published.ours.xa.mem\endcsname{8.02}
\expandafter\gdef\csname R@an.published.ours.xa.name\endcsname{{\ifdefined\archA\archA\else XX-Net-A\fi}}
\expandafter\gdef\csname R@an.published.ours.xa.nfold.acdc\endcsname{4}
\expandafter\gdef\csname R@an.published.ours.xa.nfold.amos\endcsname{4}
\expandafter\gdef\csname R@an.published.ours.xa.nfold.kits\endcsname{4}
\expandafter\gdef\csname R@an.published.ours.xa.s0.acdc\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.published.ours.xa.s0.amos\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.published.ours.xa.s0.kits\endcsname{\ensuremath{+2.55}}
\expandafter\gdef\csname R@an.published.ours.xa.tag\endcsname{V7A1}
\expandafter\gdef\csname R@an.published.ours.xa.timex\endcsname{0.95}
\expandafter\gdef\csname R@an.published.ours.xl.basis.acdc\endcsname{over folds 1-4, one seed per fold}
\expandafter\gdef\csname R@an.published.ours.xl.basis.amos\endcsname{over folds 1-4, one seed per fold}
\expandafter\gdef\csname R@an.published.ours.xl.basis.kits\endcsname{over folds 1-4, one seed per fold}
\expandafter\gdef\csname R@an.published.ours.xl.cell.acdc\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.published.ours.xl.cell.amos\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.published.ours.xl.cell.kits\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.published.ours.xl.cv.acdc\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.published.ours.xl.cv.amos\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.published.ours.xl.cv.kits\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.published.ours.xl.fresh.kits\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@an.published.ours.xl.gain.acdc\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.published.ours.xl.gain.amos\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.published.ours.xl.gain.kits\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.published.ours.xl.gpuh\endcsname{8.2}
\expandafter\gdef\csname R@an.published.ours.xl.mem\endcsname{7.65}
\expandafter\gdef\csname R@an.published.ours.xl.name\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi}}
\expandafter\gdef\csname R@an.published.ours.xl.nfold.acdc\endcsname{4}
\expandafter\gdef\csname R@an.published.ours.xl.nfold.amos\endcsname{4}
\expandafter\gdef\csname R@an.published.ours.xl.nfold.kits\endcsname{4}
\expandafter\gdef\csname R@an.published.ours.xl.s0.acdc\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.published.ours.xl.s0.amos\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.published.ours.xl.s0.kits\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.published.ours.xl.tag\endcsname{V7C1}
\expandafter\gdef\csname R@an.published.ours.xl.timex\endcsname{0.92}
\expandafter\gdef\csname R@an.published.pub.mednextl3.arch\endcsname{CNN}
\expandafter\gdef\csname R@an.published.pub.mednextl3.gain.acdc\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.published.pub.mednextl3.gain.amos\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.published.pub.mednextl3.gain.kits\endcsname{\ensuremath{+2.21}}
\expandafter\gdef\csname R@an.published.pub.mednextl3.hours\endcsname{68}
\expandafter\gdef\csname R@an.published.pub.mednextl3.name\endcsname{MedNeXt-L, $k{=}3$}
\expandafter\gdef\csname R@an.published.pub.mednextl3.timex\endcsname{7.6}
\expandafter\gdef\csname R@an.published.pub.mednextl3.vram\endcsname{17.3}
\expandafter\gdef\csname R@an.published.pub.mednextl5.arch\endcsname{CNN}
\expandafter\gdef\csname R@an.published.pub.mednextl5.gain.acdc\endcsname{\ensuremath{+1.08}}
\expandafter\gdef\csname R@an.published.pub.mednextl5.gain.amos\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.published.pub.mednextl5.gain.kits\endcsname{\ensuremath{+1.70}}
\expandafter\gdef\csname R@an.published.pub.mednextl5.hours\endcsname{233}
\expandafter\gdef\csname R@an.published.pub.mednextl5.name\endcsname{MedNeXt-L, $k{=}5$}
\expandafter\gdef\csname R@an.published.pub.mednextl5.timex\endcsname{25.9}
\expandafter\gdef\csname R@an.published.pub.mednextl5.vram\endcsname{18.0}
\expandafter\gdef\csname R@an.published.pub.nnformer.arch\endcsname{TF}
\expandafter\gdef\csname R@an.published.pub.nnformer.gain.acdc\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.published.pub.nnformer.gain.amos\endcsname{\ensuremath{-7.09}}
\expandafter\gdef\csname R@an.published.pub.nnformer.gain.kits\endcsname{\ensuremath{-10.19}}
\expandafter\gdef\csname R@an.published.pub.nnformer.hours\endcsname{8}
\expandafter\gdef\csname R@an.published.pub.nnformer.name\endcsname{nnFormer}
\expandafter\gdef\csname R@an.published.pub.nnformer.timex\endcsname{0.9}
\expandafter\gdef\csname R@an.published.pub.nnformer.vram\endcsname{5.7}
\expandafter\gdef\csname R@an.published.pub.nnunet.arch\endcsname{CNN}
\expandafter\gdef\csname R@an.published.pub.nnunet.gain.acdc\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.published.pub.nnunet.gain.amos\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.published.pub.nnunet.gain.kits\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.published.pub.nnunet.hours\endcsname{9}
\expandafter\gdef\csname R@an.published.pub.nnunet.name\endcsname{nnU-Net (orig.)}
\expandafter\gdef\csname R@an.published.pub.nnunet.timex\endcsname{1.0}
\expandafter\gdef\csname R@an.published.pub.nnunet.vram\endcsname{7.7}
\expandafter\gdef\csname R@an.published.pub.resencl.arch\endcsname{CNN}
\expandafter\gdef\csname R@an.published.pub.resencl.gain.acdc\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.published.pub.resencl.gain.amos\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.published.pub.resencl.gain.kits\endcsname{\ensuremath{+2.13}}
\expandafter\gdef\csname R@an.published.pub.resencl.hours\endcsname{35}
\expandafter\gdef\csname R@an.published.pub.resencl.name\endcsname{nnU-Net ResEnc-L}
\expandafter\gdef\csname R@an.published.pub.resencl.timex\endcsname{3.9}
\expandafter\gdef\csname R@an.published.pub.resencl.vram\endcsname{22.7}
\expandafter\gdef\csname R@an.published.pub.resencm.arch\endcsname{CNN}
\expandafter\gdef\csname R@an.published.pub.resencm.gain.acdc\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.published.pub.resencm.gain.amos\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.published.pub.resencm.gain.kits\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.published.pub.resencm.hours\endcsname{12}
\expandafter\gdef\csname R@an.published.pub.resencm.name\endcsname{nnU-Net ResEnc-M}
\expandafter\gdef\csname R@an.published.pub.resencm.timex\endcsname{1.3}
\expandafter\gdef\csname R@an.published.pub.resencm.vram\endcsname{9.1}
\expandafter\gdef\csname R@an.published.pub.resencxl.arch\endcsname{CNN}
\expandafter\gdef\csname R@an.published.pub.resencxl.gain.acdc\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.published.pub.resencxl.gain.amos\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@an.published.pub.resencxl.gain.kits\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@an.published.pub.resencxl.hours\endcsname{66}
\expandafter\gdef\csname R@an.published.pub.resencxl.name\endcsname{nnU-Net ResEnc-XL}
\expandafter\gdef\csname R@an.published.pub.resencxl.timex\endcsname{7.3}
\expandafter\gdef\csname R@an.published.pub.resencxl.vram\endcsname{36.6}
\expandafter\gdef\csname R@an.published.pub.stunetl.arch\endcsname{CNN}
\expandafter\gdef\csname R@an.published.pub.stunetl.gain.acdc\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.published.pub.stunetl.gain.amos\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.published.pub.stunetl.gain.kits\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.published.pub.stunetl.hours\endcsname{51}
\expandafter\gdef\csname R@an.published.pub.stunetl.name\endcsname{STU-Net-L}
\expandafter\gdef\csname R@an.published.pub.stunetl.timex\endcsname{5.7}
\expandafter\gdef\csname R@an.published.pub.stunetl.vram\endcsname{26.5}
\expandafter\gdef\csname R@an.published.pub.swinunetrv2.arch\endcsname{TF}
\expandafter\gdef\csname R@an.published.pub.swinunetrv2.gain.acdc\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.published.pub.swinunetrv2.gain.amos\endcsname{\ensuremath{-2.40}}
\expandafter\gdef\csname R@an.published.pub.swinunetrv2.gain.kits\endcsname{\ensuremath{-1.90}}
\expandafter\gdef\csname R@an.published.pub.swinunetrv2.hours\endcsname{15}
\expandafter\gdef\csname R@an.published.pub.swinunetrv2.name\endcsname{SwinUNETR-V2}
\expandafter\gdef\csname R@an.published.pub.swinunetrv2.timex\endcsname{1.7}
\expandafter\gdef\csname R@an.published.pub.swinunetrv2.vram\endcsname{13.4}
\expandafter\gdef\csname R@an.published.pub.umambabot.arch\endcsname{Mam}
\expandafter\gdef\csname R@an.published.pub.umambabot.gain.acdc\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.published.pub.umambabot.gain.amos\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.published.pub.umambabot.gain.kits\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.published.pub.umambabot.hours\endcsname{24}
\expandafter\gdef\csname R@an.published.pub.umambabot.name\endcsname{U-Mamba-Bot}
\expandafter\gdef\csname R@an.published.pub.umambabot.timex\endcsname{2.7}
\expandafter\gdef\csname R@an.published.pub.umambabot.vram\endcsname{12.4}
\expandafter\gdef\csname R@an.published.reach.basis\endcsname{over folds 1-4, one seed per fold}
\expandafter\gdef\csname R@an.published.reach.gain\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.published.reach.n\endcsname{4}
\expandafter\gdef\csname R@an.published.reach.names\endcsname{ResEnc-XL, MedNeXt-L k3, ResEnc-L and MedNeXt-L k5}
\expandafter\gdef\csname R@an.published.reach.ntotal\endcsname{18}
\expandafter\gdef\csname R@an.published.reach.time.hi\endcsname{25.9}
\expandafter\gdef\csname R@an.published.reach.time.lo\endcsname{3.9}
\expandafter\gdef\csname R@an.published.reach.vram.hi\endcsname{36.6}
\expandafter\gdef\csname R@an.published.reach.vram.lo\endcsname{17.3}
\expandafter\gdef\csname R@an.published.reach.xa.basis\endcsname{over folds 1-4, one seed per fold}
\expandafter\gdef\csname R@an.published.reach.xa.gain\endcsname{\ensuremath{+1.63}}
\expandafter\gdef\csname R@an.published.reach.xa.n\endcsname{4}
\expandafter\gdef\csname R@an.published.reach.xa.names\endcsname{ResEnc-XL, MedNeXt-L k3, ResEnc-L and MedNeXt-L k5}
\expandafter\gdef\csname R@an.published.reach.xa.ntotal\endcsname{18}
\expandafter\gdef\csname R@an.published.reach.xa.time.hi\endcsname{25.9}
\expandafter\gdef\csname R@an.published.reach.xa.time.lo\endcsname{3.9}
\expandafter\gdef\csname R@an.published.reach.xa.vram.hi\endcsname{36.6}
\expandafter\gdef\csname R@an.published.reach.xa.vram.lo\endcsname{17.3}
\expandafter\gdef\csname R@an.published.sent.cap\endcsname{the six published configurations that train within 12\,GB gain at most \ensuremath{+0.75}\,pp on KiTS23 over their own nnU-Net (ResEnc-M)}
\expandafter\gdef\csname R@an.published.sent.reach\endcsname{of the eighteen published configurations of nnU-Net Revisited's Table~1, four have a KiTS23 gain over their own nnU-Net at least as large as {\ifdefined\archL\archL\else XX-Net-L\fi}'s \ensuremath{+0.78}\,pp over ours (over folds 1-4, one seed per fold): ResEnc-XL, MedNeXt-L k3, ResEnc-L and MedNeXt-L k5, trained with 17.3--36.6\,GB of GPU memory and 3.9--25.9$\times$ the training time of their nnU-Net}
\expandafter\gdef\csname R@an.published.sent.reach.xa\endcsname{of the eighteen published configurations of nnU-Net Revisited's Table~1, four have a KiTS23 gain over their own nnU-Net at least as large as {\ifdefined\archA\archA\else XX-Net-A\fi}'s \ensuremath{+1.63}\,pp over ours (over folds 1-4, one seed per fold): ResEnc-XL, MedNeXt-L k3, ResEnc-L and MedNeXt-L k5, trained with 17.3--36.6\,GB of GPU memory and 3.9--25.9$\times$ the training time of their nnU-Net}
\expandafter\gdef\csname R@an.randsearch.alt.amos.mean\endcsname{87.730}
\expandafter\gdef\csname R@an.randsearch.alt.amos.n\endcsname{3}
\expandafter\gdef\csname R@an.randsearch.alt.amos.name\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.randsearch.alt.amos.shift\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.randsearch.alt.amos.short\endcsname{uncompiled}
\expandafter\gdef\csname R@an.randsearch.alt.kits.mean\endcsname{83.622}
\expandafter\gdef\csname R@an.randsearch.alt.kits.n\endcsname{6}
\expandafter\gdef\csname R@an.randsearch.alt.kits.name\endcsname{six-run reference}
\expandafter\gdef\csname R@an.randsearch.alt.kits.shift\endcsname{\ensuremath{+0.244}}
\expandafter\gdef\csname R@an.randsearch.alt.kits.short\endcsname{six-run}
\expandafter\gdef\csname R@an.randsearch.amos.ag.frac\endcsname{28}
\expandafter\gdef\csname R@an.randsearch.amos.ag.k\endcsname{7}
\expandafter\gdef\csname R@an.randsearch.amos.ag.k_alt\endcsname{4}
\expandafter\gdef\csname R@an.randsearch.amos.ag.kfire\endcsname{7}
\expandafter\gdef\csname R@an.randsearch.amos.ag.kn\endcsname{7 of 25}
\expandafter\gdef\csname R@an.randsearch.amos.ag.kn_alt\endcsname{4 of 25}
\expandafter\gdef\csname R@an.randsearch.amos.ag.kn_reg\endcsname{7 of 28}
\expandafter\gdef\csname R@an.randsearch.amos.ag.max\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.randsearch.amos.ag.max_alt\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.randsearch.amos.ag.max_arm\endcsname{HyReX-k9}
\expandafter\gdef\csname R@an.randsearch.amos.ag.mean\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.randsearch.amos.ag.mean_alt\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.randsearch.amos.ag.median\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.randsearch.amos.ag.min\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@an.randsearch.amos.ag.n\endcsname{25}
\expandafter\gdef\csname R@an.randsearch.amos.ag.n_failed\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.amos.ag.n_pend\endcsname{3}
\expandafter\gdef\csname R@an.randsearch.amos.ag.n_queued\endcsname{3}
\expandafter\gdef\csname R@an.randsearch.amos.ag.n_reg\endcsname{28}
\expandafter\gdef\csname R@an.randsearch.amos.ag.n_run\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.amos.ag.names_clear\endcsname{ConvNeXt-k3, \textbf{HyReX}, ResEnc+context, HyReX, finer ConvNeXt, HyReX+dec. capacity, LeanDeepMid+FD, HyReX-k9}
\expandafter\gdef\csname R@an.randsearch.amos.ag.sd\endcsname{0.39}
\expandafter\gdef\csname R@an.randsearch.amos.ag.state\endcsname{partial}
\expandafter\gdef\csname R@an.randsearch.amos.max\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.amos.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.amos.min\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.amos.n\endcsname{5}
\expandafter\gdef\csname R@an.randsearch.amos.n_adm\endcsname{5}
\expandafter\gdef\csname R@an.randsearch.amos.n_fin\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.amos.pct_L1\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.amos.pct_L3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.amos.rank_L1\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.amos.rank_L3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.amos.rs.frac\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.amos.rs.k\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.amos.rs.k_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.amos.rs.kfire\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.amos.rs.kn\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.amos.rs.kn_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.amos.rs.kn_reg\endcsname{0 of 5}
\expandafter\gdef\csname R@an.randsearch.amos.rs.max\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.amos.rs.max_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.amos.rs.max_arm\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.amos.rs.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.amos.rs.mean_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.amos.rs.median\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.amos.rs.min\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.amos.rs.n\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.amos.rs.n_failed\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.amos.rs.n_pend\endcsname{5}
\expandafter\gdef\csname R@an.randsearch.amos.rs.n_queued\endcsname{3}
\expandafter\gdef\csname R@an.randsearch.amos.rs.n_reg\endcsname{5}
\expandafter\gdef\csname R@an.randsearch.amos.rs.n_run\endcsname{2}
\expandafter\gdef\csname R@an.randsearch.amos.rs.names_clear\endcsname{none}
\expandafter\gdef\csname R@an.randsearch.amos.rs.sd\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.amos.rs.state\endcsname{pending}
\expandafter\gdef\csname R@an.randsearch.amos.sd\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.C1.amos.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.C1.amos.d0\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.randsearch.arm.C1.amos.d0_3\endcsname{\ensuremath{+0.390}}
\expandafter\gdef\csname R@an.randsearch.arm.C1.amos.d0_alt\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.randsearch.arm.C1.amos.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.C1.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.C1.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.C1.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.C1.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.C1.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.C1.kits.d0\endcsname{\ensuremath{+3.51}}
\expandafter\gdef\csname R@an.randsearch.arm.C1.kits.d0_3\endcsname{\ensuremath{+3.507}}
\expandafter\gdef\csname R@an.randsearch.arm.C1.kits.d0_alt\endcsname{\ensuremath{+3.26}}
\expandafter\gdef\csname R@an.randsearch.arm.C1.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.C1.kits.fresh\endcsname{\ensuremath{+2.40}}
\expandafter\gdef\csname R@an.randsearch.arm.C1.kits.fresh_alt\endcsname{\ensuremath{+2.16}}
\expandafter\gdef\csname R@an.randsearch.arm.C1.kits.move\endcsname{\ensuremath{-1.11}}
\expandafter\gdef\csname R@an.randsearch.arm.C1.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.D1.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.D1.amos.d0\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.randsearch.arm.D1.amos.d0_3\endcsname{\ensuremath{+0.278}}
\expandafter\gdef\csname R@an.randsearch.arm.D1.amos.d0_alt\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.randsearch.arm.D1.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.D1.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.D1.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.D1.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.D1.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.D1.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.D1.kits.d0\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.randsearch.arm.D1.kits.d0_3\endcsname{\ensuremath{+1.607}}
\expandafter\gdef\csname R@an.randsearch.arm.D1.kits.d0_alt\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.randsearch.arm.D1.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.D1.kits.fresh\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.randsearch.arm.D1.kits.fresh_alt\endcsname{\ensuremath{+1.23}}
\expandafter\gdef\csname R@an.randsearch.arm.D1.kits.move\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.randsearch.arm.D1.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.D2.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.D2.amos.d0\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.randsearch.arm.D2.amos.d0_3\endcsname{\ensuremath{-0.362}}
\expandafter\gdef\csname R@an.randsearch.arm.D2.amos.d0_alt\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@an.randsearch.arm.D2.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.D2.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.D2.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.D2.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.D2.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.D2.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.D2.kits.d0\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.randsearch.arm.D2.kits.d0_3\endcsname{\ensuremath{+2.355}}
\expandafter\gdef\csname R@an.randsearch.arm.D2.kits.d0_alt\endcsname{\ensuremath{+2.11}}
\expandafter\gdef\csname R@an.randsearch.arm.D2.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.D2.kits.fresh\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.randsearch.arm.D2.kits.fresh_alt\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.randsearch.arm.D2.kits.move\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.randsearch.arm.D2.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.L1.amos.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L1.amos.d0\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.randsearch.arm.L1.amos.d0_3\endcsname{\ensuremath{+0.647}}
\expandafter\gdef\csname R@an.randsearch.arm.L1.amos.d0_alt\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.randsearch.arm.L1.amos.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L1.amos.fresh\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.randsearch.arm.L1.amos.fresh_alt\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.randsearch.arm.L1.amos.move\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.randsearch.arm.L1.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.L1.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L1.kits.d0\endcsname{\ensuremath{+2.33}}
\expandafter\gdef\csname R@an.randsearch.arm.L1.kits.d0_3\endcsname{\ensuremath{+2.326}}
\expandafter\gdef\csname R@an.randsearch.arm.L1.kits.d0_alt\endcsname{\ensuremath{+2.08}}
\expandafter\gdef\csname R@an.randsearch.arm.L1.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L1.kits.fresh\endcsname{\ensuremath{+3.48}}
\expandafter\gdef\csname R@an.randsearch.arm.L1.kits.fresh_alt\endcsname{\ensuremath{+3.23}}
\expandafter\gdef\csname R@an.randsearch.arm.L1.kits.move\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.randsearch.arm.L1.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.L1b.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.L1b.amos.d0\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.randsearch.arm.L1b.amos.d0_3\endcsname{\ensuremath{+0.138}}
\expandafter\gdef\csname R@an.randsearch.arm.L1b.amos.d0_alt\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.randsearch.arm.L1b.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.L1b.amos.fresh\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.randsearch.arm.L1b.amos.fresh_alt\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.randsearch.arm.L1b.amos.move\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.randsearch.arm.L1b.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.L1b.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L1b.kits.d0\endcsname{\ensuremath{+1.74}}
\expandafter\gdef\csname R@an.randsearch.arm.L1b.kits.d0_3\endcsname{\ensuremath{+1.743}}
\expandafter\gdef\csname R@an.randsearch.arm.L1b.kits.d0_alt\endcsname{\ensuremath{+1.50}}
\expandafter\gdef\csname R@an.randsearch.arm.L1b.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L1b.kits.fresh\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.randsearch.arm.L1b.kits.fresh_alt\endcsname{\ensuremath{+2.07}}
\expandafter\gdef\csname R@an.randsearch.arm.L1b.kits.move\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.randsearch.arm.L1b.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.L2.amos.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L2.amos.d0\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.randsearch.arm.L2.amos.d0_3\endcsname{\ensuremath{+0.362}}
\expandafter\gdef\csname R@an.randsearch.arm.L2.amos.d0_alt\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.randsearch.arm.L2.amos.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L2.amos.fresh\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.randsearch.arm.L2.amos.fresh_alt\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.randsearch.arm.L2.amos.move\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.randsearch.arm.L2.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.L2.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L2.kits.d0\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.randsearch.arm.L2.kits.d0_3\endcsname{\ensuremath{+0.664}}
\expandafter\gdef\csname R@an.randsearch.arm.L2.kits.d0_alt\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.randsearch.arm.L2.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L2.kits.fresh\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.randsearch.arm.L2.kits.fresh_alt\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.randsearch.arm.L2.kits.move\endcsname{\ensuremath{-0.55}}
\expandafter\gdef\csname R@an.randsearch.arm.L2.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.L3.amos.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L3.amos.d0\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.randsearch.arm.L3.amos.d0_3\endcsname{\ensuremath{+0.382}}
\expandafter\gdef\csname R@an.randsearch.arm.L3.amos.d0_alt\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.randsearch.arm.L3.amos.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L3.amos.fresh\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.randsearch.arm.L3.amos.fresh_alt\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.randsearch.arm.L3.amos.move\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.randsearch.arm.L3.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.L3.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L3.kits.d0\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.randsearch.arm.L3.kits.d0_3\endcsname{\ensuremath{+2.842}}
\expandafter\gdef\csname R@an.randsearch.arm.L3.kits.d0_alt\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@an.randsearch.arm.L3.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L3.kits.fresh\endcsname{\ensuremath{+2.09}}
\expandafter\gdef\csname R@an.randsearch.arm.L3.kits.fresh_alt\endcsname{\ensuremath{+1.85}}
\expandafter\gdef\csname R@an.randsearch.arm.L3.kits.move\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.randsearch.arm.L3.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_L.amos.clears\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_L.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_L.amos.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_L.amos.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_L.amos.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_L.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_L.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_L.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_L.amos.state\endcsname{queued}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_L.kits.clears\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_L.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_L.kits.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_L.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_L.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_L.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_L.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_L.kits.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_L.kits.state\endcsname{queued}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_M.amos.clears\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_M.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_M.amos.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_M.amos.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_M.amos.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_M.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_M.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_M.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_M.amos.state\endcsname{queued}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_M.kits.clears\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_M.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_M.kits.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_M.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_M.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_M.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_M.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_M.kits.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L3w_M.kits.state\endcsname{queued}
\expandafter\gdef\csname R@an.randsearch.arm.L4.amos.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L4.amos.d0\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.randsearch.arm.L4.amos.d0_3\endcsname{\ensuremath{+0.430}}
\expandafter\gdef\csname R@an.randsearch.arm.L4.amos.d0_alt\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.randsearch.arm.L4.amos.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L4.amos.fresh\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.randsearch.arm.L4.amos.fresh_alt\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.randsearch.arm.L4.amos.move\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.randsearch.arm.L4.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.L4.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L4.kits.d0\endcsname{\ensuremath{+2.20}}
\expandafter\gdef\csname R@an.randsearch.arm.L4.kits.d0_3\endcsname{\ensuremath{+2.198}}
\expandafter\gdef\csname R@an.randsearch.arm.L4.kits.d0_alt\endcsname{\ensuremath{+1.95}}
\expandafter\gdef\csname R@an.randsearch.arm.L4.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L4.kits.fresh\endcsname{\ensuremath{+2.25}}
\expandafter\gdef\csname R@an.randsearch.arm.L4.kits.fresh_alt\endcsname{\ensuremath{+2.00}}
\expandafter\gdef\csname R@an.randsearch.arm.L4.kits.move\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.randsearch.arm.L4.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.L6.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.L6.amos.d0\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.randsearch.arm.L6.amos.d0_3\endcsname{\ensuremath{+0.016}}
\expandafter\gdef\csname R@an.randsearch.arm.L6.amos.d0_alt\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.randsearch.arm.L6.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.L6.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L6.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L6.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.L6.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.L6.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L6.kits.d0\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.randsearch.arm.L6.kits.d0_3\endcsname{\ensuremath{+2.526}}
\expandafter\gdef\csname R@an.randsearch.arm.L6.kits.d0_alt\endcsname{\ensuremath{+2.28}}
\expandafter\gdef\csname R@an.randsearch.arm.L6.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.L6.kits.fresh\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.randsearch.arm.L6.kits.fresh_alt\endcsname{\ensuremath{+1.35}}
\expandafter\gdef\csname R@an.randsearch.arm.L6.kits.move\endcsname{\ensuremath{-0.93}}
\expandafter\gdef\csname R@an.randsearch.arm.L6.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.N1.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.N1.amos.d0\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@an.randsearch.arm.N1.amos.d0_3\endcsname{\ensuremath{-0.923}}
\expandafter\gdef\csname R@an.randsearch.arm.N1.amos.d0_alt\endcsname{\ensuremath{-0.95}}
\expandafter\gdef\csname R@an.randsearch.arm.N1.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.N1.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.N1.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.N1.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.N1.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.N1.kits.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.N1.kits.d0\endcsname{\ensuremath{-6.49}}
\expandafter\gdef\csname R@an.randsearch.arm.N1.kits.d0_3\endcsname{\ensuremath{-6.492}}
\expandafter\gdef\csname R@an.randsearch.arm.N1.kits.d0_alt\endcsname{\ensuremath{-6.74}}
\expandafter\gdef\csname R@an.randsearch.arm.N1.kits.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.N1.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.N1.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.N1.kits.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.N1.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.P1_frcap32.amos.clears\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1_frcap32.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1_frcap32.amos.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1_frcap32.amos.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1_frcap32.amos.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1_frcap32.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1_frcap32.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1_frcap32.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1_frcap32.amos.state\endcsname{queued}
\expandafter\gdef\csname R@an.randsearch.arm.P1_frcap32.kits.clears\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1_frcap32.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1_frcap32.kits.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1_frcap32.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1_frcap32.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1_frcap32.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1_frcap32.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1_frcap32.kits.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1_frcap32.kits.state\endcsname{queued}
\expandafter\gdef\csname R@an.randsearch.arm.P1b.amos.clears\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1b.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1b.amos.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1b.amos.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1b.amos.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1b.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1b.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1b.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1b.amos.state\endcsname{queued}
\expandafter\gdef\csname R@an.randsearch.arm.P1c.amos.clears\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1c.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1c.amos.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1c.amos.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1c.amos.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1c.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1c.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1c.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1c.amos.state\endcsname{queued}
\expandafter\gdef\csname R@an.randsearch.arm.P1c.kits.clears\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1c.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1c.kits.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1c.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1c.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1c.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1c.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1c.kits.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P1c.kits.state\endcsname{queued}
\expandafter\gdef\csname R@an.randsearch.arm.P3c.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.P3c.amos.d0\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.randsearch.arm.P3c.amos.d0_3\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.randsearch.arm.P3c.amos.d0_alt\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.randsearch.arm.P3c.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.P3c.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P3c.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P3c.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P3c.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.P3c.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.P3c.kits.d0\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.randsearch.arm.P3c.kits.d0_3\endcsname{\ensuremath{+1.364}}
\expandafter\gdef\csname R@an.randsearch.arm.P3c.kits.d0_alt\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.randsearch.arm.P3c.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.P3c.kits.fresh\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.randsearch.arm.P3c.kits.fresh_alt\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.randsearch.arm.P3c.kits.move\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.randsearch.arm.P3c.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.P3lite.amos.clears\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P3lite.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P3lite.amos.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P3lite.amos.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P3lite.amos.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P3lite.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P3lite.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P3lite.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P3lite.amos.state\endcsname{queued}
\expandafter\gdef\csname R@an.randsearch.arm.P3lite.kits.clears\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P3lite.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P3lite.kits.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P3lite.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P3lite.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P3lite.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P3lite.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P3lite.kits.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.P3lite.kits.state\endcsname{queued}
\expandafter\gdef\csname R@an.randsearch.arm.S2.amos.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.S2.amos.d0\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.randsearch.arm.S2.amos.d0_3\endcsname{\ensuremath{+0.378}}
\expandafter\gdef\csname R@an.randsearch.arm.S2.amos.d0_alt\endcsname{\ensuremath{+0.349}}
\expandafter\gdef\csname R@an.randsearch.arm.S2.amos.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.S2.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.S2.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.S2.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.S2.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.S2.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.S2.kits.d0\endcsname{\ensuremath{+1.34}}
\expandafter\gdef\csname R@an.randsearch.arm.S2.kits.d0_3\endcsname{\ensuremath{+1.341}}
\expandafter\gdef\csname R@an.randsearch.arm.S2.kits.d0_alt\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@an.randsearch.arm.S2.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.S2.kits.fresh\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.randsearch.arm.S2.kits.fresh_alt\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.randsearch.arm.S2.kits.move\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.randsearch.arm.S2.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.SP1.amos.clears\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP1.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP1.amos.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP1.amos.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP1.amos.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP1.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP1.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP1.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP1.amos.state\endcsname{queued}
\expandafter\gdef\csname R@an.randsearch.arm.SP1.kits.clears\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP1.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP1.kits.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP1.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP1.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP1.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP1.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP1.kits.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP1.kits.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.arm.SP2.amos.clears\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP2.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP2.amos.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP2.amos.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP2.amos.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP2.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP2.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP2.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP2.amos.state\endcsname{queued}
\expandafter\gdef\csname R@an.randsearch.arm.SP2.kits.clears\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP2.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP2.kits.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP2.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP2.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP2.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP2.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP2.kits.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.SP2.kits.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.arm.V5A5.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V5A5.amos.d0\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.randsearch.arm.V5A5.amos.d0_3\endcsname{\ensuremath{+0.041}}
\expandafter\gdef\csname R@an.randsearch.arm.V5A5.amos.d0_alt\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.randsearch.arm.V5A5.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V5A5.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V5A5.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V5A5.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V5A5.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V5A5.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V5A5.kits.d0\endcsname{\ensuremath{+1.95}}
\expandafter\gdef\csname R@an.randsearch.arm.V5A5.kits.d0_3\endcsname{\ensuremath{+1.949}}
\expandafter\gdef\csname R@an.randsearch.arm.V5A5.kits.d0_alt\endcsname{\ensuremath{+1.71}}
\expandafter\gdef\csname R@an.randsearch.arm.V5A5.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V5A5.kits.fresh\endcsname{\ensuremath{+2.17}}
\expandafter\gdef\csname R@an.randsearch.arm.V5A5.kits.fresh_alt\endcsname{\ensuremath{+1.92}}
\expandafter\gdef\csname R@an.randsearch.arm.V5A5.kits.move\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.randsearch.arm.V5A5.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V5B1.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V5B1.amos.d0\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.randsearch.arm.V5B1.amos.d0_3\endcsname{\ensuremath{-0.261}}
\expandafter\gdef\csname R@an.randsearch.arm.V5B1.amos.d0_alt\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.randsearch.arm.V5B1.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V5B1.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V5B1.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V5B1.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V5B1.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V5B1.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V5B1.kits.d0\endcsname{\ensuremath{+2.16}}
\expandafter\gdef\csname R@an.randsearch.arm.V5B1.kits.d0_3\endcsname{\ensuremath{+2.162}}
\expandafter\gdef\csname R@an.randsearch.arm.V5B1.kits.d0_alt\endcsname{\ensuremath{+1.92}}
\expandafter\gdef\csname R@an.randsearch.arm.V5B1.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V5B1.kits.fresh\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.randsearch.arm.V5B1.kits.fresh_alt\endcsname{\ensuremath{+2.04}}
\expandafter\gdef\csname R@an.randsearch.arm.V5B1.kits.move\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.randsearch.arm.V5B1.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V5B2.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V5B2.amos.d0\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.randsearch.arm.V5B2.amos.d0_3\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.randsearch.arm.V5B2.amos.d0_alt\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.randsearch.arm.V5B2.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V5B2.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V5B2.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V5B2.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V5B2.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V5B2.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V5B2.kits.d0\endcsname{\ensuremath{+1.26}}
\expandafter\gdef\csname R@an.randsearch.arm.V5B2.kits.d0_3\endcsname{\ensuremath{+1.264}}
\expandafter\gdef\csname R@an.randsearch.arm.V5B2.kits.d0_alt\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.randsearch.arm.V5B2.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V5B2.kits.fresh\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@an.randsearch.arm.V5B2.kits.fresh_alt\endcsname{\ensuremath{+1.20}}
\expandafter\gdef\csname R@an.randsearch.arm.V5B2.kits.move\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.randsearch.arm.V5B2.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V6A1r.amos.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V6A1r.amos.d0\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.randsearch.arm.V6A1r.amos.d0_3\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.randsearch.arm.V6A1r.amos.d0_alt\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.randsearch.arm.V6A1r.amos.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V6A1r.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V6A1r.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V6A1r.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V6A1r.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V6A1r.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V6A1r.kits.d0\endcsname{\ensuremath{+2.24}}
\expandafter\gdef\csname R@an.randsearch.arm.V6A1r.kits.d0_3\endcsname{\ensuremath{+2.236}}
\expandafter\gdef\csname R@an.randsearch.arm.V6A1r.kits.d0_alt\endcsname{\ensuremath{+1.99}}
\expandafter\gdef\csname R@an.randsearch.arm.V6A1r.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V6A1r.kits.fresh\endcsname{\ensuremath{+1.70}}
\expandafter\gdef\csname R@an.randsearch.arm.V6A1r.kits.fresh_alt\endcsname{\ensuremath{+1.46}}
\expandafter\gdef\csname R@an.randsearch.arm.V6A1r.kits.move\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.randsearch.arm.V6A1r.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V7A1.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V7A1.amos.d0\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.randsearch.arm.V7A1.amos.d0_3\endcsname{\ensuremath{-0.045}}
\expandafter\gdef\csname R@an.randsearch.arm.V7A1.amos.d0_alt\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.randsearch.arm.V7A1.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V7A1.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V7A1.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V7A1.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V7A1.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V7A1.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V7A1.kits.d0\endcsname{\ensuremath{+2.55}}
\expandafter\gdef\csname R@an.randsearch.arm.V7A1.kits.d0_3\endcsname{\ensuremath{+2.548}}
\expandafter\gdef\csname R@an.randsearch.arm.V7A1.kits.d0_alt\endcsname{\ensuremath{+2.30}}
\expandafter\gdef\csname R@an.randsearch.arm.V7A1.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V7A1.kits.fresh\endcsname{\ensuremath{+2.66}}
\expandafter\gdef\csname R@an.randsearch.arm.V7A1.kits.fresh_alt\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.randsearch.arm.V7A1.kits.move\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.randsearch.arm.V7A1.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V7A2.amos.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V7A2.amos.d0\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.randsearch.arm.V7A2.amos.d0_3\endcsname{\ensuremath{+0.359}}
\expandafter\gdef\csname R@an.randsearch.arm.V7A2.amos.d0_alt\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.randsearch.arm.V7A2.amos.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V7A2.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V7A2.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V7A2.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V7A2.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V7A2.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V7A2.kits.d0\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.randsearch.arm.V7A2.kits.d0_3\endcsname{\ensuremath{+2.886}}
\expandafter\gdef\csname R@an.randsearch.arm.V7A2.kits.d0_alt\endcsname{\ensuremath{+2.64}}
\expandafter\gdef\csname R@an.randsearch.arm.V7A2.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V7A2.kits.fresh\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.randsearch.arm.V7A2.kits.fresh_alt\endcsname{\ensuremath{+2.05}}
\expandafter\gdef\csname R@an.randsearch.arm.V7A2.kits.move\endcsname{\ensuremath{-0.60}}
\expandafter\gdef\csname R@an.randsearch.arm.V7A2.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V7B1.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V7B1.amos.d0\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.randsearch.arm.V7B1.amos.d0_3\endcsname{\ensuremath{-0.436}}
\expandafter\gdef\csname R@an.randsearch.arm.V7B1.amos.d0_alt\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.randsearch.arm.V7B1.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V7B1.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V7B1.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V7B1.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V7B1.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V7B1.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V7B1.kits.d0\endcsname{\ensuremath{+1.72}}
\expandafter\gdef\csname R@an.randsearch.arm.V7B1.kits.d0_3\endcsname{\ensuremath{+1.721}}
\expandafter\gdef\csname R@an.randsearch.arm.V7B1.kits.d0_alt\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.randsearch.arm.V7B1.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V7B1.kits.fresh\endcsname{\ensuremath{+2.38}}
\expandafter\gdef\csname R@an.randsearch.arm.V7B1.kits.fresh_alt\endcsname{\ensuremath{+2.14}}
\expandafter\gdef\csname R@an.randsearch.arm.V7B1.kits.move\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.randsearch.arm.V7B1.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V7B2.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V7B2.amos.d0\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.randsearch.arm.V7B2.amos.d0_3\endcsname{\ensuremath{-0.267}}
\expandafter\gdef\csname R@an.randsearch.arm.V7B2.amos.d0_alt\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.randsearch.arm.V7B2.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V7B2.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V7B2.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V7B2.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V7B2.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V7B2.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V7B2.kits.d0\endcsname{\ensuremath{+2.82}}
\expandafter\gdef\csname R@an.randsearch.arm.V7B2.kits.d0_3\endcsname{\ensuremath{+2.824}}
\expandafter\gdef\csname R@an.randsearch.arm.V7B2.kits.d0_alt\endcsname{\ensuremath{+2.58}}
\expandafter\gdef\csname R@an.randsearch.arm.V7B2.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V7B2.kits.fresh\endcsname{\ensuremath{+1.84}}
\expandafter\gdef\csname R@an.randsearch.arm.V7B2.kits.fresh_alt\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.randsearch.arm.V7B2.kits.move\endcsname{\ensuremath{-0.99}}
\expandafter\gdef\csname R@an.randsearch.arm.V7B2.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V7C1.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V7C1.amos.d0\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.randsearch.arm.V7C1.amos.d0_3\endcsname{\ensuremath{-0.106}}
\expandafter\gdef\csname R@an.randsearch.arm.V7C1.amos.d0_alt\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.randsearch.arm.V7C1.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V7C1.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V7C1.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V7C1.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V7C1.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V7C1.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V7C1.kits.d0\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.randsearch.arm.V7C1.kits.d0_3\endcsname{\ensuremath{+2.707}}
\expandafter\gdef\csname R@an.randsearch.arm.V7C1.kits.d0_alt\endcsname{\ensuremath{+2.46}}
\expandafter\gdef\csname R@an.randsearch.arm.V7C1.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V7C1.kits.fresh\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@an.randsearch.arm.V7C1.kits.fresh_alt\endcsname{\ensuremath{+2.20}}
\expandafter\gdef\csname R@an.randsearch.arm.V7C1.kits.move\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.randsearch.arm.V7C1.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V8A1.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V8A1.amos.d0\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.randsearch.arm.V8A1.amos.d0_3\endcsname{\ensuremath{-0.505}}
\expandafter\gdef\csname R@an.randsearch.arm.V8A1.amos.d0_alt\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.randsearch.arm.V8A1.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V8A1.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V8A1.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V8A1.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V8A1.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V8A1.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V8A1.kits.d0\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.randsearch.arm.V8A1.kits.d0_3\endcsname{\ensuremath{+1.760}}
\expandafter\gdef\csname R@an.randsearch.arm.V8A1.kits.d0_alt\endcsname{\ensuremath{+1.52}}
\expandafter\gdef\csname R@an.randsearch.arm.V8A1.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V8A1.kits.fresh\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.randsearch.arm.V8A1.kits.fresh_alt\endcsname{\ensuremath{+1.01}}
\expandafter\gdef\csname R@an.randsearch.arm.V8A1.kits.move\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.randsearch.arm.V8A1.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V8A2.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V8A2.amos.d0\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.randsearch.arm.V8A2.amos.d0_3\endcsname{\ensuremath{-0.312}}
\expandafter\gdef\csname R@an.randsearch.arm.V8A2.amos.d0_alt\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.randsearch.arm.V8A2.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V8A2.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V8A2.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V8A2.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V8A2.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V8A2.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V8A2.kits.d0\endcsname{\ensuremath{+1.35}}
\expandafter\gdef\csname R@an.randsearch.arm.V8A2.kits.d0_3\endcsname{\ensuremath{+1.353}}
\expandafter\gdef\csname R@an.randsearch.arm.V8A2.kits.d0_alt\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.randsearch.arm.V8A2.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V8A2.kits.fresh\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@an.randsearch.arm.V8A2.kits.fresh_alt\endcsname{\ensuremath{+1.63}}
\expandafter\gdef\csname R@an.randsearch.arm.V8A2.kits.move\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.randsearch.arm.V8A2.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V8B1.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V8B1.amos.d0\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.randsearch.arm.V8B1.amos.d0_3\endcsname{\ensuremath{-0.751}}
\expandafter\gdef\csname R@an.randsearch.arm.V8B1.amos.d0_alt\endcsname{\ensuremath{-0.78}}
\expandafter\gdef\csname R@an.randsearch.arm.V8B1.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V8B1.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V8B1.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V8B1.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V8B1.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V8B1.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V8B1.kits.d0\endcsname{\ensuremath{+2.91}}
\expandafter\gdef\csname R@an.randsearch.arm.V8B1.kits.d0_3\endcsname{\ensuremath{+2.911}}
\expandafter\gdef\csname R@an.randsearch.arm.V8B1.kits.d0_alt\endcsname{\ensuremath{+2.67}}
\expandafter\gdef\csname R@an.randsearch.arm.V8B1.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V8B1.kits.fresh\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.randsearch.arm.V8B1.kits.fresh_alt\endcsname{\ensuremath{+1.13}}
\expandafter\gdef\csname R@an.randsearch.arm.V8B1.kits.move\endcsname{\ensuremath{-1.54}}
\expandafter\gdef\csname R@an.randsearch.arm.V8B1.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V8B2.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V8B2.amos.d0\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.randsearch.arm.V8B2.amos.d0_3\endcsname{\ensuremath{-0.287}}
\expandafter\gdef\csname R@an.randsearch.arm.V8B2.amos.d0_alt\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.randsearch.arm.V8B2.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.V8B2.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V8B2.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V8B2.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.V8B2.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.V8B2.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V8B2.kits.d0\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.randsearch.arm.V8B2.kits.d0_3\endcsname{\ensuremath{+1.646}}
\expandafter\gdef\csname R@an.randsearch.arm.V8B2.kits.d0_alt\endcsname{\ensuremath{+1.40}}
\expandafter\gdef\csname R@an.randsearch.arm.V8B2.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.V8B2.kits.fresh\endcsname{\ensuremath{+1.73}}
\expandafter\gdef\csname R@an.randsearch.arm.V8B2.kits.fresh_alt\endcsname{\ensuremath{+1.49}}
\expandafter\gdef\csname R@an.randsearch.arm.V8B2.kits.move\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.randsearch.arm.V8B2.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.W1.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.W1.amos.d0\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.randsearch.arm.W1.amos.d0_3\endcsname{\ensuremath{+0.099}}
\expandafter\gdef\csname R@an.randsearch.arm.W1.amos.d0_alt\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.randsearch.arm.W1.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.W1.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W1.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W1.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W1.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.W1c.amos.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.W1c.amos.d0\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.randsearch.arm.W1c.amos.d0_3\endcsname{\ensuremath{+0.363}}
\expandafter\gdef\csname R@an.randsearch.arm.W1c.amos.d0_alt\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.randsearch.arm.W1c.amos.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.W1c.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W1c.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W1c.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W1c.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.W1c.kits.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.W1c.kits.d0\endcsname{\ensuremath{+2.64}}
\expandafter\gdef\csname R@an.randsearch.arm.W1c.kits.d0_3\endcsname{\ensuremath{+2.636}}
\expandafter\gdef\csname R@an.randsearch.arm.W1c.kits.d0_alt\endcsname{\ensuremath{+2.39}}
\expandafter\gdef\csname R@an.randsearch.arm.W1c.kits.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.W1c.kits.fresh\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.randsearch.arm.W1c.kits.fresh_alt\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.randsearch.arm.W1c.kits.move\endcsname{\ensuremath{-1.57}}
\expandafter\gdef\csname R@an.randsearch.arm.W1c.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.W2.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.W2.amos.d0\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.randsearch.arm.W2.amos.d0_3\endcsname{\ensuremath{+0.211}}
\expandafter\gdef\csname R@an.randsearch.arm.W2.amos.d0_alt\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.randsearch.arm.W2.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.W2.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W2.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W2.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W2.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.W3.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.W3.amos.d0\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.randsearch.arm.W3.amos.d0_3\endcsname{\ensuremath{+0.270}}
\expandafter\gdef\csname R@an.randsearch.arm.W3.amos.d0_alt\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.randsearch.arm.W3.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.W3.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W3.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W3.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W3.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.W3c.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.W3c.amos.d0\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.randsearch.arm.W3c.amos.d0_3\endcsname{\ensuremath{+0.162}}
\expandafter\gdef\csname R@an.randsearch.arm.W3c.amos.d0_alt\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.randsearch.arm.W3c.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.W3c.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W3c.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W3c.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W3c.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.W4.amos.clears\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.W4.amos.d0\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.randsearch.arm.W4.amos.d0_3\endcsname{\ensuremath{+0.076}}
\expandafter\gdef\csname R@an.randsearch.arm.W4.amos.d0_alt\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.randsearch.arm.W4.amos.fires\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.arm.W4.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W4.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W4.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W4.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.arm.W4.kits.clears\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W4.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W4.kits.d0_3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W4.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W4.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W4.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W4.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W4.kits.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W4.kits.state\endcsname{queued}
\expandafter\gdef\csname R@an.randsearch.arm.W5.amos.clears\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.W5.amos.d0\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.randsearch.arm.W5.amos.d0_3\endcsname{\ensuremath{+0.591}}
\expandafter\gdef\csname R@an.randsearch.arm.W5.amos.d0_alt\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.randsearch.arm.W5.amos.fires\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.arm.W5.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W5.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W5.amos.move\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.arm.W5.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.band.amos.elig_hi\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.randsearch.band.amos.elig_lo\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.randsearch.band.amos.elig_width\endcsname{0.51}
\expandafter\gdef\csname R@an.randsearch.band.amos.m\endcsname{7}
\expandafter\gdef\csname R@an.randsearch.band.amos.n_named\endcsname{3}
\expandafter\gdef\csname R@an.randsearch.band.amos.nev_hi\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.randsearch.band.amos.nev_lo\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.randsearch.band.amos.nev_width\endcsname{0.60}
\expandafter\gdef\csname R@an.randsearch.band.amos.plug\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.randsearch.band.amos.src\endcsname{Addendum S1}
\expandafter\gdef\csname R@an.randsearch.band.kits.elig_hi\endcsname{\ensuremath{+0.267}}
\expandafter\gdef\csname R@an.randsearch.band.kits.elig_lo\endcsname{\ensuremath{-5.436}}
\expandafter\gdef\csname R@an.randsearch.band.kits.elig_width\endcsname{5.703}
\expandafter\gdef\csname R@an.randsearch.band.kits.m\endcsname{6}
\expandafter\gdef\csname R@an.randsearch.band.kits.n_named\endcsname{2}
\expandafter\gdef\csname R@an.randsearch.band.kits.nev_hi\endcsname{\ensuremath{+2.834}}
\expandafter\gdef\csname R@an.randsearch.band.kits.nev_lo\endcsname{\ensuremath{-2.837}}
\expandafter\gdef\csname R@an.randsearch.band.kits.nev_width\endcsname{5.671}
\expandafter\gdef\csname R@an.randsearch.band.kits.plug\endcsname{\ensuremath{-1.006}}
\expandafter\gdef\csname R@an.randsearch.band.kits.src\endcsname{Addendum V4}
\expandafter\gdef\csname R@an.randsearch.bar\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.randsearch.bar_ne\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.randsearch.cap_gb\endcsname{12}
\expandafter\gdef\csname R@an.randsearch.clause.cur.amos\endcsname{The current model, the same selection model run at the 25 candidate arms with a seed-0 result on AMOS22, predicts a plug-in movement of \ensuremath{-0.24} pp (5 to 95 percent range [\ensuremath{-0.61}, \ensuremath{-0.07}]); the registered prediction of Addendum S1 (m = 7, plug-in \ensuremath{-0.17} pp) stays the reference for every reading.}
\expandafter\gdef\csname R@an.randsearch.clause.cur.kits\endcsname{The current model, the same selection model run at the 22 candidate arms with a seed-0 result on KiTS23, predicts a plug-in movement of \ensuremath{-1.518} pp (5 to 95 percent range [\ensuremath{-7.287}, \ensuremath{-0.396}]); the registered prediction of Addendum V4 (m = 6, plug-in \ensuremath{-1.006} pp) stays the reference for every reading.}
\expandafter\gdef\csname R@an.randsearch.clause.descriptive\endcsname{At n = 5 admissible designs on AMOS22 and n = 15 on KiTS23, a design with no true effect would clear the screen 0.1 times in expectation on AMOS22 and 5.5 times on KiTS23, so every count is read beside those expectations; the comparison with the agent team is descriptive and is read in counts and seed-0 distributions (Addendum T3).}
\expandafter\gdef\csname R@an.randsearch.clause.dist.amos\endcsname{Seed-0 deltas on AMOS22 against the frozen pool, in pp: no random design has a seed-0 result yet; the 25 finished agent-designed arms have mean \ensuremath{-0.02}, SD 0.39 and maximum \ensuremath{+0.49}. Against the uncompiled sub-pool: agent-arm mean \ensuremath{-0.05} and maximum \ensuremath{+0.46}.}
\expandafter\gdef\csname R@an.randsearch.clause.dist.kits\endcsname{Seed-0 deltas on KiTS23 against the frozen pool, in pp: no random design has a seed-0 result yet; the 22 finished agent-designed arms have mean \ensuremath{+1.75}, SD 1.96 and maximum \ensuremath{+3.51}. Against the six-run reference: agent-arm mean \ensuremath{+1.51} and maximum \ensuremath{+3.26}.}
\expandafter\gdef\csname R@an.randsearch.clause.fresh.amos\endcsname{No Addendum Q2 design has fired the AMOS22 screen so far, so none is owed fresh seeds there.}
\expandafter\gdef\csname R@an.randsearch.clause.fresh.kits\endcsname{No Addendum Q2 design has fired the KiTS23 screen so far, so none is owed fresh seeds there.}
\expandafter\gdef\csname R@an.randsearch.clause.funnel\endcsname{Of the 24 candidates sampled from the agents' own grammar (38 sampler draws, 14 rejected by the AMOS22 parameter window), 10 fit the 12 GB cap on AMOS22 and 21 on KiTS23 (10 on both); 5 and 15 also complete the 1000-epoch budget inside the registered wall-clock limit (5 on both), which registers 20 (design, dataset) runs at seed 0.}
\expandafter\gdef\csname R@an.randsearch.clause.move.amos\endcsname{Addendum S1 registers the reading for 3 arms; 3 of the 3 have a complete fresh pair (ResEnc-matched \ensuremath{+0.16} pp, inside its never-eligible band; ConvNeXt-k3 \ensuremath{-0.17} pp, inside its eligible band; ResEnc+context \ensuremath{+0.03} pp, above its eligible band). 2 complete pairs were visible when the S1 band was written and are descriptions: movement \ensuremath{-0.22} pp on average (range \ensuremath{-0.25} to \ensuremath{-0.18}), 2 of the 2 inside the band of their class. ResEnc+context's first fresh seed had finished when the S1 band was registered, so that reading is partly seen. No random design has finished, so none has fired the screen. The eligible band is the one registered in Addendum S1 (plug-in \ensuremath{-0.17} pp for m = 7 eligible arms at registration); at 6 pool runs it spans 0.51 pp.}
\expandafter\gdef\csname R@an.randsearch.clause.move.kits\endcsname{Addendum V4 registers the reading for 2 arms; 2 of the 2 have a complete fresh pair (branch control \ensuremath{-1.57} pp, inside its never-eligible band; HyReX+dec. capacity \ensuremath{-1.11} pp, inside its eligible band). 7 complete pairs were visible when the V4 band was written and are descriptions: movement \ensuremath{-0.13} pp on average (range \ensuremath{-0.93} to \ensuremath{+1.15}), 7 of the 7 inside the band of their class. 16 further arms with a complete fresh pair are read by the same rule: movement \ensuremath{-0.23} pp on average (range \ensuremath{-1.54} to \ensuremath{+0.66}), 14 of the 16 inside the band of their class. No random design has finished, so none has fired the screen. The eligible band is the one registered in Addendum V4 (plug-in \ensuremath{-1.006} pp for m = 6 eligible arms at registration); at 3 pool runs it spans 5.703 pp.}
\expandafter\gdef\csname R@an.randsearch.clause.p3c.amos\endcsname{On AMOS22, the function-identical PlanNet control, built through the same library path as every design, reads \ensuremath{+0.01} pp (\ensuremath{-0.02} pp against the uncompiled sub-pool) at seed 0 against the frozen pool, inside the 0.50 pp one-seed pair floor, which leaves it not resolved; it does not clear the \ensuremath{+0.35} pp screen. A design's margin is read against the function-identical control; the control's own offset is \ensuremath{+0.01} pp at seed 0 against the frozen pool, which can be nothing but a difference of random realisation.}
\expandafter\gdef\csname R@an.randsearch.clause.p3c.amos.short\endcsname{On AMOS22 the function-identical control reads \ensuremath{+0.01} pp at seed 0, against the frozen pool: its own offset.}
\expandafter\gdef\csname R@an.randsearch.clause.p3c.kits\endcsname{On KiTS23, the function-identical PlanNet control, built through the same library path as every design, reads \ensuremath{+1.36} pp (\ensuremath{+1.12} pp against the six-run reference) at seed 0 against the frozen pool, beyond the 0.50 pp one-seed pair floor; it clears the \ensuremath{+0.35} pp screen. A design's margin is read against the function-identical control; the control's own offset is \ensuremath{+1.36} pp at seed 0 against the frozen pool, which can be nothing but a difference of random realisation. The control's fresh seeds 1 and 2 follow under Addendum T2: the pair is complete.}
\expandafter\gdef\csname R@an.randsearch.clause.p3c.kits.short\endcsname{On KiTS23 the function-identical control reads \ensuremath{+1.36} pp at seed 0 and \ensuremath{+1.18} pp over fresh seeds 1 and 2, against the frozen pool: its own offset.}
\expandafter\gdef\csname R@an.randsearch.clause.rank.amos\endcsname{The position of HyReX and ResEnc-M among the admissible random designs on AMOS22 is read once all 5 have finished (0 so far).}
\expandafter\gdef\csname R@an.randsearch.clause.rank.kits\endcsname{The position of HyReX and ResEnc-M among the admissible random designs on KiTS23 is read once all 15 have finished (0 so far).}
\expandafter\gdef\csname R@an.randsearch.clause.readout.amos\endcsname{On AMOS22, none of the 5 admissible random designs has a seed-0 result yet, while 7 of the 25 finished agent-designed arms clear the \ensuremath{+0.35} pp screen at the discovery seed. 3 of the 28 registered agent-designed arms are still pending. A design with no true effect clears this screen at one seed 2.3\% of the time (0.4 to 16\% across the 95\% interval of the six-run pool SD), which is 0.1 of the 5 admissible random designs in expectation (0.0 to 0.8). Against the uncompiled sub-pool the counts are 4 of 25 for the agent-designed arms.}
\expandafter\gdef\csname R@an.randsearch.clause.readout.kits\endcsname{On KiTS23, none of the 15 admissible random designs has a seed-0 result yet, while 21 of the 22 finished agent-designed arms clear the \ensuremath{+0.35} pp screen at the discovery seed. 2 of the 24 registered agent-designed arms are still pending. A design with no true effect clears this screen at one seed 37\% of the time (27 to 48\% across the 95\% interval of the three-run pool SD), which is 5.5 of the 15 admissible random designs in expectation (4.1 to 7.2). Against the six-run reference the counts are 21 of 22 for the agent-designed arms.}
\expandafter\gdef\csname R@an.randsearch.clause.scaled\endcsname{HyReX-L (99.8 M parameters on the AMOS22 plan) and ResEnc-M (102.3 M) are matched in parameters within 2.4\%. On AMOS22, the HyReX-L run is queued. On KiTS23, the HyReX-L run is queued. The width-scaled variants are new designs and enter the design count (30 designs in the registry); each seed-0 reading is a screening observation, and a variant that clears the screen receives fresh seeds 1 and 2 (Addendum S2).}
\expandafter\gdef\csname R@an.randsearch.clause.sp\endcsname{The two single-prompt designs are two labelled points (seed-0 deltas against the frozen pool): SP1 has no seed-0 result yet on AMOS22 or KiTS23; SP2 has no seed-0 result yet on AMOS22 or KiTS23.}
\expandafter\gdef\csname R@an.randsearch.clause.take.cloud.amos\endcsname{AMOS22, discovery seed 0, designs above the \ensuremath{+0.35} pp screen bar: random designs 0 finished, agent-designed arms 7 of 25 (uncompiled sub-pool: 0 finished and 4 of 25); a design with no true effect clears the bar 2.3\% of the time (0.4 to 16\%; 0.1 of 5 expected, 0.0 to 0.8).}
\expandafter\gdef\csname R@an.randsearch.clause.take.cloud.kits\endcsname{KiTS23, discovery seed 0, designs above the \ensuremath{+0.35} pp screen bar: random designs 0 finished, agent-designed arms 21 of 22 (six-run reference: 0 finished and 21 of 22); a design with no true effect clears the bar 37\% of the time (27 to 48\%; 5.5 of 15 expected, 4.1 to 7.2).}
\expandafter\gdef\csname R@an.randsearch.clause.take.move.amos\endcsname{On AMOS22, 3 of the 3 registered movement readings have a complete fresh pair and 2 of them lie inside their band; the 2 described pairs move \ensuremath{-0.25} to \ensuremath{-0.18} pp against an eligible band 0.51 pp wide.}
\expandafter\gdef\csname R@an.randsearch.clause.take.move.kits\endcsname{On KiTS23, 2 of the 2 registered movement readings have a complete fresh pair and 2 of them lie inside their band; the 7 described pairs move \ensuremath{-0.93} to \ensuremath{+1.15} pp against an eligible band 5.703 pp wide.}
\expandafter\gdef\csname R@an.randsearch.clause.w4\endcsname{The MedNeXt-like reference, built in this harness and never a passer, reads \ensuremath{+0.08} pp on AMOS22 (\ensuremath{+0.05} pp against the uncompiled sub-pool) at seed 0 and has no seed-0 result yet on KiTS23.}
\expandafter\gdef\csname R@an.randsearch.count.agent\endcsname{28}
\expandafter\gdef\csname R@an.randsearch.count.designs\endcsname{30}
\expandafter\gdef\csname R@an.randsearch.count.scaled\endcsname{2}
\expandafter\gdef\csname R@an.randsearch.count.sp\endcsname{2}
\expandafter\gdef\csname R@an.randsearch.count.sp_word\endcsname{two}
\expandafter\gdef\csname R@an.randsearch.cur.amos.hi\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.randsearch.cur.amos.lo\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.randsearch.cur.amos.m\endcsname{25}
\expandafter\gdef\csname R@an.randsearch.cur.amos.nev_hi\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.randsearch.cur.amos.nev_lo\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.randsearch.cur.amos.plug\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.randsearch.cur.kits.hi\endcsname{\ensuremath{-0.396}}
\expandafter\gdef\csname R@an.randsearch.cur.kits.lo\endcsname{\ensuremath{-7.287}}
\expandafter\gdef\csname R@an.randsearch.cur.kits.m\endcsname{22}
\expandafter\gdef\csname R@an.randsearch.cur.kits.nev_hi\endcsname{\ensuremath{+2.834}}
\expandafter\gdef\csname R@an.randsearch.cur.kits.nev_lo\endcsname{\ensuremath{-2.837}}
\expandafter\gdef\csname R@an.randsearch.cur.kits.plug\endcsname{\ensuremath{-1.518}}
\expandafter\gdef\csname R@an.randsearch.epochs\endcsname{1000}
\expandafter\gdef\csname R@an.randsearch.exp.amos.adm\endcsname{0.1}
\expandafter\gdef\csname R@an.randsearch.exp.amos.adm_hi\endcsname{0.8}
\expandafter\gdef\csname R@an.randsearch.exp.amos.adm_lo\endcsname{0.0}
\expandafter\gdef\csname R@an.randsearch.exp.amos.ag\endcsname{0.6}
\expandafter\gdef\csname R@an.randsearch.exp.amos.done\endcsname{0.0}
\expandafter\gdef\csname R@an.randsearch.exp.kits.adm\endcsname{5.5}
\expandafter\gdef\csname R@an.randsearch.exp.kits.adm_hi\endcsname{7.2}
\expandafter\gdef\csname R@an.randsearch.exp.kits.adm_lo\endcsname{4.1}
\expandafter\gdef\csname R@an.randsearch.exp.kits.ag\endcsname{8.1}
\expandafter\gdef\csname R@an.randsearch.exp.kits.done\endcsname{0.0}
\expandafter\gdef\csname R@an.randsearch.floor\endcsname{0.50}
\expandafter\gdef\csname R@an.randsearch.fresh.amos.n_complete\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.fresh.amos.n_fired\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.fresh.amos.n_notqueued\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.fresh.amos.n_owed\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.fresh.amos.n_queued\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.fresh.amos.n_running\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.fresh.amos.names\endcsname{none}
\expandafter\gdef\csname R@an.randsearch.fresh.kits.n_complete\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.fresh.kits.n_fired\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.fresh.kits.n_notqueued\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.fresh.kits.n_owed\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.fresh.kits.n_queued\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.fresh.kits.n_running\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.fresh.kits.names\endcsname{none}
\expandafter\gdef\csname R@an.randsearch.freshseeds\endcsname{seeds 1 and 2}
\expandafter\gdef\csname R@an.randsearch.funnel.adm_amos\endcsname{5}
\expandafter\gdef\csname R@an.randsearch.funnel.adm_both\endcsname{5}
\expandafter\gdef\csname R@an.randsearch.funnel.adm_kits\endcsname{15}
\expandafter\gdef\csname R@an.randsearch.funnel.draws\endcsname{38}
\expandafter\gdef\csname R@an.randsearch.funnel.fit_acdc\endcsname{10}
\expandafter\gdef\csname R@an.randsearch.funnel.fit_all3\endcsname{8}
\expandafter\gdef\csname R@an.randsearch.funnel.fit_amos\endcsname{10}
\expandafter\gdef\csname R@an.randsearch.funnel.fit_both\endcsname{10}
\expandafter\gdef\csname R@an.randsearch.funnel.fit_kits\endcsname{21}
\expandafter\gdef\csname R@an.randsearch.funnel.ids.amos\endcsname{RS07, RS08, RS13, RS15, RS23}
\expandafter\gdef\csname R@an.randsearch.funnel.ids.kits\endcsname{RS01, RS02, RS05, RS07, RS08, RS09, RS11, RS12, RS13, RS15, RS19, RS20, RS22, RS23, RS24}
\expandafter\gdef\csname R@an.randsearch.funnel.iters\endcsname{250000}
\expandafter\gdef\csname R@an.randsearch.funnel.limit.acdc\endcsname{20}
\expandafter\gdef\csname R@an.randsearch.funnel.limit.amos\endcsname{40}
\expandafter\gdef\csname R@an.randsearch.funnel.limit.kits\endcsname{50}
\expandafter\gdef\csname R@an.randsearch.funnel.mult\endcsname{1.10}
\expandafter\gdef\csname R@an.randsearch.funnel.runs\endcsname{20}
\expandafter\gdef\csname R@an.randsearch.funnel.sampled\endcsname{24}
\expandafter\gdef\csname R@an.randsearch.funnel.window_reject\endcsname{14}
\expandafter\gdef\csname R@an.randsearch.head.compare\endcsname{Arm & Params (M) & AMOS22 seed 0 & AMOS22 (uncompiled) & KiTS23 seed 0 & KiTS23 (six-run) & Fresh mean $\Delta$ (uncompiled / six-run), AMOS22 / KiTS23\\}
\expandafter\gdef\csname R@an.randsearch.head.designs\endcsname{Design & Params (M, AMOS22 plan) & AMOS22 stage & KiTS23 stage & AMOS22 $\Delta$ vs frozen pool (uncompiled) & KiTS23 $\Delta$ vs frozen pool (six-run) & Fresh pair\\}
\expandafter\gdef\csname R@an.randsearch.head.funnel\endcsname{Stage & AMOS22 & KiTS23 & Both / total\\}
\expandafter\gdef\csname R@an.randsearch.head.move\endcsname{Arm & Dataset & Class & Basis & Seed 0 $\Delta$ (alt. ref.) & Fresh mean $\Delta$ (alt. ref.) & Movement & Registered band & Reading\\}
\expandafter\gdef\csname R@an.randsearch.head.readout\endcsname{Dataset & Group & Registered & Finished & Clear \ensuremath{+0.35}\,pp & Fire & Mean $\Delta$ (alt. ref.) & SD & Max $\Delta$ (alt. ref.) & Clear (alt. ref.)\\}
\expandafter\gdef\csname R@an.randsearch.kits.ag.frac\endcsname{95}
\expandafter\gdef\csname R@an.randsearch.kits.ag.k\endcsname{21}
\expandafter\gdef\csname R@an.randsearch.kits.ag.k_alt\endcsname{21}
\expandafter\gdef\csname R@an.randsearch.kits.ag.kfire\endcsname{21}
\expandafter\gdef\csname R@an.randsearch.kits.ag.kn\endcsname{21 of 22}
\expandafter\gdef\csname R@an.randsearch.kits.ag.kn_alt\endcsname{21 of 22}
\expandafter\gdef\csname R@an.randsearch.kits.ag.kn_reg\endcsname{21 of 24}
\expandafter\gdef\csname R@an.randsearch.kits.ag.max\endcsname{\ensuremath{+3.51}}
\expandafter\gdef\csname R@an.randsearch.kits.ag.max_alt\endcsname{\ensuremath{+3.26}}
\expandafter\gdef\csname R@an.randsearch.kits.ag.max_arm\endcsname{HyReX+dec. capacity}
\expandafter\gdef\csname R@an.randsearch.kits.ag.mean\endcsname{\ensuremath{+1.75}}
\expandafter\gdef\csname R@an.randsearch.kits.ag.mean_alt\endcsname{\ensuremath{+1.51}}
\expandafter\gdef\csname R@an.randsearch.kits.ag.median\endcsname{\ensuremath{+2.18}}
\expandafter\gdef\csname R@an.randsearch.kits.ag.min\endcsname{\ensuremath{-6.49}}
\expandafter\gdef\csname R@an.randsearch.kits.ag.n\endcsname{22}
\expandafter\gdef\csname R@an.randsearch.kits.ag.n_failed\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.kits.ag.n_pend\endcsname{2}
\expandafter\gdef\csname R@an.randsearch.kits.ag.n_queued\endcsname{2}
\expandafter\gdef\csname R@an.randsearch.kits.ag.n_reg\endcsname{24}
\expandafter\gdef\csname R@an.randsearch.kits.ag.n_run\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.kits.ag.names_clear\endcsname{ConvNeXt-k3, \textbf{HyReX}, ResEnc+context, HyReX+context, HyReX, finer ConvNeXt, HyReX point-fuse, HyReX+dec. capacity, LeanDec, LeanAdd, LeanAdd-NeXt, HyReX-LeanDec, LeanTrunk, Stem1, CoarseStack, StackDec, LeanDeepMid+FD, LeanSep, LeanDil, LeanDeepMid, LeanNeXt-s5, HyReX-k9}
\expandafter\gdef\csname R@an.randsearch.kits.ag.sd\endcsname{1.96}
\expandafter\gdef\csname R@an.randsearch.kits.ag.state\endcsname{partial}
\expandafter\gdef\csname R@an.randsearch.kits.max\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.kits.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.kits.min\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.kits.n\endcsname{15}
\expandafter\gdef\csname R@an.randsearch.kits.n_adm\endcsname{15}
\expandafter\gdef\csname R@an.randsearch.kits.n_fin\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.kits.pct_L1\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.kits.pct_L3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.kits.rank_L1\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.kits.rank_L3\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.kits.rs.frac\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.kits.rs.k\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.kits.rs.k_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.kits.rs.kfire\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.kits.rs.kn\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.kits.rs.kn_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.kits.rs.kn_reg\endcsname{0 of 15}
\expandafter\gdef\csname R@an.randsearch.kits.rs.max\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.kits.rs.max_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.kits.rs.max_arm\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.kits.rs.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.kits.rs.mean_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.kits.rs.median\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.kits.rs.min\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.kits.rs.n\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.kits.rs.n_failed\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.kits.rs.n_pend\endcsname{15}
\expandafter\gdef\csname R@an.randsearch.kits.rs.n_queued\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.kits.rs.n_reg\endcsname{15}
\expandafter\gdef\csname R@an.randsearch.kits.rs.n_run\endcsname{15}
\expandafter\gdef\csname R@an.randsearch.kits.rs.names_clear\endcsname{none}
\expandafter\gdef\csname R@an.randsearch.kits.rs.sd\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.kits.rs.state\endcsname{pending}
\expandafter\gdef\csname R@an.randsearch.kits.sd\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.move.C1.kits.basis\endcsname{registered}
\expandafter\gdef\csname R@an.randsearch.move.C1.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.C1.kits.d0\endcsname{\ensuremath{+3.51}}
\expandafter\gdef\csname R@an.randsearch.move.C1.kits.d0_alt\endcsname{\ensuremath{+3.26}}
\expandafter\gdef\csname R@an.randsearch.move.C1.kits.dist\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.randsearch.move.C1.kits.fresh\endcsname{\ensuremath{+2.40}}
\expandafter\gdef\csname R@an.randsearch.move.C1.kits.fresh_alt\endcsname{\ensuremath{+2.16}}
\expandafter\gdef\csname R@an.randsearch.move.C1.kits.mv\endcsname{\ensuremath{-1.11}}
\expandafter\gdef\csname R@an.randsearch.move.C1.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.D1.kits.basis\endcsname{extension}
\expandafter\gdef\csname R@an.randsearch.move.D1.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.D1.kits.d0\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.randsearch.move.D1.kits.d0_alt\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.randsearch.move.D1.kits.dist\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.randsearch.move.D1.kits.fresh\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.randsearch.move.D1.kits.fresh_alt\endcsname{\ensuremath{+1.23}}
\expandafter\gdef\csname R@an.randsearch.move.D1.kits.mv\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.randsearch.move.D1.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.D2.kits.basis\endcsname{described}
\expandafter\gdef\csname R@an.randsearch.move.D2.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.D2.kits.d0\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.randsearch.move.D2.kits.d0_alt\endcsname{\ensuremath{+2.11}}
\expandafter\gdef\csname R@an.randsearch.move.D2.kits.dist\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.randsearch.move.D2.kits.fresh\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.randsearch.move.D2.kits.fresh_alt\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.randsearch.move.D2.kits.mv\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.randsearch.move.D2.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.L1.amos.basis\endcsname{described}
\expandafter\gdef\csname R@an.randsearch.move.L1.amos.class\endcsname{never}
\expandafter\gdef\csname R@an.randsearch.move.L1.amos.d0\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.randsearch.move.L1.amos.d0_alt\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.randsearch.move.L1.amos.dist\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.randsearch.move.L1.amos.fresh\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.randsearch.move.L1.amos.fresh_alt\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.randsearch.move.L1.amos.mv\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.randsearch.move.L1.amos.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.L1.kits.basis\endcsname{described}
\expandafter\gdef\csname R@an.randsearch.move.L1.kits.class\endcsname{never}
\expandafter\gdef\csname R@an.randsearch.move.L1.kits.d0\endcsname{\ensuremath{+2.33}}
\expandafter\gdef\csname R@an.randsearch.move.L1.kits.d0_alt\endcsname{\ensuremath{+2.08}}
\expandafter\gdef\csname R@an.randsearch.move.L1.kits.dist\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.randsearch.move.L1.kits.fresh\endcsname{\ensuremath{+3.48}}
\expandafter\gdef\csname R@an.randsearch.move.L1.kits.fresh_alt\endcsname{\ensuremath{+3.23}}
\expandafter\gdef\csname R@an.randsearch.move.L1.kits.mv\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.randsearch.move.L1.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.L1b.amos.basis\endcsname{registered}
\expandafter\gdef\csname R@an.randsearch.move.L1b.amos.class\endcsname{never}
\expandafter\gdef\csname R@an.randsearch.move.L1b.amos.d0\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.randsearch.move.L1b.amos.d0_alt\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.randsearch.move.L1b.amos.dist\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.randsearch.move.L1b.amos.fresh\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.randsearch.move.L1b.amos.fresh_alt\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.randsearch.move.L1b.amos.mv\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.randsearch.move.L1b.amos.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.L1b.kits.basis\endcsname{described}
\expandafter\gdef\csname R@an.randsearch.move.L1b.kits.class\endcsname{never}
\expandafter\gdef\csname R@an.randsearch.move.L1b.kits.d0\endcsname{\ensuremath{+1.74}}
\expandafter\gdef\csname R@an.randsearch.move.L1b.kits.d0_alt\endcsname{\ensuremath{+1.50}}
\expandafter\gdef\csname R@an.randsearch.move.L1b.kits.dist\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.randsearch.move.L1b.kits.fresh\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.randsearch.move.L1b.kits.fresh_alt\endcsname{\ensuremath{+2.07}}
\expandafter\gdef\csname R@an.randsearch.move.L1b.kits.mv\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.randsearch.move.L1b.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.L2.amos.basis\endcsname{registered}
\expandafter\gdef\csname R@an.randsearch.move.L2.amos.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.L2.amos.d0\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.randsearch.move.L2.amos.d0_alt\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.randsearch.move.L2.amos.dist\endcsname{0.00}
\expandafter\gdef\csname R@an.randsearch.move.L2.amos.fresh\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.randsearch.move.L2.amos.fresh_alt\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.randsearch.move.L2.amos.mv\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.randsearch.move.L2.amos.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.L2.kits.basis\endcsname{described}
\expandafter\gdef\csname R@an.randsearch.move.L2.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.L2.kits.d0\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.randsearch.move.L2.kits.d0_alt\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.randsearch.move.L2.kits.dist\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.randsearch.move.L2.kits.fresh\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.randsearch.move.L2.kits.fresh_alt\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.randsearch.move.L2.kits.mv\endcsname{\ensuremath{-0.55}}
\expandafter\gdef\csname R@an.randsearch.move.L2.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.L3.amos.basis\endcsname{described}
\expandafter\gdef\csname R@an.randsearch.move.L3.amos.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.L3.amos.d0\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.randsearch.move.L3.amos.d0_alt\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.randsearch.move.L3.amos.dist\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@an.randsearch.move.L3.amos.fresh\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.randsearch.move.L3.amos.fresh_alt\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.randsearch.move.L3.amos.mv\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.randsearch.move.L3.amos.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.L3.kits.basis\endcsname{described}
\expandafter\gdef\csname R@an.randsearch.move.L3.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.L3.kits.d0\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.randsearch.move.L3.kits.d0_alt\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@an.randsearch.move.L3.kits.dist\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.randsearch.move.L3.kits.fresh\endcsname{\ensuremath{+2.09}}
\expandafter\gdef\csname R@an.randsearch.move.L3.kits.fresh_alt\endcsname{\ensuremath{+1.85}}
\expandafter\gdef\csname R@an.randsearch.move.L3.kits.mv\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.randsearch.move.L3.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.L4.amos.basis\endcsname{registered}
\expandafter\gdef\csname R@an.randsearch.move.L4.amos.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.L4.amos.d0\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.randsearch.move.L4.amos.d0_alt\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.randsearch.move.L4.amos.dist\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.randsearch.move.L4.amos.fresh\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.randsearch.move.L4.amos.fresh_alt\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.randsearch.move.L4.amos.mv\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.randsearch.move.L4.amos.reading\endcsname{above}
\expandafter\gdef\csname R@an.randsearch.move.L4.kits.basis\endcsname{described}
\expandafter\gdef\csname R@an.randsearch.move.L4.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.L4.kits.d0\endcsname{\ensuremath{+2.20}}
\expandafter\gdef\csname R@an.randsearch.move.L4.kits.d0_alt\endcsname{\ensuremath{+1.95}}
\expandafter\gdef\csname R@an.randsearch.move.L4.kits.dist\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.randsearch.move.L4.kits.fresh\endcsname{\ensuremath{+2.25}}
\expandafter\gdef\csname R@an.randsearch.move.L4.kits.fresh_alt\endcsname{\ensuremath{+2.00}}
\expandafter\gdef\csname R@an.randsearch.move.L4.kits.mv\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.randsearch.move.L4.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.L6.kits.basis\endcsname{described}
\expandafter\gdef\csname R@an.randsearch.move.L6.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.L6.kits.d0\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.randsearch.move.L6.kits.d0_alt\endcsname{\ensuremath{+2.28}}
\expandafter\gdef\csname R@an.randsearch.move.L6.kits.dist\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.randsearch.move.L6.kits.fresh\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.randsearch.move.L6.kits.fresh_alt\endcsname{\ensuremath{+1.35}}
\expandafter\gdef\csname R@an.randsearch.move.L6.kits.mv\endcsname{\ensuremath{-0.93}}
\expandafter\gdef\csname R@an.randsearch.move.L6.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.P3c.kits.basis\endcsname{extension}
\expandafter\gdef\csname R@an.randsearch.move.P3c.kits.class\endcsname{never}
\expandafter\gdef\csname R@an.randsearch.move.P3c.kits.d0\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.randsearch.move.P3c.kits.d0_alt\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.randsearch.move.P3c.kits.dist\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.randsearch.move.P3c.kits.fresh\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.randsearch.move.P3c.kits.fresh_alt\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.randsearch.move.P3c.kits.mv\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.randsearch.move.P3c.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.S2.kits.basis\endcsname{extension}
\expandafter\gdef\csname R@an.randsearch.move.S2.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.S2.kits.d0\endcsname{\ensuremath{+1.34}}
\expandafter\gdef\csname R@an.randsearch.move.S2.kits.d0_alt\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@an.randsearch.move.S2.kits.dist\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.randsearch.move.S2.kits.fresh\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.randsearch.move.S2.kits.fresh_alt\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.randsearch.move.S2.kits.mv\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.randsearch.move.S2.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.V5A5.kits.basis\endcsname{extension}
\expandafter\gdef\csname R@an.randsearch.move.V5A5.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.V5A5.kits.d0\endcsname{\ensuremath{+1.95}}
\expandafter\gdef\csname R@an.randsearch.move.V5A5.kits.d0_alt\endcsname{\ensuremath{+1.71}}
\expandafter\gdef\csname R@an.randsearch.move.V5A5.kits.dist\endcsname{\ensuremath{+1.22}}
\expandafter\gdef\csname R@an.randsearch.move.V5A5.kits.fresh\endcsname{\ensuremath{+2.17}}
\expandafter\gdef\csname R@an.randsearch.move.V5A5.kits.fresh_alt\endcsname{\ensuremath{+1.92}}
\expandafter\gdef\csname R@an.randsearch.move.V5A5.kits.mv\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.randsearch.move.V5A5.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.V5B1.kits.basis\endcsname{extension}
\expandafter\gdef\csname R@an.randsearch.move.V5B1.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.V5B1.kits.d0\endcsname{\ensuremath{+2.16}}
\expandafter\gdef\csname R@an.randsearch.move.V5B1.kits.d0_alt\endcsname{\ensuremath{+1.92}}
\expandafter\gdef\csname R@an.randsearch.move.V5B1.kits.dist\endcsname{\ensuremath{+1.13}}
\expandafter\gdef\csname R@an.randsearch.move.V5B1.kits.fresh\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.randsearch.move.V5B1.kits.fresh_alt\endcsname{\ensuremath{+2.04}}
\expandafter\gdef\csname R@an.randsearch.move.V5B1.kits.mv\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.randsearch.move.V5B1.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.V5B2.kits.basis\endcsname{extension}
\expandafter\gdef\csname R@an.randsearch.move.V5B2.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.V5B2.kits.d0\endcsname{\ensuremath{+1.26}}
\expandafter\gdef\csname R@an.randsearch.move.V5B2.kits.d0_alt\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.randsearch.move.V5B2.kits.dist\endcsname{\ensuremath{+1.19}}
\expandafter\gdef\csname R@an.randsearch.move.V5B2.kits.fresh\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@an.randsearch.move.V5B2.kits.fresh_alt\endcsname{\ensuremath{+1.20}}
\expandafter\gdef\csname R@an.randsearch.move.V5B2.kits.mv\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.randsearch.move.V5B2.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.V6A1r.kits.basis\endcsname{extension}
\expandafter\gdef\csname R@an.randsearch.move.V6A1r.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.V6A1r.kits.d0\endcsname{\ensuremath{+2.24}}
\expandafter\gdef\csname R@an.randsearch.move.V6A1r.kits.d0_alt\endcsname{\ensuremath{+1.99}}
\expandafter\gdef\csname R@an.randsearch.move.V6A1r.kits.dist\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.randsearch.move.V6A1r.kits.fresh\endcsname{\ensuremath{+1.70}}
\expandafter\gdef\csname R@an.randsearch.move.V6A1r.kits.fresh_alt\endcsname{\ensuremath{+1.46}}
\expandafter\gdef\csname R@an.randsearch.move.V6A1r.kits.mv\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.randsearch.move.V6A1r.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.V7A1.kits.basis\endcsname{extension}
\expandafter\gdef\csname R@an.randsearch.move.V7A1.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.V7A1.kits.d0\endcsname{\ensuremath{+2.55}}
\expandafter\gdef\csname R@an.randsearch.move.V7A1.kits.d0_alt\endcsname{\ensuremath{+2.30}}
\expandafter\gdef\csname R@an.randsearch.move.V7A1.kits.dist\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.randsearch.move.V7A1.kits.fresh\endcsname{\ensuremath{+2.66}}
\expandafter\gdef\csname R@an.randsearch.move.V7A1.kits.fresh_alt\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.randsearch.move.V7A1.kits.mv\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.randsearch.move.V7A1.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.V7A2.kits.basis\endcsname{extension}
\expandafter\gdef\csname R@an.randsearch.move.V7A2.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.V7A2.kits.d0\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.randsearch.move.V7A2.kits.d0_alt\endcsname{\ensuremath{+2.64}}
\expandafter\gdef\csname R@an.randsearch.move.V7A2.kits.dist\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.randsearch.move.V7A2.kits.fresh\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.randsearch.move.V7A2.kits.fresh_alt\endcsname{\ensuremath{+2.05}}
\expandafter\gdef\csname R@an.randsearch.move.V7A2.kits.mv\endcsname{\ensuremath{-0.60}}
\expandafter\gdef\csname R@an.randsearch.move.V7A2.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.V7B1.kits.basis\endcsname{extension}
\expandafter\gdef\csname R@an.randsearch.move.V7B1.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.V7B1.kits.d0\endcsname{\ensuremath{+1.72}}
\expandafter\gdef\csname R@an.randsearch.move.V7B1.kits.d0_alt\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.randsearch.move.V7B1.kits.dist\endcsname{\ensuremath{+1.67}}
\expandafter\gdef\csname R@an.randsearch.move.V7B1.kits.fresh\endcsname{\ensuremath{+2.38}}
\expandafter\gdef\csname R@an.randsearch.move.V7B1.kits.fresh_alt\endcsname{\ensuremath{+2.14}}
\expandafter\gdef\csname R@an.randsearch.move.V7B1.kits.mv\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.randsearch.move.V7B1.kits.reading\endcsname{above}
\expandafter\gdef\csname R@an.randsearch.move.V7B2.kits.basis\endcsname{extension}
\expandafter\gdef\csname R@an.randsearch.move.V7B2.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.V7B2.kits.d0\endcsname{\ensuremath{+2.82}}
\expandafter\gdef\csname R@an.randsearch.move.V7B2.kits.d0_alt\endcsname{\ensuremath{+2.58}}
\expandafter\gdef\csname R@an.randsearch.move.V7B2.kits.dist\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.randsearch.move.V7B2.kits.fresh\endcsname{\ensuremath{+1.84}}
\expandafter\gdef\csname R@an.randsearch.move.V7B2.kits.fresh_alt\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.randsearch.move.V7B2.kits.mv\endcsname{\ensuremath{-0.99}}
\expandafter\gdef\csname R@an.randsearch.move.V7B2.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.V7C1.kits.basis\endcsname{extension}
\expandafter\gdef\csname R@an.randsearch.move.V7C1.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.V7C1.kits.d0\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.randsearch.move.V7C1.kits.d0_alt\endcsname{\ensuremath{+2.46}}
\expandafter\gdef\csname R@an.randsearch.move.V7C1.kits.dist\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.randsearch.move.V7C1.kits.fresh\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@an.randsearch.move.V7C1.kits.fresh_alt\endcsname{\ensuremath{+2.20}}
\expandafter\gdef\csname R@an.randsearch.move.V7C1.kits.mv\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.randsearch.move.V7C1.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.V8A1.kits.basis\endcsname{extension}
\expandafter\gdef\csname R@an.randsearch.move.V8A1.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.V8A1.kits.d0\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.randsearch.move.V8A1.kits.d0_alt\endcsname{\ensuremath{+1.52}}
\expandafter\gdef\csname R@an.randsearch.move.V8A1.kits.dist\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.randsearch.move.V8A1.kits.fresh\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.randsearch.move.V8A1.kits.fresh_alt\endcsname{\ensuremath{+1.01}}
\expandafter\gdef\csname R@an.randsearch.move.V8A1.kits.mv\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.randsearch.move.V8A1.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.V8A2.kits.basis\endcsname{extension}
\expandafter\gdef\csname R@an.randsearch.move.V8A2.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.V8A2.kits.d0\endcsname{\ensuremath{+1.35}}
\expandafter\gdef\csname R@an.randsearch.move.V8A2.kits.d0_alt\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.randsearch.move.V8A2.kits.dist\endcsname{\ensuremath{+1.53}}
\expandafter\gdef\csname R@an.randsearch.move.V8A2.kits.fresh\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@an.randsearch.move.V8A2.kits.fresh_alt\endcsname{\ensuremath{+1.63}}
\expandafter\gdef\csname R@an.randsearch.move.V8A2.kits.mv\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.randsearch.move.V8A2.kits.reading\endcsname{above}
\expandafter\gdef\csname R@an.randsearch.move.V8B1.kits.basis\endcsname{extension}
\expandafter\gdef\csname R@an.randsearch.move.V8B1.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.V8B1.kits.d0\endcsname{\ensuremath{+2.91}}
\expandafter\gdef\csname R@an.randsearch.move.V8B1.kits.d0_alt\endcsname{\ensuremath{+2.67}}
\expandafter\gdef\csname R@an.randsearch.move.V8B1.kits.dist\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.randsearch.move.V8B1.kits.fresh\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.randsearch.move.V8B1.kits.fresh_alt\endcsname{\ensuremath{+1.13}}
\expandafter\gdef\csname R@an.randsearch.move.V8B1.kits.mv\endcsname{\ensuremath{-1.54}}
\expandafter\gdef\csname R@an.randsearch.move.V8B1.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.V8B2.kits.basis\endcsname{extension}
\expandafter\gdef\csname R@an.randsearch.move.V8B2.kits.class\endcsname{eligible}
\expandafter\gdef\csname R@an.randsearch.move.V8B2.kits.d0\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.randsearch.move.V8B2.kits.d0_alt\endcsname{\ensuremath{+1.40}}
\expandafter\gdef\csname R@an.randsearch.move.V8B2.kits.dist\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.randsearch.move.V8B2.kits.fresh\endcsname{\ensuremath{+1.73}}
\expandafter\gdef\csname R@an.randsearch.move.V8B2.kits.fresh_alt\endcsname{\ensuremath{+1.49}}
\expandafter\gdef\csname R@an.randsearch.move.V8B2.kits.mv\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.randsearch.move.V8B2.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.W1c.kits.basis\endcsname{registered}
\expandafter\gdef\csname R@an.randsearch.move.W1c.kits.class\endcsname{never}
\expandafter\gdef\csname R@an.randsearch.move.W1c.kits.d0\endcsname{\ensuremath{+2.64}}
\expandafter\gdef\csname R@an.randsearch.move.W1c.kits.d0_alt\endcsname{\ensuremath{+2.39}}
\expandafter\gdef\csname R@an.randsearch.move.W1c.kits.dist\endcsname{\ensuremath{-1.57}}
\expandafter\gdef\csname R@an.randsearch.move.W1c.kits.fresh\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.randsearch.move.W1c.kits.fresh_alt\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.randsearch.move.W1c.kits.mv\endcsname{\ensuremath{-1.57}}
\expandafter\gdef\csname R@an.randsearch.move.W1c.kits.reading\endcsname{inside}
\expandafter\gdef\csname R@an.randsearch.move.amos.ag.max\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.randsearch.move.amos.ag.mean\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.randsearch.move.amos.ag.min\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.randsearch.move.amos.ag.n\endcsname{3}
\expandafter\gdef\csname R@an.randsearch.move.amos.ag.n_inside\endcsname{2}
\expandafter\gdef\csname R@an.randsearch.move.amos.ag.names\endcsname{ConvNeXt-k3, \textbf{HyReX}, ResEnc+context}
\expandafter\gdef\csname R@an.randsearch.move.amos.desc.max\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.randsearch.move.amos.desc.mean\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.randsearch.move.amos.desc.min\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.randsearch.move.amos.desc.n\endcsname{2}
\expandafter\gdef\csname R@an.randsearch.move.amos.desc.n_inside\endcsname{2}
\expandafter\gdef\csname R@an.randsearch.move.amos.desc.names\endcsname{\textbf{HyReX}, ResEnc-M}
\expandafter\gdef\csname R@an.randsearch.move.amos.ext.max\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.move.amos.ext.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.move.amos.ext.min\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.move.amos.ext.n\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.move.amos.ext.n_inside\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.move.amos.ext.names\endcsname{none}
\expandafter\gdef\csname R@an.randsearch.move.amos.nev.max\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.randsearch.move.amos.nev.mean\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.randsearch.move.amos.nev.min\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.randsearch.move.amos.nev.n\endcsname{2}
\expandafter\gdef\csname R@an.randsearch.move.amos.nev.n_inside\endcsname{2}
\expandafter\gdef\csname R@an.randsearch.move.amos.nev.names\endcsname{ResEnc-M, ResEnc-matched}
\expandafter\gdef\csname R@an.randsearch.move.amos.q2.max\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.move.amos.q2.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.move.amos.q2.min\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.move.amos.q2.n\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.move.amos.q2.n_inside\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.move.amos.q2.names\endcsname{none}
\expandafter\gdef\csname R@an.randsearch.move.amos.reg.max\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.randsearch.move.amos.reg.mean\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.randsearch.move.amos.reg.min\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.randsearch.move.amos.reg.n\endcsname{3}
\expandafter\gdef\csname R@an.randsearch.move.amos.reg.n_inside\endcsname{2}
\expandafter\gdef\csname R@an.randsearch.move.amos.reg.n_pending\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.move.amos.reg.names\endcsname{ConvNeXt-k3, ResEnc+context, ResEnc-matched}
\expandafter\gdef\csname R@an.randsearch.move.amos.reg.pending\endcsname{none}
\expandafter\gdef\csname R@an.randsearch.move.amos.rs.max\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.move.amos.rs.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.move.amos.rs.min\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.move.amos.rs.n\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.move.amos.rs.n_inside\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.move.amos.rs.names\endcsname{none}
\expandafter\gdef\csname R@an.randsearch.move.kits.ag.max\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.randsearch.move.kits.ag.mean\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.randsearch.move.kits.ag.min\endcsname{\ensuremath{-1.54}}
\expandafter\gdef\csname R@an.randsearch.move.kits.ag.n\endcsname{21}
\expandafter\gdef\csname R@an.randsearch.move.kits.ag.n_inside\endcsname{19}
\expandafter\gdef\csname R@an.randsearch.move.kits.ag.names\endcsname{ConvNeXt-k3, \textbf{HyReX}, ResEnc+context, HyReX+context, HyReX, finer ConvNeXt, HyReX point-fuse, HyReX+dec. capacity, LeanDec, LeanAdd, LeanAdd-NeXt, HyReX-LeanDec, LeanTrunk, Stem1, CoarseStack, StackDec, LeanDeepMid+FD, LeanSep, LeanDil, LeanDeepMid, LeanNeXt-s5, HyReX-k9}
\expandafter\gdef\csname R@an.randsearch.move.kits.desc.max\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.randsearch.move.kits.desc.mean\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.randsearch.move.kits.desc.min\endcsname{\ensuremath{-0.93}}
\expandafter\gdef\csname R@an.randsearch.move.kits.desc.n\endcsname{7}
\expandafter\gdef\csname R@an.randsearch.move.kits.desc.n_inside\endcsname{7}
\expandafter\gdef\csname R@an.randsearch.move.kits.desc.names\endcsname{ConvNeXt-k3, \textbf{HyReX}, ResEnc+context, HyReX+context, LeanDec, ResEnc-M, ResEnc-matched}
\expandafter\gdef\csname R@an.randsearch.move.kits.ext.max\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.randsearch.move.kits.ext.mean\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.randsearch.move.kits.ext.min\endcsname{\ensuremath{-1.54}}
\expandafter\gdef\csname R@an.randsearch.move.kits.ext.n\endcsname{16}
\expandafter\gdef\csname R@an.randsearch.move.kits.ext.n_inside\endcsname{14}
\expandafter\gdef\csname R@an.randsearch.move.kits.ext.names\endcsname{HyReX, finer ConvNeXt, HyReX point-fuse, LeanAdd, LeanAdd-NeXt, HyReX-LeanDec, LeanTrunk, Stem1, CoarseStack, StackDec, LeanDeepMid+FD, LeanSep, LeanDil, LeanDeepMid, LeanNeXt-s5, HyReX-k9, fn.-identical control}
\expandafter\gdef\csname R@an.randsearch.move.kits.nev.max\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.randsearch.move.kits.nev.mean\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.randsearch.move.kits.nev.min\endcsname{\ensuremath{-1.57}}
\expandafter\gdef\csname R@an.randsearch.move.kits.nev.n\endcsname{4}
\expandafter\gdef\csname R@an.randsearch.move.kits.nev.n_inside\endcsname{4}
\expandafter\gdef\csname R@an.randsearch.move.kits.nev.names\endcsname{ResEnc-M, ResEnc-matched, branch control, fn.-identical control}
\expandafter\gdef\csname R@an.randsearch.move.kits.q2.max\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.move.kits.q2.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.move.kits.q2.min\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.move.kits.q2.n\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.move.kits.q2.n_inside\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.move.kits.q2.names\endcsname{none}
\expandafter\gdef\csname R@an.randsearch.move.kits.reg.max\endcsname{\ensuremath{-1.11}}
\expandafter\gdef\csname R@an.randsearch.move.kits.reg.mean\endcsname{\ensuremath{-1.34}}
\expandafter\gdef\csname R@an.randsearch.move.kits.reg.min\endcsname{\ensuremath{-1.57}}
\expandafter\gdef\csname R@an.randsearch.move.kits.reg.n\endcsname{2}
\expandafter\gdef\csname R@an.randsearch.move.kits.reg.n_inside\endcsname{2}
\expandafter\gdef\csname R@an.randsearch.move.kits.reg.n_pending\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.move.kits.reg.names\endcsname{HyReX+dec. capacity, branch control}
\expandafter\gdef\csname R@an.randsearch.move.kits.reg.pending\endcsname{none}
\expandafter\gdef\csname R@an.randsearch.move.kits.rs.max\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.move.kits.rs.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.move.kits.rs.min\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.move.kits.rs.n\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.move.kits.rs.n_inside\endcsname{0}
\expandafter\gdef\csname R@an.randsearch.move.kits.rs.names\endcsname{none}
\expandafter\gdef\csname R@an.randsearch.p3c.alt_amos\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.randsearch.p3c.alt_kits\endcsname{six-run reference}
\expandafter\gdef\csname R@an.randsearch.p3c.amos.d0\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.randsearch.p3c.amos.d0_alt\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.randsearch.p3c.amos.owed\endcsname{no}
\expandafter\gdef\csname R@an.randsearch.p3c.amos.pair\endcsname{not yet queued}
\expandafter\gdef\csname R@an.randsearch.p3c.amos.reading\endcsname{not resolved}
\expandafter\gdef\csname R@an.randsearch.p3c.amos.screen\endcsname{does not clear}
\expandafter\gdef\csname R@an.randsearch.p3c.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.p3c.kits.d0\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.randsearch.p3c.kits.d0_alt\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.randsearch.p3c.kits.owed\endcsname{yes}
\expandafter\gdef\csname R@an.randsearch.p3c.kits.pair\endcsname{complete}
\expandafter\gdef\csname R@an.randsearch.p3c.kits.reading\endcsname{beyond the floor}
\expandafter\gdef\csname R@an.randsearch.p3c.kits.screen\endcsname{clears}
\expandafter\gdef\csname R@an.randsearch.p3c.kits.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.pool.amos.band2\endcsname{0.26}
\expandafter\gdef\csname R@an.randsearch.pool.amos.mean\endcsname{87.701}
\expandafter\gdef\csname R@an.randsearch.pool.amos.n\endcsname{6}
\expandafter\gdef\csname R@an.randsearch.pool.amos.nu\endcsname{5}
\expandafter\gdef\csname R@an.randsearch.pool.amos.runs\endcsname{six-run}
\expandafter\gdef\csname R@an.randsearch.pool.amos.sd\endcsname{0.122}
\expandafter\gdef\csname R@an.randsearch.pool.amos.sdd\endcsname{0.132}
\expandafter\gdef\csname R@an.randsearch.pool.kits.band2\endcsname{1.84}
\expandafter\gdef\csname R@an.randsearch.pool.kits.mean\endcsname{83.378}
\expandafter\gdef\csname R@an.randsearch.pool.kits.n\endcsname{3}
\expandafter\gdef\csname R@an.randsearch.pool.kits.nu\endcsname{2}
\expandafter\gdef\csname R@an.randsearch.pool.kits.runs\endcsname{three-run}
\expandafter\gdef\csname R@an.randsearch.pool.kits.sd\endcsname{0.795}
\expandafter\gdef\csname R@an.randsearch.pool.kits.sdd\endcsname{0.918}
\expandafter\gdef\csname R@an.randsearch.rs.RS01.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS01.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS01.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS01.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS01.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS01.kits.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.rs.RS02.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS02.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS02.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS02.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS02.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS02.kits.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.rs.RS05.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS05.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS05.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS05.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS05.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS05.kits.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.rs.RS07.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS07.amos.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS07.amos.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS07.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS07.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS07.amos.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.rs.RS07.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS07.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS07.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS07.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS07.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS07.kits.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.rs.RS08.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS08.amos.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS08.amos.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS08.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS08.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS08.amos.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.rs.RS08.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS08.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS08.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS08.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS08.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS08.kits.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.rs.RS09.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS09.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS09.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS09.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS09.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS09.kits.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.rs.RS11.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS11.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS11.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS11.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS11.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS11.kits.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.rs.RS12.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS12.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS12.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS12.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS12.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS12.kits.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.rs.RS13.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS13.amos.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS13.amos.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS13.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS13.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS13.amos.state\endcsname{queued}
\expandafter\gdef\csname R@an.randsearch.rs.RS13.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS13.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS13.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS13.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS13.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS13.kits.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.rs.RS15.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS15.amos.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS15.amos.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS15.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS15.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS15.amos.state\endcsname{queued}
\expandafter\gdef\csname R@an.randsearch.rs.RS15.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS15.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS15.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS15.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS15.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS15.kits.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.rs.RS19.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS19.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS19.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS19.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS19.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS19.kits.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.rs.RS20.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS20.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS20.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS20.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS20.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS20.kits.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.rs.RS22.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS22.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS22.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS22.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS22.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS22.kits.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.rs.RS23.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS23.amos.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS23.amos.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS23.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS23.amos.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS23.amos.state\endcsname{queued}
\expandafter\gdef\csname R@an.randsearch.rs.RS23.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS23.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS23.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS23.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS23.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS23.kits.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.rs.RS24.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS24.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS24.kits.fires\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS24.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS24.kits.fresh_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.rs.RS24.kits.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_L_vs_L1.amos\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_L_vs_L1.amos.reading\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_L_vs_L1.kits\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_L_vs_L1.kits.reading\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_L_vs_L3.amos\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_L_vs_L3.amos.reading\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_L_vs_L3.kits\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_L_vs_L3.kits.reading\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_L_vs_L3w_M.amos\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_L_vs_L3w_M.amos.reading\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_L_vs_L3w_M.kits\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_L_vs_L3w_M.kits.reading\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_M_vs_L1.amos\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_M_vs_L1.amos.reading\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_M_vs_L1.kits\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_M_vs_L1.kits.reading\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_M_vs_L3.amos\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_M_vs_L3.amos.reading\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_M_vs_L3.kits\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.L3w_M_vs_L3.kits.reading\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.scaled.gap_pct\endcsname{2.4}
\expandafter\gdef\csname R@an.randsearch.scaled.params_L\endcsname{99.8}
\expandafter\gdef\csname R@an.randsearch.scaled.params_L1\endcsname{102.3}
\expandafter\gdef\csname R@an.randsearch.scaled.params_L3\endcsname{29.6}
\expandafter\gdef\csname R@an.randsearch.scaled.params_M\endcsname{59.0}
\expandafter\gdef\csname R@an.randsearch.seed0\endcsname{seed 0}
\expandafter\gdef\csname R@an.randsearch.sp1.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.sp1.amos.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.sp1.amos.state\endcsname{queued}
\expandafter\gdef\csname R@an.randsearch.sp1.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.sp1.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.sp1.kits.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.sp2.amos.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.sp2.amos.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.sp2.amos.state\endcsname{queued}
\expandafter\gdef\csname R@an.randsearch.sp2.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.sp2.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.sp2.kits.state\endcsname{running}
\expandafter\gdef\csname R@an.randsearch.trip.amos\endcsname{2.3}
\expandafter\gdef\csname R@an.randsearch.trip.amos.hi\endcsname{16}
\expandafter\gdef\csname R@an.randsearch.trip.amos.lo\endcsname{0.4}
\expandafter\gdef\csname R@an.randsearch.trip.kits\endcsname{37}
\expandafter\gdef\csname R@an.randsearch.trip.kits.hi\endcsname{48}
\expandafter\gdef\csname R@an.randsearch.trip.kits.lo\endcsname{27}
\expandafter\gdef\csname R@an.randsearch.w4.amos.d0\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.randsearch.w4.amos.d0_alt\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.randsearch.w4.amos.state\endcsname{done}
\expandafter\gdef\csname R@an.randsearch.w4.kits.d0\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.w4.kits.d0_alt\endcsname{\pend}
\expandafter\gdef\csname R@an.randsearch.w4.kits.state\endcsname{queued}
\expandafter\gdef\csname R@an.registration.by_wave.0.finished\endcsname{31}
\expandafter\gdef\csname R@an.registration.by_wave.0.preledger\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.0.prior_results\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.0.prior_starts\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.0.runs\endcsname{66}
\expandafter\gdef\csname R@an.registration.by_wave.0.started\endcsname{31}
\expandafter\gdef\csname R@an.registration.by_wave.0.thin\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.1.finished\endcsname{96}
\expandafter\gdef\csname R@an.registration.by_wave.1.preledger\endcsname{10}
\expandafter\gdef\csname R@an.registration.by_wave.1.prior_results\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.1.prior_starts\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.1.runs\endcsname{148}
\expandafter\gdef\csname R@an.registration.by_wave.1.started\endcsname{96}
\expandafter\gdef\csname R@an.registration.by_wave.1.thin\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.2.finished\endcsname{10}
\expandafter\gdef\csname R@an.registration.by_wave.2.preledger\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.2.prior_results\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.2.prior_starts\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.2.runs\endcsname{11}
\expandafter\gdef\csname R@an.registration.by_wave.2.started\endcsname{10}
\expandafter\gdef\csname R@an.registration.by_wave.2.thin\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.3.finished\endcsname{26}
\expandafter\gdef\csname R@an.registration.by_wave.3.preledger\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.3.prior_results\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.3.prior_starts\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.3.runs\endcsname{57}
\expandafter\gdef\csname R@an.registration.by_wave.3.started\endcsname{26}
\expandafter\gdef\csname R@an.registration.by_wave.3.thin\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.4.finished\endcsname{32}
\expandafter\gdef\csname R@an.registration.by_wave.4.preledger\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.4.prior_results\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.4.prior_starts\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.4.runs\endcsname{65}
\expandafter\gdef\csname R@an.registration.by_wave.4.started\endcsname{32}
\expandafter\gdef\csname R@an.registration.by_wave.4.thin\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.5.finished\endcsname{37}
\expandafter\gdef\csname R@an.registration.by_wave.5.preledger\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.5.prior_results\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.5.prior_starts\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.5.runs\endcsname{55}
\expandafter\gdef\csname R@an.registration.by_wave.5.started\endcsname{37}
\expandafter\gdef\csname R@an.registration.by_wave.5.thin\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.6.finished\endcsname{17}
\expandafter\gdef\csname R@an.registration.by_wave.6.preledger\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.6.prior_results\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.6.prior_starts\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.6.runs\endcsname{26}
\expandafter\gdef\csname R@an.registration.by_wave.6.started\endcsname{17}
\expandafter\gdef\csname R@an.registration.by_wave.6.thin\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.7.finished\endcsname{64}
\expandafter\gdef\csname R@an.registration.by_wave.7.preledger\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.7.prior_results\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.7.prior_starts\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.7.runs\endcsname{150}
\expandafter\gdef\csname R@an.registration.by_wave.7.started\endcsname{77}
\expandafter\gdef\csname R@an.registration.by_wave.7.thin\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.8.finished\endcsname{22}
\expandafter\gdef\csname R@an.registration.by_wave.8.preledger\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.8.prior_results\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.8.prior_starts\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.8.runs\endcsname{57}
\expandafter\gdef\csname R@an.registration.by_wave.8.started\endcsname{27}
\expandafter\gdef\csname R@an.registration.by_wave.8.thin\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.list\endcsname{0,1,2,3,4,5,6,7,8,other}
\expandafter\gdef\csname R@an.registration.by_wave.other.finished\endcsname{13}
\expandafter\gdef\csname R@an.registration.by_wave.other.preledger\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.other.prior_results\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.other.prior_starts\endcsname{0}
\expandafter\gdef\csname R@an.registration.by_wave.other.runs\endcsname{92}
\expandafter\gdef\csname R@an.registration.by_wave.other.started\endcsname{32}
\expandafter\gdef\csname R@an.registration.by_wave.other.thin\endcsname{17}
\expandafter\gdef\csname R@an.registration.close.ids\endcsname{ai\_benchbase\_kits\_f0\_e1000\_s6, ai\_benchbase\_kits\_f0\_e1000\_s7}
\expandafter\gdef\csname R@an.registration.close.margins\endcsname{12 s and 42 s}
\expandafter\gdef\csname R@an.registration.close.n\endcsname{2}
\expandafter\gdef\csname R@an.registration.close.results\endcsname{0}
\expandafter\gdef\csname R@an.registration.docs.amended\endcsname{13}
\expandafter\gdef\csname R@an.registration.docs.amended.names\endcsname{Wave 1, Wave 2, Wave 3, Addendum N, Addendum O, Addendum AD, Addendum AK, Addendum AM, Addendum AN, Addendum AW, Addendum AV, Addendum AY and Addendum BA}
\expandafter\gdef\csname R@an.registration.docs.claim\endcsname{the 52 registration documents on disk are byte-identical to their last ledger entry}
\expandafter\gdef\csname R@an.registration.docs.disk\endcsname{52}
\expandafter\gdef\csname R@an.registration.docs.drift\endcsname{0}
\expandafter\gdef\csname R@an.registration.docs.identical\endcsname{52}
\expandafter\gdef\csname R@an.registration.docs.ledgered\endcsname{52}
\expandafter\gdef\csname R@an.registration.docs.process\endcsname{52}
\expandafter\gdef\csname R@an.registration.docs.unledgered\endcsname{0}
\expandafter\gdef\csname R@an.registration.files\endcsname{52}
\expandafter\gdef\csname R@an.registration.files.govern\endcsname{26}
\expandafter\gdef\csname R@an.registration.finished\endcsname{348}
\expandafter\gdef\csname R@an.registration.finished.named\endcsname{338}
\expandafter\gdef\csname R@an.registration.later.clause\endcsname{40 runs are named again by identifier in 8 documents ledgered after they started (Addendum O, Addendum AB, Addendum AI, Addendum AJ, Addendum AV, Addendum AX, Addendum AX2 and Addendum AX3); such later mentions are reported and never govern}
\expandafter\gdef\csname R@an.registration.later.docs\endcsname{Addendum O, Addendum AB, Addendum AI, Addendum AJ, Addendum AV, Addendum AX, Addendum AX2 and Addendum AX3}
\expandafter\gdef\csname R@an.registration.later.ids\endcsname{ai\_W5\_amos\_f0\_e1000\_s0, ai\_benchbase\_kits\_f0\_e1000\_s3, ai\_benchbase\_kits\_f0\_e1000\_s4, ai\_benchbase\_kits\_f0\_e1000\_s5, ai\_benchbase\_amos\_f0\_e1000\_s3, ai\_benchcvP3c\_kits\_f1\_e1000\_s0, ai\_benchcvP3c\_amos\_f1\_e1000\_s0, ai\_benchcvP3c\_kits\_f2\_e1000\_s0 and 32 more}
\expandafter\gdef\csname R@an.registration.later.ndocs\endcsname{8}
\expandafter\gdef\csname R@an.registration.later.runs\endcsname{40}
\expandafter\gdef\csname R@an.registration.ledger.first\endcsname{2026-10-04 04:29}
\expandafter\gdef\csname R@an.registration.ledger.started0\endcsname{13}
\expandafter\gdef\csname R@an.registration.ledger.witness0\endcsname{0}
\expandafter\gdef\csname R@an.registration.licensed.every\endcsname{no}
\expandafter\gdef\csname R@an.registration.licensed.results\endcsname{yes}
\expandafter\gdef\csname R@an.registration.licensed.starts\endcsname{yes}
\expandafter\gdef\csname R@an.registration.licensed.starts.all\endcsname{no}
\expandafter\gdef\csname R@an.registration.margin.result.h\endcsname{8.2}
\expandafter\gdef\csname R@an.registration.margin.result.id\endcsname{ai\_benchcvD2\_acdc\_f1\_e1000\_s0}
\expandafter\gdef\csname R@an.registration.margin.start.id\endcsname{ai\_benchbase\_kits\_f0\_e1000\_s6}
\expandafter\gdef\csname R@an.registration.margin.start.s\endcsname{12}
\expandafter\gdef\csname R@an.registration.prior_results\endcsname{0}
\expandafter\gdef\csname R@an.registration.prior_results.ids\endcsname{none}
\expandafter\gdef\csname R@an.registration.prior_results_total\endcsname{0}
\expandafter\gdef\csname R@an.registration.prior_starts\endcsname{0}
\expandafter\gdef\csname R@an.registration.prior_starts.ids\endcsname{none}
\expandafter\gdef\csname R@an.registration.runs\endcsname{727}
\expandafter\gdef\csname R@an.registration.runs.exact\endcsname{336}
\expandafter\gdef\csname R@an.registration.runs.none\endcsname{20}
\expandafter\gdef\csname R@an.registration.runs.preledger\endcsname{10}
\expandafter\gdef\csname R@an.registration.runs.preledger.wave1\endcsname{10}
\expandafter\gdef\csname R@an.registration.runs.spec\endcsname{328}
\expandafter\gdef\csname R@an.registration.runs.thin\endcsname{53}
\expandafter\gdef\csname R@an.registration.runs.weak\endcsname{33}
\expandafter\gdef\csname R@an.registration.sentence.counts\endcsname{Of the 727 runs of the study, 385 have started and 348 have a result. By registration document, 336 runs are governed by a document that names their identifier, 328 more by one that names the source or family of their design, 10 started before the ledger existed (the first wave, whose registration is a creation-time snapshot with 0 design trials with a result) and 53 are named only by their design's label or by nothing.}
\expandafter\gdef\csname R@an.registration.sentence.main\endcsname{Of the 727 runs of the study, 385 have started and 348 have a result. By registration document, 336 runs are governed by a document that names their identifier, 328 more by one that names the source or family of their design, 10 started before the ledger existed (the first wave, whose registration is a creation-time snapshot with 0 design trials with a result) and 53 are named only by their design's label or by nothing. None of the 338 finished runs that a document names had a result before the first ledger entry of the earliest document that names it; the closest result came 8.2 h after that entry. None of the 358 started runs that a document names started before it; the closest start came 12 s after the entry (2 within the 120 s clock slack). 17 started run(s) are named only by their design's label or by nothing and are outside both statements.}
\expandafter\gdef\csname R@an.registration.sentence.preledger\endcsname{10 runs of the first wave started before the ledger existed (2026-10-04 04:29 UTC): its registration is a creation-time snapshot, and the ledger records at that moment 0 design trials with a result and 13 already started.}
\expandafter\gdef\csname R@an.registration.sentence.results\endcsname{None of the 338 finished runs that a document names had a result before the first ledger entry of the earliest document that names it; the closest result came 8.2 h after that entry.}
\expandafter\gdef\csname R@an.registration.sentence.starts\endcsname{None of the 358 started runs that a document names started before it; the closest start came 12 s after the entry (2 within the 120 s clock slack).}
\expandafter\gdef\csname R@an.registration.sentence.thin\endcsname{17 started run(s) are named only by their design's label or by nothing and are outside both statements.}
\expandafter\gdef\csname R@an.registration.slack.s\endcsname{120}
\expandafter\gdef\csname R@an.registration.started\endcsname{385}
\expandafter\gdef\csname R@an.registration.started.exact\endcsname{173}
\expandafter\gdef\csname R@an.registration.started.named\endcsname{358}
\expandafter\gdef\csname R@an.registration.started.none\endcsname{17}
\expandafter\gdef\csname R@an.registration.started.spec\endcsname{185}
\expandafter\gdef\csname R@an.registration.started.weak\endcsname{0}
\expandafter\gdef\csname R@an.registration.strict.close.ids\endcsname{ai\_benchbase\_kits\_f0\_e1000\_s6, ai\_benchbase\_kits\_f0\_e1000\_s7}
\expandafter\gdef\csname R@an.registration.strict.close.n\endcsname{2}
\expandafter\gdef\csname R@an.registration.strict.margin.start.s\endcsname{12}
\expandafter\gdef\csname R@an.registration.strict.prior_results\endcsname{0}
\expandafter\gdef\csname R@an.registration.strict.prior_starts\endcsname{0}
\expandafter\gdef\csname R@an.registration.strict.runs\endcsname{383}
\expandafter\gdef\csname R@an.registration.thin.list\endcsname{benchrs01, benchrs02, benchrs05, benchrs07, benchrs08, benchrs09, benchrs11, benchrs12, benchrs13, benchrs15, benchrs19, benchrs20, benchrs22, benchrs23 and benchrs24}
\expandafter\gdef\csname R@an.registration.thin.started\endcsname{17}
\expandafter\gdef\csname R@an.registration.witness.agree\endcsname{694}
\expandafter\gdef\csname R@an.registration.witness.documented\endcsname{1}
\expandafter\gdef\csname R@an.registration.witness.entries\endcsname{695}
\expandafter\gdef\csname R@an.registration.witness.gap.s\endcsname{1}
\expandafter\gdef\csname R@an.registration.witness.unexplained\endcsname{0}
\expandafter\gdef\csname R@an.registration.witness.within\endcsname{0}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.bar0margin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.class\endcsname{never eligible}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.clears0\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.d0\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.d0_3\endcsname{\ensuremath{+0.336}}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.dfresh\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.dfresh_3\endcsname{\ensuremath{+0.242}}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.freshmean\endcsname{92.251}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.retained\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.role\endcsname{reference}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.s0\endcsname{92.345}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.s1\endcsname{92.268}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.s1reading.class\endcsname{no-selection}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.s1reading.phrase\endcsname{inside the no-selection band, a description since it carries no registered prediction (the guard dataset)}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.s2\endcsname{92.234}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.screen\endcsname{guard dataset, no screen}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.sdfresh\endcsname{0.024}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.sefresh\endcsname{0.017}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.shrink\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.shrink_3\endcsname{\ensuremath{-0.094}}
\expandafter\gdef\csname R@an.replication_all.acdc.L1.shrinkz\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.bar0margin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.class\endcsname{never eligible}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.clears0\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.d0\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.d0_3\endcsname{\ensuremath{+0.283}}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.dfresh\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.dfresh_3\endcsname{\ensuremath{+0.319}}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.freshmean\endcsname{92.328}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.retained\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.role\endcsname{control}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.s0\endcsname{92.293}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.s1\endcsname{92.296}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.s1reading.class\endcsname{no-selection}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.s1reading.phrase\endcsname{inside the no-selection band, a description since it carries no registered prediction (the guard dataset)}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.s2\endcsname{92.361}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.screen\endcsname{guard dataset, no screen}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.sdfresh\endcsname{0.046}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.sefresh\endcsname{0.033}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.shrink\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.shrink_3\endcsname{\ensuremath{+0.036}}
\expandafter\gdef\csname R@an.replication_all.acdc.L1b.shrinkz\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.bar0margin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.class\endcsname{no selection target (no screen on this dataset)}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.clears0\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.d0\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.d0_3\endcsname{\ensuremath{-0.015}}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.s0\endcsname{91.995}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.screen\endcsname{guard dataset, no screen}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L2.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.bar0margin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.class\endcsname{no selection target (no screen on this dataset)}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.clears0\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.d0\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.d0_3\endcsname{\ensuremath{+0.616}}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.dfresh\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.dfresh_3\endcsname{\ensuremath{+0.450}}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.freshmean\endcsname{92.460}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.retained\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.s0\endcsname{92.626}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.s1\endcsname{92.426}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.s1reading.class\endcsname{no-selection}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.s1reading.phrase\endcsname{inside the no-selection band, a description since it carries no registered prediction (the guard dataset)}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.s2\endcsname{92.493}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.screen\endcsname{guard dataset, no screen}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.sdfresh\endcsname{0.047}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.sefresh\endcsname{0.033}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.shrink\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.shrink_3\endcsname{\ensuremath{-0.166}}
\expandafter\gdef\csname R@an.replication_all.acdc.L3.shrinkz\endcsname{\ensuremath{-1.37}}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.bar0margin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.class\endcsname{no selection target (no screen on this dataset)}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.clears0\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.d0\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.d0_3\endcsname{\ensuremath{+0.315}}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.s0\endcsname{92.325}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.screen\endcsname{guard dataset, no screen}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L4.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.bar0margin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.class\endcsname{no selection target (no screen on this dataset)}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.clears0\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.d0\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.d0_3\endcsname{\ensuremath{+0.451}}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.s0\endcsname{92.461}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.screen\endcsname{guard dataset, no screen}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.L6.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.bar0margin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.class\endcsname{never eligible}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.clears0\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.d0\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.d0_3\endcsname{\ensuremath{-0.013}}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.dfresh\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.dfresh_3\endcsname{\ensuremath{+0.117}}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.freshmean\endcsname{92.126}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.retained\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.role\endcsname{control}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.s0\endcsname{91.997}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.s1\endcsname{92.134}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.s1reading.class\endcsname{no-selection}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.s1reading.phrase\endcsname{inside the no-selection band, a description since it carries no registered prediction (the guard dataset)}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.s2\endcsname{92.118}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.screen\endcsname{guard dataset, no screen}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.sdfresh\endcsname{0.012}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.sefresh\endcsname{0.008}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.shrink\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.shrink_3\endcsname{\ensuremath{+0.129}}
\expandafter\gdef\csname R@an.replication_all.acdc.P3c.shrinkz\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.bar0margin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.class\endcsname{no selection target (no screen on this dataset)}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.clears0\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.d0\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.d0_3\endcsname{\ensuremath{-0.181}}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.s0\endcsname{91.828}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.screen\endcsname{guard dataset, no screen}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V5B2.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.bar0margin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.class\endcsname{no selection target (no screen on this dataset)}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.clears0\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.d0\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.d0_3\endcsname{\ensuremath{+0.573}}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.s0\endcsname{92.582}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.screen\endcsname{guard dataset, no screen}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V6A1r.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.bar0margin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.class\endcsname{no selection target (no screen on this dataset)}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.clears0\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.d0\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.d0_3\endcsname{\ensuremath{+0.229}}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.s0\endcsname{92.238}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.screen\endcsname{guard dataset, no screen}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A1.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.bar0margin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.class\endcsname{no selection target (no screen on this dataset)}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.clears0\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.d0\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.d0_3\endcsname{\ensuremath{+0.362}}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.s0\endcsname{92.371}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.screen\endcsname{guard dataset, no screen}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7A2.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.bar0margin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.class\endcsname{no selection target (no screen on this dataset)}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.clears0\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.d0\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.d0_3\endcsname{\ensuremath{-0.252}}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.s0\endcsname{91.757}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.screen\endcsname{guard dataset, no screen}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.V7C1.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.altref\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.replication_all.acdc.altref.name\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.replication_all.acdc.attr.list\endcsname{none}
\expandafter\gdef\csname R@an.replication_all.acdc.attr.n\endcsname{0}
\expandafter\gdef\csname R@an.replication_all.acdc.confound\endcsname{no single family}
\expandafter\gdef\csname R@an.replication_all.acdc.confound.phrase\endcsname{the never-eligible arms span more than one family}
\expandafter\gdef\csname R@an.replication_all.acdc.ctlfire.n\endcsname{0}
\expandafter\gdef\csname R@an.replication_all.acdc.cur.hi\endcsname{\ensuremath{+0.002}}
\expandafter\gdef\csname R@an.replication_all.acdc.cur.label\endcsname{current model: the candidate designs with a finished seed-0 run now}
\expandafter\gdef\csname R@an.replication_all.acdc.cur.lo\endcsname{\ensuremath{-0.417}}
\expandafter\gdef\csname R@an.replication_all.acdc.cur.m\endcsname{9}
\expandafter\gdef\csname R@an.replication_all.acdc.cur.m_plan\endcsname{4}
\expandafter\gdef\csname R@an.replication_all.acdc.cur.never.hi\endcsname{\ensuremath{+0.243}}
\expandafter\gdef\csname R@an.replication_all.acdc.cur.never.lo\endcsname{\ensuremath{-0.244}}
\expandafter\gdef\csname R@an.replication_all.acdc.cur.plug\endcsname{\ensuremath{-0.147}}
\expandafter\gdef\csname R@an.replication_all.acdc.cur.plug_plan\endcsname{\ensuremath{-0.102}}
\expandafter\gdef\csname R@an.replication_all.acdc.desc.n\endcsname{4}
\expandafter\gdef\csname R@an.replication_all.acdc.desc.ndown\endcsname{2}
\expandafter\gdef\csname R@an.replication_all.acdc.desc.phrase\endcsname{HyReX moved \ensuremath{-0.166}\,pp, ResEnc-M moved \ensuremath{-0.094}\,pp, ResEnc-matched moved \ensuremath{+0.036}\,pp and fn.-identical control moved \ensuremath{+0.129}\,pp between the discovery seed and the fresh mean; ACDC carries no screen, so these movements describe the arms and carry no selection prediction}
\expandafter\gdef\csname R@an.replication_all.acdc.dfresh.L1minusL3\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.replication_all.acdc.dfresh.ahead\endcsname{HyReX}
\expandafter\gdef\csname R@an.replication_all.acdc.diff\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.diff.ratio\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.diff.se\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.diff.se.kind\endcsname{the no-selection model's standard error at the frozen ACDC pool seed SD, not an empirical standard error of these arms}
\expandafter\gdef\csname R@an.replication_all.acdc.diff.se.pooled\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.diff.se.welch\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.diff.sentence\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.eb.L1.pred\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.replication_all.acdc.eb.L1b.pred\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.replication_all.acdc.eb.L3.pred\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.replication_all.acdc.eb.P3c.pred\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.replication_all.acdc.eb.factor\endcsname{0.853}
\expandafter\gdef\csname R@an.replication_all.acdc.eb.meand0\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.replication_all.acdc.eb.n\endcsname{4}
\expandafter\gdef\csname R@an.replication_all.acdc.eb.tau2\endcsname{0.057}
\expandafter\gdef\csname R@an.replication_all.acdc.eb.verdict\endcsname{exceeds the single-seed variance of the pool by 0.057 pp$^2$ over the 4 arms}
\expandafter\gdef\csname R@an.replication_all.acdc.elig.list\endcsname{none}
\expandafter\gdef\csname R@an.replication_all.acdc.elig.n\endcsname{0}
\expandafter\gdef\csname R@an.replication_all.acdc.elig.nlanded\endcsname{0}
\expandafter\gdef\csname R@an.replication_all.acdc.emax\endcsname{1.484}
\expandafter\gdef\csname R@an.replication_all.acdc.expshrink\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.replication_all.acdc.expshrink_hi\endcsname{0.00}
\expandafter\gdef\csname R@an.replication_all.acdc.expshrink_lo\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.replication_all.acdc.expshrink_mc\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.replication_all.acdc.expshrink_nu\endcsname{5}
\expandafter\gdef\csname R@an.replication_all.acdc.floor\endcsname{2}
\expandafter\gdef\csname R@an.replication_all.acdc.hasscreen\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.acdc.lead\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.leadis\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.leadreg\endcsname{HyReX}
\expandafter\gdef\csname R@an.replication_all.acdc.leadreg.d0\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.replication_all.acdc.leadreg.shrink\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.replication_all.acdc.leadshrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.m\endcsname{9}
\expandafter\gdef\csname R@an.replication_all.acdc.m1.coverage\endcsname{all 4 measured shrinkages lie inside it}
\expandafter\gdef\csname R@an.replication_all.acdc.never.list\endcsname{ResEnc-M, ResEnc-matched and fn.-identical control}
\expandafter\gdef\csname R@an.replication_all.acdc.never.n\endcsname{3}
\expandafter\gdef\csname R@an.replication_all.acdc.nreg\endcsname{4}
\expandafter\gdef\csname R@an.replication_all.acdc.nrepl\endcsname{4}
\expandafter\gdef\csname R@an.replication_all.acdc.nrepl.other\endcsname{0}
\expandafter\gdef\csname R@an.replication_all.acdc.nrepl.other.line\endcsname{no random-search, scaled HyReX and single-prompt LLM design has a fresh ACDC pair yet; they are read in the random-search figures}
\expandafter\gdef\csname R@an.replication_all.acdc.nrepl.other.list\endcsname{none}
\expandafter\gdef\csname R@an.replication_all.acdc.nrepl.other.pops\endcsname{none}
\expandafter\gdef\csname R@an.replication_all.acdc.nrepl.phrase\endcsname{4 agent-team arms with a fresh ACDC pair}
\expandafter\gdef\csname R@an.replication_all.acdc.nrepl.set\endcsname{agent-team arms}
\expandafter\gdef\csname R@an.replication_all.acdc.pattern.diffphrase\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.pattern.direction\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.pattern.notisolated\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.pool\endcsname{92.009}
\expandafter\gdef\csname R@an.replication_all.acdc.pooln\endcsname{6}
\expandafter\gdef\csname R@an.replication_all.acdc.poolsd\endcsname{0.099}
\expandafter\gdef\csname R@an.replication_all.acdc.scatter.coverage\endcsname{the $\pm2$\,SD band covers every plotted arm}
\expandafter\gdef\csname R@an.replication_all.acdc.scatter.fired\endcsname{ACDC carries no screen}
\expandafter\gdef\csname R@an.replication_all.acdc.screenbar\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.sddelta\endcsname{0.107}
\expandafter\gdef\csname R@an.replication_all.acdc.sdfreshdelta\endcsname{0.081}
\expandafter\gdef\csname R@an.replication_all.acdc.sel.list\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.sel.meanshrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.sel.n\endcsname{0}
\expandafter\gdef\csname R@an.replication_all.acdc.sel.ndown\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.acdc.teammax\endcsname{45}
\expandafter\gdef\csname R@an.replication_all.acdc.unsel.hi\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.replication_all.acdc.unsel.hw\endcsname{0.237}
\expandafter\gdef\csname R@an.replication_all.acdc.unsel.list\endcsname{HyReX, ResEnc-M, ResEnc-matched, fn.-identical control}
\expandafter\gdef\csname R@an.replication_all.acdc.unsel.list.long\endcsname{HyReX, the library's residual-encoder preset, its ResEnc-matched re-implementation and the function-identical control}
\expandafter\gdef\csname R@an.replication_all.acdc.unsel.lo\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.replication_all.acdc.unsel.meanshrink\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.replication_all.acdc.unsel.n\endcsname{4}
\expandafter\gdef\csname R@an.replication_all.acdc.unsel.nup\endcsname{2}
\expandafter\gdef\csname R@an.replication_all.acdc.unsel.sdexp\endcsname{0.121}
\expandafter\gdef\csname R@an.replication_all.all.ds\endcsname{AMOS22 and KiTS23}
\expandafter\gdef\csname R@an.replication_all.all.ds.screened\endcsname{AMOS22 and KiTS23}
\expandafter\gdef\csname R@an.replication_all.all.nds\endcsname{2}
\expandafter\gdef\csname R@an.replication_all.all.pattern.direction\endcsname{no eligible arm moved up by more than 0.68 no-selection SD of its own dataset, while the never-eligible arms moved in both directions}
\expandafter\gdef\csname R@an.replication_all.all.sel.meanz\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@an.replication_all.all.sel.n\endcsname{24}
\expandafter\gdef\csname R@an.replication_all.all.sel.ndown\endcsname{15}
\expandafter\gdef\csname R@an.replication_all.all.unsel.meanz\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.replication_all.all.unsel.n\endcsname{6}
\expandafter\gdef\csname R@an.replication_all.all.unsel.nup\endcsname{3}
\expandafter\gdef\csname R@an.replication_all.amos.C1.bar0margin\endcsname{\ensuremath{+0.040}}
\expandafter\gdef\csname R@an.replication_all.amos.C1.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.C1.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.amos.C1.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.C1.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.C1.d0\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.replication_all.amos.C1.d0_3\endcsname{\ensuremath{+0.390}}
\expandafter\gdef\csname R@an.replication_all.amos.C1.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.C1.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.C1.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.C1.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.C1.repstate\endcsname{not yet run}
\expandafter\gdef\csname R@an.replication_all.amos.C1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.C1.s0\endcsname{88.091}
\expandafter\gdef\csname R@an.replication_all.amos.C1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.C1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.C1.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.amos.C1.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.C1.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.C1.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.C1.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.C1.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D1.bar0margin\endcsname{\ensuremath{-0.072}}
\expandafter\gdef\csname R@an.replication_all.amos.D1.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D1.class\endcsname{candidate whose screen did not fire}
\expandafter\gdef\csname R@an.replication_all.amos.D1.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.D1.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D1.d0\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.replication_all.amos.D1.d0_3\endcsname{\ensuremath{+0.278}}
\expandafter\gdef\csname R@an.replication_all.amos.D1.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D1.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D1.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.D1.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D1.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.D1.s0\endcsname{87.979}
\expandafter\gdef\csname R@an.replication_all.amos.D1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D1.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.D1.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D1.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D1.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D1.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D1.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D2.bar0margin\endcsname{\ensuremath{-0.712}}
\expandafter\gdef\csname R@an.replication_all.amos.D2.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D2.class\endcsname{candidate whose screen did not fire}
\expandafter\gdef\csname R@an.replication_all.amos.D2.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.D2.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D2.d0\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.replication_all.amos.D2.d0_3\endcsname{\ensuremath{-0.362}}
\expandafter\gdef\csname R@an.replication_all.amos.D2.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D2.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D2.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.D2.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D2.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.D2.s0\endcsname{87.339}
\expandafter\gdef\csname R@an.replication_all.amos.D2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D2.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.D2.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D2.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D2.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D2.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.D2.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.I1.bar0margin\endcsname{\ensuremath{-0.056}}
\expandafter\gdef\csname R@an.replication_all.amos.I1.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.I1.class\endcsname{outside the rule (attribution arm)}
\expandafter\gdef\csname R@an.replication_all.amos.I1.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.I1.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.I1.d0\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.replication_all.amos.I1.d0_3\endcsname{\ensuremath{+0.294}}
\expandafter\gdef\csname R@an.replication_all.amos.I1.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.I1.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.I1.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.I1.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.I1.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.I1.role\endcsname{attribution}
\expandafter\gdef\csname R@an.replication_all.amos.I1.s0\endcsname{87.995}
\expandafter\gdef\csname R@an.replication_all.amos.I1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.I1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.I1.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.I1.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.I1.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.I1.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.I1.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.I1.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L1.bar0margin\endcsname{\ensuremath{+0.297}}
\expandafter\gdef\csname R@an.replication_all.amos.L1.barfreshmargin\endcsname{\ensuremath{+0.115}}
\expandafter\gdef\csname R@an.replication_all.amos.L1.class\endcsname{never eligible}
\expandafter\gdef\csname R@an.replication_all.amos.L1.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.L1.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.L1.d0\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.replication_all.amos.L1.d0_3\endcsname{\ensuremath{+0.647}}
\expandafter\gdef\csname R@an.replication_all.amos.L1.dfresh\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.replication_all.amos.L1.dfresh_3\endcsname{\ensuremath{+0.465}}
\expandafter\gdef\csname R@an.replication_all.amos.L1.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.L1.freshmean\endcsname{88.166}
\expandafter\gdef\csname R@an.replication_all.amos.L1.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.amos.L1.role\endcsname{reference}
\expandafter\gdef\csname R@an.replication_all.amos.L1.s0\endcsname{88.348}
\expandafter\gdef\csname R@an.replication_all.amos.L1.s1\endcsname{88.363}
\expandafter\gdef\csname R@an.replication_all.amos.L1.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.amos.L1.s1reading.class\endcsname{never-eligible}
\expandafter\gdef\csname R@an.replication_all.amos.L1.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.amos.L1.s1reading.phrase\endcsname{inside the never-eligible band, a description since its pair finished before the registration}
\expandafter\gdef\csname R@an.replication_all.amos.L1.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.amos.L1.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.L1.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.amos.L1.s2\endcsname{87.969}
\expandafter\gdef\csname R@an.replication_all.amos.L1.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.amos.L1.sdfresh\endcsname{0.278}
\expandafter\gdef\csname R@an.replication_all.amos.L1.sefresh\endcsname{0.197}
\expandafter\gdef\csname R@an.replication_all.amos.L1.shrink\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.replication_all.amos.L1.shrink_3\endcsname{\ensuremath{-0.182}}
\expandafter\gdef\csname R@an.replication_all.amos.L1.shrinkz\endcsname{\ensuremath{-1.22}}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.bar0margin\endcsname{\ensuremath{-0.212}}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.barfreshmargin\endcsname{\ensuremath{-0.052}}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.class\endcsname{never eligible}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.clearsfresh\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.d0\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.d0_3\endcsname{\ensuremath{+0.138}}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.dfresh\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.dfresh_3\endcsname{\ensuremath{+0.298}}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.freshmean\endcsname{87.999}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.role\endcsname{control}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.s0\endcsname{87.839}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.s1\endcsname{88.127}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.s1reading\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.s1reading.class\endcsname{never-eligible}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.s1reading.phrase\endcsname{inside its registered band}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.s1reading.registered\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.s1reading.state\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.s2\endcsname{87.870}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.sdfresh\endcsname{0.182}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.sefresh\endcsname{0.129}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.shrink\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.shrink_3\endcsname{\ensuremath{+0.160}}
\expandafter\gdef\csname R@an.replication_all.amos.L1b.shrinkz\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.replication_all.amos.L2.bar0margin\endcsname{\ensuremath{+0.012}}
\expandafter\gdef\csname R@an.replication_all.amos.L2.barfreshmargin\endcsname{\ensuremath{-0.156}}
\expandafter\gdef\csname R@an.replication_all.amos.L2.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.amos.L2.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.L2.clearsfresh\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.L2.d0\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.replication_all.amos.L2.d0_3\endcsname{\ensuremath{+0.362}}
\expandafter\gdef\csname R@an.replication_all.amos.L2.dfresh\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.replication_all.amos.L2.dfresh_3\endcsname{\ensuremath{+0.194}}
\expandafter\gdef\csname R@an.replication_all.amos.L2.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.L2.freshmean\endcsname{87.895}
\expandafter\gdef\csname R@an.replication_all.amos.L2.repstate\endcsname{not survived}
\expandafter\gdef\csname R@an.replication_all.amos.L2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.L2.s0\endcsname{88.063}
\expandafter\gdef\csname R@an.replication_all.amos.L2.s1\endcsname{87.956}
\expandafter\gdef\csname R@an.replication_all.amos.L2.s1reading\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.amos.L2.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.amos.L2.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.amos.L2.s1reading.phrase\endcsname{inside its registered band}
\expandafter\gdef\csname R@an.replication_all.amos.L2.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.amos.L2.s1reading.registered\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.L2.s1reading.state\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.amos.L2.s2\endcsname{87.835}
\expandafter\gdef\csname R@an.replication_all.amos.L2.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.amos.L2.sdfresh\endcsname{0.086}
\expandafter\gdef\csname R@an.replication_all.amos.L2.sefresh\endcsname{0.061}
\expandafter\gdef\csname R@an.replication_all.amos.L2.shrink\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.replication_all.amos.L2.shrink_3\endcsname{\ensuremath{-0.168}}
\expandafter\gdef\csname R@an.replication_all.amos.L2.shrinkz\endcsname{\ensuremath{-1.12}}
\expandafter\gdef\csname R@an.replication_all.amos.L3.bar0margin\endcsname{\ensuremath{+0.032}}
\expandafter\gdef\csname R@an.replication_all.amos.L3.barfreshmargin\endcsname{\ensuremath{-0.218}}
\expandafter\gdef\csname R@an.replication_all.amos.L3.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.amos.L3.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.L3.clearsfresh\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.L3.d0\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.replication_all.amos.L3.d0_3\endcsname{\ensuremath{+0.382}}
\expandafter\gdef\csname R@an.replication_all.amos.L3.dfresh\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.replication_all.amos.L3.dfresh_3\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.replication_all.amos.L3.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.L3.freshmean\endcsname{87.833}
\expandafter\gdef\csname R@an.replication_all.amos.L3.repstate\endcsname{not survived}
\expandafter\gdef\csname R@an.replication_all.amos.L3.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.L3.s0\endcsname{88.083}
\expandafter\gdef\csname R@an.replication_all.amos.L3.s1\endcsname{87.981}
\expandafter\gdef\csname R@an.replication_all.amos.L3.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.amos.L3.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.amos.L3.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.amos.L3.s1reading.phrase\endcsname{inside the eligible band, a description since its pair finished before the registration}
\expandafter\gdef\csname R@an.replication_all.amos.L3.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.amos.L3.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.L3.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.amos.L3.s2\endcsname{87.686}
\expandafter\gdef\csname R@an.replication_all.amos.L3.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.amos.L3.sdfresh\endcsname{0.209}
\expandafter\gdef\csname R@an.replication_all.amos.L3.sefresh\endcsname{0.148}
\expandafter\gdef\csname R@an.replication_all.amos.L3.shrink\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.replication_all.amos.L3.shrink_3\endcsname{\ensuremath{-0.249}}
\expandafter\gdef\csname R@an.replication_all.amos.L3.shrinkz\endcsname{\ensuremath{-1.67}}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.bar0margin\endcsname{\ensuremath{+0.109}}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.class\endcsname{outside the rule (attribution arm)}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.d0\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.d0_3\endcsname{\ensuremath{+0.459}}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.repstate\endcsname{not yet run}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.role\endcsname{attribution}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.s0\endcsname{88.160}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3k3.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.bar0margin\endcsname{\ensuremath{-0.082}}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.class\endcsname{outside the rule (attribution arm)}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.d0\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.d0_3\endcsname{\ensuremath{+0.268}}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.role\endcsname{attribution}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.s0\endcsname{87.969}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L3ng.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L4.bar0margin\endcsname{\ensuremath{+0.080}}
\expandafter\gdef\csname R@an.replication_all.amos.L4.barfreshmargin\endcsname{\ensuremath{+0.105}}
\expandafter\gdef\csname R@an.replication_all.amos.L4.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.amos.L4.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.L4.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.L4.d0\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.replication_all.amos.L4.d0_3\endcsname{\ensuremath{+0.430}}
\expandafter\gdef\csname R@an.replication_all.amos.L4.dfresh\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.replication_all.amos.L4.dfresh_3\endcsname{\ensuremath{+0.455}}
\expandafter\gdef\csname R@an.replication_all.amos.L4.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.L4.freshmean\endcsname{88.156}
\expandafter\gdef\csname R@an.replication_all.amos.L4.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.amos.L4.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.L4.s0\endcsname{88.131}
\expandafter\gdef\csname R@an.replication_all.amos.L4.s1\endcsname{88.053}
\expandafter\gdef\csname R@an.replication_all.amos.L4.s1reading\endcsname{outside}
\expandafter\gdef\csname R@an.replication_all.amos.L4.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.amos.L4.s1reading.excess\endcsname{0.005}
\expandafter\gdef\csname R@an.replication_all.amos.L4.s1reading.phrase\endcsname{outside its registered band by 0.005\,pp, above the upper edge}
\expandafter\gdef\csname R@an.replication_all.amos.L4.s1reading.position\endcsname{above}
\expandafter\gdef\csname R@an.replication_all.amos.L4.s1reading.registered\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.L4.s1reading.state\endcsname{outside}
\expandafter\gdef\csname R@an.replication_all.amos.L4.s2\endcsname{88.258}
\expandafter\gdef\csname R@an.replication_all.amos.L4.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.amos.L4.sdfresh\endcsname{0.145}
\expandafter\gdef\csname R@an.replication_all.amos.L4.sefresh\endcsname{0.102}
\expandafter\gdef\csname R@an.replication_all.amos.L4.shrink\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.replication_all.amos.L4.shrink_3\endcsname{\ensuremath{+0.025}}
\expandafter\gdef\csname R@an.replication_all.amos.L4.shrinkz\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.replication_all.amos.L6.bar0margin\endcsname{\ensuremath{-0.334}}
\expandafter\gdef\csname R@an.replication_all.amos.L6.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L6.class\endcsname{candidate whose screen did not fire}
\expandafter\gdef\csname R@an.replication_all.amos.L6.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.L6.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L6.d0\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.replication_all.amos.L6.d0_3\endcsname{\ensuremath{+0.016}}
\expandafter\gdef\csname R@an.replication_all.amos.L6.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L6.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L6.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.L6.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L6.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L6.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.L6.s0\endcsname{87.717}
\expandafter\gdef\csname R@an.replication_all.amos.L6.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L6.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L6.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.L6.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L6.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L6.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L6.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.L6.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.N1.bar0margin\endcsname{\ensuremath{-1.273}}
\expandafter\gdef\csname R@an.replication_all.amos.N1.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.N1.class\endcsname{candidate whose screen did not fire}
\expandafter\gdef\csname R@an.replication_all.amos.N1.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.N1.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.N1.d0\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@an.replication_all.amos.N1.d0_3\endcsname{\ensuremath{-0.923}}
\expandafter\gdef\csname R@an.replication_all.amos.N1.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.N1.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.N1.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.N1.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.N1.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.N1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.N1.s0\endcsname{86.778}
\expandafter\gdef\csname R@an.replication_all.amos.N1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.N1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.N1.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.N1.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.N1.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.N1.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.N1.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.N1.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.bar0margin\endcsname{\ensuremath{-0.343}}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.class\endcsname{never eligible}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.d0\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.d0_3\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.role\endcsname{control}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.s0\endcsname{87.708}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.P3c.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.S2.bar0margin\endcsname{\ensuremath{+0.028}}
\expandafter\gdef\csname R@an.replication_all.amos.S2.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.S2.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.amos.S2.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.S2.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.S2.d0\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.replication_all.amos.S2.d0_3\endcsname{\ensuremath{+0.378}}
\expandafter\gdef\csname R@an.replication_all.amos.S2.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.S2.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.S2.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.S2.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.S2.repstate\endcsname{not yet run}
\expandafter\gdef\csname R@an.replication_all.amos.S2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.S2.s0\endcsname{88.079}
\expandafter\gdef\csname R@an.replication_all.amos.S2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.S2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.S2.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.amos.S2.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.S2.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.S2.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.S2.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.S2.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.bar0margin\endcsname{\ensuremath{-0.309}}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.class\endcsname{candidate whose screen did not fire}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.d0\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.d0_3\endcsname{\ensuremath{+0.041}}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.s0\endcsname{87.742}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5A5.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.bar0margin\endcsname{\ensuremath{-0.611}}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.class\endcsname{candidate whose screen did not fire}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.d0\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.d0_3\endcsname{\ensuremath{-0.261}}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.s0\endcsname{87.440}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B1.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.bar0margin\endcsname{\ensuremath{-0.218}}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.class\endcsname{candidate whose screen did not fire}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.d0\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.d0_3\endcsname{\ensuremath{+0.132}}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.s0\endcsname{87.833}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V5B2.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.bar0margin\endcsname{\ensuremath{+0.137}}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.d0\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.d0_3\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.repstate\endcsname{not yet run}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.s0\endcsname{88.188}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V6A1r.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.bar0margin\endcsname{\ensuremath{-0.395}}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.class\endcsname{candidate whose screen did not fire}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.d0\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.d0_3\endcsname{\ensuremath{-0.045}}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.s0\endcsname{87.657}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A1.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.bar0margin\endcsname{\ensuremath{+0.009}}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.d0\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.d0_3\endcsname{\ensuremath{+0.359}}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.repstate\endcsname{not yet run}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.s0\endcsname{88.060}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7A2.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.bar0margin\endcsname{\ensuremath{-0.786}}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.class\endcsname{candidate whose screen did not fire}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.d0\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.d0_3\endcsname{\ensuremath{-0.436}}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.s0\endcsname{87.266}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B1.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.bar0margin\endcsname{\ensuremath{-0.617}}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.class\endcsname{candidate whose screen did not fire}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.d0\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.d0_3\endcsname{\ensuremath{-0.267}}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.s0\endcsname{87.435}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7B2.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.bar0margin\endcsname{\ensuremath{-0.456}}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.class\endcsname{candidate whose screen did not fire}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.d0\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.d0_3\endcsname{\ensuremath{-0.106}}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.s0\endcsname{87.595}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V7C1.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.bar0margin\endcsname{\ensuremath{-0.855}}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.class\endcsname{candidate whose screen did not fire}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.d0\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.d0_3\endcsname{\ensuremath{-0.505}}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.s0\endcsname{87.196}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A1.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.bar0margin\endcsname{\ensuremath{-0.662}}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.class\endcsname{candidate whose screen did not fire}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.d0\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.d0_3\endcsname{\ensuremath{-0.312}}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.s0\endcsname{87.389}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8A2.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.bar0margin\endcsname{\ensuremath{-1.101}}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.class\endcsname{candidate whose screen did not fire}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.d0\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.d0_3\endcsname{\ensuremath{-0.751}}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.s0\endcsname{86.950}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B1.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.bar0margin\endcsname{\ensuremath{-0.637}}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.class\endcsname{candidate whose screen did not fire}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.d0\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.d0_3\endcsname{\ensuremath{-0.287}}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.s0\endcsname{87.414}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.V8B2.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1.bar0margin\endcsname{\ensuremath{-0.251}}
\expandafter\gdef\csname R@an.replication_all.amos.W1.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1.class\endcsname{candidate whose screen did not fire}
\expandafter\gdef\csname R@an.replication_all.amos.W1.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.W1.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1.d0\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.replication_all.amos.W1.d0_3\endcsname{\ensuremath{+0.099}}
\expandafter\gdef\csname R@an.replication_all.amos.W1.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.W1.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.W1.s0\endcsname{87.800}
\expandafter\gdef\csname R@an.replication_all.amos.W1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.W1.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.bar0margin\endcsname{\ensuremath{+0.013}}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.class\endcsname{never eligible}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.d0\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.d0_3\endcsname{\ensuremath{+0.363}}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.repstate\endcsname{not yet run}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.role\endcsname{control}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.s0\endcsname{88.064}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W1c.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W2.bar0margin\endcsname{\ensuremath{-0.139}}
\expandafter\gdef\csname R@an.replication_all.amos.W2.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W2.class\endcsname{candidate whose screen did not fire}
\expandafter\gdef\csname R@an.replication_all.amos.W2.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.W2.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W2.d0\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.replication_all.amos.W2.d0_3\endcsname{\ensuremath{+0.211}}
\expandafter\gdef\csname R@an.replication_all.amos.W2.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W2.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W2.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.W2.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W2.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.W2.s0\endcsname{87.912}
\expandafter\gdef\csname R@an.replication_all.amos.W2.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W2.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W2.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.W2.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W2.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W2.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W2.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W2.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3.bar0margin\endcsname{\ensuremath{-0.080}}
\expandafter\gdef\csname R@an.replication_all.amos.W3.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3.class\endcsname{candidate whose screen did not fire}
\expandafter\gdef\csname R@an.replication_all.amos.W3.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.W3.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3.d0\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.replication_all.amos.W3.d0_3\endcsname{\ensuremath{+0.270}}
\expandafter\gdef\csname R@an.replication_all.amos.W3.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.W3.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.amos.W3.s0\endcsname{87.971}
\expandafter\gdef\csname R@an.replication_all.amos.W3.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.W3.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.bar0margin\endcsname{\ensuremath{-0.188}}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.class\endcsname{never eligible}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.d0\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.d0_3\endcsname{\ensuremath{+0.162}}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.role\endcsname{control}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.s0\endcsname{87.863}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W3c.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W4.bar0margin\endcsname{\ensuremath{-0.274}}
\expandafter\gdef\csname R@an.replication_all.amos.W4.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W4.class\endcsname{never eligible}
\expandafter\gdef\csname R@an.replication_all.amos.W4.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.W4.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W4.d0\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.replication_all.amos.W4.d0_3\endcsname{\ensuremath{+0.076}}
\expandafter\gdef\csname R@an.replication_all.amos.W4.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W4.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W4.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.W4.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W4.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W4.role\endcsname{reference}
\expandafter\gdef\csname R@an.replication_all.amos.W4.s0\endcsname{87.777}
\expandafter\gdef\csname R@an.replication_all.amos.W4.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W4.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W4.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.amos.W4.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W4.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W4.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W4.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W4.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W5.bar0margin\endcsname{\ensuremath{+0.241}}
\expandafter\gdef\csname R@an.replication_all.amos.W5.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W5.class\endcsname{outside the rule (attribution arm)}
\expandafter\gdef\csname R@an.replication_all.amos.W5.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.W5.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W5.d0\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.replication_all.amos.W5.d0_3\endcsname{\ensuremath{+0.591}}
\expandafter\gdef\csname R@an.replication_all.amos.W5.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W5.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W5.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.W5.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W5.repstate\endcsname{not yet run}
\expandafter\gdef\csname R@an.replication_all.amos.W5.role\endcsname{control}
\expandafter\gdef\csname R@an.replication_all.amos.W5.s0\endcsname{88.292}
\expandafter\gdef\csname R@an.replication_all.amos.W5.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W5.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W5.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.amos.W5.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W5.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W5.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W5.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.W5.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.all3.sentence\endcsname{HyReX improves on the default on all three datasets}
\expandafter\gdef\csname R@an.replication_all.amos.altref\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.replication_all.amos.altref.name\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.replication_all.amos.attr.list\endcsname{pooled-skip control, HyReX w/o GRN, HyReX-k3 and HyReX+pooled skip}
\expandafter\gdef\csname R@an.replication_all.amos.attr.n\endcsname{4}
\expandafter\gdef\csname R@an.replication_all.amos.confound\endcsname{the residual family exactly}
\expandafter\gdef\csname R@an.replication_all.amos.confound.phrase\endcsname{the arms that were never targets are the residual family exactly, so selection and family coincide in this set}
\expandafter\gdef\csname R@an.replication_all.amos.ctlfire.list\endcsname{ResEnc-M, branch control}
\expandafter\gdef\csname R@an.replication_all.amos.ctlfire.max\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.replication_all.amos.ctlfire.maxname\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.replication_all.amos.ctlfire.n\endcsname{2}
\expandafter\gdef\csname R@an.replication_all.amos.cur.hi\endcsname{\ensuremath{-0.069}}
\expandafter\gdef\csname R@an.replication_all.amos.cur.label\endcsname{current model: the candidate designs with a finished seed-0 run now}
\expandafter\gdef\csname R@an.replication_all.amos.cur.lo\endcsname{\ensuremath{-0.611}}
\expandafter\gdef\csname R@an.replication_all.amos.cur.m\endcsname{25}
\expandafter\gdef\csname R@an.replication_all.amos.cur.m_plan\endcsname{12}
\expandafter\gdef\csname R@an.replication_all.amos.cur.never.hi\endcsname{\ensuremath{+0.300}}
\expandafter\gdef\csname R@an.replication_all.amos.cur.never.lo\endcsname{\ensuremath{-0.302}}
\expandafter\gdef\csname R@an.replication_all.amos.cur.plug\endcsname{\ensuremath{-0.240}}
\expandafter\gdef\csname R@an.replication_all.amos.cur.plug_plan\endcsname{\ensuremath{-0.199}}
\expandafter\gdef\csname R@an.replication_all.amos.cur.vs_reg\endcsname{The current model counts 25 candidate designs with a finished seed-0 run against the registered 7}
\expandafter\gdef\csname R@an.replication_all.amos.dfresh.L1minusL3\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.replication_all.amos.dfresh.ahead\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.replication_all.amos.diff\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.replication_all.amos.diff.ratio\endcsname{\ensuremath{-0.87}}
\expandafter\gdef\csname R@an.replication_all.amos.diff.se\endcsname{0.137}
\expandafter\gdef\csname R@an.replication_all.amos.diff.se.kind\endcsname{the no-selection model's standard error at the frozen AMOS22 pool seed SD, not an empirical standard error of these arms}
\expandafter\gdef\csname R@an.replication_all.amos.diff.se.pooled\endcsname{0.165}
\expandafter\gdef\csname R@an.replication_all.amos.diff.se.welch\endcsname{0.189}
\expandafter\gdef\csname R@an.replication_all.amos.diff.sentence\endcsname{the gap between the two groups is \ensuremath{-0.12}\,pp, with a standard error of 0.137\,pp -- the no-selection model's standard error at the frozen AMOS22 pool seed SD, not an empirical standard error of these arms (the empirical SE of these arms is 0.165\,pp pooled and 0.189\,pp unpooled)}
\expandafter\gdef\csname R@an.replication_all.amos.eb.L1.pred\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@an.replication_all.amos.eb.L1b.pred\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.replication_all.amos.eb.L2.pred\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.replication_all.amos.eb.L3.pred\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.replication_all.amos.eb.L4.pred\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.replication_all.amos.eb.factor\endcsname{0.547}
\expandafter\gdef\csname R@an.replication_all.amos.eb.meand0\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.replication_all.amos.eb.n\endcsname{5}
\expandafter\gdef\csname R@an.replication_all.amos.eb.tau2\endcsname{0.018}
\expandafter\gdef\csname R@an.replication_all.amos.eb.verdict\endcsname{exceeds the single-seed variance of the pool by 0.018 pp$^2$ over the 5 arms}
\expandafter\gdef\csname R@an.replication_all.amos.elig.list\endcsname{ConvNeXt-k3, HyReX, ResEnc+context, HyReX, finer ConvNeXt, HyReX+dec. capacity, HyReX-k9 and LeanDeepMid+FD}
\expandafter\gdef\csname R@an.replication_all.amos.elig.n\endcsname{7}
\expandafter\gdef\csname R@an.replication_all.amos.elig.nlanded\endcsname{3}
\expandafter\gdef\csname R@an.replication_all.amos.emax\endcsname{1.966}
\expandafter\gdef\csname R@an.replication_all.amos.expshrink\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.replication_all.amos.expshrink_hi\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.replication_all.amos.expshrink_lo\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.replication_all.amos.expshrink_mc\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.replication_all.amos.expshrink_nu\endcsname{5}
\expandafter\gdef\csname R@an.replication_all.amos.floor\endcsname{2}
\expandafter\gdef\csname R@an.replication_all.amos.hasscreen\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.amos.lead\endcsname{HyReX with 9-kernel coarse stages}
\expandafter\gdef\csname R@an.replication_all.amos.lead.d0\endcsname{\ensuremath{+0.487}}
\expandafter\gdef\csname R@an.replication_all.amos.lead.gap\endcsname{\ensuremath{+0.105}}
\expandafter\gdef\csname R@an.replication_all.amos.lead.nelig\endcsname{7}
\expandafter\gdef\csname R@an.replication_all.amos.lead.pair\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.lead.same.sentence\endcsname{the eligible arm with the largest discovery delta is the registered lead}
\expandafter\gdef\csname R@an.replication_all.amos.lead.two\endcsname{the eligible arm with the largest discovery delta is HyReX with 9-kernel coarse stages (\ensuremath{+0.487}\,pp); the registered lead, HyReX, has the fourth largest of the 7 eligible arms (\ensuremath{+0.382}\,pp)}
\expandafter\gdef\csname R@an.replication_all.amos.leadis\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.amos.leadreg\endcsname{HyReX}
\expandafter\gdef\csname R@an.replication_all.amos.leadreg.d0\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.replication_all.amos.leadreg.rank\endcsname{4}
\expandafter\gdef\csname R@an.replication_all.amos.leadreg.rank.ord\endcsname{fourth largest}
\expandafter\gdef\csname R@an.replication_all.amos.leadreg.shrink\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.replication_all.amos.leadshrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.amos.m\endcsname{25}
\expandafter\gdef\csname R@an.replication_all.amos.m1.coverage\endcsname{all 5 measured shrinkages lie inside it}
\expandafter\gdef\csname R@an.replication_all.amos.never.list\endcsname{ResEnc-M, ResEnc-matched, branch control, trilinear control, MedNeXt-like and fn.-identical control}
\expandafter\gdef\csname R@an.replication_all.amos.never.n\endcsname{6}
\expandafter\gdef\csname R@an.replication_all.amos.nreg\endcsname{7}
\expandafter\gdef\csname R@an.replication_all.amos.nrepl\endcsname{5}
\expandafter\gdef\csname R@an.replication_all.amos.nrepl.other\endcsname{0}
\expandafter\gdef\csname R@an.replication_all.amos.nrepl.other.line\endcsname{no random-search, scaled HyReX and single-prompt LLM design has a fresh AMOS22 pair yet; they are read in the random-search figures}
\expandafter\gdef\csname R@an.replication_all.amos.nrepl.other.list\endcsname{none}
\expandafter\gdef\csname R@an.replication_all.amos.nrepl.other.pops\endcsname{none}
\expandafter\gdef\csname R@an.replication_all.amos.nrepl.phrase\endcsname{5 agent-team arms with a fresh AMOS22 pair}
\expandafter\gdef\csname R@an.replication_all.amos.nrepl.set\endcsname{agent-team arms}
\expandafter\gdef\csname R@an.replication_all.amos.pattern.diffphrase\endcsname{the group difference (eligible minus never-eligible) is \ensuremath{-0.12}\,pp, which locates it at \ensuremath{-0.87} standard errors of the no-selection model}
\expandafter\gdef\csname R@an.replication_all.amos.pattern.direction\endcsname{no eligible arm moved up by more than 0.03\,pp, while the never-eligible arms moved in both directions}
\expandafter\gdef\csname R@an.replication_all.amos.pattern.notisolated\endcsname{The pattern is not uniformly in the direction selection predicts and does not isolate it, because the contrast is observational across designs, hosts and parameter counts; the arms that were never targets are the residual family exactly, so selection and family coincide in this set}
\expandafter\gdef\csname R@an.replication_all.amos.pool\endcsname{87.701}
\expandafter\gdef\csname R@an.replication_all.amos.pooln\endcsname{6}
\expandafter\gdef\csname R@an.replication_all.amos.poolsd\endcsname{0.122}
\expandafter\gdef\csname R@an.replication_all.amos.reg.arms.eligible\endcsname{ConvNeXt-k3 and ResEnc+context}
\expandafter\gdef\csname R@an.replication_all.amos.reg.arms.known\endcsname{HyReX and ResEnc-M}
\expandafter\gdef\csname R@an.replication_all.amos.reg.arms.never\endcsname{ResEnc-matched}
\expandafter\gdef\csname R@an.replication_all.amos.reg.hi\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.replication_all.amos.reg.label\endcsname{Addendum S1}
\expandafter\gdef\csname R@an.replication_all.amos.reg.lo\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.replication_all.amos.reg.m\endcsname{7}
\expandafter\gdef\csname R@an.replication_all.amos.reg.never.hi\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.replication_all.amos.reg.never.lo\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.replication_all.amos.reg.never.width\endcsname{0.60}
\expandafter\gdef\csname R@an.replication_all.amos.reg.nu\endcsname{5}
\expandafter\gdef\csname R@an.replication_all.amos.reg.plug\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.replication_all.amos.reg.sentence\endcsname{Addendum S1, registered 2026-10-06 14:48:52 +08:00, fixed the movement of a selection-eligible arm at \ensuremath{-0.17}\,pp, with a 5--95\,\% range of \ensuremath{-0.49} to \ensuremath{+0.02}\,pp over 7 candidate designs, and the range of a never-eligible arm at \ensuremath{-0.30} to \ensuremath{+0.30}\,pp}
\expandafter\gdef\csname R@an.replication_all.amos.reg.sentence.short\endcsname{Addendum S1 fixed the movement of a selection-eligible arm at \ensuremath{-0.17}\,pp (5--95\,\% range \ensuremath{-0.49} to \ensuremath{+0.02}\,pp) and of a never-eligible arm at \ensuremath{-0.30} to \ensuremath{+0.30}\,pp}
\expandafter\gdef\csname R@an.replication_all.amos.reg.short\endcsname{S1}
\expandafter\gdef\csname R@an.replication_all.amos.reg.time\endcsname{2026-10-06 14:48:52 +08:00}
\expandafter\gdef\csname R@an.replication_all.amos.reg.width\endcsname{0.51}
\expandafter\gdef\csname R@an.replication_all.amos.s1.desc.list\endcsname{HyReX and ResEnc-M}
\expandafter\gdef\csname R@an.replication_all.amos.s1.desc.n\endcsname{2}
\expandafter\gdef\csname R@an.replication_all.amos.s1.desc.ninside\endcsname{2}
\expandafter\gdef\csname R@an.replication_all.amos.s1.inside.list\endcsname{ConvNeXt-k3 and ResEnc-matched}
\expandafter\gdef\csname R@an.replication_all.amos.s1.ninside\endcsname{2}
\expandafter\gdef\csname R@an.replication_all.amos.s1.nlanded\endcsname{3}
\expandafter\gdef\csname R@an.replication_all.amos.s1.noutside\endcsname{1}
\expandafter\gdef\csname R@an.replication_all.amos.s1.npending\endcsname{0}
\expandafter\gdef\csname R@an.replication_all.amos.s1.nreg\endcsname{3}
\expandafter\gdef\csname R@an.replication_all.amos.s1.outside.list\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.replication_all.amos.s1.pending.list\endcsname{none}
\expandafter\gdef\csname R@an.replication_all.amos.s1.summary\endcsname{2 of the 3 registered readings that have landed are inside their band and 1 outside}
\expandafter\gdef\csname R@an.replication_all.amos.scatter.coverage\endcsname{the $\pm2$\,SD band covers every plotted arm}
\expandafter\gdef\csname R@an.replication_all.amos.scatter.fired\endcsname{4 of the 5 plotted arms fired the screen}
\expandafter\gdef\csname R@an.replication_all.amos.screenbar\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.replication_all.amos.sddelta\endcsname{0.132}
\expandafter\gdef\csname R@an.replication_all.amos.sdfreshdelta\endcsname{0.100}
\expandafter\gdef\csname R@an.replication_all.amos.sel.list\endcsname{HyReX, ConvNeXt-k3, ResEnc+context}
\expandafter\gdef\csname R@an.replication_all.amos.sel.meanshrink\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.replication_all.amos.sel.n\endcsname{3}
\expandafter\gdef\csname R@an.replication_all.amos.sel.ndown\endcsname{2}
\expandafter\gdef\csname R@an.replication_all.amos.teammax\endcsname{45}
\expandafter\gdef\csname R@an.replication_all.amos.unsel.hi\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.replication_all.amos.unsel.hw\endcsname{0.293}
\expandafter\gdef\csname R@an.replication_all.amos.unsel.list\endcsname{ResEnc-M, ResEnc-matched}
\expandafter\gdef\csname R@an.replication_all.amos.unsel.list.long\endcsname{the library's residual-encoder preset and its ResEnc-matched re-implementation}
\expandafter\gdef\csname R@an.replication_all.amos.unsel.lo\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.replication_all.amos.unsel.meanshrink\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.replication_all.amos.unsel.n\endcsname{2}
\expandafter\gdef\csname R@an.replication_all.amos.unsel.nup\endcsname{1}
\expandafter\gdef\csname R@an.replication_all.amos.unsel.sdexp\endcsname{0.150}
\expandafter\gdef\csname R@an.replication_all.kits.C1.bar0margin\endcsname{\ensuremath{+3.157}}
\expandafter\gdef\csname R@an.replication_all.kits.C1.barfreshmargin\endcsname{\ensuremath{+2.051}}
\expandafter\gdef\csname R@an.replication_all.kits.C1.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.C1.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.C1.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.C1.d0\endcsname{\ensuremath{+3.51}}
\expandafter\gdef\csname R@an.replication_all.kits.C1.d0_3\endcsname{\ensuremath{+3.507}}
\expandafter\gdef\csname R@an.replication_all.kits.C1.d0_six\endcsname{\ensuremath{+3.264}}
\expandafter\gdef\csname R@an.replication_all.kits.C1.d0pair\endcsname{\ensuremath{+3.507}\,pp over the frozen 3-run pool and \ensuremath{+3.264}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.C1.dfresh\endcsname{\ensuremath{+2.40}}
\expandafter\gdef\csname R@an.replication_all.kits.C1.dfresh_3\endcsname{\ensuremath{+2.401}}
\expandafter\gdef\csname R@an.replication_all.kits.C1.dfresh_six\endcsname{\ensuremath{+2.157}}
\expandafter\gdef\csname R@an.replication_all.kits.C1.dfreshpair\endcsname{\ensuremath{+2.401}\,pp over the frozen 3-run pool and \ensuremath{+2.157}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.C1.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.C1.freshmean\endcsname{85.779}
\expandafter\gdef\csname R@an.replication_all.kits.C1.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.C1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.C1.s0\endcsname{86.885}
\expandafter\gdef\csname R@an.replication_all.kits.C1.s1\endcsname{85.506}
\expandafter\gdef\csname R@an.replication_all.kits.C1.s1reading\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.C1.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.C1.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.C1.s1reading.phrase\endcsname{inside its registered band}
\expandafter\gdef\csname R@an.replication_all.kits.C1.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.C1.s1reading.registered\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.C1.s1reading.state\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.C1.s2\endcsname{86.052}
\expandafter\gdef\csname R@an.replication_all.kits.C1.sameseed\endcsname{\ensuremath{+2.85}}
\expandafter\gdef\csname R@an.replication_all.kits.C1.sameseed.s0\endcsname{\ensuremath{+2.61}}
\expandafter\gdef\csname R@an.replication_all.kits.C1.sameseed.s1\endcsname{\ensuremath{+2.39}}
\expandafter\gdef\csname R@an.replication_all.kits.C1.sameseed.s2\endcsname{\ensuremath{+3.30}}
\expandafter\gdef\csname R@an.replication_all.kits.C1.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.C1.sdfresh\endcsname{0.386}
\expandafter\gdef\csname R@an.replication_all.kits.C1.seedcorr\endcsname{0.805}
\expandafter\gdef\csname R@an.replication_all.kits.C1.sefresh\endcsname{0.273}
\expandafter\gdef\csname R@an.replication_all.kits.C1.shrink\endcsname{\ensuremath{-1.11}}
\expandafter\gdef\csname R@an.replication_all.kits.C1.shrink_3\endcsname{\ensuremath{-1.106}}
\expandafter\gdef\csname R@an.replication_all.kits.C1.shrinkz\endcsname{\ensuremath{-1.14}}
\expandafter\gdef\csname R@an.replication_all.kits.C1.v4reading\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.C1.v4reading.phrase\endcsname{inside its registered band}
\expandafter\gdef\csname R@an.replication_all.kits.C1.v4reading.state\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.D1.bar0margin\endcsname{\ensuremath{+1.257}}
\expandafter\gdef\csname R@an.replication_all.kits.D1.barfreshmargin\endcsname{\ensuremath{+1.127}}
\expandafter\gdef\csname R@an.replication_all.kits.D1.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.D1.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.D1.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.D1.d0\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.replication_all.kits.D1.d0_3\endcsname{\ensuremath{+1.607}}
\expandafter\gdef\csname R@an.replication_all.kits.D1.d0_six\endcsname{\ensuremath{+1.363}}
\expandafter\gdef\csname R@an.replication_all.kits.D1.d0pair\endcsname{\ensuremath{+1.607}\,pp over the frozen 3-run pool and \ensuremath{+1.363}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.D1.dfresh\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.replication_all.kits.D1.dfresh_3\endcsname{\ensuremath{+1.477}}
\expandafter\gdef\csname R@an.replication_all.kits.D1.dfresh_six\endcsname{\ensuremath{+1.233}}
\expandafter\gdef\csname R@an.replication_all.kits.D1.dfreshpair\endcsname{\ensuremath{+1.477}\,pp over the frozen 3-run pool and \ensuremath{+1.233}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.D1.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.D1.freshmean\endcsname{84.855}
\expandafter\gdef\csname R@an.replication_all.kits.D1.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.D1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.D1.s0\endcsname{84.985}
\expandafter\gdef\csname R@an.replication_all.kits.D1.s1\endcsname{85.137}
\expandafter\gdef\csname R@an.replication_all.kits.D1.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.D1.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.D1.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.D1.s1reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.D1.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.D1.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.D1.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.D1.s2\endcsname{84.572}
\expandafter\gdef\csname R@an.replication_all.kits.D1.sameseed\endcsname{\ensuremath{+1.92}}
\expandafter\gdef\csname R@an.replication_all.kits.D1.sameseed.s0\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.replication_all.kits.D1.sameseed.s1\endcsname{\ensuremath{+2.02}}
\expandafter\gdef\csname R@an.replication_all.kits.D1.sameseed.s2\endcsname{\ensuremath{+1.82}}
\expandafter\gdef\csname R@an.replication_all.kits.D1.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.D1.sdfresh\endcsname{0.400}
\expandafter\gdef\csname R@an.replication_all.kits.D1.seedcorr\endcsname{0.472}
\expandafter\gdef\csname R@an.replication_all.kits.D1.sefresh\endcsname{0.283}
\expandafter\gdef\csname R@an.replication_all.kits.D1.shrink\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.replication_all.kits.D1.shrink_3\endcsname{\ensuremath{-0.131}}
\expandafter\gdef\csname R@an.replication_all.kits.D1.shrinkz\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.replication_all.kits.D1.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.D1.v4reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.D1.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.D2.bar0margin\endcsname{\ensuremath{+2.005}}
\expandafter\gdef\csname R@an.replication_all.kits.D2.barfreshmargin\endcsname{\ensuremath{+1.542}}
\expandafter\gdef\csname R@an.replication_all.kits.D2.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.D2.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.D2.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.D2.d0\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.replication_all.kits.D2.d0_3\endcsname{\ensuremath{+2.355}}
\expandafter\gdef\csname R@an.replication_all.kits.D2.d0_six\endcsname{\ensuremath{+2.112}}
\expandafter\gdef\csname R@an.replication_all.kits.D2.d0pair\endcsname{\ensuremath{+2.355}\,pp over the frozen 3-run pool and \ensuremath{+2.112}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.D2.dfresh\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.replication_all.kits.D2.dfresh_3\endcsname{\ensuremath{+1.892}}
\expandafter\gdef\csname R@an.replication_all.kits.D2.dfresh_six\endcsname{\ensuremath{+1.648}}
\expandafter\gdef\csname R@an.replication_all.kits.D2.dfreshpair\endcsname{\ensuremath{+1.892}\,pp over the frozen 3-run pool and \ensuremath{+1.648}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.D2.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.D2.freshmean\endcsname{85.270}
\expandafter\gdef\csname R@an.replication_all.kits.D2.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.D2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.D2.s0\endcsname{85.734}
\expandafter\gdef\csname R@an.replication_all.kits.D2.s1\endcsname{85.357}
\expandafter\gdef\csname R@an.replication_all.kits.D2.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.D2.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.D2.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.D2.s1reading.phrase\endcsname{inside the eligible band, a description since its pair finished before the registration}
\expandafter\gdef\csname R@an.replication_all.kits.D2.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.D2.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.D2.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.D2.s2\endcsname{85.182}
\expandafter\gdef\csname R@an.replication_all.kits.D2.sameseed\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@an.replication_all.kits.D2.sameseed.s0\endcsname{\ensuremath{+1.46}}
\expandafter\gdef\csname R@an.replication_all.kits.D2.sameseed.s1\endcsname{\ensuremath{+2.24}}
\expandafter\gdef\csname R@an.replication_all.kits.D2.sameseed.s2\endcsname{\ensuremath{+2.43}}
\expandafter\gdef\csname R@an.replication_all.kits.D2.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.D2.sdfresh\endcsname{0.124}
\expandafter\gdef\csname R@an.replication_all.kits.D2.seedcorr\endcsname{0.996}
\expandafter\gdef\csname R@an.replication_all.kits.D2.sefresh\endcsname{0.088}
\expandafter\gdef\csname R@an.replication_all.kits.D2.shrink\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@an.replication_all.kits.D2.shrink_3\endcsname{\ensuremath{-0.464}}
\expandafter\gdef\csname R@an.replication_all.kits.D2.shrinkz\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@an.replication_all.kits.D2.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.D2.v4reading.phrase\endcsname{inside the eligible band, a description since its pair finished before the registration}
\expandafter\gdef\csname R@an.replication_all.kits.D2.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.I1.bar0margin\endcsname{\ensuremath{+1.543}}
\expandafter\gdef\csname R@an.replication_all.kits.I1.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.I1.class\endcsname{outside the rule (attribution arm)}
\expandafter\gdef\csname R@an.replication_all.kits.I1.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.I1.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.I1.d0\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.replication_all.kits.I1.d0_3\endcsname{\ensuremath{+1.893}}
\expandafter\gdef\csname R@an.replication_all.kits.I1.d0_six\endcsname{\ensuremath{+1.649}}
\expandafter\gdef\csname R@an.replication_all.kits.I1.d0pair\endcsname{\ensuremath{+1.893}\,pp over the frozen 3-run pool and \ensuremath{+1.649}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.I1.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.I1.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.I1.dfresh_six\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.I1.dfreshpair\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.I1.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.I1.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.I1.repstate\endcsname{not yet run}
\expandafter\gdef\csname R@an.replication_all.kits.I1.role\endcsname{attribution}
\expandafter\gdef\csname R@an.replication_all.kits.I1.s0\endcsname{85.271}
\expandafter\gdef\csname R@an.replication_all.kits.I1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.I1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.I1.sameseed\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.I1.sameseed.s0\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.replication_all.kits.I1.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.I1.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.I1.seedcorr\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.I1.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.I1.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.I1.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.I1.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L1.bar0margin\endcsname{\ensuremath{+1.976}}
\expandafter\gdef\csname R@an.replication_all.kits.L1.barfreshmargin\endcsname{\ensuremath{+3.125}}
\expandafter\gdef\csname R@an.replication_all.kits.L1.class\endcsname{never eligible}
\expandafter\gdef\csname R@an.replication_all.kits.L1.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.L1.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.L1.d0\endcsname{\ensuremath{+2.33}}
\expandafter\gdef\csname R@an.replication_all.kits.L1.d0_3\endcsname{\ensuremath{+2.326}}
\expandafter\gdef\csname R@an.replication_all.kits.L1.d0_six\endcsname{\ensuremath{+2.082}}
\expandafter\gdef\csname R@an.replication_all.kits.L1.d0pair\endcsname{\ensuremath{+2.326}\,pp over the frozen 3-run pool and \ensuremath{+2.082}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.L1.dfresh\endcsname{\ensuremath{+3.48}}
\expandafter\gdef\csname R@an.replication_all.kits.L1.dfresh_3\endcsname{\ensuremath{+3.475}}
\expandafter\gdef\csname R@an.replication_all.kits.L1.dfresh_six\endcsname{\ensuremath{+3.232}}
\expandafter\gdef\csname R@an.replication_all.kits.L1.dfreshpair\endcsname{\ensuremath{+3.475}\,pp over the frozen 3-run pool and \ensuremath{+3.232}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.L1.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.L1.freshmean\endcsname{86.853}
\expandafter\gdef\csname R@an.replication_all.kits.L1.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.L1.role\endcsname{reference}
\expandafter\gdef\csname R@an.replication_all.kits.L1.s0\endcsname{85.704}
\expandafter\gdef\csname R@an.replication_all.kits.L1.s1\endcsname{86.512}
\expandafter\gdef\csname R@an.replication_all.kits.L1.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L1.s1reading.class\endcsname{never-eligible}
\expandafter\gdef\csname R@an.replication_all.kits.L1.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.L1.s1reading.phrase\endcsname{inside the never-eligible band, a description since its pair finished before the registration}
\expandafter\gdef\csname R@an.replication_all.kits.L1.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.L1.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.L1.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L1.s2\endcsname{87.195}
\expandafter\gdef\csname R@an.replication_all.kits.L1.sameseed\endcsname{\ensuremath{+3.92}}
\expandafter\gdef\csname R@an.replication_all.kits.L1.sameseed.s0\endcsname{\ensuremath{+1.43}}
\expandafter\gdef\csname R@an.replication_all.kits.L1.sameseed.s1\endcsname{\ensuremath{+3.40}}
\expandafter\gdef\csname R@an.replication_all.kits.L1.sameseed.s2\endcsname{\ensuremath{+4.45}}
\expandafter\gdef\csname R@an.replication_all.kits.L1.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.L1.sdfresh\endcsname{0.483}
\expandafter\gdef\csname R@an.replication_all.kits.L1.seedcorr\endcsname{\ensuremath{-0.970}}
\expandafter\gdef\csname R@an.replication_all.kits.L1.sefresh\endcsname{0.342}
\expandafter\gdef\csname R@an.replication_all.kits.L1.shrink\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.replication_all.kits.L1.shrink_3\endcsname{\ensuremath{+1.149}}
\expandafter\gdef\csname R@an.replication_all.kits.L1.shrinkz\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.replication_all.kits.L1.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L1.v4reading.phrase\endcsname{inside the never-eligible band, a description since its pair finished before the registration}
\expandafter\gdef\csname R@an.replication_all.kits.L1.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.bar0margin\endcsname{\ensuremath{+1.393}}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.barfreshmargin\endcsname{\ensuremath{+1.963}}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.class\endcsname{never eligible}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.d0\endcsname{\ensuremath{+1.74}}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.d0_3\endcsname{\ensuremath{+1.743}}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.d0_six\endcsname{\ensuremath{+1.499}}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.d0pair\endcsname{\ensuremath{+1.743}\,pp over the frozen 3-run pool and \ensuremath{+1.499}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.dfresh\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.dfresh_3\endcsname{\ensuremath{+2.313}}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.dfresh_six\endcsname{\ensuremath{+2.070}}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.dfreshpair\endcsname{\ensuremath{+2.313}\,pp over the frozen 3-run pool and \ensuremath{+2.070}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.freshmean\endcsname{85.691}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.role\endcsname{control}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.s0\endcsname{85.121}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.s1\endcsname{85.942}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.s1reading.class\endcsname{never-eligible}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.s1reading.phrase\endcsname{inside the never-eligible band, a description since its pair finished before the registration}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.s2\endcsname{85.441}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.sameseed\endcsname{\ensuremath{+2.76}}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.sameseed.s0\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.sameseed.s1\endcsname{\ensuremath{+2.83}}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.sameseed.s2\endcsname{\ensuremath{+2.69}}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.sdfresh\endcsname{0.355}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.seedcorr\endcsname{\ensuremath{-0.636}}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.sefresh\endcsname{0.251}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.shrink\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.shrink_3\endcsname{\ensuremath{+0.571}}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.shrinkz\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.v4reading.phrase\endcsname{inside the never-eligible band, a description since its pair finished before the registration}
\expandafter\gdef\csname R@an.replication_all.kits.L1b.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L2.bar0margin\endcsname{\ensuremath{+0.314}}
\expandafter\gdef\csname R@an.replication_all.kits.L2.barfreshmargin\endcsname{\ensuremath{-0.240}}
\expandafter\gdef\csname R@an.replication_all.kits.L2.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.L2.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.L2.clearsfresh\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.L2.d0\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.replication_all.kits.L2.d0_3\endcsname{\ensuremath{+0.664}}
\expandafter\gdef\csname R@an.replication_all.kits.L2.d0_six\endcsname{\ensuremath{+0.420}}
\expandafter\gdef\csname R@an.replication_all.kits.L2.d0pair\endcsname{\ensuremath{+0.664}\,pp over the frozen 3-run pool and \ensuremath{+0.420}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.L2.dfresh\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.replication_all.kits.L2.dfresh_3\endcsname{\ensuremath{+0.110}}
\expandafter\gdef\csname R@an.replication_all.kits.L2.dfresh_six\endcsname{\ensuremath{-0.133}}
\expandafter\gdef\csname R@an.replication_all.kits.L2.dfreshpair\endcsname{\ensuremath{+0.110}\,pp over the frozen 3-run pool and \ensuremath{-0.133}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.L2.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.L2.freshmean\endcsname{83.489}
\expandafter\gdef\csname R@an.replication_all.kits.L2.repstate\endcsname{not survived}
\expandafter\gdef\csname R@an.replication_all.kits.L2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.L2.s0\endcsname{84.042}
\expandafter\gdef\csname R@an.replication_all.kits.L2.s1\endcsname{82.573}
\expandafter\gdef\csname R@an.replication_all.kits.L2.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L2.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.L2.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.L2.s1reading.phrase\endcsname{inside the eligible band, a description since its pair finished before the registration}
\expandafter\gdef\csname R@an.replication_all.kits.L2.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.L2.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.L2.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L2.s2\endcsname{84.404}
\expandafter\gdef\csname R@an.replication_all.kits.L2.sameseed\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.replication_all.kits.L2.sameseed.s0\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.replication_all.kits.L2.sameseed.s1\endcsname{\ensuremath{-0.54}}
\expandafter\gdef\csname R@an.replication_all.kits.L2.sameseed.s2\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.replication_all.kits.L2.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.L2.sdfresh\endcsname{1.295}
\expandafter\gdef\csname R@an.replication_all.kits.L2.seedcorr\endcsname{0.105}
\expandafter\gdef\csname R@an.replication_all.kits.L2.sefresh\endcsname{0.915}
\expandafter\gdef\csname R@an.replication_all.kits.L2.shrink\endcsname{\ensuremath{-0.55}}
\expandafter\gdef\csname R@an.replication_all.kits.L2.shrink_3\endcsname{\ensuremath{-0.554}}
\expandafter\gdef\csname R@an.replication_all.kits.L2.shrinkz\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.replication_all.kits.L2.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L2.v4reading.phrase\endcsname{inside the eligible band, a description since its pair finished before the registration}
\expandafter\gdef\csname R@an.replication_all.kits.L2.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L3.bar0margin\endcsname{\ensuremath{+2.492}}
\expandafter\gdef\csname R@an.replication_all.kits.L3.barfreshmargin\endcsname{\ensuremath{+1.744}}
\expandafter\gdef\csname R@an.replication_all.kits.L3.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.L3.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.L3.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.L3.d0\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.replication_all.kits.L3.d0_3\endcsname{\ensuremath{+2.842}}
\expandafter\gdef\csname R@an.replication_all.kits.L3.d0_six\endcsname{\ensuremath{+2.598}}
\expandafter\gdef\csname R@an.replication_all.kits.L3.d0pair\endcsname{\ensuremath{+2.842}\,pp over the frozen 3-run pool and \ensuremath{+2.598}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.L3.dfresh\endcsname{\ensuremath{+2.09}}
\expandafter\gdef\csname R@an.replication_all.kits.L3.dfresh_3\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.replication_all.kits.L3.dfresh_six\endcsname{\ensuremath{+1.850}}
\expandafter\gdef\csname R@an.replication_all.kits.L3.dfreshpair\endcsname{\ensuremath{+2.094}\,pp over the frozen 3-run pool and \ensuremath{+1.850}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.L3.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.L3.freshmean\endcsname{85.472}
\expandafter\gdef\csname R@an.replication_all.kits.L3.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.L3.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.L3.s0\endcsname{86.220}
\expandafter\gdef\csname R@an.replication_all.kits.L3.s1\endcsname{85.176}
\expandafter\gdef\csname R@an.replication_all.kits.L3.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L3.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.L3.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.L3.s1reading.phrase\endcsname{inside the eligible band, a description since its pair finished before the registration}
\expandafter\gdef\csname R@an.replication_all.kits.L3.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.L3.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.L3.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L3.s2\endcsname{85.768}
\expandafter\gdef\csname R@an.replication_all.kits.L3.sameseed\endcsname{\ensuremath{+2.54}}
\expandafter\gdef\csname R@an.replication_all.kits.L3.sameseed.s0\endcsname{\ensuremath{+1.95}}
\expandafter\gdef\csname R@an.replication_all.kits.L3.sameseed.s1\endcsname{\ensuremath{+2.06}}
\expandafter\gdef\csname R@an.replication_all.kits.L3.sameseed.s2\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@an.replication_all.kits.L3.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.L3.sdfresh\endcsname{0.419}
\expandafter\gdef\csname R@an.replication_all.kits.L3.seedcorr\endcsname{0.674}
\expandafter\gdef\csname R@an.replication_all.kits.L3.sefresh\endcsname{0.296}
\expandafter\gdef\csname R@an.replication_all.kits.L3.shrink\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.replication_all.kits.L3.shrink_3\endcsname{\ensuremath{-0.748}}
\expandafter\gdef\csname R@an.replication_all.kits.L3.shrinkz\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.replication_all.kits.L3.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L3.v4reading.phrase\endcsname{inside the eligible band, a description since its pair finished before the registration}
\expandafter\gdef\csname R@an.replication_all.kits.L3.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.bar0margin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.class\endcsname{outside the rule (attribution arm)}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.clears0\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.d0\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.d0_3\endcsname{\ensuremath{+1.366}}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.d0_six\endcsname{\ensuremath{+1.123}}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.d0pair\endcsname{\ensuremath{+1.366}\,pp over the frozen 3-run pool and \ensuremath{+1.123}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.dfresh_six\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.dfreshpair\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.role\endcsname{attribution}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.s0\endcsname{84.745}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.sameseed\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.sameseed.s0\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.screen\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.seedcorr\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3k3.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.bar0margin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.class\endcsname{outside the rule (attribution arm)}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.clears0\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.d0\endcsname{\ensuremath{+2.56}}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.d0_3\endcsname{\ensuremath{+2.561}}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.d0_six\endcsname{\ensuremath{+2.317}}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.d0pair\endcsname{\ensuremath{+2.561}\,pp over the frozen 3-run pool and \ensuremath{+2.317}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.dfresh_six\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.dfreshpair\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.role\endcsname{attribution}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.s0\endcsname{85.939}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.sameseed\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.sameseed.s0\endcsname{\ensuremath{+1.67}}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.screen\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.seedcorr\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L3ng.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.L4.bar0margin\endcsname{\ensuremath{+1.848}}
\expandafter\gdef\csname R@an.replication_all.kits.L4.barfreshmargin\endcsname{\ensuremath{+1.896}}
\expandafter\gdef\csname R@an.replication_all.kits.L4.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.L4.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.L4.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.L4.d0\endcsname{\ensuremath{+2.20}}
\expandafter\gdef\csname R@an.replication_all.kits.L4.d0_3\endcsname{\ensuremath{+2.198}}
\expandafter\gdef\csname R@an.replication_all.kits.L4.d0_six\endcsname{\ensuremath{+1.954}}
\expandafter\gdef\csname R@an.replication_all.kits.L4.d0pair\endcsname{\ensuremath{+2.198}\,pp over the frozen 3-run pool and \ensuremath{+1.954}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.L4.dfresh\endcsname{\ensuremath{+2.25}}
\expandafter\gdef\csname R@an.replication_all.kits.L4.dfresh_3\endcsname{\ensuremath{+2.246}}
\expandafter\gdef\csname R@an.replication_all.kits.L4.dfresh_six\endcsname{\ensuremath{+2.003}}
\expandafter\gdef\csname R@an.replication_all.kits.L4.dfreshpair\endcsname{\ensuremath{+2.246}\,pp over the frozen 3-run pool and \ensuremath{+2.003}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.L4.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.L4.freshmean\endcsname{85.625}
\expandafter\gdef\csname R@an.replication_all.kits.L4.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.L4.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.L4.s0\endcsname{85.576}
\expandafter\gdef\csname R@an.replication_all.kits.L4.s1\endcsname{86.055}
\expandafter\gdef\csname R@an.replication_all.kits.L4.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L4.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.L4.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.L4.s1reading.phrase\endcsname{inside the eligible band, a description since its pair finished before the registration}
\expandafter\gdef\csname R@an.replication_all.kits.L4.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.L4.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.L4.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L4.s2\endcsname{85.194}
\expandafter\gdef\csname R@an.replication_all.kits.L4.sameseed\endcsname{\ensuremath{+2.69}}
\expandafter\gdef\csname R@an.replication_all.kits.L4.sameseed.s0\endcsname{\ensuremath{+1.30}}
\expandafter\gdef\csname R@an.replication_all.kits.L4.sameseed.s1\endcsname{\ensuremath{+2.94}}
\expandafter\gdef\csname R@an.replication_all.kits.L4.sameseed.s2\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@an.replication_all.kits.L4.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.L4.sdfresh\endcsname{0.609}
\expandafter\gdef\csname R@an.replication_all.kits.L4.seedcorr\endcsname{0.166}
\expandafter\gdef\csname R@an.replication_all.kits.L4.sefresh\endcsname{0.431}
\expandafter\gdef\csname R@an.replication_all.kits.L4.shrink\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.replication_all.kits.L4.shrink_3\endcsname{\ensuremath{+0.048}}
\expandafter\gdef\csname R@an.replication_all.kits.L4.shrinkz\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.replication_all.kits.L4.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L4.v4reading.phrase\endcsname{inside the eligible band, a description since its pair finished before the registration}
\expandafter\gdef\csname R@an.replication_all.kits.L4.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L6.bar0margin\endcsname{\ensuremath{+2.176}}
\expandafter\gdef\csname R@an.replication_all.kits.L6.barfreshmargin\endcsname{\ensuremath{+1.241}}
\expandafter\gdef\csname R@an.replication_all.kits.L6.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.L6.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.L6.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.L6.d0\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.replication_all.kits.L6.d0_3\endcsname{\ensuremath{+2.526}}
\expandafter\gdef\csname R@an.replication_all.kits.L6.d0_six\endcsname{\ensuremath{+2.283}}
\expandafter\gdef\csname R@an.replication_all.kits.L6.d0pair\endcsname{\ensuremath{+2.526}\,pp over the frozen 3-run pool and \ensuremath{+2.283}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.L6.dfresh\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.replication_all.kits.L6.dfresh_3\endcsname{\ensuremath{+1.591}}
\expandafter\gdef\csname R@an.replication_all.kits.L6.dfresh_six\endcsname{\ensuremath{+1.348}}
\expandafter\gdef\csname R@an.replication_all.kits.L6.dfreshpair\endcsname{\ensuremath{+1.591}\,pp over the frozen 3-run pool and \ensuremath{+1.348}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.L6.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.L6.freshmean\endcsname{84.970}
\expandafter\gdef\csname R@an.replication_all.kits.L6.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.L6.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.L6.s0\endcsname{85.904}
\expandafter\gdef\csname R@an.replication_all.kits.L6.s1\endcsname{84.577}
\expandafter\gdef\csname R@an.replication_all.kits.L6.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L6.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.L6.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.L6.s1reading.phrase\endcsname{inside the eligible band, a description since its pair finished before the registration}
\expandafter\gdef\csname R@an.replication_all.kits.L6.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.L6.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.L6.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L6.s2\endcsname{85.363}
\expandafter\gdef\csname R@an.replication_all.kits.L6.sameseed\endcsname{\ensuremath{+2.04}}
\expandafter\gdef\csname R@an.replication_all.kits.L6.sameseed.s0\endcsname{\ensuremath{+1.63}}
\expandafter\gdef\csname R@an.replication_all.kits.L6.sameseed.s1\endcsname{\ensuremath{+1.46}}
\expandafter\gdef\csname R@an.replication_all.kits.L6.sameseed.s2\endcsname{\ensuremath{+2.61}}
\expandafter\gdef\csname R@an.replication_all.kits.L6.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.L6.sdfresh\endcsname{0.556}
\expandafter\gdef\csname R@an.replication_all.kits.L6.seedcorr\endcsname{0.652}
\expandafter\gdef\csname R@an.replication_all.kits.L6.sefresh\endcsname{0.393}
\expandafter\gdef\csname R@an.replication_all.kits.L6.shrink\endcsname{\ensuremath{-0.93}}
\expandafter\gdef\csname R@an.replication_all.kits.L6.shrink_3\endcsname{\ensuremath{-0.935}}
\expandafter\gdef\csname R@an.replication_all.kits.L6.shrinkz\endcsname{\ensuremath{-0.96}}
\expandafter\gdef\csname R@an.replication_all.kits.L6.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.L6.v4reading.phrase\endcsname{inside the eligible band, a description since its pair finished before the registration}
\expandafter\gdef\csname R@an.replication_all.kits.L6.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.N1.bar0margin\endcsname{\ensuremath{-6.842}}
\expandafter\gdef\csname R@an.replication_all.kits.N1.barfreshmargin\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.N1.class\endcsname{candidate whose screen did not fire}
\expandafter\gdef\csname R@an.replication_all.kits.N1.clears0\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.N1.clearsfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.N1.d0\endcsname{\ensuremath{-6.49}}
\expandafter\gdef\csname R@an.replication_all.kits.N1.d0_3\endcsname{\ensuremath{-6.492}}
\expandafter\gdef\csname R@an.replication_all.kits.N1.d0_six\endcsname{\ensuremath{-6.736}}
\expandafter\gdef\csname R@an.replication_all.kits.N1.d0pair\endcsname{\ensuremath{-6.492}\,pp over the frozen 3-run pool and \ensuremath{-6.736}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.N1.dfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.N1.dfresh_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.N1.dfresh_six\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.N1.dfreshpair\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.N1.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.N1.freshmean\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.N1.repstate\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.N1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.N1.s0\endcsname{76.886}
\expandafter\gdef\csname R@an.replication_all.kits.N1.s1\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.N1.s2\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.N1.sameseed\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.N1.sameseed.s0\endcsname{\ensuremath{-7.39}}
\expandafter\gdef\csname R@an.replication_all.kits.N1.screen\endcsname{did not fire the screen}
\expandafter\gdef\csname R@an.replication_all.kits.N1.sdfresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.N1.seedcorr\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.N1.sefresh\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.N1.shrink\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.N1.shrink_3\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.N1.shrinkz\endcsname{\pend}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.bar0margin\endcsname{\ensuremath{+1.014}}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.barfreshmargin\endcsname{\ensuremath{+0.826}}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.class\endcsname{never eligible}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.d0\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.d0_3\endcsname{\ensuremath{+1.364}}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.d0_six\endcsname{\ensuremath{+1.121}}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.d0pair\endcsname{\ensuremath{+1.364}\,pp over the frozen 3-run pool and \ensuremath{+1.121}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.dfresh\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.dfresh_3\endcsname{\ensuremath{+1.176}}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.dfresh_six\endcsname{\ensuremath{+0.932}}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.dfreshpair\endcsname{\ensuremath{+1.176}\,pp over the frozen 3-run pool and \ensuremath{+0.932}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.freshmean\endcsname{84.554}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.role\endcsname{control}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.s0\endcsname{84.743}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.s1\endcsname{84.529}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.s1reading\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.s1reading.class\endcsname{never-eligible}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.s1reading.phrase\endcsname{inside its registered band}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.s1reading.registered\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.s1reading.state\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.s2\endcsname{84.579}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.sameseed\endcsname{\ensuremath{+1.62}}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.sameseed.s0\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.sameseed.s1\endcsname{\ensuremath{+1.42}}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.sameseed.s2\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.sdfresh\endcsname{0.035}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.seedcorr\endcsname{0.898}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.sefresh\endcsname{0.025}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.shrink\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.shrink_3\endcsname{\ensuremath{-0.189}}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.shrinkz\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.v4reading\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.v4reading.phrase\endcsname{inside its registered band}
\expandafter\gdef\csname R@an.replication_all.kits.P3c.v4reading.state\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.S2.bar0margin\endcsname{\ensuremath{+0.991}}
\expandafter\gdef\csname R@an.replication_all.kits.S2.barfreshmargin\endcsname{\ensuremath{+0.220}}
\expandafter\gdef\csname R@an.replication_all.kits.S2.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.S2.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.S2.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.S2.d0\endcsname{\ensuremath{+1.34}}
\expandafter\gdef\csname R@an.replication_all.kits.S2.d0_3\endcsname{\ensuremath{+1.341}}
\expandafter\gdef\csname R@an.replication_all.kits.S2.d0_six\endcsname{\ensuremath{+1.098}}
\expandafter\gdef\csname R@an.replication_all.kits.S2.d0pair\endcsname{\ensuremath{+1.341}\,pp over the frozen 3-run pool and \ensuremath{+1.098}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.S2.dfresh\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.replication_all.kits.S2.dfresh_3\endcsname{\ensuremath{+0.570}}
\expandafter\gdef\csname R@an.replication_all.kits.S2.dfresh_six\endcsname{\ensuremath{+0.326}}
\expandafter\gdef\csname R@an.replication_all.kits.S2.dfreshpair\endcsname{\ensuremath{+0.570}\,pp over the frozen 3-run pool and \ensuremath{+0.326}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.S2.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.S2.freshmean\endcsname{83.948}
\expandafter\gdef\csname R@an.replication_all.kits.S2.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.S2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.S2.s0\endcsname{84.720}
\expandafter\gdef\csname R@an.replication_all.kits.S2.s1\endcsname{84.161}
\expandafter\gdef\csname R@an.replication_all.kits.S2.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.S2.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.S2.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.S2.s1reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.S2.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.S2.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.S2.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.S2.s2\endcsname{83.736}
\expandafter\gdef\csname R@an.replication_all.kits.S2.sameseed\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.replication_all.kits.S2.sameseed.s0\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.replication_all.kits.S2.sameseed.s1\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.replication_all.kits.S2.sameseed.s2\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.replication_all.kits.S2.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.S2.sdfresh\endcsname{0.300}
\expandafter\gdef\csname R@an.replication_all.kits.S2.seedcorr\endcsname{0.977}
\expandafter\gdef\csname R@an.replication_all.kits.S2.sefresh\endcsname{0.212}
\expandafter\gdef\csname R@an.replication_all.kits.S2.shrink\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.replication_all.kits.S2.shrink_3\endcsname{\ensuremath{-0.771}}
\expandafter\gdef\csname R@an.replication_all.kits.S2.shrinkz\endcsname{\ensuremath{-0.79}}
\expandafter\gdef\csname R@an.replication_all.kits.S2.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.S2.v4reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.S2.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.bar0margin\endcsname{\ensuremath{+1.599}}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.barfreshmargin\endcsname{\ensuremath{+1.815}}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.d0\endcsname{\ensuremath{+1.95}}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.d0_3\endcsname{\ensuremath{+1.949}}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.d0_six\endcsname{\ensuremath{+1.706}}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.d0pair\endcsname{\ensuremath{+1.949}\,pp over the frozen 3-run pool and \ensuremath{+1.706}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.dfresh\endcsname{\ensuremath{+2.17}}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.dfresh_3\endcsname{\ensuremath{+2.165}}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.dfresh_six\endcsname{\ensuremath{+1.922}}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.dfreshpair\endcsname{\ensuremath{+2.165}\,pp over the frozen 3-run pool and \ensuremath{+1.922}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.freshmean\endcsname{85.544}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.s0\endcsname{85.328}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.s1\endcsname{85.726}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.s1reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.s2\endcsname{85.361}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.sameseed\endcsname{\ensuremath{+2.61}}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.sameseed.s0\endcsname{\ensuremath{+1.06}}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.sameseed.s1\endcsname{\ensuremath{+2.61}}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.sameseed.s2\endcsname{\ensuremath{+2.61}}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.sdfresh\endcsname{0.258}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.seedcorr\endcsname{\ensuremath{-0.360}}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.sefresh\endcsname{0.182}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.shrink\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.shrink_3\endcsname{\ensuremath{+0.216}}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.shrinkz\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.v4reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V5A5.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.bar0margin\endcsname{\ensuremath{+1.812}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.barfreshmargin\endcsname{\ensuremath{+1.935}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.d0\endcsname{\ensuremath{+2.16}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.d0_3\endcsname{\ensuremath{+2.162}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.d0_six\endcsname{\ensuremath{+1.919}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.d0pair\endcsname{\ensuremath{+2.162}\,pp over the frozen 3-run pool and \ensuremath{+1.919}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.dfresh\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.dfresh_3\endcsname{\ensuremath{+2.285}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.dfresh_six\endcsname{\ensuremath{+2.042}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.dfreshpair\endcsname{\ensuremath{+2.285}\,pp over the frozen 3-run pool and \ensuremath{+2.042}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.freshmean\endcsname{85.663}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.s0\endcsname{85.541}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.s1\endcsname{85.620}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.s1reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.s2\endcsname{85.707}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.sameseed\endcsname{\ensuremath{+2.73}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.sameseed.s0\endcsname{\ensuremath{+1.27}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.sameseed.s1\endcsname{\ensuremath{+2.51}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.sameseed.s2\endcsname{\ensuremath{+2.96}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.sdfresh\endcsname{0.061}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.seedcorr\endcsname{\ensuremath{-0.950}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.sefresh\endcsname{0.043}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.shrink\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.shrink_3\endcsname{\ensuremath{+0.123}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.shrinkz\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.v4reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V5B1.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.bar0margin\endcsname{\ensuremath{+0.914}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.barfreshmargin\endcsname{\ensuremath{+1.098}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.d0\endcsname{\ensuremath{+1.26}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.d0_3\endcsname{\ensuremath{+1.264}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.d0_six\endcsname{\ensuremath{+1.021}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.d0pair\endcsname{\ensuremath{+1.264}\,pp over the frozen 3-run pool and \ensuremath{+1.021}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.dfresh\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.dfresh_3\endcsname{\ensuremath{+1.448}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.dfresh_six\endcsname{\ensuremath{+1.205}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.dfreshpair\endcsname{\ensuremath{+1.448}\,pp over the frozen 3-run pool and \ensuremath{+1.205}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.freshmean\endcsname{84.826}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.s0\endcsname{84.643}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.s1\endcsname{84.876}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.s1reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.s2\endcsname{84.777}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.sameseed\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.sameseed.s0\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.sameseed.s1\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.sameseed.s2\endcsname{\ensuremath{+2.03}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.sdfresh\endcsname{0.070}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.seedcorr\endcsname{\ensuremath{-0.786}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.sefresh\endcsname{0.049}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.shrink\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.shrink_3\endcsname{\ensuremath{+0.184}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.shrinkz\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.v4reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V5B2.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.bar0margin\endcsname{\ensuremath{+1.886}}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.barfreshmargin\endcsname{\ensuremath{+1.354}}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.d0\endcsname{\ensuremath{+2.24}}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.d0_3\endcsname{\ensuremath{+2.236}}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.d0_six\endcsname{\ensuremath{+1.992}}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.d0pair\endcsname{\ensuremath{+2.236}\,pp over the frozen 3-run pool and \ensuremath{+1.992}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.dfresh\endcsname{\ensuremath{+1.70}}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.dfresh_3\endcsname{\ensuremath{+1.704}}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.dfresh_six\endcsname{\ensuremath{+1.461}}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.dfreshpair\endcsname{\ensuremath{+1.704}\,pp over the frozen 3-run pool and \ensuremath{+1.461}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.freshmean\endcsname{85.082}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.s0\endcsname{85.614}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.s1\endcsname{85.073}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.s1reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.s2\endcsname{85.091}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.sameseed\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.sameseed.s0\endcsname{\ensuremath{+1.34}}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.sameseed.s1\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.sameseed.s2\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.sdfresh\endcsname{0.013}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.seedcorr\endcsname{0.966}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.sefresh\endcsname{0.009}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.shrink\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.shrink_3\endcsname{\ensuremath{-0.532}}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.shrinkz\endcsname{\ensuremath{-0.55}}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.v4reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V6A1r.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.bar0margin\endcsname{\ensuremath{+2.198}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.barfreshmargin\endcsname{\ensuremath{+2.312}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.d0\endcsname{\ensuremath{+2.55}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.d0_3\endcsname{\ensuremath{+2.548}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.d0_six\endcsname{\ensuremath{+2.305}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.d0pair\endcsname{\ensuremath{+2.548}\,pp over the frozen 3-run pool and \ensuremath{+2.305}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.dfresh\endcsname{\ensuremath{+2.66}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.dfresh_3\endcsname{\ensuremath{+2.662}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.dfresh_six\endcsname{\ensuremath{+2.418}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.dfreshpair\endcsname{\ensuremath{+2.662}\,pp over the frozen 3-run pool and \ensuremath{+2.418}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.freshmean\endcsname{86.040}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.s0\endcsname{85.927}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.s1\endcsname{85.705}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.s1reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.s2\endcsname{86.375}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.sameseed\endcsname{\ensuremath{+3.11}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.sameseed.s0\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.sameseed.s1\endcsname{\ensuremath{+2.59}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.sameseed.s2\endcsname{\ensuremath{+3.63}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.sdfresh\endcsname{0.474}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.seedcorr\endcsname{\ensuremath{-0.411}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.sefresh\endcsname{0.335}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.shrink\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.shrink_3\endcsname{\ensuremath{+0.113}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.shrinkz\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.v4reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V7A1.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.bar0margin\endcsname{\ensuremath{+2.536}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.barfreshmargin\endcsname{\ensuremath{+1.939}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.d0\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.d0_3\endcsname{\ensuremath{+2.886}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.d0_six\endcsname{\ensuremath{+2.642}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.d0pair\endcsname{\ensuremath{+2.886}\,pp over the frozen 3-run pool and \ensuremath{+2.642}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.dfresh\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.dfresh_3\endcsname{\ensuremath{+2.289}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.dfresh_six\endcsname{\ensuremath{+2.046}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.dfreshpair\endcsname{\ensuremath{+2.289}\,pp over the frozen 3-run pool and \ensuremath{+2.046}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.freshmean\endcsname{85.667}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.s0\endcsname{86.264}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.s1\endcsname{85.351}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.s1reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.s2\endcsname{85.984}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.sameseed\endcsname{\ensuremath{+2.74}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.sameseed.s0\endcsname{\ensuremath{+1.99}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.sameseed.s1\endcsname{\ensuremath{+2.24}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.sameseed.s2\endcsname{\ensuremath{+3.23}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.sdfresh\endcsname{0.447}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.seedcorr\endcsname{0.562}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.sefresh\endcsname{0.316}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.shrink\endcsname{\ensuremath{-0.60}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.shrink_3\endcsname{\ensuremath{-0.597}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.shrinkz\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.v4reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V7A2.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.bar0margin\endcsname{\ensuremath{+1.371}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.barfreshmargin\endcsname{\ensuremath{+2.032}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.d0\endcsname{\ensuremath{+1.72}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.d0_3\endcsname{\ensuremath{+1.721}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.d0_six\endcsname{\ensuremath{+1.478}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.d0pair\endcsname{\ensuremath{+1.721}\,pp over the frozen 3-run pool and \ensuremath{+1.478}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.dfresh\endcsname{\ensuremath{+2.38}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.dfresh_3\endcsname{\ensuremath{+2.382}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.dfresh_six\endcsname{\ensuremath{+2.138}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.dfreshpair\endcsname{\ensuremath{+2.382}\,pp over the frozen 3-run pool and \ensuremath{+2.138}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.freshmean\endcsname{85.760}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.s0\endcsname{85.100}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.s1\endcsname{85.431}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.s1reading.excess\endcsname{0.393}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.s1reading.phrase\endcsname{outside the eligible band by 0.393\,pp, above the upper edge, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.s1reading.position\endcsname{above}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.s2\endcsname{86.088}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.sameseed\endcsname{\ensuremath{+2.83}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.sameseed.s0\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.sameseed.s1\endcsname{\ensuremath{+2.32}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.sameseed.s2\endcsname{\ensuremath{+3.34}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.sdfresh\endcsname{0.465}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.seedcorr\endcsname{\ensuremath{-0.887}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.sefresh\endcsname{0.329}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.shrink\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.shrink_3\endcsname{\ensuremath{+0.660}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.shrinkz\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.v4reading.phrase\endcsname{outside the eligible band by 0.393\,pp, above the upper edge, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V7B1.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.bar0margin\endcsname{\ensuremath{+2.474}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.barfreshmargin\endcsname{\ensuremath{+1.488}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.d0\endcsname{\ensuremath{+2.82}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.d0_3\endcsname{\ensuremath{+2.824}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.d0_six\endcsname{\ensuremath{+2.581}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.d0pair\endcsname{\ensuremath{+2.824}\,pp over the frozen 3-run pool and \ensuremath{+2.581}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.dfresh\endcsname{\ensuremath{+1.84}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.dfresh_3\endcsname{\ensuremath{+1.838}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.dfresh_six\endcsname{\ensuremath{+1.595}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.dfreshpair\endcsname{\ensuremath{+1.838}\,pp over the frozen 3-run pool and \ensuremath{+1.595}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.freshmean\endcsname{85.217}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.s0\endcsname{86.203}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.s1\endcsname{85.773}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.s1reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.s2\endcsname{84.660}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.sameseed\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.sameseed.s0\endcsname{\ensuremath{+1.93}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.sameseed.s1\endcsname{\ensuremath{+2.66}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.sameseed.s2\endcsname{\ensuremath{+1.91}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.sdfresh\endcsname{0.787}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.seedcorr\endcsname{0.856}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.sefresh\endcsname{0.557}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.shrink\endcsname{\ensuremath{-0.99}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.shrink_3\endcsname{\ensuremath{-0.986}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.shrinkz\endcsname{\ensuremath{-1.01}}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.v4reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V7B2.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.bar0margin\endcsname{\ensuremath{+2.357}}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.barfreshmargin\endcsname{\ensuremath{+2.090}}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.d0\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.d0_3\endcsname{\ensuremath{+2.707}}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.d0_six\endcsname{\ensuremath{+2.463}}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.d0pair\endcsname{\ensuremath{+2.707}\,pp over the frozen 3-run pool and \ensuremath{+2.463}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.dfresh\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.dfresh_3\endcsname{\ensuremath{+2.440}}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.dfresh_six\endcsname{\ensuremath{+2.196}}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.dfreshpair\endcsname{\ensuremath{+2.440}\,pp over the frozen 3-run pool and \ensuremath{+2.196}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.freshmean\endcsname{85.818}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.s0\endcsname{86.085}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.s1\endcsname{86.137}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.s1reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.s2\endcsname{85.500}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.sameseed\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.sameseed.s0\endcsname{\ensuremath{+1.81}}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.sameseed.s1\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.sameseed.s2\endcsname{\ensuremath{+2.75}}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.sdfresh\endcsname{0.450}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.seedcorr\endcsname{0.630}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.sefresh\endcsname{0.318}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.shrink\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.shrink_3\endcsname{\ensuremath{-0.267}}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.shrinkz\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.v4reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V7C1.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.bar0margin\endcsname{\ensuremath{+1.410}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.barfreshmargin\endcsname{\ensuremath{+0.899}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.d0\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.d0_3\endcsname{\ensuremath{+1.760}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.d0_six\endcsname{\ensuremath{+1.516}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.d0pair\endcsname{\ensuremath{+1.760}\,pp over the frozen 3-run pool and \ensuremath{+1.516}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.dfresh\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.dfresh_3\endcsname{\ensuremath{+1.249}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.dfresh_six\endcsname{\ensuremath{+1.005}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.dfreshpair\endcsname{\ensuremath{+1.249}\,pp over the frozen 3-run pool and \ensuremath{+1.005}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.freshmean\endcsname{84.627}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.s0\endcsname{85.138}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.s1\endcsname{84.456}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.s1reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.s2\endcsname{84.799}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.sameseed\endcsname{\ensuremath{+1.70}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.sameseed.s0\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.sameseed.s1\endcsname{\ensuremath{+1.34}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.sameseed.s2\endcsname{\ensuremath{+2.05}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.sdfresh\endcsname{0.243}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.seedcorr\endcsname{0.726}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.sefresh\endcsname{0.172}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.shrink\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.shrink_3\endcsname{\ensuremath{-0.511}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.shrinkz\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.v4reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V8A1.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.bar0margin\endcsname{\ensuremath{+1.003}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.barfreshmargin\endcsname{\ensuremath{+1.527}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.d0\endcsname{\ensuremath{+1.35}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.d0_3\endcsname{\ensuremath{+1.353}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.d0_six\endcsname{\ensuremath{+1.110}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.d0pair\endcsname{\ensuremath{+1.353}\,pp over the frozen 3-run pool and \ensuremath{+1.110}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.dfresh\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.dfresh_3\endcsname{\ensuremath{+1.877}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.dfresh_six\endcsname{\ensuremath{+1.634}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.dfreshpair\endcsname{\ensuremath{+1.877}\,pp over the frozen 3-run pool and \ensuremath{+1.634}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.freshmean\endcsname{85.255}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.s0\endcsname{84.732}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.s1\endcsname{84.971}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.s1reading.excess\endcsname{0.257}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.s1reading.phrase\endcsname{outside the eligible band by 0.257\,pp, above the upper edge, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.s1reading.position\endcsname{above}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.s2\endcsname{85.540}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.sameseed\endcsname{\ensuremath{+2.32}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.sameseed.s0\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.sameseed.s1\endcsname{\ensuremath{+1.86}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.sameseed.s2\endcsname{\ensuremath{+2.79}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.sdfresh\endcsname{0.402}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.seedcorr\endcsname{\ensuremath{-0.866}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.sefresh\endcsname{0.284}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.shrink\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.shrink_3\endcsname{\ensuremath{+0.524}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.shrinkz\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.v4reading.phrase\endcsname{outside the eligible band by 0.257\,pp, above the upper edge, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V8A2.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.bar0margin\endcsname{\ensuremath{+2.561}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.barfreshmargin\endcsname{\ensuremath{+1.025}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.d0\endcsname{\ensuremath{+2.91}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.d0_3\endcsname{\ensuremath{+2.911}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.d0_six\endcsname{\ensuremath{+2.667}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.d0pair\endcsname{\ensuremath{+2.911}\,pp over the frozen 3-run pool and \ensuremath{+2.667}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.dfresh\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.dfresh_3\endcsname{\ensuremath{+1.375}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.dfresh_six\endcsname{\ensuremath{+1.131}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.dfreshpair\endcsname{\ensuremath{+1.375}\,pp over the frozen 3-run pool and \ensuremath{+1.131}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.freshmean\endcsname{84.753}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.s0\endcsname{86.289}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.s1\endcsname{85.457}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.s1reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.s2\endcsname{84.049}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.sameseed\endcsname{\ensuremath{+1.82}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.sameseed.s0\endcsname{\ensuremath{+2.02}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.sameseed.s1\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.sameseed.s2\endcsname{\ensuremath{+1.30}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.sdfresh\endcsname{0.996}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.seedcorr\endcsname{0.905}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.sefresh\endcsname{0.704}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.shrink\endcsname{\ensuremath{-1.54}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.shrink_3\endcsname{\ensuremath{-1.536}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.shrinkz\endcsname{\ensuremath{-1.58}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.v4reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V8B1.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.bar0margin\endcsname{\ensuremath{+1.296}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.barfreshmargin\endcsname{\ensuremath{+1.381}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.d0\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.d0_3\endcsname{\ensuremath{+1.646}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.d0_six\endcsname{\ensuremath{+1.402}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.d0pair\endcsname{\ensuremath{+1.646}\,pp over the frozen 3-run pool and \ensuremath{+1.402}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.dfresh\endcsname{\ensuremath{+1.73}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.dfresh_3\endcsname{\ensuremath{+1.731}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.dfresh_six\endcsname{\ensuremath{+1.487}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.dfreshpair\endcsname{\ensuremath{+1.731}\,pp over the frozen 3-run pool and \ensuremath{+1.487}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.eligible\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.freshmean\endcsname{85.109}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.role\endcsname{candidate}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.s0\endcsname{85.024}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.s1\endcsname{85.270}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.s1reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.s1reading.class\endcsname{eligible}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.s1reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.s1reading.registered\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.s1reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.s2\endcsname{84.949}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.sameseed\endcsname{\ensuremath{+2.18}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.sameseed.s0\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.sameseed.s1\endcsname{\ensuremath{+2.16}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.sameseed.s2\endcsname{\ensuremath{+2.20}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.sdfresh\endcsname{0.227}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.seedcorr\endcsname{\ensuremath{-0.066}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.sefresh\endcsname{0.161}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.shrink\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.shrink_3\endcsname{\ensuremath{+0.085}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.shrinkz\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.v4reading\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.v4reading.phrase\endcsname{inside the eligible band, a description since no reading was registered for it}
\expandafter\gdef\csname R@an.replication_all.kits.V8B2.v4reading.state\endcsname{description only}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.bar0margin\endcsname{\ensuremath{+2.286}}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.barfreshmargin\endcsname{\ensuremath{+0.717}}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.class\endcsname{never eligible}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.clears0\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.clearsfresh\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.d0\endcsname{\ensuremath{+2.64}}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.d0_3\endcsname{\ensuremath{+2.636}}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.d0_six\endcsname{\ensuremath{+2.392}}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.d0pair\endcsname{\ensuremath{+2.636}\,pp over the frozen 3-run pool and \ensuremath{+2.392}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.dfresh\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.dfresh_3\endcsname{\ensuremath{+1.067}}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.dfresh_six\endcsname{\ensuremath{+0.823}}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.dfreshpair\endcsname{\ensuremath{+1.067}\,pp over the frozen 3-run pool and \ensuremath{+0.823}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.eligible\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.freshmean\endcsname{84.445}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.repstate\endcsname{survived}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.role\endcsname{control}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.s0\endcsname{86.014}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.s1\endcsname{85.112}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.s1reading\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.s1reading.class\endcsname{never-eligible}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.s1reading.excess\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.s1reading.phrase\endcsname{inside its registered band}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.s1reading.position\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.s1reading.registered\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.s1reading.state\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.s2\endcsname{83.777}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.sameseed\endcsname{\ensuremath{+1.51}}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.sameseed.s0\endcsname{\ensuremath{+1.74}}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.sameseed.s1\endcsname{\ensuremath{+2.00}}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.sameseed.s2\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.screen\endcsname{fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.sdfresh\endcsname{0.944}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.seedcorr\endcsname{0.920}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.sefresh\endcsname{0.667}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.shrink\endcsname{\ensuremath{-1.57}}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.shrink_3\endcsname{\ensuremath{-1.569}}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.shrinkz\endcsname{\ensuremath{-1.61}}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.v4reading\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.v4reading.phrase\endcsname{inside its registered band}
\expandafter\gdef\csname R@an.replication_all.kits.W1c.v4reading.state\endcsname{inside}
\expandafter\gdef\csname R@an.replication_all.kits.altref\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.replication_all.kits.altref.name\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.replication_all.kits.attr.list\endcsname{HyReX w/o GRN, HyReX-k3 and HyReX+pooled skip}
\expandafter\gdef\csname R@an.replication_all.kits.attr.n\endcsname{3}
\expandafter\gdef\csname R@an.replication_all.kits.confound\endcsname{no single family}
\expandafter\gdef\csname R@an.replication_all.kits.confound.phrase\endcsname{the never-eligible arms span more than one family}
\expandafter\gdef\csname R@an.replication_all.kits.ctlfire.list\endcsname{ResEnc-M, ResEnc-matched, branch control, fn.-identical control}
\expandafter\gdef\csname R@an.replication_all.kits.ctlfire.max\endcsname{\ensuremath{+2.64}}
\expandafter\gdef\csname R@an.replication_all.kits.ctlfire.maxname\endcsname{branch control}
\expandafter\gdef\csname R@an.replication_all.kits.ctlfire.n\endcsname{4}
\expandafter\gdef\csname R@an.replication_all.kits.cur.hi\endcsname{\ensuremath{-0.396}}
\expandafter\gdef\csname R@an.replication_all.kits.cur.label\endcsname{current model: the candidate designs with a finished seed-0 run now}
\expandafter\gdef\csname R@an.replication_all.kits.cur.lo\endcsname{\ensuremath{-7.287}}
\expandafter\gdef\csname R@an.replication_all.kits.cur.m\endcsname{22}
\expandafter\gdef\csname R@an.replication_all.kits.cur.m_plan\endcsname{9}
\expandafter\gdef\csname R@an.replication_all.kits.cur.never.hi\endcsname{\ensuremath{+2.834}}
\expandafter\gdef\csname R@an.replication_all.kits.cur.never.lo\endcsname{\ensuremath{-2.837}}
\expandafter\gdef\csname R@an.replication_all.kits.cur.plug\endcsname{\ensuremath{-1.518}}
\expandafter\gdef\csname R@an.replication_all.kits.cur.plug_plan\endcsname{\ensuremath{-1.178}}
\expandafter\gdef\csname R@an.replication_all.kits.cur.vs_reg\endcsname{The current model counts 22 candidate designs with a finished seed-0 run against the registered 6}
\expandafter\gdef\csname R@an.replication_all.kits.dfresh.L1minusL3\endcsname{\ensuremath{+1.38}}
\expandafter\gdef\csname R@an.replication_all.kits.dfresh.ahead\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@an.replication_all.kits.diff\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.replication_all.kits.diff.ratio\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.replication_all.kits.diff.se\endcsname{0.531}
\expandafter\gdef\csname R@an.replication_all.kits.diff.se.kind\endcsname{the no-selection model's standard error at the frozen KiTS23 pool seed SD, not an empirical standard error of these arms}
\expandafter\gdef\csname R@an.replication_all.kits.diff.se.pooled\endcsname{0.371}
\expandafter\gdef\csname R@an.replication_all.kits.diff.se.welch\endcsname{0.601}
\expandafter\gdef\csname R@an.replication_all.kits.diff.sentence\endcsname{the gap between the two groups is \ensuremath{-0.33}\,pp, with a standard error of 0.531\,pp -- the no-selection model's standard error at the frozen KiTS23 pool seed SD, not an empirical standard error of these arms (the empirical SE of these arms is 0.371\,pp pooled and 0.601\,pp unpooled)}
\expandafter\gdef\csname R@an.replication_all.kits.eb.C1.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.D1.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.D2.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.L1.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.L1b.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.L2.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.L3.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.L4.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.L6.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.P3c.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.S2.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.V5A5.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.V5B1.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.V5B2.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.V6A1r.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.V7A1.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.V7A2.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.V7B1.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.V7B2.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.V7C1.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.V8A1.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.V8A2.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.V8B1.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.V8B2.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.W1c.pred\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.factor\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.eb.meand0\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.eb.n\endcsname{25}
\expandafter\gdef\csname R@an.replication_all.kits.eb.tau2\endcsname{0.000}
\expandafter\gdef\csname R@an.replication_all.kits.eb.verdict\endcsname{does not exceed single-seed noise over the 25 arms}
\expandafter\gdef\csname R@an.replication_all.kits.elig.list\endcsname{ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context, HyReX, finer ConvNeXt, HyReX point-fuse, HyReX+dec. capacity, LeanDec, HyReX-LeanDec, LeanAdd, LeanAdd-NeXt, HyReX-k9, LeanDeepMid, LeanDeepMid+FD, LeanSep, LeanDil, LeanNeXt-s5, CoarseStack, StackDec, LeanTrunk and Stem1}
\expandafter\gdef\csname R@an.replication_all.kits.elig.n\endcsname{21}
\expandafter\gdef\csname R@an.replication_all.kits.elig.nlanded\endcsname{21}
\expandafter\gdef\csname R@an.replication_all.kits.emax\endcsname{1.910}
\expandafter\gdef\csname R@an.replication_all.kits.expshrink\endcsname{\ensuremath{-1.52}}
\expandafter\gdef\csname R@an.replication_all.kits.expshrink_hi\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.replication_all.kits.expshrink_lo\endcsname{\ensuremath{-7.29}}
\expandafter\gdef\csname R@an.replication_all.kits.expshrink_mc\endcsname{\ensuremath{-2.68}}
\expandafter\gdef\csname R@an.replication_all.kits.expshrink_nu\endcsname{2}
\expandafter\gdef\csname R@an.replication_all.kits.floor\endcsname{2}
\expandafter\gdef\csname R@an.replication_all.kits.hasscreen\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.lead\endcsname{HyReX + decoder capacity}
\expandafter\gdef\csname R@an.replication_all.kits.lead.d0\endcsname{\ensuremath{+3.507}}
\expandafter\gdef\csname R@an.replication_all.kits.lead.gap\endcsname{\ensuremath{+0.665}}
\expandafter\gdef\csname R@an.replication_all.kits.lead.nelig\endcsname{21}
\expandafter\gdef\csname R@an.replication_all.kits.lead.pair\endcsname{landed}
\expandafter\gdef\csname R@an.replication_all.kits.lead.same.sentence\endcsname{the eligible arm with the largest discovery delta is the registered lead}
\expandafter\gdef\csname R@an.replication_all.kits.lead.two\endcsname{the eligible arm with the largest discovery delta is HyReX + decoder capacity (\ensuremath{+3.507}\,pp over the frozen 3-run pool and \ensuremath{+3.264}\,pp over the 6-run reference); the registered lead, HyReX, has the fourth largest of the 21 eligible arms (\ensuremath{+2.842}\,pp over the frozen 3-run pool and \ensuremath{+2.598}\,pp over the 6-run reference)}
\expandafter\gdef\csname R@an.replication_all.kits.leadis\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.leadreg\endcsname{HyReX}
\expandafter\gdef\csname R@an.replication_all.kits.leadreg.d0\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.replication_all.kits.leadreg.rank\endcsname{4}
\expandafter\gdef\csname R@an.replication_all.kits.leadreg.rank.ord\endcsname{fourth largest}
\expandafter\gdef\csname R@an.replication_all.kits.leadreg.shrink\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.replication_all.kits.leadshrink\endcsname{\ensuremath{-1.11}}
\expandafter\gdef\csname R@an.replication_all.kits.m\endcsname{22}
\expandafter\gdef\csname R@an.replication_all.kits.m1.coverage\endcsname{all 25 measured shrinkages lie inside it}
\expandafter\gdef\csname R@an.replication_all.kits.never.list\endcsname{ResEnc-M, ResEnc-matched, branch control and fn.-identical control}
\expandafter\gdef\csname R@an.replication_all.kits.never.n\endcsname{4}
\expandafter\gdef\csname R@an.replication_all.kits.nreg\endcsname{25}
\expandafter\gdef\csname R@an.replication_all.kits.nrepl\endcsname{25}
\expandafter\gdef\csname R@an.replication_all.kits.nrepl.other\endcsname{0}
\expandafter\gdef\csname R@an.replication_all.kits.nrepl.other.line\endcsname{no random-search, scaled HyReX and single-prompt LLM design has a fresh KiTS23 pair yet; they are read in the random-search figures}
\expandafter\gdef\csname R@an.replication_all.kits.nrepl.other.list\endcsname{none}
\expandafter\gdef\csname R@an.replication_all.kits.nrepl.other.pops\endcsname{none}
\expandafter\gdef\csname R@an.replication_all.kits.nrepl.phrase\endcsname{25 agent-team arms with a fresh KiTS23 pair}
\expandafter\gdef\csname R@an.replication_all.kits.nrepl.set\endcsname{agent-team arms}
\expandafter\gdef\csname R@an.replication_all.kits.onlysurvivor.sentence\endcsname{HyReX is the only agent design that survived KiTS23 replication}
\expandafter\gdef\csname R@an.replication_all.kits.pattern.diffphrase\endcsname{the group difference (eligible minus never-eligible) is \ensuremath{-0.33}\,pp, which locates it at \ensuremath{-0.63} standard errors of the no-selection model}
\expandafter\gdef\csname R@an.replication_all.kits.pattern.direction\endcsname{no eligible arm moved up by more than 0.67\,pp, while the never-eligible arms moved in both directions}
\expandafter\gdef\csname R@an.replication_all.kits.pattern.notisolated\endcsname{The pattern is not uniformly in the direction selection predicts and does not isolate it, because the contrast is observational across designs, hosts and parameter counts; the never-eligible arms span more than one family}
\expandafter\gdef\csname R@an.replication_all.kits.pool\endcsname{83.378}
\expandafter\gdef\csname R@an.replication_all.kits.pooln\endcsname{3}
\expandafter\gdef\csname R@an.replication_all.kits.poolsd\endcsname{0.795}
\expandafter\gdef\csname R@an.replication_all.kits.reg.arms.eligible\endcsname{HyReX+dec. capacity}
\expandafter\gdef\csname R@an.replication_all.kits.reg.arms.known\endcsname{ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context, LeanDec, ResEnc-M and ResEnc-matched}
\expandafter\gdef\csname R@an.replication_all.kits.reg.arms.never\endcsname{branch control and fn.-identical control}
\expandafter\gdef\csname R@an.replication_all.kits.reg.hi\endcsname{\ensuremath{+0.267}}
\expandafter\gdef\csname R@an.replication_all.kits.reg.label\endcsname{Addendum V4}
\expandafter\gdef\csname R@an.replication_all.kits.reg.lo\endcsname{\ensuremath{-5.436}}
\expandafter\gdef\csname R@an.replication_all.kits.reg.m\endcsname{6}
\expandafter\gdef\csname R@an.replication_all.kits.reg.never.hi\endcsname{\ensuremath{+2.834}}
\expandafter\gdef\csname R@an.replication_all.kits.reg.never.lo\endcsname{\ensuremath{-2.837}}
\expandafter\gdef\csname R@an.replication_all.kits.reg.never.width\endcsname{5.671}
\expandafter\gdef\csname R@an.replication_all.kits.reg.nu\endcsname{2}
\expandafter\gdef\csname R@an.replication_all.kits.reg.plug\endcsname{\ensuremath{-1.006}}
\expandafter\gdef\csname R@an.replication_all.kits.reg.sentence\endcsname{Addendum V4, registered 2026-10-07 13:27:42 +08:00, fixed the movement of a selection-eligible arm at \ensuremath{-1.006}\,pp, with a 5--95\,\% range of \ensuremath{-5.436} to \ensuremath{+0.267}\,pp over 6 candidate designs, and the range of a never-eligible arm at \ensuremath{-2.837} to \ensuremath{+2.834}\,pp}
\expandafter\gdef\csname R@an.replication_all.kits.reg.sentence.short\endcsname{Addendum V4 fixed the movement of a selection-eligible arm at \ensuremath{-1.006}\,pp (5--95\,\% range \ensuremath{-5.436} to \ensuremath{+0.267}\,pp) and of a never-eligible arm at \ensuremath{-2.837} to \ensuremath{+2.834}\,pp}
\expandafter\gdef\csname R@an.replication_all.kits.reg.short\endcsname{V4}
\expandafter\gdef\csname R@an.replication_all.kits.reg.time\endcsname{2026-10-07 13:27:42 +08:00}
\expandafter\gdef\csname R@an.replication_all.kits.reg.width\endcsname{5.703}
\expandafter\gdef\csname R@an.replication_all.kits.s1.desc.list\endcsname{ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context, LeanDec, ResEnc-M and ResEnc-matched}
\expandafter\gdef\csname R@an.replication_all.kits.s1.desc.n\endcsname{7}
\expandafter\gdef\csname R@an.replication_all.kits.s1.desc.ninside\endcsname{7}
\expandafter\gdef\csname R@an.replication_all.kits.s1.inside.list\endcsname{HyReX+dec. capacity, branch control and fn.-identical control}
\expandafter\gdef\csname R@an.replication_all.kits.s1.ninside\endcsname{3}
\expandafter\gdef\csname R@an.replication_all.kits.s1.nlanded\endcsname{3}
\expandafter\gdef\csname R@an.replication_all.kits.s1.noutside\endcsname{0}
\expandafter\gdef\csname R@an.replication_all.kits.s1.npending\endcsname{0}
\expandafter\gdef\csname R@an.replication_all.kits.s1.nreg\endcsname{3}
\expandafter\gdef\csname R@an.replication_all.kits.s1.outside.list\endcsname{none}
\expandafter\gdef\csname R@an.replication_all.kits.s1.pending.list\endcsname{none}
\expandafter\gdef\csname R@an.replication_all.kits.s1.summary\endcsname{3 of the 3 registered readings that have landed are inside their band and 0 outside}
\expandafter\gdef\csname R@an.replication_all.kits.scatter.coverage\endcsname{the $\pm2$\,SD band covers every plotted arm}
\expandafter\gdef\csname R@an.replication_all.kits.scatter.fired\endcsname{every plotted arm fired the screen}
\expandafter\gdef\csname R@an.replication_all.kits.screenbar\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.replication_all.kits.sddelta\endcsname{0.918}
\expandafter\gdef\csname R@an.replication_all.kits.sdfreshdelta\endcsname{0.726}
\expandafter\gdef\csname R@an.replication_all.kits.sel.list\endcsname{HyReX, ConvNeXt-k3, ResEnc+context, HyReX+context, HyReX, finer ConvNeXt, HyReX point-fuse, HyReX+dec. capacity, LeanDec, LeanAdd, LeanAdd-NeXt, HyReX-LeanDec, LeanTrunk, Stem1, CoarseStack, StackDec, LeanDeepMid+FD, LeanSep, LeanDil, LeanDeepMid, LeanNeXt-s5, HyReX-k9}
\expandafter\gdef\csname R@an.replication_all.kits.sel.meanshrink\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.replication_all.kits.sel.n\endcsname{21}
\expandafter\gdef\csname R@an.replication_all.kits.sel.ndown\endcsname{13}
\expandafter\gdef\csname R@an.replication_all.kits.six.mean\endcsname{83.622}
\expandafter\gdef\csname R@an.replication_all.kits.six.n\endcsname{6}
\expandafter\gdef\csname R@an.replication_all.kits.six.shift\endcsname{\ensuremath{+0.244}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.kidney.d0\endcsname{\ensuremath{+1.22}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.kidney.d0_six\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.kidney.dfresh\endcsname{\ensuremath{+0.97}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.kidney.dfresh_six\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.masses.d0\endcsname{\ensuremath{+4.32}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.masses.d0_six\endcsname{\ensuremath{+3.99}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.masses.dfresh\endcsname{\ensuremath{+3.42}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.masses.dfresh_six\endcsname{\ensuremath{+3.10}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.rho\endcsname{0.371}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.slope\endcsname{0.491}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.top0\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.topd0\endcsname{\ensuremath{+6.22}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.topd0_six\endcsname{\ensuremath{+6.50}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.topd0pair\endcsname{\ensuremath{+6.22}\,pp over the frozen 3-run pool and \ensuremath{+6.50}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.topdfresh\endcsname{\ensuremath{+5.15}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.topdfresh_six\endcsname{\ensuremath{+5.44}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.topdfreshpair\endcsname{\ensuremath{+5.15}\,pp over the frozen 3-run pool and \ensuremath{+5.44}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.topfresh\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.topkeep\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.topnull\endcsname{3.00}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.topz\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.tumour.d0\endcsname{\ensuremath{+4.98}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.tumour.d0_six\endcsname{\ensuremath{+4.69}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.tumour.dfresh\endcsname{\ensuremath{+2.81}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.tumour.dfresh_six\endcsname{\ensuremath{+2.52}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.vol_large.d0\endcsname{\ensuremath{+3.09}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.vol_large.d0_six\endcsname{\ensuremath{+2.62}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.vol_large.dfresh\endcsname{\ensuremath{+2.37}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.vol_large.dfresh_six\endcsname{\ensuremath{+1.90}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.vol_mid.d0\endcsname{\ensuremath{+5.58}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.vol_mid.d0_six\endcsname{\ensuremath{+4.88}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.vol_mid.dfresh\endcsname{\ensuremath{+0.90}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.vol_mid.dfresh_six\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.vol_small.d0\endcsname{\ensuremath{+6.22}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.vol_small.d0_six\endcsname{\ensuremath{+6.50}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.vol_small.dfresh\endcsname{\ensuremath{+5.15}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.C1.vol_small.dfresh_six\endcsname{\ensuremath{+5.44}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.kidney.d0\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.kidney.d0_six\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.kidney.dfresh\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.kidney.dfresh_six\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.masses.d0\endcsname{\ensuremath{+2.92}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.masses.d0_six\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.masses.dfresh\endcsname{\ensuremath{+2.07}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.masses.dfresh_six\endcsname{\ensuremath{+1.75}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.rho\endcsname{0.429}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.slope\endcsname{0.233}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.top0\endcsname{masses}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.topd0\endcsname{\ensuremath{+2.92}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.topd0_six\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.topd0pair\endcsname{\ensuremath{+2.92}\,pp over the frozen 3-run pool and \ensuremath{+2.60}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.topdfresh\endcsname{\ensuremath{+2.07}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.topdfresh_six\endcsname{\ensuremath{+1.75}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.topdfreshpair\endcsname{\ensuremath{+2.07}\,pp over the frozen 3-run pool and \ensuremath{+1.75}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.topfresh\endcsname{large third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.topkeep\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.topnull\endcsname{1.32}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.topz\endcsname{\ensuremath{-0.64}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.tumour.d0\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.tumour.d0_six\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.tumour.dfresh\endcsname{\ensuremath{+1.58}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.tumour.dfresh_six\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.vol_large.d0\endcsname{\ensuremath{+1.93}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.vol_large.d0_six\endcsname{\ensuremath{+1.46}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.vol_large.dfresh\endcsname{\ensuremath{+2.59}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.vol_large.dfresh_six\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.vol_mid.d0\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.vol_mid.d0_six\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.vol_mid.dfresh\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.vol_mid.dfresh_six\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.vol_small.d0\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.vol_small.d0_six\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.vol_small.dfresh\endcsname{\ensuremath{+2.05}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D1.vol_small.dfresh_six\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.kidney.d0\endcsname{\ensuremath{+0.72}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.kidney.d0_six\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.kidney.dfresh\endcsname{\ensuremath{+0.84}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.kidney.dfresh_six\endcsname{\ensuremath{+0.72}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.masses.d0\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.masses.d0_six\endcsname{\ensuremath{+2.30}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.masses.dfresh\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.masses.dfresh_six\endcsname{\ensuremath{+1.99}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.rho\endcsname{1.000}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.slope\endcsname{0.755}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.top0\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.topd0\endcsname{\ensuremath{+4.99}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.topd0_six\endcsname{\ensuremath{+5.27}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.topd0pair\endcsname{\ensuremath{+4.99}\,pp over the frozen 3-run pool and \ensuremath{+5.27}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.topdfresh\endcsname{\ensuremath{+4.05}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.topdfresh_six\endcsname{\ensuremath{+4.34}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.topdfreshpair\endcsname{\ensuremath{+4.05}\,pp over the frozen 3-run pool and \ensuremath{+4.34}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.topfresh\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.topkeep\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.topnull\endcsname{3.00}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.topz\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.tumour.d0\endcsname{\ensuremath{+3.72}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.tumour.d0_six\endcsname{\ensuremath{+3.43}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.tumour.dfresh\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.tumour.dfresh_six\endcsname{\ensuremath{+2.24}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.vol_large.d0\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.vol_large.d0_six\endcsname{\ensuremath{+1.87}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.vol_large.dfresh\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.vol_large.dfresh_six\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.vol_mid.d0\endcsname{\ensuremath{+3.80}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.vol_mid.d0_six\endcsname{\ensuremath{+3.10}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.vol_mid.dfresh\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.vol_mid.dfresh_six\endcsname{\ensuremath{+1.94}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.vol_small.d0\endcsname{\ensuremath{+4.99}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.vol_small.d0_six\endcsname{\ensuremath{+5.27}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.vol_small.dfresh\endcsname{\ensuremath{+4.05}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.D2.vol_small.dfresh_six\endcsname{\ensuremath{+4.34}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.kidney.d0\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.kidney.d0_six\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.kidney.dfresh\endcsname{\ensuremath{+1.19}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.kidney.dfresh_six\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.masses.d0\endcsname{\ensuremath{+3.03}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.masses.d0_six\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.masses.dfresh\endcsname{\ensuremath{+4.15}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.masses.dfresh_six\endcsname{\ensuremath{+3.82}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.rho\endcsname{0.714}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.slope\endcsname{2.078}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.top0\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.topd0\endcsname{\ensuremath{+3.42}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.topd0_six\endcsname{\ensuremath{+2.72}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.topd0pair\endcsname{\ensuremath{+3.42}\,pp over the frozen 3-run pool and \ensuremath{+2.72}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.topdfresh\endcsname{\ensuremath{+4.83}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.topdfresh_six\endcsname{\ensuremath{+4.13}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.topdfreshpair\endcsname{\ensuremath{+4.83}\,pp over the frozen 3-run pool and \ensuremath{+4.13}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.topfresh\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.topkeep\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.topnull\endcsname{0.84}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.topz\endcsname{\ensuremath{+1.68}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.tumour.d0\endcsname{\ensuremath{+2.90}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.tumour.d0_six\endcsname{\ensuremath{+2.61}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.tumour.dfresh\endcsname{\ensuremath{+5.09}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.tumour.dfresh_six\endcsname{\ensuremath{+4.80}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.vol_large.d0\endcsname{\ensuremath{+2.16}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.vol_large.d0_six\endcsname{\ensuremath{+1.69}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.vol_large.dfresh\endcsname{\ensuremath{+2.67}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.vol_large.dfresh_six\endcsname{\ensuremath{+2.20}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.vol_mid.d0\endcsname{\ensuremath{+3.42}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.vol_mid.d0_six\endcsname{\ensuremath{+2.72}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.vol_mid.dfresh\endcsname{\ensuremath{+4.83}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.vol_mid.dfresh_six\endcsname{\ensuremath{+4.13}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.vol_small.d0\endcsname{\ensuremath{+3.10}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.vol_small.d0_six\endcsname{\ensuremath{+3.39}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.vol_small.dfresh\endcsname{\ensuremath{+7.71}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1.vol_small.dfresh_six\endcsname{\ensuremath{+8.00}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.kidney.d0\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.kidney.d0_six\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.kidney.dfresh\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.kidney.dfresh_six\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.masses.d0\endcsname{\ensuremath{+2.01}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.masses.d0_six\endcsname{\ensuremath{+1.69}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.masses.dfresh\endcsname{\ensuremath{+3.26}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.masses.dfresh_six\endcsname{\ensuremath{+2.93}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.rho\endcsname{0.543}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.slope\endcsname{0.302}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.top0\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.topd0\endcsname{\ensuremath{+5.42}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.topd0_six\endcsname{\ensuremath{+5.70}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.topd0pair\endcsname{\ensuremath{+5.42}\,pp over the frozen 3-run pool and \ensuremath{+5.70}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.topdfresh\endcsname{\ensuremath{+2.92}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.topdfresh_six\endcsname{\ensuremath{+3.20}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.topdfreshpair\endcsname{\ensuremath{+2.92}\,pp over the frozen 3-run pool and \ensuremath{+3.20}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.topfresh\endcsname{masses}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.topkeep\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.topnull\endcsname{3.00}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.topz\endcsname{\ensuremath{-0.83}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.tumour.d0\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.tumour.d0_six\endcsname{\ensuremath{+2.73}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.tumour.dfresh\endcsname{\ensuremath{+2.80}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.tumour.dfresh_six\endcsname{\ensuremath{+2.51}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.vol_large.d0\endcsname{\ensuremath{+1.99}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.vol_large.d0_six\endcsname{\ensuremath{+1.52}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.vol_large.dfresh\endcsname{\ensuremath{+3.20}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.vol_large.dfresh_six\endcsname{\ensuremath{+2.73}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.vol_mid.d0\endcsname{\ensuremath{+1.62}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.vol_mid.d0_six\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.vol_mid.dfresh\endcsname{\ensuremath{+2.30}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.vol_mid.dfresh_six\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.vol_small.d0\endcsname{\ensuremath{+5.42}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.vol_small.d0_six\endcsname{\ensuremath{+5.70}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.vol_small.dfresh\endcsname{\ensuremath{+2.92}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L1b.vol_small.dfresh_six\endcsname{\ensuremath{+3.20}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.kidney.d0\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.kidney.d0_six\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.kidney.dfresh\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.kidney.dfresh_six\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.masses.d0\endcsname{\ensuremath{+1.39}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.masses.d0_six\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.masses.dfresh\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.masses.dfresh_six\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.rho\endcsname{0.200}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.slope\endcsname{0.105}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.top0\endcsname{masses}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.topd0\endcsname{\ensuremath{+1.39}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.topd0_six\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.topd0pair\endcsname{\ensuremath{+1.39}\,pp over the frozen 3-run pool and \ensuremath{+1.07}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.topdfresh\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.topdfresh_six\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.topdfreshpair\endcsname{\ensuremath{+0.60}\,pp over the frozen 3-run pool and \ensuremath{+0.28}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.topfresh\endcsname{masses}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.topkeep\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.topnull\endcsname{1.32}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.topz\endcsname{\ensuremath{-0.60}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.tumour.d0\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.tumour.d0_six\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.tumour.dfresh\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.tumour.dfresh_six\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.vol_large.d0\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.vol_large.d0_six\endcsname{\ensuremath{-1.00}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.vol_large.dfresh\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.vol_large.dfresh_six\endcsname{\ensuremath{-0.15}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.vol_mid.d0\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.vol_mid.d0_six\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.vol_mid.dfresh\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.vol_mid.dfresh_six\endcsname{\ensuremath{-1.06}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.vol_small.d0\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.vol_small.d0_six\endcsname{\ensuremath{+0.95}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.vol_small.dfresh\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L2.vol_small.dfresh_six\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.kidney.d0\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.kidney.d0_six\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.kidney.dfresh\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.kidney.dfresh_six\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.large.d0\endcsname{\ensuremath{+1.92}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.large.dfresh\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.masses.d0\endcsname{\ensuremath{+3.49}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.masses.d0_six\endcsname{\ensuremath{+3.17}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.masses.dfresh\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.masses.dfresh_six\endcsname{\ensuremath{+2.70}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.mid.d0\endcsname{\ensuremath{+3.84}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.mid.dfresh\endcsname{\ensuremath{+3.12}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.rho\endcsname{0.086}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.slope\endcsname{0.018}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.small.d0\endcsname{\ensuremath{+6.49}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.small.dfresh\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.top0\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.topd0\endcsname{\ensuremath{+6.49}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.topd0_six\endcsname{\ensuremath{+6.78}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.topd0pair\endcsname{\ensuremath{+6.49}\,pp over the frozen 3-run pool and \ensuremath{+6.78}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.topdfresh\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.topdfresh_six\endcsname{\ensuremath{+1.58}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.topdfreshpair\endcsname{\ensuremath{+1.29}\,pp over the frozen 3-run pool and \ensuremath{+1.58}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.topfresh\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.topkeep\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.topnull\endcsname{3.00}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.topz\endcsname{\ensuremath{-1.73}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.tumour.d0\endcsname{\ensuremath{+4.11}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.tumour.d0_six\endcsname{\ensuremath{+3.82}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.tumour.dfresh\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.tumour.dfresh_six\endcsname{\ensuremath{+2.04}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.vol_large.d0\endcsname{\ensuremath{+1.92}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.vol_large.d0_six\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.vol_large.dfresh\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.vol_large.dfresh_six\endcsname{\ensuremath{+2.13}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.vol_mid.d0\endcsname{\ensuremath{+3.84}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.vol_mid.d0_six\endcsname{\ensuremath{+3.15}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.vol_mid.dfresh\endcsname{\ensuremath{+3.12}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.vol_mid.dfresh_six\endcsname{\ensuremath{+2.43}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.vol_small.d0\endcsname{\ensuremath{+6.49}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.vol_small.d0_six\endcsname{\ensuremath{+6.78}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.vol_small.dfresh\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L3.vol_small.dfresh_six\endcsname{\ensuremath{+1.58}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.kidney.d0\endcsname{\ensuremath{+0.67}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.kidney.d0_six\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.kidney.dfresh\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.kidney.dfresh_six\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.masses.d0\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.masses.d0_six\endcsname{\ensuremath{+2.10}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.masses.dfresh\endcsname{\ensuremath{+2.73}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.masses.dfresh_six\endcsname{\ensuremath{+2.41}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.rho\endcsname{0.486}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.slope\endcsname{0.536}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.top0\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.topd0\endcsname{\ensuremath{+4.70}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.topd0_six\endcsname{\ensuremath{+4.98}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.topd0pair\endcsname{\ensuremath{+4.70}\,pp over the frozen 3-run pool and \ensuremath{+4.98}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.topdfresh\endcsname{\ensuremath{+2.95}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.topdfresh_six\endcsname{\ensuremath{+3.23}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.topdfreshpair\endcsname{\ensuremath{+2.95}\,pp over the frozen 3-run pool and \ensuremath{+3.23}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.topfresh\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.topkeep\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.topnull\endcsname{3.00}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.topz\endcsname{\ensuremath{-0.58}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.tumour.d0\endcsname{\ensuremath{+3.50}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.tumour.d0_six\endcsname{\ensuremath{+3.21}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.tumour.dfresh\endcsname{\ensuremath{+3.14}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.tumour.dfresh_six\endcsname{\ensuremath{+2.85}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.vol_large.d0\endcsname{\ensuremath{+2.61}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.vol_large.d0_six\endcsname{\ensuremath{+2.14}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.vol_large.dfresh\endcsname{\ensuremath{+3.23}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.vol_large.dfresh_six\endcsname{\ensuremath{+2.76}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.vol_mid.d0\endcsname{\ensuremath{+3.16}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.vol_mid.d0_six\endcsname{\ensuremath{+2.47}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.vol_mid.dfresh\endcsname{\ensuremath{+3.25}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.vol_mid.dfresh_six\endcsname{\ensuremath{+2.56}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.vol_small.d0\endcsname{\ensuremath{+4.70}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.vol_small.d0_six\endcsname{\ensuremath{+4.98}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.vol_small.dfresh\endcsname{\ensuremath{+2.95}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L4.vol_small.dfresh_six\endcsname{\ensuremath{+3.23}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.kidney.d0\endcsname{\ensuremath{+0.95}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.kidney.d0_six\endcsname{\ensuremath{+0.84}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.kidney.dfresh\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.kidney.dfresh_six\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.masses.d0\endcsname{\ensuremath{+2.73}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.masses.d0_six\endcsname{\ensuremath{+2.41}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.masses.dfresh\endcsname{\ensuremath{+1.72}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.masses.dfresh_six\endcsname{\ensuremath{+1.40}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.rho\endcsname{0.829}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.slope\endcsname{0.288}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.top0\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.topd0\endcsname{\ensuremath{+7.08}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.topd0_six\endcsname{\ensuremath{+7.37}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.topd0pair\endcsname{\ensuremath{+7.08}\,pp over the frozen 3-run pool and \ensuremath{+7.37}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.topdfresh\endcsname{\ensuremath{+2.83}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.topdfresh_six\endcsname{\ensuremath{+3.12}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.topdfreshpair\endcsname{\ensuremath{+2.83}\,pp over the frozen 3-run pool and \ensuremath{+3.12}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.topfresh\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.topkeep\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.topnull\endcsname{3.00}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.topz\endcsname{\ensuremath{-1.42}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.tumour.d0\endcsname{\ensuremath{+3.90}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.tumour.d0_six\endcsname{\ensuremath{+3.61}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.tumour.dfresh\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.tumour.dfresh_six\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.vol_large.d0\endcsname{\ensuremath{+2.13}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.vol_large.d0_six\endcsname{\ensuremath{+1.66}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.vol_large.dfresh\endcsname{\ensuremath{+1.71}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.vol_large.dfresh_six\endcsname{\ensuremath{+1.24}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.vol_mid.d0\endcsname{\ensuremath{+2.43}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.vol_mid.d0_six\endcsname{\ensuremath{+1.73}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.vol_mid.dfresh\endcsname{\ensuremath{+2.68}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.vol_mid.dfresh_six\endcsname{\ensuremath{+1.99}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.vol_small.d0\endcsname{\ensuremath{+7.08}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.vol_small.d0_six\endcsname{\ensuremath{+7.37}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.vol_small.dfresh\endcsname{\ensuremath{+2.83}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.L6.vol_small.dfresh_six\endcsname{\ensuremath{+3.12}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.kidney.d0\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.kidney.d0_six\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.kidney.dfresh\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.kidney.dfresh_six\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.masses.d0\endcsname{\ensuremath{+1.75}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.masses.d0_six\endcsname{\ensuremath{+1.43}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.masses.dfresh\endcsname{\ensuremath{+1.54}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.masses.dfresh_six\endcsname{\ensuremath{+1.22}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.rho\endcsname{0.086}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.slope\endcsname{0.162}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.top0\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.topd0\endcsname{\ensuremath{+3.19}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.topd0_six\endcsname{\ensuremath{+2.50}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.topd0pair\endcsname{\ensuremath{+3.19}\,pp over the frozen 3-run pool and \ensuremath{+2.50}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.topdfresh\endcsname{\ensuremath{+1.72}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.topdfresh_six\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.topdfreshpair\endcsname{\ensuremath{+1.72}\,pp over the frozen 3-run pool and \ensuremath{+1.03}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.topfresh\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.topkeep\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.topnull\endcsname{0.84}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.topz\endcsname{\ensuremath{-1.75}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.tumour.d0\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.tumour.d0_six\endcsname{\ensuremath{+1.47}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.tumour.dfresh\endcsname{\ensuremath{+1.44}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.tumour.dfresh_six\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.vol_large.d0\endcsname{\ensuremath{+1.60}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.vol_large.d0_six\endcsname{\ensuremath{+1.13}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.vol_large.dfresh\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.vol_large.dfresh_six\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.vol_mid.d0\endcsname{\ensuremath{+3.19}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.vol_mid.d0_six\endcsname{\ensuremath{+2.50}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.vol_mid.dfresh\endcsname{\ensuremath{+1.72}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.vol_mid.dfresh_six\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.vol_small.d0\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.vol_small.d0_six\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.vol_small.dfresh\endcsname{\ensuremath{+1.94}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.P3c.vol_small.dfresh_six\endcsname{\ensuremath{+2.23}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.kidney.d0\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.kidney.d0_six\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.kidney.dfresh\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.kidney.dfresh_six\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.masses.d0\endcsname{\ensuremath{+1.93}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.masses.d0_six\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.masses.dfresh\endcsname{\ensuremath{+1.13}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.masses.dfresh_six\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.rho\endcsname{\ensuremath{-0.657}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.slope\endcsname{\ensuremath{-0.608}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.top0\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.topd0\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.topd0_six\endcsname{\ensuremath{+1.46}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.topd0pair\endcsname{\ensuremath{+2.15}\,pp over the frozen 3-run pool and \ensuremath{+1.46}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.topdfresh\endcsname{\ensuremath{-0.70}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.topdfresh_six\endcsname{\ensuremath{-1.39}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.topdfreshpair\endcsname{\ensuremath{-0.70}\,pp over the frozen 3-run pool and \ensuremath{-1.39}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.topfresh\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.topkeep\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.topnull\endcsname{0.84}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.topz\endcsname{\ensuremath{-3.39}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.tumour.d0\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.tumour.d0_six\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.tumour.dfresh\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.tumour.dfresh_six\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.vol_large.d0\endcsname{\ensuremath{+1.70}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.vol_large.d0_six\endcsname{\ensuremath{+1.23}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.vol_large.dfresh\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.vol_large.dfresh_six\endcsname{\ensuremath{-0.76}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.vol_mid.d0\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.vol_mid.d0_six\endcsname{\ensuremath{+1.46}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.vol_mid.dfresh\endcsname{\ensuremath{-0.70}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.vol_mid.dfresh_six\endcsname{\ensuremath{-1.39}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.vol_small.d0\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.vol_small.d0_six\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.vol_small.dfresh\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.S2.vol_small.dfresh_six\endcsname{\ensuremath{+1.58}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.kidney.d0\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.kidney.d0_six\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.kidney.dfresh\endcsname{\ensuremath{+0.72}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.kidney.dfresh_six\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.masses.d0\endcsname{\ensuremath{+2.57}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.masses.d0_six\endcsname{\ensuremath{+2.24}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.masses.dfresh\endcsname{\ensuremath{+2.59}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.masses.dfresh_six\endcsname{\ensuremath{+2.27}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.rho\endcsname{0.829}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.slope\endcsname{1.198}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.top0\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.topd0\endcsname{\ensuremath{+2.88}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.topd0_six\endcsname{\ensuremath{+3.17}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.topd0pair\endcsname{\ensuremath{+2.88}\,pp over the frozen 3-run pool and \ensuremath{+3.17}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.topdfresh\endcsname{\ensuremath{+3.89}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.topdfresh_six\endcsname{\ensuremath{+4.17}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.topdfreshpair\endcsname{\ensuremath{+3.89}\,pp over the frozen 3-run pool and \ensuremath{+4.17}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.topfresh\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.topkeep\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.topnull\endcsname{3.00}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.topz\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.tumour.d0\endcsname{\ensuremath{+2.47}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.tumour.d0_six\endcsname{\ensuremath{+2.18}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.tumour.dfresh\endcsname{\ensuremath{+3.19}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.tumour.dfresh_six\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.vol_large.d0\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.vol_large.d0_six\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.vol_large.dfresh\endcsname{\ensuremath{+2.56}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.vol_large.dfresh_six\endcsname{\ensuremath{+2.09}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.vol_mid.d0\endcsname{\ensuremath{+2.86}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.vol_mid.d0_six\endcsname{\ensuremath{+2.16}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.vol_mid.dfresh\endcsname{\ensuremath{+3.09}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.vol_mid.dfresh_six\endcsname{\ensuremath{+2.40}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.vol_small.d0\endcsname{\ensuremath{+2.88}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.vol_small.d0_six\endcsname{\ensuremath{+3.17}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.vol_small.dfresh\endcsname{\ensuremath{+3.89}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5A5.vol_small.dfresh_six\endcsname{\ensuremath{+4.17}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.kidney.d0\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.kidney.d0_six\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.kidney.dfresh\endcsname{\ensuremath{+0.94}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.kidney.dfresh_six\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.masses.d0\endcsname{\ensuremath{+2.49}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.masses.d0_six\endcsname{\ensuremath{+2.17}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.masses.dfresh\endcsname{\ensuremath{+3.21}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.masses.dfresh_six\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.rho\endcsname{0.829}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.slope\endcsname{0.658}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.top0\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.topd0\endcsname{\ensuremath{+5.50}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.topd0_six\endcsname{\ensuremath{+5.79}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.topd0pair\endcsname{\ensuremath{+5.50}\,pp over the frozen 3-run pool and \ensuremath{+5.79}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.topdfresh\endcsname{\ensuremath{+4.18}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.topdfresh_six\endcsname{\ensuremath{+4.47}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.topdfreshpair\endcsname{\ensuremath{+4.18}\,pp over the frozen 3-run pool and \ensuremath{+4.47}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.topfresh\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.topkeep\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.topnull\endcsname{3.00}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.topz\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.tumour.d0\endcsname{\ensuremath{+3.29}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.tumour.d0_six\endcsname{\ensuremath{+3.00}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.tumour.dfresh\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.tumour.dfresh_six\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.vol_large.d0\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.vol_large.d0_six\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.vol_large.dfresh\endcsname{\ensuremath{+2.28}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.vol_large.dfresh_six\endcsname{\ensuremath{+1.81}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.vol_mid.d0\endcsname{\ensuremath{+1.75}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.vol_mid.d0_six\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.vol_mid.dfresh\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.vol_mid.dfresh_six\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.vol_small.d0\endcsname{\ensuremath{+5.50}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.vol_small.d0_six\endcsname{\ensuremath{+5.79}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.vol_small.dfresh\endcsname{\ensuremath{+4.18}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B1.vol_small.dfresh_six\endcsname{\ensuremath{+4.47}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.kidney.d0\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.kidney.d0_six\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.kidney.dfresh\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.kidney.dfresh_six\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.masses.d0\endcsname{\ensuremath{+1.77}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.masses.d0_six\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.masses.dfresh\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.masses.dfresh_six\endcsname{\ensuremath{+1.51}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.rho\endcsname{0.943}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.slope\endcsname{0.413}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.top0\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.topd0\endcsname{\ensuremath{+5.49}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.topd0_six\endcsname{\ensuremath{+4.80}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.topd0pair\endcsname{\ensuremath{+5.49}\,pp over the frozen 3-run pool and \ensuremath{+4.80}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.topdfresh\endcsname{\ensuremath{+3.31}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.topdfresh_six\endcsname{\ensuremath{+2.62}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.topdfreshpair\endcsname{\ensuremath{+3.31}\,pp over the frozen 3-run pool and \ensuremath{+2.62}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.topfresh\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.topkeep\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.topnull\endcsname{0.84}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.topz\endcsname{\ensuremath{-2.60}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.tumour.d0\endcsname{\ensuremath{+1.32}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.tumour.d0_six\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.tumour.dfresh\endcsname{\ensuremath{+1.60}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.tumour.dfresh_six\endcsname{\ensuremath{+1.31}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.vol_large.d0\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.vol_large.d0_six\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.vol_large.dfresh\endcsname{\ensuremath{+0.97}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.vol_large.dfresh_six\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.vol_mid.d0\endcsname{\ensuremath{+5.49}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.vol_mid.d0_six\endcsname{\ensuremath{+4.80}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.vol_mid.dfresh\endcsname{\ensuremath{+3.31}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.vol_mid.dfresh_six\endcsname{\ensuremath{+2.62}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.vol_small.d0\endcsname{\ensuremath{-1.68}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.vol_small.d0_six\endcsname{\ensuremath{-1.40}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.vol_small.dfresh\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V5B2.vol_small.dfresh_six\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.kidney.d0\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.kidney.d0_six\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.kidney.dfresh\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.kidney.dfresh_six\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.masses.d0\endcsname{\ensuremath{+3.49}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.masses.d0_six\endcsname{\ensuremath{+3.17}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.masses.dfresh\endcsname{\ensuremath{+2.32}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.masses.dfresh_six\endcsname{\ensuremath{+2.00}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.rho\endcsname{0.371}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.slope\endcsname{0.394}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.top0\endcsname{masses}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.topd0\endcsname{\ensuremath{+3.49}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.topd0_six\endcsname{\ensuremath{+3.17}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.topd0pair\endcsname{\ensuremath{+3.49}\,pp over the frozen 3-run pool and \ensuremath{+3.17}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.topdfresh\endcsname{\ensuremath{+2.32}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.topdfresh_six\endcsname{\ensuremath{+2.00}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.topdfreshpair\endcsname{\ensuremath{+2.32}\,pp over the frozen 3-run pool and \ensuremath{+2.00}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.topfresh\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.topkeep\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.topnull\endcsname{1.32}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.topz\endcsname{\ensuremath{-0.89}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.tumour.d0\endcsname{\ensuremath{+2.30}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.tumour.d0_six\endcsname{\ensuremath{+2.01}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.tumour.dfresh\endcsname{\ensuremath{+1.98}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.tumour.dfresh_six\endcsname{\ensuremath{+1.69}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.vol_large.d0\endcsname{\ensuremath{+2.24}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.vol_large.d0_six\endcsname{\ensuremath{+1.77}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.vol_large.dfresh\endcsname{\ensuremath{+1.31}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.vol_large.dfresh_six\endcsname{\ensuremath{+0.84}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.vol_mid.d0\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.vol_mid.d0_six\endcsname{\ensuremath{+1.20}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.vol_mid.dfresh\endcsname{\ensuremath{+2.98}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.vol_mid.dfresh_six\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.vol_small.d0\endcsname{\ensuremath{+2.77}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.vol_small.d0_six\endcsname{\ensuremath{+3.06}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.vol_small.dfresh\endcsname{\ensuremath{+1.63}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V6A1r.vol_small.dfresh_six\endcsname{\ensuremath{+1.92}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.kidney.d0\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.kidney.d0_six\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.kidney.dfresh\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.kidney.dfresh_six\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.masses.d0\endcsname{\ensuremath{+3.32}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.masses.d0_six\endcsname{\ensuremath{+2.99}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.masses.dfresh\endcsname{\ensuremath{+3.44}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.masses.dfresh_six\endcsname{\ensuremath{+3.12}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.rho\endcsname{0.943}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.slope\endcsname{0.875}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.top0\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.topd0\endcsname{\ensuremath{+3.98}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.topd0_six\endcsname{\ensuremath{+3.28}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.topd0pair\endcsname{\ensuremath{+3.98}\,pp over the frozen 3-run pool and \ensuremath{+3.28}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.topdfresh\endcsname{\ensuremath{+3.77}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.topdfresh_six\endcsname{\ensuremath{+3.08}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.topdfreshpair\endcsname{\ensuremath{+3.77}\,pp over the frozen 3-run pool and \ensuremath{+3.08}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.topfresh\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.topkeep\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.topnull\endcsname{0.84}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.topz\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.tumour.d0\endcsname{\ensuremath{+3.28}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.tumour.d0_six\endcsname{\ensuremath{+2.99}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.tumour.dfresh\endcsname{\ensuremath{+3.40}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.tumour.dfresh_six\endcsname{\ensuremath{+3.10}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.vol_large.d0\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.vol_large.d0_six\endcsname{\ensuremath{+1.41}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.vol_large.dfresh\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.vol_large.dfresh_six\endcsname{\ensuremath{+1.97}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.vol_mid.d0\endcsname{\ensuremath{+3.98}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.vol_mid.d0_six\endcsname{\ensuremath{+3.28}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.vol_mid.dfresh\endcsname{\ensuremath{+3.77}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.vol_mid.dfresh_six\endcsname{\ensuremath{+3.08}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.vol_small.d0\endcsname{\ensuremath{+3.94}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.vol_small.d0_six\endcsname{\ensuremath{+4.22}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.vol_small.dfresh\endcsname{\ensuremath{+3.94}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A1.vol_small.dfresh_six\endcsname{\ensuremath{+4.23}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.kidney.d0\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.kidney.d0_six\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.kidney.dfresh\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.kidney.dfresh_six\endcsname{\ensuremath{+0.94}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.masses.d0\endcsname{\ensuremath{+3.95}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.masses.d0_six\endcsname{\ensuremath{+3.63}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.masses.dfresh\endcsname{\ensuremath{+2.64}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.masses.dfresh_six\endcsname{\ensuremath{+2.32}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.rho\endcsname{0.771}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.slope\endcsname{0.768}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.top0\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.topd0\endcsname{\ensuremath{+4.52}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.topd0_six\endcsname{\ensuremath{+4.80}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.topd0pair\endcsname{\ensuremath{+4.52}\,pp over the frozen 3-run pool and \ensuremath{+4.80}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.topdfresh\endcsname{\ensuremath{+3.77}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.topdfresh_six\endcsname{\ensuremath{+4.05}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.topdfreshpair\endcsname{\ensuremath{+3.77}\,pp over the frozen 3-run pool and \ensuremath{+4.05}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.topfresh\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.topkeep\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.topnull\endcsname{3.00}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.topz\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.tumour.d0\endcsname{\ensuremath{+3.59}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.tumour.d0_six\endcsname{\ensuremath{+3.30}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.tumour.dfresh\endcsname{\ensuremath{+3.17}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.tumour.dfresh_six\endcsname{\ensuremath{+2.88}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.vol_large.d0\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.vol_large.d0_six\endcsname{\ensuremath{+2.41}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.vol_large.dfresh\endcsname{\ensuremath{+2.07}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.vol_large.dfresh_six\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.vol_mid.d0\endcsname{\ensuremath{+3.35}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.vol_mid.d0_six\endcsname{\ensuremath{+2.66}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.vol_mid.dfresh\endcsname{\ensuremath{+3.66}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.vol_mid.dfresh_six\endcsname{\ensuremath{+2.96}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.vol_small.d0\endcsname{\ensuremath{+4.52}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.vol_small.d0_six\endcsname{\ensuremath{+4.80}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.vol_small.dfresh\endcsname{\ensuremath{+3.77}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7A2.vol_small.dfresh_six\endcsname{\ensuremath{+4.05}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.kidney.d0\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.kidney.d0_six\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.kidney.dfresh\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.kidney.dfresh_six\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.masses.d0\endcsname{\ensuremath{+2.10}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.masses.d0_six\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.masses.dfresh\endcsname{\ensuremath{+3.22}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.masses.dfresh_six\endcsname{\ensuremath{+2.90}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.rho\endcsname{0.886}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.slope\endcsname{0.955}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.top0\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.topd0\endcsname{\ensuremath{+3.71}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.topd0_six\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.topd0pair\endcsname{\ensuremath{+3.71}\,pp over the frozen 3-run pool and \ensuremath{+3.02}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.topdfresh\endcsname{\ensuremath{+4.09}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.topdfresh_six\endcsname{\ensuremath{+3.39}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.topdfreshpair\endcsname{\ensuremath{+4.09}\,pp over the frozen 3-run pool and \ensuremath{+3.39}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.topfresh\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.topkeep\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.topnull\endcsname{0.84}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.topz\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.tumour.d0\endcsname{\ensuremath{+2.21}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.tumour.d0_six\endcsname{\ensuremath{+1.92}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.tumour.dfresh\endcsname{\ensuremath{+2.93}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.tumour.dfresh_six\endcsname{\ensuremath{+2.64}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.vol_large.d0\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.vol_large.d0_six\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.vol_large.dfresh\endcsname{\ensuremath{+2.14}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.vol_large.dfresh_six\endcsname{\ensuremath{+1.67}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.vol_mid.d0\endcsname{\ensuremath{+3.71}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.vol_mid.d0_six\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.vol_mid.dfresh\endcsname{\ensuremath{+4.09}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.vol_mid.dfresh_six\endcsname{\ensuremath{+3.39}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.vol_small.d0\endcsname{\ensuremath{+1.26}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.vol_small.d0_six\endcsname{\ensuremath{+1.55}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.vol_small.dfresh\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B1.vol_small.dfresh_six\endcsname{\ensuremath{+2.82}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.kidney.d0\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.kidney.d0_six\endcsname{\ensuremath{+0.91}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.kidney.dfresh\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.kidney.dfresh_six\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.masses.d0\endcsname{\ensuremath{+3.59}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.masses.d0_six\endcsname{\ensuremath{+3.27}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.masses.dfresh\endcsname{\ensuremath{+2.11}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.masses.dfresh_six\endcsname{\ensuremath{+1.79}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.rho\endcsname{0.657}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.slope\endcsname{0.701}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.top0\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.topd0\endcsname{\ensuremath{+5.02}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.topd0_six\endcsname{\ensuremath{+4.33}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.topd0pair\endcsname{\ensuremath{+5.02}\,pp over the frozen 3-run pool and \ensuremath{+4.33}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.topdfresh\endcsname{\ensuremath{+4.31}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.topdfresh_six\endcsname{\ensuremath{+3.62}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.topdfreshpair\endcsname{\ensuremath{+4.31}\,pp over the frozen 3-run pool and \ensuremath{+3.62}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.topfresh\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.topkeep\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.topnull\endcsname{0.84}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.topz\endcsname{\ensuremath{-0.85}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.tumour.d0\endcsname{\ensuremath{+3.85}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.tumour.d0_six\endcsname{\ensuremath{+3.56}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.tumour.dfresh\endcsname{\ensuremath{+2.59}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.tumour.dfresh_six\endcsname{\ensuremath{+2.30}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.vol_large.d0\endcsname{\ensuremath{+2.51}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.vol_large.d0_six\endcsname{\ensuremath{+2.03}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.vol_large.dfresh\endcsname{\ensuremath{+1.93}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.vol_large.dfresh_six\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.vol_mid.d0\endcsname{\ensuremath{+5.02}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.vol_mid.d0_six\endcsname{\ensuremath{+4.33}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.vol_mid.dfresh\endcsname{\ensuremath{+4.31}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.vol_mid.dfresh_six\endcsname{\ensuremath{+3.62}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.vol_small.d0\endcsname{\ensuremath{+3.98}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.vol_small.d0_six\endcsname{\ensuremath{+4.27}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.vol_small.dfresh\endcsname{\ensuremath{+1.52}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7B2.vol_small.dfresh_six\endcsname{\ensuremath{+1.81}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.kidney.d0\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.kidney.d0_six\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.kidney.dfresh\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.kidney.dfresh_six\endcsname{\ensuremath{+1.13}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.masses.d0\endcsname{\ensuremath{+3.64}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.masses.d0_six\endcsname{\ensuremath{+3.32}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.masses.dfresh\endcsname{\ensuremath{+3.01}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.masses.dfresh_six\endcsname{\ensuremath{+2.69}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.rho\endcsname{0.714}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.slope\endcsname{0.616}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.top0\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.topd0\endcsname{\ensuremath{+4.07}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.topd0_six\endcsname{\ensuremath{+3.38}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.topd0pair\endcsname{\ensuremath{+4.07}\,pp over the frozen 3-run pool and \ensuremath{+3.38}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.topdfresh\endcsname{\ensuremath{+3.33}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.topdfresh_six\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.topdfreshpair\endcsname{\ensuremath{+3.33}\,pp over the frozen 3-run pool and \ensuremath{+2.63}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.topfresh\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.topkeep\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.topnull\endcsname{0.84}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.topz\endcsname{\ensuremath{-0.89}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.tumour.d0\endcsname{\ensuremath{+3.39}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.tumour.d0_six\endcsname{\ensuremath{+3.09}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.tumour.dfresh\endcsname{\ensuremath{+3.06}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.tumour.dfresh_six\endcsname{\ensuremath{+2.77}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.vol_large.d0\endcsname{\ensuremath{+2.43}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.vol_large.d0_six\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.vol_large.dfresh\endcsname{\ensuremath{+2.97}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.vol_large.dfresh_six\endcsname{\ensuremath{+2.49}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.vol_mid.d0\endcsname{\ensuremath{+4.07}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.vol_mid.d0_six\endcsname{\ensuremath{+3.38}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.vol_mid.dfresh\endcsname{\ensuremath{+3.33}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.vol_mid.dfresh_six\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.vol_small.d0\endcsname{\ensuremath{+3.63}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.vol_small.d0_six\endcsname{\ensuremath{+3.91}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.vol_small.dfresh\endcsname{\ensuremath{+2.88}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V7C1.vol_small.dfresh_six\endcsname{\ensuremath{+3.16}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.kidney.d0\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.kidney.d0_six\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.kidney.dfresh\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.kidney.dfresh_six\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.masses.d0\endcsname{\ensuremath{+2.59}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.masses.d0_six\endcsname{\ensuremath{+2.27}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.masses.dfresh\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.masses.dfresh_six\endcsname{\ensuremath{+1.56}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.rho\endcsname{0.657}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.slope\endcsname{0.452}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.top0\endcsname{masses}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.topd0\endcsname{\ensuremath{+2.59}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.topd0_six\endcsname{\ensuremath{+2.27}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.topd0pair\endcsname{\ensuremath{+2.59}\,pp over the frozen 3-run pool and \ensuremath{+2.27}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.topdfresh\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.topdfresh_six\endcsname{\ensuremath{+1.56}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.topdfreshpair\endcsname{\ensuremath{+1.88}\,pp over the frozen 3-run pool and \ensuremath{+1.56}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.topfresh\endcsname{masses}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.topkeep\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.topnull\endcsname{1.32}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.topz\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.tumour.d0\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.tumour.d0_six\endcsname{\ensuremath{+1.66}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.tumour.dfresh\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.tumour.dfresh_six\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.vol_large.d0\endcsname{\ensuremath{+1.41}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.vol_large.d0_six\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.vol_large.dfresh\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.vol_large.dfresh_six\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.vol_mid.d0\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.vol_mid.d0_six\endcsname{\ensuremath{+1.67}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.vol_mid.dfresh\endcsname{\ensuremath{+0.79}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.vol_mid.dfresh_six\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.vol_small.d0\endcsname{\ensuremath{+2.09}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.vol_small.d0_six\endcsname{\ensuremath{+2.37}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.vol_small.dfresh\endcsname{\ensuremath{+1.67}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A1.vol_small.dfresh_six\endcsname{\ensuremath{+1.95}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.kidney.d0\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.kidney.d0_six\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.kidney.dfresh\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.kidney.dfresh_six\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.masses.d0\endcsname{\ensuremath{+1.69}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.masses.d0_six\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.masses.dfresh\endcsname{\ensuremath{+2.68}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.masses.dfresh_six\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.rho\endcsname{0.829}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.slope\endcsname{2.391}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.top0\endcsname{masses}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.topd0\endcsname{\ensuremath{+1.69}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.topd0_six\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.topd0pair\endcsname{\ensuremath{+1.69}\,pp over the frozen 3-run pool and \ensuremath{+1.37}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.topdfresh\endcsname{\ensuremath{+2.68}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.topdfresh_six\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.topdfreshpair\endcsname{\ensuremath{+2.68}\,pp over the frozen 3-run pool and \ensuremath{+2.36}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.topfresh\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.topkeep\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.topnull\endcsname{1.32}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.topz\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.tumour.d0\endcsname{\ensuremath{+1.57}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.tumour.d0_six\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.tumour.dfresh\endcsname{\ensuremath{+2.09}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.tumour.dfresh_six\endcsname{\ensuremath{+1.80}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.vol_large.d0\endcsname{\ensuremath{+1.58}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.vol_large.d0_six\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.vol_large.dfresh\endcsname{\ensuremath{+1.53}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.vol_large.dfresh_six\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.vol_mid.d0\endcsname{\ensuremath{+1.66}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.vol_mid.d0_six\endcsname{\ensuremath{+0.97}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.vol_mid.dfresh\endcsname{\ensuremath{+4.43}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.vol_mid.dfresh_six\endcsname{\ensuremath{+3.74}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.vol_small.d0\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.vol_small.d0_six\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.vol_small.dfresh\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8A2.vol_small.dfresh_six\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.kidney.d0\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.kidney.d0_six\endcsname{\ensuremath{+1.06}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.kidney.dfresh\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.kidney.dfresh_six\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.masses.d0\endcsname{\ensuremath{+3.55}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.masses.d0_six\endcsname{\ensuremath{+3.22}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.masses.dfresh\endcsname{\ensuremath{+1.84}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.masses.dfresh_six\endcsname{\ensuremath{+1.52}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.rho\endcsname{0.257}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.slope\endcsname{0.045}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.top0\endcsname{small third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.topd0\endcsname{\ensuremath{+5.27}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.topd0_six\endcsname{\ensuremath{+5.56}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.topd0pair\endcsname{\ensuremath{+5.27}\,pp over the frozen 3-run pool and \ensuremath{+5.56}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.topdfresh\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.topdfresh_six\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.topdfreshpair\endcsname{\ensuremath{+0.83}\,pp over the frozen 3-run pool and \ensuremath{+1.11}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.topfresh\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.topkeep\endcsname{no}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.topnull\endcsname{3.00}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.topz\endcsname{\ensuremath{-1.48}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.tumour.d0\endcsname{\ensuremath{+4.01}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.tumour.d0_six\endcsname{\ensuremath{+3.72}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.tumour.dfresh\endcsname{\ensuremath{+1.51}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.tumour.dfresh_six\endcsname{\ensuremath{+1.22}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.vol_large.d0\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.vol_large.d0_six\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.vol_large.dfresh\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.vol_large.dfresh_six\endcsname{\ensuremath{+1.30}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.vol_mid.d0\endcsname{\ensuremath{+5.09}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.vol_mid.d0_six\endcsname{\ensuremath{+4.40}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.vol_mid.dfresh\endcsname{\ensuremath{+1.93}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.vol_mid.dfresh_six\endcsname{\ensuremath{+1.24}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.vol_small.d0\endcsname{\ensuremath{+5.27}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.vol_small.d0_six\endcsname{\ensuremath{+5.56}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.vol_small.dfresh\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B1.vol_small.dfresh_six\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.kidney.d0\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.kidney.d0_six\endcsname{\ensuremath{+0.91}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.kidney.dfresh\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.kidney.dfresh_six\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.masses.d0\endcsname{\ensuremath{+1.98}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.masses.d0_six\endcsname{\ensuremath{+1.66}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.masses.dfresh\endcsname{\ensuremath{+2.07}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.masses.dfresh_six\endcsname{\ensuremath{+1.75}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.rho\endcsname{0.600}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.slope\endcsname{0.565}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.top0\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.topd0\endcsname{\ensuremath{+3.40}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.topd0_six\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.topd0pair\endcsname{\ensuremath{+3.40}\,pp over the frozen 3-run pool and \ensuremath{+2.71}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.topdfresh\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.topdfresh_six\endcsname{\ensuremath{+2.19}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.topdfreshpair\endcsname{\ensuremath{+2.89}\,pp over the frozen 3-run pool and \ensuremath{+2.19}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.topfresh\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.topkeep\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.topnull\endcsname{0.84}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.topz\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.tumour.d0\endcsname{\ensuremath{+1.93}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.tumour.d0_six\endcsname{\ensuremath{+1.64}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.tumour.dfresh\endcsname{\ensuremath{+2.37}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.tumour.dfresh_six\endcsname{\ensuremath{+2.08}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.vol_large.d0\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.vol_large.d0_six\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.vol_large.dfresh\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.vol_large.dfresh_six\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.vol_mid.d0\endcsname{\ensuremath{+3.40}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.vol_mid.d0_six\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.vol_mid.dfresh\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.vol_mid.dfresh_six\endcsname{\ensuremath{+2.19}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.vol_small.d0\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.vol_small.d0_six\endcsname{\ensuremath{+1.40}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.vol_small.dfresh\endcsname{\ensuremath{+2.62}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.V8B2.vol_small.dfresh_six\endcsname{\ensuremath{+2.90}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.kidney.d0\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.kidney.d0_six\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.kidney.dfresh\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.kidney.dfresh_six\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.masses.d0\endcsname{\ensuremath{+3.30}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.masses.d0_six\endcsname{\ensuremath{+2.98}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.masses.dfresh\endcsname{\ensuremath{+1.54}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.masses.dfresh_six\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.rho\endcsname{0.829}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.slope\endcsname{0.549}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.top0\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.topd0\endcsname{\ensuremath{+4.05}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.topd0_six\endcsname{\ensuremath{+3.35}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.topd0pair\endcsname{\ensuremath{+4.05}\,pp over the frozen 3-run pool and \ensuremath{+3.35}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.topdfresh\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.topdfresh_six\endcsname{\ensuremath{+1.27}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.topdfreshpair\endcsname{\ensuremath{+1.96}\,pp over the frozen 3-run pool and \ensuremath{+1.27}\,pp over the 6-run reference}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.topfresh\endcsname{mid third}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.topkeep\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.topnull\endcsname{0.84}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.topz\endcsname{\ensuremath{-2.48}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.tumour.d0\endcsname{\ensuremath{+3.49}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.tumour.d0_six\endcsname{\ensuremath{+3.20}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.tumour.dfresh\endcsname{\ensuremath{+1.39}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.tumour.dfresh_six\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.vol_large.d0\endcsname{\ensuremath{+2.73}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.vol_large.d0_six\endcsname{\ensuremath{+2.26}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.vol_large.dfresh\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.vol_large.dfresh_six\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.vol_mid.d0\endcsname{\ensuremath{+4.05}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.vol_mid.d0_six\endcsname{\ensuremath{+3.35}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.vol_mid.dfresh\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.vol_mid.dfresh_six\endcsname{\ensuremath{+1.27}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.vol_small.d0\endcsname{\ensuremath{+3.68}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.vol_small.d0_six\endcsname{\ensuremath{+3.97}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.vol_small.dfresh\endcsname{\ensuremath{+1.44}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.W1c.vol_small.dfresh_six\endcsname{\ensuremath{+1.72}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.kidney.null\endcsname{0.478}
\expandafter\gdef\csname R@an.replication_all.kits.sub.kidney.sd\endcsname{0.391}
\expandafter\gdef\csname R@an.replication_all.kits.sub.kidney.shift6\endcsname{\ensuremath{+0.117}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.large.null\endcsname{0.425}
\expandafter\gdef\csname R@an.replication_all.kits.sub.large.sd\endcsname{0.347}
\expandafter\gdef\csname R@an.replication_all.kits.sub.masses.null\endcsname{1.318}
\expandafter\gdef\csname R@an.replication_all.kits.sub.masses.sd\endcsname{1.076}
\expandafter\gdef\csname R@an.replication_all.kits.sub.masses.shift6\endcsname{\ensuremath{+0.321}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.measure\endcsname{physical tumour volume (mL)}
\expandafter\gdef\csname R@an.replication_all.kits.sub.mid.null\endcsname{0.839}
\expandafter\gdef\csname R@an.replication_all.kits.sub.mid.sd\endcsname{0.685}
\expandafter\gdef\csname R@an.replication_all.kits.sub.n\endcsname{98}
\expandafter\gdef\csname R@an.replication_all.kits.sub.ngroup\endcsname{6}
\expandafter\gdef\csname R@an.replication_all.kits.sub.perarm.above1.list\endcsname{StackDec, ResEnc-M, HyReX-LeanDec}
\expandafter\gdef\csname R@an.replication_all.kits.sub.perarm.n\endcsname{25}
\expandafter\gdef\csname R@an.replication_all.kits.sub.perarm.nabove1\endcsname{3}
\expandafter\gdef\csname R@an.replication_all.kits.sub.perarm.nbelow1\endcsname{22}
\expandafter\gdef\csname R@an.replication_all.kits.sub.perarm.slopemax\endcsname{2.391}
\expandafter\gdef\csname R@an.replication_all.kits.sub.perarm.slopemax.arm\endcsname{StackDec}
\expandafter\gdef\csname R@an.replication_all.kits.sub.perarm.slopemin\endcsname{\ensuremath{-0.608}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.perarm.slopemin.arm\endcsname{HyReX, finer ConvNeXt}
\expandafter\gdef\csname R@an.replication_all.kits.sub.perarm.spread\endcsname{3 of 25 steeper than the identity line}
\expandafter\gdef\csname R@an.replication_all.kits.sub.pooled.atTop\endcsname{\ensuremath{+4.01}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.pooled.intercept\endcsname{\ensuremath{+0.89}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.pooled.n\endcsname{150}
\expandafter\gdef\csname R@an.replication_all.kits.sub.pooled.nindep\endcsname{25}
\expandafter\gdef\csname R@an.replication_all.kits.sub.pooled.rho\endcsname{0.646}
\expandafter\gdef\csname R@an.replication_all.kits.sub.pooled.slope\endcsname{0.480}
\expandafter\gdef\csname R@an.replication_all.kits.sub.pooled.word\endcsname{attenuates}
\expandafter\gdef\csname R@an.replication_all.kits.sub.rule\endcsname{rank thirds (33/33/32)}
\expandafter\gdef\csname R@an.replication_all.kits.sub.six.n\endcsname{6}
\expandafter\gdef\csname R@an.replication_all.kits.sub.small.null\endcsname{2.996}
\expandafter\gdef\csname R@an.replication_all.kits.sub.small.sd\endcsname{2.447}
\expandafter\gdef\csname R@an.replication_all.kits.sub.topkeepn\endcsname{14 of 25}
\expandafter\gdef\csname R@an.replication_all.kits.sub.tumour.null\endcsname{1.303}
\expandafter\gdef\csname R@an.replication_all.kits.sub.tumour.sd\endcsname{1.064}
\expandafter\gdef\csname R@an.replication_all.kits.sub.tumour.shift6\endcsname{\ensuremath{+0.292}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.vol_large.null\endcsname{0.425}
\expandafter\gdef\csname R@an.replication_all.kits.sub.vol_large.sd\endcsname{0.347}
\expandafter\gdef\csname R@an.replication_all.kits.sub.vol_large.shift6\endcsname{\ensuremath{+0.473}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.vol_mid.null\endcsname{0.839}
\expandafter\gdef\csname R@an.replication_all.kits.sub.vol_mid.sd\endcsname{0.685}
\expandafter\gdef\csname R@an.replication_all.kits.sub.vol_mid.shift6\endcsname{\ensuremath{+0.693}}
\expandafter\gdef\csname R@an.replication_all.kits.sub.vol_small.null\endcsname{2.996}
\expandafter\gdef\csname R@an.replication_all.kits.sub.vol_small.sd\endcsname{2.447}
\expandafter\gdef\csname R@an.replication_all.kits.sub.vol_small.shift6\endcsname{\ensuremath{-0.285}}
\expandafter\gdef\csname R@an.replication_all.kits.teammax\endcsname{45}
\expandafter\gdef\csname R@an.replication_all.kits.unsel.hi\endcsname{\ensuremath{+2.83}}
\expandafter\gdef\csname R@an.replication_all.kits.unsel.hw\endcsname{1.908}
\expandafter\gdef\csname R@an.replication_all.kits.unsel.list\endcsname{ResEnc-M, ResEnc-matched, branch control, fn.-identical control}
\expandafter\gdef\csname R@an.replication_all.kits.unsel.list.long\endcsname{the library's residual-encoder preset, its ResEnc-matched re-implementation, a parameter-matched branch control and the function-identical control}
\expandafter\gdef\csname R@an.replication_all.kits.unsel.lo\endcsname{\ensuremath{-2.84}}
\expandafter\gdef\csname R@an.replication_all.kits.unsel.meanshrink\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.replication_all.kits.unsel.n\endcsname{4}
\expandafter\gdef\csname R@an.replication_all.kits.unsel.nup\endcsname{2}
\expandafter\gdef\csname R@an.replication_all.kits.unsel.sdexp\endcsname{0.974}
\expandafter\gdef\csname R@an.replication_all.rep.ds\endcsname{AMOS22 and KiTS23}
\expandafter\gdef\csname R@an.replication_all.rep.kept.list\endcsname{HyReX on KiTS23, ResEnc-M on KiTS23, ResEnc-matched on KiTS23, ResEnc+context on KiTS23, HyReX+context on KiTS23, branch control on KiTS23, HyReX, finer ConvNeXt on KiTS23, HyReX point-fuse on KiTS23, HyReX+dec. capacity on KiTS23, LeanDec on KiTS23, fn.-identical control on KiTS23, LeanAdd on KiTS23, LeanAdd-NeXt on KiTS23, HyReX-LeanDec on KiTS23, LeanTrunk on KiTS23, Stem1 on KiTS23, CoarseStack on KiTS23, StackDec on KiTS23, LeanDeepMid+FD on KiTS23, LeanSep on KiTS23, LeanDil on KiTS23, LeanDeepMid on KiTS23, LeanNeXt-s5 on KiTS23, HyReX-k9 on KiTS23, ResEnc-M on AMOS22, ResEnc+context on AMOS22}
\expandafter\gdef\csname R@an.replication_all.rep.lost.list\endcsname{ConvNeXt-k3 on KiTS23, HyReX on AMOS22, ConvNeXt-k3 on AMOS22}
\expandafter\gdef\csname R@an.replication_all.rep.n\endcsname{29}
\expandafter\gdef\csname R@an.replication_all.rep.nkept\endcsname{26}
\expandafter\gdef\csname R@an.replication_all.rep.nlost\endcsname{3}
\expandafter\gdef\csname R@an.replication_all.rep.state\endcsname{26 of 29 fired screens with a finished fresh pair still clear the registered bar on seeds 1--2}
\expandafter\gdef\csname R@an.replication_all.sel.alone.sentence\endcsname{selection alone accounts for the shrinkage}
\expandafter\gdef\csname R@an.replication_all.slope.cap\endcsname{11}
\expandafter\gdef\csname R@an.replication_all.slope.cap.kind\endcsname{derived from the measured room and the measured cost of one arm}
\expandafter\gdef\csname R@an.replication_all.slope.cont\endcsname{continued}
\expandafter\gdef\csname R@an.replication_all.slope.fig1.height\endcsname{6.37}
\expandafter\gdef\csname R@an.replication_all.slope.fig1.part\endcsname{the arms a selection step could pick, first part in registry order}
\expandafter\gdef\csname R@an.replication_all.slope.fig1.room\endcsname{6.91}
\expandafter\gdef\csname R@an.replication_all.slope.fig2.exists\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.slope.fig2.height\endcsname{6.42}
\expandafter\gdef\csname R@an.replication_all.slope.fig2.part\endcsname{the arms a selection step could pick, second part in registry order}
\expandafter\gdef\csname R@an.replication_all.slope.fig2.room\endcsname{8.28}
\expandafter\gdef\csname R@an.replication_all.slope.fig2.tag\endcsname{continued}
\expandafter\gdef\csname R@an.replication_all.slope.fig3.exists\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.slope.fig3.height\endcsname{5.80}
\expandafter\gdef\csname R@an.replication_all.slope.fig3.part\endcsname{the arms no selection step could pick, with the reference and attribution arms}
\expandafter\gdef\csname R@an.replication_all.slope.fig3.room\endcsname{8.28}
\expandafter\gdef\csname R@an.replication_all.slope.fig3.tag\endcsname{continued}
\expandafter\gdef\csname R@an.replication_all.slope.height\endcsname{6.37}
\expandafter\gdef\csname R@an.replication_all.slope.measured\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.slope.nfig\endcsname{3}
\expandafter\gdef\csname R@an.replication_all.slope.nfig.word\endcsname{three}
\expandafter\gdef\csname R@an.replication_all.slope.perarm\endcsname{0.340}
\expandafter\gdef\csname R@an.replication_all.slope.room\endcsname{6.91}
\expandafter\gdef\csname R@an.replication_all.slope.sentence\endcsname{the exhibit is drawn in three figures, split by group: the arms a selection step could pick, first part in registry order, the arms a selection step could pick, second part in registry order and the arms no selection step could pick, with the reference and attribution arms}
\expandafter\gdef\csname R@an.replication_all.slope.slack\endcsname{0.54}
\expandafter\gdef\csname R@an.replication_all.slope.split\endcsname{yes}
\expandafter\gdef\csname R@an.replication_all.status.acdc\endcsname{4 of 4 registered arms replicated on fresh seeds 1--2}
\expandafter\gdef\csname R@an.replication_all.status.amos\endcsname{5 of 7 registered arms replicated on fresh seeds 1--2}
\expandafter\gdef\csname R@an.replication_all.status.kits\endcsname{25 of 25 registered arms replicated on fresh seeds 1--2}
\expandafter\gdef\csname R@an.robustness.amos.all.L1.d0\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.robustness.amos.all.L1.dfresh\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.robustness.amos.all.L1b.d0\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.robustness.amos.all.L1b.dfresh\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.robustness.amos.all.L3.d0\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.robustness.amos.all.L3.dfresh\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.robustness.amos.all.L4.d0\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.robustness.amos.all.L4.dfresh\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.robustness.amos.all.arms_in\endcsname{HyReX}
\expandafter\gdef\csname R@an.robustness.amos.all.arms_out\endcsname{ResEnc-M, ResEnc-matched and ResEnc+context}
\expandafter\gdef\csname R@an.robustness.amos.all.band\endcsname{0.20}
\expandafter\gdef\csname R@an.robustness.amos.all.bandfresh\endcsname{0.20}
\expandafter\gdef\csname R@an.robustness.amos.all.bands0\endcsname{0.26}
\expandafter\gdef\csname R@an.robustness.amos.all.n\endcsname{40}
\expandafter\gdef\csname R@an.robustness.amos.all.nres\endcsname{3}
\expandafter\gdef\csname R@an.robustness.amos.all.split\endcsname{3 of the 4 arms in the table lie outside their own band (ResEnc-M, ResEnc-matched and ResEnc+context) and HyReX stays inside}
\expandafter\gdef\csname R@an.robustness.amos.ct_rows\endcsname{499}
\expandafter\gdef\csname R@an.robustness.amos.dev.philips.n\endcsname{68}
\expandafter\gdef\csname R@an.robustness.amos.dev.siemens.n\endcsname{50}
\expandafter\gdef\csname R@an.robustness.amos.dev.toshiba.n\endcsname{82}
\expandafter\gdef\csname R@an.robustness.amos.domaingap\endcsname{5.31}
\expandafter\gdef\csname R@an.robustness.amos.dup_id\endcsname{500}
\expandafter\gdef\csname R@an.robustness.amos.dup_rows\endcsname{2}
\expandafter\gdef\csname R@an.robustness.amos.hero.agg\endcsname{inside}
\expandafter\gdef\csname R@an.robustness.amos.hero.band\endcsname{0.20}
\expandafter\gdef\csname R@an.robustness.amos.hero.d0\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.robustness.amos.hero.dfresh\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.robustness.amos.hero.nin\endcsname{5}
\expandafter\gdef\csname R@an.robustness.amos.hero.screen\endcsname{the discovery seed cleared the registered 0.35 pp screening bar (+0.38 pp) and the two-seed fresh mean does not (+0.13 pp)}
\expandafter\gdef\csname R@an.robustness.amos.hero.screenbar\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.robustness.amos.hero.strata\endcsname{all 5}
\expandafter\gdef\csname R@an.robustness.amos.hero.tag\endcsname{HyReX}
\expandafter\gdef\csname R@an.robustness.amos.maxsplitid\endcsname{410}
\expandafter\gdef\csname R@an.robustness.amos.mri_rows\endcsname{99}
\expandafter\gdef\csname R@an.robustness.amos.nfigarms\endcsname{6}
\expandafter\gdef\csname R@an.robustness.amos.nfigarms_done\endcsname{6}
\expandafter\gdef\csname R@an.robustness.amos.nfresh_arms\endcsname{5}
\expandafter\gdef\csname R@an.robustness.amos.nfresh_seeds\endcsname{10}
\expandafter\gdef\csname R@an.robustness.amos.nstrata\endcsname{5}
\expandafter\gdef\csname R@an.robustness.amos.philips.L1.d0\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.robustness.amos.philips.L1.dfresh\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.robustness.amos.philips.L1b.d0\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.robustness.amos.philips.L1b.dfresh\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.robustness.amos.philips.L2.d0\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.robustness.amos.philips.L2.dfresh\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.robustness.amos.philips.L3.d0\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.robustness.amos.philips.L3.dfresh\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.robustness.amos.philips.L4.d0\endcsname{\ensuremath{+0.72}}
\expandafter\gdef\csname R@an.robustness.amos.philips.L4.dfresh\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.robustness.amos.philips.L6.d0\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.robustness.amos.philips.W1.d0\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.robustness.amos.philips.W1c.d0\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.robustness.amos.philips.W2.d0\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.robustness.amos.philips.W3.d0\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.robustness.amos.philips.W3c.d0\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.robustness.amos.philips.W4.d0\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.robustness.amos.philips.W5.d0\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.robustness.amos.philips.default_dice\endcsname{86.09}
\expandafter\gdef\csname R@an.robustness.amos.poolnu\endcsname{5}
\expandafter\gdef\csname R@an.robustness.amos.res.arms_in\endcsname{HyReX}
\expandafter\gdef\csname R@an.robustness.amos.res.arms_out\endcsname{ResEnc+context, ResEnc-matched and ResEnc-M}
\expandafter\gdef\csname R@an.robustness.amos.res.band\endcsname{0.38}
\expandafter\gdef\csname R@an.robustness.amos.res.bandword\endcsname{two-seed fresh-mean}
\expandafter\gdef\csname R@an.robustness.amos.res.floor\endcsname{0.50}
\expandafter\gdef\csname R@an.robustness.amos.res.lead\endcsname{ResEnc+context is the largest at +0.88 pp against its own ±0.38 pp two-seed fresh-mean band, but only 0.07 pp clear of the next arm (ResEnc-matched) — under the registered 0.50 pp one-seed pair floor, so which of them is largest is not resolved}
\expandafter\gdef\csname R@an.robustness.amos.res.names\endcsname{Philips}
\expandafter\gdef\csname R@an.robustness.amos.res.narms\endcsname{3}
\expandafter\gdef\csname R@an.robustness.amos.res.ncases\endcsname{12}
\expandafter\gdef\csname R@an.robustness.amos.res.nin\endcsname{1}
\expandafter\gdef\csname R@an.robustness.amos.res.ninside\endcsname{4}
\expandafter\gdef\csname R@an.robustness.amos.res.nstrata\endcsname{1}
\expandafter\gdef\csname R@an.robustness.amos.res.ntab\endcsname{4}
\expandafter\gdef\csname R@an.robustness.amos.res.split\endcsname{3 of the 4 arms in the table do (ResEnc+context, ResEnc-matched and ResEnc-M), while HyReX stays inside}
\expandafter\gdef\csname R@an.robustness.amos.res.widest\endcsname{ResEnc+context}
\expandafter\gdef\csname R@an.robustness.amos.res.widest_d\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.robustness.amos.res.widest_gap\endcsname{0.07}
\expandafter\gdef\csname R@an.robustness.amos.rows\endcsname{600}
\expandafter\gdef\csname R@an.robustness.amos.siemens.L1.d0\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.robustness.amos.siemens.L1.dfresh\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.robustness.amos.siemens.L1b.d0\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.robustness.amos.siemens.L1b.dfresh\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.robustness.amos.siemens.L2.d0\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.robustness.amos.siemens.L2.dfresh\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.robustness.amos.siemens.L3.d0\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.robustness.amos.siemens.L3.dfresh\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.robustness.amos.siemens.L4.d0\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.robustness.amos.siemens.L4.dfresh\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.robustness.amos.siemens.L6.d0\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.robustness.amos.siemens.W1.d0\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.robustness.amos.siemens.W1c.d0\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.robustness.amos.siemens.W2.d0\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.robustness.amos.siemens.W3.d0\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.robustness.amos.siemens.W3c.d0\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.robustness.amos.siemens.W4.d0\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.robustness.amos.siemens.W5.d0\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.robustness.amos.siemens.default_dice\endcsname{91.16}
\expandafter\gdef\csname R@an.robustness.amos.siemens.thick.n\endcsname{4}
\expandafter\gdef\csname R@an.robustness.amos.siemens.thin.n\endcsname{10}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.L1.d0\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.L1.dfresh\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.L1b.d0\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.L1b.dfresh\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.L2.d0\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.L2.dfresh\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.L3.d0\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.L3.dfresh\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.L4.d0\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.L4.dfresh\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.L6.d0\endcsname{\ensuremath{-0.76}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.W1.d0\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.W1c.d0\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.W2.d0\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.W3.d0\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.W3c.d0\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.W4.d0\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.W5.d0\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.altref_shift\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.conref_shift\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.default_dice\endcsname{93.50}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.nullsd\endcsname{0.39}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thick.nullsdfresh\endcsname{0.30}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.L1.d0\endcsname{\ensuremath{+0.89}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.L1.dfresh\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.L1b.d0\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.L1b.dfresh\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.L2.d0\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.L2.dfresh\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.L3.d0\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.L3.dfresh\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.L4.d0\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.L4.dfresh\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.L6.d0\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.W1.d0\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.W1c.d0\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.W2.d0\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.W3.d0\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.W3c.d0\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.W4.d0\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.W5.d0\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.altref_shift\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.conref_shift\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.default_dice\endcsname{90.22}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.nullsd\endcsname{0.53}
\expandafter\gdef\csname R@an.robustness.amos.siemens_thin.nullsdfresh\endcsname{0.40}
\expandafter\gdef\csname R@an.robustness.amos.site.center.L1.d0\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.robustness.amos.site.center.L1.dfresh\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.robustness.amos.site.center.L1b.d0\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.robustness.amos.site.center.L1b.dfresh\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.robustness.amos.site.center.L2.d0\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.robustness.amos.site.center.L2.dfresh\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.robustness.amos.site.center.L3.d0\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.robustness.amos.site.center.L3.dfresh\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.robustness.amos.site.center.L4.d0\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.robustness.amos.site.center.L4.dfresh\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@an.robustness.amos.site.center.L6.d0\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.robustness.amos.site.center.W1.d0\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.robustness.amos.site.center.W1c.d0\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.robustness.amos.site.center.W2.d0\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.robustness.amos.site.center.W3.d0\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.robustness.amos.site.center.W3c.d0\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.robustness.amos.site.center.W4.d0\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.robustness.amos.site.center.W5.d0\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.robustness.amos.site.center.default_dice\endcsname{85.84}
\expandafter\gdef\csname R@an.robustness.amos.site.center.n\endcsname{26}
\expandafter\gdef\csname R@an.robustness.amos.site.center.vendors\endcsname{Philips + Toshiba}
\expandafter\gdef\csname R@an.robustness.amos.site.people.L1.d0\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.robustness.amos.site.people.L1.dfresh\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.robustness.amos.site.people.L1b.d0\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.robustness.amos.site.people.L1b.dfresh\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.robustness.amos.site.people.L2.d0\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.robustness.amos.site.people.L2.dfresh\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.robustness.amos.site.people.L3.d0\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.robustness.amos.site.people.L3.dfresh\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.robustness.amos.site.people.L4.d0\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.robustness.amos.site.people.L4.dfresh\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.robustness.amos.site.people.L6.d0\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.robustness.amos.site.people.W1.d0\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.robustness.amos.site.people.W1c.d0\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.robustness.amos.site.people.W2.d0\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.robustness.amos.site.people.W3.d0\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.robustness.amos.site.people.W3c.d0\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.robustness.amos.site.people.W4.d0\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.robustness.amos.site.people.W5.d0\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.robustness.amos.site.people.default_dice\endcsname{91.16}
\expandafter\gdef\csname R@an.robustness.amos.site.people.n\endcsname{14}
\expandafter\gdef\csname R@an.robustness.amos.site.people.vendors\endcsname{Siemens}
\expandafter\gdef\csname R@an.robustness.amos.stratum.philips.nres\endcsname{3}
\expandafter\gdef\csname R@an.robustness.amos.stratum.siemens.nres\endcsname{0}
\expandafter\gdef\csname R@an.robustness.amos.stratum.siemens_thick.nres\endcsname{0}
\expandafter\gdef\csname R@an.robustness.amos.stratum.siemens_thin.nres\endcsname{0}
\expandafter\gdef\csname R@an.robustness.amos.stratum.toshiba.nres\endcsname{0}
\expandafter\gdef\csname R@an.robustness.amos.tcrit\endcsname{2.57}
\expandafter\gdef\csname R@an.robustness.amos.thick.n\endcsname{30}
\expandafter\gdef\csname R@an.robustness.amos.thickgap\endcsname{3.27}
\expandafter\gdef\csname R@an.robustness.amos.thin.model\endcsname{SOMATOM Force}
\expandafter\gdef\csname R@an.robustness.amos.thin.n\endcsname{10}
\expandafter\gdef\csname R@an.robustness.amos.thin_all_siemens\endcsname{10 of 10}
\expandafter\gdef\csname R@an.robustness.amos.toshiba.L1.d0\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.robustness.amos.toshiba.L1.dfresh\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.robustness.amos.toshiba.L1b.d0\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.robustness.amos.toshiba.L1b.dfresh\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.robustness.amos.toshiba.L2.d0\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.robustness.amos.toshiba.L2.dfresh\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.robustness.amos.toshiba.L3.d0\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.robustness.amos.toshiba.L3.dfresh\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.robustness.amos.toshiba.L4.d0\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.robustness.amos.toshiba.L4.dfresh\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.robustness.amos.toshiba.L6.d0\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.robustness.amos.toshiba.W1.d0\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.robustness.amos.toshiba.W1c.d0\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.robustness.amos.toshiba.W2.d0\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.robustness.amos.toshiba.W3.d0\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.robustness.amos.toshiba.W3c.d0\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.robustness.amos.toshiba.W4.d0\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.robustness.amos.toshiba.W5.d0\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.robustness.amos.toshiba.default_dice\endcsname{85.62}
\expandafter\gdef\csname R@an.robustness.amos.train.philips.n\endcsname{56}
\expandafter\gdef\csname R@an.robustness.amos.train.siemens.n\endcsname{36}
\expandafter\gdef\csname R@an.robustness.amos.train.toshiba.n\endcsname{68}
\expandafter\gdef\csname R@an.robustness.amos.uncmax\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.robustness.amos.uncmin\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.robustness.amos.uncompiled_shift\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.robustness.amos.uncspread\endcsname{0.61}
\expandafter\gdef\csname R@an.robustness.amos.val.philips.n\endcsname{12}
\expandafter\gdef\csname R@an.robustness.amos.val.siemens.n\endcsname{14}
\expandafter\gdef\csname R@an.robustness.amos.val.toshiba.n\endcsname{14}
\expandafter\gdef\csname R@an.robustness.amos.vendor.L1.npos\endcsname{3}
\expandafter\gdef\csname R@an.robustness.amos.vendor.L1.nres\endcsname{1}
\expandafter\gdef\csname R@an.robustness.amos.vendor.L1b.npos\endcsname{3}
\expandafter\gdef\csname R@an.robustness.amos.vendor.L1b.nres\endcsname{1}
\expandafter\gdef\csname R@an.robustness.amos.vendor.L2.npos\endcsname{3}
\expandafter\gdef\csname R@an.robustness.amos.vendor.L2.nres\endcsname{0}
\expandafter\gdef\csname R@an.robustness.amos.vendor.L3.npos\endcsname{3}
\expandafter\gdef\csname R@an.robustness.amos.vendor.L3.nres\endcsname{0}
\expandafter\gdef\csname R@an.robustness.amos.vendor.L4.npos\endcsname{3}
\expandafter\gdef\csname R@an.robustness.amos.vendor.L4.nres\endcsname{1}
\expandafter\gdef\csname R@an.robustness.amos.vendor.L6.npos\endcsname{2}
\expandafter\gdef\csname R@an.robustness.amos.vendor.L6.nres\endcsname{0}
\expandafter\gdef\csname R@an.robustness.amos.vendor.W1.npos\endcsname{2}
\expandafter\gdef\csname R@an.robustness.amos.vendor.W1.nres\endcsname{0}
\expandafter\gdef\csname R@an.robustness.amos.vendor.W1c.npos\endcsname{3}
\expandafter\gdef\csname R@an.robustness.amos.vendor.W1c.nres\endcsname{0}
\expandafter\gdef\csname R@an.robustness.amos.vendor.W2.npos\endcsname{3}
\expandafter\gdef\csname R@an.robustness.amos.vendor.W2.nres\endcsname{0}
\expandafter\gdef\csname R@an.robustness.amos.vendor.W3.npos\endcsname{2}
\expandafter\gdef\csname R@an.robustness.amos.vendor.W3.nres\endcsname{0}
\expandafter\gdef\csname R@an.robustness.amos.vendor.W3c.npos\endcsname{2}
\expandafter\gdef\csname R@an.robustness.amos.vendor.W3c.nres\endcsname{0}
\expandafter\gdef\csname R@an.robustness.amos.vendor.W4.npos\endcsname{2}
\expandafter\gdef\csname R@an.robustness.amos.vendor.W4.nres\endcsname{0}
\expandafter\gdef\csname R@an.robustness.amos.vendor.W5.npos\endcsname{3}
\expandafter\gdef\csname R@an.robustness.amos.vendor.W5.nres\endcsname{1}
\expandafter\gdef\csname R@an.robustness.amos.vendor.philips.altref_shift\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.robustness.amos.vendor.philips.conref_shift\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.robustness.amos.vendor.philips.n\endcsname{12}
\expandafter\gdef\csname R@an.robustness.amos.vendor.philips.nullsd\endcsname{0.25}
\expandafter\gdef\csname R@an.robustness.amos.vendor.philips.nullsdfresh\endcsname{0.19}
\expandafter\gdef\csname R@an.robustness.amos.vendor.siemens.altref_shift\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.robustness.amos.vendor.siemens.conref_shift\endcsname{0.00}
\expandafter\gdef\csname R@an.robustness.amos.vendor.siemens.n\endcsname{14}
\expandafter\gdef\csname R@an.robustness.amos.vendor.siemens.nullsd\endcsname{0.36}
\expandafter\gdef\csname R@an.robustness.amos.vendor.siemens.nullsdfresh\endcsname{0.27}
\expandafter\gdef\csname R@an.robustness.amos.vendor.toshiba.altref_shift\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@an.robustness.amos.vendor.toshiba.conref_shift\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.robustness.amos.vendor.toshiba.n\endcsname{14}
\expandafter\gdef\csname R@an.robustness.amos.vendor.toshiba.nullsd\endcsname{0.49}
\expandafter\gdef\csname R@an.robustness.amos.vendor.toshiba.nullsdfresh\endcsname{0.37}
\expandafter\gdef\csname R@an.robustness.amos.vendor_site_aliased\endcsname{yes}
\expandafter\gdef\csname R@an.robustness.amos.vendormax.L1\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.robustness.amos.vendormax.L1b\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.robustness.amos.vendormax.L2\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.robustness.amos.vendormax.L3\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.robustness.amos.vendormax.L4\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.robustness.amos.vendormax.L6\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.robustness.amos.vendormax.W1\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.robustness.amos.vendormax.W1c\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.robustness.amos.vendormax.W2\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.robustness.amos.vendormax.W3\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.robustness.amos.vendormax.W3c\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.robustness.amos.vendormax.W4\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.robustness.amos.vendormax.W5\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.robustness.amos.vendormin.L1\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.robustness.amos.vendormin.L1b\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.robustness.amos.vendormin.L2\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.robustness.amos.vendormin.L3\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.robustness.amos.vendormin.L4\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@an.robustness.amos.vendormin.L6\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.robustness.amos.vendormin.W1\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.robustness.amos.vendormin.W1c\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.robustness.amos.vendormin.W2\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.robustness.amos.vendormin.W3\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.robustness.amos.vendormin.W3c\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.robustness.amos.vendormin.W4\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.robustness.amos.vendormin.W5\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.robustness.amos.vendorspread.L1\endcsname{0.30}
\expandafter\gdef\csname R@an.robustness.amos.vendorspread.L1b\endcsname{0.78}
\expandafter\gdef\csname R@an.robustness.amos.vendorspread.L2\endcsname{0.29}
\expandafter\gdef\csname R@an.robustness.amos.vendorspread.L3\endcsname{0.16}
\expandafter\gdef\csname R@an.robustness.amos.vendorspread.L4\endcsname{0.67}
\expandafter\gdef\csname R@an.robustness.amos.vendorspread.L6\endcsname{0.71}
\expandafter\gdef\csname R@an.robustness.amos.vendorspread.W1\endcsname{0.22}
\expandafter\gdef\csname R@an.robustness.amos.vendorspread.W1c\endcsname{0.21}
\expandafter\gdef\csname R@an.robustness.amos.vendorspread.W2\endcsname{0.12}
\expandafter\gdef\csname R@an.robustness.amos.vendorspread.W3\endcsname{0.82}
\expandafter\gdef\csname R@an.robustness.amos.vendorspread.W3c\endcsname{0.87}
\expandafter\gdef\csname R@an.robustness.amos.vendorspread.W4\endcsname{0.48}
\expandafter\gdef\csname R@an.robustness.amos.vendorspread.W5\endcsname{0.77}
\expandafter\gdef\csname R@an.robustness.kits.L3.ccrcc_minus_other\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.robustness.kits.L3.ccrcc_minus_other.p\endcsname{0.762}
\expandafter\gdef\csname R@an.robustness.kits.L3.ccrcc_n\endcsname{61}
\expandafter\gdef\csname R@an.robustness.kits.L3.other_n\endcsname{34}
\expandafter\gdef\csname R@an.robustness.kits.ahead.L3_over_L1.n\endcsname{2}
\expandafter\gdef\csname R@an.robustness.kits.ahead.L3_over_L1.nbehind\endcsname{20}
\expandafter\gdef\csname R@an.robustness.kits.ahead.L3_over_L1.nbig\endcsname{2}
\expandafter\gdef\csname R@an.robustness.kits.ahead.L3_over_L1.of\endcsname{22}
\expandafter\gdef\csname R@an.robustness.kits.ahead.L3_over_L1.ofbig\endcsname{16}
\expandafter\gdef\csname R@an.robustness.kits.all.L1.d0\endcsname{\ensuremath{+2.90}}
\expandafter\gdef\csname R@an.robustness.kits.all.L1.dfresh\endcsname{\ensuremath{+5.09}}
\expandafter\gdef\csname R@an.robustness.kits.all.L1.kidfresh\endcsname{\ensuremath{+1.19}}
\expandafter\gdef\csname R@an.robustness.kits.all.L1.shift\endcsname{\ensuremath{+2.19}}
\expandafter\gdef\csname R@an.robustness.kits.all.L1b.d0\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@an.robustness.kits.all.L1b.dfresh\endcsname{\ensuremath{+2.80}}
\expandafter\gdef\csname R@an.robustness.kits.all.L1b.kidfresh\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.robustness.kits.all.L1b.shift\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.robustness.kits.all.L2.d0\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.robustness.kits.all.L2.dfresh\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.robustness.kits.all.L2.kidfresh\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.robustness.kits.all.L2.shift\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.robustness.kits.all.L3.d0\endcsname{\ensuremath{+4.11}}
\expandafter\gdef\csname R@an.robustness.kits.all.L3.dfresh\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@an.robustness.kits.all.L3.kidfresh\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.robustness.kits.all.L3.shift\endcsname{\ensuremath{-1.77}}
\expandafter\gdef\csname R@an.robustness.kits.all.L4.d0\endcsname{\ensuremath{+3.50}}
\expandafter\gdef\csname R@an.robustness.kits.all.L4.dfresh\endcsname{\ensuremath{+3.14}}
\expandafter\gdef\csname R@an.robustness.kits.all.L4.kidfresh\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.robustness.kits.all.L4.shift\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.robustness.kits.all.L6.d0\endcsname{\ensuremath{+3.90}}
\expandafter\gdef\csname R@an.robustness.kits.all.L6.dfresh\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.robustness.kits.all.L6.kidfresh\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.robustness.kits.all.L6.shift\endcsname{\ensuremath{-1.48}}
\expandafter\gdef\csname R@an.robustness.kits.bandk\endcsname{2}
\expandafter\gdef\csname R@an.robustness.kits.big.L1.max\endcsname{\ensuremath{+6.72}}
\expandafter\gdef\csname R@an.robustness.kits.big.L1.min\endcsname{\ensuremath{+2.23}}
\expandafter\gdef\csname R@an.robustness.kits.big.L1.npos\endcsname{16}
\expandafter\gdef\csname R@an.robustness.kits.big.L1.nres\endcsname{16}
\expandafter\gdef\csname R@an.robustness.kits.big.L1b.max\endcsname{\ensuremath{+3.61}}
\expandafter\gdef\csname R@an.robustness.kits.big.L1b.min\endcsname{\ensuremath{+2.09}}
\expandafter\gdef\csname R@an.robustness.kits.big.L1b.npos\endcsname{16}
\expandafter\gdef\csname R@an.robustness.kits.big.L1b.nres\endcsname{12}
\expandafter\gdef\csname R@an.robustness.kits.big.L2.max\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.robustness.kits.big.L2.min\endcsname{\ensuremath{-1.86}}
\expandafter\gdef\csname R@an.robustness.kits.big.L2.npos\endcsname{10}
\expandafter\gdef\csname R@an.robustness.kits.big.L2.nres\endcsname{2}
\expandafter\gdef\csname R@an.robustness.kits.big.L3.max\endcsname{\ensuremath{+5.26}}
\expandafter\gdef\csname R@an.robustness.kits.big.L3.min\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.robustness.kits.big.L3.npos\endcsname{16}
\expandafter\gdef\csname R@an.robustness.kits.big.L3.nres\endcsname{9}
\expandafter\gdef\csname R@an.robustness.kits.big.L4.max\endcsname{\ensuremath{+4.78}}
\expandafter\gdef\csname R@an.robustness.kits.big.L4.min\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@an.robustness.kits.big.L4.npos\endcsname{16}
\expandafter\gdef\csname R@an.robustness.kits.big.L4.nres\endcsname{13}
\expandafter\gdef\csname R@an.robustness.kits.big.L6.max\endcsname{\ensuremath{+3.51}}
\expandafter\gdef\csname R@an.robustness.kits.big.L6.min\endcsname{\ensuremath{+1.32}}
\expandafter\gdef\csname R@an.robustness.kits.big.L6.npos\endcsname{16}
\expandafter\gdef\csname R@an.robustness.kits.big.L6.nres\endcsname{9}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.L1.d0\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.L1.dfresh\endcsname{\ensuremath{+5.49}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.L1.kidfresh\endcsname{\ensuremath{+1.16}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.L1b.d0\endcsname{\ensuremath{+1.77}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.L1b.dfresh\endcsname{\ensuremath{+2.22}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.L1b.kidfresh\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.L2.d0\endcsname{\ensuremath{-0.64}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.L2.dfresh\endcsname{\ensuremath{-0.89}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.L2.kidfresh\endcsname{\ensuremath{-0.58}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.L3.d0\endcsname{\ensuremath{+4.49}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.L3.dfresh\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.L3.kidfresh\endcsname{\ensuremath{+0.67}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.L4.d0\endcsname{\ensuremath{+2.57}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.L4.dfresh\endcsname{\ensuremath{+1.87}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.L4.kidfresh\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.L6.d0\endcsname{\ensuremath{+4.66}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.L6.dfresh\endcsname{\ensuremath{+1.32}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.L6.kidfresh\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.altref_shift\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.defdice\endcsname{73.35}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.kiddice\endcsname{96.07}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.n\endcsname{49}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.nullsd\endcsname{1.68}
\expandafter\gdef\csname R@an.robustness.kits.bmi.high.nullsd0\endcsname{2.13}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.L1.d0\endcsname{\ensuremath{+3.46}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.L1.dfresh\endcsname{\ensuremath{+4.70}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.L1.kidfresh\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.L1b.d0\endcsname{\ensuremath{+4.27}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.L1b.dfresh\endcsname{\ensuremath{+3.38}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.L1b.kidfresh\endcsname{\ensuremath{+1.36}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.L2.d0\endcsname{\ensuremath{+1.17}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.L2.dfresh\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.L2.kidfresh\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.L3.d0\endcsname{\ensuremath{+3.72}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.L3.dfresh\endcsname{\ensuremath{+3.68}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.L3.kidfresh\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.L4.d0\endcsname{\ensuremath{+4.43}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.L4.dfresh\endcsname{\ensuremath{+4.41}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.L4.kidfresh\endcsname{\ensuremath{+1.20}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.L6.d0\endcsname{\ensuremath{+3.14}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.L6.dfresh\endcsname{\ensuremath{+3.51}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.L6.kidfresh\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.altref_shift\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.defdice\endcsname{75.20}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.kiddice\endcsname{95.97}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.n\endcsname{49}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.nullsd\endcsname{1.04}
\expandafter\gdef\csname R@an.robustness.kits.bmi.low.nullsd0\endcsname{1.32}
\expandafter\gdef\csname R@an.robustness.kits.bmi.phet\endcsname{0.249}
\expandafter\gdef\csname R@an.robustness.kits.bmicut\endcsname{31.165}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.L1.d0\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.L1.dfresh\endcsname{\ensuremath{+4.49}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.L1.kidfresh\endcsname{\ensuremath{+1.20}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.L1b.d0\endcsname{\ensuremath{+1.75}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.L1b.dfresh\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.L1b.kidfresh\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.L2.d0\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.L2.dfresh\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.L2.kidfresh\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.L3.d0\endcsname{\ensuremath{+2.17}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.L3.dfresh\endcsname{\ensuremath{+2.28}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.L3.kidfresh\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.L4.d0\endcsname{\ensuremath{+3.65}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.L4.dfresh\endcsname{\ensuremath{+3.04}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.L4.kidfresh\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.L6.d0\endcsname{\ensuremath{+2.14}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.L6.dfresh\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.L6.kidfresh\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.altref_shift\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.defdice\endcsname{82.31}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.kiddice\endcsname{96.22}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.n\endcsname{60}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.nullsd\endcsname{0.52}
\expandafter\gdef\csname R@an.robustness.kits.cohort.early.nullsd0\endcsname{0.66}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.L1.d0\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.L1.dfresh\endcsname{\ensuremath{+6.04}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.L1.kidfresh\endcsname{\ensuremath{+1.16}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.L1b.d0\endcsname{\ensuremath{+5.03}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.L1b.dfresh\endcsname{\ensuremath{+3.61}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.L1b.kidfresh\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.L2.d0\endcsname{\ensuremath{+0.95}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.L2.dfresh\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.L2.kidfresh\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.L3.d0\endcsname{\ensuremath{+7.18}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.L3.dfresh\endcsname{\ensuremath{+2.43}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.L3.kidfresh\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.L4.d0\endcsname{\ensuremath{+3.26}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.L4.dfresh\endcsname{\ensuremath{+3.30}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.L4.kidfresh\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.L6.d0\endcsname{\ensuremath{+6.69}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.L6.dfresh\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.L6.kidfresh\endcsname{\ensuremath{+0.91}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.altref_shift\endcsname{\ensuremath{+1.23}}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.defdice\endcsname{61.58}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.kiddice\endcsname{95.71}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.n\endcsname{38}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.nullsd\endcsname{1.71}
\expandafter\gdef\csname R@an.robustness.kits.cohort.new.nullsd0\endcsname{2.17}
\expandafter\gdef\csname R@an.robustness.kits.cohort.phet\endcsname{0.951}
\expandafter\gdef\csname R@an.robustness.kits.defdice\endcsname{74.27}
\expandafter\gdef\csname R@an.robustness.kits.fwer_p\endcsname{0.141}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.L1.d0\endcsname{\ensuremath{+2.43}}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.L1.dfresh\endcsname{\ensuremath{+4.28}}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.L1.kidfresh\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.L1b.d0\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.L1b.dfresh\endcsname{\ensuremath{+2.96}}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.L1b.kidfresh\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.L2.d0\endcsname{\ensuremath{+0.91}}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.L2.dfresh\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.L2.kidfresh\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.L3.d0\endcsname{\ensuremath{+4.88}}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.L3.dfresh\endcsname{\ensuremath{+2.95}}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.L3.kidfresh\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.L4.d0\endcsname{\ensuremath{+2.43}}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.L4.dfresh\endcsname{\ensuremath{+2.96}}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.L4.kidfresh\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.L6.d0\endcsname{\ensuremath{+3.21}}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.L6.dfresh\endcsname{\ensuremath{+1.98}}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.L6.kidfresh\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.altref_shift\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.defdice\endcsname{75.68}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.kiddice\endcsname{96.63}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.n\endcsname{61}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.nullsd\endcsname{1.07}
\expandafter\gdef\csname R@an.robustness.kits.hist.ccrcc.nullsd0\endcsname{1.35}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.L1.d0\endcsname{\ensuremath{+5.02}}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.L1.dfresh\endcsname{\ensuremath{+5.39}}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.L1.kidfresh\endcsname{\ensuremath{+1.39}}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.L1b.d0\endcsname{\ensuremath{+4.39}}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.L1b.dfresh\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.L1b.kidfresh\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.L2.d0\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.L2.dfresh\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.L2.kidfresh\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.L3.d0\endcsname{\ensuremath{+3.45}}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.L3.dfresh\endcsname{\ensuremath{+2.20}}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.L3.kidfresh\endcsname{\ensuremath{+1.44}}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.L4.d0\endcsname{\ensuremath{+5.20}}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.L4.dfresh\endcsname{\ensuremath{+4.14}}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.L4.kidfresh\endcsname{\ensuremath{+1.43}}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.L6.d0\endcsname{\ensuremath{+3.96}}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.L6.dfresh\endcsname{\ensuremath{+3.50}}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.L6.kidfresh\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.altref_shift\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.defdice\endcsname{73.79}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.kiddice\endcsname{95.41}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.n\endcsname{34}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.nullsd\endcsname{1.14}
\expandafter\gdef\csname R@an.robustness.kits.hist.other.nullsd0\endcsname{1.44}
\expandafter\gdef\csname R@an.robustness.kits.hist.phet\endcsname{0.198}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.L1.d0\endcsname{\ensuremath{-11.70}}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.L1.dfresh\endcsname{\ensuremath{+18.27}}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.L1.kidfresh\endcsname{\ensuremath{+4.36}}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.L1b.d0\endcsname{\ensuremath{-4.49}}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.L1b.dfresh\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.L1b.kidfresh\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.L2.d0\endcsname{\ensuremath{-10.61}}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.L2.dfresh\endcsname{\ensuremath{-15.69}}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.L2.kidfresh\endcsname{\ensuremath{-0.72}}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.L3.d0\endcsname{\ensuremath{-4.01}}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.L3.dfresh\endcsname{\ensuremath{-8.62}}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.L3.kidfresh\endcsname{\ensuremath{-1.11}}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.L4.d0\endcsname{\ensuremath{+5.91}}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.L4.dfresh\endcsname{\ensuremath{-4.58}}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.L4.kidfresh\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.L6.d0\endcsname{\ensuremath{+17.22}}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.L6.dfresh\endcsname{\ensuremath{-1.01}}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.L6.kidfresh\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.altref_shift\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.defdice\endcsname{51.26}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.kiddice\endcsname{90.49}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.n\endcsname{3}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.nullsd\endcsname{11.73}
\expandafter\gdef\csname R@an.robustness.kits.hist.unknown.nullsd0\endcsname{14.83}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.L1.d0\endcsname{\ensuremath{+15.84}}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.L1.dfresh\endcsname{\ensuremath{+12.34}}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.L1.kidfresh\endcsname{\ensuremath{+3.56}}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.L1b.d0\endcsname{\ensuremath{+2.26}}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.L1b.dfresh\endcsname{\ensuremath{+6.75}}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.L1b.kidfresh\endcsname{\ensuremath{+4.72}}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.L2.d0\endcsname{\ensuremath{-5.60}}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.L2.dfresh\endcsname{\ensuremath{+4.65}}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.L2.kidfresh\endcsname{\ensuremath{+2.86}}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.L3.d0\endcsname{\ensuremath{+6.83}}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.L3.dfresh\endcsname{\ensuremath{+3.30}}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.L3.kidfresh\endcsname{\ensuremath{+3.49}}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.L4.d0\endcsname{\ensuremath{+7.77}}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.L4.dfresh\endcsname{\ensuremath{+6.55}}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.L4.kidfresh\endcsname{\ensuremath{+4.00}}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.L6.d0\endcsname{\ensuremath{+3.17}}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.L6.dfresh\endcsname{\ensuremath{+6.89}}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.L6.kidfresh\endcsname{\ensuremath{+2.28}}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.altref_shift\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.defdice\endcsname{58.51}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.kiddice\endcsname{91.92}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.n\endcsname{6}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.nullsd\endcsname{3.84}
\expandafter\gdef\csname R@an.robustness.kits.malig.no.nullsd0\endcsname{4.86}
\expandafter\gdef\csname R@an.robustness.kits.malig.phet\endcsname{0.199}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.L1.d0\endcsname{\ensuremath{-11.70}}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.L1.dfresh\endcsname{\ensuremath{+18.27}}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.L1.kidfresh\endcsname{\ensuremath{+4.36}}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.L1b.d0\endcsname{\ensuremath{-4.49}}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.L1b.dfresh\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.L1b.kidfresh\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.L2.d0\endcsname{\ensuremath{-10.61}}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.L2.dfresh\endcsname{\ensuremath{-15.69}}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.L2.kidfresh\endcsname{\ensuremath{-0.72}}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.L3.d0\endcsname{\ensuremath{-4.01}}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.L3.dfresh\endcsname{\ensuremath{-8.62}}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.L3.kidfresh\endcsname{\ensuremath{-1.11}}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.L4.d0\endcsname{\ensuremath{+5.91}}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.L4.dfresh\endcsname{\ensuremath{-4.58}}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.L4.kidfresh\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.L6.d0\endcsname{\ensuremath{+17.22}}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.L6.dfresh\endcsname{\ensuremath{-1.01}}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.L6.kidfresh\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.altref_shift\endcsname{\ensuremath{-0.66}}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.defdice\endcsname{51.26}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.kiddice\endcsname{90.49}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.n\endcsname{3}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.nullsd\endcsname{11.73}
\expandafter\gdef\csname R@an.robustness.kits.malig.unknown.nullsd0\endcsname{14.83}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.L1.d0\endcsname{\ensuremath{+2.52}}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.L1.dfresh\endcsname{\ensuremath{+4.16}}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.L1.kidfresh\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.L1b.d0\endcsname{\ensuremath{+3.32}}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.L1b.dfresh\endcsname{\ensuremath{+2.61}}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.L1b.kidfresh\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.L2.d0\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.L2.dfresh\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.L2.kidfresh\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.L3.d0\endcsname{\ensuremath{+4.20}}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.L3.dfresh\endcsname{\ensuremath{+2.64}}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.L3.kidfresh\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.L4.d0\endcsname{\ensuremath{+3.13}}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.L4.dfresh\endcsname{\ensuremath{+3.17}}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.L4.kidfresh\endcsname{\ensuremath{+0.67}}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.L6.d0\endcsname{\ensuremath{+3.50}}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.L6.dfresh\endcsname{\ensuremath{+2.23}}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.L6.kidfresh\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.altref_shift\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.defdice\endcsname{76.11}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.kiddice\endcsname{96.48}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.n\endcsname{89}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.nullsd\endcsname{0.79}
\expandafter\gdef\csname R@an.robustness.kits.malig.yes.nullsd0\endcsname{1.00}
\expandafter\gdef\csname R@an.robustness.kits.minp_factor\endcsname{Sex}
\expandafter\gdef\csname R@an.robustness.kits.n\endcsname{98}
\expandafter\gdef\csname R@an.robustness.kits.nbig\endcsname{16}
\expandafter\gdef\csname R@an.robustness.kits.nbig_min\endcsname{10}
\expandafter\gdef\csname R@an.robustness.kits.neg.L1.n\endcsname{0}
\expandafter\gdef\csname R@an.robustness.kits.neg.L1b.n\endcsname{0}
\expandafter\gdef\csname R@an.robustness.kits.neg.L2.defdice_hi\endcsname{78.95}
\expandafter\gdef\csname R@an.robustness.kits.neg.L2.defdice_lo\endcsname{48.15}
\expandafter\gdef\csname R@an.robustness.kits.neg.L2.maxcases\endcsname{61}
\expandafter\gdef\csname R@an.robustness.kits.neg.L2.n\endcsname{11}
\expandafter\gdef\csname R@an.robustness.kits.neg.L2.nmissing\endcsname{4}
\expandafter\gdef\csname R@an.robustness.kits.neg.L2.nrecorded\endcsname{7}
\expandafter\gdef\csname R@an.robustness.kits.neg.L2.nres_pairs\endcsname{19}
\expandafter\gdef\csname R@an.robustness.kits.neg.L2.nres_self\endcsname{1}
\expandafter\gdef\csname R@an.robustness.kits.neg.L2.nres_strata\endcsname{9}
\expandafter\gdef\csname R@an.robustness.kits.neg.L2.nullsd_hi\endcsname{11.73}
\expandafter\gdef\csname R@an.robustness.kits.neg.L2.nullsd_lo\endcsname{0.34}
\expandafter\gdef\csname R@an.robustness.kits.neg.L2.worst\endcsname{\ensuremath{-15.69}}
\expandafter\gdef\csname R@an.robustness.kits.neg.L3.defdice_hi\endcsname{58.55}
\expandafter\gdef\csname R@an.robustness.kits.neg.L3.defdice_lo\endcsname{48.15}
\expandafter\gdef\csname R@an.robustness.kits.neg.L3.maxcases\endcsname{9}
\expandafter\gdef\csname R@an.robustness.kits.neg.L3.n\endcsname{5}
\expandafter\gdef\csname R@an.robustness.kits.neg.L3.nmissing\endcsname{4}
\expandafter\gdef\csname R@an.robustness.kits.neg.L3.nrecorded\endcsname{1}
\expandafter\gdef\csname R@an.robustness.kits.neg.L3.nres_pairs\endcsname{4}
\expandafter\gdef\csname R@an.robustness.kits.neg.L3.nres_self\endcsname{1}
\expandafter\gdef\csname R@an.robustness.kits.neg.L3.nres_strata\endcsname{3}
\expandafter\gdef\csname R@an.robustness.kits.neg.L3.nullsd_hi\endcsname{11.73}
\expandafter\gdef\csname R@an.robustness.kits.neg.L3.nullsd_lo\endcsname{3.28}
\expandafter\gdef\csname R@an.robustness.kits.neg.L3.worst\endcsname{\ensuremath{-8.62}}
\expandafter\gdef\csname R@an.robustness.kits.neg.L4.defdice_hi\endcsname{58.55}
\expandafter\gdef\csname R@an.robustness.kits.neg.L4.defdice_lo\endcsname{48.15}
\expandafter\gdef\csname R@an.robustness.kits.neg.L4.maxcases\endcsname{7}
\expandafter\gdef\csname R@an.robustness.kits.neg.L4.n\endcsname{4}
\expandafter\gdef\csname R@an.robustness.kits.neg.L4.nmissing\endcsname{3}
\expandafter\gdef\csname R@an.robustness.kits.neg.L4.nrecorded\endcsname{1}
\expandafter\gdef\csname R@an.robustness.kits.neg.L4.nres_pairs\endcsname{3}
\expandafter\gdef\csname R@an.robustness.kits.neg.L4.nres_self\endcsname{0}
\expandafter\gdef\csname R@an.robustness.kits.neg.L4.nres_strata\endcsname{2}
\expandafter\gdef\csname R@an.robustness.kits.neg.L4.nullsd_hi\endcsname{11.73}
\expandafter\gdef\csname R@an.robustness.kits.neg.L4.nullsd_lo\endcsname{3.59}
\expandafter\gdef\csname R@an.robustness.kits.neg.L4.worst\endcsname{\ensuremath{-5.08}}
\expandafter\gdef\csname R@an.robustness.kits.neg.L6.defdice_hi\endcsname{51.26}
\expandafter\gdef\csname R@an.robustness.kits.neg.L6.defdice_lo\endcsname{51.26}
\expandafter\gdef\csname R@an.robustness.kits.neg.L6.maxcases\endcsname{3}
\expandafter\gdef\csname R@an.robustness.kits.neg.L6.n\endcsname{2}
\expandafter\gdef\csname R@an.robustness.kits.neg.L6.nmissing\endcsname{2}
\expandafter\gdef\csname R@an.robustness.kits.neg.L6.nrecorded\endcsname{0}
\expandafter\gdef\csname R@an.robustness.kits.neg.L6.nres_pairs\endcsname{0}
\expandafter\gdef\csname R@an.robustness.kits.neg.L6.nres_self\endcsname{0}
\expandafter\gdef\csname R@an.robustness.kits.neg.L6.nres_strata\endcsname{0}
\expandafter\gdef\csname R@an.robustness.kits.neg.L6.nullsd_hi\endcsname{11.73}
\expandafter\gdef\csname R@an.robustness.kits.neg.L6.nullsd_lo\endcsname{11.73}
\expandafter\gdef\csname R@an.robustness.kits.neg.L6.worst\endcsname{\ensuremath{-1.01}}
\expandafter\gdef\csname R@an.robustness.kits.nraw05\endcsname{1}
\expandafter\gdef\csname R@an.robustness.kits.nstrata\endcsname{22}
\expandafter\gdef\csname R@an.robustness.kits.nullsd\endcsname{0.97}
\expandafter\gdef\csname R@an.robustness.kits.oof.all.L1.d5\endcsname{\ensuremath{+3.07}}
\expandafter\gdef\csname R@an.robustness.kits.oof.all.L1.dcv\endcsname{\ensuremath{+2.57}}
\expandafter\gdef\csname R@an.robustness.kits.oof.all.L1.nposfolds\endcsname{4 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.all.L1.sdfold\endcsname{1.14}
\expandafter\gdef\csname R@an.robustness.kits.oof.all.L1.se\endcsname{0.57}
\expandafter\gdef\csname R@an.robustness.kits.oof.all.L3.d5\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.robustness.kits.oof.all.L3.dcv\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.robustness.kits.oof.all.L3.nposfolds\endcsname{2 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.all.L3.sdfold\endcsname{1.58}
\expandafter\gdef\csname R@an.robustness.kits.oof.all.L3.se\endcsname{0.79}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.high.L1.d5\endcsname{\ensuremath{+4.14}}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.high.L1.dcv\endcsname{\ensuremath{+3.80}}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.high.L1.nposfolds\endcsname{4 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.high.L1.sdfold\endcsname{1.59}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.high.L1.se\endcsname{0.79}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.high.L3.d5\endcsname{\ensuremath{+1.24}}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.high.L3.dcv\endcsname{\ensuremath{+1.30}}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.high.L3.nposfolds\endcsname{3 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.high.L3.sdfold\endcsname{1.98}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.high.L3.se\endcsname{0.99}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.high.defdice\endcsname{77.61}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.high.n\endcsname{154}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.low.L1.d5\endcsname{\ensuremath{+2.39}}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.low.L1.dcv\endcsname{\ensuremath{+1.81}}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.low.L1.nposfolds\endcsname{4 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.low.L1.sdfold\endcsname{1.25}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.low.L1.se\endcsname{0.63}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.low.L3.d5\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.low.L3.dcv\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.low.L3.nposfolds\endcsname{2 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.low.L3.sdfold\endcsname{2.29}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.low.L3.se\endcsname{1.15}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.low.defdice\endcsname{76.54}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.low.n\endcsname{236}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.unknown.L1.dcv\endcsname{\ensuremath{+5.15}}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.unknown.L1.nposfolds\endcsname{1 of 1}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.unknown.L3.dcv\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.unknown.L3.nposfolds\endcsname{1 of 1}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.unknown.defdice\endcsname{6.02}
\expandafter\gdef\csname R@an.robustness.kits.oof.bmi.unknown.n\endcsname{1}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.early.L1.d5\endcsname{\ensuremath{+4.57}}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.early.L1.dcv\endcsname{\ensuremath{+4.58}}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.early.L1.nposfolds\endcsname{4 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.early.L1.sdfold\endcsname{1.42}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.early.L1.se\endcsname{0.71}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.early.L3.d5\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.early.L3.dcv\endcsname{\ensuremath{+1.64}}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.early.L3.nposfolds\endcsname{3 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.early.L3.sdfold\endcsname{2.08}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.early.L3.se\endcsname{1.04}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.early.defdice\endcsname{79.58}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.early.n\endcsname{240}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.new.L1.d5\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.new.L1.dcv\endcsname{\ensuremath{-0.60}}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.new.L1.nposfolds\endcsname{1 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.new.L1.sdfold\endcsname{1.52}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.new.L1.se\endcsname{0.76}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.new.L3.d5\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.new.L3.dcv\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.new.L3.nposfolds\endcsname{2 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.new.L3.sdfold\endcsname{1.50}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.new.L3.se\endcsname{0.75}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.new.defdice\endcsname{72.54}
\expandafter\gdef\csname R@an.robustness.kits.oof.cohort.new.n\endcsname{151}
\expandafter\gdef\csname R@an.robustness.kits.oof.fold1.L1.d\endcsname{\ensuremath{+3.36}}
\expandafter\gdef\csname R@an.robustness.kits.oof.fold1.L3.d\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.robustness.kits.oof.fold2.L1.d\endcsname{\ensuremath{+3.35}}
\expandafter\gdef\csname R@an.robustness.kits.oof.fold2.L3.d\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.robustness.kits.oof.fold3.L1.d\endcsname{\ensuremath{+2.61}}
\expandafter\gdef\csname R@an.robustness.kits.oof.fold3.L3.d\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.robustness.kits.oof.fold4.L1.d\endcsname{\ensuremath{+0.94}}
\expandafter\gdef\csname R@an.robustness.kits.oof.fold4.L3.d\endcsname{\ensuremath{-0.80}}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.ccrcc.L1.d5\endcsname{\ensuremath{+4.03}}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.ccrcc.L1.dcv\endcsname{\ensuremath{+3.97}}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.ccrcc.L1.nposfolds\endcsname{4 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.ccrcc.L1.sdfold\endcsname{1.94}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.ccrcc.L1.se\endcsname{0.97}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.ccrcc.L3.d5\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.ccrcc.L3.dcv\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.ccrcc.L3.nposfolds\endcsname{3 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.ccrcc.L3.sdfold\endcsname{0.69}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.ccrcc.L3.se\endcsname{0.34}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.ccrcc.defdice\endcsname{79.12}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.ccrcc.n\endcsname{249}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.other.L1.d5\endcsname{\ensuremath{+1.17}}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.other.L1.dcv\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.other.L1.nposfolds\endcsname{2 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.other.L1.sdfold\endcsname{2.35}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.other.L1.se\endcsname{1.18}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.other.L3.d5\endcsname{\ensuremath{+1.53}}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.other.L3.dcv\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.other.L3.nposfolds\endcsname{2 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.other.L3.sdfold\endcsname{3.55}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.other.L3.se\endcsname{1.78}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.other.defdice\endcsname{74.03}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.other.n\endcsname{139}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.unknown.L1.d5\endcsname{\ensuremath{+7.31}}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.unknown.L1.dcv\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.unknown.L1.nposfolds\endcsname{1 of 2}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.unknown.L1.sdfold\endcsname{4.69}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.unknown.L1.se\endcsname{3.31}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.unknown.L3.d5\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.unknown.L3.dcv\endcsname{\ensuremath{+5.79}}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.unknown.L3.nposfolds\endcsname{2 of 2}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.unknown.L3.sdfold\endcsname{7.42}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.unknown.L3.se\endcsname{5.25}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.unknown.defdice\endcsname{40.41}
\expandafter\gdef\csname R@an.robustness.kits.oof.hist.unknown.n\endcsname{3}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.no.L1.d5\endcsname{\ensuremath{+3.43}}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.no.L1.dcv\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.no.L1.nposfolds\endcsname{2 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.no.L1.sdfold\endcsname{4.44}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.no.L1.se\endcsname{2.22}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.no.L3.d5\endcsname{\ensuremath{+3.09}}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.no.L3.dcv\endcsname{\ensuremath{+3.04}}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.no.L3.nposfolds\endcsname{2 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.no.L3.sdfold\endcsname{5.36}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.no.L3.se\endcsname{2.68}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.no.defdice\endcsname{76.03}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.no.n\endcsname{37}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.unknown.L1.d5\endcsname{\ensuremath{+6.45}}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.unknown.L1.dcv\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.unknown.L1.nposfolds\endcsname{1 of 2}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.unknown.L1.sdfold\endcsname{2.87}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.unknown.L1.se\endcsname{2.03}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.unknown.L3.d5\endcsname{\ensuremath{+0.90}}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.unknown.L3.dcv\endcsname{\ensuremath{+5.66}}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.unknown.L3.nposfolds\endcsname{2 of 2}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.unknown.L3.sdfold\endcsname{7.61}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.unknown.L3.se\endcsname{5.38}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.unknown.defdice\endcsname{38.91}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.unknown.n\endcsname{4}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.yes.L1.d5\endcsname{\ensuremath{+2.99}}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.yes.L1.dcv\endcsname{\ensuremath{+2.70}}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.yes.L1.nposfolds\endcsname{4 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.yes.L1.sdfold\endcsname{1.21}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.yes.L1.se\endcsname{0.60}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.yes.L3.d5\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.yes.L3.dcv\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.yes.L3.nposfolds\endcsname{3 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.yes.L3.sdfold\endcsname{1.09}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.yes.L3.se\endcsname{0.55}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.yes.defdice\endcsname{77.38}
\expandafter\gdef\csname R@an.robustness.kits.oof.malig.yes.n\endcsname{350}
\expandafter\gdef\csname R@an.robustness.kits.oof.n\endcsname{391}
\expandafter\gdef\csname R@an.robustness.kits.oof.n5\endcsname{489}
\expandafter\gdef\csname R@an.robustness.kits.oof.nfolds\endcsname{4}
\expandafter\gdef\csname R@an.robustness.kits.oof.npos.L1\endcsname{21}
\expandafter\gdef\csname R@an.robustness.kits.oof.npos.L3\endcsname{20}
\expandafter\gdef\csname R@an.robustness.kits.oof.nstrata\endcsname{24}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.other.L1.d5\endcsname{\ensuremath{-0.82}}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.other.L1.dcv\endcsname{\ensuremath{-2.89}}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.other.L1.nposfolds\endcsname{1 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.other.L1.sdfold\endcsname{3.65}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.other.L1.se\endcsname{1.82}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.other.L3.d5\endcsname{\ensuremath{-1.95}}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.other.L3.dcv\endcsname{\ensuremath{-1.57}}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.other.L3.nposfolds\endcsname{2 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.other.L3.sdfold\endcsname{4.54}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.other.L3.se\endcsname{2.27}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.other.defdice\endcsname{56.58}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.other.n\endcsname{30}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.partial.L1.d5\endcsname{\ensuremath{+5.01}}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.partial.L1.dcv\endcsname{\ensuremath{+4.89}}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.partial.L1.nposfolds\endcsname{4 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.partial.L1.sdfold\endcsname{1.92}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.partial.L1.se\endcsname{0.96}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.partial.L3.d5\endcsname{\ensuremath{+1.63}}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.partial.L3.dcv\endcsname{\ensuremath{+1.50}}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.partial.L3.nposfolds\endcsname{3 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.partial.L3.sdfold\endcsname{2.38}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.partial.L3.se\endcsname{1.19}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.partial.defdice\endcsname{74.45}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.partial.n\endcsname{211}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.radical.L1.d5\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.radical.L1.dcv\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.radical.L1.nposfolds\endcsname{3 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.radical.L1.sdfold\endcsname{1.63}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.radical.L1.se\endcsname{0.81}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.radical.L3.d5\endcsname{\ensuremath{+1.51}}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.radical.L3.dcv\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.radical.L3.nposfolds\endcsname{2 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.radical.L3.sdfold\endcsname{1.73}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.radical.L3.se\endcsname{0.87}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.radical.defdice\endcsname{83.85}
\expandafter\gdef\csname R@an.robustness.kits.oof.proc.radical.n\endcsname{150}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.female.L1.d5\endcsname{\ensuremath{+1.99}}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.female.L1.dcv\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.female.L1.nposfolds\endcsname{3 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.female.L1.sdfold\endcsname{1.82}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.female.L1.se\endcsname{0.91}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.female.L3.d5\endcsname{\ensuremath{+1.39}}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.female.L3.dcv\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.female.L3.nposfolds\endcsname{2 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.female.L3.sdfold\endcsname{0.93}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.female.L3.se\endcsname{0.47}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.female.defdice\endcsname{80.69}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.female.n\endcsname{141}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.male.L1.d5\endcsname{\ensuremath{+3.67}}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.male.L1.dcv\endcsname{\ensuremath{+3.39}}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.male.L1.nposfolds\endcsname{4 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.male.L1.sdfold\endcsname{1.89}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.male.L1.se\endcsname{0.94}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.male.L3.d5\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.male.L3.dcv\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.male.L3.nposfolds\endcsname{3 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.male.L3.sdfold\endcsname{2.67}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.male.L3.se\endcsname{1.33}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.male.defdice\endcsname{74.64}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.male.n\endcsname{249}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.other.L1.dcv\endcsname{\ensuremath{-1.03}}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.other.L1.nposfolds\endcsname{0 of 1}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.other.L3.dcv\endcsname{\ensuremath{+1.53}}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.other.L3.nposfolds\endcsname{1 of 1}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.other.defdice\endcsname{78.42}
\expandafter\gdef\csname R@an.robustness.kits.oof.sex.other.n\endcsname{1}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.gt4.L1.d5\endcsname{\ensuremath{+1.27}}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.gt4.L1.dcv\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.gt4.L1.nposfolds\endcsname{3 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.gt4.L1.sdfold\endcsname{1.72}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.gt4.L1.se\endcsname{0.86}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.gt4.L3.d5\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.gt4.L3.dcv\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.gt4.L3.nposfolds\endcsname{1 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.gt4.L3.sdfold\endcsname{0.55}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.gt4.L3.se\endcsname{0.28}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.gt4.defdice\endcsname{84.94}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.gt4.n\endcsname{197}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.le4.L1.d5\endcsname{\ensuremath{+4.80}}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.le4.L1.dcv\endcsname{\ensuremath{+4.33}}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.le4.L1.nposfolds\endcsname{4 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.le4.L1.sdfold\endcsname{1.63}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.le4.L1.se\endcsname{0.81}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.le4.L3.d5\endcsname{\ensuremath{+2.55}}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.le4.L3.dcv\endcsname{\ensuremath{+2.37}}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.le4.L3.nposfolds\endcsname{3 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.le4.L3.sdfold\endcsname{2.45}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.le4.L3.se\endcsname{1.22}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.le4.defdice\endcsname{69.15}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.le4.n\endcsname{178}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.unknown.L1.d5\endcsname{\ensuremath{+3.60}}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.unknown.L1.dcv\endcsname{\ensuremath{+2.35}}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.unknown.L1.nposfolds\endcsname{3 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.unknown.L1.sdfold\endcsname{2.58}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.unknown.L1.se\endcsname{1.29}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.unknown.L3.d5\endcsname{\ensuremath{-0.96}}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.unknown.L3.dcv\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.unknown.L3.nposfolds\endcsname{3 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.unknown.L3.sdfold\endcsname{6.48}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.unknown.L3.se\endcsname{3.24}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.unknown.defdice\endcsname{55.82}
\expandafter\gdef\csname R@an.robustness.kits.oof.size.unknown.n\endcsname{16}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.ge2.L1.d5\endcsname{\ensuremath{+1.94}}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.ge2.L1.dcv\endcsname{\ensuremath{+1.87}}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.ge2.L1.nposfolds\endcsname{4 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.ge2.L1.sdfold\endcsname{1.44}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.ge2.L1.se\endcsname{0.72}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.ge2.L3.d5\endcsname{\ensuremath{+0.89}}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.ge2.L3.dcv\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.ge2.L3.nposfolds\endcsname{2 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.ge2.L3.sdfold\endcsname{1.16}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.ge2.L3.se\endcsname{0.58}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.ge2.defdice\endcsname{82.08}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.ge2.n\endcsname{138}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.na.L1.d5\endcsname{\ensuremath{+3.87}}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.na.L1.dcv\endcsname{\ensuremath{+1.26}}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.na.L1.nposfolds\endcsname{2 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.na.L1.sdfold\endcsname{3.92}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.na.L1.se\endcsname{1.96}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.na.L3.d5\endcsname{\ensuremath{+2.14}}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.na.L3.dcv\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.na.L3.nposfolds\endcsname{2 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.na.L3.sdfold\endcsname{5.41}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.na.L3.se\endcsname{2.70}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.na.defdice\endcsname{71.35}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.na.n\endcsname{46}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1a.L1.d5\endcsname{\ensuremath{+4.52}}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1a.L1.dcv\endcsname{\ensuremath{+4.24}}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1a.L1.nposfolds\endcsname{4 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1a.L1.sdfold\endcsname{1.78}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1a.L1.se\endcsname{0.89}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1a.L3.d5\endcsname{\ensuremath{+1.94}}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1a.L3.dcv\endcsname{\ensuremath{+1.70}}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1a.L3.nposfolds\endcsname{3 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1a.L3.sdfold\endcsname{2.24}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1a.L3.se\endcsname{1.12}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1a.defdice\endcsname{71.25}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1a.n\endcsname{144}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1b.L1.d5\endcsname{\ensuremath{+1.34}}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1b.L1.dcv\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1b.L1.nposfolds\endcsname{3 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1b.L1.sdfold\endcsname{2.65}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1b.L1.se\endcsname{1.33}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1b.L3.d5\endcsname{\ensuremath{-1.40}}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1b.L3.dcv\endcsname{\ensuremath{-2.23}}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1b.L3.nposfolds\endcsname{2 of 4}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1b.L3.sdfold\endcsname{4.37}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1b.L3.se\endcsname{2.19}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1b.defdice\endcsname{82.35}
\expandafter\gdef\csname R@an.robustness.kits.oof.tstage.t1b.n\endcsname{63}
\expandafter\gdef\csname R@an.robustness.kits.pool\endcsname{83.38}
\expandafter\gdef\csname R@an.robustness.kits.pool_vs_pub\endcsname{\ensuremath{-2.87}}
\expandafter\gdef\csname R@an.robustness.kits.pooln\endcsname{3}
\expandafter\gdef\csname R@an.robustness.kits.poolnu\endcsname{2}
\expandafter\gdef\csname R@an.robustness.kits.poolsd\endcsname{0.79}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.L1.d0\endcsname{\ensuremath{-7.09}}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.L1.dfresh\endcsname{\ensuremath{+7.46}}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.L1.kidfresh\endcsname{\ensuremath{+2.04}}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.L1b.d0\endcsname{\ensuremath{+3.95}}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.L1b.dfresh\endcsname{\ensuremath{+3.27}}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.L1b.kidfresh\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.L2.d0\endcsname{\ensuremath{-2.13}}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.L2.dfresh\endcsname{\ensuremath{-7.06}}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.L2.kidfresh\endcsname{\ensuremath{-0.81}}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.L3.d0\endcsname{\ensuremath{-2.66}}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.L3.dfresh\endcsname{\ensuremath{-3.46}}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.L3.kidfresh\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.L4.d0\endcsname{\ensuremath{+4.49}}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.L4.dfresh\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.L4.kidfresh\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.L6.d0\endcsname{\ensuremath{+9.77}}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.L6.dfresh\endcsname{\ensuremath{+1.79}}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.L6.kidfresh\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.altref_shift\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.defdice\endcsname{48.15}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.kiddice\endcsname{94.18}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.n\endcsname{7}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.nullsd\endcsname{3.59}
\expandafter\gdef\csname R@an.robustness.kits.proc.other.nullsd0\endcsname{4.54}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.L1.d0\endcsname{\ensuremath{+3.33}}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.L1.dfresh\endcsname{\ensuremath{+5.48}}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.L1.kidfresh\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.L1b.d0\endcsname{\ensuremath{+2.99}}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.L1b.dfresh\endcsname{\ensuremath{+2.92}}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.L1b.kidfresh\endcsname{\ensuremath{+1.03}}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.L2.d0\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.L2.dfresh\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.L2.kidfresh\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.L3.d0\endcsname{\ensuremath{+4.44}}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.L3.dfresh\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.L3.kidfresh\endcsname{\ensuremath{+0.72}}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.L4.d0\endcsname{\ensuremath{+3.17}}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.L4.dfresh\endcsname{\ensuremath{+2.90}}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.L4.kidfresh\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.L6.d0\endcsname{\ensuremath{+3.35}}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.L6.dfresh\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.L6.kidfresh\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.altref_shift\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.defdice\endcsname{75.16}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.kiddice\endcsname{96.51}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.n\endcsname{64}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.nullsd\endcsname{1.06}
\expandafter\gdef\csname R@an.robustness.kits.proc.partial.nullsd0\endcsname{1.34}
\expandafter\gdef\csname R@an.robustness.kits.proc.phet\endcsname{0.255}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.L1.d0\endcsname{\ensuremath{+4.48}}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.L1.dfresh\endcsname{\ensuremath{+3.57}}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.L1.kidfresh\endcsname{\ensuremath{+1.56}}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.L1b.d0\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.L1b.dfresh\endcsname{\ensuremath{+2.41}}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.L1b.kidfresh\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.L2.d0\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.L2.dfresh\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.L2.kidfresh\endcsname{\ensuremath{-0.95}}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.L3.d0\endcsname{\ensuremath{+5.09}}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.L3.dfresh\endcsname{\ensuremath{+4.29}}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.L3.kidfresh\endcsname{\ensuremath{+1.70}}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.L4.d0\endcsname{\ensuremath{+4.02}}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.L4.dfresh\endcsname{\ensuremath{+4.78}}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.L4.kidfresh\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.L6.d0\endcsname{\ensuremath{+3.67}}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.L6.dfresh\endcsname{\ensuremath{+2.88}}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.L6.kidfresh\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.altref_shift\endcsname{\ensuremath{+2.02}}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.defdice\endcsname{78.95}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.kiddice\endcsname{95.33}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.n\endcsname{27}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.nullsd\endcsname{0.34}
\expandafter\gdef\csname R@an.robustness.kits.proc.radical.nullsd0\endcsname{0.43}
\expandafter\gdef\csname R@an.robustness.kits.pub_f0\endcsname{86.25}
\expandafter\gdef\csname R@an.robustness.kits.pub_f0.src\endcsname{arXiv:2404.09556v2 Appendix Tab. 2 (fetched 2026-10-05)}
\expandafter\gdef\csname R@an.robustness.kits.refctl.d0head\endcsname{\ensuremath{+2.64}}
\expandafter\gdef\csname R@an.robustness.kits.refctl.d0tum\endcsname{\ensuremath{+3.49}}
\expandafter\gdef\csname R@an.robustness.kits.refctl.name\endcsname{branch control}
\expandafter\gdef\csname R@an.robustness.kits.refctl.of\endcsname{z-dilation mixing}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.L1.d0\endcsname{\ensuremath{+5.22}}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.L1.dfresh\endcsname{\ensuremath{+5.56}}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.L1.kidfresh\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.L1b.d0\endcsname{\ensuremath{+2.16}}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.L1b.dfresh\endcsname{\ensuremath{+3.25}}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.L1b.kidfresh\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.L2.d0\endcsname{\ensuremath{+2.04}}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.L2.dfresh\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.L2.kidfresh\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.L3.d0\endcsname{\ensuremath{+5.73}}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.L3.dfresh\endcsname{\ensuremath{+5.26}}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.L3.kidfresh\endcsname{\ensuremath{+1.32}}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.L4.d0\endcsname{\ensuremath{+2.28}}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.L4.dfresh\endcsname{\ensuremath{+3.15}}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.L4.kidfresh\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.L6.d0\endcsname{\ensuremath{+4.57}}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.L6.dfresh\endcsname{\ensuremath{+3.06}}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.L6.kidfresh\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.altref_shift\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.defdice\endcsname{77.21}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.kiddice\endcsname{95.54}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.n\endcsname{41}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.nullsd\endcsname{0.84}
\expandafter\gdef\csname R@an.robustness.kits.sex.female.nullsd0\endcsname{1.06}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.L1.d0\endcsname{\ensuremath{+1.23}}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.L1.dfresh\endcsname{\ensuremath{+4.76}}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.L1.kidfresh\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.L1b.d0\endcsname{\ensuremath{+3.64}}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.L1b.dfresh\endcsname{\ensuremath{+2.48}}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.L1b.kidfresh\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.L2.d0\endcsname{\ensuremath{-1.01}}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.L2.dfresh\endcsname{\ensuremath{-1.86}}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.L2.kidfresh\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.L3.d0\endcsname{\ensuremath{+2.94}}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.L3.dfresh\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.L3.kidfresh\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.L4.d0\endcsname{\ensuremath{+4.38}}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.L4.dfresh\endcsname{\ensuremath{+3.14}}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.L4.kidfresh\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.L6.d0\endcsname{\ensuremath{+3.42}}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.L6.dfresh\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.L6.kidfresh\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.altref_shift\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.defdice\endcsname{72.16}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.kiddice\endcsname{96.37}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.n\endcsname{57}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.nullsd\endcsname{1.27}
\expandafter\gdef\csname R@an.robustness.kits.sex.male.nullsd0\endcsname{1.61}
\expandafter\gdef\csname R@an.robustness.kits.sex.phet\endcsname{0.024}
\expandafter\gdef\csname R@an.robustness.kits.shift.ndown\endcsname{3}
\expandafter\gdef\csname R@an.robustness.kits.shift.nup\endcsname{1}
\expandafter\gdef\csname R@an.robustness.kits.shift.span\endcsname{3.97}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.L1.d0\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.L1.dfresh\endcsname{\ensuremath{+2.40}}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.L1.kidfresh\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.L1b.d0\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.L1b.dfresh\endcsname{\ensuremath{+3.31}}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.L1b.kidfresh\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.L2.d0\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.L2.dfresh\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.L2.kidfresh\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.L3.d0\endcsname{\ensuremath{+3.44}}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.L3.dfresh\endcsname{\ensuremath{+2.37}}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.L3.kidfresh\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.L4.d0\endcsname{\ensuremath{+2.54}}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.L4.dfresh\endcsname{\ensuremath{+2.81}}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.L4.kidfresh\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.L6.d0\endcsname{\ensuremath{+1.47}}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.L6.dfresh\endcsname{\ensuremath{+1.86}}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.L6.kidfresh\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.altref_shift\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.defdice\endcsname{78.60}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.kiddice\endcsname{96.34}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.n\endcsname{39}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.nullsd\endcsname{0.37}
\expandafter\gdef\csname R@an.robustness.kits.size.gt4.nullsd0\endcsname{0.47}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.L1.d0\endcsname{\ensuremath{+4.65}}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.L1.dfresh\endcsname{\ensuremath{+6.72}}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.L1.kidfresh\endcsname{\ensuremath{+1.08}}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.L1b.d0\endcsname{\ensuremath{+3.97}}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.L1b.dfresh\endcsname{\ensuremath{+2.68}}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.L1b.kidfresh\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.L2.d0\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.L2.dfresh\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.L2.kidfresh\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.L3.d0\endcsname{\ensuremath{+5.31}}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.L3.dfresh\endcsname{\ensuremath{+3.27}}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.L3.kidfresh\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.L4.d0\endcsname{\ensuremath{+4.23}}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.L4.dfresh\endcsname{\ensuremath{+4.15}}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.L4.kidfresh\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.L6.d0\endcsname{\ensuremath{+4.98}}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.L6.dfresh\endcsname{\ensuremath{+2.95}}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.L6.kidfresh\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.altref_shift\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.defdice\endcsname{72.60}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.kiddice\endcsname{96.00}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.n\endcsname{54}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.nullsd\endcsname{1.64}
\expandafter\gdef\csname R@an.robustness.kits.size.le4.nullsd0\endcsname{2.08}
\expandafter\gdef\csname R@an.robustness.kits.size.phet\endcsname{0.109}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.L1.d0\endcsname{\ensuremath{-8.69}}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.L1.dfresh\endcsname{\ensuremath{+8.58}}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.L1.kidfresh\endcsname{\ensuremath{+2.65}}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.L1b.d0\endcsname{\ensuremath{-1.86}}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.L1b.dfresh\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.L1b.kidfresh\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.L2.d0\endcsname{\ensuremath{-4.99}}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.L2.dfresh\endcsname{\ensuremath{-12.38}}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.L2.kidfresh\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.L3.d0\endcsname{\ensuremath{-3.57}}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.L3.dfresh\endcsname{\ensuremath{-8.03}}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.L3.kidfresh\endcsname{\ensuremath{-0.67}}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.L4.d0\endcsname{\ensuremath{+3.13}}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.L4.dfresh\endcsname{\ensuremath{-5.08}}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.L4.kidfresh\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.L6.d0\endcsname{\ensuremath{+11.21}}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.L6.dfresh\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.L6.kidfresh\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.altref_shift\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.defdice\endcsname{58.55}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.kiddice\endcsname{93.77}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.n\endcsname{5}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.nullsd\endcsname{4.00}
\expandafter\gdef\csname R@an.robustness.kits.size.unknown.nullsd0\endcsname{5.06}
\expandafter\gdef\csname R@an.robustness.kits.size_vol_n\endcsname{93}
\expandafter\gdef\csname R@an.robustness.kits.size_vol_rho\endcsname{0.82}
\expandafter\gdef\csname R@an.robustness.kits.size_vol_rho.p\endcsname{\ensuremath{<}0.0001}
\expandafter\gdef\csname R@an.robustness.kits.sizevol.nagree\endcsname{85}
\expandafter\gdef\csname R@an.robustness.kits.sizevol.ndisagree\endcsname{8}
\expandafter\gdef\csname R@an.robustness.kits.tcrit\endcsname{4.30}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.L1.d0\endcsname{\ensuremath{+1.66}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.L1.dfresh\endcsname{\ensuremath{+2.23}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.L1.kidfresh\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.L1b.d0\endcsname{\ensuremath{+4.77}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.L1b.dfresh\endcsname{\ensuremath{+3.44}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.L1b.kidfresh\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.L2.d0\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.L2.dfresh\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.L2.kidfresh\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.L3.d0\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.L3.dfresh\endcsname{\ensuremath{+2.91}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.L3.kidfresh\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.L4.d0\endcsname{\ensuremath{+4.86}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.L4.dfresh\endcsname{\ensuremath{+4.30}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.L4.kidfresh\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.L6.d0\endcsname{\ensuremath{+2.03}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.L6.dfresh\endcsname{\ensuremath{+1.67}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.L6.kidfresh\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.altref_shift\endcsname{\ensuremath{+1.67}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.defdice\endcsname{78.61}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.kiddice\endcsname{95.48}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.n\endcsname{18}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.nullsd\endcsname{0.61}
\expandafter\gdef\csname R@an.robustness.kits.tstage.ge2.nullsd0\endcsname{0.77}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.L1.d0\endcsname{\ensuremath{+6.66}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.L1.dfresh\endcsname{\ensuremath{+14.32}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.L1.kidfresh\endcsname{\ensuremath{+3.82}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.L1b.d0\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.L1b.dfresh\endcsname{\ensuremath{+4.73}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.L1b.kidfresh\endcsname{\ensuremath{+3.43}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.L2.d0\endcsname{\ensuremath{-7.27}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.L2.dfresh\endcsname{\ensuremath{-2.13}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.L2.kidfresh\endcsname{\ensuremath{+1.66}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.L3.d0\endcsname{\ensuremath{+3.22}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.L3.dfresh\endcsname{\ensuremath{-0.67}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.L3.kidfresh\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.L4.d0\endcsname{\ensuremath{+7.15}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.L4.dfresh\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.L4.kidfresh\endcsname{\ensuremath{+2.78}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.L6.d0\endcsname{\ensuremath{+7.85}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.L6.dfresh\endcsname{\ensuremath{+4.26}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.L6.kidfresh\endcsname{\ensuremath{+1.60}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.altref_shift\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.defdice\endcsname{56.09}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.kiddice\endcsname{91.44}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.n\endcsname{9}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.nullsd\endcsname{3.28}
\expandafter\gdef\csname R@an.robustness.kits.tstage.na.nullsd0\endcsname{4.15}
\expandafter\gdef\csname R@an.robustness.kits.tstage.phet\endcsname{0.829}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.L1.d0\endcsname{\ensuremath{+3.03}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.L1.dfresh\endcsname{\ensuremath{+5.65}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.L1.kidfresh\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.L1b.d0\endcsname{\ensuremath{+4.17}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.L1b.dfresh\endcsname{\ensuremath{+2.09}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.L1b.kidfresh\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.L2.d0\endcsname{\ensuremath{+1.62}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.L2.dfresh\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.L2.kidfresh\endcsname{\ensuremath{-0.85}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.L3.d0\endcsname{\ensuremath{+4.86}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.L3.dfresh\endcsname{\ensuremath{+2.88}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.L3.kidfresh\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.L4.d0\endcsname{\ensuremath{+3.67}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.L4.dfresh\endcsname{\ensuremath{+3.53}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.L4.kidfresh\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.L6.d0\endcsname{\ensuremath{+5.20}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.L6.dfresh\endcsname{\ensuremath{+2.57}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.L6.kidfresh\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.altref_shift\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.defdice\endcsname{73.97}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.kiddice\endcsname{96.59}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.n\endcsname{49}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.nullsd\endcsname{1.60}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1a.nullsd0\endcsname{2.03}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.L1.d0\endcsname{\ensuremath{+2.10}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.L1.dfresh\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.L1.kidfresh\endcsname{\ensuremath{+0.72}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.L1b.d0\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.L1b.dfresh\endcsname{\ensuremath{+3.08}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.L1b.kidfresh\endcsname{\ensuremath{+0.73}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.L2.d0\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.L2.dfresh\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.L2.kidfresh\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.L3.d0\endcsname{\ensuremath{+4.61}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.L3.dfresh\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.L3.kidfresh\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.L4.d0\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.L4.dfresh\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.L4.kidfresh\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.L6.d0\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.L6.dfresh\endcsname{\ensuremath{+1.93}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.L6.kidfresh\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.altref_shift\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.defdice\endcsname{78.84}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.kiddice\endcsname{97.06}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.n\endcsname{22}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.nullsd\endcsname{1.07}
\expandafter\gdef\csname R@an.robustness.kits.tstage.t1b.nullsd0\endcsname{1.36}
\expandafter\gdef\csname R@an.robustness.kits.volcut.hi\endcsname{44.67}
\expandafter\gdef\csname R@an.robustness.kits.volcut.lo\endcsname{9.88}
\expandafter\gdef\csname R@an.robustness.kits.widest_factor\endcsname{Sex}
\expandafter\gdef\csname R@an.robustness.kits.widest_spread\endcsname{5.02}
\expandafter\gdef\csname R@an.robustness.status.amos\endcsname{pinned}
\expandafter\gdef\csname R@an.robustness.status.amos_altref\endcsname{contemporaneous default runs available (3 of 3)}
\expandafter\gdef\csname R@an.robustness.status.amos_fresh\endcsname{10 fresh AMOS22 seeds finished; 5 of 6 figure arms report a fresh mean and the rest the discovery seed 0}
\expandafter\gdef\csname R@an.robustness.status.amos_mixed\endcsname{the AMOS22 rows are not on one estimand — HyReX, ResEnc-M, ResEnc-matched, ResEnc+context and ConvNeXt-k3 report a two-seed fresh mean and the other 1 the discovery seed 0 — so each row is read against the band of its own estimand and no arm-vs-arm ordering may be read off these panels}
\expandafter\gdef\csname R@an.robustness.status.kits_altref\endcsname{contemporaneous default runs available (3 of 3)}
\expandafter\gdef\csname R@an.robustness.status.kits_oof\endcsname{12 of 12 runs finished; 489 cases over 5 folds}
\expandafter\gdef\csname R@an.round4_followup.d2.amos.base_step\endcsname{100.7}
\expandafter\gdef\csname R@an.round4_followup.d2.amos.batch\endcsname{2}
\expandafter\gdef\csname R@an.round4_followup.d2.amos.device\endcsname{NVIDIA A100-SXM4-80GB}
\expandafter\gdef\csname R@an.round4_followup.d2.amos.gate\endcsname{95.7}
\expandafter\gdef\csname R@an.round4_followup.d2.amos.patch\endcsname{$64\!\times\!192\!\times\!160$}
\expandafter\gdef\csname R@an.round4_followup.d2.amos.reduction\endcsname{16.087}
\expandafter\gdef\csname R@an.round4_followup.d2.amos.step\endcsname{84.5}
\expandafter\gdef\csname R@an.round4_followup.d2.amos.torch\endcsname{2.13.0+cu130}
\expandafter\gdef\csname R@an.round4_followup.w5.amos.aggregate\endcsname{+0.453}
\expandafter\gdef\csname R@an.round4_followup.w5.amos.imp4\endcsname{+0.523}
\expandafter\gdef\csname R@an.round4_followup.w5.amos.pair_floor\endcsname{0.50}
\expandafter\gdef\csname R@an.round4_followup.w5.amos.prediction_thr\endcsname{0.67}
\expandafter\gdef\csname R@an.round4_followup.w5.amos.queue_thr\endcsname{0.40}
\expandafter\gdef\csname R@an.round4_followup.w5.amos.seed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arch.arch_fixed.b_done\endcsname{2}
\expandafter\gdef\csname R@an.stage1.arch.arch_fixed.b_pending\endcsname{14}
\expandafter\gdef\csname R@an.stage1.arch.arch_fixed.best\endcsname{\ensuremath{+1.60}}
\expandafter\gdef\csname R@an.stage1.arch.arch_fixed.best_b\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.stage1.arch.arch_fixed.conf\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arch.arch_fixed.n\endcsname{36}
\expandafter\gdef\csname R@an.stage1.arch.arch_fixed.priv\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arch.arch_fixed.promoted\endcsname{16}
\expandafter\gdef\csname R@an.stage1.arch.arch_fixed.scored\endcsname{33}
\expandafter\gdef\csname R@an.stage1.arch.arch_fixed.smoke_failed\endcsname{3}
\expandafter\gdef\csname R@an.stage1.arch.arch_fixed.trial_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arch.arch_rsi.b_done\endcsname{4}
\expandafter\gdef\csname R@an.stage1.arch.arch_rsi.b_pending\endcsname{14}
\expandafter\gdef\csname R@an.stage1.arch.arch_rsi.best\endcsname{\ensuremath{+2.80}}
\expandafter\gdef\csname R@an.stage1.arch.arch_rsi.best_b\endcsname{\ensuremath{+1.42}}
\expandafter\gdef\csname R@an.stage1.arch.arch_rsi.conf\endcsname{1}
\expandafter\gdef\csname R@an.stage1.arch.arch_rsi.n\endcsname{36}
\expandafter\gdef\csname R@an.stage1.arch.arch_rsi.priv\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arch.arch_rsi.promoted\endcsname{18}
\expandafter\gdef\csname R@an.stage1.arch.arch_rsi.scored\endcsname{35}
\expandafter\gdef\csname R@an.stage1.arch.arch_rsi.smoke_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arch.arch_rsi.trial_failed\endcsname{1}
\expandafter\gdef\csname R@an.stage1.arch.b_done\endcsname{6}
\expandafter\gdef\csname R@an.stage1.arch.b_pending\endcsname{28}
\expandafter\gdef\csname R@an.stage1.arch.conf\endcsname{1}
\expandafter\gdef\csname R@an.stage1.arch.conf.acdc\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.stage1.arch.conf.amos\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.stage1.arch.conf.arm\endcsname{Arch-RSI}
\expandafter\gdef\csname R@an.stage1.arch.conf.name\endcsname{\texttt{phase\_complete\_encoder\_reduction}}
\expandafter\gdef\csname R@an.stage1.arch.n\endcsname{72}
\expandafter\gdef\csname R@an.stage1.arch.promoted\endcsname{34}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.best_conf\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.best_priv\endcsname{none}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.best_score\endcsname{1.60}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.calls\endcsname{9}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.calls_design\endcsname{9}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.calls_meta\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.conf\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.conf_own\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.confirming\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.confirming_list\endcsname{none}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.copies_h\endcsname{0.0}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.copies_n\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.gens\endcsname{9}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.gens_own\endcsname{9}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.gpuh\endcsname{153.9}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.gpuh_cum\endcsname{153.9}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.gpuh_fin\endcsname{146.9}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.gpuh_stop\endcsname{7.0}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.improver\endcsname{v0}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.n\endcsname{36}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.n_inh\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.n_own\endcsname{36}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.n_priv\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.name\endcsname{Arch-fixed}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.parconf\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.scored\endcsname{33}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.scored_own\endcsname{33}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.smoke_failed\endcsname{3}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.stop_n\endcsname{2}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.tok_completion\endcsname{135416}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.tok_completion_k\endcsname{135}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.tok_completion_m\endcsname{0.14}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.tok_prompt\endcsname{185537}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.tok_prompt_k\endcsname{186}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.tok_prompt_m\endcsname{0.19}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.track\endcsname{architecture}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.trial_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.arch_fixed.versions\endcsname{1}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.best_conf\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.best_priv\endcsname{none}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.best_score\endcsname{2.80}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.calls\endcsname{24}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.calls_design\endcsname{22}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.calls_meta\endcsname{2}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.conf\endcsname{1}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.conf_own\endcsname{1}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.confirming\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.confirming_list\endcsname{none}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.copies_h\endcsname{0.0}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.copies_n\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.gens\endcsname{9}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.gens_own\endcsname{9}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.gpuh\endcsname{169.6}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.gpuh_cum\endcsname{169.6}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.gpuh_fin\endcsname{163.5}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.gpuh_stop\endcsname{6.1}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.improver\endcsname{v2}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.n\endcsname{36}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.n_inh\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.n_own\endcsname{36}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.n_priv\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.name\endcsname{Arch-RSI}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.parconf\endcsname{3}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.scored\endcsname{35}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.scored_own\endcsname{35}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.smoke_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.stop_n\endcsname{2}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.tok_completion\endcsname{321603}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.tok_completion_k\endcsname{322}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.tok_completion_m\endcsname{0.32}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.tok_prompt\endcsname{876086}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.tok_prompt_k\endcsname{876}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.tok_prompt_m\endcsname{0.88}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.track\endcsname{architecture}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.trial_failed\endcsname{1}
\expandafter\gdef\csname R@an.stage1.arm.arch_rsi.versions\endcsname{3}
\expandafter\gdef\csname R@an.stage1.arm.crsi.best_conf\endcsname{\ensuremath{+2.28}}
\expandafter\gdef\csname R@an.stage1.arm.crsi.best_priv\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.stage1.arm.crsi.best_score\endcsname{6.24}
\expandafter\gdef\csname R@an.stage1.arm.crsi.calls\endcsname{29}
\expandafter\gdef\csname R@an.stage1.arm.crsi.calls_design\endcsname{26}
\expandafter\gdef\csname R@an.stage1.arm.crsi.calls_meta\endcsname{3}
\expandafter\gdef\csname R@an.stage1.arm.crsi.conf\endcsname{39}
\expandafter\gdef\csname R@an.stage1.arm.crsi.conf_own\endcsname{26}
\expandafter\gdef\csname R@an.stage1.arm.crsi.confirming\endcsname{4}
\expandafter\gdef\csname R@an.stage1.arm.crsi.confirming_list\endcsname{g012\_1, g012\_3, g014\_3, g015\_3}
\expandafter\gdef\csname R@an.stage1.arm.crsi.copies_h\endcsname{0.0}
\expandafter\gdef\csname R@an.stage1.arm.crsi.copies_n\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.crsi.gens\endcsname{18}
\expandafter\gdef\csname R@an.stage1.arm.crsi.gens_own\endcsname{9}
\expandafter\gdef\csname R@an.stage1.arm.crsi.gpuh\endcsname{285.6}
\expandafter\gdef\csname R@an.stage1.arm.crsi.gpuh_cum\endcsname{526.6}
\expandafter\gdef\csname R@an.stage1.arm.crsi.gpuh_fin\endcsname{279.1}
\expandafter\gdef\csname R@an.stage1.arm.crsi.gpuh_inh\endcsname{241.0}
\expandafter\gdef\csname R@an.stage1.arm.crsi.gpuh_stop\endcsname{6.5}
\expandafter\gdef\csname R@an.stage1.arm.crsi.improver\endcsname{v5}
\expandafter\gdef\csname R@an.stage1.arm.crsi.n\endcsname{72}
\expandafter\gdef\csname R@an.stage1.arm.crsi.n_inh\endcsname{33}
\expandafter\gdef\csname R@an.stage1.arm.crsi.n_own\endcsname{39}
\expandafter\gdef\csname R@an.stage1.arm.crsi.n_priv\endcsname{6}
\expandafter\gdef\csname R@an.stage1.arm.crsi.name\endcsname{RSI fork}
\expandafter\gdef\csname R@an.stage1.arm.crsi.parconf\endcsname{100}
\expandafter\gdef\csname R@an.stage1.arm.crsi.scored\endcsname{66}
\expandafter\gdef\csname R@an.stage1.arm.crsi.scored_own\endcsname{34}
\expandafter\gdef\csname R@an.stage1.arm.crsi.smoke_failed\endcsname{2}
\expandafter\gdef\csname R@an.stage1.arm.crsi.stop_n\endcsname{10}
\expandafter\gdef\csname R@an.stage1.arm.crsi.tok_completion\endcsname{372181}
\expandafter\gdef\csname R@an.stage1.arm.crsi.tok_completion_k\endcsname{372}
\expandafter\gdef\csname R@an.stage1.arm.crsi.tok_completion_m\endcsname{0.37}
\expandafter\gdef\csname R@an.stage1.arm.crsi.tok_prompt\endcsname{1582245}
\expandafter\gdef\csname R@an.stage1.arm.crsi.tok_prompt_k\endcsname{1582}
\expandafter\gdef\csname R@an.stage1.arm.crsi.tok_prompt_m\endcsname{1.58}
\expandafter\gdef\csname R@an.stage1.arm.crsi.track\endcsname{recipe}
\expandafter\gdef\csname R@an.stage1.arm.crsi.trial_failed\endcsname{3}
\expandafter\gdef\csname R@an.stage1.arm.crsi.versions\endcsname{6}
\expandafter\gdef\csname R@an.stage1.arm.fixed.best_conf\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.stage1.arm.fixed.best_priv\endcsname{\ensuremath{+1.82}}
\expandafter\gdef\csname R@an.stage1.arm.fixed.best_score\endcsname{5.73}
\expandafter\gdef\csname R@an.stage1.arm.fixed.calls\endcsname{18}
\expandafter\gdef\csname R@an.stage1.arm.fixed.calls_design\endcsname{18}
\expandafter\gdef\csname R@an.stage1.arm.fixed.calls_meta\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.fixed.conf\endcsname{23}
\expandafter\gdef\csname R@an.stage1.arm.fixed.conf_own\endcsname{23}
\expandafter\gdef\csname R@an.stage1.arm.fixed.confirming\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.fixed.confirming_list\endcsname{none}
\expandafter\gdef\csname R@an.stage1.arm.fixed.copies_h\endcsname{2.8}
\expandafter\gdef\csname R@an.stage1.arm.fixed.copies_n\endcsname{4}
\expandafter\gdef\csname R@an.stage1.arm.fixed.gens\endcsname{18}
\expandafter\gdef\csname R@an.stage1.arm.fixed.gens_own\endcsname{18}
\expandafter\gdef\csname R@an.stage1.arm.fixed.gpuh\endcsname{479.6}
\expandafter\gdef\csname R@an.stage1.arm.fixed.gpuh_cum\endcsname{479.6}
\expandafter\gdef\csname R@an.stage1.arm.fixed.gpuh_fin\endcsname{479.6}
\expandafter\gdef\csname R@an.stage1.arm.fixed.gpuh_stop\endcsname{0.0}
\expandafter\gdef\csname R@an.stage1.arm.fixed.improver\endcsname{v0}
\expandafter\gdef\csname R@an.stage1.arm.fixed.n\endcsname{70}
\expandafter\gdef\csname R@an.stage1.arm.fixed.n_inh\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.fixed.n_own\endcsname{70}
\expandafter\gdef\csname R@an.stage1.arm.fixed.n_priv\endcsname{12}
\expandafter\gdef\csname R@an.stage1.arm.fixed.name\endcsname{Fixed}
\expandafter\gdef\csname R@an.stage1.arm.fixed.parconf\endcsname{33}
\expandafter\gdef\csname R@an.stage1.arm.fixed.scored\endcsname{68}
\expandafter\gdef\csname R@an.stage1.arm.fixed.scored_own\endcsname{68}
\expandafter\gdef\csname R@an.stage1.arm.fixed.smoke_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.fixed.stop_n\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.fixed.tok_completion\endcsname{243741}
\expandafter\gdef\csname R@an.stage1.arm.fixed.tok_completion_k\endcsname{244}
\expandafter\gdef\csname R@an.stage1.arm.fixed.tok_completion_m\endcsname{0.24}
\expandafter\gdef\csname R@an.stage1.arm.fixed.tok_prompt\endcsname{331381}
\expandafter\gdef\csname R@an.stage1.arm.fixed.tok_prompt_k\endcsname{331}
\expandafter\gdef\csname R@an.stage1.arm.fixed.tok_prompt_m\endcsname{0.33}
\expandafter\gdef\csname R@an.stage1.arm.fixed.track\endcsname{recipe}
\expandafter\gdef\csname R@an.stage1.arm.fixed.trial_failed\endcsname{2}
\expandafter\gdef\csname R@an.stage1.arm.fixed.versions\endcsname{1}
\expandafter\gdef\csname R@an.stage1.arm.rsi.best_conf\endcsname{\ensuremath{+1.81}}
\expandafter\gdef\csname R@an.stage1.arm.rsi.best_priv\endcsname{\ensuremath{+1.53}}
\expandafter\gdef\csname R@an.stage1.arm.rsi.best_score\endcsname{6.15}
\expandafter\gdef\csname R@an.stage1.arm.rsi.calls\endcsname{54}
\expandafter\gdef\csname R@an.stage1.arm.rsi.calls_design\endcsname{49}
\expandafter\gdef\csname R@an.stage1.arm.rsi.calls_meta\endcsname{5}
\expandafter\gdef\csname R@an.stage1.arm.rsi.conf\endcsname{26}
\expandafter\gdef\csname R@an.stage1.arm.rsi.conf_own\endcsname{26}
\expandafter\gdef\csname R@an.stage1.arm.rsi.confirming\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.rsi.confirming_list\endcsname{none}
\expandafter\gdef\csname R@an.stage1.arm.rsi.copies_h\endcsname{0.0}
\expandafter\gdef\csname R@an.stage1.arm.rsi.copies_n\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.rsi.gens\endcsname{18}
\expandafter\gdef\csname R@an.stage1.arm.rsi.gens_own\endcsname{18}
\expandafter\gdef\csname R@an.stage1.arm.rsi.gpuh\endcsname{408.8}
\expandafter\gdef\csname R@an.stage1.arm.rsi.gpuh_cum\endcsname{408.8}
\expandafter\gdef\csname R@an.stage1.arm.rsi.gpuh_fin\endcsname{408.8}
\expandafter\gdef\csname R@an.stage1.arm.rsi.gpuh_stop\endcsname{0.0}
\expandafter\gdef\csname R@an.stage1.arm.rsi.improver\endcsname{v5}
\expandafter\gdef\csname R@an.stage1.arm.rsi.n\endcsname{49}
\expandafter\gdef\csname R@an.stage1.arm.rsi.n_inh\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.rsi.n_own\endcsname{49}
\expandafter\gdef\csname R@an.stage1.arm.rsi.n_priv\endcsname{12}
\expandafter\gdef\csname R@an.stage1.arm.rsi.name\endcsname{RSI}
\expandafter\gdef\csname R@an.stage1.arm.rsi.parconf\endcsname{59}
\expandafter\gdef\csname R@an.stage1.arm.rsi.scored\endcsname{48}
\expandafter\gdef\csname R@an.stage1.arm.rsi.scored_own\endcsname{48}
\expandafter\gdef\csname R@an.stage1.arm.rsi.smoke_failed\endcsname{1}
\expandafter\gdef\csname R@an.stage1.arm.rsi.stop_n\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.rsi.tok_completion\endcsname{466002}
\expandafter\gdef\csname R@an.stage1.arm.rsi.tok_completion_k\endcsname{466}
\expandafter\gdef\csname R@an.stage1.arm.rsi.tok_completion_m\endcsname{0.47}
\expandafter\gdef\csname R@an.stage1.arm.rsi.tok_prompt\endcsname{2311538}
\expandafter\gdef\csname R@an.stage1.arm.rsi.tok_prompt_k\endcsname{2312}
\expandafter\gdef\csname R@an.stage1.arm.rsi.tok_prompt_m\endcsname{2.31}
\expandafter\gdef\csname R@an.stage1.arm.rsi.track\endcsname{recipe}
\expandafter\gdef\csname R@an.stage1.arm.rsi.trial_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.arm.rsi.versions\endcsname{6}
\expandafter\gdef\csname R@an.stage1.base.crsi.conf\endcsname{0}
\expandafter\gdef\csname R@an.stage1.base.crsi.last_block\endcsname{none}
\expandafter\gdef\csname R@an.stage1.base.crsi.med\endcsname{none}
\expandafter\gdef\csname R@an.stage1.base.crsi.n\endcsname{0}
\expandafter\gdef\csname R@an.stage1.base.crsi.scored\endcsname{0}
\expandafter\gdef\csname R@an.stage1.base.crsi.z1pct\endcsname{none}
\expandafter\gdef\csname R@an.stage1.base.fixed.conf\endcsname{1}
\expandafter\gdef\csname R@an.stage1.base.fixed.last_block\endcsname{5}
\expandafter\gdef\csname R@an.stage1.base.fixed.med\endcsname{-0.09}
\expandafter\gdef\csname R@an.stage1.base.fixed.n\endcsname{37}
\expandafter\gdef\csname R@an.stage1.base.fixed.scored\endcsname{36}
\expandafter\gdef\csname R@an.stage1.base.fixed.z1pct\endcsname{11}
\expandafter\gdef\csname R@an.stage1.base.late.crsi.k\endcsname{0}
\expandafter\gdef\csname R@an.stage1.base.late.crsi.n\endcsname{39}
\expandafter\gdef\csname R@an.stage1.base.late.fixed.k\endcsname{23}
\expandafter\gdef\csname R@an.stage1.base.late.fixed.n\endcsname{48}
\expandafter\gdef\csname R@an.stage1.base.late.rsi.k\endcsname{0}
\expandafter\gdef\csname R@an.stage1.base.late.rsi.n\endcsname{28}
\expandafter\gdef\csname R@an.stage1.base.matched.crsi.conf\endcsname{0}
\expandafter\gdef\csname R@an.stage1.base.matched.crsi.med\endcsname{none}
\expandafter\gdef\csname R@an.stage1.base.matched.crsi.n\endcsname{0}
\expandafter\gdef\csname R@an.stage1.base.matched.crsi.scored\endcsname{0}
\expandafter\gdef\csname R@an.stage1.base.matched.crsi.z1\endcsname{0}
\expandafter\gdef\csname R@an.stage1.base.matched.fixed.conf\endcsname{1}
\expandafter\gdef\csname R@an.stage1.base.matched.fixed.med\endcsname{0.23}
\expandafter\gdef\csname R@an.stage1.base.matched.fixed.n\endcsname{14}
\expandafter\gdef\csname R@an.stage1.base.matched.fixed.scored\endcsname{14}
\expandafter\gdef\csname R@an.stage1.base.matched.fixed.z1\endcsname{2}
\expandafter\gdef\csname R@an.stage1.base.matched.rsi.conf\endcsname{2}
\expandafter\gdef\csname R@an.stage1.base.matched.rsi.med\endcsname{0.17}
\expandafter\gdef\csname R@an.stage1.base.matched.rsi.n\endcsname{17}
\expandafter\gdef\csname R@an.stage1.base.matched.rsi.scored\endcsname{16}
\expandafter\gdef\csname R@an.stage1.base.matched.rsi.z1\endcsname{5}
\expandafter\gdef\csname R@an.stage1.base.rsi.conf\endcsname{2}
\expandafter\gdef\csname R@an.stage1.base.rsi.last_block\endcsname{1}
\expandafter\gdef\csname R@an.stage1.base.rsi.med\endcsname{0.17}
\expandafter\gdef\csname R@an.stage1.base.rsi.n\endcsname{17}
\expandafter\gdef\csname R@an.stage1.base.rsi.scored\endcsname{16}
\expandafter\gdef\csname R@an.stage1.base.rsi.z1pct\endcsname{31}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.0.best\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.0.conf\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.0.gens\endcsname{1--3}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.0.improver\endcsname{v0}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.0.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.0.mean\endcsname{\ensuremath{-0.82}}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.0.median\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.0.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.0.parconf\endcsname{0.00}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.0.parconfpct\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.0.parin\endcsname{0.17}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.0.parinpct\endcsname{17}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.0.priv\endcsname{none}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.0.scored\endcsname{9}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.0.z1\endcsname{0.00}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.0.z1pct\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.1.best\endcsname{\ensuremath{+1.60}}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.1.conf\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.1.gens\endcsname{4--6}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.1.improver\endcsname{v0}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.1.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.1.mean\endcsname{\ensuremath{-1.12}}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.1.median\endcsname{\ensuremath{-0.74}}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.1.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.1.parconf\endcsname{0.00}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.1.parconfpct\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.1.parin\endcsname{0.50}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.1.parinpct\endcsname{50}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.1.priv\endcsname{none}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.1.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.1.z1\endcsname{0.08}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.1.z1pct\endcsname{8}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.2.best\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.2.conf\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.2.gens\endcsname{7--9}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.2.improver\endcsname{v0}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.2.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.2.mean\endcsname{\ensuremath{-5.35}}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.2.median\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.2.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.2.parconf\endcsname{0.00}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.2.parconfpct\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.2.parin\endcsname{0.50}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.2.parinpct\endcsname{50}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.2.priv\endcsname{none}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.2.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.2.z1\endcsname{0.08}
\expandafter\gdef\csname R@an.stage1.blk.arch_fixed.2.z1pct\endcsname{8}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.0.best\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.0.conf\endcsname{1}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.0.gens\endcsname{1--3}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.0.improver\endcsname{v0}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.0.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.0.mean\endcsname{\ensuremath{-0.70}}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.0.median\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.0.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.0.parconf\endcsname{0.00}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.0.parconfpct\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.0.parin\endcsname{0.00}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.0.parinpct\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.0.priv\endcsname{none}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.0.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.0.z1\endcsname{0.25}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.0.z1pct\endcsname{25}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.1.best\endcsname{\ensuremath{+2.80}}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.1.conf\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.1.gens\endcsname{4--6}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.1.improver\endcsname{v1}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.1.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.1.mean\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.1.median\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.1.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.1.parconf\endcsname{0.08}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.1.parconfpct\endcsname{8}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.1.parin\endcsname{0.08}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.1.parinpct\endcsname{8}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.1.priv\endcsname{none}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.1.scored\endcsname{11}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.1.z1\endcsname{0.27}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.1.z1pct\endcsname{27}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.2.best\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.2.conf\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.2.gens\endcsname{7--9}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.2.improver\endcsname{v2}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.2.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.2.mean\endcsname{\ensuremath{-1.48}}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.2.median\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.2.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.2.parconf\endcsname{0.00}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.2.parconfpct\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.2.parin\endcsname{0.00}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.2.parinpct\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.2.priv\endcsname{none}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.2.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.2.z1\endcsname{0.08}
\expandafter\gdef\csname R@an.stage1.blk.arch_rsi.2.z1pct\endcsname{8}
\expandafter\gdef\csname R@an.stage1.blk.crsi.0.best\endcsname{\ensuremath{+1.91}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.0.conf\endcsname{1}
\expandafter\gdef\csname R@an.stage1.blk.crsi.0.gens\endcsname{1--3}
\expandafter\gdef\csname R@an.stage1.blk.crsi.0.improver\endcsname{v0}
\expandafter\gdef\csname R@an.stage1.blk.crsi.0.inherited\endcsname{yes}
\expandafter\gdef\csname R@an.stage1.blk.crsi.0.mean\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.0.median\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.0.n\endcsname{9}
\expandafter\gdef\csname R@an.stage1.blk.crsi.0.parconf\endcsname{0.00}
\expandafter\gdef\csname R@an.stage1.blk.crsi.0.parconfpct\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.crsi.0.parin\endcsname{0.00}
\expandafter\gdef\csname R@an.stage1.blk.crsi.0.parinpct\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.crsi.0.priv\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.0.scored\endcsname{8}
\expandafter\gdef\csname R@an.stage1.blk.crsi.0.z1\endcsname{0.38}
\expandafter\gdef\csname R@an.stage1.blk.crsi.0.z1pct\endcsname{38}
\expandafter\gdef\csname R@an.stage1.blk.crsi.1.best\endcsname{\ensuremath{+2.46}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.1.conf\endcsname{4}
\expandafter\gdef\csname R@an.stage1.blk.crsi.1.gens\endcsname{4--6}
\expandafter\gdef\csname R@an.stage1.blk.crsi.1.improver\endcsname{v1}
\expandafter\gdef\csname R@an.stage1.blk.crsi.1.inherited\endcsname{yes}
\expandafter\gdef\csname R@an.stage1.blk.crsi.1.mean\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.1.median\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.1.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.crsi.1.parconf\endcsname{0.08}
\expandafter\gdef\csname R@an.stage1.blk.crsi.1.parconfpct\endcsname{8}
\expandafter\gdef\csname R@an.stage1.blk.crsi.1.parin\endcsname{0.33}
\expandafter\gdef\csname R@an.stage1.blk.crsi.1.parinpct\endcsname{33}
\expandafter\gdef\csname R@an.stage1.blk.crsi.1.priv\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.1.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.crsi.1.z1\endcsname{0.33}
\expandafter\gdef\csname R@an.stage1.blk.crsi.1.z1pct\endcsname{33}
\expandafter\gdef\csname R@an.stage1.blk.crsi.2.best\endcsname{\ensuremath{+5.19}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.2.conf\endcsname{8}
\expandafter\gdef\csname R@an.stage1.blk.crsi.2.gens\endcsname{7--9}
\expandafter\gdef\csname R@an.stage1.blk.crsi.2.improver\endcsname{v2}
\expandafter\gdef\csname R@an.stage1.blk.crsi.2.inherited\endcsname{yes}
\expandafter\gdef\csname R@an.stage1.blk.crsi.2.mean\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.2.median\endcsname{\ensuremath{+2.73}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.2.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.crsi.2.parconf\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.crsi.2.parconfpct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.crsi.2.parin\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.crsi.2.parinpct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.crsi.2.priv\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.2.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.crsi.2.z1\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.crsi.2.z1pct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.crsi.3.best\endcsname{\ensuremath{+5.78}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.3.conf\endcsname{9}
\expandafter\gdef\csname R@an.stage1.blk.crsi.3.gens\endcsname{10--12}
\expandafter\gdef\csname R@an.stage1.blk.crsi.3.improver\endcsname{v3}
\expandafter\gdef\csname R@an.stage1.blk.crsi.3.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.crsi.3.mean\endcsname{\ensuremath{+4.60}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.3.median\endcsname{\ensuremath{+4.65}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.3.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.crsi.3.parconf\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.crsi.3.parconfpct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.crsi.3.parin\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.crsi.3.parinpct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.crsi.3.priv\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.3.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.crsi.3.z1\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.crsi.3.z1pct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.crsi.4.best\endcsname{\ensuremath{+5.80}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.4.conf\endcsname{7}
\expandafter\gdef\csname R@an.stage1.blk.crsi.4.gens\endcsname{13--15}
\expandafter\gdef\csname R@an.stage1.blk.crsi.4.improver\endcsname{v4}
\expandafter\gdef\csname R@an.stage1.blk.crsi.4.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.crsi.4.mean\endcsname{\ensuremath{+4.59}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.4.median\endcsname{\ensuremath{+4.48}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.4.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.crsi.4.parconf\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.crsi.4.parconfpct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.crsi.4.parin\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.crsi.4.parinpct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.crsi.4.priv\endcsname{\ensuremath{+1.33}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.4.scored\endcsname{10}
\expandafter\gdef\csname R@an.stage1.blk.crsi.4.z1\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.crsi.4.z1pct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.crsi.5.best\endcsname{\ensuremath{+6.24}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.5.conf\endcsname{10}
\expandafter\gdef\csname R@an.stage1.blk.crsi.5.gens\endcsname{16--18}
\expandafter\gdef\csname R@an.stage1.blk.crsi.5.improver\endcsname{v5}
\expandafter\gdef\csname R@an.stage1.blk.crsi.5.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.crsi.5.mean\endcsname{\ensuremath{+5.21}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.5.median\endcsname{\ensuremath{+5.67}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.5.n\endcsname{15}
\expandafter\gdef\csname R@an.stage1.blk.crsi.5.parconf\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.crsi.5.parconfpct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.crsi.5.parin\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.crsi.5.parinpct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.crsi.5.priv\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.stage1.blk.crsi.5.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.crsi.5.z1\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.crsi.5.z1pct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.fixed.0.best\endcsname{\ensuremath{+1.58}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.0.conf\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.fixed.0.gens\endcsname{1--3}
\expandafter\gdef\csname R@an.stage1.blk.fixed.0.improver\endcsname{v0}
\expandafter\gdef\csname R@an.stage1.blk.fixed.0.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.fixed.0.mean\endcsname{\ensuremath{-9.92}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.0.median\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.0.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.fixed.0.parconf\endcsname{0.00}
\expandafter\gdef\csname R@an.stage1.blk.fixed.0.parconfpct\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.fixed.0.parin\endcsname{0.17}
\expandafter\gdef\csname R@an.stage1.blk.fixed.0.parinpct\endcsname{17}
\expandafter\gdef\csname R@an.stage1.blk.fixed.0.priv\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.0.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.fixed.0.z1\endcsname{0.08}
\expandafter\gdef\csname R@an.stage1.blk.fixed.0.z1pct\endcsname{8}
\expandafter\gdef\csname R@an.stage1.blk.fixed.1.best\endcsname{\ensuremath{+3.09}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.1.conf\endcsname{3}
\expandafter\gdef\csname R@an.stage1.blk.fixed.1.gens\endcsname{4--6}
\expandafter\gdef\csname R@an.stage1.blk.fixed.1.improver\endcsname{v0}
\expandafter\gdef\csname R@an.stage1.blk.fixed.1.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.fixed.1.mean\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.1.median\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.1.n\endcsname{10}
\expandafter\gdef\csname R@an.stage1.blk.fixed.1.parconf\endcsname{0.00}
\expandafter\gdef\csname R@an.stage1.blk.fixed.1.parconfpct\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.fixed.1.parin\endcsname{0.60}
\expandafter\gdef\csname R@an.stage1.blk.fixed.1.parinpct\endcsname{60}
\expandafter\gdef\csname R@an.stage1.blk.fixed.1.priv\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.1.scored\endcsname{10}
\expandafter\gdef\csname R@an.stage1.blk.fixed.1.z1\endcsname{0.40}
\expandafter\gdef\csname R@an.stage1.blk.fixed.1.z1pct\endcsname{40}
\expandafter\gdef\csname R@an.stage1.blk.fixed.2.best\endcsname{\ensuremath{+3.49}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.2.conf\endcsname{2}
\expandafter\gdef\csname R@an.stage1.blk.fixed.2.gens\endcsname{7--9}
\expandafter\gdef\csname R@an.stage1.blk.fixed.2.improver\endcsname{v0}
\expandafter\gdef\csname R@an.stage1.blk.fixed.2.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.fixed.2.mean\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.2.median\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.2.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.fixed.2.parconf\endcsname{0.42}
\expandafter\gdef\csname R@an.stage1.blk.fixed.2.parconfpct\endcsname{42}
\expandafter\gdef\csname R@an.stage1.blk.fixed.2.parin\endcsname{0.50}
\expandafter\gdef\csname R@an.stage1.blk.fixed.2.parinpct\endcsname{50}
\expandafter\gdef\csname R@an.stage1.blk.fixed.2.priv\endcsname{\ensuremath{+1.35}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.2.scored\endcsname{11}
\expandafter\gdef\csname R@an.stage1.blk.fixed.2.z1\endcsname{0.45}
\expandafter\gdef\csname R@an.stage1.blk.fixed.2.z1pct\endcsname{45}
\expandafter\gdef\csname R@an.stage1.blk.fixed.3.best\endcsname{\ensuremath{+4.12}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.3.conf\endcsname{6}
\expandafter\gdef\csname R@an.stage1.blk.fixed.3.gens\endcsname{10--12}
\expandafter\gdef\csname R@an.stage1.blk.fixed.3.improver\endcsname{v0}
\expandafter\gdef\csname R@an.stage1.blk.fixed.3.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.fixed.3.mean\endcsname{\ensuremath{+1.44}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.3.median\endcsname{\ensuremath{+1.42}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.3.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.fixed.3.parconf\endcsname{0.50}
\expandafter\gdef\csname R@an.stage1.blk.fixed.3.parconfpct\endcsname{50}
\expandafter\gdef\csname R@an.stage1.blk.fixed.3.parin\endcsname{0.50}
\expandafter\gdef\csname R@an.stage1.blk.fixed.3.parinpct\endcsname{50}
\expandafter\gdef\csname R@an.stage1.blk.fixed.3.priv\endcsname{\ensuremath{+1.82}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.3.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.fixed.3.z1\endcsname{0.58}
\expandafter\gdef\csname R@an.stage1.blk.fixed.3.z1pct\endcsname{58}
\expandafter\gdef\csname R@an.stage1.blk.fixed.4.best\endcsname{\ensuremath{+5.73}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.4.conf\endcsname{6}
\expandafter\gdef\csname R@an.stage1.blk.fixed.4.gens\endcsname{13--15}
\expandafter\gdef\csname R@an.stage1.blk.fixed.4.improver\endcsname{v0}
\expandafter\gdef\csname R@an.stage1.blk.fixed.4.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.fixed.4.mean\endcsname{\ensuremath{+2.04}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.4.median\endcsname{\ensuremath{+3.55}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.4.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.fixed.4.parconf\endcsname{0.50}
\expandafter\gdef\csname R@an.stage1.blk.fixed.4.parconfpct\endcsname{50}
\expandafter\gdef\csname R@an.stage1.blk.fixed.4.parin\endcsname{0.50}
\expandafter\gdef\csname R@an.stage1.blk.fixed.4.parinpct\endcsname{50}
\expandafter\gdef\csname R@an.stage1.blk.fixed.4.priv\endcsname{\ensuremath{+1.64}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.4.scored\endcsname{11}
\expandafter\gdef\csname R@an.stage1.blk.fixed.4.z1\endcsname{0.55}
\expandafter\gdef\csname R@an.stage1.blk.fixed.4.z1pct\endcsname{55}
\expandafter\gdef\csname R@an.stage1.blk.fixed.5.best\endcsname{\ensuremath{+5.44}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.5.conf\endcsname{6}
\expandafter\gdef\csname R@an.stage1.blk.fixed.5.gens\endcsname{16--18}
\expandafter\gdef\csname R@an.stage1.blk.fixed.5.improver\endcsname{v0}
\expandafter\gdef\csname R@an.stage1.blk.fixed.5.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.fixed.5.mean\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.5.median\endcsname{\ensuremath{+2.74}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.5.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.fixed.5.parconf\endcsname{0.50}
\expandafter\gdef\csname R@an.stage1.blk.fixed.5.parconfpct\endcsname{50}
\expandafter\gdef\csname R@an.stage1.blk.fixed.5.parin\endcsname{0.58}
\expandafter\gdef\csname R@an.stage1.blk.fixed.5.parinpct\endcsname{58}
\expandafter\gdef\csname R@an.stage1.blk.fixed.5.priv\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.stage1.blk.fixed.5.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.fixed.5.z1\endcsname{0.58}
\expandafter\gdef\csname R@an.stage1.blk.fixed.5.z1pct\endcsname{58}
\expandafter\gdef\csname R@an.stage1.blk.rsi.0.best\endcsname{\ensuremath{+1.91}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.0.conf\endcsname{1}
\expandafter\gdef\csname R@an.stage1.blk.rsi.0.gens\endcsname{1--3}
\expandafter\gdef\csname R@an.stage1.blk.rsi.0.improver\endcsname{v0}
\expandafter\gdef\csname R@an.stage1.blk.rsi.0.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.rsi.0.mean\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.0.median\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.0.n\endcsname{9}
\expandafter\gdef\csname R@an.stage1.blk.rsi.0.parconf\endcsname{0.00}
\expandafter\gdef\csname R@an.stage1.blk.rsi.0.parconfpct\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.rsi.0.parin\endcsname{0.00}
\expandafter\gdef\csname R@an.stage1.blk.rsi.0.parinpct\endcsname{0}
\expandafter\gdef\csname R@an.stage1.blk.rsi.0.priv\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.0.scored\endcsname{8}
\expandafter\gdef\csname R@an.stage1.blk.rsi.0.z1\endcsname{0.38}
\expandafter\gdef\csname R@an.stage1.blk.rsi.0.z1pct\endcsname{38}
\expandafter\gdef\csname R@an.stage1.blk.rsi.1.best\endcsname{\ensuremath{+2.46}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.1.conf\endcsname{4}
\expandafter\gdef\csname R@an.stage1.blk.rsi.1.gens\endcsname{4--6}
\expandafter\gdef\csname R@an.stage1.blk.rsi.1.improver\endcsname{v1}
\expandafter\gdef\csname R@an.stage1.blk.rsi.1.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.rsi.1.mean\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.1.median\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.1.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.rsi.1.parconf\endcsname{0.08}
\expandafter\gdef\csname R@an.stage1.blk.rsi.1.parconfpct\endcsname{8}
\expandafter\gdef\csname R@an.stage1.blk.rsi.1.parin\endcsname{0.33}
\expandafter\gdef\csname R@an.stage1.blk.rsi.1.parinpct\endcsname{33}
\expandafter\gdef\csname R@an.stage1.blk.rsi.1.priv\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.1.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.rsi.1.z1\endcsname{0.33}
\expandafter\gdef\csname R@an.stage1.blk.rsi.1.z1pct\endcsname{33}
\expandafter\gdef\csname R@an.stage1.blk.rsi.2.best\endcsname{\ensuremath{+5.19}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.2.conf\endcsname{8}
\expandafter\gdef\csname R@an.stage1.blk.rsi.2.gens\endcsname{7--9}
\expandafter\gdef\csname R@an.stage1.blk.rsi.2.improver\endcsname{v2}
\expandafter\gdef\csname R@an.stage1.blk.rsi.2.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.rsi.2.mean\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.2.median\endcsname{\ensuremath{+2.73}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.2.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.rsi.2.parconf\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.rsi.2.parconfpct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.rsi.2.parin\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.rsi.2.parinpct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.rsi.2.priv\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.2.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.blk.rsi.2.z1\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.rsi.2.z1pct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.rsi.3.best\endcsname{\ensuremath{+5.62}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.3.conf\endcsname{6}
\expandafter\gdef\csname R@an.stage1.blk.rsi.3.gens\endcsname{10--12}
\expandafter\gdef\csname R@an.stage1.blk.rsi.3.improver\endcsname{v3}
\expandafter\gdef\csname R@an.stage1.blk.rsi.3.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.rsi.3.mean\endcsname{\ensuremath{+3.82}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.3.median\endcsname{\ensuremath{+4.71}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.3.n\endcsname{7}
\expandafter\gdef\csname R@an.stage1.blk.rsi.3.parconf\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.rsi.3.parconfpct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.rsi.3.parin\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.rsi.3.parinpct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.rsi.3.priv\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.3.scored\endcsname{7}
\expandafter\gdef\csname R@an.stage1.blk.rsi.3.z1\endcsname{0.86}
\expandafter\gdef\csname R@an.stage1.blk.rsi.3.z1pct\endcsname{86}
\expandafter\gdef\csname R@an.stage1.blk.rsi.4.best\endcsname{\ensuremath{+5.72}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.4.conf\endcsname{4}
\expandafter\gdef\csname R@an.stage1.blk.rsi.4.gens\endcsname{13--15}
\expandafter\gdef\csname R@an.stage1.blk.rsi.4.improver\endcsname{v4}
\expandafter\gdef\csname R@an.stage1.blk.rsi.4.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.rsi.4.mean\endcsname{\ensuremath{-1.55}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.4.median\endcsname{\ensuremath{+3.08}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.4.n\endcsname{6}
\expandafter\gdef\csname R@an.stage1.blk.rsi.4.parconf\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.rsi.4.parconfpct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.rsi.4.parin\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.rsi.4.parinpct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.rsi.4.priv\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.4.scored\endcsname{6}
\expandafter\gdef\csname R@an.stage1.blk.rsi.4.z1\endcsname{0.67}
\expandafter\gdef\csname R@an.stage1.blk.rsi.4.z1pct\endcsname{67}
\expandafter\gdef\csname R@an.stage1.blk.rsi.5.best\endcsname{\ensuremath{+6.15}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.5.conf\endcsname{3}
\expandafter\gdef\csname R@an.stage1.blk.rsi.5.gens\endcsname{16--18}
\expandafter\gdef\csname R@an.stage1.blk.rsi.5.improver\endcsname{v5}
\expandafter\gdef\csname R@an.stage1.blk.rsi.5.inherited\endcsname{no}
\expandafter\gdef\csname R@an.stage1.blk.rsi.5.mean\endcsname{\ensuremath{+4.41}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.5.median\endcsname{\ensuremath{+4.13}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.5.n\endcsname{3}
\expandafter\gdef\csname R@an.stage1.blk.rsi.5.parconf\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.rsi.5.parconfpct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.rsi.5.parin\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.rsi.5.parinpct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.blk.rsi.5.priv\endcsname{\ensuremath{+1.53}}
\expandafter\gdef\csname R@an.stage1.blk.rsi.5.scored\endcsname{3}
\expandafter\gdef\csname R@an.stage1.blk.rsi.5.z1\endcsname{1.00}
\expandafter\gdef\csname R@an.stage1.blk.rsi.5.z1pct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.cmp.100.crsi.conf\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.stage1.cmp.100.crsi.priv\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.stage1.cmp.100.crsi.score\endcsname{2.46}
\expandafter\gdef\csname R@an.stage1.cmp.100.fixed.conf\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.stage1.cmp.100.fixed.priv\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.stage1.cmp.100.fixed.score\endcsname{1.69}
\expandafter\gdef\csname R@an.stage1.cmp.100.rsi.conf\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.stage1.cmp.100.rsi.priv\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.stage1.cmp.100.rsi.score\endcsname{2.46}
\expandafter\gdef\csname R@an.stage1.cmp.200.crsi.conf\endcsname{\ensuremath{+1.54}}
\expandafter\gdef\csname R@an.stage1.cmp.200.crsi.priv\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.stage1.cmp.200.crsi.score\endcsname{5.19}
\expandafter\gdef\csname R@an.stage1.cmp.200.fixed.conf\endcsname{\ensuremath{+1.49}}
\expandafter\gdef\csname R@an.stage1.cmp.200.fixed.priv\endcsname{\ensuremath{+1.35}}
\expandafter\gdef\csname R@an.stage1.cmp.200.fixed.score\endcsname{3.49}
\expandafter\gdef\csname R@an.stage1.cmp.200.rsi.conf\endcsname{\ensuremath{+1.54}}
\expandafter\gdef\csname R@an.stage1.cmp.200.rsi.priv\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.stage1.cmp.200.rsi.score\endcsname{5.19}
\expandafter\gdef\csname R@an.stage1.cmp.300.crsi.conf\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@an.stage1.cmp.300.crsi.priv\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@an.stage1.cmp.300.crsi.score\endcsname{5.78}
\expandafter\gdef\csname R@an.stage1.cmp.300.fixed.conf\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.stage1.cmp.300.fixed.priv\endcsname{\ensuremath{+1.82}}
\expandafter\gdef\csname R@an.stage1.cmp.300.fixed.score\endcsname{4.12}
\expandafter\gdef\csname R@an.stage1.cmp.300.rsi.conf\endcsname{\ensuremath{+1.81}}
\expandafter\gdef\csname R@an.stage1.cmp.300.rsi.priv\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.stage1.cmp.300.rsi.score\endcsname{5.62}
\expandafter\gdef\csname R@an.stage1.cmp.400.crsi.conf\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.stage1.cmp.400.crsi.priv\endcsname{\ensuremath{+1.33}}
\expandafter\gdef\csname R@an.stage1.cmp.400.crsi.score\endcsname{5.80}
\expandafter\gdef\csname R@an.stage1.cmp.400.fixed.conf\endcsname{\ensuremath{+2.21}}
\expandafter\gdef\csname R@an.stage1.cmp.400.fixed.priv\endcsname{\ensuremath{+1.82}}
\expandafter\gdef\csname R@an.stage1.cmp.400.fixed.score\endcsname{5.73}
\expandafter\gdef\csname R@an.stage1.cmp.400.rsi.conf\endcsname{\ensuremath{+1.81}}
\expandafter\gdef\csname R@an.stage1.cmp.400.rsi.priv\endcsname{\ensuremath{+1.53}}
\expandafter\gdef\csname R@an.stage1.cmp.400.rsi.score\endcsname{6.15}
\expandafter\gdef\csname R@an.stage1.cmp.common.crsi.conf\endcsname{\ensuremath{+1.96}}
\expandafter\gdef\csname R@an.stage1.cmp.common.crsi.priv\endcsname{\ensuremath{+1.33}}
\expandafter\gdef\csname R@an.stage1.cmp.common.crsi.score\endcsname{5.80}
\expandafter\gdef\csname R@an.stage1.cmp.common.fixed.conf\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.stage1.cmp.common.fixed.priv\endcsname{\ensuremath{+1.82}}
\expandafter\gdef\csname R@an.stage1.cmp.common.fixed.score\endcsname{5.73}
\expandafter\gdef\csname R@an.stage1.cmp.common.gpuh\endcsname{408.8}
\expandafter\gdef\csname R@an.stage1.cmp.common.rsi.conf\endcsname{\ensuremath{+1.81}}
\expandafter\gdef\csname R@an.stage1.cmp.common.rsi.priv\endcsname{\ensuremath{+1.53}}
\expandafter\gdef\csname R@an.stage1.cmp.common.rsi.score\endcsname{6.15}
\expandafter\gdef\csname R@an.stage1.cmp.n_budgets\endcsname{4}
\expandafter\gdef\csname R@an.stage1.cmp.priv_fixed_ahead\endcsname{3}
\expandafter\gdef\csname R@an.stage1.cmp.score_rsi_ahead\endcsname{4}
\expandafter\gdef\csname R@an.stage1.conf.crsi\endcsname{26}
\expandafter\gdef\csname R@an.stage1.conf.fixed\endcsname{23}
\expandafter\gdef\csname R@an.stage1.conf.rsi\endcsname{26}
\expandafter\gdef\csname R@an.stage1.end.gen.arch_fixed\endcsname{9}
\expandafter\gdef\csname R@an.stage1.end.gen.arch_rsi\endcsname{9}
\expandafter\gdef\csname R@an.stage1.end.gen.crsi\endcsname{18}
\expandafter\gdef\csname R@an.stage1.end.gen.fixed\endcsname{18}
\expandafter\gdef\csname R@an.stage1.end.gen.rsi\endcsname{18}
\expandafter\gdef\csname R@an.stage1.end.imp.arch_fixed\endcsname{v0}
\expandafter\gdef\csname R@an.stage1.end.imp.arch_rsi\endcsname{v2}
\expandafter\gdef\csname R@an.stage1.end.imp.crsi\endcsname{v5}
\expandafter\gdef\csname R@an.stage1.end.imp.fixed\endcsname{v0}
\expandafter\gdef\csname R@an.stage1.end.imp.rsi\endcsname{v5}
\expandafter\gdef\csname R@an.stage1.fid.acdc.above\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.acdc.above_unc\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.acdc.below\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.acdc.below_unc\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.acdc.hi\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.stage1.fid.acdc.lo\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.stage1.fid.acdc.mean\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.stage1.fid.acdc.mean100\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.stage1.fid.acdc.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.fid.acdc.pos\endcsname{9}
\expandafter\gdef\csname R@an.stage1.fid.amos.above\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.amos.above_unc\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.amos.below\endcsname{1}
\expandafter\gdef\csname R@an.stage1.fid.amos.below_unc\endcsname{2}
\expandafter\gdef\csname R@an.stage1.fid.amos.hi\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.stage1.fid.amos.lo\endcsname{\ensuremath{-0.62}}
\expandafter\gdef\csname R@an.stage1.fid.amos.mean\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@an.stage1.fid.amos.mean100\endcsname{\ensuremath{+1.23}}
\expandafter\gdef\csname R@an.stage1.fid.amos.n\endcsname{7}
\expandafter\gdef\csname R@an.stage1.fid.amos.pos\endcsname{2}
\expandafter\gdef\csname R@an.stage1.fid.arch_fixed.acdc.above\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.arch_fixed.acdc.below\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.arch_fixed.acdc.hi\endcsname{none}
\expandafter\gdef\csname R@an.stage1.fid.arch_fixed.acdc.lo\endcsname{none}
\expandafter\gdef\csname R@an.stage1.fid.arch_fixed.acdc.mean\endcsname{none}
\expandafter\gdef\csname R@an.stage1.fid.arch_fixed.acdc.n\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.arch_fixed.acdc.pos\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.arch_fixed.amos.above\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.arch_fixed.amos.below\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.arch_fixed.amos.hi\endcsname{none}
\expandafter\gdef\csname R@an.stage1.fid.arch_fixed.amos.lo\endcsname{none}
\expandafter\gdef\csname R@an.stage1.fid.arch_fixed.amos.mean\endcsname{none}
\expandafter\gdef\csname R@an.stage1.fid.arch_fixed.amos.n\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.arch_fixed.amos.pos\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.arch_fixed.cand\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.arch_fixed.queued\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.arch_fixed.runs\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.arch_rsi.acdc.above\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.arch_rsi.acdc.below\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.arch_rsi.acdc.hi\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.stage1.fid.arch_rsi.acdc.lo\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.stage1.fid.arch_rsi.acdc.mean\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.stage1.fid.arch_rsi.acdc.n\endcsname{1}
\expandafter\gdef\csname R@an.stage1.fid.arch_rsi.acdc.pos\endcsname{1}
\expandafter\gdef\csname R@an.stage1.fid.arch_rsi.amos.above\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.arch_rsi.amos.below\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.arch_rsi.amos.hi\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.stage1.fid.arch_rsi.amos.lo\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.stage1.fid.arch_rsi.amos.mean\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.stage1.fid.arch_rsi.amos.n\endcsname{1}
\expandafter\gdef\csname R@an.stage1.fid.arch_rsi.amos.pos\endcsname{1}
\expandafter\gdef\csname R@an.stage1.fid.arch_rsi.cand\endcsname{1}
\expandafter\gdef\csname R@an.stage1.fid.arch_rsi.queued\endcsname{2}
\expandafter\gdef\csname R@an.stage1.fid.arch_rsi.runs\endcsname{2}
\expandafter\gdef\csname R@an.stage1.fid.band.acdc\endcsname{0.21}
\expandafter\gdef\csname R@an.stage1.fid.band.amos\endcsname{0.26}
\expandafter\gdef\csname R@an.stage1.fid.cand\endcsname{12}
\expandafter\gdef\csname R@an.stage1.fid.cand_both\endcsname{7}
\expandafter\gdef\csname R@an.stage1.fid.cand_freeze\endcsname{11}
\expandafter\gdef\csname R@an.stage1.fid.crsi.acdc.above\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.crsi.acdc.below\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.crsi.acdc.hi\endcsname{none}
\expandafter\gdef\csname R@an.stage1.fid.crsi.acdc.lo\endcsname{none}
\expandafter\gdef\csname R@an.stage1.fid.crsi.acdc.mean\endcsname{none}
\expandafter\gdef\csname R@an.stage1.fid.crsi.acdc.n\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.crsi.acdc.pos\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.crsi.amos.above\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.crsi.amos.below\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.crsi.amos.hi\endcsname{none}
\expandafter\gdef\csname R@an.stage1.fid.crsi.amos.lo\endcsname{none}
\expandafter\gdef\csname R@an.stage1.fid.crsi.amos.mean\endcsname{none}
\expandafter\gdef\csname R@an.stage1.fid.crsi.amos.n\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.crsi.amos.pos\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.crsi.cand\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.crsi.queued\endcsname{52}
\expandafter\gdef\csname R@an.stage1.fid.crsi.runs\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.fixed.acdc.above\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.fixed.acdc.below\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.fixed.acdc.hi\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.stage1.fid.fixed.acdc.lo\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.stage1.fid.fixed.acdc.mean\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.stage1.fid.fixed.acdc.n\endcsname{3}
\expandafter\gdef\csname R@an.stage1.fid.fixed.acdc.pos\endcsname{2}
\expandafter\gdef\csname R@an.stage1.fid.fixed.amos.above\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.fixed.amos.below\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.fixed.amos.hi\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.stage1.fid.fixed.amos.lo\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.stage1.fid.fixed.amos.mean\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.stage1.fid.fixed.amos.n\endcsname{1}
\expandafter\gdef\csname R@an.stage1.fid.fixed.amos.pos\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.fixed.cand\endcsname{3}
\expandafter\gdef\csname R@an.stage1.fid.fixed.queued\endcsname{46}
\expandafter\gdef\csname R@an.stage1.fid.fixed.runs\endcsname{4}
\expandafter\gdef\csname R@an.stage1.fid.hold\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.pool.acdc.mean\endcsname{92.009}
\expandafter\gdef\csname R@an.stage1.fid.pool.acdc.n\endcsname{6}
\expandafter\gdef\csname R@an.stage1.fid.pool.acdc.sd\endcsname{0.099}
\expandafter\gdef\csname R@an.stage1.fid.pool.amos.mean\endcsname{87.701}
\expandafter\gdef\csname R@an.stage1.fid.pool.amos.n\endcsname{6}
\expandafter\gdef\csname R@an.stage1.fid.pool.amos.sd\endcsname{0.122}
\expandafter\gdef\csname R@an.stage1.fid.pos_all\endcsname{6}
\expandafter\gdef\csname R@an.stage1.fid.positive_both\endcsname{2}
\expandafter\gdef\csname R@an.stage1.fid.queued\endcsname{152}
\expandafter\gdef\csname R@an.stage1.fid.rsi.acdc.above\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.rsi.acdc.below\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.rsi.acdc.hi\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.stage1.fid.rsi.acdc.lo\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.stage1.fid.rsi.acdc.mean\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.stage1.fid.rsi.acdc.n\endcsname{8}
\expandafter\gdef\csname R@an.stage1.fid.rsi.acdc.pos\endcsname{6}
\expandafter\gdef\csname R@an.stage1.fid.rsi.amos.above\endcsname{0}
\expandafter\gdef\csname R@an.stage1.fid.rsi.amos.below\endcsname{1}
\expandafter\gdef\csname R@an.stage1.fid.rsi.amos.hi\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.stage1.fid.rsi.amos.lo\endcsname{\ensuremath{-0.62}}
\expandafter\gdef\csname R@an.stage1.fid.rsi.amos.mean\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.stage1.fid.rsi.amos.n\endcsname{5}
\expandafter\gdef\csname R@an.stage1.fid.rsi.amos.pos\endcsname{1}
\expandafter\gdef\csname R@an.stage1.fid.rsi.cand\endcsname{8}
\expandafter\gdef\csname R@an.stage1.fid.rsi.queued\endcsname{52}
\expandafter\gdef\csname R@an.stage1.fid.rsi.runs\endcsname{13}
\expandafter\gdef\csname R@an.stage1.fid.runs\endcsname{19}
\expandafter\gdef\csname R@an.stage1.fid.runs_freeze\endcsname{17}
\expandafter\gdef\csname R@an.stage1.fid.runs_post\endcsname{2}
\expandafter\gdef\csname R@an.stage1.fid.shift_unc.acdc\endcsname{\ensuremath{+0.007}}
\expandafter\gdef\csname R@an.stage1.fid.shift_unc.amos\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.stage1.fid.unfinished\endcsname{133}
\expandafter\gdef\csname R@an.stage1.fork.arm\endcsname{rsi}
\expandafter\gdef\csname R@an.stage1.fork.date\endcsname{2026-09-27}
\expandafter\gdef\csname R@an.stage1.fork.gen\endcsname{9}
\expandafter\gdef\csname R@an.stage1.fork.model\endcsname{Claude Opus 5.5}
\expandafter\gdef\csname R@an.stage1.fork.n\endcsname{33}
\expandafter\gdef\csname R@an.stage1.fork.noop\endcsname{v4}
\expandafter\gdef\csname R@an.stage1.fork.noop.reason\endcsname{meta response cut off at max\_tokens=48000 (finish\_reason length; $\sim$36k of the 48k tokens were reasoning)}
\expandafter\gdef\csname R@an.stage1.fork.time\endcsname{21:30}
\expandafter\gdef\csname R@an.stage1.fork.versions\endcsname{v0--v2}
\expandafter\gdef\csname R@an.stage1.freeze.date\endcsname{2026-09-29}
\expandafter\gdef\csname R@an.stage1.freeze.time\endcsname{10:20}
\expandafter\gdef\csname R@an.stage1.gens\endcsname{18}
\expandafter\gdef\csname R@an.stage1.gpuh\endcsname{1497.5}
\expandafter\gdef\csname R@an.stage1.gpuh.recipe\endcsname{1173.9}
\expandafter\gdef\csname R@an.stage1.inh.child.crsi.above\endcsname{2}
\expandafter\gdef\csname R@an.stage1.inh.child.crsi.n\endcsname{26}
\expandafter\gdef\csname R@an.stage1.inh.child.fixed.above\endcsname{3}
\expandafter\gdef\csname R@an.stage1.inh.child.fixed.n\endcsname{19}
\expandafter\gdef\csname R@an.stage1.inh.child.rsi.above\endcsname{10}
\expandafter\gdef\csname R@an.stage1.inh.child.rsi.n\endcsname{22}
\expandafter\gdef\csname R@an.stage1.inh.late.crsi.k\endcsname{39}
\expandafter\gdef\csname R@an.stage1.inh.late.crsi.n\endcsname{39}
\expandafter\gdef\csname R@an.stage1.inh.late.crsi.pct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.inh.late.fixed.k\endcsname{23}
\expandafter\gdef\csname R@an.stage1.inh.late.fixed.n\endcsname{48}
\expandafter\gdef\csname R@an.stage1.inh.late.fixed.pct\endcsname{48}
\expandafter\gdef\csname R@an.stage1.inh.late.rsi.k\endcsname{28}
\expandafter\gdef\csname R@an.stage1.inh.late.rsi.n\endcsname{28}
\expandafter\gdef\csname R@an.stage1.inh.late.rsi.pct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.inh.npc.crsi.med\endcsname{none}
\expandafter\gdef\csname R@an.stage1.inh.npc.crsi.n\endcsname{0}
\expandafter\gdef\csname R@an.stage1.inh.npc.fixed.med\endcsname{0.13}
\expandafter\gdef\csname R@an.stage1.inh.npc.fixed.n\endcsname{46}
\expandafter\gdef\csname R@an.stage1.inh.npc.rsi.med\endcsname{0.29}
\expandafter\gdef\csname R@an.stage1.inh.npc.rsi.n\endcsname{19}
\expandafter\gdef\csname R@an.stage1.inh.pc.crsi.med\endcsname{4.91}
\expandafter\gdef\csname R@an.stage1.inh.pc.crsi.n\endcsname{34}
\expandafter\gdef\csname R@an.stage1.inh.pc.fixed.med\endcsname{4.05}
\expandafter\gdef\csname R@an.stage1.inh.pc.fixed.n\endcsname{22}
\expandafter\gdef\csname R@an.stage1.inh.pc.rsi.med\endcsname{3.72}
\expandafter\gdef\csname R@an.stage1.inh.pc.rsi.n\endcsname{29}
\expandafter\gdef\csname R@an.stage1.inh.thr.acdc\endcsname{0.15}
\expandafter\gdef\csname R@an.stage1.inh.thr.amos\endcsname{1.16}
\expandafter\gdef\csname R@an.stage1.llm.designer\endcsname{gpt-6-astra}
\expandafter\gdef\csname R@an.stage1.llm.meta\endcsname{Claude Opus 5.5 and gpt-6-astra}
\expandafter\gdef\csname R@an.stage1.llm.meta.crsi\endcsname{Claude Opus 5.5}
\expandafter\gdef\csname R@an.stage1.parentconf.crsi\endcsname{100\%}
\expandafter\gdef\csname R@an.stage1.parentconf.fixed\endcsname{48\%}
\expandafter\gdef\csname R@an.stage1.parentconf.rsi\endcsname{100\%}
\expandafter\gdef\csname R@an.stage1.priv.crsi\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.stage1.priv.fixed\endcsname{\ensuremath{+1.82}}
\expandafter\gdef\csname R@an.stage1.priv.rsi\endcsname{\ensuremath{+1.53}}
\expandafter\gdef\csname R@an.stage1.ratio.calls.rsi_fixed\endcsname{3.0}
\expandafter\gdef\csname R@an.stage1.ratio.cand.rsi_fixed\endcsname{0.70}
\expandafter\gdef\csname R@an.stage1.ratio.gpuh.rsi_fixed\endcsname{0.85}
\expandafter\gdef\csname R@an.stage1.ratio.tokc.rsi_fixed\endcsname{1.9}
\expandafter\gdef\csname R@an.stage1.ratio.tokp.rsi_fixed\endcsname{7.0}
\expandafter\gdef\csname R@an.stage1.reach.t10.crsi.gen\endcsname{10}
\expandafter\gdef\csname R@an.stage1.reach.t10.crsi.gpuh\endcsname{281}
\expandafter\gdef\csname R@an.stage1.reach.t10.fixed.gen\endcsname{6}
\expandafter\gdef\csname R@an.stage1.reach.t10.fixed.gpuh\endcsname{112}
\expandafter\gdef\csname R@an.stage1.reach.t10.rsi.gen\endcsname{10}
\expandafter\gdef\csname R@an.stage1.reach.t10.rsi.gpuh\endcsname{283}
\expandafter\gdef\csname R@an.stage1.reach.t15.crsi.gen\endcsname{16}
\expandafter\gdef\csname R@an.stage1.reach.t15.crsi.gpuh\endcsname{454}
\expandafter\gdef\csname R@an.stage1.reach.t15.fixed.gen\endcsname{11}
\expandafter\gdef\csname R@an.stage1.reach.t15.fixed.gpuh\endcsname{246}
\expandafter\gdef\csname R@an.stage1.reach.t15.rsi.gen\endcsname{17}
\expandafter\gdef\csname R@an.stage1.reach.t15.rsi.gpuh\endcsname{399}
\expandafter\gdef\csname R@an.stage1.report.date\endcsname{2026-09-29}
\expandafter\gdef\csname R@an.stage1.report.time\endcsname{10:20}
\expandafter\gdef\csname R@an.stage1.runvar\endcsname{0.61}
\expandafter\gdef\csname R@an.stage1.sent.arch\endcsname{The architecture track screened 72 candidates at 100 epochs (3 smoke failures and 1 failed run; best screen score \ensuremath{+1.60} Arch-fixed, \ensuremath{+2.80} Arch-RSI), promoted 34 to 250 epochs and finished that evaluation for 6 before the freeze; 1 candidate passed the 3-seed confirmation (Arch-RSI \texttt{phase\_complete\_encoder\_reduction}: \ensuremath{+0.06} Dice points on ACDC, \ensuremath{+0.70} on AMOS22), and 0 received a private grade.}
\expandafter\gdef\csname R@an.stage1.sent.fid\endcsname{Full-budget (1000-epoch) runs finished for 12 confirmed trainers (19 runs: RSI 8 trainers, fixed 3, Arch-RSI 1; single seed, fold 0, the search fold; none for the RSI fork). Against the frozen default pools their Dice differences lie between \ensuremath{-0.06} and \ensuremath{+0.17} points on ACDC (single-seed noise band $\pm$0.21) and between \ensuremath{-0.62} and \ensuremath{+0.10} on AMOS22 ($\pm$0.26); none of the 12 trainers exceeds the band on either dataset. The mean 3-seed gain of the same trainers at 100 epochs, \ensuremath{+0.28} on ACDC and \ensuremath{+1.23} on AMOS22, is \ensuremath{+0.05} and \ensuremath{-0.16} at 1000 epochs.}
\expandafter\gdef\csname R@an.stage1.sent.fid.line\endcsname{None of the 12 confirmed trainers hold a gain above the single-seed noise band at 1000 epochs; 6 of 12 are positive on every full-budget run they have.}
\expandafter\gdef\csname R@an.stage1.sent.fork\endcsname{The RSI fork copies the first 9 generations of the RSI arm (33 candidates, improver versions v0--v2) on 2026-09-27 at 21:30 and continues generations 10--18 with Claude Opus 5.5 as meta-level and the same designer; its rewrite v4 left the improver unchanged because the meta-level response was cut off.}
\expandafter\gdef\csname R@an.stage1.sent.gpuh\endcsname{At the common budget of 408.8 GPU-hours the best private grade is \ensuremath{+1.82} Dice points for the fixed improver, \ensuremath{+1.53} for the rewritten improver (RSI) and \ensuremath{+1.33} for the RSI fork. The fixed improver's grade is at or above both RSI arms' at 3 of the 4 budgets compared (100, 200, 300, 400 GPU-hours). The exception is 100 GPU-hours (\ensuremath{-0.07} against \ensuremath{+0.54}). The best in-loop candidate score is higher for both RSI arms at 4 of 4 (6.15 and 5.80 against 5.73 at 408.8 GPU-hours).}
\expandafter\gdef\csname R@an.stage1.sent.inherit\endcsname{From block 2 on, 28 of 28 candidates of the RSI arm and 39 of 39 own candidates of the RSI fork descend from a confirmed parent, against 23 of 48 for the fixed improver. Over all blocks, a candidate with a confirmed parent has a median score of 4.05 (fixed), 3.72 (RSI) and 4.91 (RSI fork); one without, 0.13 (fixed) and 0.29 (RSI).}
\expandafter\gdef\csname R@an.stage1.sent.inherit.base\endcsname{Among candidates that start from the unmodified baseline, which have nothing to inherit, blocks 0 to 1 (the blocks in which the RSI arm proposes any): fixed 14 (median score 0.23, 2 of 14 above z = 1, 1 confirmed), RSI 17 (median score 0.17, 5 of 16 above z = 1, 2 confirmed). From block 2 on, 23 of 48 fixed candidates still start from the baseline, against 0 of 28 for the RSI arm and 0 of 39 for the RSI fork.}
\expandafter\gdef\csname R@an.stage1.sent.inherit.gain\endcsname{Of the confirmed candidates that descend from a confirmed parent, 3 of 19 (fixed), 10 of 22 (RSI) and 2 of 26 (RSI fork) gain more than 2 standard errors over that parent (0.15 Dice points on ACDC, 1.16 on AMOS22).}
\expandafter\gdef\csname R@an.stage1.sent.llm\endcsname{Stage 1 made 134 LLM calls (124 designer calls, 10 meta-level rewrites) and used 5.29 million prompt and 1.54 million completion tokens; the designer is gpt-6-astra, the meta-level of the RSI arms gpt-6-astra and the meta-level of the RSI fork Claude Opus 5.5.}
\expandafter\gdef\csname R@an.stage1.sent.reach\endcsname{The best private grade first reaches \ensuremath{+1.0} Dice points after 112 (fixed improver), 283 (RSI arm) and 281 (RSI fork) GPU-hours, and \ensuremath{+1.5} after 246 (fixed improver), 399 (RSI arm) and 454 (RSI fork) GPU-hours.}
\expandafter\gdef\csname R@an.stage1.span.hours\endcsname{58}
\expandafter\gdef\csname R@an.stage1.start.date\endcsname{2026-09-27}
\expandafter\gdef\csname R@an.stage1.start.time\endcsname{00:13}
\expandafter\gdef\csname R@an.stage1.total.arms\endcsname{5}
\expandafter\gdef\csname R@an.stage1.total.calls\endcsname{134}
\expandafter\gdef\csname R@an.stage1.total.calls_design\endcsname{124}
\expandafter\gdef\csname R@an.stage1.total.calls_meta\endcsname{10}
\expandafter\gdef\csname R@an.stage1.total.conf\endcsname{76}
\expandafter\gdef\csname R@an.stage1.total.gpuh\endcsname{1497.5}
\expandafter\gdef\csname R@an.stage1.total.n\endcsname{230}
\expandafter\gdef\csname R@an.stage1.total.scored\endcsname{218}
\expandafter\gdef\csname R@an.stage1.total.tok_completion\endcsname{1538943}
\expandafter\gdef\csname R@an.stage1.total.tok_completion_m\endcsname{1.54}
\expandafter\gdef\csname R@an.stage1.total.tok_prompt\endcsname{5286787}
\expandafter\gdef\csname R@an.stage1.total.tok_prompt_m\endcsname{5.29}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v0.best\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v0.block\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v0.conf\endcsname{1}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v0.gens\endcsname{1--3}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v0.mean\endcsname{\ensuremath{-0.70}}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v0.model\endcsname{hand-written}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v0.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v0.noop\endcsname{no}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v0.parent\endcsname{none}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v0.priv\endcsname{none}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v0.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v0.smoke_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v0.trial_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v0.z1pct\endcsname{25}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v1.best\endcsname{\ensuremath{+2.80}}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v1.block\endcsname{1}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v1.conf\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v1.gens\endcsname{4--6}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v1.mean\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v1.model\endcsname{gpt-6-astra}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v1.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v1.noop\endcsname{no}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v1.parent\endcsname{v0}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v1.priv\endcsname{none}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v1.scored\endcsname{11}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v1.smoke_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v1.trial_failed\endcsname{1}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v1.z1pct\endcsname{27}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v2.best\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v2.block\endcsname{2}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v2.conf\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v2.gens\endcsname{7--9}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v2.mean\endcsname{\ensuremath{-1.48}}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v2.model\endcsname{gpt-6-astra}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v2.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v2.noop\endcsname{no}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v2.parent\endcsname{v1}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v2.priv\endcsname{none}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v2.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v2.smoke_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v2.trial_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.arch_rsi.v2.z1pct\endcsname{8}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v0.best\endcsname{\ensuremath{+1.91}}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v0.block\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v0.conf\endcsname{1}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v0.desc\endcsname{initial hand-written improver}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v0.gens\endcsname{1--3}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v0.mean\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v0.model\endcsname{hand-written}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v0.n\endcsname{9}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v0.noop\endcsname{no}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v0.parent\endcsname{none}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v0.priv\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v0.scored\endcsname{8}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v0.smoke_failed\endcsname{1}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v0.trial_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v0.z1pct\endcsname{38}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v1.best\endcsname{\ensuremath{+2.46}}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v1.block\endcsname{1}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v1.conf\endcsname{4}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v1.desc\endcsname{portable gains, controlled contrasts, executable code}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v1.gens\endcsname{4--6}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v1.mean\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v1.model\endcsname{gpt-6-astra}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v1.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v1.noop\endcsname{no}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v1.parent\endcsname{v0}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v1.priv\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v1.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v1.smoke_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v1.trial_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v1.z1pct\endcsname{33}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v2.best\endcsname{\ensuremath{+5.19}}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v2.block\endcsname{2}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v2.conf\endcsname{8}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v2.desc\endcsname{improve selection, not just executability}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v2.gens\endcsname{7--9}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v2.mean\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v2.model\endcsname{gpt-6-astra}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v2.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v2.noop\endcsname{no}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v2.parent\endcsname{v1}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v2.priv\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v2.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v2.smoke_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v2.trial_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v2.z1pct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v3.best\endcsname{\ensuremath{+5.78}}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v3.block\endcsname{3}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v3.conf\endcsname{9}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v3.desc\endcsname{climb the confirmed frontier, keep exploring}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v3.gens\endcsname{10--12}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v3.mean\endcsname{\ensuremath{+4.60}}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v3.model\endcsname{Claude Opus 5.5}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v3.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v3.noop\endcsname{no}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v3.parent\endcsname{v2}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v3.priv\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v3.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v3.smoke_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v3.trial_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v3.z1pct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v4.best\endcsname{\ensuremath{+5.80}}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v4.block\endcsname{4}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v4.conf\endcsname{7}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v4.desc\endcsname{climb the confirmed frontier, keep exploring}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v4.gens\endcsname{13--15}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v4.mean\endcsname{\ensuremath{+4.59}}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v4.model\endcsname{Claude Opus 5.5}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v4.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v4.noop\endcsname{yes}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v4.parent\endcsname{v3}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v4.priv\endcsname{\ensuremath{+1.33}}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v4.scored\endcsname{10}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v4.smoke_failed\endcsname{2}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v4.trial_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v4.z1pct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v5.best\endcsname{\ensuremath{+6.24}}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v5.block\endcsname{5}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v5.conf\endcsname{10}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v5.desc\endcsname{marginal effects, not inherited z}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v5.gens\endcsname{16--18}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v5.mean\endcsname{\ensuremath{+5.21}}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v5.model\endcsname{Claude Opus 5.5}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v5.n\endcsname{15}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v5.noop\endcsname{no}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v5.parent\endcsname{v4}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v5.priv\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v5.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v5.smoke_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v5.trial_failed\endcsname{3}
\expandafter\gdef\csname R@an.stage1.ver.crsi.v5.z1pct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v0.best\endcsname{\ensuremath{+1.91}}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v0.block\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v0.conf\endcsname{1}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v0.desc\endcsname{initial hand-written improver}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v0.gens\endcsname{1--3}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v0.mean\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v0.model\endcsname{hand-written}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v0.n\endcsname{9}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v0.noop\endcsname{no}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v0.parent\endcsname{none}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v0.priv\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v0.scored\endcsname{8}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v0.smoke_failed\endcsname{1}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v0.trial_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v0.z1pct\endcsname{38}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v1.best\endcsname{\ensuremath{+2.46}}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v1.block\endcsname{1}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v1.conf\endcsname{4}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v1.desc\endcsname{portable gains, controlled contrasts, executable code}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v1.gens\endcsname{4--6}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v1.mean\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v1.model\endcsname{gpt-6-astra}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v1.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v1.noop\endcsname{no}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v1.parent\endcsname{v0}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v1.priv\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v1.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v1.smoke_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v1.trial_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v1.z1pct\endcsname{33}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v2.best\endcsname{\ensuremath{+5.19}}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v2.block\endcsname{2}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v2.conf\endcsname{8}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v2.desc\endcsname{improve selection, not just executability}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v2.gens\endcsname{7--9}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v2.mean\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v2.model\endcsname{gpt-6-astra}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v2.n\endcsname{12}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v2.noop\endcsname{no}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v2.parent\endcsname{v1}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v2.priv\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v2.scored\endcsname{12}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v2.smoke_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v2.trial_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v2.z1pct\endcsname{100}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v3.best\endcsname{\ensuremath{+5.62}}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v3.block\endcsname{3}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v3.conf\endcsname{6}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v3.desc\endcsname{preserve v2's selection gains, improve frontier quality}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v3.gens\endcsname{10--12}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v3.mean\endcsname{\ensuremath{+3.82}}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v3.model\endcsname{gpt-6-astra}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v3.n\endcsname{7}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v3.noop\endcsname{no}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v3.parent\endcsname{v2}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v3.priv\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v3.scored\endcsname{7}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v3.smoke_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v3.trial_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v3.z1pct\endcsname{86}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v4.best\endcsname{\ensuremath{+5.72}}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v4.block\endcsname{4}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v4.conf\endcsname{4}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v4.desc\endcsname{refresh the frontier, escape the exhausted lattice}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v4.gens\endcsname{13--15}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v4.mean\endcsname{\ensuremath{-1.55}}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v4.model\endcsname{gpt-6-astra}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v4.n\endcsname{6}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v4.noop\endcsname{no}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v4.parent\endcsname{v3}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v4.priv\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v4.scored\endcsname{6}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v4.smoke_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v4.trial_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v4.z1pct\endcsname{67}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v5.best\endcsname{\ensuremath{+6.15}}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v5.block\endcsname{5}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v5.conf\endcsname{3}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v5.desc\endcsname{portable marginal gains with bounded downside}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v5.gens\endcsname{16--18}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v5.mean\endcsname{\ensuremath{+4.41}}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v5.model\endcsname{gpt-6-astra}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v5.n\endcsname{3}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v5.noop\endcsname{no}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v5.parent\endcsname{v4}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v5.priv\endcsname{\ensuremath{+1.53}}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v5.scored\endcsname{3}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v5.smoke_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v5.trial_failed\endcsname{0}
\expandafter\gdef\csname R@an.stage1.ver.rsi.v5.z1pct\endcsname{100}
\expandafter\gdef\csname R@an.stage_allocation.D1.coarse.encoder.M\endcsname{12.976256}
\expandafter\gdef\csname R@an.stage_allocation.D1.coarse.encoder.M2\endcsname{12.98}
\expandafter\gdef\csname R@an.stage_allocation.D1.coarse.encoder.exact\endcsname{12976256}
\expandafter\gdef\csname R@an.stage_allocation.D1.coarse.encoder.share\endcsname{62.21}
\expandafter\gdef\csname R@an.stage_allocation.D1.decoder.M\endcsname{5.026720}
\expandafter\gdef\csname R@an.stage_allocation.D1.decoder.M2\endcsname{5.03}
\expandafter\gdef\csname R@an.stage_allocation.D1.decoder.exact\endcsname{5026720}
\expandafter\gdef\csname R@an.stage_allocation.D1.decoder.share\endcsname{24.10}
\expandafter\gdef\csname R@an.stage_allocation.D1.fine.encoder.M\endcsname{2.843808}
\expandafter\gdef\csname R@an.stage_allocation.D1.fine.encoder.M2\endcsname{2.84}
\expandafter\gdef\csname R@an.stage_allocation.D1.fine.encoder.exact\endcsname{2843808}
\expandafter\gdef\csname R@an.stage_allocation.D1.fine.encoder.share\endcsname{13.63}
\expandafter\gdef\csname R@an.stage_allocation.D1.heads.M\endcsname{0.012880}
\expandafter\gdef\csname R@an.stage_allocation.D1.heads.M2\endcsname{0.01}
\expandafter\gdef\csname R@an.stage_allocation.D1.heads.exact\endcsname{12880}
\expandafter\gdef\csname R@an.stage_allocation.D1.heads.share\endcsname{0.06}
\expandafter\gdef\csname R@an.stage_allocation.D1.total.M\endcsname{20.859664}
\expandafter\gdef\csname R@an.stage_allocation.D1.total.M2\endcsname{20.86}
\expandafter\gdef\csname R@an.stage_allocation.D1.total.exact\endcsname{20859664}
\expandafter\gdef\csname R@an.stage_allocation.D2.coarse.encoder.M\endcsname{13.165824}
\expandafter\gdef\csname R@an.stage_allocation.D2.coarse.encoder.M2\endcsname{13.17}
\expandafter\gdef\csname R@an.stage_allocation.D2.coarse.encoder.exact\endcsname{13165824}
\expandafter\gdef\csname R@an.stage_allocation.D2.coarse.encoder.share\endcsname{50.59}
\expandafter\gdef\csname R@an.stage_allocation.D2.decoder.M\endcsname{12.006528}
\expandafter\gdef\csname R@an.stage_allocation.D2.decoder.M2\endcsname{12.01}
\expandafter\gdef\csname R@an.stage_allocation.D2.decoder.exact\endcsname{12006528}
\expandafter\gdef\csname R@an.stage_allocation.D2.decoder.share\endcsname{46.13}
\expandafter\gdef\csname R@an.stage_allocation.D2.fine.encoder.M\endcsname{0.840288}
\expandafter\gdef\csname R@an.stage_allocation.D2.fine.encoder.M2\endcsname{0.84}
\expandafter\gdef\csname R@an.stage_allocation.D2.fine.encoder.exact\endcsname{840288}
\expandafter\gdef\csname R@an.stage_allocation.D2.fine.encoder.share\endcsname{3.23}
\expandafter\gdef\csname R@an.stage_allocation.D2.heads.M\endcsname{0.012880}
\expandafter\gdef\csname R@an.stage_allocation.D2.heads.M2\endcsname{0.01}
\expandafter\gdef\csname R@an.stage_allocation.D2.heads.exact\endcsname{12880}
\expandafter\gdef\csname R@an.stage_allocation.D2.heads.share\endcsname{0.05}
\expandafter\gdef\csname R@an.stage_allocation.D2.total.M\endcsname{26.025520}
\expandafter\gdef\csname R@an.stage_allocation.D2.total.M2\endcsname{26.03}
\expandafter\gdef\csname R@an.stage_allocation.D2.total.exact\endcsname{26025520}
\expandafter\gdef\csname R@an.stage_allocation.L1.coarse.encoder.M\endcsname{86.299264}
\expandafter\gdef\csname R@an.stage_allocation.L1.coarse.encoder.M2\endcsname{86.30}
\expandafter\gdef\csname R@an.stage_allocation.L1.coarse.encoder.exact\endcsname{86299264}
\expandafter\gdef\csname R@an.stage_allocation.L1.coarse.encoder.share\endcsname{84.38}
\expandafter\gdef\csname R@an.stage_allocation.L1.decoder.M\endcsname{12.006528}
\expandafter\gdef\csname R@an.stage_allocation.L1.decoder.M2\endcsname{12.01}
\expandafter\gdef\csname R@an.stage_allocation.L1.decoder.exact\endcsname{12006528}
\expandafter\gdef\csname R@an.stage_allocation.L1.decoder.share\endcsname{11.74}
\expandafter\gdef\csname R@an.stage_allocation.L1.fine.encoder.M\endcsname{3.959872}
\expandafter\gdef\csname R@an.stage_allocation.L1.fine.encoder.M2\endcsname{3.96}
\expandafter\gdef\csname R@an.stage_allocation.L1.fine.encoder.exact\endcsname{3959872}
\expandafter\gdef\csname R@an.stage_allocation.L1.fine.encoder.share\endcsname{3.87}
\expandafter\gdef\csname R@an.stage_allocation.L1.heads.M\endcsname{0.012880}
\expandafter\gdef\csname R@an.stage_allocation.L1.heads.M2\endcsname{0.01}
\expandafter\gdef\csname R@an.stage_allocation.L1.heads.exact\endcsname{12880}
\expandafter\gdef\csname R@an.stage_allocation.L1.heads.share\endcsname{0.01}
\expandafter\gdef\csname R@an.stage_allocation.L1.total.M\endcsname{102.278544}
\expandafter\gdef\csname R@an.stage_allocation.L1.total.M2\endcsname{102.28}
\expandafter\gdef\csname R@an.stage_allocation.L1.total.exact\endcsname{102278544}
\expandafter\gdef\csname R@an.stage_allocation.L3.coarse.encoder.M\endcsname{12.976256}
\expandafter\gdef\csname R@an.stage_allocation.L3.coarse.encoder.M2\endcsname{12.98}
\expandafter\gdef\csname R@an.stage_allocation.L3.coarse.encoder.exact\endcsname{12976256}
\expandafter\gdef\csname R@an.stage_allocation.L3.coarse.encoder.share\endcsname{43.85}
\expandafter\gdef\csname R@an.stage_allocation.L3.decoder.M\endcsname{13.759392}
\expandafter\gdef\csname R@an.stage_allocation.L3.decoder.M2\endcsname{13.76}
\expandafter\gdef\csname R@an.stage_allocation.L3.decoder.exact\endcsname{13759392}
\expandafter\gdef\csname R@an.stage_allocation.L3.decoder.share\endcsname{46.50}
\expandafter\gdef\csname R@an.stage_allocation.L3.fine.encoder.M\endcsname{2.843808}
\expandafter\gdef\csname R@an.stage_allocation.L3.fine.encoder.M2\endcsname{2.84}
\expandafter\gdef\csname R@an.stage_allocation.L3.fine.encoder.exact\endcsname{2843808}
\expandafter\gdef\csname R@an.stage_allocation.L3.fine.encoder.share\endcsname{9.61}
\expandafter\gdef\csname R@an.stage_allocation.L3.heads.M\endcsname{0.012880}
\expandafter\gdef\csname R@an.stage_allocation.L3.heads.M2\endcsname{0.01}
\expandafter\gdef\csname R@an.stage_allocation.L3.heads.exact\endcsname{12880}
\expandafter\gdef\csname R@an.stage_allocation.L3.heads.share\endcsname{0.04}
\expandafter\gdef\csname R@an.stage_allocation.L3.reduction.percent\endcsname{4.922}
\expandafter\gdef\csname R@an.stage_allocation.L3.reduction.percent.precise\endcsname{4.922291113}
\expandafter\gdef\csname R@an.stage_allocation.L3.total.M\endcsname{29.592336}
\expandafter\gdef\csname R@an.stage_allocation.L3.total.M2\endcsname{29.59}
\expandafter\gdef\csname R@an.stage_allocation.L3.total.exact\endcsname{29592336}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.coarse.encoder.M\endcsname{\ensuremath{-0.189568}}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.coarse.encoder.M2\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.coarse.encoder.exact\endcsname{\ensuremath{-189568}}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.coarse.encoder.step\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.decoder.M\endcsname{\ensuremath{-3.345984}}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.decoder.M2\endcsname{\ensuremath{-3.35}}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.decoder.exact\endcsname{\ensuremath{-3345984}}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.decoder.step\endcsname{\ensuremath{-3.35}}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.fine.encoder.M\endcsname{\ensuremath{+2.003520}}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.fine.encoder.M2\endcsname{\ensuremath{+2.00}}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.fine.encoder.exact\endcsname{\ensuremath{+2003520}}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.fine.encoder.step\endcsname{\ensuremath{+2.00}}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.heads.M\endcsname{\ensuremath{+0.000000}}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.heads.M2\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.heads.exact\endcsname{\ensuremath{+0}}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.heads.step\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.total.M\endcsname{\ensuremath{-1.532032}}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.total.M2\endcsname{\ensuremath{-1.53}}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.total.exact\endcsname{\ensuremath{-1532032}}
\expandafter\gdef\csname R@an.stage_allocation.L3minusdefault.total.step\endcsname{\ensuremath{-1.53}}
\expandafter\gdef\csname R@an.stage_allocation.default.coarse.encoder.M\endcsname{13.165824}
\expandafter\gdef\csname R@an.stage_allocation.default.coarse.encoder.M2\endcsname{13.17}
\expandafter\gdef\csname R@an.stage_allocation.default.coarse.encoder.exact\endcsname{13165824}
\expandafter\gdef\csname R@an.stage_allocation.default.coarse.encoder.share\endcsname{42.30}
\expandafter\gdef\csname R@an.stage_allocation.default.decoder.M\endcsname{17.105376}
\expandafter\gdef\csname R@an.stage_allocation.default.decoder.M2\endcsname{17.11}
\expandafter\gdef\csname R@an.stage_allocation.default.decoder.exact\endcsname{17105376}
\expandafter\gdef\csname R@an.stage_allocation.default.decoder.share\endcsname{54.96}
\expandafter\gdef\csname R@an.stage_allocation.default.fine.encoder.M\endcsname{0.840288}
\expandafter\gdef\csname R@an.stage_allocation.default.fine.encoder.M2\endcsname{0.84}
\expandafter\gdef\csname R@an.stage_allocation.default.fine.encoder.exact\endcsname{840288}
\expandafter\gdef\csname R@an.stage_allocation.default.fine.encoder.share\endcsname{2.70}
\expandafter\gdef\csname R@an.stage_allocation.default.heads.M\endcsname{0.012880}
\expandafter\gdef\csname R@an.stage_allocation.default.heads.M2\endcsname{0.01}
\expandafter\gdef\csname R@an.stage_allocation.default.heads.exact\endcsname{12880}
\expandafter\gdef\csname R@an.stage_allocation.default.heads.share\endcsname{0.04}
\expandafter\gdef\csname R@an.stage_allocation.default.total.M\endcsname{31.124368}
\expandafter\gdef\csname R@an.stage_allocation.default.total.M2\endcsname{31.12}
\expandafter\gdef\csname R@an.stage_allocation.default.total.exact\endcsname{31124368}
\expandafter\gdef\csname R@an.stage_allocation.fig.h\endcsname{2.68}
\expandafter\gdef\csname R@an.stage_allocation.fig.w\endcsname{6.79}
\expandafter\gdef\csname R@an.stage_allocation.heads.perarm.exact\endcsname{12880}
\expandafter\gdef\csname R@an.stage_allocation.n.arms\endcsname{5}
\expandafter\gdef\csname R@an.stagecost.V8B2.D0.gmac\endcsname{1.5}
\expandafter\gdef\csname R@an.stagecost.V8B2.D0.params\endcsname{3.59}
\expandafter\gdef\csname R@an.stagecost.V8B2.D0.pshare\endcsname{17.0}
\expandafter\gdef\csname R@an.stagecost.V8B2.D0.share\endcsname{0.7}
\expandafter\gdef\csname R@an.stagecost.V8B2.D1.gmac\endcsname{7.6}
\expandafter\gdef\csname R@an.stagecost.V8B2.D1.params\endcsname{2.43}
\expandafter\gdef\csname R@an.stagecost.V8B2.D1.pshare\endcsname{11.5}
\expandafter\gdef\csname R@an.stagecost.V8B2.D1.share\endcsname{3.8}
\expandafter\gdef\csname R@an.stagecost.V8B2.D2.gmac\endcsname{15.6}
\expandafter\gdef\csname R@an.stagecost.V8B2.D2.params\endcsname{0.71}
\expandafter\gdef\csname R@an.stagecost.V8B2.D2.pshare\endcsname{3.3}
\expandafter\gdef\csname R@an.stagecost.V8B2.D2.share\endcsname{7.8}
\expandafter\gdef\csname R@an.stagecost.V8B2.D3.gmac\endcsname{31.1}
\expandafter\gdef\csname R@an.stagecost.V8B2.D3.params\endcsname{0.18}
\expandafter\gdef\csname R@an.stagecost.V8B2.D3.pshare\endcsname{0.8}
\expandafter\gdef\csname R@an.stagecost.V8B2.D3.share\endcsname{15.6}
\expandafter\gdef\csname R@an.stagecost.V8B2.D4.gmac\endcsname{62.3}
\expandafter\gdef\csname R@an.stagecost.V8B2.D4.params\endcsname{0.04}
\expandafter\gdef\csname R@an.stagecost.V8B2.D4.pshare\endcsname{0.2}
\expandafter\gdef\csname R@an.stagecost.V8B2.D4.share\endcsname{31.3}
\expandafter\gdef\csname R@an.stagecost.V8B2.E0.gmac\endcsname{1.8}
\expandafter\gdef\csname R@an.stagecost.V8B2.E0.params\endcsname{0.00}
\expandafter\gdef\csname R@an.stagecost.V8B2.E0.pshare\endcsname{0.0}
\expandafter\gdef\csname R@an.stagecost.V8B2.E0.share\endcsname{0.9}
\expandafter\gdef\csname R@an.stagecost.V8B2.E1.gmac\endcsname{43.5}
\expandafter\gdef\csname R@an.stagecost.V8B2.E1.params\endcsname{0.17}
\expandafter\gdef\csname R@an.stagecost.V8B2.E1.pshare\endcsname{0.8}
\expandafter\gdef\csname R@an.stagecost.V8B2.E1.share\endcsname{21.8}
\expandafter\gdef\csname R@an.stagecost.V8B2.E2.gmac\endcsname{21.7}
\expandafter\gdef\csname R@an.stagecost.V8B2.E2.params\endcsname{0.66}
\expandafter\gdef\csname R@an.stagecost.V8B2.E2.pshare\endcsname{3.2}
\expandafter\gdef\csname R@an.stagecost.V8B2.E2.share\endcsname{10.9}
\expandafter\gdef\csname R@an.stagecost.V8B2.E3.gmac\endcsname{10.9}
\expandafter\gdef\csname R@an.stagecost.V8B2.E3.params\endcsname{2.66}
\expandafter\gdef\csname R@an.stagecost.V8B2.E3.pshare\endcsname{12.6}
\expandafter\gdef\csname R@an.stagecost.V8B2.E3.share\endcsname{5.5}
\expandafter\gdef\csname R@an.stagecost.V8B2.E4.gmac\endcsname{2.5}
\expandafter\gdef\csname R@an.stagecost.V8B2.E4.params\endcsname{4.98}
\expandafter\gdef\csname R@an.stagecost.V8B2.E4.pshare\endcsname{23.6}
\expandafter\gdef\csname R@an.stagecost.V8B2.E4.share\endcsname{1.3}
\expandafter\gdef\csname R@an.stagecost.V8B2.E5.gmac\endcsname{0.4}
\expandafter\gdef\csname R@an.stagecost.V8B2.E5.params\endcsname{5.68}
\expandafter\gdef\csname R@an.stagecost.V8B2.E5.pshare\endcsname{26.9}
\expandafter\gdef\csname R@an.stagecost.V8B2.E5.share\endcsname{0.2}
\expandafter\gdef\csname R@an.stagecost.V8B2.heads.gmac\endcsname{0.3}
\expandafter\gdef\csname R@an.stagecost.V8B2.heads.params\endcsname{0.00}
\expandafter\gdef\csname R@an.stagecost.V8B2.heads.pshare\endcsname{0.0}
\expandafter\gdef\csname R@an.stagecost.V8B2.heads.share\endcsname{0.1}
\expandafter\gdef\csname R@an.stagecost.V8B2.other.gmac\endcsname{0.0}
\expandafter\gdef\csname R@an.stagecost.V8B2.other.params\endcsname{0.00}
\expandafter\gdef\csname R@an.stagecost.V8B2.other.pshare\endcsname{0.0}
\expandafter\gdef\csname R@an.stagecost.V8B2.other.share\endcsname{0.0}
\expandafter\gdef\csname R@an.stagecost.V8B2.total.gmac\endcsname{199.1}
\expandafter\gdef\csname R@an.stagecost.V8B2.total.gmac_infer\endcsname{199.1}
\expandafter\gdef\csname R@an.stagecost.V8B2.total.params\endcsname{21.08}
\expandafter\gdef\csname R@an.stagecost.V8B2.total.paramsexact\endcsname{21\,084\,015}
\expandafter\gdef\csname R@an.stagecost.default.D0.gmac\endcsname{4.3}
\expandafter\gdef\csname R@an.stagecost.default.D0.params\endcsname{9.12}
\expandafter\gdef\csname R@an.stagecost.default.D0.pshare\endcsname{29.2}
\expandafter\gdef\csname R@an.stagecost.default.D0.share\endcsname{0.9}
\expandafter\gdef\csname R@an.stagecost.default.D1.gmac\endcsname{22.1}
\expandafter\gdef\csname R@an.stagecost.default.D1.params\endcsname{5.97}
\expandafter\gdef\csname R@an.stagecost.default.D1.pshare\endcsname{19.1}
\expandafter\gdef\csname R@an.stagecost.default.D1.share\endcsname{4.6}
\expandafter\gdef\csname R@an.stagecost.default.D2.gmac\endcsname{44.6}
\expandafter\gdef\csname R@an.stagecost.default.D2.params\endcsname{1.59}
\expandafter\gdef\csname R@an.stagecost.default.D2.pshare\endcsname{5.1}
\expandafter\gdef\csname R@an.stagecost.default.D2.share\endcsname{9.3}
\expandafter\gdef\csname R@an.stagecost.default.D3.gmac\endcsname{89.1}
\expandafter\gdef\csname R@an.stagecost.default.D3.params\endcsname{0.40}
\expandafter\gdef\csname R@an.stagecost.default.D3.pshare\endcsname{1.3}
\expandafter\gdef\csname R@an.stagecost.default.D3.share\endcsname{18.7}
\expandafter\gdef\csname R@an.stagecost.default.D4.gmac\endcsname{178.2}
\expandafter\gdef\csname R@an.stagecost.default.D4.params\endcsname{0.10}
\expandafter\gdef\csname R@an.stagecost.default.D4.pshare\endcsname{0.3}
\expandafter\gdef\csname R@an.stagecost.default.D4.share\endcsname{37.3}
\expandafter\gdef\csname R@an.stagecost.default.E0.gmac\endcsname{59.8}
\expandafter\gdef\csname R@an.stagecost.default.E0.params\endcsname{0.03}
\expandafter\gdef\csname R@an.stagecost.default.E0.pshare\endcsname{0.1}
\expandafter\gdef\csname R@an.stagecost.default.E0.share\endcsname{12.5}
\expandafter\gdef\csname R@an.stagecost.default.E1.gmac\endcsname{43.5}
\expandafter\gdef\csname R@an.stagecost.default.E1.params\endcsname{0.17}
\expandafter\gdef\csname R@an.stagecost.default.E1.pshare\endcsname{0.5}
\expandafter\gdef\csname R@an.stagecost.default.E1.share\endcsname{9.1}
\expandafter\gdef\csname R@an.stagecost.default.E2.gmac\endcsname{21.7}
\expandafter\gdef\csname R@an.stagecost.default.E2.params\endcsname{0.66}
\expandafter\gdef\csname R@an.stagecost.default.E2.pshare\endcsname{2.1}
\expandafter\gdef\csname R@an.stagecost.default.E2.share\endcsname{4.6}
\expandafter\gdef\csname R@an.stagecost.default.E3.gmac\endcsname{10.9}
\expandafter\gdef\csname R@an.stagecost.default.E3.params\endcsname{2.66}
\expandafter\gdef\csname R@an.stagecost.default.E3.pshare\endcsname{8.5}
\expandafter\gdef\csname R@an.stagecost.default.E3.share\endcsname{2.3}
\expandafter\gdef\csname R@an.stagecost.default.E4.gmac\endcsname{2.5}
\expandafter\gdef\csname R@an.stagecost.default.E4.params\endcsname{4.98}
\expandafter\gdef\csname R@an.stagecost.default.E4.pshare\endcsname{16.0}
\expandafter\gdef\csname R@an.stagecost.default.E4.share\endcsname{0.5}
\expandafter\gdef\csname R@an.stagecost.default.E5.gmac\endcsname{0.4}
\expandafter\gdef\csname R@an.stagecost.default.E5.params\endcsname{5.53}
\expandafter\gdef\csname R@an.stagecost.default.E5.pshare\endcsname{17.7}
\expandafter\gdef\csname R@an.stagecost.default.E5.share\endcsname{0.1}
\expandafter\gdef\csname R@an.stagecost.default.heads.gmac\endcsname{0.3}
\expandafter\gdef\csname R@an.stagecost.default.heads.params\endcsname{0.00}
\expandafter\gdef\csname R@an.stagecost.default.heads.pshare\endcsname{0.0}
\expandafter\gdef\csname R@an.stagecost.default.heads.share\endcsname{0.1}
\expandafter\gdef\csname R@an.stagecost.default.other.gmac\endcsname{0.0}
\expandafter\gdef\csname R@an.stagecost.default.other.params\endcsname{0.00}
\expandafter\gdef\csname R@an.stagecost.default.other.pshare\endcsname{0.0}
\expandafter\gdef\csname R@an.stagecost.default.other.share\endcsname{0.0}
\expandafter\gdef\csname R@an.stagecost.default.total.gmac\endcsname{477.4}
\expandafter\gdef\csname R@an.stagecost.default.total.gmac_infer\endcsname{477.3}
\expandafter\gdef\csname R@an.stagecost.default.total.params\endcsname{31.20}
\expandafter\gdef\csname R@an.stagecost.default.total.paramsexact\endcsname{31\,196\,399}
\expandafter\gdef\csname R@an.stagecost.fine2.default.gmac\endcsname{56.0}
\expandafter\gdef\csname R@an.stagecost.fine2.default.params\endcsname{1.6}
\expandafter\gdef\csname R@an.stagecost.fine2.kept\endcsname{34.9}
\expandafter\gdef\csname R@an.stagecost.fine2.keptp\endcsname{44.3}
\expandafter\gdef\csname R@an.stagecost.fine2.xl.gmac\endcsname{36.3}
\expandafter\gdef\csname R@an.stagecost.fine2.xl.params\endcsname{1.0}
\expandafter\gdef\csname R@an.stagecost.sentence\endcsname{the two finest decoder stages hold 1.6\,\% of nnU-Net's parameters and 56.0\,\% of its multiply-adds on the KiTS23 plan; {\ifdefined\archL\archL\else XX-Net-L\fi} keeps 34.9\,\% of those multiply-adds (36.3\,\% of its own) and 44.3\,\% of those parameters}
\expandafter\gdef\csname R@an.stagecost.xl.D0.gmac\endcsname{1.5}
\expandafter\gdef\csname R@an.stagecost.xl.D0.params\endcsname{3.59}
\expandafter\gdef\csname R@an.stagecost.xl.D0.pshare\endcsname{17.0}
\expandafter\gdef\csname R@an.stagecost.xl.D0.share\endcsname{0.6}
\expandafter\gdef\csname R@an.stagecost.xl.D1.gmac\endcsname{7.6}
\expandafter\gdef\csname R@an.stagecost.xl.D1.params\endcsname{2.43}
\expandafter\gdef\csname R@an.stagecost.xl.D1.pshare\endcsname{11.5}
\expandafter\gdef\csname R@an.stagecost.xl.D1.share\endcsname{2.9}
\expandafter\gdef\csname R@an.stagecost.xl.D2.gmac\endcsname{15.6}
\expandafter\gdef\csname R@an.stagecost.xl.D2.params\endcsname{0.71}
\expandafter\gdef\csname R@an.stagecost.xl.D2.pshare\endcsname{3.3}
\expandafter\gdef\csname R@an.stagecost.xl.D2.share\endcsname{6.1}
\expandafter\gdef\csname R@an.stagecost.xl.D3.gmac\endcsname{31.1}
\expandafter\gdef\csname R@an.stagecost.xl.D3.params\endcsname{0.18}
\expandafter\gdef\csname R@an.stagecost.xl.D3.pshare\endcsname{0.8}
\expandafter\gdef\csname R@an.stagecost.xl.D3.share\endcsname{12.1}
\expandafter\gdef\csname R@an.stagecost.xl.D4.gmac\endcsname{62.3}
\expandafter\gdef\csname R@an.stagecost.xl.D4.params\endcsname{0.04}
\expandafter\gdef\csname R@an.stagecost.xl.D4.pshare\endcsname{0.2}
\expandafter\gdef\csname R@an.stagecost.xl.D4.share\endcsname{24.2}
\expandafter\gdef\csname R@an.stagecost.xl.E0.gmac\endcsname{59.8}
\expandafter\gdef\csname R@an.stagecost.xl.E0.params\endcsname{0.03}
\expandafter\gdef\csname R@an.stagecost.xl.E0.pshare\endcsname{0.1}
\expandafter\gdef\csname R@an.stagecost.xl.E0.share\endcsname{23.3}
\expandafter\gdef\csname R@an.stagecost.xl.E1.gmac\endcsname{43.5}
\expandafter\gdef\csname R@an.stagecost.xl.E1.params\endcsname{0.17}
\expandafter\gdef\csname R@an.stagecost.xl.E1.pshare\endcsname{0.8}
\expandafter\gdef\csname R@an.stagecost.xl.E1.share\endcsname{16.9}
\expandafter\gdef\csname R@an.stagecost.xl.E2.gmac\endcsname{21.7}
\expandafter\gdef\csname R@an.stagecost.xl.E2.params\endcsname{0.66}
\expandafter\gdef\csname R@an.stagecost.xl.E2.pshare\endcsname{3.1}
\expandafter\gdef\csname R@an.stagecost.xl.E2.share\endcsname{8.5}
\expandafter\gdef\csname R@an.stagecost.xl.E3.gmac\endcsname{10.9}
\expandafter\gdef\csname R@an.stagecost.xl.E3.params\endcsname{2.66}
\expandafter\gdef\csname R@an.stagecost.xl.E3.pshare\endcsname{12.6}
\expandafter\gdef\csname R@an.stagecost.xl.E3.share\endcsname{4.2}
\expandafter\gdef\csname R@an.stagecost.xl.E4.gmac\endcsname{2.5}
\expandafter\gdef\csname R@an.stagecost.xl.E4.params\endcsname{4.98}
\expandafter\gdef\csname R@an.stagecost.xl.E4.pshare\endcsname{23.6}
\expandafter\gdef\csname R@an.stagecost.xl.E4.share\endcsname{1.0}
\expandafter\gdef\csname R@an.stagecost.xl.E5.gmac\endcsname{0.4}
\expandafter\gdef\csname R@an.stagecost.xl.E5.params\endcsname{5.68}
\expandafter\gdef\csname R@an.stagecost.xl.E5.pshare\endcsname{26.9}
\expandafter\gdef\csname R@an.stagecost.xl.E5.share\endcsname{0.1}
\expandafter\gdef\csname R@an.stagecost.xl.heads.gmac\endcsname{0.3}
\expandafter\gdef\csname R@an.stagecost.xl.heads.params\endcsname{0.00}
\expandafter\gdef\csname R@an.stagecost.xl.heads.pshare\endcsname{0.0}
\expandafter\gdef\csname R@an.stagecost.xl.heads.share\endcsname{0.1}
\expandafter\gdef\csname R@an.stagecost.xl.other.gmac\endcsname{0.0}
\expandafter\gdef\csname R@an.stagecost.xl.other.params\endcsname{0.00}
\expandafter\gdef\csname R@an.stagecost.xl.other.pshare\endcsname{0.0}
\expandafter\gdef\csname R@an.stagecost.xl.other.share\endcsname{0.0}
\expandafter\gdef\csname R@an.stagecost.xl.tag\endcsname{V7C1}
\expandafter\gdef\csname R@an.stagecost.xl.total.gmac\endcsname{257.1}
\expandafter\gdef\csname R@an.stagecost.xl.total.gmac_infer\endcsname{257.0}
\expandafter\gdef\csname R@an.stagecost.xl.total.params\endcsname{21.11}
\expandafter\gdef\csname R@an.stagecost.xl.total.paramsexact\endcsname{21\,111\,759}
\expandafter\gdef\csname R@an.stockref.amos.L1.delta_pool\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.stockref.amos.L1.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L1.delta_stock\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.stockref.amos.L1.incl0.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L1.incl0.delta_stock\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.stockref.amos.L1.incl0.mean\endcsname{88.23}
\expandafter\gdef\csname R@an.stockref.amos.L1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L1.incl0.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L1.incl0.se_stock\endcsname{0.10}
\expandafter\gdef\csname R@an.stockref.amos.L1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of ResEnc-M on AMOS22 fold 0 is 88.23 Dice: \ensuremath{+0.51}\,pp from the stock mean (SE 0.10, 3 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.L1.mean\endcsname{88.17}
\expandafter\gdef\csname R@an.stockref.amos.L1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.amos.L1.n_reb\endcsname{0}
\expandafter\gdef\csname R@an.stockref.amos.L1.n_stock\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L1.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L1.se_stock\endcsname{0.11}
\expandafter\gdef\csname R@an.stockref.amos.L1.sentence\endcsname{on AMOS22 fold 0 the mean of fresh seeds 1 and 2 of ResEnc-M is 88.17 Dice: \ensuremath{+0.45}\,pp from the stock mean (SE 0.11, 2 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.L1b.delta_pool\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.stockref.amos.L1b.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L1b.delta_stock\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.stockref.amos.L1b.incl0.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L1b.incl0.delta_stock\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.stockref.amos.L1b.incl0.mean\endcsname{87.95}
\expandafter\gdef\csname R@an.stockref.amos.L1b.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L1b.incl0.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L1b.incl0.se_stock\endcsname{0.10}
\expandafter\gdef\csname R@an.stockref.amos.L1b.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of ResEnc-matched on AMOS22 fold 0 is 87.95 Dice: \ensuremath{+0.23}\,pp from the stock mean (SE 0.10, 3 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.L1b.mean\endcsname{88.00}
\expandafter\gdef\csname R@an.stockref.amos.L1b.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.amos.L1b.n_reb\endcsname{0}
\expandafter\gdef\csname R@an.stockref.amos.L1b.n_stock\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L1b.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L1b.se_stock\endcsname{0.11}
\expandafter\gdef\csname R@an.stockref.amos.L1b.sentence\endcsname{on AMOS22 fold 0 the mean of fresh seeds 1 and 2 of ResEnc-matched is 88.00 Dice: \ensuremath{+0.29}\,pp from the stock mean (SE 0.11, 2 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.L2.delta_pool\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.stockref.amos.L2.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L2.delta_stock\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.stockref.amos.L2.incl0.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L2.incl0.delta_stock\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.stockref.amos.L2.incl0.mean\endcsname{87.95}
\expandafter\gdef\csname R@an.stockref.amos.L2.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L2.incl0.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L2.incl0.se_stock\endcsname{0.10}
\expandafter\gdef\csname R@an.stockref.amos.L2.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of ConvNeXt-k3 on AMOS22 fold 0 is 87.95 Dice: \ensuremath{+0.24}\,pp from the stock mean (SE 0.10, 3 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.L2.mean\endcsname{87.90}
\expandafter\gdef\csname R@an.stockref.amos.L2.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.amos.L2.n_reb\endcsname{0}
\expandafter\gdef\csname R@an.stockref.amos.L2.n_stock\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L2.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L2.se_stock\endcsname{0.11}
\expandafter\gdef\csname R@an.stockref.amos.L2.sentence\endcsname{on AMOS22 fold 0 the mean of fresh seeds 1 and 2 of ConvNeXt-k3 is 87.90 Dice: \ensuremath{+0.18}\,pp from the stock mean (SE 0.11, 2 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.L3.delta_pool\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.stockref.amos.L3.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L3.delta_stock\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.stockref.amos.L3.incl0.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L3.incl0.delta_stock\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.stockref.amos.L3.incl0.mean\endcsname{87.92}
\expandafter\gdef\csname R@an.stockref.amos.L3.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L3.incl0.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L3.incl0.se_stock\endcsname{0.10}
\expandafter\gdef\csname R@an.stockref.amos.L3.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of HyReX on AMOS22 fold 0 is 87.92 Dice: \ensuremath{+0.20}\,pp from the stock mean (SE 0.10, 3 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.L3.mean\endcsname{87.83}
\expandafter\gdef\csname R@an.stockref.amos.L3.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.amos.L3.n_reb\endcsname{0}
\expandafter\gdef\csname R@an.stockref.amos.L3.n_stock\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L3.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L3.se_stock\endcsname{0.11}
\expandafter\gdef\csname R@an.stockref.amos.L3.sentence\endcsname{on AMOS22 fold 0 the mean of fresh seeds 1 and 2 of HyReX is 87.83 Dice: \ensuremath{+0.12}\,pp from the stock mean (SE 0.11, 2 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.L4.delta_pool\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.stockref.amos.L4.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L4.delta_stock\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.stockref.amos.L4.incl0.delta_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L4.incl0.delta_stock\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.stockref.amos.L4.incl0.mean\endcsname{88.15}
\expandafter\gdef\csname R@an.stockref.amos.L4.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L4.incl0.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L4.incl0.se_stock\endcsname{0.10}
\expandafter\gdef\csname R@an.stockref.amos.L4.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of ResEnc+context on AMOS22 fold 0 is 88.15 Dice: \ensuremath{+0.44}\,pp from the stock mean (SE 0.10, 3 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.L4.mean\endcsname{88.16}
\expandafter\gdef\csname R@an.stockref.amos.L4.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.amos.L4.n_reb\endcsname{0}
\expandafter\gdef\csname R@an.stockref.amos.L4.n_stock\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.L4.se_reb\endcsname{\pend}
\expandafter\gdef\csname R@an.stockref.amos.L4.se_stock\endcsname{0.11}
\expandafter\gdef\csname R@an.stockref.amos.L4.sentence\endcsname{on AMOS22 fold 0 the mean of fresh seeds 1 and 2 of ResEnc+context is 88.16 Dice: \ensuremath{+0.44}\,pp from the stock mean (SE 0.11, 2 runs against 3), and no finished run of the rebuild reference yet}
\expandafter\gdef\csname R@an.stockref.amos.arms\endcsname{L1, L1b, L2, L3, L4}
\expandafter\gdef\csname R@an.stockref.amos.pool.mean\endcsname{87.70}
\expandafter\gdef\csname R@an.stockref.amos.pool.n\endcsname{6}
\expandafter\gdef\csname R@an.stockref.amos.reb.n\endcsname{0}
\expandafter\gdef\csname R@an.stockref.amos.stock.mean\endcsname{87.71}
\expandafter\gdef\csname R@an.stockref.amos.stock.n\endcsname{3}
\expandafter\gdef\csname R@an.stockref.amos.stock.sd\endcsname{0.12}
\expandafter\gdef\csname R@an.stockref.amos.stock.seeds\endcsname{3--5}
\expandafter\gdef\csname R@an.stockref.amos.stock.sentence\endcsname{the stock reference of AMOS22 fold 0 is the mean of the 3 finished plain-default runs (seeds 3--5) of the harness, 87.71 Dice (SD 0.12), \ensuremath{+0.01}\,pp from the frozen pool of 6 runs (87.70); the pool and its sub-pools are not part of it}
\expandafter\gdef\csname R@an.stockref.amos.stock.vspool\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.stockref.kits.C1.delta_pool\endcsname{\ensuremath{+2.40}}
\expandafter\gdef\csname R@an.stockref.kits.C1.delta_reb\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@an.stockref.kits.C1.delta_stock\endcsname{\ensuremath{+1.52}}
\expandafter\gdef\csname R@an.stockref.kits.C1.incl0.delta_reb\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.stockref.kits.C1.incl0.delta_stock\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.stockref.kits.C1.incl0.mean\endcsname{86.15}
\expandafter\gdef\csname R@an.stockref.kits.C1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.C1.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.C1.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.C1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of HyReX+dec. capacity on KiTS23 fold 0 is 86.15 Dice: \ensuremath{+1.89}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+1.48}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.C1.mean\endcsname{85.78}
\expandafter\gdef\csname R@an.stockref.kits.C1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.C1.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.C1.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.C1.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.C1.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.C1.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of HyReX+dec. capacity is 85.78 Dice: \ensuremath{+1.52}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+1.11}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.D1.delta_pool\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.stockref.kits.D1.delta_reb\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.stockref.kits.D1.delta_stock\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.stockref.kits.D1.incl0.delta_reb\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.stockref.kits.D1.incl0.delta_stock\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.stockref.kits.D1.incl0.mean\endcsname{84.90}
\expandafter\gdef\csname R@an.stockref.kits.D1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.D1.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.D1.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.D1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of HyReX point-fuse on KiTS23 fold 0 is 84.90 Dice: \ensuremath{+0.64}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.23}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.D1.mean\endcsname{84.85}
\expandafter\gdef\csname R@an.stockref.kits.D1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.D1.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.D1.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.D1.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.D1.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.D1.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of HyReX point-fuse is 84.85 Dice: \ensuremath{+0.60}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.18}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.D2.delta_pool\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.stockref.kits.D2.delta_reb\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.stockref.kits.D2.delta_stock\endcsname{\ensuremath{+1.01}}
\expandafter\gdef\csname R@an.stockref.kits.D2.incl0.delta_reb\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.stockref.kits.D2.incl0.delta_stock\endcsname{\ensuremath{+1.17}}
\expandafter\gdef\csname R@an.stockref.kits.D2.incl0.mean\endcsname{85.42}
\expandafter\gdef\csname R@an.stockref.kits.D2.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.D2.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.D2.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.D2.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of LeanDec on KiTS23 fold 0 is 85.42 Dice: \ensuremath{+1.17}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.75}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.D2.mean\endcsname{85.27}
\expandafter\gdef\csname R@an.stockref.kits.D2.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.D2.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.D2.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.D2.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.D2.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.D2.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of LeanDec is 85.27 Dice: \ensuremath{+1.01}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.60}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L1.delta_pool\endcsname{\ensuremath{+3.48}}
\expandafter\gdef\csname R@an.stockref.kits.L1.delta_reb\endcsname{\ensuremath{+2.18}}
\expandafter\gdef\csname R@an.stockref.kits.L1.delta_stock\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@an.stockref.kits.L1.incl0.delta_reb\endcsname{\ensuremath{+1.80}}
\expandafter\gdef\csname R@an.stockref.kits.L1.incl0.delta_stock\endcsname{\ensuremath{+2.21}}
\expandafter\gdef\csname R@an.stockref.kits.L1.incl0.mean\endcsname{86.47}
\expandafter\gdef\csname R@an.stockref.kits.L1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.L1.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L1.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.L1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of ResEnc-M on KiTS23 fold 0 is 86.47 Dice: \ensuremath{+2.21}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+1.80}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L1.mean\endcsname{86.85}
\expandafter\gdef\csname R@an.stockref.kits.L1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.L1.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.L1.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.L1.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.L1.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L1.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of ResEnc-M is 86.85 Dice: \ensuremath{+2.60}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+2.18}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L1b.delta_pool\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@an.stockref.kits.L1b.delta_reb\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.stockref.kits.L1b.delta_stock\endcsname{\ensuremath{+1.43}}
\expandafter\gdef\csname R@an.stockref.kits.L1b.incl0.delta_reb\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@an.stockref.kits.L1b.incl0.delta_stock\endcsname{\ensuremath{+1.24}}
\expandafter\gdef\csname R@an.stockref.kits.L1b.incl0.mean\endcsname{85.50}
\expandafter\gdef\csname R@an.stockref.kits.L1b.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.L1b.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L1b.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.L1b.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of ResEnc-matched on KiTS23 fold 0 is 85.50 Dice: \ensuremath{+1.24}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.83}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L1b.mean\endcsname{85.69}
\expandafter\gdef\csname R@an.stockref.kits.L1b.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.L1b.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.L1b.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.L1b.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.L1b.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L1b.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of ResEnc-matched is 85.69 Dice: \ensuremath{+1.43}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+1.02}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L2.delta_pool\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.stockref.kits.L2.delta_reb\endcsname{\ensuremath{-1.18}}
\expandafter\gdef\csname R@an.stockref.kits.L2.delta_stock\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.stockref.kits.L2.incl0.delta_reb\endcsname{\ensuremath{-1.00}}
\expandafter\gdef\csname R@an.stockref.kits.L2.incl0.delta_stock\endcsname{\ensuremath{-0.58}}
\expandafter\gdef\csname R@an.stockref.kits.L2.incl0.mean\endcsname{83.67}
\expandafter\gdef\csname R@an.stockref.kits.L2.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.L2.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L2.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.L2.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of ConvNeXt-k3 on KiTS23 fold 0 is 83.67 Dice: \ensuremath{-0.58}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{-1.00}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L2.mean\endcsname{83.49}
\expandafter\gdef\csname R@an.stockref.kits.L2.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.L2.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.L2.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.L2.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.L2.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L2.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of ConvNeXt-k3 is 83.49 Dice: \ensuremath{-0.77}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{-1.18}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L3.delta_pool\endcsname{\ensuremath{+2.09}}
\expandafter\gdef\csname R@an.stockref.kits.L3.delta_reb\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.stockref.kits.L3.delta_stock\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.stockref.kits.L3.incl0.delta_reb\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.stockref.kits.L3.incl0.delta_stock\endcsname{\ensuremath{+1.46}}
\expandafter\gdef\csname R@an.stockref.kits.L3.incl0.mean\endcsname{85.72}
\expandafter\gdef\csname R@an.stockref.kits.L3.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.L3.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L3.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.L3.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of HyReX on KiTS23 fold 0 is 85.72 Dice: \ensuremath{+1.46}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+1.05}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L3.mean\endcsname{85.47}
\expandafter\gdef\csname R@an.stockref.kits.L3.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.L3.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.L3.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.L3.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.L3.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L3.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of HyReX is 85.47 Dice: \ensuremath{+1.21}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.80}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L4.delta_pool\endcsname{\ensuremath{+2.25}}
\expandafter\gdef\csname R@an.stockref.kits.L4.delta_reb\endcsname{\ensuremath{+0.95}}
\expandafter\gdef\csname R@an.stockref.kits.L4.delta_stock\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.stockref.kits.L4.incl0.delta_reb\endcsname{\ensuremath{+0.94}}
\expandafter\gdef\csname R@an.stockref.kits.L4.incl0.delta_stock\endcsname{\ensuremath{+1.35}}
\expandafter\gdef\csname R@an.stockref.kits.L4.incl0.mean\endcsname{85.61}
\expandafter\gdef\csname R@an.stockref.kits.L4.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.L4.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L4.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.L4.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of ResEnc+context on KiTS23 fold 0 is 85.61 Dice: \ensuremath{+1.35}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.94}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L4.mean\endcsname{85.62}
\expandafter\gdef\csname R@an.stockref.kits.L4.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.L4.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.L4.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.L4.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.L4.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L4.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of ResEnc+context is 85.62 Dice: \ensuremath{+1.37}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.95}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L6.delta_pool\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.stockref.kits.L6.delta_reb\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.stockref.kits.L6.delta_stock\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.stockref.kits.L6.incl0.delta_reb\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.stockref.kits.L6.incl0.delta_stock\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.stockref.kits.L6.incl0.mean\endcsname{85.28}
\expandafter\gdef\csname R@an.stockref.kits.L6.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.L6.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L6.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.L6.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of HyReX+context on KiTS23 fold 0 is 85.28 Dice: \ensuremath{+1.02}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.61}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.L6.mean\endcsname{84.97}
\expandafter\gdef\csname R@an.stockref.kits.L6.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.L6.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.L6.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.L6.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.L6.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.L6.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of HyReX+context is 84.97 Dice: \ensuremath{+0.71}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.30}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.P3c.delta_pool\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@an.stockref.kits.P3c.delta_reb\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.stockref.kits.P3c.delta_stock\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.stockref.kits.P3c.incl0.delta_reb\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.stockref.kits.P3c.incl0.delta_stock\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.stockref.kits.P3c.incl0.mean\endcsname{84.62}
\expandafter\gdef\csname R@an.stockref.kits.P3c.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.P3c.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.P3c.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.P3c.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of fn.-identical control on KiTS23 fold 0 is 84.62 Dice: \ensuremath{+0.36}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{-0.05}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.P3c.mean\endcsname{84.55}
\expandafter\gdef\csname R@an.stockref.kits.P3c.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.P3c.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.P3c.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.P3c.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.P3c.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.P3c.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of fn.-identical control is 84.55 Dice: \ensuremath{+0.30}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{-0.12}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.S2.delta_pool\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.stockref.kits.S2.delta_reb\endcsname{\ensuremath{-0.72}}
\expandafter\gdef\csname R@an.stockref.kits.S2.delta_stock\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.stockref.kits.S2.incl0.delta_reb\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.stockref.kits.S2.incl0.delta_stock\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@an.stockref.kits.S2.incl0.mean\endcsname{84.21}
\expandafter\gdef\csname R@an.stockref.kits.S2.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.S2.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.S2.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.S2.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of HyReX, finer ConvNeXt on KiTS23 fold 0 is 84.21 Dice: \ensuremath{-0.05}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{-0.47}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.S2.mean\endcsname{83.95}
\expandafter\gdef\csname R@an.stockref.kits.S2.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.S2.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.S2.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.S2.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.S2.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.S2.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of HyReX, finer ConvNeXt is 83.95 Dice: \ensuremath{-0.31}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{-0.72}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.delta_pool\endcsname{\ensuremath{+2.17}}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.delta_reb\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.delta_stock\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.incl0.delta_reb\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.incl0.delta_stock\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.incl0.mean\endcsname{85.47}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of HyReX-LeanDec on KiTS23 fold 0 is 85.47 Dice: \ensuremath{+1.21}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.80}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.mean\endcsname{85.54}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V5A5.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of HyReX-LeanDec is 85.54 Dice: \ensuremath{+1.29}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.87}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.delta_pool\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.delta_reb\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.delta_stock\endcsname{\ensuremath{+1.41}}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.incl0.delta_reb\endcsname{\ensuremath{+0.95}}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.incl0.delta_stock\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.incl0.mean\endcsname{85.62}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of LeanAdd on KiTS23 fold 0 is 85.62 Dice: \ensuremath{+1.37}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.95}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.mean\endcsname{85.66}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V5B1.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of LeanAdd is 85.66 Dice: \ensuremath{+1.41}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.99}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.delta_pool\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.delta_reb\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.delta_stock\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.incl0.delta_reb\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.incl0.delta_stock\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.incl0.mean\endcsname{84.77}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of LeanAdd-NeXt on KiTS23 fold 0 is 84.77 Dice: \ensuremath{+0.51}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.09}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.mean\endcsname{84.83}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V5B2.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of LeanAdd-NeXt is 84.83 Dice: \ensuremath{+0.57}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.16}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.delta_pool\endcsname{\ensuremath{+1.70}}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.delta_reb\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.delta_stock\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.incl0.delta_reb\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.incl0.delta_stock\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.incl0.mean\endcsname{85.26}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of HyReX-k9 on KiTS23 fold 0 is 85.26 Dice: \ensuremath{+1.00}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.59}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.mean\endcsname{85.08}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V6A1r.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of HyReX-k9 is 85.08 Dice: \ensuremath{+0.82}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.41}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.delta_pool\endcsname{\ensuremath{+2.66}}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.delta_reb\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.delta_stock\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.incl0.delta_reb\endcsname{\ensuremath{+1.33}}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.incl0.delta_stock\endcsname{\ensuremath{+1.74}}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.incl0.mean\endcsname{86.00}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of {\ifdefined\archA\archA\else XX-Net-A\fi} on KiTS23 fold 0 is 86.00 Dice: \ensuremath{+1.74}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+1.33}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.mean\endcsname{86.04}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7A1.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of {\ifdefined\archA\archA\else XX-Net-A\fi} is 86.04 Dice: \ensuremath{+1.78}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+1.37}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.delta_pool\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.delta_reb\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.delta_stock\endcsname{\ensuremath{+1.41}}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.incl0.delta_reb\endcsname{\ensuremath{+1.20}}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.incl0.delta_stock\endcsname{\ensuremath{+1.61}}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.incl0.mean\endcsname{85.87}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of LeanDeepMid+FD on KiTS23 fold 0 is 85.87 Dice: \ensuremath{+1.61}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+1.20}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.mean\endcsname{85.67}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7A2.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of LeanDeepMid+FD is 85.67 Dice: \ensuremath{+1.41}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+1.00}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.delta_pool\endcsname{\ensuremath{+2.38}}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.delta_reb\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.delta_stock\endcsname{\ensuremath{+1.50}}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.incl0.delta_reb\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.incl0.delta_stock\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.incl0.mean\endcsname{85.54}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of LeanSep on KiTS23 fold 0 is 85.54 Dice: \ensuremath{+1.28}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.87}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.mean\endcsname{85.76}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7B1.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of LeanSep is 85.76 Dice: \ensuremath{+1.50}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+1.09}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.delta_pool\endcsname{\ensuremath{+1.84}}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.delta_reb\endcsname{\ensuremath{+0.55}}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.delta_stock\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.incl0.delta_reb\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.incl0.delta_stock\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.incl0.mean\endcsname{85.55}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of LeanDil on KiTS23 fold 0 is 85.55 Dice: \ensuremath{+1.29}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.87}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.mean\endcsname{85.22}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7B2.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of LeanDil is 85.22 Dice: \ensuremath{+0.96}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.55}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.delta_pool\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.delta_reb\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.delta_stock\endcsname{\ensuremath{+1.56}}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.incl0.delta_reb\endcsname{\ensuremath{+1.24}}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.incl0.delta_stock\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.incl0.mean\endcsname{85.91}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of {\ifdefined\archL\archL\else XX-Net-L\fi} on KiTS23 fold 0 is 85.91 Dice: \ensuremath{+1.65}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+1.24}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.mean\endcsname{85.82}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V7C1.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of {\ifdefined\archL\archL\else XX-Net-L\fi} is 85.82 Dice: \ensuremath{+1.56}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+1.15}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.delta_pool\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.delta_reb\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.delta_stock\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.incl0.delta_reb\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.incl0.delta_stock\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.incl0.mean\endcsname{84.80}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of CoarseStack on KiTS23 fold 0 is 84.80 Dice: \ensuremath{+0.54}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.13}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.mean\endcsname{84.63}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V8A1.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of CoarseStack is 84.63 Dice: \ensuremath{+0.37}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{-0.04}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.delta_pool\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.delta_reb\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.delta_stock\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.incl0.delta_reb\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.incl0.delta_stock\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.incl0.mean\endcsname{85.08}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of StackDec on KiTS23 fold 0 is 85.08 Dice: \ensuremath{+0.82}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.41}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.mean\endcsname{85.26}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V8A2.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of StackDec is 85.26 Dice: \ensuremath{+1.00}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.58}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.delta_pool\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.delta_reb\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.delta_stock\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.incl0.delta_reb\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.incl0.delta_stock\endcsname{\ensuremath{+1.01}}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.incl0.mean\endcsname{85.26}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of LeanTrunk on KiTS23 fold 0 is 85.26 Dice: \ensuremath{+1.01}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.59}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.mean\endcsname{84.75}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V8B1.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of LeanTrunk is 84.75 Dice: \ensuremath{+0.50}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.08}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.delta_pool\endcsname{\ensuremath{+1.73}}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.delta_reb\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.delta_stock\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.incl0.delta_reb\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.incl0.delta_stock\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.incl0.mean\endcsname{85.08}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of Stem1 on KiTS23 fold 0 is 85.08 Dice: \ensuremath{+0.82}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.41}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.mean\endcsname{85.11}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.V8B2.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of Stem1 is 85.11 Dice: \ensuremath{+0.85}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{+0.44}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.W1c.delta_pool\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@an.stockref.kits.W1c.delta_reb\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.stockref.kits.W1c.delta_stock\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.stockref.kits.W1c.incl0.delta_reb\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.stockref.kits.W1c.incl0.delta_stock\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.stockref.kits.W1c.incl0.mean\endcsname{84.97}
\expandafter\gdef\csname R@an.stockref.kits.W1c.incl0.n_arm\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.W1c.incl0.se_reb\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.W1c.incl0.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.stockref.kits.W1c.incl0.sentence\endcsname{with the discovery seed included (seeds 0, 1 and 2) the mean of branch control on KiTS23 fold 0 is 84.97 Dice: \ensuremath{+0.71}\,pp from the stock mean (SE 0.42, 3 runs against 9), and \ensuremath{+0.30}\,pp from the mean of the function-identical rebuild (SE 0.49, 3 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.W1c.mean\endcsname{84.44}
\expandafter\gdef\csname R@an.stockref.kits.W1c.n_arm\endcsname{2}
\expandafter\gdef\csname R@an.stockref.kits.W1c.n_reb\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.W1c.n_stock\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.W1c.se_reb\endcsname{0.55}
\expandafter\gdef\csname R@an.stockref.kits.W1c.se_stock\endcsname{0.49}
\expandafter\gdef\csname R@an.stockref.kits.W1c.sentence\endcsname{on KiTS23 fold 0 the mean of fresh seeds 1 and 2 of branch control is 84.44 Dice: \ensuremath{+0.19}\,pp from the stock mean (SE 0.49, 2 runs against 9), and \ensuremath{-0.23}\,pp from the mean of the function-identical rebuild (SE 0.55, 2 runs against 5)}
\expandafter\gdef\csname R@an.stockref.kits.arms\endcsname{C1, D1, D2, L1, L1b, L2, L3, L4, L6, P3c, S2, V5A5, V5B1, V5B2, V6A1r, V7A1, V7A2, V7B1, V7B2, V7C1, V8A1, V8A2, V8B1, V8B2, W1c}
\expandafter\gdef\csname R@an.stockref.kits.pool.mean\endcsname{83.38}
\expandafter\gdef\csname R@an.stockref.kits.pool.n\endcsname{3}
\expandafter\gdef\csname R@an.stockref.kits.reb.mean\endcsname{84.67}
\expandafter\gdef\csname R@an.stockref.kits.reb.n\endcsname{5}
\expandafter\gdef\csname R@an.stockref.kits.reb.sd\endcsname{0.72}
\expandafter\gdef\csname R@an.stockref.kits.reb.seeds\endcsname{3--7}
\expandafter\gdef\csname R@an.stockref.kits.reb.vspool\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.stockref.kits.reb.vsstock\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@an.stockref.kits.stock.mean\endcsname{84.26}
\expandafter\gdef\csname R@an.stockref.kits.stock.n\endcsname{9}
\expandafter\gdef\csname R@an.stockref.kits.stock.sd\endcsname{0.63}
\expandafter\gdef\csname R@an.stockref.kits.stock.seeds\endcsname{3--11}
\expandafter\gdef\csname R@an.stockref.kits.stock.sentence\endcsname{the stock reference of KiTS23 fold 0 is the mean of the 9 finished plain-default runs (seeds 3--11) of the harness, 84.26 Dice (SD 0.63), \ensuremath{+0.88}\,pp from the frozen pool of 3 runs (83.38); the pool and its sub-pools are not part of it}
\expandafter\gdef\csname R@an.stockref.kits.stock.vspool\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.stockref.rule\endcsname{the standard error is the Welch form sqrt(s_arm^2/n_arm + s_ref^2/n_ref) of a difference of two means, with the arm's SD taken as the SD of the stock runs (an arm's own SD of two or three runs, one of them the selected discovery run, is not a run-level SD) and the reference's SD its own; it describes how far two means of that many runs can differ through run-to-run variation of the recipe alone, and states no inference}
\expandafter\gdef\csname R@an.stockref.state\endcsname{KiTS23: 25 of 46 arms with a fresh pair, 9 stock runs, 5 rebuild runs, AMOS22: 5 of 46 arms with a fresh pair, 3 stock runs, 0 rebuild runs}
\expandafter\gdef\csname R@an.strata_amos.L1.cs.d\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@an.strata_amos.L1.cs.hi\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.strata_amos.L1.cs.lo\endcsname{\ensuremath{-2.18}}
\expandafter\gdef\csname R@an.strata_amos.L1.cs.ne.d\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.strata_amos.L1.cs.ne.hi\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@an.strata_amos.L1.cs.ne.lo\endcsname{\ensuremath{-0.63}}
\expandafter\gdef\csname R@an.strata_amos.L1.ct.d\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.strata_amos.L1.ct.hi\endcsname{\ensuremath{+1.70}}
\expandafter\gdef\csname R@an.strata_amos.L1.ct.lo\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.strata_amos.L1.ct.ne.d\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.strata_amos.L1.ct.ne.hi\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.strata_amos.L1.ct.ne.lo\endcsname{\ensuremath{-0.67}}
\expandafter\gdef\csname R@an.strata_amos.L1.head.d\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.strata_amos.L1.head.ne.d\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.strata_amos.L1.large.d\endcsname{\ensuremath{+0.84}}
\expandafter\gdef\csname R@an.strata_amos.L1.large.hi\endcsname{\ensuremath{+1.91}}
\expandafter\gdef\csname R@an.strata_amos.L1.large.lo\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.strata_amos.L1.large.ne.d\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.strata_amos.L1.large.ne.hi\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.strata_amos.L1.large.ne.lo\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.strata_amos.L1.med.d\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.strata_amos.L1.med.hi\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.strata_amos.L1.med.lo\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.strata_amos.L1.med.ne.d\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.strata_amos.L1.med.ne.hi\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@an.strata_amos.L1.med.ne.lo\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.strata_amos.L1.small.d\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.strata_amos.L1.small.hi\endcsname{\ensuremath{+1.56}}
\expandafter\gdef\csname R@an.strata_amos.L1.small.lo\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.strata_amos.L1.small.ne.d\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.strata_amos.L1.small.ne.hi\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@an.strata_amos.L1.small.ne.lo\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.strata_amos.L1.thick.d\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.strata_amos.L1.thick.hi\endcsname{\ensuremath{+1.16}}
\expandafter\gdef\csname R@an.strata_amos.L1.thick.lo\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.strata_amos.L1.thick.ne.d\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.strata_amos.L1.thick.ne.hi\endcsname{\ensuremath{+1.01}}
\expandafter\gdef\csname R@an.strata_amos.L1.thick.ne.lo\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.strata_amos.L1.thin.d\endcsname{\ensuremath{+0.89}}
\expandafter\gdef\csname R@an.strata_amos.L1.thin.hi\endcsname{\ensuremath{+2.20}}
\expandafter\gdef\csname R@an.strata_amos.L1.thin.lo\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.strata_amos.L1.thin.ne.d\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.strata_amos.L1.thin.ne.hi\endcsname{\ensuremath{+1.06}}
\expandafter\gdef\csname R@an.strata_amos.L1.thin.ne.lo\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.strata_amos.L3.cs.d\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.strata_amos.L3.cs.hi\endcsname{\ensuremath{+1.71}}
\expandafter\gdef\csname R@an.strata_amos.L3.cs.lo\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.strata_amos.L3.cs.ne.d\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.strata_amos.L3.cs.ne.hi\endcsname{\ensuremath{+1.40}}
\expandafter\gdef\csname R@an.strata_amos.L3.cs.ne.lo\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.strata_amos.L3.ct.d\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.strata_amos.L3.ct.hi\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.strata_amos.L3.ct.lo\endcsname{\ensuremath{-0.52}}
\expandafter\gdef\csname R@an.strata_amos.L3.ct.ne.d\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@an.strata_amos.L3.ct.ne.hi\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.strata_amos.L3.ct.ne.lo\endcsname{\ensuremath{-0.61}}
\expandafter\gdef\csname R@an.strata_amos.L3.head.d\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.strata_amos.L3.head.ne.d\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.strata_amos.L3.large.d\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.strata_amos.L3.large.hi\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.strata_amos.L3.large.lo\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.strata_amos.L3.large.ne.d\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.strata_amos.L3.large.ne.hi\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.strata_amos.L3.large.ne.lo\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.strata_amos.L3.med.d\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.strata_amos.L3.med.hi\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.strata_amos.L3.med.lo\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.strata_amos.L3.med.ne.d\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.strata_amos.L3.med.ne.hi\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.strata_amos.L3.med.ne.lo\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.strata_amos.L3.small.d\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.strata_amos.L3.small.hi\endcsname{\ensuremath{+1.75}}
\expandafter\gdef\csname R@an.strata_amos.L3.small.lo\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.strata_amos.L3.small.ne.d\endcsname{\ensuremath{+0.72}}
\expandafter\gdef\csname R@an.strata_amos.L3.small.ne.hi\endcsname{\ensuremath{+1.32}}
\expandafter\gdef\csname R@an.strata_amos.L3.small.ne.lo\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.strata_amos.L3.thick.d\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.strata_amos.L3.thick.hi\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.strata_amos.L3.thick.lo\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.strata_amos.L3.thick.ne.d\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.strata_amos.L3.thick.ne.hi\endcsname{\ensuremath{+0.67}}
\expandafter\gdef\csname R@an.strata_amos.L3.thick.ne.lo\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.strata_amos.L3.thin.d\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.strata_amos.L3.thin.hi\endcsname{\ensuremath{+1.55}}
\expandafter\gdef\csname R@an.strata_amos.L3.thin.lo\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.strata_amos.L3.thin.ne.d\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.strata_amos.L3.thin.ne.hi\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.strata_amos.L3.thin.ne.lo\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.strata_amos.altref.contemporaneous.absmax\endcsname{0.43}
\expandafter\gdef\csname R@an.strata_amos.altref.contemporaneous.estimand\endcsname{registered headline statistic}
\expandafter\gdef\csname R@an.strata_amos.altref.contemporaneous.head\endcsname{\ensuremath{+0.011}}
\expandafter\gdef\csname R@an.strata_amos.altref.contemporaneous.max\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.strata_amos.altref.contemporaneous.min\endcsname{\ensuremath{-0.14}}
\expandafter\gdef\csname R@an.strata_amos.altref.contemporaneous.n\endcsname{3}
\expandafter\gdef\csname R@an.strata_amos.altref.contemporaneous.ncells\endcsname{10}
\expandafter\gdef\csname R@an.strata_amos.altref.contemporaneous.ratio\endcsname{1.1}
\expandafter\gdef\csname R@an.strata_amos.altref.contemporaneous.short\endcsname{contemporaneous default runs}
\expandafter\gdef\csname R@an.strata_amos.altref.contemporaneous.vs\endcsname{the strata's own median deltas}
\expandafter\gdef\csname R@an.strata_amos.altref.n\endcsname{2}
\expandafter\gdef\csname R@an.strata_amos.altref.uncompiled.absmax\endcsname{0.29}
\expandafter\gdef\csname R@an.strata_amos.altref.uncompiled.estimand\endcsname{registered headline statistic}
\expandafter\gdef\csname R@an.strata_amos.altref.uncompiled.head\endcsname{\ensuremath{+0.029}}
\expandafter\gdef\csname R@an.strata_amos.altref.uncompiled.max\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.strata_amos.altref.uncompiled.min\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.strata_amos.altref.uncompiled.n\endcsname{3}
\expandafter\gdef\csname R@an.strata_amos.altref.uncompiled.ncells\endcsname{10}
\expandafter\gdef\csname R@an.strata_amos.altref.uncompiled.ratio\endcsname{1.6}
\expandafter\gdef\csname R@an.strata_amos.altref.uncompiled.short\endcsname{uncompiled sub-pool}
\expandafter\gdef\csname R@an.strata_amos.altref.uncompiled.vs\endcsname{the strata's own median deltas}
\expandafter\gdef\csname R@an.strata_amos.bladder.gap\endcsname{\ensuremath{+1.44}}
\expandafter\gdef\csname R@an.strata_amos.bladder.gapcommon\endcsname{\ensuremath{+1.44}}
\expandafter\gdef\csname R@an.strata_amos.bladder.med\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.strata_amos.bladder.name\endcsname{bladder}
\expandafter\gdef\csname R@an.strata_amos.bladder.nbig\endcsname{4}
\expandafter\gdef\csname R@an.strata_amos.bladder.nbigne\endcsname{4}
\expandafter\gdef\csname R@an.strata_amos.bladder.nne\endcsname{40}
\expandafter\gdef\csname R@an.strata_amos.bladder.npos\endcsname{21}
\expandafter\gdef\csname R@an.strata_amos.bladder.poolgap.l1\endcsname{\ensuremath{+1.60}}
\expandafter\gdef\csname R@an.strata_amos.bladder.poolgap.l1b\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.strata_amos.bladder.rest\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.strata_amos.bladder.top1.case\endcsname{amos\_0113}
\expandafter\gdef\csname R@an.strata_amos.bladder.top1.share\endcsname{96}
\expandafter\gdef\csname R@an.strata_amos.bladder.top3.share\endcsname{124}
\expandafter\gdef\csname R@an.strata_amos.bladder.ushare\endcsname{0}
\expandafter\gdef\csname R@an.strata_amos.bladder.z\endcsname{\ensuremath{+4.3}}
\expandafter\gdef\csname R@an.strata_amos.bladder.zcommon\endcsname{\ensuremath{+4.3}}
\expandafter\gdef\csname R@an.strata_amos.blc1.case\endcsname{amos\_0113}
\expandafter\gdef\csname R@an.strata_amos.blc1.contrib\endcsname{\ensuremath{+0.092}}
\expandafter\gdef\csname R@an.strata_amos.blc1.lower\endcsname{L1b}
\expandafter\gdef\csname R@an.strata_amos.blc1.precision\endcsname{78}
\expandafter\gdef\csname R@an.strata_amos.blc1.recall\endcsname{19}
\expandafter\gdef\csname R@an.strata_amos.blc2.case\endcsname{amos\_0351}
\expandafter\gdef\csname R@an.strata_amos.blc2.contrib\endcsname{\ensuremath{+0.063}}
\expandafter\gdef\csname R@an.strata_amos.blc2.lower\endcsname{L1b}
\expandafter\gdef\csname R@an.strata_amos.blc2.precision\endcsname{98}
\expandafter\gdef\csname R@an.strata_amos.blc2.recall\endcsname{41}
\expandafter\gdef\csname R@an.strata_amos.cm.large.below\endcsname{thickness-gated}
\expandafter\gdef\csname R@an.strata_amos.cm.large.med\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.strata_amos.cm.large.ne.below\endcsname{thickness-gated}
\expandafter\gdef\csname R@an.strata_amos.cm.large.ne.med\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.strata_amos.cm.large.ne.npos\endcsname{12}
\expandafter\gdef\csname R@an.strata_amos.cm.large.npos\endcsname{12}
\expandafter\gdef\csname R@an.strata_amos.cm.med.below\endcsname{z-dilation mixing, MedNeXt-like}
\expandafter\gdef\csname R@an.strata_amos.cm.med.med\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.strata_amos.cm.med.ne.below\endcsname{z-dilation mixing, MedNeXt-like}
\expandafter\gdef\csname R@an.strata_amos.cm.med.ne.med\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.strata_amos.cm.med.ne.npos\endcsname{11}
\expandafter\gdef\csname R@an.strata_amos.cm.med.npos\endcsname{11}
\expandafter\gdef\csname R@an.strata_amos.cm.narms\endcsname{13}
\expandafter\gdef\csname R@an.strata_amos.cm.small.below\endcsname{HyReX+context}
\expandafter\gdef\csname R@an.strata_amos.cm.small.med\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.strata_amos.cm.small.ne.below\endcsname{none}
\expandafter\gdef\csname R@an.strata_amos.cm.small.ne.med\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.strata_amos.cm.small.ne.npos\endcsname{13}
\expandafter\gdef\csname R@an.strata_amos.cm.small.npos\endcsname{12}
\expandafter\gdef\csname R@an.strata_amos.cm.thick.below\endcsname{trilinear control}
\expandafter\gdef\csname R@an.strata_amos.cm.thick.med\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.strata_amos.cm.thick.ne.below\endcsname{none}
\expandafter\gdef\csname R@an.strata_amos.cm.thick.ne.med\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.strata_amos.cm.thick.ne.npos\endcsname{13}
\expandafter\gdef\csname R@an.strata_amos.cm.thick.npos\endcsname{12}
\expandafter\gdef\csname R@an.strata_amos.cm.thin.below\endcsname{ResEnc-matched, HyReX+context, MedNeXt-like}
\expandafter\gdef\csname R@an.strata_amos.cm.thin.med\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.strata_amos.cm.thin.ne.below\endcsname{HyReX+context, z-dilation mixing, thickness-gated, MedNeXt-like}
\expandafter\gdef\csname R@an.strata_amos.cm.thin.ne.med\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.strata_amos.cm.thin.ne.npos\endcsname{9}
\expandafter\gdef\csname R@an.strata_amos.cm.thin.npos\endcsname{10}
\expandafter\gdef\csname R@an.strata_amos.ev1.case\endcsname{amos\_0057}
\expandafter\gdef\csname R@an.strata_amos.ev1.class\endcsname{spleen}
\expandafter\gdef\csname R@an.strata_amos.ev1.contrib\endcsname{\ensuremath{+0.157}}
\expandafter\gdef\csname R@an.strata_amos.ev1.nrun\endcsname{19}
\expandafter\gdef\csname R@an.strata_amos.ev1.nrun0\endcsname{1}
\expandafter\gdef\csname R@an.strata_amos.ev1.nvox.a\endcsname{0}
\expandafter\gdef\csname R@an.strata_amos.ev1.nvox.b\endcsname{17}
\expandafter\gdef\csname R@an.strata_amos.ev2.case\endcsname{amos\_0294}
\expandafter\gdef\csname R@an.strata_amos.ev2.class\endcsname{gallbladder}
\expandafter\gdef\csname R@an.strata_amos.ev2.contrib\endcsname{\ensuremath{+0.143}}
\expandafter\gdef\csname R@an.strata_amos.ev2.nrun\endcsname{19}
\expandafter\gdef\csname R@an.strata_amos.ev2.nrun0\endcsname{12}
\expandafter\gdef\csname R@an.strata_amos.ev2.nvox.a\endcsname{0}
\expandafter\gdef\csname R@an.strata_amos.ev2.nvox.b\endcsname{13}
\expandafter\gdef\csname R@an.strata_amos.figcm.large.below\endcsname{none}
\expandafter\gdef\csname R@an.strata_amos.figcm.large.med\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.strata_amos.figcm.large.ne.below\endcsname{none}
\expandafter\gdef\csname R@an.strata_amos.figcm.large.ne.med\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.strata_amos.figcm.large.ne.npos\endcsname{6}
\expandafter\gdef\csname R@an.strata_amos.figcm.large.npos\endcsname{6}
\expandafter\gdef\csname R@an.strata_amos.figcm.med.below\endcsname{none}
\expandafter\gdef\csname R@an.strata_amos.figcm.med.med\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.strata_amos.figcm.med.ne.below\endcsname{none}
\expandafter\gdef\csname R@an.strata_amos.figcm.med.ne.med\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.strata_amos.figcm.med.ne.npos\endcsname{6}
\expandafter\gdef\csname R@an.strata_amos.figcm.med.npos\endcsname{6}
\expandafter\gdef\csname R@an.strata_amos.figcm.narms\endcsname{6}
\expandafter\gdef\csname R@an.strata_amos.figcm.small.below\endcsname{HyReX+context}
\expandafter\gdef\csname R@an.strata_amos.figcm.small.med\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.strata_amos.figcm.small.ne.below\endcsname{none}
\expandafter\gdef\csname R@an.strata_amos.figcm.small.ne.med\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@an.strata_amos.figcm.small.ne.npos\endcsname{6}
\expandafter\gdef\csname R@an.strata_amos.figcm.small.npos\endcsname{5}
\expandafter\gdef\csname R@an.strata_amos.figcm.thick.below\endcsname{none}
\expandafter\gdef\csname R@an.strata_amos.figcm.thick.med\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.strata_amos.figcm.thick.ne.below\endcsname{none}
\expandafter\gdef\csname R@an.strata_amos.figcm.thick.ne.med\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.strata_amos.figcm.thick.ne.npos\endcsname{6}
\expandafter\gdef\csname R@an.strata_amos.figcm.thick.npos\endcsname{6}
\expandafter\gdef\csname R@an.strata_amos.figcm.thin.below\endcsname{ResEnc-matched, HyReX+context}
\expandafter\gdef\csname R@an.strata_amos.figcm.thin.med\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.strata_amos.figcm.thin.ne.below\endcsname{HyReX+context}
\expandafter\gdef\csname R@an.strata_amos.figcm.thin.ne.med\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.strata_amos.figcm.thin.ne.npos\endcsname{5}
\expandafter\gdef\csname R@an.strata_amos.figcm.thin.npos\endcsname{4}
\expandafter\gdef\csname R@an.strata_amos.four.share\endcsname{71}
\expandafter\gdef\csname R@an.strata_amos.four.sum\endcsname{\ensuremath{+5.39}}
\expandafter\gdef\csname R@an.strata_amos.four.top3.share\endcsname{87}
\expandafter\gdef\csname R@an.strata_amos.four.top3.sum\endcsname{\ensuremath{+4.68}}
\expandafter\gdef\csname R@an.strata_amos.grp.large.n\endcsname{5}
\expandafter\gdef\csname R@an.strata_amos.grp.large.names\endcsname{spleen, R kidney, L kidney, liver, stomach}
\expandafter\gdef\csname R@an.strata_amos.grp.med.n\endcsname{5}
\expandafter\gdef\csname R@an.strata_amos.grp.med.names\endcsname{aorta, IVC, pancreas, duodenum, bladder}
\expandafter\gdef\csname R@an.strata_amos.grp.small.n\endcsname{5}
\expandafter\gdef\csname R@an.strata_amos.grp.small.names\endcsname{gallbladder, esophagus, R adrenal, L adrenal, prostate/uterus}
\expandafter\gdef\csname R@an.strata_amos.head.empty\endcsname{\ensuremath{+0.300}}
\expandafter\gdef\csname R@an.strata_amos.head.empty.share\endcsname{59}
\expandafter\gdef\csname R@an.strata_amos.head.gap\endcsname{\ensuremath{+0.509}}
\expandafter\gdef\csname R@an.strata_amos.head.ne\endcsname{\ensuremath{+0.207}}
\expandafter\gdef\csname R@an.strata_amos.head.rest\endcsname{\ensuremath{+0.054}}
\expandafter\gdef\csname R@an.strata_amos.head.top4\endcsname{\ensuremath{+0.455}}
\expandafter\gdef\csname R@an.strata_amos.head.top4.share\endcsname{89}
\expandafter\gdef\csname R@an.strata_amos.head.top4dir\endcsname{\ensuremath{+0.455}}
\expandafter\gdef\csname R@an.strata_amos.head.top4dir.share\endcsname{89}
\expandafter\gdef\csname R@an.strata_amos.ivc.gap\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.strata_amos.ivc.gapcommon\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.strata_amos.ivc.med\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.strata_amos.ivc.name\endcsname{IVC}
\expandafter\gdef\csname R@an.strata_amos.ivc.nbig\endcsname{1}
\expandafter\gdef\csname R@an.strata_amos.ivc.nbigne\endcsname{1}
\expandafter\gdef\csname R@an.strata_amos.ivc.nne\endcsname{40}
\expandafter\gdef\csname R@an.strata_amos.ivc.npos\endcsname{26}
\expandafter\gdef\csname R@an.strata_amos.ivc.poolgap.l1\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.strata_amos.ivc.poolgap.l1b\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.strata_amos.ivc.rest\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.strata_amos.ivc.top1.case\endcsname{amos\_0006}
\expandafter\gdef\csname R@an.strata_amos.ivc.top1.share\endcsname{39}
\expandafter\gdef\csname R@an.strata_amos.ivc.top3.share\endcsname{58}
\expandafter\gdef\csname R@an.strata_amos.ivc.ushare\endcsname{0}
\expandafter\gdef\csname R@an.strata_amos.ivc.z\endcsname{\ensuremath{+4.5}}
\expandafter\gdef\csname R@an.strata_amos.ivc.zcommon\endcsname{\ensuremath{+4.5}}
\expandafter\gdef\csname R@an.strata_amos.miss.n\endcsname{0}
\expandafter\gdef\csname R@an.strata_amos.miss.nf\endcsname{9}
\expandafter\gdef\csname R@an.strata_amos.miss.pairs\endcsname{1256}
\expandafter\gdef\csname R@an.strata_amos.miss.runs\endcsname{8}
\expandafter\gdef\csname R@an.strata_amos.n.cls\endcsname{15}
\expandafter\gdef\csname R@an.strata_amos.n.emptyref\endcsname{6}
\expandafter\gdef\csname R@an.strata_amos.n.pairs\endcsname{600}
\expandafter\gdef\csname R@an.strata_amos.n.thick\endcsname{30}
\expandafter\gdef\csname R@an.strata_amos.n.thin\endcsname{10}
\expandafter\gdef\csname R@an.strata_amos.n.val\endcsname{40}
\expandafter\gdef\csname R@an.strata_amos.nover.large.ne.nsd\endcsname{6}
\expandafter\gdef\csname R@an.strata_amos.nover.large.ne.sd\endcsname{6}
\expandafter\gdef\csname R@an.strata_amos.nover.large.nsd\endcsname{6}
\expandafter\gdef\csname R@an.strata_amos.nover.large.sd\endcsname{6}
\expandafter\gdef\csname R@an.strata_amos.nover.med.ne.nsd\endcsname{7}
\expandafter\gdef\csname R@an.strata_amos.nover.med.ne.sd\endcsname{7}
\expandafter\gdef\csname R@an.strata_amos.nover.med.nsd\endcsname{7}
\expandafter\gdef\csname R@an.strata_amos.nover.med.sd\endcsname{7}
\expandafter\gdef\csname R@an.strata_amos.nover.small.ne.nsd\endcsname{11}
\expandafter\gdef\csname R@an.strata_amos.nover.small.ne.sd\endcsname{11}
\expandafter\gdef\csname R@an.strata_amos.nover.small.nsd\endcsname{9}
\expandafter\gdef\csname R@an.strata_amos.nover.small.sd\endcsname{11}
\expandafter\gdef\csname R@an.strata_amos.nover.thick.ne.nsd\endcsname{11}
\expandafter\gdef\csname R@an.strata_amos.nover.thick.ne.sd\endcsname{11}
\expandafter\gdef\csname R@an.strata_amos.nover.thick.nsd\endcsname{7}
\expandafter\gdef\csname R@an.strata_amos.nover.thick.sd\endcsname{8}
\expandafter\gdef\csname R@an.strata_amos.nover.thin.ne.nsd\endcsname{5}
\expandafter\gdef\csname R@an.strata_amos.nover.thin.ne.sd\endcsname{5}
\expandafter\gdef\csname R@an.strata_amos.nover.thin.nsd\endcsname{5}
\expandafter\gdef\csname R@an.strata_amos.nover.thin.sd\endcsname{7}
\expandafter\gdef\csname R@an.strata_amos.nsd.argmax\endcsname{thin slices}
\expandafter\gdef\csname R@an.strata_amos.nsd.large\endcsname{0.16}
\expandafter\gdef\csname R@an.strata_amos.nsd.large.ne\endcsname{0.16}
\expandafter\gdef\csname R@an.strata_amos.nsd.med\endcsname{0.20}
\expandafter\gdef\csname R@an.strata_amos.nsd.med.ne\endcsname{0.20}
\expandafter\gdef\csname R@an.strata_amos.nsd.ne.argmax\endcsname{thin slices}
\expandafter\gdef\csname R@an.strata_amos.nsd.small\endcsname{0.39}
\expandafter\gdef\csname R@an.strata_amos.nsd.small.ne\endcsname{0.28}
\expandafter\gdef\csname R@an.strata_amos.nsd.thick\endcsname{0.20}
\expandafter\gdef\csname R@an.strata_amos.nsd.thick.ne\endcsname{0.15}
\expandafter\gdef\csname R@an.strata_amos.nsd.thin\endcsname{0.53}
\expandafter\gdef\csname R@an.strata_amos.nsd.thin.ne\endcsname{0.32}
\expandafter\gdef\csname R@an.strata_amos.pool.empty.max\endcsname{0.28}
\expandafter\gdef\csname R@an.strata_amos.pool.empty.med\endcsname{0.14}
\expandafter\gdef\csname R@an.strata_amos.pool.empty.nsmaller\endcsname{15}
\expandafter\gdef\csname R@an.strata_amos.pool.head.max\endcsname{0.32}
\expandafter\gdef\csname R@an.strata_amos.pool.head.maxabs\endcsname{0.321}
\expandafter\gdef\csname R@an.strata_amos.pool.head.med\endcsname{0.14}
\expandafter\gdef\csname R@an.strata_amos.pool.head.nsmaller\endcsname{15}
\expandafter\gdef\csname R@an.strata_amos.pool.ne.max\endcsname{0.32}
\expandafter\gdef\csname R@an.strata_amos.pool.ne.med\endcsname{0.12}
\expandafter\gdef\csname R@an.strata_amos.pool.ne.nsmaller\endcsname{13}
\expandafter\gdef\csname R@an.strata_amos.pool.npairs\endcsname{15}
\expandafter\gdef\csname R@an.strata_amos.pool.top4.max\endcsname{0.32}
\expandafter\gdef\csname R@an.strata_amos.pool.top4.med\endcsname{0.11}
\expandafter\gdef\csname R@an.strata_amos.pool.top4.nsmaller\endcsname{15}
\expandafter\gdef\csname R@an.strata_amos.pool.top4.share.max\endcsname{309}
\expandafter\gdef\csname R@an.strata_amos.pool.top4.share.med\endcsname{77}
\expandafter\gdef\csname R@an.strata_amos.pool.top4.share.min\endcsname{\ensuremath{-267}}
\expandafter\gdef\csname R@an.strata_amos.pool.top4.share.nlower\endcsname{9}
\expandafter\gdef\csname R@an.strata_amos.pool.top4dir.max\endcsname{0.42}
\expandafter\gdef\csname R@an.strata_amos.pool.top4dir.med\endcsname{0.30}
\expandafter\gdef\csname R@an.strata_amos.pool.top4dir.nsmaller\endcsname{15}
\expandafter\gdef\csname R@an.strata_amos.pool.top4dir.share.max\endcsname{581}
\expandafter\gdef\csname R@an.strata_amos.pool.top4dir.share.med\endcsname{207}
\expandafter\gdef\csname R@an.strata_amos.pool.top4dir.share.min\endcsname{89}
\expandafter\gdef\csname R@an.strata_amos.pool.top4dir.share.nlower\endcsname{1}
\expandafter\gdef\csname R@an.strata_amos.radr.gap\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.strata_amos.radr.gapcommon\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@an.strata_amos.radr.med\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.strata_amos.radr.name\endcsname{R adrenal}
\expandafter\gdef\csname R@an.strata_amos.radr.nbig\endcsname{3}
\expandafter\gdef\csname R@an.strata_amos.radr.nbigne\endcsname{3}
\expandafter\gdef\csname R@an.strata_amos.radr.nne\endcsname{39}
\expandafter\gdef\csname R@an.strata_amos.radr.npos\endcsname{21}
\expandafter\gdef\csname R@an.strata_amos.radr.poolgap.l1\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.strata_amos.radr.poolgap.l1b\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.strata_amos.radr.rest\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.strata_amos.radr.top1.case\endcsname{amos\_0294}
\expandafter\gdef\csname R@an.strata_amos.radr.top1.share\endcsname{27}
\expandafter\gdef\csname R@an.strata_amos.radr.top3.share\endcsname{70}
\expandafter\gdef\csname R@an.strata_amos.radr.ushare\endcsname{0}
\expandafter\gdef\csname R@an.strata_amos.radr.z\endcsname{\ensuremath{+3.5}}
\expandafter\gdef\csname R@an.strata_amos.radr.zcommon\endcsname{\ensuremath{+3.5}}
\expandafter\gdef\csname R@an.strata_amos.sd.cs\endcsname{0.48}
\expandafter\gdef\csname R@an.strata_amos.sd.cs.ne\endcsname{0.35}
\expandafter\gdef\csname R@an.strata_amos.sd.ct\endcsname{0.61}
\expandafter\gdef\csname R@an.strata_amos.sd.ct.ne\endcsname{0.37}
\expandafter\gdef\csname R@an.strata_amos.sd.large\endcsname{0.14}
\expandafter\gdef\csname R@an.strata_amos.sd.large.ne\endcsname{0.15}
\expandafter\gdef\csname R@an.strata_amos.sd.med\endcsname{0.18}
\expandafter\gdef\csname R@an.strata_amos.sd.med.ne\endcsname{0.18}
\expandafter\gdef\csname R@an.strata_amos.sd.small\endcsname{0.36}
\expandafter\gdef\csname R@an.strata_amos.sd.small.ne\endcsname{0.26}
\expandafter\gdef\csname R@an.strata_amos.sd.thick\endcsname{0.18}
\expandafter\gdef\csname R@an.strata_amos.sd.thick.ne\endcsname{0.14}
\expandafter\gdef\csname R@an.strata_amos.sd.thin\endcsname{0.49}
\expandafter\gdef\csname R@an.strata_amos.sd.thin.ne\endcsname{0.30}
\expandafter\gdef\csname R@an.strata_amos.spleen.gap\endcsname{\ensuremath{+2.45}}
\expandafter\gdef\csname R@an.strata_amos.spleen.gapcommon\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.strata_amos.spleen.med\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.strata_amos.spleen.name\endcsname{spleen}
\expandafter\gdef\csname R@an.strata_amos.spleen.nbig\endcsname{2}
\expandafter\gdef\csname R@an.strata_amos.spleen.nbigne\endcsname{1}
\expandafter\gdef\csname R@an.strata_amos.spleen.nne\endcsname{38}
\expandafter\gdef\csname R@an.strata_amos.spleen.npos\endcsname{26}
\expandafter\gdef\csname R@an.strata_amos.spleen.poolgap.l1\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@an.strata_amos.spleen.poolgap.l1b\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.strata_amos.spleen.rest\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.strata_amos.spleen.top1.case\endcsname{amos\_0057}
\expandafter\gdef\csname R@an.strata_amos.spleen.top1.share\endcsname{96}
\expandafter\gdef\csname R@an.strata_amos.spleen.top3.share\endcsname{94}
\expandafter\gdef\csname R@an.strata_amos.spleen.ushare\endcsname{96}
\expandafter\gdef\csname R@an.strata_amos.spleen.z\endcsname{\ensuremath{+6.5}}
\expandafter\gdef\csname R@an.strata_amos.spleen.zcommon\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.strata_amos.strat.spread.hi\endcsname{small organs}
\expandafter\gdef\csname R@an.strata_amos.strat.spread.lo\endcsname{large organs}
\expandafter\gdef\csname R@an.strata_amos.strat.spread.med\endcsname{0.47}
\expandafter\gdef\csname R@an.strata_amos.strat.spread.ne.hi\endcsname{small organs}
\expandafter\gdef\csname R@an.strata_amos.strat.spread.ne.lo\endcsname{large organs}
\expandafter\gdef\csname R@an.strata_amos.strat.spread.ne.med\endcsname{0.34}
\expandafter\gdef\csname R@an.strata_kits.arms.n\endcsname{6}
\expandafter\gdef\csname R@an.strata_kits.band.k\endcsname{2}
\expandafter\gdef\csname R@an.strata_kits.band2.tum.all\endcsname{1.94}
\expandafter\gdef\csname R@an.strata_kits.band2.tum.large\endcsname{0.63}
\expandafter\gdef\csname R@an.strata_kits.band2.tum.mid\endcsname{1.25}
\expandafter\gdef\csname R@an.strata_kits.band2.tum.small\endcsname{4.47}
\expandafter\gdef\csname R@an.strata_kits.band2pair.tum.all\endcsname{2.13}
\expandafter\gdef\csname R@an.strata_kits.band2pair.tum.large\endcsname{0.69}
\expandafter\gdef\csname R@an.strata_kits.band2pair.tum.mid\endcsname{1.37}
\expandafter\gdef\csname R@an.strata_kits.band2pair.tum.small\endcsname{4.89}
\expandafter\gdef\csname R@an.strata_kits.cap.scatter\endcsname{\textbf{On seeds the design never saw, HyReX's cross-fitted change on the hard cases is \R{an.strata_kits.rep.hard.xfit.L3}~pp, above the \R{an.strata_kits.rescue.ref.xfit.range}~pp that a default run reaches; \R{an.strata_kits.rescue.xfit.above.fresh.count.clause}.} Per-case tumour Dice of HyReX against the per-case mean of the \R{an.strata_kits.pool.n} frozen default runs (KiTS23 fold~0, \R{an.strata_kits.n.all} validation cases): the hollow marker \lgSeedZero\ is the discovery seed the design was selected on and the filled marker \lgFreshMean\ is the mean of its \R{an.strata_kits.rep.nseed} fresh seeds. The band marks the points within \R{an.strata_kits.cut.move}~pp of the pool mean, the diagonal is no change, and the vertical hairlines are the \R{an.strata_kits.cut.hard} and \R{an.strata_kits.cut.easy} cuts that define the hard (\R{an.strata_kits.n.hard} cases) and easy (\R{an.strata_kits.n.easy} cases) sets from the default pool alone. Of the hard cases HyReX improves \R{an.strata_kits.hard.up.L3} by more than \R{an.strata_kits.cut.move}~pp at the discovery seed and \R{an.strata_kits.rep.hard.up.L3} on the fresh mean (\R{an.strata_kits.rescue.ref.kind}: \R{an.strata_kits.rescue.ref.up.range}) and loses on \R{an.strata_kits.hard.dn.L3} and \R{an.strata_kits.rep.hard.dn.L3} (\R{an.strata_kits.rescue.ref.dn.range}); of the easy cases it loses on \R{an.strata_kits.easy.dn.L3} and \R{an.strata_kits.rep.easy.dn.L3} (\R{an.strata_kits.rescue.ref.edn.range}). Cross-fitting removes regression to the mean from the hard-case change: \R{an.strata_kits.tum.L3.hard.xfit}~pp at the discovery seed and \R{an.strata_kits.rep.hard.xfit.L3}~pp on the fresh seeds. \R{an.strata_kits.rep.L3.hard.conc.clause}}
\expandafter\gdef\csname R@an.strata_kits.cap.strata\endcsname{\textbf{The fresh seeds re-measure where along tumour size the gain sits: HyReX's tumour gain is \R{an.strata_kits.rep.L3.tum.pos.clause}, and the smallest third, which carried \R{an.strata_kits.tum.L3.sh.small}\,\% of it at the discovery seed, carries \R{an.strata_kits.rep.L3.tum.sh.small}\,\% on the fresh seeds.} Change in tumour Dice against the frozen default pool (KiTS23 fold~0, \R{an.strata_kits.n.all} validation cases, baseline pool $n\,{=}\,\R{an.strata_kits.pool.n}$), by thirds of physical reference-tumour volume cut at \R{an.strata_kits.cut1.ml} and \R{an.strata_kits.cut2.ml}\,mL --- cut once from the validation cases' reference volumes, which no run's output enters, so each third holds the same cases for every arm, seed and estimand. \emph{Both estimands are drawn, for every arm}: the hollow role marker \lgSeedZero\ is the discovery seed the design was selected on, the small dots \lgFresh\ are its individual fresh seeds, and the heavy filled marker \lgFreshMean\ is their mean --- the registered replication estimand --- with a dotted link joining them. Bars \lgCI, drawn just right of each marker so that the link stays visible, are case-bootstrap \R{an.strata_kits.ci.level}\,\% intervals of the fresh mean, so they cover validation-case sampling only; the grey band \lgBand\ is $\pm$\R{an.strata_kits.band.k} SD of the default's own \R{an.strata_kits.rep.nseed}-seed-mean noise, re-derived \emph{inside each group} from the pool's runs, and a value inside it is not resolved; \R{an.strata_kits.refsens.fig.clause}. In the smallest third HyReX reads \R{an.strata_kits.rep.L3.tum.small}~pp, \R{an.strata_kits.rep.L3.tum.small.band} its band, and ResEnc-M (library preset) reads \R{an.strata_kits.rep.L1.tum.small}~pp, \R{an.strata_kits.rep.L1.tum.small.band} it; HyReX minus the preset is \R{an.strata_kits.repd31.tum.small}, \R{an.strata_kits.repd31.tum.mid} and \R{an.strata_kits.repd31.tum.large}~pp in the three thirds, and \R{an.strata_kits.repd31.tum.thirds.clause}. The band locates a fresh gain among the default's own seed noise (Statistical-conventions box). HyReX \lgHero, the other agent-designed arms \lgAgent, ResEnc-M (library preset) \lgResM\ and ResEnc-matched \lgResMatched; inside every group the arms keep one left-to-right order, which the panel states.}
\expandafter\gdef\csname R@an.strata_kits.captab.alt\endcsname{\textbf{\R{an.strata_kits.captab.alt.lead}} Alternative stratifications of the KiTS23 tumour gain, at each arm's discovery seed. (a)~Thirds of the native \emph{voxel count} instead of volume, the stratification an earlier version of this analysis used: it moves \R{an.strata_kits.vox.moved} of the \R{an.strata_kits.n.all} cases into a different third and raises HyReX's smallest-third share from \R{an.strata_kits.tum.L3.sh.small}\,\% to \R{an.strata_kits.vox.tum.L3.sh.small}\,\%, because a voxel count also orders the cases by slice thickness (mean thickness \R{an.strata_kits.vox.thk.small} / \R{an.strata_kits.vox.thk.mid} / \R{an.strata_kits.vox.thk.large}\,mm against \R{an.strata_kits.thk.small} / \R{an.strata_kits.thk.mid} / \R{an.strata_kits.thk.large} by volume). (b)~Each region stratified by its own volume instead of by tumour volume, point estimates only. (c)~Exploratory split by native slice thickness at \R{an.strata_kits.zs.split}\,mm (\R{an.strata_kits.zs.n.thick} thick cases, \R{an.strata_kits.zs.n.thin} thinner), and (d)~its crossing with the volume thirds, in cells too small to carry intervals. (c) and (d) are one post-hoc cut borrowed from another dataset's registration: a lead for a registered test, not a result.}
\expandafter\gdef\csname R@an.strata_kits.captab.alt.lead\endcsname{Stratifying the same 98 cases by native voxel count instead of physical volume moves 32 of them into a different third and raises HyReX's smallest-third share of the tumour gain from 53\,\% to 90\,\%.}
\expandafter\gdef\csname R@an.strata_kits.captab.altref\endcsname{\textbf{\R{an.strata_kits.captab.altref.lead}} The registered contemporaneous sensitivity reference, by group. The reference is \R{an.strata_kits.refsens.status}. The table gives the mean of the contemporaneous default runs and their range, as change against the frozen default pool in Dice points of the tumour label, over all \R{an.strata_kits.n.all} cases and in each third of physical tumour volume; below, HyReX's and ResEnc-M's fresh-mean change minus that reference mean. Every KiTS23 delta in the paper is against the frozen pool, whose own runs span \R{an.strata_kits.pool.spread}~pp on the headline (\R{an.strata_kits.pool.spread.bars} registered screen bars); this table reads the same deltas against the contemporaneous runs instead.}
\expandafter\gdef\csname R@an.strata_kits.captab.altref.lead\endcsname{Read against the 3 contemporaneous default runs instead of the frozen pool, HyReX's fresh tumour gain stays positive in three of the three thirds of reference-tumour volume (\ensuremath{+1.86}, \ensuremath{+1.73} and \ensuremath{+1.66}~pp).}
\expandafter\gdef\csname R@an.strata_kits.captab.conc\endcsname{\textbf{\R{an.strata_kits.captab.conc.lead}} How the cross-fitted hard-case change is made up, on the fresh seeds. For each arm's fresh mean and for each contemporaneous default run, the change on the hard cases (pool-mean tumour Dice below \R{an.strata_kits.cut.hard}, \R{an.strata_kits.n.hard} cases), cross-fitted (hard set from two pool seeds, change against the held-out one), is the sum of per-case contributions in pp. Columns: the cross-fitted change; the contribution of the single largest case; that case's share of the change (beyond the whole when the other hard cases net-lose); and the change with that case removed. The last row is the range over the contemporaneous default runs (\R{an.strata_kits.refsens.ndone} of \R{an.strata_kits.refsens.nreg} finished), each reduced by its own largest case the same way.}
\expandafter\gdef\csname R@an.strata_kits.captab.conc.lead\endcsname{On the fresh seeds one case carries 55\,\% of HyReX's cross-fitted change on the hard KiTS23 tumour cases, and the change reads \ensuremath{+2.96}~pp with that case removed.}
\expandafter\gdef\csname R@an.strata_kits.captab.estimands\endcsname{\textbf{\R{an.strata_kits.captab.estimands.lead}} HyReX and ResEnc-M (library preset) on both estimands, by thirds of physical tumour volume. Tumour Dice change against the frozen default pool of \R{an.strata_kits.pool.n} runs [case-bootstrap \R{an.strata_kits.ci.level}\,\% interval], at the discovery seed the design was selected on and on the mean of the \R{an.strata_kits.rep.nseed} fresh seeds, over all \R{an.strata_kits.n.all} cases and in each third (cut at \R{an.strata_kits.cut1.ml} and \R{an.strata_kits.cut2.ml}\,mL); the cells are those of the discovery-seed and fresh-seed tables, side by side. The noise band of a \R{an.strata_kits.rep.nseed}-seed mean is $\pm$\R{an.strata_kits.band2.tum.all}~pp over all cases and $\pm$\R{an.strata_kits.band2.tum.small} / \R{an.strata_kits.band2.tum.mid} / \R{an.strata_kits.band2.tum.large}~pp in the three thirds.}
\expandafter\gdef\csname R@an.strata_kits.captab.estimands.lead\endcsname{Read by thirds of tumour volume, ResEnc-M (library preset) is ahead of HyReX in the smallest third; the contrast is not resolved in the middle and largest thirds.}
\expandafter\gdef\csname R@an.strata_kits.captab.regions\endcsname{\textbf{\R{an.strata_kits.captab.regions.lead}} KiTS23 change against the frozen default pool by thirds of physical reference-tumour volume, at each arm's discovery seed. Dice points [case-bootstrap \R{an.strata_kits.ci.level}\,\% interval]; the discovery seed is the seed the design was selected on, and the fresh-seed means of the same cells are the estimand of the replication tables. Pool $n\,{=}\,\R{an.strata_kits.pool.n}$, \R{an.strata_kits.n.all} validation cases; the thirds are cut at \R{an.strata_kits.cut1.ml} and \R{an.strata_kits.cut2.ml}\,mL of tumour volume and hold the same cases (\R{an.strata_kits.n.small} / \R{an.strata_kits.n.mid} / \R{an.strata_kits.n.large}) in all three panels, for the tumour, masses and kidney regions. The intervals cover validation-case sampling only; seed noise is the second, separate scale, re-derived inside each third from the pool's own runs (smallest / middle / largest): SD of the third's mean \R{an.strata_kits.psd.tum.small} / \R{an.strata_kits.psd.tum.mid} / \R{an.strata_kits.psd.tum.large}~pp, no-effect SD of a single-seed delta \R{an.strata_kits.nsd.tum.small} / \R{an.strata_kits.nsd.tum.mid} / \R{an.strata_kits.nsd.tum.large}~pp, of a one-versus-one difference \R{an.strata_kits.pair.tum.small} / \R{an.strata_kits.pair.tum.mid} / \R{an.strata_kits.pair.tum.large}~pp. Pool-mean tumour Dice by third is \R{an.strata_kits.pool.tum.small} / \R{an.strata_kits.pool.tum.mid} / \R{an.strata_kits.pool.tum.large}. The last row is HyReX minus ResEnc-M (library preset), paired on the same cases.}
\expandafter\gdef\csname R@an.strata_kits.captab.regions.lead\endcsname{At the seed each design was selected on, HyReX's KiTS23 tumour gain falls across the thirds of reference-tumour volume (\ensuremath{+6.49}, \ensuremath{+3.84} and \ensuremath{+1.92}~pp from the smallest to the largest), and 53\,\% of its aggregate gain comes from the smallest third.}
\expandafter\gdef\csname R@an.strata_kits.captab.repregions\endcsname{\textbf{\R{an.strata_kits.captab.repregions.lead}} KiTS23 change against the frozen default pool by thirds of physical reference-tumour volume, on the fresh seeds. Dice points [case-bootstrap \R{an.strata_kits.ci.level}\,\% interval] of the mean of the \R{an.strata_kits.rep.nseed} fresh seeds, the registered replication estimand, in the layout of the discovery-seed table; an arm without both fresh seeds shows its cells as pending and nothing is imputed. Pool $n\,{=}\,\R{an.strata_kits.pool.n}$, \R{an.strata_kits.n.all} validation cases; the thirds are the same cases as in the discovery-seed table, cut at \R{an.strata_kits.cut1.ml} and \R{an.strata_kits.cut2.ml}\,mL. The intervals cover validation-case sampling only; the noise band of a \R{an.strata_kits.rep.nseed}-seed mean (\R{an.strata_kits.band.k}~SD, re-derived inside each group from the pool's runs) is $\pm$\R{an.strata_kits.band2.tum.small} / \R{an.strata_kits.band2.tum.mid} / \R{an.strata_kits.band2.tum.large}~pp in the smallest, middle and largest third and $\pm$\R{an.strata_kits.band2.tum.all}~pp over all cases for the tumour, and the band of a difference of two fresh means is $\pm$\R{an.strata_kits.band2pair.tum.small} / \R{an.strata_kits.band2pair.tum.mid} / \R{an.strata_kits.band2pair.tum.large}~pp; a value inside its band is not resolved. The last row is HyReX minus ResEnc-M (library preset).}
\expandafter\gdef\csname R@an.strata_kits.captab.repregions.lead\endcsname{On the registered replication estimand HyReX's KiTS23 tumour gain is positive in every third of tumour volume (\ensuremath{+1.29}, \ensuremath{+3.12} and \ensuremath{+2.60}~pp from the smallest to the largest), and two of the three lie outside the two-seed noise band of its own third.}
\expandafter\gdef\csname R@an.strata_kits.captab.represcue\endcsname{\textbf{\R{an.strata_kits.captab.represcue.lead}} Hard and easy cases on the KiTS23 tumour, on the fresh seeds. The sets, thresholds and columns of the discovery-seed table (hard: pool mean below Dice \R{an.strata_kits.cut.hard}, \R{an.strata_kits.n.hard} cases; easy: above \R{an.strata_kits.cut.easy}, \R{an.strata_kits.n.easy} cases; a change above \R{an.strata_kits.cut.move} Dice points) on the mean of the \R{an.strata_kits.rep.nseed} fresh seeds; an arm without both fresh seeds shows pending cells. The last row is the registered reference, the contemporaneous default runs scored exactly as an arm is (\R{an.strata_kits.refsens.ndone} of \R{an.strata_kits.refsens.nreg} finished), so a count or a cross-fitted change reads against what a default run reaches by regression to the mean.}
\expandafter\gdef\csname R@an.strata_kits.captab.represcue.lead\endcsname{On the 13 hard KiTS23 tumour cases at the fresh seeds, read cross-fitted so that a no-effect arm reads zero, the 3 contemporaneous default runs themselves reach \ensuremath{+0.57} to \ensuremath{+0.85}~pp and 5 of the 6 arms are above that range.}
\expandafter\gdef\csname R@an.strata_kits.captab.rescue\endcsname{\textbf{\R{an.strata_kits.captab.rescue.lead}} Hard and easy cases on the KiTS23 tumour, at each arm's discovery seed. Hard cases are those on which the frozen default pool averages below Dice \R{an.strata_kits.cut.hard} (\R{an.strata_kits.n.hard} cases, \R{an.strata_kits.hard.in.small} of them in the smallest volume third), easy cases those above \R{an.strata_kits.cut.easy} (\R{an.strata_kits.n.easy}); a gain or a loss is a change above \R{an.strata_kits.cut.move} Dice points. The hard set is selected on the pool's own outcome, so regression to the mean inflates every count, and the table carries two no-effect references. \emph{Contemporaneous default runs} are the \R{an.strata_kits.refsens.nreg} registered default runs outside the pool (\R{an.strata_kits.refsens.ndone} finished), scored against the pool exactly as an arm is; \emph{default seed vs other two} plays each pool seed in turn against the other two, whose hard set comes from two runs and so over-states the no-effect count, and is the last row. The cross-fitted column chooses the hard set on two pool seeds and reads the change against the held-out one, where the expectation under no effect is zero; its reference is the range of the default runs' own cross-fitted change. Contribution is the hard cases' part of the aggregate tumour gain, in pp.}
\expandafter\gdef\csname R@an.strata_kits.captab.rescue.lead\endcsname{On the 13 hard KiTS23 tumour cases at the seed each design was selected on, read cross-fitted so that a no-effect arm reads zero, the 3 contemporaneous default runs themselves reach \ensuremath{+0.57} to \ensuremath{+0.85}~pp and 5 of the 6 arms are above that range.}
\expandafter\gdef\csname R@an.strata_kits.caseSD.tum.large\endcsname{1.7}
\expandafter\gdef\csname R@an.strata_kits.caseSD.tum.mid\endcsname{3.4}
\expandafter\gdef\csname R@an.strata_kits.caseSD.tum.small\endcsname{7.8}
\expandafter\gdef\csname R@an.strata_kits.ci.level\endcsname{95}
\expandafter\gdef\csname R@an.strata_kits.cut.easy\endcsname{0.9}
\expandafter\gdef\csname R@an.strata_kits.cut.hard\endcsname{0.5}
\expandafter\gdef\csname R@an.strata_kits.cut.move\endcsname{5}
\expandafter\gdef\csname R@an.strata_kits.cut1.ml\endcsname{9.9}
\expandafter\gdef\csname R@an.strata_kits.cut2.ml\endcsname{44.7}
\expandafter\gdef\csname R@an.strata_kits.easy.dn.L1\endcsname{0}
\expandafter\gdef\csname R@an.strata_kits.easy.dn.L1b\endcsname{0}
\expandafter\gdef\csname R@an.strata_kits.easy.dn.L2\endcsname{5}
\expandafter\gdef\csname R@an.strata_kits.easy.dn.L3\endcsname{0}
\expandafter\gdef\csname R@an.strata_kits.easy.dn.L4\endcsname{1}
\expandafter\gdef\csname R@an.strata_kits.easy.dn.L6\endcsname{0}
\expandafter\gdef\csname R@an.strata_kits.grid.nspac\endcsname{84}
\expandafter\gdef\csname R@an.strata_kits.grid.vox.max\endcsname{5.418}
\expandafter\gdef\csname R@an.strata_kits.grid.vox.med\endcsname{1.98}
\expandafter\gdef\csname R@an.strata_kits.grid.vox.min\endcsname{0.204}
\expandafter\gdef\csname R@an.strata_kits.grid.vox.ratio\endcsname{26.6}
\expandafter\gdef\csname R@an.strata_kits.hard.dn.L1\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.hard.dn.L1b\endcsname{2}
\expandafter\gdef\csname R@an.strata_kits.hard.dn.L2\endcsname{4}
\expandafter\gdef\csname R@an.strata_kits.hard.dn.L3\endcsname{2}
\expandafter\gdef\csname R@an.strata_kits.hard.dn.L4\endcsname{1}
\expandafter\gdef\csname R@an.strata_kits.hard.dn.L6\endcsname{1}
\expandafter\gdef\csname R@an.strata_kits.hard.in.large\endcsname{2}
\expandafter\gdef\csname R@an.strata_kits.hard.in.mid\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.hard.in.small\endcsname{8}
\expandafter\gdef\csname R@an.strata_kits.hard.up.L1\endcsname{4}
\expandafter\gdef\csname R@an.strata_kits.hard.up.L1b\endcsname{7}
\expandafter\gdef\csname R@an.strata_kits.hard.up.L2\endcsname{6}
\expandafter\gdef\csname R@an.strata_kits.hard.up.L3\endcsname{9}
\expandafter\gdef\csname R@an.strata_kits.hard.up.L4\endcsname{5}
\expandafter\gdef\csname R@an.strata_kits.hard.up.L6\endcsname{5}
\expandafter\gdef\csname R@an.strata_kits.head.rep.L1\endcsname{\ensuremath{+3.475}}
\expandafter\gdef\csname R@an.strata_kits.head.rep.L1.s1\endcsname{\ensuremath{+3.134}}
\expandafter\gdef\csname R@an.strata_kits.head.rep.L1.s2\endcsname{\ensuremath{+3.817}}
\expandafter\gdef\csname R@an.strata_kits.head.rep.L1b\endcsname{\ensuremath{+2.313}}
\expandafter\gdef\csname R@an.strata_kits.head.rep.L1b.s1\endcsname{\ensuremath{+2.564}}
\expandafter\gdef\csname R@an.strata_kits.head.rep.L1b.s2\endcsname{\ensuremath{+2.062}}
\expandafter\gdef\csname R@an.strata_kits.head.rep.L2\endcsname{\ensuremath{+0.110}}
\expandafter\gdef\csname R@an.strata_kits.head.rep.L2.s1\endcsname{\ensuremath{-0.805}}
\expandafter\gdef\csname R@an.strata_kits.head.rep.L2.s2\endcsname{\ensuremath{+1.026}}
\expandafter\gdef\csname R@an.strata_kits.head.rep.L3\endcsname{\ensuremath{+2.094}}
\expandafter\gdef\csname R@an.strata_kits.head.rep.L3.s1\endcsname{\ensuremath{+1.798}}
\expandafter\gdef\csname R@an.strata_kits.head.rep.L3.s2\endcsname{\ensuremath{+2.390}}
\expandafter\gdef\csname R@an.strata_kits.head.rep.L4\endcsname{\ensuremath{+2.246}}
\expandafter\gdef\csname R@an.strata_kits.head.rep.L4.s1\endcsname{\ensuremath{+2.677}}
\expandafter\gdef\csname R@an.strata_kits.head.rep.L4.s2\endcsname{\ensuremath{+1.815}}
\expandafter\gdef\csname R@an.strata_kits.head.rep.L6\endcsname{\ensuremath{+1.591}}
\expandafter\gdef\csname R@an.strata_kits.head.rep.L6.s1\endcsname{\ensuremath{+1.198}}
\expandafter\gdef\csname R@an.strata_kits.head.rep.L6.s2\endcsname{\ensuremath{+1.984}}
\expandafter\gdef\csname R@an.strata_kits.head.rep.refminushero\endcsname{\ensuremath{+1.382}}
\expandafter\gdef\csname R@an.strata_kits.head.s0.L1\endcsname{\ensuremath{+2.326}}
\expandafter\gdef\csname R@an.strata_kits.head.s0.L1b\endcsname{\ensuremath{+1.743}}
\expandafter\gdef\csname R@an.strata_kits.head.s0.L2\endcsname{\ensuremath{+0.664}}
\expandafter\gdef\csname R@an.strata_kits.head.s0.L3\endcsname{\ensuremath{+2.842}}
\expandafter\gdef\csname R@an.strata_kits.head.s0.L4\endcsname{\ensuremath{+2.198}}
\expandafter\gdef\csname R@an.strata_kits.head.s0.L6\endcsname{\ensuremath{+2.526}}
\expandafter\gdef\csname R@an.strata_kits.kid.L1.all\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.strata_kits.kid.L1.all.ci\endcsname{\ensuremath{[+0.3,\,+1.9]}}
\expandafter\gdef\csname R@an.strata_kits.kid.L1.large\endcsname{\ensuremath{+1.16}}
\expandafter\gdef\csname R@an.strata_kits.kid.L1.large.ci\endcsname{\ensuremath{[+0.5,\,+2.0]}}
\expandafter\gdef\csname R@an.strata_kits.kid.L1.mid\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.strata_kits.kid.L1.mid.ci\endcsname{\ensuremath{[-0.7,\,+2.6]}}
\expandafter\gdef\csname R@an.strata_kits.kid.L1.small\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.strata_kits.kid.L1.small.ci\endcsname{\ensuremath{[+0.3,\,+2.9]}}
\expandafter\gdef\csname R@an.strata_kits.kid.L3.all\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.strata_kits.kid.L3.all.ci\endcsname{\ensuremath{[+0.2,\,+1.8]}}
\expandafter\gdef\csname R@an.strata_kits.kid.L3.large\endcsname{\ensuremath{+0.80}}
\expandafter\gdef\csname R@an.strata_kits.kid.L3.large.ci\endcsname{\ensuremath{[+0.2,\,+1.5]}}
\expandafter\gdef\csname R@an.strata_kits.kid.L3.mid\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.strata_kits.kid.L3.mid.ci\endcsname{\ensuremath{[-0.7,\,+2.8]}}
\expandafter\gdef\csname R@an.strata_kits.kid.L3.small\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.strata_kits.kid.L3.small.ci\endcsname{\ensuremath{[+0.2,\,+2.9]}}
\expandafter\gdef\csname R@an.strata_kits.kid.d31.all\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.strata_kits.kid.d31.all.ci\endcsname{\ensuremath{[-0.3,\,+0.1]}}
\expandafter\gdef\csname R@an.strata_kits.kid.d31.large\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.strata_kits.kid.d31.large.ci\endcsname{\ensuremath{[-0.74,\,-0.02]}}
\expandafter\gdef\csname R@an.strata_kits.kid.d31.mid\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.strata_kits.kid.d31.mid.ci\endcsname{\ensuremath{[-0.3,\,+0.4]}}
\expandafter\gdef\csname R@an.strata_kits.kid.d31.small\endcsname{0.00}
\expandafter\gdef\csname R@an.strata_kits.kid.d31.small.ci\endcsname{\ensuremath{[-0.4,\,+0.5]}}
\expandafter\gdef\csname R@an.strata_kits.mas.L1.all\endcsname{\ensuremath{+3.03}}
\expandafter\gdef\csname R@an.strata_kits.mas.L1.all.ci\endcsname{\ensuremath{[+0.8,\,+5.5]}}
\expandafter\gdef\csname R@an.strata_kits.mas.L1.large\endcsname{\ensuremath{+2.22}}
\expandafter\gdef\csname R@an.strata_kits.mas.L1.large.ci\endcsname{\ensuremath{[+0.3,\,+4.9]}}
\expandafter\gdef\csname R@an.strata_kits.mas.L1.mid\endcsname{\ensuremath{+1.73}}
\expandafter\gdef\csname R@an.strata_kits.mas.L1.mid.ci\endcsname{\ensuremath{[-2.4,\,+5.7]}}
\expandafter\gdef\csname R@an.strata_kits.mas.L1.small\endcsname{\ensuremath{+5.11}}
\expandafter\gdef\csname R@an.strata_kits.mas.L1.small.ci\endcsname{\ensuremath{[+0.6,\,+10.6]}}
\expandafter\gdef\csname R@an.strata_kits.mas.L3.all\endcsname{\ensuremath{+3.49}}
\expandafter\gdef\csname R@an.strata_kits.mas.L3.all.ci\endcsname{\ensuremath{[+1.2,\,+6.0]}}
\expandafter\gdef\csname R@an.strata_kits.mas.L3.large\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@an.strata_kits.mas.L3.large.ci\endcsname{\ensuremath{[+0.04,\,+4.26]}}
\expandafter\gdef\csname R@an.strata_kits.mas.L3.mid\endcsname{\ensuremath{+1.87}}
\expandafter\gdef\csname R@an.strata_kits.mas.L3.mid.ci\endcsname{\ensuremath{[-2.6,\,+6.9]}}
\expandafter\gdef\csname R@an.strata_kits.mas.L3.small\endcsname{\ensuremath{+6.71}}
\expandafter\gdef\csname R@an.strata_kits.mas.L3.small.ci\endcsname{\ensuremath{[+2.2,\,+12.0]}}
\expandafter\gdef\csname R@an.strata_kits.mas.d31.all\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.strata_kits.mas.d31.all.ci\endcsname{\ensuremath{[-0.9,\,+2.1]}}
\expandafter\gdef\csname R@an.strata_kits.mas.d31.large\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.strata_kits.mas.d31.large.ci\endcsname{\ensuremath{[-1.7,\,+1.1]}}
\expandafter\gdef\csname R@an.strata_kits.mas.d31.mid\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.strata_kits.mas.d31.mid.ci\endcsname{\ensuremath{[-1.1,\,+1.6]}}
\expandafter\gdef\csname R@an.strata_kits.mas.d31.small\endcsname{\ensuremath{+1.60}}
\expandafter\gdef\csname R@an.strata_kits.mas.d31.small.ci\endcsname{\ensuremath{[-2.0,\,+6.0]}}
\expandafter\gdef\csname R@an.strata_kits.ml.large.max\endcsname{777.0}
\expandafter\gdef\csname R@an.strata_kits.ml.large.med\endcsname{95.3}
\expandafter\gdef\csname R@an.strata_kits.ml.large.min\endcsname{45.1}
\expandafter\gdef\csname R@an.strata_kits.ml.mid.max\endcsname{44.7}
\expandafter\gdef\csname R@an.strata_kits.ml.mid.med\endcsname{25.5}
\expandafter\gdef\csname R@an.strata_kits.ml.mid.min\endcsname{10.0}
\expandafter\gdef\csname R@an.strata_kits.ml.small.max\endcsname{9.9}
\expandafter\gdef\csname R@an.strata_kits.ml.small.med\endcsname{4.7}
\expandafter\gdef\csname R@an.strata_kits.ml.small.min\endcsname{0.9}
\expandafter\gdef\csname R@an.strata_kits.n.all\endcsname{98}
\expandafter\gdef\csname R@an.strata_kits.n.easy\endcsname{31}
\expandafter\gdef\csname R@an.strata_kits.n.hard\endcsname{13}
\expandafter\gdef\csname R@an.strata_kits.n.large\endcsname{32}
\expandafter\gdef\csname R@an.strata_kits.n.mid\endcsname{33}
\expandafter\gdef\csname R@an.strata_kits.n.midr\endcsname{54}
\expandafter\gdef\csname R@an.strata_kits.n.small\endcsname{33}
\expandafter\gdef\csname R@an.strata_kits.nsd.tum.all\endcsname{1.23}
\expandafter\gdef\csname R@an.strata_kits.nsd.tum.large\endcsname{0.40}
\expandafter\gdef\csname R@an.strata_kits.nsd.tum.mid\endcsname{0.79}
\expandafter\gdef\csname R@an.strata_kits.nsd.tum.small\endcsname{2.83}
\expandafter\gdef\csname R@an.strata_kits.nsd2.tum.all\endcsname{0.97}
\expandafter\gdef\csname R@an.strata_kits.nsd2.tum.large\endcsname{0.32}
\expandafter\gdef\csname R@an.strata_kits.nsd2.tum.mid\endcsname{0.63}
\expandafter\gdef\csname R@an.strata_kits.nsd2.tum.small\endcsname{2.23}
\expandafter\gdef\csname R@an.strata_kits.null.easy.dn.max\endcsname{1}
\expandafter\gdef\csname R@an.strata_kits.null.easy.dn.min\endcsname{0}
\expandafter\gdef\csname R@an.strata_kits.null.extra.all.max\endcsname{\ensuremath{+2.16}}
\expandafter\gdef\csname R@an.strata_kits.null.extra.all.mean\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.strata_kits.null.extra.all.min\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.strata_kits.null.extra.easy.dn.max\endcsname{2}
\expandafter\gdef\csname R@an.strata_kits.null.extra.easy.dn.min\endcsname{0}
\expandafter\gdef\csname R@an.strata_kits.null.extra.hard.dn.max\endcsname{4}
\expandafter\gdef\csname R@an.strata_kits.null.extra.hard.dn.min\endcsname{2}
\expandafter\gdef\csname R@an.strata_kits.null.extra.hard.mean.max\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.strata_kits.null.extra.hard.mean.min\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.strata_kits.null.extra.hard.up.max\endcsname{4}
\expandafter\gdef\csname R@an.strata_kits.null.extra.hard.up.min\endcsname{4}
\expandafter\gdef\csname R@an.strata_kits.null.extra.large.max\endcsname{\ensuremath{+1.58}}
\expandafter\gdef\csname R@an.strata_kits.null.extra.large.mean\endcsname{\ensuremath{+0.95}}
\expandafter\gdef\csname R@an.strata_kits.null.extra.large.min\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.strata_kits.null.extra.mid.max\endcsname{\ensuremath{+1.92}}
\expandafter\gdef\csname R@an.strata_kits.null.extra.mid.mean\endcsname{\ensuremath{+1.39}}
\expandafter\gdef\csname R@an.strata_kits.null.extra.mid.min\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@an.strata_kits.null.extra.n\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.null.extra.small.max\endcsname{\ensuremath{+3.78}}
\expandafter\gdef\csname R@an.strata_kits.null.extra.small.mean\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.strata_kits.null.extra.small.min\endcsname{\ensuremath{-3.19}}
\expandafter\gdef\csname R@an.strata_kits.null.hard.dn.max\endcsname{6}
\expandafter\gdef\csname R@an.strata_kits.null.hard.dn.min\endcsname{2}
\expandafter\gdef\csname R@an.strata_kits.null.hard.mean.max\endcsname{\ensuremath{+9.4}}
\expandafter\gdef\csname R@an.strata_kits.null.hard.mean.min\endcsname{\ensuremath{-1.5}}
\expandafter\gdef\csname R@an.strata_kits.null.hard.up.max\endcsname{7}
\expandafter\gdef\csname R@an.strata_kits.null.hard.up.min\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.null.n.hard.max\endcsname{16}
\expandafter\gdef\csname R@an.strata_kits.null.n.hard.min\endcsname{14}
\expandafter\gdef\csname R@an.strata_kits.pair.tum.large\endcsname{0.49}
\expandafter\gdef\csname R@an.strata_kits.pair.tum.mid\endcsname{0.97}
\expandafter\gdef\csname R@an.strata_kits.pair.tum.small\endcsname{3.46}
\expandafter\gdef\csname R@an.strata_kits.pair2.tum.all\endcsname{1.06}
\expandafter\gdef\csname R@an.strata_kits.pair2.tum.large\endcsname{0.35}
\expandafter\gdef\csname R@an.strata_kits.pair2.tum.mid\endcsname{0.68}
\expandafter\gdef\csname R@an.strata_kits.pair2.tum.small\endcsname{2.45}
\expandafter\gdef\csname R@an.strata_kits.par.L1\endcsname{102.35}
\expandafter\gdef\csname R@an.strata_kits.par.L1b\endcsname{102.43}
\expandafter\gdef\csname R@an.strata_kits.par.L2\endcsname{24.50}
\expandafter\gdef\csname R@an.strata_kits.par.L3\endcsname{29.66}
\expandafter\gdef\csname R@an.strata_kits.par.L4\endcsname{102.82}
\expandafter\gdef\csname R@an.strata_kits.par.L6\endcsname{31.17}
\expandafter\gdef\csname R@an.strata_kits.par.base\endcsname{31.20}
\expandafter\gdef\csname R@an.strata_kits.pool.hi\endcsname{84.272}
\expandafter\gdef\csname R@an.strata_kits.pool.lo\endcsname{82.749}
\expandafter\gdef\csname R@an.strata_kits.pool.mean\endcsname{83.378}
\expandafter\gdef\csname R@an.strata_kits.pool.n\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.pool.pub.clause\endcsname{2.87~pp below the published fold-0 default}
\expandafter\gdef\csname R@an.strata_kits.pool.pub.offset\endcsname{\ensuremath{-2.87}}
\expandafter\gdef\csname R@an.strata_kits.pool.pub.ref\endcsname{86.25}
\expandafter\gdef\csname R@an.strata_kits.pool.sd\endcsname{0.795}
\expandafter\gdef\csname R@an.strata_kits.pool.spread\endcsname{1.522}
\expandafter\gdef\csname R@an.strata_kits.pool.spread.bars\endcsname{4.35}
\expandafter\gdef\csname R@an.strata_kits.pool.tum.large\endcsname{82.1}
\expandafter\gdef\csname R@an.strata_kits.pool.tum.mid\endcsname{78.0}
\expandafter\gdef\csname R@an.strata_kits.pool.tum.small\endcsname{62.9}
\expandafter\gdef\csname R@an.strata_kits.psd.tum.all\endcsname{1.06}
\expandafter\gdef\csname R@an.strata_kits.psd.tum.large\endcsname{0.35}
\expandafter\gdef\csname R@an.strata_kits.psd.tum.mid\endcsname{0.68}
\expandafter\gdef\csname R@an.strata_kits.psd.tum.small\endcsname{2.45}
\expandafter\gdef\csname R@an.strata_kits.refsens.alt.clause\endcsname{Read against those runs instead, HyReX's fresh tumour gains are \ensuremath{+1.86}, \ensuremath{+1.73} and \ensuremath{+1.66}~pp in the smallest, middle and largest third, positive in every third against that reference too.}
\expandafter\gdef\csname R@an.strata_kits.refsens.clause\endcsname{the mean of those runs sits 0.49 pp above the frozen mean on the headline Dice}
\expandafter\gdef\csname R@an.strata_kits.refsens.fig.clause\endcsname{the dash-dot segment in each group is the mean of the 3 contemporaneous default runs (the registered sensitivity reference, not a pool member) over that group's cases}
\expandafter\gdef\csname R@an.strata_kits.refsens.ndone\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.refsens.nreg\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.refsens.shift\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.strata_kits.refsens.status\endcsname{complete: all 3 contemporaneous default runs have finished}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.hard.conc.clause\endcsname{On the fresh seeds one case carries 18\,\% of ResEnc-M's cross-fitted change, and with each run's largest case removed ResEnc-M reads \ensuremath{+10.83}~pp, above the \ensuremath{-3.66} to \ensuremath{-0.29}~pp range of a default run reduced the same way.}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.hard.drop1\endcsname{\ensuremath{+10.83}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.hard.top1\endcsname{18}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.hard.top1.pp\endcsname{\ensuremath{+2.38}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.kid.all\endcsname{\ensuremath{+1.19}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.kid.all.ci\endcsname{\ensuremath{[+0.6,\,+1.8]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.kid.large\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.kid.large.ci\endcsname{\ensuremath{[+0.5,\,+2.2]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.kid.mid\endcsname{\ensuremath{+0.94}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.kid.mid.ci\endcsname{\ensuremath{[+0.1,\,+2.1]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.kid.small\endcsname{\ensuremath{+1.38}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.kid.small.ci\endcsname{\ensuremath{[+0.4,\,+2.7]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.mas.all\endcsname{\ensuremath{+4.15}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.mas.all.ci\endcsname{\ensuremath{[+2.2,\,+6.4]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.mas.large\endcsname{\ensuremath{+2.46}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.mas.large.ci\endcsname{\ensuremath{[+0.1,\,+5.6]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.mas.mid\endcsname{\ensuremath{+3.17}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.mas.mid.ci\endcsname{\ensuremath{[+0.6,\,+6.8]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.mas.small\endcsname{\ensuremath{+6.76}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.mas.small.ci\endcsname{\ensuremath{[+2.8,\,+11.5]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.reg.npos\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.reg.pos.clause\endcsname{positive in every region (tumour, masses, kidney)}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.spread.all\endcsname{1.22}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.spread.large\endcsname{0.15}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.spread.mid\endcsname{1.72}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.spread.small\endcsname{1.75}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.all\endcsname{\ensuremath{+5.09}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.all.band\endcsname{outside}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.all.ci\endcsname{\ensuremath{[+3.2,\,+7.2]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.all.resolved\endcsname{resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.c.easy\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.c.hard\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.c.large\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.c.mid\endcsname{\ensuremath{+1.63}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.c.midr\endcsname{\ensuremath{+3.24}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.c.small\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.large\endcsname{\ensuremath{+2.67}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.large.band\endcsname{outside}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.large.ci\endcsname{\ensuremath{[+0.3,\,+5.8]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.large.resolved\endcsname{resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.mid\endcsname{\ensuremath{+4.83}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.mid.band\endcsname{outside}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.mid.ci\endcsname{\ensuremath{[+2.0,\,+8.5]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.mid.resolved\endcsname{resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.npos\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.pos.clause\endcsname{positive in every third of tumour volume}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.sh.large\endcsname{17}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.sh.mid\endcsname{32}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.sh.small\endcsname{51}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.small\endcsname{\ensuremath{+7.71}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.small.band\endcsname{outside}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.small.ci\endcsname{\ensuremath{[+3.7,\,+11.8]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.small.resolved\endcsname{resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.t2.all\endcsname{\ensuremath{+5.2}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.t2.large\endcsname{\ensuremath{+8.4}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.t2.mid\endcsname{\ensuremath{+7.7}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.tum.t2.small\endcsname{\ensuremath{+3.5}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.zs.all\endcsname{\ensuremath{+5.09}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.zs.thick\endcsname{\ensuremath{+4.74}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1.zs.thin\endcsname{\ensuremath{+5.40}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.hard.conc.clause\endcsname{On the fresh seeds one case carries 32\,\% of ResEnc-matched's cross-fitted change, and with each run's largest case removed ResEnc-matched reads \ensuremath{+3.05}~pp, above the \ensuremath{-3.66} to \ensuremath{-0.29}~pp range of a default run reduced the same way.}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.hard.drop1\endcsname{\ensuremath{+3.05}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.hard.top1\endcsname{32}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.hard.top1.pp\endcsname{\ensuremath{+1.42}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.kid.all\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.kid.all.ci\endcsname{\ensuremath{[+0.4,\,+1.6]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.kid.large\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.kid.large.ci\endcsname{\ensuremath{[+0.4,\,+2.0]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.kid.mid\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.kid.mid.ci\endcsname{\ensuremath{[-0.3,\,+1.1]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.kid.small\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.kid.small.ci\endcsname{\ensuremath{[+0.3,\,+2.8]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.mas.all\endcsname{\ensuremath{+3.26}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.mas.all.ci\endcsname{\ensuremath{[+1.4,\,+5.3]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.mas.large\endcsname{\ensuremath{+2.82}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.mas.large.ci\endcsname{\ensuremath{[+0.6,\,+6.1]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.mas.mid\endcsname{\ensuremath{+1.93}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.mas.mid.ci\endcsname{\ensuremath{[-0.8,\,+5.5]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.mas.small\endcsname{\ensuremath{+5.00}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.mas.small.ci\endcsname{\ensuremath{[+1.3,\,+9.2]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.reg.npos\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.reg.pos.clause\endcsname{positive in every region (tumour, masses, kidney)}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.spread.all\endcsname{0.92}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.spread.large\endcsname{0.45}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.spread.mid\endcsname{1.09}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.spread.small\endcsname{1.21}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.all\endcsname{\ensuremath{+2.80}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.all.band\endcsname{outside}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.all.ci\endcsname{\ensuremath{[+0.9,\,+4.7]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.all.resolved\endcsname{resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.c.easy\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.c.hard\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.c.large\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.c.mid\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.c.midr\endcsname{\ensuremath{+2.14}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.c.small\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.large\endcsname{\ensuremath{+3.20}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.large.band\endcsname{outside}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.large.ci\endcsname{\ensuremath{[+1.0,\,+6.3]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.large.resolved\endcsname{resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.mid\endcsname{\ensuremath{+2.30}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.mid.band\endcsname{outside}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.mid.ci\endcsname{\ensuremath{[-0.5,\,+5.6]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.mid.resolved\endcsname{resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.npos\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.pos.clause\endcsname{positive in every third of tumour volume}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.sh.large\endcsname{37}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.sh.mid\endcsname{28}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.sh.small\endcsname{35}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.small\endcsname{\ensuremath{+2.92}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.small.band\endcsname{inside}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.small.ci\endcsname{\ensuremath{[-1.3,\,+6.9]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.small.resolved\endcsname{not resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.t2.all\endcsname{\ensuremath{+2.9}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.t2.large\endcsname{\ensuremath{+10.1}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.t2.mid\endcsname{\ensuremath{+3.7}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.tum.t2.small\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.zs.all\endcsname{\ensuremath{+2.80}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.zs.thick\endcsname{\ensuremath{+2.90}}
\expandafter\gdef\csname R@an.strata_kits.rep.L1b.zs.thin\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.hard.conc.clause\endcsname{On the fresh seeds one case carries more than the whole of ConvNeXt-k3's cross-fitted change (the other hard cases net-lose), and with each run's largest case removed ConvNeXt-k3 reads \ensuremath{-2.58}~pp, inside the \ensuremath{-3.66} to \ensuremath{-0.29}~pp range of a default run reduced the same way.}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.hard.drop1\endcsname{\ensuremath{-2.58}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.hard.top1\endcsname{\ensuremath{>}100}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.hard.top1.pp\endcsname{\ensuremath{+2.66}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.kid.all\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.kid.all.ci\endcsname{\ensuremath{[-1.0,\,+0.4]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.kid.large\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.kid.large.ci\endcsname{\ensuremath{[-0.6,\,+0.3]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.kid.mid\endcsname{\ensuremath{-1.08}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.kid.mid.ci\endcsname{\ensuremath{[-2.9,\,+0.2]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.kid.small\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.kid.small.ci\endcsname{\ensuremath{[-0.3,\,+1.6]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.mas.all\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.mas.all.ci\endcsname{\ensuremath{[-1.4,\,+2.7]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.mas.large\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.mas.large.ci\endcsname{\ensuremath{[-1.7,\,+0.9]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.mas.mid\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.mas.mid.ci\endcsname{\ensuremath{[-4.4,\,+3.0]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.mas.small\endcsname{\ensuremath{+2.80}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.mas.small.ci\endcsname{\ensuremath{[-1.6,\,+7.3]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.reg.npos\endcsname{1}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.reg.pos.clause\endcsname{positive in 1 of the 3 regions (tumour, masses, kidney)}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.spread.all\endcsname{2.00}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.spread.large\endcsname{1.64}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.spread.mid\endcsname{0.98}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.spread.small\endcsname{3.37}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.all\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.all.band\endcsname{inside}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.all.ci\endcsname{\ensuremath{[-2.2,\,+2.1]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.all.resolved\endcsname{not resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.c.easy\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.c.hard\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.c.large\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.c.mid\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.c.midr\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.c.small\endcsname{0.00}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.large\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.large.band\endcsname{inside}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.large.ci\endcsname{\ensuremath{[-0.9,\,+1.6]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.large.resolved\endcsname{not resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.mid\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.mid.band\endcsname{inside}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.mid.ci\endcsname{\ensuremath{[-4.0,\,+3.1]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.mid.resolved\endcsname{not resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.npos\endcsname{1}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.pos.clause\endcsname{positive in 1 of the 3 thirds of tumour volume}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.sh.large\endcsname{\pend[share undefined: the aggregate it is a share of is not positive]}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.sh.mid\endcsname{\pend[share undefined: the aggregate it is a share of is not positive]}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.sh.small\endcsname{\pend[share undefined: the aggregate it is a share of is not positive]}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.small\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.small.band\endcsname{inside}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.small.ci\endcsname{\ensuremath{[-5.2,\,+5.1]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.small.resolved\endcsname{not resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.t2.all\endcsname{0.0}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.t2.large\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.t2.mid\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.tum.t2.small\endcsname{0.0}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.zs.all\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.zs.thick\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.strata_kits.rep.L2.zs.thin\endcsname{\ensuremath{-0.58}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.hard.conc.clause\endcsname{On the fresh seeds one case carries 55\,\% of HyReX's cross-fitted change, and with each run's largest case removed HyReX reads \ensuremath{+2.96}~pp, above the \ensuremath{-3.66} to \ensuremath{-0.29}~pp range of a default run reduced the same way.}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.hard.drop1\endcsname{\ensuremath{+2.96}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.hard.top1\endcsname{55}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.hard.top1.pp\endcsname{\ensuremath{+3.59}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.kid.all\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.kid.all.ci\endcsname{\ensuremath{[+0.4,\,+1.6]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.kid.large\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.kid.large.ci\endcsname{\ensuremath{[+0.4,\,+2.1]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.kid.mid\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.kid.mid.ci\endcsname{\ensuremath{[+0.1,\,+2.0]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.kid.small\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.kid.small.ci\endcsname{\ensuremath{[+0.02,\,+2.10]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.mas.all\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.mas.all.ci\endcsname{\ensuremath{[+1.2,\,+5.0]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.mas.large\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.mas.large.ci\endcsname{\ensuremath{[+0.6,\,+4.7]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.mas.mid\endcsname{\ensuremath{+2.57}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.mas.mid.ci\endcsname{\ensuremath{[-0.05,\,+6.08]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.mas.small\endcsname{\ensuremath{+4.05}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.mas.small.ci\endcsname{\ensuremath{[+0.1,\,+8.2]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.reg.npos\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.reg.pos.clause\endcsname{positive in every region (tumour, masses, kidney)}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.spread.all\endcsname{1.20}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.spread.large\endcsname{0.93}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.spread.mid\endcsname{2.70}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.spread.small\endcsname{0.05}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.all\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.all.band\endcsname{outside}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.all.ci\endcsname{\ensuremath{[+0.2,\,+4.6]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.all.resolved\endcsname{resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.c.easy\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.c.hard\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.c.large\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.c.mid\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.c.midr\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.c.small\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.large\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.large.band\endcsname{outside}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.large.ci\endcsname{\ensuremath{[+0.6,\,+5.2]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.large.resolved\endcsname{resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.large.vsalt\endcsname{\ensuremath{+1.66}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.mid\endcsname{\ensuremath{+3.12}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.mid.band\endcsname{outside}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.mid.ci\endcsname{\ensuremath{[+0.1,\,+7.3]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.mid.resolved\endcsname{resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.mid.vsalt\endcsname{\ensuremath{+1.73}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.npos\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.pos.clause\endcsname{positive in every third of tumour volume}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.sh.large\endcsname{36}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.sh.mid\endcsname{45}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.sh.small\endcsname{19}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.small\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.small.band\endcsname{inside}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.small.ci\endcsname{\ensuremath{[-3.8,\,+6.0]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.small.resolved\endcsname{not resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.small.vsalt\endcsname{\ensuremath{+1.86}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.t2.all\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.t2.large\endcsname{\ensuremath{+8.2}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.t2.mid\endcsname{\ensuremath{+5.0}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.tum.t2.small\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.zs.all\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.zs.thick\endcsname{\ensuremath{+4.10}}
\expandafter\gdef\csname R@an.strata_kits.rep.L3.zs.thin\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.hard.conc.clause\endcsname{On the fresh seeds one case carries 32\,\% of ResEnc+context's cross-fitted change, and with each run's largest case removed ResEnc+context reads \ensuremath{+4.69}~pp, above the \ensuremath{-3.66} to \ensuremath{-0.29}~pp range of a default run reduced the same way.}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.hard.drop1\endcsname{\ensuremath{+4.69}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.hard.top1\endcsname{32}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.hard.top1.pp\endcsname{\ensuremath{+2.26}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.kid.all\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.kid.all.ci\endcsname{\ensuremath{[+0.4,\,+1.4]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.kid.large\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.kid.large.ci\endcsname{\ensuremath{[+0.4,\,+1.8]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.kid.mid\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.kid.mid.ci\endcsname{\ensuremath{[+0.1,\,+1.2]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.kid.small\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.kid.small.ci\endcsname{\ensuremath{[+0.2,\,+2.3]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.mas.all\endcsname{\ensuremath{+2.73}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.mas.all.ci\endcsname{\ensuremath{[+1.2,\,+4.5]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.mas.large\endcsname{\ensuremath{+2.37}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.mas.large.ci\endcsname{\ensuremath{[+0.2,\,+5.3]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.mas.mid\endcsname{\ensuremath{+1.56}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.mas.mid.ci\endcsname{\ensuremath{[-0.6,\,+4.2]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.mas.small\endcsname{\ensuremath{+4.26}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.mas.small.ci\endcsname{\ensuremath{[+1.2,\,+8.0]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.reg.npos\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.reg.pos.clause\endcsname{positive in every region (tumour, masses, kidney)}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.spread.all\endcsname{1.18}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.spread.large\endcsname{0.02}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.spread.mid\endcsname{4.08}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.spread.small\endcsname{0.58}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.all\endcsname{\ensuremath{+3.14}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.all.band\endcsname{outside}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.all.ci\endcsname{\ensuremath{[+1.1,\,+5.2]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.all.resolved\endcsname{resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.c.easy\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.c.hard\endcsname{\ensuremath{+1.13}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.c.large\endcsname{\ensuremath{+1.06}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.c.mid\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.c.midr\endcsname{\ensuremath{+2.24}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.c.small\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.large\endcsname{\ensuremath{+3.23}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.large.band\endcsname{outside}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.large.ci\endcsname{\ensuremath{[+0.8,\,+6.3]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.large.resolved\endcsname{resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.mid\endcsname{\ensuremath{+3.25}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.mid.band\endcsname{outside}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.mid.ci\endcsname{\ensuremath{[+0.6,\,+6.3]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.mid.resolved\endcsname{resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.npos\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.pos.clause\endcsname{positive in every third of tumour volume}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.sh.large\endcsname{34}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.sh.mid\endcsname{35}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.sh.small\endcsname{32}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.small\endcsname{\ensuremath{+2.95}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.small.band\endcsname{inside}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.small.ci\endcsname{\ensuremath{[-1.8,\,+7.6]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.small.resolved\endcsname{not resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.t2.all\endcsname{\ensuremath{+3.2}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.t2.large\endcsname{\ensuremath{+10.2}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.t2.mid\endcsname{\ensuremath{+5.2}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.tum.t2.small\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.zs.all\endcsname{\ensuremath{+3.14}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.zs.thick\endcsname{\ensuremath{+3.56}}
\expandafter\gdef\csname R@an.strata_kits.rep.L4.zs.thin\endcsname{\ensuremath{+2.77}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.hard.conc.clause\endcsname{On the fresh seeds one case carries 72\,\% of HyReX+context's cross-fitted change, and with each run's largest case removed HyReX+context reads \ensuremath{+1.21}~pp, above the \ensuremath{-3.66} to \ensuremath{-0.29}~pp range of a default run reduced the same way.}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.hard.drop1\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.hard.top1\endcsname{72}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.hard.top1.pp\endcsname{\ensuremath{+3.08}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.kid.all\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.kid.all.ci\endcsname{\ensuremath{[+0.2,\,+1.2]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.kid.large\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.kid.large.ci\endcsname{\ensuremath{[-0.04,\,+1.33]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.kid.mid\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.kid.mid.ci\endcsname{\ensuremath{[-0.3,\,+2.2]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.kid.small\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.kid.small.ci\endcsname{\ensuremath{[+0.1,\,+1.4]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.mas.all\endcsname{\ensuremath{+1.72}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.mas.all.ci\endcsname{\ensuremath{[-0.2,\,+3.7]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.mas.large\endcsname{\ensuremath{+1.52}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.mas.large.ci\endcsname{\ensuremath{[-0.2,\,+4.1]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.mas.mid\endcsname{\ensuremath{+1.53}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.mas.mid.ci\endcsname{\ensuremath{[-2.2,\,+5.6]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.mas.small\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.mas.small.ci\endcsname{\ensuremath{[-1.6,\,+6.0]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.reg.npos\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.reg.pos.clause\endcsname{positive in every region (tumour, masses, kidney)}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.spread.all\endcsname{1.60}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.spread.large\endcsname{1.91}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.spread.mid\endcsname{2.89}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.spread.small\endcsname{3.71}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.all\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.all.band\endcsname{outside}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.all.ci\endcsname{\ensuremath{[+0.5,\,+4.4]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.all.resolved\endcsname{resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.c.easy\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.c.hard\endcsname{\ensuremath{+0.67}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.c.large\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.c.mid\endcsname{\ensuremath{+0.90}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.c.midr\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.c.small\endcsname{\ensuremath{+0.95}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.large\endcsname{\ensuremath{+1.71}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.large.band\endcsname{outside}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.large.ci\endcsname{\ensuremath{[-0.1,\,+4.2]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.large.resolved\endcsname{resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.mid\endcsname{\ensuremath{+2.68}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.mid.band\endcsname{outside}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.mid.ci\endcsname{\ensuremath{[-1.1,\,+6.8]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.mid.resolved\endcsname{resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.npos\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.pos.clause\endcsname{positive in every third of tumour volume}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.sh.large\endcsname{23}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.sh.mid\endcsname{37}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.sh.small\endcsname{39}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.small\endcsname{\ensuremath{+2.83}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.small.band\endcsname{inside}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.small.ci\endcsname{\ensuremath{[-0.9,\,+6.5]}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.small.resolved\endcsname{not resolved}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.t2.all\endcsname{\ensuremath{+2.5}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.t2.large\endcsname{\ensuremath{+5.4}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.t2.mid\endcsname{\ensuremath{+4.3}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.tum.t2.small\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.zs.all\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.zs.thick\endcsname{\ensuremath{+1.81}}
\expandafter\gdef\csname R@an.strata_kits.rep.L6.zs.thin\endcsname{\ensuremath{+2.95}}
\expandafter\gdef\csname R@an.strata_kits.rep.arms.n\endcsname{6}
\expandafter\gdef\csname R@an.strata_kits.rep.easy.dn.L1\endcsname{1}
\expandafter\gdef\csname R@an.strata_kits.rep.easy.dn.L1b\endcsname{0}
\expandafter\gdef\csname R@an.strata_kits.rep.easy.dn.L2\endcsname{2}
\expandafter\gdef\csname R@an.strata_kits.rep.easy.dn.L3\endcsname{0}
\expandafter\gdef\csname R@an.strata_kits.rep.easy.dn.L4\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.rep.easy.dn.L6\endcsname{2}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.dn.L1\endcsname{0}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.dn.L1b\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.dn.L2\endcsname{4}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.dn.L3\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.dn.L4\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.dn.L6\endcsname{2}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.mean.L1\endcsname{\ensuremath{+14.2}}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.mean.L1b\endcsname{\ensuremath{+4.7}}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.mean.L2\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.mean.L3\endcsname{\ensuremath{+8.2}}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.mean.L4\endcsname{\ensuremath{+8.5}}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.mean.L6\endcsname{\ensuremath{+5.0}}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.up.L1\endcsname{8}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.up.L1b\endcsname{7}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.up.L2\endcsname{4}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.up.L3\endcsname{5}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.up.L4\endcsname{7}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.up.L6\endcsname{5}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.xfit.L1\endcsname{\ensuremath{+13.2}}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.xfit.L1b\endcsname{\ensuremath{+4.5}}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.xfit.L2\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.xfit.L3\endcsname{\ensuremath{+6.5}}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.xfit.L4\endcsname{\ensuremath{+6.9}}
\expandafter\gdef\csname R@an.strata_kits.rep.hard.xfit.L6\endcsname{\ensuremath{+4.3}}
\expandafter\gdef\csname R@an.strata_kits.rep.nseed\endcsname{2}
\expandafter\gdef\csname R@an.strata_kits.rep.small.dn.L1\endcsname{1}
\expandafter\gdef\csname R@an.strata_kits.rep.small.dn.L1b\endcsname{5}
\expandafter\gdef\csname R@an.strata_kits.rep.small.dn.L2\endcsname{8}
\expandafter\gdef\csname R@an.strata_kits.rep.small.dn.L3\endcsname{7}
\expandafter\gdef\csname R@an.strata_kits.rep.small.dn.L4\endcsname{6}
\expandafter\gdef\csname R@an.strata_kits.rep.small.dn.L6\endcsname{4}
\expandafter\gdef\csname R@an.strata_kits.rep.small.med.L1\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.strata_kits.rep.small.med.L1b\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.strata_kits.rep.small.med.L2\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.strata_kits.rep.small.med.L3\endcsname{\ensuremath{+0.5}}
\expandafter\gdef\csname R@an.strata_kits.rep.small.med.L4\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.strata_kits.rep.small.med.L6\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.strata_kits.rep.small.up.L1\endcsname{14}
\expandafter\gdef\csname R@an.strata_kits.rep.small.up.L1b\endcsname{11}
\expandafter\gdef\csname R@an.strata_kits.rep.small.up.L2\endcsname{7}
\expandafter\gdef\csname R@an.strata_kits.rep.small.up.L3\endcsname{10}
\expandafter\gdef\csname R@an.strata_kits.rep.small.up.L4\endcsname{11}
\expandafter\gdef\csname R@an.strata_kits.rep.small.up.L6\endcsname{11}
\expandafter\gdef\csname R@an.strata_kits.repd31.kid.all\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.strata_kits.repd31.kid.all.ci\endcsname{\ensuremath{[-0.67,\,+0.02]}}
\expandafter\gdef\csname R@an.strata_kits.repd31.kid.large\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@an.strata_kits.repd31.kid.large.ci\endcsname{\ensuremath{[-0.4,\,+0.1]}}
\expandafter\gdef\csname R@an.strata_kits.repd31.kid.mid\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.strata_kits.repd31.kid.mid.ci\endcsname{\ensuremath{[-0.6,\,+0.2]}}
\expandafter\gdef\csname R@an.strata_kits.repd31.kid.small\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.strata_kits.repd31.kid.small.ci\endcsname{\ensuremath{[-1.6,\,+0.1]}}
\expandafter\gdef\csname R@an.strata_kits.repd31.mas.all\endcsname{\ensuremath{-1.13}}
\expandafter\gdef\csname R@an.strata_kits.repd31.mas.all.ci\endcsname{\ensuremath{[-2.8,\,+0.4]}}
\expandafter\gdef\csname R@an.strata_kits.repd31.mas.large\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.strata_kits.repd31.mas.large.ci\endcsname{\ensuremath{[-1.8,\,+1.5]}}
\expandafter\gdef\csname R@an.strata_kits.repd31.mas.mid\endcsname{\ensuremath{-0.60}}
\expandafter\gdef\csname R@an.strata_kits.repd31.mas.mid.ci\endcsname{\ensuremath{[-2.9,\,+1.6]}}
\expandafter\gdef\csname R@an.strata_kits.repd31.mas.small\endcsname{\ensuremath{-2.71}}
\expandafter\gdef\csname R@an.strata_kits.repd31.mas.small.ci\endcsname{\ensuremath{[-6.9,\,+0.7]}}
\expandafter\gdef\csname R@an.strata_kits.repd31.tum.all\endcsname{\ensuremath{-2.76}}
\expandafter\gdef\csname R@an.strata_kits.repd31.tum.all.ci\endcsname{\ensuremath{[-5.3,\,-0.6]}}
\expandafter\gdef\csname R@an.strata_kits.repd31.tum.all.lead\endcsname{ResEnc-M (library preset) is ahead of HyReX}
\expandafter\gdef\csname R@an.strata_kits.repd31.tum.large\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@an.strata_kits.repd31.tum.large.ci\endcsname{\ensuremath{[-2.0,\,+1.7]}}
\expandafter\gdef\csname R@an.strata_kits.repd31.tum.large.lead\endcsname{the contrast is inside that group's pair band and is not resolved}
\expandafter\gdef\csname R@an.strata_kits.repd31.tum.mid\endcsname{\ensuremath{-1.71}}
\expandafter\gdef\csname R@an.strata_kits.repd31.tum.mid.ci\endcsname{\ensuremath{[-3.7,\,+0.4]}}
\expandafter\gdef\csname R@an.strata_kits.repd31.tum.mid.lead\endcsname{the contrast clears that group's pair band but its case-bootstrap interval includes zero, so it is not resolved}
\expandafter\gdef\csname R@an.strata_kits.repd31.tum.small\endcsname{\ensuremath{-6.42}}
\expandafter\gdef\csname R@an.strata_kits.repd31.tum.small.ci\endcsname{\ensuremath{[-12.9,\,-0.8]}}
\expandafter\gdef\csname R@an.strata_kits.repd31.tum.small.lead\endcsname{ResEnc-M (library preset) is ahead of HyReX}
\expandafter\gdef\csname R@an.strata_kits.repd31.tum.thirds.clause\endcsname{ResEnc-M (library preset) is ahead of HyReX in the smallest third; the contrast is not resolved in the middle and largest thirds}
\expandafter\gdef\csname R@an.strata_kits.repd31.zs.all\endcsname{\ensuremath{-2.76}}
\expandafter\gdef\csname R@an.strata_kits.repd31.zs.thick\endcsname{\ensuremath{-0.64}}
\expandafter\gdef\csname R@an.strata_kits.repd31.zs.thin\endcsname{\ensuremath{-4.63}}
\expandafter\gdef\csname R@an.strata_kits.rescue.ref.dn.range\endcsname{2 to 4}
\expandafter\gdef\csname R@an.strata_kits.rescue.ref.drop1.range\endcsname{\ensuremath{-3.66} to \ensuremath{-0.29}}
\expandafter\gdef\csname R@an.strata_kits.rescue.ref.edn.range\endcsname{0 to 2}
\expandafter\gdef\csname R@an.strata_kits.rescue.ref.kind\endcsname{the contemporaneous default runs}
\expandafter\gdef\csname R@an.strata_kits.rescue.ref.n\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.rescue.ref.top1.range\endcsname{\ensuremath{+1.14} to \ensuremath{+4.39}}
\expandafter\gdef\csname R@an.strata_kits.rescue.ref.up.range\endcsname{4}
\expandafter\gdef\csname R@an.strata_kits.rescue.ref.xfit.range\endcsname{\ensuremath{+0.57} to \ensuremath{+0.85}}
\expandafter\gdef\csname R@an.strata_kits.rescue.verb.L1\endcsname{rises}
\expandafter\gdef\csname R@an.strata_kits.rescue.verb.L3\endcsname{falls}
\expandafter\gdef\csname R@an.strata_kits.rescue.xfit.above.disc.clause\endcsname{5 of the 6 arms are above that range (HyReX, ResEnc-M, ResEnc-matched, ResEnc+context, HyReX+context)}
\expandafter\gdef\csname R@an.strata_kits.rescue.xfit.above.disc.count.clause\endcsname{5 of the 6 arms are above that range}
\expandafter\gdef\csname R@an.strata_kits.rescue.xfit.above.disc.n\endcsname{5}
\expandafter\gdef\csname R@an.strata_kits.rescue.xfit.above.disc.names\endcsname{HyReX, ResEnc-M, ResEnc-matched, ResEnc+context, HyReX+context}
\expandafter\gdef\csname R@an.strata_kits.rescue.xfit.above.fresh.clause\endcsname{5 of the 6 arms are above that range (HyReX, ResEnc-M, ResEnc-matched, ResEnc+context, HyReX+context)}
\expandafter\gdef\csname R@an.strata_kits.rescue.xfit.above.fresh.count.clause\endcsname{5 of the 6 arms are above that range}
\expandafter\gdef\csname R@an.strata_kits.rescue.xfit.above.fresh.n\endcsname{5}
\expandafter\gdef\csname R@an.strata_kits.rescue.xfit.above.fresh.names\endcsname{HyReX, ResEnc-M, ResEnc-matched, ResEnc+context, HyReX+context}
\expandafter\gdef\csname R@an.strata_kits.seed.L1.s0.all\endcsname{\ensuremath{+2.90}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1.s0.large\endcsname{\ensuremath{+2.16}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1.s0.mid\endcsname{\ensuremath{+3.42}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1.s0.small\endcsname{\ensuremath{+3.10}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1.s0.zs.gap\endcsname{\ensuremath{-1.1}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1.s1.all\endcsname{\ensuremath{+4.49}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1.s1.large\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1.s1.mid\endcsname{\ensuremath{+3.97}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1.s1.small\endcsname{\ensuremath{+6.84}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1.s1.zs.gap\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1.s2.all\endcsname{\ensuremath{+5.70}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1.s2.large\endcsname{\ensuremath{+2.74}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1.s2.mid\endcsname{\ensuremath{+5.69}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1.s2.small\endcsname{\ensuremath{+8.59}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1.s2.zs.gap\endcsname{\ensuremath{-1.4}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1b.s0.all\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1b.s0.large\endcsname{\ensuremath{+1.99}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1b.s0.mid\endcsname{\ensuremath{+1.62}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1b.s0.small\endcsname{\ensuremath{+5.42}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1b.s0.zs.gap\endcsname{\ensuremath{-0.3}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1b.s1.all\endcsname{\ensuremath{+3.26}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1b.s1.large\endcsname{\ensuremath{+3.43}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1b.s1.mid\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1b.s1.small\endcsname{\ensuremath{+3.52}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1b.s1.zs.gap\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1b.s2.all\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1b.s2.large\endcsname{\ensuremath{+2.98}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1b.s2.mid\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1b.s2.small\endcsname{\ensuremath{+2.32}}
\expandafter\gdef\csname R@an.strata_kits.seed.L1b.s2.zs.gap\endcsname{\ensuremath{-1.1}}
\expandafter\gdef\csname R@an.strata_kits.seed.L2.s0.all\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.strata_kits.seed.L2.s0.large\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.strata_kits.seed.L2.s0.mid\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.strata_kits.seed.L2.s0.small\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.strata_kits.seed.L2.s0.zs.gap\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.strata_kits.seed.L2.s1.all\endcsname{\ensuremath{-1.02}}
\expandafter\gdef\csname R@an.strata_kits.seed.L2.s1.large\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.strata_kits.seed.L2.s1.mid\endcsname{\ensuremath{-0.86}}
\expandafter\gdef\csname R@an.strata_kits.seed.L2.s1.small\endcsname{\ensuremath{-1.69}}
\expandafter\gdef\csname R@an.strata_kits.seed.L2.s1.zs.gap\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.strata_kits.seed.L2.s2.all\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.strata_kits.seed.L2.s2.large\endcsname{\ensuremath{+1.14}}
\expandafter\gdef\csname R@an.strata_kits.seed.L2.s2.mid\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.strata_kits.seed.L2.s2.small\endcsname{\ensuremath{+1.68}}
\expandafter\gdef\csname R@an.strata_kits.seed.L2.s2.zs.gap\endcsname{\ensuremath{+0.1}}
\expandafter\gdef\csname R@an.strata_kits.seed.L3.s0.all\endcsname{\ensuremath{+4.11}}
\expandafter\gdef\csname R@an.strata_kits.seed.L3.s0.large\endcsname{\ensuremath{+1.92}}
\expandafter\gdef\csname R@an.strata_kits.seed.L3.s0.mid\endcsname{\ensuremath{+3.84}}
\expandafter\gdef\csname R@an.strata_kits.seed.L3.s0.small\endcsname{\ensuremath{+6.49}}
\expandafter\gdef\csname R@an.strata_kits.seed.L3.s0.zs.gap\endcsname{\ensuremath{+4.3}}
\expandafter\gdef\csname R@an.strata_kits.seed.L3.s1.all\endcsname{\ensuremath{+1.74}}
\expandafter\gdef\csname R@an.strata_kits.seed.L3.s1.large\endcsname{\ensuremath{+2.14}}
\expandafter\gdef\csname R@an.strata_kits.seed.L3.s1.mid\endcsname{\ensuremath{+1.77}}
\expandafter\gdef\csname R@an.strata_kits.seed.L3.s1.small\endcsname{\ensuremath{+1.32}}
\expandafter\gdef\csname R@an.strata_kits.seed.L3.s1.zs.gap\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.strata_kits.seed.L3.s2.all\endcsname{\ensuremath{+2.94}}
\expandafter\gdef\csname R@an.strata_kits.seed.L3.s2.large\endcsname{\ensuremath{+3.07}}
\expandafter\gdef\csname R@an.strata_kits.seed.L3.s2.mid\endcsname{\ensuremath{+4.47}}
\expandafter\gdef\csname R@an.strata_kits.seed.L3.s2.small\endcsname{\ensuremath{+1.27}}
\expandafter\gdef\csname R@an.strata_kits.seed.L3.s2.zs.gap\endcsname{\ensuremath{+4.0}}
\expandafter\gdef\csname R@an.strata_kits.seed.L4.s0.all\endcsname{\ensuremath{+3.50}}
\expandafter\gdef\csname R@an.strata_kits.seed.L4.s0.large\endcsname{\ensuremath{+2.61}}
\expandafter\gdef\csname R@an.strata_kits.seed.L4.s0.mid\endcsname{\ensuremath{+3.16}}
\expandafter\gdef\csname R@an.strata_kits.seed.L4.s0.small\endcsname{\ensuremath{+4.70}}
\expandafter\gdef\csname R@an.strata_kits.seed.L4.s0.zs.gap\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.strata_kits.seed.L4.s1.all\endcsname{\ensuremath{+3.73}}
\expandafter\gdef\csname R@an.strata_kits.seed.L4.s1.large\endcsname{\ensuremath{+3.24}}
\expandafter\gdef\csname R@an.strata_kits.seed.L4.s1.mid\endcsname{\ensuremath{+5.29}}
\expandafter\gdef\csname R@an.strata_kits.seed.L4.s1.small\endcsname{\ensuremath{+2.66}}
\expandafter\gdef\csname R@an.strata_kits.seed.L4.s1.zs.gap\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.strata_kits.seed.L4.s2.all\endcsname{\ensuremath{+2.55}}
\expandafter\gdef\csname R@an.strata_kits.seed.L4.s2.large\endcsname{\ensuremath{+3.22}}
\expandafter\gdef\csname R@an.strata_kits.seed.L4.s2.mid\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.strata_kits.seed.L4.s2.small\endcsname{\ensuremath{+3.24}}
\expandafter\gdef\csname R@an.strata_kits.seed.L4.s2.zs.gap\endcsname{\ensuremath{-0.5}}
\expandafter\gdef\csname R@an.strata_kits.seed.L6.s0.all\endcsname{\ensuremath{+3.90}}
\expandafter\gdef\csname R@an.strata_kits.seed.L6.s0.large\endcsname{\ensuremath{+2.13}}
\expandafter\gdef\csname R@an.strata_kits.seed.L6.s0.mid\endcsname{\ensuremath{+2.43}}
\expandafter\gdef\csname R@an.strata_kits.seed.L6.s0.small\endcsname{\ensuremath{+7.08}}
\expandafter\gdef\csname R@an.strata_kits.seed.L6.s0.zs.gap\endcsname{\ensuremath{-0.1}}
\expandafter\gdef\csname R@an.strata_kits.seed.L6.s1.all\endcsname{\ensuremath{+1.62}}
\expandafter\gdef\csname R@an.strata_kits.seed.L6.s1.large\endcsname{\ensuremath{+2.67}}
\expandafter\gdef\csname R@an.strata_kits.seed.L6.s1.mid\endcsname{\ensuremath{+1.24}}
\expandafter\gdef\csname R@an.strata_kits.seed.L6.s1.small\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.strata_kits.seed.L6.s1.zs.gap\endcsname{\ensuremath{+0.3}}
\expandafter\gdef\csname R@an.strata_kits.seed.L6.s2.all\endcsname{\ensuremath{+3.22}}
\expandafter\gdef\csname R@an.strata_kits.seed.L6.s2.large\endcsname{\ensuremath{+0.76}}
\expandafter\gdef\csname R@an.strata_kits.seed.L6.s2.mid\endcsname{\ensuremath{+4.13}}
\expandafter\gdef\csname R@an.strata_kits.seed.L6.s2.small\endcsname{\ensuremath{+4.69}}
\expandafter\gdef\csname R@an.strata_kits.seed.L6.s2.zs.gap\endcsname{\ensuremath{-2.6}}
\expandafter\gdef\csname R@an.strata_kits.tcrit.df2\endcsname{4.30}
\expandafter\gdef\csname R@an.strata_kits.thk.large\endcsname{3.7}
\expandafter\gdef\csname R@an.strata_kits.thk.mid\endcsname{3.3}
\expandafter\gdef\csname R@an.strata_kits.thk.small\endcsname{2.9}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.all\endcsname{\ensuremath{+2.90}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.all.ci\endcsname{\ensuremath{[+0.4,\,+5.5]}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.c.easy\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.c.hard\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.c.large\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.c.mid\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.c.midr\endcsname{\ensuremath{+2.13}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.c.small\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.hard.mean\endcsname{\ensuremath{+4.7}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.hard.xfit\endcsname{\ensuremath{+4.1}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.large\endcsname{\ensuremath{+2.16}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.large.ci\endcsname{\ensuremath{[-0.04,\,+5.17]}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.mid\endcsname{\ensuremath{+3.42}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.mid.ci\endcsname{\ensuremath{[-1.6,\,+8.9]}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.sh.hard\endcsname{22}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.sh.large\endcsname{24}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.sh.mid\endcsname{40}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.sh.small\endcsname{36}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.small\endcsname{\ensuremath{+3.10}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.small.ci\endcsname{\ensuremath{[-1.7,\,+7.9]}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.small.dn\endcsname{5}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.small.med\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.small.top3\endcsname{86}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.small.up\endcsname{10}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.t.all\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.t.large\endcsname{\ensuremath{+5.4}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.t.mid\endcsname{\ensuremath{+4.3}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1.t.small\endcsname{\ensuremath{+1.1}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1b.all\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1b.large\endcsname{\ensuremath{+1.99}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1b.mid\endcsname{\ensuremath{+1.62}}
\expandafter\gdef\csname R@an.strata_kits.tum.L1b.small\endcsname{\ensuremath{+5.42}}
\expandafter\gdef\csname R@an.strata_kits.tum.L2.all\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.strata_kits.tum.L2.large\endcsname{\ensuremath{-0.53}}
\expandafter\gdef\csname R@an.strata_kits.tum.L2.mid\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.strata_kits.tum.L2.small\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.all\endcsname{\ensuremath{+4.11}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.all.ci\endcsname{\ensuremath{[+1.7,\,+6.9]}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.c.easy\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.c.hard\endcsname{\ensuremath{+2.18}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.c.large\endcsname{\ensuremath{+0.63}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.c.mid\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.c.midr\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.c.small\endcsname{\ensuremath{+2.19}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.hard.mean\endcsname{\ensuremath{+16.4}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.hard.top3\endcsname{77}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.hard.xfit\endcsname{\ensuremath{+14.0}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.large\endcsname{\ensuremath{+1.92}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.large.ci\endcsname{\ensuremath{[-0.1,\,+4.5]}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.mid\endcsname{\ensuremath{+3.84}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.mid.ci\endcsname{\ensuremath{[-1.2,\,+9.9]}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.sh.hard\endcsname{53}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.sh.large\endcsname{15}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.sh.mid\endcsname{32}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.sh.small\endcsname{53}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.small\endcsname{\ensuremath{+6.49}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.small.ci\endcsname{\ensuremath{[+1.9,\,+11.5]}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.small.dn\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.small.med\endcsname{\ensuremath{+2.0}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.small.top3\endcsname{54}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.small.up\endcsname{15}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.t.all\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.t.large\endcsname{\ensuremath{+4.8}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.t.mid\endcsname{\ensuremath{+4.9}}
\expandafter\gdef\csname R@an.strata_kits.tum.L3.t.small\endcsname{\ensuremath{+2.3}}
\expandafter\gdef\csname R@an.strata_kits.tum.L4.all\endcsname{\ensuremath{+3.50}}
\expandafter\gdef\csname R@an.strata_kits.tum.L4.large\endcsname{\ensuremath{+2.61}}
\expandafter\gdef\csname R@an.strata_kits.tum.L4.mid\endcsname{\ensuremath{+3.16}}
\expandafter\gdef\csname R@an.strata_kits.tum.L4.small\endcsname{\ensuremath{+4.70}}
\expandafter\gdef\csname R@an.strata_kits.tum.L6.all\endcsname{\ensuremath{+3.90}}
\expandafter\gdef\csname R@an.strata_kits.tum.L6.large\endcsname{\ensuremath{+2.13}}
\expandafter\gdef\csname R@an.strata_kits.tum.L6.mid\endcsname{\ensuremath{+2.43}}
\expandafter\gdef\csname R@an.strata_kits.tum.L6.small\endcsname{\ensuremath{+7.08}}
\expandafter\gdef\csname R@an.strata_kits.tum.d31.all\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.strata_kits.tum.d31.all.ci\endcsname{\ensuremath{[-0.9,\,+3.7]}}
\expandafter\gdef\csname R@an.strata_kits.tum.d31.large\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.strata_kits.tum.d31.large.ci\endcsname{\ensuremath{[-1.5,\,+1.2]}}
\expandafter\gdef\csname R@an.strata_kits.tum.d31.mid\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.strata_kits.tum.d31.mid.ci\endcsname{\ensuremath{[-1.2,\,+2.3]}}
\expandafter\gdef\csname R@an.strata_kits.tum.d31.small\endcsname{\ensuremath{+3.39}}
\expandafter\gdef\csname R@an.strata_kits.tum.d31.small.ci\endcsname{\ensuremath{[-2.5,\,+10.2]}}
\expandafter\gdef\csname R@an.strata_kits.vox.cut1\endcsname{7619}
\expandafter\gdef\csname R@an.strata_kits.vox.cut2\endcsname{28542}
\expandafter\gdef\csname R@an.strata_kits.vox.d31.all\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.strata_kits.vox.d31.all.ci\endcsname{\ensuremath{[-0.9,\,+3.7]}}
\expandafter\gdef\csname R@an.strata_kits.vox.d31.large\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.strata_kits.vox.d31.large.ci\endcsname{\ensuremath{[-1.9,\,+0.2]}}
\expandafter\gdef\csname R@an.strata_kits.vox.d31.mid\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.strata_kits.vox.d31.mid.ci\endcsname{\ensuremath{[-1.7,\,+2.9]}}
\expandafter\gdef\csname R@an.strata_kits.vox.d31.small\endcsname{\ensuremath{+3.98}}
\expandafter\gdef\csname R@an.strata_kits.vox.d31.small.ci\endcsname{\ensuremath{[-1.6,\,+10.4]}}
\expandafter\gdef\csname R@an.strata_kits.vox.hard.in.small\endcsname{10}
\expandafter\gdef\csname R@an.strata_kits.vox.ml.large.max\endcsname{777.0}
\expandafter\gdef\csname R@an.strata_kits.vox.ml.large.med\endcsname{95.3}
\expandafter\gdef\csname R@an.strata_kits.vox.ml.large.min\endcsname{11.5}
\expandafter\gdef\csname R@an.strata_kits.vox.ml.mid.max\endcsname{88.0}
\expandafter\gdef\csname R@an.strata_kits.vox.ml.mid.med\endcsname{32.5}
\expandafter\gdef\csname R@an.strata_kits.vox.ml.mid.min\endcsname{3.9}
\expandafter\gdef\csname R@an.strata_kits.vox.ml.small.max\endcsname{39.5}
\expandafter\gdef\csname R@an.strata_kits.vox.ml.small.med\endcsname{5.1}
\expandafter\gdef\csname R@an.strata_kits.vox.ml.small.min\endcsname{0.9}
\expandafter\gdef\csname R@an.strata_kits.vox.moved\endcsname{32}
\expandafter\gdef\csname R@an.strata_kits.vox.nsd.tum.large\endcsname{0.84}
\expandafter\gdef\csname R@an.strata_kits.vox.nsd.tum.mid\endcsname{2.39}
\expandafter\gdef\csname R@an.strata_kits.vox.nsd.tum.small\endcsname{1.98}
\expandafter\gdef\csname R@an.strata_kits.vox.pair.tum.large\endcsname{1.03}
\expandafter\gdef\csname R@an.strata_kits.vox.pair.tum.mid\endcsname{2.92}
\expandafter\gdef\csname R@an.strata_kits.vox.pair.tum.small\endcsname{2.43}
\expandafter\gdef\csname R@an.strata_kits.vox.pool.tum.large\endcsname{83.1}
\expandafter\gdef\csname R@an.strata_kits.vox.pool.tum.mid\endcsname{82.9}
\expandafter\gdef\csname R@an.strata_kits.vox.pool.tum.small\endcsname{57.1}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L1.tum.all\endcsname{\ensuremath{+5.09}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L1.tum.large\endcsname{\ensuremath{+3.06}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L1.tum.mid\endcsname{\ensuremath{+3.15}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L1.tum.sh.large\endcsname{20}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L1.tum.sh.mid\endcsname{21}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L1.tum.sh.small\endcsname{60}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L1.tum.small\endcsname{\ensuremath{+9.01}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L1b.tum.all\endcsname{\ensuremath{+2.80}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L1b.tum.large\endcsname{\ensuremath{+3.15}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L1b.tum.mid\endcsname{\ensuremath{-0.60}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L1b.tum.sh.large\endcsname{37}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L1b.tum.sh.mid\endcsname{\ensuremath{-7}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L1b.tum.sh.small\endcsname{70}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L1b.tum.small\endcsname{\ensuremath{+5.86}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L2.tum.all\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L2.tum.large\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L2.tum.mid\endcsname{\ensuremath{-3.16}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L2.tum.sh.large\endcsname{\pend[share undefined: the aggregate it is a share of is not positive]}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L2.tum.sh.mid\endcsname{\pend[share undefined: the aggregate it is a share of is not positive]}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L2.tum.sh.small\endcsname{\pend[share undefined: the aggregate it is a share of is not positive]}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L2.tum.small\endcsname{\ensuremath{+3.09}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L3.tum.all\endcsname{\ensuremath{+2.34}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L3.tum.large\endcsname{\ensuremath{+2.59}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L3.tum.mid\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L3.tum.sh.large\endcsname{36}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L3.tum.sh.mid\endcsname{8}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L3.tum.sh.small\endcsname{56}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L3.tum.small\endcsname{\ensuremath{+3.89}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L4.tum.all\endcsname{\ensuremath{+3.14}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L4.tum.large\endcsname{\ensuremath{+3.62}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L4.tum.mid\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L4.tum.sh.large\endcsname{38}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L4.tum.sh.mid\endcsname{13}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L4.tum.sh.small\endcsname{49}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L4.tum.small\endcsname{\ensuremath{+4.57}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L6.tum.all\endcsname{\ensuremath{+2.42}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L6.tum.large\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L6.tum.mid\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L6.tum.sh.large\endcsname{32}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L6.tum.sh.mid\endcsname{\ensuremath{-5}}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L6.tum.sh.small\endcsname{73}
\expandafter\gdef\csname R@an.strata_kits.vox.rep.L6.tum.small\endcsname{\ensuremath{+5.24}}
\expandafter\gdef\csname R@an.strata_kits.vox.repd31.all\endcsname{\ensuremath{-2.76}}
\expandafter\gdef\csname R@an.strata_kits.vox.repd31.large\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@an.strata_kits.vox.repd31.mid\endcsname{\ensuremath{-2.61}}
\expandafter\gdef\csname R@an.strata_kits.vox.repd31.small\endcsname{\ensuremath{-5.11}}
\expandafter\gdef\csname R@an.strata_kits.vox.rho\endcsname{0.83}
\expandafter\gdef\csname R@an.strata_kits.vox.thk.large\endcsname{2.8}
\expandafter\gdef\csname R@an.strata_kits.vox.thk.mid\endcsname{3.1}
\expandafter\gdef\csname R@an.strata_kits.vox.thk.small\endcsname{3.9}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L1.all\endcsname{\ensuremath{+2.90}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L1.all.ci\endcsname{\ensuremath{[+0.4,\,+5.5]}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L1.large\endcsname{\ensuremath{+2.58}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L1.large.ci\endcsname{\ensuremath{[+0.5,\,+5.5]}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L1.mid\endcsname{\ensuremath{-0.93}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L1.mid.ci\endcsname{\ensuremath{[-5.1,\,+2.3]}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L1.sh.large\endcsname{29}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L1.sh.mid\endcsname{\ensuremath{-11}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L1.sh.small\endcsname{82}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L1.small\endcsname{\ensuremath{+7.04}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L1.small.ci\endcsname{\ensuremath{[+1.8,\,+12.9]}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L1.t.all\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L1.t.large\endcsname{\ensuremath{+3.1}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L1.t.mid\endcsname{\ensuremath{-0.4}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L1.t.small\endcsname{\ensuremath{+3.6}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L3.all\endcsname{\ensuremath{+4.11}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L3.all.ci\endcsname{\ensuremath{[+1.7,\,+6.9]}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L3.large\endcsname{\ensuremath{+1.80}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L3.large.ci\endcsname{\ensuremath{[-0.1,\,+4.2]}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L3.mid\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L3.mid.ci\endcsname{\ensuremath{[-4.1,\,+2.1]}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L3.sh.large\endcsname{14}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L3.sh.mid\endcsname{\ensuremath{-5}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L3.sh.small\endcsname{90}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L3.small\endcsname{\ensuremath{+11.02}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L3.small.ci\endcsname{\ensuremath{[+5.5,\,+17.5]}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L3.t.all\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L3.t.large\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L3.t.mid\endcsname{\ensuremath{-0.2}}
\expandafter\gdef\csname R@an.strata_kits.vox.tum.L3.t.small\endcsname{\ensuremath{+5.6}}
\expandafter\gdef\csname R@an.strata_kits.zs.d31.all\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.strata_kits.zs.d31.all.ci\endcsname{\ensuremath{[-0.9,\,+3.7]}}
\expandafter\gdef\csname R@an.strata_kits.zs.d31.thick\endcsname{\ensuremath{+4.06}}
\expandafter\gdef\csname R@an.strata_kits.zs.d31.thick.ci\endcsname{\ensuremath{[+0.9,\,+8.4]}}
\expandafter\gdef\csname R@an.strata_kits.zs.d31.thin\endcsname{\ensuremath{-1.31}}
\expandafter\gdef\csname R@an.strata_kits.zs.d31.thin.ci\endcsname{\ensuremath{[-3.8,\,+1.1]}}
\expandafter\gdef\csname R@an.strata_kits.zs.hard.dn.L1.thick\endcsname{1}
\expandafter\gdef\csname R@an.strata_kits.zs.hard.dn.L1.thin\endcsname{2}
\expandafter\gdef\csname R@an.strata_kits.zs.hard.dn.L3.thick\endcsname{0}
\expandafter\gdef\csname R@an.strata_kits.zs.hard.dn.L3.thin\endcsname{2}
\expandafter\gdef\csname R@an.strata_kits.zs.hard.n.thick\endcsname{7}
\expandafter\gdef\csname R@an.strata_kits.zs.hard.n.thin\endcsname{6}
\expandafter\gdef\csname R@an.strata_kits.zs.hard.up.L1.thick\endcsname{2}
\expandafter\gdef\csname R@an.strata_kits.zs.hard.up.L1.thin\endcsname{2}
\expandafter\gdef\csname R@an.strata_kits.zs.hard.up.L3.thick\endcsname{6}
\expandafter\gdef\csname R@an.strata_kits.zs.hard.up.L3.thin\endcsname{3}
\expandafter\gdef\csname R@an.strata_kits.zs.n.thick\endcsname{46}
\expandafter\gdef\csname R@an.strata_kits.zs.n.thin\endcsname{52}
\expandafter\gdef\csname R@an.strata_kits.zs.nsd.thick\endcsname{1.20}
\expandafter\gdef\csname R@an.strata_kits.zs.nsd.thin\endcsname{1.58}
\expandafter\gdef\csname R@an.strata_kits.zs.pair.thick\endcsname{1.47}
\expandafter\gdef\csname R@an.strata_kits.zs.pair.thin\endcsname{1.93}
\expandafter\gdef\csname R@an.strata_kits.zs.pool.thick\endcsname{72.8}
\expandafter\gdef\csname R@an.strata_kits.zs.pool.thin\endcsname{75.6}
\expandafter\gdef\csname R@an.strata_kits.zs.split\endcsname{4}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L1.all\endcsname{\ensuremath{+2.90}}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L1.all.ci\endcsname{\ensuremath{[+0.4,\,+5.5]}}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L1.sh.thick\endcsname{38}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L1.sh.thin\endcsname{62}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L1.t.all\endcsname{\ensuremath{+2.4}}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L1.t.thick\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L1.t.thin\endcsname{\ensuremath{+2.2}}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L1.thick\endcsname{\ensuremath{+2.33}}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L1.thick.ci\endcsname{\ensuremath{[-1.7,\,+6.8]}}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L1.thin\endcsname{\ensuremath{+3.40}}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L1.thin.ci\endcsname{\ensuremath{[+0.6,\,+6.4]}}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L3.all\endcsname{\ensuremath{+4.11}}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L3.all.ci\endcsname{\ensuremath{[+1.7,\,+6.9]}}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L3.sh.thick\endcsname{73}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L3.sh.thin\endcsname{27}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L3.t.all\endcsname{\ensuremath{+3.3}}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L3.t.thick\endcsname{\ensuremath{+5.3}}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L3.t.thin\endcsname{\ensuremath{+1.3}}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L3.thick\endcsname{\ensuremath{+6.39}}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L3.thick.ci\endcsname{\ensuremath{[+1.8,\,+11.5]}}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L3.thin\endcsname{\ensuremath{+2.09}}
\expandafter\gdef\csname R@an.strata_kits.zs.tum.L3.thin.ci\endcsname{\ensuremath{[+0.01,\,+4.29]}}
\expandafter\gdef\csname R@an.strata_kits.zs.x.L1.thick.large\endcsname{\ensuremath{+1.7}}
\expandafter\gdef\csname R@an.strata_kits.zs.x.L1.thick.mid\endcsname{\ensuremath{+3.4}}
\expandafter\gdef\csname R@an.strata_kits.zs.x.L1.thick.small\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.strata_kits.zs.x.L1.thin.large\endcsname{\ensuremath{+2.7}}
\expandafter\gdef\csname R@an.strata_kits.zs.x.L1.thin.mid\endcsname{\ensuremath{+3.4}}
\expandafter\gdef\csname R@an.strata_kits.zs.x.L1.thin.small\endcsname{\ensuremath{+4.0}}
\expandafter\gdef\csname R@an.strata_kits.zs.x.L3.thick.large\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.strata_kits.zs.x.L3.thick.mid\endcsname{\ensuremath{+5.9}}
\expandafter\gdef\csname R@an.strata_kits.zs.x.L3.thick.small\endcsname{\ensuremath{+11.2}}
\expandafter\gdef\csname R@an.strata_kits.zs.x.L3.thin.large\endcsname{\ensuremath{+0.9}}
\expandafter\gdef\csname R@an.strata_kits.zs.x.L3.thin.mid\endcsname{\ensuremath{+2.1}}
\expandafter\gdef\csname R@an.strata_kits.zs.x.L3.thin.small\endcsname{\ensuremath{+3.0}}
\expandafter\gdef\csname R@an.strata_kits.zs.xn.thick.large\endcsname{17}
\expandafter\gdef\csname R@an.strata_kits.zs.xn.thick.mid\endcsname{15}
\expandafter\gdef\csname R@an.strata_kits.zs.xn.thick.small\endcsname{14}
\expandafter\gdef\csname R@an.strata_kits.zs.xn.thin.large\endcsname{15}
\expandafter\gdef\csname R@an.strata_kits.zs.xn.thin.mid\endcsname{18}
\expandafter\gdef\csname R@an.strata_kits.zs.xn.thin.small\endcsname{19}
\expandafter\gdef\csname R@an.wall.def.hosts\endcsname{6}
\expandafter\gdef\csname R@an.wall.def.hours\endcsname{9.57}
\expandafter\gdef\csname R@an.wall.def.hours.sd\endcsname{0.77}
\expandafter\gdef\csname R@an.wall.def.n\endcsname{9}
\expandafter\gdef\csname R@an.wall.def.seeds\endcsname{3, 4, 5, 6, 7, 8, 9, 10, 11}
\expandafter\gdef\csname R@an.wall.def.spe\endcsname{33.3}
\expandafter\gdef\csname R@an.wall.def.spe.max\endcsname{38.2}
\expandafter\gdef\csname R@an.wall.def.spe.min\endcsname{31.6}
\expandafter\gdef\csname R@an.wall.def.spe.sd\endcsname{2.8}
\expandafter\gdef\csname R@an.wall.def.trainh\endcsname{9.26}
\expandafter\gdef\csname R@an.wall.pool.hosts\endcsname{1}
\expandafter\gdef\csname R@an.wall.pool.hours\endcsname{9.18}
\expandafter\gdef\csname R@an.wall.pool.hours.sd\endcsname{0.03}
\expandafter\gdef\csname R@an.wall.pool.n\endcsname{3}
\expandafter\gdef\csname R@an.wall.pool.seeds\endcsname{0, 1, 2}
\expandafter\gdef\csname R@an.wall.pool.spe\endcsname{32.0}
\expandafter\gdef\csname R@an.wall.pool.spe.max\endcsname{32.1}
\expandafter\gdef\csname R@an.wall.pool.spe.min\endcsname{31.9}
\expandafter\gdef\csname R@an.wall.pool.spe.sd\endcsname{0.1}
\expandafter\gdef\csname R@an.wall.pool.trainh\endcsname{8.88}
\expandafter\gdef\csname R@an.wall.reconcile\endcsname{the two earlier ratios of {\ifdefined\archL\archL\else XX-Net-L\fi} differ in which runs enter, not in the quantity: an.cost_accuracy divides the seed-0 run's training hours by the frozen pool's mean (one run against 3: 1.00$\times$), the published table divides the mean of its 3 finished runs by the same pool mean (0.92$\times$), and this family divides the mean of its 3 runs by the mean of the 9 stock runs (0.88$\times$); the 3 {\ifdefined\archL\archL\else XX-Net-L\fi} runs ran on 3 nodes and take 27.4 to 31.8 s per epoch (the 9 stock runs 31.6 to 38.2), so the ratio of one run carries that spread}
\expandafter\gdef\csname R@an.wall.resm.hosts\endcsname{2}
\expandafter\gdef\csname R@an.wall.resm.hours\endcsname{12.17}
\expandafter\gdef\csname R@an.wall.resm.hours.sd\endcsname{0.06}
\expandafter\gdef\csname R@an.wall.resm.n\endcsname{3}
\expandafter\gdef\csname R@an.wall.resm.s0.xpool\endcsname{1.32}
\expandafter\gdef\csname R@an.wall.resm.seeds\endcsname{0, 1, 2}
\expandafter\gdef\csname R@an.wall.resm.spe\endcsname{42.5}
\expandafter\gdef\csname R@an.wall.resm.spe.max\endcsname{42.6}
\expandafter\gdef\csname R@an.wall.resm.spe.min\endcsname{42.2}
\expandafter\gdef\csname R@an.wall.resm.spe.sd\endcsname{0.2}
\expandafter\gdef\csname R@an.wall.resm.trainh\endcsname{11.79}
\expandafter\gdef\csname R@an.wall.resm.x.hours\endcsname{1.27}
\expandafter\gdef\csname R@an.wall.resm.x.spe\endcsname{1.27}
\expandafter\gdef\csname R@an.wall.resm.xpool.trainh\endcsname{1.33}
\expandafter\gdef\csname R@an.wall.sentence\endcsname{on KiTS23 fold 0 a 1000-epoch training run takes 29.4 s per training epoch for {\ifdefined\archL\archL\else XX-Net-L\fi} (mean of 3 runs, SD 2.2), 42.5 s for ResEnc-M (3 runs, SD 0.2) and 33.3 s for the nnU-Net default (9 stock runs, SD 2.8), that is 0.88$\times$ and 1.27$\times$ of the default's; with the final validation a run takes 8.42, 12.17 and 9.57 hours}
\expandafter\gdef\csname R@an.wall.state\endcsname{def 9 runs, pool 3 runs, xl 3 runs, xa 3 runs, resm 3 runs}
\expandafter\gdef\csname R@an.wall.xa.hosts\endcsname{2}
\expandafter\gdef\csname R@an.wall.xa.hours\endcsname{8.74}
\expandafter\gdef\csname R@an.wall.xa.hours.sd\endcsname{0.35}
\expandafter\gdef\csname R@an.wall.xa.n\endcsname{3}
\expandafter\gdef\csname R@an.wall.xa.s0.xpool\endcsname{0.96}
\expandafter\gdef\csname R@an.wall.xa.seeds\endcsname{0, 1, 2}
\expandafter\gdef\csname R@an.wall.xa.spe\endcsname{30.4}
\expandafter\gdef\csname R@an.wall.xa.spe.max\endcsname{31.6}
\expandafter\gdef\csname R@an.wall.xa.spe.min\endcsname{29.2}
\expandafter\gdef\csname R@an.wall.xa.spe.sd\endcsname{1.2}
\expandafter\gdef\csname R@an.wall.xa.trainh\endcsname{8.46}
\expandafter\gdef\csname R@an.wall.xa.x.hours\endcsname{0.91}
\expandafter\gdef\csname R@an.wall.xa.x.spe\endcsname{0.91}
\expandafter\gdef\csname R@an.wall.xa.xpool.trainh\endcsname{0.95}
\expandafter\gdef\csname R@an.wall.xl.hosts\endcsname{3}
\expandafter\gdef\csname R@an.wall.xl.hours\endcsname{8.42}
\expandafter\gdef\csname R@an.wall.xl.hours.sd\endcsname{0.62}
\expandafter\gdef\csname R@an.wall.xl.n\endcsname{3}
\expandafter\gdef\csname R@an.wall.xl.s0.xpool\endcsname{1.00}
\expandafter\gdef\csname R@an.wall.xl.seeds\endcsname{0, 1, 2}
\expandafter\gdef\csname R@an.wall.xl.spe\endcsname{29.4}
\expandafter\gdef\csname R@an.wall.xl.spe.max\endcsname{31.8}
\expandafter\gdef\csname R@an.wall.xl.spe.min\endcsname{27.4}
\expandafter\gdef\csname R@an.wall.xl.spe.sd\endcsname{2.2}
\expandafter\gdef\csname R@an.wall.xl.trainh\endcsname{8.17}
\expandafter\gdef\csname R@an.wall.xl.x.hours\endcsname{0.88}
\expandafter\gdef\csname R@an.wall.xl.x.spe\endcsname{0.88}
\expandafter\gdef\csname R@an.wall.xl.xpool.trainh\endcsname{0.92}
\expandafter\gdef\csname R@an.wavefunnel.ablation.arms\endcsname{AB1, AB2, AB3, AB4, AB5, AB6, AB7, AB8, AB9, AB10, AB11}
\expandafter\gdef\csname R@an.wavefunnel.ablation.files\endcsname{cand_S1_xl_k3.py, cand_S2_xl_nogrn.py, cand_S3_xl_cat.py, cand_S4_xl_dec2.py, cand_S5_xl_b2.py, cand_S6_xl_s4only.py, cand_S7_iso_width.py, cand_S8_hand_effidec.py, cand_S9_xl_w075.py, cand_S10_xl_w125.py, cand_S11_iso_params.py}
\expandafter\gdef\csname R@an.wavefunnel.ablation.n\endcsname{11}
\expandafter\gdef\csname R@an.wavefunnel.candidate.files\endcsname{63}
\expandafter\gdef\csname R@an.wavefunnel.designs\endcsname{51}
\expandafter\gdef\csname R@an.wavefunnel.ideas.documents\endcsname{24}
\expandafter\gdef\csname R@an.wavefunnel.ideas.ledger\endcsname{87}
\expandafter\gdef\csname R@an.wavefunnel.review.docs\endcsname{6}
\expandafter\gdef\csname R@an.wavefunnel.review.of\endcsname{50}
\expandafter\gdef\csname R@an.wavefunnel.review.phrase\endcsname{38 of the 50 ideas of the six waves with a per-idea review record (waves 2, 3, 5, 6, 7 and 8) carry a recorded verdict}
\expandafter\gdef\csname R@an.wavefunnel.review.waves\endcsname{2,3,5,6,7,8}
\expandafter\gdef\csname R@an.wavefunnel.total.built\endcsname{51}
\expandafter\gdef\csname R@an.wavefunnel.total.crossvalidated\endcsname{12}
\expandafter\gdef\csname R@an.wavefunnel.total.cvruns\endcsname{128}
\expandafter\gdef\csname R@an.wavefunnel.total.default.built\endcsname{1}
\expandafter\gdef\csname R@an.wavefunnel.total.fired\endcsname{31}
\expandafter\gdef\csname R@an.wavefunnel.total.fits3\endcsname{44}
\expandafter\gdef\csname R@an.wavefunnel.total.funded\endcsname{44}
\expandafter\gdef\csname R@an.wavefunnel.total.passed\endcsname{9}
\expandafter\gdef\csname R@an.wavefunnel.total.profiled\endcsname{51}
\expandafter\gdef\csname R@an.wavefunnel.total.proposed\endcsname{111}
\expandafter\gdef\csname R@an.wavefunnel.total.rep_amos\endcsname{5}
\expandafter\gdef\csname R@an.wavefunnel.total.rep_kits\endcsname{25}
\expandafter\gdef\csname R@an.wavefunnel.total.replicated\endcsname{25}
\expandafter\gdef\csname R@an.wavefunnel.total.reviewed\endcsname{38}
\expandafter\gdef\csname R@an.wavefunnel.total.screened\endcsname{38}
\expandafter\gdef\csname R@an.wavefunnel.w1.built\endcsname{6}
\expandafter\gdef\csname R@an.wavefunnel.w1.crossvalidated\endcsname{3}
\expandafter\gdef\csname R@an.wavefunnel.w1.cvruns\endcsname{36}
\expandafter\gdef\csname R@an.wavefunnel.w1.fired\endcsname{6}
\expandafter\gdef\csname R@an.wavefunnel.w1.fits3\endcsname{6}
\expandafter\gdef\csname R@an.wavefunnel.w1.funded\endcsname{6}
\expandafter\gdef\csname R@an.wavefunnel.w1.passed\endcsname{6}
\expandafter\gdef\csname R@an.wavefunnel.w1.profiled\endcsname{6}
\expandafter\gdef\csname R@an.wavefunnel.w1.proposed\endcsname{6}
\expandafter\gdef\csname R@an.wavefunnel.w1.rep_amos\endcsname{5}
\expandafter\gdef\csname R@an.wavefunnel.w1.rep_kits\endcsname{6}
\expandafter\gdef\csname R@an.wavefunnel.w1.replicated\endcsname{6}
\expandafter\gdef\csname R@an.wavefunnel.w1.reviewed\endcsname{none}
\expandafter\gdef\csname R@an.wavefunnel.w1.screened\endcsname{6}
\expandafter\gdef\csname R@an.wavefunnel.w2.built\endcsname{7}
\expandafter\gdef\csname R@an.wavefunnel.w2.crossvalidated\endcsname{0}
\expandafter\gdef\csname R@an.wavefunnel.w2.cvruns\endcsname{0}
\expandafter\gdef\csname R@an.wavefunnel.w2.fired\endcsname{2}
\expandafter\gdef\csname R@an.wavefunnel.w2.fits3\endcsname{6}
\expandafter\gdef\csname R@an.wavefunnel.w2.funded\endcsname{7}
\expandafter\gdef\csname R@an.wavefunnel.w2.passed\endcsname{0}
\expandafter\gdef\csname R@an.wavefunnel.w2.profiled\endcsname{7}
\expandafter\gdef\csname R@an.wavefunnel.w2.proposed\endcsname{8}
\expandafter\gdef\csname R@an.wavefunnel.w2.rep_amos\endcsname{0}
\expandafter\gdef\csname R@an.wavefunnel.w2.rep_kits\endcsname{1}
\expandafter\gdef\csname R@an.wavefunnel.w2.replicated\endcsname{1}
\expandafter\gdef\csname R@an.wavefunnel.w2.reviewed\endcsname{6}
\expandafter\gdef\csname R@an.wavefunnel.w2.screened\endcsname{7}
\expandafter\gdef\csname R@an.wavefunnel.w3.built\endcsname{11}
\expandafter\gdef\csname R@an.wavefunnel.w3.crossvalidated\endcsname{1}
\expandafter\gdef\csname R@an.wavefunnel.w3.cvruns\endcsname{12}
\expandafter\gdef\csname R@an.wavefunnel.w3.fired\endcsname{2}
\expandafter\gdef\csname R@an.wavefunnel.w3.fits3\endcsname{8}
\expandafter\gdef\csname R@an.wavefunnel.w3.funded\endcsname{9}
\expandafter\gdef\csname R@an.wavefunnel.w3.passed\endcsname{0}
\expandafter\gdef\csname R@an.wavefunnel.w3.profiled\endcsname{11}
\expandafter\gdef\csname R@an.wavefunnel.w3.proposed\endcsname{18}
\expandafter\gdef\csname R@an.wavefunnel.w3.rep_amos\endcsname{0}
\expandafter\gdef\csname R@an.wavefunnel.w3.rep_kits\endcsname{1}
\expandafter\gdef\csname R@an.wavefunnel.w3.replicated\endcsname{1}
\expandafter\gdef\csname R@an.wavefunnel.w3.reviewed\endcsname{8}
\expandafter\gdef\csname R@an.wavefunnel.w3.screened\endcsname{3}
\expandafter\gdef\csname R@an.wavefunnel.w4.built\endcsname{6}
\expandafter\gdef\csname R@an.wavefunnel.w4.crossvalidated\endcsname{1}
\expandafter\gdef\csname R@an.wavefunnel.w4.cvruns\endcsname{12}
\expandafter\gdef\csname R@an.wavefunnel.w4.fired\endcsname{5}
\expandafter\gdef\csname R@an.wavefunnel.w4.fits3\endcsname{5}
\expandafter\gdef\csname R@an.wavefunnel.w4.funded\endcsname{6}
\expandafter\gdef\csname R@an.wavefunnel.w4.passed\endcsname{0}
\expandafter\gdef\csname R@an.wavefunnel.w4.profiled\endcsname{6}
\expandafter\gdef\csname R@an.wavefunnel.w4.proposed\endcsname{55}
\expandafter\gdef\csname R@an.wavefunnel.w4.rep_amos\endcsname{0}
\expandafter\gdef\csname R@an.wavefunnel.w4.rep_kits\endcsname{4}
\expandafter\gdef\csname R@an.wavefunnel.w4.replicated\endcsname{4}
\expandafter\gdef\csname R@an.wavefunnel.w4.reviewed\endcsname{none}
\expandafter\gdef\csname R@an.wavefunnel.w4.screened\endcsname{6}
\expandafter\gdef\csname R@an.wavefunnel.w5.built\endcsname{7}
\expandafter\gdef\csname R@an.wavefunnel.w5.crossvalidated\endcsname{2}
\expandafter\gdef\csname R@an.wavefunnel.w5.cvruns\endcsname{24}
\expandafter\gdef\csname R@an.wavefunnel.w5.fired\endcsname{3}
\expandafter\gdef\csname R@an.wavefunnel.w5.fits3\endcsname{5}
\expandafter\gdef\csname R@an.wavefunnel.w5.funded\endcsname{3}
\expandafter\gdef\csname R@an.wavefunnel.w5.passed\endcsname{0}
\expandafter\gdef\csname R@an.wavefunnel.w5.profiled\endcsname{7}
\expandafter\gdef\csname R@an.wavefunnel.w5.proposed\endcsname{10}
\expandafter\gdef\csname R@an.wavefunnel.w5.rep_amos\endcsname{0}
\expandafter\gdef\csname R@an.wavefunnel.w5.rep_kits\endcsname{3}
\expandafter\gdef\csname R@an.wavefunnel.w5.replicated\endcsname{3}
\expandafter\gdef\csname R@an.wavefunnel.w5.reviewed\endcsname{10}
\expandafter\gdef\csname R@an.wavefunnel.w5.screened\endcsname{3}
\expandafter\gdef\csname R@an.wavefunnel.w6.built\endcsname{2}
\expandafter\gdef\csname R@an.wavefunnel.w6.crossvalidated\endcsname{1}
\expandafter\gdef\csname R@an.wavefunnel.w6.cvruns\endcsname{12}
\expandafter\gdef\csname R@an.wavefunnel.w6.fired\endcsname{1}
\expandafter\gdef\csname R@an.wavefunnel.w6.fits3\endcsname{2}
\expandafter\gdef\csname R@an.wavefunnel.w6.funded\endcsname{1}
\expandafter\gdef\csname R@an.wavefunnel.w6.passed\endcsname{1}
\expandafter\gdef\csname R@an.wavefunnel.w6.profiled\endcsname{2}
\expandafter\gdef\csname R@an.wavefunnel.w6.proposed\endcsname{1}
\expandafter\gdef\csname R@an.wavefunnel.w6.rep_amos\endcsname{0}
\expandafter\gdef\csname R@an.wavefunnel.w6.rep_kits\endcsname{1}
\expandafter\gdef\csname R@an.wavefunnel.w6.replicated\endcsname{1}
\expandafter\gdef\csname R@an.wavefunnel.w6.reviewed\endcsname{1}
\expandafter\gdef\csname R@an.wavefunnel.w6.screened\endcsname{1}
\expandafter\gdef\csname R@an.wavefunnel.w7.built\endcsname{7}
\expandafter\gdef\csname R@an.wavefunnel.w7.crossvalidated\endcsname{3}
\expandafter\gdef\csname R@an.wavefunnel.w7.cvruns\endcsname{28}
\expandafter\gdef\csname R@an.wavefunnel.w7.fired\endcsname{7}
\expandafter\gdef\csname R@an.wavefunnel.w7.fits3\endcsname{7}
\expandafter\gdef\csname R@an.wavefunnel.w7.funded\endcsname{7}
\expandafter\gdef\csname R@an.wavefunnel.w7.passed\endcsname{2}
\expandafter\gdef\csname R@an.wavefunnel.w7.profiled\endcsname{7}
\expandafter\gdef\csname R@an.wavefunnel.w7.proposed\endcsname{8}
\expandafter\gdef\csname R@an.wavefunnel.w7.rep_amos\endcsname{0}
\expandafter\gdef\csname R@an.wavefunnel.w7.rep_kits\endcsname{5}
\expandafter\gdef\csname R@an.wavefunnel.w7.replicated\endcsname{5}
\expandafter\gdef\csname R@an.wavefunnel.w7.reviewed\endcsname{8}
\expandafter\gdef\csname R@an.wavefunnel.w7.screened\endcsname{7}
\expandafter\gdef\csname R@an.wavefunnel.w8.built\endcsname{5}
\expandafter\gdef\csname R@an.wavefunnel.w8.crossvalidated\endcsname{1}
\expandafter\gdef\csname R@an.wavefunnel.w8.cvruns\endcsname{4}
\expandafter\gdef\csname R@an.wavefunnel.w8.fired\endcsname{5}
\expandafter\gdef\csname R@an.wavefunnel.w8.fits3\endcsname{5}
\expandafter\gdef\csname R@an.wavefunnel.w8.funded\endcsname{5}
\expandafter\gdef\csname R@an.wavefunnel.w8.passed\endcsname{0}
\expandafter\gdef\csname R@an.wavefunnel.w8.profiled\endcsname{5}
\expandafter\gdef\csname R@an.wavefunnel.w8.proposed\endcsname{5}
\expandafter\gdef\csname R@an.wavefunnel.w8.rep_amos\endcsname{0}
\expandafter\gdef\csname R@an.wavefunnel.w8.rep_kits\endcsname{4}
\expandafter\gdef\csname R@an.wavefunnel.w8.replicated\endcsname{4}
\expandafter\gdef\csname R@an.wavefunnel.w8.reviewed\endcsname{5}
\expandafter\gdef\csname R@an.wavefunnel.w8.screened\endcsname{5}
\expandafter\gdef\csname R@an.wavefunnel.waves\endcsname{8}
\expandafter\gdef\csname R@an.winners.arm.C1.gain0\endcsname{\ensuremath{+1.52}}
\expandafter\gdef\csname R@an.winners.arm.C1.gain14\endcsname{\pend}
\expandafter\gdef\csname R@an.winners.arm.C1.nfold\endcsname{0}
\expandafter\gdef\csname R@an.winners.arm.C1.z0\endcsname{\ensuremath{+3.1}}
\expandafter\gdef\csname R@an.winners.arm.D1.gain0\endcsname{\ensuremath{+0.60}}
\expandafter\gdef\csname R@an.winners.arm.D1.gain14\endcsname{\pend}
\expandafter\gdef\csname R@an.winners.arm.D1.nfold\endcsname{0}
\expandafter\gdef\csname R@an.winners.arm.D1.z0\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.winners.arm.D2.gain0\endcsname{\ensuremath{+1.01}}
\expandafter\gdef\csname R@an.winners.arm.D2.gain14\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@an.winners.arm.D2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.winners.arm.D2.ratio\endcsname{1.03}
\expandafter\gdef\csname R@an.winners.arm.D2.z0\endcsname{\ensuremath{+2.0}}
\expandafter\gdef\csname R@an.winners.arm.L1.gain0\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@an.winners.arm.L1.gain14\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@an.winners.arm.L1.nfold\endcsname{4}
\expandafter\gdef\csname R@an.winners.arm.L1.ratio\endcsname{0.827}
\expandafter\gdef\csname R@an.winners.arm.L1.z0\endcsname{\ensuremath{+5.3}}
\expandafter\gdef\csname R@an.winners.arm.L1b.gain0\endcsname{\ensuremath{+1.43}}
\expandafter\gdef\csname R@an.winners.arm.L1b.gain14\endcsname{\ensuremath{+1.54}}
\expandafter\gdef\csname R@an.winners.arm.L1b.nfold\endcsname{4}
\expandafter\gdef\csname R@an.winners.arm.L1b.ratio\endcsname{1.08}
\expandafter\gdef\csname R@an.winners.arm.L1b.z0\endcsname{\ensuremath{+2.9}}
\expandafter\gdef\csname R@an.winners.arm.L2.gain0\endcsname{\ensuremath{-0.77}}
\expandafter\gdef\csname R@an.winners.arm.L2.gain14\endcsname{\pend}
\expandafter\gdef\csname R@an.winners.arm.L2.nfold\endcsname{0}
\expandafter\gdef\csname R@an.winners.arm.L2.z0\endcsname{\ensuremath{-1.6}}
\expandafter\gdef\csname R@an.winners.arm.L3.gain0\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.winners.arm.L3.gain14\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@an.winners.arm.L3.nfold\endcsname{4}
\expandafter\gdef\csname R@an.winners.arm.L3.ratio\endcsname{0.56}
\expandafter\gdef\csname R@an.winners.arm.L3.z0\endcsname{\ensuremath{+2.5}}
\expandafter\gdef\csname R@an.winners.arm.L4.gain0\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.winners.arm.L4.gain14\endcsname{\pend}
\expandafter\gdef\csname R@an.winners.arm.L4.nfold\endcsname{0}
\expandafter\gdef\csname R@an.winners.arm.L4.z0\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.winners.arm.L6.gain0\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@an.winners.arm.L6.gain14\endcsname{\pend}
\expandafter\gdef\csname R@an.winners.arm.L6.nfold\endcsname{0}
\expandafter\gdef\csname R@an.winners.arm.L6.z0\endcsname{\ensuremath{+1.4}}
\expandafter\gdef\csname R@an.winners.arm.P3c.gain0\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.winners.arm.P3c.gain14\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@an.winners.arm.P3c.nfold\endcsname{4}
\expandafter\gdef\csname R@an.winners.arm.P3c.ratio\endcsname{1.87}
\expandafter\gdef\csname R@an.winners.arm.P3c.z0\endcsname{\ensuremath{+0.6}}
\expandafter\gdef\csname R@an.winners.arm.S2.gain0\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.winners.arm.S2.gain14\endcsname{\pend}
\expandafter\gdef\csname R@an.winners.arm.S2.nfold\endcsname{0}
\expandafter\gdef\csname R@an.winners.arm.S2.z0\endcsname{\ensuremath{-0.6}}
\expandafter\gdef\csname R@an.winners.arm.V5A5.gain0\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.winners.arm.V5A5.gain14\endcsname{\pend}
\expandafter\gdef\csname R@an.winners.arm.V5A5.nfold\endcsname{0}
\expandafter\gdef\csname R@an.winners.arm.V5A5.z0\endcsname{\ensuremath{+2.6}}
\expandafter\gdef\csname R@an.winners.arm.V5B1.gain0\endcsname{\ensuremath{+1.41}}
\expandafter\gdef\csname R@an.winners.arm.V5B1.gain14\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.winners.arm.V5B1.nfold\endcsname{4}
\expandafter\gdef\csname R@an.winners.arm.V5B1.ratio\endcsname{0.70}
\expandafter\gdef\csname R@an.winners.arm.V5B1.z0\endcsname{\ensuremath{+2.8}}
\expandafter\gdef\csname R@an.winners.arm.V5B2.gain0\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.winners.arm.V5B2.gain14\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.winners.arm.V5B2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.winners.arm.V5B2.ratio\endcsname{\ensuremath{-1.32}}
\expandafter\gdef\csname R@an.winners.arm.V5B2.z0\endcsname{\ensuremath{+1.2}}
\expandafter\gdef\csname R@an.winners.arm.V6A1r.gain0\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@an.winners.arm.V6A1r.gain14\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.winners.arm.V6A1r.nfold\endcsname{4}
\expandafter\gdef\csname R@an.winners.arm.V6A1r.ratio\endcsname{0.34}
\expandafter\gdef\csname R@an.winners.arm.V6A1r.z0\endcsname{\ensuremath{+1.7}}
\expandafter\gdef\csname R@an.winners.arm.V7A1.gain0\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.winners.arm.V7A1.gain14\endcsname{\ensuremath{+1.63}}
\expandafter\gdef\csname R@an.winners.arm.V7A1.nfold\endcsname{4}
\expandafter\gdef\csname R@an.winners.arm.V7A1.ratio\endcsname{0.916}
\expandafter\gdef\csname R@an.winners.arm.V7A1.z0\endcsname{\ensuremath{+3.6}}
\expandafter\gdef\csname R@an.winners.arm.V7A2.gain0\endcsname{\ensuremath{+1.41}}
\expandafter\gdef\csname R@an.winners.arm.V7A2.gain14\endcsname{\ensuremath{+0.91}}
\expandafter\gdef\csname R@an.winners.arm.V7A2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.winners.arm.V7A2.ratio\endcsname{0.65}
\expandafter\gdef\csname R@an.winners.arm.V7A2.z0\endcsname{\ensuremath{+2.9}}
\expandafter\gdef\csname R@an.winners.arm.V7B1.gain0\endcsname{\ensuremath{+1.50}}
\expandafter\gdef\csname R@an.winners.arm.V7B1.gain14\endcsname{\pend}
\expandafter\gdef\csname R@an.winners.arm.V7B1.nfold\endcsname{0}
\expandafter\gdef\csname R@an.winners.arm.V7B1.z0\endcsname{\ensuremath{+3.0}}
\expandafter\gdef\csname R@an.winners.arm.V7B2.gain0\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@an.winners.arm.V7B2.gain14\endcsname{\pend}
\expandafter\gdef\csname R@an.winners.arm.V7B2.nfold\endcsname{0}
\expandafter\gdef\csname R@an.winners.arm.V7B2.z0\endcsname{\ensuremath{+1.9}}
\expandafter\gdef\csname R@an.winners.arm.V7C1.gain0\endcsname{\ensuremath{+1.56}}
\expandafter\gdef\csname R@an.winners.arm.V7C1.gain14\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.winners.arm.V7C1.nfold\endcsname{4}
\expandafter\gdef\csname R@an.winners.arm.V7C1.ratio\endcsname{0.50}
\expandafter\gdef\csname R@an.winners.arm.V7C1.z0\endcsname{\ensuremath{+3.2}}
\expandafter\gdef\csname R@an.winners.arm.V8A1.gain0\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.winners.arm.V8A1.gain14\endcsname{\pend}
\expandafter\gdef\csname R@an.winners.arm.V8A1.nfold\endcsname{0}
\expandafter\gdef\csname R@an.winners.arm.V8A1.z0\endcsname{\ensuremath{+0.7}}
\expandafter\gdef\csname R@an.winners.arm.V8A2.gain0\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.winners.arm.V8A2.gain14\endcsname{\pend}
\expandafter\gdef\csname R@an.winners.arm.V8A2.nfold\endcsname{0}
\expandafter\gdef\csname R@an.winners.arm.V8A2.z0\endcsname{\ensuremath{+2.0}}
\expandafter\gdef\csname R@an.winners.arm.V8B1.gain0\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.winners.arm.V8B1.gain14\endcsname{\pend}
\expandafter\gdef\csname R@an.winners.arm.V8B1.nfold\endcsname{0}
\expandafter\gdef\csname R@an.winners.arm.V8B1.z0\endcsname{\ensuremath{+1.0}}
\expandafter\gdef\csname R@an.winners.arm.V8B2.gain0\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.winners.arm.V8B2.gain14\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.winners.arm.V8B2.nfold\endcsname{4}
\expandafter\gdef\csname R@an.winners.arm.V8B2.ratio\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.winners.arm.V8B2.z0\endcsname{\ensuremath{+1.7}}
\expandafter\gdef\csname R@an.winners.arm.W1c.gain0\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@an.winners.arm.W1c.gain14\endcsname{\pend}
\expandafter\gdef\csname R@an.winners.arm.W1c.nfold\endcsname{0}
\expandafter\gdef\csname R@an.winners.arm.W1c.z0\endcsname{\ensuremath{+0.4}}
\expandafter\gdef\csname R@an.winners.arm.list\endcsname{ResEnc-M; ResEnc-matched; HyReX; fn.-identical control; LeanDec; LeanAdd; LeanAdd-NeXt; HyReX-k9; {\ifdefined\archA\archA\else XX-Net-A\fi}; {\ifdefined\archL\archL\else XX-Net-L\fi}; LeanDeepMid+FD; Stem1}
\expandafter\gdef\csname R@an.winners.curse.B\endcsname{100\,000}
\expandafter\gdef\csname R@an.winners.curse.agent.top.drop\endcsname{\ensuremath{-1.11}}
\expandafter\gdef\csname R@an.winners.curse.agent.top.fresh\endcsname{85.78}
\expandafter\gdef\csname R@an.winners.curse.agent.top.name\endcsname{HyReX+dec. capacity}
\expandafter\gdef\csname R@an.winners.curse.agent.top.null.drop.hi\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.winners.curse.agent.top.null.drop.lo\endcsname{\ensuremath{-2.43}}
\expandafter\gdef\csname R@an.winners.curse.agent.top.null.drop.mean\endcsname{\ensuremath{-1.37}}
\expandafter\gdef\csname R@an.winners.curse.agent.top.null.hi\endcsname{86.70}
\expandafter\gdef\csname R@an.winners.curse.agent.top.null.lo\endcsname{85.49}
\expandafter\gdef\csname R@an.winners.curse.agent.top.null.med\endcsname{86.01}
\expandafter\gdef\csname R@an.winners.curse.agent.top.pos\endcsname{98}
\expandafter\gdef\csname R@an.winners.curse.agent.top.rank\endcsname{1}
\expandafter\gdef\csname R@an.winners.curse.agent.top.s0\endcsname{86.89}
\expandafter\gdef\csname R@an.winners.curse.alt.sd\endcsname{0.63}
\expandafter\gdef\csname R@an.winners.curse.alt.top.drop.mean\endcsname{\ensuremath{-1.29}}
\expandafter\gdef\csname R@an.winners.curse.alt.top.hi\endcsname{86.52}
\expandafter\gdef\csname R@an.winners.curse.alt.top.lo\endcsname{85.50}
\expandafter\gdef\csname R@an.winners.curse.alt.top.med\endcsname{85.93}
\expandafter\gdef\csname R@an.winners.curse.alt.xl.drop.mean\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.winners.curse.kfresh\endcsname{2}
\expandafter\gdef\csname R@an.winners.curse.n.agent\endcsname{22}
\expandafter\gdef\csname R@an.winners.curse.n.all\endcsname{30}
\expandafter\gdef\csname R@an.winners.curse.null.mean\endcsname{84.67}
\expandafter\gdef\csname R@an.winners.curse.null.n\endcsname{5}
\expandafter\gdef\csname R@an.winners.curse.null.sd\endcsname{0.72}
\expandafter\gdef\csname R@an.winners.curse.r1.drop\endcsname{\ensuremath{-1.11}}
\expandafter\gdef\csname R@an.winners.curse.r1.fresh\endcsname{85.78}
\expandafter\gdef\csname R@an.winners.curse.r1.name\endcsname{HyReX+dec. capacity}
\expandafter\gdef\csname R@an.winners.curse.r1.null.drop.hi\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.winners.curse.r1.null.drop.lo\endcsname{\ensuremath{-2.51}}
\expandafter\gdef\csname R@an.winners.curse.r1.null.drop.mean\endcsname{\ensuremath{-1.47}}
\expandafter\gdef\csname R@an.winners.curse.r1.null.hi\endcsname{86.77}
\expandafter\gdef\csname R@an.winners.curse.r1.null.lo\endcsname{85.62}
\expandafter\gdef\csname R@an.winners.curse.r1.null.med\endcsname{86.11}
\expandafter\gdef\csname R@an.winners.curse.r1.pos\endcsname{97}
\expandafter\gdef\csname R@an.winners.curse.r1.rank\endcsname{1}
\expandafter\gdef\csname R@an.winners.curse.r1.s0\endcsname{86.89}
\expandafter\gdef\csname R@an.winners.curse.r2.drop\endcsname{\ensuremath{-1.54}}
\expandafter\gdef\csname R@an.winners.curse.r2.fresh\endcsname{84.75}
\expandafter\gdef\csname R@an.winners.curse.r2.name\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.winners.curse.r2.null.drop.hi\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@an.winners.curse.r2.null.drop.lo\endcsname{\ensuremath{-2.11}}
\expandafter\gdef\csname R@an.winners.curse.r2.null.drop.mean\endcsname{\ensuremath{-1.16}}
\expandafter\gdef\csname R@an.winners.curse.r2.null.hi\endcsname{86.29}
\expandafter\gdef\csname R@an.winners.curse.r2.null.lo\endcsname{85.42}
\expandafter\gdef\csname R@an.winners.curse.r2.null.med\endcsname{85.82}
\expandafter\gdef\csname R@an.winners.curse.r2.pos\endcsname{95}
\expandafter\gdef\csname R@an.winners.curse.r2.rank\endcsname{2}
\expandafter\gdef\csname R@an.winners.curse.r2.s0\endcsname{86.29}
\expandafter\gdef\csname R@an.winners.curse.r3.drop\endcsname{\ensuremath{-0.60}}
\expandafter\gdef\csname R@an.winners.curse.r3.fresh\endcsname{85.67}
\expandafter\gdef\csname R@an.winners.curse.r3.name\endcsname{LeanDeepMid+FD}
\expandafter\gdef\csname R@an.winners.curse.r3.null.drop.hi\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.winners.curse.r3.null.drop.lo\endcsname{\ensuremath{-1.90}}
\expandafter\gdef\csname R@an.winners.curse.r3.null.drop.mean\endcsname{\ensuremath{-0.98}}
\expandafter\gdef\csname R@an.winners.curse.r3.null.hi\endcsname{86.05}
\expandafter\gdef\csname R@an.winners.curse.r3.null.lo\endcsname{85.29}
\expandafter\gdef\csname R@an.winners.curse.r3.null.med\endcsname{85.64}
\expandafter\gdef\csname R@an.winners.curse.r3.pos\endcsname{99}
\expandafter\gdef\csname R@an.winners.curse.r3.rank\endcsname{3}
\expandafter\gdef\csname R@an.winners.curse.r3.s0\endcsname{86.26}
\expandafter\gdef\csname R@an.winners.curse.r4.drop\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.winners.curse.r4.fresh\endcsname{85.47}
\expandafter\gdef\csname R@an.winners.curse.r4.name\endcsname{HyReX}
\expandafter\gdef\csname R@an.winners.curse.r4.null.drop.hi\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.winners.curse.r4.null.drop.lo\endcsname{\ensuremath{-1.75}}
\expandafter\gdef\csname R@an.winners.curse.r4.null.drop.mean\endcsname{\ensuremath{-0.84}}
\expandafter\gdef\csname R@an.winners.curse.r4.null.hi\endcsname{85.88}
\expandafter\gdef\csname R@an.winners.curse.r4.null.lo\endcsname{85.18}
\expandafter\gdef\csname R@an.winners.curse.r4.null.med\endcsname{85.51}
\expandafter\gdef\csname R@an.winners.curse.r4.pos\endcsname{more than 99}
\expandafter\gdef\csname R@an.winners.curse.r4.rank\endcsname{4}
\expandafter\gdef\csname R@an.winners.curse.r4.s0\endcsname{86.22}
\expandafter\gdef\csname R@an.winners.curse.r5.drop\endcsname{\ensuremath{-0.99}}
\expandafter\gdef\csname R@an.winners.curse.r5.fresh\endcsname{85.22}
\expandafter\gdef\csname R@an.winners.curse.r5.name\endcsname{LeanDil}
\expandafter\gdef\csname R@an.winners.curse.r5.null.drop.hi\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.winners.curse.r5.null.drop.lo\endcsname{\ensuremath{-1.64}}
\expandafter\gdef\csname R@an.winners.curse.r5.null.drop.mean\endcsname{\ensuremath{-0.74}}
\expandafter\gdef\csname R@an.winners.curse.r5.null.hi\endcsname{85.74}
\expandafter\gdef\csname R@an.winners.curse.r5.null.lo\endcsname{85.09}
\expandafter\gdef\csname R@an.winners.curse.r5.null.med\endcsname{85.40}
\expandafter\gdef\csname R@an.winners.curse.r5.pos\endcsname{more than 99}
\expandafter\gdef\csname R@an.winners.curse.r5.rank\endcsname{5}
\expandafter\gdef\csname R@an.winners.curse.r5.s0\endcsname{86.20}
\expandafter\gdef\csname R@an.winners.curse.r6.drop\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.winners.curse.r6.fresh\endcsname{85.82}
\expandafter\gdef\csname R@an.winners.curse.r6.name\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi}}
\expandafter\gdef\csname R@an.winners.curse.r6.null.drop.hi\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.winners.curse.r6.null.drop.lo\endcsname{\ensuremath{-1.54}}
\expandafter\gdef\csname R@an.winners.curse.r6.null.drop.mean\endcsname{\ensuremath{-0.64}}
\expandafter\gdef\csname R@an.winners.curse.r6.null.hi\endcsname{85.63}
\expandafter\gdef\csname R@an.winners.curse.r6.null.lo\endcsname{85.01}
\expandafter\gdef\csname R@an.winners.curse.r6.null.med\endcsname{85.31}
\expandafter\gdef\csname R@an.winners.curse.r6.pos\endcsname{more than 99}
\expandafter\gdef\csname R@an.winners.curse.r6.rank\endcsname{6}
\expandafter\gdef\csname R@an.winners.curse.r6.s0\endcsname{86.09}
\expandafter\gdef\csname R@an.winners.curse.r7.drop\endcsname{\ensuremath{-1.57}}
\expandafter\gdef\csname R@an.winners.curse.r7.fresh\endcsname{84.44}
\expandafter\gdef\csname R@an.winners.curse.r7.name\endcsname{branch control}
\expandafter\gdef\csname R@an.winners.curse.r7.null.drop.hi\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.winners.curse.r7.null.drop.lo\endcsname{\ensuremath{-1.45}}
\expandafter\gdef\csname R@an.winners.curse.r7.null.drop.mean\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.winners.curse.r7.null.hi\endcsname{85.53}
\expandafter\gdef\csname R@an.winners.curse.r7.null.lo\endcsname{84.93}
\expandafter\gdef\csname R@an.winners.curse.r7.null.med\endcsname{85.23}
\expandafter\gdef\csname R@an.winners.curse.r7.pos\endcsname{more than 99}
\expandafter\gdef\csname R@an.winners.curse.r7.rank\endcsname{7}
\expandafter\gdef\csname R@an.winners.curse.r7.s0\endcsname{86.01}
\expandafter\gdef\csname R@an.winners.curse.r8.drop\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.winners.curse.r8.fresh\endcsname{86.04}
\expandafter\gdef\csname R@an.winners.curse.r8.name\endcsname{{\ifdefined\archA\archA\else XX-Net-A\fi}}
\expandafter\gdef\csname R@an.winners.curse.r8.null.drop.hi\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.winners.curse.r8.null.drop.lo\endcsname{\ensuremath{-1.36}}
\expandafter\gdef\csname R@an.winners.curse.r8.null.drop.mean\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@an.winners.curse.r8.null.hi\endcsname{85.45}
\expandafter\gdef\csname R@an.winners.curse.r8.null.lo\endcsname{84.86}
\expandafter\gdef\csname R@an.winners.curse.r8.null.med\endcsname{85.15}
\expandafter\gdef\csname R@an.winners.curse.r8.pos\endcsname{more than 99}
\expandafter\gdef\csname R@an.winners.curse.r8.rank\endcsname{8}
\expandafter\gdef\csname R@an.winners.curse.r8.s0\endcsname{85.93}
\expandafter\gdef\csname R@an.winners.curse.rep.agent.max\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@an.winners.curse.rep.agent.max.name\endcsname{LeanSep}
\expandafter\gdef\csname R@an.winners.curse.rep.agent.mean\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.winners.curse.rep.agent.min\endcsname{\ensuremath{-1.54}}
\expandafter\gdef\csname R@an.winners.curse.rep.agent.min.name\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.winners.curse.rep.agent.n\endcsname{21}
\expandafter\gdef\csname R@an.winners.curse.rep.other.max\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@an.winners.curse.rep.other.max.name\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.winners.curse.rep.other.mean\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.winners.curse.rep.other.min\endcsname{\ensuremath{-1.57}}
\expandafter\gdef\csname R@an.winners.curse.rep.other.min.name\endcsname{branch control}
\expandafter\gdef\csname R@an.winners.curse.rep.other.n\endcsname{4}
\expandafter\gdef\csname R@an.winners.curse.seed\endcsname{20261011}
\expandafter\gdef\csname R@an.winners.curse.top.drop.hi\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@an.winners.curse.top.drop.lo\endcsname{\ensuremath{-2.51}}
\expandafter\gdef\csname R@an.winners.curse.top.drop.mean\endcsname{\ensuremath{-1.47}}
\expandafter\gdef\csname R@an.winners.curse.top.hi\endcsname{86.77}
\expandafter\gdef\csname R@an.winners.curse.top.lo\endcsname{85.62}
\expandafter\gdef\csname R@an.winners.curse.top.med\endcsname{86.11}
\expandafter\gdef\csname R@an.winners.curse.top.obs\endcsname{86.89}
\expandafter\gdef\csname R@an.winners.curse.top.obs.drop\endcsname{\ensuremath{-1.11}}
\expandafter\gdef\csname R@an.winners.curse.top.obs.name\endcsname{HyReX+dec. capacity}
\expandafter\gdef\csname R@an.winners.curse.top.pos\endcsname{97}
\expandafter\gdef\csname R@an.winners.curse.topk.drop.mean\endcsname{\ensuremath{-0.84}}
\expandafter\gdef\csname R@an.winners.curse.topk.k\endcsname{8}
\expandafter\gdef\csname R@an.winners.curse.topk.n\endcsname{8}
\expandafter\gdef\csname R@an.winners.curse.topk.null.drop.mean\endcsname{\ensuremath{-0.86}}
\expandafter\gdef\csname R@an.winners.curse.xa.agent.drop\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.winners.curse.xa.agent.fresh\endcsname{86.04}
\expandafter\gdef\csname R@an.winners.curse.xa.agent.name\endcsname{{\ifdefined\archA\archA\else XX-Net-A\fi}}
\expandafter\gdef\csname R@an.winners.curse.xa.agent.null.drop.hi\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.winners.curse.xa.agent.null.drop.lo\endcsname{\ensuremath{-1.28}}
\expandafter\gdef\csname R@an.winners.curse.xa.agent.null.drop.mean\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@an.winners.curse.xa.agent.null.hi\endcsname{85.39}
\expandafter\gdef\csname R@an.winners.curse.xa.agent.null.lo\endcsname{84.73}
\expandafter\gdef\csname R@an.winners.curse.xa.agent.null.med\endcsname{85.05}
\expandafter\gdef\csname R@an.winners.curse.xa.agent.pos\endcsname{more than 99}
\expandafter\gdef\csname R@an.winners.curse.xa.agent.rank\endcsname{7}
\expandafter\gdef\csname R@an.winners.curse.xa.agent.s0\endcsname{85.93}
\expandafter\gdef\csname R@an.winners.curse.xa.drop\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.winners.curse.xa.fresh\endcsname{86.04}
\expandafter\gdef\csname R@an.winners.curse.xa.name\endcsname{{\ifdefined\archA\archA\else XX-Net-A\fi}}
\expandafter\gdef\csname R@an.winners.curse.xa.null.drop.hi\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.winners.curse.xa.null.drop.lo\endcsname{\ensuremath{-1.36}}
\expandafter\gdef\csname R@an.winners.curse.xa.null.drop.mean\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@an.winners.curse.xa.null.hi\endcsname{85.45}
\expandafter\gdef\csname R@an.winners.curse.xa.null.lo\endcsname{84.86}
\expandafter\gdef\csname R@an.winners.curse.xa.null.med\endcsname{85.15}
\expandafter\gdef\csname R@an.winners.curse.xa.pos\endcsname{more than 99}
\expandafter\gdef\csname R@an.winners.curse.xa.rank\endcsname{8}
\expandafter\gdef\csname R@an.winners.curse.xa.s0\endcsname{85.93}
\expandafter\gdef\csname R@an.winners.curse.xl.agent.drop\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.winners.curse.xl.agent.fresh\endcsname{85.82}
\expandafter\gdef\csname R@an.winners.curse.xl.agent.name\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi}}
\expandafter\gdef\csname R@an.winners.curse.xl.agent.null.drop.hi\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.winners.curse.xl.agent.null.drop.lo\endcsname{\ensuremath{-1.39}}
\expandafter\gdef\csname R@an.winners.curse.xl.agent.null.drop.mean\endcsname{\ensuremath{-0.48}}
\expandafter\gdef\csname R@an.winners.curse.xl.agent.null.hi\endcsname{85.49}
\expandafter\gdef\csname R@an.winners.curse.xl.agent.null.lo\endcsname{84.81}
\expandafter\gdef\csname R@an.winners.curse.xl.agent.null.med\endcsname{85.15}
\expandafter\gdef\csname R@an.winners.curse.xl.agent.pos\endcsname{more than 99}
\expandafter\gdef\csname R@an.winners.curse.xl.agent.rank\endcsname{6}
\expandafter\gdef\csname R@an.winners.curse.xl.agent.s0\endcsname{86.09}
\expandafter\gdef\csname R@an.winners.curse.xl.drop\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.winners.curse.xl.fresh\endcsname{85.82}
\expandafter\gdef\csname R@an.winners.curse.xl.name\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi}}
\expandafter\gdef\csname R@an.winners.curse.xl.null.drop.hi\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@an.winners.curse.xl.null.drop.lo\endcsname{\ensuremath{-1.54}}
\expandafter\gdef\csname R@an.winners.curse.xl.null.drop.mean\endcsname{\ensuremath{-0.64}}
\expandafter\gdef\csname R@an.winners.curse.xl.null.hi\endcsname{85.63}
\expandafter\gdef\csname R@an.winners.curse.xl.null.lo\endcsname{85.01}
\expandafter\gdef\csname R@an.winners.curse.xl.null.med\endcsname{85.31}
\expandafter\gdef\csname R@an.winners.curse.xl.pos\endcsname{more than 99}
\expandafter\gdef\csname R@an.winners.curse.xl.rank\endcsname{6}
\expandafter\gdef\csname R@an.winners.curse.xl.s0\endcsname{86.09}
\expandafter\gdef\csname R@an.winners.dataset\endcsname{KiTS23}
\expandafter\gdef\csname R@an.winners.fc.arms\endcsname{ResEnc-M; ResEnc-matched; HyReX; LeanDec; fn.-identical control; LeanAdd; LeanAdd-NeXt; HyReX-k9}
\expandafter\gdef\csname R@an.winners.fc.caveat\endcsname{the range follows from the ratio of the registered arms and allows for neither the fold-to-fold scatter of a four-fold mean nor the single-seed default of each fold (the registered arms scatter around the pooled line with an SD of 0.55\,pp), so a realised value outside it is located by its distance from the point in units of that scatter}
\expandafter\gdef\csname R@an.winners.fc.dataset\endcsname{KiTS23}
\expandafter\gdef\csname R@an.winners.fc.g\endcsname{\ensuremath{+1.56}}
\expandafter\gdef\csname R@an.winners.fc.hi\endcsname{\ensuremath{+1.29}}
\expandafter\gdef\csname R@an.winners.fc.live.done\endcsname{12}
\expandafter\gdef\csname R@an.winners.fc.lo\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@an.winners.fc.n\endcsname{8}
\expandafter\gdef\csname R@an.winners.fc.nfold\endcsname{4}
\expandafter\gdef\csname R@an.winners.fc.off\endcsname{\ensuremath{-0.30}}
\expandafter\gdef\csname R@an.winners.fc.off.scatter\endcsname{-0.6}
\expandafter\gdef\csname R@an.winners.fc.point\endcsname{\ensuremath{+1.08}}
\expandafter\gdef\csname R@an.winners.fc.prereg.done\endcsname{0}
\expandafter\gdef\csname R@an.winners.fc.prereg.total\endcsname{12}
\expandafter\gdef\csname R@an.winners.fc.ratio\endcsname{0.695}
\expandafter\gdef\csname R@an.winners.fc.ratio.hi\endcsname{0.825}
\expandafter\gdef\csname R@an.winners.fc.ratio.lo\endcsname{0.625}
\expandafter\gdef\csname R@an.winners.fc.ratio.wide.hi\endcsname{1.881}
\expandafter\gdef\csname R@an.winners.fc.ratio.wide.lo\endcsname{\ensuremath{-1.322}}
\expandafter\gdef\csname R@an.winners.fc.real\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@an.winners.fc.real.ratio\endcsname{0.50}
\expandafter\gdef\csname R@an.winners.fc.scatter\endcsname{0.55}
\expandafter\gdef\csname R@an.winners.fc.stamp\endcsname{2026-10-11 13:08}
\expandafter\gdef\csname R@an.winners.fc.state\endcsname{realised}
\expandafter\gdef\csname R@an.winners.fc.sum.gain0\endcsname{\ensuremath{+9.35}}
\expandafter\gdef\csname R@an.winners.fc.sum.gain14\endcsname{\ensuremath{+6.50}}
\expandafter\gdef\csname R@an.winners.fc.target.name\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi}}
\expandafter\gdef\csname R@an.winners.fc.target.tag\endcsname{V7C1}
\expandafter\gdef\csname R@an.winners.fc.where\endcsname{below}
\expandafter\gdef\csname R@an.winners.fc.where.wide\endcsname{inside}
\expandafter\gdef\csname R@an.winners.fc.wide.hi\endcsname{\ensuremath{+2.94}}
\expandafter\gdef\csname R@an.winners.fc.wide.lo\endcsname{\ensuremath{-2.06}}
\expandafter\gdef\csname R@an.winners.hit.all.n\endcsname{21}
\expandafter\gdef\csname R@an.winners.hit.all.npos\endcsname{19}
\expandafter\gdef\csname R@an.winners.hit.all.nreb\endcsname{18}
\expandafter\gdef\csname R@an.winners.hit.all.nscr\endcsname{22}
\expandafter\gdef\csname R@an.winners.hit.caveat\endcsname{the shares are counts of a few designs each, conditional on a design having cleared its seed-0 screen before it was replicated, and the designs of the later waves descend from the earlier waves' winners}
\expandafter\gdef\csname R@an.winners.hit.early.n\endcsname{8}
\expandafter\gdef\csname R@an.winners.hit.early.npos\endcsname{6}
\expandafter\gdef\csname R@an.winners.hit.early.nreb\endcsname{6}
\expandafter\gdef\csname R@an.winners.hit.early.waves\endcsname{1 to 4}
\expandafter\gdef\csname R@an.winners.hit.late.n\endcsname{13}
\expandafter\gdef\csname R@an.winners.hit.late.npos\endcsname{13}
\expandafter\gdef\csname R@an.winners.hit.late.nreb\endcsname{12}
\expandafter\gdef\csname R@an.winners.hit.late.waves\endcsname{5 to 8}
\expandafter\gdef\csname R@an.winners.hit.ref.reb.n\endcsname{5}
\expandafter\gdef\csname R@an.winners.hit.ref.stock.n\endcsname{9}
\expandafter\gdef\csname R@an.winners.hit.trend.pos\endcsname{higher}
\expandafter\gdef\csname R@an.winners.hit.trend.reb\endcsname{higher}
\expandafter\gdef\csname R@an.winners.hit.w1.list\endcsname{ConvNeXt-k3; HyReX; ResEnc+context; HyReX+context}
\expandafter\gdef\csname R@an.winners.hit.w1.n\endcsname{4}
\expandafter\gdef\csname R@an.winners.hit.w1.npos\endcsname{3}
\expandafter\gdef\csname R@an.winners.hit.w1.nreb\endcsname{3}
\expandafter\gdef\csname R@an.winners.hit.w1.nscr\endcsname{4}
\expandafter\gdef\csname R@an.winners.hit.w1.share.pos\endcsname{75}
\expandafter\gdef\csname R@an.winners.hit.w1.share.reb\endcsname{75}
\expandafter\gdef\csname R@an.winners.hit.w2.list\endcsname{none}
\expandafter\gdef\csname R@an.winners.hit.w2.n\endcsname{0}
\expandafter\gdef\csname R@an.winners.hit.w2.npos\endcsname{0}
\expandafter\gdef\csname R@an.winners.hit.w2.nreb\endcsname{0}
\expandafter\gdef\csname R@an.winners.hit.w2.nscr\endcsname{0}
\expandafter\gdef\csname R@an.winners.hit.w3.list\endcsname{none}
\expandafter\gdef\csname R@an.winners.hit.w3.n\endcsname{0}
\expandafter\gdef\csname R@an.winners.hit.w3.npos\endcsname{0}
\expandafter\gdef\csname R@an.winners.hit.w3.nreb\endcsname{0}
\expandafter\gdef\csname R@an.winners.hit.w3.nscr\endcsname{0}
\expandafter\gdef\csname R@an.winners.hit.w4.list\endcsname{LeanDec; HyReX+dec. capacity; HyReX, finer ConvNeXt; HyReX point-fuse}
\expandafter\gdef\csname R@an.winners.hit.w4.n\endcsname{4}
\expandafter\gdef\csname R@an.winners.hit.w4.npos\endcsname{3}
\expandafter\gdef\csname R@an.winners.hit.w4.nreb\endcsname{3}
\expandafter\gdef\csname R@an.winners.hit.w4.nscr\endcsname{5}
\expandafter\gdef\csname R@an.winners.hit.w4.share.pos\endcsname{75}
\expandafter\gdef\csname R@an.winners.hit.w4.share.reb\endcsname{75}
\expandafter\gdef\csname R@an.winners.hit.w5.list\endcsname{LeanAdd; LeanAdd-NeXt; HyReX-LeanDec}
\expandafter\gdef\csname R@an.winners.hit.w5.n\endcsname{3}
\expandafter\gdef\csname R@an.winners.hit.w5.npos\endcsname{3}
\expandafter\gdef\csname R@an.winners.hit.w5.nreb\endcsname{3}
\expandafter\gdef\csname R@an.winners.hit.w5.nscr\endcsname{3}
\expandafter\gdef\csname R@an.winners.hit.w5.share.pos\endcsname{100}
\expandafter\gdef\csname R@an.winners.hit.w5.share.reb\endcsname{100}
\expandafter\gdef\csname R@an.winners.hit.w6.list\endcsname{HyReX-k9}
\expandafter\gdef\csname R@an.winners.hit.w6.n\endcsname{1}
\expandafter\gdef\csname R@an.winners.hit.w6.npos\endcsname{1}
\expandafter\gdef\csname R@an.winners.hit.w6.nreb\endcsname{1}
\expandafter\gdef\csname R@an.winners.hit.w6.nscr\endcsname{1}
\expandafter\gdef\csname R@an.winners.hit.w6.share.pos\endcsname{100}
\expandafter\gdef\csname R@an.winners.hit.w6.share.reb\endcsname{100}
\expandafter\gdef\csname R@an.winners.hit.w7.list\endcsname{{\ifdefined\archA\archA\else XX-Net-A\fi}; LeanSep; LeanDil; {\ifdefined\archL\archL\else XX-Net-L\fi}; LeanDeepMid+FD}
\expandafter\gdef\csname R@an.winners.hit.w7.n\endcsname{5}
\expandafter\gdef\csname R@an.winners.hit.w7.npos\endcsname{5}
\expandafter\gdef\csname R@an.winners.hit.w7.nreb\endcsname{5}
\expandafter\gdef\csname R@an.winners.hit.w7.nscr\endcsname{5}
\expandafter\gdef\csname R@an.winners.hit.w7.share.pos\endcsname{100}
\expandafter\gdef\csname R@an.winners.hit.w7.share.reb\endcsname{100}
\expandafter\gdef\csname R@an.winners.hit.w8.list\endcsname{CoarseStack; LeanTrunk; Stem1; StackDec}
\expandafter\gdef\csname R@an.winners.hit.w8.n\endcsname{4}
\expandafter\gdef\csname R@an.winners.hit.w8.npos\endcsname{4}
\expandafter\gdef\csname R@an.winners.hit.w8.nreb\endcsname{3}
\expandafter\gdef\csname R@an.winners.hit.w8.nscr\endcsname{4}
\expandafter\gdef\csname R@an.winners.hit.w8.share.pos\endcsname{100}
\expandafter\gdef\csname R@an.winners.hit.w8.share.reb\endcsname{75}
\expandafter\gdef\csname R@an.winners.live.arms\endcsname{ResEnc-M; ResEnc-matched; HyReX; fn.-identical control; LeanDec; LeanAdd; LeanAdd-NeXt; HyReX-k9; {\ifdefined\archA\archA\else XX-Net-A\fi}; {\ifdefined\archL\archL\else XX-Net-L\fi}; LeanDeepMid+FD; Stem1}
\expandafter\gdef\csname R@an.winners.live.n\endcsname{12}
\expandafter\gdef\csname R@an.winners.live.ratio\endcsname{0.640}
\expandafter\gdef\csname R@an.winners.live.ratio.hi\endcsname{0.718}
\expandafter\gdef\csname R@an.winners.live.ratio.lo\endcsname{0.594}
\expandafter\gdef\csname R@an.winners.live.ratio.wide.hi\endcsname{1.881}
\expandafter\gdef\csname R@an.winners.live.ratio.wide.lo\endcsname{\ensuremath{-1.322}}
\expandafter\gdef\csname R@an.winners.live.scatter\endcsname{0.54}
\expandafter\gdef\csname R@an.winners.live.sum.gain0\endcsname{\ensuremath{+14.96}}
\expandafter\gdef\csname R@an.winners.live.sum.gain14\endcsname{\ensuremath{+9.58}}
\expandafter\gdef\csname R@an.winners.rule\endcsname{descriptive only: a position in a reference distribution locates a number and states nothing about it; shares are counts; the forecast is a registered arithmetic on the arms that existed, and no interval of the ratio is claimed}
\expandafter\gdef\csname R@an.winners.sent.curse\endcsname{Of the 30 registered designs with a seed-0 KiTS23 run, the highest seed-0 value is 86.89 Dice (HyReX+dec. capacity). Were every design's true fold-0 Dice that of the function-identical rebuild (mean 84.67, SD 0.72 over 5 runs), the highest of 30 draws would have a median of 86.11 (5 to 95 \% of the draws: 85.62 to 86.77) and the design with the highest seed-0 value would be expected to drop \ensuremath{-1.47}\,pp (\ensuremath{-2.51} to \ensuremath{-0.47}) from seed 0 to the mean of two fresh seeds; the observed highest design dropped \ensuremath{-1.11}\,pp; the 8 designs of highest seed-0 value that have a fresh pair dropped \ensuremath{-0.84}\,pp on average, against \ensuremath{-0.86}\,pp expected for designs of ranks 1 to 8 in the reference world, and the 21 agent-designed designs with both readings dropped \ensuremath{-0.34}\,pp on average (\ensuremath{-1.54} to \ensuremath{+0.66})}
\expandafter\gdef\csname R@an.winners.sent.curse.xl\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi} has the seed-0 value 86.09 Dice, rank 6 of 30; the share of the reference draws of that rank at or below that value is more than 99 \% (median of the draws 85.31), and the design dropped \ensuremath{-0.27}\,pp from seed 0 to its fresh mean, against an expected \ensuremath{-0.64}\,pp in the reference world}
\expandafter\gdef\csname R@an.winners.sent.fc\endcsname{Computed 2026-10-11 13:08 from the data that existed then and registered with this module, before any cross-validation fold of {\ifdefined\archL\archL\else XX-Net-L\fi} had finished (0 of its 12 runs): from the 8 arms with both a fold-0 fresh pair and four finished folds the ratio of the folds 1 to 4 gain to the fold-0 gain over the stock mean is 0.695 pooled (0.625 to 0.825 with one arm left out; the per-arm ratios run from \ensuremath{-1.322} to 1.881), so a fold-0 gain of \ensuremath{+1.56}\,pp on KiTS23 implies a folds 1 to 4 gain of \ensuremath{+1.08}\,pp (\ensuremath{+0.98} to \ensuremath{+1.29}\,pp; per-arm band \ensuremath{-2.06} to \ensuremath{+2.94}\,pp); the realised folds 1 to 4 gain is \ensuremath{+0.78}\,pp, below the pooled range and inside the per-arm band, \ensuremath{-0.30}\,pp from the forecast point (-0.6 scatter units of the registered arms, 0.55\,pp)}
\expandafter\gdef\csname R@an.winners.sent.hit\endcsname{Among the agent-designed designs with a fresh KiTS23 pair, 6 of 8 in waves 1 to 4 and 13 of 13 in waves 5 to 8 have a fresh mean above the mean of the 9 stock runs (the share of the later waves is higher than that of the earlier ones), and 6 of 8 and 12 of 13 above the mean of the 5 rebuild runs (higher); 21 of the 22 agent-designed designs with a seed-0 run have a fresh pair}
\expandafter\gdef\csname R@an.winners.sent.shrink\endcsname{Over the 12 arms with both a fold-0 fresh pair and four finished KiTS23 folds, the folds 1 to 4 gain is 0.640 of the fold-0 gain over the stock mean pooled (0.594 to 0.718 with one arm left out; the per-arm ratios run from \ensuremath{-1.322} to 1.881)}
\expandafter\gdef\csname R@an.winners.state\endcsname{30 registered designs with a seed-0 KiTS23 run (22 agent-designed), 25 with a fresh pair; 9 stock runs and 5 rebuild runs; 12 arms with both a fold-0 fresh pair and four finished folds}
\expandafter\gdef\csname R@an.xx.amos.cases\endcsname{amos\_0057 (p10), amos\_0358 (p50), amos\_0141 (p90)}
\expandafter\gdef\csname R@an.xx.amos.def.assd\endcsname{1.58}
\expandafter\gdef\csname R@an.xx.amos.def.dice\endcsname{87.79}
\expandafter\gdef\csname R@an.xx.amos.def.hd95\endcsname{8.00}
\expandafter\gdef\csname R@an.xx.amos.def.nsd1\endcsname{80.27}
\expandafter\gdef\csname R@an.xx.amos.def.nsd2\endcsname{88.14}
\expandafter\gdef\csname R@an.xx.amos.def.tag\endcsname{ai_benchbase_amos_f0_e1000_s3}
\expandafter\gdef\csname R@an.xx.amos.sentence\endcsname{on fold 0 of AMOS22 (one checkpoint each, descriptive), {\ifdefined\archL\archL\else XX-Net-L\fi} reaches a mean normalised surface Dice of 79.69\,\% at 1\,mm and 87.80\,\% at 2\,mm against the default's 80.27\,\% and 88.14\,\%, and a mean HD95 of 8.57\,mm against 8.00\,mm}
\expandafter\gdef\csname R@an.xx.amos.state\endcsname{2 of 2 records}
\expandafter\gdef\csname R@an.xx.amos.xl.assd\endcsname{1.71}
\expandafter\gdef\csname R@an.xx.amos.xl.d.assd\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.xx.amos.xl.d.dice\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.xx.amos.xl.d.hd95\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.xx.amos.xl.d.nsd1\endcsname{\ensuremath{-0.58}}
\expandafter\gdef\csname R@an.xx.amos.xl.d.nsd2\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.xx.amos.xl.dice\endcsname{87.60}
\expandafter\gdef\csname R@an.xx.amos.xl.hd95\endcsname{8.57}
\expandafter\gdef\csname R@an.xx.amos.xl.nsd1\endcsname{79.69}
\expandafter\gdef\csname R@an.xx.amos.xl.nsd2\endcsname{87.80}
\expandafter\gdef\csname R@an.xx.amos.xl.tag\endcsname{ai_V7C1_amos_f0_e1000_s0}
\expandafter\gdef\csname R@an.xx.kits.cases\endcsname{case\_00048 (p10), case\_00255 (p50), case\_00148 (p90)}
\expandafter\gdef\csname R@an.xx.kits.def.assd\endcsname{11.37}
\expandafter\gdef\csname R@an.xx.kits.def.dice\endcsname{83.75}
\expandafter\gdef\csname R@an.xx.kits.def.hd95\endcsname{53.04}
\expandafter\gdef\csname R@an.xx.kits.def.nsd1\endcsname{72.78}
\expandafter\gdef\csname R@an.xx.kits.def.nsd2\endcsname{80.31}
\expandafter\gdef\csname R@an.xx.kits.def.tag\endcsname{ai_benchbase_kits_f0_e1000_s3}
\expandafter\gdef\csname R@an.xx.kits.erf.bound\endcsname{both are bounded by the patch at r90 (inscribed radius 49.2\,mm)}
\expandafter\gdef\csname R@an.xx.kits.erf.def.beyond\endcsname{0.28}
\expandafter\gdef\csname R@an.xx.kits.erf.def.floor\endcsname{0.44}
\expandafter\gdef\csname R@an.xx.kits.erf.def.r50\endcsname{29.2}
\expandafter\gdef\csname R@an.xx.kits.erf.def.r50.flag\endcsname{inside the patch}
\expandafter\gdef\csname R@an.xx.kits.erf.def.r50.pp\endcsname{29.3}
\expandafter\gdef\csname R@an.xx.kits.erf.def.r50.ppsd\endcsname{7.0}
\expandafter\gdef\csname R@an.xx.kits.erf.def.r50loc\endcsname{15.4}
\expandafter\gdef\csname R@an.xx.kits.erf.def.r90\endcsname{64.5}
\expandafter\gdef\csname R@an.xx.kits.erf.def.r90.flag\endcsname{bounded by the patch}
\expandafter\gdef\csname R@an.xx.kits.erf.def.r90.pp\endcsname{64.0}
\expandafter\gdef\csname R@an.xx.kits.erf.def.r90.ppsd\endcsname{2.9}
\expandafter\gdef\csname R@an.xx.kits.erf.def.r90loc\endcsname{41.5}
\expandafter\gdef\csname R@an.xx.kits.erf.def.tag\endcsname{ai_benchbase_kits_f0_e1000_s3}
\expandafter\gdef\csname R@an.xx.kits.erf.k\endcsname{98}
\expandafter\gdef\csname R@an.xx.kits.erf.legend\endcsname{the gradient effective receptive field of the foreground logit at the output centre voxel of the $128^3$ patch, the mean of 98 patches (one per fold-0 validation case, unit mass each, the same patches for every network); (a) the central plane $z=0$ (top) and the central plane $y=0$ (bottom) on one colour scale of 4 decades below the largest centre value shown, the dashed and the solid circle the radii of 50 and 90\,\% of the mass; (b) the share of the mass inside a ball of radius $r$, with markers at 50 and 90\,\%; (c) the mass per voxel at distance $r$; the dotted vertical line is the inscribed radius of the patch (49.2\,mm), beyond which a ball is cut by the patch}
\expandafter\gdef\csname R@an.xx.kits.erf.rin\endcsname{49.2}
\expandafter\gdef\csname R@an.xx.kits.erf.scope\endcsname{this measurement describes the field of influence of each trained network and does not isolate the large kernel: that question is answered by the ablation arm with a $3^3$ coarse kernel (benchAB1), not here}
\expandafter\gdef\csname R@an.xx.kits.erf.sentence\endcsname{on KiTS23 fold 0 (one checkpoint each, descriptive) the gradient effective receptive field at the output centre voxel of {\ifdefined\archL\archL\else XX-Net-L\fi} matches that of the nnU-Net default: 50\,\% of its mass lies within 27.8\,mm of that voxel against 29.2\,mm and 90\,\% within 65.2\,mm against 64.5\,mm; both are bounded by the patch at r90 (inscribed radius 49.2\,mm)}
\expandafter\gdef\csname R@an.xx.kits.erf.short\endcsname{the effective receptive field of {\ifdefined\archL\archL\else XX-Net-L\fi} matches that of the nnU-Net default (r50 27.8 against 29.2\,mm; both are bounded by the patch at r90)}
\expandafter\gdef\csname R@an.xx.kits.erf.state\endcsname{3 of 3 records}
\expandafter\gdef\csname R@an.xx.kits.erf.tag\endcsname{trained_k98}
\expandafter\gdef\csname R@an.xx.kits.erf.xa.beyond\endcsname{0.27}
\expandafter\gdef\csname R@an.xx.kits.erf.xa.floor\endcsname{0.43}
\expandafter\gdef\csname R@an.xx.kits.erf.xa.r50\endcsname{27.5}
\expandafter\gdef\csname R@an.xx.kits.erf.xa.r50.flag\endcsname{inside the patch}
\expandafter\gdef\csname R@an.xx.kits.erf.xa.r50.pp\endcsname{27.7}
\expandafter\gdef\csname R@an.xx.kits.erf.xa.r50.ppsd\endcsname{5.2}
\expandafter\gdef\csname R@an.xx.kits.erf.xa.r50loc\endcsname{15.0}
\expandafter\gdef\csname R@an.xx.kits.erf.xa.r90\endcsname{64.2}
\expandafter\gdef\csname R@an.xx.kits.erf.xa.r90.flag\endcsname{bounded by the patch}
\expandafter\gdef\csname R@an.xx.kits.erf.xa.r90.pp\endcsname{63.8}
\expandafter\gdef\csname R@an.xx.kits.erf.xa.r90.ppsd\endcsname{2.6}
\expandafter\gdef\csname R@an.xx.kits.erf.xa.r90loc\endcsname{38.3}
\expandafter\gdef\csname R@an.xx.kits.erf.xa.tag\endcsname{ai_V7A1_kits_f0_e1000_s0}
\expandafter\gdef\csname R@an.xx.kits.erf.xl.beyond\endcsname{0.28}
\expandafter\gdef\csname R@an.xx.kits.erf.xl.floor\endcsname{0.45}
\expandafter\gdef\csname R@an.xx.kits.erf.xl.r50\endcsname{27.8}
\expandafter\gdef\csname R@an.xx.kits.erf.xl.r50.flag\endcsname{inside the patch}
\expandafter\gdef\csname R@an.xx.kits.erf.xl.r50.pp\endcsname{28.4}
\expandafter\gdef\csname R@an.xx.kits.erf.xl.r50.ppsd\endcsname{5.5}
\expandafter\gdef\csname R@an.xx.kits.erf.xl.r50loc\endcsname{14.9}
\expandafter\gdef\csname R@an.xx.kits.erf.xl.r90\endcsname{65.2}
\expandafter\gdef\csname R@an.xx.kits.erf.xl.r90.flag\endcsname{bounded by the patch}
\expandafter\gdef\csname R@an.xx.kits.erf.xl.r90.pp\endcsname{64.8}
\expandafter\gdef\csname R@an.xx.kits.erf.xl.r90.ppsd\endcsname{2.8}
\expandafter\gdef\csname R@an.xx.kits.erf.xl.r90loc\endcsname{38.6}
\expandafter\gdef\csname R@an.xx.kits.erf.xl.tag\endcsname{ai_V7C1_kits_f0_e1000_s0}
\expandafter\gdef\csname R@an.xx.kits.err.def.kidney.dice\endcsname{96.31}
\expandafter\gdef\csname R@an.xx.kits.err.def.kidney.hd95med\endcsname{1.21}
\expandafter\gdef\csname R@an.xx.kits.err.def.kidney.hd95p90\endcsname{115.9}
\expandafter\gdef\csname R@an.xx.kits.err.def.kidney.ndist\endcsname{19}
\expandafter\gdef\csname R@an.xx.kits.err.def.masses.dice\endcsname{80.58}
\expandafter\gdef\csname R@an.xx.kits.err.def.masses.hd95med\endcsname{5.82}
\expandafter\gdef\csname R@an.xx.kits.err.def.masses.hd95p90\endcsname{172.0}
\expandafter\gdef\csname R@an.xx.kits.err.def.masses.ndist\endcsname{35}
\expandafter\gdef\csname R@an.xx.kits.err.def.ndist.any\endcsname{55}
\expandafter\gdef\csname R@an.xx.kits.err.def.tumour.dice\endcsname{74.36}
\expandafter\gdef\csname R@an.xx.kits.err.def.tumour.hd95med\endcsname{5.97}
\expandafter\gdef\csname R@an.xx.kits.err.def.tumour.hd95p90\endcsname{199.4}
\expandafter\gdef\csname R@an.xx.kits.err.def.tumour.ndist\endcsname{42}
\expandafter\gdef\csname R@an.xx.kits.err.ncases\endcsname{98}
\expandafter\gdef\csname R@an.xx.kits.err.pair.both\endcsname{42}
\expandafter\gdef\csname R@an.xx.kits.err.pair.defonly\endcsname{13}
\expandafter\gdef\csname R@an.xx.kits.err.pair.xlonly\endcsname{4}
\expandafter\gdef\csname R@an.xx.kits.err.sentence\endcsname{on KiTS23 fold 0 (one checkpoint each, descriptive), 46 of the 98 validation cases have a distant error (an HD95 above 30\,mm in at least one region) with {\ifdefined\archL\archL\else XX-Net-L\fi} and 55 with the default (4 with {\ifdefined\archL\archL\else XX-Net-L\fi} only, 13 with the default only); the median tumour HD95 is 5.08\,mm against 5.97\,mm}
\expandafter\gdef\csname R@an.xx.kits.err.thr\endcsname{30}
\expandafter\gdef\csname R@an.xx.kits.err.xl.kidney.dice\endcsname{97.11}
\expandafter\gdef\csname R@an.xx.kits.err.xl.kidney.hd95med\endcsname{1.13}
\expandafter\gdef\csname R@an.xx.kits.err.xl.kidney.hd95p90\endcsname{12.0}
\expandafter\gdef\csname R@an.xx.kits.err.xl.kidney.ndist\endcsname{9}
\expandafter\gdef\csname R@an.xx.kits.err.xl.masses.dice\endcsname{83.48}
\expandafter\gdef\csname R@an.xx.kits.err.xl.masses.hd95med\endcsname{5.27}
\expandafter\gdef\csname R@an.xx.kits.err.xl.masses.hd95p90\endcsname{139.8}
\expandafter\gdef\csname R@an.xx.kits.err.xl.masses.ndist\endcsname{27}
\expandafter\gdef\csname R@an.xx.kits.err.xl.ndist.any\endcsname{46}
\expandafter\gdef\csname R@an.xx.kits.err.xl.tumour.dice\endcsname{77.66}
\expandafter\gdef\csname R@an.xx.kits.err.xl.tumour.hd95med\endcsname{5.08}
\expandafter\gdef\csname R@an.xx.kits.err.xl.tumour.hd95p90\endcsname{171.7}
\expandafter\gdef\csname R@an.xx.kits.err.xl.tumour.ndist\endcsname{33}
\expandafter\gdef\csname R@an.xx.kits.gallery.case\endcsname{case\_00048}
\expandafter\gdef\csname R@an.xx.kits.gallery.def.fpvox\endcsname{8291}
\expandafter\gdef\csname R@an.xx.kits.gallery.def.hd95\endcsname{103.1}
\expandafter\gdef\csname R@an.xx.kits.gallery.def.mm2\endcsname{690}
\expandafter\gdef\csname R@an.xx.kits.gallery.def.n\endcsname{1}
\expandafter\gdef\csname R@an.xx.kits.gallery.def.px\endcsname{637}
\expandafter\gdef\csname R@an.xx.kits.gallery.key\endcsname{overlay: green kidney, red tumour, violet cyst; the yellow ring marks a predicted mass that lies more than 30\,mm from every reference mass}
\expandafter\gdef\csname R@an.xx.kits.gallery.ql\endcsname{p10}
\expandafter\gdef\csname R@an.xx.kits.gallery.sentence\endcsname{in the 10th-percentile case nnU-Net predicts a mass of 690\,mm$^2$ on the slice shown with no reference mass within 30\,mm (8291 false-positive voxels of the masses region in the volume, HD95 103.1\,mm), {\ifdefined\archL\archL\else XX-Net-L\fi} a fragment of 122\,mm$^2$ (2035 voxels, HD95 96.8\,mm)}
\expandafter\gdef\csname R@an.xx.kits.gallery.xl.fpvox\endcsname{2035}
\expandafter\gdef\csname R@an.xx.kits.gallery.xl.hd95\endcsname{96.8}
\expandafter\gdef\csname R@an.xx.kits.gallery.xl.mm2\endcsname{122}
\expandafter\gdef\csname R@an.xx.kits.gallery.xl.n\endcsname{1}
\expandafter\gdef\csname R@an.xx.kits.gallery.xl.px\endcsname{113}
\expandafter\gdef\csname R@an.xx.kits.sentence\endcsname{on fold 0 of KiTS23 (one checkpoint each, descriptive), {\ifdefined\archL\archL\else XX-Net-L\fi} reaches a mean normalised surface Dice of 74.52\,\% at 1\,mm and 82.63\,\% at 2\,mm against the default's 72.78\,\% and 80.31\,\%, and a mean HD95 of 32.53\,mm against 53.04\,mm}
\expandafter\gdef\csname R@an.xx.kits.state\endcsname{3 of 3 records}
\expandafter\gdef\csname R@an.xx.kits.xa.assd\endcsname{7.29}
\expandafter\gdef\csname R@an.xx.kits.xa.dice\endcsname{85.93}
\expandafter\gdef\csname R@an.xx.kits.xa.hd95\endcsname{32.95}
\expandafter\gdef\csname R@an.xx.kits.xa.nsd1\endcsname{74.89}
\expandafter\gdef\csname R@an.xx.kits.xa.nsd2\endcsname{82.89}
\expandafter\gdef\csname R@an.xx.kits.xa.tag\endcsname{ai_V7A1_kits_f0_e1000_s0}
\expandafter\gdef\csname R@an.xx.kits.xl.assd\endcsname{6.67}
\expandafter\gdef\csname R@an.xx.kits.xl.d.assd\endcsname{\ensuremath{-4.70}}
\expandafter\gdef\csname R@an.xx.kits.xl.d.dice\endcsname{\ensuremath{+2.33}}
\expandafter\gdef\csname R@an.xx.kits.xl.d.hd95\endcsname{\ensuremath{-20.51}}
\expandafter\gdef\csname R@an.xx.kits.xl.d.nsd1\endcsname{\ensuremath{+1.74}}
\expandafter\gdef\csname R@an.xx.kits.xl.d.nsd2\endcsname{\ensuremath{+2.32}}
\expandafter\gdef\csname R@an.xx.kits.xl.dice\endcsname{86.08}
\expandafter\gdef\csname R@an.xx.kits.xl.hd95\endcsname{32.53}
\expandafter\gdef\csname R@an.xx.kits.xl.nsd1\endcsname{74.52}
\expandafter\gdef\csname R@an.xx.kits.xl.nsd2\endcsname{82.63}
\expandafter\gdef\csname R@an.xx.kits.xl.tag\endcsname{ai_V7C1_kits_f0_e1000_s0}
\expandafter\gdef\csname R@an.xxablation.D2.amos.basis\endcsname{seed 0}
\expandafter\gdef\csname R@an.xxablation.D2.amos.cell\endcsname{\ensuremath{-0.36}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxablation.D2.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.D2.amos.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.D2.amos.s0\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.xxablation.D2.amos.vsparent.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.D2.amos.vsparent.s0\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.xxablation.D2.change\endcsname{1 conv per dec. stage}
\expandafter\gdef\csname R@an.xxablation.D2.delta_pool\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.xxablation.D2.gmac\endcsname{367.2}
\expandafter\gdef\csname R@an.xxablation.D2.gmacx\endcsname{0.77}
\expandafter\gdef\csname R@an.xxablation.D2.group\endcsname{path}
\expandafter\gdef\csname R@an.xxablation.D2.kits.basis\endcsname{two fresh seeds}
\expandafter\gdef\csname R@an.xxablation.D2.kits.cell\endcsname{\ensuremath{+1.01}}
\expandafter\gdef\csname R@an.xxablation.D2.kits.fresh\endcsname{\ensuremath{+1.01}}
\expandafter\gdef\csname R@an.xxablation.D2.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.D2.kits.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.D2.kits.pool.fresh\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@an.xxablation.D2.kits.pool.s0\endcsname{\ensuremath{+2.36}}
\expandafter\gdef\csname R@an.xxablation.D2.kits.s0\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.xxablation.D2.kits.se\endcsname{0.49}
\expandafter\gdef\csname R@an.xxablation.D2.kits.vsparent.fresh\endcsname{\ensuremath{+1.01}}
\expandafter\gdef\csname R@an.xxablation.D2.kits.vsparent.s0\endcsname{\ensuremath{+1.48}}
\expandafter\gdef\csname R@an.xxablation.D2.name\endcsname{LeanDec}
\expandafter\gdef\csname R@an.xxablation.D2.params\endcsname{26.08}
\expandafter\gdef\csname R@an.xxablation.D2.paramsx\endcsname{0.84}
\expandafter\gdef\csname R@an.xxablation.D2.parent\endcsname{nnU-Net}
\expandafter\gdef\csname R@an.xxablation.D2.sentence\endcsname{one convolution per decoder stage (LeanDec) brings the parameters to 0.84$\times$ and the profiled training step to 0.81$\times$ the default's; against the default: KiTS23 \ensuremath{+1.01}\,pp (two fresh seeds, SE 0.49), AMOS22 \ensuremath{-0.36}\,pp (seed 0)}
\expandafter\gdef\csname R@an.xxablation.D2.step\endcsname{99.6}
\expandafter\gdef\csname R@an.xxablation.D2.stepx\endcsname{0.81}
\expandafter\gdef\csname R@an.xxablation.V5B1.amos.basis\endcsname{seed 0}
\expandafter\gdef\csname R@an.xxablation.V5B1.amos.cell\endcsname{\ensuremath{-0.26}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxablation.V5B1.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V5B1.amos.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.V5B1.amos.s0\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.xxablation.V5B1.amos.vsparent.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V5B1.amos.vsparent.s0\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.xxablation.V5B1.change\endcsname{+ additive skips}
\expandafter\gdef\csname R@an.xxablation.V5B1.delta_pool\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.xxablation.V5B1.gmac\endcsname{257.1}
\expandafter\gdef\csname R@an.xxablation.V5B1.gmacx\endcsname{0.54}
\expandafter\gdef\csname R@an.xxablation.V5B1.group\endcsname{path}
\expandafter\gdef\csname R@an.xxablation.V5B1.kits.basis\endcsname{two fresh seeds}
\expandafter\gdef\csname R@an.xxablation.V5B1.kits.cell\endcsname{\ensuremath{+1.41}}
\expandafter\gdef\csname R@an.xxablation.V5B1.kits.fresh\endcsname{\ensuremath{+1.41}}
\expandafter\gdef\csname R@an.xxablation.V5B1.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V5B1.kits.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V5B1.kits.pool.fresh\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.xxablation.V5B1.kits.pool.s0\endcsname{\ensuremath{+2.16}}
\expandafter\gdef\csname R@an.xxablation.V5B1.kits.s0\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.xxablation.V5B1.kits.se\endcsname{0.49}
\expandafter\gdef\csname R@an.xxablation.V5B1.kits.vsparent.fresh\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.xxablation.V5B1.kits.vsparent.s0\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@an.xxablation.V5B1.name\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.xxablation.V5B1.params\endcsname{20.96}
\expandafter\gdef\csname R@an.xxablation.V5B1.paramsx\endcsname{0.67}
\expandafter\gdef\csname R@an.xxablation.V5B1.parent\endcsname{LeanDec}
\expandafter\gdef\csname R@an.xxablation.V5B1.sentence\endcsname{additive instead of concatenated skips (LeanAdd) brings the parameters to 0.67$\times$ and the profiled training step to 0.73$\times$ the default's; against the default: KiTS23 \ensuremath{+1.41}\,pp (two fresh seeds, SE 0.49), AMOS22 \ensuremath{-0.26}\,pp (seed 0)}
\expandafter\gdef\csname R@an.xxablation.V5B1.step\endcsname{89.6}
\expandafter\gdef\csname R@an.xxablation.V5B1.stepx\endcsname{0.73}
\expandafter\gdef\csname R@an.xxablation.V5B2.amos.basis\endcsname{seed 0}
\expandafter\gdef\csname R@an.xxablation.V5B2.amos.cell\endcsname{\ensuremath{+0.13}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxablation.V5B2.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V5B2.amos.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.V5B2.amos.s0\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@an.xxablation.V5B2.amos.vsparent.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V5B2.amos.vsparent.s0\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.xxablation.V5B2.change\endcsname{+ ConvNeXt $7^3$, st. 4--5}
\expandafter\gdef\csname R@an.xxablation.V5B2.delta_pool\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@an.xxablation.V5B2.gmac\endcsname{257.2}
\expandafter\gdef\csname R@an.xxablation.V5B2.gmacx\endcsname{0.54}
\expandafter\gdef\csname R@an.xxablation.V5B2.group\endcsname{path}
\expandafter\gdef\csname R@an.xxablation.V5B2.kits.basis\endcsname{two fresh seeds}
\expandafter\gdef\csname R@an.xxablation.V5B2.kits.cell\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.xxablation.V5B2.kits.fresh\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@an.xxablation.V5B2.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V5B2.kits.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V5B2.kits.pool.fresh\endcsname{\ensuremath{+1.45}}
\expandafter\gdef\csname R@an.xxablation.V5B2.kits.pool.s0\endcsname{\ensuremath{+1.26}}
\expandafter\gdef\csname R@an.xxablation.V5B2.kits.s0\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.xxablation.V5B2.kits.se\endcsname{0.49}
\expandafter\gdef\csname R@an.xxablation.V5B2.kits.vsparent.fresh\endcsname{\ensuremath{-0.84}}
\expandafter\gdef\csname R@an.xxablation.V5B2.kits.vsparent.s0\endcsname{\ensuremath{-0.90}}
\expandafter\gdef\csname R@an.xxablation.V5B2.name\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.xxablation.V5B2.params\endcsname{21.26}
\expandafter\gdef\csname R@an.xxablation.V5B2.paramsx\endcsname{0.68}
\expandafter\gdef\csname R@an.xxablation.V5B2.parent\endcsname{LeanAdd}
\expandafter\gdef\csname R@an.xxablation.V5B2.sentence\endcsname{a large-kernel ($7^3$) ConvNeXt operator at encoder stages 4 and 5 (LeanAdd-NeXt) brings the parameters to 0.68$\times$ and the profiled training step to 0.84$\times$ the default's; against the default: KiTS23 \ensuremath{+0.57}\,pp (two fresh seeds, SE 0.49), AMOS22 \ensuremath{+0.13}\,pp (seed 0)}
\expandafter\gdef\csname R@an.xxablation.V5B2.step\endcsname{103.1}
\expandafter\gdef\csname R@an.xxablation.V5B2.stepx\endcsname{0.84}
\expandafter\gdef\csname R@an.xxablation.V7A1.amos.basis\endcsname{seed 0}
\expandafter\gdef\csname R@an.xxablation.V7A1.amos.cell\endcsname{\ensuremath{-0.04}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxablation.V7A1.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7A1.amos.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.V7A1.amos.s0\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@an.xxablation.V7A1.amos.vsparent.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7A1.amos.vsparent.s0\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.xxablation.V7A1.change\endcsname{+ res. depth, st. 2--3}
\expandafter\gdef\csname R@an.xxablation.V7A1.delta_pool\endcsname{\ensuremath{+2.66}}
\expandafter\gdef\csname R@an.xxablation.V7A1.gmac\endcsname{373.5}
\expandafter\gdef\csname R@an.xxablation.V7A1.gmacx\endcsname{0.78}
\expandafter\gdef\csname R@an.xxablation.V7A1.group\endcsname{swap}
\expandafter\gdef\csname R@an.xxablation.V7A1.kits.basis\endcsname{two fresh seeds}
\expandafter\gdef\csname R@an.xxablation.V7A1.kits.cell\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.xxablation.V7A1.kits.fresh\endcsname{\ensuremath{+1.78}}
\expandafter\gdef\csname R@an.xxablation.V7A1.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V7A1.kits.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V7A1.kits.pool.fresh\endcsname{\ensuremath{+2.66}}
\expandafter\gdef\csname R@an.xxablation.V7A1.kits.pool.s0\endcsname{\ensuremath{+2.55}}
\expandafter\gdef\csname R@an.xxablation.V7A1.kits.s0\endcsname{\ensuremath{+1.67}}
\expandafter\gdef\csname R@an.xxablation.V7A1.kits.se\endcsname{0.49}
\expandafter\gdef\csname R@an.xxablation.V7A1.kits.vsparent.fresh\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@an.xxablation.V7A1.kits.vsparent.s0\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@an.xxablation.V7A1.name\endcsname{{\ifdefined\archA\archA\else XX-Net-A\fi}}
\expandafter\gdef\csname R@an.xxablation.V7A1.params\endcsname{31.04}
\expandafter\gdef\csname R@an.xxablation.V7A1.paramsx\endcsname{0.99}
\expandafter\gdef\csname R@an.xxablation.V7A1.parent\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.xxablation.V7A1.sentence\endcsname{on LeanAdd-NeXt, residual depth added at encoder stages 2 and 3 ({\ifdefined\archA\archA\else XX-Net-A\fi}) brings the parameters to 0.99$\times$ and the profiled training step to 0.92$\times$ the default's; against the default: KiTS23 \ensuremath{+1.78}\,pp (two fresh seeds, SE 0.49), AMOS22 \ensuremath{-0.04}\,pp (seed 0)}
\expandafter\gdef\csname R@an.xxablation.V7A1.step\endcsname{113.1}
\expandafter\gdef\csname R@an.xxablation.V7A1.stepx\endcsname{0.92}
\expandafter\gdef\csname R@an.xxablation.V7A2.amos.basis\endcsname{seed 0}
\expandafter\gdef\csname R@an.xxablation.V7A2.amos.cell\endcsname{\ensuremath{+0.36}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxablation.V7A2.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7A2.amos.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.V7A2.amos.s0\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@an.xxablation.V7A2.amos.vsparent.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7A2.amos.vsparent.s0\endcsname{\ensuremath{+0.40}}
\expandafter\gdef\csname R@an.xxablation.V7A2.change\endcsname{+ fine decoder convs}
\expandafter\gdef\csname R@an.xxablation.V7A2.delta_pool\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.xxablation.V7A2.gmac\endcsname{460.5}
\expandafter\gdef\csname R@an.xxablation.V7A2.gmacx\endcsname{0.96}
\expandafter\gdef\csname R@an.xxablation.V7A2.group\endcsname{swap}
\expandafter\gdef\csname R@an.xxablation.V7A2.kits.basis\endcsname{two fresh seeds}
\expandafter\gdef\csname R@an.xxablation.V7A2.kits.cell\endcsname{\ensuremath{+1.41}}
\expandafter\gdef\csname R@an.xxablation.V7A2.kits.fresh\endcsname{\ensuremath{+1.41}}
\expandafter\gdef\csname R@an.xxablation.V7A2.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V7A2.kits.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V7A2.kits.pool.fresh\endcsname{\ensuremath{+2.29}}
\expandafter\gdef\csname R@an.xxablation.V7A2.kits.pool.s0\endcsname{\ensuremath{+2.89}}
\expandafter\gdef\csname R@an.xxablation.V7A2.kits.s0\endcsname{\ensuremath{+2.01}}
\expandafter\gdef\csname R@an.xxablation.V7A2.kits.se\endcsname{0.49}
\expandafter\gdef\csname R@an.xxablation.V7A2.kits.vsparent.fresh\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@an.xxablation.V7A2.kits.vsparent.s0\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@an.xxablation.V7A2.name\endcsname{LeanDeepMid+FD}
\expandafter\gdef\csname R@an.xxablation.V7A2.params\endcsname{31.18}
\expandafter\gdef\csname R@an.xxablation.V7A2.paramsx\endcsname{1.00}
\expandafter\gdef\csname R@an.xxablation.V7A2.parent\endcsname{{\ifdefined\archA\archA\else XX-Net-A\fi}}
\expandafter\gdef\csname R@an.xxablation.V7A2.sentence\endcsname{on LeanDeepMid, the two finest decoder convolutions restored (LeanDeepMid+FD) brings the parameters to 1.00$\times$ and the profiled training step to 1.09$\times$ the default's; against the default: KiTS23 \ensuremath{+1.41}\,pp (two fresh seeds, SE 0.49), AMOS22 \ensuremath{+0.36}\,pp (seed 0)}
\expandafter\gdef\csname R@an.xxablation.V7A2.step\endcsname{134.7}
\expandafter\gdef\csname R@an.xxablation.V7A2.stepx\endcsname{1.09}
\expandafter\gdef\csname R@an.xxablation.V7A3.amos.basis\endcsname{seed 0}
\expandafter\gdef\csname R@an.xxablation.V7A3.amos.cell\endcsname{\ensuremath{-0.22}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxablation.V7A3.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7A3.amos.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.V7A3.amos.s0\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@an.xxablation.V7A3.amos.vsparent.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7A3.amos.vsparent.s0\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@an.xxablation.V7A3.change\endcsname{decoder convs restored}
\expandafter\gdef\csname R@an.xxablation.V7A3.delta_pool\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.xxablation.V7A3.gmac\endcsname{367.3}
\expandafter\gdef\csname R@an.xxablation.V7A3.gmacx\endcsname{0.77}
\expandafter\gdef\csname R@an.xxablation.V7A3.group\endcsname{swap}
\expandafter\gdef\csname R@an.xxablation.V7A3.kits.basis\endcsname{seed 0}
\expandafter\gdef\csname R@an.xxablation.V7A3.kits.cell\endcsname{\ensuremath{-0.34}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxablation.V7A3.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7A3.kits.n\endcsname{1}
\expandafter\gdef\csname R@an.xxablation.V7A3.kits.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.V7A3.kits.pool.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7A3.kits.pool.s0\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@an.xxablation.V7A3.kits.s0\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@an.xxablation.V7A3.kits.se\endcsname{0.67}
\expandafter\gdef\csname R@an.xxablation.V7A3.kits.vsparent.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7A3.kits.vsparent.s0\endcsname{\ensuremath{-0.72}}
\expandafter\gdef\csname R@an.xxablation.V7A3.name\endcsname{LeanFullDec}
\expandafter\gdef\csname R@an.xxablation.V7A3.params\endcsname{26.38}
\expandafter\gdef\csname R@an.xxablation.V7A3.paramsx\endcsname{0.85}
\expandafter\gdef\csname R@an.xxablation.V7A3.parent\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.xxablation.V7A3.sentence\endcsname{on LeanAdd-NeXt, the second decoder convolution restored at every stage (LeanFullDec) brings the parameters to 0.85$\times$ and the profiled training step to 1.02$\times$ the default's; against the default: KiTS23 \ensuremath{-0.34}\,pp (seed 0, SE 0.67), AMOS22 \ensuremath{-0.22}\,pp (seed 0)}
\expandafter\gdef\csname R@an.xxablation.V7A3.step\endcsname{125.5}
\expandafter\gdef\csname R@an.xxablation.V7A3.stepx\endcsname{1.02}
\expandafter\gdef\csname R@an.xxablation.V7B1.amos.basis\endcsname{seed 0}
\expandafter\gdef\csname R@an.xxablation.V7B1.amos.cell\endcsname{\ensuremath{-0.44}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxablation.V7B1.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7B1.amos.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.V7B1.amos.s0\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@an.xxablation.V7B1.amos.vsparent.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7B1.amos.vsparent.s0\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@an.xxablation.V7B1.change\endcsname{separable kernel}
\expandafter\gdef\csname R@an.xxablation.V7B1.delta_pool\endcsname{\ensuremath{+2.38}}
\expandafter\gdef\csname R@an.xxablation.V7B1.gmac\endcsname{256.9}
\expandafter\gdef\csname R@an.xxablation.V7B1.gmacx\endcsname{0.54}
\expandafter\gdef\csname R@an.xxablation.V7B1.group\endcsname{swap}
\expandafter\gdef\csname R@an.xxablation.V7B1.kits.basis\endcsname{two fresh seeds}
\expandafter\gdef\csname R@an.xxablation.V7B1.kits.cell\endcsname{\ensuremath{+1.50}}
\expandafter\gdef\csname R@an.xxablation.V7B1.kits.fresh\endcsname{\ensuremath{+1.50}}
\expandafter\gdef\csname R@an.xxablation.V7B1.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V7B1.kits.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V7B1.kits.pool.fresh\endcsname{\ensuremath{+2.38}}
\expandafter\gdef\csname R@an.xxablation.V7B1.kits.pool.s0\endcsname{\ensuremath{+1.72}}
\expandafter\gdef\csname R@an.xxablation.V7B1.kits.s0\endcsname{\ensuremath{+0.84}}
\expandafter\gdef\csname R@an.xxablation.V7B1.kits.se\endcsname{0.49}
\expandafter\gdef\csname R@an.xxablation.V7B1.kits.vsparent.fresh\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@an.xxablation.V7B1.kits.vsparent.s0\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@an.xxablation.V7B1.name\endcsname{LeanSep}
\expandafter\gdef\csname R@an.xxablation.V7B1.params\endcsname{20.43}
\expandafter\gdef\csname R@an.xxablation.V7B1.paramsx\endcsname{0.66}
\expandafter\gdef\csname R@an.xxablation.V7B1.parent\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.xxablation.V7B1.sentence\endcsname{on LeanAdd-NeXt, a separable coarse kernel (LeanSep) brings the parameters to 0.66$\times$ and the profiled training step to 0.77$\times$ the default's; against the default: KiTS23 \ensuremath{+1.50}\,pp (two fresh seeds, SE 0.49), AMOS22 \ensuremath{-0.44}\,pp (seed 0)}
\expandafter\gdef\csname R@an.xxablation.V7B1.step\endcsname{95.3}
\expandafter\gdef\csname R@an.xxablation.V7B1.stepx\endcsname{0.77}
\expandafter\gdef\csname R@an.xxablation.V7B2.amos.basis\endcsname{seed 0}
\expandafter\gdef\csname R@an.xxablation.V7B2.amos.cell\endcsname{\ensuremath{-0.27}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxablation.V7B2.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7B2.amos.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.V7B2.amos.s0\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@an.xxablation.V7B2.amos.vsparent.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7B2.amos.vsparent.s0\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.xxablation.V7B2.change\endcsname{dilated coarse kernel}
\expandafter\gdef\csname R@an.xxablation.V7B2.delta_pool\endcsname{\ensuremath{+1.84}}
\expandafter\gdef\csname R@an.xxablation.V7B2.gmac\endcsname{256.9}
\expandafter\gdef\csname R@an.xxablation.V7B2.gmacx\endcsname{0.54}
\expandafter\gdef\csname R@an.xxablation.V7B2.group\endcsname{swap}
\expandafter\gdef\csname R@an.xxablation.V7B2.kits.basis\endcsname{two fresh seeds}
\expandafter\gdef\csname R@an.xxablation.V7B2.kits.cell\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@an.xxablation.V7B2.kits.fresh\endcsname{\ensuremath{+0.96}}
\expandafter\gdef\csname R@an.xxablation.V7B2.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V7B2.kits.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V7B2.kits.pool.fresh\endcsname{\ensuremath{+1.84}}
\expandafter\gdef\csname R@an.xxablation.V7B2.kits.pool.s0\endcsname{\ensuremath{+2.82}}
\expandafter\gdef\csname R@an.xxablation.V7B2.kits.s0\endcsname{\ensuremath{+1.95}}
\expandafter\gdef\csname R@an.xxablation.V7B2.kits.se\endcsname{0.49}
\expandafter\gdef\csname R@an.xxablation.V7B2.kits.vsparent.fresh\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@an.xxablation.V7B2.kits.vsparent.s0\endcsname{\ensuremath{+1.56}}
\expandafter\gdef\csname R@an.xxablation.V7B2.name\endcsname{LeanDil}
\expandafter\gdef\csname R@an.xxablation.V7B2.params\endcsname{20.45}
\expandafter\gdef\csname R@an.xxablation.V7B2.paramsx\endcsname{0.66}
\expandafter\gdef\csname R@an.xxablation.V7B2.parent\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.xxablation.V7B2.sentence\endcsname{on LeanAdd-NeXt, a dilated coarse kernel of the same extent (LeanDil) brings the parameters to 0.66$\times$ and the profiled training step to 0.76$\times$ the default's; against the default: KiTS23 \ensuremath{+0.96}\,pp (two fresh seeds, SE 0.49), AMOS22 \ensuremath{-0.27}\,pp (seed 0)}
\expandafter\gdef\csname R@an.xxablation.V7B2.step\endcsname{94.0}
\expandafter\gdef\csname R@an.xxablation.V7B2.stepx\endcsname{0.76}
\expandafter\gdef\csname R@an.xxablation.V7C1.amos.basis\endcsname{seed 0}
\expandafter\gdef\csname R@an.xxablation.V7C1.amos.cell\endcsname{\ensuremath{-0.11}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxablation.V7C1.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7C1.amos.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.V7C1.amos.s0\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.xxablation.V7C1.amos.vsparent.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7C1.amos.vsparent.s0\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@an.xxablation.V7C1.change\endcsname{ConvNeXt at st. 5 only}
\expandafter\gdef\csname R@an.xxablation.V7C1.delta_pool\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@an.xxablation.V7C1.gmac\endcsname{257.1}
\expandafter\gdef\csname R@an.xxablation.V7C1.gmacx\endcsname{0.54}
\expandafter\gdef\csname R@an.xxablation.V7C1.group\endcsname{path}
\expandafter\gdef\csname R@an.xxablation.V7C1.kits.basis\endcsname{two fresh seeds}
\expandafter\gdef\csname R@an.xxablation.V7C1.kits.cell\endcsname{\ensuremath{+1.56}}
\expandafter\gdef\csname R@an.xxablation.V7C1.kits.fresh\endcsname{\ensuremath{+1.56}}
\expandafter\gdef\csname R@an.xxablation.V7C1.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V7C1.kits.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V7C1.kits.pool.fresh\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@an.xxablation.V7C1.kits.pool.s0\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@an.xxablation.V7C1.kits.s0\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@an.xxablation.V7C1.kits.se\endcsname{0.49}
\expandafter\gdef\csname R@an.xxablation.V7C1.kits.vsparent.fresh\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@an.xxablation.V7C1.kits.vsparent.s0\endcsname{\ensuremath{+1.44}}
\expandafter\gdef\csname R@an.xxablation.V7C1.name\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi}}
\expandafter\gdef\csname R@an.xxablation.V7C1.params\endcsname{21.11}
\expandafter\gdef\csname R@an.xxablation.V7C1.paramsx\endcsname{0.68}
\expandafter\gdef\csname R@an.xxablation.V7C1.parent\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.xxablation.V7C1.sentence\endcsname{the ConvNeXt operator at encoder stage 5 only ({\ifdefined\archL\archL\else XX-Net-L\fi}) brings the parameters to 0.68$\times$ and the profiled training step to 0.77$\times$ the default's; against the default: KiTS23 \ensuremath{+1.56}\,pp (two fresh seeds, SE 0.49), AMOS22 \ensuremath{-0.11}\,pp (seed 0)}
\expandafter\gdef\csname R@an.xxablation.V7C1.step\endcsname{95.1}
\expandafter\gdef\csname R@an.xxablation.V7C1.stepx\endcsname{0.77}
\expandafter\gdef\csname R@an.xxablation.V7C2.amos.basis\endcsname{seed 0}
\expandafter\gdef\csname R@an.xxablation.V7C2.amos.cell\endcsname{\ensuremath{-0.36}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxablation.V7C2.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7C2.amos.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.V7C2.amos.s0\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.xxablation.V7C2.amos.vsparent.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7C2.amos.vsparent.s0\endcsname{\ensuremath{-0.49}}
\expandafter\gdef\csname R@an.xxablation.V7C2.change\endcsname{coarse kernel $3^3$}
\expandafter\gdef\csname R@an.xxablation.V7C2.delta_pool\endcsname{\ensuremath{+2.00}}
\expandafter\gdef\csname R@an.xxablation.V7C2.gmac\endcsname{256.9}
\expandafter\gdef\csname R@an.xxablation.V7C2.gmacx\endcsname{0.54}
\expandafter\gdef\csname R@an.xxablation.V7C2.group\endcsname{swap}
\expandafter\gdef\csname R@an.xxablation.V7C2.kits.basis\endcsname{seed 0}
\expandafter\gdef\csname R@an.xxablation.V7C2.kits.cell\endcsname{\ensuremath{+1.12}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxablation.V7C2.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7C2.kits.n\endcsname{1}
\expandafter\gdef\csname R@an.xxablation.V7C2.kits.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.V7C2.kits.pool.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7C2.kits.pool.s0\endcsname{\ensuremath{+2.00}}
\expandafter\gdef\csname R@an.xxablation.V7C2.kits.s0\endcsname{\ensuremath{+1.12}}
\expandafter\gdef\csname R@an.xxablation.V7C2.kits.se\endcsname{0.67}
\expandafter\gdef\csname R@an.xxablation.V7C2.kits.vsparent.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V7C2.kits.vsparent.s0\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.xxablation.V7C2.name\endcsname{LeanNeXt-k3}
\expandafter\gdef\csname R@an.xxablation.V7C2.params\endcsname{20.45}
\expandafter\gdef\csname R@an.xxablation.V7C2.paramsx\endcsname{0.66}
\expandafter\gdef\csname R@an.xxablation.V7C2.parent\endcsname{LeanAdd-NeXt}
\expandafter\gdef\csname R@an.xxablation.V7C2.sentence\endcsname{on LeanAdd-NeXt, a $3^3$ instead of a $7^3$ coarse kernel (LeanNeXt-k3) brings the parameters to 0.66$\times$ and the profiled training step to 0.76$\times$ the default's; against the default: KiTS23 \ensuremath{+1.12}\,pp (seed 0, SE 0.67), AMOS22 \ensuremath{-0.36}\,pp (seed 0)}
\expandafter\gdef\csname R@an.xxablation.V7C2.step\endcsname{94.2}
\expandafter\gdef\csname R@an.xxablation.V7C2.stepx\endcsname{0.76}
\expandafter\gdef\csname R@an.xxablation.V8A1.amos.basis\endcsname{seed 0}
\expandafter\gdef\csname R@an.xxablation.V8A1.amos.cell\endcsname{\ensuremath{-0.50}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxablation.V8A1.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V8A1.amos.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.V8A1.amos.s0\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@an.xxablation.V8A1.amos.vsparent.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V8A1.amos.vsparent.s0\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@an.xxablation.V8A1.change\endcsname{18 coarse blocks}
\expandafter\gdef\csname R@an.xxablation.V8A1.delta_pool\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.xxablation.V8A1.gmac\endcsname{257.8}
\expandafter\gdef\csname R@an.xxablation.V8A1.gmacx\endcsname{0.54}
\expandafter\gdef\csname R@an.xxablation.V8A1.group\endcsname{swap}
\expandafter\gdef\csname R@an.xxablation.V8A1.kits.basis\endcsname{two fresh seeds}
\expandafter\gdef\csname R@an.xxablation.V8A1.kits.cell\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.xxablation.V8A1.kits.fresh\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@an.xxablation.V8A1.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V8A1.kits.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V8A1.kits.pool.fresh\endcsname{\ensuremath{+1.25}}
\expandafter\gdef\csname R@an.xxablation.V8A1.kits.pool.s0\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@an.xxablation.V8A1.kits.s0\endcsname{\ensuremath{+0.88}}
\expandafter\gdef\csname R@an.xxablation.V8A1.kits.se\endcsname{0.49}
\expandafter\gdef\csname R@an.xxablation.V8A1.kits.vsparent.fresh\endcsname{\ensuremath{-1.19}}
\expandafter\gdef\csname R@an.xxablation.V8A1.kits.vsparent.s0\endcsname{\ensuremath{-0.95}}
\expandafter\gdef\csname R@an.xxablation.V8A1.name\endcsname{CoarseStack}
\expandafter\gdef\csname R@an.xxablation.V8A1.params\endcsname{31.31}
\expandafter\gdef\csname R@an.xxablation.V8A1.paramsx\endcsname{1.00}
\expandafter\gdef\csname R@an.xxablation.V8A1.parent\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi}}
\expandafter\gdef\csname R@an.xxablation.V8A1.sentence\endcsname{on {\ifdefined\archL\archL\else XX-Net-L\fi}, eighteen coarse blocks instead of four (CoarseStack) brings the parameters to 1.00$\times$ and the profiled training step to 0.91$\times$ the default's; against the default: KiTS23 \ensuremath{+0.37}\,pp (two fresh seeds, SE 0.49), AMOS22 \ensuremath{-0.50}\,pp (seed 0)}
\expandafter\gdef\csname R@an.xxablation.V8A1.step\endcsname{112.4}
\expandafter\gdef\csname R@an.xxablation.V8A1.stepx\endcsname{0.91}
\expandafter\gdef\csname R@an.xxablation.V8A2.amos.basis\endcsname{seed 0}
\expandafter\gdef\csname R@an.xxablation.V8A2.amos.cell\endcsname{\ensuremath{-0.31}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxablation.V8A2.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V8A2.amos.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.V8A2.amos.s0\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@an.xxablation.V8A2.amos.vsparent.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V8A2.amos.vsparent.s0\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.xxablation.V8A2.change\endcsname{12 blocks, coarse dec.}
\expandafter\gdef\csname R@an.xxablation.V8A2.delta_pool\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@an.xxablation.V8A2.gmac\endcsname{266.1}
\expandafter\gdef\csname R@an.xxablation.V8A2.gmacx\endcsname{0.56}
\expandafter\gdef\csname R@an.xxablation.V8A2.group\endcsname{swap}
\expandafter\gdef\csname R@an.xxablation.V8A2.kits.basis\endcsname{two fresh seeds}
\expandafter\gdef\csname R@an.xxablation.V8A2.kits.cell\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.xxablation.V8A2.kits.fresh\endcsname{\ensuremath{+1.00}}
\expandafter\gdef\csname R@an.xxablation.V8A2.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V8A2.kits.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V8A2.kits.pool.fresh\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@an.xxablation.V8A2.kits.pool.s0\endcsname{\ensuremath{+1.35}}
\expandafter\gdef\csname R@an.xxablation.V8A2.kits.s0\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.xxablation.V8A2.kits.se\endcsname{0.49}
\expandafter\gdef\csname R@an.xxablation.V8A2.kits.vsparent.fresh\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@an.xxablation.V8A2.kits.vsparent.s0\endcsname{\ensuremath{-1.35}}
\expandafter\gdef\csname R@an.xxablation.V8A2.name\endcsname{StackDec}
\expandafter\gdef\csname R@an.xxablation.V8A2.params\endcsname{31.47}
\expandafter\gdef\csname R@an.xxablation.V8A2.paramsx\endcsname{1.01}
\expandafter\gdef\csname R@an.xxablation.V8A2.parent\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi}}
\expandafter\gdef\csname R@an.xxablation.V8A2.sentence\endcsname{on {\ifdefined\archL\archL\else XX-Net-L\fi}, twelve coarse blocks instead of four and the second convolution restored at the two coarse decoder stages (StackDec) brings the parameters to 1.01$\times$ and the profiled training step to 0.85$\times$ the default's; against the default: KiTS23 \ensuremath{+1.00}\,pp (two fresh seeds, SE 0.49), AMOS22 \ensuremath{-0.31}\,pp (seed 0)}
\expandafter\gdef\csname R@an.xxablation.V8A2.step\endcsname{105.3}
\expandafter\gdef\csname R@an.xxablation.V8A2.stepx\endcsname{0.85}
\expandafter\gdef\csname R@an.xxablation.V8B1.amos.basis\endcsname{seed 0}
\expandafter\gdef\csname R@an.xxablation.V8B1.amos.cell\endcsname{\ensuremath{-0.75}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxablation.V8B1.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V8B1.amos.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.V8B1.amos.s0\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@an.xxablation.V8B1.amos.vsparent.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V8B1.amos.vsparent.s0\endcsname{\ensuremath{-0.64}}
\expandafter\gdef\csname R@an.xxablation.V8B1.change\endcsname{1 conv at st. 0, 1, 4}
\expandafter\gdef\csname R@an.xxablation.V8B1.delta_pool\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.xxablation.V8B1.gmac\endcsname{168.7}
\expandafter\gdef\csname R@an.xxablation.V8B1.gmacx\endcsname{0.35}
\expandafter\gdef\csname R@an.xxablation.V8B1.group\endcsname{swap}
\expandafter\gdef\csname R@an.xxablation.V8B1.kits.basis\endcsname{two fresh seeds}
\expandafter\gdef\csname R@an.xxablation.V8B1.kits.cell\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.xxablation.V8B1.kits.fresh\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.xxablation.V8B1.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V8B1.kits.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V8B1.kits.pool.fresh\endcsname{\ensuremath{+1.37}}
\expandafter\gdef\csname R@an.xxablation.V8B1.kits.pool.s0\endcsname{\ensuremath{+2.91}}
\expandafter\gdef\csname R@an.xxablation.V8B1.kits.s0\endcsname{\ensuremath{+2.03}}
\expandafter\gdef\csname R@an.xxablation.V8B1.kits.se\endcsname{0.49}
\expandafter\gdef\csname R@an.xxablation.V8B1.kits.vsparent.fresh\endcsname{\ensuremath{-1.07}}
\expandafter\gdef\csname R@an.xxablation.V8B1.kits.vsparent.s0\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@an.xxablation.V8B1.name\endcsname{LeanTrunk}
\expandafter\gdef\csname R@an.xxablation.V8B1.params\endcsname{18.21}
\expandafter\gdef\csname R@an.xxablation.V8B1.paramsx\endcsname{0.58}
\expandafter\gdef\csname R@an.xxablation.V8B1.parent\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi}}
\expandafter\gdef\csname R@an.xxablation.V8B1.sentence\endcsname{on {\ifdefined\archL\archL\else XX-Net-L\fi}, one convolution at encoder stages 0, 1 and 4 (LeanTrunk) brings the parameters to 0.58$\times$ and the profiled training step to 0.59$\times$ the default's; against the default: KiTS23 \ensuremath{+0.50}\,pp (two fresh seeds, SE 0.49), AMOS22 \ensuremath{-0.75}\,pp (seed 0)}
\expandafter\gdef\csname R@an.xxablation.V8B1.step\endcsname{72.5}
\expandafter\gdef\csname R@an.xxablation.V8B1.stepx\endcsname{0.59}
\expandafter\gdef\csname R@an.xxablation.V8B2.amos.basis\endcsname{seed 0}
\expandafter\gdef\csname R@an.xxablation.V8B2.amos.cell\endcsname{\ensuremath{-0.29}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxablation.V8B2.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V8B2.amos.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.V8B2.amos.s0\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.xxablation.V8B2.amos.vsparent.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V8B2.amos.vsparent.s0\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@an.xxablation.V8B2.change\endcsname{1 conv at st. 0}
\expandafter\gdef\csname R@an.xxablation.V8B2.delta_pool\endcsname{\ensuremath{+1.73}}
\expandafter\gdef\csname R@an.xxablation.V8B2.gmac\endcsname{199.1}
\expandafter\gdef\csname R@an.xxablation.V8B2.gmacx\endcsname{0.42}
\expandafter\gdef\csname R@an.xxablation.V8B2.group\endcsname{swap}
\expandafter\gdef\csname R@an.xxablation.V8B2.kits.basis\endcsname{two fresh seeds}
\expandafter\gdef\csname R@an.xxablation.V8B2.kits.cell\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.xxablation.V8B2.kits.fresh\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@an.xxablation.V8B2.kits.n\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V8B2.kits.nfresh\endcsname{2}
\expandafter\gdef\csname R@an.xxablation.V8B2.kits.pool.fresh\endcsname{\ensuremath{+1.73}}
\expandafter\gdef\csname R@an.xxablation.V8B2.kits.pool.s0\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.xxablation.V8B2.kits.s0\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.xxablation.V8B2.kits.se\endcsname{0.49}
\expandafter\gdef\csname R@an.xxablation.V8B2.kits.vsparent.fresh\endcsname{\ensuremath{-0.71}}
\expandafter\gdef\csname R@an.xxablation.V8B2.kits.vsparent.s0\endcsname{\ensuremath{-1.06}}
\expandafter\gdef\csname R@an.xxablation.V8B2.name\endcsname{Stem1}
\expandafter\gdef\csname R@an.xxablation.V8B2.params\endcsname{21.08}
\expandafter\gdef\csname R@an.xxablation.V8B2.paramsx\endcsname{0.68}
\expandafter\gdef\csname R@an.xxablation.V8B2.parent\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi}}
\expandafter\gdef\csname R@an.xxablation.V8B2.sentence\endcsname{on {\ifdefined\archL\archL\else XX-Net-L\fi}, one convolution at encoder stage 0 (Stem1) brings the parameters to 0.68$\times$ and the profiled training step to 0.63$\times$ the default's; against the default: KiTS23 \ensuremath{+0.85}\,pp (two fresh seeds, SE 0.49), AMOS22 \ensuremath{-0.29}\,pp (seed 0)}
\expandafter\gdef\csname R@an.xxablation.V8B2.step\endcsname{77.6}
\expandafter\gdef\csname R@an.xxablation.V8B2.stepx\endcsname{0.63}
\expandafter\gdef\csname R@an.xxablation.V8X1.amos.basis\endcsname{seed 0}
\expandafter\gdef\csname R@an.xxablation.V8X1.amos.cell\endcsname{\ensuremath{-0.36}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxablation.V8X1.amos.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V8X1.amos.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.V8X1.amos.s0\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@an.xxablation.V8X1.amos.vsparent.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V8X1.amos.vsparent.s0\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.xxablation.V8X1.change\endcsname{stages 3--5 narrowed}
\expandafter\gdef\csname R@an.xxablation.V8X1.delta_pool\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.xxablation.V8X1.gmac\endcsname{255.3}
\expandafter\gdef\csname R@an.xxablation.V8X1.gmacx\endcsname{0.53}
\expandafter\gdef\csname R@an.xxablation.V8X1.group\endcsname{swap}
\expandafter\gdef\csname R@an.xxablation.V8X1.kits.basis\endcsname{seed 0}
\expandafter\gdef\csname R@an.xxablation.V8X1.kits.cell\endcsname{\ensuremath{+1.66}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxablation.V8X1.kits.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V8X1.kits.n\endcsname{1}
\expandafter\gdef\csname R@an.xxablation.V8X1.kits.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.V8X1.kits.pool.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V8X1.kits.pool.s0\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@an.xxablation.V8X1.kits.s0\endcsname{\ensuremath{+1.66}}
\expandafter\gdef\csname R@an.xxablation.V8X1.kits.se\endcsname{0.67}
\expandafter\gdef\csname R@an.xxablation.V8X1.kits.vsparent.fresh\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.V8X1.kits.vsparent.s0\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@an.xxablation.V8X1.name\endcsname{NarrowTrunk}
\expandafter\gdef\csname R@an.xxablation.V8X1.params\endcsname{18.25}
\expandafter\gdef\csname R@an.xxablation.V8X1.paramsx\endcsname{0.58}
\expandafter\gdef\csname R@an.xxablation.V8X1.parent\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi}}
\expandafter\gdef\csname R@an.xxablation.V8X1.sentence\endcsname{on {\ifdefined\archL\archL\else XX-Net-L\fi}, the widths of stages 3 to 5 narrowed to the parameter count of LeanTrunk (NarrowTrunk) brings the parameters to 0.58$\times$ and the profiled training step to 0.77$\times$ the default's; against the default: KiTS23 \ensuremath{+1.66}\,pp (seed 0, SE 0.67), AMOS22 \ensuremath{-0.36}\,pp (seed 0)}
\expandafter\gdef\csname R@an.xxablation.V8X1.step\endcsname{94.6}
\expandafter\gdef\csname R@an.xxablation.V8X1.stepx\endcsname{0.77}
\expandafter\gdef\csname R@an.xxablation.base.amos.basis\endcsname{reference}
\expandafter\gdef\csname R@an.xxablation.base.amos.cell\endcsname{ref.}
\expandafter\gdef\csname R@an.xxablation.base.amos.fresh\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.xxablation.base.amos.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.base.amos.s0\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.xxablation.base.change\endcsname{--}
\expandafter\gdef\csname R@an.xxablation.base.delta_pool\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.xxablation.base.gmac\endcsname{477.4}
\expandafter\gdef\csname R@an.xxablation.base.gmacx\endcsname{1.00}
\expandafter\gdef\csname R@an.xxablation.base.group\endcsname{path}
\expandafter\gdef\csname R@an.xxablation.base.kits.basis\endcsname{reference}
\expandafter\gdef\csname R@an.xxablation.base.kits.cell\endcsname{ref.}
\expandafter\gdef\csname R@an.xxablation.base.kits.fresh\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.xxablation.base.kits.n\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.base.kits.nfresh\endcsname{0}
\expandafter\gdef\csname R@an.xxablation.base.kits.pool.fresh\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.xxablation.base.kits.pool.s0\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.xxablation.base.kits.s0\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.xxablation.base.kits.se\endcsname{\pend}
\expandafter\gdef\csname R@an.xxablation.base.name\endcsname{nnU-Net}
\expandafter\gdef\csname R@an.xxablation.base.params\endcsname{31.20}
\expandafter\gdef\csname R@an.xxablation.base.paramsx\endcsname{1.00}
\expandafter\gdef\csname R@an.xxablation.base.parent\endcsname{none}
\expandafter\gdef\csname R@an.xxablation.base.step\endcsname{123.3}
\expandafter\gdef\csname R@an.xxablation.base.stepx\endcsname{1.00}
\expandafter\gdef\csname R@an.xxablation.caption\endcsname{Ablation of {\ifdefined\archL\archL\else XX-Net-L\fi} along the agents' design path from the nnU-Net default and the registered operator swaps around it (rows grouped by the arm they change). Parameters and profiled training step on the KiTS23 plan as multiples of the nnU-Net default's (31.20\,M, 123.3\,ms); Dice differences in pp on KiTS23 to the stock default, the mean of nnU-Net's 9 runs of the same pipeline (84.26; the frozen pool of 3 runs reads 83.38), on AMOS22 to the frozen default pool of 6 runs (87.70; its 3 stock runs average 87.71); unmarked: mean of fresh seeds 1 and 2 of fold 0; \textsuperscript{\dag}: seed 0, one run (the discovery value).}
\expandafter\gdef\csname R@an.xxablation.default.gmac\endcsname{477.4}
\expandafter\gdef\csname R@an.xxablation.default.params\endcsname{31.20}
\expandafter\gdef\csname R@an.xxablation.default.step\endcsname{123.3}
\expandafter\gdef\csname R@an.xxablation.legend\endcsname{parameters and profiled training step on the KiTS23 plan as multiples of the nnU-Net default's (31.20\,M, 123.3\,ms); Dice differences in pp on KiTS23 to the stock default, the mean of nnU-Net's 9 runs of the same pipeline (84.26; the frozen pool of 3 runs reads 83.38), on AMOS22 to the frozen default pool of 6 runs (87.70; its 3 stock runs average 87.71); unmarked: mean of fresh seeds 1 and 2 of fold 0; \textsuperscript{\dag}: seed 0, one run (the discovery value)}
\expandafter\gdef\csname R@an.xxablation.path.n\endcsname{4}
\expandafter\gdef\csname R@an.xxablation.path.names\endcsname{nnU-Net $\to$ LeanDec $\to$ LeanAdd $\to$ LeanAdd-NeXt $\to$ {\ifdefined\archL\archL\else XX-Net-L\fi}}
\expandafter\gdef\csname R@an.xxablation.pool.amos\endcsname{87.70}
\expandafter\gdef\csname R@an.xxablation.pool.kits\endcsname{83.38}
\expandafter\gdef\csname R@an.xxablation.rows.n\endcsname{16}
\expandafter\gdef\csname R@an.xxablation.sent.path\endcsname{the agents reached {\ifdefined\archL\archL\else XX-Net-L\fi} from the nnU-Net default in 4 registered steps (nnU-Net $\to$ LeanDec $\to$ LeanAdd $\to$ LeanAdd-NeXt $\to$ {\ifdefined\archL\archL\else XX-Net-L\fi}), ending at 0.68$\times$ the default's parameters, 0.54$\times$ its multiply-adds and 0.77$\times$ its profiled training step on the KiTS23 plan}
\expandafter\gdef\csname R@an.xxablation.stock.amos.mean\endcsname{87.71}
\expandafter\gdef\csname R@an.xxablation.stock.amos.n\endcsname{3}
\expandafter\gdef\csname R@an.xxablation.stock.kits.mean\endcsname{84.26}
\expandafter\gdef\csname R@an.xxablation.stock.kits.n\endcsname{9}
\expandafter\gdef\csname R@an.xxablation.stock.kits.sd\endcsname{0.63}
\expandafter\gdef\csname R@an.xxablation.swaps.n\endcsname{11}
\expandafter\gdef\csname R@an.xxablation.xl.name\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi}}
\expandafter\gdef\csname R@an.xxablation.xl.tag\endcsname{V7C1}
\expandafter\gdef\csname R@an.xxloo.AB1.amos\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB1.amos.cell\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB1.amos.floor\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB1.change\endcsname{coarsest kernel $3^3$}
\expandafter\gdef\csname R@an.xxloo.AB1.delta_amos_pool\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB1.delta_amos_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB1.delta_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB1.delta_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB1.gmacx\endcsname{0.54}
\expandafter\gdef\csname R@an.xxloo.AB1.group\endcsname{loo}
\expandafter\gdef\csname R@an.xxloo.AB1.kits.cell\endcsname{\ensuremath{-0.31}\textsuperscript{1/3}}
\expandafter\gdef\csname R@an.xxloo.AB1.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB1.n\endcsname{1}
\expandafter\gdef\csname R@an.xxloo.AB1.name\endcsname{Kernel 3}
\expandafter\gdef\csname R@an.xxloo.AB1.paramsx\endcsname{0.66}
\expandafter\gdef\csname R@an.xxloo.AB1.partial\endcsname{83.95 (1 of 3 seeds, partial)}
\expandafter\gdef\csname R@an.xxloo.AB1.se_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB1.se_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB1.sentence\endcsname{on KiTS23 1 of the 3 runs of Kernel 3 have finished (partial, no mean is printed); the AMOS22 run has not finished}
\expandafter\gdef\csname R@an.xxloo.AB1.state\endcsname{partial: 1 of 3 seeds}
\expandafter\gdef\csname R@an.xxloo.AB1.stepx\endcsname{0.75}
\expandafter\gdef\csname R@an.xxloo.AB10.amos\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB10.amos.cell\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB10.amos.floor\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB10.change\endcsname{widths $\times1.25$}
\expandafter\gdef\csname R@an.xxloo.AB10.delta_amos_pool\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB10.delta_amos_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB10.delta_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB10.delta_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB10.gmacx\endcsname{0.84}
\expandafter\gdef\csname R@an.xxloo.AB10.group\endcsname{width}
\expandafter\gdef\csname R@an.xxloo.AB10.kits.cell\endcsname{\ensuremath{+1.84}\textsuperscript{1/3}}
\expandafter\gdef\csname R@an.xxloo.AB10.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB10.n\endcsname{1}
\expandafter\gdef\csname R@an.xxloo.AB10.name\endcsname{Width 1.25}
\expandafter\gdef\csname R@an.xxloo.AB10.paramsx\endcsname{1.05}
\expandafter\gdef\csname R@an.xxloo.AB10.partial\endcsname{86.10 (1 of 3 seeds, partial)}
\expandafter\gdef\csname R@an.xxloo.AB10.se_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB10.se_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB10.sentence\endcsname{on KiTS23 1 of the 3 runs of Width 1.25 have finished (partial, no mean is printed); the AMOS22 run has not finished}
\expandafter\gdef\csname R@an.xxloo.AB10.state\endcsname{partial: 1 of 3 seeds}
\expandafter\gdef\csname R@an.xxloo.AB10.stepx\endcsname{1.10}
\expandafter\gdef\csname R@an.xxloo.AB11.amos\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB11.amos.cell\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB11.amos.floor\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB11.change\endcsname{default, widths $\times0.82$}
\expandafter\gdef\csname R@an.xxloo.AB11.delta_amos_pool\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB11.delta_amos_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB11.delta_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB11.delta_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB11.gmacx\endcsname{0.64}
\expandafter\gdef\csname R@an.xxloo.AB11.group\endcsname{cost}
\expandafter\gdef\csname R@an.xxloo.AB11.kits.cell\endcsname{\ensuremath{-1.41}\textsuperscript{1/3}}
\expandafter\gdef\csname R@an.xxloo.AB11.match\endcsname{matched parameters}
\expandafter\gdef\csname R@an.xxloo.AB11.matched\endcsname{the matched parameters comparison of {\ifdefined\archL\archL\else XX-Net-L\fi} waits for the three KiTS23 runs of the control (1 finished)}
\expandafter\gdef\csname R@an.xxloo.AB11.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB11.n\endcsname{1}
\expandafter\gdef\csname R@an.xxloo.AB11.name\endcsname{Narrow default (params)}
\expandafter\gdef\csname R@an.xxloo.AB11.paramsx\endcsname{0.67}
\expandafter\gdef\csname R@an.xxloo.AB11.partial\endcsname{82.84 (1 of 3 seeds, partial)}
\expandafter\gdef\csname R@an.xxloo.AB11.se_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB11.se_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB11.sentence\endcsname{on KiTS23 1 of the 3 runs of Narrow default (params) have finished (partial, no mean is printed); the AMOS22 run has not finished}
\expandafter\gdef\csname R@an.xxloo.AB11.state\endcsname{partial: 1 of 3 seeds}
\expandafter\gdef\csname R@an.xxloo.AB11.stepx\endcsname{1.01}
\expandafter\gdef\csname R@an.xxloo.AB2.amos\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB2.amos.cell\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB2.amos.floor\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB2.change\endcsname{no GRN, coarsest blocks}
\expandafter\gdef\csname R@an.xxloo.AB2.delta_amos_pool\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB2.delta_amos_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB2.delta_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB2.delta_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB2.gmacx\endcsname{0.54}
\expandafter\gdef\csname R@an.xxloo.AB2.group\endcsname{loo}
\expandafter\gdef\csname R@an.xxloo.AB2.kits.cell\endcsname{\ensuremath{+1.76}\textsuperscript{1/3}}
\expandafter\gdef\csname R@an.xxloo.AB2.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB2.n\endcsname{1}
\expandafter\gdef\csname R@an.xxloo.AB2.name\endcsname{No GRN}
\expandafter\gdef\csname R@an.xxloo.AB2.paramsx\endcsname{0.68}
\expandafter\gdef\csname R@an.xxloo.AB2.partial\endcsname{86.02 (1 of 3 seeds, partial)}
\expandafter\gdef\csname R@an.xxloo.AB2.se_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB2.se_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB2.sentence\endcsname{on KiTS23 1 of the 3 runs of No GRN have finished (partial, no mean is printed); the AMOS22 run has not finished}
\expandafter\gdef\csname R@an.xxloo.AB2.state\endcsname{partial: 1 of 3 seeds}
\expandafter\gdef\csname R@an.xxloo.AB2.stepx\endcsname{0.77}
\expandafter\gdef\csname R@an.xxloo.AB3.amos\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB3.amos.cell\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB3.amos.floor\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB3.change\endcsname{skips concatenated}
\expandafter\gdef\csname R@an.xxloo.AB3.delta_amos_pool\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB3.delta_amos_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB3.delta_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB3.delta_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB3.gmacx\endcsname{0.77}
\expandafter\gdef\csname R@an.xxloo.AB3.group\endcsname{loo}
\expandafter\gdef\csname R@an.xxloo.AB3.kits.cell\endcsname{\ensuremath{+1.28}\textsuperscript{1/3}}
\expandafter\gdef\csname R@an.xxloo.AB3.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB3.n\endcsname{1}
\expandafter\gdef\csname R@an.xxloo.AB3.name\endcsname{Concat skips}
\expandafter\gdef\csname R@an.xxloo.AB3.paramsx\endcsname{0.84}
\expandafter\gdef\csname R@an.xxloo.AB3.partial\endcsname{85.54 (1 of 3 seeds, partial)}
\expandafter\gdef\csname R@an.xxloo.AB3.se_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB3.se_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB3.sentence\endcsname{on KiTS23 1 of the 3 runs of Concat skips have finished (partial, no mean is printed); the AMOS22 run has not finished}
\expandafter\gdef\csname R@an.xxloo.AB3.state\endcsname{partial: 1 of 3 seeds}
\expandafter\gdef\csname R@an.xxloo.AB3.stepx\endcsname{0.86}
\expandafter\gdef\csname R@an.xxloo.AB4.amos\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB4.amos.cell\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB4.amos.floor\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB4.change\endcsname{second decoder conv restored}
\expandafter\gdef\csname R@an.xxloo.AB4.delta_amos_pool\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB4.delta_amos_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB4.delta_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB4.delta_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB4.gmacx\endcsname{0.77}
\expandafter\gdef\csname R@an.xxloo.AB4.group\endcsname{loo}
\expandafter\gdef\csname R@an.xxloo.AB4.kits.cell\endcsname{\ensuremath{+0.51}\textsuperscript{1/3}}
\expandafter\gdef\csname R@an.xxloo.AB4.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB4.n\endcsname{1}
\expandafter\gdef\csname R@an.xxloo.AB4.name\endcsname{Full decoder}
\expandafter\gdef\csname R@an.xxloo.AB4.paramsx\endcsname{0.84}
\expandafter\gdef\csname R@an.xxloo.AB4.partial\endcsname{84.77 (1 of 3 seeds, partial)}
\expandafter\gdef\csname R@an.xxloo.AB4.se_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB4.se_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB4.sentence\endcsname{on KiTS23 1 of the 3 runs of Full decoder have finished (partial, no mean is printed); the AMOS22 run has not finished}
\expandafter\gdef\csname R@an.xxloo.AB4.state\endcsname{partial: 1 of 3 seeds}
\expandafter\gdef\csname R@an.xxloo.AB4.stepx\endcsname{0.96}
\expandafter\gdef\csname R@an.xxloo.AB5.amos\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB5.amos.cell\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB5.amos.floor\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB5.change\endcsname{2 blocks at the coarsest stage}
\expandafter\gdef\csname R@an.xxloo.AB5.delta_amos_pool\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB5.delta_amos_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB5.delta_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB5.delta_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB5.gmacx\endcsname{0.54}
\expandafter\gdef\csname R@an.xxloo.AB5.group\endcsname{loo}
\expandafter\gdef\csname R@an.xxloo.AB5.kits.cell\endcsname{\ensuremath{+0.69}\textsuperscript{1/3}}
\expandafter\gdef\csname R@an.xxloo.AB5.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB5.n\endcsname{1}
\expandafter\gdef\csname R@an.xxloo.AB5.name\endcsname{Two blocks}
\expandafter\gdef\csname R@an.xxloo.AB5.paramsx\endcsname{0.63}
\expandafter\gdef\csname R@an.xxloo.AB5.partial\endcsname{84.95 (1 of 3 seeds, partial)}
\expandafter\gdef\csname R@an.xxloo.AB5.se_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB5.se_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB5.sentence\endcsname{on KiTS23 1 of the 3 runs of Two blocks have finished (partial, no mean is printed); the AMOS22 run has not finished}
\expandafter\gdef\csname R@an.xxloo.AB5.state\endcsname{partial: 1 of 3 seeds}
\expandafter\gdef\csname R@an.xxloo.AB5.stepx\endcsname{0.77}
\expandafter\gdef\csname R@an.xxloo.AB6.amos\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB6.amos.cell\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB6.amos.floor\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB6.change\endcsname{4 blocks at stage 4, not 5}
\expandafter\gdef\csname R@an.xxloo.AB6.delta_amos_pool\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB6.delta_amos_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB6.delta_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB6.delta_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB6.gmacx\endcsname{0.54}
\expandafter\gdef\csname R@an.xxloo.AB6.group\endcsname{loo}
\expandafter\gdef\csname R@an.xxloo.AB6.kits.cell\endcsname{\ensuremath{+0.90}\textsuperscript{1/3}}
\expandafter\gdef\csname R@an.xxloo.AB6.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB6.n\endcsname{1}
\expandafter\gdef\csname R@an.xxloo.AB6.name\endcsname{Stage-4 blocks}
\expandafter\gdef\csname R@an.xxloo.AB6.paramsx\endcsname{0.68}
\expandafter\gdef\csname R@an.xxloo.AB6.partial\endcsname{85.15 (1 of 3 seeds, partial)}
\expandafter\gdef\csname R@an.xxloo.AB6.se_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB6.se_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB6.sentence\endcsname{on KiTS23 1 of the 3 runs of Stage-4 blocks have finished (partial, no mean is printed); the AMOS22 run has not finished}
\expandafter\gdef\csname R@an.xxloo.AB6.state\endcsname{partial: 1 of 3 seeds}
\expandafter\gdef\csname R@an.xxloo.AB6.stepx\endcsname{0.79}
\expandafter\gdef\csname R@an.xxloo.AB7.amos\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB7.amos.cell\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB7.amos.floor\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB7.change\endcsname{default, widths $\times0.70$}
\expandafter\gdef\csname R@an.xxloo.AB7.delta_amos_pool\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB7.delta_amos_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB7.delta_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB7.delta_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB7.gmacx\endcsname{0.54}
\expandafter\gdef\csname R@an.xxloo.AB7.group\endcsname{cost}
\expandafter\gdef\csname R@an.xxloo.AB7.kits.cell\endcsname{\ensuremath{-1.03}\textsuperscript{1/3}}
\expandafter\gdef\csname R@an.xxloo.AB7.match\endcsname{matched multiply-adds}
\expandafter\gdef\csname R@an.xxloo.AB7.matched\endcsname{the matched multiply-adds comparison of {\ifdefined\archL\archL\else XX-Net-L\fi} waits for the three KiTS23 runs of the control (1 finished)}
\expandafter\gdef\csname R@an.xxloo.AB7.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB7.n\endcsname{1}
\expandafter\gdef\csname R@an.xxloo.AB7.name\endcsname{Narrow default (MACs)}
\expandafter\gdef\csname R@an.xxloo.AB7.paramsx\endcsname{0.49}
\expandafter\gdef\csname R@an.xxloo.AB7.partial\endcsname{83.23 (1 of 3 seeds, partial)}
\expandafter\gdef\csname R@an.xxloo.AB7.se_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB7.se_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB7.sentence\endcsname{on KiTS23 1 of the 3 runs of Narrow default (MACs) have finished (partial, no mean is printed); the AMOS22 run has not finished}
\expandafter\gdef\csname R@an.xxloo.AB7.state\endcsname{partial: 1 of 3 seeds}
\expandafter\gdef\csname R@an.xxloo.AB7.stepx\endcsname{0.96}
\expandafter\gdef\csname R@an.xxloo.AB8.amos\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB8.amos.cell\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB8.amos.floor\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB8.change\endcsname{hand-made efficient decoder}
\expandafter\gdef\csname R@an.xxloo.AB8.delta_amos_pool\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB8.delta_amos_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB8.delta_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB8.delta_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB8.gmacx\endcsname{0.56}
\expandafter\gdef\csname R@an.xxloo.AB8.group\endcsname{cost}
\expandafter\gdef\csname R@an.xxloo.AB8.kits.cell\endcsname{\ensuremath{+0.46}\textsuperscript{1/3}}
\expandafter\gdef\csname R@an.xxloo.AB8.match\endcsname{matched multiply-adds}
\expandafter\gdef\csname R@an.xxloo.AB8.matched\endcsname{the matched multiply-adds comparison of {\ifdefined\archL\archL\else XX-Net-L\fi} waits for the three KiTS23 runs of the control (1 finished)}
\expandafter\gdef\csname R@an.xxloo.AB8.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB8.n\endcsname{1}
\expandafter\gdef\csname R@an.xxloo.AB8.name\endcsname{Hand EffiDec}
\expandafter\gdef\csname R@an.xxloo.AB8.paramsx\endcsname{0.54}
\expandafter\gdef\csname R@an.xxloo.AB8.partial\endcsname{84.72 (1 of 3 seeds, partial)}
\expandafter\gdef\csname R@an.xxloo.AB8.se_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB8.se_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB8.sentence\endcsname{on KiTS23 1 of the 3 runs of Hand EffiDec have finished (partial, no mean is printed); the AMOS22 run has not finished}
\expandafter\gdef\csname R@an.xxloo.AB8.state\endcsname{partial: 1 of 3 seeds}
\expandafter\gdef\csname R@an.xxloo.AB8.stepx\endcsname{0.68}
\expandafter\gdef\csname R@an.xxloo.AB9.amos\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB9.amos.cell\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB9.amos.floor\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB9.change\endcsname{widths $\times0.75$}
\expandafter\gdef\csname R@an.xxloo.AB9.delta_amos_pool\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB9.delta_amos_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB9.delta_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB9.delta_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB9.gmacx\endcsname{0.30}
\expandafter\gdef\csname R@an.xxloo.AB9.group\endcsname{width}
\expandafter\gdef\csname R@an.xxloo.AB9.kits.cell\endcsname{\ensuremath{+0.77}\textsuperscript{1/3}}
\expandafter\gdef\csname R@an.xxloo.AB9.mean\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB9.n\endcsname{1}
\expandafter\gdef\csname R@an.xxloo.AB9.name\endcsname{Width 0.75}
\expandafter\gdef\csname R@an.xxloo.AB9.paramsx\endcsname{0.38}
\expandafter\gdef\csname R@an.xxloo.AB9.partial\endcsname{85.03 (1 of 3 seeds, partial)}
\expandafter\gdef\csname R@an.xxloo.AB9.se_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB9.se_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.AB9.sentence\endcsname{on KiTS23 1 of the 3 runs of Width 0.75 have finished (partial, no mean is printed); the AMOS22 run has not finished}
\expandafter\gdef\csname R@an.xxloo.AB9.state\endcsname{partial: 1 of 3 seeds}
\expandafter\gdef\csname R@an.xxloo.AB9.stepx\endcsname{0.73}
\expandafter\gdef\csname R@an.xxloo.def.amos\endcsname{87.70}
\expandafter\gdef\csname R@an.xxloo.def.amos.cell\endcsname{ref.}
\expandafter\gdef\csname R@an.xxloo.def.amos.floor\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.def.change\endcsname{stock nnU-Net}
\expandafter\gdef\csname R@an.xxloo.def.delta_amos_pool\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.xxloo.def.delta_amos_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.def.delta_stock\endcsname{\ensuremath{+0.00}}
\expandafter\gdef\csname R@an.xxloo.def.delta_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.def.gmacx\endcsname{1.00}
\expandafter\gdef\csname R@an.xxloo.def.group\endcsname{ref}
\expandafter\gdef\csname R@an.xxloo.def.kits.cell\endcsname{ref.}
\expandafter\gdef\csname R@an.xxloo.def.mean\endcsname{84.26}
\expandafter\gdef\csname R@an.xxloo.def.n\endcsname{9}
\expandafter\gdef\csname R@an.xxloo.def.name\endcsname{nnU-Net default}
\expandafter\gdef\csname R@an.xxloo.def.paramsx\endcsname{1.00}
\expandafter\gdef\csname R@an.xxloo.def.se_stock\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.def.se_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.def.state\endcsname{reference}
\expandafter\gdef\csname R@an.xxloo.def.stepx\endcsname{1.00}
\expandafter\gdef\csname R@an.xxloo.floor\endcsname{0.50}
\expandafter\gdef\csname R@an.xxloo.legend\endcsname{leave-one-out arms of {\ifdefined\archL\archL\else XX-Net-L\fi} (each removes or changes one element), the cost controls (matched multiply-adds) and the width family; parameters and profiled step as multiples of the nnU-Net default's on the KiTS23 plan; KiTS23: the signed difference of the arm's mean from the stock mean (the mean of nnU-Net's 9 runs of the same pipeline, 84.26); a superscript k/3 marks an arm with only k of its three seeds finished and the pending mark one with none; the {\ifdefined\archL\archL\else XX-Net-L\fi} row is the mean of its three runs, \ensuremath{+1.65}\,pp from the stock mean (SE 0.42), where the ablation table of the design path prints the mean of its fresh seeds 1 and 2 alone, \ensuremath{+1.56}\,pp (SE 0.49); AMOS22: the seed-0 run against the frozen default pool, one run, marked with the dagger}
\expandafter\gdef\csname R@an.xxloo.note\endcsname{KiTS23: the signed difference of the arm's mean from the stock mean (the mean of nnU-Net's 9 runs of the same pipeline, 84.26); a superscript k/3 marks an arm with only k of its three seeds finished and the pending mark one with none; the {\ifdefined\archL\archL\else XX-Net-L\fi} row is the mean of its three runs, \ensuremath{+1.65}\,pp from the stock mean (SE 0.42), where the ablation table of the design path prints the mean of its fresh seeds 1 and 2 alone, \ensuremath{+1.56}\,pp (SE 0.49); AMOS22: the seed-0 run against the frozen default pool, one run, marked with the dagger}
\expandafter\gdef\csname R@an.xxloo.resm.amos\endcsname{88.35}
\expandafter\gdef\csname R@an.xxloo.resm.amos.cell\endcsname{\ensuremath{+0.65}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxloo.resm.amos.floor\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.resm.change\endcsname{library residual preset}
\expandafter\gdef\csname R@an.xxloo.resm.delta_amos_pool\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@an.xxloo.resm.delta_amos_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.resm.delta_stock\endcsname{\ensuremath{+2.21}}
\expandafter\gdef\csname R@an.xxloo.resm.delta_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.resm.gmacx\endcsname{1.50}
\expandafter\gdef\csname R@an.xxloo.resm.group\endcsname{ref}
\expandafter\gdef\csname R@an.xxloo.resm.kits.cell\endcsname{\ensuremath{+2.21}}
\expandafter\gdef\csname R@an.xxloo.resm.mean\endcsname{86.47}
\expandafter\gdef\csname R@an.xxloo.resm.n\endcsname{3}
\expandafter\gdef\csname R@an.xxloo.resm.name\endcsname{ResEnc-M}
\expandafter\gdef\csname R@an.xxloo.resm.paramsx\endcsname{3.28}
\expandafter\gdef\csname R@an.xxloo.resm.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.xxloo.resm.se_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.resm.state\endcsname{complete}
\expandafter\gdef\csname R@an.xxloo.resm.stepx\endcsname{1.33}
\expandafter\gdef\csname R@an.xxloo.state\endcsname{0 of 11 arms complete on KiTS23 (three seeds), 11 partial, 0 with the AMOS22 run}
\expandafter\gdef\csname R@an.xxloo.stock.mean\endcsname{84.26}
\expandafter\gdef\csname R@an.xxloo.stock.n\endcsname{9}
\expandafter\gdef\csname R@an.xxloo.stock.sd\endcsname{0.63}
\expandafter\gdef\csname R@an.xxloo.width.sentence\endcsname{the width family is pending: Width 0.75 1 of 3 seeds, Width 1.25 1 of 3 seeds}
\expandafter\gdef\csname R@an.xxloo.xl.amos\endcsname{87.60}
\expandafter\gdef\csname R@an.xxloo.xl.amos.cell\endcsname{\ensuremath{-0.11}\textsuperscript{\dag}}
\expandafter\gdef\csname R@an.xxloo.xl.amos.floor\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.xl.change\endcsname{ConvNeXt at stage 5 only}
\expandafter\gdef\csname R@an.xxloo.xl.delta_amos_pool\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.xxloo.xl.delta_amos_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.xl.delta_stock\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.xxloo.xl.delta_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.xl.fresh\endcsname{\ensuremath{+1.56}}
\expandafter\gdef\csname R@an.xxloo.xl.fresh.se\endcsname{0.49}
\expandafter\gdef\csname R@an.xxloo.xl.gmacx\endcsname{0.54}
\expandafter\gdef\csname R@an.xxloo.xl.group\endcsname{ref}
\expandafter\gdef\csname R@an.xxloo.xl.kits.cell\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@an.xxloo.xl.mean\endcsname{85.91}
\expandafter\gdef\csname R@an.xxloo.xl.n\endcsname{3}
\expandafter\gdef\csname R@an.xxloo.xl.name\endcsname{{\ifdefined\archL\archL\else XX-Net-L\fi}}
\expandafter\gdef\csname R@an.xxloo.xl.paramsx\endcsname{0.68}
\expandafter\gdef\csname R@an.xxloo.xl.se_stock\endcsname{0.42}
\expandafter\gdef\csname R@an.xxloo.xl.se_xl\endcsname{\pend}
\expandafter\gdef\csname R@an.xxloo.xl.state\endcsname{complete}
\expandafter\gdef\csname R@an.xxloo.xl.stepx\endcsname{0.77}
\makeatother


==> results/numbers.tex <==
% AUTO-GENERATED by scripts/build_numbers.py -- do not edit by hand.
% manifest generated 2026-10-04 02:34:14 UTC; built 2026-10-10 11:45:51
\makeatletter
\expandafter\gdef\csname R@arm.L1.kits.h\endcsname{11.7}
\expandafter\gdef\csname R@arm.L1.kits.p\endcsname{0.063}
\expandafter\gdef\csname R@arm.L1.kits.t\endcsname{2.53}
\expandafter\gdef\csname R@arm.L1b.kits.h\endcsname{10.8}
\expandafter\gdef\csname R@arm.L1b.kits.p\endcsname{0.099}
\expandafter\gdef\csname R@arm.L1b.kits.t\endcsname{1.90}
\expandafter\gdef\csname R@arm.L2.kits.h\endcsname{11.6}
\expandafter\gdef\csname R@arm.L2.kits.p\endcsname{0.272}
\expandafter\gdef\csname R@arm.L2.kits.t\endcsname{0.72}
\expandafter\gdef\csname R@arm.L3.kits.h\endcsname{12.3}
\expandafter\gdef\csname R@arm.L3.kits.p\endcsname{0.045}
\expandafter\gdef\csname R@arm.L3.kits.t\endcsname{3.10}
\expandafter\gdef\csname R@arm.L4.kits.h\endcsname{11.5}
\expandafter\gdef\csname R@arm.L4.kits.p\endcsname{0.069}
\expandafter\gdef\csname R@arm.L4.kits.t\endcsname{2.39}
\expandafter\gdef\csname R@arm.L6.kits.h\endcsname{14.5}
\expandafter\gdef\csname R@arm.L6.kits.p\endcsname{0.055}
\expandafter\gdef\csname R@arm.L6.kits.t\endcsname{2.75}
\expandafter\gdef\csname R@arm.W1c.kits.h\endcsname{9.8}
\expandafter\gdef\csname R@arm.W1c.kits.p\endcsname{0.051}
\expandafter\gdef\csname R@arm.W1c.kits.t\endcsname{2.87}
\expandafter\gdef\csname R@arm.lead.h\endcsname{12.3}
\expandafter\gdef\csname R@arm.lead.h.ratio\endcsname{1.39}
\expandafter\gdef\csname R@arm.lead.kits.d\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@arm.lead.label\endcsname{L3}
\expandafter\gdef\csname R@arm.lead.name\endcsname{HyReX}
\expandafter\gdef\csname R@arm.lead.par\endcsname{29.6}
\expandafter\gdef\csname R@arm.lead.par.pctctrl\endcsname{29}
\expandafter\gdef\csname R@arm.lead.par.pctdef\endcsname{95}
\expandafter\gdef\csname R@arm.p.list\endcsname{0.045, 0.051, 0.055, 0.063, 0.069, 0.099, 0.272}
\expandafter\gdef\csname R@base.acdc.hours.max\endcsname{8.2}
\expandafter\gdef\csname R@base.acdc.hours.min\endcsname{8.1}
\expandafter\gdef\csname R@base.acdc.params\endcsname{30.38}
\expandafter\gdef\csname R@base.acdc.sd.fmt\endcsname{0.14}
\expandafter\gdef\csname R@base.acdc.vram\endcsname{10.23}
\expandafter\gdef\csname R@base.amos.hours.max\endcsname{28.0}
\expandafter\gdef\csname R@base.amos.hours.min\endcsname{17.8}
\expandafter\gdef\csname R@base.amos.params\endcsname{31.12}
\expandafter\gdef\csname R@base.amos.sd.fmt\endcsname{0.12}
\expandafter\gdef\csname R@base.amos.vram\endcsname{8.98}
\expandafter\gdef\csname R@base100.acdc.mean\endcsname{91.63}
\expandafter\gdef\csname R@base100.acdc.sd\endcsname{0.09}
\expandafter\gdef\csname R@base100.amos.mean\endcsname{77.76}
\expandafter\gdef\csname R@base100.amos.sd\endcsname{0.71}
\expandafter\gdef\csname R@base250.acdc.mean\endcsname{91.77}
\expandafter\gdef\csname R@base250.acdc.sd\endcsname{0.05}
\expandafter\gdef\csname R@base250.amos.mean\endcsname{84.61}
\expandafter\gdef\csname R@base250.amos.sd\endcsname{0.19}
\expandafter\gdef\csname R@base3.acdc.max\endcsname{92.13}
\expandafter\gdef\csname R@base3.acdc.mean\endcsname{92.00}
\expandafter\gdef\csname R@base3.acdc.min\endcsname{91.85}
\expandafter\gdef\csname R@base3.acdc.sd\endcsname{0.14}
\expandafter\gdef\csname R@base3.amos.max\endcsname{87.79}
\expandafter\gdef\csname R@base3.amos.mean\endcsname{87.67}
\expandafter\gdef\csname R@base3.amos.min\endcsname{87.55}
\expandafter\gdef\csname R@base3.amos.sd\endcsname{0.12}
\expandafter\gdef\csname R@base6.acdc.max\endcsname{92.13}
\expandafter\gdef\csname R@base6.acdc.mean\endcsname{92.01}
\expandafter\gdef\csname R@base6.acdc.min\endcsname{91.85}
\expandafter\gdef\csname R@base6.acdc.sd\endcsname{0.10}
\expandafter\gdef\csname R@base6.amos.max\endcsname{87.87}
\expandafter\gdef\csname R@base6.amos.mean\endcsname{87.70}
\expandafter\gdef\csname R@base6.amos.min\endcsname{87.55}
\expandafter\gdef\csname R@base6.amos.sd\endcsname{0.12}
\expandafter\gdef\csname R@budget.admissible\endcsname{nnU-Net ResEnc-M}
\expandafter\gdef\csname R@budget.admissible.vram\endcsname{9.10}
\expandafter\gdef\csname R@budget.over.resencl\endcsname{1.9}
\expandafter\gdef\csname R@budget.over.resencxl\endcsname{3.1}
\expandafter\gdef\csname R@cal.abs.base\endcsname{\ensuremath{-2.87}}
\expandafter\gdef\csname R@cal.abs.l1\endcsname{\ensuremath{-2.21}}
\expandafter\gdef\csname R@cal.amos.l1\endcsname{\ensuremath{+0.647}}
\expandafter\gdef\csname R@cal.amos.l1b\endcsname{\ensuremath{+0.138}}
\expandafter\gdef\csname R@cal.amos.near\endcsname{\ensuremath{+0.138}}
\expandafter\gdef\csname R@cal.amos.pub\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@cal.amos.spread\endcsname{0.509}
\expandafter\gdef\csname R@cal.kits.nse\endcsname{0.73}
\expandafter\gdef\csname R@cal.kits.ours\endcsname{\ensuremath{+2.33}}
\expandafter\gdef\csname R@cal.kits.ours3\endcsname{\ensuremath{+2.326}}
\expandafter\gdef\csname R@cal.kits.ratio\endcsname{1.40}
\expandafter\gdef\csname R@cal.kits.se\endcsname{0.92}
\expandafter\gdef\csname R@cal.l1l1b.ci\endcsname{4.84}
\expandafter\gdef\csname R@cal.l1l1b.d\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@cal.l1l1b.se\endcsname{1.12}
\expandafter\gdef\csname R@cal.nval.kits\endcsname{98}
\expandafter\gdef\csname R@cal.ours.base.h\endcsname{8.88}
\expandafter\gdef\csname R@cal.ours.base.h1\endcsname{8.9}
\expandafter\gdef\csname R@cal.ours.l1.h\endcsname{11.72}
\expandafter\gdef\csname R@cal.pub.base\endcsname{86.25}
\expandafter\gdef\csname R@cal.pub.base.h\endcsname{8.88}
\expandafter\gdef\csname R@cal.pub.base.vram\endcsname{6.9}
\expandafter\gdef\csname R@cal.pub.delta\endcsname{\ensuremath{+1.66}}
\expandafter\gdef\csname R@cal.pub.resencm\endcsname{87.91}
\expandafter\gdef\csname R@cal.pub.resencm.h\endcsname{11.39}
\expandafter\gdef\csname R@cal.pub.resencm.vram\endcsname{8.8}
\expandafter\gdef\csname R@cap.fit\endcsname{11.60}
\expandafter\gdef\csname R@cap.fithead.acdc\endcsname{1.33}
\expandafter\gdef\csname R@cap.fithead.amos\endcsname{2.59}
\expandafter\gdef\csname R@cap.fithead.kits\endcsname{3.09}
\expandafter\gdef\csname R@cap.fitres\endcsname{12.00}
\expandafter\gdef\csname R@cap.gb\endcsname{12}
\expandafter\gdef\csname R@cap.gib\endcsname{11.18}
\expandafter\gdef\csname R@cap.head.acdc\endcsname{1.73}
\expandafter\gdef\csname R@cap.head.amos\endcsname{2.99}
\expandafter\gdef\csname R@cap.head.kits\endcsname{3.49}
\expandafter\gdef\csname R@cap.peak.acdc\endcsname{10.27}
\expandafter\gdef\csname R@cap.peak.amos\endcsname{9.01}
\expandafter\gdef\csname R@cap.peak.kits\endcsname{8.51}
\expandafter\gdef\csname R@cls.amos.low1.name\endcsname{left adrenal gland}
\expandafter\gdef\csname R@cls.amos.low1.val\endcsname{76.17}
\expandafter\gdef\csname R@cls.amos.low2.name\endcsname{right adrenal gland}
\expandafter\gdef\csname R@cls.amos.low2.val\endcsname{76.58}
\expandafter\gdef\csname R@cls.amos.low3.name\endcsname{duodenum}
\expandafter\gdef\csname R@cls.amos.low3.val\endcsname{81.61}
\expandafter\gdef\csname R@cls.amos.low4.name\endcsname{prostate/uterus}
\expandafter\gdef\csname R@cls.amos.low4.val\endcsname{84.25}
\expandafter\gdef\csname R@cls.amos.lowmean\endcsname{82.60}
\expandafter\gdef\csname R@cls.amos.n\endcsname{15}
\expandafter\gdef\csname R@cls.amos.nsat\endcsname{4}
\expandafter\gdef\csname R@cls.amos.spd.maxabs\endcsname{1.06}
\expandafter\gdef\csname R@cls.amos.spd.nconsistent\endcsname{2}
\expandafter\gdef\csname R@cls.amos.spd.npos\endcsname{8}
\expandafter\gdef\csname R@cls.amos.top7mean\endcsname{93.47}
\expandafter\gdef\csname R@data.acdc.grouped\endcsname{patient}
\expandafter\gdef\csname R@data.acdc.ncases\endcsname{300}
\expandafter\gdef\csname R@data.acdc.nclasses\endcsname{3}
\expandafter\gdef\csname R@data.acdc.ndev\endcsname{200}
\expandafter\gdef\csname R@data.acdc.nfolds\endcsname{5}
\expandafter\gdef\csname R@data.acdc.ntest\endcsname{100}
\expandafter\gdef\csname R@data.acdc.ntrain\endcsname{160}
\expandafter\gdef\csname R@data.acdc.nval\endcsname{40}
\expandafter\gdef\csname R@data.amos.grouped\endcsname{case}
\expandafter\gdef\csname R@data.amos.ncases\endcsname{300}
\expandafter\gdef\csname R@data.amos.nclasses\endcsname{15}
\expandafter\gdef\csname R@data.amos.ndev\endcsname{200}
\expandafter\gdef\csname R@data.amos.nfolds\endcsname{5}
\expandafter\gdef\csname R@data.amos.ntest\endcsname{100}
\expandafter\gdef\csname R@data.amos.ntrain\endcsname{160}
\expandafter\gdef\csname R@data.amos.nval\endcsname{40}
\expandafter\gdef\csname R@ds.nout\endcsname{5}
\expandafter\gdef\csname R@ds.nsup\endcsname{4}
\expandafter\gdef\csname R@ds.w0\endcsname{53.3}
\expandafter\gdef\csname R@embargo.open\endcsname{open}
\expandafter\gdef\csname R@err.bin0\endcsname{1.67}
\expandafter\gdef\csname R@err.bin1\endcsname{1.07}
\expandafter\gdef\csname R@err.bin2\endcsname{3.39}
\expandafter\gdef\csname R@err.bin3\endcsname{3.19}
\expandafter\gdef\csname R@err.bin4\endcsname{3.02}
\expandafter\gdef\csname R@err.high\endcsname{6.21}
\expandafter\gdef\csname R@err.low\endcsname{2.73}
\expandafter\gdef\csname R@err.mid\endcsname{3.39}
\expandafter\gdef\csname R@err.need\endcsname{10}
\expandafter\gdef\csname R@err.nseeds\endcsname{3}
\expandafter\gdef\csname R@err.total\endcsname{12.33}
\expandafter\gdef\csname R@fp.ndes\endcsname{9}
\expandafter\gdef\csname R@fr.acdc.act2\endcsname{89.9}
\expandafter\gdef\csname R@fr.acdc.dec\endcsname{15.29}
\expandafter\gdef\csname R@fr.acdc.enc\endcsname{14.00}
\expandafter\gdef\csname R@fr.acdc.frpar\endcsname{37\,152}
\expandafter\gdef\csname R@fr.acdc.share\endcsname{0.122}
\expandafter\gdef\csname R@fr.acdc.tenmb\endcsname{294}
\expandafter\gdef\csname R@fr.amos.act2\endcsname{90.3}
\expandafter\gdef\csname R@fr.amos.dec\endcsname{15.29}
\expandafter\gdef\csname R@fr.amos.enc\endcsname{14.00}
\expandafter\gdef\csname R@fr.amos.frpar\endcsname{37\,152}
\expandafter\gdef\csname R@fr.amos.share\endcsname{0.119}
\expandafter\gdef\csname R@fr.amos.tenmb\endcsname{252}
\expandafter\gdef\csname R@fr.kits.act2\endcsname{93.9}
\expandafter\gdef\csname R@fr.kits.dec\endcsname{15.34}
\expandafter\gdef\csname R@fr.kits.enc\endcsname{14.02}
\expandafter\gdef\csname R@fr.kits.frpar\endcsname{111\,456}
\expandafter\gdef\csname R@fr.kits.share\endcsname{0.357}
\expandafter\gdef\csname R@fr.kits.tenmb\endcsname{268}
\expandafter\gdef\csname R@hand.control.acdc.d\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@hand.control.acdc.dice\endcsname{91.72}
\expandafter\gdef\csname R@hand.control.amos.d\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@hand.control.amos.dice\endcsname{84.78}
\expandafter\gdef\csname R@hand.control.params\endcsname{28.65}
\expandafter\gdef\csname R@hand.dense.acdc.d\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@hand.dense.acdc.dice\endcsname{91.74}
\expandafter\gdef\csname R@hand.dense.amos.d\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@hand.dense.amos.dice\endcsname{84.83}
\expandafter\gdef\csname R@hand.dense.params\endcsname{30.38}
\expandafter\gdef\csname R@hand.dynamic.acdc.d\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@hand.dynamic.acdc.dice\endcsname{91.54}
\expandafter\gdef\csname R@hand.dynamic.amos.d\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@hand.dynamic.amos.dice\endcsname{84.79}
\expandafter\gdef\csname R@hand.dynamic.params\endcsname{31.44}
\expandafter\gdef\csname R@hand.fine.acdc.d\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@hand.fine.acdc.dice\endcsname{91.55}
\expandafter\gdef\csname R@hand.fine.amos.d\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@hand.fine.amos.dice\endcsname{84.80}
\expandafter\gdef\csname R@hand.fine.params\endcsname{28.65}
\expandafter\gdef\csname R@hand.flatcontext.acdc.d\endcsname{\ensuremath{-2.12}}
\expandafter\gdef\csname R@hand.flatcontext.acdc.dice\endcsname{89.65}
\expandafter\gdef\csname R@hand.flatcontext.amos.d\endcsname{\ensuremath{-5.74}}
\expandafter\gdef\csname R@hand.flatcontext.amos.dice\endcsname{78.87}
\expandafter\gdef\csname R@hand.flatcontext.params\endcsname{1.96}
\expandafter\gdef\csname R@hand.flatlocal.acdc.d\endcsname{\ensuremath{-1.70}}
\expandafter\gdef\csname R@hand.flatlocal.acdc.dice\endcsname{90.07}
\expandafter\gdef\csname R@hand.flatlocal.amos.d\endcsname{\ensuremath{-4.56}}
\expandafter\gdef\csname R@hand.flatlocal.amos.dice\endcsname{80.05}
\expandafter\gdef\csname R@hand.flatlocal.params\endcsname{1.89}
\expandafter\gdef\csname R@hand.radius.acdc.d\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@hand.radius.acdc.dice\endcsname{91.83}
\expandafter\gdef\csname R@hand.radius.amos.d\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@hand.radius.amos.dice\endcsname{84.64}
\expandafter\gdef\csname R@hand.radius.params\endcsname{30.38}
\expandafter\gdef\csname R@hand.static.acdc.d\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@hand.static.acdc.dice\endcsname{91.75}
\expandafter\gdef\csname R@hand.static.amos.d\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@hand.static.amos.dice\endcsname{85.08}
\expandafter\gdef\csname R@hand.static.params\endcsname{31.44}
\expandafter\gdef\csname R@hand.uref.acdc.d\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@hand.uref.acdc.dice\endcsname{91.71}
\expandafter\gdef\csname R@hand.uref.amos.d\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@hand.uref.amos.dice\endcsname{84.69}
\expandafter\gdef\csname R@hand.uref.params\endcsname{44.98}
\expandafter\gdef\csname R@harness.iters\endcsname{250}
\expandafter\gdef\csname R@harness.iters.1000\endcsname{250\,k}
\expandafter\gdef\csname R@impl.L1.n6\endcsname{4}
\expandafter\gdef\csname R@impl.L1b.n6\endcsname{0}
\expandafter\gdef\csname R@impl.n\endcsname{15}
\expandafter\gdef\csname R@impl.r1.d\endcsname{\ensuremath{+2.45}}
\expandafter\gdef\csname R@impl.r1.name\endcsname{spleen}
\expandafter\gdef\csname R@impl.r1.z\endcsname{\ensuremath{+6.5}}
\expandafter\gdef\csname R@impl.r2.d\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@impl.r2.name\endcsname{postcava}
\expandafter\gdef\csname R@impl.r2.z\endcsname{\ensuremath{+4.5}}
\expandafter\gdef\csname R@impl.r3.d\endcsname{\ensuremath{+1.44}}
\expandafter\gdef\csname R@impl.r3.name\endcsname{bladder}
\expandafter\gdef\csname R@impl.r3.z\endcsname{\ensuremath{+4.3}}
\expandafter\gdef\csname R@impl.r4.d\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@impl.r4.name\endcsname{right adrenal gland}
\expandafter\gdef\csname R@impl.r4.z\endcsname{\ensuremath{+3.5}}
\expandafter\gdef\csname R@impl.rest.mean\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@impl.top4.share\endcsname{71}
\expandafter\gdef\csname R@impl.w5.thr\endcsname{0.67}
\expandafter\gdef\csname R@kid.max\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@lead.kits\endcsname{86.22}
\expandafter\gdef\csname R@lead.name\endcsname{HyReX}
\expandafter\gdef\csname R@lead.par.ratio\endcsname{3.5}
\expandafter\gdef\csname R@lead.vsref.clause\endcsname{HyReX reads \ensuremath{+0.516}\,pp from ResEnc-M (library preset) at seed 0 on KiTS23, 0.46 one-versus-one standard errors, inside one}
\expandafter\gdef\csname R@lead.vsref.d\endcsname{\ensuremath{+0.516}}
\expandafter\gdef\csname R@lead.vsref.nse\endcsname{0.46}
\expandafter\gdef\csname R@lead.vsref.read\endcsname{inside}
\expandafter\gdef\csname R@lead.vsrefmean.clause\endcsname{HyReX reads \ensuremath{-0.25}\,pp from the mean of the 3 finished seeds of ResEnc-M (library preset) at seed 0 on KiTS23, 0.27 one-versus-one standard errors, inside one}
\expandafter\gdef\csname R@lead.vsrefmean.d\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@lead.vsrefmean.inrange\endcsname{inside}
\expandafter\gdef\csname R@lead.vsrefmean.nse\endcsname{0.27}
\expandafter\gdef\csname R@lead.vsrefmean.read\endcsname{inside}
\expandafter\gdef\csname R@lead.vsrefmean.seed0gap\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@lit.mednextl3.acdc\endcsname{92.65}
\expandafter\gdef\csname R@lit.mednextl3.amos\endcsname{89.62}
\expandafter\gdef\csname R@lit.mednextl3.hours\endcsname{68}
\expandafter\gdef\csname R@lit.mednextl3.kits\endcsname{88.25}
\expandafter\gdef\csname R@lit.mednextl3.vram\endcsname{17.3}
\expandafter\gdef\csname R@lit.mednextl5.acdc\endcsname{92.62}
\expandafter\gdef\csname R@lit.mednextl5.amos\endcsname{89.73}
\expandafter\gdef\csname R@lit.mednextl5.hours\endcsname{233}
\expandafter\gdef\csname R@lit.mednextl5.kits\endcsname{87.74}
\expandafter\gdef\csname R@lit.mednextl5.vram\endcsname{18.0}
\expandafter\gdef\csname R@lit.nnformer.acdc\endcsname{92.40}
\expandafter\gdef\csname R@lit.nnformer.amos\endcsname{81.55}
\expandafter\gdef\csname R@lit.nnformer.hours\endcsname{8}
\expandafter\gdef\csname R@lit.nnformer.kits\endcsname{75.85}
\expandafter\gdef\csname R@lit.nnformer.vram\endcsname{5.7}
\expandafter\gdef\csname R@lit.nnunet.acdc\endcsname{91.54}
\expandafter\gdef\csname R@lit.nnunet.amos\endcsname{88.64}
\expandafter\gdef\csname R@lit.nnunet.hours\endcsname{9}
\expandafter\gdef\csname R@lit.nnunet.kits\endcsname{86.04}
\expandafter\gdef\csname R@lit.nnunet.vram\endcsname{7.7}
\expandafter\gdef\csname R@lit.resencl.acdc\endcsname{91.69}
\expandafter\gdef\csname R@lit.resencl.amos\endcsname{89.41}
\expandafter\gdef\csname R@lit.resencl.hours\endcsname{35}
\expandafter\gdef\csname R@lit.resencl.kits\endcsname{88.17}
\expandafter\gdef\csname R@lit.resencl.vram\endcsname{22.7}
\expandafter\gdef\csname R@lit.resencm.acdc\endcsname{91.99}
\expandafter\gdef\csname R@lit.resencm.amos\endcsname{88.77}
\expandafter\gdef\csname R@lit.resencm.gain.acdc\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@lit.resencm.gain.amos\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@lit.resencm.gain.kits\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@lit.resencm.hours\endcsname{12}
\expandafter\gdef\csname R@lit.resencm.kits\endcsname{86.79}
\expandafter\gdef\csname R@lit.resencm.vram\endcsname{9.1}
\expandafter\gdef\csname R@lit.resencm.vram.ratio\endcsname{1.18}
\expandafter\gdef\csname R@lit.resencxl.acdc\endcsname{91.48}
\expandafter\gdef\csname R@lit.resencxl.amos\endcsname{89.68}
\expandafter\gdef\csname R@lit.resencxl.hours\endcsname{66}
\expandafter\gdef\csname R@lit.resencxl.kits\endcsname{88.67}
\expandafter\gdef\csname R@lit.resencxl.vram\endcsname{36.6}
\expandafter\gdef\csname R@lit.span.acdc\endcsname{1.11}
\expandafter\gdef\csname R@lit.span.amos\endcsname{1.09}
\expandafter\gdef\csname R@lit.span.kits\endcsname{2.63}
\expandafter\gdef\csname R@lit.stunetl.acdc\endcsname{91.31}
\expandafter\gdef\csname R@lit.stunetl.amos\endcsname{89.34}
\expandafter\gdef\csname R@lit.stunetl.hours\endcsname{51}
\expandafter\gdef\csname R@lit.stunetl.kits\endcsname{85.84}
\expandafter\gdef\csname R@lit.stunetl.vram\endcsname{26.5}
\expandafter\gdef\csname R@lit.swinunetrv2.acdc\endcsname{92.01}
\expandafter\gdef\csname R@lit.swinunetrv2.amos\endcsname{86.24}
\expandafter\gdef\csname R@lit.swinunetrv2.hours\endcsname{15}
\expandafter\gdef\csname R@lit.swinunetrv2.kits\endcsname{84.14}
\expandafter\gdef\csname R@lit.swinunetrv2.vram\endcsname{13.4}
\expandafter\gdef\csname R@lit.umambabot.acdc\endcsname{91.79}
\expandafter\gdef\csname R@lit.umambabot.amos\endcsname{89.13}
\expandafter\gdef\csname R@lit.umambabot.hours\endcsname{24}
\expandafter\gdef\csname R@lit.umambabot.kits\endcsname{86.22}
\expandafter\gdef\csname R@lit.umambabot.vram\endcsname{12.4}
\expandafter\gdef\csname R@manifest.generated\endcsname{2026-10-04 02:34:14}
\expandafter\gdef\csname R@manifest.ntrials\endcsname{134}
\expandafter\gdef\csname R@metric.acdc.artefact\endcsname{0.00}
\expandafter\gdef\csname R@metric.acdc.artefact.sd\endcsname{0}
\expandafter\gdef\csname R@metric.amos.artefact\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@metric.amos.artefact.sd\endcsname{6}
\expandafter\gdef\csname R@metric.ncls\endcsname{15}
\expandafter\gdef\csname R@metric.pairweight\endcsname{0.17}
\expandafter\gdef\csname R@new.best.acdc.d\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@new.best.acdc.d3\endcsname{\pend{}}
\expandafter\gdef\csname R@new.best.acdc.sd3\endcsname{\pend{}}
\expandafter\gdef\csname R@new.best.amos.d\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@new.best.amos.d3\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@new.best.amos.sd3\endcsname{0.10}
\expandafter\gdef\csname R@new.best.ctrl.acdc.d\endcsname{\pend{}}
\expandafter\gdef\csname R@new.best.ctrl.amos.d\endcsname{\pend{}}
\expandafter\gdef\csname R@new.best.name\endcsname{ResEnc+context}
\expandafter\gdef\csname R@new.fired.kindsay\endcsname{4 are reference or control arms (ResEnc-M (library preset), ResEnc-matched (re-implemented), branch control and pooled-skip control) and 4 are mechanisms the agents designed}
\expandafter\gdef\csname R@new.fired.mechnames\endcsname{ConvNeXt-k3, HyReX, ResEnc+context, HyReX+context}
\expandafter\gdef\csname R@new.fired.names\endcsname{ResEnc-M (library preset) and ResEnc-matched (re-implemented) and ConvNeXt-k3 and HyReX and ResEnc+context and HyReX+context and branch control and pooled-skip control}
\expandafter\gdef\csname R@new.later.names\endcsname{C1\_deccap, D1\_pointfuse, D2\_dec1, I1\_L3pool, L3k3, L3ng, N1\_gnw16, P1\_frcap32, P1b\_kernel, P1c\_coarsecap, P3c, P3lite, S2\_s2next, V5A5, V5B1, V5B2, V6A1r, V7A1, V7A2, V7A3, V7B1, V7B2, V7C1, V7C2, V8A1, V8B1, V8B2}
\expandafter\gdef\csname R@new.nawaitrep\endcsname{1}
\expandafter\gdef\csname R@new.ncand\endcsname{7}
\expandafter\gdef\csname R@new.nctrl\endcsname{4}
\expandafter\gdef\csname R@new.ndecided\endcsname{13}
\expandafter\gdef\csname R@new.ndiffgate\endcsname{\pend[37 runs]}
\expandafter\gdef\csname R@new.ndone\endcsname{9}
\expandafter\gdef\csname R@new.nfired\endcsname{8}
\expandafter\gdef\csname R@new.nfired.amos\endcsname{6}
\expandafter\gdef\csname R@new.nfired.kits\endcsname{7}
\expandafter\gdef\csname R@new.nfired.mech\endcsname{4}
\expandafter\gdef\csname R@new.nlater\endcsname{27}
\expandafter\gdef\csname R@new.nmech\endcsname{7}
\expandafter\gdef\csname R@new.nmech.decided\endcsname{7}
\expandafter\gdef\csname R@new.npass\endcsname{5}
\expandafter\gdef\csname R@new.npass.amosonly\endcsname{4}
\expandafter\gdef\csname R@new.nreg\endcsname{13}
\expandafter\gdef\csname R@new.nreplicated\endcsname{6}
\expandafter\gdef\csname R@new.nreplicated.ctrl\endcsname{3}
\expandafter\gdef\csname R@new.nreplicated.mech\endcsname{3}
\expandafter\gdef\csname R@new.nrows\endcsname{13}
\expandafter\gdef\csname R@new.nscreened\endcsname{9}
\expandafter\gdef\csname R@new.nverd.pass\endcsname{6}
\expandafter\gdef\csname R@new.nverd.pass.cells\endcsname{5}
\expandafter\gdef\csname R@new.nverd.pass.ctrl\endcsname{1}
\expandafter\gdef\csname R@new.nverd.pass.kindsay\endcsname{6 arm(s), of which 4 agent-designed: this sentence must be rewritten by a human}
\expandafter\gdef\csname R@new.nverd.pass.mech\endcsname{4}
\expandafter\gdef\csname R@new.nverd.pass.names\endcsname{ResEnc-M (library preset) and ResEnc-matched (re-implemented) and ConvNeXt-k3 and HyReX and ResEnc+context and HyReX+context}
\expandafter\gdef\csname R@new.nverd.pending\endcsname{7}
\expandafter\gdef\csname R@new.nwaves\endcsname{2}
\expandafter\gdef\csname R@nnunet.version\endcsname{2.8.1}
\expandafter\gdef\csname R@noise.acdc.2se\endcsname{0.32}
\expandafter\gdef\csname R@noise.acdc.frac\endcsname{36}
\expandafter\gdef\csname R@noise.acdc.npair\endcsname{3}
\expandafter\gdef\csname R@noise.acdc.total\endcsname{0.10}
\expandafter\gdef\csname R@noise.acdc.within\endcsname{0.06}
\expandafter\gdef\csname R@noise.amos.2se\endcsname{0.28}
\expandafter\gdef\csname R@noise.amos.frac\endcsname{51}
\expandafter\gdef\csname R@noise.amos.npair\endcsname{3}
\expandafter\gdef\csname R@noise.amos.total\endcsname{0.12}
\expandafter\gdef\csname R@noise.amos.within\endcsname{0.09}
\expandafter\gdef\csname R@op.axial_dw7.s1\endcsname{26.2}
\expandafter\gdef\csname R@op.axial_dw7.s2\endcsname{6.8}
\expandafter\gdef\csname R@op.axial_dw7.s3\endcsname{1.7}
\expandafter\gdef\csname R@op.axial_dw7.s4\endcsname{0.5}
\expandafter\gdef\csname R@op.bottleneck_r4.s1\endcsname{8.2}
\expandafter\gdef\csname R@op.bottleneck_r4.s2\endcsname{1.7}
\expandafter\gdef\csname R@op.bottleneck_r4.s3\endcsname{1.2}
\expandafter\gdef\csname R@op.bottleneck_r4.s4\endcsname{1.1}
\expandafter\gdef\csname R@op.convnext_k3_e2.s1\endcsname{19.9}
\expandafter\gdef\csname R@op.convnext_k3_e2.s2\endcsname{5.1}
\expandafter\gdef\csname R@op.convnext_k3_e2.s3\endcsname{1.4}
\expandafter\gdef\csname R@op.convnext_k3_e2.s4\endcsname{0.8}
\expandafter\gdef\csname R@op.convnext_k5_e2.s1\endcsname{68.6}
\expandafter\gdef\csname R@op.convnext_k5_e2.s2\endcsname{17.4}
\expandafter\gdef\csname R@op.convnext_k5_e2.s3\endcsname{4.6}
\expandafter\gdef\csname R@op.convnext_k5_e2.s4\endcsname{1.2}
\expandafter\gdef\csname R@op.cross.axial_dw7\endcsname{no stage}
\expandafter\gdef\csname R@op.cross.bottleneck_r4\endcsname{s2}
\expandafter\gdef\csname R@op.cross.convnext_k3_e2\endcsname{no stage}
\expandafter\gdef\csname R@op.cross.convnext_k5_e2\endcsname{no stage}
\expandafter\gdef\csname R@op.cross.dense3x3x3\endcsname{s1}
\expandafter\gdef\csname R@op.cross.dilated3x3x3_d2\endcsname{s1}
\expandafter\gdef\csname R@op.cross.dw3\endcsname{s3}
\expandafter\gdef\csname R@op.cross.dw5\endcsname{no stage}
\expandafter\gdef\csname R@op.cross.dw7\endcsname{no stage}
\expandafter\gdef\csname R@op.cross.grouped3x3x3_g8\endcsname{s2}
\expandafter\gdef\csname R@op.crossfine.axial_dw7\endcsname{s3}
\expandafter\gdef\csname R@op.crossfine.bottleneck_r4\endcsname{s2}
\expandafter\gdef\csname R@op.crossfine.convnext_k3_e2\endcsname{s2}
\expandafter\gdef\csname R@op.crossfine.convnext_k5_e2\endcsname{s3}
\expandafter\gdef\csname R@op.crossfine.dense3x3x3\endcsname{s1}
\expandafter\gdef\csname R@op.crossfine.dilated3x3x3_d2\endcsname{s1}
\expandafter\gdef\csname R@op.crossfine.dw3\endcsname{s2}
\expandafter\gdef\csname R@op.crossfine.dw5\endcsname{s3}
\expandafter\gdef\csname R@op.crossfine.dw7\endcsname{s4}
\expandafter\gdef\csname R@op.crossfine.grouped3x3x3_g8\endcsname{s2}
\expandafter\gdef\csname R@op.dense3x3x3.s1\endcsname{6.3}
\expandafter\gdef\csname R@op.dense3x3x3.s2\endcsname{2.0}
\expandafter\gdef\csname R@op.dense3x3x3.s3\endcsname{0.9}
\expandafter\gdef\csname R@op.dense3x3x3.s4\endcsname{0.4}
\expandafter\gdef\csname R@op.device\endcsname{NVIDIA A100-SXM4-80GB}
\expandafter\gdef\csname R@op.dilated.s1\endcsname{5.7}
\expandafter\gdef\csname R@op.dilated3x3x3_d2.s1\endcsname{5.7}
\expandafter\gdef\csname R@op.dilated3x3x3_d2.s2\endcsname{1.9}
\expandafter\gdef\csname R@op.dilated3x3x3_d2.s3\endcsname{0.9}
\expandafter\gdef\csname R@op.dilated3x3x3_d2.s4\endcsname{0.4}
\expandafter\gdef\csname R@op.dw3.s1\endcsname{10.7}
\expandafter\gdef\csname R@op.dw3.s2\endcsname{2.9}
\expandafter\gdef\csname R@op.dw3.s3\endcsname{0.8}
\expandafter\gdef\csname R@op.dw3.s4\endcsname{0.3}
\expandafter\gdef\csname R@op.dw5.s1\endcsname{59.4}
\expandafter\gdef\csname R@op.dw5.s2\endcsname{15.1}
\expandafter\gdef\csname R@op.dw5.s3\endcsname{4.0}
\expandafter\gdef\csname R@op.dw5.s4\endcsname{0.9}
\expandafter\gdef\csname R@op.dw7.s1\endcsname{143.9}
\expandafter\gdef\csname R@op.dw7.s2\endcsname{36.6}
\expandafter\gdef\csname R@op.dw7.s3\endcsname{9.6}
\expandafter\gdef\csname R@op.dw7.s4\endcsname{2.0}
\expandafter\gdef\csname R@op.grouped3x3x3_g8.s1\endcsname{6.3}
\expandafter\gdef\csname R@op.grouped3x3x3_g8.s2\endcsname{1.7}
\expandafter\gdef\csname R@op.grouped3x3x3_g8.s3\endcsname{0.4}
\expandafter\gdef\csname R@op.grouped3x3x3_g8.s4\endcsname{0.3}
\expandafter\gdef\csname R@op.nbench\endcsname{13}
\expandafter\gdef\csname R@op.ncross\endcsname{5}
\expandafter\gdef\csname R@op.ncross.other\endcsname{4}
\expandafter\gdef\csname R@op.nother\endcsname{9}
\expandafter\gdef\csname R@op.notshown\endcsname{dense3x3x3\_IN\_lrelu, axial\_dw13, pw\_1x1\_c\_to\_2c}
\expandafter\gdef\csname R@op.nshown\endcsname{10}
\expandafter\gdef\csname R@op.ratio.cnx5.dense.s1\endcsname{11}
\expandafter\gdef\csname R@op.ratio.cnx5.s1.s3\endcsname{15}
\expandafter\gdef\csname R@op.ratio.cnx5.s1.s4\endcsname{57}
\expandafter\gdef\csname R@op.ratio.dw5.dense.s1\endcsname{9}
\expandafter\gdef\csname R@op.ratio.dw7.dense.s1\endcsname{23}
\expandafter\gdef\csname R@op.rel.axial_dw7.s1\endcsname{4.17}
\expandafter\gdef\csname R@op.rel.axial_dw7.s2\endcsname{3.46}
\expandafter\gdef\csname R@op.rel.axial_dw7.s3\endcsname{1.78}
\expandafter\gdef\csname R@op.rel.axial_dw7.s4\endcsname{1.32}
\expandafter\gdef\csname R@op.rel.bottleneck_r4.s1\endcsname{1.31}
\expandafter\gdef\csname R@op.rel.bottleneck_r4.s2\endcsname{0.87}
\expandafter\gdef\csname R@op.rel.bottleneck_r4.s3\endcsname{1.33}
\expandafter\gdef\csname R@op.rel.bottleneck_r4.s4\endcsname{2.92}
\expandafter\gdef\csname R@op.rel.convnext_k3_e2.s1\endcsname{3.17}
\expandafter\gdef\csname R@op.rel.convnext_k3_e2.s2\endcsname{2.59}
\expandafter\gdef\csname R@op.rel.convnext_k3_e2.s3\endcsname{1.48}
\expandafter\gdef\csname R@op.rel.convnext_k3_e2.s4\endcsname{2.21}
\expandafter\gdef\csname R@op.rel.convnext_k5_e2.s1\endcsname{10.94}
\expandafter\gdef\csname R@op.rel.convnext_k5_e2.s2\endcsname{8.83}
\expandafter\gdef\csname R@op.rel.convnext_k5_e2.s3\endcsname{4.92}
\expandafter\gdef\csname R@op.rel.convnext_k5_e2.s4\endcsname{3.18}
\expandafter\gdef\csname R@op.rel.dense3x3x3.s1\endcsname{1.00}
\expandafter\gdef\csname R@op.rel.dense3x3x3.s2\endcsname{1.00}
\expandafter\gdef\csname R@op.rel.dense3x3x3.s3\endcsname{1.00}
\expandafter\gdef\csname R@op.rel.dense3x3x3.s4\endcsname{1.00}
\expandafter\gdef\csname R@op.rel.dilated3x3x3_d2.s1\endcsname{0.91}
\expandafter\gdef\csname R@op.rel.dilated3x3x3_d2.s2\endcsname{0.99}
\expandafter\gdef\csname R@op.rel.dilated3x3x3_d2.s3\endcsname{0.99}
\expandafter\gdef\csname R@op.rel.dilated3x3x3_d2.s4\endcsname{0.95}
\expandafter\gdef\csname R@op.rel.dw3.s1\endcsname{1.70}
\expandafter\gdef\csname R@op.rel.dw3.s2\endcsname{1.45}
\expandafter\gdef\csname R@op.rel.dw3.s3\endcsname{0.81}
\expandafter\gdef\csname R@op.rel.dw3.s4\endcsname{0.68}
\expandafter\gdef\csname R@op.rel.dw5.s1\endcsname{9.48}
\expandafter\gdef\csname R@op.rel.dw5.s2\endcsname{7.69}
\expandafter\gdef\csname R@op.rel.dw5.s3\endcsname{4.25}
\expandafter\gdef\csname R@op.rel.dw5.s4\endcsname{2.42}
\expandafter\gdef\csname R@op.rel.dw7.s1\endcsname{22.95}
\expandafter\gdef\csname R@op.rel.dw7.s2\endcsname{18.59}
\expandafter\gdef\csname R@op.rel.dw7.s3\endcsname{10.31}
\expandafter\gdef\csname R@op.rel.dw7.s4\endcsname{5.21}
\expandafter\gdef\csname R@op.rel.grouped3x3x3_g8.s1\endcsname{1.01}
\expandafter\gdef\csname R@op.rel.grouped3x3x3_g8.s2\endcsname{0.86}
\expandafter\gdef\csname R@op.rel.grouped3x3x3_g8.s3\endcsname{0.47}
\expandafter\gdef\csname R@op.rel.grouped3x3x3_g8.s4\endcsname{0.92}
\expandafter\gdef\csname R@op.span.axial_dw7\endcsname{52}
\expandafter\gdef\csname R@op.span.bottleneck_r4\endcsname{7}
\expandafter\gdef\csname R@op.span.convnext_k3_e2\endcsname{24}
\expandafter\gdef\csname R@op.span.convnext_k5_e2\endcsname{57}
\expandafter\gdef\csname R@op.span.dense3x3x3\endcsname{16}
\expandafter\gdef\csname R@op.span.dilated3x3x3_d2\endcsname{16}
\expandafter\gdef\csname R@op.span.dw3\endcsname{41}
\expandafter\gdef\csname R@op.span.dw5\endcsname{65}
\expandafter\gdef\csname R@op.span.dw7\endcsname{73}
\expandafter\gdef\csname R@op.span.grouped3x3x3_g8\endcsname{18}
\expandafter\gdef\csname R@op.stagehead\endcsname{64\,ch, $64{\times}96{\times}80$ & 128\,ch, $32{\times}48{\times}40$ & 256\,ch, $16{\times}24{\times}20$ & 320\,ch, $8{\times}12{\times}10$}
\expandafter\gdef\csname R@op.stagelist\endcsname{64\,ch, $64{\times}96{\times}80$; 128\,ch, $32{\times}48{\times}40$; 256\,ch, $16{\times}24{\times}20$; 320\,ch, $8{\times}12{\times}10$}
\expandafter\gdef\csname R@op.torch\endcsname{2.13.0+cu130}
\expandafter\gdef\csname R@pair.floor\endcsname{0.50}
\expandafter\gdef\csname R@pair.lead.L1.d\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@pair.lead.L1.nse\endcsname{0.46}
\expandafter\gdef\csname R@pair.lead.L1b.d\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@pair.lead.L1b.nse\endcsname{0.98}
\expandafter\gdef\csname R@pair.lead.L2.d\endcsname{\ensuremath{+2.18}}
\expandafter\gdef\csname R@pair.lead.L2.nse\endcsname{1.94}
\expandafter\gdef\csname R@pair.lead.L4.d\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@pair.lead.L4.nse\endcsname{0.57}
\expandafter\gdef\csname R@pair.lead.L6.d\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@pair.lead.L6.nse\endcsname{0.28}
\expandafter\gdef\csname R@pair.lead.W1c.d\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@pair.lead.W1c.nse\endcsname{0.18}
\expandafter\gdef\csname R@pair.se.hi\endcsname{0.34}
\expandafter\gdef\csname R@pair.se.lo\endcsname{0.17}
\expandafter\gdef\csname R@pair.se1v1\endcsname{1.12}
\expandafter\gdef\csname R@pairamos.clause\endcsname{Of the 5 registered pair contrasts decided on AMOS22, one reaches the 0.50\,pp floor, the contrast between ResEnc-M (library preset) and ResEnc-matched (re-implemented): \ensuremath{+0.509}\,pp, 2.9 one-versus-one standard errors}
\expandafter\gdef\csname R@pairamos.impl.d\endcsname{\ensuremath{+0.509}}
\expandafter\gdef\csname R@pairamos.impl.nse\endcsname{2.9}
\expandafter\gdef\csname R@pairamos.impl.rank\endcsname{1}
\expandafter\gdef\csname R@pairamos.max.a\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@pairamos.max.b\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@pairamos.max.d\endcsname{\ensuremath{+0.509}}
\expandafter\gdef\csname R@pairamos.max.nse\endcsname{2.9}
\expandafter\gdef\csname R@pairamos.max.pair\endcsname{L1 $-$ L1b}
\expandafter\gdef\csname R@pairamos.max.par.a\endcsname{102.3}
\expandafter\gdef\csname R@pairamos.max.par.b\endcsname{102.4}
\expandafter\gdef\csname R@pairamos.mech.cap\endcsname{every measured mechanism pair reads inside its control's registered standard on AMOS22 (0 of 4 clear the AMOS22 floor)}
\expandafter\gdef\csname R@pairamos.mech.clause\endcsname{Of the 4 mechanism pairs the largest is 0.453\,pp and none clears the floor}
\expandafter\gdef\csname R@pairamos.mech.head\endcsname{every registered mechanism pair reads inside the one-seed floor of its control}
\expandafter\gdef\csname R@pairamos.mech.maxabs\endcsname{0.453}
\expandafter\gdef\csname R@pairamos.mech.n\endcsname{4}
\expandafter\gdef\csname R@pairamos.mech.nabove\endcsname{0}
\expandafter\gdef\csname R@pairamos.nabove\endcsname{1}
\expandafter\gdef\csname R@pairamos.ndecided\endcsname{5}
\expandafter\gdef\csname R@pairamos.se\endcsname{0.173}
\expandafter\gdef\csname R@pc.L1.max\endcsname{9.7}
\expandafter\gdef\csname R@pc.L1.n4\endcsname{4}
\expandafter\gdef\csname R@pc.L1.n6\endcsname{4}
\expandafter\gdef\csname R@pc.L1.top.d\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@pc.L1.top.name\endcsname{spleen}
\expandafter\gdef\csname R@pc.L1.top.nsd\endcsname{9.7}
\expandafter\gdef\csname R@pc.L1.topraw.d\endcsname{\ensuremath{+2.60}}
\expandafter\gdef\csname R@pc.L1.topraw.name\endcsname{spleen}
\expandafter\gdef\csname R@pc.L1.topraw.nsd\endcsname{9.7}
\expandafter\gdef\csname R@pc.L2.max\endcsname{4.3}
\expandafter\gdef\csname R@pc.L2.n4\endcsname{1}
\expandafter\gdef\csname R@pc.L2.n6\endcsname{0}
\expandafter\gdef\csname R@pc.L2.top.d\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@pc.L2.top.name\endcsname{right adrenal gland}
\expandafter\gdef\csname R@pc.L2.top.nsd\endcsname{4.3}
\expandafter\gdef\csname R@pc.L2.topraw.d\endcsname{\ensuremath{+1.21}}
\expandafter\gdef\csname R@pc.L2.topraw.name\endcsname{left adrenal gland}
\expandafter\gdef\csname R@pc.L2.topraw.nsd\endcsname{1.4}
\expandafter\gdef\csname R@pc.L3.max\endcsname{4.2}
\expandafter\gdef\csname R@pc.L3.n4\endcsname{1}
\expandafter\gdef\csname R@pc.L3.n6\endcsname{0}
\expandafter\gdef\csname R@pc.L3.top.d\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@pc.L3.top.name\endcsname{postcava}
\expandafter\gdef\csname R@pc.L3.top.nsd\endcsname{4.2}
\expandafter\gdef\csname R@pc.L3.topraw.d\endcsname{\ensuremath{+1.73}}
\expandafter\gdef\csname R@pc.L3.topraw.name\endcsname{gall bladder}
\expandafter\gdef\csname R@pc.L3.topraw.nsd\endcsname{1.4}
\expandafter\gdef\csname R@pc.arms\endcsname{ResEnc-M (library preset), ConvNeXt-k3, HyReX}
\expandafter\gdef\csname R@pc.n\endcsname{6}
\expandafter\gdef\csname R@pc.ncls\endcsname{15}
\expandafter\gdef\csname R@pc.sd.max\endcsname{1.229}
\expandafter\gdef\csname R@pc.sd.maxname\endcsname{gall bladder}
\expandafter\gdef\csname R@pc.sd.min\endcsname{0.107}
\expandafter\gdef\csname R@pc.sd.minname\endcsname{aorta}
\expandafter\gdef\csname R@pc.sd.ratio\endcsname{11.5}
\expandafter\gdef\csname R@plan.acdc.batch\endcsname{4}
\expandafter\gdef\csname R@plan.acdc.nconv\endcsname{2}
\expandafter\gdef\csname R@plan.acdc.nstages\endcsname{6}
\expandafter\gdef\csname R@plan.acdc.patch\endcsname{$20{\times}256{\times}224$}
\expandafter\gdef\csname R@plan.acdc.spacing\endcsname{$5{\times}1.52{\times}1.52$\,mm}
\expandafter\gdef\csname R@plan.acdc.widths\endcsname{32, 64, 128, 256, 320, 320}
\expandafter\gdef\csname R@plan.amos.batch\endcsname{2}
\expandafter\gdef\csname R@plan.amos.nconv\endcsname{2}
\expandafter\gdef\csname R@plan.amos.nstages\endcsname{6}
\expandafter\gdef\csname R@plan.amos.patch\endcsname{$64{\times}192{\times}160$}
\expandafter\gdef\csname R@plan.amos.spacing\endcsname{$2{\times}0.68{\times}0.68$\,mm}
\expandafter\gdef\csname R@plan.amos.widths\endcsname{32, 64, 128, 256, 320, 320}
\expandafter\gdef\csname R@prec.bound.hi\endcsname{0.50}
\expandafter\gdef\csname R@prec.bound.lo\endcsname{0.27}
\expandafter\gdef\csname R@prec.nbase\endcsname{3}
\expandafter\gdef\csname R@prec.sd.base\endcsname{0.12}
\expandafter\gdef\csname R@prec.sd.worst\endcsname{0.24}
\expandafter\gdef\csname R@prec.se.hi\endcsname{0.25}
\expandafter\gdef\csname R@prec.se.lo\endcsname{0.14}
\expandafter\gdef\csname R@prof.base.mem\endcsname{9.0}
\expandafter\gdef\csname R@prof.base.ms\endcsname{140.4}
\expandafter\gdef\csname R@prof.w1.n\endcsname{6}
\expandafter\gdef\csname R@prof.w1.step.max\endcsname{1.88}
\expandafter\gdef\csname R@prof.w1.step.min\endcsname{1.38}
\expandafter\gdef\csname R@pw.acdc.barsd\endcsname{\ensuremath{-1.40}}
\expandafter\gdef\csname R@pw.acdc.mean\endcsname{92.009}
\expandafter\gdef\csname R@pw.acdc.n\endcsname{6}
\expandafter\gdef\csname R@pw.acdc.nseed\endcsname{3}
\expandafter\gdef\csname R@pw.acdc.sd\endcsname{0.099}
\expandafter\gdef\csname R@pw.acdc.se\endcsname{0.107}
\expandafter\gdef\csname R@pw.acdc.se.cl\endcsname{0.114}
\expandafter\gdef\csname R@pw.acdc.seunder\endcsname{40}
\expandafter\gdef\csname R@pw.acdc.trip\endcsname{11.0}
\expandafter\gdef\csname R@pw.acdc.trip.chi\endcsname{15.9}
\expandafter\gdef\csname R@pw.acdc.trip.clo\endcsname{12.2}
\expandafter\gdef\csname R@pw.amos.barsd\endcsname{\ensuremath{+2.65}}
\expandafter\gdef\csname R@pw.amos.mean\endcsname{87.701}
\expandafter\gdef\csname R@pw.amos.n\endcsname{6}
\expandafter\gdef\csname R@pw.amos.nseed\endcsname{3}
\expandafter\gdef\csname R@pw.amos.repbar\endcsname{3.51}
\expandafter\gdef\csname R@pw.amos.reptrip\endcsname{0.9}
\expandafter\gdef\csname R@pw.amos.sd\endcsname{0.122}
\expandafter\gdef\csname R@pw.amos.se\endcsname{0.132}
\expandafter\gdef\csname R@pw.amos.se.cl\endcsname{0.139}
\expandafter\gdef\csname R@pw.amos.seunder\endcsname{32}
\expandafter\gdef\csname R@pw.amos.trip\endcsname{2.3}
\expandafter\gdef\csname R@pw.amos.trip.chi\endcsname{6.4}
\expandafter\gdef\csname R@pw.amos.trip.clo\endcsname{2.6}
\expandafter\gdef\csname R@pw.kits.barsd\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@pw.kits.df\endcsname{2}
\expandafter\gdef\csname R@pw.kits.mean\endcsname{83.378}
\expandafter\gdef\csname R@pw.kits.n\endcsname{3}
\expandafter\gdef\csname R@pw.kits.nseed\endcsname{3}
\expandafter\gdef\csname R@pw.kits.repbar\endcsname{0.48}
\expandafter\gdef\csname R@pw.kits.reptrip\endcsname{33.9}
\expandafter\gdef\csname R@pw.kits.screenrep\endcsname{12.5}
\expandafter\gdef\csname R@pw.kits.sd\endcsname{0.795}
\expandafter\gdef\csname R@pw.kits.sd.hi\endcsname{5.00}
\expandafter\gdef\csname R@pw.kits.sd.lo\endcsname{0.41}
\expandafter\gdef\csname R@pw.kits.se\endcsname{0.918}
\expandafter\gdef\csname R@pw.kits.trip\endcsname{37.0}
\expandafter\gdef\csname R@pw.kits.trip.hi\endcsname{48}
\expandafter\gdef\csname R@pw.kits.trip.lo\endcsname{27}
\expandafter\gdef\csname R@pw.nreg\endcsname{13}
\expandafter\gdef\csname R@pw.null.amos\endcsname{1.1}
\expandafter\gdef\csname R@pw.null.amos.exp\endcsname{0.1}
\expandafter\gdef\csname R@pw.null.kits\endcsname{27.9}
\expandafter\gdef\csname R@pw.null.kits.exp\endcsname{3.6}
\expandafter\gdef\csname R@pw.ratio\endcsname{16}
\expandafter\gdef\csname R@rank.both.par.amos.rho\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@rank.n\endcsname{7}
\expandafter\gdef\csname R@rank.p\endcsname{0.70}
\expandafter\gdef\csname R@rank.par.amos.p\endcsname{0.48}
\expandafter\gdef\csname R@rank.par.kits.p\endcsname{0.70}
\expandafter\gdef\csname R@rank.par.kits.rho\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@rank.rho\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@recipe.acdc.ci1k.frozen\endcsname{0.21}
\expandafter\gdef\csname R@recipe.acdc.ci1k.gap\endcsname{0.11}
\expandafter\gdef\csname R@recipe.acdc.ci1k.study\endcsname{0.31}
\expandafter\gdef\csname R@recipe.acdc.e100.ci95\endcsname{0.13}
\expandafter\gdef\csname R@recipe.acdc.e100.max\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@recipe.acdc.e100.mean\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@recipe.acdc.e100.min\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@recipe.acdc.e100.ninside\endcsname{2}
\expandafter\gdef\csname R@recipe.acdc.e100.npool\endcsname{5}
\expandafter\gdef\csname R@recipe.acdc.e100.npos\endcsname{11}
\expandafter\gdef\csname R@recipe.acdc.e1000.max\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@recipe.acdc.e1000.mean\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@recipe.acdc.e1000.min\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@recipe.acdc.n\endcsname{11}
\expandafter\gdef\csname R@recipe.acdc.nabove1sd\endcsname{3}
\expandafter\gdef\csname R@recipe.acdc.nge035\endcsname{0}
\expandafter\gdef\csname R@recipe.acdc.npos\endcsname{8}
\expandafter\gdef\csname R@recipe.acdc.refn\endcsname{3}
\expandafter\gdef\csname R@recipe.acdc.refshift\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@recipe.acdc.spearman\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@recipe.amos.ci1k.frozen\endcsname{0.26}
\expandafter\gdef\csname R@recipe.amos.ci1k.gap\endcsname{0.01}
\expandafter\gdef\csname R@recipe.amos.ci1k.study\endcsname{0.27}
\expandafter\gdef\csname R@recipe.amos.e100.ci95\endcsname{1.02}
\expandafter\gdef\csname R@recipe.amos.e100.max\endcsname{\ensuremath{+1.64}}
\expandafter\gdef\csname R@recipe.amos.e100.mean\endcsname{\ensuremath{+1.32}}
\expandafter\gdef\csname R@recipe.amos.e100.min\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@recipe.amos.e100.ninside\endcsname{1}
\expandafter\gdef\csname R@recipe.amos.e100.npool\endcsname{5}
\expandafter\gdef\csname R@recipe.amos.e100.npos\endcsname{6}
\expandafter\gdef\csname R@recipe.amos.e1000.max\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@recipe.amos.e1000.mean\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@recipe.amos.e1000.min\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@recipe.amos.n\endcsname{6}
\expandafter\gdef\csname R@recipe.amos.nabove1sd\endcsname{1}
\expandafter\gdef\csname R@recipe.amos.nge035\endcsname{0}
\expandafter\gdef\csname R@recipe.amos.npos\endcsname{1}
\expandafter\gdef\csname R@recipe.amos.refn\endcsname{3}
\expandafter\gdef\csname R@recipe.amos.refshift\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@recipe.amos.spearman\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@recipe.n.both\endcsname{17}
\expandafter\gdef\csname R@recipe.ncand\endcsname{11}
\expandafter\gdef\csname R@ref.acdc.uncompiled.mean\endcsname{92.02}
\expandafter\gdef\csname R@ref.acdc.uncompiled.n\endcsname{3}
\expandafter\gdef\csname R@ref.acdc.uncompiled.shift\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@ref.amos.contemporaneous.mean\endcsname{87.71}
\expandafter\gdef\csname R@ref.amos.contemporaneous.n\endcsname{3}
\expandafter\gdef\csname R@ref.amos.contemporaneous.shift\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@ref.amos.uncompiled.mean\endcsname{87.73}
\expandafter\gdef\csname R@ref.amos.uncompiled.n\endcsname{3}
\expandafter\gdef\csname R@ref.amos.uncompiled.shift\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@ref.kits\endcsname{85.70}
\expandafter\gdef\csname R@ref.kits.contemporaneous.mean\endcsname{83.87}
\expandafter\gdef\csname R@ref.kits.contemporaneous.n\endcsname{3}
\expandafter\gdef\csname R@ref.kits.contemporaneous.shift\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@ref.kits.max\endcsname{87.20}
\expandafter\gdef\csname R@ref.kits.mean\endcsname{86.47}
\expandafter\gdef\csname R@ref.kits.min\endcsname{85.70}
\expandafter\gdef\csname R@ref.kits.n\endcsname{3}
\expandafter\gdef\csname R@ref.kits.sd\endcsname{0.75}
\expandafter\gdef\csname R@rep.L1.d\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@rep.L1.disc\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@rep.L1.ds\endcsname{AMOS}
\expandafter\gdef\csname R@rep.L1.gap\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@rep.L1.z\endcsname{4.66}
\expandafter\gdef\csname R@rep.L1b.d\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@rep.L1b.disc\endcsname{\ensuremath{+1.74}}
\expandafter\gdef\csname R@rep.L1b.ds\endcsname{KiTS23}
\expandafter\gdef\csname R@rep.L1b.gap\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@rep.L1b.z\endcsname{3.19}
\expandafter\gdef\csname R@rep.L2.d\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.L2.disc\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.L2.ds\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.L2.gap\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.L2.z\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.L3.d\endcsname{\ensuremath{+2.09}}
\expandafter\gdef\csname R@rep.L3.disc\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@rep.L3.ds\endcsname{KiTS23}
\expandafter\gdef\csname R@rep.L3.gap\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@rep.L3.z\endcsname{2.89}
\expandafter\gdef\csname R@rep.L4.d\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@rep.L4.disc\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@rep.L4.ds\endcsname{AMOS}
\expandafter\gdef\csname R@rep.L4.gap\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@rep.L4.z\endcsname{4.56}
\expandafter\gdef\csname R@rep.L6.d\endcsname{\ensuremath{+1.59}}
\expandafter\gdef\csname R@rep.L6.disc\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@rep.L6.ds\endcsname{KiTS23}
\expandafter\gdef\csname R@rep.L6.gap\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@rep.L6.z\endcsname{2.19}
\expandafter\gdef\csname R@rep.W1.d\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W1.disc\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W1.ds\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W1.gap\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W1.z\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W1c.d\endcsname{\ensuremath{+1.07}}
\expandafter\gdef\csname R@rep.W1c.disc\endcsname{\ensuremath{+2.64}}
\expandafter\gdef\csname R@rep.W1c.ds\endcsname{KiTS23}
\expandafter\gdef\csname R@rep.W1c.gap\endcsname{\ensuremath{+1.57}}
\expandafter\gdef\csname R@rep.W1c.z\endcsname{1.47}
\expandafter\gdef\csname R@rep.W2.d\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W2.disc\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W2.ds\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W2.gap\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W2.z\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W3.d\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W3.disc\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W3.ds\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W3.gap\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W3.z\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W3c.d\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W3c.disc\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W3c.ds\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W3c.gap\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W3c.z\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W4.d\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W4.disc\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W4.ds\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W4.gap\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W4.z\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W5.d\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W5.disc\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W5.ds\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W5.gap\endcsname{\pend{}}
\expandafter\gdef\csname R@rep.W5.z\endcsname{\pend{}}
\expandafter\gdef\csname R@rulebase.acdc.mean\endcsname{92.01}
\expandafter\gdef\csname R@rulebase.acdc.n\endcsname{6}
\expandafter\gdef\csname R@rulebase.amos.mean\endcsname{87.70}
\expandafter\gdef\csname R@rulebase.amos.n\endcsname{6}
\expandafter\gdef\csname R@run.acdc.0.dice\endcsname{92.13}
\expandafter\gdef\csname R@run.acdc.1.dice\endcsname{91.85}
\expandafter\gdef\csname R@run.acdc.2.dice\endcsname{92.03}
\expandafter\gdef\csname R@run.acdc.3.dice\endcsname{92.10}
\expandafter\gdef\csname R@run.acdc.4.dice\endcsname{91.98}
\expandafter\gdef\csname R@run.acdc.5.dice\endcsname{91.97}
\expandafter\gdef\csname R@run.amos.0.dice\endcsname{87.67}
\expandafter\gdef\csname R@run.amos.1.dice\endcsname{87.55}
\expandafter\gdef\csname R@run.amos.2.dice\endcsname{87.79}
\expandafter\gdef\csname R@run.amos.3.dice\endcsname{87.59}
\expandafter\gdef\csname R@run.amos.4.dice\endcsname{87.73}
\expandafter\gdef\csname R@run.amos.5.dice\endcsname{87.87}
\expandafter\gdef\csname R@runs.arm.cap\endcsname{12}
\expandafter\gdef\csname R@runs.arm.n\endcsname{46}
\expandafter\gdef\csname R@runs.pool.legacycap\endcsname{24}
\expandafter\gdef\csname R@runs.pool.n\endcsname{12}
\expandafter\gdef\csname R@runs.pool.nlegacy\endcsname{5}
\expandafter\gdef\csname R@runs.pool.ntta\endcsname{6}
\expandafter\gdef\csname R@runs.pool.ttads\endcsname{ACDC}
\expandafter\gdef\csname R@runs.tta.ds\endcsname{ACDC}
\expandafter\gdef\csname R@runs.tta.nods\endcsname{AMOS/KiTS23}
\expandafter\gdef\csname R@search.arch.ncand\endcsname{72}
\expandafter\gdef\csname R@search.arch.nconfirmed\endcsname{1}
\expandafter\gdef\csname R@search.recipe.ncand\endcsname{119}
\expandafter\gdef\csname R@search.recipe.nconfirmed\endcsname{49}
\expandafter\gdef\csname R@spd.acdc.e1000.abs\endcsname{91.98}
\expandafter\gdef\csname R@spd.acdc.e1000.max\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@spd.acdc.e1000.mean\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@spd.acdc.e1000.min\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@spd.acdc.e1000.ms\endcsname{\ensuremath{-0.03}\ensuremath{\pm}0.11}
\expandafter\gdef\csname R@spd.acdc.e1000.s0\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@spd.acdc.e1000.s1\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@spd.acdc.e1000.s2\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@spd.acdc.e1000.sd\endcsname{0.11}
\expandafter\gdef\csname R@spd.acdc.e250.abs\endcsname{91.84}
\expandafter\gdef\csname R@spd.acdc.e250.max\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@spd.acdc.e250.mean\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@spd.acdc.e250.min\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@spd.acdc.e250.ms\endcsname{\ensuremath{+0.06}\ensuremath{\pm}0.11}
\expandafter\gdef\csname R@spd.acdc.e250.s0\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@spd.acdc.e250.s1\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@spd.acdc.e250.s2\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@spd.acdc.e250.sd\endcsname{0.11}
\expandafter\gdef\csname R@spd.acdc.params\endcsname{25.34}
\expandafter\gdef\csname R@spd.acdc.vram\endcsname{10.40}
\expandafter\gdef\csname R@spd.amos.e1000.abs\endcsname{87.68}
\expandafter\gdef\csname R@spd.amos.e1000.max\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@spd.amos.e1000.mean\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@spd.amos.e1000.min\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@spd.amos.e1000.ms\endcsname{\ensuremath{+0.01}\ensuremath{\pm}0.36}
\expandafter\gdef\csname R@spd.amos.e1000.s0\endcsname{\ensuremath{+0.04}}
\expandafter\gdef\csname R@spd.amos.e1000.s1\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@spd.amos.e1000.s2\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@spd.amos.e1000.sd\endcsname{0.36}
\expandafter\gdef\csname R@spd.amos.e250.abs\endcsname{85.31}
\expandafter\gdef\csname R@spd.amos.e250.max\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@spd.amos.e250.mean\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@spd.amos.e250.min\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@spd.amos.e250.ms\endcsname{\ensuremath{+0.70}\ensuremath{\pm}0.28}
\expandafter\gdef\csname R@spd.amos.e250.s0\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@spd.amos.e250.s1\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@spd.amos.e250.s2\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@spd.amos.e250.sd\endcsname{0.28}
\expandafter\gdef\csname R@spd.amos.params\endcsname{26.83}
\expandafter\gdef\csname R@spd.amos.vram\endcsname{9.12}
\expandafter\gdef\csname R@spd.both.e1000.mean\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@split.acdc.covered\endcsname{no}
\expandafter\gdef\csname R@split.acdc.ncases\endcsname{300}
\expandafter\gdef\csname R@split.acdc.ncv\endcsname{200}
\expandafter\gdef\csname R@split.acdc.nfolds\endcsname{5}
\expandafter\gdef\csname R@split.acdc.nheld\endcsname{100}
\expandafter\gdef\csname R@split.amos.covered\endcsname{no}
\expandafter\gdef\csname R@split.amos.ncases\endcsname{300}
\expandafter\gdef\csname R@split.amos.ncv\endcsname{200}
\expandafter\gdef\csname R@split.amos.nfolds\endcsname{5}
\expandafter\gdef\csname R@split.amos.nheld\endcsname{100}
\expandafter\gdef\csname R@split.kits.covered\endcsname{yes}
\expandafter\gdef\csname R@split.kits.ncases\endcsname{489}
\expandafter\gdef\csname R@split.kits.ncv\endcsname{489}
\expandafter\gdef\csname R@split.kits.nfolds\endcsname{5}
\expandafter\gdef\csname R@split.kits.nheld\endcsname{0}
\expandafter\gdef\csname R@src.results_json\endcsname{research/agent\_team\_20261004/experiments/RESULTS.json}
\expandafter\gdef\csname R@src.results_json.generated\endcsname{2026-10-10 11:32:38}
\expandafter\gdef\csname R@static.acdc.e1000.mean\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@static.acdc.e1000.sd\endcsname{0.16}
\expandafter\gdef\csname R@static.amos.e1000.mean\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@static.amos.e1000.sd\endcsname{0.18}
\expandafter\gdef\csname R@thr.acdc\endcsname{0.15}
\expandafter\gdef\csname R@thr.amos\endcsname{0.35}
\expandafter\gdef\csname R@thr.nonempty\endcsname{0.20}
\expandafter\gdef\csname R@tum.L1.d\endcsname{\ensuremath{+2.90}}
\expandafter\gdef\csname R@tum.L1b.d\endcsname{\ensuremath{+3.02}}
\expandafter\gdef\csname R@tum.L2.d\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@tum.L3.d\endcsname{\ensuremath{+4.11}}
\expandafter\gdef\csname R@tum.L3.nsd\endcsname{3.3}
\expandafter\gdef\csname R@tum.L4.d\endcsname{\ensuremath{+3.50}}
\expandafter\gdef\csname R@tum.L6.d\endcsname{\ensuremath{+3.90}}
\expandafter\gdef\csname R@tum.base\endcsname{74.27}
\expandafter\gdef\csname R@tum.min.exL2\endcsname{\ensuremath{+2.90}}
\expandafter\gdef\csname R@w.L1.amos\endcsname{88.35}
\expandafter\gdef\csname R@w.L1.amos.d\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@w.L1.amos.nonempty.d\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@w.L1.kits.d\endcsname{\ensuremath{+2.33}}
\expandafter\gdef\csname R@w.L1.kits.nonempty.d\endcsname{\ensuremath{+2.33}}
\expandafter\gdef\csname R@w.L1.mem\endcsname{10.9}
\expandafter\gdef\csname R@w.L1.name\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@w.L1.nofit\endcsname{none}
\expandafter\gdef\csname R@w.L1.par\endcsname{102.3}
\expandafter\gdef\csname R@w.L1.step\endcsname{1.46}
\expandafter\gdef\csname R@w.L1.verdict\endcsname{\textbf{pass}}
\expandafter\gdef\csname R@w.L1.vsctrl\endcsname{\pend[7 runs]}
\expandafter\gdef\csname R@w.L1b.amos\endcsname{87.84}
\expandafter\gdef\csname R@w.L1b.amos.d\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@w.L1b.amos.nonempty.d\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@w.L1b.kits.d\endcsname{\ensuremath{+1.74}}
\expandafter\gdef\csname R@w.L1b.kits.nonempty.d\endcsname{\ensuremath{+1.74}}
\expandafter\gdef\csname R@w.L1b.mem\endcsname{10.6}
\expandafter\gdef\csname R@w.L1b.name\endcsname{ResEnc-matched (re-implemented)}
\expandafter\gdef\csname R@w.L1b.nofit\endcsname{none}
\expandafter\gdef\csname R@w.L1b.par\endcsname{102.4}
\expandafter\gdef\csname R@w.L1b.step\endcsname{1.38}
\expandafter\gdef\csname R@w.L1b.verdict\endcsname{\textbf{pass}}
\expandafter\gdef\csname R@w.L1b.vsctrl\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@w.L2.amos\endcsname{88.06}
\expandafter\gdef\csname R@w.L2.amos.d\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@w.L2.amos.nonempty.d\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@w.L2.kits.d\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@w.L2.kits.nonempty.d\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@w.L2.mem\endcsname{9.9}
\expandafter\gdef\csname R@w.L2.name\endcsname{ConvNeXt-k3}
\expandafter\gdef\csname R@w.L2.nofit\endcsname{none}
\expandafter\gdef\csname R@w.L2.par\endcsname{24.4}
\expandafter\gdef\csname R@w.L2.step\endcsname{1.46}
\expandafter\gdef\csname R@w.L2.verdict\endcsname{\textbf{pass}}
\expandafter\gdef\csname R@w.L2.vsctrl\endcsname{\pend[7 runs]}
\expandafter\gdef\csname R@w.L3.amos\endcsname{88.08}
\expandafter\gdef\csname R@w.L3.amos.d\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@w.L3.amos.nonempty.d\endcsname{\ensuremath{+0.39}}
\expandafter\gdef\csname R@w.L3.kits.d\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@w.L3.kits.nonempty.d\endcsname{\ensuremath{+2.84}}
\expandafter\gdef\csname R@w.L3.mem\endcsname{10.7}
\expandafter\gdef\csname R@w.L3.name\endcsname{HyReX}
\expandafter\gdef\csname R@w.L3.nofit\endcsname{none}
\expandafter\gdef\csname R@w.L3.par\endcsname{29.6}
\expandafter\gdef\csname R@w.L3.step\endcsname{1.53}
\expandafter\gdef\csname R@w.L3.verdict\endcsname{\textbf{pass}}
\expandafter\gdef\csname R@w.L3.vsctrl\endcsname{\pend[7 runs]}
\expandafter\gdef\csname R@w.L4.amos\endcsname{88.13}
\expandafter\gdef\csname R@w.L4.amos.d\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@w.L4.amos.nonempty.d\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@w.L4.kits.d\endcsname{\ensuremath{+2.20}}
\expandafter\gdef\csname R@w.L4.kits.nonempty.d\endcsname{\ensuremath{+2.20}}
\expandafter\gdef\csname R@w.L4.mem\endcsname{10.7}
\expandafter\gdef\csname R@w.L4.name\endcsname{ResEnc+context}
\expandafter\gdef\csname R@w.L4.nofit\endcsname{none}
\expandafter\gdef\csname R@w.L4.par\endcsname{102.8}
\expandafter\gdef\csname R@w.L4.step\endcsname{1.46}
\expandafter\gdef\csname R@w.L4.verdict\endcsname{\textbf{pass}}
\expandafter\gdef\csname R@w.L4.vsctrl\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@w.L6.amos\endcsname{87.72}
\expandafter\gdef\csname R@w.L6.amos.d\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@w.L6.amos.nonempty.d\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@w.L6.kits.d\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@w.L6.kits.nonempty.d\endcsname{\ensuremath{+2.53}}
\expandafter\gdef\csname R@w.L6.mem\endcsname{10.2}
\expandafter\gdef\csname R@w.L6.name\endcsname{HyReX+context}
\expandafter\gdef\csname R@w.L6.nofit\endcsname{none}
\expandafter\gdef\csname R@w.L6.par\endcsname{31.1}
\expandafter\gdef\csname R@w.L6.step\endcsname{1.88}
\expandafter\gdef\csname R@w.L6.verdict\endcsname{\textbf{pass}}
\expandafter\gdef\csname R@w.L6.vsctrl\endcsname{\pend[5 runs]}
\expandafter\gdef\csname R@w.W1.amos\endcsname{87.80}
\expandafter\gdef\csname R@w.W1.amos.d\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@w.W1.amos.nonempty.d\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@w.W1.kits.d\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W1.kits.nonempty.d\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W1.mem\endcsname{9.4}
\expandafter\gdef\csname R@w.W1.name\endcsname{$z$-dilation mixing}
\expandafter\gdef\csname R@w.W1.nofit\endcsname{none}
\expandafter\gdef\csname R@w.W1.par\endcsname{31.1}
\expandafter\gdef\csname R@w.W1.step\endcsname{1.14}
\expandafter\gdef\csname R@w.W1.verdict\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W1.vsctrl\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@w.W1c.amos\endcsname{88.06}
\expandafter\gdef\csname R@w.W1c.amos.d\endcsname{\ensuremath{+0.36}}
\expandafter\gdef\csname R@w.W1c.amos.nonempty.d\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@w.W1c.kits.d\endcsname{\ensuremath{+2.64}}
\expandafter\gdef\csname R@w.W1c.kits.nonempty.d\endcsname{\ensuremath{+2.64}}
\expandafter\gdef\csname R@w.W1c.mem\endcsname{9.4}
\expandafter\gdef\csname R@w.W1c.name\endcsname{branch control}
\expandafter\gdef\csname R@w.W1c.nofit\endcsname{none}
\expandafter\gdef\csname R@w.W1c.par\endcsname{31.1}
\expandafter\gdef\csname R@w.W1c.step\endcsname{1.15}
\expandafter\gdef\csname R@w.W1c.verdict\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W1c.vsctrl\endcsname{\pend[2 runs]}
\expandafter\gdef\csname R@w.W2.amos\endcsname{87.91}
\expandafter\gdef\csname R@w.W2.amos.d\endcsname{\ensuremath{+0.21}}
\expandafter\gdef\csname R@w.W2.amos.nonempty.d\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@w.W2.kits.d\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W2.kits.nonempty.d\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W2.mem\endcsname{9.4}
\expandafter\gdef\csname R@w.W2.name\endcsname{thickness-gated mixing}
\expandafter\gdef\csname R@w.W2.nofit\endcsname{none}
\expandafter\gdef\csname R@w.W2.par\endcsname{31.1}
\expandafter\gdef\csname R@w.W2.step\endcsname{1.15}
\expandafter\gdef\csname R@w.W2.verdict\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W2.vsctrl\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@w.W3.amos\endcsname{87.97}
\expandafter\gdef\csname R@w.W3.amos.d\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@w.W3.amos.nonempty.d\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@w.W3.kits.d\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W3.kits.nonempty.d\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W3.mem\endcsname{9.3}
\expandafter\gdef\csname R@w.W3.name\endcsname{offset upsampling}
\expandafter\gdef\csname R@w.W3.nofit\endcsname{none}
\expandafter\gdef\csname R@w.W3.par\endcsname{29.6}
\expandafter\gdef\csname R@w.W3.step\endcsname{1.08}
\expandafter\gdef\csname R@w.W3.verdict\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W3.vsctrl\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@w.W3c.amos\endcsname{87.86}
\expandafter\gdef\csname R@w.W3c.amos.d\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@w.W3c.amos.nonempty.d\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@w.W3c.kits.d\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W3c.kits.nonempty.d\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W3c.mem\endcsname{9.5}
\expandafter\gdef\csname R@w.W3c.name\endcsname{trilinear-decoder control}
\expandafter\gdef\csname R@w.W3c.nofit\endcsname{none}
\expandafter\gdef\csname R@w.W3c.par\endcsname{29.5}
\expandafter\gdef\csname R@w.W3c.step\endcsname{1.07}
\expandafter\gdef\csname R@w.W3c.verdict\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W3c.vsctrl\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W4.amos\endcsname{87.78}
\expandafter\gdef\csname R@w.W4.amos.d\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@w.W4.amos.nonempty.d\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@w.W4.kits.d\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W4.kits.nonempty.d\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W4.mem\endcsname{10.5}
\expandafter\gdef\csname R@w.W4.name\endcsname{ConvNeXt-4$\times$-GRN (MedNeXt-like reference)}
\expandafter\gdef\csname R@w.W4.nofit\endcsname{none}
\expandafter\gdef\csname R@w.W4.par\endcsname{34.2}
\expandafter\gdef\csname R@w.W4.step\endcsname{3.51}
\expandafter\gdef\csname R@w.W4.verdict\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W4.vsctrl\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W5.amos\endcsname{88.29}
\expandafter\gdef\csname R@w.W5.amos.d\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@w.W5.amos.nonempty.d\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@w.W5.kits.d\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W5.kits.nonempty.d\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W5.mem\endcsname{10.7}
\expandafter\gdef\csname R@w.W5.name\endcsname{pooled-skip control}
\expandafter\gdef\csname R@w.W5.nofit\endcsname{ACDC}
\expandafter\gdef\csname R@w.W5.par\endcsname{102.4}
\expandafter\gdef\csname R@w.W5.step\endcsname{1.37}
\expandafter\gdef\csname R@w.W5.verdict\endcsname{\pend{}}
\expandafter\gdef\csname R@w.W5.vsctrl\endcsname{\pend{}}
\expandafter\gdef\csname R@wave1.best.amos.d\endcsname{\ensuremath{+0.65}}
\expandafter\gdef\csname R@wave1.best.name\endcsname{ResEnc-M (library preset)}
\expandafter\gdef\csname R@wave1.best.nonempty.d\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@wave1.n\endcsname{6}
\expandafter\gdef\csname R@wave1.ncand\endcsname{5}
\expandafter\gdef\csname R@wave1.nctrl\endcsname{1}
\expandafter\gdef\csname R@wave1.ndone\endcsname{5}
\expandafter\gdef\csname R@wave1.npass\endcsname{5}
\expandafter\gdef\csname R@wave2.best.amos.d\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@wave2.best.name\endcsname{offset upsampling}
\expandafter\gdef\csname R@wave2.best.nonempty.d\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@wave2.n\endcsname{7}
\expandafter\gdef\csname R@wave2.ncand\endcsname{4}
\expandafter\gdef\csname R@wave2.nctrl\endcsname{3}
\expandafter\gdef\csname R@wave2.ndone\endcsname{4}
\expandafter\gdef\csname R@wave2.npass\endcsname{0}
\expandafter\gdef\csname R@wbase.acdc.mean\endcsname{92.01}
\expandafter\gdef\csname R@wbase.acdc.n\endcsname{6}
\expandafter\gdef\csname R@wbase.acdc.nonempty\endcsname{92.01}
\expandafter\gdef\csname R@wbase.amos.fpvox\endcsname{46\,076}
\expandafter\gdef\csname R@wbase.amos.mean\endcsname{87.70}
\expandafter\gdef\csname R@wbase.amos.n\endcsname{6}
\expandafter\gdef\csname R@wbase.amos.nempty\endcsname{6}
\expandafter\gdef\csname R@wbase.amos.nonempty\endcsname{88.45}
\expandafter\gdef\csname R@wbase.amos.z5\endcsname{86.86}
\expandafter\gdef\csname R@wbase.amos.zthin\endcsname{90.22}
\expandafter\gdef\csname R@wbase.kits.mean\endcsname{83.38}
\expandafter\gdef\csname R@wbase.kits.n\endcsname{3}
\expandafter\gdef\csname R@wbase.kits.nonempty\endcsname{83.38}
\expandafter\gdef\csname R@zs.acc.train\endcsname{0.91}
\expandafter\gdef\csname R@zs.alt.train\endcsname{0.85}
\expandafter\gdef\csname R@zs.auc.central\endcsname{1.00}
\expandafter\gdef\csname R@zs.auc.train\endcsname{0.93}
\expandafter\gdef\csname R@zs.auc.val\endcsname{1.00}
\expandafter\gdef\csname R@zs.n5\endcsname{30}
\expandafter\gdef\csname R@zs.npatch\endcsname{140}
\expandafter\gdef\csname R@zs.nthin\endcsname{10}
\expandafter\gdef\csname R@zs.nval\endcsname{40}
\expandafter\gdef\csname R@zs.trainshare\endcsname{81}
\makeatother


==> results/xref_main.tex <==
\makeatletter
\expandafter\gdef\csname XM@fig:p-fig1\endcsname{1}
\expandafter\gdef\csname XM@fig:p-fig1@cref\endcsname{[figure][1][]1}
\expandafter\gdef\csname XM@sec:p-intro\endcsname{1}
\expandafter\gdef\csname XM@sec:p-intro@cref\endcsname{[section][1][]1}
\expandafter\gdef\csname XM@sec:p-related\endcsname{2}
\expandafter\gdef\csname XM@sec:p-related@cref\endcsname{[section][2][]2}
\expandafter\gdef\csname XM@sec:p-method\endcsname{3}
\expandafter\gdef\csname XM@sec:p-method@cref\endcsname{[section][3][]3}
\expandafter\gdef\csname XM@sec:p-loop\endcsname{3.1}
\expandafter\gdef\csname XM@sec:p-loop@cref\endcsname{[subsection][1][3]3.1}
\expandafter\gdef\csname XM@sec:p-network\endcsname{3.2}
\expandafter\gdef\csname XM@sec:p-network@cref\endcsname{[subsection][2][3]3.2}
\expandafter\gdef\csname XM@sec:p-experiments\endcsname{4}
\expandafter\gdef\csname XM@sec:p-experiments@cref\endcsname{[section][4][]4}
\expandafter\gdef\csname XM@sec:p-setup\endcsname{4.1}
\expandafter\gdef\csname XM@sec:p-setup@cref\endcsname{[subsection][1][4]4.1}
\expandafter\gdef\csname XM@sec:p-results\endcsname{4.2}
\expandafter\gdef\csname XM@sec:p-results@cref\endcsname{[subsection][2][4]4.2}
\expandafter\gdef\csname XM@fig:p-network\endcsname{2}
\expandafter\gdef\csname XM@fig:p-network@cref\endcsname{[figure][2][]2}
\expandafter\gdef\csname XM@sec:p-efficiency\endcsname{4.3}
\expandafter\gdef\csname XM@sec:p-efficiency@cref\endcsname{[subsection][3][4]4.3}
\expandafter\gdef\csname XM@sec:p-heldout\endcsname{4.4}
\expandafter\gdef\csname XM@sec:p-heldout@cref\endcsname{[subsection][4][4]4.4}
\expandafter\gdef\csname XM@tab:p-master\endcsname{1}
\expandafter\gdef\csname XM@tab:p-master@cref\endcsname{[table][1][]1}
\expandafter\gdef\csname XM@fig:p-cvfolds\endcsname{3}
\expandafter\gdef\csname XM@fig:p-cvfolds@cref\endcsname{[figure][3][]3}
\expandafter\gdef\csname XM@tab:p-cost\endcsname{2}
\expandafter\gdef\csname XM@tab:p-cost@cref\endcsname{[table][2][]2}
\expandafter\gdef\csname XM@tab:p-heldout\endcsname{3}
\expandafter\gdef\csname XM@tab:p-heldout@cref\endcsname{[table][3][]3}
\expandafter\gdef\csname XM@sec:p-ablation\endcsname{4.5}
\expandafter\gdef\csname XM@sec:p-ablation@cref\endcsname{[subsection][5][4]4.5}
\expandafter\gdef\csname XM@sec:p-perclass\endcsname{4.6}
\expandafter\gdef\csname XM@sec:p-perclass@cref\endcsname{[subsection][6][4]4.6}
\expandafter\gdef\csname XM@fig:p-stagecost\endcsname{4}
\expandafter\gdef\csname XM@fig:p-stagecost@cref\endcsname{[figure][4][]4}
\expandafter\gdef\csname XM@sec:p-process\endcsname{4.7}
\expandafter\gdef\csname XM@sec:p-process@cref\endcsname{[subsection][7][4]4.7}
\expandafter\gdef\csname XM@fig:p-tree\endcsname{5}
\expandafter\gdef\csname XM@fig:p-tree@cref\endcsname{[figure][5][]5}
\expandafter\gdef\csname XM@fig:p-front\endcsname{6}
\expandafter\gdef\csname XM@fig:p-front@cref\endcsname{[figure][6][]6}
\expandafter\gdef\csname XM@tab:p-ablation\endcsname{4}
\expandafter\gdef\csname XM@tab:p-ablation@cref\endcsname{[table][4][]4}
\expandafter\gdef\csname XM@tab:p-perclass\endcsname{5}
\expandafter\gdef\csname XM@tab:p-perclass@cref\endcsname{[table][5][]5}
\expandafter\gdef\csname XM@tab:p-errors\endcsname{6}
\expandafter\gdef\csname XM@tab:p-errors@cref\endcsname{[table][6][]6}
\expandafter\gdef\csname XM@tab:p-bdry\endcsname{7}
\expandafter\gdef\csname XM@tab:p-bdry@cref\endcsname{[table][7][]7}
\expandafter\gdef\csname XM@sec:p-stage1\endcsname{4.7}
\expandafter\gdef\csname XM@sec:p-stage1@cref\endcsname{[subsection][7][4]4.7}
\expandafter\gdef\csname XM@fig:p-gallery\endcsname{7}
\expandafter\gdef\csname XM@fig:p-gallery@cref\endcsname{[figure][7][]7}
\expandafter\gdef\csname XM@sec:p-conclusion\endcsname{5}
\expandafter\gdef\csname XM@sec:p-conclusion@cref\endcsname{[section][5][]5}
\expandafter\gdef\csname XM@endofbody\endcsname{5}
\expandafter\gdef\csname XM@endofbody@cref\endcsname{[section][5][]5}
\makeatother


==> supp_keys.tex <==
% AUTO-GENERATED by paper_v1/supp_keys.py from runs/trials/*/result.json, the candidate specs and the KiTS23 plan -- do not edit by hand
\makeatletter
\expandafter\gdef\csname R@s1.amos.stock.mean\endcsname{87.71}
\expandafter\gdef\csname R@s1.amos.stock.n\endcsname{3}
\expandafter\gdef\csname R@s1.arch.V7A1.dec.gmac\endcsname{118.0}
\expandafter\gdef\csname R@s1.arch.V7A1.dec.gmac_pct\endcsname{35}
\expandafter\gdef\csname R@s1.arch.V7A1.dec.params\endcsname{6.94}
\expandafter\gdef\csname R@s1.arch.V7A1.enc.gmac\endcsname{255.2}
\expandafter\gdef\csname R@s1.arch.V7A1.enc.params\endcsname{24.10}
\expandafter\gdef\csname R@s1.arch.V7A1.gmac\endcsname{373.5}
\expandafter\gdef\csname R@s1.arch.V7A1.params\endcsname{31.04}
\expandafter\gdef\csname R@s1.arch.V7C1.dec.gmac\endcsname{118.0}
\expandafter\gdef\csname R@s1.arch.V7C1.dec.gmac_pct\endcsname{35}
\expandafter\gdef\csname R@s1.arch.V7C1.dec.params\endcsname{6.94}
\expandafter\gdef\csname R@s1.arch.V7C1.enc.gmac\endcsname{138.8}
\expandafter\gdef\csname R@s1.arch.V7C1.enc.params\endcsname{14.17}
\expandafter\gdef\csname R@s1.arch.V7C1.gmac\endcsname{257.0}
\expandafter\gdef\csname R@s1.arch.V7C1.params\endcsname{21.11}
\expandafter\gdef\csname R@s1.arch.base.dec.gmac\endcsname{338.3}
\expandafter\gdef\csname R@s1.arch.base.dec.params\endcsname{17.17}
\expandafter\gdef\csname R@s1.arch.base.enc.gmac\endcsname{138.8}
\expandafter\gdef\csname R@s1.arch.base.enc.params\endcsname{14.03}
\expandafter\gdef\csname R@s1.arch.base.gmac\endcsname{477.3}
\expandafter\gdef\csname R@s1.arch.base.params\endcsname{31.20}
\expandafter\gdef\csname R@s1.fresh.agent.2se\endcsname{11}
\expandafter\gdef\csname R@s1.fresh.agent.n\endcsname{21}
\expandafter\gdef\csname R@s1.fresh.agent.pos\endcsname{19}
\expandafter\gdef\csname R@s1.fresh.n\endcsname{25}
\expandafter\gdef\csname R@s1.fresh.n.2se\endcsname{13}
\expandafter\gdef\csname R@s1.fresh.n.pos\endcsname{23}
\expandafter\gdef\csname R@s1.ho.brats.L1.d\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@s1.ho.brats.L1.mean\endcsname{82.95}
\expandafter\gdef\csname R@s1.ho.brats.L1.n\endcsname{1}
\expandafter\gdef\csname R@s1.ho.brats.L1.s0\endcsname{82.95}
\expandafter\gdef\csname R@s1.ho.brats.L3.d\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@s1.ho.brats.L3.mean\endcsname{83.05}
\expandafter\gdef\csname R@s1.ho.brats.L3.n\endcsname{1}
\expandafter\gdef\csname R@s1.ho.brats.L3.s0\endcsname{83.05}
\expandafter\gdef\csname R@s1.ho.brats.V7A1.d\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@s1.ho.brats.V7A1.mean\endcsname{83.17}
\expandafter\gdef\csname R@s1.ho.brats.V7A1.n\endcsname{3}
\expandafter\gdef\csname R@s1.ho.brats.V7A1.s0\endcsname{83.21}
\expandafter\gdef\csname R@s1.ho.brats.V7A1.s1\endcsname{83.16}
\expandafter\gdef\csname R@s1.ho.brats.V7A1.s2\endcsname{83.15}
\expandafter\gdef\csname R@s1.ho.brats.V7C1.d\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@s1.ho.brats.V7C1.mean\endcsname{83.15}
\expandafter\gdef\csname R@s1.ho.brats.V7C1.n\endcsname{3}
\expandafter\gdef\csname R@s1.ho.brats.V7C1.s0\endcsname{83.12}
\expandafter\gdef\csname R@s1.ho.brats.V7C1.s1\endcsname{83.39}
\expandafter\gdef\csname R@s1.ho.brats.V7C1.s2\endcsname{82.93}
\expandafter\gdef\csname R@s1.ho.brats.base.mean\endcsname{83.23}
\expandafter\gdef\csname R@s1.ho.brats.base.n\endcsname{3}
\expandafter\gdef\csname R@s1.ho.brats.base.s0\endcsname{82.98}
\expandafter\gdef\csname R@s1.ho.brats.base.s1\endcsname{83.29}
\expandafter\gdef\csname R@s1.ho.brats.base.s2\endcsname{83.44}
\expandafter\gdef\csname R@s1.ho.btcv.L1.d\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@s1.ho.btcv.L1.mean\endcsname{78.52}
\expandafter\gdef\csname R@s1.ho.btcv.L1.n\endcsname{3}
\expandafter\gdef\csname R@s1.ho.btcv.L1.s0\endcsname{79.24}
\expandafter\gdef\csname R@s1.ho.btcv.L1.s1\endcsname{78.23}
\expandafter\gdef\csname R@s1.ho.btcv.L1.s2\endcsname{78.10}
\expandafter\gdef\csname R@s1.ho.btcv.L3.d\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@s1.ho.btcv.L3.mean\endcsname{78.53}
\expandafter\gdef\csname R@s1.ho.btcv.L3.n\endcsname{3}
\expandafter\gdef\csname R@s1.ho.btcv.L3.s0\endcsname{77.85}
\expandafter\gdef\csname R@s1.ho.btcv.L3.s1\endcsname{79.74}
\expandafter\gdef\csname R@s1.ho.btcv.L3.s2\endcsname{78.00}
\expandafter\gdef\csname R@s1.ho.btcv.V7A1.d\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@s1.ho.btcv.V7A1.mean\endcsname{78.30}
\expandafter\gdef\csname R@s1.ho.btcv.V7A1.n\endcsname{3}
\expandafter\gdef\csname R@s1.ho.btcv.V7A1.s0\endcsname{78.43}
\expandafter\gdef\csname R@s1.ho.btcv.V7A1.s1\endcsname{78.26}
\expandafter\gdef\csname R@s1.ho.btcv.V7A1.s2\endcsname{78.22}
\expandafter\gdef\csname R@s1.ho.btcv.V7C1.d\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@s1.ho.btcv.V7C1.mean\endcsname{77.50}
\expandafter\gdef\csname R@s1.ho.btcv.V7C1.n\endcsname{3}
\expandafter\gdef\csname R@s1.ho.btcv.V7C1.s0\endcsname{77.67}
\expandafter\gdef\csname R@s1.ho.btcv.V7C1.s1\endcsname{77.29}
\expandafter\gdef\csname R@s1.ho.btcv.V7C1.s2\endcsname{77.54}
\expandafter\gdef\csname R@s1.ho.btcv.base.mean\endcsname{77.82}
\expandafter\gdef\csname R@s1.ho.btcv.base.n\endcsname{3}
\expandafter\gdef\csname R@s1.ho.btcv.base.s0\endcsname{77.57}
\expandafter\gdef\csname R@s1.ho.btcv.base.s1\endcsname{78.15}
\expandafter\gdef\csname R@s1.ho.btcv.base.s2\endcsname{77.73}
\expandafter\gdef\csname R@s1.ho.lits.L1.d\endcsname{\ensuremath{+1.13}}
\expandafter\gdef\csname R@s1.ho.lits.L1.mean\endcsname{81.93}
\expandafter\gdef\csname R@s1.ho.lits.L1.n\endcsname{3}
\expandafter\gdef\csname R@s1.ho.lits.L1.s0\endcsname{81.80}
\expandafter\gdef\csname R@s1.ho.lits.L1.s1\endcsname{81.76}
\expandafter\gdef\csname R@s1.ho.lits.L1.s2\endcsname{82.22}
\expandafter\gdef\csname R@s1.ho.lits.L3.d\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@s1.ho.lits.L3.mean\endcsname{81.29}
\expandafter\gdef\csname R@s1.ho.lits.L3.n\endcsname{3}
\expandafter\gdef\csname R@s1.ho.lits.L3.s0\endcsname{80.80}
\expandafter\gdef\csname R@s1.ho.lits.L3.s1\endcsname{82.17}
\expandafter\gdef\csname R@s1.ho.lits.L3.s2\endcsname{80.90}
\expandafter\gdef\csname R@s1.ho.lits.V7A1.d\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@s1.ho.lits.V7A1.mean\endcsname{82.44}
\expandafter\gdef\csname R@s1.ho.lits.V7A1.n\endcsname{3}
\expandafter\gdef\csname R@s1.ho.lits.V7A1.s0\endcsname{81.83}
\expandafter\gdef\csname R@s1.ho.lits.V7A1.s1\endcsname{84.16}
\expandafter\gdef\csname R@s1.ho.lits.V7A1.s2\endcsname{81.34}
\expandafter\gdef\csname R@s1.ho.lits.V7C1.d\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@s1.ho.lits.V7C1.mean\endcsname{81.65}
\expandafter\gdef\csname R@s1.ho.lits.V7C1.n\endcsname{3}
\expandafter\gdef\csname R@s1.ho.lits.V7C1.s0\endcsname{79.54}
\expandafter\gdef\csname R@s1.ho.lits.V7C1.s1\endcsname{82.76}
\expandafter\gdef\csname R@s1.ho.lits.V7C1.s2\endcsname{82.65}
\expandafter\gdef\csname R@s1.ho.lits.base.mean\endcsname{80.79}
\expandafter\gdef\csname R@s1.ho.lits.base.n\endcsname{3}
\expandafter\gdef\csname R@s1.ho.lits.base.s0\endcsname{79.86}
\expandafter\gdef\csname R@s1.ho.lits.base.s1\endcsname{79.98}
\expandafter\gdef\csname R@s1.ho.lits.base.s2\endcsname{82.54}
\expandafter\gdef\csname R@s1.mirror.amos.L1\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@s1.mirror.amos.L3\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@s1.mirror.amos.base\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@s1.mirror.kits.L1\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@s1.mirror.kits.L3\endcsname{\ensuremath{+1.41}}
\expandafter\gdef\csname R@s1.mirror.kits.base\endcsname{\ensuremath{+1.52}}
\expandafter\gdef\csname R@s1.nval.acdc\endcsname{40}
\expandafter\gdef\csname R@s1.nval.amos\endcsname{40}
\expandafter\gdef\csname R@s1.nval.brats\endcsname{97}
\expandafter\gdef\csname R@s1.nval.btcv\endcsname{6}
\expandafter\gdef\csname R@s1.nval.kits\endcsname{98}
\expandafter\gdef\csname R@s1.nval.lits\endcsname{27}
\expandafter\gdef\csname R@s1.plan.kits.widths\endcsname{32, 64, 128, 256, 320, 320}
\expandafter\gdef\csname R@s1.rs.07.amos.d\endcsname{\ensuremath{+0.82}}
\expandafter\gdef\csname R@s1.rs.08.amos.d\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@s1.rs.13.amos.d\endcsname{\ensuremath{-0.97}}
\expandafter\gdef\csname R@s1.rs.15.amos.d\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@s1.rs.23.amos.d\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@s1.sp.1.amos.d\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@s1.sp.2.amos.d\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@s1.stage.C1\endcsname{replicated}
\expandafter\gdef\csname R@s1.stage.D1\endcsname{replicated}
\expandafter\gdef\csname R@s1.stage.D2\endcsname{cross-validated}
\expandafter\gdef\csname R@s1.stage.L2\endcsname{replicated}
\expandafter\gdef\csname R@s1.stage.L3\endcsname{held-out}
\expandafter\gdef\csname R@s1.stage.L4\endcsname{replicated}
\expandafter\gdef\csname R@s1.stage.L6\endcsname{replicated}
\expandafter\gdef\csname R@s1.stage.N1\endcsname{screened}
\expandafter\gdef\csname R@s1.stage.S2\endcsname{replicated}
\expandafter\gdef\csname R@s1.stage.V5A5\endcsname{replicated}
\expandafter\gdef\csname R@s1.stage.V5B1\endcsname{cross-validated}
\expandafter\gdef\csname R@s1.stage.V5B2\endcsname{cross-validated}
\expandafter\gdef\csname R@s1.stage.V6A1r\endcsname{cross-validated}
\expandafter\gdef\csname R@s1.stage.V7A1\endcsname{held-out}
\expandafter\gdef\csname R@s1.stage.V7A2\endcsname{cross-validated}
\expandafter\gdef\csname R@s1.stage.V7B1\endcsname{replicated}
\expandafter\gdef\csname R@s1.stage.V7B2\endcsname{replicated}
\expandafter\gdef\csname R@s1.stage.V7C1\endcsname{held-out}
\expandafter\gdef\csname R@s1.stage.V8A1\endcsname{replicated}
\expandafter\gdef\csname R@s1.stage.V8A2\endcsname{replicated}
\expandafter\gdef\csname R@s1.stage.V8B1\endcsname{replicated}
\expandafter\gdef\csname R@s1.stage.V8B2\endcsname{cross-validated}
\expandafter\gdef\csname R@s1.stage.W1\endcsname{screened}
\expandafter\gdef\csname R@s1.stage.W2\endcsname{screened}
\expandafter\gdef\csname R@s1.stage.W3\endcsname{screened}
\expandafter\gdef\csname R@s1.stage.n.all\endcsname{25}
\expandafter\gdef\csname R@s1.stage.n.cross-validated\endcsname{6}
\expandafter\gdef\csname R@s1.stage.n.cvplus\endcsname{9}
\expandafter\gdef\csname R@s1.stage.n.held-out\endcsname{3}
\expandafter\gdef\csname R@s1.stage.n.replicated\endcsname{12}
\expandafter\gdef\csname R@s1.stage.n.screened\endcsname{4}
\expandafter\gdef\csname R@s1.tta.acdc\endcsname{with mirroring}
\expandafter\gdef\csname R@s1.tta.amos\endcsname{without test-time augmentation}
\expandafter\gdef\csname R@s1.tta.brats\endcsname{without test-time augmentation}
\expandafter\gdef\csname R@s1.tta.btcv\endcsname{without test-time augmentation}
\expandafter\gdef\csname R@s1.tta.kits\endcsname{without test-time augmentation}
\expandafter\gdef\csname R@s1.tta.lits\endcsname{without test-time augmentation}
\makeatother


==> v1keys.tex <==
% AUTO-GENERATED by paper_v1/v1keys.py from runs/trials/*/result.json -- do not edit by hand
\makeatletter
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.clause\endcsname{LeanDec minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold, no test-time mirroring): \ensuremath{+0.02}}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.est\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.hi\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.lo\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@an.cv.acdc.D2.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.clause\endcsname{LeanDec minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold, no test-time mirroring): \ensuremath{+0.11}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.est\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.hi\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.lo\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@an.cv.acdc.D2P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.clause\endcsname{ResEnc-M minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold, no test-time mirroring): \ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.est\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.hi\endcsname{\ensuremath{+0.62}}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.lo\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.acdc.L1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.clause\endcsname{ResEnc-M minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold, no test-time mirroring): \ensuremath{+0.53}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.est\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.hi\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.lo\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@an.cv.acdc.L1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.clause\endcsname{ResEnc-matched minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold, no test-time mirroring): \ensuremath{+0.29}}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.est\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.hi\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.lo\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@an.cv.acdc.L1b.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L1bP3c.cbs.est\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@an.cv.acdc.L1bP3c.cbs.hi\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@an.cv.acdc.L1bP3c.cbs.lo\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@an.cv.acdc.L1bP3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.clause\endcsname{HyReX minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold, no test-time mirroring): \ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.est\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.hi\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.lo\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@an.cv.acdc.L3.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.clause\endcsname{HyReX minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold, no test-time mirroring): \ensuremath{+0.43}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.est\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.hi\endcsname{\ensuremath{+0.64}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.lo\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.acdc.L3P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.clause\endcsname{the function-identical control minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold, no test-time mirroring): \ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.est\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.hi\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.lo\endcsname{\ensuremath{-0.26}}
\expandafter\gdef\csname R@an.cv.acdc.P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.clause\endcsname{LeanAdd minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold, no test-time mirroring): \ensuremath{-0.13}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.est\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.hi\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.lo\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.clause\endcsname{LeanAdd minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold, no test-time mirroring): \ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.est\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.hi\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.lo\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.acdc.V5B1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.clause\endcsname{LeanAdd-NeXt minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold, no test-time mirroring): \ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.est\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.hi\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.lo\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.clause\endcsname{LeanAdd-NeXt minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold, no test-time mirroring): \ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.est\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.hi\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.lo\endcsname{\ensuremath{-0.21}}
\expandafter\gdef\csname R@an.cv.acdc.V5B2P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.clause\endcsname{HyReX-k9 minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold, no test-time mirroring): \ensuremath{+0.42}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.est\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.hi\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.lo\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1r.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.clause\endcsname{HyReX-k9 minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold, no test-time mirroring): \ensuremath{+0.52}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.est\endcsname{\ensuremath{+0.52}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.hi\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.lo\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@an.cv.acdc.V6A1rP3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.clause\endcsname{LeanDeepMid minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold, no test-time mirroring): \ensuremath{+0.17}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.est\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.hi\endcsname{\ensuremath{+0.35}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.lo\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.clause\endcsname{LeanDeepMid minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold, no test-time mirroring): \ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.est\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.hi\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.lo\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V7A1cov.cbs.est\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1cov.cbs.hi\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1cov.cbs.lo\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1cov.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V7A1covP3c.cbs.est\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1covP3c.cbs.hi\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1covP3c.cbs.lo\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@an.cv.acdc.V7A1covP3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.clause\endcsname{LeanNeXt-s5 minus the default, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold, no test-time mirroring): \ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.est\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.hi\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.lo\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.clause\endcsname{LeanNeXt-s5 minus the function-identical control, case-level paired bootstrap over the 160 validation cases of the four folds (10000 resamples stratified by fold, one seed per fold, no test-time mirroring): \ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.est\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.hi\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.lo\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@an.cv.acdc.V7C1P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V9R2.cbs.est\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@an.cv.acdc.V9R2.cbs.hi\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@an.cv.acdc.V9R2.cbs.lo\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@an.cv.acdc.V9R2.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@an.cv.acdc.V9R2P3c.cbs.est\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@an.cv.acdc.V9R2P3c.cbs.hi\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@an.cv.acdc.V9R2P3c.cbs.lo\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@an.cv.acdc.V9R2P3c.cbs.ncases\endcsname{160}
\expandafter\gdef\csname R@v1.ab.1.kits.dstock\endcsname{\ensuremath{-0.31}}
\expandafter\gdef\csname R@v1.ab.1.kits.dxl\endcsname{\ensuremath{-2.13}}
\expandafter\gdef\csname R@v1.ab.1.kits.s0\endcsname{83.95}
\expandafter\gdef\csname R@v1.ab.10.kits.dstock\endcsname{\ensuremath{+1.84}}
\expandafter\gdef\csname R@v1.ab.10.kits.dxl\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@v1.ab.10.kits.s0\endcsname{86.10}
\expandafter\gdef\csname R@v1.ab.11.kits.dstock\endcsname{\ensuremath{-1.41}}
\expandafter\gdef\csname R@v1.ab.11.kits.dxl\endcsname{\ensuremath{-3.24}}
\expandafter\gdef\csname R@v1.ab.11.kits.s0\endcsname{82.84}
\expandafter\gdef\csname R@v1.ab.2.kits.dstock\endcsname{\ensuremath{+1.76}}
\expandafter\gdef\csname R@v1.ab.2.kits.dxl\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@v1.ab.2.kits.s0\endcsname{86.02}
\expandafter\gdef\csname R@v1.ab.3.kits.dstock\endcsname{\ensuremath{+1.28}}
\expandafter\gdef\csname R@v1.ab.3.kits.dxl\endcsname{\ensuremath{-0.55}}
\expandafter\gdef\csname R@v1.ab.3.kits.s0\endcsname{85.54}
\expandafter\gdef\csname R@v1.ab.4.kits.dstock\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@v1.ab.4.kits.dxl\endcsname{\ensuremath{-1.32}}
\expandafter\gdef\csname R@v1.ab.4.kits.s0\endcsname{84.77}
\expandafter\gdef\csname R@v1.ab.5.kits.dstock\endcsname{\ensuremath{+0.69}}
\expandafter\gdef\csname R@v1.ab.5.kits.dxl\endcsname{\ensuremath{-1.14}}
\expandafter\gdef\csname R@v1.ab.5.kits.s0\endcsname{84.95}
\expandafter\gdef\csname R@v1.ab.6.kits.dstock\endcsname{\ensuremath{+0.90}}
\expandafter\gdef\csname R@v1.ab.6.kits.dxl\endcsname{\ensuremath{-0.93}}
\expandafter\gdef\csname R@v1.ab.6.kits.s0\endcsname{85.15}
\expandafter\gdef\csname R@v1.ab.7.kits.dstock\endcsname{\ensuremath{-1.03}}
\expandafter\gdef\csname R@v1.ab.7.kits.dxl\endcsname{\ensuremath{-2.86}}
\expandafter\gdef\csname R@v1.ab.7.kits.s0\endcsname{83.23}
\expandafter\gdef\csname R@v1.ab.8.kits.dstock\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@v1.ab.8.kits.dxl\endcsname{\ensuremath{-1.37}}
\expandafter\gdef\csname R@v1.ab.8.kits.s0\endcsname{84.72}
\expandafter\gdef\csname R@v1.ab.9.kits.dstock\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@v1.ab.9.kits.dxl\endcsname{\ensuremath{-1.05}}
\expandafter\gdef\csname R@v1.ab.9.kits.s0\endcsname{85.03}
\expandafter\gdef\csname R@v1.ab.xl.dstock\endcsname{\ensuremath{+1.83}}
\expandafter\gdef\csname R@v1.acdc.mirroroff\endcsname{1}
\expandafter\gdef\csname R@v1.ag.best\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@v1.ag.fastallpos\endcsname{1}
\expandafter\gdef\csname R@v1.ag.median\endcsname{\ensuremath{+1.30}}
\expandafter\gdef\csname R@v1.ag.n\endcsname{22}
\expandafter\gdef\csname R@v1.ag.nabove_rsbest\endcsname{1}
\expandafter\gdef\csname R@v1.ag.nfast\endcsname{11}
\expandafter\gdef\csname R@v1.ag.nfast_pos\endcsname{11}
\expandafter\gdef\csname R@v1.ag.npos\endcsname{20}
\expandafter\gdef\csname R@v1.ag.nscreen\endcsname{20}
\expandafter\gdef\csname R@v1.amos0.C1.d\endcsname{\ensuremath{+0.38}}
\expandafter\gdef\csname R@v1.amos0.D2.d\endcsname{\ensuremath{-0.37}}
\expandafter\gdef\csname R@v1.amos0.V5A5.d\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@v1.amos0.V5B1.d\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@v1.amos0.V5B2.d\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@v1.cv.acdc.D2.d\endcsname{\ensuremath{+0.02}}
\expandafter\gdef\csname R@v1.cv.acdc.D2.dabs\endcsname{0.02}
\expandafter\gdef\csname R@v1.cv.acdc.D2.f1\endcsname{91.15}
\expandafter\gdef\csname R@v1.cv.acdc.D2.f2\endcsname{91.36}
\expandafter\gdef\csname R@v1.cv.acdc.D2.f3\endcsname{91.20}
\expandafter\gdef\csname R@v1.cv.acdc.D2.f4\endcsname{90.15}
\expandafter\gdef\csname R@v1.cv.acdc.D2.hi\endcsname{\ensuremath{+0.22}}
\expandafter\gdef\csname R@v1.cv.acdc.D2.lo\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@v1.cv.acdc.D2.mean\endcsname{90.96}
\expandafter\gdef\csname R@v1.cv.acdc.D2.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.acdc.D2.npos\endcsname{2}
\expandafter\gdef\csname R@v1.cv.acdc.L1.d\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@v1.cv.acdc.L1.dabs\endcsname{0.44}
\expandafter\gdef\csname R@v1.cv.acdc.L1.f1\endcsname{91.55}
\expandafter\gdef\csname R@v1.cv.acdc.L1.f2\endcsname{91.70}
\expandafter\gdef\csname R@v1.cv.acdc.L1.f3\endcsname{91.75}
\expandafter\gdef\csname R@v1.cv.acdc.L1.f4\endcsname{90.53}
\expandafter\gdef\csname R@v1.cv.acdc.L1.hi\endcsname{\ensuremath{+0.58}}
\expandafter\gdef\csname R@v1.cv.acdc.L1.lo\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@v1.cv.acdc.L1.mean\endcsname{91.38}
\expandafter\gdef\csname R@v1.cv.acdc.L1.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.acdc.L1.npos\endcsname{4}
\expandafter\gdef\csname R@v1.cv.acdc.L1b.d\endcsname{\ensuremath{+0.29}}
\expandafter\gdef\csname R@v1.cv.acdc.L1b.dabs\endcsname{0.29}
\expandafter\gdef\csname R@v1.cv.acdc.L1b.f1\endcsname{91.38}
\expandafter\gdef\csname R@v1.cv.acdc.L1b.f2\endcsname{91.62}
\expandafter\gdef\csname R@v1.cv.acdc.L1b.f3\endcsname{91.54}
\expandafter\gdef\csname R@v1.cv.acdc.L1b.f4\endcsname{90.39}
\expandafter\gdef\csname R@v1.cv.acdc.L1b.hi\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@v1.cv.acdc.L1b.lo\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@v1.cv.acdc.L1b.mean\endcsname{91.23}
\expandafter\gdef\csname R@v1.cv.acdc.L1b.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.acdc.L1b.npos\endcsname{4}
\expandafter\gdef\csname R@v1.cv.acdc.L3.d\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@v1.cv.acdc.L3.dabs\endcsname{0.33}
\expandafter\gdef\csname R@v1.cv.acdc.L3.f1\endcsname{91.59}
\expandafter\gdef\csname R@v1.cv.acdc.L3.f2\endcsname{91.71}
\expandafter\gdef\csname R@v1.cv.acdc.L3.f3\endcsname{91.53}
\expandafter\gdef\csname R@v1.cv.acdc.L3.f4\endcsname{90.29}
\expandafter\gdef\csname R@v1.cv.acdc.L3.hi\endcsname{\ensuremath{+0.48}}
\expandafter\gdef\csname R@v1.cv.acdc.L3.lo\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@v1.cv.acdc.L3.mean\endcsname{91.28}
\expandafter\gdef\csname R@v1.cv.acdc.L3.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.acdc.L3.npos\endcsname{4}
\expandafter\gdef\csname R@v1.cv.acdc.P3c.d\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@v1.cv.acdc.P3c.dabs\endcsname{0.09}
\expandafter\gdef\csname R@v1.cv.acdc.P3c.f1\endcsname{90.97}
\expandafter\gdef\csname R@v1.cv.acdc.P3c.f2\endcsname{91.06}
\expandafter\gdef\csname R@v1.cv.acdc.P3c.f3\endcsname{91.36}
\expandafter\gdef\csname R@v1.cv.acdc.P3c.f4\endcsname{90.02}
\expandafter\gdef\csname R@v1.cv.acdc.P3c.hi\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@v1.cv.acdc.P3c.lo\endcsname{\ensuremath{-0.35}}
\expandafter\gdef\csname R@v1.cv.acdc.P3c.mean\endcsname{90.85}
\expandafter\gdef\csname R@v1.cv.acdc.P3c.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.acdc.P3c.npos\endcsname{2}
\expandafter\gdef\csname R@v1.cv.acdc.V5B1.d\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@v1.cv.acdc.V5B1.dabs\endcsname{0.13}
\expandafter\gdef\csname R@v1.cv.acdc.V5B1.f1\endcsname{91.23}
\expandafter\gdef\csname R@v1.cv.acdc.V5B1.f2\endcsname{91.27}
\expandafter\gdef\csname R@v1.cv.acdc.V5B1.f3\endcsname{91.05}
\expandafter\gdef\csname R@v1.cv.acdc.V5B1.f4\endcsname{89.72}
\expandafter\gdef\csname R@v1.cv.acdc.V5B1.hi\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@v1.cv.acdc.V5B1.lo\endcsname{\ensuremath{-0.38}}
\expandafter\gdef\csname R@v1.cv.acdc.V5B1.mean\endcsname{90.82}
\expandafter\gdef\csname R@v1.cv.acdc.V5B1.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.acdc.V5B1.npos\endcsname{1}
\expandafter\gdef\csname R@v1.cv.acdc.V5B2.d\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@v1.cv.acdc.V5B2.dabs\endcsname{0.09}
\expandafter\gdef\csname R@v1.cv.acdc.V5B2.f1\endcsname{90.85}
\expandafter\gdef\csname R@v1.cv.acdc.V5B2.f2\endcsname{91.36}
\expandafter\gdef\csname R@v1.cv.acdc.V5B2.f3\endcsname{91.24}
\expandafter\gdef\csname R@v1.cv.acdc.V5B2.f4\endcsname{89.97}
\expandafter\gdef\csname R@v1.cv.acdc.V5B2.hi\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@v1.cv.acdc.V5B2.lo\endcsname{\ensuremath{-0.36}}
\expandafter\gdef\csname R@v1.cv.acdc.V5B2.mean\endcsname{90.86}
\expandafter\gdef\csname R@v1.cv.acdc.V5B2.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.acdc.V5B2.npos\endcsname{2}
\expandafter\gdef\csname R@v1.cv.acdc.V6A1r.d\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@v1.cv.acdc.V6A1r.dabs\endcsname{0.42}
\expandafter\gdef\csname R@v1.cv.acdc.V6A1r.f1\endcsname{91.67}
\expandafter\gdef\csname R@v1.cv.acdc.V6A1r.f2\endcsname{91.70}
\expandafter\gdef\csname R@v1.cv.acdc.V6A1r.f3\endcsname{91.65}
\expandafter\gdef\csname R@v1.cv.acdc.V6A1r.f4\endcsname{90.45}
\expandafter\gdef\csname R@v1.cv.acdc.V6A1r.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@v1.cv.acdc.V6A1r.lo\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@v1.cv.acdc.V6A1r.mean\endcsname{91.37}
\expandafter\gdef\csname R@v1.cv.acdc.V6A1r.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.acdc.V6A1r.npos\endcsname{4}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1.d\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1.dabs\endcsname{0.17}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1.f1\endcsname{91.30}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1.f2\endcsname{91.49}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1.f3\endcsname{91.13}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1.f4\endcsname{90.53}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1.hi\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1.lo\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1.mean\endcsname{91.11}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1.npos\endcsname{3}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1cov.d\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1cov.dabs\endcsname{0.14}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1cov.f1\endcsname{91.30}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1cov.f2\endcsname{91.35}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1cov.f3\endcsname{91.26}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1cov.f4\endcsname{90.43}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1cov.hi\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1cov.lo\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1cov.mean\endcsname{91.08}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1cov.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.acdc.V7A1cov.npos\endcsname{3}
\expandafter\gdef\csname R@v1.cv.acdc.V7C1.d\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@v1.cv.acdc.V7C1.dabs\endcsname{0.11}
\expandafter\gdef\csname R@v1.cv.acdc.V7C1.f1\endcsname{90.99}
\expandafter\gdef\csname R@v1.cv.acdc.V7C1.f2\endcsname{91.24}
\expandafter\gdef\csname R@v1.cv.acdc.V7C1.f3\endcsname{91.18}
\expandafter\gdef\csname R@v1.cv.acdc.V7C1.f4\endcsname{89.91}
\expandafter\gdef\csname R@v1.cv.acdc.V7C1.hi\endcsname{\ensuremath{-0.01}}
\expandafter\gdef\csname R@v1.cv.acdc.V7C1.lo\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@v1.cv.acdc.V7C1.mean\endcsname{90.83}
\expandafter\gdef\csname R@v1.cv.acdc.V7C1.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.acdc.V7C1.npos\endcsname{0}
\expandafter\gdef\csname R@v1.cv.acdc.V9R2.d\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@v1.cv.acdc.V9R2.dabs\endcsname{0.12}
\expandafter\gdef\csname R@v1.cv.acdc.V9R2.f1\endcsname{91.32}
\expandafter\gdef\csname R@v1.cv.acdc.V9R2.f2\endcsname{91.58}
\expandafter\gdef\csname R@v1.cv.acdc.V9R2.f3\endcsname{91.11}
\expandafter\gdef\csname R@v1.cv.acdc.V9R2.f4\endcsname{90.27}
\expandafter\gdef\csname R@v1.cv.acdc.V9R2.hi\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@v1.cv.acdc.V9R2.lo\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@v1.cv.acdc.V9R2.mean\endcsname{91.07}
\expandafter\gdef\csname R@v1.cv.acdc.V9R2.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.acdc.V9R2.npos\endcsname{3}
\expandafter\gdef\csname R@v1.cv.acdc.base.f1\endcsname{91.18}
\expandafter\gdef\csname R@v1.cv.acdc.base.f2\endcsname{91.31}
\expandafter\gdef\csname R@v1.cv.acdc.base.f3\endcsname{91.32}
\expandafter\gdef\csname R@v1.cv.acdc.base.f4\endcsname{89.97}
\expandafter\gdef\csname R@v1.cv.acdc.base.mean\endcsname{90.94}
\expandafter\gdef\csname R@v1.cv.amos.D2.d\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@v1.cv.amos.D2.dabs\endcsname{0.44}
\expandafter\gdef\csname R@v1.cv.amos.D2.f1\endcsname{88.83}
\expandafter\gdef\csname R@v1.cv.amos.D2.f2\endcsname{87.92}
\expandafter\gdef\csname R@v1.cv.amos.D2.f3\endcsname{88.14}
\expandafter\gdef\csname R@v1.cv.amos.D2.f4\endcsname{86.74}
\expandafter\gdef\csname R@v1.cv.amos.D2.hi\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@v1.cv.amos.D2.lo\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@v1.cv.amos.D2.mean\endcsname{87.91}
\expandafter\gdef\csname R@v1.cv.amos.D2.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.amos.D2.npos\endcsname{0}
\expandafter\gdef\csname R@v1.cv.amos.L1.d\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@v1.cv.amos.L1.dabs\endcsname{0.41}
\expandafter\gdef\csname R@v1.cv.amos.L1.f1\endcsname{89.46}
\expandafter\gdef\csname R@v1.cv.amos.L1.f2\endcsname{89.25}
\expandafter\gdef\csname R@v1.cv.amos.L1.f3\endcsname{88.63}
\expandafter\gdef\csname R@v1.cv.amos.L1.f4\endcsname{87.68}
\expandafter\gdef\csname R@v1.cv.amos.L1.hi\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@v1.cv.amos.L1.lo\endcsname{\ensuremath{-0.27}}
\expandafter\gdef\csname R@v1.cv.amos.L1.mean\endcsname{88.75}
\expandafter\gdef\csname R@v1.cv.amos.L1.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.amos.L1.npos\endcsname{3}
\expandafter\gdef\csname R@v1.cv.amos.L1b.d\endcsname{\ensuremath{+0.43}}
\expandafter\gdef\csname R@v1.cv.amos.L1b.dabs\endcsname{0.43}
\expandafter\gdef\csname R@v1.cv.amos.L1b.f1\endcsname{89.63}
\expandafter\gdef\csname R@v1.cv.amos.L1b.f2\endcsname{89.03}
\expandafter\gdef\csname R@v1.cv.amos.L1b.f3\endcsname{88.69}
\expandafter\gdef\csname R@v1.cv.amos.L1b.f4\endcsname{87.74}
\expandafter\gdef\csname R@v1.cv.amos.L1b.hi\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@v1.cv.amos.L1b.lo\endcsname{\ensuremath{-0.16}}
\expandafter\gdef\csname R@v1.cv.amos.L1b.mean\endcsname{88.78}
\expandafter\gdef\csname R@v1.cv.amos.L1b.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.amos.L1b.npos\endcsname{3}
\expandafter\gdef\csname R@v1.cv.amos.L3.d\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@v1.cv.amos.L3.dabs\endcsname{0.23}
\expandafter\gdef\csname R@v1.cv.amos.L3.f1\endcsname{89.09}
\expandafter\gdef\csname R@v1.cv.amos.L3.f2\endcsname{88.84}
\expandafter\gdef\csname R@v1.cv.amos.L3.f3\endcsname{88.99}
\expandafter\gdef\csname R@v1.cv.amos.L3.f4\endcsname{87.38}
\expandafter\gdef\csname R@v1.cv.amos.L3.hi\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@v1.cv.amos.L3.lo\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@v1.cv.amos.L3.mean\endcsname{88.58}
\expandafter\gdef\csname R@v1.cv.amos.L3.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.amos.L3.npos\endcsname{3}
\expandafter\gdef\csname R@v1.cv.amos.P3c.d\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@v1.cv.amos.P3c.dabs\endcsname{0.03}
\expandafter\gdef\csname R@v1.cv.amos.P3c.f1\endcsname{88.77}
\expandafter\gdef\csname R@v1.cv.amos.P3c.f2\endcsname{88.64}
\expandafter\gdef\csname R@v1.cv.amos.P3c.f3\endcsname{88.52}
\expandafter\gdef\csname R@v1.cv.amos.P3c.f4\endcsname{87.34}
\expandafter\gdef\csname R@v1.cv.amos.P3c.hi\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@v1.cv.amos.P3c.lo\endcsname{\ensuremath{-0.57}}
\expandafter\gdef\csname R@v1.cv.amos.P3c.mean\endcsname{88.32}
\expandafter\gdef\csname R@v1.cv.amos.P3c.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.amos.P3c.npos\endcsname{2}
\expandafter\gdef\csname R@v1.cv.amos.V5B1.d\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@v1.cv.amos.V5B1.dabs\endcsname{0.46}
\expandafter\gdef\csname R@v1.cv.amos.V5B1.f1\endcsname{88.65}
\expandafter\gdef\csname R@v1.cv.amos.V5B1.f2\endcsname{88.11}
\expandafter\gdef\csname R@v1.cv.amos.V5B1.f3\endcsname{88.03}
\expandafter\gdef\csname R@v1.cv.amos.V5B1.f4\endcsname{86.76}
\expandafter\gdef\csname R@v1.cv.amos.V5B1.hi\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@v1.cv.amos.V5B1.lo\endcsname{\ensuremath{-0.82}}
\expandafter\gdef\csname R@v1.cv.amos.V5B1.mean\endcsname{87.89}
\expandafter\gdef\csname R@v1.cv.amos.V5B1.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.amos.V5B1.npos\endcsname{0}
\expandafter\gdef\csname R@v1.cv.amos.V5B2.d\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@v1.cv.amos.V5B2.dabs\endcsname{0.25}
\expandafter\gdef\csname R@v1.cv.amos.V5B2.f1\endcsname{88.56}
\expandafter\gdef\csname R@v1.cv.amos.V5B2.f2\endcsname{88.28}
\expandafter\gdef\csname R@v1.cv.amos.V5B2.f3\endcsname{88.30}
\expandafter\gdef\csname R@v1.cv.amos.V5B2.f4\endcsname{87.23}
\expandafter\gdef\csname R@v1.cv.amos.V5B2.hi\endcsname{\ensuremath{+0.32}}
\expandafter\gdef\csname R@v1.cv.amos.V5B2.lo\endcsname{\ensuremath{-0.83}}
\expandafter\gdef\csname R@v1.cv.amos.V5B2.mean\endcsname{88.09}
\expandafter\gdef\csname R@v1.cv.amos.V5B2.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.amos.V5B2.npos\endcsname{1}
\expandafter\gdef\csname R@v1.cv.amos.V6A1r.d\endcsname{\ensuremath{+0.20}}
\expandafter\gdef\csname R@v1.cv.amos.V6A1r.dabs\endcsname{0.20}
\expandafter\gdef\csname R@v1.cv.amos.V6A1r.f1\endcsname{89.02}
\expandafter\gdef\csname R@v1.cv.amos.V6A1r.f2\endcsname{88.68}
\expandafter\gdef\csname R@v1.cv.amos.V6A1r.f3\endcsname{88.82}
\expandafter\gdef\csname R@v1.cv.amos.V6A1r.f4\endcsname{87.67}
\expandafter\gdef\csname R@v1.cv.amos.V6A1r.hi\endcsname{\ensuremath{+0.74}}
\expandafter\gdef\csname R@v1.cv.amos.V6A1r.lo\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@v1.cv.amos.V6A1r.mean\endcsname{88.55}
\expandafter\gdef\csname R@v1.cv.amos.V6A1r.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.amos.V6A1r.npos\endcsname{3}
\expandafter\gdef\csname R@v1.cv.amos.V7A1.d\endcsname{\ensuremath{+0.26}}
\expandafter\gdef\csname R@v1.cv.amos.V7A1.dabs\endcsname{0.26}
\expandafter\gdef\csname R@v1.cv.amos.V7A1.f1\endcsname{88.96}
\expandafter\gdef\csname R@v1.cv.amos.V7A1.f2\endcsname{88.99}
\expandafter\gdef\csname R@v1.cv.amos.V7A1.f3\endcsname{88.66}
\expandafter\gdef\csname R@v1.cv.amos.V7A1.f4\endcsname{87.80}
\expandafter\gdef\csname R@v1.cv.amos.V7A1.hi\endcsname{\ensuremath{+1.02}}
\expandafter\gdef\csname R@v1.cv.amos.V7A1.lo\endcsname{\ensuremath{-0.50}}
\expandafter\gdef\csname R@v1.cv.amos.V7A1.mean\endcsname{88.61}
\expandafter\gdef\csname R@v1.cv.amos.V7A1.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.amos.V7A1.npos\endcsname{2}
\expandafter\gdef\csname R@v1.cv.amos.V7A1cov.d\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@v1.cv.amos.V7A1cov.dabs\endcsname{0.19}
\expandafter\gdef\csname R@v1.cv.amos.V7A1cov.f1\endcsname{89.23}
\expandafter\gdef\csname R@v1.cv.amos.V7A1cov.f2\endcsname{88.75}
\expandafter\gdef\csname R@v1.cv.amos.V7A1cov.f3\endcsname{88.51}
\expandafter\gdef\csname R@v1.cv.amos.V7A1cov.f4\endcsname{87.66}
\expandafter\gdef\csname R@v1.cv.amos.V7A1cov.hi\endcsname{\ensuremath{+0.81}}
\expandafter\gdef\csname R@v1.cv.amos.V7A1cov.lo\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@v1.cv.amos.V7A1cov.mean\endcsname{88.54}
\expandafter\gdef\csname R@v1.cv.amos.V7A1cov.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.amos.V7A1cov.npos\endcsname{3}
\expandafter\gdef\csname R@v1.cv.amos.V7C1.d\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@v1.cv.amos.V7C1.dabs\endcsname{0.46}
\expandafter\gdef\csname R@v1.cv.amos.V7C1.f1\endcsname{88.54}
\expandafter\gdef\csname R@v1.cv.amos.V7C1.f2\endcsname{88.20}
\expandafter\gdef\csname R@v1.cv.amos.V7C1.f3\endcsname{88.09}
\expandafter\gdef\csname R@v1.cv.amos.V7C1.f4\endcsname{86.72}
\expandafter\gdef\csname R@v1.cv.amos.V7C1.hi\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@v1.cv.amos.V7C1.lo\endcsname{\ensuremath{-0.81}}
\expandafter\gdef\csname R@v1.cv.amos.V7C1.mean\endcsname{87.89}
\expandafter\gdef\csname R@v1.cv.amos.V7C1.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.amos.V7C1.npos\endcsname{0}
\expandafter\gdef\csname R@v1.cv.amos.V9R2.d\endcsname{\ensuremath{+0.16}}
\expandafter\gdef\csname R@v1.cv.amos.V9R2.dabs\endcsname{0.16}
\expandafter\gdef\csname R@v1.cv.amos.V9R2.f1\endcsname{89.22}
\expandafter\gdef\csname R@v1.cv.amos.V9R2.f2\endcsname{89.04}
\expandafter\gdef\csname R@v1.cv.amos.V9R2.f3\endcsname{88.45}
\expandafter\gdef\csname R@v1.cv.amos.V9R2.f4\endcsname{87.32}
\expandafter\gdef\csname R@v1.cv.amos.V9R2.hi\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@v1.cv.amos.V9R2.lo\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@v1.cv.amos.V9R2.mean\endcsname{88.51}
\expandafter\gdef\csname R@v1.cv.amos.V9R2.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.amos.V9R2.npos\endcsname{3}
\expandafter\gdef\csname R@v1.cv.amos.Y2.d\endcsname{\ensuremath{+0.23}}
\expandafter\gdef\csname R@v1.cv.amos.Y2.dabs\endcsname{0.23}
\expandafter\gdef\csname R@v1.cv.amos.Y2.f1\endcsname{89.09}
\expandafter\gdef\csname R@v1.cv.amos.Y2.f2\endcsname{89.02}
\expandafter\gdef\csname R@v1.cv.amos.Y2.f3\endcsname{88.54}
\expandafter\gdef\csname R@v1.cv.amos.Y2.f4\endcsname{87.65}
\expandafter\gdef\csname R@v1.cv.amos.Y2.hi\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@v1.cv.amos.Y2.lo\endcsname{\ensuremath{-0.47}}
\expandafter\gdef\csname R@v1.cv.amos.Y2.mean\endcsname{88.57}
\expandafter\gdef\csname R@v1.cv.amos.Y2.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.amos.Y2.npos\endcsname{2}
\expandafter\gdef\csname R@v1.cv.amos.base.f1\endcsname{89.12}
\expandafter\gdef\csname R@v1.cv.amos.base.f2\endcsname{88.48}
\expandafter\gdef\csname R@v1.cv.amos.base.f3\endcsname{88.80}
\expandafter\gdef\csname R@v1.cv.amos.base.f4\endcsname{87.00}
\expandafter\gdef\csname R@v1.cv.amos.base.mean\endcsname{88.35}
\expandafter\gdef\csname R@v1.cv.kits.D2.d\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@v1.cv.kits.D2.dabs\endcsname{1.04}
\expandafter\gdef\csname R@v1.cv.kits.D2.f1\endcsname{84.58}
\expandafter\gdef\csname R@v1.cv.kits.D2.f2\endcsname{84.62}
\expandafter\gdef\csname R@v1.cv.kits.D2.f3\endcsname{87.94}
\expandafter\gdef\csname R@v1.cv.kits.D2.f4\endcsname{83.01}
\expandafter\gdef\csname R@v1.cv.kits.D2.hi\endcsname{\ensuremath{+2.12}}
\expandafter\gdef\csname R@v1.cv.kits.D2.lo\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@v1.cv.kits.D2.mean\endcsname{85.04}
\expandafter\gdef\csname R@v1.cv.kits.D2.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.kits.D2.npos\endcsname{4}
\expandafter\gdef\csname R@v1.cv.kits.L1.d\endcsname{\ensuremath{+2.15}}
\expandafter\gdef\csname R@v1.cv.kits.L1.dabs\endcsname{2.15}
\expandafter\gdef\csname R@v1.cv.kits.L1.f1\endcsname{85.44}
\expandafter\gdef\csname R@v1.cv.kits.L1.f2\endcsname{86.25}
\expandafter\gdef\csname R@v1.cv.kits.L1.f3\endcsname{88.27}
\expandafter\gdef\csname R@v1.cv.kits.L1.f4\endcsname{84.60}
\expandafter\gdef\csname R@v1.cv.kits.L1.hi\endcsname{\ensuremath{+3.32}}
\expandafter\gdef\csname R@v1.cv.kits.L1.lo\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@v1.cv.kits.L1.mean\endcsname{86.14}
\expandafter\gdef\csname R@v1.cv.kits.L1.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.kits.L1.npos\endcsname{4}
\expandafter\gdef\csname R@v1.cv.kits.L1b.d\endcsname{\ensuremath{+1.54}}
\expandafter\gdef\csname R@v1.cv.kits.L1b.dabs\endcsname{1.54}
\expandafter\gdef\csname R@v1.cv.kits.L1b.f1\endcsname{85.21}
\expandafter\gdef\csname R@v1.cv.kits.L1b.f2\endcsname{84.96}
\expandafter\gdef\csname R@v1.cv.kits.L1b.f3\endcsname{88.40}
\expandafter\gdef\csname R@v1.cv.kits.L1b.f4\endcsname{83.58}
\expandafter\gdef\csname R@v1.cv.kits.L1b.hi\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@v1.cv.kits.L1b.lo\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@v1.cv.kits.L1b.mean\endcsname{85.54}
\expandafter\gdef\csname R@v1.cv.kits.L1b.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.kits.L1b.npos\endcsname{4}
\expandafter\gdef\csname R@v1.cv.kits.L3.d\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@v1.cv.kits.L3.dabs\endcsname{0.68}
\expandafter\gdef\csname R@v1.cv.kits.L3.f1\endcsname{85.17}
\expandafter\gdef\csname R@v1.cv.kits.L3.f2\endcsname{83.51}
\expandafter\gdef\csname R@v1.cv.kits.L3.f3\endcsname{87.29}
\expandafter\gdef\csname R@v1.cv.kits.L3.f4\endcsname{82.74}
\expandafter\gdef\csname R@v1.cv.kits.L3.hi\endcsname{\ensuremath{+2.44}}
\expandafter\gdef\csname R@v1.cv.kits.L3.lo\endcsname{\ensuremath{-1.08}}
\expandafter\gdef\csname R@v1.cv.kits.L3.mean\endcsname{84.67}
\expandafter\gdef\csname R@v1.cv.kits.L3.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.kits.L3.npos\endcsname{3}
\expandafter\gdef\csname R@v1.cv.kits.P3c.d\endcsname{\ensuremath{+0.56}}
\expandafter\gdef\csname R@v1.cv.kits.P3c.dabs\endcsname{0.56}
\expandafter\gdef\csname R@v1.cv.kits.P3c.f1\endcsname{85.24}
\expandafter\gdef\csname R@v1.cv.kits.P3c.f2\endcsname{83.41}
\expandafter\gdef\csname R@v1.cv.kits.P3c.f3\endcsname{87.68}
\expandafter\gdef\csname R@v1.cv.kits.P3c.f4\endcsname{81.87}
\expandafter\gdef\csname R@v1.cv.kits.P3c.hi\endcsname{\ensuremath{+2.82}}
\expandafter\gdef\csname R@v1.cv.kits.P3c.lo\endcsname{\ensuremath{-1.71}}
\expandafter\gdef\csname R@v1.cv.kits.P3c.mean\endcsname{84.55}
\expandafter\gdef\csname R@v1.cv.kits.P3c.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.kits.P3c.npos\endcsname{3}
\expandafter\gdef\csname R@v1.cv.kits.V5B1.d\endcsname{\ensuremath{+0.99}}
\expandafter\gdef\csname R@v1.cv.kits.V5B1.dabs\endcsname{0.99}
\expandafter\gdef\csname R@v1.cv.kits.V5B1.f1\endcsname{84.58}
\expandafter\gdef\csname R@v1.cv.kits.V5B1.f2\endcsname{85.20}
\expandafter\gdef\csname R@v1.cv.kits.V5B1.f3\endcsname{87.50}
\expandafter\gdef\csname R@v1.cv.kits.V5B1.f4\endcsname{82.66}
\expandafter\gdef\csname R@v1.cv.kits.V5B1.hi\endcsname{\ensuremath{+2.58}}
\expandafter\gdef\csname R@v1.cv.kits.V5B1.lo\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@v1.cv.kits.V5B1.mean\endcsname{84.99}
\expandafter\gdef\csname R@v1.cv.kits.V5B1.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.kits.V5B1.npos\endcsname{3}
\expandafter\gdef\csname R@v1.cv.kits.V5B2.d\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@v1.cv.kits.V5B2.dabs\endcsname{0.75}
\expandafter\gdef\csname R@v1.cv.kits.V5B2.f1\endcsname{83.53}
\expandafter\gdef\csname R@v1.cv.kits.V5B2.f2\endcsname{82.53}
\expandafter\gdef\csname R@v1.cv.kits.V5B2.f3\endcsname{86.32}
\expandafter\gdef\csname R@v1.cv.kits.V5B2.f4\endcsname{80.59}
\expandafter\gdef\csname R@v1.cv.kits.V5B2.hi\endcsname{\ensuremath{+1.18}}
\expandafter\gdef\csname R@v1.cv.kits.V5B2.lo\endcsname{\ensuremath{-2.69}}
\expandafter\gdef\csname R@v1.cv.kits.V5B2.mean\endcsname{83.24}
\expandafter\gdef\csname R@v1.cv.kits.V5B2.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.kits.V5B2.npos\endcsname{1}
\expandafter\gdef\csname R@v1.cv.kits.V6A1r.d\endcsname{\ensuremath{+0.28}}
\expandafter\gdef\csname R@v1.cv.kits.V6A1r.dabs\endcsname{0.28}
\expandafter\gdef\csname R@v1.cv.kits.V6A1r.f1\endcsname{84.22}
\expandafter\gdef\csname R@v1.cv.kits.V6A1r.f2\endcsname{82.53}
\expandafter\gdef\csname R@v1.cv.kits.V6A1r.f3\endcsname{87.94}
\expandafter\gdef\csname R@v1.cv.kits.V6A1r.f4\endcsname{82.41}
\expandafter\gdef\csname R@v1.cv.kits.V6A1r.hi\endcsname{\ensuremath{+1.98}}
\expandafter\gdef\csname R@v1.cv.kits.V6A1r.lo\endcsname{\ensuremath{-1.42}}
\expandafter\gdef\csname R@v1.cv.kits.V6A1r.mean\endcsname{84.27}
\expandafter\gdef\csname R@v1.cv.kits.V6A1r.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.kits.V6A1r.npos\endcsname{2}
\expandafter\gdef\csname R@v1.cv.kits.V7A1.d\endcsname{\ensuremath{+1.63}}
\expandafter\gdef\csname R@v1.cv.kits.V7A1.dabs\endcsname{1.63}
\expandafter\gdef\csname R@v1.cv.kits.V7A1.f1\endcsname{84.89}
\expandafter\gdef\csname R@v1.cv.kits.V7A1.f2\endcsname{85.71}
\expandafter\gdef\csname R@v1.cv.kits.V7A1.f3\endcsname{88.89}
\expandafter\gdef\csname R@v1.cv.kits.V7A1.f4\endcsname{83.01}
\expandafter\gdef\csname R@v1.cv.kits.V7A1.hi\endcsname{\ensuremath{+3.27}}
\expandafter\gdef\csname R@v1.cv.kits.V7A1.lo\endcsname{\ensuremath{0.00}}
\expandafter\gdef\csname R@v1.cv.kits.V7A1.mean\endcsname{85.63}
\expandafter\gdef\csname R@v1.cv.kits.V7A1.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.kits.V7A1.npos\endcsname{4}
\expandafter\gdef\csname R@v1.cv.kits.V7A2.d\endcsname{\ensuremath{+0.91}}
\expandafter\gdef\csname R@v1.cv.kits.V7A2.dabs\endcsname{0.91}
\expandafter\gdef\csname R@v1.cv.kits.V7A2.f1\endcsname{84.67}
\expandafter\gdef\csname R@v1.cv.kits.V7A2.f2\endcsname{84.21}
\expandafter\gdef\csname R@v1.cv.kits.V7A2.f3\endcsname{88.06}
\expandafter\gdef\csname R@v1.cv.kits.V7A2.f4\endcsname{82.65}
\expandafter\gdef\csname R@v1.cv.kits.V7A2.hi\endcsname{\ensuremath{+2.27}}
\expandafter\gdef\csname R@v1.cv.kits.V7A2.lo\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@v1.cv.kits.V7A2.mean\endcsname{84.90}
\expandafter\gdef\csname R@v1.cv.kits.V7A2.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.kits.V7A2.npos\endcsname{3}
\expandafter\gdef\csname R@v1.cv.kits.V7C1.d\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@v1.cv.kits.V7C1.dabs\endcsname{0.78}
\expandafter\gdef\csname R@v1.cv.kits.V7C1.f1\endcsname{85.00}
\expandafter\gdef\csname R@v1.cv.kits.V7C1.f2\endcsname{84.05}
\expandafter\gdef\csname R@v1.cv.kits.V7C1.f3\endcsname{87.64}
\expandafter\gdef\csname R@v1.cv.kits.V7C1.f4\endcsname{82.42}
\expandafter\gdef\csname R@v1.cv.kits.V7C1.hi\endcsname{\ensuremath{+2.48}}
\expandafter\gdef\csname R@v1.cv.kits.V7C1.lo\endcsname{\ensuremath{-0.92}}
\expandafter\gdef\csname R@v1.cv.kits.V7C1.mean\endcsname{84.78}
\expandafter\gdef\csname R@v1.cv.kits.V7C1.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.kits.V7C1.npos\endcsname{3}
\expandafter\gdef\csname R@v1.cv.kits.V8B2.d\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@v1.cv.kits.V8B2.dabs\endcsname{0.24}
\expandafter\gdef\csname R@v1.cv.kits.V8B2.f1\endcsname{84.09}
\expandafter\gdef\csname R@v1.cv.kits.V8B2.f2\endcsname{83.33}
\expandafter\gdef\csname R@v1.cv.kits.V8B2.f3\endcsname{87.02}
\expandafter\gdef\csname R@v1.cv.kits.V8B2.f4\endcsname{80.56}
\expandafter\gdef\csname R@v1.cv.kits.V8B2.hi\endcsname{\ensuremath{+2.13}}
\expandafter\gdef\csname R@v1.cv.kits.V8B2.lo\endcsname{\ensuremath{-2.62}}
\expandafter\gdef\csname R@v1.cv.kits.V8B2.mean\endcsname{83.75}
\expandafter\gdef\csname R@v1.cv.kits.V8B2.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.kits.V8B2.npos\endcsname{3}
\expandafter\gdef\csname R@v1.cv.kits.V9R2.d\endcsname{\ensuremath{+1.33}}
\expandafter\gdef\csname R@v1.cv.kits.V9R2.dabs\endcsname{1.33}
\expandafter\gdef\csname R@v1.cv.kits.V9R2.f1\endcsname{84.47}
\expandafter\gdef\csname R@v1.cv.kits.V9R2.f2\endcsname{85.62}
\expandafter\gdef\csname R@v1.cv.kits.V9R2.f3\endcsname{88.89}
\expandafter\gdef\csname R@v1.cv.kits.V9R2.f4\endcsname{82.30}
\expandafter\gdef\csname R@v1.cv.kits.V9R2.hi\endcsname{\ensuremath{+3.42}}
\expandafter\gdef\csname R@v1.cv.kits.V9R2.lo\endcsname{\ensuremath{-0.76}}
\expandafter\gdef\csname R@v1.cv.kits.V9R2.mean\endcsname{85.32}
\expandafter\gdef\csname R@v1.cv.kits.V9R2.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.kits.V9R2.npos\endcsname{3}
\expandafter\gdef\csname R@v1.cv.kits.Y2.d\endcsname{\ensuremath{+2.71}}
\expandafter\gdef\csname R@v1.cv.kits.Y2.dabs\endcsname{2.71}
\expandafter\gdef\csname R@v1.cv.kits.Y2.f1\endcsname{86.33}
\expandafter\gdef\csname R@v1.cv.kits.Y2.f2\endcsname{86.28}
\expandafter\gdef\csname R@v1.cv.kits.Y2.f3\endcsname{89.25}
\expandafter\gdef\csname R@v1.cv.kits.Y2.f4\endcsname{84.93}
\expandafter\gdef\csname R@v1.cv.kits.Y2.hi\endcsname{\ensuremath{+3.73}}
\expandafter\gdef\csname R@v1.cv.kits.Y2.lo\endcsname{\ensuremath{+1.68}}
\expandafter\gdef\csname R@v1.cv.kits.Y2.mean\endcsname{86.70}
\expandafter\gdef\csname R@v1.cv.kits.Y2.n\endcsname{4}
\expandafter\gdef\csname R@v1.cv.kits.Y2.npos\endcsname{4}
\expandafter\gdef\csname R@v1.cv.kits.base.f1\endcsname{82.86}
\expandafter\gdef\csname R@v1.cv.kits.base.f2\endcsname{83.31}
\expandafter\gdef\csname R@v1.cv.kits.base.f3\endcsname{86.91}
\expandafter\gdef\csname R@v1.cv.kits.base.f4\endcsname{82.89}
\expandafter\gdef\csname R@v1.cv.kits.base.mean\endcsname{83.99}
\expandafter\gdef\csname R@v1.ho.V7A1.npos\endcsname{two}
\expandafter\gdef\csname R@v1.ho.V7C1.npos\endcsname{one}
\expandafter\gdef\csname R@v1.ho.brats.L1.d\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@v1.ho.brats.L1.mean\endcsname{82.95}
\expandafter\gdef\csname R@v1.ho.brats.L1.n\endcsname{1}
\expandafter\gdef\csname R@v1.ho.brats.L1.single\endcsname{1}
\expandafter\gdef\csname R@v1.ho.brats.L3.d\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@v1.ho.brats.L3.mean\endcsname{83.05}
\expandafter\gdef\csname R@v1.ho.brats.L3.n\endcsname{1}
\expandafter\gdef\csname R@v1.ho.brats.L3.single\endcsname{1}
\expandafter\gdef\csname R@v1.ho.brats.V7A1.d\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@v1.ho.brats.V7A1.mean\endcsname{83.17}
\expandafter\gdef\csname R@v1.ho.brats.V7A1.n\endcsname{3}
\expandafter\gdef\csname R@v1.ho.brats.V7A1.sd\endcsname{0.03}
\expandafter\gdef\csname R@v1.ho.brats.V7C1.d\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@v1.ho.brats.V7C1.mean\endcsname{83.15}
\expandafter\gdef\csname R@v1.ho.brats.V7C1.n\endcsname{3}
\expandafter\gdef\csname R@v1.ho.brats.V7C1.sd\endcsname{0.23}
\expandafter\gdef\csname R@v1.ho.brats.Y2.d\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@v1.ho.brats.Y2.mean\endcsname{83.10}
\expandafter\gdef\csname R@v1.ho.brats.Y2.n\endcsname{3}
\expandafter\gdef\csname R@v1.ho.brats.Y2.sd\endcsname{0.12}
\expandafter\gdef\csname R@v1.ho.brats.base.mean\endcsname{83.23}
\expandafter\gdef\csname R@v1.ho.brats.base.n\endcsname{3}
\expandafter\gdef\csname R@v1.ho.brats.base.sd\endcsname{0.23}
\expandafter\gdef\csname R@v1.ho.btcv.L1.d\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@v1.ho.btcv.L1.mean\endcsname{78.52}
\expandafter\gdef\csname R@v1.ho.btcv.L1.n\endcsname{3}
\expandafter\gdef\csname R@v1.ho.btcv.L1.sd\endcsname{0.62}
\expandafter\gdef\csname R@v1.ho.btcv.L3.d\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@v1.ho.btcv.L3.mean\endcsname{78.53}
\expandafter\gdef\csname R@v1.ho.btcv.L3.n\endcsname{3}
\expandafter\gdef\csname R@v1.ho.btcv.L3.sd\endcsname{1.05}
\expandafter\gdef\csname R@v1.ho.btcv.V7A1.d\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@v1.ho.btcv.V7A1.mean\endcsname{78.30}
\expandafter\gdef\csname R@v1.ho.btcv.V7A1.n\endcsname{3}
\expandafter\gdef\csname R@v1.ho.btcv.V7A1.sd\endcsname{0.11}
\expandafter\gdef\csname R@v1.ho.btcv.V7C1.d\endcsname{\ensuremath{-0.32}}
\expandafter\gdef\csname R@v1.ho.btcv.V7C1.mean\endcsname{77.50}
\expandafter\gdef\csname R@v1.ho.btcv.V7C1.n\endcsname{3}
\expandafter\gdef\csname R@v1.ho.btcv.V7C1.sd\endcsname{0.19}
\expandafter\gdef\csname R@v1.ho.btcv.base.mean\endcsname{77.82}
\expandafter\gdef\csname R@v1.ho.btcv.base.n\endcsname{3}
\expandafter\gdef\csname R@v1.ho.btcv.base.sd\endcsname{0.30}
\expandafter\gdef\csname R@v1.ho.lits.L1.d\endcsname{\ensuremath{+1.13}}
\expandafter\gdef\csname R@v1.ho.lits.L1.mean\endcsname{81.93}
\expandafter\gdef\csname R@v1.ho.lits.L1.n\endcsname{3}
\expandafter\gdef\csname R@v1.ho.lits.L1.sd\endcsname{0.25}
\expandafter\gdef\csname R@v1.ho.lits.L3.d\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@v1.ho.lits.L3.mean\endcsname{81.29}
\expandafter\gdef\csname R@v1.ho.lits.L3.n\endcsname{3}
\expandafter\gdef\csname R@v1.ho.lits.L3.sd\endcsname{0.76}
\expandafter\gdef\csname R@v1.ho.lits.V7A1.d\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@v1.ho.lits.V7A1.mean\endcsname{82.44}
\expandafter\gdef\csname R@v1.ho.lits.V7A1.n\endcsname{3}
\expandafter\gdef\csname R@v1.ho.lits.V7A1.sd\endcsname{1.51}
\expandafter\gdef\csname R@v1.ho.lits.V7C1.d\endcsname{\ensuremath{+0.85}}
\expandafter\gdef\csname R@v1.ho.lits.V7C1.mean\endcsname{81.65}
\expandafter\gdef\csname R@v1.ho.lits.V7C1.n\endcsname{3}
\expandafter\gdef\csname R@v1.ho.lits.V7C1.sd\endcsname{1.83}
\expandafter\gdef\csname R@v1.ho.lits.Y2.d\endcsname{\ensuremath{+1.65}}
\expandafter\gdef\csname R@v1.ho.lits.Y2.mean\endcsname{82.45}
\expandafter\gdef\csname R@v1.ho.lits.Y2.n\endcsname{3}
\expandafter\gdef\csname R@v1.ho.lits.Y2.sd\endcsname{0.95}
\expandafter\gdef\csname R@v1.ho.lits.base.mean\endcsname{80.79}
\expandafter\gdef\csname R@v1.ho.lits.base.n\endcsname{3}
\expandafter\gdef\csname R@v1.ho.lits.base.sd\endcsname{1.52}
\expandafter\gdef\csname R@v1.lin.stepstone\endcsname{1}
\expandafter\gdef\csname R@v1.nest.12.acdc\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@v1.nest.12.amos\endcsname{\ensuremath{+0.34}}
\expandafter\gdef\csname R@v1.nest.12.kits\endcsname{\ensuremath{+1.05}}
\expandafter\gdef\csname R@v1.nest.34.acdc\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@v1.nest.34.amos\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@v1.nest.34.kits\endcsname{\ensuremath{+2.22}}
\expandafter\gdef\csname R@v1.nest.n\endcsname{7}
\expandafter\gdef\csname R@v1.nest.pick12\endcsname{V7A1}
\expandafter\gdef\csname R@v1.nest.pick34\endcsname{V7A1}
\expandafter\gdef\csname R@v1.nest.robust\endcsname{1}
\expandafter\gdef\csname R@v1.organ.D2.aorta\endcsname{\ensuremath{-0.13}}
\expandafter\gdef\csname R@v1.organ.D2.bladder\endcsname{\ensuremath{-1.00}}
\expandafter\gdef\csname R@v1.organ.D2.duodenum\endcsname{\ensuremath{-0.45}}
\expandafter\gdef\csname R@v1.organ.D2.esophagus\endcsname{\ensuremath{-1.05}}
\expandafter\gdef\csname R@v1.organ.D2.gallbladder\endcsname{\ensuremath{-2.32}}
\expandafter\gdef\csname R@v1.organ.D2.ivc\endcsname{\ensuremath{-0.34}}
\expandafter\gdef\csname R@v1.organ.D2.ladrenal\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@v1.organ.D2.liver\endcsname{\ensuremath{-0.02}}
\expandafter\gdef\csname R@v1.organ.D2.lkidney\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@v1.organ.D2.pancreas\endcsname{\ensuremath{-0.71}}
\expandafter\gdef\csname R@v1.organ.D2.prostuterus\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@v1.organ.D2.radrenal\endcsname{\ensuremath{-0.71}}
\expandafter\gdef\csname R@v1.organ.D2.rkidney\endcsname{\ensuremath{-0.22}}
\expandafter\gdef\csname R@v1.organ.D2.spleen\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@v1.organ.D2.stomach\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@v1.organ.L1.aorta\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@v1.organ.L1.bladder\endcsname{\ensuremath{+1.44}}
\expandafter\gdef\csname R@v1.organ.L1.duodenum\endcsname{\ensuremath{+0.90}}
\expandafter\gdef\csname R@v1.organ.L1.esophagus\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@v1.organ.L1.gallbladder\endcsname{\ensuremath{+0.66}}
\expandafter\gdef\csname R@v1.organ.L1.ivc\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@v1.organ.L1.ladrenal\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@v1.organ.L1.liver\endcsname{\ensuremath{+0.11}}
\expandafter\gdef\csname R@v1.organ.L1.lkidney\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@v1.organ.L1.pancreas\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@v1.organ.L1.prostuterus\endcsname{\ensuremath{+2.01}}
\expandafter\gdef\csname R@v1.organ.L1.radrenal\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@v1.organ.L1.rkidney\endcsname{\ensuremath{+0.24}}
\expandafter\gdef\csname R@v1.organ.L1.spleen\endcsname{\ensuremath{+0.05}}
\expandafter\gdef\csname R@v1.organ.L1.stomach\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@v1.organ.L3.aorta\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@v1.organ.L3.bladder\endcsname{\ensuremath{+0.78}}
\expandafter\gdef\csname R@v1.organ.L3.duodenum\endcsname{\ensuremath{+0.51}}
\expandafter\gdef\csname R@v1.organ.L3.esophagus\endcsname{\ensuremath{+0.07}}
\expandafter\gdef\csname R@v1.organ.L3.gallbladder\endcsname{\ensuremath{+0.54}}
\expandafter\gdef\csname R@v1.organ.L3.ivc\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@v1.organ.L3.ladrenal\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@v1.organ.L3.liver\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@v1.organ.L3.lkidney\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@v1.organ.L3.pancreas\endcsname{\ensuremath{-0.56}}
\expandafter\gdef\csname R@v1.organ.L3.prostuterus\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@v1.organ.L3.radrenal\endcsname{\ensuremath{+0.46}}
\expandafter\gdef\csname R@v1.organ.L3.rkidney\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@v1.organ.L3.spleen\endcsname{\ensuremath{+0.03}}
\expandafter\gdef\csname R@v1.organ.L3.stomach\endcsname{\ensuremath{+0.92}}
\expandafter\gdef\csname R@v1.organ.V5B1.aorta\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@v1.organ.V5B1.bladder\endcsname{\ensuremath{-0.33}}
\expandafter\gdef\csname R@v1.organ.V5B1.duodenum\endcsname{\ensuremath{-0.29}}
\expandafter\gdef\csname R@v1.organ.V5B1.esophagus\endcsname{\ensuremath{-1.29}}
\expandafter\gdef\csname R@v1.organ.V5B1.gallbladder\endcsname{\ensuremath{-1.81}}
\expandafter\gdef\csname R@v1.organ.V5B1.ivc\endcsname{\ensuremath{-0.43}}
\expandafter\gdef\csname R@v1.organ.V5B1.ladrenal\endcsname{\ensuremath{-0.86}}
\expandafter\gdef\csname R@v1.organ.V5B1.liver\endcsname{\ensuremath{-0.10}}
\expandafter\gdef\csname R@v1.organ.V5B1.lkidney\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@v1.organ.V5B1.pancreas\endcsname{\ensuremath{-0.64}}
\expandafter\gdef\csname R@v1.organ.V5B1.prostuterus\endcsname{\ensuremath{+0.59}}
\expandafter\gdef\csname R@v1.organ.V5B1.radrenal\endcsname{\ensuremath{-0.76}}
\expandafter\gdef\csname R@v1.organ.V5B1.rkidney\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@v1.organ.V5B1.spleen\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@v1.organ.V5B1.stomach\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@v1.organ.V5B2.aorta\endcsname{\ensuremath{-0.04}}
\expandafter\gdef\csname R@v1.organ.V5B2.bladder\endcsname{\ensuremath{+0.30}}
\expandafter\gdef\csname R@v1.organ.V5B2.duodenum\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@v1.organ.V5B2.esophagus\endcsname{\ensuremath{-0.96}}
\expandafter\gdef\csname R@v1.organ.V5B2.gallbladder\endcsname{\ensuremath{-1.21}}
\expandafter\gdef\csname R@v1.organ.V5B2.ivc\endcsname{\ensuremath{-0.42}}
\expandafter\gdef\csname R@v1.organ.V5B2.ladrenal\endcsname{\ensuremath{-0.69}}
\expandafter\gdef\csname R@v1.organ.V5B2.liver\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@v1.organ.V5B2.lkidney\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@v1.organ.V5B2.pancreas\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@v1.organ.V5B2.prostuterus\endcsname{\ensuremath{+1.10}}
\expandafter\gdef\csname R@v1.organ.V5B2.radrenal\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@v1.organ.V5B2.rkidney\endcsname{\ensuremath{-0.17}}
\expandafter\gdef\csname R@v1.organ.V5B2.spleen\endcsname{\ensuremath{-0.03}}
\expandafter\gdef\csname R@v1.organ.V5B2.stomach\endcsname{\ensuremath{-0.18}}
\expandafter\gdef\csname R@v1.organ.V7A1.aorta\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@v1.organ.V7A1.bladder\endcsname{\ensuremath{+1.30}}
\expandafter\gdef\csname R@v1.organ.V7A1.duodenum\endcsname{\ensuremath{+0.42}}
\expandafter\gdef\csname R@v1.organ.V7A1.esophagus\endcsname{\ensuremath{-0.59}}
\expandafter\gdef\csname R@v1.organ.V7A1.gallbladder\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@v1.organ.V7A1.ivc\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@v1.organ.V7A1.ladrenal\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@v1.organ.V7A1.liver\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@v1.organ.V7A1.lkidney\endcsname{\ensuremath{-0.40}}
\expandafter\gdef\csname R@v1.organ.V7A1.pancreas\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@v1.organ.V7A1.prostuterus\endcsname{\ensuremath{+2.85}}
\expandafter\gdef\csname R@v1.organ.V7A1.radrenal\endcsname{\ensuremath{+0.09}}
\expandafter\gdef\csname R@v1.organ.V7A1.rkidney\endcsname{\ensuremath{+0.01}}
\expandafter\gdef\csname R@v1.organ.V7A1.spleen\endcsname{\ensuremath{+0.14}}
\expandafter\gdef\csname R@v1.organ.V7A1.stomach\endcsname{\ensuremath{+0.53}}
\expandafter\gdef\csname R@v1.organ.V7C1.aorta\endcsname{\ensuremath{-0.07}}
\expandafter\gdef\csname R@v1.organ.V7C1.bladder\endcsname{\ensuremath{-0.25}}
\expandafter\gdef\csname R@v1.organ.V7C1.duodenum\endcsname{\ensuremath{-0.74}}
\expandafter\gdef\csname R@v1.organ.V7C1.esophagus\endcsname{\ensuremath{-1.31}}
\expandafter\gdef\csname R@v1.organ.V7C1.gallbladder\endcsname{\ensuremath{-1.44}}
\expandafter\gdef\csname R@v1.organ.V7C1.ivc\endcsname{\ensuremath{-0.28}}
\expandafter\gdef\csname R@v1.organ.V7C1.ladrenal\endcsname{\ensuremath{-0.67}}
\expandafter\gdef\csname R@v1.organ.V7C1.liver\endcsname{\ensuremath{+0.06}}
\expandafter\gdef\csname R@v1.organ.V7C1.lkidney\endcsname{\ensuremath{-0.46}}
\expandafter\gdef\csname R@v1.organ.V7C1.pancreas\endcsname{\ensuremath{-0.64}}
\expandafter\gdef\csname R@v1.organ.V7C1.prostuterus\endcsname{\ensuremath{+0.50}}
\expandafter\gdef\csname R@v1.organ.V7C1.radrenal\endcsname{\ensuremath{-0.75}}
\expandafter\gdef\csname R@v1.organ.V7C1.rkidney\endcsname{\ensuremath{-0.51}}
\expandafter\gdef\csname R@v1.organ.V7C1.spleen\endcsname{\ensuremath{-0.09}}
\expandafter\gdef\csname R@v1.organ.V7C1.stomach\endcsname{\ensuremath{-0.24}}
\expandafter\gdef\csname R@v1.pc.L1.kidney\endcsname{97.21}
\expandafter\gdef\csname R@v1.pc.L1.kidney.d\endcsname{\ensuremath{+0.87}}
\expandafter\gdef\csname R@v1.pc.L1.kidney.se\endcsname{0.26}
\expandafter\gdef\csname R@v1.pc.L1.masses\endcsname{83.99}
\expandafter\gdef\csname R@v1.pc.L1.masses.d\endcsname{\ensuremath{+3.01}}
\expandafter\gdef\csname R@v1.pc.L1.masses.se\endcsname{0.71}
\expandafter\gdef\csname R@v1.pc.L1.tumour\endcsname{79.37}
\expandafter\gdef\csname R@v1.pc.L1.tumour.d\endcsname{\ensuremath{+3.90}}
\expandafter\gdef\csname R@v1.pc.L1.tumour.se\endcsname{0.74}
\expandafter\gdef\csname R@v1.pc.L3.kidney\endcsname{96.95}
\expandafter\gdef\csname R@v1.pc.L3.kidney.d\endcsname{\ensuremath{+0.61}}
\expandafter\gdef\csname R@v1.pc.L3.kidney.se\endcsname{0.26}
\expandafter\gdef\csname R@v1.pc.L3.masses\endcsname{82.86}
\expandafter\gdef\csname R@v1.pc.L3.masses.d\endcsname{\ensuremath{+1.89}}
\expandafter\gdef\csname R@v1.pc.L3.masses.se\endcsname{0.71}
\expandafter\gdef\csname R@v1.pc.L3.tumour\endcsname{76.61}
\expandafter\gdef\csname R@v1.pc.L3.tumour.d\endcsname{\ensuremath{+1.15}}
\expandafter\gdef\csname R@v1.pc.L3.tumour.se\endcsname{0.74}
\expandafter\gdef\csname R@v1.pc.V7A1.kidney\endcsname{97.17}
\expandafter\gdef\csname R@v1.pc.V7A1.kidney.d\endcsname{\ensuremath{+0.83}}
\expandafter\gdef\csname R@v1.pc.V7A1.kidney.se\endcsname{0.26}
\expandafter\gdef\csname R@v1.pc.V7A1.masses\endcsname{83.28}
\expandafter\gdef\csname R@v1.pc.V7A1.masses.d\endcsname{\ensuremath{+2.31}}
\expandafter\gdef\csname R@v1.pc.V7A1.masses.se\endcsname{0.71}
\expandafter\gdef\csname R@v1.pc.V7A1.tumour\endcsname{77.67}
\expandafter\gdef\csname R@v1.pc.V7A1.tumour.d\endcsname{\ensuremath{+2.21}}
\expandafter\gdef\csname R@v1.pc.V7A1.tumour.se\endcsname{0.74}
\expandafter\gdef\csname R@v1.pc.V7C1.kidney\endcsname{97.27}
\expandafter\gdef\csname R@v1.pc.V7C1.kidney.d\endcsname{\ensuremath{+0.93}}
\expandafter\gdef\csname R@v1.pc.V7C1.kidney.se\endcsname{0.26}
\expandafter\gdef\csname R@v1.pc.V7C1.masses\endcsname{82.85}
\expandafter\gdef\csname R@v1.pc.V7C1.masses.d\endcsname{\ensuremath{+1.88}}
\expandafter\gdef\csname R@v1.pc.V7C1.masses.se\endcsname{0.71}
\expandafter\gdef\csname R@v1.pc.V7C1.mean3\endcsname{85.82}
\expandafter\gdef\csname R@v1.pc.V7C1.tumour\endcsname{77.33}
\expandafter\gdef\csname R@v1.pc.V7C1.tumour.d\endcsname{\ensuremath{+1.87}}
\expandafter\gdef\csname R@v1.pc.V7C1.tumour.se\endcsname{0.74}
\expandafter\gdef\csname R@v1.pc.base.kidney\endcsname{96.34}
\expandafter\gdef\csname R@v1.pc.base.masses\endcsname{80.97}
\expandafter\gdef\csname R@v1.pc.base.tumour\endcsname{75.46}
\expandafter\gdef\csname R@v1.pub.mednextl3.acdc.d\endcsname{\ensuremath{+1.11}}
\expandafter\gdef\csname R@v1.pub.mednextl3.amos.d\endcsname{\ensuremath{+0.98}}
\expandafter\gdef\csname R@v1.pub.mednextl3.kits.d\endcsname{\ensuremath{+2.21}}
\expandafter\gdef\csname R@v1.pub.mednextl5.acdc.d\endcsname{\ensuremath{+1.08}}
\expandafter\gdef\csname R@v1.pub.mednextl5.amos.d\endcsname{\ensuremath{+1.09}}
\expandafter\gdef\csname R@v1.pub.mednextl5.kits.d\endcsname{\ensuremath{+1.70}}
\expandafter\gdef\csname R@v1.pub.nnformer.acdc.d\endcsname{\ensuremath{+0.86}}
\expandafter\gdef\csname R@v1.pub.nnformer.amos.d\endcsname{\ensuremath{-7.09}}
\expandafter\gdef\csname R@v1.pub.nnformer.kits.d\endcsname{\ensuremath{-10.19}}
\expandafter\gdef\csname R@v1.pub.resencl.acdc.d\endcsname{\ensuremath{+0.15}}
\expandafter\gdef\csname R@v1.pub.resencl.amos.d\endcsname{\ensuremath{+0.77}}
\expandafter\gdef\csname R@v1.pub.resencl.kits.d\endcsname{\ensuremath{+2.13}}
\expandafter\gdef\csname R@v1.pub.resencm.acdc.d\endcsname{\ensuremath{+0.45}}
\expandafter\gdef\csname R@v1.pub.resencm.amos.d\endcsname{\ensuremath{+0.13}}
\expandafter\gdef\csname R@v1.pub.resencm.kits.d\endcsname{\ensuremath{+0.75}}
\expandafter\gdef\csname R@v1.pub.resencxl.acdc.d\endcsname{\ensuremath{-0.06}}
\expandafter\gdef\csname R@v1.pub.resencxl.amos.d\endcsname{\ensuremath{+1.04}}
\expandafter\gdef\csname R@v1.pub.resencxl.kits.d\endcsname{\ensuremath{+2.63}}
\expandafter\gdef\csname R@v1.pub.stunetl.acdc.d\endcsname{\ensuremath{-0.23}}
\expandafter\gdef\csname R@v1.pub.stunetl.amos.d\endcsname{\ensuremath{+0.70}}
\expandafter\gdef\csname R@v1.pub.stunetl.kits.d\endcsname{\ensuremath{-0.20}}
\expandafter\gdef\csname R@v1.pub.swinunetrv2.acdc.d\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@v1.pub.swinunetrv2.amos.d\endcsname{\ensuremath{-2.40}}
\expandafter\gdef\csname R@v1.pub.swinunetrv2.kits.d\endcsname{\ensuremath{-1.90}}
\expandafter\gdef\csname R@v1.pub.umambabot.acdc.d\endcsname{\ensuremath{+0.25}}
\expandafter\gdef\csname R@v1.pub.umambabot.amos.d\endcsname{\ensuremath{+0.49}}
\expandafter\gdef\csname R@v1.pub.umambabot.kits.d\endcsname{\ensuremath{+0.18}}
\expandafter\gdef\csname R@v1.ratio.kits.V7A1.L1\endcsname{76}
\expandafter\gdef\csname R@v1.ratio.mac.V7A1.L1\endcsname{52}
\expandafter\gdef\csname R@v1.rs.01.d\endcsname{\ensuremath{-0.44}}
\expandafter\gdef\csname R@v1.rs.02.d\endcsname{\ensuremath{+0.71}}
\expandafter\gdef\csname R@v1.rs.05.d\endcsname{\ensuremath{-5.55}}
\expandafter\gdef\csname R@v1.rs.07.amos.s0\endcsname{88.53}
\expandafter\gdef\csname R@v1.rs.07.d\endcsname{\ensuremath{+0.68}}
\expandafter\gdef\csname R@v1.rs.08.amos.s0\endcsname{87.92}
\expandafter\gdef\csname R@v1.rs.08.d\endcsname{\ensuremath{+0.27}}
\expandafter\gdef\csname R@v1.rs.09.d\endcsname{\ensuremath{-5.14}}
\expandafter\gdef\csname R@v1.rs.11.d\endcsname{\ensuremath{-5.22}}
\expandafter\gdef\csname R@v1.rs.12.d\endcsname{\ensuremath{-8.61}}
\expandafter\gdef\csname R@v1.rs.13.amos.s0\endcsname{86.74}
\expandafter\gdef\csname R@v1.rs.13.d\endcsname{\ensuremath{-6.05}}
\expandafter\gdef\csname R@v1.rs.15.amos.s0\endcsname{87.50}
\expandafter\gdef\csname R@v1.rs.15.d\endcsname{\ensuremath{+1.49}}
\expandafter\gdef\csname R@v1.rs.19.d\endcsname{\ensuremath{+2.18}}
\expandafter\gdef\csname R@v1.rs.20.d\endcsname{\ensuremath{-5.99}}
\expandafter\gdef\csname R@v1.rs.22.d\endcsname{\ensuremath{-4.79}}
\expandafter\gdef\csname R@v1.rs.23.amos.s0\endcsname{87.29}
\expandafter\gdef\csname R@v1.rs.23.d\endcsname{\ensuremath{-4.05}}
\expandafter\gdef\csname R@v1.rs.24.d\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@v1.rs.best\endcsname{\ensuremath{+2.18}}
\expandafter\gdef\csname R@v1.rs.complete\endcsname{1}
\expandafter\gdef\csname R@v1.rs.median\endcsname{\ensuremath{-4.05}}
\expandafter\gdef\csname R@v1.rs.n\endcsname{15}
\expandafter\gdef\csname R@v1.rs.nfast\endcsname{0}
\expandafter\gdef\csname R@v1.rs.nlarger\endcsname{14}
\expandafter\gdef\csname R@v1.rs.npos\endcsname{6}
\expandafter\gdef\csname R@v1.rs.nscreen\endcsname{4}
\expandafter\gdef\csname R@v1.rs.ntrained\endcsname{15}
\expandafter\gdef\csname R@v1.rs.step.max\endcsname{5.27}
\expandafter\gdef\csname R@v1.rs.step.min\endcsname{1.75}
\expandafter\gdef\csname R@v1.rssp.step.min\endcsname{1.69}
\expandafter\gdef\csname R@v1.sp.1.d\endcsname{\ensuremath{+2.38}}
\expandafter\gdef\csname R@v1.sp.1.par\endcsname{3.46}
\expandafter\gdef\csname R@v1.sp.2.d\endcsname{\ensuremath{+2.05}}
\expandafter\gdef\csname R@v1.sp.2.par\endcsname{3.46}
\expandafter\gdef\csname R@v1.steperr.w5\endcsname{12.6}
\expandafter\gdef\csname R@v1.steperr.w7\endcsname{2.0}
\expandafter\gdef\csname R@v1.steperr.w8\endcsname{2.8}
\expandafter\gdef\csname R@v1.tta.acdc.D2.d\endcsname{\ensuremath{-0.05}}
\expandafter\gdef\csname R@v1.tta.acdc.D2.mean\endcsname{91.33}
\expandafter\gdef\csname R@v1.tta.acdc.L1.d\endcsname{\ensuremath{+0.37}}
\expandafter\gdef\csname R@v1.tta.acdc.L1.mean\endcsname{91.75}
\expandafter\gdef\csname R@v1.tta.acdc.L1b.d\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@v1.tta.acdc.L1b.mean\endcsname{91.57}
\expandafter\gdef\csname R@v1.tta.acdc.L3.d\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@v1.tta.acdc.L3.mean\endcsname{91.71}
\expandafter\gdef\csname R@v1.tta.acdc.P3c.d\endcsname{\ensuremath{-0.08}}
\expandafter\gdef\csname R@v1.tta.acdc.P3c.mean\endcsname{91.30}
\expandafter\gdef\csname R@v1.tta.acdc.V5B1.d\endcsname{\ensuremath{-0.12}}
\expandafter\gdef\csname R@v1.tta.acdc.V5B1.mean\endcsname{91.26}
\expandafter\gdef\csname R@v1.tta.acdc.V5B2.d\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@v1.tta.acdc.V5B2.mean\endcsname{91.27}
\expandafter\gdef\csname R@v1.tta.acdc.V6A1r.d\endcsname{\ensuremath{+0.31}}
\expandafter\gdef\csname R@v1.tta.acdc.V6A1r.mean\endcsname{91.69}
\expandafter\gdef\csname R@v1.tta.acdc.V7A1.d\endcsname{\ensuremath{+0.08}}
\expandafter\gdef\csname R@v1.tta.acdc.V7A1.mean\endcsname{91.46}
\expandafter\gdef\csname R@v1.tta.acdc.V7A1cov.d\endcsname{\ensuremath{+0.10}}
\expandafter\gdef\csname R@v1.tta.acdc.V7A1cov.mean\endcsname{91.48}
\expandafter\gdef\csname R@v1.tta.acdc.V7C1.d\endcsname{\ensuremath{-0.19}}
\expandafter\gdef\csname R@v1.tta.acdc.V7C1.mean\endcsname{91.19}
\expandafter\gdef\csname R@v1.tta.acdc.V9R2.d\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@v1.tta.acdc.V9R2.mean\endcsname{91.50}
\expandafter\gdef\csname R@v1.tta.acdc.base.mean\endcsname{91.38}
\expandafter\gdef\csname R@v1.tta.amos.L1.d\endcsname{\ensuremath{+0.41}}
\expandafter\gdef\csname R@v1.tta.amos.L1.mean\endcsname{89.24}
\expandafter\gdef\csname R@v1.tta.amos.L3.d\endcsname{\ensuremath{+0.19}}
\expandafter\gdef\csname R@v1.tta.amos.L3.mean\endcsname{89.02}
\expandafter\gdef\csname R@v1.tta.amos.V7A1.d\endcsname{\ensuremath{+0.12}}
\expandafter\gdef\csname R@v1.tta.amos.V7A1.mean\endcsname{88.95}
\expandafter\gdef\csname R@v1.tta.amos.V7C1.d\endcsname{\ensuremath{-0.39}}
\expandafter\gdef\csname R@v1.tta.amos.V7C1.mean\endcsname{88.44}
\expandafter\gdef\csname R@v1.tta.amos.base.mean\endcsname{88.83}
\expandafter\gdef\csname R@v1.tta.kits.L1.d\endcsname{\ensuremath{+1.49}}
\expandafter\gdef\csname R@v1.tta.kits.L1.mean\endcsname{87.01}
\expandafter\gdef\csname R@v1.tta.kits.L3.d\endcsname{\ensuremath{+0.57}}
\expandafter\gdef\csname R@v1.tta.kits.L3.mean\endcsname{86.09}
\expandafter\gdef\csname R@v1.tta.kits.V7A1.d\endcsname{\ensuremath{+1.06}}
\expandafter\gdef\csname R@v1.tta.kits.V7A1.mean\endcsname{86.58}
\expandafter\gdef\csname R@v1.tta.kits.V7C1.d\endcsname{\ensuremath{+0.47}}
\expandafter\gdef\csname R@v1.tta.kits.V7C1.mean\endcsname{85.99}
\expandafter\gdef\csname R@v1.tta.kits.base.mean\endcsname{85.51}
\expandafter\gdef\csname R@v1.ttaoff.acdc.L1.d\endcsname{\ensuremath{+0.44}}
\expandafter\gdef\csname R@v1.ttaoff.acdc.L1.mean\endcsname{91.38}
\expandafter\gdef\csname R@v1.ttaoff.acdc.L3.d\endcsname{\ensuremath{+0.33}}
\expandafter\gdef\csname R@v1.ttaoff.acdc.L3.mean\endcsname{91.28}
\expandafter\gdef\csname R@v1.ttaoff.acdc.V7A1.d\endcsname{\ensuremath{+0.17}}
\expandafter\gdef\csname R@v1.ttaoff.acdc.V7A1.mean\endcsname{91.11}
\expandafter\gdef\csname R@v1.ttaoff.acdc.V7C1.d\endcsname{\ensuremath{-0.11}}
\expandafter\gdef\csname R@v1.ttaoff.acdc.V7C1.mean\endcsname{90.83}
\expandafter\gdef\csname R@v1.ttaoff.acdc.base.mean\endcsname{90.94}
\expandafter\gdef\csname R@v1.xl.kits.s0\endcsname{86.09}
\makeatother

